Transient temperature calculation method for complex fluid-solid heat transfer problems with scattering boundary conditions

A calculation method for engine temperatures is presented. Special focus is placed on the transient and scattering boundary conditions within the combustion chamber, including fired and coasting conditions, as well as the dynamic heat transfer of the water jacket. Model reduction is achieved with dimensional analysis and the application of probability density functions, which allows for a timescale separation. Stationary in-cylinder pressure measurements are used as input values and, according to the transient behavior, modified with an own part-load model. A turbocharged SI race engine is equipped with 70 thermocouples at various positions in proximity to the combustion chamber. Differentiating from already published works, the method deals with the transient engine behavior during a race lap, which undergoes a frequency range of 0.1-1 Hz. This includes engine speed build-ups under gear changes, torque variations, or the transition from fired to coasting conditions. Different thermal behaviors of various measuring positions can be simulated successfully. Additionally, cylinder individual temperature effects resulting from an unsymmetrical ignition sequence and different volumetric efficiencies with unequal residual gas can be predicted. Up to a few percent, the energy balance of the water jacket is fulfilled and variations of water inlet temperatures can be simulated accurately enough.

==> library_app <==
Automatically generated by Mendeley Desktop 1.17.10
Any changes to this file will be lost if it is regenerated by Mendeley.

BibTeX export options can be customized via Options -> BibTeX in Mendeley Desktop

@article{PeterReduction2017,
author = {H{\"{o}}lz, Peter and B{\"{o}}hlke, Thomas and Kr{\"{a}}mer, Thomas},
doi = {https://doi.org/10.1016/j.applthermaleng.2018.05.099},
journal = {Appl. Therm. Eng.},
pages = {101--113},
title = {{Fast algorithms for generating thermal boundary conditions in combustion chambers}},
volume = {141},
year = {2018}
}
@article{Zienkiewiczb,
author = {Zienkiewicz, O C and Taylor, R L},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Zienkiewicz FEM - Vol 2 Solid Structural Mechanics/63212{\_}fm.pdf:pdf},
title = {{Method for Solid and Structural Mechanics UNESCO Professor of Numerical Methods in Engineering}}
}

@article{Energiewandlung,
author = {Energiewandlung, Einzelprozesse},
title = {{2 Energieumsetzung im Verbrennungsmotor}}
}
@article{Mughrabi2009,
abstract = {In this article, the physical origin of fatigue crack initiation in ductile metals is discussed from a historical perspective. The main focus is to assess those cyclic slip irreversibilities in a microstructural sense that occur not only at the surface but also in the bulk at the dislocation scale and to show how they contribute to surface fatigue damage. The evolution of early fatigue damage, as evidenced experimentally in the last decades, is reviewed. The phenomenon of cyclic strain localization in persistent slip bands (PSBs) and models of the formation of extrusions, intrusions, and microcracks are discussed in detail. The predictions of these models are compared with experimental evidence obtained on mono- and polycrystalline face-centered-cubic (fcc) metals. In addition, examples of the evolution of fatigue damage in selected fcc solid solution alloys and precipitation-hardened alloys and in body-centered-cubic (bcc) metals are analyzed. Where possible, the cyclic slip irreversibilities p, defined as the fraction of plastic shear strain that is microstructurally irreversible, have been estimated quantitatively. Broadly speaking, p has been found to vary over orders of magnitude (0 p 1), being almost negligible at low loading amplitudes (high fatigue lives) and substantial at larger loading amplitudes (low fatigue lives). 2009 The Minerals, Metals Materials Society and ASM International.},
author = {Mughrabi, Hael},
doi = {10.1007/s11663-009-9240-4},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/2008{\_}Mughrabi{\_}Cyclic Slip Irreversibilities and the Evolution of Fatigue Damage.pdf:pdf},
isbn = {10735615},
issn = {10735615},
journal = {Met. Mater. Trans. B Process Met. Mater. Process. Sci.},
number = {4},
pages = {431--453},
title = {{Cyclic slip irreversibilities and the evolution of fatigue damage}},
volume = {40},
year = {2009}
}
@article{Poll,
author = {Poll, Gerhard and Deters, Ludger and Gleitlager, Fettgeschmierte and Radialgleitlager, Hydrostatische and Axialgleitlager, Hydrostatische and Anfahrhilfe, Hydrostatische},
title = {{Kapitel 11 Lagerungen, Gleitlager, W{\"{a}}lzlager}}
}
@article{Adair1972c,
abstract = {This study first reviews, discusses, and compares existing correlations$\backslash$nfor heat transfer in reciprocating compressors and engines. Then$\backslash$nafter a discussion of the significance of obtaining accurate instantaneous$\backslash$nheat transfer data, the authors describe an experimental investigation$\backslash$nof the instantaneous heat transfer rates to the cylinder wall of$\backslash$na reciprocating refrigerating compressor. Finally, this report presents$\backslash$nan expression which correlates the time averaged data within 20{\%}.},
author = {Adair, R P and Qvale, E B and Pearson, J T},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Heat Transfer Combustion Chamber/1972{\_}Adair{\_}Instantaneous Heat Transfer to the Cylinder Wall in Reciprocating compressors and engines.pdf:pdf},
journal = {Purdue Compress. Technol. Conf.},
pages = {521--526},
title = {{Instantaneous heat transfer to cylinder wall in reciprocating compressors}},
year = {1972}
}
@article{Akustik1989,
author = {Akustik, Technischen},
pages = {401--432},
title = {{6 Motorger{\"{a}}usch}},
year = {1989}
}
@book{VDI-Warmeatlas2013,
abstract = {Der VDI-W{\"{a}}rmeatlas blickt im Jahr 2013, dem Erscheinungsjahr dieser 11. deutschen Auflage, auf eine 50-j{\"{a}}hrige Historie zur{\"{u}}ck. Im Jahre 1963 erschien die erste Auflage. Ziel war und ist es, Ingenieuren in einem {\"{u}}bersichtlichen und umfassenden Werk verl{\"{a}}ssliche Methoden zur Berechnung von W{\"{a}}rme{\"{u}}bertragern und w{\"{a}}rmetechnischen Apparaten an die Hand zu geben. Hierzu z{\"{a}}hlte und z{\"{a}}hlt auch die Bereitstellung von Stoffdaten. In diesen 50 Jahren ist der VDI-W{\"{a}}rmeatlas zu einem Standardwerk geworden. Nach der 10. deutschen Auflage, die im Jahr 2006 erschien, folgte 2010 die 2. englische Auflage. Der Redaktionsausschuss hatte bei diesem {\"{U}}bergang nicht nur alle Berechnungsverfahren und Stoffdaten aktualisiert, sondern auch die urspr{\"{u}}ngliche, {\"{u}}ber die Jahre gewachsene Gliederung {\"{u}}berarbeitet, um einige Themen neu ordnen und neue Themen aufnehmen zu k{\"{o}}nnen. Diese {\"{u}}berarbeitete Gliederung ist nun auch in der 11. deutschen Auflage zu finden. Zudem wurden zahlreiche Abschnitte wieder aktualisiert, so dass der VDI-W{\"{a}}rmeatlas auch weiterhin als aktuelles Standardwerk zur Auslegung von W{\"{a}}rme{\"{u}}bertragern und w{\"{a}}rmetechnischen Apparaten dienen kann. Im Namen der Mitglieder des Redaktionsausschusses danke ich allen Autoren der einzelnen Kapitel f{\"{u}}r ihr gro{\ss}es Engagement. Dem Springer-Verlag danke ich f{\"{u}}r die stets sehr gute Zusammenarbeit und die gelungene Umsetzung, insbesondere den Lekto- rinnen Frau Sigrid Cuneus und Frau Dr. Sylvia Blago.},
author = {VDI-W{\"{a}}rmeatlas},
doi = {10.1007/978-3-642-19981-3},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/2013{\_}VDI{\_}Waermeatlas.pdf:pdf},
isbn = {978-3-642-19980-6},
pages = {1784},
title = {{VDI-W{\"{a}}rmeatlas}},
url = {http://link.springer.com/10.1007/978-3-642-19981-3},
year = {2013}
}
@article{Agarwal2006b,
abstract = {Thermal loading of diesel engine pistons has increased dramatically in recent years owing to applications of various technologies to meet low emission and high power density requirements. Control of piston temperatures by cooling of these pistons has become one of the determining factors in a successful engine design. The pistons are cooled by oil jets fired at the underside from the crankcase. Any excessive piston temperature rise may lead to engine seizure because of piston warping. However, if the temperature at the underside of the piston, where the oil jet strikes the piston, is above the boiling range of the oil being used, it may contribute to the generation of mist. This mist significantly contributes to the non-tailpipe emissions in the form of unburnt hydrocarbons (UBHCs). The problem of non-tailpipe emissions has unfortunately not been looked into so seriously, as the current stress of all automobile manufacturers is to meet the tailpipe emission legislative limits.A numerical model has been developed using finite element methods for studying the oil jet cooling of pistons and has been validated experimentally on a flat plate cooled by oil jet. Using numerical modelling, the heat transfer coefficient (h) at the underside of the piston is predicted. This predicted value of heat transfer coefficient significantly helps in selecting the correct oil type, oil jet velocity, oil jet diameter, and distance of oil nozzle from the underside of the piston. It also helps to predict whether the selected grade of oil will contribute to mist generation. Isotherms of the predicted temperature profiles in a production grade piston have been plotted.},
author = {Agarwal, A K and Varghese, M B},
doi = {10.1243/14680874JER01804},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/W{\"{a}}rme-RBen Kolben/2004{\_}Varghese{\_}Numerical investigation of piston cooling using oil jet.pdf:pdf},
issn = {1468-0874},
journal = {Int. J. Engine Res.},
number = {5},
pages = {411--421},
title = {{Numerical investigations of piston cooling using oil jet in heavy duty diesel engines}},
url = {http://journals.sagepub.com/doi/10.1243/14680874JER01804},
volume = {7},
year = {2006}
}
@article{Gross2011b,
author = {Gross, Dietmar and Seelig, Thomas},
doi = {10.1007/978-3-642-10196-0},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Gross, Selig 2011 - Bruchmechanik/Gross, Seelig - 2011 - BruchmechanikSV.pdf:pdf},
isbn = {978-3-642-10195-3},
title = {{Bruchmechanik}},
url = {http://link.springer.com/10.1007/978-3-642-10196-0},
year = {2011}
}
@article{Hill1966,
abstract = {A general, type of cross-coupling between glide and hardening on different slip-systems is proposed. Its implications in regard to the character of the connexion between the overall stress-rate and strain-rate in multislip are investigated. Uniqueness theorems and extremal properties are established in respect both of the overall constitutive law itself and any boundary-value problem for non-uniform deformation of a single crystal or aggregate.},
author = {Hill, R.},
doi = {10.1016/0022-5096(66)90040-8},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/1966{\_}Hill{\_}Generalized consititutive relations for incremental defo of metal crystals by multislip.pdf:pdf},
isbn = {0022-5096},
issn = {00225096},
journal = {J. Mech. Phys. Solids},
number = {2},
pages = {95--102},
title = {{Generalized constitutive relations for incremental deformation of metal crystals by multislip}},
volume = {14},
year = {1966}
}

@article{Chang2004a,
abstract = {An experimental study has been carried out to provide qualitative and quantitative insight into gas to wall heat transfer in a gasoline fueled Homogeneous Charge Compression Ignition (HCCI) engine. Fast response thermocouples are embedded in the piston top and cylinder head surface to measure instantaneous wall temperature and heat flux. Heat flux measurements obtained at multiple locations show small spatial variations, thus confirming relative uniformity of incylinder conditions in a HCCI engine operating with premixed charge. Consequently, the spatially-averaged heat flux represents well the global heat transfer from the gas to the combustion chamber walls in the premixed HCCI engine, as confirmed through the gross heat release analysis. Heat flux measurements were used for assessing several existing heat transfer correlations. One of the most popular models, the Woschni expression, was shown to be inadequate for the HCCI engine. The problem is traced back to the flame propagation term which is not appropriate for the HCCI combustion. Subsequently, a modified model is proposed which significantly improves the prediction of heat transfer in a gasoline HCCI engine and shows very good agreement over a range of conditions},
author = {Chang, Junseok and G{\"{u}}ralp, Orgun and Filipi, Zoran and Assanis, Dennis N and Kuo, Tang-Wei and Najt, Paul and Rask, Rod},
doi = {10.4271/2004-01-2996},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2004{\_}Chang{\_}New Heat Transfer Correlation for an HCCI Engine Derived from Measurements of Instantaneous Surface Heat Flux.pdf:pdf},
isbn = {0148-7191},
issn = {0148-7191},
number = {724},
title = {{New Heat Transfer Correlation for an HCCI Engine Derived from Measurements of Instantaneous Surface Heat Flux}},
url = {http://papers.sae.org/2004-01-2996/},
year = {2004}
}
@book{HorstCzickosTechnischeFachhochschuleBerlin2008,
author = {{Horst Czickos (Technische Fachhochschule Berlin)}, Manfred Hennecke (BAM)},
isbn = {9783540718512},
title = {{H{\"{u}}tte Das Ingenieurwissen}},
year = {2008}
}
@book{Streicher-abel,
author = {Streicher-abel, Christian Demant Bernd},
booktitle = {Media},
doi = {10.1007/s10531-008-9469-2},
isbn = {9783642130960},
title = {{1 C}}
}
@article{Feldhusen,
author = {Feldhusen, J{\"{o}}rg},
pages = {2--11},
title = {{1 Einleitung}}
}
@article{Kocks2003a,
author = {Kocks, U.F and {H. Mecking}},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/Hardening Recovery Creep/2002{\_}Kocks+Mecking{\_}Physics and phenomenology of strain hardening{\_}fcc case.pdf:pdf},
isbn = {4042878407},
journal = {Prog. Mater. Sci.},
pages = {171--273},
title = {{Physics and phenomenology of strainhardening: the FCC case}},
url = {https://www.academia.edu/8128075/Physics{\_}and{\_}phenomenology{\_}of{\_}strain{\_}hardening{\_}the{\_}FCC{\_}case},
volume = {48},
year = {2003}
}
@article{Notation,
author = {Notation, Matrix},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Stupkievicz 2007 - Micromechanics of Contact and Interphase Layers/97165{\_}apdx01.pdf:pdf},
title = {{Micro-Macro Transit ion Relations for Simple}}
}
@article{Polak2014,
abstract = {Experimental data on the formation of persistent slip markings (PSMs) at the egressing persistent slip bands (PSBs) and physically based models of surface relief formation and fatigue crack initiation are surveyed. The original Pol{\'{a}}k's model of fatigue crack initiation based on the formation, migration and annihilation of vacancy-type defects in PSBs is further refined and extended by taking into consideration the annihilation of vacancies in the matrix and the formation of internal stresses. The proposed mechanisms of surface relief formation are based on the plastic relaxation of internal compression stresses in PSBs and internal tensile stresses in the matrix. By solving the migration of vacancies from the PSB and their annihilation in the matrix, the shapes of extrusion and parallel intrusions are derived analytically under some simplifying assumptions. {\textcopyright} 2013 Elsevier B.V.},
author = {Pol{\'{a}}k, J. and Man, J.},
doi = {10.1016/j.msea.2013.12.005},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/2014{\_}Polak+Man{\_}Mechanisms of extrusion and intrusion formation in fatigued crystalline materials.htm.pdf:pdf},
issn = {09215093},
journal = {Mater. Sci. Eng. A},
keywords = {Crack initiation,Extrusion,Fatigue,Intrusion,Persistent slip band (PSB)},
pages = {15--24},
publisher = {Elsevier},
title = {{Mechanisms of extrusion and intrusion formation in fatigued crystalline materials}},
url = {http://dx.doi.org/10.1016/j.msea.2013.12.005},
volume = {596},
year = {2014}
}
@article{Finol2006,
abstract = {Over the last 40 years, several empirical correlations have been developed to estimate heat fluxes from the combustion chambers of internal combustion engines. Some of these expressions are based on correlations to compute the Nusselt number for forced convection in turbulent flow inside circular tubes. The fundamental suitability of this kind of empirical model in representing the highly complex processes of in-cylinder heat transfer is questionable, but in practice the models have steadily improved owing to contributions from numerous investigators. Other correlations have a less theoretical basis than those of the Nusselt number form. Formulae of this type have been obtained from the application of simple statistical techniques to large datasets, taking into account several engine operational parameters and engine types. The resulting correlations provide reasonable estimates but perform poorly when extrapolated or applied to novel concepts. In this paper, the most important correlations are reviewed against the features of a modern diesel engine, and research requirements for future modelling developments are identified and discussed. {\{}{\textcopyright}{\}} IMechE 2006.},
author = {Finol, C A and Robinson, K},
doi = {https://doi.org/10.1243/09544070JAUTO202},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2006{\_}Finol{\_}Thermal modelling of modern engines - A review of empirical correlations to estimate the in-cylinder heat transfer coefficient .pdf:pdf},
journal = {Proc. Inst. Mech. Eng. Part D J. Automob. Eng.},
keywords = {cient,heat flux,heat transfer coe ffi,in-cylinder heat transfer models},
number = {12},
pages = {1765--1781},
title = {{Thermal modelling of modern engines: a review of empirical correlations to estimate the in-cylinder heat transfer coefficient}},
volume = {220},
year = {2006}
}
@article{Reichardt1951,
author = {Reichardt, H.},
doi = {10.1002/zamm.19510310704},
journal = {Z. Angew. Math. Mech},
number = {7},
pages = {208--219},
title = {{Vollst{\"{a}}ndige Darstellung der turbulenten Geschwindigkeitsverteilung in glatten Leitungen}},
volume = {31},
year = {1951}
}
@article{Verwendung,
author = {Verwendung, Funktion},
doi = {10.1007/978-3-8348-8279-0},
isbn = {9783834882790},
pages = {744--764},
title = {{¨ der und Kegelradgetriebe}}
}

@article{Hbs,
author = {Hbs, Bezeichnung},
pages = {93--113},
title = {( 0 , 204}
}
@article{Sanli2009c,
author = {Sanli, A. and Sayin, C. and Gumus, M. and Kilicaslan, I. and Canakci, M.},
file = {:C$\backslash$:/Users/p327208/Desktop/Promotion/Literature/Motorspezifisch/Heat Transfer Combustion Chamber/2009{\_}Sanli{\_}Numerical evaluation by models of load and spark timing effects on the in-cylinder heat transfer of a si engine.pdf:pdf},
journal = {Numer. Heat Transf. Part A Appl.},
number = {5},
pages = {444--458},
title = {{Numerical Evaluation by Models of Load and Spark Timing Effects on the In-Cylinder Heat Transfer of a SI Engine}},
volume = {56},
year = {2009}
}
@article{Zahoransky2013e,
author = {Zahoransky, Richard A. and Allelein, Hans-Josef and Schelling, Udo and Schwarz, Harald and Bollin, Elmar and Oehler, Helmut},
doi = {10.1007/978-3-8348-2279-6},
isbn = {978-3-8348-1869-0},
journal = {Energietechnik - Syst. zur Energieumwandlung},
pages = {30},
title = {{9 Brennstoffzellen}},
url = {http://www.springerlink.com/index/10.1007/978-3-8348-2279-6},
year = {2013}
}
@article{Maere2012,
author = {Maere, Steven and Biology, Course Computational},
doi = {10.1002/wsbm.033},
number = {December},
title = {{Multiscale modelling}},
year = {2012}
}
@article{Muhs2007,
author = {Muhs, Dieter and Wittel, Herbert and Jannasch, Dieter and Vo{\ss}iek, Joachim},
doi = {10.1007/978-3-8348-9406-9},
isbn = {978-3-8348-0262-0},
journal = {Roloff / Matek Maschinenelemente},
pages = {21--36},
title = {{Toleranzen, Passungen, Oberfl{\{}{\"{a}}{\}}chenbeschaffenheit}},
url = {http://www.springerlink.com/index/10.1007/978-3-8348-9406-9},
year = {2007}
}
@article{Huang2004a,
abstract = {For a fine grained pure copper (grain size, 3.8 ??m) with a weak initial texture, the flow stress and the microstructure have been examined. The stress-strain curve has been compared with that of a coarse grained copper with a weak texture and a similar curve shape has been found, indicating no change in the strain hardening behavior as the grain size is decreased. The validity of the Hall-Petch relationship has been demonstrated down to a grain size of 3.8 ??m. Careful microstructural characterization of deformed specimens has shown that the microstructural evolution in the fine grained copper follows the same pattern previously established for larger grain sizes, which is characterized by the formation of three types of microstructures depending on the grain orientation. This observation suggests that the slip patterns in the fine grained and coarse grained copper are comparable, which underpin the observation of a comparable stress-strain behavior. ?? 2004 Elsevier B.V. All rights reserved.},
author = {Huang, Xiaoxu and Hansen, N},
doi = {10.1016/j.msea.2004.02.081},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2005{\_}Huang{\_}Hansen Flow stress and microstructures of fine grained copper.pdf:pdf},
isbn = {0921-5093},
issn = {09215093},
journal = {Mater. Sci. Eng. A},
keywords = {Copper,Deformation microstructure,Flow stress,Grain orientation,Hall-Petch relationship,Slip pattern},
number = {1-2 SPEC. ISS.},
pages = {186--190},
title = {{Flow stress and microstructures of fine grained copper}},
volume = {387-389},
year = {2004}
}
@article{Arnold1998,
author = {Arnold, J{\"{o}}rg and Verkehrsunf{\"{a}}llen, Bei},
pages = {781--786},
title = {{C4 C4 Schutzhelme Erste Untersuchungen am Helm C4 Besch{\"{a}}digungen am Helm}},
year = {1998}
}
@article{Elastizit,
author = {Elastizit, Grundlagen Der},
doi = {10.1007/978-3-642-16828-4},
isbn = {9783642168284},
title = {{Grundlagen der Elastizit¨ atstheorie 2}}
}
@article{Materials2003,
author = {Materials, Thermoinelastic},
pages = {243--256},
title = {{Inelastic and Thermoinelastic Materials 19.1}},
volume = {22},
year = {2003}
}
@article{Ritchie1985,
abstract = {Relationships between crack initiation and crack growth toughness are reviewed by examining the crack tip fields and microscopic (local) and macroscopic (continuum) fracture criteria for the onset and continued quasi-static extension of cracks in ductile materials. By comparison of the micromechanisms of crack initiation via transgranular cleavage and crack initiation and subsequent growth via microvoid coalescence, expressions are shown for the fracture toughness of materials in terms of microstructural parameters. Utilizing the exact asymptotic crack tip deformation fields for the nonstationary plane strain Mode I crack and evoking various microscopic failure criteria for such stable crack growth, a relationship between the tearing modulus TR and the nondimensionalized crack initiation fracture toughness Jlc is described and shown to yield a good fit to experimental toughness data for a wide range of steels},
author = {Ritchie, R O and Thompson, A W},
doi = {10.1007/BF02815305},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/1985{\_}RichtieAndThompson{\_}On Macroscopic and Microscopic Analyses for Crack Initiation and Crack Groth Toughness in Ductile Alloys.pdf:pdf},
isbn = {0360-2133},
issn = {03602133},
journal = {Met. Trans. A},
number = {1},
pages = {233--248},
title = {{On macroscopic and microscopic analyses for crack initiation and crack growth toughness in ductile alloys}},
volume = {16},
year = {1985}
}
@article{Lcmaitrca,
author = {Lcmaitrc, Cordchois},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Plasticity models/On Energy based coupled elastoplastic damage theories{\_}Ju1988.pdf:pdf},
title = {{1989-Ju{\_} On energy-based coupled elastoplastic damage theories{\_}constitutive modeling and computational aspects.pdf}}
}
@article{Sauzay2002,
author = {Sauzay, M and Gilormini, P},
doi = {10.1016/S0167-8442(02)00080-0},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/2002{\_}Sauzay + Gilmormini{\_}Influence of surface effects on fatigue of microcracks nucleation.pdf:pdf},
issn = {01678442},
journal = {Evaluation},
keywords = {crack nucleation,cyclic plasticity,fatigue,persistent slip band,surface},
pages = {53--62},
title = {{Influence of surface effects on fatigue of microcracks nucleation}},
volume = {38},
year = {2002}
}
@article{Stra,
author = {Str, Die and Str, Die and Ei-, Diese and Ei-, Diese and Gegensatz, Im and Gegensatz, Im and Veranschaulichung, Zur and Veranschaulichung, Zur and Festk, Hookesche and Festk, Hookesche and Zusammenhang, Der and Zusammenhang, Der},
number = {$\gamma$ 1},
pages = {1--36},
title = {{1 Kontinuumsbegri und Kinematik 1.1}}
}
@article{Castillo2009b,
author = {Castillo, E},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Probabilistic Aspects/A Unified Statistical Methodology for Modeling Fatigue Damage{\_}Castillo/Kap3{\_}Length Effect.pdf:pdf},
journal = {Media},
pages = {91--109},
title = {{Length Effect}},
year = {2009}
}
@misc{Banabic2000,
abstract = {After a brief introduction into crystal plasticity, the fun- damentals of crystallographic textures and plastic anisotro- py, a main topic of this book, are outlined. A large chapter is devoted to formability testing both for bulk metal and sheet metal forming. For the first time testing methods for plastic anisotropy of round bars and tubes are included. A profound survey is given of literature about yield criteria for anisotropic materials up to most recent developments and the calculation of forming limits of anisotropic sheet me- tal. Other chapters are concerned with properties of workpieces after metal forming as well as the fundamentals of the theory of plasticity and finite element simulation of metal forming processes. The book is completed by a collection of tables of international standards for formability testing and of flow curves of metals which are most commonly used in metal forming. It is addressed both to university and industrial readers.},
author = {Banabic, Dorel},
doi = {\url{10.1007/978-3-662-04013-3}},
isbn = {3540679065},
title = {{Formability of metallic materials: plastic anisotropy, formability testing, forming limits}},
year = {2000}
}
@article{Hill1952,
abstract = {The connection between the elastic behaviour of an aggregate and a single crystal is considered, with special reference to the theories of Voigt, Reuss, and Huber and Schmid. The elastic limit under various stress systems is also considered, in particular, it is shown that the tensile elastic limit of a face-centred aggregate cannot exceed two-thirds of the stress at which pronounced plastic distortion occurs.},
author = {Hill, R},
doi = {10.1088/0370-1298/65/5/307},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/Strukturmechanik MMS/Literatur/Hill 1952.pdf:pdf},
isbn = {0370-1298},
issn = {0370-1298},
journal = {Proc. Phys. Soc. Sect. A},
number = {5},
pages = {349--354},
title = {{The Elastic Behaviour of a Crystalline Aggregate}},
url = {http://stacks.iop.org/0370-1298/65/i=5/a=307?key=crossref.630b67f122246b4defcc5fda55c7bf20},
volume = {65},
year = {1952}
}
@article{Wolfstein1969,
author = {Wolfstein, M},
doi = {https://doi.org/10.1016/0017-9310(69)90012-X},
journal = {Int. J. Heat Mass Transf.},
pages = {301--318},
title = {{The velocity and temperature distribution in one-dimensional flow with turbulence augmentation and pressure gradient}},
volume = {12},
year = {1969}
}
@article{Pahl2007b,
author = {Pahl, Gerhard and Beitz, Wolfgang and Feldhusen, J{\"{o}}rg and Grote, Karl-Heinrich},
journal = {Konstr. Grundlagen erfolgreicher Produktentwicklung, Methoden und Anwendung},
pages = {39--92},
title = {{Grundlagen}},
year = {2007}
}
@article{M1959,
author = {M, M Grundlagen Der Elektrotechnik},
doi = {10.1002/prop.19590071309},
journal = {Fortschritte der Phys.},
number = {S1},
pages = {162--167},
title = {{Literaturverzeichnis}},
volume = {7},
year = {1959}
}
@article{Wang1985c,
abstract = {A heat transfer model has been developed that uses quasi-steady heat flux relations to calculate the heat transfer from combustion gases through the cylinder wall to the coolant in an internal combustion engine. The treatment of convective heat transfer accounts for the physical problems of rotating and impinging axial flow inside the engine cylinder. The radiative heat transfer includes gas radiation (CO 2 , H 2 0, and CO) and soot-particle radiation. Cylinder wall temperatures can be accurately predicted from this model for both the gas and the coolant sides. The present model's heat transfer results for the motoring case are in good agreement with results from empirical correlations based on instantaneous heat flux data. The calculated radiative heat flux and gas emissivity show reasonable agreement with data in the literature. NOMENCLATURE A area, m 2 a parameter defined in Eq. 19 Cp heat capacity, J • kg -1 • K -1 D diameter, m Gr Grashof number H heat transfer coefficient, W • m -2 . • K -1 I Planck function, W • m -1 k thermal conductivity, W • m -1 • K -1 , or refractive index K absorption coefficient, m -1 L distance between cylinder head and piston top, m M mass flow rate, kg • s -1 n refractive index Pr Prandl number q heat transfer rate, W • m -2 Q total heat loss per cycle, W • m -2 R radius, m Re Reynolds number T Temperature, K U overall heat transfer coefficient, W • m -2 • K -1},
author = {Wang, C S and Berry, G F},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Heat Transfer Combustion Chamber/1985{\_}Wang{\_}Heat Transfer in Internal Combustion Engines.pdf:pdf},
journal = {Asme},
number = {Ic},
pages = {1--7},
title = {{Heat Transfer in Internal Combustion Engines}},
year = {1985}
}
@article{Sources1995,
author = {Sources, A Neutron},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/Advanced Materials and Structures for Extreme Operating Conditions - Skrzypek/Backmatter.pdf:pdf},
title = {{Appendix : European Sources of Neutrons and X-ray Synchrotron Radiation and their Main}},
year = {1995}
}
@article{Wirkung,
author = {Wirkung, Funktion},
number = {Lagerschale 2},
pages = {522--576},
title = {15 15.1.2},
volume = {0}
}
@article{Zahoransky2013a,
author = {Zahoransky, Richard a. and Allelein, Hans-Josef and Schelling, Udo and Schwarz, Harald and Bollin, Elmar and Oehler, Helmut},
doi = {10.1007/978-3-8348-2279-6},
isbn = {978-3-8348-1869-0},
journal = {Energietechnik - Syst. zur Energieumwandlung},
pages = {286--326},
title = {{12 Solartechnik}},
url = {http://www.springerlink.com/index/10.1007/978-3-8348-2279-6},
year = {2013}
}
@article{Manonukul2004a,
abstract = {A polycrystal plasticity finite–element model has been developed for nickel–base alloy C263. That is, a representative region of the material, containing about 60 grains, has been modelled using crystal plasticity, taking account of grain morphology and crystallographic orientation. With just a single material property (in addition to standard elastic properties), namely, the critical resolved shear stress, the model is shown to be capable of predicting correctly a wide range of cyclic plasticity behaviour in face–centred cubic nickel alloy C263. A fatigue crack initiation criterion is proposed, based simply on a critical accumulated slip. When this critical slip is achieved within the microstructure, crack initiation is taken to have occurred. The model predicts the development of persistent slip bands within individual grains with a width of ca. 10 {\$}\mu{\$}m. The model also predicts that crack initiation can occur preferentially at grain triple points under both low– (LCF) and high–cycle fatigue (HCF). For the case of HCF, this also corresponds to a free surface. The polycrystal plasticity model combined with the fatigue crack initiation criterion are shown to predict correctly the standard Basquin and Goodman correlations in HCF, and the Coffin–Manson correlation in LCF. The model predictions are based on just two material properties: the critical resolved shear stress and the critical accumulated slip. Just one experimental test is required to determine these properties, for a given temperature, which have been obtained for nickel alloy C263. Predictions of life for nickel alloy C263 are then made over a broad range of loading conditions covering both LCF and HCF. Good agreement with experiments is achieved, despite the simplicity of the proposed ‘two–parameter' model. A simple three–dimensional form of the model has provided an estimate of the fatigue limit for HCF crack initiation in C263.},
author = {Manonukul, A and Dunne, F P E},
doi = {10.1098/rspa.2003.1258},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2003{\_}Manonukul+Dunne{\_}High- and low-cycle fatigue crack initiation using polcrystal plasticity.pdf:pdf},
isbn = {1364-5021},
issn = {1364-5021},
journal = {Proc. R. Soc. A Math. Phys. Eng. Sci.},
keywords = {crack initiation,hcf,high-cycle fatigue,lcf,low-cycle fatigue,polycrystal plasticity},
number = {2047},
pages = {1881--1903},
title = {{High- and low-cycle fatigue crack initiation using polycrystal plasticity}},
url = {http://rspa.royalsocietypublishing.org/cgi/doi/10.1098/rspa.2003.1258},
volume = {460},
year = {2004}
}
@article{Broekaert2016II,
author = {Cuyper, Thomas De and Demuynck, Joachim and Broekaert, Stijn and Paepe, Michel De and Verhelst, Sebastian},
doi = {http://dx.doi.org/10.1016/j.energy.2016.10.032},
file = {:C$\backslash$:/Users/p327208/Desktop/Promotion/Literature/Motorspezifisch/Heat Transfer Combustion Chamber/2016{\_}Broekaert{\_}Heat transfer in premixed spark ignition engines part II - Systematicanalysis of the heat transfer phenomena.pdf:pdf},
journal = {Energy},
pages = {851--860},
publisher = {Elsevier Ltd},
title = {{Heat transfer in premixed spark ignition engines part II : Systematic analysis of the heat transfer phenomena}},
volume = {116},
year = {2016}
}
@article{Vick,
author = {Vick, Prof Ralf},
title = {{11 Modellierung und Bewertung von St{\"{o}}rfestigkeitsnachweisen}}
}
@book{Murakami2012b,
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Murakami, Sumio},
doi = {10.1007/978-94-007-2666-6},
eprint = {arXiv:1011.1669v3},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/Continuum Damage Mechanics - SumioMurakami/Kap8{\_}Creep Damage and Creep-Fatigue Damage.pdf:pdf},
isbn = {978-94-007-2665-9},
issn = {09250042},
pages = {217--251},
pmid = {25246403},
title = {{Continuum Damage Mechanics}},
url = {http://link.springer.com/10.1007/978-94-007-2666-6},
volume = {185},
year = {2012}
}
@article{Aslan2010,
author = {Aslan, Ozgur},
title = {{Numerical modeling of fatigue crack growth in single crystal nickel based superalloys Ozgur Aslan l ' {\{}{\'{E}}{\}}cole nationale sup{\{}{\'{e}}{\}}rieure des mines de Paris Sp{\{}{\'{e}}{\}}cialit{\{}{\'{e}}{\}} « Sciences et G{\{}{\'{e}}{\}}nie des Mat{\{}{\'{e}}{\}}riaux » Simulation num{\{}{\'{e}}{\}}rique de la fissuration par fat}},
year = {2010}
}
@article{Widerst,
author = {Widerst, Fahrzeug and Fahrwiderst, Die and Rollwiderstand, Rollwiderstand Der},
pages = {10--20},
title = {{2 Fahrwiderst{\"{a}}nde , Leistungsbedarf und Fahrleistungen}}
}
@article{Pokluda2010,
author = {Pokluda, Jaroslav and Andera, Pavel},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2010{\_}Jaroslav Pokluda+Pavel {\v{S}}andera{\_}Micromechanisms of fracture and fatigue{\_}Buch/Kap3{\_}BrittleAndDuctileFracture.pdf:pdf},
journal = {Micromechanisms Fract. Fatigue},
pages = {69--123},
title = {{Brittle and Ductile Fracture}},
year = {2010}
}
@article{Schwerpunkt,
author = {Schwerpunkt, Der},
title = {{Antriebstrang- und Getriebekonzepte f u ¨ r PKW und Nutzfahrzeuge}}
}
@article{Hettinger2009,
abstract = {It is a well known fact that indicated efficiency of a SI engine at WOT is predominantly limited by knock occurrence. Therefore many investigations have been carried out to avoid knocking. Considering the further development of downsized engines knocking will also pose a greater challenge. Not only knocking but also irregular combustion in general will require further investigation in supercharged SI eingines. Premature ignition, for instance, hasn't yet been completely understood and therefore limits the low end torque of supercharged SI engines.The purpose of this paper is to introduce different analysis methods which allow to identify the knock onset and the knocking zones in the combustion chamber. In addition to established methods new techniques have been developed to account for the complex nature of pressure oscillation during knocking combustion.Experimental data was acquired on a single cylinder research engine to validate the methodology using six pressure transducers.},
author = {Hettinger, Alexander and Kulzer, Andr{\'{e}}},
doi = {10.4271/2009-01-0698},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2009{\_}Hettinger+Kulzer{\_}A new method to detect Knocking Zones.pdf:pdf},
isbn = {2009010698},
issn = {1946-3944},
journal = {SAE Int. J. Engines},
number = {1},
pages = {698--2009},
title = {{A New Method to Detect Knocking Zones}},
url = {http://papers.sae.org/2009-01-0698/},
volume = {2},
year = {2009}
}
@article{Germain1983,
abstract = {cp},
author = {Germain, P. and Nguyen, Q. S. and Suquet, P.},
doi = {10.1115/1.3167184},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Thermodynamik/1983{\_}Germain{\_}Continuum Thermodynamics.pdf:pdf},
isbn = {9789812835567},
issn = {00218936},
journal = {J. Appl. Mech.},
number = {4b},
pages = {1010},
title = {{Continuum Thermodynamics}},
url = {http://appliedmechanics.asmedigitalcollection.asme.org/article.aspx?articleid=1407311},
volume = {50},
year = {1983}
}
@book{Naumenko2016,
author = {Naumenko, Konstantin},
doi = {10.1007/978-3-319-31629-1},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/2015{\_}Naumenko+Altenbach{\_}Modeling high temperature materials behavior for structural analysis.pdf:pdf},
isbn = {9783319316277},
title = {{Modeling High Temperature Materials Behavior for Structural Analysis Part I : Continuum Mechanics}},
year = {2016}
}
@article{Krumweide1998,
author = {Krumweide, G C and Derby, A},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/{\_}buecherSong/HandbookofComposites/V/47{\_}AerospaceEquipmentandInstrumentStructure.pdf:pdf},
journal = {Small},
title = {{Aerospace Equipment and Instrument Structure}},
year = {1998}
}
@article{Banvillet2003a,
abstract = {A reliable design of industrial parts against high-cycle multiaxial fatigue requires a fatigue criterion capable of predicting both the stress gradient and the load-type effects. These effects are very important in the transfer of fatigue data from specimen to component. By using the concept of volume influencing fatigue crack initiation proposed by Palin-Luc and Lasserre with an energy based approach, a new criterion is presented. Based on the strain-work density given to the material, this proposal is usable whatever the constant amplitude loading is: in and out-of-phase combined loadings, with or without mean stress. Its predictions are compared both with a total of 38 experiments on four materials (a mild steel, two high strength steels and a spheroidal graphite cast iron) and with the predictions of local criteria (Crossland, Dang Van, Papadopoulos and Morel). The comparison shows that the predictions of the volumetric proposal are very good and less scattered than those of the local approaches, especially for loadings with mean stresses or under non-proportional loadings. ?? 2003 Elsevier Science Ltd. All rights reserved.},
author = {Banvillet, A. and Palin-Luc, T. and Lasserre, S.},
doi = {10.1016/S0142-1123(03)00048-3},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Empirical Fatigue Models + Validation/Energy based models/A volumetric energy based high  cycle multiaxial fatigue criterion.pdf:pdf},
issn = {01421123},
journal = {Int. J. Fatigue},
keywords = {Criterion,Energy,Gradient,High cycle fatigue,Multiaxial,Volume},
number = {8},
pages = {755--769},
title = {{A volumetric energy based high cycle multiaxial fatigue citerion}},
volume = {25},
year = {2003}
}
@article{Wendel2007,
author = {Wendel, Jan},
doi = {10.1524/9783486595154.5},
isbn = {9783486595154},
number = {in m},
title = {{2 Lineare Systeme}},
year = {2007}
}
@article{Vorgang,
author = {Vorgang, Experimenteller},
pages = {217--232},
title = {{1.1 Begriffe}}
}
@article{Frischdampf-2013,
author = {Frischdampf-, Entwicklung},
doi = {10.1007/978-3-8348-2279-6},
isbn = {9783834822796},
pages = {28--74},
title = {{4 Konventionelle Dampfkraftwerke}},
year = {2013}
}
@article{Anforderungena,
author = {Anforderungen, Die and Sicherheitsaspekte, Die and Komfort, Beim and Handling-, Beim and Schr, Reifeneigenschaften and Winterreifen, Bei},
title = {{4 Reifenlastenheft}}
}
@article{Strictest2011,
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Strictest, In and Confidence, Commercial and One, Part and Strictest, In and Confidence, Commercial},
doi = {10.1002/ejoc.201200111},
eprint = {arXiv:1011.1669v3},
isbn = {9781107671812},
issn = {0196-6553},
journal = {Eng. Med. Biol. Soc. 2008. EMBS 2008. 30th Annu. Int. Conf. IEEE},
number = {August},
pages = {2004},
pmid = {26840611},
title = {{Table of of contents}},
year = {2011}
}
@article{Kontinuumsmechanik2013,
author = {Kontinuumsmechanik, Grundlagen D E R},
number = {November},
pages = {1--46},
title = {{Prozesssimulation in Der Einf{\"{u}}hrung in Die Mathematischen}},
year = {2013}
}
@article{Olmeda2015,
author = {Olmeda, Pablo and Mart{\'{i}}n, Jaime and Novella, Ricardo and Carre{\~{n}}o, Ricardo},
doi = {http://dx.doi.org/10.1016/j.apenergy.2015.08.051},
file = {:C$\backslash$:/Users/p327208/Desktop/Promotion/Literature/Motorspezifisch/Heat Transfer Combustion Chamber/2015{\_}Olmeda{\_}An adapted heat transfer model for engines with tumble motion.pdf:pdf},
journal = {Appl. Energy},
keywords = {combustion diagnosis,engine heat transfer},
pages = {190--202},
publisher = {Elsevier Ltd},
title = {{An adapted heat transfer model for engines with tumble motion before Top Dead Centre}},
volume = {158},
year = {2015}
}
@article{Einzelkr,
author = {Einzelkr, Kapitel and Kraftsysteme, Solche and Kr, Die and Erfahrungstatsache, Diese and Satz, Der and Kraft, Die and Wirkung, Die},
doi = {10.1007/978-3-642-13806-5},
isbn = {9783642138065},
title = {{afte mit gemeinsamem Angriffspunkt 2 Kr ¨}}
}
@article{Work2003,
author = {Work, O F Virtual},
journal = {Work},
pages = {139--151},
title = {{Element and Global Stiffness and Mass Matrices 10.1}},
year = {2003}
}
@article{Terms2014,
author = {Terms, Index},
doi = {10.1016/B978-0-12-416677-6.00029-9},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Zienkiewicz FEM - Vol 2 Solid Structural Mechanics/63212{\_}sindx.pdf:pdf},
isbn = {978-0-08-043408-7},
issn = {00220248},
journal = {Seeds},
pages = {1573--1586},
pmid = {24263858},
title = {{Subject Index}},
url = {http://linkinghub.elsevier.com/retrieve/pii/B9780124166776000299},
year = {2014}
}
@article{Nitsche2006,
author = {Nitsche, Wolfgang and Brunn, Andr{\'{e}}},
isbn = {3540209905},
journal = {Str{\{}{\"{o}}{\}}mungsmesstechnik},
pages = {7--40},
title = {{Druckmessung}},
volume = {6},
year = {2006}
}
@article{Hoffmeyer2006,
abstract = {Experimental results of a research project on short crack growth under multiaxial nonproportional loading are presented. Fatigue lives, crack growth curves and the deformation behaviour of hollow tube specimens and notched specimens were investigated under combined tension and torsion loading. The results served as basis for the development of a cyclic plasticity model [D??ring R, Hoffmeyer J, Vormwald M, Seeger T. A plasticity model for calculating stress-strain sequences under multiaxial nonproportional cyclic loading. In: Comput Mater Sci. 28(3-4);2003:587-96; D??ring R, Hoffmeyer J, Seeger T, Vormwald M. Constitutive modelling of nonproportional hardening, cyclic hardening and ratchetting. In: Proceedings of the seventh international conference on biaxial/multiaxial fatigue and fracture, DVM, Berlin; 2004. p. 291-6; Hoffmeyer J. Anrisslebensdauervorhersage bei mehrachsiger Beanspruchung auf Basis des Kurzrisskonzepts. PhD-Thesis, TU Darmstadt; 2004.] and a short crack model [Hoffmeyer J. Anrisslebensdauervorhersage bei mehrachsiger Beanspruchung auf Basis des Kurzrisskonzepts. PhD-Thesis, TU Darmstadt; 2004; D??ring R, Hoffmeyer J, Seeger T, Vormwald M. Fatigue lifetime prediction based on a short crack growth model for multiaxial nonproportional loading. In: Proceedings of the seventh international conference on biaxial and multiaxial fatigue and fracture, DVM, Berlin; 2004. p. 253-8]. Stress-strain paths including nonproportional hardening and experimental fatigue lives of the unnotched specimens under different loading cases are discussed and compared with calculations. Load-time-sequences were in-phase, 45?? and 90?? out-of-phase loading with constant and variable amplitudes, torsion without and with superimposed static normal stress, and strain paths like box, butterfly, diamond and cross path. For the notched specimens fatigue lives under 0?? and 90?? out-of-phase loading are compared with calculations based on finite element results and the short crack model. During some tests the initiation, growth and orientation of short cracks was studied using the plastic replica technique. ?? 2005 Elsevier Ltd. All rights reserved.},
author = {Hoffmeyer, J and D{\"{o}}ring, R and Seeger, T and Vormwald, M},
doi = {10.1016/j.ijfatigue.2005.05.014},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/2005{\_}Hoffmeyer{\_}Deformation behaviour, short crack growth and fatigue lives under multiaxial nonproportional loading.pdf:pdf},
isbn = {0142-1123},
issn = {01421123},
journal = {Int. J. Fatigue},
keywords = {Cyclic deformation,Experiments,Multiaxial loading,Replica technique,Short cracks},
number = {5-6},
pages = {508--520},
title = {{Deformation behaviour, short crack growth and fatigue lives under multiaxial nonproportional loading}},
volume = {28},
year = {2006}
}
@article{Gross2011a,
author = {Gross, Dietmar and Seelig, Thomas},
doi = {10.1007/978-3-642-10196-0},
isbn = {978-3-642-10195-3},
title = {{Bruchmechanik}},
url = {http://link.springer.com/10.1007/978-3-642-10196-0},
year = {2011}
}
@article{Procedure,
author = {Procedure, Accounting and Mass, Air and Gemisch, Ammoniak-wasser and Industrie, Deutschen},
title = {{Sachwortverzeichnis}}
}
@article{DASGUPTA2001,
abstract = {This paper presents a micro-mechanistic approach for modeling fatigue damage initiation due to cyclic plasticity and cyclic creep in eutectic Pb-Sn solder. The issue of damage evolution is deferred to a future paper. Fatigue damage model due to cyclic plasticity is modeled with dislocation mechanics. A conceptual framework is provided to quantify the influence of temperature on fatigue damage due to cyclic plasticity. Damage mechanics due to cyclic creep is modeled with a void nucleation model based on micro-structural stress fields. Micro-structural stress states are estimated under viscoplastic phenomena like grain boundary sliding and its blocking at second phase particles, and diffusional creep relaxation. A conceptual framework is provided to quantify the creep-fatigue damage due to thermo-mechanical cycling.},
author = {DASGUPTA, A. and SHARMA, P. and UPADHYAYULA, K.},
doi = {10.1106/NM1B-1UQH-DJCT-4YH1},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Kriechen{\_}Spannungsrelaxation/2001{\_}Dasgubta{\_}Micro-Mechanics of fatigue due to vibration and thermal cycling.pdf:pdf},
issn = {10567895},
journal = {Int. J. Damage Mech.},
number = {2},
pages = {101--132},
title = {{Micro-Mechanics of Fatigue Damage in Pb-Sn Solder Due to Vibration and Thermal Cycling}},
url = {http://techpub.metapress.com/link.asp?target=contribution{\&}id=NM1B1UQHDJCT4YH1},
volume = {10},
year = {2001}
}
@article{VODA199541,
author = {Voda, A A and Landau, I D},
doi = {https://doi.org/10.1016/0005-1098(94)00067-S},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Vorlesungen/Messtechnik+Regelungstechnik/1993{\_}Voda+Landau{\_}AMethodForTheAutoCalibrationOfPIDControllers.pdf:pdf},
journal = {Automatica},
keywords = {PID control,automatic calibration,neglected dynamics,robustness margins},
number = {1},
pages = {41--53},
title = {{A method for the auto-calibration of PID controllers}},
volume = {31},
year = {1995}
}
@book{Merker2000,
author = {Merker, G{\"{u}}nter and Baumgarten, Carsten},
publisher = {Vieweg+Teubner Verlag},
title = {{Fluid- und W{\"{a}}rmetransport Str{\"{o}}mungslehre}},
year = {2000}
}
@article{Wulfinghoff2010a,
author = {Wulfinghoff, Stephan and B{\"{o}}hlke, Thomas},
doi = {10.1002/pamm.201010168},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2010{\_}Wulfinghoff{\_}Gradient Plasticity for Single Crystals.pdf:pdf},
issn = {16177061},
pages = {351--352},
title = {{Gradient Plasticity for Single Crystals}},
volume = {352},
year = {2010}
}
@article{Brosdorf,
author = {Br{\"{o}}sdorf, Klaus-dieter and Depr{\'{e}}, Klaus and G{\"{o}}ritz, J{\"{o}}rg},
pages = {471--558},
title = {{A17 A17 Schadenaufkl{\{}{\"{a}}{\}}rung A17}}
}
@article{Gu2002a,
author = {Gu, Minyi and Die, Lynda and Frank, R C and Mark, I D},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2012{\_}Trijselaar{\_}KNOCK PREDICTION IN GAS FIRED RECIPROCATING ENGINES.pdf:pdf},
pages = {8--15},
title = {{A N ew Vec t or f or H i gh - Throughpu t , L i ga t i on - I ndependen t C l on i ng E ncod i ng a Tobacco E t ch V i rus Pro t e ase C l e avage S i t e}},
volume = {15},
year = {2002}
}
@article{Kreher1996,
author = {Kreher, Wolfgang S},
doi = {10.1016/S0927-0256(96)00073-0},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Probabilistic Aspects/1996{\_}Kreher{\_}Modeling of random microstructural stresses and grain boundary damage in polycrystals.pdf:pdf},
issn = {09270256},
journal = {Comput. Mater. Sci.},
keywords = {damage,internal stresses,polycrystals,randomness},
number = {1-2},
pages = {147--153},
title = {{Modeling of random microstructural stresses and grain boundary damage in polycrystals}},
url = {http://linkinghub.elsevier.com/retrieve/pii/S0927025696000730},
volume = {7},
year = {1996}
}
@article{Rice1969a,
abstract = {The fracture of ductile solids has frequently been observed to result from the large growth and coalescence of microscopic voids, a process enhanced by the superposition of hydrostatic tensile stresses on a plastic deformation field. The ductile growth of voids is treated here as a problem in continuum plasticity. First, a variational principle is established to characterize the flow field in an elastically rigid and incompressible plastic material containing an internal void or voids, and subjected to a remotely uniform stress and strain rate field. Then an approximate Rayleigh-Ritz procedure is developed and applied to the enlargement of an isolated spherical void in a nonhardening material. Growth is studied in some detail for the case of a remote tensile extension field with superposed hydrostatic stresses. The volume changing contribution to void growth is found to overwhelm the shape changing part when the mean remote normal stress is large, so that growth is essentially spherical. Further, it is found that for any remote strain rate field, the void enlargement rate is amplified over the remote strain rate by a factor rising exponentially with the ratio of mean normal stress to yield stress. Some related results are discussed, including the long cylindrical void considered by F.A. McClintock (1968, J. appl. Mech. 35, 363), and an approximate relation is given to describe growth of a spherical void in a general remote field. The results suggest a rapidly decreasing fracture ductility with increasing hydrostatic tension.},
author = {Rice, J.R. and Tracey, D.M.},
doi = {10.1016/0022-5096(69)90033-7},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Plasticity models/On the ductile enlargement of voids in triaxial stress fields {\_}RiceAndTracey.pdf:pdf},
isbn = {0022-5096},
issn = {00225096},
journal = {J. Mech. Phys. Solids},
number = {3},
pages = {201--217},
title = {{On the ductile enlargement of voids in triaxial stress fields∗}},
url = {http://linkinghub.elsevier.com/retrieve/pii/0022509669900337},
volume = {17},
year = {1969}
}
@article{Lucas,
author = {Lucas, Klaus},
journal = {Arbeit},
title = {{4. Die Energiebilanz}}
}
@article{Wasserwellen2006,
author = {Wasserwellen, Den},
journal = {Gerthsen Phys.},
pages = {519--568},
title = {{10 - Wellenoptik}},
year = {2006}
}
@article{Feng2002a,
author = {Feng, L and Zhang, K-S. and Zhang, G and Yu, H-D.},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2002{\_}Feng{\_}Anisotropic-damage-model-under-continuum-slip-crystal-plasticity-theory-for-single-crystals.pdf:pdf},
journal = {Int. J. Solids Struct.},
keywords = {anisotropic damage,continuum damage mechanics,creep damage,crystal plasticity},
pages = {5279--5293},
title = {{Anisotropic damage model under continuum slip plasticity theory for single crystals}},
volume = {39},
year = {2002}
}
@article{Druck,
author = {Druck, Der},
journal = {Hand, The},
pages = {30--33},
title = {{4 Messmethoden}}
}
@article{Brecq2005a,
abstract = {High frequency pressure oscillations are generated under knocking conditions within the combustion chamber of Spark Ignition engines. Although acoustic-oscillation model can give the natural frequencies of these oscillations, very few mathematical models are today available, in scientific literature, to describe the oscillation deadening effect. An analytical formulation of the deadening has been highlighted. Analytical solution has been established for future ECU implementation. Coupling this new concept and an existing high-frequency model, an achieved model of the knocking pressure high frequencies is compared to experimental data. Good behavior is obtained on a natural gas fuelled spark ignition engine.},
author = {Brecq, G. and {Le Corre}, O.},
doi = {10.4271/2005-01-1126},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2005{\_}Brecq{\_}Modeling of In-cylinder Pressure Oscillations under Knocking conditions - Intro to Pressure Envelope Curve.pdf:pdf},
isbn = {2005011126},
issn = {0148-7191},
title = {{Modeling of In-cylinder Pressure Oscillations under Knocking Conditions: Introduction to Pressure Envelope Curve}},
url = {http://papers.sae.org/2005-01-1126/},
year = {2005}
}
@article{Wertung,
author = {Wertung, Der and Fe-methode, Der},
doi = {10.1007/978-3-8348-2134-8},
isbn = {9783834821348},
pages = {266--278},
title = {{11 W{\"{a}}rme{\"{u}}bertragungsprobleme}}
}
@article{Fritz2008,
author = {Fritz, Alfred Herbert and Schulze, G{\"{u}}nter},
doi = {10.1007/978-3-540-76696-4},
isbn = {978-3-540-76695-7},
pages = {494},
title = {{Fertigungstechnik}},
year = {2008}
}
@article{Lal1977a,
abstract = {This paper reviews and compares the various approaches for finding monotonic and cyclic plastic zone sizes for elastic-perfectly plastic and strain hardening materials. All through the analysis Ramberg-Osgood relationship has been used representing the monotonic and cyclic stress-strain curves. The results for elastic-perfectly plastic materials are compared with those available using finite-element technique. The ratio of monotonic plastic zone sizes strain hardening and elastic perfectly plastic materials are found to be related to the Ramberg-Osgood index n. The values of cyclic plastic zone size are found to depend upon factors like crack opening stress, material properties and specimen geometry. The cyclic plastic zone size obtained in this paper compare well with those given by Antolovich. ?? 1977.},
author = {Lal, K. M. and Garg, S. B L},
doi = {10.1016/0013-7944(77)90036-4},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/1977{\_}LAL+GARG{\_}On the evaluation of monotonic and cyclic plastic zones.pdf:pdf},
issn = {00137944},
journal = {Eng. Fract. Mech.},
number = {2},
pages = {433--442},
title = {{On the evaluation of monotonic and cyclic plastic zones}},
volume = {9},
year = {1977}
}
@article{Grosskreutz1971,
abstract = {Fatigue crack initiation Fatigue crack growth},
author = {Grosskreutz, J G},
doi = {10.1002/pssb.2220470202},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/1971{\_}Grosskreutz{\_}The Mechanisms of metal fatigue Some Details.pdf:pdf},
isbn = {0370-1972},
issn = {15213951},
journal = {Phys. Status Solidi},
number = {2},
pages = {359--396},
title = {{The mechanisms of metal fatigue (II)}},
volume = {47},
year = {1971}
}
@article{Papula2014,
abstract = {Diese Formelsammlung enth{\"{a}}lt die wichtigsten mathematischen Formeln f{\"{u}}r Mathematiker, Naturwissenschaftler und Ingenieure. Sie entspricht in ihrer Zusammensetzung dem heutigen Bedarf in Wissenschaft und Technik und ist bestimmt f{\"{u}}r den Gebrauch in Schulen, Hochschulen und in der Praxis. Aus dem Inhalt: Arithmetik, Algebra, Geometrie, Koordinatensysteme, spezielle Funktionen, Differentialrechnung, Integralrechnung und Integraltafel.},
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Papula, Lothar},
doi = {10.1007/978-3-8348-2311-3},
eprint = {arXiv:1011.1669v3},
isbn = {978-3-8348-1913-0},
issn = {0026-9255},
pmid = {15003161},
title = {{Mathematische Formelsammlung}},
url = {http://link.springer.com/10.1007/978-3-8348-2311-3},
year = {2014}
}
@article{Betrachtungend,
author = {Betrachtungen, Allgemeine},
title = {{omungen und laminar-turbulenter Umschlag}}
}
@article{Hinblick2000,
author = {Hinblick, Im},
pages = {3--8},
title = {{Einleitung}},
year = {2000}
}
@article{Felderb,
author = {Felder, Magnetische},
title = {( ) (4.1)}
}
@article{Michl2016,
author = {Michl, Johannes and Neumann, Jens and Rottengruber, Hermann and Wensing, Michael},
doi = {http://dx.doi.org/10.1016/j.applthermaleng.2015.12.062},
file = {:C$\backslash$:/Users/p327208/Desktop/Promotion/Literature/Motorspezifisch/Heat Transfer Combustion Chamber/2016{\_}Michl+Neumann{\_}Derivation and validation of a heat transfer model in a hydrogen combustion egnine.pdf:pdf},
journal = {Appl. Therm. Eng.},
pages = {502--512},
title = {{Derivation and validation of a heat transfer model in a hydrogen combustion engine}},
volume = {98},
year = {2016}
}
@article{Elektrotechnik2006,
author = {Elektrotechnik, Fachbereich and Elektrotechnik, Fachgebiet Theoretische and Tet, F G},
isbn = {3184014479},
number = {Get Ii},
pages = {0--11},
title = {{Grundlagen der Elektrotechnik II ( GET II )}},
volume = {1603},
year = {2006}
}
@article{Lin1969b,
abstract = {The mechanics of the build-up of large local plastic strains at the free surface of a polycrystal under fatigue loading is shown. Two closely located thin slices in a most-favourably-oriented crystal located at a free surface of the polycrystal are assumed to have an initial resolved shear stress of a few psi of opposite sign. Under cyclic loading, the two thin slices slide in opposite directions, one during the forward loading and the other during the reversed loading. Based on the dependency of slip on the resolved shear stress, the increase of local plastic strain in the slices with cycles of loading is calculated by applying the analogy between plastic strain and external force. The calculated local plastic shear strain in both slices (one positive and the other negative) reaches 100 per cent at the free surface in a few hundred cycles. These large plastic shear strains clearly cause the start of an extrusion or intrusion and the nucleation of a fatigue crack.},
author = {Lin, TH and Ito, YM},
doi = {doi: DOI: 10.1016/0022-5096(69)90006-4},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/1969{\_}Lin{\_}Mechanics of a fatigue crack nucleation mechanism.pdf:pdf},
isbn = {0022-5096},
issn = {0022-5096},
journal = {J. Mech. Phys. Solids},
pages = {511--523},
title = {{Mechanics of a Fatigue Crack Nucleation Mechanism}},
url = {http://www.sciencedirect.com/science/article/pii/0022509669900064},
volume = {17},
year = {1969}
}
@article{Seyedia,
author = {Seyedi, M and Desmorat, R},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/2 scale models papers/Seyedi+Desmorat+Sermage{\_}A TWO SCALE DAMAGE MODEL FOR THERMOMECHANICAL HIGH CYCLE FATIQUE FAILURE.pdf:pdf},
title = {{Two Scale Damage Model for Thermomechanical High Cycle Fatigue Failure}}
}
@book{Reuter2008a,
author = {Reuter, Manfred and Zacher, Serge},
booktitle = {Anal. Simul. und Entwurf von Regelkreisen},
doi = {10.1007/978-3-8348-9273-7},
isbn = {978-3-8348-0018-3},
title = {{Aus dem Programm}},
year = {2008}
}
@article{Tillock1996a,
abstract = {Control of the flow of thermal energy in an air-cooled engine is important to the overall performance of the engine because of potential effects on engine performance, durability, design, and emissions. A methodology is being developed for the assessment of thermal flows in air-cooled engines, which includes the use of cycle simulation and in-cylinder heat flux measurements. The mechanism for the combination of cycle simulation, the measurement of in-cylinder heat flux and wall temperatures, and comparison of predicted and measured heat flux in the methodology is presented. The methodology consists of both simulation and experimental phases. To begin, a one-dimensional gas dynamics code (WAVE) has been used in conjunction with a detailed in-cylinder flow and combustion model (IRIS) in order to simulate engine operation in a variety of operating conditions. The methods used to apply the model to the air-cooled engine case are described in detail. Sensitivity studies have been performed demonstrating the effects of unknown parameters of importance to the model predictions, but not available from experiments. After the engine model has been tuned to produce the measured pressure history, it is then used to predict the in-cylinder heat flux. Experimentally, a thermopile-based heat flux sensor has been used to measure in-cylinder surface heat flux and surface temperatures. Cycle-resolved heat flux and surface temperature measurements have been obtained over a range of air/fuel ratios. It is observed that the individual cycle heat flux varies substantially from one cycle to the next. The amount of variability in the instantaneous flux was a strong function of air/fuel ratio, with the least variability occurring near the peak power point. Peak wall temperatures were observed at the peak power point (298.5°C), with some reduction further on the rich side of stoichiometric, and substantial reductions on the lean side ({\textgreater}279.8°C at A/F = 15.75.) Comparison of the model predictions of the instantaneous in-cylinder heat flux with that measured shows that the measured heat flux tends to peak earlier in the burn, and the predicted value for the integrated heat flux over the cycle is about 15{\%} higher than that measured. {\textcopyright} 1996 Society of Automotive Engineers, Inc.},
author = {Tillock, B R and Martin, J K},
doi = {https://doi.org/10.4271/961731},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Heat Transfer Combustion Chamber/1996{\_}Tillock{\_}Meausrement and Modeling of Thermal Flows in an Air-Cooled Engine.pdf:pdf},
journal = {SAE Tech. Pap.},
number = {412},
title = {{Measurement and modeling of thermal flows in an air-cooled engine}},
url = {https://www.scopus.com/inward/record.uri?eid=2-s2.0-84877426805{\&}partnerID=40{\&}md5=99ebf800bd8e2decfb8fea0d364b6563},
year = {1996}
}
@article{Anfang,
author = {Anfang, Seit and Ars, Wankstabilisierung and Drive, Namen Dynamik and Daimlerchrysler, Hause and Beschleunigungs-, Bei and Fahrsicherheit, Richtung},
isbn = {3-8348-0109-7},
journal = {Integr. Vlsi J.},
pages = {253--264},
title = {{11 Semiaktive Sto{\ss}d{\"{a}}mpfer und aktive}}
}
@article{Pahl2007i,
author = {Pahl, Gerhard and Beitz†, Wolfgang and Feldhusen, J{\"{o}}rg and Grote, Karl-H.},
journal = {Pahl/Beitz Konstr. - Grundlagen},
title = {{Sachverzeichnis}},
year = {2007}
}
@article{Burmester,
abstract = {Seit Mitte der neunziger Jahre nimmt die Informationsf{\"{u}}lle und die Funktionalit{\"{a}}t in Fahrzeugen zu. Neben der gesamten Komfortfunktionalit{\"{a}}t, wie Klimaanlagen, elektrische Fensterheber, elektronische Sitzverstellung etc., kamen Informations- und Kommunikationssysteme, wie Telefon, Navigationssystem, E.Mail sowie {\"{u}}ber das Autoradio hinausgehende Unterhaltungssysteme, wie CD-Wechsler, Equalizer, Fernsehen, DVD hinzu. Dies zeigte sich zun{\"{a}}chst in der steigenden Anzahl von Bedienelementen wie Schaltern, Regler und Anzeigen im Fahrzeug, was bereits zu Un{\"{u}}bersichtlichkeit und Nutzungsschwierigkeiten f{\"{u}}hrte. Als Reaktion darauf entstand der Ansatz die vielen Informationen und Funktionalit{\"{a}}ten zentraler anzuzeigen und die Funktionen einheitlicher steuerbar zu machen. Einer der bekanntesten Ans{\"{a}}tze war die Einf{\"{u}}hrung des iDrives von BMW. Als Eingabeger{\"{a}}t steht ein Dreh-Dr{\"{u}}ck-Regler in der Mittelkonsole zur Verf{\"{u}}gung, der zus{\"{a}}tzlich in vier bzw. acht Richtungen geschoben und gezogen werden kann. Dieses Eingabeger{\"{a}}t zusammen mit einem zentralen Display erm{\"{o}}glicht einen Gro{\ss}teil der Interaktionen mit Informationen und Funktionen. Bei der Einf{\"{u}}hrung des iDrives im Jahre 2001 wurde schnell deutlich, dass diese eigentlich gute Idee nicht optimal umgesetzt wurde. Der {\"{O}}{\"{A}}MTC schrieb im Jahre 2003 dazu „IDrive erfordert besonders von Menschen, die den Umgang mit Computern scheuen, viel {\"{U}}bung, kann aber selbst von computervertrauten UserInnen nicht immer verl{\"{a}}sslich bedient werden. Obwohl der Einstellknopf sogar {\"{u}}ber variablen Bedienwiderstand verf{\"{u}}gt, ist die Anwendung von iDrive w{\"{a}}hrend der Fahrt fast unm{\"{o}}glich, da der Bildschirm st{\"{a}}ndig im Auge behalten werden muss“ [{\"{O}}AM03] und USA Today brachte es auf den Punkt mit „it manages to complicate simple functions beyond belief“ (zitiert nach [Nor03]). Obwohl es sicher die Absicht war, die Nutzung der Fahrzeugkomfort- und Infotainmentsysteme zu vereinfachen, so wird doch deutlich, dass dies nicht vollst{\"{a}}ndig gelungen war. Wenn Nutzungsprobleme nach der Einf{\"{u}}hrung der Produkte auftreten, so kann h{\"{a}}ufig festgestellt werden, dass die vorausgegangenen Gestaltungsprozesse ohne die Ber{\"{u}}cksichtigung der Anforderungen und Verhaltensgewohnheiten der betreffenden Nutzergruppen, des vorliegenden Usability-Gestaltungswissens oder ohne Anwendung von Usability-Methoden ausgef{\"{u}}hrt wurden [Mar05].},
author = {Burmester, Michael and Graf, Ralf and Hellbr{\"{u}}ck, J{\"{u}}rgen and Meroth, Ansgar},
doi = {10.1007/978-3-8348-9430-4_8},
isbn = {978-3-8348-9430-4},
issn = {978-3-8348-0285-9},
journal = {Infotainmentsysteme im Kraftfahrzeug},
pages = {321--355},
title = {{Usability — Der Mensch im Fahrzeug}},
url = {http://www.springerlink.com/index/10.1007/978-3-8348-9430-4{\_}8}
}
@article{Background,
author = {Background, General},
journal = {Mathematica},
pages = {1--207},
title = {{1.0 Remarks}}
}
@article{Gross2011a,
author = {Gross, Dietmar and Seelig, Thomas},
doi = {10.1007/978-3-642-10196-0},
isbn = {978-3-642-10195-3},
title = {{Bruchmechanik}},
url = {http://link.springer.com/10.1007/978-3-642-10196-0},
year = {2011}
}
@article{Prozesse,
author = {Prozesse, Aussagen and Hauptsatz, Zweiter},
journal = {Arbeit},
pages = {84--115},
title = {{5 Prozesse 5.1}}
}
@article{Grafenhorst2016,
author = {Grafenhorst, Matthias and Hartmann, Stefan and Rang, Joachim},
doi = {10.1002/pamm.201610210},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Numerik UMATS FE-Codes/2016{\_}Hartmann{\_}Time-adaptive non-linear ﬁnite-element computa tions for thermo-mechanically coupled analysis in elastic dynamical systems.pdf:pdf},
issn = {16177061},
journal = {Pamm},
number = {1},
pages = {443--444},
title = {{Time-adaptive non-linear finite-element computations for thermo-mechanically coupled analysis in inelastic dynamical systems}},
url = {http://doi.wiley.com/10.1002/pamm.201610210},
volume = {16},
year = {2016}
}
@article{Stupkiewicz2007d,
abstract = {Micromechanical analysis of heterogeneous materials allows prediction of their macroscopic behaviour from the known properties, microstructure, and interaction mechanisms of the constituents at the micro-scale. At the same$\backslash$n time, it allows determination of the microscopic response at each point of a macroscopic body subjected to external loading. The micromechanical analysis involves thus, at least,$\backslash$n two different scales of observation. The actual characteristic dimensions at these scales are, in fact, arbitrary, as long$\backslash$n as they differ sufficiently, so that the two scales can be separated.},
author = {Stupkiewicz, Stanislaw and Stupkiewicz, Stanislaw},
doi = {10.1007/978-3-540-49717-2},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Stupkievicz 2007 - Micromechanics of Contact and Interphase Layers/97165{\_}fm.pdf:pdf},
isbn = {978-3-540-49716-5},
journal = {Micromechanics of Contact and Interphase Layers},
pages = {1 -- 6},
title = {{Micromechanics of Contact and Interphase Layers}},
url = {http://www.springerlink.com/index/10.1007/978-3-540-49717-2},
volume = {30},
year = {2007}
}
@article{Weertman1956,
abstract = {Polycrystalline samples of high purity aluminium have been tested in a strain rate machine over a wide temperature range. The relationship which exists between the maximum stress, strain rate, and temperature is strain rate = A (stress)4.4exp( — QRT) where A is a constant, R is the gas constant, T is the absolute temperature, Q is an activation energy equal to 36,000 cal/mole. The results are compared with those of Servi and Grant on constant stress creep tests and shown to be almost identical.},
author = {Weertman, J.},
doi = {10.1016/0022-5096(56)90031-X},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Kriechen{\_}Spannungsrelaxation/1956{\_}Weertman{\_}Creep of polycrystalline aluminium as determined from strain rate tests.pdf:pdf},
isbn = {0022-5096},
issn = {00225096},
journal = {J. Mech. Phys. Solids},
number = {4},
pages = {230--234},
title = {{Creep of polycrystalline aluminium as determined from strain rate tests}},
url = {http://www.sciencedirect.com/science/article/pii/002250965690031X},
volume = {4},
year = {1956}
}
@article{Fan1992a,
author = {Fan, H. and Keer, L.M.},
doi = {10.1016/0013-7944(92)90059-N},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/1977{\_}Morris{\_}The early stage of fatigue crack propagation in al 2048.pdf:pdf},
issn = {00137944},
journal = {Eng. Fract. Mech.},
number = {5},
pages = {789--796},
title = {{The early stage of fatigue crack propagation}},
volume = {42},
year = {1992}
}
@article{Sauzay2002,
author = {Sauzay, M and Gilormini, P},
doi = {10.1016/S0167-8442(02)00080-0},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/2002{\_}Sauzay + Gilmormini{\_}Influence of surface effects on fatigue of microcracks nucleation.pdf:pdf},
issn = {01678442},
journal = {Evaluation},
keywords = {crack nucleation,cyclic plasticity,fatigue,persistent slip band,surface},
pages = {53--62},
title = {{Influence of surface effects on fatigue of microcracks nucleation}},
volume = {38},
year = {2002}
}
@article{Popov2009a,
author = {Popov, Valentin and Schargott, Martin},
title = {{Materialtheorie}},
year = {2009}
}
@article{Papula2011e,
author = {Papula, Lothar},
isbn = {978-3-38348-1227-8},
pages = {795},
title = {{Lothar Papula Mathematik f{\"{u}}r Ingenieure und Naturwissenschaftler Band 2}},
year = {2011}
}
@article{Berdichevsky2006,
abstract = {hepapercontinuesthediscussionofcontinuumtheoryofdislocationssuggestedbyBerdichevsky and Sedov (PMM 31(6): 981--1000, 1967). The major new points are: the choice of energy, the variational form of the governing dynamical equations, the variational principle for the final plastic state.},
author = {Berdichevsky, Victor L},
doi = {10.1007/s00161-006-0024-7},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/2006{\_}Berdichevsky{\_}Continuum theory of dislocations revisited.pdf:pdf},
issn = {09351175},
journal = {Contin. Mech. Thermodyn.},
keywords = {Continuum theory of dislocations,Plastic spin,Strain gradient plasticity},
number = {3-4},
pages = {195--222},
title = {{Continuum theory of dislocations revisited}},
volume = {18},
year = {2006}
}
@article{MacCamhaoil1989a,
author = {MacCamhaoil, Macdara},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Dynamics/Static and dynamic balancing of rigid rotors.pdf:pdf},
pages = {2},
title = {{Static and Dynamic Balancing of Rigid Rotors}},
year = {1989}
}
@article{Vikram2013,
author = {Vikram, Nirpesh and Kumar, Raghuvir},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/2013{\_}Vikram+Kumar{\_}Review-on-Fatigue-Crack-Growth-and-Finite-Element-Method.pdf:pdf},
journal = {Int. J. Sci. Eng. Res.},
number = {4},
pages = {833--843},
title = {{Review on Fatigue-Crack Growth and Finite Element Method}},
url = {http://www.ijser.org/researchpaper{\%}5CReview-on-Fatigue-Crack-Growth-and-Finite-Element-Method.pdf},
volume = {4},
year = {2013}
}
@article{Bohlke2012a,
author = {B{\"{o}}hlke, Prof Thomas},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Vorlesungen/HTF{\_}Skript.pdf:pdf},
journal = {Mechanik},
title = {{Skript zur Vorlesung H{\"{o}}here Technische Festigkeitslehre}},
year = {2012}
}
@article{Grundfunktionen2010,
author = {Grundfunktionen, Die},
doi = {10.1007/978-3-642-05455-6},
isbn = {9783642054556},
title = {{Analoges Messen elektrischer Gr ¨ o{\ss}en}},
year = {2010}
}
@article{Dampf-kraftwerke,
author = {Dampf-kraftwerke, Gas-},
doi = {10.1007/978-3-8348-2279-6},
isbn = {9783834822796},
pages = {133--150},
title = {{7 Kombinationskraftwerke}}
}
@article{Wirkung2011,
author = {Wirkung, Funktion},
doi = {10.1007/978-3-8348-8279-0},
isbn = {9783834882790},
pages = {653--672},
title = {{19 Dichtungen 19.1}},
year = {2011}
}
@article{Gedanke1953,
author = {Gedanke, Der},
number = {1860},
title = {{3 Dampfturbinen und Dampfkraftanlagen}},
year = {1953}
}
@article{Wellen,
author = {Wellen, Elektromagnetische},
title = {{Strahlung}}
}
@article{Stupkiewicz2007b,
author = {Stupkiewicz, Stanis{\l}aw},
doi = {10.1007/978-3-540-49717-2_5},
isbn = {3540497161},
issn = {16137736},
journal = {Lect. Notes Appl. Comput. Mech.},
number = {30},
pages = {59--73},
title = {{Micromechanics of boundary layers}},
volume = {2006},
year = {2007}
}
@article{Wilhelm2001,
author = {Wilhelm, Mark and Commercial, Boeing and Company, Airplane},
doi = {10.1361/asmhba0003477},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/{\_}buecherSong/HandbookofComposites/V/48{\_}AircraftApplications.pdf:pdf},
isbn = {9781467399395},
title = {{Aircraft Applications}},
volume = {21},
year = {2001}
}
@book{Gross2011d,
author = {Gross, Dietmar and Seelig, Thomas},
doi = {10.1007/978-3-642-10196-0},
isbn = {978-3-642-10195-3},
title = {{Bruchmechanik}},
url = {http://link.springer.com/10.1007/978-3-642-10196-0},
year = {2011}
}
@article{Uberschlagsunfalle,
author = {{\"{U}}berschlagsunf{\"{a}}lle, A},
pages = {451--460},
title = {{A15 A15 {\{}{\"{U}}{\}}berschlagsunf{\{}{\"{a}}{\}}lle}}
}
@article{Morris1978,
author = {Morris, W L},
doi = {10.1007/BF02652263},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/1978{\_}Morris{\_}The effect of IMP and microstructure on fatigue crack initiation in AL2219.pdf:pdf},
issn = {03602133},
journal = {Met. Trans. A},
number = {9},
pages = {1345--1348},
title = {{The effect of intermetallics composition and microstructure on fatigue crack initiation in AI 2219-T851}},
volume = {9},
year = {1978}
}
@book{Editiona,
author = {Edition, Fourth},
isbn = {9780080966724},
title = {{Introduction to Dislocations Fourth Edition}}
}
@inproceedings{Chiodi2001,
abstract = {Improvement of heat-transfer calculation for SI-engines in the three-dimensional simulation has been achieved and widely been tested by using a phenomenological heat-transfer model. The model is based on the local application of an improved Re-Nu-correlation (dimensional analysis) proposed by Bargende [1]. This approach takes advantage of long experience in engine heat transfer modeling in the real working process analysis. The results of numerous simulations of different engine meshes show that the proposed heat-transfer model enables to calculate the overall as well as the local heat transfer in good agreement with both real working process analyses and experimental investigations. The influence of the mesh structure has also been remarkably reduced and compared to the standard wall function approach, no additional CPU-time is required.},
author = {Chiodi, Marco and Bargende, Michael},
booktitle = {SAE Tech. Pap. 2001-01-3601},
doi = {https://doi.org/10.4271/2001-01-3601},
file = {:C$\backslash$:/Users/p327208/Desktop/Promotion/Literature/Motorspezifisch/2001{\_}Chiodi + Bargende{\_}Improvement of engine heat transfer.pdf:pdf},
publisher = {SAE international},
title = {{Improvement of Engine Heat-Transfer Calculation in the Three-Dimensional Simulation Using a Phenomenological Heat-Transfer Model}},
year = {2001}
}
@article{Sun2016c,
abstract = {A multi-scale model is developed in this study for linking collective behavior of short and long cracks to continuous average fatigue damage. By using the developed model, the average fatigue damage evolution can be evaluated through some parameters that reflect collective behavior of short and long cracks, while collective behavior of short and long cracks can be reflected from the measured continuous average fatigue damage evolution based on the effective stress concept. The effectiveness of the model is verified by comparing numerical results with experimental data. The comparative results show that the developed model can be used to study the metal fatigue failure mechanisms from both macro- and micro-scale viewpoint.},
author = {Sun, Bin and Xu, You Lin and Li, Zhaoxia},
doi = {10.1016/j.engfracmech.2016.02.013},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/2 scale models papers/2016{\_}Sun+Lu{\_}Multi-scale model for linking collective behavior of short.pdf:pdf},
issn = {00137944},
journal = {Eng. Fract. Mech.},
keywords = {Crack,Effective stress,Fatigue damage,Multi-scale},
pages = {141--153},
publisher = {Elsevier Ltd},
title = {{Multi-scale model for linking collective behavior of short and long cracks to continuous average fatigue damage}},
url = {http://dx.doi.org/10.1016/j.engfracmech.2016.02.013},
volume = {157},
year = {2016}
}
@book{In1993,
author = {In, North-holland Series and Achenbach, J D and Budiansky, B and Lauwerier, H a and Wijngaarden, L V a N and Willis, J R},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/Strukturmechanik MMS/Literatur/Mikromechanik{\_}B{\"{u}}cher{\_}Literaturvorschlag{\_}MMS/Nemat-Nasser 1993 Micromechanics.pdf:pdf},
isbn = {0444898816},
title = {{APPLIED MATHEMATICS AND MECHANICS MICROMECHANICS : Overall Properties}},
volume = {37},
year = {1993}
}
@article{Hochhalter2011,
abstract = {It has been observed during fatigue cracking of AA 7075-T651 that a small percentage of Al 7 Cu 2 Fe particles crack during manufacturing or very early in their life. Some of the cracked particles eventually nucleate cracks into the surrounding microstructure, and among these the number of cycles required for nucleation varies widely. It is important to comprehend the mechanics underpinning the observed variation so that the subsequent propagation stage can be accurately modeled. To this end, finite element models of replicated grain and particle geometry are used to compute mechanical fields near monitored cracked particles using an elastic–viscoplastic crystal plasticity model that captures the effect of the orientation of the grains near each monitored particle. Nonlocal, slip-based metrics are used to study the localization and cyclic accumulation of slip near the cracked particles providing mechanics-based insight into the actuation of the nucleation event. A high slip localization and cyclic accumulation rate are found to be a necessary, but not sufficient, condition for nucleation from cracked particles. A sufficient local driving stress must also be present, which is strongly dependent on the local microstructure and accumulated slip. Furthermore, the simulation results elucidate a quantitative relationship between the slip accumulated during fatigue loading and a consequential reduction of the critical local driving stress for nucleation, providing a physical basis for the fatigue damage concept. The observed nucleation direction is orthogonal to the computed local maximum tangential stress direction, as expected for this alloy. The main result is a semi-empirical model for the number of cycles required for nucleation, which is dependent on the maximum tangential stress and cyclic slip-accumulation rate near a cracked particle.},
author = {Hochhalter, J D and Littlewood, D J and Veilleux, M G and Bozek, J E and Maniatty, A M and Rollett, A D and Ingraffea, A R},
doi = {10.1088/0965-0393/19/3/035008},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/2011{\_}Hochhalter{\_}AL7075AgeometricapproachIII{\_}SemiempiricalApproachNucleation.pdf:pdf},
isbn = {09650393 (ISSN)},
issn = {0965-0393},
journal = {Model. Simul. Mater. Sci. Eng.},
number = {3},
pages = {35008},
title = {{A geometric approach to modeling microstructurally small fatigue crack formation: III. Development of a semi-empirical model for nucleation}},
url = {http://stacks.iop.org/0965-0393/19/i=3/a=035008?key=crossref.8640954c7485639bf37ab73e6f2eb0ad},
volume = {19},
year = {2011}
}
@article{Kenjeres2005,
author = {Kenjeres, S. and Gunarjo, S.B. and Hanjalic, K.},
doi = {https://doi.org/10.1016/j.ijheatfluidflow.2005.03.007},
journal = {Int. J. Heat Fluid Flow},
number = {4},
pages = {569--586},
title = {{Contribution to elliptic relaxation modelling of turbulent natural and mixed convection}},
volume = {26},
year = {2005}
}
@article{Messtechnika,
author = {Messtechnik, Der},
pages = {1--5},
title = {{1 Messen ; Voraussetzungen und Durchf{\{}{\"{u}}{\}}hrung}}
}
@book{Habenicht2012a,
author = {Habenicht, Gerd},
isbn = {9783834802958},
title = {{Aus dem Programm Fertigungstechnik}},
year = {2012}
}
@article{Konstruktion,
author = {Konstruktion, Zur},
pages = {376},
title = {{Teil II}}
}
@article{Wimmer2000e,
abstract = {This paper summarizes the results of several investigations on in-cylinder heat transfer during high-pressure and gas exchange phases as well as heat transfer in the inlet and outlet ports for a number of different engine types (DI Diesel, SI and gaseous fueled engine). The paper contains a comparision of simulation results and experimental data derived from heat flux measurements. Numerical results were obtained from zero-, one- and three-dimensional simulation methods. Time and spatially resolved heat fluxes were measured applying the surface temperature method and special heat flux sensors. The paper also includes an assessment of different sensor types with respect to accuracy and applicability.ER -},
author = {Wimmer, Andreas and Pivec, Robert and Sams, Theodor},
doi = {10.4271/2000-01-0568},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Heat Transfer Combustion Chamber/2000{\_}Wimmer{\_}Heat Transfer to the Combustion Cahmber and Port Walls of IC Engines - Measurement and Prediction.pdf:pdf},
isbn = {5612296614},
journal = {SAE Pap.},
number = {724},
title = {{Heat Transfer to the Combustion Chamber and Port Walls of IC Engines - Measurement and Prediction}},
url = {http://papers.sae.org/2000-01-0568},
volume = {2000-01-05},
year = {2000}
}
@article{Dr-IngPischinger,
abstract = {Wie in den vergangenen Jahren {\"{u}}blich, sind im Zuge von technischen Weiterentwick-lungen einige Kapitel erg{\"{a}}nzt bzw. {\"{u}}berarbeitet worden. Die erweiterte 22. Auflage beinhaltet den Stand der Vorlesungen in W{\"{a}}rme-, Kraft-und Arbeitsmaschinen (Kol-benmaschinen) sowie Verbrennungskraftmaschinen I und II. Zur Vorlesung Energie-wandlungsmaschinen ist ein eigener Umdruck erh{\"{a}}ltlich. Der Umdruck stellt eine Arbeitsunterlage f{\"{u}}r das Studium dar, kann aber den Vorle-sungs-und {\"{U}}bungsbesuch nicht ersetzen. Abweichungen zwischen Umdruck und Vorlesungen sind nicht auszuschlie{\ss}en.},
author = {{Dr-Ing Pischinger}, Univ-Prof S},
title = {{VERBRENNUNGSMOTOREN Band II}}
}
@article{Litewka2008,
author = {Litewka, Andrzej},
doi = {10.1080/01495730802199465},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/Advanced Materials and Structures for Extreme Operating Conditions - Skrzypek/Frontmatter.pdf:pdf},
isbn = {9783540742999},
issn = {0149-5739},
journal = {J. Therm. Stress.},
number = {8},
pages = {788--790},
title = {{Advanced Materials and Structures for Extreme Operating Conditions}},
url = {http://www.informaworld.com/openurl?genre=article{\&}doi=10.1080/01495730802199465{\&}magic=crossref{\%}7C{\%}7CD404A21C5BB053405B1A640AFFD44AE3},
volume = {31},
year = {2008}
}
@article{Azzouz2010,
author = {Azzouz, F and Cailletaud, G and Quilici, S},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Kriechen{\_}Spannungsrelaxation/xxx{\_}Chaboche+Azzouz{\_}Cyclic calculations and life estimation in thermomechanical fatigue.pdf:pdf},
pages = {785--793},
title = {{Cyclic calculations and life estimation in thermomechanical fatigue}},
year = {2010}
}
@article{Mohammadi2008,
abstract = {A computational fluid dynamics (CFD) code is applied to simulate fluid flow, heat transfer and combustion in a four-stroke single cylinder engine with pent roof combustion chamber geometry, having two inlet valves and two exhaust valves. Heat flux and heat transfer coefficient on the cylinder head, cylinder wall, piston, intake and exhaust valves are determined with respect to crank angle position. Results for a certain condition are compared for total heat transfer coefficient of the cylinder engine with available correlation proposed by experimental measurement in the literature and close agreement are observed. It was found that the local value of heat transfer coefficient varies considerably in different parts of the cylinder, but they have equivalent trend with crank angle. Based on the results, new correlations are suggested to predict maximum and minimum convective heat transfer coefficient in the combustion chamber of a SI engine. ?? 2007 Elsevier Ltd. All rights reserved.},
author = {Mohammadi, A and Yaghoubi, M and Rashidi, M},
doi = {10.1016/j.icheatmasstransfer.2007.06.008},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2008{\_}Mohammadi{\_}Analysis of local convective heat transfer in a spark ignition engine.pdf:pdf},
isbn = {0735-1933},
issn = {07351933},
journal = {Int. Commun. Heat Mass Transf.},
keywords = {Combustion chamber,Heat flux,Heat transfer coefficient,SI engine},
number = {2},
pages = {215--224},
title = {{Analysis of local convective heat transfer in a spark ignition engine}},
volume = {35},
year = {2008}
}
@article{Eds,
author = {Eds, Firma},
pages = {322--403},
title = {{Fallstudien *)}}
}
@article{Walgraef1985,
abstract = {The nucleation of persistent slip bands (PSBs) in stressed metals may be interpreted as a cooperative phenomenon for dislocation populations. The competition between their mobility and nonlinear interaction (creation, annihilation, pinning) induces an instability of uniform dislocation distributions vs inhomogeneous ones and leads to the formation and persistence of spatial patterns. In particular, we have shown in preceding publications that the nucleation and coexistence of the layered structure of PSBs and the rodlike structure of the surrounding matrix can be described by a system of coupled partial differential equations of the reaction-diffusion type for immobile and mobile dislocations. Here we consider explicitly the motion and interaction of positive and negative mobile dislocations and derive an expression for their effective diffusivity. Moreover we show how these effects together with secondary slip activity may trigger the formation of walls in different directions in analogy with observations of labyrinth structures. ?? 1986.},
author = {Walgraef, Daniel and Aifantis, Elias C.},
doi = {10.1063/1.336183},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/1985{\_}WalgraefAndAifantis{\_}Dislocation patterning in fatigued metals as a result of dynamical instabilities.pdf:pdf},
issn = {00218979},
journal = {J. Appl. Phys.},
number = {2},
pages = {688--691},
title = {{Dislocation patterning in fatigued metals as a result of dynamical instabilities}},
volume = {58},
year = {1985}
}
@article{Bertram2009,
author = {Bertram, Albrecht},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/{\_}skripte/Bertram 2006 - Kontinuumsmechanik Skript.pdf:pdf},
pages = {1--241},
title = {{Vorlesungsmanuskript zur Festigkeitslehre I + II}},
year = {2009}
}
@article{Endokrinologiea,
author = {Endokrinologie, Das Forschungsgebiet Der},
pages = {1--2},
title = {{1 Einf{\{}{\"{u}}{\}}hrung}}
}
@article{Thon2015,
author = {Thon, M},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Vorlesungen/p{\_}script{\_}em1{\_}ws1516.pdf:pdf},
pages = {2--4},
title = {{Engineering Mechanics I}},
volume = {2},
year = {2015}
}
@article{Technologya,
author = {Technology, O F},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Heat Transfer Combustion Chamber/2013{\_}HEAT TRANSFER INSIDE INTERNAL COMBUSTION ENGINE - MODELLING AND COMPARISON WITH EXPERIMENTAL DATA{\_}Spitsov{\_}MastersThesis.pdf:pdf},
keywords = {combustion engine,degree program in energy,faculty of technology,heat transfer inside internal,peenranta university of technology,technology},
title = {{Heat Transfer Inside Internal Combustion Engine :}}
}
@article{Wallentowitz2006,
author = {Wallentowitz, Henning and Reif, Konrad},
doi = {10.1007/978-3-8348-9121-1_1},
isbn = {978-3-528-03971-4},
journal = {Handb. Kraftfahrzeugelektronik - Grundlagen, Kompon. Syst. Anwendungen},
pages = {1--4},
title = {{Einleitung}},
url = {http://www.springerlink.com/index/10.1007/978-3-8348-9121-1{\_}1},
year = {2006}
}
@article{Elasticity2003,
author = {Elasticity, Linear},
pages = {95--106},
title = {{Stress-Strain Relation and the Tangent-Modulus Tensor 6.1}},
year = {2003}
}
@article{Piero2005,
author = {Piero, D E L},
number = {1967},
title = {{10 Plasticity}},
year = {2005}
}
@article{Spencer1998,
author = {Spencer, Brian E},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/{\_}buecherSong/HandbookofComposites/V/49{\_}CompositesintheSportingGoodsIndustry.pdf:pdf},
issn = {08910138},
journal = {Composites},
title = {{Composites in the Sporting Goods Industry}},
year = {1998}
}
@article{Beanspruchungsablauf,
author = {Beanspruchungsablauf, Der},
title = {{5 Betriebsfestigkeit 5.1}}
}
@article{Werkstoffkennwertea,
author = {Werkstoffkennwerte, Werkstoffs},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Empirical Fatigue Models + Validation/Erm{\"{u}}dungsfestigkeit{\_}Radaj/Kap3{\_}Einfl{\"{u}}sse auf die Schwingfestigkeit.pdf:pdf},
title = {{Einfl{\"{u}}sse auf die Schwingfestigkeit}}
}
@article{Peerlings2001,
author = {Peerlings, R and Geers, M and de Borst, R and Brekelmans, W},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/2001{\_}Peerlings{\_}A{\_}critical{\_}comparison{\_}of{\_}nonlocal{\_}and{\_}grandient-enhanced{\_}softening{\_}continua.pdf:pdf},
journal = {Int. J. Solids Struct.},
keywords = {continuum damage mechanics,fracture,gradient enhancement,localisation,nonlocality,wave propagation},
pages = {7723--7746},
title = {{A critical comparison of nonlocal and gradient enhanced softening continua}},
volume = {38},
year = {2001}
}
@article{Weertman1955,
abstract = {A theory of steady-state creep is developed using Mott's mechanism of dislocation climb. It is assumed in the analysis that the rate-controlling process is the diffusion of vacancies between dislocations which are creating vacancies and those which are destroying them. The concentration of vacancies along a dislocation line is determined by setting the change in the free energy caused by a decrease or increase in the number of vacancies equal to the change in the elastic energy occuring during dislocation climb. The creep equation that results from the analysis is creep rate=const (o-{\{}{\textless}{\}}Y./kT)exp(-Q/kT) where" is a constant ("",3 to 4), Q is the activation energy of self-diffusion, kT has its usual meaning, and 0- to 108 is the stress. This equation is valid in the stress range from the critical shear stress to a stress about equal to 10' dynes/cm'. At larger stresses the creep rate increases much more rapidly with stress.},
author = {Weertman, J},
doi = {10.1063/1.1721875},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Kriechen{\_}Spannungsrelaxation/1955{\_}Weertman{\_}Theory of Steady-State Creep Based on Dislocation Climb.pdf:pdf},
isbn = {0021-8979},
issn = {00218979},
journal = {J. Appl. Phys.},
number = {10},
pages = {1213--1217},
title = {{Theory of steady-state creep based on dislocation climb}},
volume = {26},
year = {1955}
}
@article{Mechatronika,
author = {Mechatronik, Die and Feinwerktechnik, Der},
journal = {System},
pages = {183--196},
title = {{10 Feinwerktechnik}}
}
@article{Schalenbauweise,
author = {Schalenbauweise, Die},
pages = {140--146},
title = {{21 Ausstattung 21.1}}
}
@article{Burge,
author = {Burg, Heinz},
pages = {695--703},
title = {{B8 B8 Unf{\"{a}}lle mit land- oder forstwirtschaftlichen Fahrzeugen {\"{U}}berholender Pkw kollidiert mit nach links abbiegendem Traktor B8}}
}
@article{Temperatur,
author = {Temperatur, Die},
title = {{W{\"{a}}rme{\"{u}}bertrager}}
}
@article{Chaboche2008a,
abstract = {The purpose of the present review article is twofold:???recall elementary notions as well as the main ingredients and assumptions of developing macroscopic inelastic constitutive equations, mainly for metals and low strain cyclic conditions. The explicit models considered have been essentially developed by the author and co-workers, along the past 30 years;???summarize and discuss a certain number of alternative theoretical frameworks, with some comparisons made with the previous ones, including more recent developments that offer potential new capabilities. ?? 2008 Elsevier Ltd. All rights reserved.},
author = {Chaboche, J L},
doi = {10.1016/j.ijplas.2008.03.009},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/Hardening Recovery Creep/2008{\_}Chaboche{\_}A-review-of-some-plasticity-and-viscoplasticity-constitutive-theories.pdf:pdf},
isbn = {0749-6419},
issn = {07496419},
journal = {Int. J. Plast.},
keywords = {Continuum mechanics,Plasticity,Ratchetting,Strain hardening,Viscoplasticity},
number = {10},
pages = {1642--1693},
title = {{A review of some plasticity and viscoplasticity constitutive theories}},
volume = {24},
year = {2008}
}
@book{Cherkaoui2009b,
author = {Cherkaoui, Mohammed and Capolungo, Laurent},
doi = {10.1007/978-0-387-46771-9},
isbn = {978-0-387-46765-8},
title = {{Atomistic and Continuum Modeling of Nanocrystalline Materials}},
url = {http://link.springer.com/10.1007/978-0-387-46771-9},
volume = {112},
year = {2009}
}
@article{Gross2011i,
author = {Gross, Dietmar and Seelig, Thomas},
doi = {10.1007/978-3-642-10196-0},
isbn = {978-3-642-10195-3},
title = {{Bruchmechanik}},
url = {http://link.springer.com/10.1007/978-3-642-10196-0},
year = {2011}
}
@article{Grosskreutz1971a,
abstract = {Fatigue crack initiation Fatigue crack growth},
author = {Grosskreutz, J G},
doi = {10.1002/pssb.2220470202},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/1971{\_}Grosskreutz{\_}The Mechanisms of metal fatigue Some Details.pdf:pdf},
isbn = {0370-1972},
issn = {15213951},
journal = {Phys. Status Solidi},
number = {2},
pages = {359--396},
title = {{The mechanisms of metal fatigue (II)}},
volume = {47},
year = {1971}
}
@article{Bindeglied,
author = {Bindeglied, Das and Beginn, Zu and Auswahl, Die and Bemerkung, Die},
journal = {Sensors (Peterborough, NH)},
title = {{10 Sensoren}}
}
@article{Aufbau,
author = {Aufbau, Der},
title = {{1 Aufbau und Eigenschaften von Kunststoffen}}
}
@article{Grundlagen,
author = {Grundlagen, I Anmerkungen Den},
title = {{I Anmerkungen zu den Grundlagen der Finite-Element-Methode (FEM)}}
}
@article{Hdw2018,
author = {Hdw, D Q G and Lq, O X},
doi = {10.1016/j.mspro.2014.07.351},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Heat Transfer Combustion Chamber/1997{\_}Choi{\_}Analysisi of Combustion Chamber Temperature and Heat Flux in a DOHC Engine.pdf:pdf},
title = {{{\$} QDO \backslash VLV RI {\&} RPEXVWLRQ {\&} KDPEHU 7HPSHUDWXUH Temperturen Kolben und Kopf : von Last und Drehzahl -- {\textgreater} Instantan aber auch zus{\"{a}}tzlich mitgemessen !}},
volume = {7},
year = {2018}
}
@article{SMA2000,
author = {SMA},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fatigue{\_}Folien{\_}Ueberblick{\_}Standardgesetze.pdf:pdf},
pages = {35},
title = {{Fatigue: Total Life Approaches}},
year = {2000}
}
@article{Depcik2002c,
abstract = {In this paper, the available correlations proposed in the literature for the gas-side heat transfer in the intake and exhaust system of a spark-ignition internal combustion engine were surveyed. It was noticed that theseAB - {\{}{\textless}{\}}inline-graphic xlink:href="2002-01-0372{\{}{\_}{\}}fig0001" xmlns:xlink="http://www.w3.org/1999/xlink"/{\{}{\textgreater}{\}}AB - only by empirically fitted constants. This similarity provided the impetus for the authors to explore if a universal correlation could be developed. Based on a scaling approach using microscales of turbulence, the authors have fixed the exponential factor on the Reynolds number and thus reduced the number of adjustable coefficients to just one; the latter can be determined from a least squares curve-fit of available experimental data. Using intake and exhaust side data, it was shown that the universal correlationAB - {\{}{\textless}{\}}inline-graphic xlink:href="2002-01-0372{\{}{\_}{\}}fig0002" xmlns:xlink="http://www.w3.org/1999/xlink"/{\{}{\textgreater}{\}}AB - The correlation coefficient of this proposed heat transfer model with all available experimental data is 0.845 for the intake side and 0.800 for the exhaust side.ER -},
author = {Depcik, Christopher and Assanis, Dennis},
doi = {10.4271/2002-01-0372},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2002{\_}Assanis{\_}A Universal Heat Transfer Correlation for Intake and Exhaust flows in an SI INternal Combustion Engine.pdf:pdf},
journal = {SAE Pap.},
number = {January 2016},
title = {{A Universal Heat Transfer Correlation for Intake and Exhaust Flows in an Spark-Ignition Internal Combustion Engine}},
url = {http://papers.sae.org/2002-01-0372},
volume = {2002-01-03},
year = {2002}
}
@article{Potirniche2006,
abstract = {Void growth and coalescence in fcc single crystals were studied using crystal plasticity under uniaxial and biaxial loading conditions and various orientations of the crystalline lattice. A 2D plane strain unit cell with one and two cylindrical voids was employed using three-dimensional 12 potentially active slip systems. The results were compared to five representative orientations of the tensile axis on the stereographic triangle. For uniaxial tension conditions, the void volume fraction increase under the applied load is strongly dependent on the crystallographic orientation with respect to the tensile axis. For some orientations of the tensile axis, such as [1 0 0] or [1 1 0], the voids exhibited a growth rate twice as fast compared with other orientations ([1 0 0], [2 1 1]). Void growth and coalescence simulations under uniaxial loading indicated that during deformation along some orientations with asymmetry of the slip systems, the voids experienced rotation and shape distortion, due mainly to lattice reorientation. Coalescence effects are shown to diminish the influence of lattice orientation on the void volume fraction increase, but noteworthy differences are still present. Under biaxial loading conditions, practically all differences in the void volume fraction for different orientations of the tensile axes during void growth vanish. These results lead to the conclusion that at microstructural length scales in regions under intense biaxiality/triaxiality conditions, such as crack tip or notched regions, the plastic anisotropy due to the initial lattice orientation has only a minor role in influencing the void growth rate. In such situations, void growth and coalescence are mainly determined by the stress triaxiality, the magnitude of accumulated strain, and the spatial localization of such plastic strains.},
author = {Potirniche, G P and Hearndon, J L and Horstemeyer, M F and Ling, X W},
doi = {10.1016/j.ijplas.2005.06.003},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2005{\_}Horstemeyer{\_}Lattice-orientation-effects-on-void-growth-and-coalescence-in-fcc-single-crystals.pdf:pdf},
isbn = {07496419},
issn = {07496419},
journal = {Int. J. Plast.},
keywords = {Fcc Single crystal,Finite element method,Void coalescence,Void growth},
number = {5},
pages = {921--942},
title = {{Lattice orientation effects on void growth and coalescence in fcc single crystals}},
volume = {22},
year = {2006}
}
@article{Becken,
author = {Becken, Das and Haltungsbestimmungen, Bei and Beispiel, Ein},
pages = {15--20},
title = {{8 Styling und Design}}
}
@article{Kanchanomai2007,
abstract = {Fatigue cracking due to traffic load is a major factor in road damage. Therefore, durability and lifetime prediction of roads plays a substantial role for road maintenance and cost planning. This paper reports a study of fatigue crack performance of solid asphalt and asphalt-asphalt interfaces by means of the wedge-splitting test. Instead of beams and the three- or four-point bending test, the wedge splitting method was used for the first time to observe crack growth on bituminous drilling cores. Samples of solid asphalt and samples with asphalt-interfaces were tested. One group of asphalt interfaces was untreated and the other was sandblasted before spreading the top layer during manufacturing. Due to the temperature dependency of material properties of asphalt, the tests were performed in a compact climate chamber at -10, 0 and + 10(' The challenge of determining the crack length and the crack tip were detected with an optical measurement system and picture analysis after testing. The results prove that the wedge splitting method is a highly practicable and repeatable method for crack growth testing of bituminous materials.},
author = {Kanchanomai, C and Mutoh, Y},
doi = {10.1111/j.1460-2695.2006.01088.x},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/1979{\_}Kung+Fine{\_}Fatigue crack initiation and microcrack growth in 2024-T4 and 2124-T4 Alu alloy.pdf:pdf},
issn = {8756758X},
journal = {Eng. Fract. Mech.},
keywords = {fatigue crack growth,fatigue crack initiation,lead free,low cycle fatigue},
number = {5},
pages = {443--457},
title = {{Fatigue crack initiation and growth in solder alloys}},
url = {http://doi.wiley.com/10.1111/j.1460-2695.2006.01088.x},
volume = {30},
year = {2007}
}
@article{Hettinger2009c,
abstract = {It is a well known fact that indicated efficiency of a SI engine at WOT is predominantly limited by knock occurrence. Therefore many investigations have been carried out to avoid knocking. Considering the further development of downsized engines knocking will also pose a greater challenge. Not only knocking but also irregular combustion in general will require further investigation in supercharged SI eingines. Premature ignition, for instance, hasn't yet been completely understood and therefore limits the low end torque of supercharged SI engines.The purpose of this paper is to introduce different analysis methods which allow to identify the knock onset and the knocking zones in the combustion chamber. In addition to established methods new techniques have been developed to account for the complex nature of pressure oscillation during knocking combustion.Experimental data was acquired on a single cylinder research engine to validate the methodology using six pressure transducers.},
author = {Hettinger, Alexander and Kulzer, Andr{\'{e}}},
doi = {10.4271/2009-01-0698},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2009{\_}Hettinger+Kulzer{\_}A new method to detect Knocking Zones.pdf:pdf},
isbn = {2009010698},
issn = {1946-3944},
journal = {SAE Int. J. Engines},
number = {1},
pages = {698--2009},
title = {{A New Method to Detect Knocking Zones}},
url = {http://papers.sae.org/2009-01-0698/},
volume = {2},
year = {2009}
}
@book{Gross2011f,
author = {Gross, Dietmar and Seelig, Thomas},
doi = {10.1007/978-3-642-10196-0},
isbn = {978-3-642-10195-3},
title = {{Bruchmechanik}},
url = {http://link.springer.com/10.1007/978-3-642-10196-0},
year = {2011}
}
@article{Lin1969,
abstract = {The mechanics of the build-up of large local plastic strains at the free surface of a polycrystal under fatigue loading is shown. Two closely located thin slices in a most-favourably-oriented crystal located at a free surface of the polycrystal are assumed to have an initial resolved shear stress of a few psi of opposite sign. Under cyclic loading, the two thin slices slide in opposite directions, one during the forward loading and the other during the reversed loading. Based on the dependency of slip on the resolved shear stress, the increase of local plastic strain in the slices with cycles of loading is calculated by applying the analogy between plastic strain and external force. The calculated local plastic shear strain in both slices (one positive and the other negative) reaches 100 per cent at the free surface in a few hundred cycles. These large plastic shear strains clearly cause the start of an extrusion or intrusion and the nucleation of a fatigue crack.},
author = {Lin, TH and Ito, YM},
doi = {doi: DOI: 10.1016/0022-5096(69)90006-4},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/1969{\_}Lin{\_}Mechanics of a fatigue crack nucleation mechanism.pdf:pdf},
isbn = {0022-5096},
issn = {0022-5096},
journal = {J. Mech. Phys. Solids},
pages = {511--523},
title = {{Mechanics of a Fatigue Crack Nucleation Mechanism}},
url = {http://www.sciencedirect.com/science/article/pii/0022509669900064},
volume = {17},
year = {1969}
}
@book{Melorose2015,
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Melorose, J. and Perroy, R. and Careas, S.},
booktitle = {Statew. Agric. L. Use Baseline 2015},
doi = {10.1017/CBO9781107415324.004},
eprint = {arXiv:1011.1669v3},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Hull 2011 - Introduction to Dislocation.pdf:pdf},
isbn = {9788578110796},
issn = {1098-6596},
keywords = {icle},
pmid = {25246403},
title = {{Introduction to dislocations}},
volume = {1},
year = {2015}
}
@article{Murakami2012j,
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Murakami, Sumio},
doi = {10.1007/978-94-007-2666-6},
eprint = {arXiv:1011.1669v3},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/Continuum Damage Mechanics - SumioMurakami/Kap9{\_}Elastic-Brittle Damage.pdf:pdf},
isbn = {978-94-007-2665-9},
issn = {09250042},
pages = {253--276},
pmid = {25246403},
title = {{Continuum Damage Mechanics}},
url = {http://link.springer.com/10.1007/978-94-007-2666-6},
volume = {185},
year = {2012}
}
@article{General1971,
author = {General, The and Model, Linear},
doi = {10.1016/B978-0-12-627865-1.00015-5},
isbn = {9780126278651},
title = {15 15.1},
year = {1971}
}
@article{Potirniche2006b,
abstract = {Void growth and coalescence in fcc single crystals were studied using crystal plasticity under uniaxial and biaxial loading conditions and various orientations of the crystalline lattice. A 2D plane strain unit cell with one and two cylindrical voids was employed using three-dimensional 12 potentially active slip systems. The results were compared to five representative orientations of the tensile axis on the stereographic triangle. For uniaxial tension conditions, the void volume fraction increase under the applied load is strongly dependent on the crystallographic orientation with respect to the tensile axis. For some orientations of the tensile axis, such as [1 0 0] or [1 1 0], the voids exhibited a growth rate twice as fast compared with other orientations ([1 0 0], [2 1 1]). Void growth and coalescence simulations under uniaxial loading indicated that during deformation along some orientations with asymmetry of the slip systems, the voids experienced rotation and shape distortion, due mainly to lattice reorientation. Coalescence effects are shown to diminish the influence of lattice orientation on the void volume fraction increase, but noteworthy differences are still present. Under biaxial loading conditions, practically all differences in the void volume fraction for different orientations of the tensile axes during void growth vanish. These results lead to the conclusion that at microstructural length scales in regions under intense biaxiality/triaxiality conditions, such as crack tip or notched regions, the plastic anisotropy due to the initial lattice orientation has only a minor role in influencing the void growth rate. In such situations, void growth and coalescence are mainly determined by the stress triaxiality, the magnitude of accumulated strain, and the spatial localization of such plastic strains.},
author = {Potirniche, G. P. and Hearndon, J. L. and Horstemeyer, M. F. and Ling, X. W.},
doi = {10.1016/j.ijplas.2005.06.003},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2005{\_}Horstemeyer{\_}Lattice-orientation-effects-on-void-growth-and-coalescence-in-fcc-single-crystals.pdf:pdf},
isbn = {07496419},
issn = {07496419},
journal = {Int. J. Plast.},
keywords = {Fcc Single crystal,Finite element method,Void coalescence,Void growth},
number = {5},
pages = {921--942},
title = {{Lattice orientation effects on void growth and coalescence in fcc single crystals}},
volume = {22},
year = {2006}
}
@article{Gurson1977a,
abstract = {Widely used constitutive laws for engineering materials assume plastic incompressibility, and no effect on yield of the hydrostatic component of stress. However, void nucleation and growth (and thus bulk dilatancy) are commonly observed is some processes which are characterized by large local plastic flow, such as ductile fracture.},
author = {Gurson, A. L.},
doi = {10.1115/1.3443401},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Plasticity models/Continuum Theory of Ductile Rupture by Void Nucleation and  Growth-PartI{\_}ByGurson.pdf:pdf},
isbn = {0094-4289},
issn = {00944289},
journal = {J. Eng. Mater. Technol.},
number = {1},
pages = {2},
title = {{Continuum Theory of Ductile Rupture by Void Nucleation and Growth: Part I—Yield Criteria and Flow Rules for Porous Ductile Media}},
url = {http://materialstechnology.asmedigitalcollection.asme.org/article.aspx?articleid=1422194},
volume = {99},
year = {1977}
}
@article{Bedeutung2004,
author = {Bedeutung, Die and Elektronifizierung, Die and Kompetenz, Oems and Zulieferer, Die and Kapitel, Dieses and Beispiel, Am and Weiteren, Im},
pages = {323--344},
title = {{15 Systemvernetzung und Funktionseigenentwicklung im Fahrwerk – Neue Herausforderung f{\"{u}}r Hersteller und}},
year = {2004}
}
@book{Steinbach2008,
author = {Steinbach, Olaf},
booktitle = {English},
doi = {10.1007/978-0-387-68805-3},
isbn = {978-0-387-31312-2},
title = {{Numerical Approximation Methods for Elliptic Boundary Value Problems}},
url = {http://www.springerlink.com/index/10.1007/978-0-387-68805-3},
year = {2008}
}
@article{Polyacrylic,
author = {Polyacrylic, A C M},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Stupkievicz 2007 - Micromechanics of Contact and Interphase Layers/97165{\_}indx.pdf:pdf},
title = {{Index Terms A}}
}
@book{Dhondt2004,
author = {Dhondt, G.},
booktitle = {Wiley},
doi = {10.1002/0470021217},
isbn = {0470857528},
pages = {340},
title = {{The Finite Element Method for Three-dimensional Thermo- mechanical Applications}},
year = {2004}
}
@article{Hochrainer2009a,
abstract = {Crystal plasticity is the result of the motion and interaction of dislocations. There is, however, still a major gap between microscopic and mesoscopic simulations and continuum crystal plasticity models. Only recently a higher dimensional dislocation density tensor was defined which overcomes some drawbacks of earlier dislocation density measures. The evolution equation for this tensor can be considered as a continuum version of dislocation dynamics. We use this evolution equation to develop evolution equations for the total dislocation density and an average curvature which together govern a faithful representation of the dislocation kinematics without having to use extra dimensions.},
archivePrefix = {arXiv},
arxivId = {1010.2884},
author = {Hochrainer, T. and Zaiser, M. and Gumbsch, P.},
doi = {10.1063/1.3241258},
eprint = {1010.2884},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2010{\_}Hochrainer{\_}Dislocation transport and line length increase in averageddescription of dislocations.pdf:pdf},
isbn = {9780735407091},
issn = {0094243X},
journal = {AIP Conf. Proc.},
keywords = {Continuum tlieory of dislocations,Dislocations dynamics},
pages = {1133--1136},
title = {{Dislocation transport and line length increase in averaged descriptions of dislocations}},
volume = {1168},
year = {2009}
}
@article{Newman1984,
abstract = {A general crack opening stress equation is presented which may be used to correlate crack growth rate data for various materials and thicknesses, under constant amplitude loading, once the proper constraint factor has been determined. The constraint factor, alpha, is a constraint on tensile yielding; the material yields when the stress is equal to the product of alpha and sigma. Delta-K (LEFM) is plotted against rate for 2024-T3 aluminum alloy specimens 2.3 mm thick at various stress ratios. Delta-K sub eff was plotted against rate for the same data with alpha = 1.8; the rates correlate well within a factor of two.},
author = {Newman, J C},
doi = {10.1007/BF00020751},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/1984{\_}Newman{\_}A Crack opening stress equation for fatigue crack growth.pdf:pdf},
isbn = {0376-9429},
issn = {03769429},
journal = {Int. J. Fract.},
number = {4},
pages = {131--135},
title = {{A crack opening stress equation for fatigue crack growth}},
volume = {24},
year = {1984}
}
@article{Adrian2013,
author = {Irimescu, Adrian},
doi = {http://dx.doi.org/10.1016/j.applthermaleng.2012.06.051},
file = {:C$\backslash$:/Users/p327208/Desktop/Promotion/Literature/Motorspezifisch/Heat Transfer Combustion Chamber/2013{\_}Irimescu{\_}Convective heat transfer equation for turbulent flow in tubes applied to ICE operated under motored conditions.pdf:pdf},
journal = {Appl. Therm. Eng.},
keywords = {convective heat transfer,internal combustion engines},
number = {1},
pages = {536--545},
publisher = {Elsevier Ltd},
title = {{Convective heat transfer equation for turbulent flow in tubes applied to internal combustion engines operated under motored conditions}},
volume = {50},
year = {2013}
}
@article{Stanley1999,
abstract = {This paper presents a simplified piston ring assembly (PRA) friction model of the piston ring pack and the piston skirt. The ring model considers both mixed and hydrodynamic lubrication; the skirt model considers hydrodynamic lubrication only. The Reynold's equation is used as a governing equation for the hydrodynamic regimes of both models. Simplified assumptions are used to include mixed lubrication in the ring model. The ring model generates unique Stribeck curves for a given ring's geometry; the skirt model generates generic relationships between the friction force and skirt geometry, piston speed, oil viscosity, and assumed boundary conditions. Inter-ring starvation effects are introduced by varying the boundary conditions, as appropriate. The models are compared to measurements made on a motored and fired single-cylinder diesel engine; the theoretical calculations provide a reasonable estimate of the measured data. .},
author = {Stanley, Richard and Taraza, Dinu and Henein, Naeim and Bryzik, Walter},
doi = {10.4271/1999-01-0974},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Mechanik+Reibung/1999{\_}Stanley{\_}A Simplified Friction Model of the Piston Ring Assembly.pdf:pdf},
isbn = {SAE 1999-01-0974},
number = {724},
title = {{A Simplified Friction Model of the Piston Ring Assembly}},
url = {http://papers.sae.org/1999-01-0974/},
year = {1999}
}
@article{Murakami2012b,
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Murakami, Sumio},
doi = {10.1007/978-94-007-2666-6},
eprint = {arXiv:1011.1669v3},
isbn = {978-94-007-2665-9},
issn = {09250042},
pages = {57--76},
pmid = {25246403},
title = {{Continuum Damage Mechanics}},
url = {http://link.springer.com/10.1007/978-94-007-2666-6},
volume = {185},
year = {2012}
}
@article{Fitton1992a,
author = {Fitton, J C and Nates, R J},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Klopfen{\_}Ottomotor/1992{\_}Fitton{\_}and{\_}Nates{\_}Investigation into the relationship between knock intensity and piston seizure.pdf:pdf},
journal = {N{\{}{\&}{\}}O J.},
title = {{Investigation into the relationship between knock intensity and piston Seizure}},
year = {1992}
}
@article{Bozek2008,
abstract = {Microstructurally small fatigue crack (MSFC) formation includes stages of incubation, nucleation and microstructurally small propagation. In AA 7075-T651, the fracture of Al 7 Cu 2 Fe constituent particles is the major incubation source. In experiments, it has been observed that only a small percentage of these Fe-bearing particles crack in a highly stressed volume. The work presented here addresses the identification of the particles prone to cracking and the prediction of particle cracking frequency, given a distribution of particles and crystallographic texture in such a volume. Three-dimensional elasto-viscoplastic finite element analyses are performed to develop a response surface for the tensile stress in the particle as a function of the strain level surrounding the particle, parent grain orientation and particle aspect ratio. A technique for estimating particle strength from fracture toughness, particle size and intrinsic flaw size is developed. Particle cracking is then determined by comparing particle stress and strength. The frequency of particle cracking is then predicted from sampling measured distributions of grain orientation, particle aspect ratio and size. Good agreement is found between the predicted frequency of particle cracking and two preliminary validation experiments. An estimate of particle cracking frequency is important for simulating the next stages of MSFC formation: inserting all particles into a microstructural model for these stages is computationally intractable and physically unnecessary.},
author = {Bozek, J E and Hochhalter, J D and Veilleux, M G and Liu, M and Heber, G and Sintay, S D and Rollett, A D and Littlewood, D J and Maniatty, A M and Weiland, H and Christ, R J and Payne, J and Welsh, G and Harlow, D G and Wawrzynek, P A and Ingraffea, A R},
doi = {10.1088/0965-0393/16/6/065007},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/2008{\_}Hochhalter{\_}AL7075AgeometricapproachI{\_}ParticeleCracking.pdf:pdf},
isbn = {09650393 (ISSN)},
issn = {0965-0393},
journal = {Model. Simul. Mater. Sci. Eng.},
number = {6},
pages = {65007},
title = {{A geometric approach to modeling microstructurally small fatigue crack formation: I. Probabilistic simulation of constituent particle cracking in AA 7075-T651}},
url = {http://stacks.iop.org/0965-0393/16/i=6/a=065007?key=crossref.c2c7fddb48a7b52013977b4d25c503c4},
volume = {16},
year = {2008}
}
@article{Merhy2013,
abstract = {This paper presents results and interpretations of several long crack thermo-mechanical fatigue tests on A356-T7 cast aluminum alloy used in automotive cylinder heads. These tests were conducted on CT16 and SEN specimens for different positive and negative load ratios, temperatures, frequencies and stress intensity factor values in order to establish the contribution of each parameter governing the fatigue crack propagation. It was shown that the decrease of the frequency causes significant increase of the crack growth rate especially at high temperatures and load ratios. The performing of negative load ratio tests had shown a primordial importance of the compressive load part of fatigue on the crack advance. In addition, SEM, optical microscopy and other metallographic techniques were used to examine fracture surfaces and to analyze particles cracking. For positive load ratios tests, it was shown that in stage II (Paris regime) and stage III (high crack growth rates) the number of cracked particles increases with Kmax and gradual changes in fracture surface appearance occur. These changes were associated with different crack growth mechanisms at the microstructural scale. The amplitude of the inelastic deformations and the extent of the plastic zone ahead of the crack tip were used to explain the observed changes in crack growth mechanisms. The crack growth under negative load ratio loads is especially analyzed, and a way of deriving this rate is given and shown to be relevant even for nonisothermal loading. ?? 2013 Elsevier Ltd.},
author = {Merhy, E. and R??my, L. and Maitournam, H. and Augustins, L.},
doi = {10.1016/j.engfracmech.2013.03.019},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/2013{\_}Merhy{\_}Crack growth characterisation of A356-T7 aluminium alloy under TMF.pdf:pdf},
issn = {00137944},
journal = {Eng. Fract. Mech.},
keywords = {A356 cast alloy,Crack growth rate,Damage tolerant design,Life time prediction,Thermal-mechanical fatigue},
pages = {99--112},
publisher = {Elsevier Ltd},
title = {{Crack growth characterisation of A356-T7 aluminum alloy under thermo-mechanical fatigue loading}},
url = {http://dx.doi.org/10.1016/j.engfracmech.2013.03.019},
volume = {110},
year = {2013}
}
@article{Stab,
author = {Stab, Torsionswinkel and Biegung, Balken and Biegesteifigkeit, Biegemoment and Verbundbedingung, Biegespannung},
doi = {10.1007/978-3-642-19984-4},
isbn = {9783642199844},
title = {{Ucke}}
}
@article{Seifert2010,
abstract = {In the present paper, mechanism-based models are developed to describe the time and temperature dependent cyclic plasticity and damage of cast iron materials. The cyclic plasticity model is a combination of a viscoplastic model with kinematic hardening and a porous plasticity model to take the effect of graphite inclusions into account. Thus, the model can describe creep, relaxation and the Bauschinger-effect as well as the tension-compression asymmetry often observed for cast iron. The model for thermomechanical fatigue life prediction is based on a crack growth law, which assumes that the crack growth per cycle, da/dN, is correlated with the cyclic crack-tip opening displacement, ?? CTOD. The effect of the graphite inclusions on crack growth is incorporated with a scalar factor into the crack growth law. Both models can describe the essential phenomena which are relevant for cast iron materials. ?? 2010 Elsevier Ltd. All rights reserved.},
author = {Seifert, T and Riedel, H},
doi = {10.1016/j.ijfatigue.2010.02.004},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/2010{\_}Seifert+Riedel{\_}Mechanism-based thermomechanical fatigue life prediction of cast iron PartOne Models.pdf:pdf},
isbn = {01421123},
issn = {01421123},
journal = {Int. J. Fatigue},
keywords = {Cast iron,Fatigue crack growth,Life prediction,Plasticity,Thermomechanical fatigue},
number = {8},
pages = {1358--1367},
publisher = {Elsevier Ltd},
title = {{Mechanism-based thermomechanical fatigue life prediction of cast iron. Part I: Models}},
url = {http://dx.doi.org/10.1016/j.ijfatigue.2010.02.004},
volume = {32},
year = {2010}
}
@article{Eslami2015a,
abstract = {An approach for prediction of high cycle fatigue (HCF) at a length scale of 5-100 ??m is established, which evaluates the accumulated plastic shear strain in slip bands of grains. Damage mechanisms initiated by dislocations and the grain microstructure are the key factors that influence the fatigue of metals in small dimensions. For this reason the HCF model considers the elasto-plastic behavior of metals at the grain level and microstructural parameters, specifically grain size and grain orientation. The HCF model can be applied either as a criterion for deterministic predictions of the failure in individual grains, or as a failure function in probabilistic studies on aggregates of grains, if the input parameters are given by specific distributions. This is addressed in a parameter study and a sensitivity analysis of the failure function with respect to different parameters. For model verification, the predicted results of the failure function are compared with the observed micro-damage in individual grains of nickel micro-samples. It is shown that the overall predictive power of the HCF model is fairly good. Nevertheless, some misclassifications occur as some grains are damaged, which were predicted to be safe. Those misclassifications are addressed in post-fatigue investigations on individual grains.},
author = {Eslami, R and Riesch-Oppermann, H and Kraft, O},
doi = {10.1016/j.ijfatigue.2015.03.029},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2015{\_}Eslami+Kraft{\_}Prediction of multiaxial high cycle fatigue at small scales based on an micro-mecahnical model{\_}IAM{\_}KIT{\_}KRAFT.pdf:pdf},
issn = {01421123},
journal = {Int. J. Fatigue},
keywords = {Accumulated plastic shear strain,Micro electro mechanical systems (MEMS),Multiaxial high cycle fatigue (HCF),Probability methods,Surface damage},
pages = {66--74},
publisher = {Elsevier Ltd},
title = {{Prediction of multiaxial high cycle fatigue at small scales based on a micro-mechanical model}},
url = {http://dx.doi.org/10.1016/j.ijfatigue.2015.03.029},
volume = {83},
year = {2015}
}
@article{KOTHARE1996,
author = {Kothare, Mayuresh V and Balakrishnan, Venkataramanan and Morari, Manfred},
doi = {https://doi.org/10.1016/0005-1098(96)00063-5},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Vorlesungen/Messtechnik+Regelungstechnik/1996{\_}Kothare{\_}Robust constrained model predictive control using linear matrix inequalities.pdf:pdf},
journal = {Automatica},
keywords = {Model predictive control,convex optimization,linear matrix inequalities,multivariable control systems,on-line operation,robust control,robust stability,state-feedback,time-varying systems},
number = {10},
pages = {1361--1379},
title = {{Robust constrained model predictive control using linear matrix inequalities}},
volume = {32},
year = {1996}
}
@article{Broekaert2017HCCI,
author = {Broekaert, Stijn and Cuyper, Thomas De and Paepe, Michel De and Verhelst, Sebastian},
doi = {http://dx.doi.org/10.1016/j.apenergy.2017.08.100},
file = {:C$\backslash$:/Users/p327208/Desktop/Promotion/Literature/Motorspezifisch/Heat Transfer Combustion Chamber/2017{\_}Broekaert{\_}Evaluation of empirical heat transfer models for HCCI combustion in a CFR engine.pdf:pdf},
journal = {Appl. Energy},
keywords = {Experimental,Heat transfer,Homogeneous charge compression ignition,Internal combustion engine},
pages = {1141--1150},
publisher = {Elsevier},
title = {{Evaluation of empirical heat transfer models for HCCI combustion in a CFR engine}},
volume = {205},
year = {2017}
}
@book{Ibrahimbegovic2009,
abstract = {This volume provides insight into modelling and ultimate limit computation$\backslash$nof complex structures, with their components represented by solid$\backslash$ndeformable bodies. The book examines practically all the important$\backslash$nquestions of current interests for nonlinear solid mechanics: plasticity,$\backslash$ndamage, large deformations, contact, dynamics, instability, localisation$\backslash$nand failure, discrete models, multi-scale, multi-physics and parallel$\backslash$ncomputing, with special attention given to finite element solution$\backslash$nmethods. The presentation of topics is structured around different$\backslash$naspects of typical boundary value problems in nonlinear solid mechanics,$\backslash$nwhich provides the best pedagogical approach while keeping the book$\backslash$nsize reasonable despite its very broad contents. Other strong points$\backslash$nare the exhaustive treatment of subjects, with each question studied$\backslash$nfrom different angles of mechanics, mathematics and computation,$\backslash$nas well as a successful merger of scientific cultures and heritage$\backslash$nfrom Europe and the USA. The book content and style is also the product$\backslash$nof rich international experience in teaching Master and Doctoral$\backslash$nlevel courses, as well as the courses organized for participants$\backslash$nfrom industry (IPSI courses) in France, and similar courses in Germany$\backslash$nand Italy. Every effort was made to make the contents accessible$\backslash$nto non-specialists and users of computer programs.},
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Ibrahimbegovic, Adnan},
booktitle = {Solid Mech. its Appl.},
doi = {10.1007/978-90-481-2331-5_1},
eprint = {arXiv:1011.1669v3},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Ibrahimbegovic 2009 - Nonlinear Solid Mechanics.pdf:pdf},
isbn = {9789048123308},
issn = {09250042},
pages = {1--594},
pmid = {25246403},
title = {{Nonlinear solid mechanics}},
volume = {160},
year = {2009}
}
@article{Xu1993,
abstract = {In a numerical micromechanical study of void nucleation, a framework is used where
constitutive relations are specified independently for the matrix, the void-nucleating particles and the interface. Plane strain analyses are carried out for a doubly periodic array of circular cylindrical particles. The particles are taken to be rigid and the elastic-plastic deformations of the matrix are decribed in terms of continuum crystalline plasticity, using a planar crystal model that allows for three slip systems. Comparison is made with void-nucleation predictions based on a corresponding flow theory of plasticity with isotropic hardening. The crystal model on give rise to shear localization at the particle-matrix interface and shear localization, which leads to large localized strains in the matrix. is found to inhibit decohesion. The role of the triaxiality of the stress state in determining whether decohesion or localization occurs first is investigated. A parametric study is also carried out for a crystal matrix using two descriptions of the interface shear behaviour; one is periodic in the shear displacement across the interface while the other allows for shear decohesion.},
author = {Xu, X -P and Needleman, A},
doi = {10.1088/0965-0393/1/2/001},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/1993{\_}Needleman{\_}Void nucleation by inclusion debonding in a crystal matrix.pdf:pdf},
issn = {0965-0393},
journal = {Model. Simul. Mater. Sci. Eng.},
number = {2},
pages = {111--132},
title = {{Void nucleation by inclusion debonding in a crystal matrix}},
url = {http://stacks.iop.org/0965-0393/1/i=2/a=001?key=crossref.0ad72f94185990833a445936aea2f0ba},
volume = {1},
year = {1993}
}
@article{Metallplastizit2013e,
author = {Metallplastizit, Hrungdie and Helm, Dirk},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/{\_}skripte/Helm - Prozesssimulation und Umformtechnik/Kapitel2{\_}3.pdf:pdf},
number = {November},
pages = {1--29},
title = {{Prozesssimulation in Der Umformtechnik}},
year = {2013}
}
@article{Druckindizierung2008,
author = {Druckindizierung, Grundlagen Der},
pages = {39--114},
title = {{Verbrennungsdiagnostik}},
volume = {1},
year = {2008}
}
@article{Systems2009,
author = {Systems, Linear Shift-invariant},
number = {x},
pages = {407--418},
title = {{The Discrete Fourier Transform}},
year = {2009}
}
@article{Schallgeschwindigkeit,
author = {Schallgeschwindigkeit, Aufgrund Der},
pages = {200--210},
title = {{4 Motorleistungsab stimmung im Versuch}}
}
@book{ONeal1972,
abstract = {This book provides an applications-oriented introduction to digital signal processing written primarily for electrical engineering undergraduates. Practicing engineers and graduate students may also find it useful as a first text on the subject. Digital signal processing is everywhere. Today's college students hear “DSP” all the time in their everyday life—from their CD players, to their electronic music synthesizers, to the sound cards in their PCs. They hear all about “DSP chips”, “oversampling digital filters”, “1-bit A/D and D/A converters”, “wavetable sound synthesis”, “audio effects processors”, “all-digital audio studios”. By the time they reach their junior year, they are already very eager to learn more about DSP. Approach},
author = {O'Neal, J},
booktitle = {IEEE Trans. Commun.},
doi = {10.1109/TCOM.1972.1091274},
isbn = {0-13-209172-0.},
issn = {0090-6778},
number = {5},
pages = {1046--1047},
pmid = {22203662},
title = {{Introduction to Signal Transmission}},
url = {http://ieeexplore.ieee.org/document/1091274/},
volume = {20},
year = {1972}
}
@article{Senkung2007,
author = {Senkung, Die and Statements, Aktuelle and Motoren, Erste and Chrysler, Daimler- and Hersteller, Weitere and Einspritzdr, Heutige},
journal = {Stand},
pages = {427--432},
title = {{16 Ausblick}},
year = {2007}
}
@article{Leidich,
author = {Leidich, Erhard and Deters, Ludger},
doi = {10.1007/978-3-540-76647-6},
isbn = {978-3-540-76647-6},
issn = {0937-7433},
journal = {Konstr. des Maschinenbaus},
pages = {13--69},
title = {{Normen, Toleranzen, Passungen und Technische Oberfl{\{}{\"{a}}{\}}chen}},
url = {http://www.springerlink.com/content/k3qk85404263063q/}
}
@article{Rudolf2007,
author = {Rudolf, Als and Ende, Diesel},
title = {{Kraftstoffe}},
year = {2007}
}
@article{Wirsching1983b,
abstract = {Two methods are discussed for constructing a design curve on the safe side of fatigue data. Both the tolerance interval and equivalent prediction interval (EPI) concepts provide such a curve while accounting for both the distribution of the estimators in small samples and the data scatter. The EPI is also useful as a mechanism for providing necessary statistics on S-N data for a full reliability analysis which includes uncertainty in all fatigue design factors. Examples of statistical analyses of the general strain life relationship are presented. The tolerance limit and EPI techniques for defining a design curve are demonstrated. Examples usng WASPALOY B and RQC-100 data demonstrate that a reliability model could be constructed by considering the fatigue strength and fatigue ductility coefficients as two independent random variables. A technique given for establishing the fatigue strength for high cycle lives relies on an extrapolation technique and also accounts for "runners." A reliability model or design value can be specified.},
author = {Wirsching, P. H.},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Probabilistic Aspects/1983{\_}Wirsching{\_}Statistical summaries of fatigue data for design purposes.pdf:pdf},
issn = {05657059},
journal = {Nasa Cr 3697},
number = {July},
title = {{Statistical Summaries of Fatigue Data for Design Purposes}},
year = {1983}
}
@article{Verdichtung,
author = {Verdichtung, Begrenzte},
title = {{Die dieselmotorische Verbrennung}}
}
@article{Lange2002a,
abstract = {Ein Grundkurs zur Theorie des Systems Atmosph{\"{a}}re},
author = {Lange, Hans-Joachim},
doi = {10.1007/978-3-8348-9781-7},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/xxx{\_}Herzog{\_}Kolbenmaschinen{\_}2{\_}ThermodynamischeGrundlagen.pdf:pdf},
isbn = {978-3-8348-1404-3},
journal = {Die Phys. des Wetters und des Klimas},
pages = {1--64},
title = {{Thermodynamische Grundlagen}},
year = {2002}
}
@article{Zienkiewicz2014a,
abstract = {This chapter is dedicated to fully describing the characteristic based split (CBS) algorithm. Both the compressible and incompressible flow problems are explained within a unified framework of the CBS algorithm. In addition to explaining various time discretization schemes within the CBS algorithm, two approaches to the split are also presented and tested. The stability properties, accuracy and many other aspects of the CBS algorithm are analysed in depth. Some examples are also provided to demonstrate the accuracy of the CBS scheme.},
author = {Zienkiewicz, O.C. and Taylor, R.L. and Nithiarasu, P.},
doi = {10.1016/B978-1-85617-635-4.00003-0},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Zienkiewicz FEM - Vol 3 Fluid Dynamics/63229{\_}03.pdf:pdf},
isbn = {9781856176354},
journal = {Finite Elem. Method Fluid Dyn.},
pages = {87--125},
title = {{The Characteristic-Based Split (CBS) Algorithm: A General Procedure for Compressible and Incompressible Flow}},
url = {http://linkinghub.elsevier.com/retrieve/pii/B9781856176354000030},
year = {2014}
}
@article{Verbrennungsmotoren2012a,
author = {Verbrennungsmotoren, Grundlagen},
doi = {10.1007/978-3-8348-1988-8},
isbn = {9783834819888},
pages = {591--602},
title = {{15 3D-Simulation der Aufladung 15.1}},
year = {2012}
}
@article{Schweißen1990,
author = {Schwei{\ss}en, Das F{\"{u}}geverfahren},
title = {{3 F{\"{u}}gen 3.1}},
year = {1990}
}
@article{Tabellenb,
author = {Tabellen, Die and Zahlenwerte, Tabelle and Gau{\ss}, Der},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Empirical Fatigue Models + Validation/Betriebsfestigkeit{\_}ErwinHaibach/Kap5 Anhang.pdf:pdf},
title = {{5 Anhang Daten zu statistischen Verfahren}}
}
@article{Liu2005a,
abstract = {A new high-cycle fatigue criterion based on the critical plane approach is proposed in this paper. Unlike most of the other multiaxial fatigue criteria based on the critical plane approach, the critical plane is directly correlated with the fatigue fracture plane. The proposed criterion has a wide range of applicability from very ductile metals to extremely brittle metals. Mean stress effect is also included in this criterion. The new fatigue criterion is then extended to a fatigue life prediction model. The results of the proposed fatigue criterion and fatigue life prediction model are validated with experimental results from the literature. ?? 2005 Elsevier Ltd. All rights reserved.},
author = {Liu, Yongming and Mahadevan, Sankaran},
doi = {10.1016/j.ijfatigue.2005.01.003},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Empirical Fatigue Models + Validation/2005{\_}Mahadevan{\_}Multiaxial high-cycle fatigue criterion and life prediction for metals.pdf:pdf},
isbn = {01421123},
issn = {01421123},
journal = {Int. J. Fatigue},
keywords = {Critical plane,High-cycle fatigue,Life prediction,Metals,Multiaxial fatigue},
number = {7},
pages = {790--800},
title = {{Multiaxial high-cycle fatigue criterion and life prediction for metals}},
volume = {27},
year = {2005}
}
@article{Habenicht2012e,
author = {Habenicht, Gerd},
isbn = {9783834802958},
title = {{Aus dem Programm Fertigungstechnik}},
year = {2012}
}
@article{Zheng2001a,
abstract = {Research on the basic fatigue formula, the criterion for omitting small loads, the rule for cumulative fatigue damage, and models for predicting the fatigue crack initiation (FCI) life and probability distribution under variable-amplitude loading are comprehensively studied and summarized in the present paper. First, the formula for FCI life is given as a function of the equivalent stress amplitude, and the procedures for investigating overload effects are introduced. Using the above formula to analyze test results of the overload effect on FCI life yields the formula for FCI life containing the overload effect factor, z, which can be adopted to characterize the load interaction effect when Miner's rule is used to compute the cumulative fatigue damage. Fatigue test results and analysis of the underload effect show that the FCI threshold in the FCI life formula can be taken as the criterion for omitting small loads in life prediction and in compilation of the load spectrum. Then, the fatigue damage functi on is defined, the cumulative fatigue damage can be computed and the FCI life of structure members under variable-amplitude loading can be obtained by using Miner's rule. Procedures for predicting the probability distribution of FCI life or fatigue life are described and examples are introduced. Furthermore, factors affecting the value of z and the applicability of Miner's rule are briefly discussed. Finally, further areas for fatigue research are tentatively proposed. Most interest should be focused on research into generally applicable life prediction models and the approach for fatigue reliability assessment of structure details made of the metals with continuous strain-hardening characteristics, which have been widely adopted in aeronautical engineering, under service load and environments. ?? 2001 Elsevier Science Ltd. All rights reserved.},
author = {Zheng, Xiulin},
doi = {10.1016/S0142-1123(01)00040-8},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Empirical Fatigue Models + Validation/2001{\_}Zheng{\_}On some basic problems of fatigue research in engineering{\_}ModelsAccumulationProbabilityOverloadeffect.pdf:pdf},
issn = {01421123},
journal = {Int. J. Fatigue},
keywords = {Criterion for omitting small load,Fatigue crack initiation,Fatigue damage function,Fatigue formula,Joints,Life prediction,Miner's rule,Overload effect,Strain-hardening characteristics},
number = {9},
pages = {751--766},
title = {{On some basic problems of fatigue research in engineering}},
volume = {23},
year = {2001}
}
@article{Lucas,
author = {Lucas, Klaus},
journal = {Arbeit},
title = {{4. Die Energiebilanz}}
}
@article{Ewing2003,
author = {Ewing, Following},
journal = {Methods},
pages = {43--49},
title = {{Introduction to Variational and Numerical Methods 3.1}},
year = {2003}
}
@article{Publishing2011,
author = {Publishing, Ebsco and Library, Sheffield},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Zienkiewicz FEM - Vol 3 Fluid Dynamics/63229{\_}01.pdf:pdf},
isbn = {9780750663229},
pages = {1--27},
title = {{Introduction to the equations of fluid dynamics and the finite}},
year = {2011}
}
@article{Normzustand,
author = {Normzustand, Physikalischer and Normzustand, Physikalischer and Wichte, Die and Wichte, Die and Kelvin, Das and Kelvin, Das},
journal = {Arbeit},
pages = {161--176},
title = {{6.1 Grundbegriffe}}
}
@article{Loubar2005c,
abstract = {This paper deals with the transient thermal signal around an engine cylinder in order to propose a new and nonintrusive method of knock detection. Numerical simulations of unsteady heat transfer through the cylinder and inside the coolant flow are carried out to account for heat flux variations due to normal and knocking combustion. The effect of rib roughened surfaces on thermal signal amplification is investigated. The geometric parameters are fixed at Pi/h=70 and w/h=1 with a Reynolds number based on hydraulic diameter of 12,000. The results reveal that square ribs give better performance in term of thermal signal amplification within the fluid. An amplification of the temperature variation up to 20 times higher is found. Finally, flow analysis shows that amplification depends on the position where the thermal signal is collected.},
author = {Loubar, Khaled and Bellettre, Jérôme and Tazerout, Mohand},
doi = {10.1115/1.1857943},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2005{\_}Loubar{\_}Unsteady Heat Transfer enhancement around an engine cylinder in order to detect knockpdf.pdf:pdf},
isbn = {0022-1481},
issn = {00221481},
journal = {J. Heat Transf.},
number = {3},
pages = {278},
title = {{Unsteady Heat Transfer Enhancement Around an Engine Cylinder in Order to Detect Knock}},
url = {http://heattransfer.asmedigitalcollection.asme.org/article.aspx?articleid=1447711},
volume = {127},
year = {2005}
}
@article{Prof.Dr.-Ing.Dietmar2012,
author = {{Prof. Dr. -Ing. Dietmar}, Gross},
journal = {Springer},
title = {{Kap. 5 Schwingungen Technishce Mechanik 3}},
year = {2012}
}
@article{Outline,
author = {Outline, Historical},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/Advanced Materials and Structures for Extreme Operating Conditions - Skrzypek/Kapitel2 Material Properties for High Temperature.pdf:pdf},
journal = {High Temp.},
pages = {1--12},
title = {{Material Properties for High Temperature}}
}
@article{Pahl2007i,
author = {Pahl, Gerhard and Beitz†, Wolfgang and Feldhusen, J{\"{o}}rg and Grote, Karl-H.},
journal = {Pahl/Beitz Konstr. - Grundlagen},
title = {{Sachverzeichnis}},
year = {2007}
}
@article{Sommitsch2007,
abstract = {During hot extrusion of aluminium alloys, extrusion dies experience cyclic temperature changes as well as multiaxial loadings. To improve the service life of the dies, cleaner and high hot strength materials are designed as well as an optimised process control is performed. For the improvement of the process guiding and a comparison of lifetime behaviour of different hot work tool steels, modelling and simulation are appropriate means. The extrusion process has been simulated using the FE-program Deform to find the stress and temperature history at the inner diameter of the liner, i.e. the boundary conditions for the subsequent cyclic simulation of the container during service. Inelastic constitutive equations have been implemented into Abaqus Standard to describe strain hardening and time recovery effects. They include the Norton viscoplastic flow rule, thermo-mechanical isotropic hardening and two non-linear kinematic hardening laws. A damage-rate model predicts failure and thus the lifetime of the container. The procedure for the identification of material parameters for both the constitutive and the damage model is described in detail for the hot work tool steel B{\{}{\"{o}}{\}}hler W400 VMR (EN 1.2343). {\{}{\textcopyright}{\}} 2006 Elsevier B.V. All rights reserved.},
author = {Sommitsch, C and Sievert, R and Wlanis, T and G{\"{u}}nther, B and Wieser, V},
doi = {10.1016/j.commatsci.2006.03.024},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Kriechen{\_}Spannungsrelaxation/2007{\_}Sommitsch{\_}Modelling of creep-fatigue in containers during aluminium and copper extrusion.pdf:pdf},
isbn = {09270256},
issn = {09270256},
journal = {Comput. Mater. Sci.},
keywords = {Creep-fatigue,Damage,Extrusion,Hot work tool steels,Lifetime},
number = {1 SPEC. ISS.},
pages = {55--64},
title = {{Modelling of creep-fatigue in containers during aluminium and copper extrusion}},
volume = {39},
year = {2007}
}
@article{Tanaka1982a,
abstract = {The fatigue crack initiation along the slip banks emanating from notches is analyzed theoretically with the use of the dislocation dipole accumulation model proposed previously by the authors. The complex function analysis for an elliptical notch under the anti-plane shear gives a quantitative method for assessment of the reduction of fatigue strength as a function of the notch tip radius, the notch size and the elastic stress concentration factor. Special cases of this theoretical analysis yield several semi-empirical formulae commonly used by engineers for data collection. In the derivation, the limitations for each engineering approach are clarified. The material properties are included in the present micromechanical theory as the slip band length and the dislocation frictional stress. ?? 1982.},
author = {Tanaka, K and Mura, T},
doi = {10.1016/0167-6636(82)90024-2},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/1981{\_}Mura+Tanaka{\_}A micromechanical theory of fatigue crack initiation from notches.pdf:pdf},
isbn = {0921-5093},
issn = {01676636},
journal = {Mech. Mater.},
number = {1},
pages = {63--73},
title = {{A micromechanical theory of fatique crack initiation from notches}},
volume = {1},
year = {1982}
}
@article{Kreher1985a,
author = {Kreher, W and Pompe, W},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Probabilistic Aspects/1985{\_}Kreher{\_}Field Fluctuations in a heterogeneous elastic material - an info theory approach.pdf:pdf},
journal = {J. Mech. Phys. Solids},
number = {5},
pages = {419--445},
title = {{Field fluctuations in a heterogeneous elastic material: An information theory approach}},
volume = {33},
year = {1985}
}
@article{Meschede2010,
abstract = {F{\"{u}}r die Studierenden der Physik im Haupt- und Nebenfach ist der Gerthsen ein unverzichtbarer und kompetenter Begleiter durch das gesamte Studium. Nahezu alle Studierenden beginnen mit dem Klassiker Gerthsen. S{\"{a}}mtliche Gebiete der Physik werden ausf{\"{u}}hrlich und gut verst{\"{a}}ndlich dargestellt. Das Buch beginnt bei den klassischen Themen - Mechanik, Elektrodynamik, Optik, Festk{\"{o}}rperphysik - und f{\"{u}}hrt auf dieser Grundlage in die mikroskopischen Eigenschaften der Materie, die statistische Physik und die Relativit{\"{a}}tstheorie ein und erkl{\"{a}}rt schlie{\ss}lich die faszinierenden Konsequenzen f{\"{u}}r unser Verst{\"{a}}ndnis von der Nichtlinearen Dynamik unserer Welt und der Entwicklung des Kosmos.},
author = {Meschede, Dieter},
doi = {10.1007/978-3-642-12894-3},
isbn = {978-3-642-12893-6},
issn = {09377433},
journal = {Gerthsen Phys.},
pages = {1047},
title = {{Elektromagnetismus: Ladungen und Str{\"{o}}me}},
url = {http://www.springerlink.com/index/10.1007/3-540-29973-4{\%}5Cnhttp://link.springer.com/chapter/10.1007/978-3-642-12894-3{\_}8},
volume = {22},
year = {2010}
}
@article{Merker2003a,
author = {Merker, G{\"{u}}nter and Schwarz, Christian and Stiesch, Gunnar and Otto, Frank},
doi = {10.1007/978-3-8351-9069-6},
isbn = {3-8351-0080-7},
journal = {Simul. der Verbrennung und Schadstoffbildung},
title = {{Simulation der Verbrennung und Schadstoffbildung}},
year = {2003}
}
@book{Zybell2016,
author = {Zybell, Lutz},
doi = {10.1007/978-3-319-21467-2},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/Damage books proposals by Johannes G{\"{o}}rthofer/H{\"{u}}tter{\_}2016{\_}Recent{\_}Trends{\_}in{\_}Fracture{\_}and{\_}Damage{\_}Mechanics.pdf:pdf},
isbn = {978-3-319-21466-5},
title = {{Recent Trends in Fracture and Damage Mechanics}},
url = {http://link.springer.com/10.1007/978-3-319-21467-2},
year = {2016}
}
@article{Conduction,
author = {Conduction, Heat},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/Advanced Materials and Structures for Extreme Operating Conditions - Skrzypek/Kapitel3 Thermodynamics of Constitutive Modelling of.pdf:pdf},
number = {x},
title = {{Thermodynamics of Constitutive Modelling of 2 . 1 Effect of Damage on the Mechanical and Thermal}}
}
@article{Kocks2003a,
author = {Kocks, U F and {H. Mecking}},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/Hardening Recovery Creep/2002{\_}Kocks+Mecking{\_}Physics and phenomenology of strain hardening{\_}fcc case.pdf:pdf},
isbn = {4042878407},
journal = {Prog. Mater. Sci.},
pages = {171--273},
title = {{Physics and phenomenology of strainhardening: the FCC case}},
url = {https://www.academia.edu/8128075/Physics{\%}7B{\_}{\%}7Dand{\%}7B{\_}{\%}7Dphenomenology{\%}7B{\_}{\%}7Dof{\%}7B{\_}{\%}7Dstrain{\%}7B{\_}{\%}7Dhardening{\%}7B{\_}{\%}7Dthe{\%}7B{\_}{\%}7DFCC{\%}7B{\_}{\%}7Dcase},
volume = {48},
year = {2003}
}
@article{Tschirschwitzc,
author = {Tschirschwitz, Christian},
pages = {629--643},
title = {{B4 B4 Unf{\{}{\"{a}}{\}}lle mit motorisierten Zweir{\{}{\"{a}}{\}}dern B4}}
}
@book{Voyiadjis2021,
author = {Voyiadjis, George Z},
doi = {10.1007/978-1-4614-8968-9},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/Damage books proposals by Johannes G{\"{o}}rthofer/Voyiadjis{\_}Handbook{\_}of{\_}Damage{\_}Mechanics.pdf:pdf},
isbn = {978-1-4614-8968-9},
title = {{Handbook of Damage Mechanics}},
url = {http://link.springer.com/10.1007/978-1-4614-8968-9},
year = {2021}
}
@article{Grosskreutz1971b,
abstract = {Fatigue crack initiation Fatigue crack growth},
author = {Grosskreutz, J. G.},
doi = {10.1002/pssb.2220470202},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/1971{\_}Grosskreutz{\_}The Mechanisms of metal fatigue Some Details.pdf:pdf},
isbn = {0370-1972},
issn = {15213951},
journal = {Phys. Status Solidi},
number = {2},
pages = {359--396},
title = {{The mechanisms of metal fatigue (II)}},
volume = {47},
year = {1971}
}
@article{Morris1979a,
author = {Morris, W. L.},
doi = {10.1007/BF02686400},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/1979{\_}Morris{\_}Microcrack closure phenomena for AL2219-T851.pdf:pdf},
issn = {03602133},
journal = {Metall. Trans. A},
number = {1},
pages = {5--11},
title = {{Microcrack closure phenomena for AI 2219-T851}},
volume = {10},
year = {1979}
}
@article{Positionierungstechnik,
author = {Positionierungstechnik, Die},
pages = {135--142},
title = {{8 Positionierungstechnik und Robotik}}
}
@article{Fatemi1998a,
abstract = {Fatigue damage increases with applied load cycles in a cumulative manner. Cumulative fatigue damage analysis plays a key role in life prediction of components and structures subjected to field load histories. Since the introduction of damage accumulation concept by Palmgren about 70 years ago and 'linear damage rule' by Miner about 50 years ago, the treatment of cumulative fatigue damage has received increasingly more attention. As a result, many damage models have been developed. Even though early theories on cumulative fatigue damage have been reviewed by several researchers, no comprehensive report has appeared recently to review the considerable efforts made since the late 1970s. This article provides a comprehensive review of cumulative fatigue damage theories for metals and their alloys, emphasizing the approaches developed between the early 1970s to the early 1990s. These theories are grouped into six categories: linear damage rules; nonlinear damage curve and two-stage linearization approaches; life curve modification methods; approaches based on crack growth concepts; continuum damage mechanics models; and energy-based theories. {\textcopyright}},
author = {Fatemi, A. and Yang, L.},
doi = {10.1016/S0142-1123(97)00081-9},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/1997{\_}Fatemi{\_}Cumulative fatigue damage and life prdeiction theories-a survey of the state of the art for homogeneous materials.pdf:pdf},
isbn = {0142-1123},
issn = {01421123},
journal = {Int. J. Fatigue},
keywords = {cumulative damage rules,cumulative fatigue damage,fatigue damage accumulation,fatigue life predictions,load interac-,tion effects},
number = {1},
pages = {9--34},
title = {{Cumulative fatigue damage and life prediction theories: a survey of the state of the art for homogeneous materials}},
url = {http://linkinghub.elsevier.com/retrieve/pii/S0142112397000819},
volume = {20},
year = {1998}
}
@article{Steuerungstechnik,
author = {Steuerungstechnik, Grundlagen Der},
pages = {199--216},
title = {{1.1 Steuerung und Regelung}}
}
@article{Betrachtungenl,
author = {Betrachtungen, Allgemeine},
journal = {Integr. Vlsi J.},
title = {{9 Stromfadentheorie 9.1}}
}
@misc{Vagera1971a,
author = {Vagera, I.},
booktitle = {Scr. Metall.},
doi = {10.1016/0036-9748(71)90036-6},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/1971{\_}Vagera{\_}A PileUp or a dislocation model of crack in an interface between two isotropic or anisotropic media.pdf:pdf},
issn = {00369748},
number = {2},
pages = {93--96},
title = {{A pile-up or a dislocation model of crack in an interface between two isotropic or anisotropic media}},
volume = {5},
year = {1971}
}
@article{Hill1931,
author = {Hill, Constraint},
doi = {http://dx.doi.org/10.1016/B978-012566251-2/50019-8},
isbn = {978-0-12-566251-2},
issn = {1076-1608},
journal = {J. Physiol.},
pages = {1--58},
title = {{Subject Index}},
volume = {71},
year = {1931}
}
@article{Hansen1998,
abstract = {The relation between polycrystal deformation and single crystal deformation has been studied in this work. A pure aluminium polycrystal having an average grain size of 300 [mu]m has been strained in tension at room temperature. The flow stress has been determined at four different strains (0.05, 0.14, 0.22 and 0.34) and deformation microstructures have been characterized qualitatively and quantitatively by transmission electron microscopy. Improved experimental techniques have allowed large foil areas to be characterized and in total 89 grains have been examined. At the four strains examined a classification of the deformation microstructures into three different types has shown a correlation between the grain orientation and the type of deformation microstructure which develops during straining. The dislocation density has been calculated at each strain and by assuming that the shear stress is proportional to the square root of the dislocation density the shear stress-strain relationship has been derived for each of the three groups of grains showing different deformation microstructures. The stress-strain curves show a strain hardening behaviour which depends on the orientation of the grain. The behaviour of the grains embedded in the polycrystal is compared with the behaviour of single crystals and the stress-strain curve of the polycrystal is estimated with good accuracy from single crystal data, which are weighted based on a quantitative texture analysis of the polycrystal.},
author = {Hansen, N. and Huang, X.},
doi = {10.1016/S1359-6454(97)00365-0},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/1998{\_}Hansen{\_}Huang MICROSTRUCTURE AND FLOW STRESS OF.pdf:pdf},
isbn = {1359-6454},
issn = {13596454},
journal = {Acta Mater.},
number = {5},
pages = {1827--1836},
title = {{Microstructure and flow stress of polycrystals and single crystals}},
url = {http://linkinghub.elsevier.com/retrieve/pii/S1359645497003650},
volume = {46},
year = {1998}
}
@article{Burga,
author = {Burg, Heinz and Moser, Andreas and Steffan, Hermann},
journal = {Simulation},
pages = {585--592},
title = {{A20 A20 Simulation und Animation A20}}
}
@article{Kramer2005,
author = {Kramer, Florian},
pages = {757--759},
title = {{C1 C1 Aktive und passive Sicherheit Die Fahrzeugsicherheit und das Risiko Die aktive Sicherheit C1 Die passive Sicherheit Nutzung von Daten und Informationen aus der aktiven f{\"{u}}r die passive Sicherheit}},
year = {2005}
}
@article{Seifert2010c,
abstract = {In the present paper, predictions of mechanism-based models for cast iron are compared to experimental results obtained for the nodular cast iron EN-GJS-700, the vermicular cast iron EN-GJV-450 and the lamellar cast iron EN-GJL-250. A strategy is proposed to efficiently identify the model parameters based on isothermal experiments. In particular, complex low cycle fatigue (LCF) tests, tension tests and compression tests are used to adjust the time and temperature dependent cyclic plasticity model. The time and temperature dependent fatigue life prediction model is adjusted to LCF tests. For all investigated cast iron materials, good predictions of thermomechanical fatigue (TMF) tests are possible with the models. Additionally, the location of failure and fatigue life of a thermomechanically loaded double-sided notched specimen are predicted with high accuracy. ?? 2010 Elsevier Ltd. All rights reserved.},
author = {Seifert, T. and Maier, G. and Uihlein, A. and Lang, K. H. and Riedel, H.},
doi = {10.1016/j.ijfatigue.2010.02.005},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/2010{\_}Seiffert+Riedel{\_}Mechanism-based thermomechanical fatigue life prediction of cast iron PartTwo Comparison of model with experiment.pdf:pdf},
isbn = {01421123},
issn = {01421123},
journal = {Int. J. Fatigue},
keywords = {Cast iron,Experimental data,Life prediction,Thermomechanical fatigue},
number = {8},
pages = {1368--1377},
publisher = {Elsevier Ltd},
title = {{Mechanism-based thermomechanical fatigue life prediction of cast iron. Part II: Comparison of model predictions with experiments}},
url = {http://dx.doi.org/10.1016/j.ijfatigue.2010.02.005},
volume = {32},
year = {2010}
}
@article{Transformatoren,
author = {Transformatoren, {\"{U}}bersicht},
pages = {218--248},
title = {{6 Der Transformator}}
}
@article{Peerlings2001,
author = {Peerlings, R and Geers, M and de Borst, R and Brekelmans, W},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/2001{\_}Peerlings{\_}A{\_}critical{\_}comparison{\_}of{\_}nonlocal{\_}and{\_}grandient-enhanced{\_}softening{\_}continua.pdf:pdf},
journal = {Int. J. Solids Struct.},
keywords = {continuum damage mechanics,fracture,gradient enhancement,localisation,nonlocality,wave propagation},
pages = {7723--7746},
title = {{A critical comparison of nonlocal and gradient enhanced softening continua}},
volume = {38},
year = {2001}
}
@article{Merker2003,
author = {Merker, G{\"{u}}nter and Schwarz, Christian and Stiesch, Gunnar and Otto, Frank},
journal = {Simul. der Verbrennung und Schadstoffbildung},
title = {{5 Ph{\{}{\"{a}}{\}}nomenologische Verbrennungsmodelle}},
year = {2003}
}
@article{Fischerauer,
author = {Fischerauer, G and Tr{\"{a}}nkler, H},
journal = {H{\"{u}}tte},
pages = {1--96},
title = {{H-Messtechnik}}
}
@article{Metallplastizit2013d,
author = {Metallplastizit, Hrungdie and Helm, Dirk},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/{\_}skripte/Helm - Prozesssimulation und Umformtechnik/Kapitel2{\_}3mitAnhang.pdf:pdf},
number = {November},
pages = {1--29},
title = {{Prozesssimulation in Der Umformtechnik}},
year = {2013}
}
@book{Ochsner2016,
author = {{\"{O}}chsner, Andreas},
doi = {10.1007/978-981-287-865-6},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/Damage books proposals by Johannes G{\"{o}}rthofer/{\"{O}}chsner{\_}Continuum{\_}Damage{\_}and{\_}Fracture{\_}Mechanics.pdf:pdf},
isbn = {9789812878632},
title = {{Continuum Damage and Fracture Mechanics}},
year = {2016}
}
@article{Spencer1998,
author = {Spencer, Brian E},
issn = {08910138},
journal = {Composites},
title = {{Composites in the Sporting Goods Industry}},
year = {1998}
}
@article{Pahl2007a,
author = {Pahl, Gerhard and Beitz†, Wolfgang and Feldhusen, J{\"{o}}rg and Grote, Karl-H.},
journal = {Pahl/Beitz Konstr. - Grundlagen},
title = {{Rechnerunterst{\{}{\"{u}}{\}}tzung}},
year = {2007}
}
@article{Feng2002a,
author = {Feng, L and Zhang, K-S. and Zhang, G and Yu, H-D.},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2002{\_}Feng{\_}Anisotropic-damage-model-under-continuum-slip-crystal-plasticity-theory-for-single-crystals.pdf:pdf},
journal = {Int. J. Solids Struct.},
keywords = {anisotropic damage,continuum damage mechanics,creep damage,crystal plasticity},
pages = {5279--5293},
title = {{Anisotropic damage model under continuum slip plasticity theory for single crystals}},
volume = {39},
year = {2002}
}
@article{Xu1993a,
abstract = {In a numerical micromechanical study of void nucleation, a framework is used where
constitutive relations are specified independently for the matrix, the void-nucleating particles and the interface. Plane strain analyses are carried out for a doubly periodic array of circular cylindrical particles. The particles are taken to be rigid and the elastic-plastic deformations of the matrix are decribed in terms of continuum crystalline plasticity, using a planar crystal model that allows for three slip systems. Comparison is made with void-nucleation predictions based on a corresponding flow theory of plasticity with isotropic hardening. The crystal model on give rise to shear localization at the particle-matrix interface and shear localization, which leads to large localized strains in the matrix. is found to inhibit decohesion. The role of the triaxiality of the stress state in determining whether decohesion or localization occurs first is investigated. A parametric study is also carried out for a crystal matrix using two descriptions of the interface shear behaviour; one is periodic in the shear displacement across the interface while the other allows for shear decohesion.},
author = {Xu, X -P and Needleman, A},
doi = {10.1088/0965-0393/1/2/001},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/1993{\_}Needleman{\_}Void nucleation by inclusion debonding in a crystal matrix.pdf:pdf},
issn = {0965-0393},
journal = {Model. Simul. Mater. Sci. Eng.},
number = {2},
pages = {111--132},
title = {{Void nucleation by inclusion debonding in a crystal matrix}},
url = {http://stacks.iop.org/0965-0393/1/i=2/a=001?key=crossref.0ad72f94185990833a445936aea2f0ba},
volume = {1},
year = {1993}
}
@article{Stebbins1967,
author = {Stebbins, Jeun},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Empirical Fatigue Models + Validation/1965{\_}NASA+Hudson{\_}Studies of fatigue crack growth in alloys suitable for elevated temperature-Al2618.pdf:pdf},
number = {May},
title = {{Nasa Technical N O T E}},
year = {1967}
}
@article{Kochmann2009a,
author = {Kochmann, D M and Hackl, Klaus. and Le, K C},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/2009{\_}Le{\_}A continuum dislocation theory for modeling dislocation microstructures in crystal plasticity.pdf:pdf},
journal = {Conf. Pap.},
keywords = {abstract,and pile up near,anisms related to the,continuum mechanics,dislocation,dislocation network,high degree on the,in order to accommodate,material moderling,mech-,microstructure,new dislocations are nucleated,plastic deformation and,plastic deformation of crystalline,plasticity,s energy,solids depends to a,the grain or,to reduce the crystal},
number = {September},
pages = {7--11},
title = {{a Continuum-Dislocation Theory for Modeling Dislocation Microstructures and Size Effects in Crystal Plastiticy}},
year = {2009}
}
@article{Darstellungsform,
author = {Darstellungsform, Beschreibende and Menge, Leere},
title = {{I Allgemeine Grundlagen aus Algebra, Arithmetik und Geometrie 1}}
}
@article{Koutiri2013,
abstract = {This article is dedicated to the high cycle fatigue behaviour of cast hypo-eutectic Al–Si alloys and in particular the AlSi7Cu05Mg03 alloy. In a vast experimental campaign undertaken to investigate the fatigue damage mechanisms operating in this alloy, subject to complex loading conditions, it was shown that two different coexisting fatigue damage mechanisms occur in this materials, depending on the presence of different microstructural heterogeneities (i.e. micro-shrinkage pores, Si particles, Fe-rich intermetallic phases, DAS of the Al-matrix, etc.). In order to take into account both of these damage mechanisms, a probabilistic approach using the weakest link concept is introduced to model the competition between the two mechanisms. This approach leads naturally to a probabilistic Kitagawa type diagram, which explains the relationship between the fatigue behaviour of the material and the different casting processes or post-treatments (e.g. gravity casting and HIP). It is shown that the sensitivity to the different loading modes (i.e. uniaxial with and without mean stress, torsion and equibiaxial tension) depends on the microstructural heterogeneities responsible for crack initiation. For a porosity-free alloy, the predictions are very good for combined tension–torsion loading modes. When pores are present and control the fatigue strength, the predictions are very satisfactory for the uniaxial loads with different R-ratios and slightly conservative for multiaxial loads (i.e. torsion and equibiaxial tension). Never-the-less, they are much better than the predictions of the Dang Van criterion [1].},
author = {Koutiri, I. and Bellett, D. and Morel, F. and Pessard, E.},
doi = {10.1016/j.ijfatigue.2012.08.004},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Probabilistic Aspects/xxxx{\_}Koutiri{\_}A probabilistic model for the high cycle fatigue behaviour of cast aluminium alloys subject to complex loads.pdf:pdf},
issn = {01421123},
journal = {Int. J. Fatigue},
keywords = {AlSi7Cu05Mg03-T7,Fatigue damage mechanisms,High cycle fatigue,Multiaxial loads,Probabilistic model},
pages = {137--147},
title = {{A probabilistic model for the high cycle fatigue behaviour of cast aluminium alloys subject to complex loads}},
url = {http://www.sciencedirect.com/science/article/pii/S0142112312002472},
volume = {47},
year = {2013}
}
@article{Caton1981b,
abstract = {Because of the increasing need for precise information on engine processes, this study developed and experimentally verified models for the instantaneous heat transfer in an engine exhaust port. Experimental measurements were made of the instantaneous cylinder pressure and instantaneous exhaust gas temperature for a range of engine operating conditions. The pressure measurements were used to obtain the instantaneous cylinder gas state and the temperature measurements were used to validate the heat transfer models. The exhaust port heat transfer was dominated by jet induced large-scale fluid motion as opposed to wallshear generated fluid motion. An analysis based on the jet velocity through the valve opening correctly estimated the heat transfer due to this large-scale motion. Models for the instantaneous exhaust port heat transfer provided excellent agreement with measurements as a function of engine operating conditions. A cause d'un besoin croissant d'information pr{\'{e}}cise sur le fonctionnement d'un moteur, on d{\'{e}}veloppe une {\'{e}}tude et on v{\'{e}}rifie exp{\'{e}}rimentalement des mod{\`{e}}les sur le transfert de chaleur instantan{\'{e}} {\`{a}} l'{\'{e}}chappement d'un cylindre. Des mesures de la pression instantan{\'{e}}e dans le cylindre et de la temp{\'{e}}rature instantan{\'{e}}e {\`{a}} l'{\'{e}}chappement sont effectu{\'{e}}es pour un domaine de conditions de fonctionnement d'un moteur. Les mesures de pression permettent d'atteindre l'{\'{e}}tat instantan{\'{e}} du gaz dans le cylindre et les mesures de temp{\'{e}}rature permettent de valider les mod{\`{e}}les de transfert thermique. Le transfert {\`{a}} l'{\'{e}}chappement est domin{\'{e}} par un mouvement de jet {\`{a}} large {\'{e}}chelle au contraire du mouvement de fluide {\`{a}} frottement pari{\'{e}}tal. Une analyse bas{\'{e}}e sur la vitesse du jet {\`{a}} travers l'ouverture de la soupape pr{\'{e}}dit correctement le transfert de chaleur d{\^{u}} {\`{a}} ce mouvement {\`{a}} grande {\'{e}}chelle. Des mod{\`{e}}les pour l'{\'{e}}chappement instantan{\'{e}} fournissent un accord excellent avec des mesures pour les conditions de fonctionnement du moteur. Wegen des zunehmenden Bedarfs an genauer Information {\"{u}}ber Verbrennungsmotoren-Prozesse wurden in dieser Studie Modelle f{\"{u}}r den momentanen W{\"{a}}rme{\"{u}}bergang in einer Motor-Ausla$\beta$-{\"{O}}ffnung entwickelt und experimentell best{\"{a}}tigt. Die Momentanwerte des Zylinderdrucks und der Abgastemperatur wurden in Versuchen f{\"{u}}r einen ausgedehnten Betriebsbereich gemessen. Druckmessungen wurden verwendet, um den momentanen Gaszustand im Zylinder zu bestimmenn und Temperaturmessungen dienten zur Best{\"{a}}tigung der W{\"{a}}rme{\"{u}}bergangs-Modelle. Der W{\"{a}}rme{\"{u}}bergang in der Ausla$\beta$-{\"{O}}ffnung wurde im wesentlichen durch die strahlinduzierte Makro-Bewegung des Fluides entgegen der durch Wandschubspannung erzeugten Fluidbewegung bestimmt. Eine theoretische Untersuchung, die sich auf die Strahlgeschwindigkeit durch die Ventil{\"{o}}ffnung st{\"{u}}tzt, liefert korrekt den W{\"{a}}rme{\"{u}}bergang, hervorgerufen durch diese Makro-Bewegung. Die Modelle f{\"{u}}r den momentanen W{\"{a}}rme{\"{u}}bergang in der Ausla$\beta$-{\"{O}}ffnung als Funktion der Arbeitsbedingungen des Motors zeigten vorz{\"{u}}gliche {\"{U}}bereinstimmung mit den Messungen. B cвязи c вce бoлee вoзpacтaющeй нeoбчoдимocтью в тoчнoй инфopмaции o пpoцeccaч, пpoиcчoдящич в двигaтeляч, пpeдлoзeны мoдeди тeплoпepeнoca в вычлoпнoм oтвepcтии двигaтeля. Измepялиcь дaвлeниe в цилиндpe и тeмпepaтypa вычлoпнoгo гaзa пpи paздичныч peзимaч paбoты двигaтeля. Дaнныe пo дaвлeнию иcпoльзoвaлиcь для oпpeдeлeния cocтoяния гaзa в цилиндpe, a пo тeмпepaтype — для пpoвepки cпpaвeдливocти пpeдлoзeнныч мoдeлeй. Teплoпepeнoc в вычлoпнoм oтвepcтии oпpeдeляeтcя кpyпнoмacштaбными пepeмeщeниями зидкocти, вoзникaющими пpи cтpyйнoм иcтeчeнии, кoтopыe cyщecтвeннo oтличaютcя oт пepeмeщeний, вызывaeмыч нaпpязeниeм cдвигa нa cтeнкe. Aнaлиз, ocнoвaный нa cкopocти иcтeчeния cтpyи чepeз oтвepcтиe клaпaнa, пoзвoляeт кoppeктнo oцeнить вeличинy тeплoвoгo пoтoкa пpи тaкич кpyпнoмacщтaбпыч пepeмeщeнияч. Moдeли тeплoпepeнoca в вычлoпнoм oтвepcтии чopoшo coглacyютcя c peзyльтaтaми измepeний пpи paзличныч peзимaч paбoты двигaтeдя.},
author = {Caton, J.A. and Heywood, J.B.},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Heat transfer intake+exhaust system/1981{\_}An experimental and analytical study of heat transfer in an engine exhaust port{\_}Caton.pdf:pdf},
journal = {Int. J. Heat Mass Transf.},
number = {4},
pages = {581--595},
title = {{An experimental and analytical study of heat transfer in an engine exhaust port}},
volume = {24},
year = {1981}
}
@article{Ritchie1985a,
abstract = {Relationships between crack initiation and crack growth toughness are reviewed by examining the crack tip fields and microscopic (local) and macroscopic (continuum) fracture criteria for the onset and continued quasi-static extension of cracks in ductile materials. By comparison of the micromechanisms of crack initiation via transgranular cleavage and crack initiation and subsequent growth via microvoid coalescence, expressions are shown for the fracture toughness of materials in terms of microstructural parameters. Utilizing the exact asymptotic crack tip deformation fields for the nonstationary plane strain Mode I crack and evoking various microscopic failure criteria for such stable crack growth, a relationship between the tearing modulus TR and the nondimensionalized crack initiation fracture toughness Jlc is described and shown to yield a good fit to experimental toughness data for a wide range of steels},
author = {Ritchie, R. O. and Thompson, A. W.},
doi = {10.1007/BF02815305},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/1985{\_}RichtieAndThompson{\_}On Macroscopic and Microscopic Analyses for Crack Initiation and Crack Groth Toughness in Ductile Alloys.pdf:pdf},
isbn = {0360-2133},
issn = {03602133},
journal = {Metall. Trans. A},
number = {1},
pages = {233--248},
title = {{On macroscopic and microscopic analyses for crack initiation and crack growth toughness in ductile alloys}},
volume = {16},
year = {1985}
}
@article{Essmann1981c,
abstract = {Based on recent experimental observations a realistic model of the evolution of the surface profile of persistent slip bands (PSBs) in fatigued metals is proposed. An essential feature of the model is the production of vacancies by the annihilation of edge dislocations which, combined with irreversible slip processes, leads to an elongation of the PSB parallel to the active slip vector. It is shown that a net extrusion forms rather rapidly. The growth processes and their dependence on temperature are discussed in detail. It is proposed that cracks initiate at the surface steps at the PSB{\{}{\&}{\}}ndash;matrix interface and, at a later stage, also at the notch-peak profile from the random slip processes.},
author = {Essmann, U and G{\"{o}}sele, U and Mughrabi, H},
doi = {10.1080/01418618108239541},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2016{\_}Mughrabi{\_}A model of extrusions and intrusions in fatigued metals I  Point defect production and the growth of extrusions.pdf:pdf},
isbn = {0141-8610},
issn = {0141-8610},
journal = {Philos. Mag. A},
number = {2},
pages = {405--426},
title = {{A model of extrusions and intrusions in fatigued metals I. Point-defect production and the growth of extrusions}},
url = {http://www.tandfonline.com/doi/abs/10.1080/01418618108239541},
volume = {44},
year = {1981}
}
@article{Konzepte,
author = {Konzepte, Downsizing- and Steigerung, Eine and Gegensatz, Im and Geschwindigkeit, Die},
title = {{3 Downsizing}}
}
@article{Meister2011a,
abstract = {Die wichtigsten Verfahren zur numerischen L{\{}{\"{o}}{\}}sung von linearen Gleichungssystemen in einer umfassenden Einf{\{}{\"{u}}{\}}hrung, die zum Verst{\{}{\"{a}}{\}}ndnis nur geringe mathematische Vorkenntnisse ben{\{}{\"{o}}{\}}tigt. Behandelt werden sowohl die direkten als auch die iterativen Verfahren, wobei der Autor gro{\{}{\ss}{\}}en Wert auf eine sorgf{\{}{\"{a}}{\}}ltige Herleitung dieser Verfahren legt. Au{\{}{\ss}{\}}erdem sind sehr detaillierte Pseudocodes enthalten, mit deren Hilfe sich die jeweiligen Verfahren in einer beliebigen Programmiersprache sofort auf dem Computer realisieren lassen. Das Lehrbuch ist auch f{\{}{\"{u}}{\}}r Natur- und Ingenieurwissenschaftler geeignet, die in vielen praktischen Anwendungen mit der L{\{}{\"{o}}{\}}sung von linearen Gleichungssystemen konfrontiert sind.},
archivePrefix = {arXiv},
arxivId = {1011.1669v3},
author = {Meister, Andreas},
doi = {10.1007/978-3-8348-8100-7},
eprint = {1011.1669v3},
isbn = {978-3-8348-1550-7},
issn = {1098-6596},
journal = {Matrix},
pages = {36--68},
pmid = {25246403},
title = {{Numerik linearer Gleichungssysteme}},
url = {http://link.springer.com/10.1007/978-3-8348-8100-7},
year = {2011}
}
@article{Bauer1998a,
abstract = {Entry flow heat transfer experiments are reported in steady and pulsating flows of air at mean Reynolds numbers of 3000-35 000. THe ducts are chosen to match typical spark-ignition engine manifolds: a highly curved and a straight pipe, which together bracket most practical geometries. The pulsating engine intake flow encompasses an approximate half sine wave followed by a stagnant phase three itmes as long, all at a repetition rate of 16-50 Hz. Heat flow is imposed through electric heating of the outsides of the manifolds. Heat transfer in the curved pipe is closely comparable to the straight geometry, and it is concluded that entrance effects dominate. Time-averaged axially resolved and axially averaged Nusselt numbers are reported. The unsteady nature of the intake flow enhances heat transfer significantly, between 50{\%} and 100{\%}. Time-resolved wall heat flux measurements at a location close to the exit of the system show that heat transfer is delayed relative to the onset of the flow. During the stagnant flow phase, heat transfer and turbulence decay slowly from their high levels during the induction flow phase. Heat transfer enhancement in the pulsating flow case is caused by the contribution of the stagnant phase.},
author = {Bauer, Wolf D. and Wenisch, Joseph and Heywood, John B.},
doi = {https://doi.org/10.1016/S0142-727X(97)10001-7},
file = {:C$\backslash$:/Users/p327208/Desktop/Promotion/Literature/Motorspezifisch/Heat transfer intake+exhaust system/1998{\_}Bauer{\_}Averaged and time-resolved heat transfer of steady and pulsating entry flow in intake manifold of a SI engine.pdf:pdf},
journal = {Int. J. Heat Fluid Flow},
keywords = {intake manifold,internal combustion engine,ow,pulsating,transient heat,ux measurements},
number = {1},
pages = {1--9},
title = {{Averaged and time-resolved heat transfer of steady and pulsating entry flow in intake manifold of a spark-ignition engine}},
volume = {19},
year = {1998}
}
@article{Anfanga,
author = {Anfang, Am},
journal = {Chart},
pages = {93--116},
title = {{5 Anwendungsorientierte {\"{U}}bersicht kommerzieller}}
}
@article{Cherkaoui2009f,
author = {Cherkaoui, Mohammed and Capolungo, Laurent},
doi = {10.1007/978-0-387-46771-9},
isbn = {978-0-387-46765-8},
pages = {353--378},
title = {{Atomistic and Continuum Modeling of Nanocrystalline Materials}},
url = {http://link.springer.com/10.1007/978-0-387-46771-9},
volume = {112},
year = {2009}
}
@article{Thon2015a,
author = {Thon, M},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Vorlesungen/p{\_}script{\_}em1{\_}ws1516.pdf:pdf},
pages = {2--4},
title = {{Engineering Mechanics I}},
volume = {2},
year = {2015}
}
@article{Gross2011j,
author = {Gross, Dietmar and Seelig, Thomas},
doi = {10.1007/978-3-642-10196-0},
isbn = {978-3-642-10195-3},
title = {{Bruchmechanik}},
url = {http://link.springer.com/10.1007/978-3-642-10196-0},
year = {2011}
}
@article{Pahl2007g,
author = {Pahl, Gerhard and Beitz†, Wolfgang and Feldhusen, J{\"{o}}rg and Grote, Karl-H.},
journal = {Pahl/Beitz Konstr. - Grundlagen},
title = {{L{\{}{\"{o}}{\}}sungsfelder}},
year = {2007}
}
@article{Negi2015,
author = {Negi, Anjna},
doi = {10.1016/j.pedn.2008},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Stupkievicz 2007 - Micromechanics of Contact and Interphase Layers/97165{\_}refs.pdf:pdf},
isbn = {0514190450},
issn = {1095-9203},
number = {2},
pages = {464--467},
pmid = {12399572},
title = {{References 1.}},
volume = {6},
year = {2015}
}
@article{Berg1998a,
author = {Berg, Kenneth R},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/{\_}buecherSong/HandbookofComposites/VI/AppendixA{\_}TypicalPropertiesforAdvancedComposites.pdf:pdf},
title = {{Typical Properties for Advanced Composites}},
year = {1998}
}
@article{Raillard2015,
author = {Raillard, B and Mu, F},
doi = {10.1016/B978-1-78242-074-3.00024-6},
isbn = {9781782420743},
title = {24 24.1},
year = {2015}
}
@article{Mughrabi2013a,
abstract = {The primary cause of fatigue damage is usually intimately related to some form of cyclic slip irreversibilities. Depending on material and details of the loading conditions, various types of fatigue crack initiation are observed. Here, typical examples of fatigue damage evolution in low and high cycle fatigue (LCF, HCF) and ultrahigh cycle fatigue (UHCF) will be discussed. Various forms of fatigue damage and life-controlling microstructural mechanisms in different metals and alloys will be illustrated. In particular, the fatigue properties of ultrafine-grained (UFG) materials will be discussed, and the microstructural mechanisms and the question of the existence of a fatigue limit in the UHCF regime will be considered. ?? 2013 The Authors.},
author = {Mughrabi, Hael},
doi = {10.1016/j.proeng.2013.03.307},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2013{\_}Mughrabi{\_}Damage mechanisms and fatigue lives - From the low to the very high cycle regime.pdf:pdf},
isbn = {9781627486361},
issn = {18777058},
journal = {Procedia Eng.},
keywords = {Fatigue crack initiation,Fatigue limit,Fatigue lives,HCF,LCF,UHCF},
pages = {636--644},
publisher = {Elsevier B.V.},
title = {{Damage mechanisms and fatigue lives: From the low to the very high cycle regime}},
url = {http://dx.doi.org/10.1016/j.proeng.2013.03.307},
volume = {55},
year = {2013}
}
@book{In1993,
author = {In, North-holland Series and Achenbach, J D and Budiansky, B and Lauwerier, H a and Wijngaarden, L V a N and Willis, J R},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/Strukturmechanik MMS/Literatur/Mikromechanik{\_}B{\"{u}}cher{\_}Literaturvorschlag{\_}MMS/Nemat-Nasser 1993 Micromechanics.pdf:pdf},
isbn = {0444898816},
title = {{APPLIED MATHEMATICS AND MECHANICS MICROMECHANICS : Overall Properties}},
volume = {37},
year = {1993}
}
@article{Stoffregen2012,
author = {Stoffregen, J},
pages = {334--351},
title = {{Motorradtechnik}},
year = {2012}
}
@article{Denton,
author = {Denton, Douglas L},
journal = {Composites},
title = {{Land Transportation Applications}}
}
@article{Hamilton2014,
abstract = {The continuous growth of the worldwide vehicle fleet is leading to many private initiatives and governmental policies for the achievement of lower pollutant and greenhouse gas emissions through energetic efficiency improvement. The in-cylinder heat transfer has been generally recognised as a major factor influencing internal combustion engines efficiency and exhaust emissions. Therefore, the analysis of in-cylinder heat transfer is of importance for fuel economy, as well as for environmental preservation. In the present paper, the use of particle filters applied on the time-dependent heat transfer coefficient estimation of a combustion process in a spark-ignition internal combustion engine is presented. The combustion process was modelled as a transient zero-dimensional process based on the First Law of Thermodynamics for a perfect gas, and the fuel burned fraction was modelled through a Wiebe's function model. Results with different measurement frequencies and errors are available, using a sample importance resampling filter, showing a very good estimate, even for initial guesses far away from the real value of the unknown function. {\{}{\textcopyright}{\}} 2013 Taylor {\{}{\&}{\}} Francis.},
author = {Hamilton, F.C.a and Cola{\c{c}}o, M.J.a and Carvalho, R.N.a B and Leiroz, A.J.K.a},
doi = {10.1080/17415977.2013.797411},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2013{\_}Hamilton{\_}Heat transfer coefficient estimation of an internal combustion engine using particle filters.pdf:pdf},
issn = {1741-5977},
journal = {Inverse Probl. Sci. Eng.},
keywords = {1741-5977,1741-5985,and engineering,com,combustion engine using particle,erse problems in science,filters,gipe20,heat transfer coefficient estimation,http,issn,journal homepage,loi,of an internal,online,print,tandfonline,www},
number = {3},
pages = {483--506},
title = {{Heat transfer coefficient estimation of an internal combustion engine using particle filters}},
url = {http://www.scopus.com/inward/record.url?eid=2-s2.0-84892543088{\%}7B{\&}{\%}7DpartnerID=40{\%}7B{\&}{\%}7Dmd5=b4dec32ec5b338e03414a6e59567e78d},
volume = {22},
year = {2014}
}
@article{Bonnet2009,
abstract = {Ein Verbundwerkstoff ist ein Werkstoff aus zwei oder mehr verbundenen Materialien. Der Verbundwerkstoff besitzt andere Werkstoffeigenschaften als seine einzelnen Komponenten.},
author = {Bonnet, Martin},
doi = {10.1007/978-3-8348-9303-1},
isbn = {978-3-8348-0349-8},
issn = {00182001},
pages = {79},
title = {{Kunststoffe in der Ingenieuranwendung}},
url = {http://link.springer.com/10.1007/978-3-8348-9303-1},
year = {2009}
}
@article{Fara-2006,
author = {Fara-, Michael and Maxwell, James Clerk},
journal = {Gerthsen Phys.},
pages = {379--445},
title = {{07 - Elektrodynamik}},
year = {2006}
}
@article{Eigenschaften,
author = {Eigenschaften, Aufbau},
title = {{4 Der Reifen}}
}
@article{Woytowitz1999,
abstract = {Solid-particle erosion (SPE) is studied by constructing finite-element (FE) models of elastic spheres impacting normally on the surface of a kinematically hardening, elastic-plastic material. The full effects of the contact surfaces and the impact dynamics are included. An earlier phase of this study modeled multiple, coincident impacts with two-dimensional (2D) analysis, in which damage computations by strain-life, cyclic plastic work (CPW), and continuum damage mechanics (CDM) methods were shown to be roughly equivalent. Here, it is shown that a 2D model is incorrect for non-coincident impacts; a 3D FE analysis is necessary. A stochastic model of multiple impacting spheres is developed, which can describe spatial and temporal accumulation of damage. Finally, erosion rates are estimated by extrapolating the average rates of damage accumulation in the outermost layers of the target material to a value of 1.0.},
author = {Woytowitz, P J and Richman, R H},
doi = {10.1016/S0043-1648(99)00173-8},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Erosion{\_}CDM/Modeling of damage from multiple impacts by spherical particles{\_}Woytowitz.pdf:pdf},
issn = {00431648},
journal = {Wear},
keywords = {Continuum damage,Cyclic plastic work,Fatigue,Finite-element analysis,Impact damage,Solid-particle erosion,Strain-life},
pages = {120--133},
title = {{Modeling of damage from multiple impacts by spherical particles}},
volume = {233-235},
year = {1999}
}
@article{Ganczarski2003a,
author = {Ganczarski, A.},
doi = {10.1007/978-3-540-36418-4_10},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Anisotropic Behaviouir of Damaged Materials{\_}Skrzypek{\_}ARTICEL/Kap10{\_}Thermo-Damage Coupling Modelling and Applications for Creep Conditions.pdf:pdf},
isbn = {9783642055874},
issn = {16137736},
journal = {Lect. Notes Appl. Comput. Mech.},
keywords = {creep conditions,metallic materials,thermo-damage coupling},
pages = {317--349},
title = {{Thermo-Damage Coupling Modelling and Applications for Creep Conditions}},
volume = {9},
year = {2003}
}
@article{Iliev,
author = {Iliev, Simeon},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Heat transfer intake+exhaust system/2013{\_}Iliev{\_}HEAT TRANSFER INVESTIGATION IN THE INTAKE PORT OF FOUR STROKE DI COMPRESSION IGNITION ENGINE.pdf:pdf},
number = {1},
pages = {133--138},
title = {{Heat Transfer Investigation in the Intake Port of Four Stroke Direct Injection Compression Ignition}}
}
@article{FISER2015,
annote = {12th IFAC Workshop onTime Delay SystemsTDS 2015},
author = {Fi{\v{s}}er, Jarom{\'{i}}r and Z{\'{i}}tek, Pavel and Vyhl{\'{i}}dal, Tom{\'{a}}{\v{s}}},
doi = {https://doi.org/10.1016/j.ifacol.2015.09.419},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Vorlesungen/Messtechnik+Regelungstechnik/2015{\_}Fiser{\_}Magnitude Optimum Design of PID Control Loop with Delay.pdf:pdf},
journal = {IFAC-PapersOnLine},
keywords = {Magnitude optimum criterion,dimensional analysis,disturbance rejection,dominant poles},
number = {12},
pages = {446--451},
title = {{Magnitude Optimum Design of PID Control Loop with Delay}},
volume = {48},
year = {2015}
}
@article{Chemisky2013,
author = {Chemisky, Yves and Meraghni, Fodil},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/Micromechanics formulas{\_}Overview{\_}EshelbyHillAndMore.pdf:pdf},
journal = {Presentations},
title = {{Micromechanics based on the Eshelby solution : Concepts and formulas}},
year = {2013}
}
@article{Energie1997,
author = {Energie, Mit Der Beherrschung Der},
pages = {2--4},
title = {{1 Einleitung}},
year = {1997}
}
@article{Agarwal2006,
abstract = {Thermal loading of diesel engine pistons has increased dramatically in recent years owing to applications of various technologies to meet low emission and high power density requirements. Control of piston temperatures by cooling of these pistons has become one of the determining factors in a successful engine design. The pistons are cooled by oil jets fired at the underside from the crankcase. Any excessive piston temperature rise may lead to engine seizure because of piston warping. However, if the temperature at the underside of the piston, where the oil jet strikes the piston, is above the boiling range of the oil being used, it may contribute to the generation of mist. This mist significantly contributes to the non-tailpipe emissions in the form of unburnt hydrocarbons (UBHCs). The problem of non-tailpipe emissions has unfortunately not been looked into so seriously, as the current stress of all automobile manufacturers is to meet the tailpipe emission legislative limits.A numerical model has been developed using finite element methods for studying the oil jet cooling of pistons and has been validated experimentally on a flat plate cooled by oil jet. Using numerical modelling, the heat transfer coefficient (h) at the underside of the piston is predicted. This predicted value of heat transfer coefficient significantly helps in selecting the correct oil type, oil jet velocity, oil jet diameter, and distance of oil nozzle from the underside of the piston. It also helps to predict whether the selected grade of oil will contribute to mist generation. Isotherms of the predicted temperature profiles in a production grade piston have been plotted.},
author = {Agarwal, A K and Varghese, M B},
doi = {10.1243/14680874JER01804},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/W{\"{a}}rme-RBen Kolben/2004{\_}Varghese{\_}Numerical investigation of piston cooling using oil jet.pdf:pdf},
issn = {1468-0874},
journal = {Int. J. Engine Res.},
number = {5},
pages = {411--421},
title = {{Numerical investigations of piston cooling using oil jet in heavy duty diesel engines}},
url = {http://journals.sagepub.com/doi/10.1243/14680874JER01804},
volume = {7},
year = {2006}
}
@article{Sauzay2000,
author = {Sauzay, M. and Gilormini, P.},
doi = {10.1046/j.1460-2695.2000.00307.x},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2000{\_}Sauzay{\_}Surface and cyclic microplasticity{\_}SurfaceAndPlasticityInMicro.pdf:pdf},
issn = {8756758X},
journal = {Fatigue Fract. Eng. Mater. Struct.},
keywords = {crystallographic glide,fatigue,free surface,microplasticity},
number = {7},
pages = {573--579},
title = {{Surface and cyclic microplasticity}},
volume = {23},
year = {2000}
}
@article{Block2010,
author = {Block, Katharina},
number = {April},
pages = {2--5},
title = {{Green ' sche Funktionen als Hilfsmittel zur Konstruktion klassischer L{\{}{\"{o}}{\}}sungen von partiellen Di erentialgleichungen 2 Mathematische Grundlagen}},
volume = {0},
year = {2010}
}
@article{Schwartz1997,
author = {Schwartz, Mel M},
doi = {10.1177/0892705712453152},
isbn = {0444888527},
issn = {21554854},
pages = {43--44},
title = {{Composite Materials}},
year = {1997}
}
@article{Papula2009a,
author = {Papula, Lothar},
journal = {Math. Formelsammlung},
pages = {174--190},
title = {{Unendliche Reihen, Taylor- und Fourier-Reihen 1}},
year = {2009}
}
@article{Sauzay2002a,
author = {Sauzay, M and Gilormini, P},
doi = {10.1016/S0167-8442(02)00080-0},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/2002{\_}Sauzay + Gilmormini{\_}Influence of surface effects on fatigue of microcracks nucleation.pdf:pdf},
issn = {01678442},
journal = {Evaluation},
keywords = {crack nucleation,cyclic plasticity,fatigue,persistent slip band,surface},
pages = {53--62},
title = {{Influence of surface effects on fatigue of microcracks nucleation}},
volume = {38},
year = {2002}
}
@article{Roentgenium2006,
author = {Roentgenium, Rg and Conrad, Wilhelm},
journal = {Gerthsen Phys.},
pages = {847--882},
title = {{16 - Die Elemente und die Chemie}},
year = {2006}
}
@article{Moscatelli2017,
author = {Moscatelli, D and Sponchioni, M},
doi = {10.1016/B978-0-08-100262-9.00012-4},
isbn = {9780081002629},
title = {12 12.1},
year = {2017}
}
@article{Formeln,
author = {Formeln, Binomische},
pages = {1--49},
title = {{Arithmetik 1 1 Arithmetik}}
}
@article{Thorium,
author = {Thorium, Elemente},
doi = {10.1007/978-3-8348-2279-6},
isbn = {9783834822796},
journal = {Arbeit},
pages = {326--341},
title = {{15 Geothermie}}
}
@article{Eigenschaften1903,
author = {Eigenschaften, Diese and Thermodynamik, Die},
doi = {10.1007/978-3-642-24161-1},
isbn = {9783642241611},
journal = {Society},
title = {{4 Die thermodynamischen Eigenschaften reiner Fluide}},
year = {1903}
}
@book{ErogluS.ToprakS.UrganOMDOzgeE.OnurMDArzuDenizbasiMDHaldunAkogluMDCigdemOzpolatMDEbruAkoglu2012,
abstract = {The objective of this case study was to obtain some first-hand information about the functional consequences of a cosmetic tongue split operation for speech and tongue motility. One male patient who had performed the operation on himself was interviewed and underwent a tongue motility assessment, as well as an ultrasound examination. Tongue motility was mildly reduced as a result of tissue scarring. Speech was rated to be fully intelligible and highly acceptable by 4 raters, although 2 raters noticed slight distortions of the sibilants /s/ and /z/. The 3-dimensional ultrasound demonstrated that the synergy of the 2 sides of the tongue was preserved. A notably deep posterior genioglossus furrow indicated compensation for the reduced length of the tongue blade. It is concluded that the tongue split procedure did not significantly affect the participant's speech intelligibility and tongue motility.},
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {{Eroglu S., Toprak S., Urgan O, MD, Ozge E. Onur, MD, Arzu Denizbasi, MD, Haldun Akoglu, MD, Cigdem Ozpolat, MD, Ebru Akoglu}, Md},
booktitle = {Saudi Med J},
doi = {10.1073/pnas.0703993104},
eprint = {arXiv:1011.1669v3},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Itskov 2007 - Tensor Algebra and Tensor Analysis for Engineers.pdf:pdf},
isbn = {9781604138795},
issn = {1098-6596},
keywords = {emergency,luation of non-urgent visits,to a busy urban},
pages = {3--8},
pmid = {25246403},
title = {{Tensor Algebra and Tensor Analysis for Engineers}},
volume = {33},
year = {2012}
}
@article{Doquet1997,
abstract = {The development of fatigue damage in Co45Ni specimens during push-pull and reversed torsion tests, performed inside a scanning electron microscope, was observed and the different stress states compared. It appeared that transgranular crack initiation and development is delayed and intergranular crack initiation promoted under torsional loading. This was explained in terms of reduced surface distortion at the emergence of persistent slip bands (PSBs) and smaller compatibility stresses at the PSB-matrix interfaces. The influence of the mechanical strength of grain boundaries on the difference between tensile and torsional fatigue lives is discussed.},
author = {Doquet, V.},
doi = {10.1111/j.1460-2695.1997.tb00280.x},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/1996{\_}Doquet{\_}CRACK INITIATION MECHANISMS IN TORSIONAL FATIGUE.pdf:pdf},
issn = {8756758X},
journal = {Fatigue Fract. Eng. Mater. Struct.},
keywords = {-torsional fatigue,intergranular crack initiation},
number = {2},
pages = {227--235},
title = {{Crack Initiation Mechanisms in Torsional Fatigue}},
url = {http://doi.wiley.com/10.1111/j.1460-2695.1997.tb00280.x},
volume = {20},
year = {1997}
}
@book{Cherkaoui2009h,
author = {Cherkaoui, Mohammed and Capolungo, Laurent},
doi = {10.1007/978-0-387-46771-9},
isbn = {978-0-387-46765-8},
title = {{Atomistic and Continuum Modeling of Nanocrystalline Materials}},
url = {http://link.springer.com/10.1007/978-0-387-46771-9},
volume = {112},
year = {2009}
}
@book{Gross2011d,
author = {Gross, Dietmar and Seelig, Thomas},
doi = {10.1007/978-3-642-10196-0},
isbn = {978-3-642-10195-3},
title = {{Bruchmechanik}},
url = {http://link.springer.com/10.1007/978-3-642-10196-0},
year = {2011}
}
@article{Morris1980,
author = {Morris, W L},
doi = {10.1007/BF02668135},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/1980{\_}Morris{\_}The noncontinuum crack tip defo behavior of surface microcracks.pdf:pdf},
issn = {03602133},
journal = {Met. Trans. A},
number = {7},
pages = {1117--1123},
title = {{The noncontinuum crack tip deformation behavior of surface microcracks}},
volume = {11},
year = {1980}
}
@article{Palin-Luc1998a,
abstract = {In spite of the great number of high cycle multiaxial fatigue criteria in the literature, none predicts the difference that exists between the endurance limits in traction, four point rotative bending and four point plane bending. An energy based criterion based on a new concept using the strain energy density is proposed in this paper. This new calculation method explains the previous differences by taking into account the volumic distribution of the strain energy density around the considered critical point in fatigue. This method, available now under fully reversed multiaxial loadings, also takes into account the stress state triaxiality. Under combined plane bending and torsion the predictions of the new proposal lead to Gough and Pollard's ellipse quadrant for ductile materials and lead to a curve close to an ellipse are for brittle materials. Under other multiaxial loadings, predictions are always close to an ellipse quadrant dependent on the loading mode. This method has been tested on smooth cylindrical specimens with several materials; calculations are in very good agreement with multiaxial experimental data.},
author = {Palin-Luc, Thierry and Lasserre, Serge},
doi = {10.1016/S0997-7538(98)80084-3},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Empirical Fatigue Models + Validation/Energy based models/A energy based criterion for high  cycle multiaxial fatigue.pdf:pdf},
issn = {09977538},
journal = {Eur. J. Mech. - A/Solids},
number = {2},
pages = {237--251},
title = {{An energy based criterion for high cycle multiaxial fatigue}},
volume = {17},
year = {1998}
}
@article{V.Winterfeldt,
author = {V.Winterfeldt, J. Schade},
journal = {H{\"{u}}tte},
pages = {1--21},
title = {{Q-Patente}}
}
@article{Foreste,
author = {Forest, Samuel},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/Folien CISM Summer School Mai2017 - Mesoscale Models/courses{\_}C1703{\_}forest{\_}Forest1-Micromorphic.pdf:pdf},
title = {{Micromorphic media}}
}
@article{Loubar2005a,
abstract = {This paper deals with the transient thermal signal around an engine cylinder in order to propose a new and nonintrusive method of knock detection. Numerical simulations of unsteady heat transfer through the cylinder and inside the coolant flow are carried out to account for heat flux variations due to normal and knocking combustion. The effect of rib roughened surfaces on thermal signal amplification is investigated. The geometric parameters are fixed at Pi/h=70 and w/h=1 with a Reynolds number based on hydraulic diameter of 12,000. The results reveal that square ribs give better performance in term of thermal signal amplification within the fluid. An amplification of the temperature variation up to 20 times higher is found. Finally, flow analysis shows that amplification depends on the position where the thermal signal is collected.},
author = {Loubar, Khaled and Bellettre, Jérôme and Tazerout, Mohand},
doi = {10.1115/1.1857943},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2005{\_}Loubar{\_}Unsteady Heat Transfer enhancement around an engine cylinder in order to detect knockpdf.pdf:pdf},
isbn = {0022-1481},
issn = {00221481},
journal = {J. Heat Transf.},
number = {3},
pages = {278},
title = {{Unsteady Heat Transfer Enhancement Around an Engine Cylinder in Order to Detect Knock}},
url = {http://heattransfer.asmedigitalcollection.asme.org/article.aspx?articleid=1447711},
volume = {127},
year = {2005}
}
@article{Chen2014,
abstract = {A predictive knock model is crucial for one dimensional (1-D) engine cycle simulation that has been proven to be a powerful tool in both optimization of the conceptual design and reduction of calibration efforts in development of spark-ignition (SI) engines. With application of advanced technologies such as exhaust gas recirculation (EGR) in modern SI engines, update of knock model is needed to give an acceptable prediction of knock onset. In this study, bench tests of a turbocharged gasoline SI engine with cooled EGR system operated under knocking conditions were conducted, the cylinder pressure traces were analyzed by the band-pass filtering technique, and the crank angle of knock onset was determined by the signal energy ratio (SER) and image processing method. A knock model considering multi-variable effects including pressure, temperature, EGR ratio and excess air ratio (??) is formulated and calibrated with the experimental data using the multi-island genetic algorithm (GA). The calculation method of the end gas temperature, the impacts of the ratio of specific heats as well as the temperature at the intake valve closure on the end gas temperature are discussed. The performance of the new model is compared with the widely-used phenomenological knock models such as Douaud-Eyzat model and Hoepke model. While the widely-used knock models fail to give acceptable predictions when increasing EGR with fuel enrichment operations, the new model predicts the knock onset with high accuracy under the fuel enrichment conditions both with and without EGR. Performance of the newly developed model is also examined in a different engine and a higher predictive accuracy of the new model than other models is obtained. ?? 2014 Elsevier Ltd. All rights reserved.},
author = {Chen, Longhua and Li, Tie and Yin, Tao and Zheng, Bin},
doi = {10.1016/j.enconman.2014.08.002},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2014{\_}Chen+Li{\_}A predictive model for knock onset in spark-ignition engines with cooled EGR.pdf:pdf},
issn = {01968904},
journal = {Energy Convers. Manag.},
keywords = {Excess air ratio,Exhaust gas recirculation,Knock modeling,Knock onset,Spark ignition engines},
pages = {946--955},
publisher = {Elsevier Ltd},
title = {{A predictive model for knock onset in spark-ignition engines with cooled EGR}},
url = {http://dx.doi.org/10.1016/j.enconman.2014.08.002},
volume = {87},
year = {2014}
}
@article{2012,
author = {Ε{\$}\pi{\$}{\$}\iota{\$}{\$}\tau{\$}{\$}\rho{\$}ο{\$}\pi{\$}ά{\$}\kappa{\$}{\$}\eta{\$}ς, Ι},
title = {{Χ{\$}\alpha{\$}{\$}\rho{\$}{\$}\alpha{\$}{\$}\kappa{\$}{\$}\tau{\$}{\$}\eta{\$}{\$}\rho{\$}{\$}\iota{\$}{\$}\sigma{\$}{\$}\mu{\$}ός {\$}\Sigma{\$}ύ{\$}\nu{\$}{\$}\theta{\$}{\$}\epsilon{\$}{\$}\tau{\$}{\$}\omega{\$}{\$}\nu{\$} {\$}\Upsilon{\$}{\$}\lambda{\$}{\$}\iota{\$}{\$}\kappa{\$}ώ{\$}\nu{\$} Α{\$}\nu{\$}{\$}\theta{\$}{\$}\rho{\$}{\$}\alpha{\$}{\$}\kappa{\$}ο{\$}\nu{\$}{\$}\eta{\$}{\$}\mu{\$}ά{\$}\tau{\$}{\$}\omega{\$}{\$}\nu{\$} Κ{\$}\alpha{\$}{\$}\tau{\$}{\$}\alpha{\$}{\$}\sigma{\$}{\$}\kappa{\$}{\$}\epsilon{\$}{\$}\upsilon{\$}{\$}\alpha{\$}{\$}\sigma{\$}{\$}\mu{\$}έ{\$}\nu{\$}{\$}\omega{\$}{\$}\nu{\$} Μ{\$}\epsilon{\$} Τ{\$}\eta{\$} Μέ{\$}\theta{\$}ο{\$}\delta{\$}ο {\$}\Pi{\$}{\$}\epsilon{\$}{\$}\rho{\$}{\$}\iota{\$}έ{\$}\lambda{\$}{\$}\iota{\$}{\$}\xi{\$}{\$}\eta{\$}ς Τ{\$}\omega{\$}{\$}\nu{\$} Ι{\$}\nu{\$}ώ{\$}\nu{\$} (Filament Winding)}},
year = {2012}
}
@article{Stab,
author = {Stab, Torsionswinkel and Biegung, Balken and Biegesteifigkeit, Biegemoment and Verbundbedingung, Biegespannung},
doi = {10.1007/978-3-642-19984-4},
isbn = {9783642199844},
title = {{Ucke}}
}
@article{Chang2004d,
abstract = {An experimental study has been carried out to provide qualitative and quantitative insight into gas to wall heat transfer in a gasoline fueled Homogeneous Charge Compression Ignition (HCCI) engine. Fast response thermocouples are embedded in the piston top and cylinder head surface to measure instantaneous wall temperature and heat flux. Heat flux measurements obtained at multiple locations show small spatial variations, thus confirming relative uniformity of incylinder conditions in a HCCI engine operating with premixed charge. Consequently, the spatially-averaged heat flux represents well the global heat transfer from the gas to the combustion chamber walls in the premixed HCCI engine, as confirmed through the gross heat release analysis. Heat flux measurements were used for assessing several existing heat transfer correlations. One of the most popular models, the Woschni expression, was shown to be inadequate for the HCCI engine. The problem is traced back to the flame propagation term which is not appropriate for the HCCI combustion. Subsequently, a modified model is proposed which significantly improves the prediction of heat transfer in a gasoline HCCI engine and shows very good agreement over a range of conditions},
author = {Chang, Junseok and G{\"{u}}ralp, Orgun and Filipi, Zoran and Assanis, Dennis N. and Kuo, Tang-Wei and Najt, Paul and Rask, Rod},
doi = {10.4271/2004-01-2996},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Heat Transfer Combustion Chamber/2004{\_}Chang{\_}New Heat Transfer Correlation for an HCCI Engine Derived from Measurements of Instantaneous Surface Heat Flux.pdf:pdf},
isbn = {0148-7191},
issn = {0148-7191},
number = {724},
title = {{New Heat Transfer Correlation for an HCCI Engine Derived from Measurements of Instantaneous Surface Heat Flux}},
url = {http://papers.sae.org/2004-01-2996/},
year = {2004}
}
@article{Wirsching1983a,
abstract = {Two methods are discussed for constructing a design curve on the safe side of fatigue data. Both the tolerance interval and equivalent prediction interval (EPI) concepts provide such a curve while accounting for both the distribution of the estimators in small samples and the data scatter. The EPI is also useful as a mechanism for providing necessary statistics on S-N data for a full reliability analysis which includes uncertainty in all fatigue design factors. Examples of statistical analyses of the general strain life relationship are presented. The tolerance limit and EPI techniques for defining a design curve are demonstrated. Examples usng WASPALOY B and RQC-100 data demonstrate that a reliability model could be constructed by considering the fatigue strength and fatigue ductility coefficients as two independent random variables. A technique given for establishing the fatigue strength for high cycle lives relies on an extrapolation technique and also accounts for "runners." A reliability model or design value can be specified.},
author = {Wirsching, P H},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Probabilistic Aspects/1983{\_}Wirsching{\_}Statistical summaries of fatigue data for design purposes.pdf:pdf},
issn = {05657059},
journal = {Nasa Cr 3697},
number = {July},
title = {{Statistical Summaries of Fatigue Data for Design Purposes}},
year = {1983}
}
@article{Wang2016,
abstract = {Cracks encountered in engineering structures are typically three dimensional, and the fracture mechanism remains unclear because of the superimposed stresses induced by mixed-mode I/II/III loading. This paper introduces a general 3D mixed-mode fracture criterion based on the maximum mean principal stress (MMPS) by introducing the concept of a characteristic fracture length that is related to the material tensile strength. This criterion has clear physical significance, a systematic mathematical expression and a wide scope of applications to estimate both the in- and out-of-plane fracture angles and fracture strength. The proposed criterion is validated for all mixed-mode conditions (I/II, I/III and II/III) and is compared with several widely used criteria based on experimental results reported in previous studies. Good agreement is achieved in terms of the fracture angles and, in particular, the fracture strength between the results predicted by the new criterion and the experimental results of various brittle materials.},
author = {Wang, J and Ren, L and Xie, L Z and Xie, H P and Ai, T},
doi = {10.1016/j.ijsolstr.2016.10.009},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/2016{\_}Wang{\_}Maximum mean principal stress criterion for 3D brittle fracture.pdf:pdf},
issn = {00207683},
journal = {Int. J. Solids Struct.},
keywords = {3D fracture criterion,Characteristic fracture length,Mean stress,Mixed-mode loading},
pages = {142--154},
title = {{Maximum mean principal stress criterion for three-dimensional brittle fracture}},
volume = {102-103},
year = {2016}
}
@article{Betriebsfestigkeita,
author = {Betriebsfestigkeit, Problemstellung Der},
pages = {1--19},
title = {{1 Einf{\{}{\"{u}}{\}}hrung und {\{}{\"{U}}{\}}bersicht}}
}
@article{Sietsmaa,
author = {Sietsma, J},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/Hardening Recovery Creep/KocksMecking{\_}Annihilation of dislocation in plastic deformation.pdf:pdf},
pages = {1--24},
title = {{Dislocation annihilation in plastic deformation}}
}
@article{Werkstoffe,
author = {Werkstoffe, Bedeutung Der},
title = {{Werkstoffe und ihre Auswahl}}
}
@article{Tarnopolskii1998,
author = {Tarnopol'skii, Yu.M. and Kulakov, V.L.},
isbn = {0-412-54020-7},
journal = {Handb. Compos.},
pages = {778--793},
title = {{Mechanical tests}},
year = {1998}
}
@article{Entwicklung,
author = {Entwicklung, Geschichtliche},
pages = {534--537},
title = {{Index}}
}
@article{Anwendungen,
author = {Anwendungen, Bei and Fahrer, Der and Kraftfahrzeug, Systems},
pages = {211--226},
title = {{13 Fahrzeugtechnik}}
}
@article{Gaborit2015,
abstract = {The aim of this work is to develop a lifetime prediction model based oncontinuum damage mechanics that can unify the Low Cycle Fatigue (LCF) and HighCycle Fatigue (HCF) domains. The concept of an inclusion embedded in a matrix isused to describe the fact that plasticity is no more observable when the load is belowthe yield stress. A review of the localization rules used in the literature for damagemodeling is done and two new ones have been proposed. A numerical implementationallows us to calculate the responses of the inclusions for the different localization rules.Some calculations are presented under cyclic loadings.},
author = {Gaborit, P and Desmorat, R and du Tertre, A and Pyre, A},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/Localization rules for the extension of a HCF two-scale damage model to a Lemaitre LCF damage model {\_} Desmorat.pdf:pdf},
journal = {Icmff10},
title = {{Localization rules for the extension of a HCF two-scale damage model to a Lemaitre LCF damage model}},
url = {http://www.gruppofrattura.it/ocs/index.php/ICMFF/ICMFF10/paper/view/12106},
year = {2015}
}
@article{Frage2007,
author = {Frage, Die and Wirkungen, Den and Hilfen, Den},
doi = {10.1007/978-3-531-19320-5},
isbn = {9783531193199},
journal = {Arbeit},
pages = {17--20},
title = {{1 Einleitung}},
year = {2007}
}
@article{Palin-Luc1998a,
abstract = {In spite of the great number of high cycle multiaxial fatigue criteria in the literature, none predicts the difference that exists between the endurance limits in traction, four point rotative bending and four point plane bending. An energy based criterion based on a new concept using the strain energy density is proposed in this paper. This new calculation method explains the previous differences by taking into account the volumic distribution of the strain energy density around the considered critical point in fatigue. This method, available now under fully reversed multiaxial loadings, also takes into account the stress state triaxiality. Under combined plane bending and torsion the predictions of the new proposal lead to Gough and Pollard's ellipse quadrant for ductile materials and lead to a curve close to an ellipse are for brittle materials. Under other multiaxial loadings, predictions are always close to an ellipse quadrant dependent on the loading mode. This method has been tested on smooth cylindrical specimens with several materials; calculations are in very good agreement with multiaxial experimental data.},
author = {Palin-Luc, Thierry and Lasserre, Serge},
doi = {10.1016/S0997-7538(98)80084-3},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Empirical Fatigue Models + Validation/Energy based models/A energy based criterion for high  cycle multiaxial fatigue.pdf:pdf},
issn = {09977538},
journal = {Eur. J. Mech. - A/Solids},
number = {2},
pages = {237--251},
title = {{An energy based criterion for high cycle multiaxial fatigue}},
volume = {17},
year = {1998}
}
@article{Geometrie,
author = {Geometrie, Die and Innendurchmesser, Der},
title = {{3 Geometrie und Tragf{\"{a}}higkeit}}
}
@book{ErogluS.ToprakS.UrganOMDOzgeE.OnurMDArzuDenizbasiMDHaldunAkogluMDCigdemOzpolatMDEbruAkoglu2012,
abstract = {The objective of this case study was to obtain some first-hand information about the functional consequences of a cosmetic tongue split operation for speech and tongue motility. One male patient who had performed the operation on himself was interviewed and underwent a tongue motility assessment, as well as an ultrasound examination. Tongue motility was mildly reduced as a result of tissue scarring. Speech was rated to be fully intelligible and highly acceptable by 4 raters, although 2 raters noticed slight distortions of the sibilants /s/ and /z/. The 3-dimensional ultrasound demonstrated that the synergy of the 2 sides of the tongue was preserved. A notably deep posterior genioglossus furrow indicated compensation for the reduced length of the tongue blade. It is concluded that the tongue split procedure did not significantly affect the participant's speech intelligibility and tongue motility.},
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {{Eroglu S., Toprak S., Urgan O, MD, Ozge E. Onur, MD, Arzu Denizbasi, MD, Haldun Akoglu, MD, Cigdem Ozpolat, MD, Ebru Akoglu}, Md},
booktitle = {Saudi Med J},
doi = {10.1073/pnas.0703993104},
eprint = {arXiv:1011.1669v3},
isbn = {9781604138795},
issn = {1098-6596},
keywords = {emergency,luation of non-urgent visits,to a busy urban},
pages = {3--8},
pmid = {25246403},
title = {{Tensor Algebra and Tensor Analysis for Engineers}},
volume = {33},
year = {2012}
}
@book{Gross2011i,
author = {Gross, Dietmar and Seelig, Thomas},
doi = {10.1007/978-3-642-10196-0},
isbn = {978-3-642-10195-3},
title = {{Bruchmechanik}},
url = {http://link.springer.com/10.1007/978-3-642-10196-0},
year = {2011}
}
@book{Elshahawy2008,
author = {Elshahawy, Waleed},
isbn = {0120020211},
title = {{Advances i}},
year = {2008}
}
@article{Fatemi1998,
abstract = {Fatigue damage increases with applied load cycles in a cumulative manner. Cumulative fatigue damage analysis plays a key role in life prediction of components and structures subjected to field load histories. Since the introduction of damage accumulation concept by Palmgren about 70 years ago and 'linear damage rule' by Miner about 50 years ago, the treatment of cumulative fatigue damage has received increasingly more attention. As a result, many damage models have been developed. Even though early theories on cumulative fatigue damage have been reviewed by several researchers, no comprehensive report has appeared recently to review the considerable efforts made since the late 1970s. This article provides a comprehensive review of cumulative fatigue damage theories for metals and their alloys, emphasizing the approaches developed between the early 1970s to the early 1990s. These theories are grouped into six categories: linear damage rules; nonlinear damage curve and two-stage linearization approaches; life curve modification methods; approaches based on crack growth concepts; continuum damage mechanics models; and energy-based theories. {\textcopyright}},
author = {Fatemi, A. and Yang, L.},
doi = {10.1016/S0142-1123(97)00081-9},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/1997{\_}Fatemi{\_}Cumulative fatigue damage and life prdeiction theories-a survey of the state of the art for homogeneous materials.pdf:pdf},
isbn = {0142-1123},
issn = {01421123},
journal = {Int. J. Fatigue},
keywords = {cumulative damage rules,cumulative fatigue damage,fatigue damage accumulation,fatigue life predictions,load interac-,tion effects},
number = {1},
pages = {9--34},
title = {{Cumulative fatigue damage and life prediction theories: a survey of the state of the art for homogeneous materials}},
url = {http://linkinghub.elsevier.com/retrieve/pii/S0142112397000819},
volume = {20},
year = {1998}
}
@article{Kapitele,
author = {Kapitel, Dieses and Zeitsignale, Derartige and Faltung, Die and Erinnerung, Zur and Entwicklung, Potenzreihen-},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Mathematik/Fourier Faltung Overview{\_}ETHZ.pdf:pdf},
title = {{Fourier-Transformation 6.1}}
}
@article{Starten,
author = {Starten, Das},
title = {{Start- und Z{\"{u}}ndhilfesysteme}}
}
@article{Buryachenko1995a,
abstract = {We consider a linearly elastic composite medium, which consists of a homogeneous matrix containing a homogeneous and statistically uniform random set of ellipsoidal inclusions. Because of the differential thermal expansion, a microstructural residual stress state arises. By means of the "multiparticle effective field" method we first derive the functional relation between the stored elastic energy and the thermoelastic constants of the components. Using this result an exact estimation of all components of the statistical second moment tensor of the stress fields is given. Furthermore, an expression for the second moment of the stress in the matrix in the vicinity of the ellipsoidal inclusion and a correlation function of internal stresses is obtained. The application of the theory is demonstrated by some numerical results for a WC-Co composite. ?? 1995.},
author = {Buryachenko, Valeriy A. and Kreher, Wolfgang S.},
doi = {10.1016/0022-5096(95)00029-I},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Probabilistic Aspects/1995{\_}Kreher{\_}Internal residual stresses in heterogeneous solids - a statistical theory for particulate composites.pdf:pdf},
isbn = {0022-5096},
issn = {00225096},
journal = {J. Mech. Phys. Solids},
number = {7},
pages = {1105--1125},
title = {{Internal residual stresses in heterogeneous solids-A statistical theory for particulate composites}},
volume = {43},
year = {1995}
}
@article{Grandin2002a,
abstract = {Heat transfer to the walls of the combustion chamber is increased by engine knock. In this study the influence of knock onset and knock intensity on the heat flux is investigated by examining over 10 000 individual engine cycles with a varying degree of knock. The heat transfer to the walls was estimated by measuring the combustion chamber wall temperature in an SI engine under knocking conditions. The influence of the air-fuel ratio and the orientation of the oscillating cylinder pressure-relative to the combustion chamber wall-were also investigated.It was found that knock intensities above 0.2 Mpa influenced the heat flux. At knock intensities above 0.6 Mpa, the peak heat flux was 2.5 times higher than for a non-knocking cycle. The direction of the oscillations did not affect the heat transfer.ER -},
author = {Grandin, B{\"{o}}rje and Denbratt, Ingemar},
doi = {10.4271/2002-01-0238},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Klopfen{\_}Ottomotor/2002{\_}Grandin{\_}The Effect of Knock on Heat Transfer in SI Engines-Experimental Results.pdf:pdf},
journal = {Sae Tech. Pap. Ser.},
number = {724},
title = {{The Effect of Knock on Heat Transfer in SI Engines}},
url = {http://papers.sae.org/2002-01-0238},
year = {2002}
}
@article{Taylor--galerkin,
author = {Taylor--galerkin, E The},
journal = {Order A J. Theory Ordered Sets Its Appl.},
title = {{Convection--diffusion equations : vector-valued variables and differentiating}}
}
@article{Reihen,
author = {Reihen, Unendliche and Vi-, Þ and Vi-, Þ},
pages = {570--639},
title = {{VI Potenzreihenentwicklungen}}
}
@article{Torrilhon2007,
author = {Torrilhon, Manuel},
doi = {10.1002/theDOIsuffix},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Thermodynamik/PhasenFeld/Nestler{\_}Crack{\_}propagation{\_}on{\_}mesoscopic{\_}length{\_}scale.pdf:pdf},
journal = {Pamm},
keywords = {chemo-mechanical coupling,crack propagation,multiphase-field,phase-field},
pages = {1--2},
title = {{Stability of reduced electric arc models}},
url = {http://onlinelibrary.wiley.com/doi/10.1002/pamm.200700318/abstract},
volume = {2},
year = {2007}
}
@article{Bridier2008a,
abstract = {The purpose of this experimental study is to investigate the micromechanical fatigue behavior, in terms of slip nature and preferential cracking sites, of a commercial ??/??-forged Ti-6Al-4V alloy. Electron backscattering diffraction is extensively used to identify the deformation (prismatic, basal, pyramidal slip) and crack formation modes activated by fatigue at the surface of several hundred primary ?? nodules. Some fatal crack formation sites are also characterized. Cracking in basal planes is identified as the most critical damage mode leading to fracture. An explanation is proposed which involves the resolved shear stress, taking into account the Schmid factor and the normal stress in relation to the elastic anisotropy of the ??-phase. Finally, the spatial distribution of the secondary cracks is analyzed according to the crystallographic textures (macrozones) present on a mesoscopic scale in the Ti-6Al-4V alloy. ?? 2008 Acta Materialia Inc.},
author = {Bridier, F. and Villechaise, P. and Mendez, J.},
doi = {10.1016/j.actamat.2008.04.036},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2008{\_}Villechaise{\_}Slip and fatigue crack formation processes in an titanium alloy in relation to crystallographic texture on different scales.pdf:pdf},
isbn = {1359-6454},
issn = {13596454},
journal = {Acta Mater.},
keywords = {Electron backscattering diffraction,Fatigue,Slip,Texture,Titanium alloys},
number = {15},
pages = {3951--3962},
title = {{Slip and fatigue crack formation processes in an ??/?? titanium alloy in relation to crystallographic texture on different scales}},
volume = {56},
year = {2008}
}
@article{Wei1970,
abstract = {Metal fatigue as an engineering problem has been well recognized. Many experiments have been carried out in recent years to assess the effects of load amplitude, mean load, load range and test frequency on the rate of fatigue-crack growth to characterize material response to different load profiles and to develop methods for estimating the service behavior of structural components. Recent studies have shown that fatigue-crack growth can be influenced strongly by the test environment; the effect being dependent on the particular material-environment involved. These results suggest that careful reassessments of the data of previous studies and of the proper direction for future fatigue research will be required. Hence, a critical review and analysis of existing fatigue-crack-growth data on high-strength aluminum and titanium alloys and high-strength steels has been made. The influences of load profile, test frequency, temperature, test environment and state-of-stress on fatigue-crack growth are discussed. Correlation with environment-enhanced crack growth under sustained loads and the associated changes in material response are examined. Possible mechanisms, synergistic effects and implications regarding methods for service-life estimation are considered. ?? 1970.},
author = {Wei, R. P.},
doi = {10.1016/0013-7944(70)90004-4},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/1970{\_}Wei{\_}Some aspects of environment-enhanced fatigue crack growth{\_}For example frequency in Al7075.pdf:pdf},
issn = {00137944},
journal = {Eng. Fract. Mech.},
number = {4},
pages = {633--651},
title = {{Some aspects of environment-enhanced fatigue-crack growth}},
volume = {1},
year = {1970}
}
@article{Fertigung2007,
author = {Fertigung, Wirtschaftliche and Bauteile, Verzahnte and Teile, Sonstige},
journal = {Fahrzeuggetriebe},
title = {{16 Fertigungstechnik von Fahrzeuggetrieben}},
year = {2007}
}
@article{Motorverhalten,
author = {Motorverhalten, Thermisches},
title = {{8 Gesamtprozessanalyse 8.1}}
}
@article{Baehr2010a,
author = {Baehr, H D and Stephan, K},
doi = {10.1007/978-3-642-10194-6},
isbn = {9783642101946},
title = {{Konvektiver W ¨ arme- und Stoff u omungen ¨ bergang . Einphasige Str ¨}},
year = {2010}
}
@book{Davies2008,
abstract = {Texture analysis is one of the fundamental aspects of human vision by which we discriminate between surfaces and objects. In a similar manner, computer vision can take advantage of the cues provided by surface texture to distinguish and recognize objects. In computer vision, texture analysis may be used alone or in combination with other sensed features (e.g. color, shape, or motion) to perform the task of recognition. Either way, it is a feature of paramount importance and boasts a tremendous body of work in terms of both research and applications. Currently, the main approaches to texture analysis must be sought out through a variety of research papers. This collection of chapters brings together in one handy volume the major topics of importance, and categorizes the various techniques into comprehensible concepts. The methods covered will not only be relevant to those working in computer vision, but will also be of benefit to the computer graphics, psychophysics, and pattern recognition communities, academic or industrial.},
author = {Davies, E. R.},
booktitle = {Handb. Texture Anal.},
doi = {interface shear stre},
isbn = {978-1-84816-115-3},
issn = {04515994},
pages = {1--31},
pmid = {15680927},
title = {{Introduction to Texture Analysis}},
year = {2008}
}
@article{Papula2009c,
author = {Papula, Lothar},
doi = {10.1007/978-3-8348-8285-1},
isbn = {9783834882851},
journal = {Math. Formelsammlung},
pages = {308--397},
title = {{Differentialrechnung 1}},
year = {2009}
}
@article{Aslan2011a,
abstract = {Proper life-time prediction modeling of single crystalline components is of increasing importance due to their common use in turbine industry. Viscoplastic damage approaches are of great interest in that context. However, mechanical properties of single crystals are strongly anisotropic and nonlinear in service conditions, bringing certain complexity into constitutive and numerical modeling. The aim of this work is to develop a thermodynamically consistent constitutive model based on generalized continua in order to simulate fatigue crack initiation and growth in single crystals. For that purpose, a standard crystal plasticity model is taken as a basis and coupled with the continuous damage model developed by Marchal et al. (2006a) [Marchal, N., Forest, S., Remy, L. and Duvinage, S. (2006a). Simulation of Fatigue Crack Growth in Single Crystal Superalloys Using Local Approach to Fracture, In: Moinereau, D., Steglich, D. and Besson, J. (eds.), Local Approach to Fracture, 9th European Mechanics of Materials Conference, Euromech–Mechamat, Moret–Sur–Loing, France, Presses de l'Ecole des mines de Paris, pp. 353–358]. As a variant of micromorphic theory, microdamage approach is applied to the model in order to obtain a regularized continuum damage formulation which solves mesh dependency problem by introducing an intrinsic length scale. A detailed finite element implementation procedure and its validation for monotonic crack growth areshown. Fatigue crack growth analyses have been performed on a single edge notched geometry and a comparison between numerical and experimental results is presented.},
author = {Aslan, Ozgur and Quilici, St{\'{e}}phane and Forest, Samuel},
doi = {10.1177/1056789510395738},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/2011{\_}Aslan{\_}Numerical Modeling of Fatigue Crack Growth in Single Crystals Based on micodamage theory.pdf:pdf},
issn = {1056-7895},
journal = {Int. J. Damage Mech.},
number = {5},
pages = {681--705},
title = {{Numerical Modeling of Fatigue Crack Growth in Single Crystals Based on Microdamage Theory}},
url = {http://journals.sagepub.com/doi/10.1177/1056789510395738},
volume = {20},
year = {2011}
}
@article{Ziegler1942,
author = {Ziegler, J.G and Nichols, N.B},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Vorlesungen/Messtechnik+Regelungstechnik/1993{\_}Ziegler+Nichols{\_}Optimum Settings for Automatic Controllers.pdf:pdf},
journal = {Trans. ASME,},
pages = {759--768},
title = {{Optimum settings for automatic controllers}},
volume = {64},
year = {1942}
}
@article{Murakami2012d,
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Murakami, Sumio},
doi = {10.1007/978-94-007-2666-6},
eprint = {arXiv:1011.1669v3},
isbn = {978-94-007-2665-9},
issn = {09250042},
pages = {253--276},
pmid = {25246403},
title = {{Continuum Damage Mechanics}},
url = {http://link.springer.com/10.1007/978-94-007-2666-6},
volume = {185},
year = {2012}
}
@article{Metallplastizit2013c,
author = {Metallplastizit, Hrungdie and Helm, Dirk},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/{\_}skripte/Helm - Prozesssimulation und Umformtechnik/Presentation1{\_}Metallplastizitaet{\_}1.pdf:pdf},
number = {November},
pages = {1--29},
title = {{Prozesssimulation in Der Umformtechnik}},
year = {2013}
}
@article{Grandin2002c,
abstract = {Heat transfer to the walls of the combustion chamber is increased by engine knock. In this study the influence of knock onset and knock intensity on the heat flux is investigated by examining over 10 000 individual engine cycles with a varying degree of knock. The heat transfer to the walls was estimated by measuring the combustion chamber wall temperature in an SI engine under knocking conditions. The influence of the air-fuel ratio and the orientation of the oscillating cylinder pressure-relative to the combustion chamber wall-were also investigated.It was found that knock intensities above 0.2 Mpa influenced the heat flux. At knock intensities above 0.6 Mpa, the peak heat flux was 2.5 times higher than for a non-knocking cycle. The direction of the oscillations did not affect the heat transfer.ER -},
author = {Grandin, B{\"{o}}rje and Denbratt, Ingemar},
doi = {10.4271/2002-01-0238},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Klopfen{\_}Ottomotor/2002{\_}Grandin{\_}The Effect of Knock on Heat Transfer in SI Engines-Experimental Results.pdf:pdf},
journal = {Sae Tech. Pap. Ser.},
number = {724},
title = {{The Effect of Knock on Heat Transfer in SI Engines}},
url = {http://papers.sae.org/2002-01-0238},
year = {2002}
}
@article{Ahnlichkeitstheorie,
author = {Ahnlichkeitstheorie, Die and Ahnlichkeitstheorie, Der},
title = {{¨ 7 Ahnlichkeitstheorie 7.1}}
}
@article{Gasgemischen1801,
author = {Gasgemischen, Teilgr{\"{o}}{\ss}en Von and Gesetz, D Alton},
pages = {155--184},
title = {{8 Ideale Gas- und Gas-Dampf-Gemische}},
year = {1801}
}
@article{Depcik2002a,
abstract = {In this paper, the available correlations proposed in the literature for the gas-side heat transfer in the intake and exhaust system of a spark-ignition internal combustion engine were surveyed. It was noticed that theseAB - {\{}{\textless}{\}}inline-graphic xlink:href="2002-01-0372{\{}{\_}{\}}fig0001" xmlns:xlink="http://www.w3.org/1999/xlink"/{\{}{\textgreater}{\}}AB - only by empirically fitted constants. This similarity provided the impetus for the authors to explore if a universal correlation could be developed. Based on a scaling approach using microscales of turbulence, the authors have fixed the exponential factor on the Reynolds number and thus reduced the number of adjustable coefficients to just one; the latter can be determined from a least squares curve-fit of available experimental data. Using intake and exhaust side data, it was shown that the universal correlationAB - {\{}{\textless}{\}}inline-graphic xlink:href="2002-01-0372{\{}{\_}{\}}fig0002" xmlns:xlink="http://www.w3.org/1999/xlink"/{\{}{\textgreater}{\}}AB - The correlation coefficient of this proposed heat transfer model with all available experimental data is 0.845 for the intake side and 0.800 for the exhaust side.ER -},
author = {Depcik, Christopher and Assanis, Dennis},
doi = {10.4271/2002-01-0372},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2002{\_}Assanis{\_}A Universal Heat Transfer Correlation for Intake and Exhaust flows in an SI INternal Combustion Engine.pdf:pdf},
journal = {SAE Pap.},
number = {January 2016},
title = {{A Universal Heat Transfer Correlation for Intake and Exhaust Flows in an Spark-Ignition Internal Combustion Engine}},
url = {http://papers.sae.org/2002-01-0372},
volume = {2002-01-03},
year = {2002}
}
@misc{Boeffa,
author = {Boeff, Martin and Gutknecht, Florian and Engels, Philipp S and Ma, Anxin},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/2015{\_}Boeff{\_}Formulation of nonlocal damag models based on spectral methods for application to complex micostructures.pdf:pdf},
keywords = {nonlocal damage modelling,plasticity,rve,spectral solver},
title = {{Formulation of nonlocal damage models based on spectral methods for application to complex microstructures}}
}
@article{Verschleißteile,
author = {Verschlei{\ss}teile, Reifen},
title = {{5 Mobilit{\{}{\"{a}}{\}}tsstrategie}}
}
@book{Zaefferer2009,
author = {Zaefferer, Stefan and Wright, Stuart I},
doi = {10.1007/978-0-387-88136-2},
isbn = {978-0-387-88135-5},
pages = {109--122},
title = {{Electron Backscatter Diffraction in Materials Science}},
url = {http://www.springerlink.com/index/10.1007/978-0-387-88136-2},
year = {2009}
}
@article{Zienkiewicz2014,
author = {Zienkiewicz, O.C. and Taylor, R.L. and Nithiarasu, P.},
doi = {10.1016/B978-1-85617-635-4.00007-8},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Zienkiewicz FEM - Vol 3 Fluid Dynamics/63229{\_}07.pdf:pdf},
isbn = {9781856176354},
journal = {Finite Elem. Method Fluid Dyn.},
pages = {225--281},
title = {{Compressible High-Speed Gas Flow}},
url = {http://linkinghub.elsevier.com/retrieve/pii/B9781856176354000078},
year = {2014}
}
@article{Constitutive,
author = {Constitutive, The},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/Advanced Materials and Structures for Extreme Operating Conditions - Skrzypek/Kapitel4 Developing and Implementing Selected.pdf:pdf},
title = {{Developing and Implementing Selected Constitutive Models for Elasto-Plastic-Damage}}
}
@article{Datei,
author = {Datei, Neue},
title = {{3 Computermaus}}
}
@article{Johnson2004a,
author = {Johnson, Ws and Hillberry, Bm},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Probabilistic Aspects/2004{\_}StevenJohnson{\_}Probabilistic Aspects of Life Prediction.pdf:pdf},
journal = {Book},
title = {{Probabilistic aspects of life prediction}},
url = {http://books.google.com/books?hl=en{\&}lr={\&}id=pDtb-CJLVbYC{\&}oi=fnd{\&}pg=PP7{\&}dq=Probabilistic+Aspects+of+Life+Prediction{\&}ots=fII0k-XR1K{\&}sig=qyo{\_}6w{\_}nT7cN1tqI8pird5rUdts},
year = {2004}
}
@article{Getriebelehre,
author = {Getriebelehre, Der},
title = {{3 Kinematische Analyse der Radf{\{}{\"{u}}{\}}hrungen}}
}
@article{Kre2006,
author = {Kre, Der and Gl, Zum and Betrag, Der},
journal = {Gerthsen Phys.},
pages = {71--92},
title = {{02 - Mechanik des starren K{\{}{\"{o}}{\}}rpers}},
year = {2006}
}
@article{John,
author = {John, T K and Berg, Jerome S},
journal = {Design},
title = {{Table rolling of composite tubes}}
}
@inproceedings{Luo2015Temperature,
author = {Luo, Xi and Yu, Xin and Jansons, Marcis},
booktitle = {SAE Tech. Pap. 2005-01-1658},
doi = {10.4271/2015-01-1658.Copyright},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Heat Transfer Combustion Chamber/2015{\_}Luo+Yu{\_}Simultaneous In-Cylinder Surface Temperature Measurements.pdf:pdf},
publisher = {SAE international},
title = {{Simultaneous In-Cylinder Surface Temperature Measurements with Thermocouple , Laser-induced Phosphorescence , and Dual Wavelength Infrared Diagnostic Techniques in an Optical Engine}},
year = {2015}
}
@article{Dampf-kraftwerke,
author = {Dampf-kraftwerke, Gas-},
doi = {10.1007/978-3-8348-2279-6},
isbn = {9783834822796},
pages = {133--150},
title = {{7 Kombinationskraftwerke}}
}
@article{Weertman1956,
abstract = {Polycrystalline samples of high purity aluminium have been tested in a strain rate machine over a wide temperature range. The relationship which exists between the maximum stress, strain rate, and temperature is strain rate = A (stress)4.4exp( — QRT) where A is a constant, R is the gas constant, T is the absolute temperature, Q is an activation energy equal to 36,000 cal/mole. The results are compared with those of Servi and Grant on constant stress creep tests and shown to be almost identical.},
author = {Weertman, J},
doi = {10.1016/0022-5096(56)90031-X},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Kriechen{\_}Spannungsrelaxation/1956{\_}Weertman{\_}Creep of polycrystalline aluminium as determined from strain rate tests.pdf:pdf},
isbn = {0022-5096},
issn = {00225096},
journal = {J. Mech. Phys. Solids},
number = {4},
pages = {230--234},
title = {{Creep of polycrystalline aluminium as determined from strain rate tests}},
url = {http://www.sciencedirect.com/science/article/pii/002250965690031X},
volume = {4},
year = {1956}
}
@article{Leiden1973,
author = {Leiden, Noordhoff International Publishing-},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/1971{\_}Bowles{\_}The role of inclusions in fatigue crack initiation in an aluminum alloy.pdf:pdf},
journal = {Int. J.},
number = {2},
pages = {171--179},
title = {{The role of inclusions in fatigue crack initiation in an alumS ' mum alloy}},
volume = {9},
year = {1973}
}
@article{Agarwal2006a,
abstract = {Thermal loading of diesel engine pistons has increased dramatically in recent years owing to applications of various technologies to meet low emission and high power density requirements. Control of piston temperatures by cooling of these pistons has become one of the determining factors in a successful engine design. The pistons are cooled by oil jets fired at the underside from the crankcase. Any excessive piston temperature rise may lead to engine seizure because of piston warping. However, if the temperature at the underside of the piston, where the oil jet strikes the piston, is above the boiling range of the oil being used, it may contribute to the generation of mist. This mist significantly contributes to the non-tailpipe emissions in the form of unburnt hydrocarbons (UBHCs). The problem of non-tailpipe emissions has unfortunately not been looked into so seriously, as the current stress of all automobile manufacturers is to meet the tailpipe emission legislative limits.A numerical model has been developed using finite element methods for studying the oil jet cooling of pistons and has been validated experimentally on a flat plate cooled by oil jet. Using numerical modelling, the heat transfer coefficient (h) at the underside of the piston is predicted. This predicted value of heat transfer coefficient significantly helps in selecting the correct oil type, oil jet velocity, oil jet diameter, and distance of oil nozzle from the underside of the piston. It also helps to predict whether the selected grade of oil will contribute to mist generation. Isotherms of the predicted temperature profiles in a production grade piston have been plotted.},
author = {Agarwal, A K and Varghese, M B},
doi = {10.1243/14680874JER01804},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/W{\"{a}}rme-RBen Kolben/2004{\_}Varghese{\_}Numerical investigation of piston cooling using oil jet.pdf:pdf},
issn = {1468-0874},
journal = {Int. J. Engine Res.},
number = {5},
pages = {411--421},
title = {{Numerical investigations of piston cooling using oil jet in heavy duty diesel engines}},
url = {http://journals.sagepub.com/doi/10.1243/14680874JER01804},
volume = {7},
year = {2006}
}
@article{Rostampour2015,
abstract = {This investigation deals with the EF7 (TC) engine, a dual fuel engine equipped with a turbocharger system, consequently with a high probability of knock inception. In this study, an operating cycle of the engine was simulated using KIVA-3V code. Some modifications were carried out on the KIVA method of calculating pressure in the intake port in order to simulate turbocharger pressure correctly. Auto-ignition and knock were then simulated using the auto-ignition integral model. The modified code and the simulation were verified using three different methods; in-cylinder average pressure, gas temperature of the exhaust port, and auto-ignition timing. The simulation results using the auto-ignition integral model, as compared with the experimental data, proved to be reasonably accurate. Following this validation, the effect of the knock phenomenon on the engine heat transfer through the walls was investigated. The simulations showed that the rate of heat transfer through the walls under knocking conditions is about 2.2 times higher than that under normal conditions. However, it was also shown that the total heat transfer increases about 15{\%}.},
author = {Rostampour, Arman and Toosi, Ali Nassiri},
doi = {10.1115/1.4030517},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2015{\_}Rostampour{\_}Numerical Investigation of the effect of knock on heat transfer in a turbo si engine.pdf:pdf},
issn = {0742-4795},
journal = {J. Eng. Gas Turbines Power},
number = {12},
pages = {121502},
title = {{Numerical Investigation of the Effect of Knock on Heat Transfer in a Turbocharged Spark Ignition Engine}},
url = {http://www.scopus.com/inward/record.url?eid=2-s2.0-84930634240{\&}partnerID=tZOtx3y1},
volume = {137},
year = {2015}
}
@article{Methodology,
author = {Methodology, Simulation and Gradation, Properties},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/Advanced Materials and Structures for Extreme Operating Conditions - Skrzypek/Kapitel5 Developing and Implementing Constitutive.pdf:pdf},
journal = {Order A J. Theory Ordered Sets Its Appl.},
title = {{Developing and Implementing Constitutive Models for Specific FGM Applications}}
}
@article{Isermann2006,
author = {Isermann, Rolf},
doi = {10.1007/978-3-8348-9049-8_18},
isbn = {978-3-8348-0109-8},
journal = {Fahrdynamik-Regelung},
pages = {377--406},
title = {{Modellgest{\{}{\"{u}}{\}}tzte {\{}{\"{U}}{\}}berwachung und Fehlerdiagnose f{\{}{\"{u}}{\}}r Kraftfahrzeuge}},
year = {2006}
}
@article{Wang1985a,
author = {Wang, C S and Berry, G F},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/1985{\_}Wang{\_}Heat Transfer in Internal Combustion Engines.pdf:pdf},
journal = {Asme},
number = {Ic},
pages = {1--7},
title = {{Heat Transfer in Internal Combustion Engines}},
year = {1985}
}
@article{Kratzsch2013,
author = {Kratzsch, Matthias and G{\"{u}}nther, Michael},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Klopfen{\_}Ottomotor/4. Internationale Tagung Ottomotorisches Klopfen - Berlin 12{\_}2013/Knocking+in+Gasoline+Engines.pdf:pdf},
pages = {445},
title = {{Knocking in Gasoline Engines}},
year = {2013}
}
@article{Lenkung,
author = {Lenkung, Die and Verfahren, Beide and Im, Fahrzeuglenkung and Lan-, Kutschwagenbauer},
title = {{8 Die Lenkung}}
}
@book{Niemann2005,
abstract = {Konstruktion und Berechnung von Verbindungen, Lagern,Wellen},
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Niemann, G. and Winter, H. and H{\"{o}}hn, B. R.},
booktitle = {New York},
eprint = {arXiv:1011.1669v3},
isbn = {3540251251},
issn = {1098-6596},
pages = {244--270, 368--459, 569--630, 738--777},
pmid = {25246403},
title = {{Maschinenelemente Band 1}},
year = {2005}
}
@article{Quation2003,
author = {Quation, F Inite Lement E},
title = {{By the}},
volume = {2},
year = {2003}
}
@article{Oo1962,
author = {Oчирoв, У У},
journal = {Записки Калмыцкого Научно-Исследовательского Института Языка, Литературы И Истории},
pages = {167--192},
title = {{Придатoчныe Прeдлo{\{}{\v{z}}{\}}eния Врeмeни}},
volume = {Выпуск 2},
year = {1962}
}
@article{Silitonga2013a,
abstract = {Engineering methods to predict the fatigue life of structures have been available since the beginning of the 20th century. However, a practical problem arises from complex loading conditions and a significant concern is the accuracy of the methods under variable amplitude loading. This paper provides an overview of existing fatigue damage models with emphasis on relatively new alternative models and computational strategies to predict fatigue life. These models are compared and promising new capabilities are discussed.},
author = {Silitonga, S. and Maljaars, J. and Soetens, F. and Snijder, H. H.},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/2013{\_} Silitonga{\_}Maljaars{\_}Soetens{\_}Snijder{\_}Survey on damage mechanics models for fatique life prediction.pdf:pdf},
issn = {15744078},
journal = {Heron},
keywords = {Cohesive zone,Continuum damage mechanics,Fatigue damage},
number = {1},
pages = {25--60},
title = {{Survey on damage mechanics models for fatigue life prediction}},
volume = {58},
year = {2013}
}
@book{Streicher-abel,
author = {Streicher-abel, Christian Demant Bernd},
booktitle = {Media},
doi = {10.1007/s10531-008-9469-2},
isbn = {9783642130960},
title = {{1 C}}
}
@article{Beanspruchungsablauf,
author = {Beanspruchungsablauf, Der},
title = {{5 Betriebsfestigkeit 5.1}}
}
@article{Materialerma,
author = {Materialerm, Unter and Anrisse, Schwingspielzahl and Risse, Die and Gefahr, Die},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Empirical Fatigue Models + Validation/Erm{\"{u}}dungsfestigkeit{\_}Radaj/Kap1{\_}Einfuehrung.pdf:pdf},
pages = {1--13},
title = {{Problem des Erm{\"{u}}dungsschadens}}
}
@article{Singer1977a,
abstract = {The aluminum alloy investigated contained about 2. 7{\%} Cu, 1. 6{\%} Mg, 1. 1{\%} Fe, 1{\%} Ni, and small amounts of Si, Zn, and Ti. Creep at 473 K resulted in deformation-induced softening because of microstructural instability. Creep tests at varied stresses and temperatures were performed to explore the dislocation mechanisms during creep in specimens subjected to 13 different thermomechanical treatments. It was found that the room temperature yield stress and creep resistance after prolonged creep stressing can be improved by preliminary deformation, whereas the initial creep resistance is decreased. This is explained in terms of the effect of deformation on the structure and its stability.},
author = {Singer, Robert and Blum, Wolfgang},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Empirical Fatigue Models + Validation/1975{\_}Blum{\_}The influence of thermomechanical treatment on the creep resistance of RR58 - Al2618.pdf:pdf},
issn = {00443093},
journal = {Zeitschrift fuer Met. Res. Adv. Tech.},
number = {5},
title = {{Influence of Thermomechanical Treatments on the Creep Resistance of Rr 58 At Elevated Temperature.}},
volume = {68},
year = {1977}
}
@article{Lubliner2006,
abstract = {This self-contained text for advanced undergraduate and graduate students is devoted to classical quasistatic problems of rate-independent plasticity theory. It discusses the finite element method for both viscoplastic and rate-independent plastic solids, in addition to large deformation plasticity numerical methods for rate-based formulations and hyperelastic methods.},
author = {Lubliner, Jacob},
doi = {10.1115/1.2899459},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Lubliner - 2006 - Plasticity Theory.pdf:pdf},
isbn = {0023721618},
issn = {00218936},
journal = {J. Appl. Mech.},
number = {1},
pages = {540},
pmid = {15010233},
title = {{PLASTICITY Revised Edition ( PDF )}},
url = {http://www.getcited.org/pub/102800120},
volume = {59},
year = {2006}
}
@book{Qu2007a,
abstract = {The complete primer to micromechanics$\backslash$n$\backslash$n$\backslash$nFundamentals of Micromechanics of Solids is the first book integrating various approaches in micromechanics into a unified mathematical framework, complete with coverage of both linear and nonlinear behaviors. Based on this unified framework, results from the authors' own research, as well as existing results in the literature are re-derived in a logical, pedagogical, and understandable approach. It enables readers to follow the various developments of micromechanics theories and quickly understand its wide range of applications of micromechanics.$\backslash$n$\backslash$nThis helpful guide is a powerful tool for learning the most fundamental ideas and approaches, basic concepts, principles, and methodologies of micromechanics. Readers will find:$\backslash$n* Vigorous derivations of the mathematical framework$\backslash$n* Introductions to both linear and nonlinear material behavior$\backslash$n* Unique coverage of brittle damage, shape memory alloys, and TRIP steels$\backslash$n* Large numbers of problems and exercises to support teaching and learning the concepts$\backslash$n* Lists of references and suggested readings in each chapter},
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Qu, Jianmin and Cherkaoui, Mohammed},
booktitle = {Fundam. Micromechanics Solids},
doi = {10.1002/9780470117835},
eprint = {arXiv:1011.1669v3},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/Strukturmechanik MMS/Literatur/Mikromechanik{\_}B{\"{u}}cher{\_}Literaturvorschlag{\_}MMS/Qu 2006 Micromechanics.pdf:pdf},
isbn = {0471464511},
issn = {16137736},
pages = {1--386},
pmid = {21972053},
title = {{Fundamentals of Micromechanics of Solidss}},
year = {2007}
}
@article{Fl,
author = {Fl, Nicht-newtonsche and Fl, Nicht-newtonsche and Gleichungen, Navier-stokesschen and Gleichungen, Navier-stokesschen and Gebrauch, Bewegungsgleichungen and Gebrauch, Bewegungsgleichungen},
journal = {Integr. Vlsi J.},
title = {{6 Laminare Schichtenstr o ¨ mungen}}
}
@article{McEvily1991a,
abstract = {The behavior of short fatigue cracks cannot be analysed by linear elastic methods because of large scale plasticity effects as well as a breakdown in the stress intensity factor correlation of fatigue crack growth rates for crack sizes less than a millimeter in length. In the present paper a number of modifications are introduced to the linear elastic approach to establish a new parameter which is capable of correlating both long crack and short crack fatigue crack growth data. These modifications include the use of a material constant, re; an allowance for large scale plasticity effects; allowance for the development of crack closure; and the incorporation of the fatigue crack growth threshold. The new parameter is used with reasonable success in calculating fatigue crack growth behavior of short cracks in notched and unnotched specimens, and comparing with experimental data. In addition the analysis leads to a rationale for the dependence of the stress amplitude at the endurance level on the mean stress in a manner consistent with Gerber's parabolic relationship.},
author = {McEvily, A.J. and Eifler, D. and Macherauch, E.},
doi = {10.1016/0013-7944(91)90151-P},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/1991{\_}McEvily{\_}An analysis of the growth of short fatigue cracks.pdf:pdf},
issn = {00137944},
journal = {Eng. Fract. Mech.},
number = {3},
pages = {571--584},
title = {{An analysis of the growth of short fatigue cracks}},
url = {http://www.sciencedirect.com/science/article/pii/001379449190151P},
volume = {40},
year = {1991}
}
@article{Iliev,
author = {Iliev, Simeon},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Heat transfer intake+exhaust system/2013{\_}Iliev{\_}HEAT TRANSFER INVESTIGATION IN THE INTAKE PORT OF FOUR STROKE DI COMPRESSION IGNITION ENGINE.pdf:pdf},
number = {1},
pages = {133--138},
title = {{Heat Transfer Investigation in the Intake Port of Four Stroke Direct Injection Compression Ignition}}
}
@article{Gmund2010,
author = {Gm{\"{u}}nd, D},
doi = {10.1007/978-3-8348-9772-5},
isbn = {9780113310456},
journal = {Diss.Fu-Berlin.De},
pages = {10--12},
title = {{11. ANHANG 11.1. Materialliste}},
url = {http://www.diss.fu-berlin.de/diss/servlets/MCRFileNodeServlet/FUDISS{\_}derivate{\_}000000002409/11{\_}kapitel11.pdf?hosts=},
year = {2010}
}
@article{Papier,
author = {Papier, Blatt},
journal = {System},
title = {{3 Systemauslegung von Antriebstr¨ angen}}
}
@article{Potirniche2007a,
abstract = {This paper presents a polycrystalline plasticity theory including damage evolution in FCC materials. The formulation is thermodynamically-based and involves a multiplicative decomposition of the deformation gradient into its elastic, plastic and volumetric components. Plastic deformation at the grain level is assumed to occur by rate-dependent crystallographic slip. As a result of accumulated plastic strain and stress triaxiality, damage evolution leading to volumetric deformation is considered to occur within a single crystal by void nucleation, growth and coalescence. The overall stress-strain response of the polycrystalline material is obtained by Taylor averaging on the stress response of each grain. In the model, damage progression arises naturally from averaging each single crystal's damage evolution. A parametric study is performed to evaluate the amount of damage and strains at fracture on both single and polycrystals in order to understand crystal orientation effects. For validation purposes, model predictions of uniaxial stress-strain data are compared with experimental results for some aluminum alloys, and the comparison is shown to agree very well. ?? 2007 Elsevier Ltd. All rights reserved.},
author = {Potirniche, G P and Horstemeyer, M F and Ling, X W},
doi = {10.1016/j.mechmat.2007.04.004},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2006{\_}Potirniche{\_}An internal state variable damage model in crystal plasticity.pdf:pdf},
isbn = {0167-6636},
issn = {01676636},
journal = {Mech. Mater.},
keywords = {Crystal plasticity,Damage,Nucleation,Polycrystals,Void growth},
number = {10},
pages = {941--952},
title = {{An internal state variable damage model in crystal plasticity}},
volume = {39},
year = {2007}
}
@article{Chaboche2003,
abstract = {Constitutive and damage mechanics equations of composite materials are developed and discussed in the framework of micromechanics based approaches, including some recent modeling capabilities. The approach is based on the Transformation Field Analysis (TFA) promoted by Dvorak. A correction method is proposed in order to obtain a softer overall hardening response in case of the model restriction to only two subdomains (the elastic fibre, and the elasto-plastic matrix). In order to take into account the effects of temperature and damage on the elastic properties, a Generalised Eigenstrain Method (GEM) is developed, that uses the corresponding additional strains as eigenstrains. Its validity is checked by means of finite element numerical simulations based on periodic homogenisation. The methodology is further developed for metal matrix composites in which the matrix is treated as a polycristalline aggregate and slip plasticity is written at the level of slip systems. Two imbricated scale transitions are performed, both based on TFA like rules and it is shown how the overall constitutive equations can be considered as a multi-mechanism flow rule with pseudo-slip systems. Application of the model is made for a SiC/Ti composite. The capabilities are discussed by comparison with some experimental results, including monotonic and cyclic transverse loading conditions.},
author = {Chaboche, J L and Carr??re, N},
doi = {10.1007/978-3-540-36418-4_2},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Anisotropic Behaviouir of Damaged Materials{\_}Skrzypek{\_}ARTICEL/Kap2{\_}Multiscale Structural Analyses Incorporating Damage Mechanics at the Meso- or Micro-Scales.pdf:pdf},
isbn = {9783642055874},
issn = {16137736},
journal = {Lect. Notes Appl. Comput. Mech.},
keywords = {Viscoplasticity,damage mechanics,metal matrix composites,micromechanics,scale transitions},
pages = {35--74},
title = {{Multiscale Structural Analyses Incorporating Damage Mechanics at the Meso- or Micro-Scales}},
volume = {9},
year = {2003}
}
@article{Talbot1987,
abstract = {Bounds of Hashin-Shtrikman type and self-consistent estimates for the overall properties of composites, which may be anisotropic, are developed. Bodies containing aligned ellipsoidal inclusions are considered particularly, generalizing previously known results. The overall thermal conductivity of a body containing aligned spheroidal inclusions is discussed as an example including, as limiting cases, bodies containing highly-conducting aligned needles and bodies containing aligned pennyshaped cracks. ?? 1977.},
author = {Talbot, D. R.S. and Willis, J. R.},
doi = {10.1093/imamat/39.3.215},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/Strukturmechanik MMS/Literatur/Willis 1977.pdf:pdf},
isbn = {0022-5096},
issn = {02724960},
journal = {IMA J. Appl. Math. (Institute Math. Its Appl.},
number = {3},
pages = {215--240},
title = {{Bounds and self-consistent estimates for the overall properties of nonlinear composites}},
volume = {39},
year = {1987}
}
@book{Reuter2008b,
author = {Reuter, Manfred and Zacher, Serge},
booktitle = {Anal. Simul. und Entwurf von Regelkreisen},
doi = {10.1007/978-3-8348-9273-7},
isbn = {978-3-8348-0018-3},
title = {{Aus dem Programm}},
year = {2008}
}
@article{Wimmer2000b,
abstract = {This paper summarizes the results of several investigations on in-cylinder heat transfer during high-pressure and gas exchange phases as well as heat transfer in the inlet and outlet ports for a number of different engine types (DI Diesel, SI and gaseous fueled engine). The paper contains a comparision of simulation results and experimental data derived from heat flux measurements. Numerical results were obtained from zero-, one- and three-dimensional simulation methods. Time and spatially resolved heat fluxes were measured applying the surface temperature method and special heat flux sensors. The paper also includes an assessment of different sensor types with respect to accuracy and applicability.ER -},
author = {Wimmer, Andreas and Pivec, Robert and Sams, Theodor},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Heat transfer intake+exhaust system/2000{\_}Wimmer{\_}Heat Transfer to the Combustion Cahmber and Port Walls of IC Engines - Measurement and Prediction.pdf:pdf},
number = {724},
title = {{Heat Transfer to the Combustion Chamber and Port Walls of IC Engines - Measurement and Prediction}},
year = {2000}
}
@article{Bodies2003,
author = {Bodies, Elastic},
journal = {Elements},
pages = {167--172},
title = {{Rotating and Unrestrained Elastic Bodies 12.1}},
year = {2003}
}
@article{Gross2011,
author = {Gross, Dietmar and Seelig, Thomas},
doi = {10.1007/978-3-642-10196-0},
isbn = {978-3-642-10195-3},
title = {{Bruchmechanik}},
url = {http://link.springer.com/10.1007/978-3-642-10196-0},
year = {2011}
}
@article{Donnet1998,
author = {Donnet, JB},
doi = {10.1361/asmhba0003354},
pages = {35--40},
title = {{Carbon fibers}},
url = {http://books.google.com/books?hl=en{\&}lr={\&}id=YkN8xIwL0dsC{\&}oi=fnd{\&}pg=PR7{\&}dq=Carbon+Fibers{\&}ots=TSZQ3MkZPG{\&}sig=PRk4Wzq5SDVhtEJ4e1z7FG8j2ek},
volume = {21},
year = {1998}
}
@article{Din,
author = {Din, Rundwerte and Din, Ordnungssystem and Din, Fertigung and Din, Iso-passungen and Din, Einheitsbohrung and Din, Einheitswelle and Din, Passtoleranzen and Iso, E N and Iso, Produktdokumentation D I N},
pages = {247--328},
title = {10 10.1.1}
}
@article{Wallentowitz2006h,
author = {Wallentowitz, Henning and Reif, Konrad},
doi = {10.1007/978-3-8348-9121-1_2},
isbn = {978-3-528-03971-4},
journal = {Handb. Kraftfahrzeugelektronik - Grundlagen, Kompon. Syst. Anwendungen},
number = {x},
pages = {5--112},
title = {{Motor und Antriebsstrang}},
url = {http://www.springerlink.com/index/10.1007/978-3-8348-9121-1{\_}2},
year = {2006}
}
@article{Erma,
author = {Erm, Unter and Beanspruchungsablauf, Der and Versagenskriterium, Als and Vorgehensweise, Diese and Vorgaben, Den and Erweiterungen, Notwendige},
title = {{2 Schwingfestigkeit 2.1}}
}
@article{Statik,
author = {Statik, Band},
doi = {10.1007/978-3-642-19984-4},
isbn = {9783642199844},
pages = {2--4},
title = {{Uhrung}}
}
@article{Methodology,
author = {Methodology, Simulation and Gradation, Properties},
journal = {Order A J. Theory Ordered Sets Its Appl.},
title = {{Developing and Implementing Constitutive Models for Specific FGM Applications}}
}
@book{Voyiadjis2005,
abstract = {The solutions to most of the given problems appear in an appendix at the end of the book.},
author = {Voyiadjis, G Z and Kattan, P I},
booktitle = {New York},
doi = {10.1007/3-540-27710-2},
isbn = {9783540243533},
issn = {00223514},
number = {1},
pages = {9--13},
pmid = {14588922},
title = {{Mechanics of composite materials with MATLAB}},
url = {http://books.google.com/books?id=p4diQgAACAAJ{\&}printsec=frontcover},
volume = {1},
year = {2005}
}
@article{Pokluda2010b,
author = {Pokluda, Jaroslav and Andera, Pavel},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2010{\_}Jaroslav Pokluda+Pavel {\v{S}}andera{\_}Micromechanisms of fracture and fatigue{\_}Buch/Kap3{\_}BrittleAndDuctileFracture.pdf:pdf},
journal = {Micromechanisms Fract. Fatigue},
pages = {69--123},
title = {{Brittle and Ductile Fracture}},
year = {2010}
}
@article{Garikipati2001,
abstract = {This work represents a first step toward the development of a continuum field formulation for the coupled phenomena of diffusion and mechanics in polycrystalline solids. The basis of the formulation lies in lattice-level mechanisms, from which a continuum thermodynamic description of processes at micron length scales is developed. Considering self-diffusion, the composition problem is posed in terms of a binary vacancy-atom mixture. For mechanics, isotropic linear elasticity and isothermal conditions are assumed. The coupled constitutive relations for composition and mechanics are formally derived from the underlying thermodynamic principles. When applied to governing partial differential equations for each subproblem, the coupled nature is realized. Under applied tractions or intrinsic stress, the atoms diffuse - in general from surfaces with compressive normal traction to those with relatively tensile normal traction. The flow is mediated by electric fields via the mechanism of electromigration. In the case of metal interconnect lines in integrated circuit devices, the results of these microscopic processes are manifested in phenomena such as diffusional creep, hillock formation, grain growth, grain boundary motion, void formation and void evolution. These phenomena have a significant impact on the function, performance and failure of interconnect lines. A computational framework based on the finite element method has been developed to solve the coupled equations. Several numerical examples are presented and comparisons with analytical results are provided where the latter are available. ?? 2001 Elsevier Science Ltd.},
author = {Garikipati, Krishna and Bassman, Lori and Deal, Michael},
doi = {10.1016/S0022-5096(00)00081-8},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Kriechen{\_}Spannungsrelaxation/2001{\_}Garikipati+Bassman+Deal{\_}A lattice-based micromechanical continuum formulation for stress-driven mass transport in polycrystalline solids.pdf:pdf},
issn = {00225096},
journal = {J. Mech. Phys. Solids},
keywords = {C. Finite elements,Coupling,Diffusion,Stress,Thermodynamics},
number = {6},
pages = {1209--1237},
title = {{A lattice-based micromechanical continuum formulation for stress-driven mass transport in polycrystalline solids}},
volume = {49},
year = {2001}
}
@article{Mechanismen,
author = {Mechanismen, Die},
title = {{8 Kr{\{}{\"{a}}{\}}fte und Momente}}
}
@article{Opitz1959,
author = {Opitz, Herwart},
doi = {10.1007/978-3-663-05002-5_6},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Empirical Fatigue Models + Validation/Betriebsfestigkeit{\_}ErwinHaibach/Backmatter.pdf:pdf},
isbn = {978-3-663-03813-9},
pages = {33},
title = {{Verwendete Formelzeichen}},
year = {1959}
}
@inproceedings{Wisniewski1998,
abstract = {An experimental study was conducted in order to determine some heat transfer coefficients and to measure temperatures and heat fluxes in exhaust valves of 4C90 diesel engine. Measurements were performed both on a model stand and on a firing engine.The experimental stand for model studies was built with use of 4C90 engine parts. The thermal contact conductance between a valve face and a seat as a function of mechanical load was determined. Heat transfer between valve face and seat and between valve stem and guide was measured in some range of valve gear speed.The temperatures and heat fluxes, measured in exhaust valves and valve seat of firing 4C90 diesel engine, were presented as a function of its torque and speed.},
author = {Wisniewski, Tomasz S},
booktitle = {Int. Congr. Expo.},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Heat transfer intake+exhaust system/1998{\_}Wisniewski{\_}Experimental Study of Heat Transfer on Exhaust Valves of 4C90 Diesel Engine.pdf:pdf},
month = {feb},
publisher = {SAE International},
title = {{Experimental Study of Heat Transfer on Exhaust Valves of 4C90 Diesel Engine}},
year = {1998}
}
@article{Mcdowell2017a,
author = {Mcdowell, David L},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/Folien CISM Summer School Mai2017 - Mesoscale Models/courses{\_}C1703{\_}mcdowell{\_}CISM.atomistic.mcdowell.lecture+1.final.pdf:pdf},
title = {{Atomistic Modeling for Crystalline Nanostructures}},
year = {2017}
}
@article{Rice1969,
abstract = {The fracture of ductile solids has frequently been observed to result from the large growth and coalescence of microscopic voids, a process enhanced by the superposition of hydrostatic tensile stresses on a plastic deformation field. The ductile growth of voids is treated here as a problem in continuum plasticity. First, a variational principle is established to characterize the flow field in an elastically rigid and incompressible plastic material containing an internal void or voids, and subjected to a remotely uniform stress and strain rate field. Then an approximate Rayleigh-Ritz procedure is developed and applied to the enlargement of an isolated spherical void in a nonhardening material. Growth is studied in some detail for the case of a remote tensile extension field with superposed hydrostatic stresses. The volume changing contribution to void growth is found to overwhelm the shape changing part when the mean remote normal stress is large, so that growth is essentially spherical. Further, it is found that for any remote strain rate field, the void enlargement rate is amplified over the remote strain rate by a factor rising exponentially with the ratio of mean normal stress to yield stress. Some related results are discussed, including the long cylindrical void considered by F.A. McClintock (1968, J. appl. Mech. 35, 363), and an approximate relation is given to describe growth of a spherical void in a general remote field. The results suggest a rapidly decreasing fracture ductility with increasing hydrostatic tension.},
author = {Rice, J R and Tracey, D M},
doi = {10.1016/0022-5096(69)90033-7},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Plasticity models/On the ductile enlargement of voids in triaxial stress fields {\_}RiceAndTracey.pdf:pdf},
isbn = {0022-5096},
issn = {00225096},
journal = {J. Mech. Phys. Solids},
number = {3},
pages = {201--217},
title = {{On the ductile enlargement of voids in triaxial stress fields∗}},
url = {http://linkinghub.elsevier.com/retrieve/pii/0022509669900337},
volume = {17},
year = {1969}
}
@article{Betrachtungenb,
author = {Betrachtungen, Allgemeine},
title = {{are , eindimensionale Str ¨ omungen inkompressibler , viskoser Fluide}}
}
@article{Ziegler1995,
abstract = {In this paper, the three principal control effects found in present controllers are examined and practical names and units of measurement are proposed for each effect. Corresponding units are proposed for a classification of industrial processes in terms of the two principal characteristics affecting their controllability. Formulas are given which enable the controller settings to be determined from the experimental or calculated values of the lag and unit reaction rate of the process to be controlled. These units form the basis of a quick method for adjusting a controller on the job. The effect of varying each controller setting is shown in a series of chart records. It is believed that the conceptions of control presented in this paper will be of assistance in the adjustment of existing controller applications and in the design of new installations.},
author = {Ziegler, J. G. and Nichols, N. B.},
doi = {10.1115/1.2899060},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Vorlesungen/Messtechnik+Regelungstechnik/1993{\_}Ziegler+Nichols{\_}Optimum Settings for Automatic Controllers.pdf:pdf},
isbn = {0022-0434},
issn = {0192303X},
journal = {InTech},
number = {6},
pages = {94--100},
title = {{Optimum settings for automatic controllers}},
volume = {42},
year = {1995}
}
@article{Januszka2015,
author = {Januszka, Marcin and Panfil, Wawrzyniec},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2016{\_}Lasocki{\_}ENGINE KNOCK DETECTION AND EVALUATION - A REVIEW.pdf:pdf},
number = {102},
pages = {37--48},
title = {{Proceedings of the institute of vehicles 2(102)/2015}},
volume = {2},
year = {2015}
}
@article{Eekoye1996b,
abstract = {Heat-transfer rates present in an engine cylinder undergoing knock are known to be larger than the rates associated with normal engine operation. Further, at the time of knock, the largest heat fluxes are associated with locations on the cylinder wall where the flame is locally quenching. In this study, heat-transfer processes at the flame-wall interface during a knock event are investigated computationally and analytically. Computationally, the governing equations for a one-dimensional, flame-quenching event are solved using a reduced chemical reaction mechanism. Analytically, scaling relations for the flame heat-release rates are used in the governing equations to determine the heat-transfer rates. It is found that while pressure transients modify the wall heat flux, the absolute value of the pressure is the most significant parameter in predicting the maximum heat flux. The wall heat flux profiles are predicted for both the analytical and computational models. In the range of pressures examined, a linear relationship was found between the peak flux and pressure, both for the computational and analytical models. The linear relationship between the pressure and peak flux was found to be invalid when the flame-quenching process was disrupted by the pressure fluctuations for pressure oscillations with a characteristic time on the order of the quenching process. ?? 1996 Combustion Institute.},
author = {Eekoye, O A},
doi = {10.1016/S0082-0784(96)80101-9},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/1996{\_}Ezekoye{\_}Heat transfer modeling during knock and flame quenching in an engine chamber.pdf:pdf},
isbn = {0082-0784},
issn = {00820784},
journal = {Symp. Combust.},
number = {2},
pages = {2661--2668},
title = {{Heat transfer modeling during knock and flame quenching in an engine chamber}},
volume = {26},
year = {1996}
}
@article{Pahl2007d,
abstract = {Kap. 5},
author = {Pahl, Gerhard and Beitz, Wolfgang and Feldhusen, J{\"{o}}rg and Grote, Karl-Heinz},
isbn = {9783540340607},
pages = {213--230},
title = {{Konstruktionslehre}},
year = {2007}
}
@article{Schubert2005a,
abstract = {A realistic simulation of the wall heat transfer is an imperative condition for the accurate analysis and simulation of the working process of IC engines. Due to its simplicity in application, zero-dimensional wall heat transfer models dominate engine cycle simulation in practice. However, experience shows that existing zero-dimensional models for wall heat transfer do not yield satisfactory results in certain applications. This is mainly due to a lack of consideration of the actual flow field in the cylinder.In this paper a quasi-dimensional heat transfer model, which is based on a detailed description of the turbulent flow field in the combustion chamber, is described. The model presents a consistent approach for the high pressure as well as the low pressure part of the cycle. The results of the heat transfer model are compared with results from the correlation by Woschni/Huber and with experimental results from various DI Diesel engines.},
author = {Schubert, Claudia and Wimmer, Andreas and Chmela, Franz},
doi = {10.4271/2005-01-0695},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Heat Transfer Combustion Chamber/2005{\_}Schubert{\_}Advanced Heat Transfer Model for CI Engines.pdf:pdf},
isbn = {0148-7191},
journal = {SAE Tech. Pap.},
number = {724},
title = {{Advanced Heat Transfer Model for CI Engines}},
url = {http://dx.doi.org/10.4271/2005-01-0695},
volume = {2005},
year = {2005}
}
@article{Forest,
author = {Forest, Samuel},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/Folien CISM Summer School Mai2017 - Mesoscale Models/courses{\_}C1703{\_}forest{\_}Forest1-Micromorphic.pdf:pdf},
title = {{Micromorphic media}}
}
@article{Dera,
author = {Der, Einteilung Vorteile},
title = {{5 Umformen 5.1}}
}
@article{Wellen2005,
author = {Wellen, Schwingungen},
doi = {10.1007/3-540-27217-8_9},
isbn = {3540221484},
pages = {214--243},
title = {{Schwingungen und Wellen}},
year = {2005}
}
@article{Depcik2002c,
abstract = {In this paper, the available correlations proposed in the literature for the gas-side heat transfer in the intake and exhaust system of a spark-ignition internal combustion engine were surveyed. It was noticed that theseAB - {\textless}inline-graphic xlink:href="2002-01-0372{\_}fig0001" xmlns:xlink="http://www.w3.org/1999/xlink"/{\textgreater}AB - only by empirically fitted constants. This similarity provided the impetus for the authors to explore if a universal correlation could be developed. Based on a scaling approach using microscales of turbulence, the authors have fixed the exponential factor on the Reynolds number and thus reduced the number of adjustable coefficients to just one; the latter can be determined from a least squares curve-fit of available experimental data. Using intake and exhaust side data, it was shown that the universal correlationAB - {\textless}inline-graphic xlink:href="2002-01-0372{\_}fig0002" xmlns:xlink="http://www.w3.org/1999/xlink"/{\textgreater}AB - The correlation coefficient of this proposed heat transfer model with all available experimental data is 0.845 for the intake side and 0.800 for the exhaust side.ER -},
author = {Depcik, Christopher and Assanis, Dennis},
doi = {10.4271/2002-01-0372},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Heat transfer intake+exhaust system/2002{\_}Assanis{\_}A Universal Heat Transfer Correlation for Intake and Exhaust flows in an SI INternal Combustion Engine.pdf:pdf},
journal = {SAE Pap.},
number = {January 2016},
title = {{A Universal Heat Transfer Correlation for Intake and Exhaust Flows in an Spark-Ignition Internal Combustion Engine}},
url = {http://papers.sae.org/2002-01-0372},
volume = {2002-01-03},
year = {2002}
}
@article{Manonukul2004a,
abstract = {A polycrystal plasticity finite–element model has been developed for nickel–base alloy C263. That is, a representative region of the material, containing about 60 grains, has been modelled using crystal plasticity, taking account of grain morphology and crystallographic orientation. With just a single material property (in addition to standard elastic properties), namely, the critical resolved shear stress, the model is shown to be capable of predicting correctly a wide range of cyclic plasticity behaviour in face–centred cubic nickel alloy C263. A fatigue crack initiation criterion is proposed, based simply on a critical accumulated slip. When this critical slip is achieved within the microstructure, crack initiation is taken to have occurred. The model predicts the development of persistent slip bands within individual grains with a width of ca. 10 $\mu$m. The model also predicts that crack initiation can occur preferentially at grain triple points under both low– (LCF) and high–cycle fatigue (HCF). For the case of HCF, this also corresponds to a free surface. The polycrystal plasticity model combined with the fatigue crack initiation criterion are shown to predict correctly the standard Basquin and Goodman correlations in HCF, and the Coffin–Manson correlation in LCF. The model predictions are based on just two material properties: the critical resolved shear stress and the critical accumulated slip. Just one experimental test is required to determine these properties, for a given temperature, which have been obtained for nickel alloy C263. Predictions of life for nickel alloy C263 are then made over a broad range of loading conditions covering both LCF and HCF. Good agreement with experiments is achieved, despite the simplicity of the proposed ‘two–parameter' model. A simple three–dimensional form of the model has provided an estimate of the fatigue limit for HCF crack initiation in C263.},
author = {Manonukul, A. and Dunne, F. P. E.},
doi = {10.1098/rspa.2003.1258},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2003{\_}Manonukul+Dunne{\_}High- and low-cycle fatigue crack initiation using polcrystal plasticity.pdf:pdf},
isbn = {1364-5021},
issn = {1364-5021},
journal = {Proc. R. Soc. A Math. Phys. Eng. Sci.},
keywords = {crack initiation,hcf,high-cycle fatigue,lcf,low-cycle fatigue,polycrystal plasticity},
number = {2047},
pages = {1881--1903},
title = {{High- and low-cycle fatigue crack initiation using polycrystal plasticity}},
url = {http://rspa.royalsocietypublishing.org/cgi/doi/10.1098/rspa.2003.1258},
volume = {460},
year = {2004}
}
@article{Brown2000,
abstract = {Persistent slip bands dominate plastic how under conditions of 'saturation', i.e. when a ductile material is cycled at constant plastic strain amplitude, the maximum stress in one cycle rises and then saturates. The saturation stress is identified as being to an excellent approximation equal to the endurance limit of the material, as measured by conventional stress cycling tests. When saturation is attained, plastic flow is confined to well-defined slip bands, which persist after electropolishing and resuming cyclic straining. These persistent slip bands have a well-defined dislocation structure, characterised by a length, which separates walls of dislocation dipoles. The persistent slip bands have a unique stress-strain curve, caused by the backward and forward motion of screw dislocations between the walls. Many authors have worked on these structures, and their main features are widely agreed. Persistent slip bands lead to the initiation of fatigue cracks, because where they intersect the external surface of the material, they cause stress concentrations and generate intrusions, which follow the interface between the persistent slip band and the matrix within which it is embedded. Many features of the cyclic plastic flow can be understood in terms of two basic concepts. Firstly, it is assumed that the bands are dissipative structures, shear structures, with a spacing determined by dynamic processes including the laying down of edge dislocation dipoles and the forces on groups of dipoles resulting from the motion of the screw dislocations producing them. Secondly, the mean free path of screw dislocations in the bands is determined by the probability of meeting and annihilating another screw dislocation of opposite sign. Very simple equations show that the saturation stress is equal to the plastic strain in the band multiplied by the elastic shear modulus divided by 4 pi. This very simple result is borne out to within a few percent by recent data on copper single crystals. Other data relating the wall spacing to the saturation stress and the minimum distance apart of stable screw dislocations is accurately rationalised by the theory. Several aspects of the theory deserve comment. The theory indicates that the dislocation density does not matter. The strong temperature dependence of the wall spacing and the saturation stress receive natural explanation. And if the saturation stress is equal to the stress for the onset of stage III unidirectional work-hardening, one can rationalise one of the oldest rules in fatigue strength - the so-called 'fatigue ratio', whereby the endurance limit is proportional to the ultimate tensile strength. The picture of cyclic hardening implies that materials with steep initial hardening rates show low saturation stresses; cyclic hardening curves always cross. This is in agreement with observation. Objections raised by other authors are analysed briefly. The existence of internal stress in the structures, as deduced by Mughrabi in neutron irradiated copper, can be re-interpreted on the basis of the normally assumed variation of dislocation line tension with character. The picture of cross-slip which emerges, implies that cross-slip occurs at all stages in the stress-strain curve, but at the onset of stage III, every screw dislocation cross-slips to annihilation - no screw dipoles are possible. This seems consistent with observation. (C) 2000 Elsevier Science S.A. All rights reserved.},
author = {Brown, L M M},
doi = {10.1016/S0921-5093(00)00662-6},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/2000{\_}Brown{\_}Dislocation plasticity in persistent slip bands.pdf:pdf},
isbn = {0921-5093},
issn = {09215093},
journal = {Mater. Sci. Eng. A},
keywords = {cyclic plasticity,screw dislocation,slip bands},
number = {1-2},
pages = {35--42},
title = {{Dislocation plasticity in persistent slip bands}},
url = {http://linkinghub.elsevier.com/retrieve/pii/S0921509300006626},
volume = {285},
year = {2000}
}
@article{Schwingbeanspruchung,
author = {Schwingbeanspruchung, Kennzeichnung Der},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Empirical Fatigue Models + Validation/Betriebsfestigkeit{\_}ErwinHaibach/Kap2 Experimentelle Grundlagen und Betriebsfestigkeit.pdf:pdf},
title = {{2 Experimentelle Grundlagen der Betriebsfestigkeit}}
}
@article{Zahnrad,
author = {Zahnrad, B},
doi = {10.1007/978-3-8348-8279-0},
isbn = {9783834882790},
pages = {410--474},
title = {{13 Kupplungen und Bremsen 13.1}}
}
@article{Na,
author = {Na, Meoy},
title = {{12 Mehrk{\"{o}}rpersysteme}}
}
@article{Ottosen1992,
author = {Ottosen, Niels Sadrje and Petersson, Hans},
pages = {117--120},
title = {{Introduction to the Finite Element Method}},
year = {1992}
}
@article{Kanchanomai2007a,
abstract = {Fatigue cracking due to traffic load is a major factor in road damage. Therefore, durability and lifetime prediction of roads plays a substantial role for road maintenance and cost planning. This paper reports a study of fatigue crack performance of solid asphalt and asphalt-asphalt interfaces by means of the wedge-splitting test. Instead of beams and the three- or four-point bending test, the wedge splitting method was used for the first time to observe crack growth on bituminous drilling cores. Samples of solid asphalt and samples with asphalt-interfaces were tested. One group of asphalt interfaces was untreated and the other was sandblasted before spreading the top layer during manufacturing. Due to the temperature dependency of material properties of asphalt, the tests were performed in a compact climate chamber at -10, 0 and + 10(' The challenge of determining the crack length and the crack tip were detected with an optical measurement system and picture analysis after testing. The results prove that the wedge splitting method is a highly practicable and repeatable method for crack growth testing of bituminous materials.},
author = {Kanchanomai, C and Mutoh, Y},
doi = {10.1111/j.1460-2695.2006.01088.x},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/1979{\_}Kung+Fine{\_}Fatigue crack initiation and microcrack growth in 2024-T4 and 2124-T4 Alu alloy.pdf:pdf},
issn = {8756758X},
journal = {Eng. Fract. Mech.},
keywords = {fatigue crack growth,fatigue crack initiation,lead free,low cycle fatigue},
number = {5},
pages = {443--457},
title = {{Fatigue crack initiation and growth in solder alloys}},
url = {http://doi.wiley.com/10.1111/j.1460-2695.2006.01088.x},
volume = {30},
year = {2007}
}
@article{Borg2006b,
author = {Borg, Jm and Alkidas, Ac},
doi = {10.4271/2006-01-3341},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2006{\_}Borg{\_}Characterisation of autoignition in a knocking si engine using heat release analysis.pdf:pdf},
journal = {SAE Tech. Pap.},
number = {724},
pages = {776--790},
title = {{Characterization of autoignition in a knocking SI engine using heat release analysis}},
url = {http://papers.sae.org/2006-01-3341/},
volume = {2006-01-33},
year = {2006}
}
@article{Thon2015,
author = {Thon, M},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Vorlesungen/p{\_}script{\_}em1{\_}ws1516.pdf:pdf},
pages = {2--4},
title = {{Engineering Mechanics I}},
volume = {2},
year = {2015}
}
@article{Conduction,
author = {Conduction, Heat},
number = {x},
title = {{Thermodynamics of Constitutive Modelling of 2 . 1 Effect of Damage on the Mechanical and Thermal}}
}
@article{Hild2015a,
abstract = {{\textcopyright} Springer Science+Business Media New York 2015.This chapter is devoted to the evaluation of damage with digital image correlation (DIC). This measurement technique provides displacement fields that can be used to tune material parameters of damage models. The potential of DIC for identification purposes is illustrated hereafter for simple 1D-type geometries in the context of quasi-brittle and ductile behaviors. Beams and frames as encountered in civil engineering application can be described through damage laws. The localization of damage at single points (lumped damage mechanics) and the resulting damage law can be determined very precisely based on dedicated versions of DIC incorporating the descriptive language of beam theory. At smaller scale, plasterboards (plaster core lined with paper) constitute another example of a structure (rather than a material), which can be described as damageable. Those cases will be analyzed in details.},
author = {Hild, Fran{\c{c}}ois and Roux, St{\'{e}}phane},
doi = {10.1007/978-1-4614-5589-9},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/2015{\_}Sun+Liu{\_}Particel-Debonding modeling of metal-matrix composites.pdf:pdf},
isbn = {9781461455899},
journal = {Handb. Damage Mech. Nano to Macro Scale Mater. Struct.},
pages = {1277--1299},
title = {{Evaluating damage with digital image correlation: b. from physical to mechanical damage}},
year = {2015}
}
@article{Man2009,
abstract = {Current state and historical progress in experimental and theoretical studies of surface relief appertaining to persistent slip bands (PSBs) and leading to fatigue crack initiation in cyclically deformed metals is presented as a thorough critical overview. A comprehensive inventory of microscopic techniques used for this study is tabulated chronologically with emphasis to their applicability to polycrystals. The most relevant experimental characteristics concerning surface relief evolution, namely the form of extrusions and intrusions in single- and polycrystalline materials, are surveyed. Theoretical models and computational simulations of extrusion and intrusion formation and fatigue crack initiation are critically reviewed.},
author = {Man, J and Obrtl{\'{i}}k, K and Pol{\'{a}}k, J},
doi = {10.1080/14786430902917616},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/2009{\_}Man + Polak{\_}Extrusions and intrusions in fatigued metals Part 1 State of the art and history.pdf:pdf},
isbn = {1478-6435},
issn = {1478-6435},
journal = {Philos. Mag.},
number = {16},
pages = {1295--1336},
title = {{Extrusions and intrusions in fatigued metals. Part 1. State of the art and history†}},
url = {http://www.tandfonline.com/doi/abs/10.1080/14786430902917616},
volume = {89},
year = {2009}
}
@article{Xu1993,
abstract = {In a numerical micromechanical study of void nucleation, a framework is used where
constitutive relations are specified independently for the matrix, the void-nucleating particles and the interface. Plane strain analyses are carried out for a doubly periodic array of circular cylindrical particles. The particles are taken to be rigid and the elastic-plastic deformations of the matrix are decribed in terms of continuum crystalline plasticity, using a planar crystal model that allows for three slip systems. Comparison is made with void-nucleation predictions based on a corresponding flow theory of plasticity with isotropic hardening. The crystal model on give rise to shear localization at the particle-matrix interface and shear localization, which leads to large localized strains in the matrix. is found to inhibit decohesion. The role of the triaxiality of the stress state in determining whether decohesion or localization occurs first is investigated. A parametric study is also carried out for a crystal matrix using two descriptions of the interface shear behaviour; one is periodic in the shear displacement across the interface while the other allows for shear decohesion.},
author = {Xu, X -P and Needleman, A},
doi = {10.1088/0965-0393/1/2/001},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/1993{\_}Needleman{\_}Void nucleation by inclusion debonding in a crystal matrix.pdf:pdf},
issn = {0965-0393},
journal = {Model. Simul. Mater. Sci. Eng.},
number = {2},
pages = {111--132},
title = {{Void nucleation by inclusion debonding in a crystal matrix}},
url = {http://stacks.iop.org/0965-0393/1/i=2/a=001?key=crossref.0ad72f94185990833a445936aea2f0ba},
volume = {1},
year = {1993}
}
@article{Chaboche1986,
author = {Chaboche, J L},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/Hardening Recovery Creep/1986{\_}Chaboche{\_}Time-independent-constitutive-theories-for-cyclic-plasticity.pdf:pdf},
journal = {Int. J. Plast.},
number = {2},
pages = {149--188},
title = {{Time-independent constitutive theorems for cyclic plasticity}},
volume = {2},
year = {1986}
}
@article{Auflagen,
author = {Auflagen, Gesetzliche},
title = {{17 Zuverl{\"{a}}ssigkeit und Erprobung von Fahrzeuggetrieben}}
}
@article{Journal2008,
author = {Journal, American and Sciences, Applied and Publications, Science},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Heat transfer intake+exhaust system/2008{\_}Semin+Ismail{\_}Heat Transfer Investigation of Intake Port Engine Based on Steady-State and Transient Simulation.pdf:pdf},
keywords = {compression ignition engine,computational model,heat transfer,intake port,simulation},
number = {11},
pages = {1572--1579},
title = {{Heat Transfer Investigation of Intake Port Engine Based on Steady-State and Transient Simulation Semin , 2 Abdul Rahim Ismail , 2 Rosli Abu Bakar and 2 Ismail Ali Institute of Technology Sepuluh Nopember , Surabaya 60111 , Indonesia Faculty of Mechanical }},
volume = {5},
year = {2008}
}
@article{Normzustand,
author = {Normzustand, Physikalischer and Normzustand, Physikalischer and Wichte, Die and Wichte, Die and Kelvin, Das and Kelvin, Das},
journal = {Arbeit},
pages = {161--176},
title = {{6.1 Grundbegriffe}}
}
@article{Finol2006d,
abstract = {Over the last 40 years, several empirical correlations have been developed to estimate heat fluxes from the combustion chambers of internal combustion engines. Some of these expressions are based on correlations to compute the Nusselt number for forced convection in turbulent flow inside circular tubes. The fundamental suitability of this kind of empirical model in representing the highly complex processes of in-cylinder heat transfer is questionable, but in practice the models have steadily improved owing to contributions from numerous investigators. Other correlations have a less theoretical basis than those of the Nusselt number form. Formulae of this type have been obtained from the application of simple statistical techniques to large datasets, taking into account several engine operational parameters and engine types. The resulting correlations provide reasonable estimates but perform poorly when extrapolated or applied to novel concepts. In this paper, the most important correlations are reviewed against the features of a modern diesel engine, and research requirements for future modelling developments are identified and discussed. {\textcopyright} IMechE 2006.},
author = {Finol, C. A. and Robinson, K.},
doi = {10.1243/09544070JAUTO202},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Heat Transfer Combustion Chamber/2006{\_}Finol{\_}Thermal modelling of modern engines - A review of empirical correlations to estimate the in-cylinder heat transfer coefficient .pdf:pdf},
isbn = {0954407011407},
issn = {09544070},
journal = {Proc. Inst. Mech. Eng. Part D J. Automob. Eng.},
keywords = {Heat flux,Heat transfer coefficient,In-cylinder heat transfer models},
number = {12},
pages = {1765--1781},
title = {{Thermal modelling of modern engines: A review of empirical correlations to estimate the in-cylinder heat transfer coefficient}},
volume = {220},
year = {2006}
}
@book{Habenicht2012f,
author = {Habenicht, Gerd},
isbn = {9783834802958},
title = {{Aus dem Programm Fertigungstechnik}},
year = {2012}
}
@book{HorstCzickosTechnischeFachhochschuleBerlin2008,
author = {{Horst Czickos (Technische Fachhochschule Berlin)}, Manfred Hennecke (BAM)},
isbn = {9783540718512},
title = {{H{\{}{\"{u}}{\}}tte Das Ingenieurwissen}},
year = {2008}
}
@article{Allianz2003,
author = {Allianz, Von M Pfender and Berlin, M{\"{u}}nchen},
isbn = {3540440631},
number = {2},
title = {{6 Schrifttumshinweise}},
volume = {6},
year = {2003}
}
@article{Johnson2004,
author = {Johnson, Ws and Hillberry, Bm},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Probabilistic Aspects/2004{\_}StevenJohnson{\_}Probabilistic Aspects of Life Prediction.pdf:pdf},
journal = {Book},
title = {{Probabilistic aspects of life prediction}},
url = {http://books.google.com/books?hl=en{\&}lr={\&}id=pDtb-CJLVbYC{\&}oi=fnd{\&}pg=PP7{\&}dq=Probabilistic+Aspects+of+Life+Prediction{\&}ots=fII0k-XR1K{\&}sig=qyo{\_}6w{\_}nT7cN1tqI8pird5rUdts},
year = {2004}
}
@article{Esfahanian2006,
abstract = {In this study, the heat transfer to an engine piston crown is calculated. Three different methods for the combustion boundary condition are used. The results of different combustion side boundary condition treatments are compared and their effects on the thermal behavior of the piston are investigated. It has been shown that using spatial and time averaged combustion side boundary condition is a suitable treatment method within engineering approximations. An interface between KIVA-3V and NASTRAN codes is developed. ?? 2005 Elsevier Ltd. All rights reserved.},
author = {Esfahanian, V. and Javaheri, A. and Ghaffarpour, M.},
doi = {10.1016/j.applthermaleng.2005.05.002},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2006{\_}Esfahanian{\_}Thermal analysis of an SI engine piston using different combustion boundary condition treatements.pdf:pdf},
issn = {13594311},
journal = {Appl. Therm. Eng.},
keywords = {Boundary Condition Treatment,Combustion,Heat transfer,Piston},
number = {2-3},
pages = {277--287},
title = {{Thermal analysis of an SI engine piston using different combustion boundary condition treatments}},
volume = {26},
year = {2006}
}
@article{Betrachtungenf,
author = {Betrachtungen, Allgemeine},
title = {{19 Numerische L ¨ osungen der str o ¨ mungsmechanischen Grundgleichungen}},
volume = {2}
}
@article{Durst,
author = {Durst, Franz},
isbn = {9783540313236},
journal = {New York},
title = {{Franz Durst Grundlagen der Str{\{}{\"{o}}{\}}mungsmechanik}}
}
@article{Anwendungen,
author = {Anwendungen, Bei and Fahrer, Der and Kraftfahrzeug, Systems},
pages = {211--226},
title = {{13 Fahrzeugtechnik}}
}
@article{Prinzip,
author = {Prinzip, Archimedisches and Gleichung, Bernoullische},
title = {{Ucke}}
}
@article{Grosskreutz1971b,
abstract = {Fatigue crack initiation Fatigue crack growth},
author = {Grosskreutz, J G},
doi = {10.1002/pssb.2220470202},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/1971{\_}Grosskreutz{\_}The Mechanisms of metal fatigue Some Details.pdf:pdf},
isbn = {0370-1972},
issn = {15213951},
journal = {Phys. Status Solidi},
number = {2},
pages = {359--396},
title = {{The mechanisms of metal fatigue (II)}},
volume = {47},
year = {1971}
}
@article{RajuP2011a,
abstract = {This paper presents the details of method of sample size determination to estimate the characteristic fatigue life of aluminum alloy, A356.2-T6. The characteristic fatigue life of the alloy has been estimated by assuming log normal distribution model. A step wise procedure is outlined to determine the number of specimens required at predetermined stress amplitude to estimate the fatigue life with an acceptable error at 50{\%} probability and various confidence levels, 90{\%}, 95{\%} and 99{\%}. Maximum percentage of errors has also been calculated for the above probability and confidence levels. Details of generation of S-N curve for aluminum alloy A356.2-T6 using regression analysis have been explained. From this study, the adequate sample size required for evaluating the average fatigue life of A356.2-T6 with an acceptable error at 50{\%} probability and 90{\%} confidence level using log normal distribution is established. In order to check the significance of regression equation, analysis of variance (ANOVA) is performed. Copyright 2011 Tech Science Press.},
author = {{Raju P}, R and Rajesh, S and Satyanarayana, B and Ramji, K},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Probabilistic Aspects/2011{\_}Ramamurty{\_}Statistical Analysis of Fatigue Life Data of A356.2-T6 Aluminium Alloy.pdf:pdf},
journal = {Struct. Durab. Heal. Monit.},
keywords = {aluminum alloy,fatigue life,log normal distribution,s n curve},
number = {1-2},
pages = {139--152},
title = {{Statistical analysis of fatigue life data of A356.2-T6 aluminum alloy}},
url = {http://www.scopus.com/inward/record.url?eid=2-s2.0-79957943262{\&}partnerID=40{\&}md5=a5890475316795056516da22de2c7672},
volume = {7},
year = {2011}
}
@article{Din,
author = {Din, Rundwerte and Din, Ordnungssystem and Din, Fertigung and Din, Iso-passungen and Din, Einheitsbohrung and Din, Einheitswelle and Din, Passtoleranzen and Iso, E N and Iso, Produktdokumentation D I N},
pages = {247--328},
title = {10 10.1.1}
}
@article{Hill1966a,
abstract = {A general, type of cross-coupling between glide and hardening on different slip-systems is proposed. Its implications in regard to the character of the connexion between the overall stress-rate and strain-rate in multislip are investigated. Uniqueness theorems and extremal properties are established in respect both of the overall constitutive law itself and any boundary-value problem for non-uniform deformation of a single crystal or aggregate.},
author = {Hill, R},
doi = {10.1016/0022-5096(66)90040-8},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/1966{\_}Hill{\_}Generalized consititutive relations for incremental defo of metal crystals by multislip.pdf:pdf},
isbn = {0022-5096},
issn = {00225096},
journal = {J. Mech. Phys. Solids},
number = {2},
pages = {95--102},
title = {{Generalized constitutive relations for incremental deformation of metal crystals by multislip}},
volume = {14},
year = {1966}
}
@article{Chang2004b,
abstract = {An experimental study has been carried out to provide qualitative and quantitative insight into gas to wall heat transfer in a gasoline fueled Homogeneous Charge Compression Ignition (HCCI) engine. Fast response thermocouples are embedded in the piston top and cylinder head surface to measure instantaneous wall temperature and heat flux. Heat flux measurements obtained at multiple locations show small spatial variations, thus confirming relative uniformity of incylinder conditions in a HCCI engine operating with premixed charge. Consequently, the spatially-averaged heat flux represents well the global heat transfer from the gas to the combustion chamber walls in the premixed HCCI engine, as confirmed through the gross heat release analysis. Heat flux measurements were used for assessing several existing heat transfer correlations. One of the most popular models, the Woschni expression, was shown to be inadequate for the HCCI engine. The problem is traced back to the flame propagation term which is not appropriate for the HCCI combustion. Subsequently, a modified model is proposed which significantly improves the prediction of heat transfer in a gasoline HCCI engine and shows very good agreement over a range of conditions},
author = {Chang, Junseok and G{\"{u}}ralp, Orgun and Filipi, Zoran and Assanis, Dennis N and Kuo, Tang-Wei and Najt, Paul and Rask, Rod},
doi = {10.4271/2004-01-2996},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2004{\_}Chang{\_}New Heat Transfer Correlation for an HCCI Engine Derived from Measurements of Instantaneous Surface Heat Flux.pdf:pdf},
isbn = {0148-7191},
issn = {0148-7191},
number = {724},
title = {{New Heat Transfer Correlation for an HCCI Engine Derived from Measurements of Instantaneous Surface Heat Flux}},
url = {http://papers.sae.org/2004-01-2996/},
year = {2004}
}
@article{Zienkiewicza,
author = {Zienkiewicz, O C and Taylor, R L},
title = {{Method for Solid and Structural Mechanics UNESCO Professor of Numerical Methods in Engineering}}
}
@article{Mohammadi2008b,
abstract = {A computational fluid dynamics (CFD) code is applied to simulate fluid flow, heat transfer and combustion in a four-stroke single cylinder engine with pent roof combustion chamber geometry, having two inlet valves and two exhaust valves. Heat flux and heat transfer coefficient on the cylinder head, cylinder wall, piston, intake and exhaust valves are determined with respect to crank angle position. Results for a certain condition are compared for total heat transfer coefficient of the cylinder engine with available correlation proposed by experimental measurement in the literature and close agreement are observed. It was found that the local value of heat transfer coefficient varies considerably in different parts of the cylinder, but they have equivalent trend with crank angle. Based on the results, new correlations are suggested to predict maximum and minimum convective heat transfer coefficient in the combustion chamber of a SI engine. ?? 2007 Elsevier Ltd. All rights reserved.},
author = {Mohammadi, A and Yaghoubi, M and Rashidi, M},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2008{\_}Mohammadi{\_}Analysis of local convective heat transfer in a spark ignition engine.pdf:pdf},
journal = {Int. Commun. Heat Mass Transf.},
keywords = {Combustion chamber,Heat flux,Heat transfer coefficient,SI engine},
number = {2},
pages = {215--224},
title = {{Analysis of local convective heat transfer in a spark ignition engine}},
volume = {35},
year = {2008}
}
@article{Fs2013,
author = {Fs},
doi = {10.1007/978-1-4614-0502-3},
isbn = {2009004043},
number = {1},
pages = {0--10},
title = {{Chapter 0}},
year = {2013}
}
@article{Strb,
author = {Str, Die},
pages = {1--6},
title = {{¨ Hrung}}
}
@article{Heinisch1994,
author = {Heinisch, Rudolf and Rogowski, Andreas and Sch{\"{u}}tt, Ehrenfried},
doi = {10.1007/BF02600863},
issn = {14340860},
journal = {Forsch. im Ingenieurwes. Eng. Res.},
number = {1},
pages = {29--35},
title = {{Der 1. Hauptsatz der Thermodynamik—ein Sonderfall der Energiebilanz}},
volume = {60},
year = {1994}
}
@article{Publishing2011,
author = {Publishing, Ebsco and Library, Sheffield},
isbn = {9780750663229},
pages = {1--27},
title = {{Introduction to the equations of fluid dynamics and the finite}},
year = {2011}
}
@book{Heywood,
author = {Heywood, John B.},
publisher = {Mcraw-Hill},
title = {{Internal Combustion Engine Fundamentals}},
year = {1988}
}
@article{Tarnopolskii1998,
author = {Tarnopol'skii, Yu.M. and Kulakov, V L},
isbn = {0-412-54020-7},
journal = {Handb. Compos.},
pages = {778--793},
title = {{Mechanical tests}},
year = {1998}
}
@article{Arnoldc,
author = {Arnold, J{\"{o}}rg and Braun, Marcel},
pages = {835--847},
title = {{C10 C10 Zuk{\{}{\"{u}}{\}}nftige Methoden bei der Spurensicherung C10 Neue M{\{}{\"{o}}{\}}glichkeiten und Bed{\{}{\"{u}}{\}}rfnisse}}
}
@article{Remy2002,
abstract = {The purpose of the paper is to show the successive steps of a numerical method for the predic-tion of crack initiation in industrial components submitted to thermo-mechanical fatigue. Finite element computations using realistic constitutive equations are first used to determine the stress and strain fields in the component. The constitutive equations account for cyclic viscoplasticity, creep, and aging effect. The industrial use of such theories requires robust integration techniques to reach the mechanical steady state. Since the real meshes have 10{\{}{\^{}}{\}}-10{\{}{\^{}}{\}} degrees of freedom, parallel computers are also needed. Damage models with creep-fatigue interaction are finally applied to determine crack initiation. The example of aluminum cylinder heads is chosen to illustrate the demonstration.},
author = {Remy, L and Petit, J and Nicouleau, E and Feyel, F and Quilici, S and Cailletaud, G},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/2002{\_}Nicouleau+Feyel{\_}STRUCTURAL CALCULATION AND LIFETIME-PREDICTION IN THERMOMECHANICAL FATIGUE OF ENGINE COMPONENTS.pdf:pdf},
keywords = {FE struc-tural calculation Cycle skip,Parallel computations,Thermomechanical fatigue,Viscoplastic modeling Aging effect Aluminum alloys},
title = {{Temperature-Fatigue Interaction STRUCTURAL CALCULATION AND LIFETIME- PREDICTION IN THERMOMECHANICAL FATIGUE OF ENGINE COMPONENTS}},
year = {2002}
}
@article{Bungartz2010,
abstract = {Stra{\{}{\ss}{\}}enverkehr geht uns alle an, jeder ist davon betroffen. Unsere W{\{}{\"{u}}{\}}nsche und Vorstellungen bez{\{}{\"{u}}{\}}glich des Stra{\{}{\ss}{\}}enverkehrs sind jedoch in der Regel etwas widerspr{\{}{\"{u}}{\}}chlich: Einerseits wollen wir m{\{}{\"{o}}{\}}glichst viel davon. Wir wollen mobil sein und so schnell und angenehm wie m{\{}{\"{o}}{\}}glich von der Wohnung zur Uni oder Arbeit, vom Heimatort zum Ferienziel oder vom Einkaufen zur Freizeitbesch{\{}{\"{a}}{\}}ftigung gelangen. Wir w{\{}{\"{u}}{\}}nschen uns dazu gut ausgebaute Stra{\{}{\ss}{\}}en und Parkpl{\{}{\"{a}}{\}}tze oder h{\{}{\"{a}}{\}}ufig fahrenden Personennahverkehr. Andererseits wollen wir m{\{}{\"{o}}{\}}glichst wenig davon. Stra{\{}{\ss}{\}}enverkehr soll uns nicht bel{\{}{\"{a}}{\}}stigen. Wir m{\{}{\"{o}}{\}}chten nicht im Berufsverkehr oder in den kilometerlangen Mammutstaus zu Ferienbeginn und -ende stehen, w{\{}{\"{u}}{\}}nschen uns, von L{\{}{\"{a}}{\}}rm- und Abgasemissionen unbehelligt zu bleiben, und bevorzugen Gr{\{}{\"{u}}{\}}nstreifen anstelle von Stra{\{}{\ss}{\}}enasphalt.},
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Bungartz and Zimmer and Buchholz and Pfl{\"{u}}ger},
doi = {10.1515/bmt.2010.712},
eprint = {arXiv:1011.1669v3},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Vorlesungen/Modellbildung{\_}und{\_}Simulation/Skript{\_}Modellbildung{\_}und{\_}Simulation.pdf:pdf},
isbn = {9783642054600},
issn = {0013-5585},
journal = {Biomed. Tech. Eng.},
keywords = {Stichw䣏rter des Dokuments},
number = {s1},
pages = {1--237},
pmid = {14685750},
title = {{Modellbildung und Simulation}},
volume = {55},
year = {2010}
}
@article{Geologie2009,
author = {Geologie, Allgemeine},
doi = {10.1007/978-3-540-92940-6},
isbn = {9783540929406},
pages = {1--36},
title = {{Kapitel 10}},
year = {2009}
}
@article{Lcmaitrc,
author = {Lcmaitrc, Cordchois},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Plasticity models/On Energy based coupled elastoplastic damage theories{\_}Ju1988.pdf:pdf},
title = {{1989-Ju{\_} On energy-based coupled elastoplastic damage theories{\_}constitutive modeling and computational aspects.pdf}}
}
@article{Sauer,
author = {Sauer, Bernd and Schraube, Wirkprinzip Der},
title = {{Kapitel 6}}
}
@article{Doudard2005,
abstract = {It is proposed to develop and identify a probabilistic two-scale model for HCF that accounts for the failure of samples, but also for the thermal effects during cyclic loadings in a unified framework. The probabilistic model is based on a Poisson point process. Within the weakest link theory, the model corresponds to a Weibull law for the fatigue limits. The thermal effects can be described if one considers the same hypotheses apart from the weakest link assumption. A method of identification is proposed and uses temperature measurements to identify the scatter in an S/N curve. The validation of the model is obtained by predicting S/N curves for different effective volumes of a dual-phase steel},
author = {Doudard, C and Calloch, S and Cugy, P and Galtier, A and Hild, F},
doi = {10.1111/j.1460-2695.2005.00854.x},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Surface effects + Frequency effects/A probabilistic two-scale model for high-cycle fatigue life predictions {\_} Doudard {\_} CACHEN{\_}Paris.pdf:pdf},
isbn = {8756758X (ISSN)},
issn = {8756758X},
journal = {Fatigue Fract. Eng. Mater. Struct.},
keywords = {Fatigue limits,Microplasticity,Thermomechanics,Weibull model},
number = {3},
pages = {279--288},
title = {{A probabilistic two-scale model for high-cycle fatigue life predictions}},
volume = {28},
year = {2005}
}
@article{Materialerma,
author = {Materialerm, Unter and Anrisse, Schwingspielzahl and Risse, Die and Gefahr, Die},
pages = {1--13},
title = {{Problem des Erm{\{}{\"{u}}{\}}dungsschadens}}
}
@article{Kr??mer2013,
author = {Kr??mer, Stephan and Rothe, Steffen and Hartmann, Stefan},
doi = {10.1007/s00366-013-0337-7},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Parametersch{\"{a}}tzung/2013{\_}Hartmann{\_}Homogeneous stress–strain states computed by 3D-stress algorithms of FE-codes - application to material parameter identification.pdf:pdf},
issn = {14355663},
journal = {Eng. Comput.},
keywords = {DAE-systems,Finite elements,Material parameter identification,Plane stress,Stress algorithms},
number = {1},
pages = {141--159},
title = {{Homogeneous stress???strain states computed by 3D-stress algorithms of FE-codes: application to material parameter identification}},
volume = {31},
year = {2013}
}
@article{Variablesa,
author = {Variables, Biowin State},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Probabilistic Aspects/A Unified Statistical Methodology for Modeling Fatigue Damage{\_}Castillo/Backmatter{\_}MitModelle.pdf:pdf},
pages = {1--72},
title = {{Models Used In BioWin}}
}
@article{Depcik2002e,
abstract = {In this paper, the available correlations proposed in the literature for the gas-side heat transfer in the intake and exhaust system of a spark-ignition internal combustion engine were surveyed. It was noticed that theseAB - {\textless}inline-graphic xlink:href="2002-01-0372{\_}fig0001" xmlns:xlink="http://www.w3.org/1999/xlink"/{\textgreater}AB - only by empirically fitted constants. This similarity provided the impetus for the authors to explore if a universal correlation could be developed. Based on a scaling approach using microscales of turbulence, the authors have fixed the exponential factor on the Reynolds number and thus reduced the number of adjustable coefficients to just one; the latter can be determined from a least squares curve-fit of available experimental data. Using intake and exhaust side data, it was shown that the universal correlationAB - {\textless}inline-graphic xlink:href="2002-01-0372{\_}fig0002" xmlns:xlink="http://www.w3.org/1999/xlink"/{\textgreater}AB - The correlation coefficient of this proposed heat transfer model with all available experimental data is 0.845 for the intake side and 0.800 for the exhaust side.ER -},
author = {Depcik, Christopher and Assanis, Dennis},
doi = {10.4271/2002-01-0372},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Heat transfer intake+exhaust system/2002{\_}Depcik{\_}A Universal Heat Transfer Correlation for intake and exhaust flows in an SI internal combustion engine.pdf:pdf},
journal = {SAE Pap.},
number = {January 2016},
title = {{A Universal Heat Transfer Correlation for Intake and Exhaust Flows in an Spark-Ignition Internal Combustion Engine}},
url = {http://papers.sae.org/2002-01-0372},
volume = {2002-01-03},
year = {2002}
}
@article{Ziel,
author = {Ziel, Nutzfahrzeugs Das and Ii, Dingo and Testrig, Camel-view},
journal = {Auslegung A Grad. J. Philos.},
pages = {117--136},
title = {{6 Dom{\"{a}}nen{\"{u}}bergreifende Modellbildung eines aktiv gefederten Nutzfahrzeugs ( CAMel-View TestRig )}}
}
@book{DeSouzaNeto2008,
abstract = {Two integration algorithms, namely the implicit return mapping and explicit sub-stepping schemes, are adopted in the anisotropic bounding surface plasticity model for cyclic behaviours of saturated clay and are implemented into finite element code. The model is a representative of a series of bounding surface models that have typical characteristics, including isotropic and kinematic hardening rules and a rotational bounding surface to capture complex but important cyclic behaviours of soils, such as cyclic shakedown and degradation. However, there is no explicit current yield surface in the model to which the conventional implicit algorithm returns the stress state back or the sub-stepping integration corrects the drift of the stress state. Hence, necessary modifications have been made for both of the integration schemes. First, the image stress point is mapped or corrected to the bounding surface instead of mapping back or correcting the stress state to the yield surface. Second, the unloading–loading criterion is checked to determine the image stress point rather than checking the yield criterion after giving the trial stress state in a conventional way. Comparative studies on the accuracy, stability and efficiency of the two integration schemes are conducted not only at the element level but also in solving boundary value problems of monotonic and cyclic bearing behaviours of rigid footings on saturated clay. For smaller strain increments, there is no significant difference in the accuracy between the two integration schemes, but the explicit integration shows a higher efficiency and accuracy. For relatively larger increments, the implicit return mapping algorithm presents good accuracy and more robustness, while the sub-stepping algorithm shows deteriorating accuracy and suffers the convergence problem. With the tolerance used in the present model, the bearing capacity of the rigid footing predicted by the return mapping algorithm is closer to the available analytical and numerical solutions, while the bearing capacity predicted by the sub-stepping algorithm shows a marginal increase.},
author = {{de Souza Neto}, E. A. and Peri, D. and Owen, D. R. J.},
doi = {10.1002/9780470694626},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Neto 2008 - Computational Methods for Plasticity.pdf:pdf},
isbn = {9780470694626},
issn = {0266352X},
title = {{Computational Methods for Plasticity}},
url = {http://doi.wiley.com/10.1002/9780470694626},
year = {2008}
}
@article{Depcik2002e,
abstract = {In this paper, the available correlations proposed in the literature for the gas-side heat transfer in the intake and exhaust system of a spark-ignition internal combustion engine were surveyed. It was noticed that theseAB - {\{}{\textless}{\}}inline-graphic xlink:href="2002-01-0372{\{}{\_}{\}}fig0001" xmlns:xlink="http://www.w3.org/1999/xlink"/{\{}{\textgreater}{\}}AB - only by empirically fitted constants. This similarity provided the impetus for the authors to explore if a universal correlation could be developed. Based on a scaling approach using microscales of turbulence, the authors have fixed the exponential factor on the Reynolds number and thus reduced the number of adjustable coefficients to just one; the latter can be determined from a least squares curve-fit of available experimental data. Using intake and exhaust side data, it was shown that the universal correlationAB - {\{}{\textless}{\}}inline-graphic xlink:href="2002-01-0372{\{}{\_}{\}}fig0002" xmlns:xlink="http://www.w3.org/1999/xlink"/{\{}{\textgreater}{\}}AB - The correlation coefficient of this proposed heat transfer model with all available experimental data is 0.845 for the intake side and 0.800 for the exhaust side.ER -},
author = {Depcik, Christopher and Assanis, Dennis},
doi = {10.4271/2002-01-0372},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2002{\_}Assanis{\_}A Universal Heat Transfer Correlation for Intake and Exhaust flows in an SI INternal Combustion Engine.pdf:pdf},
journal = {SAE Pap.},
number = {January 2016},
title = {{A Universal Heat Transfer Correlation for Intake and Exhaust Flows in an Spark-Ignition Internal Combustion Engine}},
url = {http://papers.sae.org/2002-01-0372},
volume = {2002-01-03},
year = {2002}
}
@article{Steffan1988,
author = {Steffan, Hermann and Moser, Andreas and Burg, Heinz and Dynamik, Die and Mechanik, Der},
journal = {Computer (Long. Beach. Calif).},
pages = {171--216},
title = {{A6 A6 Kinetik A6}},
year = {1988}
}
@article{Kratzsch2013,
author = {Kratzsch, Matthias and G{\"{u}}nther, Michael},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Klopfen{\_}Ottomotor/4. Internationale Tagung Ottomotorisches Klopfen - Berlin 12{\_}2013/Knocking+in+Gasoline+Engines.pdf:pdf},
pages = {445},
title = {{Knocking in Gasoline Engines}},
year = {2013}
}
@article{Cantrell2009,
author = {Cantrell, John H.},
doi = {10.1063/1.3254223},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2009{\_}Cantrell{\_}Ultrasonic harmonic generation from fatigue-induced dislocation substructures in planar slip metals and assessment of remaining fatigue life.pdf:pdf},
issn = {00218979},
journal = {J. Appl. Phys.},
number = {9},
title = {{Ultrasonic harmonic generation from fatigue-induced dislocation substructures in planar slip metals and assessment of remaining fatigue life}},
volume = {106},
year = {2009}
}
@article{Functions2003,
author = {Functions, Mathematical and Wiley, John},
title = {{Articles and Other Sources}},
volume = {2},
year = {2003}
}
@article{Remy2002a,
abstract = {The purpose of the paper is to show the successive steps of a numerical method for the predic-tion of crack initiation in industrial components submitted to thermo-mechanical fatigue. Finite element computations using realistic constitutive equations are first used to determine the stress and strain fields in the component. The constitutive equations account for cyclic viscoplasticity, creep, and aging effect. The industrial use of such theories requires robust integration techniques to reach the mechanical steady state. Since the real meshes have 10{\^{}}-10{\^{}} degrees of freedom, parallel computers are also needed. Damage models with creep-fatigue interaction are finally applied to determine crack initiation. The example of aluminum cylinder heads is chosen to illustrate the demonstration.},
author = {Remy, L and Petit, J and Nicouleau, E and Feyel, F and Quilici, S and Cailletaud, G},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/2002{\_}Nicouleau+Feyel{\_}STRUCTURAL CALCULATION AND LIFETIME-PREDICTION IN THERMOMECHANICAL FATIGUE OF ENGINE COMPONENTS.pdf:pdf},
keywords = {FE struc-tural calculation Cycle skip,Parallel computations,Thermomechanical fatigue,Viscoplastic modeling Aging effect Aluminum alloys},
title = {{Temperature-Fatigue Interaction STRUCTURAL CALCULATION AND LIFETIME- PREDICTION IN THERMOMECHANICAL FATIGUE OF ENGINE COMPONENTS}},
year = {2002}
}
@article{Metallplastizit2013a,
author = {Metallplastizit, Hrungdie and Helm, Dirk},
number = {November},
pages = {1--29},
title = {{Prozesssimulation in Der Umformtechnik}},
year = {2013}
}
@misc{Eshelby1951,
abstract = {The parallel between the classical theory of elasticity and the modern physical theory of the solid state is incomplete; the former has nothing analogous to the concept of the force acting on an imperfection (dislocation, foreign atom, etc.) in a stressed crystal lattice. To remedy this a general theory of the forces on singularities in a Hookean elastic continuum is developed. The singularity is taken to be any state of internal stress satisfying the equilibrium equations but not the compatibility conditions. The force on a singularity can be given as an integral over a surface enclosing it. The integral contains the elastic field quantities which would surround the singularity in an infinite medium, multiplied by the difference between these quantities and those actually present. The expression for the force is thus of essentially the same form whether the force is due to applied surface tractions, other singularities or the presence of the free surface of the body ({\{}'{\}}image force{\{}'{\}}). A region of inhomogeneity in the elastic constants modifies the stress field; if it is mobile one can define and calculate the force on it. The total force on the singularities and inhomogeneities inside a surface can be expressed in terms of the integral of a {\{}'{\}}Maxwell tensor of elasticity{\{}'{\}} taken over the surface. Possible extensions to the dynamical case are discussed.},
author = {Eshelby, J. D.},
booktitle = {Philos. Trans. R. Soc. A Math. Phys. Eng. Sci.},
doi = {10.1098/rsta.1951.0016},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/1951{\_}Eshelby{\_}The force oo an elastic singularity.pdf:pdf},
isbn = {00804614},
issn = {1364-503X},
number = {877},
pages = {87--112},
title = {{The Force on an Elastic Singularity}},
url = {http://rsta.royalsocietypublishing.org/cgi/doi/10.1098/rsta.1951.0016},
volume = {244},
year = {1951}
}
@article{Bridier2009a,
abstract = {Deformation micromechanisms of a Ti-6Al-4V alloy under fatigue loading at room temperature are studied using a three-dimensional crystal plasticity constitutive model. The model employs a minimum set of fitting parameters based on experimental data for Ti-6Al-4V. Single slip is strongly favored through a softening law that affects mainly the driving force for slip on the first activated slip system. Cyclic deformation behavior at the macroscopic scale and at the local scale of grains is analyzed through the simulation of 20 cycles of fatigue on a polycrystalline structure of 900 randomly oriented grains. The progressive activation of slip (basal, prismatic, and pyramidal) is analyzed and compared to experimental observations. {\textcopyright} 2008 Elsevier Ltd. All rights reserved.},
author = {Bridier, Florent and McDowell, David L. and Villechaise, Patrick and Mendez, Jos{\'{e}}},
doi = {10.1016/j.ijplas.2008.08.004},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2008{\_}Bridier{\_}Crystal plasticity modeling of slip activity in Ti–6Al–4V under high cycle fatigue loading.pdf:pdf},
isbn = {0749-6419},
issn = {07496419},
journal = {Int. J. Plast.},
keywords = {A. Microstructures,B. Anisotropic material,B. Crystal plasticity,B. Polycrystalline material,C. Finite elements},
number = {6},
pages = {1066--1082},
publisher = {Elsevier Ltd},
title = {{Crystal plasticity modeling of slip activity in Ti-6Al-4V under high cycle fatigue loading}},
url = {http://dx.doi.org/10.1016/j.ijplas.2008.08.004},
volume = {25},
year = {2009}
}
@article{Yildinm2015,
abstract = {This paper presents a simple PI tuning method for first order plus dead time (FOPDT) systems. Firstly, stabilizing PI parameters region is found for these kinds of systems. Then, optimal point of this region is selected using the Big Bang Big Crunch optimization algorithm and this work is extended to FOPDT systems that contain parameter uncertainty. After the optimizations done for a wide range of systems, an optimal and robust PI tuning method is proposed with a curve fitting of the obtained optimization data. Lastly, the proposed method is compared with other PI tuning methods for their performance and robustness.},
author = {Yildinm, Uʇur and Mutlu, Ilhan and S{\"{o}}ylemez, Mehmet T.},
doi = {10.1016/j.ifacol.2015.09.445},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Vorlesungen/Messtechnik+Regelungstechnik/2015{\_}Yildirim{\_}An Optimal Robust Tuning Method for First Order plus Dead Time Systems with Parameter Uncertainty.pdf:pdf},
issn = {24058963},
journal = {IFAC-PapersOnLine},
keywords = {Optimization,PI controllers,Robust control,Stabilizing controllers,Uncertain linear systems},
number = {14},
pages = {126--131},
title = {{An optimal robust tuning method for first order plus dead time systems with parameter uncertainty}},
volume = {28},
year = {2015}
}
@book{Ochsner2016,
author = {{\"{O}}chsner, Andreas},
doi = {10.1007/978-981-287-865-6},
isbn = {9789812878632},
title = {{Continuum Damage and Fracture Mechanics}},
year = {2016}
}
@book{Gross2011i,
author = {Gross, Dietmar and Seelig, Thomas},
doi = {10.1007/978-3-642-10196-0},
isbn = {978-3-642-10195-3},
title = {{Bruchmechanik}},
url = {http://link.springer.com/10.1007/978-3-642-10196-0},
year = {2011}
}
@inproceedings{2000-01-0564,
abstract = {Engine valve is one of the most important parts of an engine. In order to assess engine valve's reliability, it is necessary to predict its in-operation temperature distribution with a high degree of accuracy.Conventional methods for predicting a valve's temperature distribution had particularly poor generality and accuracy. After much testing, we have collected data on how valve temperature reacts to changing engine operating conditions. We learned from this data that the key factors in valve temperature distribution are ignition advance, air-fuel ratio, and engine speed. We were also able to use this data to optimize the heat release pattern and heat transmission coefficient used for predicting valve temperatures. This allowed us to make the prediction of valve temperature responsive to changes in engine operating conditions, general, and highly accurate. In this paper we discuss gasoline engines; this system is also applicable to diesel engines, but we believe that further testing and evaluation will be required before we can proceed with implementation.},
author = {Yang, L C and Hamada, A and Ohtsubo, K},
booktitle = {SAE Tech. Pap.},
doi = {10.4271/2000-01-0564},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Heat transfer intake+exhaust system/2000{\_}Yang+Hamada{\_}Engine Valve Temperature Simulation System.pdf:pdf},
publisher = {SAE International},
title = {{Engine Valve Temperature Simulation System}},
url = {https://doi.org/10.4271/2000-01-0564},
year = {2000}
}
@article{Cantrell2009a,
author = {Cantrell, John H.},
doi = {10.1063/1.3254223},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2009{\_}Cantrell{\_}Ultrasonic harmonic generation from fatigue-induced dislocation substructures in planar slip metals and assessment of remaining fatigue life.pdf:pdf},
issn = {00218979},
journal = {J. Appl. Phys.},
number = {9},
title = {{Ultrasonic harmonic generation from fatigue-induced dislocation substructures in planar slip metals and assessment of remaining fatigue life}},
volume = {106},
year = {2009}
}
@article{Burgh,
author = {Burg, Heinz and Reaktionspunktes, Festlegung},
pages = {251--260},
title = {{A8 A8 Vermeidbarkeitsbetrachtungen A8}}
}
@article{Federungskomfort2007,
author = {Federungskomfort, Den},
journal = {Fahrzeuggetriebe},
title = {{6 Systematik der Fahrzeuggetriebe : Konstruktive Grundkonzepte}},
year = {2007}
}
@article{Evert2006a,
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Evert, Ray F},
doi = {10.1002/0470047380.indauth},
eprint = {arXiv:1011.1669v3},
isbn = {9780470047385},
issn = {15672719},
journal = {Esau's Plant Anat.},
pages = {541--566},
pmid = {20348824},
title = {{Author Index}},
url = {http://dx.doi.org/10.1002/0470047380.indauth},
year = {2006}
}
@article{Loubar2005b,
abstract = {This paper deals with the transient thermal signal around an engine cylinder in order to propose a new and nonintrusive method of knock detection. Numerical simulations of unsteady heat transfer through the cylinder and inside the coolant flow are carried out to account for heat flux variations due to normal and knocking combustion. The effect of rib roughened surfaces on thermal signal amplification is investigated. The geometric parameters are fixed at Pi/h=70 and w/h=1 with a Reynolds number based on hydraulic diameter of 12,000. The results reveal that square ribs give better performance in term of thermal signal amplification within the fluid. An amplification of the temperature variation up to 20 times higher is found. Finally, flow analysis shows that amplification depends on the position where the thermal signal is collected.},
author = {Loubar, Khaled and Bellettre, Jérôme and Tazerout, Mohand},
doi = {10.1115/1.1857943},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2005{\_}Loubar{\_}Unsteady Heat Transfer enhancement around an engine cylinder in order to detect knockpdf.pdf:pdf},
isbn = {0022-1481},
issn = {00221481},
journal = {J. Heat Transf.},
number = {3},
pages = {278},
title = {{Unsteady Heat Transfer Enhancement Around an Engine Cylinder in Order to Detect Knock}},
url = {http://heattransfer.asmedigitalcollection.asme.org/article.aspx?articleid=1447711},
volume = {127},
year = {2005}
}
@article{YILDIRIM2015,
annote = {8th IFAC Symposium on Robust Control Design ROCOND 2015},
author = {Yildirim, Ugur and Mutlu, Alhan and S{\"{o}}ylemez, Mehmet T},
doi = {https://doi.org/10.1016/j.ifacol.2015.09.445},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Vorlesungen/Messtechnik+Regelungstechnik/2015{\_}Yildirim{\_}An Optimal Robust Tuning Method for First Order plus Dead Time Systems with Parameter Uncertainty.pdf:pdf},
journal = {IFAC-PapersOnLine},
keywords = {PI controllers,optimization,robust control,stabilizing controllers,uncertain linear systems},
number = {14},
pages = {126--131},
title = {{An Optimal Robust Tuning Method for First Order plus Dead Time Systems with Parameter Uncertainty}},
volume = {48},
year = {2015}
}
@incollection{Nicouleau2002,
author = {Nicouleau, E and Feyel, F and Quilici, S and Cailletaud, G},
booktitle = {Temp. Interact.},
doi = {https://doi.org/10.1016/S1566-1369(02)80089-9},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/2002{\_}Nicouleau+Feyel{\_}STRUCTURAL CALCULATION AND LIFETIME-PREDICTION IN THERMOMECHANICAL FATIGUE OF ENGINE COMPONENTS.pdf:pdf},
keywords = {Aging effect,Aluminum alloys,Cycle skip,F.E. structural calculation,Parallel computations,Thermomechanical fatigue,Viscoplastic modeling},
number = {Supplement C},
pages = {331--340},
series = {European Structural Integrity Society},
title = {{Structural calculation and lifetime-prediction in thermomechanical fatigue of engine components}},
volume = {29},
year = {2002}
}
@article{Energie,
author = {Energie, Kinetische and Energie, Potenzielle and Energie, Elektrische and Energie, Thermische and Mikrowellen, Energie and Energie, Innere},
pages = {5--13},
title = {{2 Energietechnische Grundlagen}}
}
@book{DanielGhebru2013,
author = {{Daniel Ghebru}, Dipl-Ing and {Ulrich Spicher Korreferent}, Dr-Ing and techn {Andreas Wimmer Korreferent} and sc {techn Thomas Koch}},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2009{\_}GhebruDaniel{\_}Modellierung und Analyse des instationaeren thermischen Verhaltens von VKM und Gesamtfahrzeug - Beitrag Woschni+Zapf.pdf:pdf},
isbn = {9783832534325},
keywords = {Co-Simulation,Instation{\"{a}}res Thermomanagement,Modellbildung,Thermische Gesamtfahrzeugsimulation,Thermisches Motormodell},
number = {April},
title = {{Modellierung und Analyse des instation{\"{a}}ren thermischen Verhaltens von Verbrennungsmotor und Gesamtfahrzeug}},
year = {2013}
}
@article{General1971,
author = {General, The and Model, Linear},
doi = {10.1016/B978-0-12-627865-1.00015-5},
isbn = {9780126278651},
title = {15 15.1},
year = {1971}
}
@article{Eiamsa-Ard2010,
abstract = {The article presents an investigation of the effect of twisted tape with serrated-edge insert on heat transfer and pressure loss behaviors in a constant heat-fluxed tube. In the experiments, the serrated twisted tape (STT) was inserted into the entire test tube with a constant twist ratio in order to generate a continuous swirling airflow. Two geometry parameters of the STT to be considered in the present work are the serration width ratio and the serration depth ratio. The measurements have been conducted for the airflow rate based on Reynolds numbers in the turbulent regime from 4000 to 20,000. The experimental results of the STT inserted tube are compared with those of the plain tube fitted with typical twisted tape (TT). The results show that the heat transfer rate in terms of Nusselt number, Nu increases with the rise in the depth ratio but decreases with raising the width ratio. The heat transfer rate is up to 72.2{\{}{\%}{\}} and 27{\{}{\%}{\}} relative to the plain tube and the TT inserted tube, respectively. The use of the STT leads to higher heat transfer rate and friction factor than that of the TT for all cases. The thermal performance factor of the STT tube under constant pumping power is evaluated and found to be above unity indicating that using the STT tube is advantageous over the TT tube or the plain tube. In addition, the empirical correlations developed by relating the serration width ratio, serration depth ratio and Reynolds number are determined. ?? 2010 Elsevier Ltd. All rights reserved.},
author = {Eiamsa-Ard, Smith and Promvonge, Pongjet},
doi = {10.1016/j.applthermaleng.2010.03.026},
journal = {Appl. Therm. Eng.},
keywords = {Friction factor,Heat transfer,Serrated twisted tape,Swirl flow,Typical twisted tape},
number = {13},
pages = {1673--1682},
title = {{Thermal characteristics in round tube fitted with serrated twisted tape}},
volume = {30},
year = {2010}
}
@article{Schraubenver-,
author = {Schraubenver-, Anziehen Der},
pages = {784--802},
title = {{Sachwortverzeichnis}}
}
@article{Hauptsatz2011,
author = {Hauptsatz, Erster},
doi = {10.1007/978-3-8348-9903-3},
isbn = {9783834899033},
pages = {60--84},
title = {{4 Energien 4.1}},
year = {2011}
}
@article{Bohlke2012a,
author = {B{\"{o}}hlke, Prof Thomas},
journal = {Mechanik},
number = {September},
title = {{Skript zur Vorlesung H{\{}{\"{o}}{\}}here Technische Festigkeitslehre}},
year = {2012}
}
@article{Massenkraft,
author = {Massenkraft, Der and Massenkraft, Der and Dichte, Der and Dichte, Der},
journal = {Entropie},
title = {{5 Hydrostatik 5.1}}
}
@article{Tanaka1981,
abstract = {The effects of grain size and crack length on the threshold condition of fatigue growth of small cracks are analysed both theoretically and experimentally. The theoretical model is based on the assumption that the threshold condition is determined by whether the crack-tip slip band blocked by the grain boundary propagates into an adjacent grain or not. By comparing the model analysis with the experiments of mild steel, it was found that the threshold stress estimated from the fatigue limit of the smooth specimen gave the effective components of the applied stress. When the threshold stress normalized by the fatigue limit of the smooth specimen was correlated to the crack length normalized by a certain crack length, the theoretical relation was found to agree well with the experimental data. From a further analysis of the published data of various materials, the theoretical normalized relation was found to give a lower bound of the threshold values of the stress and the stress intensity factor. A deviation from the theoretical relation seen in the cases of hard metals was explained through an extension of the model by regarding that hard metals contained initial, inherent flaws even in the smooth specimen.},
author = {Tanaka, K. and Nakai, Y. and Yamashita, M.},
doi = {10.1007/BF00033345},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/1981{\_}Tanaka{\_}Fatigue growth threshold of small cracks.pdf:pdf},
isbn = {0376-9429},
issn = {03769429},
journal = {Int. J. Fract.},
number = {5},
pages = {519--533},
title = {{Fatigue growth threshold of small cracks}},
volume = {17},
year = {1981}
}
@article{Reifen,
author = {Reifen, Der},
title = {{2 Der Reifen}}
}
@article{Fahrzeughersteller,
author = {Fahrzeughersteller, Der},
title = {{Anhang : Hinweise und Bedienungsanleitung}}
}
@article{Kontinuumsmechanik2013,
author = {Kontinuumsmechanik, Grundlagen D E R},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/{\_}skripte/Helm - Prozesssimulation und Umformtechnik/Presentation3{\_}Kontinuumsmechanik.pdf:pdf},
number = {November},
pages = {1--46},
title = {{Prozesssimulation in Der Einf{\"{u}}hrung in Die Mathematischen}},
year = {2013}
}
@article{Moser,
author = {Moser, Andreas and Steffan, Hermann},
journal = {Simulation},
pages = {559--568},
title = {{A18 A18 Insassensimulation A18}}
}
@article{Temperaturgradienten,
author = {Temperaturgradienten, Nicht and Wellenl, Diese and Auffinden, Das and Abschnitt, Im},
title = {{W ¨ armestrahlung}}
}
@article{Foundations2003a,
author = {Foundations, Mathematical},
pages = {25--42},
title = {{Mathematical Foundations: Tensors 2.1}},
year = {2003}
}
@book{Ibrahimbegovic2009,
abstract = {This volume provides insight into modelling and ultimate limit computation$\backslash$nof complex structures, with their components represented by solid$\backslash$ndeformable bodies. The book examines practically all the important$\backslash$nquestions of current interests for nonlinear solid mechanics: plasticity,$\backslash$ndamage, large deformations, contact, dynamics, instability, localisation$\backslash$nand failure, discrete models, multi-scale, multi-physics and parallel$\backslash$ncomputing, with special attention given to finite element solution$\backslash$nmethods. The presentation of topics is structured around different$\backslash$naspects of typical boundary value problems in nonlinear solid mechanics,$\backslash$nwhich provides the best pedagogical approach while keeping the book$\backslash$nsize reasonable despite its very broad contents. Other strong points$\backslash$nare the exhaustive treatment of subjects, with each question studied$\backslash$nfrom different angles of mechanics, mathematics and computation,$\backslash$nas well as a successful merger of scientific cultures and heritage$\backslash$nfrom Europe and the USA. The book content and style is also the product$\backslash$nof rich international experience in teaching Master and Doctoral$\backslash$nlevel courses, as well as the courses organized for participants$\backslash$nfrom industry (IPSI courses) in France, and similar courses in Germany$\backslash$nand Italy. Every effort was made to make the contents accessible$\backslash$nto non-specialists and users of computer programs.},
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Ibrahimbegovic, Adnan},
booktitle = {Solid Mech. its Appl.},
doi = {10.1007/978-90-481-2331-5_1},
eprint = {arXiv:1011.1669v3},
isbn = {9789048123308},
issn = {09250042},
pages = {1--594},
pmid = {25246403},
title = {{Nonlinear solid mechanics}},
volume = {160},
year = {2009}
}
@article{Zienkiewicz2014g,
abstract = {Mutations in the human L1CAM gene cause neurodevelopmental disorders collectively referred to as L1 syndrome. Here, we investigated cellular pathomechanisms underlying two L1 syndrome mutations, R184Q and W1036L. We demonstrate that these mutations cause partial endoplasmic reticulum (ER) retention of L1, reduce L1 cell surface expression, but do not induce ER stress in neuronal NSC-34 cells. We provide evidence that surface trafficking of mutated L1 is affected by defective sorting to ER exit sites and attenuated ER export. However, in differentiated neuronal cultures and long-term cultured hippocampal slices, the L1-R184Q protein is restricted to cell bodies, whereas L1-W1036L also aberrantly localizes to dendrites. These trafficking defects preclude axonal targeting of L1, thereby affecting L1-mediated axon growth and arborization. Our results indicate that L1 syndrome mutations impair neuronal L1 function at different levels, firstly by attenuating ER export and secondly by interfering with polarized neuronal trafficking.},
author = {Zienkiewicz, O.C. and Taylor, R.L. and Nithiarasu, P.},
doi = {10.1016/B978-1-85617-635-4.00015-7},
isbn = {9781856176354},
journal = {Finite Elem. Method Fluid Dyn.},
number = {1},
pages = {485--491},
title = {{Computer Implementation of the CBS Algorithm}},
url = {http://linkinghub.elsevier.com/retrieve/pii/B9781856176354000157},
year = {2014}
}
@article{Tanaka1982b,
abstract = {The fatigue crack initiation along the slip banks emanating from notches is analyzed theoretically with the use of the dislocation dipole accumulation model proposed previously by the authors. The complex function analysis for an elliptical notch under the anti-plane shear gives a quantitative method for assessment of the reduction of fatigue strength as a function of the notch tip radius, the notch size and the elastic stress concentration factor. Special cases of this theoretical analysis yield several semi-empirical formulae commonly used by engineers for data collection. In the derivation, the limitations for each engineering approach are clarified. The material properties are included in the present micromechanical theory as the slip band length and the dislocation frictional stress. ?? 1982.},
author = {Tanaka, K. and Mura, T.},
doi = {10.1016/0167-6636(82)90024-2},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/1981{\_}Mura+Tanaka{\_}A micromechanical theory of fatigue crack initiation from notches.pdf:pdf},
isbn = {0921-5093},
issn = {01676636},
journal = {Mech. Mater.},
number = {1},
pages = {63--73},
title = {{A micromechanical theory of fatique crack initiation from notches}},
volume = {1},
year = {1982}
}
@article{Foundations2003,
author = {Foundations, Mathematical},
pages = {1--23},
title = {and},
year = {2003}
}
@article{Verger2002,
abstract = {This paper presents a global approach of thermomechanical design in the automotive industry. The three steps of the method are the following: the loading definition, the modelling of the constitutive law, a failure criterion. Cracked area and lifetime prediction are described in the case of aluminium alloy cylinder heads submitted to transient thermal loadings. The main hypothesis and modelling choices are presented and results are illustrated by a series of computations on real 3D structures. {\{}{\textcopyright}{\}} 2002 Elsevier Ltd. All rights reserved.},
author = {Verger, L and Constantinescu, A and Charkaluk, E},
doi = {10.1016/S1566-1369(02)80087-5},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Kriechen{\_}Spannungsrelaxation/2002{\_}Verger{\_}THERMOMECHANICAL FATIGUE DESIGN OF ALUMINIUM COMPONENTS.pdf:pdf},
issn = {15661369},
journal = {Eur. Struct. Integr. Soc.},
number = {C},
pages = {309--318},
title = {{Thermomechanical fatigue design of aluminium components}},
volume = {29},
year = {2002}
}
@article{Ruzzene2009,
abstract = {This article presents an overview of damage measures proposed in the area of structural health monitoring. This is an extremely active, open, and vast research field, as demonstrated by the variety of topics presented in this encyclopedia. The direction taken in this article is to present some examples of techniques that have been proposed, or that are promising tools for the estimation of location and extent of structural damage. All of the techniques considered are based on the analysis of the dynamic response of the structure under consideration. The organization of the article is based on the frequency range of analysis, which spans the low-frequency range, and correspondingly long response times, associated with the modal analysis of the structure, to frequencies associated with the propagation of guided ultrasonic waves. Hence, the methods presented belong to the classes of vibration-based and guided waves-based techniques. The damage measures discussed rely on the estimation of changes in modal parameters of the structure (natural frequencies, mode shapes, and strain energy distributions), or on features associated with the signal corresponding to the measured dynamic response. This overview is not meant to be exhaustive, but rather it provides examples of interesting solutions and approaches proposed in this area.},
author = {Ruzzene, M},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Probabilistic Aspects/A Unified Statistical Methodology for Modeling Fatigue Damage{\_}Castillo/Kap6{\_}Damage Measures.pdf:pdf},
isbn = {978-0-470-05822-0},
journal = {Encycl. Struct. Heal. Monit.},
keywords = {damage measures,guided ultrasonic waves,vibration-based technique},
number = {48},
pages = {--},
title = {{Damage measures}},
year = {2009}
}
@article{Apparaten,
author = {Apparaten, Berechnung Von},
title = {{Verdampfung}}
}
@article{Kadija1993,
author = {Kadija, K. and Martinis, M.},
doi = {10.1103/PhysRevD.48.2027},
isbn = {1550-7998},
issn = {05562821},
journal = {Phys. Rev. D},
number = {5},
pages = {2027--2034},
pmid = {10016439},
title = {{Inelasticity distribution and relationship between e+e- and pp hadron-production mechanisms}},
volume = {48},
year = {1993}
}
@article{Galindo-Nava2012,
abstract = {A new theory for describing plastic deformation in metals is presented. The approach focuses on obtaining an expression for the dislocation recovery term in terms of the energy barrier for dislocation annihilation, ?????. G???. This term is obtained from the contributions of dislocation formation and migration, the statistical entropy inherent to the annihilation process, and the chemical work due to the presence of vacancies. It is shown that at high temperatures, vacancy migration features strongly in dislocation recovery via a climb-assisted process. Employing only input parameters reported in the literature, the theory is able to reproduce experimental stress-strain relationships at temperatures ranging from cryogenic conditions to near-melting temperatures for Cu, Al, Ni and Ag at a variety of strain rates. It is demonstrated that low temperature cross-slip can operate at higher temperatures by increasing the strain rate, and that high temperature dislocation climb can feature at low temperatures by reducing the vacancy migration energy. ?? 2012 Elsevier B.V..},
author = {Galindo-Nava, E. I. and Rivera-D??az-del-Castillo, P. E J},
doi = {10.1016/j.msea.2012.02.055},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Kriechen{\_}Spannungsrelaxation/2012{\_}Galindo-Nava+Castillo{\_}A thermostatistical theory of low and high temperature deformation in metals.pdf:pdf},
isbn = {0921-5093},
issn = {09215093},
journal = {Mater. Sci. Eng. A},
keywords = {Dislocations,Hardening,Non-ferrous alloys,Plasticity},
pages = {110--116},
publisher = {Elsevier B.V.},
title = {{A thermostatistical theory of low and high temperature deformation in metals}},
url = {http://dx.doi.org/10.1016/j.msea.2012.02.055},
volume = {543},
year = {2012}
}
@article{Hauptteil,
author = {Hauptteil, Der and Technik, Rem-kl and Mikroskopie, Rem-kl and Vordergrund, Im and Mikroskopie, Kl- and Untersuchungen, Dynamische Rem-kl and Cdte, Mit and Bestandteil, Wichtiger and Versetzungen, Material},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/Crystall Plasticity Basics/Beitrag{\_}zur{\_}Versetzungsdynamik.pdf:pdf},
pages = {59--89},
title = {{Untersuchungen zur Versetzungsdynamik}}
}
@article{Kirchner2007,
abstract = {Vorwort$\backslash$r$\backslash$n$\backslash$r$\backslash$nEigentlich sollte man annehmen, dass nach mehr als 100 Jahren Automobilbau$\backslash$r$\backslash$n$\backslash$r$\backslash$nalles ¨uber die Leistungs¨ubertragung in Fahrzeuggetrieben in schriftlicher$\backslash$r$\backslash$n$\backslash$r$\backslash$nForm dokumentiert ist. Aber weit gefehlt: Das Fahrzeuggetriebe besch¨aftigt$\backslash$r$\backslash$n$\backslash$r$\backslash$nmehr denn je die Ingenieure in Forschung und Entwicklung, um unter dem$\backslash$r$\backslash$n$\backslash$r$\backslash$nDruck der Selbstverpflichtung der Automobilindustrie das technisch und ¨okonomisch$\backslash$r$\backslash$n$\backslash$r$\backslash$nM¨ogliche zur Senkung von Kraftstoffverbrauch und CO2-Aussto{\ss} bei$\backslash$r$\backslash$n$\backslash$r$\backslash$ngleichzeitiger Steigerung der Tragf¨ahigkeit zu leisten.$\backslash$r$\backslash$n$\backslash$r$\backslash$nDas Manuskript zu diesem Buch entsteht also mitten in einer Zeit, in der die$\backslash$r$\backslash$n$\backslash$r$\backslash$nAutomobilwirtschaft mit gro{\ss}em technischen Ehrgeiz nach neuen technischen$\backslash$r$\backslash$n$\backslash$r$\backslash$nM¨oglichkeiten zur Reduktion des Kraftstoffverbrauchs bei gleichzeitiger Beibehaltung$\backslash$r$\backslash$n$\backslash$r$\backslash$nder ¨ublichen Fahrleistungen sucht. Zeitgleich haben Kostendruck$\backslash$r$\backslash$n$\backslash$r$\backslash$nund Aufgabenteilung in der Entwicklung ein bisher noch nicht bekanntes Niveau$\backslash$r$\backslash$n$\backslash$r$\backslash$nerreicht. Hinzu kommen die Anforderungen des Kunden nach immer$\backslash$r$\backslash$n$\backslash$r$\backslash$nkomfortableren, robusten Getrieben, die ihn begeistern und nicht nur zufriedenstellen.$\backslash$r$\backslash$n$\backslash$r$\backslash$nDer Aspekt der Kundensicht und mit ihm die vielf¨altigen Fragestellungen$\backslash$r$\backslash$n$\backslash$r$\backslash$nnach komfortrelevanten Ph¨anomenen verbunden mit einem soliden ¨Uberblick$\backslash$r$\backslash$n$\backslash$r$\backslash$n¨uber konstruktive und entwicklungsmethodische Grundz¨uge der Fahrzeuggetriebe$\backslash$r$\backslash$n$\backslash$r$\backslash$nwar meine urspr¨ungliche Motivation f¨ur dieses Buch. Es entstand auf$\backslash$r$\backslash$n$\backslash$r$\backslash$nder Grundlage einer Vorlesung, die ich f¨ur Studierende des Maschinenbaus$\backslash$r$\backslash$n$\backslash$r$\backslash$nhalte; die positiven R¨uckmeldungen zum Inhalt der Vorlesung haben das Entstehen$\backslash$r$\backslash$n$\backslash$r$\backslash$ndieses Buches vorangetrieben.$\backslash$r$\backslash$n$\backslash$r$\backslash$nDie Zielgruppe dieses Buches ist somit in meinem ehemaligen T¨atigkeitsbereich$\backslash$r$\backslash$n$\backslash$r$\backslash$n? der Fahrzeug- und insbesondere in der Getriebeentwicklung ? zu suchen;$\backslash$r$\backslash$n$\backslash$r$\backslash$nes ist als Einf¨uhrungs- und Nachschlagewerk gleicherma{\ss}en konzipiert.$\backslash$r$\backslash$n$\backslash$r$\backslash$nHinzu kommen als potentielle Leser die Studierenden an den deutschsprachigen$\backslash$r$\backslash$n$\backslash$r$\backslash$ningenieurwissenschaftlichen Fakult¨aten, die sich f¨ur den Antrieb von$\backslash$r$\backslash$n$\backslash$r$\backslash$nKraftfahrzeugen interessieren. Die Ausf¨uhrungen und Auslegungsrichtlinien$\backslash$r$\backslash$n$\backslash$r$\backslash$nsind jeweils f¨ur einen Erstentwurf und dessen Dimensionierung der verschiedenen$\backslash$r$\backslash$n$\backslash$r$\backslash$nGetriebekonzepte und ihrer Komponenten umfangreich genug, f¨ur die$\backslash$r$\backslash$n$\backslash$r$\backslash$nOptimierung der Einzelteile werden viele Hinweise auf tiefergehende Quellen$\backslash$r$\backslash$n$\backslash$r$\backslash$ngegeben. Auf den Einsatz einer speziellen Software wurde ganz bewusst verzichtet,$\backslash$r$\backslash$n$\backslash$r$\backslash$nalle Auslegungsaufgaben und Beispiele sind mit dem Taschenrechner$\backslash$r$\backslash$n$\backslash$r$\backslash$noder einem einfachen Tabellenkalkulationsprogramm l¨osbar. Die ausf¨uhrlichen$\backslash$r$\backslash$n$\backslash$r$\backslash$nL¨osungen zu den enthaltenen Auslegungsfragen stelle ich gerne auf Anfrage$\backslash$r$\backslash$n$\backslash$r$\backslash$nzur Verf¨ugung.$\backslash$r$\backslash$n$\backslash$r$\backslash$nZumindest indirekt geholfen beim Entstehen haben viele ehemalige Kollegen,$\backslash$r$\backslash$n$\backslash$r$\backslash$nmit denen ich viele der hier zusammengetragenen Fakten diskutieren konnte;$\backslash$r$\backslash$n$\backslash$r$\backslash$nnamentlich genannt seien ? stellvertretend ? Georg Bednarek, Friedhelm$\backslash$r$\backslash$n$\backslash$r$\backslash$nKrake, Josef Hau und J¨org B¨onning (Alle GM Powertrain Europe) aber auch$\backslash$r$\backslash$n$\backslash$r$\backslash$nDr. Klaus Kalmbach, Dr. Peter Werth, Thomas Hackl, Ulf Polzin und Patrick$\backslash$r$\backslash$n$\backslash$r$\backslash$nVikari, alle hofer powertrain GmbH. Die letztgenannten Herren, ihre Begeisterung$\backslash$r$\backslash$n$\backslash$r$\backslash$nund ihr Wissen um die Thematik haben viele Punkte einflie{\ss}en lassen,$\backslash$r$\backslash$n$\backslash$r$\backslash$ndie hier zusammengetragen sind. Dar¨uber hinaus hat die hofer powertrain$\backslash$r$\backslash$n$\backslash$r$\backslash$nGmbH mir die Einbindung der Bilder in Farbe erm¨oglicht und stand meinen$\backslash$r$\backslash$n$\backslash$r$\backslash$nBildw¨unschen immer aufgeschlossen gegen¨uber.$\backslash$r$\backslash$n$\backslash$r$\backslash$nViele wertvolle Denkanst¨o{\ss}e zur Darstellung einzelner Fragestellungen habe$\backslash$r$\backslash$n$\backslash$r$\backslash$nich von Herrn Prof. Dr.-Ing. B. Sauer, TU Kaiserslautern erhalten; zu nennen$\backslash$r$\backslash$n$\backslash$r$\backslash$nist hier beispielsweise die explizite Auseinandersetzung mit den Wirkprinzipien$\backslash$r$\backslash$n$\backslash$r$\backslash$nmechanischer Leistungs¨ubertragung direkt in der Einleitung.$\backslash$r$\backslash$n$\backslash$r$\backslash$nWeiterhin m¨ochte ich mit bei einer Reihe von Studierenden bedanken, die im$\backslash$r$\backslash$n$\backslash$r$\backslash$nRahmen von Studien- und Diplomarbeiten Bausteine zu abgeschlossenen Themen$\backslash$r$\backslash$n$\backslash$r$\backslash$nerarbeitet und so zu diesem Buch beigetragen haben. Genannt seien hier$\backslash$r$\backslash$n$\backslash$r$\backslash$nFrau Rike Grotepass sowie die Herren Rene Johne, Hagen Plisch, Tillmann$\backslash$r$\backslash$n$\backslash$r$\backslash$nSch¨afer, Martin S¨anger, Christian Lunkenheimer, Florian Herbold, Matthias$\backslash$r$\backslash$n$\backslash$r$\backslash$nReimann und Christian Hamann. Die Herren Dr.-Ing. Andreas Laschet (Arla$\backslash$r$\backslash$n$\backslash$r$\backslash$nMaschinentechnik, K¨urten) und Dr. Jan Schlipf (GIF GmbH, Alsdorf) sowie$\backslash$r$\backslash$n$\backslash$r$\backslash$ndie Firmen GM Powertrain Europe, DaimlerChrysler, BMW, ZF Zahnradfabrik$\backslash$r$\backslash$n$\backslash$r$\backslash$nFriedrichshafen, Voith Turbo Systems, ElringKlinger, H¨orbiger Antriebstechnik,$\backslash$r$\backslash$n$\backslash$r$\backslash$nLuK, INA, Jopp, MagnaSteyr und AGCO haben mir Material zur$\backslash$r$\backslash$n$\backslash$r$\backslash$nVerf¨ugung gestellt. Ich bitte um Nachsicht, wenn ich jemanden vergessen haben$\backslash$r$\backslash$n$\backslash$r$\backslash$nsollte, der zu diesem Buch beigetragen hat.$\backslash$r$\backslash$n$\backslash$r$\backslash$nDem Springer Verlag, insbesondere Herrn Dr.-Ing. B. Gebhardt, danke ich f¨ur$\backslash$r$\backslash$n$\backslash$r$\backslash$ndie gute konstruktive Zusammenarbeit und die Unterst¨utzung bei der Wahl$\backslash$r$\backslash$n$\backslash$r$\backslash$nder Schwerpunkte dieses Buchs.$\backslash$r$\backslash$n$\backslash$r$\backslash$nEs bleibt ein riesiges Danke an meine Frau Dr. Nina Kirchner f¨ur ihre Hilfe$\backslash$r$\backslash$n$\backslash$r$\backslash$nbeim Korrekturlesen und ihre vielen Verbesserungsvorschl¨age sowie meinen$\backslash$r$\backslash$n$\backslash$r$\backslash$nKindern f¨ur ihr Verst¨andnis, wenn ich am Manuskript gearbeitet habe anstatt$\backslash$r$\backslash$n$\backslash$r$\backslash$nmit ihnen zu spielen. Mir hat es Spass gemacht, mein Wissen zum Thema Getriebe$\backslash$r$\backslash$n$\backslash$r$\backslash$nsoweit m¨oglich niederzuschreiben; ich hoffe, dass man das merkt.$\backslash$r$\backslash$n$\backslash$r$\backslash$nSaulheim bei Mainz, im Mai 2007 Eckhard Kirchner},
author = {Kirchner, Eckhard},
doi = {10.1007/978-3-540-35292-1},
isbn = {9783540352884},
journal = {Zhurnal Eksp. i Teor. Fiz.},
pages = {699},
title = {{Leistungs{\"{u}}bertragung in Fahrzeuggetrieben}},
year = {2007}
}
@article{Tsurushima2002,
abstract = {One of the problems in HCCI combustion is a knocking in higher load conditions. It governs the high load limit, and it is suggested that the knock increases heat loss[1], because it breaks the thermal boundary layer. But it is not clear how much knock affects on heat loss in the HCCI combustion in various conditions, such as ignition timing and load. The motivation of this study is to clarify the ratio of heat loss caused by knock in HCCI engines. The heat loss from zero-dimensional calculations with modified heat transfer coefficient, which is considering the effect of knock by adding a term of cylinder pressure rising rate dp/dt, agreed well with the results from the thermodynamic analysis in various conditions. And the results show that it is possible to avoid heat loss by knock by controlling the ignition timing at appropriate timing after T.D.C. and it will be possible to expand the load range if knock can be avoided. Copyright {\{}{\textcopyright}{\}} 2002 Society of Automotive Engineers, Inc.},
author = {Tsurushima, T and Kunishima, E and Asaumi, Y and Aoyagi, Y and Enomoto, Y},
doi = {10.4271/2002-01-0108},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2002{\_}Tsurushima{\_}The Effect of Knock on Heat Loss in HCCI Engines-Modified Woschni.pdf:pdf},
journal = {SAE Tech. Pap.},
number = {724},
title = {{The effect of knock on heat loss in homogeneous charge compression ignition engines}},
volume = {2002},
year = {2002}
}
@article{Betrachtungenc,
author = {Betrachtungen, Allgemeine},
title = {{omungen kleiner Reynolds-Zahlen}}
}
@article{Ruzzene2009a,
abstract = {This article presents an overview of damage measures proposed in the area of structural health monitoring. This is an extremely active, open, and vast research field, as demonstrated by the variety of topics presented in this encyclopedia. The direction taken in this article is to present some examples of techniques that have been proposed, or that are promising tools for the estimation of location and extent of structural damage. All of the techniques considered are based on the analysis of the dynamic response of the structure under consideration. The organization of the article is based on the frequency range of analysis, which spans the low-frequency range, and correspondingly long response times, associated with the modal analysis of the structure, to frequencies associated with the propagation of guided ultrasonic waves. Hence, the methods presented belong to the classes of vibration-based and guided waves-based techniques. The damage measures discussed rely on the estimation of changes in modal parameters of the structure (natural frequencies, mode shapes, and strain energy distributions), or on features associated with the signal corresponding to the measured dynamic response. This overview is not meant to be exhaustive, but rather it provides examples of interesting solutions and approaches proposed in this area.},
author = {Ruzzene, M},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Probabilistic Aspects/A Unified Statistical Methodology for Modeling Fatigue Damage{\_}Castillo/Kap6{\_}Damage Measures.pdf:pdf},
isbn = {978-0-470-05822-0},
journal = {Encycl. Struct. Heal. Monit.},
keywords = {damage measures,guided ultrasonic waves,vibration-based technique},
number = {48},
pages = {--},
title = {{Damage measures}},
year = {2009}
}
@article{Rahmen,
author = {Rahmen, Im and Zeichnungsvorlagen, Bauteile and Verlauf, Im},
journal = {Pro-Engineer Prakt.},
pages = {25--30},
title = {{3 Aufgabenstellungen}}
}
@article{Kratzsch2013a,
author = {Kratzsch, Matthias and G{\"{u}}nther, Michael},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Klopfen{\_}Ottomotor/4. Internationale Tagung Ottomotorisches Klopfen - Berlin 12{\_}2013/Knocking+in+Gasoline+Engines.pdf:pdf},
pages = {445},
title = {{Knocking in Gasoline Engines}},
year = {2013}
}
@article{Ladungstrager,
author = {Ladungstr{\"{a}}ger, Driftbewegung Der},
title = {{3 Elektrisches Str{\"{o}}mungsfeld}}
}
@article{Vergleich,
author = {Vergleich, Im},
title = {{2 2.1 Urformen}}
}
@article{Foundations2003a,
author = {Foundations, Mathematical},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Nicholson 2003 - Finite Element Analysis Thermomechanics of Solids/0749{\_}C02.pdf:pdf},
pages = {25--42},
title = {{Mathematical Foundations: Tensors 2.1}},
year = {2003}
}
@article{Metallplastizit2013,
author = {Metallplastizit, Hrungdie and Helm, Dirk},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/{\_}skripte/Helm - Prozesssimulation und Umformtechnik/Presentation4{\_}Materialtheorie.pdf:pdf},
number = {November},
pages = {1--29},
title = {{Prozesssimulation in Der Umformtechnik}},
year = {2013}
}
@article{Jiang2004a,
abstract = {Fatigue crack propagation was modeled by using the cyclic plasticity material properties and fatigue constants for crack initiation. The cyclic elastic-plastic stress-strain field near the crack tip was analyzed using the finite element method with the implementation of a robust cyclic plasticity theory. An incremental multiaxial fatigue criterion was employed to determine the fatigue damage. A straightforward method was developed to determine the fatigue crack growth rate. Crack propagation behavior of a material was obtained without any additional assumptions or fitting. Benchmark Mode I fatigue crack growth experiments were conducted using 1070 steel at room temperature. The approach developed was able to quantitatively capture all the important fatigue crack propagation behaviors including the overload and the R-ratio effects on crack propagation and threshold. The models provide a new perspective for the R-ratio effects. The results support the notion that the fatigue crack initiation and propagation behaviors are governed by the same fatigue damage mechanisms. Crack growth can be treated as a process of continuous crack nucleation. },
author = {Jiang, Yanyao and Feng, Miaolin},
doi = {10.1115/1.1631026},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/2004{\_}Jiang{\_}Modeling of Fatigue Crack Propagation.pdf:pdf},
issn = {00944289},
journal = {J. Eng. Mater. Technol.},
number = {1},
pages = {77},
title = {{Modeling of Fatigue Crack Propagation}},
url = {http://materialstechnology.asmedigitalcollection.asme.org/article.aspx?articleid=1427113},
volume = {126},
year = {2004}
}
@article{Kupplungssystem2001,
author = {Kupplungssystem, Das and Verzahnungstechnik, Die and Gleichungen, Die},
title = {{Auslegung und Charakteristika spezieller Systeme und Baugruppen von manuellen Schaltgetrieben}},
year = {2001}
}
@article{Variationsrechnung,
author = {Variationsrechnung, Gegenstand Der},
title = {{10 Variationsrechnung}}
}
@book{Zheng-Ping2013,
abstract = {In this paper, the Turing instability in reaction-diffusion models defined on complex networks is studied. Here, we focus on three types of models which generate complex networks, i.e. the Erd$\backslash$H{\{}o{\}}s-R$\backslash$'enyi, the Watts-Strogatz and the threshold network models. From analysis of the Laplacian matrices of graphs generated by these models, we reveal that the stable-unstable regions of a spatially homogeneous solution completely differ, depending on network structures. In particular, we approximately argue the existence of the stable-unstable regions in the cases of regular enhanced ring lattices which include regular circles, and networks generated by the threshold network model when the number of vertices is large enough.},
archivePrefix = {arXiv},
arxivId = {1406.6401},
author = {Zheng-Ping, Fu and Xin-Hang, Xu and Hong-Li, Wang and Qi, Ouyang and Yang, Lingfa and Zhabotinsky, Anatol M. and Epstein, Irving R. and Wiggins, L Sirovich S and Toole, Gregory and Hurdal, Monica K. and Cogan, Nick and Shi, Junping and Search, Home and Journals, Collections and Contact, About and Iopscience, My and Rozhnova, G. and Nunes, a. and McKane, Alan J. and Page, Karen and Maini, Philip K. and a.M. Monk, Nicholas and Li, Qian Shu and Ji, Lin and Levine, Herbert and Rappel, Wouter Jan and Kumar, Niraj and Horsthemke, Werner and Kov{\'{a}}cs, S{\'{a}}ndor and Judd, Stephen L and Silber, Mary and Ide, Yusuke and Izuhara, Hirofumi and Machida, Takuya and Hori, Yutaka and Guiu-Souto, Jacobo and Carballido-Landeira, Jorge and P{\'{e}}rez-Villar, Vicente and Mu{\~{n}}uzuri, Alberto P. and Gambino, G. and Lombardo, M.C. C. and Sammartino, M. and Fanelli, Duccio and Cianci, Claudia and {Di Patti}, Francesca and Cao, Yang and Erban, Radek and Cantini, Laura and Massi, Emma and Barletti, Luigi and Biancalani, Tommaso and Bhattacharyay, a. and Berenstein, Igal and Dolnik, Milos and Asslani, Malbor and Asllani, Malbor and Busiello, Daniel M. and Carletti, Timoteo and Planchon, Gwendoline and Access, Open},
booktitle = {Phys. Rev. E - Stat. Nonlinear, Soft Matter Phys.},
doi = {10.1016/j.camwa.2013.03.019},
eprint = {1406.6401},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/Strukturmechanik MMS/Literatur/Mikromechanik{\_}B{\"{u}}cher{\_}Literaturvorschlag{\_}MMS/Torquato 2002 RHM.pdf:pdf},
isbn = {4420767936},
issn = {1539-3755},
keywords = {05c82,1,2010 msc,35k57,60g05,60j60,70k50,92c15,92c40,Amplitude equation,Cortical folding,Cross diffusion,Ginzburg-Landau equation,Growing domain,Linearised stability,Morphology,Nonlinear diffusion,Pattern formation,Quintic Stuart-Landau equation,Reaction-diffusion system,Turing bifurcation,Turing system,activator,ams subject classifications,and another for inhibitor,and diffusion,approaches to the mathematical,based,clo,compartment-based models,complex network,cross-diffusion,cross-diffusion systems,deterministic models which are,diffusion models,diffusion system,epstein,growing domain,holling type-ii functional response,i,instability,introduction,le,lengyel,model,modelling of chemical reactions,non-constant positive steady state,pattern,pattern formation,reaction,reaction-diffusion,reaction-diffusion models on networks,reaction-diffusion processes,reaction-diffusion systems,self-organised spatial pattern,stationary patterns,stochastic processes,stochastic simulations,stochastic turing patterns,systems,there are two fundamental,turing instability,turing pattern,turing reaction,turing system},
number = {4},
pages = {476},
pmid = {15267983},
title = {{Interdisciplinary Applied Mathematics}},
url = {http://link.springer.com/10.1140/epjb/e2013-40570-8{\%}5Cnhttp://arxiv.org/abs/1406.6401{\%}5Cnhttp://arxiv.org/abs/1204.1475{\%}5Cnhttp://link.aps.org/doi/10.1103/PhysRevLett.91.058302{\%}5Cnhttp://arxiv.org/abs/nlin/0111059{\%}5Cnhttp://link.aps.org/doi/10.1103/PhysRe},
volume = {82},
year = {2013}
}
@inproceedings{2005-01-0999,
abstract = {Temperature measurement experiments with intake port model were done to achieve the fundamental information on constructing physical model that expresses the heat transfer phenomena in the intake manifold and intake port. The experiments were done with steady airflow, and the size, shape, heating condition of the port model and mass flow rate were changed as experimental parameters. As the results, it was clear that the developing condition of velocity and thermal boundary layer had greater influence than the shape factor, and the coefficient and the exponent of the equation derived from the relationship between Nusselt number and Reynolds number had great difference from those of generally used Colburn's equation in undeveloped entrance region, but they got closer as developing boundary layer.},
author = {Uchida, Keisuke and Suzuki, Takashi and Oguri, Yasufumi and Yoshida, Masatake},
booktitle = {SAE Tech. Pap.},
doi = {10.4271/2005-01-0999},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2005{\_}Uchida{\_}Precise Measurement of Heat Transfer to the Inlet Air unsing Intake Port Model.pdf:pdf},
publisher = {SAE International},
title = {{Precise Measurement of Heat Transfer to the Inlet Air using Intake Port Model}},
url = {https://doi.org/10.4271/2005-01-0999},
year = {2005}
}
@article{Band-,
author = {Band-, Die and Systeme, Moderne and Wabenstruktur, Die},
pages = {365--382},
title = {{Abgasnachbehandlungssysteme}}
}
@article{Quation2003,
author = {Quation, F Inite Lement E},
title = {{By the}},
volume = {2},
year = {2003}
}
@article{Poll,
author = {Poll, Gerhard and Deters, Ludger and Gleitlager, Fettgeschmierte and Radialgleitlager, Hydrostatische and Axialgleitlager, Hydrostatische and Anfahrhilfe, Hydrostatische},
title = {{Kapitel 11 Lagerungen, Gleitlager, W{\{}{\"{a}}{\}}lzlager}}
}
@article{Pokluda2010,
author = {Pokluda, Jaroslav and Andera, Pavel},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2010{\_}Jaroslav Pokluda+Pavel {\v{S}}andera{\_}Micromechanisms of fracture and fatigue{\_}Buch/Kap3{\_}BrittleAndDuctileFracture.pdf:pdf},
journal = {Micromechanisms Fract. Fatigue},
pages = {69--123},
title = {{Brittle and Ductile Fracture}},
year = {2010}
}
@article{Burg2006,
author = {Burg, Heinz and Rekonstruktion, Die and Nutzfahrzeugunf{\"{a}}llen, Von},
pages = {439--442},
title = {{A13 A13 Unf{\{}{\"{a}}{\}}lle mit Nutzfahrzeugen A13}},
year = {2006}
}
@article{Jiang2004,
abstract = {Fatigue crack propagation was modeled by using the cyclic plasticity material properties and fatigue constants for crack initiation. The cyclic elastic-plastic stress-strain field near the crack tip was analyzed using the finite element method with the implementation of a robust cyclic plasticity theory. An incremental multiaxial fatigue criterion was employed to determine the fatigue damage. A straightforward method was developed to determine the fatigue crack growth rate. Crack propagation behavior of a material was obtained without any additional assumptions or fitting. Benchmark Mode I fatigue crack growth experiments were conducted using 1070 steel at room temperature. The approach developed was able to quantitatively capture all the important fatigue crack propagation behaviors including the overload and the R-ratio effects on crack propagation and threshold. The models provide a new perspective for the R-ratio effects. The results support the notion that the fatigue crack initiation and propagation behaviors are governed by the same fatigue damage mechanisms. Crack growth can be treated as a process of continuous crack nucleation. },
author = {Jiang, Yanyao and Feng, Miaolin},
doi = {10.1115/1.1631026},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/2004{\_}Jiang{\_}Modeling of Fatigue Crack Propagation.pdf:pdf},
issn = {00944289},
journal = {J. Eng. Mater. Technol.},
number = {1},
pages = {77},
title = {{Modeling of Fatigue Crack Propagation}},
url = {http://materialstechnology.asmedigitalcollection.asme.org/article.aspx?articleid=1427113},
volume = {126},
year = {2004}
}
@article{Grundaufgabe,
author = {Grundaufgabe, Die},
doi = {10.1007/978-3-642-24161-1},
isbn = {9783642241611},
journal = {System},
title = {{9 Thermodynamik des Heizens und K u ¨ hlens}}
}
@article{Shudo2000a,
abstract = {Hydrogen has higher flame velocity and shorter quenching distance than hydrocarbon fuels, and is supposed to have special characteristics in the combustion process of internal combustion engines. In this research, contributors to thermal efficiency in a hydrogen premixed spark ignition engine were analyzed and compared with methane combustion. Results showed hydrogen combustion had higher cooling loss to combustion chamber wall, and thermal efficiency of hydrogen combustion was mainly dominated by both cooling loss to combustion chamber wall and degree of constant volume combustion.},
author = {Shudo, T},
doi = {10.1016/S0389-4304(99)00091-0},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Heat Transfer Combustion Chamber/2007{\_}Shudo{\_}Thermal efficiency analysis in a hydrogen premixed combustion engine.pdf:pdf},
issn = {03894304},
journal = {JSAE Rev.},
number = {2},
pages = {177--182},
title = {{Thermal efficiency analysis in a hydrogen premixed combustion engine}},
url = {http://www.sciencedirect.com/science/article/pii/S0389430499000910},
volume = {21},
year = {2000}
}
@article{Tribologie2000,
author = {Tribologie, Fachgebiet},
doi = {10.1007/978-3-8348-8279-0},
isbn = {9783834882790},
pages = {2000},
title = {{4 Tribologie 4 4.1}},
year = {2000}
}
@article{Tschirschwitzc,
author = {Tschirschwitz, Christian},
pages = {629--643},
title = {{B4 B4 Unf{\"{a}}lle mit motorisierten Zweir{\"{a}}dern B4}}
}
@article{Method,
author = {Method, Finite Element and Method, Boundary Element and Analysis, Transformation Field and Tanaka, Mori},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/{\_}buecherSong/ComputationalMechanicsofCompositeMaterials/03{\_}ElastoplasticProblem.pdf:pdf},
title = {{3 Elastoplastic Problems}}
}
@article{Corti2009b,
abstract = {Specific power and efficiency of gasoline engines are influenced by factors such as compression ratio and Spark Advance (SA) regulation. These factors influence the combustion development over the crank angle: the trade-off between performance and the risk of irreversible damages is still a key element in the design of both high-performance (racing) and low-consumption engines. This paper presents a novel approach to the problem, with the objective of defining a damage-related and operating conditions-independent index. The methodology is based on the combined analysis of indicating parameters, such as Cumulated Heat Release (CHR), Indicated Mean Effective Pressure (IMEP) and 50{\{}{\%}{\}} Mass Fraction Burned (MFB50), and typical knock detection parameters, estimated by means of the in-cylinder pressure sensor signal. Knocking combustions have several consequences, therefore they can be detected in many ways. As it is well known, knock excites the combustion chamber resonant frequencies, rising high frequency components in the in-cylinder pressure signal. Additionally, knocking combustions cause a higher heat flux through the combustion chamber walls, increasing the heat losses and lowering the IMEP: this effect can be observed by evaluating IMEP or CHR, that are based on the low-frequency content of the in-cylinder signal spectrum. A knock detection index can then be based on the crossed-observation of two phenomena, one set in the low-frequencies range and the other one on the high frequencies range of the in-cylinder pressure signal. Knock-related parameters have been analyzed with a statistical approach, in order to define a detection strategy based on one single threshold value, to be used for all the engines, independently of engine speed and load: IMEP and CHR have been related to a typical high-frequency knock index, based on the Maximum Amplitude of Pressure Oscillations (MAPO) evaluated over the combustion angular window. It can be observed that, as knock intensity increases, the relationships between these parameters change. This change can be seized by evaluating the correlation coefficient between the parameters distributions and observing its trend as a function of SA (Spark Advance). The correlation coefficient is intrinsically normalized, therefore the index range is the same for every engine operating condition, and the paper shows that the threshold level, too, is constant. The same approach can be applied to determine SA corresponding to the best combustion phase, simply by evaluating the correlation coefficient for IMEP and MFB50 distributions. The methodology has been successfully applied to different engines running in different speed and load conditions.},
author = {Corti, Enrico and Forte, Claudio},
doi = {10.4271/2009-24-0019},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Klopfen{\_}Ottomotor/2009{\_}Forte+Corti{\_}Statistical Analysis of Indicating Parameters for Knock Detection Purposes.pdf:pdf},
issn = {19463936},
journal = {SAE Tech. Pap.},
number = {2009-01-0237},
title = {{Statistical Analysis of Indicating Parameters for Knock Detection Purposes}},
url = {http://papers.sae.org/2009-01-0237/},
year = {2009}
}
@article{Leichtbaustruktur,
author = {Leichtbaustruktur, Eine and Zuverl, Forderung and Bewertung, Zur and Bewertung, Die and Weiteren, Im},
pages = {370--378},
title = {{25 Strukturzuverl{\{}{\"{a}}{\}}ssigkeit}}
}
@book{Lienhard2003,
address = {Cambridge Massachusetts},
author = {Lienhard, John H I V and Lienhard, John H V},
edition = {3},
pages = {762},
publisher = {Phlogiston Press},
title = {{A heat transfer textbook}},
year = {2003}
}
@article{Darstellungb,
author = {Darstellung, Zur and Hilfe, Mit and Geschwindigkeit, Position and Verbindungsreaktion, Beschleunigung and Impuls, Lastenreaktion},
pages = {70--92},
title = {{7 Bewegungssimulation}}
}
@article{Unterflurverkleidung,
author = {Unterflurverkleidung, Die},
pages = {35--36},
title = {{14 Unterflur}}
}
@article{Zhen2012,
abstract = {Knocking combustion in spark-ignition (SI) engines is an abnormal combustion phenomenon which can constrain the engine performance and thermal efficiency. It can also result in severe permanent engine damage under certain operating conditions. This paper systematically reviews the engine knock phenomenon, including the mechanisms, influencing factors, consequences and detection methods etc. It introduces the visualization researches, simulations and some judging indexes of engine knock. Three mathematical models which can predict the engine knock, and various kinds of methods of suppressing knock are summarized. Finally, this paper puts forward some new suggestions on the weakness in the researches of knocking combustion. {\{}{\textcopyright}{\}} 2011 Elsevier Ltd.},
author = {Zhen, Xudong and Wang, Yang and Xu, Shuaiqing and Zhu, Yongsheng and Tao, Chengjun and Xu, Tao and Song, Mingzhi},
doi = {10.1016/j.apenergy.2011.11.079},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Klopfen{\_}Ottomotor/2012{\_}Zhen{\_}The engine knock analysis - an overview about models and index.pdf:pdf},
isbn = {0306-2619},
issn = {03062619},
journal = {Appl. Energy},
keywords = {Detection methods,Knock,Models,Simulations,Suppressing methods,Visualization researches},
pages = {628--636},
publisher = {Elsevier Ltd},
title = {{The engine knock analysis - An overview}},
url = {http://dx.doi.org/10.1016/j.apenergy.2011.11.079},
volume = {92},
year = {2012}
}
@article{Winkler2014,
author = {Winkler, N.},
doi = {10.1177/1468087414544899},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2015{\_}Winkler{\_}Effect of pressure oscillations on in-cylinder heat transfer  - through LES Simulation.pdf:pdf},
isbn = {1468087414544},
issn = {1468-0874},
journal = {Int. J. Engine Res.},
keywords = {24 june 2014,6 march 2014,accepted,computational fluid dynamics,date received,heat transfer,internal combustion engines,large eddy simulation,pressure oscillations},
number = {6},
pages = {705--715},
title = {{Effect of pressure oscillations on in-cylinder heat transfer - through large eddy simulation}},
url = {http://jer.sagepub.com/lookup/doi/10.1177/1468087414544899},
volume = {16},
year = {2014}
}
@book{Murakami2012,
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Murakami, Sumio},
doi = {10.1007/978-94-007-2666-6},
eprint = {arXiv:1011.1669v3},
isbn = {978-94-007-2665-9},
issn = {09250042},
number = {Cdm},
pages = {141--200},
pmid = {25246403},
title = {{Continuum Damage Mechanics}},
url = {http://link.springer.com/10.1007/978-94-007-2666-6},
volume = {185},
year = {2012}
}
@article{Haslam2013,
author = {Haslam, Antony and Laskaridis, Panos},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2010{\_}Jaroslav Pokluda+Pavel {\v{S}}andera{\_}Micromechanisms of fracture and fatigue{\_}Buch/Kap4{\_}FatigueFracture.pdf:pdf},
title = {{Fatigue {\{}{\&}{\}} Fracture}},
year = {2013}
}
@article{Schneider2016a,
abstract = {{\{}{\textcopyright}{\}} 2016 Elsevier B.V.Modeling of crack propagation in materials has long been a challenge in solid-state physics and materials science. The phase-field method has now established as one of the tools for the description of crack propagation. The applied models are thermodynamically consistent and predict crack propagation in homogeneous materials under the consideration of different loading types, multiple physical fields and geometrical nonlinearities. Even dynamic loading processes are studied, including plastic effects. A multiphase-field model for crack propagation, which is indispensable to describe crack propagation on a mesoscopic length scale, is still missing. In this work, we overcome this deficiency and combine a crack propagation approach, which is based on Griffith's theory, with an established multiphase-field model for phase transformation.},
author = {Schneider, D and Schoof, E and Huang, Y and Selzer, M and Nestler, B},
doi = {10.1016/j.cma.2016.04.009},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Thermodynamik/PhasenFeld/Schneider{\_}Crack{\_}propagation{\_}multiphase{\_}systems-Dez2015.pdf:pdf},
issn = {00457825},
journal = {Comput. Methods Appl. Mech. Eng.},
keywords = {crack propagation,multiphase-field,phase-field,polycrystalline material},
title = {{Phase-field modeling of crack propagation in multiphase systems}},
url = {http://dx.doi.org/10.1016/j.cma.2016.04.009},
year = {2016}
}
@article{Mousavi2016,
abstract = {{\{}{\textcopyright}{\}} 2016 Springer Science+Business Media DordrechtThe in-plane classical dislocation-based linear elastic fracture mechanics analysis is extended to the case of strain gradient elasticity. Nonsingular stress and smooth-closure crack profiles are derived. As in the classical treatment, the crack is represented by a distribution of climb edge dislocations (for Mode I) or glide edge dislocations (for mode II). These distributions are determined through the solution of corresponding integral equations based on variationally consistent boundary conditions. An incompatible framework is used and the nonsingular full-field plastic distortion tensor components are calculated. Numerical results and related graphs are provided illustrating the nonsingular behaviour of the stress/strain components and the smooth cusp-like closure of the crack faces at the crack tip. The work provides an alternative approach to celebrated “Barenblatt's treatment” of cracks, without the introduction of a cohesive zone and related to intermolecular forces ahead of the physical crack tip. It also supplements a recent paper by the authors in which the mode III crack, represented by an array of screw dislocations, was solved within the present gradient elasticity framework.},
author = {Mousavi, S Mahmoud and Aifantis, Elias C},
doi = {10.1007/s10704-016-0143-5},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/2016{\_}Mousavi{\_}Dislocation-based gradient elastic fracture mechanics.pdf:pdf},
issn = {15732673},
journal = {Int. J. Fract.},
keywords = {Crack tip plasticity,Gradient elasticity,Nonsingular cracks,Nonsingular dislocations},
number = {1},
pages = {93--110},
title = {{Dislocation-based gradient elastic fracture mechanics for in-plane analysis of cracks}},
volume = {202},
year = {2016}
}
@article{Techniken,
author = {Techniken, Konstruktive},
journal = {Auslegung A Grad. J. Philos.},
pages = {10--16},
title = {{3 Methoden und Hilfsmittel im Leichtbau}}
}
@article{Luftschall,
author = {Luftschall, Direkter and Biegeschwin-, Allgemeinen and Ger, Das and Lokalisierung, Zur and Motor-, Quellen and Anschl, Linearantriebe and Bild, Rohrleitungen and Betriebskr, Typische and Schaffung, Die},
title = {{26 Strukturakustik}}
}
@article{Wallentowitz2006d,
author = {Wallentowitz, Henning and Reif, Konrad},
doi = {10.1007/978-3-8348-9121-1_10},
journal = {Handb. Kraftfahrzeugelektronik - Grundlagen, Kompon. Syst. Anwendungen},
title = {{Telematik}},
url = {http://www.springerlink.com/index/10.1007/978-3-8348-9121-1{\_}10},
year = {2006}
}
@article{Battjes2001,
author = {Battjes, Jurjen A.},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Zienkiewicz FEM - Vol 3 Fluid Dynamics/63229{\_}12.pdf:pdf},
issn = {02748096},
title = {{Short Waves}},
year = {2001}
}
@article{Carlo,
author = {Carlo, Monte},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/{\_}buecherSong/ComputationalMechanicsofCompositeMaterials/02{\_}ElasticityProblem.pdf:pdf},
title = {{2 Elasticity 2.1}}
}
@article{ConferenceonFatigueMechanisms:AdvancesinQuantitativeMeasurementofPhysicalDamage1983a,
author = {{Conference on Fatigue Mechanisms: Advances in Quantitative Measurement of Physical Damage}},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/1983{\_}Lankford{\_}Fatigue Mechanisms Advances in quantitative   meausrements of physical damage.pdf:pdf},
issn = {10403094},
journal = {Stp 811},
keywords = {An{\'{a}}lise quantitativa,Congresso,Dano f{\'{i}}sico,Fadiga de materiais},
pages = {496},
title = {{Fatigue mechanisms advances in quantitative measurement of physical damage {\textless}{\textless}a{\textgreater}{\textgreater} conference}},
year = {1983}
}
@book{Riccardella1992e,
author = {Riccardella, PC and Deardorff, AF and Griesbach, TJ},
booktitle = {Adv. Fatigue Lifetime Predict. Tech.},
doi = {10.1520/STP1122-EB},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Neuer Ordner/Advances in fatigue lifetime predictive techniques Part1.pdf:pdf},
isbn = {978-0-8031-1423-4},
issn = {00660558},
keywords = {FATIGUE,MONITORING,POWER PLANTS,PRESSURE VESSELS AND PIPING,THERMAL STRESSES},
pages = {460--473},
pmid = {11439068},
title = {{Advances in Fatigue Lifetime Predictive Techniques}},
url = {https://apps.webofknowledge.com/full{\_}record.do?product=UA{\&}search{\_}mode=GeneralSearch{\&}qid=11{\&}SID=Z1UxbH6jtsqo8n9kPQr{\&}page=1{\&}doc=1},
volume = {1122},
year = {1992}
}
@article{Baehr2006,
abstract = {Bevor wir einige Grundbegriffe der Thermodynamik einf{\{}{\"{u}}{\}}hren, gehen wir kurz auf ihre geschichtliche Entwicklung ein und versuchen dann, die Frage zu beantworten: Was ist Thermodynamik? In den darauf folgenden Ab- schnitten definieren wir das thermodynamische System und behandeln seine Beschreibung durch Zustandsgr{\{}{\"{o}}{\}}{\{}{\ss}{\}}en. Dabei f{\{}{\"{u}}{\}}hren wir den f{\{}{\"{u}}{\}}r die klassische Thermodynamik grundlegenden Begriff der Phase ein. Bei der daran anschlie{\{}{\ss}{\}}enden Behandlung der thermodynamischen Prozesse erhalten wir mit dem Prinzip der Irreversibilit{\{}{\"{a}}{\}}t eine erste Formulierung des 2. Hauptsatzes der Thermodynamik. Schlie{\{}{\ss}{\}}lich f¨ uhren wir die Temperatur als die erste typisch thermodynamische Zustandsgr{\{}{\"{o}}{\}}{\{}{\ss}{\}}e ein.},
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Baehr, Hans Dieter and Kabelac, Stephan},
doi = {10.1017/CBO9781107415324.004},
eprint = {arXiv:1011.1669v3},
isbn = {9783834882851},
issn = {0302-4350},
journal = {Springer},
keywords = {Grundlagen,Thermodynamik,Verbrennung},
pages = {1--42},
pmid = {25246403},
title = {{Thermodynamik}},
url = {http://www.springerlink.com/index/w26t7673r61611tj.pdf},
volume = {1},
year = {2006}
}
@article{Hashin1963a,
abstract = {Variational principles in the linear theory of elasticity, involving the elastic polarization tensor, have been applied to the derivation of upper and lower bounds for the effective elastic moduli of quasi-isotropic and quasi-homogeneous multiphase materials of arbitrary phase geometry. When the ratios between the different phase moduli are not too large the bounds derived are close enough to provide a good estimate for the effective moduli. Comparison of theoretical and experimental results for a two-phase alloy showed good agreement.},
author = {Hashin, Zvi and Shtrikman, Shmuel},
doi = {10.1016/0022-5096(63)90060-7},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/Strukturmechanik MMS/Literatur/Hashin Shtrikman 1963.pdf:pdf},
isbn = {0022-5096},
issn = {00225096},
journal = {J. Mech. Phys. Solids},
number = {2},
pages = {127--140},
title = {{A variational approach to the theory of the elastic behaviour of multiphase materials}},
url = {http://linkinghub.elsevier.com/retrieve/pii/0022509663900607},
volume = {11},
year = {1963}
}
@article{Stoffe,
author = {Stoffe, Der},
number = {1},
pages = {65--81},
title = {{1.1 Eigenschaften der Stoffe}}
}
@article{Shojaefard2005a,
author = {Shojaefard, M. H. and Noorpoor, A. R. and Bozchaloe, D. A. and Ghaffarpour, M.},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Heat transfer intake+exhaust system/2005{\_}Shojaefard+Noorpoor{\_}Transient Thermal Analysis of Engine Exhaust Valve.pdf:pdf},
journal = {Numer. Heat Transf. Part A Appl.},
number = {7},
pages = {627--644},
title = {{Transient Thermal Analysis of Engine Exhaust Valve}},
volume = {48},
year = {2005}
}
@article{Foundations2003,
author = {Foundations, Mathematical},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Nicholson 2003 - Finite Element Analysis Thermomechanics of Solids/0749{\_}C01.pdf:pdf},
pages = {1--23},
title = {and},
year = {2003}
}
@article{Moschandreou1997,
author = {Moschandreou, T and Zamir, M},
doi = {https://doi.org/10.1016/S0017-9310(96)00266-9},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Thermal Coating + Water Heat Transfer + Applikation/1996{\_}Zamir+Moschandreau{\_}Heat Transfer in a tube with pulsating flow and constant heat flux.pdf:pdf},
journal = {Int. J. Heat Mass Transf.},
number = {10},
pages = {2461--2466},
title = {{Heat transfer in a tube with pulsating flow and constant heat flux}},
volume = {40},
year = {1997}
}
@article{Materials,
author = {Materials, Engineering},
journal = {Corros. Prot.},
title = {{Engineering Materials and Processes}}
}
@article{Durst,
author = {Durst, Franz},
isbn = {9783540313236},
journal = {New York},
title = {{Franz Durst Grundlagen der Str{\"{o}}mungsmechanik}}
}
@article{Doudard2005,
abstract = {It is proposed to develop and identify a probabilistic two-scale model for HCF that accounts for the failure of samples, but also for the thermal effects during cyclic loadings in a unified framework. The probabilistic model is based on a Poisson point process. Within the weakest link theory, the model corresponds to a Weibull law for the fatigue limits. The thermal effects can be described if one considers the same hypotheses apart from the weakest link assumption. A method of identification is proposed and uses temperature measurements to identify the scatter in an S/N curve. The validation of the model is obtained by predicting S/N curves for different effective volumes of a dual-phase steel},
author = {Doudard, C. and Calloch, S. and Cugy, P. and Galtier, A. and Hild, F.},
doi = {10.1111/j.1460-2695.2005.00854.x},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Surface effects + Frequency effects/A probabilistic two-scale model for high-cycle fatigue life predictions {\_} Doudard {\_} CACHEN{\_}Paris.pdf:pdf},
isbn = {8756758X (ISSN)},
issn = {8756758X},
journal = {Fatigue Fract. Eng. Mater. Struct.},
keywords = {Fatigue limits,Microplasticity,Thermomechanics,Weibull model},
number = {3},
pages = {279--288},
title = {{A probabilistic two-scale model for high-cycle fatigue life predictions}},
volume = {28},
year = {2005}
}
@article{Wallentowitz2006m,
author = {Wallentowitz, Henning and Reif, Konrad},
doi = {10.1007/978-3-8348-9121-1_9},
isbn = {978-3-528-03971-4},
journal = {Handb. Kraftfahrzeugelektronik - Grundlagen, Kompon. Syst. Anwendungen},
title = {{Fahrerassistenzsysteme und Verkehr}},
url = {http://www.springerlink.com/index/10.1007/978-3-8348-9121-1{\_}9},
year = {2006}
}
@article{Messtechnik,
author = {Messtechnik, Grundbegriffe Der},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Vorlesungen/Messtechnik+Regelungstechnik/gmrt06.pdf:pdf},
pages = {1--17},
title = {{6 Grundbegriffe der Messtechnik}}
}
@article{Stebbins1967a,
author = {Stebbins, Jeun},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Empirical Fatigue Models + Validation/1965{\_}NASA+Hudson{\_}Studies of fatigue crack growth in alloys suitable for elevated temperature-Al2618.pdf:pdf},
number = {May},
title = {{Nasa Technical N O T E}},
year = {1967}
}
@article{Rest,
author = {Rest, Der and Zwangskr, Ladungstrennung and Ladungen, Energiezufuhr and Spannung, Elektrische and Spannung, Die and Stromst, Elektrische},
journal = {System},
title = {{2 Gleichstromkreis 2.1}}
}
@article{Helmholtz1969,
author = {Helmholtz, The},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Zienkiewicz FEM - Vol 3 Fluid Dynamics/63229{\_}11.pdf:pdf},
title = {{Long and medium waves ∗}},
year = {1969}
}
@article{Zienkiewicz2013,
abstract = {Abstract This chapter describes discrete systems and their mathematical representation by what we define as a standard discrete system. The system is defined by components we call elements which are joined together at discrete points we call nodes. Today, discrete problems can generally be solved using computers even if the number of elements is very large. Systems which are continuous are often defined using differential equations or equivalent statements which imply an infinite number of elements. Engineering solutions to continuous problems can be attained using discretization methods. This volume presents a view of the finite element method as a general discretization procedure of continuous systems. Finite element analyses follow a standard pattern which is universally adaptable to all discrete systems. The goal of this volume is to show how finite element methods lead to a standard discrete system. This chapter is primarily concerned with establishing the processes applicable to such systems.},
author = {Zienkiewicz, O.C. and Taylor, R.L. and Zhu, J.Z.},
doi = {10.1016/B978-1-85617-633-0.00001-0},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Zienkiewicz FEM - Vol 1 Basics Fundamentals/63205{\_}01.pdf:pdf},
isbn = {978-1-85617-633-0},
issn = {00295981},
journal = {Finite Elem. Method its Basis Fundam.},
pages = {1--20},
pmid = {21333062},
title = {{The Standard Discrete System and Origins of the Finite Element Method}},
url = {http://linkinghub.elsevier.com/retrieve/pii/B9781856176330000010},
year = {2013}
}
@article{Aslan2010a,
author = {Aslan, Ozgur},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/2010{\_}Aslan{\_}Numerical modeling of fatigue crack growth in single crystal nickel based superalloys.pdf:pdf},
title = {{Numerical modeling of fatigue crack growth in single crystal nickel based superalloys Ozgur Aslan l ' {\'{E}}cole nationale sup{\'{e}}rieure des mines de Paris Sp{\'{e}}cialit{\'{e}} « Sciences et G{\'{e}}nie des Mat{\'{e}}riaux » Simulation num{\'{e}}rique de la fissuration par fatigue dans les }},
year = {2010}
}
@article{Kreher1985a,
author = {Kreher, W and Pompe, W},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Probabilistic Aspects/1985{\_}Kreher{\_}Field Fluctuations in a heterogeneous elastic material - an info theory approach.pdf:pdf},
journal = {J. Mech. Phys. Solids},
number = {5},
pages = {419--445},
title = {{Field fluctuations in a heterogeneous elastic material: An information theory approach}},
volume = {33},
year = {1985}
}
@article{Wirsching1983b,
abstract = {Two methods are discussed for constructing a design curve on the safe side of fatigue data. Both the tolerance interval and equivalent prediction interval (EPI) concepts provide such a curve while accounting for both the distribution of the estimators in small samples and the data scatter. The EPI is also useful as a mechanism for providing necessary statistics on S-N data for a full reliability analysis which includes uncertainty in all fatigue design factors. Examples of statistical analyses of the general strain life relationship are presented. The tolerance limit and EPI techniques for defining a design curve are demonstrated. Examples usng WASPALOY B and RQC-100 data demonstrate that a reliability model could be constructed by considering the fatigue strength and fatigue ductility coefficients as two independent random variables. A technique given for establishing the fatigue strength for high cycle lives relies on an extrapolation technique and also accounts for "runners." A reliability model or design value can be specified.},
author = {Wirsching, P H},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Probabilistic Aspects/1983{\_}Wirsching{\_}Statistical summaries of fatigue data for design purposes.pdf:pdf},
issn = {05657059},
journal = {Nasa Cr 3697},
number = {July},
title = {{Statistical Summaries of Fatigue Data for Design Purposes}},
year = {1983}
}
@article{Materials,
author = {Materials, Engineering},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/Micromechanisms of fracture and fatigue/Front.pdf:pdf},
journal = {Corros. Prot.},
title = {{Engineering Materials and Processes}}
}
@article{Hill1952,
abstract = {The connection between the elastic behaviour of an aggregate and a single crystal is considered, with special reference to the theories of Voigt, Reuss, and Huber and Schmid. The elastic limit under various stress systems is also considered, in particular, it is shown that the tensile elastic limit of a face-centred aggregate cannot exceed two-thirds of the stress at which pronounced plastic distortion occurs.},
author = {Hill, R},
doi = {10.1088/0370-1298/65/5/307},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/Strukturmechanik MMS/Literatur/Hill 1952.pdf:pdf},
isbn = {0370-1298},
issn = {0370-1298},
journal = {Proc. Phys. Soc. Sect. A},
number = {5},
pages = {349--354},
title = {{The Elastic Behaviour of a Crystalline Aggregate}},
url = {http://stacks.iop.org/0370-1298/65/i=5/a=307?key=crossref.630b67f122246b4defcc5fda55c7bf20},
volume = {65},
year = {1952}
}
@article{Variationsrechnunga,
author = {Variationsrechnung, Gegenstand Der},
title = {{10 Variationsrechnung}}
}
@article{Amara1994,
abstract = {LES VARIATIONS RAPIDES DE PRESSION ET DE TEMPERATURE INFLUENT CONSIDERABLEMENT SUR LES ECHANGES THERMIQUES INSTANTANES ENTRE LE GAZ ET LES PAROIS DE LA CHAMBRE DE COMBUSTION. UNE ETUDE EXPERIMENTALE DE LA DENSITE SURFACIQUE DU FLUX DE CHALEUR ECHANGE EN DEUX POINTS DE LA PAROI DE LA CULASSE A PERMIS EN EFFET DE METTRE EN EVIDENCE L'ACCUMULATION D'ENERGIE DANS LA COUCHE LIMITE THERMIQUE QUI SE MANIFESTE PAR UN DEPHASAGE TEMPOREL ENTRE LE FLUX ET L'ECART DE TEMPERATURE GLOBAL GAZ-PAROI. EN REGIME LAMINAIRE INSTATIONNAIRE, UNE SIMULATION DE CES ECHANGES FAIT BIEN APPARAITRE DES EXTREMA LOCAUX DE TEMPERATURE DANS LA COUCHE LIMITE THERMIQUE. UNE INTERPRETATION DU MECANISME DE FORMATION ET DE DEPLACEMENT DE CES EXTREMA EST DONNEE. LES ECHANGES THERMIQUES EN REGIME TURBULENT SONT DECRITS A L'AIDE DU MODELE MONODIMENSIONNEL DE YANG ET MARTIN OU L'EFFET DE LA TURBULENCE EST PRIS EN COMPTE PAR LE BIAIS DE LA CONDUCTIVITE THERMIQUE TURBULENTE. CE MODELE A ETE MODIFIE POUR LIMITER L'AUGMENTATION DE LA CONDUCTIVITE THERMIQUE TURBULENTE AVEC LA DISTANCE A LA PAROI. LE PARAMETRE DE LIMITATION EST LIE A LA VALEUR LOCALE DE LA VISCOSITE TURBULENTE. LE MODELE AINSI OBTENU PERMET UNE MEILLEURE DETERMINATION DE L'EPAISSEUR DE LA COUCHE LIMITE THERMIQUE ET S'ADAPTE DE LUI-MEME A TOUTE SITUATION INTERMEDIAIRE ENTRE LE REGIME LAMINAIRE ET LES REGIMES FORTEMENT TURBULENTS, LA DENSITE DU FLUX DE CHALEUR ETANT MODULEE EN CONSEQUENCE. L'IMPLANTATION DE CE MODELE DANS LE CODE DE SIMULATION KIVA2 A MONTRE QUE LA PRISE EN COMPTE DES INSTATIONNARITES DE TEMPERATURE ET DE PRESSION CONSTITUE UNE AMELIORATION PAR RAPPORT AUX LOIS DE PAROI LOGARITHMIQUES MAIS SE REVELE INSUFFISANTE. UNE SUPERPOSITION DU MODELE MONODIMENSIONNEL ET D'UNE LOI DE PAROI LOGARITHMIQUE RENDANT COMPTE DE L'EFFET DE LA VITESSE TANGENTIELLE DONNE DES RESULTATS SE RAPPROCHANT AU MIEUX DES EVOLUTIONS EXPERIMENTALES ET CECI POUR DIFFERENTES VITESSES DE ROTATION. UNE ETUDE PARAMETRIQUE COMPARATIVE EST ENSUITE REALISEE POUR MONTRER L'IMPACT DU CHOIX D'UN MODELE DE CALCUL DU FLUX DE CHALEUR PARIETAL SUR LA DETERMINATION DES CHAMPS DE VITESSE, DE TEMPERATURE, D'ENERGIE CINETIQUE TURBULENTE ET DE SON TAUX DE DISSIPATION A LA FIN DE LA COURSE DE COMPRESSION.},
author = {Amara, S},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Heat Transfer Combustion Chamber/1994{\_}Amara{\_}Elaboration et validation dun modele de transferts thermiques dun moteur{\_}UebersichtWaermeuebergangsmodelle.pdf:pdf},
keywords = {Chambre de combustion,Cin{\'{e}}tique turbulente,R{\'{e}}gime laminaire},
publisher = {{\'{E}}cole centrale de Lyon},
title = {{Elaboration et validation d'un mod{\`{e}}le de transferts thermiques instationnaires gaz paroi dans la chambre de combustion d'un moteur}},
url = {http://cat.inist.fr/?aModele=afficheN{\&}cpsidt=162697},
year = {1994}
}
@article{Gu2002,
author = {Gu, Minyi and Die, Lynda and Frank, R C and Mark, I D},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2012{\_}Trijselaar{\_}KNOCK PREDICTION IN GAS FIRED RECIPROCATING ENGINES.pdf:pdf},
pages = {8--15},
title = {{A N ew Vec t or f or H i gh - Throughpu t , L i ga t i on - I ndependen t C l on i ng E ncod i ng a Tobacco E t ch V i rus Pro t e ase C l e avage S i t e}},
volume = {15},
year = {2002}
}
@article{Hart-Smith1998,
author = {Hart-Smith, L J and Brown, D and Wong, S},
isbn = {0412540207},
journal = {Handb. Compos.},
pages = {667--685},
title = {{Surface preparations for ensuring that the glue will stick in bonded composite structures}},
year = {1998}
}
@article{Oberbegriff,
author = {Oberbegriff, Emv-intrasystemma{\ss}nahmen Der},
title = {{7 Intrasystemma{\{}{\ss}{\}}nahmen}}
}
@article{Gross2011f,
author = {Gross, Dietmar and Seelig, Thomas},
doi = {10.1007/978-3-642-10196-0},
isbn = {978-3-642-10195-3},
title = {{Bruchmechanik}},
url = {http://link.springer.com/10.1007/978-3-642-10196-0},
year = {2011}
}
@article{Ss,
author = {Ss, V and Cc, V},
title = {{3 Aufbau von µ-Controllern der 8051-Familie}}
}
@article{Schabacker2011a,
author = {Schabacker, M},
doi = {10.1007/978-3-8348-8161-8},
isbn = {9783834881618},
pages = {39--60},
title = {{4 Geometriemodellierung}},
year = {2011}
}
@article{Ieee,
author = {Ieee, Recent and Dae, The},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/{\_}buecherSong/ComputationalMechanicsofCompositeMaterials/04{\_}SensitivityAnalysisforSomeComposite.pdf:pdf},
title = {{4 Sensitivity Analysis for Voltage Stability}}
}
@article{Essmann1981a,
abstract = {Based on recent experimental observations a realistic model of the evolution of the surface profile of persistent slip bands (PSBs) in fatigued metals is proposed. An essential feature of the model is the production of vacancies by the annihilation of edge dislocations which, combined with irreversible slip processes, leads to an elongation of the PSB parallel to the active slip vector. It is shown that a net extrusion forms rather rapidly. The growth processes and their dependence on temperature are discussed in detail. It is proposed that cracks initiate at the surface steps at the PSB{\{}{\&}{\}}ndash;matrix interface and, at a later stage, also at the notch-peak profile from the random slip processes.},
author = {Essmann, U and G{\"{o}}sele, U and Mughrabi, H},
doi = {10.1080/01418618108239541},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2016{\_}Mughrabi{\_}A model of extrusions and intrusions in fatigued metals I  Point defect production and the growth of extrusions.pdf:pdf},
isbn = {0141-8610},
issn = {0141-8610},
journal = {Philos. Mag. A},
number = {2},
pages = {405--426},
title = {{A model of extrusions and intrusions in fatigued metals I. Point-defect production and the growth of extrusions}},
url = {http://www.tandfonline.com/doi/abs/10.1080/01418618108239541},
volume = {44},
year = {1981}
}
@article{Wertung,
author = {Wertung, Der and Fe-methode, Der},
doi = {10.1007/978-3-8348-2134-8},
isbn = {9783834821348},
pages = {266--278},
title = {{11 W{\{}{\"{a}}{\}}rme{\{}{\"{u}}{\}}bertragungsprobleme}}
}
@book{Rieger,
author = {Rieger, Florian},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Plasticity models/2015{\_}Rieger{\_}Work-hardening of dual-phase steel.pdf:pdf},
isbn = {9783731505136},
title = {{Florian Rieger Work-hardening of dual-phase steel}}
}
@article{Rojas2016,
abstract = {? 2016 by the authors; licensee MDPI, Basel, Switzerland.The viscoelastic response of pure Al and 7075 (AlZnMg) and 2024 (AlCuMg) alloys, obtained with a dynamic-mechanical analyzer (DMA), is studied. The purpose is to identify relationships between the viscoelasticity and fatigue response of these materials, of great interest for structural applications, in view of their mutual dependence on intrinsic microstructural effects associated with internal friction. The objective is to investigate the influence of dynamic loading frequency and temperature on fatigue, based on their effect on the viscoelastic behavior. This research suggests that the decrease of yield and fatigue behavior reported for Al alloys as temperature increases may be associated with the increase of internal friction. Furthermore, materials subjected to dynamic loading below a given threshold frequency exhibit a static-like response, such that creep mechanisms dominate and fatigue effects are negligible. In this work, an alternative procedure to the time-consuming fatigue tests is proposed to estimate this threshold frequency, based on the frequency dependence of the initial decrease of the storage modulus with temperature, obtained from the relatively short DMA tests. This allows for a fast estimation of the threshold frequency. The frequencies obtained for pure Al and 2024 and 7075 alloys are 0.001-0.005, 0.006 and 0.075-0.350 Hz, respectively.},
author = {Rojas, J I and Crespo, D},
doi = {10.3390/met6030050},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Surface effects + Frequency effects/Frequency effect regarding EModulus and fatigue of some aluminium alloys .pdf:pdf},
issn = {20754701},
journal = {Met. (Basel).},
keywords = {AlZnMg,Aluminum alloys,Dynamic-mechanic,[AlCuMg},
number = {3},
pages = {1--13},
title = {{Onset frequency of fatigue effects in pure aluminum and 7075 (AlznMg) and 2024 (AlCuMg) alloys}},
volume = {6},
year = {2016}
}
@article{Fiser2015,
abstract = {The paper deals with a magnitude-optimum based synthesis of PID control loops with respect to the disturbance rejection. To obtain as general as possible formulation of the control synthesis the dimensional analysis is applied resulting in the use of similarity numbers of the so-called swingability and laggardness of the time delay plant. Just this approach lias made it possible to work with the transcendental form of the optimized magnitude function. From the meromorphic description of the control loop with delay the PID setting then can be evaluated by means of Levenberg-Marquardt iteration method. The obtained PID settings are systematically compared from the viewpoint of the dominant modes of the control loop responses.},
author = {Fiser, Jarom{\'{i}}r and Z{\'{i}}tek, Pavel and Vyhl{\'{i}}dal, Tom{\'{a}}{\v{s}}},
doi = {10.1016/j.ifacol.2015.09.419},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Vorlesungen/Messtechnik+Regelungstechnik/2015{\_}Fiser{\_}Magnitude Optimum Design of PID Control Loop with Delay.pdf:pdf},
journal = {IFAC-PapersOnLine},
keywords = {Dimensional analysis,Disturbance rejection,Dominant poles,Magnitude optimum criterion},
number = {12},
pages = {446--451},
publisher = {Elsevier Ltd.},
title = {{Magnitude optimum design of PID control loop with delay}},
volume = {28},
year = {2015}
}
@article{Trend,
author = {Trend, Der and Forderungen, Diese and Strips, Tailored and Erl, Zur},
journal = {Stahlbau},
pages = {152--158},
title = {{12 Schubwandtr{\"{a}}ger-Profile}}
}
@article{Hoffmeyer2006,
abstract = {Experimental results of a research project on short crack growth under multiaxial nonproportional loading are presented. Fatigue lives, crack growth curves and the deformation behaviour of hollow tube specimens and notched specimens were investigated under combined tension and torsion loading. The results served as basis for the development of a cyclic plasticity model [D??ring R, Hoffmeyer J, Vormwald M, Seeger T. A plasticity model for calculating stress-strain sequences under multiaxial nonproportional cyclic loading. In: Comput Mater Sci. 28(3-4);2003:587-96; D??ring R, Hoffmeyer J, Seeger T, Vormwald M. Constitutive modelling of nonproportional hardening, cyclic hardening and ratchetting. In: Proceedings of the seventh international conference on biaxial/multiaxial fatigue and fracture, DVM, Berlin; 2004. p. 291-6; Hoffmeyer J. Anrisslebensdauervorhersage bei mehrachsiger Beanspruchung auf Basis des Kurzrisskonzepts. PhD-Thesis, TU Darmstadt; 2004.] and a short crack model [Hoffmeyer J. Anrisslebensdauervorhersage bei mehrachsiger Beanspruchung auf Basis des Kurzrisskonzepts. PhD-Thesis, TU Darmstadt; 2004; D??ring R, Hoffmeyer J, Seeger T, Vormwald M. Fatigue lifetime prediction based on a short crack growth model for multiaxial nonproportional loading. In: Proceedings of the seventh international conference on biaxial and multiaxial fatigue and fracture, DVM, Berlin; 2004. p. 253-8]. Stress-strain paths including nonproportional hardening and experimental fatigue lives of the unnotched specimens under different loading cases are discussed and compared with calculations. Load-time-sequences were in-phase, 45?? and 90?? out-of-phase loading with constant and variable amplitudes, torsion without and with superimposed static normal stress, and strain paths like box, butterfly, diamond and cross path. For the notched specimens fatigue lives under 0?? and 90?? out-of-phase loading are compared with calculations based on finite element results and the short crack model. During some tests the initiation, growth and orientation of short cracks was studied using the plastic replica technique. ?? 2005 Elsevier Ltd. All rights reserved.},
author = {Hoffmeyer, J. and D{\"{o}}ring, R. and Seeger, T. and Vormwald, M.},
doi = {10.1016/j.ijfatigue.2005.05.014},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/2005{\_}Hoffmeyer{\_}Deformation behaviour, short crack growth and fatigue lives under multiaxial nonproportional loading.pdf:pdf},
isbn = {0142-1123},
issn = {01421123},
journal = {Int. J. Fatigue},
keywords = {Cyclic deformation,Experiments,Multiaxial loading,Replica technique,Short cracks},
number = {5-6},
pages = {508--520},
title = {{Deformation behaviour, short crack growth and fatigue lives under multiaxial nonproportional loading}},
volume = {28},
year = {2006}
}
@article{Von,
author = {Von, Fourierreihenentwicklung},
title = {{Wechselgr{\"{o}}{\ss}en und nichtperiodische Gr{\"{o}}{\ss}en}}
}
@article{Metallplastizit2013b,
author = {Metallplastizit, Hrungdie and Helm, Dirk},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/{\_}skripte/Helm - Prozesssimulation und Umformtechnik/Presentation5{\_}Plastizit{\"{a}}tsmodelle.pdf:pdf},
number = {November},
pages = {1--29},
title = {{Prozesssimulation in Der Umformtechnik}},
year = {2013}
}
@article{General1971,
author = {General, The and Model, Linear},
doi = {10.1016/B978-0-12-627865-1.00015-5},
isbn = {9780126278651},
title = {15 15.1},
year = {1971}
}
@article{Unfallrekonstruktion,
author = {Unfallrekonstruktion, Begriffe Der},
pages = {937--965},
title = {{D1 D1 Fachbegriffe nach DIN 75204 Stra{\{}{\ss}{\}}enfahrzeuge D1}}
}
@article{Clementa,
author = {Clement, Steffen and Informationstechnik, Elektro- and Klein, Bernd and Engelken, Gerhard and Konstruktion, Maschinenelemente and Czichos, Horst and Theumert, Hans and Maschinenbau, Grundlagen and Hei, Bernd and Ersoy, Metin and Isermann, Rolf and Schabacker, Michael and Fiala, Ernst and Klette, Guido},
isbn = {9783528331245},
journal = {Konstruktion},
title = {{Aus dem Programm}}
}
@article{Rojas2016a,
abstract = {? 2016 by the authors; licensee MDPI, Basel, Switzerland.The viscoelastic response of pure Al and 7075 (AlZnMg) and 2024 (AlCuMg) alloys, obtained with a dynamic-mechanical analyzer (DMA), is studied. The purpose is to identify relationships between the viscoelasticity and fatigue response of these materials, of great interest for structural applications, in view of their mutual dependence on intrinsic microstructural effects associated with internal friction. The objective is to investigate the influence of dynamic loading frequency and temperature on fatigue, based on their effect on the viscoelastic behavior. This research suggests that the decrease of yield and fatigue behavior reported for Al alloys as temperature increases may be associated with the increase of internal friction. Furthermore, materials subjected to dynamic loading below a given threshold frequency exhibit a static-like response, such that creep mechanisms dominate and fatigue effects are negligible. In this work, an alternative procedure to the time-consuming fatigue tests is proposed to estimate this threshold frequency, based on the frequency dependence of the initial decrease of the storage modulus with temperature, obtained from the relatively short DMA tests. This allows for a fast estimation of the threshold frequency. The frequencies obtained for pure Al and 2024 and 7075 alloys are 0.001-0.005, 0.006 and 0.075-0.350 Hz, respectively.},
author = {Rojas, J.I. and Crespo, D.},
doi = {10.3390/met6030050},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Surface effects + Frequency effects/Frequency effect regarding EModulus and fatigue of some aluminium alloys .pdf:pdf},
issn = {20754701},
journal = {Metals (Basel).},
keywords = {[AlCuMg, Aluminum alloys, AlZnMg, Dynamic-mechanic},
number = {3},
pages = {1--13},
title = {{Onset frequency of fatigue effects in pure aluminum and 7075 (AlznMg) and 2024 (AlCuMg) alloys}},
volume = {6},
year = {2016}
}
@article{Mollenhauer2002,
author = {Mollenhauer, Ik},
journal = {Handb. Dieselmotoren},
title = {{Belastung von Motorbauteilen}},
url = {http://link.springer.com/content/pdf/10.1007/978-3-662-07709-2{\_}6.pdf},
year = {2002}
}
@article{Winkel,
author = {Winkel, Machschen},
title = {{Omungen ¨}}
}
@article{Murakami2012f,
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Murakami, Sumio},
doi = {10.1007/978-94-007-2666-6},
eprint = {arXiv:1011.1669v3},
isbn = {978-94-007-2665-9},
issn = {09250042},
pages = {277--303},
pmid = {25246403},
title = {{Continuum Damage Mechanics}},
url = {http://link.springer.com/10.1007/978-94-007-2666-6},
volume = {185},
year = {2012}
}
@article{Zienkiewicz2000a,
abstract = {We have so far dealt with one possible approach to the approximate solution of the particular problem of linear elasticity. Many other continuum problems arise in engineering and physics and usually these problems are posed by appropriate differ- ential equations and boundary conditions to be imposed on the unknown function or functions. It is the object of this chapter to show that all such problems can be dealt with by the finite element method.},
author = {Zienkiewicz, O.C. and Taylor, R.L.},
doi = {http://dx.doi.org/10.1016/B978-075066431-8.50171-5},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Zienkiewicz FEM - Vol 1 Basics Fundamentals/63205{\_}03.pdf:pdf},
isbn = {0 7506 5049 4},
journal = {Finite Elem. Method Vol. 1 Basis},
pages = {39--60},
title = {{Generalization of the finite element concepts. Galerkin-weighted residual and variational approaches}},
url = {http://freeit.free.fr/Finite Element/Zienkiewicz/Volume 1 The Basis/},
year = {2000}
}
@article{Lerch2010,
author = {Lerch, R},
doi = {10.1007/978-3-642-05455-6},
isbn = {9783642054556},
title = {{Schaltungen und Systeme}},
year = {2010}
}
@article{Constitutive,
author = {Constitutive, The},
title = {{Developing and Implementing Selected Constitutive Models for Elasto-Plastic-Damage}}
}
@article{Ewing2003,
author = {Ewing, Following},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Nicholson 2003 - Finite Element Analysis Thermomechanics of Solids/0749{\_}C03.pdf:pdf},
journal = {Methods},
pages = {43--49},
title = {{Introduction to Variational and Numerical Methods 3.1}},
year = {2003}
}
@article{Watzig2009,
author = {W{\"{a}}tzig, H. and Mehnert, W. and B{\"{u}}hler, W.},
isbn = {978-3-8047-2439-6},
pages = {1--339},
title = {{Mathematik und Statistik kompakt}},
year = {2009}
}
@article{Steffen,
author = {Steffen, Horst and Bausch, Hansj{\"{u}}rgen},
isbn = {9783835100145},
title = {{Horst Steffen, Hansj{\"{u}}rgen Bausch}}
}
@article{Zienkiewiczb,
author = {Zienkiewicz, O C},
title = {{Method for Fluid Dynamics}}
}
@article{Amara1994,
abstract = {LES VARIATIONS RAPIDES DE PRESSION ET DE TEMPERATURE INFLUENT CONSIDERABLEMENT SUR LES ECHANGES THERMIQUES INSTANTANES ENTRE LE GAZ ET LES PAROIS DE LA CHAMBRE DE COMBUSTION. UNE ETUDE EXPERIMENTALE DE LA DENSITE SURFACIQUE DU FLUX DE CHALEUR ECHANGE EN DEUX POINTS DE LA PAROI DE LA CULASSE A PERMIS EN EFFET DE METTRE EN EVIDENCE L'ACCUMULATION D'ENERGIE DANS LA COUCHE LIMITE THERMIQUE QUI SE MANIFESTE PAR UN DEPHASAGE TEMPOREL ENTRE LE FLUX ET L'ECART DE TEMPERATURE GLOBAL GAZ-PAROI. EN REGIME LAMINAIRE INSTATIONNAIRE, UNE SIMULATION DE CES ECHANGES FAIT BIEN APPARAITRE DES EXTREMA LOCAUX DE TEMPERATURE DANS LA COUCHE LIMITE THERMIQUE. UNE INTERPRETATION DU MECANISME DE FORMATION ET DE DEPLACEMENT DE CES EXTREMA EST DONNEE. LES ECHANGES THERMIQUES EN REGIME TURBULENT SONT DECRITS A L'AIDE DU MODELE MONODIMENSIONNEL DE YANG ET MARTIN OU L'EFFET DE LA TURBULENCE EST PRIS EN COMPTE PAR LE BIAIS DE LA CONDUCTIVITE THERMIQUE TURBULENTE. CE MODELE A ETE MODIFIE POUR LIMITER L'AUGMENTATION DE LA CONDUCTIVITE THERMIQUE TURBULENTE AVEC LA DISTANCE A LA PAROI. LE PARAMETRE DE LIMITATION EST LIE A LA VALEUR LOCALE DE LA VISCOSITE TURBULENTE. LE MODELE AINSI OBTENU PERMET UNE MEILLEURE DETERMINATION DE L'EPAISSEUR DE LA COUCHE LIMITE THERMIQUE ET S'ADAPTE DE LUI-MEME A TOUTE SITUATION INTERMEDIAIRE ENTRE LE REGIME LAMINAIRE ET LES REGIMES FORTEMENT TURBULENTS, LA DENSITE DU FLUX DE CHALEUR ETANT MODULEE EN CONSEQUENCE. L'IMPLANTATION DE CE MODELE DANS LE CODE DE SIMULATION KIVA2 A MONTRE QUE LA PRISE EN COMPTE DES INSTATIONNARITES DE TEMPERATURE ET DE PRESSION CONSTITUE UNE AMELIORATION PAR RAPPORT AUX LOIS DE PAROI LOGARITHMIQUES MAIS SE REVELE INSUFFISANTE. UNE SUPERPOSITION DU MODELE MONODIMENSIONNEL ET D'UNE LOI DE PAROI LOGARITHMIQUE RENDANT COMPTE DE L'EFFET DE LA VITESSE TANGENTIELLE DONNE DES RESULTATS SE RAPPROCHANT AU MIEUX DES EVOLUTIONS EXPERIMENTALES ET CECI POUR DIFFERENTES VITESSES DE ROTATION. UNE ETUDE PARAMETRIQUE COMPARATIVE EST ENSUITE REALISEE POUR MONTRER L'IMPACT DU CHOIX D'UN MODELE DE CALCUL DU FLUX DE CHALEUR PARIETAL SUR LA DETERMINATION DES CHAMPS DE VITESSE, DE TEMPERATURE, D'ENERGIE CINETIQUE TURBULENTE ET DE SON TAUX DE DISSIPATION A LA FIN DE LA COURSE DE COMPRESSION.},
author = {Amara, S},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Heat Transfer Combustion Chamber/1994{\_}Amara{\_}Elaboration et validation dun modele de transferts thermiques dun moteur{\_}UebersichtWaermeuebergangsmodelle.pdf:pdf},
keywords = {Chambre de combustion,Cin{\{}{\'{e}}{\}}tique turbulente,R{\{}{\'{e}}{\}}gime laminaire},
publisher = {{\{}{\'{E}}{\}}cole centrale de Lyon},
title = {{Elaboration et validation d'un mod{\{}{\`{e}}{\}}le de transferts thermiques instationnaires gaz paroi dans la chambre de combustion d'un moteur}},
url = {http://cat.inist.fr/?aModele=afficheN{\%}7B{\&}{\%}7Dcpsidt=162697},
year = {1994}
}
@article{McDowell2003,
abstract = {High cycle fatigue (HCF) life in cast Al-Mg-Si alloys is particularly sensitive to the combination of microstructural inclusions and stress concentrations. Inclusions can range from large-scale shrinkage porosity with a tortuous surface profile to entrapped oxides introduced during the pour. When shrinkage porosity is controlled, the relevant microstructural initiation sites are often the larger Si particles within eutectic regions. In this paper, a HCF model is introduced which recognizes multiple inclusion severity scales for crack formation. The model addresses the role of constrained microplasticity around debonded particles or shrinkage pores in forming and growing microstructurally small fatigue cracks and is based on the cyclic crack tip displacement rather than linear elastic fracture mechanics stress intensity factor. Conditions for transitioning to long crack fatigue crack growth behavior are introduced. The model is applied to a cast A356-T6 Al alloy over a range of inclusion severities. ?? 2002 Elsevier Science Ltd. All rights reserved.},
author = {McDowell, D L and Gall, K and Horstemeyer, M F and Fan, J},
doi = {10.1016/S0013-7944(02)00021-8},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/2003{\_}McDowell{\_}Microstructure-based fatigue modeling of cast A356-T6 alloy.pdf:pdf},
isbn = {0013-7944},
issn = {00137944},
journal = {Eng. Fract. Mech.},
keywords = {A356,Cast alloys,High cycle fatigue,Microstructure},
number = {1},
pages = {49--80},
pmid = {119},
title = {{Microstructure-based fatigue modeling of cast A356-T6 alloy}},
volume = {70},
year = {2003}
}
@phdthesis{Hoelz2015,
author = {H{\"{o}}lz, Peter},
school = {Institute of Fusion and Reactor Technology (KIT)},
title = {{Thermische Untersuchung einer Radialturbine zur Abgasenergier{\"{u}}ckgewinnung}},
type = {Master thesis},
year = {2015}
}
@article{Berechnungsprogramme,
author = {Berechnungsprogramme, Finite Elemente and Elemente, Finite},
title = {{5 Optimierungsprogrammsysteme}}
}
@article{Castillo2009b,
author = {Castillo, E},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Probabilistic Aspects/A Unified Statistical Methodology for Modeling Fatigue Damage{\_}Castillo/Kap3{\_}Length Effect.pdf:pdf},
journal = {Media},
pages = {91--109},
title = {{Length Effect}},
year = {2009}
}
@article{Devulder2010a,
author = {Devulder, Anne and Aubry, Denis and Puel, Guillaume},
doi = {10.1007/s00466-010-0476-2},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/2 scale models papers/2010{\_}Devulder+Aubrypouel{\_}Two time scale fatigue modelling-application to damage.pdf:pdf},
issn = {01787675},
journal = {Comput. Mech.},
keywords = {Bone,Damage,Fatigue,Time homogenization},
number = {6},
pages = {637--646},
title = {{Two-time scale fatigue modelling: Application to damage}},
volume = {45},
year = {2010}
}
@article{Zavala2011a,
author = {Zavala, Jos{\'{e}} Carlos and Folkerts, Charles},
doi = {10.4271/2011-01-1409},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2011{\_}Zavala{\_}Knock Detection and Estimation Based on Heat Release Startegies.pdf:pdf},
title = {{Knock Detection and Estimation Based on Heat Release Strategies}},
url = {http://papers.sae.org/2011-01-1409/},
year = {2011}
}
@article{Zienkiewicza,
abstract = {In Chapters 4, 5, and 6 the reader was shown in some detail how linear elasticity problems could be formulated and solved using very simple {\textregistered}nite element forms. In Chapter 7 this process was repeated for the quasi-harmonic equation. Although the detailed algebra was concerned with shape functions which arose from triangular and tetrahedral shapes only it should by now be obvious that other element forms could equally well be used. Indeed, once the element and the corresponding shape functions are determined, subsequent operations follow a standard, well-de{\textregistered}ned path which could be entrusted to an algebraist not familiar with the physical aspects of the problem. It will be seen later that in fact it is possible to program a computer to deal with wide classes of problems by specifying the shape functions only. The choice of these is, however, a matter to which intelligence has to be applied and in which the human factor remains paramount. In this chapter some rules for the generation of several families of one-, two-, and three-dimensional elements will be presented. In the problems of elasticity illustrated in Chapters 4, 5, and 6 the displacement variable was a vector with two or three components and the shape functions were written in matrix form. They were, however, derived for each component separately and in fact the matrix expressions in these were derived by multiplying a scalar function by an identity matrix [e.g., Eqs (4.7), (5.3), and (6.7)]. This scalar form was used directly in Chapter 7 for the quasi-harmonic equation. We shall therefore concentrate in this chapter on the scalar shape function forms, calling these simply N i . The shape functions used in the displacement formulation of elasticity problems were such that they satisfy the convergence criteria of Chapter 2: (a) the continuity of the unknown only had to occur between elements (i.e., slope continuity is not required), or, in mathematical language, C 0 continuity was needed; (b) the function has to allow any arbitrary linear form to be taken so that the constant strain (constant {\textregistered}rst derivative) criterion could be observed. The shape functions described in this chapter will require the satisfaction of these two criteria. They will thus be applicable to all the problems of the preceding chapters},
author = {Zienkiewicz, O.C.},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Zienkiewicz FEM - Vol 1 Basics Fundamentals/63205{\_}04.pdf:pdf},
title = {{Standard ' anhierarchical' element shape functions: some general families of C{\_}0 continuity 8.1 Introduction}}
}
@article{Rangarajan2012a,
abstract = {We describe a method for discretizing planar C2-regular domains immersed in non-conforming triangulations. The method consists in constructing mappings from triangles in a background mesh to curvilinear ones that conform exactly to the immersed domain. Constructing such a map relies on a novel way of parameterizing the immersed boundary over a collection of nearby edges with its closest point projection. By interpolating the mappings to curvilinear triangles at select points, we recover isoparametric mappings for the immersed domain defined over the background mesh. Indeed, interpolating the constructed mappings just at the vertices of the background mesh yields a fast meshing algorithm that involves only perturbing a few vertices near the boundary. For the discretization of a curved domain to be robust, we have to impose restrictions on the background mesh. Conversely, these restrictions define a family of domains that can be discretized with a given background mesh. We then say that the background mesh is a universal mesh for such a family of domains. The notion of universal meshes is particularly useful in free/moving boundary problems because the same background mesh can serve as the universal mesh for the evolving domain for time intervals that are independent of the time step. Hence it facilitates a framework for finite element calculations over evolving domains while using a fixed background mesh. Furthermore, since the evolving geometry can be approximated with any desired order, numerical solutions can be computed with high-order accuracy. We demonstrate these ideas with various numerical examples.},
archivePrefix = {arXiv},
arxivId = {1201.4903},
author = {Rangarajan, Ramsharan and Lew, Adrian J.},
doi = {10.1002/nme},
eprint = {1201.4903},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/2010{\_}Miehe{\_}Thermodynamically consistent phase-field models of fracture-Variational principles and multi field FE implementations.pdf:pdf},
keywords = {coupled multi-field problems,crack propagation,finite elements,fracture,gradient-type damage,incremental variational,phase-fields,principles},
number = {March},
pages = {1273--1311},
title = {{Universal Meshes: A new paradigm for computing with nonconforming triangulations}},
url = {http://arxiv.org/abs/1201.4903},
year = {2012}
}
@article{Mutzke2016a,
abstract = {{\{}{\textcopyright}{\}} 2016 SAE International.Knocking combustion places a major limit on the performance and efficiency of spark ignition engines. Spontaneous ignition of the unburned air-fuel mixture ahead of the flame front leads to a rapid release of energy, which produces pressure waves that cause the engine structure to vibrate at its natural frequencies and produce an audible 'pinging' sound. In extreme cases of knock, increased temperatures and pressures in the cylinder can cause severe engine damage. Damage is thought to be caused by thermal strain effects that are directly related to the heat flux. Since it will be the maximum values that are potentially the most damaging, then the heat flux needs to be measured on a cycle-by-cycle basis. Previous work has correlated heat flux with the pressure fluctuations on an average basis, but the work here shows a correlation on a cycle-by-cycle basis. The in-cylinder pressure and surface temperature were measured using a pressure transducer and eroding-type thermocouple. These sensors were installed side-by-side at the surface of the cylinder in order to investigate the relationship between knock and heat flux on a cycle-by-cycle basis. A finite difference method was implemented to solve the one-dimensional unsteady heat conduction equation and calculate the temperature distribution away from the surface of the combustion chamber, and thus the instantaneous heat flux. The knock intensity was varied by controlling the fuel quality, compression ratio, ignition timing and air-fuel ratio. The measured heat flux was compared with pressure-based knock indices and it was found that as knock intensity increases, the correlation with peak heat flux became stronger. Results from different fuels and engine operating conditions did not collapse onto the same trend line. At higher speeds and higher compression ratios the heat flux was higher at a given level of knock intensity. The co-location of the pressure transducer and heat flux sensor meant that a correlation was found on a cycle-by-cycle basis.},
author = {Mutzke, J and Scott, B and Stone, R and Williams, J},
doi = {10.4271/2016-01-0700},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2016{\_}Mutzke{\_}The Effect of Combustion Knock on the Instantaneous Heat Flux in Spark Ignition Engines.pdf:pdf},
journal = {SAE Tech. Pap.},
title = {{The Effect of Combustion Knock on the Instantaneous Heat Flux in Spark Ignition Engines}},
volume = {2016-April},
year = {2016}
}
@article{Leiden1973,
author = {Leiden, Noordhoff International Publishing-},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/1971{\_}Bowles{\_}The role of inclusions in fatigue crack initiation in an aluminum alloy.pdf:pdf},
journal = {Int. J.},
number = {2},
pages = {171--179},
title = {{The role of inclusions in fatigue crack initiation in an alumS ' mum alloy}},
volume = {9},
year = {1973}
}
@article{Esfahanian2006a,
abstract = {In this study, the heat transfer to an engine piston crown is calculated. Three different methods for the combustion boundary condition are used. The results of different combustion side boundary condition treatments are compared and their effects on the thermal behavior of the piston are investigated. It has been shown that using spatial and time averaged combustion side boundary condition is a suitable treatment method within engineering approximations. An interface between KIVA-3V and NASTRAN codes is developed. ?? 2005 Elsevier Ltd. All rights reserved.},
author = {Esfahanian, V and Javaheri, A and Ghaffarpour, M},
doi = {10.1016/j.applthermaleng.2005.05.002},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2006{\_}Esfahanian{\_}Thermal analysis of an SI engine piston using different combustion boundary condition treatements.pdf:pdf},
journal = {Appl. Therm. Eng.},
keywords = {Boundary Condition Treatment,Combustion,Heat transfer,Piston},
number = {2-3},
pages = {277--287},
title = {{Thermal analysis of an SI engine piston using different combustion boundary condition treatments}},
volume = {26},
year = {2006}
}
@article{G,
author = {G, Lutering and Williams, J.C.},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2010{\_}Jaroslav Pokluda+Pavel {\v{S}}andera{\_}Micromechanisms of fracture and fatigue{\_}Buch/Front.pdf:pdf},
isbn = {9781848825062},
journal = {New York},
title = {{Engineering Materials and Processes}}
}
@book{Lienhard2003,
address = {Cambridge Massachusetts},
author = {Lienhard, John H. IV and Lienhard, John H. V},
edition = {3},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/J.H.Lienhard{\_}AHeatTransferBook.pdf:pdf},
pages = {762},
publisher = {Phlogiston Press},
title = {{A heat transfer textbook}},
year = {2003}
}
@article{Zienkiewicz2013c,
abstract = {In this chapter we present matrix differential equations governing transient problems for a variety of physical situations. A finite element discretization in the space dimension is used and a semi-discretization process followed (as introducled in Chapters 3 and 5). For structural problems the result is a set of equations involving a mass, damping and stiffness matrix. The second order equation in time may be solved formally using analytical methods in which time is represented by exponential functions. For undamped systems this leads to a classical eigen-problem in which the natural frequencies and mode shapes for a system may be identified. Including damping makes the solution feasible in complex arithmetic. General transient solutions are obtained from modal representations. A second form is forced periodic response in which applied force is represented in periodic form.},
author = {Zienkiewicz, O.C. and Taylor, R.L. and Zhu, J.Z.},
doi = {10.1016/B978-1-85617-633-0.00012-5},
isbn = {9781856176330},
issn = {00295981},
journal = {Finite Elem. Method its Basis Fundam.},
pages = {379--405},
title = {{The Time Dimension: Semi-Discretization of Field and Dynamic Problems}},
url = {http://linkinghub.elsevier.com/retrieve/pii/B9781856176330000125},
year = {2013}
}
@article{Meister2011d,
abstract = {Die wichtigsten Verfahren zur numerischen L{\{}{\"{o}}{\}}sung von linearen Gleichungssystemen in einer umfassenden Einf{\{}{\"{u}}{\}}hrung, die zum Verst{\{}{\"{a}}{\}}ndnis nur geringe mathematische Vorkenntnisse ben{\{}{\"{o}}{\}}tigt. Behandelt werden sowohl die direkten als auch die iterativen Verfahren, wobei der Autor gro{\{}{\ss}{\}}en Wert auf eine sorgf{\{}{\"{a}}{\}}ltige Herleitung dieser Verfahren legt. Au{\{}{\ss}{\}}erdem sind sehr detaillierte Pseudocodes enthalten, mit deren Hilfe sich die jeweiligen Verfahren in einer beliebigen Programmiersprache sofort auf dem Computer realisieren lassen. Das Lehrbuch ist auch f{\{}{\"{u}}{\}}r Natur- und Ingenieurwissenschaftler geeignet, die in vielen praktischen Anwendungen mit der L{\{}{\"{o}}{\}}sung von linearen Gleichungssystemen konfrontiert sind.},
archivePrefix = {arXiv},
arxivId = {1011.1669v3},
author = {Meister, Andreas},
doi = {10.1007/978-3-8348-8100-7},
eprint = {1011.1669v3},
isbn = {978-3-8348-1550-7},
issn = {1098-6596},
journal = {Matrix},
pages = {36--68},
pmid = {25246403},
title = {{Numerik linearer Gleichungssysteme}},
url = {http://link.springer.com/10.1007/978-3-8348-8100-7},
year = {2011}
}
@article{Energiea,
author = {Energie, Thermische and Energie, Mechanische and Energie, Elektrische},
title = {{Der Hubkolbenmotor}}
}
@article{Kametani1980,
author = {Kametani, T and Umezawa, O},
doi = {10.1248/cpb.37.3229},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Heat Transfer Combustion Chamber/1986{\_}Enomoto{\_}Heat Loss to Combustion Chamber Wall of 4-Stroke Gasoline Engine - Heat Loss to Head and Valves.pdf:pdf},
issn = {09168451},
journal = {Chem. Pharm. Bull.},
number = {6},
pages = {369--375},
pmid = {8987871},
title = {{NII-Electronic Library Service}},
volume = {28},
year = {1980}
}
@article{Mohammadi2008a,
abstract = {A computational fluid dynamics (CFD) code is applied to simulate fluid flow, heat transfer and combustion in a four-stroke single cylinder engine with pent roof combustion chamber geometry, having two inlet valves and two exhaust valves. Heat flux and heat transfer coefficient on the cylinder head, cylinder wall, piston, intake and exhaust valves are determined with respect to crank angle position. Results for a certain condition are compared for total heat transfer coefficient of the cylinder engine with available correlation proposed by experimental measurement in the literature and close agreement are observed. It was found that the local value of heat transfer coefficient varies considerably in different parts of the cylinder, but they have equivalent trend with crank angle. Based on the results, new correlations are suggested to predict maximum and minimum convective heat transfer coefficient in the combustion chamber of a SI engine. ?? 2007 Elsevier Ltd. All rights reserved.},
author = {Mohammadi, A. and Yaghoubi, M. and Rashidi, M.},
doi = {https://doi.org/10.1016/j.icheatmasstransfer.2007.06.008},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2008{\_}Mohammadi{\_}Analysis of local convective heat transfer in a spark ignition engine.pdf:pdf},
journal = {Int. Commun. Heat Mass Transf.},
keywords = {Combustion chamber,Heat flux,Heat transfer coefficient,SI engine},
number = {2},
pages = {215--224},
title = {{Analysis of local convective heat transfer in a spark ignition engine}},
volume = {35},
year = {2008}
}
@article{Feldera,
author = {Felder, Elektromagnetische and Emv, Der},
title = {{5 Elektromagnetische Felder}}
}
@article{Stromfunktiona,
author = {Stromfunktion, Potential-},
pages = {293--326},
title = {{10 Potentialstr o ¨ mungen}}
}
@article{Auflagen,
author = {Auflagen, Gesetzliche},
title = {{17 Zuverl{\{}{\"{a}}{\}}ssigkeit und Erprobung von Fahrzeuggetrieben}}
}
@article{Reifen1972,
author = {Reifen, Der Entwicklungsprozess and Reifen, Die and Beispiel, Am and Fahrzeughersteller, Jeder and Beispiel, Zum and Fahrzeuge, Mercedes-benz and Erstausr, Diese},
pages = {1--4},
title = {{1 Einleitung}},
year = {1972}
}
@article{Programmiersprachen,
author = {Programmiersprachen, H{\"{o}}here and Vorteil, Den},
title = {{Projekte in C gel{\{}{\"{o}}{\}}st}}
}
@article{Hansen2004a,
abstract = {The Hall-Petch relation is discussed separately for the yield stress of undeformed polycrystalline metals and for the flow stress of deformed metals. Key structural parameters are the boundary spacing, between grain boundaries in the former case and between dislocation boundaries and high angle boundaries in the latter. An analysis of experimental data supports the Hall-Petch relation for undeformed metals over a grain size range from about 20 nm to hundreds of micrometers. For deformed metals, boundary strengthening is not a constant and the Hall-Petch relation must be modified. ?? 2004 Acta Materialia Inc. Published by Elsevier Ltd. All rights reserved.},
author = {Hansen, Niels},
doi = {10.1016/j.scriptamat.2004.06.002},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2004{\_}Hansen Hall–Petch relation and boundary strengthening.pdf:pdf},
isbn = {1359-6462},
issn = {13596462},
journal = {Scr. Mater.},
keywords = {Dislocation boundaries,Flow stress,Grain size,Nanostructure,Yield stress},
number = {8 SPEC. ISS.},
pages = {801--806},
title = {{Hall-petch relation and boundary strengthening}},
volume = {51},
year = {2004}
}
@article{Universit2001a,
author = {Universit, Technischen},
title = {{Technische Universit{\{}{\"{a}}{\}}t M{\{}{\"{u}}{\}}nchen Institut f{\{}{\"{u}}{\}}r Werkstoffe und Verarbeitung Forschungsgruppe Prof . Schmitt-Thomas Werkstoffgerechte Auslegung und Festigkeitsnachweis f{\{}{\"{u}}{\}}r Verbrennungsmotorkolben aus Mesophasenkohlenstoff}},
year = {2001}
}
@article{Pang2004,
abstract = {The performance of the conventional engine-cooling system has always been constrained by the passive nature of the system and the need to provide the required heat-rejection capability at high-power conditions. This leads to considerable losses in the cooling system at part-load conditions where vehicles operate most of the time. A set of design and operating features from advanced enginecooling systems is reviewed and evaluated for their potential to provide improved engine protection while improving fuel efficiency and emissions output. Although these features demonstrate significant potential to improve engine performance, their full potential is limited by the need to balance between satisfying the engine-cooling requirement under all operating ambient conditions and the system effectiveness, as with any conventional engine-cooling system. The introduction of controllable elements allows limits to be placed on the operating envelope of the cooling system without restricting the benefits offered by adopting these features. The integration of split cooling and precision cooling with controllable elements has been identified as the most promising set of concepts to be adopted in a modern engine-cooling system. C1 Univ Bath, Dept Mech Engn, Bath BA2 7AY, Avon, England},
author = {Pang, H. H. and Brace, C. J.},
doi = {10.1243/0954407042580110},
file = {:C$\backslash$:/Users/p327208/Desktop/Promotion/Literature/Motorspezifisch/Thermal Coating + Water Heat Transfer + Applikation/2004{\_}Pang+Brace{\_}Review of engine cooling technologies for modern engines.pdf:pdf},
journal = {Proc. Inst. Mech. Eng. Part D J. Automob. Eng.},
keywords = {Emissions reduction,Engine cooling,Fuel efficiency},
number = {11},
pages = {1209--1215},
title = {{Review of engine cooling technologies for modern engines}},
volume = {218},
year = {2004}
}
@article{Prinzip,
author = {Prinzip, Archimedisches and Gleichung, Bernoullische},
title = {{Ucke}}
}
@article{Stupkiewicz2007,
author = {Stupkiewicz, Stanis{\l}aw},
doi = {10.1007/978-3-540-49717-2_3},
isbn = {3540497161},
issn = {16137736},
journal = {Lect. Notes Appl. Comput. Mech.},
number = {30},
pages = {17--35},
title = {{Homogeneous surface layers}},
volume = {2006},
year = {2007}
}
@article{Metzger2014,
abstract = {This paper reports on the evolution of cracks in the cylinder heads of a large V8 Diesel engine during cyclic engine tests. The observations are compared with the predictions of a lifetime model for combined thermo-mechanical (TMF) and high cycle fatigue (HCF) loading, which is based on a fracture mechanics analysis of microcrack growth in viscoplastic solids and assumes that the crack advance per cycle is proportional to the cyclic crack tip opening displacement. Since the material of the cylinder heads, the cast iron EN-GJV450, exhibits the typical features of cast iron, namely pressure dependence of the yield stress, dilatancy and tension-compression asymmetry, the Gurson model is applied and combined with the viscoplastic Chaboche model. This constitutive model together with the lifetime model is implemented into a finite element code as a user defined material routine. Published model parameters for the considered cast iron are used to carry out the simulation of the engine test. This simulation comprises a CFD analysis to determine the heat transfer coefficients, a thermal analysis of the load cycle and the mechanical analysis. The thermal analysis reproduces the temperatures at various measuring points sufficiently accurately. Finally, the mechanical analysis predicts the location and orientation of the cracks in the valve bridges correctly in all cases. However, the lifetime predictions are rather conservative compared to the tests (by a factor of 1 to 5 in lifetime). This is discussed and explained by the fact that the cracks were detected in the tests only when they had already spread over a substantial fraction of the valve bridge width. To describe this situation a long-crack analysis would be necessary, which is not yet included in the applied lifetime model},
author = {Metzger, Mario and Leidenfrost, Marc and Werner, Ewald and Riedel, Hermann and Seifert, Thomas},
doi = {10.4271/2014-01-9047},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2014{\_}Metzger{\_}Lifetime prediction of EN-GJV 450 Cast Iron Cylinder Heads und combined thermo-mechanical and hcf loading.pdf:pdf},
journal = {SAE Int. J. Engines},
number = {2},
pages = {2014--01--9047},
title = {{Lifetime Prediction of EN-GJV 450 Cast Iron Cylinder Heads under Combined Thermo-Mechanical and High Cycle Fatigue Loading}},
volume = {7},
year = {2014}
}
@article{Lakes2006,
author = {Lakes, Roderic S},
doi = {doi:10.1201/9781420049510.ch40},
isbn = {0-8493-1491-7},
journal = {Biomed. Eng. Fundam.},
number = {1},
pages = {14--1--41--14},
pmid = {1022301},
title = {{Composite Biomaterials}},
year = {2006}
}
@article{Oplinger1998,
author = {Oplinger, D W},
journal = {Handb. Compos.},
pages = {57},
title = {{Mechanical Fastening and Adhesive Bonding}},
year = {1998}
}
@article{To2013a,
author = {To, Nswers},
doi = {http://dx.doi.org/10.1016/B978-343722790-5.50023-3},
isbn = {978-3-437-22790-5},
number = {450},
pages = {96--99},
title = {{Kapitel 17}},
volume = {5975},
year = {2013}
}
@article{Wang1985b,
author = {Wang, C S and Berry, G F},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/1985{\_}Wang{\_}Heat Transfer in Internal Combustion Engines.pdf:pdf},
journal = {Asme},
number = {Ic},
pages = {1--7},
title = {{Heat Transfer in Internal Combustion Engines}},
year = {1985}
}
@article{Liu1972a,
author = {Liu, I. Shih and M{\"{u}}ller, Ingo},
doi = {10.1007/BF00250689},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Thermodynamik/Liu{\_}Entropieprinzip{\_}Lagrange/On the Thermodynamics and Thermostatics of Fluid in Electromagnetic Fields {\_}Liu.pdf:pdf},
issn = {00039527},
journal = {Arch. Ration. Mech. Anal.},
number = {2},
pages = {149--176},
title = {{On the thermodynamics and thermostatics of fluids in electromagnetic fields}},
volume = {46},
year = {1972}
}
@article{Shimada2004,
abstract = {The effect of local lubricant viscosity on the temperature and thickness of oil film on a piston ring in a diesel engine is analyzed by using the Reynolds equation, and unsteady and two-dimensional energy equation with heat generated from viscous dissipation. The oil film viscosity for a multi-grade oil is then estimated by using the local oil film temperature and the local shear rate. Moreover, the heat transfer between ring and liner surfaces is examined. The oil film thickness calculated from this method is lesser than that of the case where the viscosity is based on the liner temperature and the mean shear rate. Maximum values of heat transfer at the ring and liner surfaces are obtained at the vicinity of crank angle where the oil film thickness is at a minimum.ER -},
author = {Shimada, Akiko and Harigaya, Yasuo and Suzuki, Michiyoshi and Takiguchi, Masaaki},
doi = {10.4271/2004-32-0024},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Heat Transfer Combustion Chamber/2004{\_}Shimada{\_}An Analysis of Oil Film Temperature - Oil Film Thickness and Heat Transfer on a piston ring of internal combustion engine.pdf:pdf},
isbn = {0791846628},
issn = {07424795},
number = {724},
title = {{An Analysis of Oil Film Temperature, Oil Film Thickness and Heat Transfer on a Piston Ring of Internal Combustion Engine: The Effect of Local Lubricant Viscosity}},
url = {http://papers.sae.org/2004-32-0024/},
year = {2004}
}
@article{Wang2007a,
abstract = {Heat flux measurement and pressure-based heat release analysis have been performed on a spray-guided direct-injection spark-ignition single-cylinder research engine. A two-dimensional model of the heat flux sensor has been used to calculate the heat flux from the measured surface temperature. The effects of the ignition timing, air-fuel ratio, and mixture preparation on the engine heat flux and heat release have been investigated at a specific operating condition. An engine thermodynamic simulation code has been used to predict the gas-to-wall heat transfer using different heat transfer correlations. It was found that both the heat release rate and the heat flux are strongly influenced by ignition timing and air-fuel ratio. The results also show that late direct injection has a faster initial burn rate even compared with the plenum injection mode. The modelled heat transfer has been compared with the measured results and a modified Woschni correlation has been proposed. JAUTO586 {\textcopyright} IMechE 2007.},
author = {Wang, X. and Price, P. and Stone, C. R. and Richardson, D.},
doi = {10.1243/09544070JAUTO586},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Heat Transfer Combustion Chamber/2007{\_}Wang{\_}Heat release and heat flux in a spray-guided direct-injection gasoline engine.pdf:pdf},
issn = {09544070},
journal = {Proc. Inst. Mech. Eng. Part D J. Automob. Eng.},
keywords = {Direct-injection spark ignition,Heat release,Heat transfer},
number = {11},
pages = {1441--1452},
title = {{Heat release and heat flux in a spray-guided direct-injection gasoline engine}},
volume = {221},
year = {2007}
}
@article{Ness1998,
author = {Ness, Van},
title = {{ahlte Lehrb u ¨ cher der Thermodynamik}},
year = {1998}
}
@article{Metallplastizit2013e,
author = {Metallplastizit, Hrungdie and Helm, Dirk},
number = {November},
pages = {1--29},
title = {{Prozesssimulation in Der Umformtechnik}},
year = {2013}
}
@article{Wallentowitz2006j,
author = {Wallentowitz, Henning and Reif, Konrad},
doi = {10.1007/978-3-8348-9121-1_5},
journal = {Handb. Kraftfahrzeugelektronik - Grundlagen, Kompon. Syst. Anwendungen},
title = {{Beleuchtung}},
url = {http://www.springerlink.com/index/10.1007/978-3-8348-9121-1{\%}7B{\_}{\%}7D5},
year = {2006}
}
@article{Lastenheft,
author = {Lastenheft, Zielkatalog},
pages = {22},
title = {{6 Konzeptentwicklung / Projekthandhabung}}
}
@article{Lubarda2002,
abstract = {In this chapter we briefly summarize the fundamental relations of$\backslash$nthe kinematics of large deformations, restricting ourselves to the$\backslash$napplications we have in mind. For concise treatments we advise the$\backslash$nliterature on continuum mechanics},
author = {Lubarda, Vlado a.},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Nicholson 2003 - Finite Element Analysis Thermomechanics of Solids/0749{\_}C04.pdf:pdf},
isbn = {0849311381},
journal = {Elastoplast. Theory},
pages = {51--71},
title = {{Kinematics of deformation}},
year = {2002}
}
@article{Fs2013b,
author = {Fs},
doi = {10.1007/978-1-4614-0502-3},
file = {:C$\backslash$:/Users/p327208/Desktop/Promotion/Literature/Crystal Plasticity Approaches/2010{\_}Jaroslav Pokluda+Pavel {\v{S}}andera{\_}Micromechanisms of fracture and fatigue{\_}Buch/Kap0{\_}Introduction.pdf:pdf},
isbn = {2009004043},
number = {1},
pages = {0--10},
title = {{Chapter 0}},
year = {2013}
}
@article{Linear2014,
author = {Linear, D},
doi = {10.1016/B978-1-85617-635-4.00029-7},
isbn = {9781856176354},
journal = {Finite Elem. Method Fluid Dyn.},
pages = {509--510},
title = {{Integration Formulae}},
url = {http://linkinghub.elsevier.com/retrieve/pii/B9781856176354000297},
year = {2014}
}
@article{Metallplastizit2013a,
author = {Metallplastizit, Hrungdie and Helm, Dirk},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/{\_}skripte/Helm - Prozesssimulation und Umformtechnik/Vorlesung-011-2012-2013-Handout.pdf:pdf},
number = {November},
pages = {1--29},
title = {{Prozesssimulation in Der Umformtechnik}},
year = {2013}
}
@article{Fs2013,
author = {Fs},
doi = {10.1007/978-1-4614-0502-3},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/Micromechanisms of fracture and fatigue/Kap0{\_}Introduction.pdf:pdf},
isbn = {2009004043},
number = {1},
pages = {0--10},
title = {{Chapter 0}},
year = {2013}
}
@article{Kalghatgi1995,
abstract = {Net heat release, knock characteristics and temperature were derived{\$}\backslash{\$}nfrom in-cylinder pressure and end-gas CARS measurements for different{\$}\backslash{\$}nfuels in a single-cylinder engine. The maximum net heat release rate{\$}\backslash{\$}nresulting from the final phase of autoignition is closely associated{\$}\backslash{\$}nwith knock intensity. Aromatic fuels have lower maximum heat release{\$}\backslash{\$}nrates and lower knock intensities than expected from their octane number{\$}\backslash{\$}nwhen compared to paraffinic fuels; this is observed even when there is{\$}\backslash{\$}nsignificant heating of the end-gas from pre-flame reactions. Leaner{\$}\backslash{\$}nmixtures have lower combustion rates so that pressure development is{\$}\backslash{\$}nslowed and hence ignition needs to be more advanced to get knock to{\$}\backslash{\$}noccur as frequently as in a richer mixture. However, for a given{\$}\backslash{\$}nfrequency of knock occurrence, there is no significant difference in{\$}\backslash{\$}npeak net heat release rates and hence in knock intensities for different{\$}\backslash{\$}nmixture strengths.},
author = {Kalghatgi, G T and Golombok, M and Snowdon, P},
doi = {10.1080/00102209508951924},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Klopfen{\_}Ottomotor/2007{\_}Kalghatgi{\_}Fuel effect on knock - heat release and CARS tempertures in SI Engine.pdf:pdf},
issn = {0010-2202},
journal = {Combust. Sci. Technol.},
number = {March},
pages = {209--228},
title = {{Fuel effects on knock, heat release and `'CARS'' temperatures in a spark ignition engine}},
volume = {111},
year = {1995}
}
@article{Senkung2007,
author = {Senkung, Die and Statements, Aktuelle and Motoren, Erste and Chrysler, Daimler- and Hersteller, Weitere and Einspritzdr, Heutige},
journal = {Stand},
pages = {427--432},
title = {{16 Ausblick}},
year = {2007}
}
@article{Sinne1884,
author = {Sinne, Im and Joseph, Jean and Lenoir, Etienne and Jahr, Im and Otto, Nikolaus August and Benz, Carl and Daimler, Gottlieb and Maybach, Wilhelm and Spritzd, Maybachschen and Benzineinspritzung, Die and Jahre, Im and Station, Maschinenfabrik and Spiel, Johannes},
pages = {3--27},
title = {{2 Geschichte der Benzin-Direkteinspritzung}},
year = {1884}
}
@article{Morris1979,
author = {Morris, W L},
doi = {10.1007/BF02686400},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/1979{\_}Morris{\_}Microcrack closure phenomena for AL2219-T851.pdf:pdf},
issn = {03602133},
journal = {Met. Trans. A},
number = {1},
pages = {5--11},
title = {{Microcrack closure phenomena for AI 2219-T851}},
volume = {10},
year = {1979}
}
@article{Fallis2013,
abstract = {Predicting the binding mode of flexible polypeptides to proteins is an important task that falls outside the domain of applicability of most small molecule and protein−protein docking tools. Here, we test the small molecule flexible ligand docking program Glide on a set of 19 non-$\alpha$-helical peptides and systematically improve pose prediction accuracy by enhancing Glide sampling for flexible polypeptides. In addition, scoring of the poses was improved by post-processing with physics-based implicit solvent MM- GBSA calculations. Using the best RMSD among the top 10 scoring poses as a metric, the success rate (RMSD ≤ 2.0 {\AA} for the interface backbone atoms) increased from 21{\%} with default Glide SP settings to 58{\%} with the enhanced peptide sampling and scoring protocol in the case of redocking to the native protein structure. This approaches the accuracy of the recently developed Rosetta FlexPepDock method (63{\%} success for these 19 peptides) while being over 100 times faster. Cross-docking was performed for a subset of cases where an unbound receptor structure was available, and in that case, 40{\%} of peptides were docked successfully. We analyze the results and find that the optimized polypeptide protocol is most accurate for extended peptides of limited size and number of formal charges, defining a domain of applicability for this approach.},
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Fallis, A.G},
doi = {10.1017/CBO9781107415324.004},
eprint = {arXiv:1011.1669v3},
isbn = {9788578110796},
issn = {1098-6596},
journal = {J. Chem. Inf. Model.},
keywords = {icle},
number = {9},
pages = {1689--1699},
pmid = {25246403},
title = {{Grundlagen der Elektrotechnik}},
volume = {53},
year = {2013}
}
@article{Guennec2013a,
abstract = {Ultrasonic testing method has allowed some impressive improvements in order to better grasp fatigue properties of various metallic materials the latest 20 years. It is particularly the case in the very high cycle regime since ultrasonic fatigue tests are conducted at very high stressing frequencies. However, the question of a potential difference of fatigue strengths due to huge frequency gap between ultrasonic method (usually carried out at 20 kHz) and servo-hydraulic one (usually in the range of 1?100 Hz) is still unclear and needs to be studied for a various kind of metallic materials. The case of low carbon steels presents a singularity, as fatigue properties are significantly different between these two fatigue tests methods. It seems particularly interesting to study this kind of materials in order to get a better overview of frequency effect in metallic materials fatigue. Aim of the present work, which consists of a general survey of JIS S15C steel (0.15{\%} C) fatigue properties, is firstly to reconfirm such a frequency effect. Secondly, based on several experiments related to micro-plasticity behavior, some discussions will be held in order to explain this frequency effect in the case of low carbon steels.},
author = {Guennec, B. and Ueno, A. and Sakai, T. and Takanashi, M. and Itabashi, Y.},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Surface effects + Frequency effects/Frequency effects on high cycle fatigue of low carbon steel.PDF:PDF},
journal = {13th Int. Conf. Fract.},
keywords = {cyclic hardening,ebsd observations,frequency effect,low carbon steel,ultrasonic test},
pages = {1--10},
title = {{Effect of Loading Frequency in Fatigue Properties and Micro-Plasticity Behavior of JIS S15C Low Carbon Steel}},
year = {2013}
}
@article{Regelung,
author = {Regelung, Mechanische},
title = {{Regelung und Steuerung der Kraftstoffeinspritzsysteme}}
}
@article{Spurk2010,
author = {Spurk, Joseph H},
doi = {10.1007/978-3-642-13143-1},
isbn = {9783642131431},
journal = {Str{\"{o}}mungslehre Einf{\"{u}}hrung die Theor. der Str{\"{o}}mungen [7. Auflage]},
title = {{2-Grundgleichungen der Kontinuumsmechanik}},
year = {2010}
}
@article{Zienkiewicz2005f,
abstract = {Publisher Summary Some general families of finite elements can be obtained for C0 interpolations. A progressively increasing number of nodes, and hence improved accuracy characterizes each new member of the family and presumably the number of such elements required to obtain an adequate solution decreases rapidly. To ensure that a small number of elements can represent a relatively complex form of the type that is liable to occur in real, rather than academic, problems, simple rectangles, and triangles no longer suffice. This chapter is concerned with the subject of distorting such simple forms into others of more arbitrary shape. Elements of the basic one-, two-, or three-dimensional types are mapped into distorted forms. Not only can two-dimensional elements be distorted into others in two dimensions but the mapping of these can be taken into three dimensions also as indicated by the flat sheet elements distorting into a three-dimensional space. This principle applies generally, providing a one-to-one correspondence between Cartesian and curvilinear coordinates can be established. Once such coordinate relationships are known, shape functions can be specified in local coordinates and by suitable transformations the element properties established in the global coordinate system.},
author = {Zienkiewicz, O C and Taylor, R L and Zhu, J Z},
doi = {http://dx.doi.org/10.1016/B978-075066431-8.50173-9},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Zienkiewicz FEM - Vol 1 Basics Fundamentals/63205{\_}05.pdf:pdf},
isbn = {978-0-7506-6431-8},
journal = {Finite Elem. Method Set (Sixth Ed.},
pages = {138--186},
title = {{5 - Mapped elements and numerical integration — ‘infinite' and ‘singularity elements'}},
url = {http://www.sciencedirect.com/science/article/pii/B9780750664318501739},
year = {2005}
}
@article{Walgraef1985a,
abstract = {The nucleation of persistent slip bands (PSBs) in stressed metals may be interpreted as a cooperative phenomenon for dislocation populations. The competition between their mobility and nonlinear interaction (creation, annihilation, pinning) induces an instability of uniform dislocation distributions vs inhomogeneous ones and leads to the formation and persistence of spatial patterns. In particular, we have shown in preceding publications that the nucleation and coexistence of the layered structure of PSBs and the rodlike structure of the surrounding matrix can be described by a system of coupled partial differential equations of the reaction-diffusion type for immobile and mobile dislocations. Here we consider explicitly the motion and interaction of positive and negative mobile dislocations and derive an expression for their effective diffusivity. Moreover we show how these effects together with secondary slip activity may trigger the formation of walls in different directions in analogy with observations of labyrinth structures. ?? 1986.},
author = {Walgraef, Daniel and Aifantis, Elias C.},
doi = {10.1063/1.336183},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/1985{\_}WalgraefAndAifantis{\_}Dislocation patterning in fatigued metals as a result of dynamical instabilities.pdf:pdf},
issn = {00218979},
journal = {J. Appl. Phys.},
number = {2},
pages = {688--691},
title = {{Dislocation patterning in fatigued metals as a result of dynamical instabilities}},
volume = {58},
year = {1985}
}
@article{Proakis1996,
abstract = {The author and publisher of this book have used their best efforts in preparing this book. These efforts include the development, research, and testing of the theories and programs to determine their effectiveness. The author and publisher make no warranty of any kind, expressed or implied, with regard to these programs or the documentation contained in this book. The author and publisher shall not be liable in any event for incidental or consequential damages in connection with, or arising out of. the furnishing, performance, or use of these programs.},
author = {Proakis, John G and Monolakis, Dimitri G},
isbn = {0-13-394338-9},
journal = {Pentice Hall},
pages = {1--42},
title = {{Digital signal processing: principles, algorithms, and applications}},
year = {1996}
}
@article{Endo2007,
abstract = {A modified linear-elastic fracture mechanics approach has been proposed and developed by McEvily and co-workers, with which the fatigue crack growth rates of both small cracks and large cracks can be quantitatively evaluated. This paper reviews the recent results of applications of this approach to the following fatigue problems involving the prediction of the behavior of small fatigue cracks: (1) in an examination of the use of Miner's rule in fatigue life estimation under variable amplitude loading, (2) in the verification of the sqrt(a r e a) parameter model, and (3) in the prediction of the fatigue life and strength of defect-containing components subjected to multiaxial stress. ?? 2006 Elsevier B.V. All rights reserved.},
author = {Endo, M. and McEvily, A. J.},
doi = {10.1016/j.msea.2006.09.084},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/2007{\_}Endo+McEvily{\_}Prediction of the behavior of small fatigue cracks.pdf:pdf},
issn = {09215093},
journal = {Mater. Sci. Eng. A},
keywords = {Crack closure,Elastic-plastic behavior,Fatigue crack growth,Fatigue lifetime estimate,Fatigue thresholds,Multiaxial stress},
number = {SPEC. ISS.},
pages = {51--58},
title = {{Prediction of the behavior of small fatigue cracks}},
volume = {468-470},
year = {2007}
}
@article{Svoboda2008a,
abstract = {An extremal principle is formulated for thermodynamic systems near equi- librium subjected to various external conditions. It is shown that the principle describes un- ambiguously the kinetics of the thermodynamic system and replaces classical phenomeno- logical equations. Thus the principle can be considered as an effective tool for the treatment of non-equilibrium thermodynamic systems. In two examples the principle is used for the description of Dufour and Soret effects and plasticity. 1.},
author = {Svoboda, Jiř{\'{i}} and Fischer, Franz Dieter and Vala, Jiř{\'{i}}},
doi = {10.1478/C1S0801022},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Thermodynamik/2008{\_}Svoboda+Fischer{\_}Thermodynamic extremal principle and its application to Dufour and Soret effects and Plasticity.pdf:pdf},
issn = {03650359},
journal = {AAPP Atti della Accad. Peloritana dei Pericolanti, Cl. di Sci. Fis. Mat. e Nat.},
number = {SUPPL.1},
pages = {1--11},
title = {{Thermodynamic extremal principle and its application to dufour and soret effects and plasticity}},
volume = {86},
year = {2008}
}
@article{Burgd,
author = {Burg, Heinz and Moser, Andreas and Steffan, Hermann},
journal = {Messtechnik},
pages = {59--71},
title = {{A3 A3 Messtechnik A3}}
}
@article{Kress2004,
author = {Kress, Gerald},
journal = {Cent. Struct. Technol. ETHZ},
pages = {1--124},
title = {{Strukturanalyse mit FEM}},
url = {http://www.structures.ethz.ch/education/master/analysis/Skript/FEM{\_}D{\_}Main{\_}2009.pdf},
year = {2004}
}
@article{Habib2004,
author = {Habib, M A and Attya, A M and Said, S A M and Eid, A I and Aly, A Z},
doi = {10.1007/s00231-003-0456-6},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Thermal Coating + Water Heat Transfer + Applikation/2004{\_}Habib+Attya{\_}Heat transfer characteristics and Nusselt number correlation of turbulent pulsating pipe air flows.pdf:pdf},
journal = {Heat Mass Transf.},
pages = {307--318},
title = {{Heat transfer characteristics and Nusselt number correlation of turbulent pulsating pipe air flows}},
volume = {40},
year = {2004}
}
@article{St,
author = {St, Die and Modelle, Die and Sa, Sichtbegrenzung},
pages = {7--9},
title = {{5 Richtlinien und Vorschriften}}
}
@article{Hill1966,
abstract = {A general, type of cross-coupling between glide and hardening on different slip-systems is proposed. Its implications in regard to the character of the connexion between the overall stress-rate and strain-rate in multislip are investigated. Uniqueness theorems and extremal properties are established in respect both of the overall constitutive law itself and any boundary-value problem for non-uniform deformation of a single crystal or aggregate.},
author = {Hill, R},
doi = {10.1016/0022-5096(66)90040-8},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/1966{\_}Hill{\_}Generalized consititutive relations for incremental defo of metal crystals by multislip.pdf:pdf},
isbn = {0022-5096},
issn = {00225096},
journal = {J. Mech. Phys. Solids},
number = {2},
pages = {95--102},
title = {{Generalized constitutive relations for incremental deformation of metal crystals by multislip}},
volume = {14},
year = {1966}
}
@article{Zahlen,
author = {Zahlen, Reynoldsschen and Zahlen, Reynoldsschen and Uberschrei-, Beim and Uberschrei-, Beim and Teilchenbahnen, Die and Teilchenbahnen, Die and Faden, Der and Faden, Der and Merkmale, Andere and Merkmale, Andere and Umschlag, Der and Umschlag, Der and Gleichungen, Navier-stokesschen and Gleichungen, Navier-stokesschen},
title = {{7 Grundz u ¨ ge turbulenter Str o ¨ mungen 7.1}}
}
@article{Bozek2008,
abstract = {Microstructurally small fatigue crack (MSFC) formation includes stages of incubation, nucleation and microstructurally small propagation. In AA 7075-T651, the fracture of Al 7 Cu 2 Fe constituent particles is the major incubation source. In experiments, it has been observed that only a small percentage of these Fe-bearing particles crack in a highly stressed volume. The work presented here addresses the identification of the particles prone to cracking and the prediction of particle cracking frequency, given a distribution of particles and crystallographic texture in such a volume. Three-dimensional elasto-viscoplastic finite element analyses are performed to develop a response surface for the tensile stress in the particle as a function of the strain level surrounding the particle, parent grain orientation and particle aspect ratio. A technique for estimating particle strength from fracture toughness, particle size and intrinsic flaw size is developed. Particle cracking is then determined by comparing particle stress and strength. The frequency of particle cracking is then predicted from sampling measured distributions of grain orientation, particle aspect ratio and size. Good agreement is found between the predicted frequency of particle cracking and two preliminary validation experiments. An estimate of particle cracking frequency is important for simulating the next stages of MSFC formation: inserting all particles into a microstructural model for these stages is computationally intractable and physically unnecessary.},
author = {Bozek, J E and Hochhalter, J D and Veilleux, M G and Liu, M and Heber, G and Sintay, S D and Rollett, A D and Littlewood, D J and Maniatty, A M and Weiland, H and Christ, R J and Payne, J and Welsh, G and Harlow, D G and Wawrzynek, P A and Ingraffea, A R},
doi = {10.1088/0965-0393/16/6/065007},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/2008{\_}Hochhalter{\_}AL7075AgeometricapproachI{\_}ParticeleCracking.pdf:pdf},
isbn = {09650393 (ISSN)},
issn = {0965-0393},
journal = {Model. Simul. Mater. Sci. Eng.},
number = {6},
pages = {065007},
title = {{A geometric approach to modeling microstructurally small fatigue crack formation: I. Probabilistic simulation of constituent particle cracking in AA 7075-T651}},
url = {http://stacks.iop.org/0965-0393/16/i=6/a=065007?key=crossref.c2c7fddb48a7b52013977b4d25c503c4},
volume = {16},
year = {2008}
}
@article{Buque2001a,
abstract = {The influence of the plastic strain amplitude (??pa) and the crystallographic grain orientation on the occurrence of the ladder-like dislocation substructure characteristic of persistent slip bands (PSBs) was studied by scanning electron microscopy (SEM) on individual grains of cycled nickel polycrystals. The ladder substructures were found to occur in the range of plastic strain amplitudes of 1??10-4?????pa???1??10-3 on grains having considerable different axial orientations. Studies of the slip activity show that all ladder dislocation patterns are correlated with the well-known PSBs. Apart from projection effects, the ladder-like dislocation configuration of PSBs remains unchanged for all grain orientations. The effect of crystallographic orientation concerns only the matrix surrounding the PSBs which is determined by the axial grain orientation. An increase of ??pa results in a reduction of the mean PSB wall spacing and in higher effective PSB volume fractions. The mean shear plastic strain amplitude of primary PSBs in polycrystals is estimated to be about 2??10-3. ?? 2001 Elsevier Science Ltd.},
author = {Buque, C},
doi = {10.1016/S0142-1123(01)00013-5},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2001{\_}Buque{\_}Persistent slip bands in cyclically deformed nickel polycrystals.pdf:pdf},
issn = {01421123},
journal = {Int. J. Fatigue},
keywords = {Dislocation structure,Grain orientation,Low cycle fatigue,Nickel polycrystals,Persistent slip bands},
number = {6},
pages = {459--466},
title = {{Persistent slip bands in cyclically deformed nickel polycrystals}},
volume = {23},
year = {2001}
}
@article{Gemische2009,
author = {Gemische, Allgemeinen and Komponenten, Diese and Grenzwerte, Die and Dieselkraftstoff, En-normen and Ottokraftstoff, Fame and Biodiesel, Ethanol and Folgenden, Im},
pages = {115--166},
title = {{Motorische Verbrennung}},
year = {2009}
}
@article{Pahl2007c,
author = {Pahl, Gerhard and Beitz, Wolfgang},
journal = {Konstruktionslehre},
title = {{14 Begriffs{\{}{\"{u}}{\}}bersicht}},
year = {2007}
}
@article{Fem,
author = {Fem, Engineering},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/{\_}buecherSong/ComputationalMechanicsofCompositeMaterials/05{\_}FractureandFatigueModelsforComposites.pdf:pdf},
title = {{{\textless}Fracture and Fatigue Models for Composites.pdf{\textgreater}}}
}
@article{Wishington2012a,
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Wishington, D C},
doi = {10.1002/ejoc.201200111},
eprint = {arXiv:1011.1669v3},
isbn = {3082342418},
issn = {0196-6553},
journal = {Bioinforma. Biomed. Eng. 2008. ICBBE 2008. 2nd Int. Conf.},
pages = {7--58},
pmid = {26840611},
title = {{Table of of contents}},
year = {2012}
}
@article{Foresta,
author = {Forest, Samuel},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/Folien CISM Summer School Mai2017 - Mesoscale Models/courses{\_}C1703{\_}forest{\_}Forest4-Homog.pdf:pdf},
title = {{Generalized continuum modelling of heterogeneous materials From a heterogeneous Cauchy continuum to an homogeneous equivalent micromorphic continuum}}
}
@article{Forster2013,
author = {Forster, Caroline},
doi = {10.1007/978-3-642-24303-5},
isbn = {9783642243035},
pages = {1--8},
title = {{Kapitel 16:}},
year = {2013}
}
@article{Patel2016,
author = {Patel, Juber T and Attal, Manish H},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Thermal Coating + Water Heat Transfer + Applikation/2016{\_}Patel+Attal{\_}An Experimental Investigation of Heat Transfer Characteristics of Pulsating Flow in Pipe.pdf:pdf},
journal = {Int. J. Curr. Eng. Technol.},
keywords = {heat transfer enhancement,pulsating flow,pulsator,turbulent flow},
number = {5},
pages = {1515--1521},
title = {{An Experimental Investigation of Heat Transfer Characteristics of Pulsating Flow in Pipe}},
volume = {6},
year = {2016}
}
@article{Pahl2007b,
author = {Pahl, Gerhard and Beitz, Wolfgang and Feldhusen, J{\"{o}}rg and Grote, Karl-Heinrich},
journal = {Konstr. Grundlagen erfolgreicher Produktentwicklung, Methoden und Anwendung},
pages = {39--92},
title = {{Grundlagen}},
year = {2007}
}
@article{Reifendruck,
author = {Reifendruck, Der},
journal = {System},
number = {Xl},
pages = {1--7},
title = {{10 Reifendruck}}
}
@article{Sauzay2002a,
author = {Sauzay, M and Gilormini, P},
doi = {10.1016/S0167-8442(02)00080-0},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/2002{\_}Sauzay + Gilmormini{\_}Influence of surface effects on fatigue of microcracks nucleation.pdf:pdf},
issn = {01678442},
journal = {Evaluation},
keywords = {crack nucleation,cyclic plasticity,fatigue,persistent slip band,surface},
pages = {53--62},
title = {{Influence of surface effects on fatigue of microcracks nucleation}},
volume = {38},
year = {2002}
}
@article{Chemie1806a,
author = {Chemie, Organische},
pages = {1--3},
title = {{1 Einf{\"{u}}hrung}},
year = {1806}
}
@article{Svendsen1999,
author = {Svendsen, B},
doi = {10.1007/s001610050114},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Thermodynamik/Liu-Entropieprinzip{\_}Lukas{\_}Fraunhofer/Liu-Entropieprinzip/Svendsen{\_}thermoelasticity{\_}with{\_}additional{\_}DOF{\_}1999.pdf:pdf},
issn = {0935-1175},
journal = {Contin. Mech. Therm.},
pages = {247--262},
title = {{On the thermodynamics of thermoelastic materials with additional scalar degrees of freedom}},
volume = {4},
year = {1999}
}
@article{Quarteroni2004,
author = {Quarteroni, Alfio and Saleri, Fausto},
doi = {10.1007/3-540-29307-8},
isbn = {9783540250050},
journal = {New York},
keywords = {MatLab},
pages = {272},
title = {{Wissenschaftliches Rechnen mit MATLAB}},
year = {2004}
}
@article{Tress2003,
author = {Tress, C Auchy S},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Nicholson 2003 - Finite Element Analysis Thermomechanics of Solids/0749{\_}C05.pdf:pdf},
pages = {73--93},
title = {{Mechanical Equilibrium and the Principle of Virtual Work 5.1}},
year = {2003}
}
@article{Lin1989a,
author = {Lin, T. H. and Lin, S. R. and Wu, X. Q.},
doi = {10.1080/01418618908221174},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/1989{\_}Lin{\_}Micromechanics of an extrusion in high-cycle fatigue.pdf:pdf},
issn = {0141-8610},
journal = {Philos. Mag. A},
number = {6},
pages = {1263--1276},
title = {{Micromechanics of an extrusion in high-cycle fatigue}},
url = {http://www.tandfonline.com/doi/abs/10.1080/01418618908221174},
volume = {59},
year = {1989}
}
@article{Results1994,
abstract = {As a concluding comment, I should like to return to the point raised by Ayres, that it is not enough simply to tell a better version of the fourth-century history in the expectation that modern theologians will finally get it straight! This is a valid point: if we want to have Christianity's fourth-century heritage taken seriously, we need to be in dialogue with modern writers. But, if there is to be a dialogue, both sides must be allowed to speak, and so we are also responsible for expounding the historical material on its own terms. As Heidegger put it, “[O]nly when we think through what has been thought will we be of any use for what must still be thought.” Perhaps studying the figures from a distant era will open up for us possibilities we would never have dreamed of within our own modern presuppositions, so that we can recognize differences even beyond those which lie within our own horizon or tradition. If I am right in affirming that there is a different style of doing theology prior to Augustine and after him in the East than that which we find in the theological and scholarly tradition in which Ayres's book stands, then we must ask whether we need to address the question of the legitimacy of each (and ponder how one might even answer that) or whether a plurality of approaches is possible without reducing one to the other. In a way, this would be a further step toward deconstructing monolithic notions of “Orthodoxy” in recognition of genuine and legitimate diversity within early Christianity and among modern Christians. Might it be better not to speak of Nicaea and its legacy, but of the legacies of Nicaea—or better—“Christ and him crucified” (2 Cor 2:2) and the ways in which Nicaea and its interpreters affirm the true divinity of this one?},
author = {Results, Useful},
doi = {10.1007/BF02600226},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2010{\_}Jaroslav Pokluda+Pavel {\v{S}}andera{\_}Micromechanisms of fracture and fatigue{\_}Buch/Kap5{\_}FinalReflection.pdf:pdf},
isbn = {9780470434673},
issn = {08848734},
journal = {J. Gen. Intern. Med.},
number = {3 Supplement},
pages = {243--247},
title = {{Final reflections}},
volume = {9},
year = {1994}
}
@article{Lankford1973,
abstract = {Electron microscopy of surface replicas has been employed to determine the metallurgical micromechanics of fatigue crack initiation at surface and shallow subsurface inclusions in 4340 steel. The experimental results are considered in terms of current theoretical anal- yses of elastic stress distributions around hard inclusions imbedded in soft matrices. A model for crack nucleation at surface inclusions is suggested, based upon debonding of the inclusion/matrix interface at the tensile pole of the inclusion, followed by growth of the debond seam toward the inclusion "equator". Subsequent generation of a matrix crack is associated with the initiation of "point" surface defects some distance from the inclusion/ma- trix boundary, but in the plane of the inclusion "equator". Surface slip plays no discernible role in nucleation of surface inclusions, but slip bands are formed at crack sites above sub- surface inclusions. However, the microcracks continue to form through the link-up of point surface defects.},
author = {Lankford, James and Kusenberger, F N},
doi = {10.1007/BF02648709},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/1973{\_}Lankford{\_}Initiation of fatigue cracks in 4340 steel.pdf:pdf},
issn = {0360-2133},
journal = {Met. Trans.},
number = {February},
pages = {553--559},
title = {{Initiation of fatigue cracks in 4340 steel}},
volume = {4},
year = {1973}
}
@article{Entwicklung,
author = {Entwicklung, Geschichtliche},
pages = {534--537},
title = {{Index}}
}
@book{Milton2002,
abstract = {Some of the greatest scientists including Poisson, Faraday, Maxwell, Rayleigh, and Einstein have contributed to the theory of composite materials. Mathematically, it is the study of partial differential equations with rapid oscillations in their coefficients. Although extensively studied for more than a hundred years, an explosion of ideas in the last four decades (and particularly in the last two decades) has dramatically increased our understanding of the relationship between the properties of the constituent materials, the underlying microstructure of a composite, and the overall effective (electrical, thermal, elastic) moduli which govern the macroscopic behavior. This book surveys these exciting developments at the frontier of mathematics and presents many new results.},
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Milton, Graeme W.},
doi = {10.1017/CBO9780511613357},
eprint = {arXiv:1011.1669v3},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/Strukturmechanik MMS/Literatur/Mikromechanik{\_}B{\"{u}}cher{\_}Literaturvorschlag{\_}MMS/Milton 2004 Composites.pdf:pdf},
isbn = {9780511613357},
issn = {1098-6596},
pmid = {12215489},
title = {{The Theory of Composites}},
url = {http://ebooks.cambridge.org/ref/id/CBO9780511613357},
year = {2002}
}
@article{Grandin2000a,
abstract = {It is generally accepted that knocking combustion influences the heat transfer in SI engines. However, the effects of heat transfer on the onset of knock is still not clear due to lack of experimental data of the thermal boundary layer close to the combustion chamber wall. This paper presents measurements of the temperature in the thermal boundary layer under knocking and non-knocking conditions. The temperature was measured using dual-broadband rotational Coherent anti-Stokes Raman Spectroscopy (CARS). Simultaneous time-resolved measurements of the cylinder pressure, at three different locations, and the heat flux to the wall were carried out. Optical access to the region near the combustion chamber wall was achieved by using a horseshoe-shaped combustion chamber with windows installed in the rectangular part of the chamber. This arrangement made CARS temperature measurements close to the wall possible and results are presented in the range 0.1-5 mm from the wall. The engine was run with constant fuel flow under near stoichiometric conditions. Knocking and non-knocking conditions were achieved by using different mixtures of n-heptane and iso-octane.},
author = {Grandin, B{\"{o}}rje and Denbratt, Ingemar and Bood, Joakim and Brackmann, Christian and Bengtsson, Per-Erik},
doi = {10.4271/2000-01-2831},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2000{\_}Grandin{\_}The Effect of Knock on the Heat Transfer in an SI Engine.pdf:pdf},
journal = {SAE Tech. Pap.},
number = {2000-01-2831},
title = {{The Effect of Knock on the Heat Transfer in an SI Engine: Thermal Boundary Layer Investigation using CARS Temperature Measurements and Heat Flux Measurements}},
url = {http://dx.doi.org/10.4271/2000-01-2831},
year = {2000}
}
@article{Gutbrod1954,
author = {Gutbrod, Firmen and Zweitaktmotoren, Bosch and Superior, Gutbrod and Fahr-, Beide},
journal = {Transport},
title = {{14 Motorkonzepte}},
year = {1954}
}
@article{Verbindungen2007,
author = {Verbindungen, Wechselnde},
journal = {Fahrzeuggetriebe},
title = {{9 Schalteinrichtungen}},
year = {2007}
}
@article{Tragwerke,
author = {Tragwerke, Statik},
doi = {10.1007/978-3-642-16828-4},
isbn = {9783642168284},
title = {3}
}
@article{Chaboche2003a,
abstract = {Constitutive and damage mechanics equations of composite materials are developed and discussed in the framework of micromechanics based approaches, including some recent modeling capabilities. The approach is based on the Transformation Field Analysis (TFA) promoted by Dvorak. A correction method is proposed in order to obtain a softer overall hardening response in case of the model restriction to only two subdomains (the elastic fibre, and the elasto-plastic matrix). In order to take into account the effects of temperature and damage on the elastic properties, a Generalised Eigenstrain Method (GEM) is developed, that uses the corresponding additional strains as eigenstrains. Its validity is checked by means of finite element numerical simulations based on periodic homogenisation. The methodology is further developed for metal matrix composites in which the matrix is treated as a polycristalline aggregate and slip plasticity is written at the level of slip systems. Two imbricated scale transitions are performed, both based on TFA like rules and it is shown how the overall constitutive equations can be considered as a multi-mechanism flow rule with pseudo-slip systems. Application of the model is made for a SiC/Ti composite. The capabilities are discussed by comparison with some experimental results, including monotonic and cyclic transverse loading conditions.},
author = {Chaboche, J L and Carr??re, N},
doi = {10.1007/978-3-540-36418-4_2},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Anisotropic Behaviouir of Damaged Materials{\_}Skrzypek{\_}ARTICEL/Kap2{\_}Multiscale Structural Analyses Incorporating Damage Mechanics at the Meso- or Micro-Scales.pdf:pdf},
isbn = {9783642055874},
issn = {16137736},
journal = {Lect. Notes Appl. Comput. Mech.},
keywords = {Viscoplasticity,damage mechanics,metal matrix composites,micromechanics,scale transitions},
pages = {35--74},
title = {{Multiscale Structural Analyses Incorporating Damage Mechanics at the Meso- or Micro-Scales}},
volume = {9},
year = {2003}
}
@article{Herman1968,
author = {Herman, H. and Herman, H. and Mura, T. and Mura, T.},
journal = {Il, Moscow},
pages = {1--108},
title = {{Continuum theory of dislocations}},
url = {https://scholar.google.co.uk/scholar?start=300{\&}q=translation+theory{\&}hl=en{\&}as{\_}sdt=0,5{\#}13},
volume = {3},
year = {1968}
}
@article{Wallentowitz2006j,
author = {Wallentowitz, Henning and Reif, Konrad},
doi = {10.1007/978-3-8348-9121-1_5},
journal = {Handb. Kraftfahrzeugelektronik - Grundlagen, Kompon. Syst. Anwendungen},
title = {{Beleuchtung}},
url = {http://www.springerlink.com/index/10.1007/978-3-8348-9121-1{\_}5},
year = {2006}
}
@article{Anwendung,
author = {Anwendung, Die and Hauptsache, Der},
journal = {Arbeit},
pages = {177--183},
title = {{15 Energie- und Arbeitsprinzip}}
}
@book{Murakami2012i,
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Murakami, Sumio},
doi = {10.1007/978-94-007-2666-6},
eprint = {arXiv:1011.1669v3},
isbn = {978-94-007-2665-9},
issn = {09250042},
pages = {217--251},
pmid = {25246403},
title = {{Continuum Damage Mechanics}},
url = {http://link.springer.com/10.1007/978-94-007-2666-6},
volume = {185},
year = {2012}
}
@article{Murakami2012h,
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Murakami, Sumio},
doi = {10.1007/978-94-007-2666-6},
eprint = {arXiv:1011.1669v3},
isbn = {978-94-007-2665-9},
issn = {09250042},
pages = {3--13},
pmid = {25246403},
title = {{Continuum Damage Mechanics}},
url = {http://link.springer.com/10.1007/978-94-007-2666-6},
volume = {185},
year = {2012}
}
@article{Kochmann2009,
author = {Kochmann, D M and Hackl, Klaus. and Le, K C},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/2009{\_}Le{\_}A continuum dislocation theory for modeling dislocation microstructures in crystal plasticity.pdf:pdf},
journal = {Conf. Pap.},
keywords = {abstract,and pile up near,anisms related to the,continuum mechanics,dislocation,dislocation network,high degree on the,in order to accommodate,material moderling,mech-,microstructure,new dislocations are nucleated,plastic deformation and,plastic deformation of crystalline,plasticity,s energy,solids depends to a,the grain or,to reduce the crystal},
number = {September},
pages = {7--11},
title = {{a Continuum-Dislocation Theory for Modeling Dislocation Microstructures and Size Effects in Crystal Plastiticy}},
year = {2009}
}
@article{Pahl2007f,
author = {Pahl, Gerhard and Beitz†, Wolfgang and Feldhusen, J{\"{o}}rg and Grote, Karl-H.},
journal = {Pahl/Beitz Konstr. - Grundlagen},
title = {{Inhaltsverzeichnis}},
year = {2007}
}
@article{Forestc,
author = {Forest, Samuel},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/Folien CISM Summer School Mai2017 - Mesoscale Models/courses{\_}C1703{\_}forest{\_}Forest1-Micromorphic.pdf:pdf},
title = {{Micromorphic media}}
}
@article{Klassifizierung,
author = {Klassifizierung, Die and Unterschied, Wesentlichster and Wesentlichen, Im},
pages = {14--29},
title = {{3 Charakterisierung von Messsignalen}}
}
@article{Steigerungen,
author = {Steigerungen, Weitere and Jahr, Jedes and Erkennt, Die and Ausweitung, Eine},
pages = {415--422},
title = {{Zukunftsentwicklungen 14 Trends und zuk{\{}{\"{u}}{\}}nftige Anforder ungen im Motor radbau}}
}
@article{Stupkiewicz2007c,
author = {Stupkiewicz, Stanis{\l}aw},
doi = {10.1007/978-3-540-49717-2_8},
isbn = {3540497161},
issn = {16137736},
journal = {Lect. Notes Appl. Comput. Mech.},
number = {30},
pages = {115--149},
title = {{Evolving laminates in shape memory alloys}},
volume = {2006},
year = {2007}
}
@article{Evert2006a,
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Evert, Ray F},
doi = {10.1002/0470047380.indauth},
eprint = {arXiv:1011.1669v3},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Zienkiewicz FEM - Vol 3 Fluid Dynamics/63229{\_}aindx.pdf:pdf},
isbn = {9780470047385},
issn = {15672719},
journal = {Esau's Plant Anat.},
pages = {541--566},
pmid = {20348824},
title = {{Author Index}},
url = {http://dx.doi.org/10.1002/0470047380.indauth},
year = {2006}
}
@article{Remarks,
author = {Remarks, Introductory},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/{\_}buecherSong/ComputationalMechanicsofCompositeMaterials/06{\_}ReliabilityAnalysis.pdf:pdf},
title = {{6 Reliability Analysis}}
}
@article{Vielfalt,
author = {Vielfalt, Diese},
title = {{und Impedanzen}}
}
@article{Caton1981b,
abstract = {Because of the increasing need for precise information on engine processes, this study developed and experimentally verified models for the instantaneous heat transfer in an engine exhaust port. Experimental measurements were made of the instantaneous cylinder pressure and instantaneous exhaust gas temperature for a range of engine operating conditions. The pressure measurements were used to obtain the instantaneous cylinder gas state and the temperature measurements were used to validate the heat transfer models. The exhaust port heat transfer was dominated by jet induced large-scale fluid motion as opposed to wallshear generated fluid motion. An analysis based on the jet velocity through the valve opening correctly estimated the heat transfer due to this large-scale motion. Models for the instantaneous exhaust port heat transfer provided excellent agreement with measurements as a function of engine operating conditions. A cause d'un besoin croissant d'information pr{\{}{\'{e}}{\}}cise sur le fonctionnement d'un moteur, on d{\{}{\'{e}}{\}}veloppe une {\{}{\'{e}}{\}}tude et on v{\{}{\'{e}}{\}}rifie exp{\{}{\'{e}}{\}}rimentalement des mod{\{}{\`{e}}{\}}les sur le transfert de chaleur instantan{\{}{\'{e}}{\}} {\{}{\`{a}}{\}} l'{\{}{\'{e}}{\}}chappement d'un cylindre. Des mesures de la pression instantan{\{}{\'{e}}{\}}e dans le cylindre et de la temp{\{}{\'{e}}{\}}rature instantan{\{}{\'{e}}{\}}e {\{}{\`{a}}{\}} l'{\{}{\'{e}}{\}}chappement sont effectu{\{}{\'{e}}{\}}es pour un domaine de conditions de fonctionnement d'un moteur. Les mesures de pression permettent d'atteindre l'{\{}{\'{e}}{\}}tat instantan{\{}{\'{e}}{\}} du gaz dans le cylindre et les mesures de temp{\{}{\'{e}}{\}}rature permettent de valider les mod{\{}{\`{e}}{\}}les de transfert thermique. Le transfert {\{}{\`{a}}{\}} l'{\{}{\'{e}}{\}}chappement est domin{\{}{\'{e}}{\}} par un mouvement de jet {\{}{\`{a}}{\}} large {\{}{\'{e}}{\}}chelle au contraire du mouvement de fluide {\{}{\`{a}}{\}} frottement pari{\{}{\'{e}}{\}}tal. Une analyse bas{\{}{\'{e}}{\}}e sur la vitesse du jet {\{}{\`{a}}{\}} travers l'ouverture de la soupape pr{\{}{\'{e}}{\}}dit correctement le transfert de chaleur d{\{}{\^{u}}{\}} {\{}{\`{a}}{\}} ce mouvement {\{}{\`{a}}{\}} grande {\{}{\'{e}}{\}}chelle. Des mod{\{}{\`{e}}{\}}les pour l'{\{}{\'{e}}{\}}chappement instantan{\{}{\'{e}}{\}} fournissent un accord excellent avec des mesures pour les conditions de fonctionnement du moteur. Wegen des zunehmenden Bedarfs an genauer Information {\{}{\"{u}}{\}}ber Verbrennungsmotoren-Prozesse wurden in dieser Studie Modelle f{\{}{\"{u}}{\}}r den momentanen W{\{}{\"{a}}{\}}rme{\{}{\"{u}}{\}}bergang in einer Motor-Ausla{\$}\beta{\$}-{\{}{\"{O}}{\}}ffnung entwickelt und experimentell best{\{}{\"{a}}{\}}tigt. Die Momentanwerte des Zylinderdrucks und der Abgastemperatur wurden in Versuchen f{\{}{\"{u}}{\}}r einen ausgedehnten Betriebsbereich gemessen. Druckmessungen wurden verwendet, um den momentanen Gaszustand im Zylinder zu bestimmenn und Temperaturmessungen dienten zur Best{\{}{\"{a}}{\}}tigung der W{\{}{\"{a}}{\}}rme{\{}{\"{u}}{\}}bergangs-Modelle. Der W{\{}{\"{a}}{\}}rme{\{}{\"{u}}{\}}bergang in der Ausla{\$}\beta{\$}-{\{}{\"{O}}{\}}ffnung wurde im wesentlichen durch die strahlinduzierte Makro-Bewegung des Fluides entgegen der durch Wandschubspannung erzeugten Fluidbewegung bestimmt. Eine theoretische Untersuchung, die sich auf die Strahlgeschwindigkeit durch die Ventil{\{}{\"{o}}{\}}ffnung st{\{}{\"{u}}{\}}tzt, liefert korrekt den W{\{}{\"{a}}{\}}rme{\{}{\"{u}}{\}}bergang, hervorgerufen durch diese Makro-Bewegung. Die Modelle f{\{}{\"{u}}{\}}r den momentanen W{\{}{\"{a}}{\}}rme{\{}{\"{u}}{\}}bergang in der Ausla{\$}\beta{\$}-{\{}{\"{O}}{\}}ffnung als Funktion der Arbeitsbedingungen des Motors zeigten vorz{\{}{\"{u}}{\}}gliche {\{}{\"{U}}{\}}bereinstimmung mit den Messungen. B cвязи c вce бoлee вoзpacтaющeй нeoбчoдимocтью в тoчнoй инфopмaции o пpoцeccaч, пpoиcчoдящич в двигaтeляч, пpeдлoзeны мoдeди тeплoпepeнoca в вычлoпнoм oтвepcтии двигaтeля. Измepялиcь дaвлeниe в цилиндpe и тeмпepaтypa вычлoпнoгo гaзa пpи paздичныч peзимaч paбoты двигaтeля. Дaнныe пo дaвлeнию иcпoльзoвaлиcь для oпpeдeлeния cocтoяния гaзa в цилиндpe, a пo тeмпepaтype — для пpoвepки cпpaвeдливocти пpeдлoзeнныч мoдeлeй. Teплoпepeнoc в вычлoпнoм oтвepcтии oпpeдeляeтcя кpyпнoмacштaбными пepeмeщeниями зидкocти, вoзникaющими пpи cтpyйнoм иcтeчeнии, кoтopыe cyщecтвeннo oтличaютcя oт пepeмeщeний, вызывaeмыч нaпpязeниeм cдвигa нa cтeнкe. Aнaлиз, ocнoвaный нa cкopocти иcтeчeния cтpyи чepeз oтвepcтиe клaпaнa, пoзвoляeт кoppeктнo oцeнить вeличинy тeплoвoгo пoтoкa пpи тaкич кpyпнoмacщтaбпыч пepeмeщeнияч. Moдeли тeплoпepeнoca в вычлoпнoм oтвepcтии чopoшo coглacyютcя c peзyльтaтaми измepeний пpи paзличныч peзимaч paбoты двигaтeдя.},
author = {Caton, J A and Heywood, J B},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/1981{\_}An experimental and analytical study of heat transfer in an engine exhaust port{\_}Caton.pdf:pdf},
journal = {Int. J. Heat Mass Transf.},
number = {4},
pages = {581--595},
title = {{An experimental and analytical study of heat transfer in an engine exhaust port}},
volume = {24},
year = {1981}
}
@article{Hansen1998,
abstract = {The relation between polycrystal deformation and single crystal deformation has been studied in this work. A pure aluminium polycrystal having an average grain size of 300 [mu]m has been strained in tension at room temperature. The flow stress has been determined at four different strains (0.05, 0.14, 0.22 and 0.34) and deformation microstructures have been characterized qualitatively and quantitatively by transmission electron microscopy. Improved experimental techniques have allowed large foil areas to be characterized and in total 89 grains have been examined. At the four strains examined a classification of the deformation microstructures into three different types has shown a correlation between the grain orientation and the type of deformation microstructure which develops during straining. The dislocation density has been calculated at each strain and by assuming that the shear stress is proportional to the square root of the dislocation density the shear stress-strain relationship has been derived for each of the three groups of grains showing different deformation microstructures. The stress-strain curves show a strain hardening behaviour which depends on the orientation of the grain. The behaviour of the grains embedded in the polycrystal is compared with the behaviour of single crystals and the stress-strain curve of the polycrystal is estimated with good accuracy from single crystal data, which are weighted based on a quantitative texture analysis of the polycrystal.},
author = {Hansen, N and Huang, X},
doi = {10.1016/S1359-6454(97)00365-0},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/1998{\_}Hansen{\_}Huang MICROSTRUCTURE AND FLOW STRESS OF.pdf:pdf},
isbn = {1359-6454},
issn = {13596454},
journal = {Acta Mater.},
number = {5},
pages = {1827--1836},
title = {{Microstructure and flow stress of polycrystals and single crystals}},
url = {http://linkinghub.elsevier.com/retrieve/pii/S1359645497003650},
volume = {46},
year = {1998}
}
@article{Santner1976,
author = {Santner, J. S. and Fine, M. E.},
doi = {10.1007/BF02643972},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/1976{\_}Morris+Buck{\_}Fatigue crack propagation in AL-base copper alloys.pdf:pdf},
issn = {03602133},
journal = {Metall. Trans. A},
number = {3},
pages = {583--593},
title = {{Fatigue crack propagation in aluminum-base copper alloys}},
volume = {7},
year = {1976}
}
@article{Journal2008a,
author = {Journal, American and Sciences, Applied and Publications, Science},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Heat transfer intake+exhaust system/2008{\_}Semin+Ismail{\_}Heat Transfer Investigation of Intake Port Engine Based on Steady-State and Transient Simulation.pdf:pdf},
keywords = {compression ignition engine,computational model,heat transfer,intake port,simulation},
number = {11},
pages = {1572--1579},
title = {{Heat Transfer Investigation of Intake Port Engine Based on Steady-State and Transient Simulation Semin , 2 Abdul Rahim Ismail , 2 Rosli Abu Bakar and 2 Ismail Ali Institute of Technology Sepuluh Nopember , Surabaya 60111 , Indonesia Faculty of Mechanical }},
volume = {5},
year = {2008}
}
@article{Produkte2003,
author = {Produkte, Prozesse and Kfz-branche, Besonderheiten Der},
pages = {199--244},
title = {{7 Projekte, Prozesse und Produkte 7.1}},
year = {2003}
}
@article{Zahoransky2013,
author = {Zahoransky, Richard A. and Allelein, Hans-Josef and Schelling, Udo and Schwarz, Harald and Bollin, Elmar and Oehler, Helmut},
doi = {10.1007/978-3-8348-2279-6},
isbn = {978-3-8348-1869-0},
journal = {Energietechnik - Syst. zur Energieumwandlung},
pages = {23},
title = {{10 Kraft-W{\"{a}}rmekopplung und Blockheiz-Kraftwerke}},
url = {http://www.springerlink.com/index/10.1007/978-3-8348-2279-6},
year = {2013}
}
@article{Luthi2013,
abstract = {Professor Robert M. Koerner (Bob) has successfully and elegantly transitioned his research programs throughout his career. Each successive program has brought new collaborators, contacts and consumers of his developments. Past research efforts may remain unknown to those who only more recently began an association with Bob. It is interesting and insightful to develop and follow the some times convoluted path that has led to the current, well-recognized Geosynthetics Institute. In this paper, I will provide insight into what may be the missing link between Bob's research in acoustic emissions and his current program in geosythethics.},
author = {L{\"{u}}thi, Thomas},
title = {{Non-Destructive Evaluation Methods}},
year = {2013}
}
@article{Dietmann1973a,
author = {Dietmann, H},
doi = {10.1002/mawe.19730040608},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Empirical Fatigue Models + Validation/1973{\_}Dietmann Materialwissenschaft{\_}und{\_}Werkstofftechnik{\_}ExperimentelleUntersuchungenZuFatigue.pdf:pdf},
issn = {15214052},
journal = {Materwiss. Werksttech.},
number = {6},
pages = {322--333},
title = {{Werkstoffverhalten unter mehrachsiger schwingender Beanspruchung. Teil 2: Experimentelle Untersuchungen}},
volume = {4},
year = {1973}
}
@article{Burgf,
author = {Burg, Heinz},
pages = {645--651},
title = {{B5 B5 Unf{\"{a}}lle mit Pkw B5}}
}
@article{Zienkiewicz2014g,
abstract = {Mutations in the human L1CAM gene cause neurodevelopmental disorders collectively referred to as L1 syndrome. Here, we investigated cellular pathomechanisms underlying two L1 syndrome mutations, R184Q and W1036L. We demonstrate that these mutations cause partial endoplasmic reticulum (ER) retention of L1, reduce L1 cell surface expression, but do not induce ER stress in neuronal NSC-34 cells. We provide evidence that surface trafficking of mutated L1 is affected by defective sorting to ER exit sites and attenuated ER export. However, in differentiated neuronal cultures and long-term cultured hippocampal slices, the L1-R184Q protein is restricted to cell bodies, whereas L1-W1036L also aberrantly localizes to dendrites. These trafficking defects preclude axonal targeting of L1, thereby affecting L1-mediated axon growth and arborization. Our results indicate that L1 syndrome mutations impair neuronal L1 function at different levels, firstly by attenuating ER export and secondly by interfering with polarized neuronal trafficking.},
author = {Zienkiewicz, O.C. and Taylor, R.L. and Nithiarasu, P.},
doi = {10.1016/B978-1-85617-635-4.00015-7},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Zienkiewicz FEM - Vol 3 Fluid Dynamics/63229{\_}13.pdf:pdf},
isbn = {9781856176354},
journal = {Finite Elem. Method Fluid Dyn.},
number = {1},
pages = {485--491},
title = {{Computer Implementation of the CBS Algorithm}},
url = {http://linkinghub.elsevier.com/retrieve/pii/B9781856176354000157},
year = {2014}
}
@article{Tragwerke,
author = {Tragwerke, Statik},
doi = {10.1007/978-3-642-16828-4},
isbn = {9783642168284},
title = {3}
}
@book{Oerteljr.2011,
author = {Oertel jr., Herbert and B{\"{o}}hle, Martin and Reviol, Thomas},
isbn = {9783834813978},
pages = {479},
title = {{Str{\{}{\"{o}}{\}}mungs- mechanik}},
year = {2011}
}
@article{Stupkiewicz2007e,
abstract = {Micromechanical analysis of heterogeneous materials allows prediction of their macroscopic behaviour from the known properties, microstructure, and interaction mechanisms of the constituents at the micro-scale. At the same$\backslash$n time, it allows determination of the microscopic response at each point of a macroscopic body subjected to external loading. The micromechanical analysis involves thus, at least,$\backslash$n two different scales of observation. The actual characteristic dimensions at these scales are, in fact, arbitrary, as long$\backslash$n as they differ sufficiently, so that the two scales can be separated.},
author = {Stupkiewicz, Stanislaw and Stupkiewicz, Stanislaw},
doi = {10.1007/978-3-540-49717-2},
isbn = {978-3-540-49716-5},
journal = {Micromechanics of Contact and Interphase Layers},
pages = {1 -- 6},
title = {{Micromechanics of Contact and Interphase Layers}},
url = {http://www.springerlink.com/index/10.1007/978-3-540-49717-2},
volume = {30},
year = {2007}
}
@article{Mesarovic2017a,
author = {Mesarovic, S},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/Folien CISM Summer School Mai2017 - Mesoscale Models/courses{\_}C1703{\_}Mesarovic+Lecture+3+CORR+2.pdf:pdf},
title = {{Physical foundations of meso-scale continua Part 2 : ( Thermo- ) Dynamics}},
year = {2017}
}
@article{Bohlke2001,
author = {B{\"{o}}hlke, Thomas and Br{\"{u}}ggemann, C},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/Strukturmechanik MMS/Literatur/Graphical Representation of the Generalized Hooke's Law{\_}SingleCrystals{\_}B{\"{o}}hlke{\_}Kommentar.pdf:pdf},
journal = {Techn,sche Mech.},
number = {2},
pages = {145--158},
title = {{Graphical Representation of the Generalized Hooke's Law}},
volume = {21},
year = {2001}
}
@article{DeBellis2014,
author = {Bellis, Vincenzo De and Severi, Elena and Fontanesi, Stefano and Bozza, Fabio},
doi = {10.1016/j.egypro.2014.01.088},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Injection+Combustion+Ignitionsystems/2014{\_}Bellis+Fontanesi{\_}Hierarchical 1D3D approach for the development of a turbulence combustion model for turbo engine - turbulence model.pdf:pdf},
journal = {Energy Procedia},
pages = {829--838},
publisher = {Elsevier B.V.},
title = {{Hierarchical 1D / 3D approach for the development of a turbulent combustion model applied to a VVA turbocharged engine . Part I : turbulence model}},
volume = {45},
year = {2014}
}
@article{Sanli2008a,
abstract = {In this study, the heat transfer characteristics between gases and in-cylinder walls at fired and motored conditions in a diesel engine were investigated by using engine data obtained experimentally. For this investigation, a four-cylinder, indirect injection (IDI) diesel engine was tested under different engine speeds and loads. The heat transfer coefficient was calculated by using Woschni expression correlated for the IDI diesel engines, and also using Annand and Hohenberg expressions. The temperature of in-cylinder gases were determined from a basic model based on the first law of thermodynamics after measuring in-cylinder pressure experimentally. The results show that the heat transfer characteristics of the IDI diesel engine strongly depend on the engine speed and load as a function of crank angle at fired and motored conditions. {\textcopyright} 2007 Elsevier Ltd. All rights reserved.},
author = {Sanli, Ali and Ozsezen, Ahmet N. and Kilicaslan, Ibrahim and Canakci, Mustafa},
doi = {10.1016/j.applthermaleng.2007.10.005},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Heat Transfer Combustion Chamber/2008{\_}Sanli{\_}The influence of engine speed and load on the heat transfer between gases an incylinder walls at firted and motored conditions.pdf:pdf},
journal = {Appl. Therm. Eng.},
keywords = {Heat flux,Heat transfer coefficient,IDI diesel engine},
number = {11-12},
pages = {1395--1404},
title = {{The influence of engine speed and load on the heat transfer between gases and in-cylinder walls at fired and motored conditions of an IDI diesel engine}},
volume = {28},
year = {2008}
}
@article{Schwartz1997,
author = {Schwartz, Mel M.},
doi = {10.1177/0892705712453152},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/{\_}buecherSong/HandbookofComposites/I/01{\_}OverviewofCompositeMaterials.pdf:pdf},
isbn = {0444888527},
issn = {21554854},
pages = {43--44},
title = {{Composite Materials}},
year = {1997}
}
@article{Raillard2015,
author = {Raillard, B and Mu, F},
doi = {10.1016/B978-1-78242-074-3.00024-6},
isbn = {9781782420743},
title = {24 24.1},
year = {2015}
}
@article{Wimmer2000,
abstract = {This paper summarizes the results of several investigations on in-cylinder heat transfer during high-pressure and gas exchange phases as well as heat transfer in the inlet and outlet ports for a number of different engine types (DI Diesel, SI and gaseous fueled engine). The paper contains a comparision of simulation results and experimental data derived from heat flux measurements. Numerical results were obtained from zero-, one- and three-dimensional simulation methods. Time and spatially resolved heat fluxes were measured applying the surface temperature method and special heat flux sensors. The paper also includes an assessment of different sensor types with respect to accuracy and applicability.ER -},
author = {Wimmer, Andreas and Pivec, Robert and Sams, Theodor},
doi = {https://doi.org/10.4271/2000-01-0568},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2000{\_}Wimmer{\_}Heat Transfer to the Combustion Cahmber and Port Walls of IC Engines - Measurement and Prediction.pdf:pdf},
journal = {SAE Tech. Pap. Ser.},
title = {{Heat Transfer to the Combustion Chamber and Port Walls of IC Engines - Measurement and Prediction}},
year = {2000}
}
@book{Gross2011g,
author = {Gross, Dietmar and Seelig, Thomas},
doi = {10.1007/978-3-642-10196-0},
isbn = {978-3-642-10195-3},
title = {{Bruchmechanik}},
url = {http://link.springer.com/10.1007/978-3-642-10196-0},
year = {2011}
}
@article{Dera,
author = {Der, Einteilung Vorteile},
title = {{5 Umformen 5.1}}
}
@inproceedings{Chang2004,
abstract = {An experimental study has been carried out to provide qualitative and quantitative insight into gas to wall heat transfer in a gasoline fueled Homogeneous Charge Compression Ignition (HCCI) engine. Fast response thermocouples are embedded in the piston top and cylinder head surface to measure instantaneous wall temperature and heat flux. Heat flux measurements obtained at multiple locations show small spatial variations, thus confirming relative uniformity of incylinder conditions in a HCCI engine operating with premixed charge. Consequently, the spatially-averaged heat flux represents well the global heat transfer from the gas to the combustion chamber walls in the premixed HCCI engine, as confirmed through the gross heat release analysis. Heat flux measurements were used for assessing several existing heat transfer correlations. One of the most popular models, the Woschni expression, was shown to be inadequate for the HCCI engine. The problem is traced back to the flame propagation term which is not appropriate for the HCCI combustion. Subsequently, a modified model is proposed which significantly improves the prediction of heat transfer in a gasoline HCCI engine and shows very good agreement over a range of conditions},
author = {Chang, Junseok and G{\"{u}}ralp, Orgun and Filipi, Zoran and Assanis, Dennis N. and Kuo, Tang-Wei and Najt, Paul and Rask, Rod},
booktitle = {SAE Tech. Pap. 2004-01-2996},
doi = {10.4271/2004-01-2996},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2004{\_}Chang{\_}New Heat Transfer Correlation for an HCCI Engine Derived from Measurements of Instantaneous Surface Heat Flux.pdf:pdf},
publisher = {SAE international},
title = {{New Heat Transfer Correlation for an HCCI Engine Derived from Measurements of Instantaneous Surface Heat Flux}},
year = {2004}
}
@article{Pokluda2010,
author = {Pokluda, Jaroslav and Andera, Pavel},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2010{\_}Jaroslav Pokluda+Pavel {\v{S}}andera{\_}Micromechanisms of fracture and fatigue{\_}Buch/Kap3{\_}BrittleAndDuctileFracture.pdf:pdf},
journal = {Micromechanisms Fract. Fatigue},
pages = {69--123},
title = {{Brittle and Ductile Fracture}},
year = {2010}
}
@article{Meneghetti2016,
abstract = {Fatigue crack initiation and propagation involve plastic strains that require some work to be done on the material. Most part of this irreversible energy is dissipated as heat and consequently the material temperature increases. The heat being an indicator of the intense plastic strains occurring at the tip of a propagating fatigue crack, the hypothesis is formed that it can be used to assess the fatigue damage accumulation rate of cracked components. Moreover, the heat energy at the crack tip is averaged according to Neuber's finite particle concept. The aim of the present paper is to present the theoretical framework and the corresponding experimental technique to evaluate the heat energy dissipated in a structural volume surrounding the crack tip. The shape and size of the structural volume have been assumed according to the literature, even though the definition of the structural volume size of the analysed material in a fatigue sense is not the scope of the present paper. The proposed experimental technique to evaluate the averaged heat energy is based on the radial temperature profiles measured around the crack tip by means of an infrared camera. The temperature fields measured within few millimetres from the crack tip have been compared successfully with existing analytical solutions.},
author = {Meneghetti, G. and Ricotta, M.},
doi = {10.1016/j.ijfatigue.2016.04.001},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/2016{\_}Meneghetti{\_}Evaluating the heat energy dissipated in a small volume surrounding the tip of a fatigue crack.pdf:pdf},
issn = {01421123},
journal = {Int. J. Fatigue},
keywords = {AISI 304L,Averaging approaches,Crack propagation,Crack tip,Critical distance mechanics,Energy approaches,Fatigue assessment},
pages = {605--615},
publisher = {Elsevier Ltd},
title = {{Evaluating the heat energy dissipated in a small volume surrounding the tip of a fatigue crack}},
url = {http://dx.doi.org/10.1016/j.ijfatigue.2016.04.001},
volume = {92},
year = {2016}
}
@article{Launder1972,
author = {Launder, B E},
doi = {https://doi.org/10.1016/0017-9310(72)90076-2},
journal = {Int. J Heat Mass Transf.},
pages = {301--314},
title = {{The prediciton of laminarization with a two-equation model of turbulence}},
volume = {15},
year = {1972}
}
@article{Quation2003,
author = {Quation, F Inite Lement E},
title = {{By the}},
volume = {2},
year = {2003}
}
@article{Background,
author = {Background, General},
journal = {Mathematica},
pages = {1--207},
title = {{1.0 Remarks}}
}
@article{Jiang2004a,
abstract = {Fatigue crack propagation was modeled by using the cyclic plasticity material properties and fatigue constants for crack initiation. The cyclic elastic-plastic stress-strain field near the crack tip was analyzed using the finite element method with the implementation of a robust cyclic plasticity theory. An incremental multiaxial fatigue criterion was employed to determine the fatigue damage. A straightforward method was developed to determine the fatigue crack growth rate. Crack propagation behavior of a material was obtained without any additional assumptions or fitting. Benchmark Mode I fatigue crack growth experiments were conducted using 1070 steel at room temperature. The approach developed was able to quantitatively capture all the important fatigue crack propagation behaviors including the overload and the R-ratio effects on crack propagation and threshold. The models provide a new perspective for the R-ratio effects. The results support the notion that the fatigue crack initiation and propagation behaviors are governed by the same fatigue damage mechanisms. Crack growth can be treated as a process of continuous crack nucleation. },
author = {Jiang, Yanyao and Feng, Miaolin},
doi = {10.1115/1.1631026},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/2004{\_}Jiang{\_}Modeling of Fatigue Crack Propagation.pdf:pdf},
issn = {00944289},
journal = {J. Eng. Mater. Technol.},
number = {1},
pages = {77},
title = {{Modeling of Fatigue Crack Propagation}},
url = {http://materialstechnology.asmedigitalcollection.asme.org/article.aspx?articleid=1427113},
volume = {126},
year = {2004}
}
@article{Liu1973,
author = {Liu, I. Shih},
doi = {10.1007/BF00251292},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Thermodynamik/Liu-Entropieprinzip{\_}Lukas{\_}Fraunhofer/Liu-Entropieprinzip/Liu{\_}heat-conducting{\_}fluid{\_}1973.pdf:pdf},
issn = {00039527},
journal = {Arch. Ration. Mech. Anal.},
number = {1},
pages = {26--33},
title = {{A non-simple heat-conducting fluid}},
volume = {50},
year = {1973}
}
@article{Morris1981,
author = {Morris, W L and James, M R and Buck, O},
doi = {10.1007/BF02648508},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/1981{\_}Morris+James{\_}Growth rate models for short surface cracks in Al 2219-T851.pdf:pdf},
issn = {0360-2133},
journal = {Met. Trans. A},
number = {January},
pages = {57--64},
title = {{Growth rate models for short surface cracks in AI 2219-T851}},
volume = {12},
year = {1981}
}
@article{Gleichstromkreisa,
author = {Gleichstromkreis, Der},
pages = {83--92},
title = {{Der Gleichstromkreis 4 1 Grundbegriffe}}
}
@article{Planck2006,
author = {Planck, Max and Bahnen, Neue},
journal = {Gerthsen Phys.},
pages = {569--606},
title = {{11 - Strahlungsfelder}},
year = {2006}
}
@article{Desmorat2006,
abstract = {Application of damage mechanics to fatigue is addressed in the present paper. The ability of Lemaitre's damage law to describe low and high cycle fatigue failure of metals is illustrated. Its generalization into an evolution law modeling a damage rate governed by the main dissipative mechanics applies to concrete, elastomers, rocks and to probably other materials. The importance of rate written laws is emphasized.},
author = {Desmorat, Rodrigue},
doi = {10.1080/17747120.2006.9692859},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/2006{\_}Desmorat{\_}SummerSchool{\_}Damage and Fatigue Overview Evolution Equation.pdf:pdf},
isbn = {9780387739052},
issn = {1774-7120},
journal = {Rev. Eur. G{\{}{\'{e}}{\}}nie Civ.},
keywords = {concrete,damage,elastomers,fatigue,metals,rocks},
number = {6-7},
pages = {849--877},
title = {{Damage and Fatigue: Continuum damage mechanics modeling for fatigue of materials and structures}},
volume = {10},
year = {2006}
}
@article{Konzepte,
author = {Konzepte, Downsizing- and Steigerung, Eine and Gegensatz, Im and Geschwindigkeit, Die},
title = {{3 Downsizing}}
}
@article{Essmann1981c,
abstract = {Based on recent experimental observations a realistic model of the evolution of the surface profile of persistent slip bands (PSBs) in fatigued metals is proposed. An essential feature of the model is the production of vacancies by the annihilation of edge dislocations which, combined with irreversible slip processes, leads to an elongation of the PSB parallel to the active slip vector. It is shown that a net extrusion forms rather rapidly. The growth processes and their dependence on temperature are discussed in detail. It is proposed that cracks initiate at the surface steps at the PSB{\&}ndash;matrix interface and, at a later stage, also at the notch-peak profile from the random slip processes.},
author = {Essmann, U. and G{\"{o}}sele, U. and Mughrabi, H.},
doi = {10.1080/01418618108239541},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/2006{\_}Mughrabi + Essmann{\_}A model of extrusions and   intrusions in fatigued metals I Point defect production and the growth of   extrusions.pdf:pdf},
isbn = {0141-8610},
issn = {0141-8610},
journal = {Philos. Mag. A},
number = {2},
pages = {405--426},
title = {{A model of extrusions and intrusions in fatigued metals I. Point-defect production and the growth of extrusions}},
url = {http://www.tandfonline.com/doi/abs/10.1080/01418618108239541},
volume = {44},
year = {1981}
}
@article{Bennett2003a,
author = {Bennett, V and McDowell, D.{\~{}}L.{\~{}}},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2001{\_}Bennet{\_}Polycrystal orientation distribution effects on microslip  in high cycle fatigue.pdf:pdf},
journal = {Int. J. Fatigue},
keywords = {fatigue,microslip,orientation distribution},
pages = {27--39},
title = {{Polycrystal orientation distribution effects on microslip in high cycle fatigue}},
volume = {25},
year = {2003}
}
@article{Forest2004,
abstract = {The modeling of damage processes at the material point scale through a specific constitutive law addresses a wide variety of constitutive behaviors, for instance brittle elasticity where the evolution of damage degrades the elastic stiffness, or ductile plasticity where both dissipative mechanisms (plasticity and damage) are intimately coupled. In spite of their obvious differences, all these laws possess a common feature: beyond some load level, the domain of reversibility expressed in the stress space shrinks. This phenomenon is called strain-softening. This essential property, characteristic of damage mechanisms, is responsible for the localization of the mechanical fields (strain, damage, plastic strain, . . .) inside narrow bands, an experimental fact observed on many degrading materials such as soils, concrete, metals, etc., see for instance Desrues and Chambon (1985). Despite twenty years of intensive research, numerical modeling of the localization phenomenon remains a challenging objective which has not yet been given a fully satisfactory answer. This is in contrast with the great progresses that have been achieved regarding the local description of damage mechanisms for various materials, on the basis of micro–macro derivations as well as phenomenological intuitions. Unfortunately, localization partially hinders predictive computations of propagating damaged zones in real-life structures submitted to a given load history. The difficulty originates from the fact that the equations that describe the structural behavior (including not only the constitutive law but also the equilibrium and compat-ibility equations) result in an ill-posed problem which manifests itself by a spurious mesh-dependency when making use of finite element solutions. After a first insight into the localization phenomena, the problem of loss of uniqueness and loss of ellipticity is addressed for elastoplastic solids. General (diffuse) and localized bifurcation modes are distinguished. The existence of jumps of the velocity gradient is explored in the dynamic (acceleration waves) and static cases (stationary waves). Critical values of hardening moduli for loss of uniqueness or loss of ellipticity are derived. A link between the notion of material stability and acceleration waves is also presented. The collected strain localization criteria are summarized in section 1.2.6. Note that the derivations and formula are presented in the case of elastoplastic ma-terials. However the results can be extended to damaging materials in a straightforward 311 312 Local approach to fracture manner. In fact it deals with all incremental models involving a fourth–rank tangent operator L ∼ ∼ .},
author = {Forest, S and Lorentz, E},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/xxx{\_}Forst+Lorentz{\_}Localization{\_}phenomena{\_}and{\_}regularization{\_}methods-damage.pdf:pdf},
journal = {Local Approach to Fract.},
pages = {311--371},
title = {{Localization phenomena and regularization methods}},
volume = {1},
year = {2004}
}
@article{Wei2007,
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Wei, Wilfried},
doi = {10.1007/978-3-8348-0353-5},
eprint = {arXiv:1011.1669v3},
isbn = {978-3-8348-0058-9},
issn = {0717-6163},
pmid = {15003161},
title = {{Elektrotechnik f{\"{u}}r Ingenieure 1}},
year = {2007}
}
@article{Abbrennstumpfschwei,
author = {Abbrennstumpfschwei, A-stabelektrode and Prototyping, Rapid and Abk, Abkantpresse and Abschr, Abschmelzleistung and Abstreckziehen, Sintern and Abtrennen, Erodieren and Acetylen, Acc-regelung Aceton and Acetylenzerfall, Verbrennungsstufe and Aktivkraft, Aco-regelung Aggregat and Aluminiumlegierung, Aluminiumbasislot and Anschmelzung, Anodenfall and Anschnittsystem, Anschnittquerschnitt and Arbeitsbedarf, Apfelsinenhaut and Arbeitsebene, Walzen and Arbeitstemperatur, Arbeitseingriff and Aufschmelzgrad, Aufbauschneide Aufheizgeschwindigkeit},
title = {{6 Sachwortverzeichnis}}
}
@article{Rostampour2015a,
abstract = {This investigation deals with the EF7 (TC) engine, a dual fuel engine equipped with a turbocharger system, consequently with a high probability of knock inception. In this study, an operating cycle of the engine was simulated using KIVA-3V code. Some modifications were carried out on the KIVA method of calculating pressure in the intake port in order to simulate turbocharger pressure correctly. Auto-ignition and knock were then simulated using the auto-ignition integral model. The modified code and the simulation were verified using three different methods; in-cylinder average pressure, gas temperature of the exhaust port, and auto-ignition timing. The simulation results using the auto-ignition integral model, as compared with the experimental data, proved to be reasonably accurate. Following this validation, the effect of the knock phenomenon on the engine heat transfer through the walls was investigated. The simulations showed that the rate of heat transfer through the walls under knocking conditions is about 2.2 times higher than that under normal conditions. However, it was also shown that the total heat transfer increases about 15{\{}{\%}{\}}.},
author = {Rostampour, Arman and Toosi, Ali Nassiri},
doi = {10.1115/1.4030517},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2015{\_}Rostampour{\_}Numerical Investigation of the effect of knock on heat transfer in a turbo si engine.pdf:pdf},
issn = {0742-4795},
journal = {J. Eng. Gas Turbines Power},
number = {12},
pages = {121502},
title = {{Numerical Investigation of the Effect of Knock on Heat Transfer in a Turbocharged Spark Ignition Engine}},
url = {http://www.scopus.com/inward/record.url?eid=2-s2.0-84930634240{\%}7B{\&}{\%}7DpartnerID=tZOtx3y1},
volume = {137},
year = {2015}
}
@article{Science1979,
author = {Science, Greek and Imagery, Social},
journal = {Text},
title = {{Kapitel 3}},
year = {1979}
}
@article{Verbrennungsprozess,
author = {Verbrennungsprozess, Der},
pages = {282--299},
title = {{11 Verbrennung 11.1}}
}
@article{Meneghetti2016a,
abstract = {Fatigue crack initiation and propagation involve plastic strains that require some work to be done on the material. Most part of this irreversible energy is dissipated as heat and consequently the material temperature increases. The heat being an indicator of the intense plastic strains occurring at the tip of a propagating fatigue crack, the hypothesis is formed that it can be used to assess the fatigue damage accumulation rate of cracked components. Moreover, the heat energy at the crack tip is averaged according to Neuber's finite particle concept. The aim of the present paper is to present the theoretical framework and the corresponding experimental technique to evaluate the heat energy dissipated in a structural volume surrounding the crack tip. The shape and size of the structural volume have been assumed according to the literature, even though the definition of the structural volume size of the analysed material in a fatigue sense is not the scope of the present paper. The proposed experimental technique to evaluate the averaged heat energy is based on the radial temperature profiles measured around the crack tip by means of an infrared camera. The temperature fields measured within few millimetres from the crack tip have been compared successfully with existing analytical solutions.},
author = {Meneghetti, G. and Ricotta, M.},
doi = {10.1016/j.ijfatigue.2016.04.001},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2016{\_}Meneghetti{\_}Evaluating the heat energy dissipated in a small volume surrounding the tip of a fatigue crack.pdf:pdf},
issn = {01421123},
journal = {Int. J. Fatigue},
keywords = {AISI 304L,Averaging approaches,Crack propagation,Crack tip,Critical distance mechanics,Energy approaches,Fatigue assessment},
pages = {605--615},
publisher = {Elsevier Ltd},
title = {{Evaluating the heat energy dissipated in a small volume surrounding the tip of a fatigue crack}},
url = {http://dx.doi.org/10.1016/j.ijfatigue.2016.04.001},
volume = {92},
year = {2016}
}
@article{Beispielb,
author = {Beispiel, Zum and Interpolation, Die and Computerspiel, Ein},
title = {{A Interpolation}}
}
@article{Horstemeyer1999a,
abstract = {A phenomenological void–crack nucleation model for ductile metals with secondphases is described which is motivated from fracture mechanics and microscale physicalobservations. The void–crack nucleation model is a function of the fracture toughness of theaggregate material, length scale parameter (taken to be the average size of the second phaseparticles in the examples shown in this writing) , the volume fraction of the second phase, strainlevel, and stress state. These parameters are varied to explore their effects upon the nucleationand damage rates. Examples of correlating the void–crack nucleation model to tension data in theliterature illustrate the utility of the model for several ductile metals. Furthermore, compression,tension, and torsion experiments on a cast Al–Si–Mg alloy were conducted to determinevoid–crack nucleation rates under different loading conditions. The nucleation model was thencorrelated to the cast Al–Si–Mg data as well.},
author = {Horstemeyer, Mark F and Gokhale, Arun M},
doi = {10.1016/S0020-7683(98)00239-X},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Plasticity models/A void crack nucleation model for ductile metals with or without inclusions{\_}HorstemeyerAndGokhale.pdf:pdf},
isbn = {00207683 (ISSN)},
issn = {00207683},
journal = {Int. J. Solids Struct.},
pages = {5029--5055},
pmid = {111},
title = {{A Void-Crack Nucleation Model for Ductile Metals}},
volume = {36},
year = {1999}
}
@article{Wimmer2000c,
abstract = {This paper summarizes the results of several investigations on in-cylinder heat transfer during high-pressure and gas exchange phases as well as heat transfer in the inlet and outlet ports for a number of different engine types (DI Diesel, SI and gaseous fueled engine). The paper contains a comparision of simulation results and experimental data derived from heat flux measurements. Numerical results were obtained from zero-, one- and three-dimensional simulation methods. Time and spatially resolved heat fluxes were measured applying the surface temperature method and special heat flux sensors. The paper also includes an assessment of different sensor types with respect to accuracy and applicability.ER -},
author = {Wimmer, Andreas and Pivec, Robert and Sams, Theodor},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2000{\_}Wimmer{\_}Heat Transfer to the Combustion Cahmber and Port Walls of IC Engines - Measurement and Prediction.pdf:pdf},
number = {724},
title = {{Heat Transfer to the Combustion Chamber and Port Walls of IC Engines - Measurement and Prediction}},
year = {2000}
}
@article{Wang2016a,
abstract = {Cracks encountered in engineering structures are typically three dimensional, and the fracture mechanism remains unclear because of the superimposed stresses induced by mixed-mode I/II/III loading. This paper introduces a general 3D mixed-mode fracture criterion based on the maximum mean principal stress (MMPS) by introducing the concept of a characteristic fracture length that is related to the material tensile strength. This criterion has clear physical significance, a systematic mathematical expression and a wide scope of applications to estimate both the in- and out-of-plane fracture angles and fracture strength. The proposed criterion is validated for all mixed-mode conditions (I/II, I/III and II/III) and is compared with several widely used criteria based on experimental results reported in previous studies. Good agreement is achieved in terms of the fracture angles and, in particular, the fracture strength between the results predicted by the new criterion and the experimental results of various brittle materials.},
author = {Wang, J. and Ren, L. and Xie, L. Z. and Xie, H. P. and Ai, T.},
doi = {10.1016/j.ijsolstr.2016.10.009},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/2016{\_}Wang{\_}Maximum mean principal stress criterion for 3D brittle fracture.pdf:pdf},
issn = {00207683},
journal = {Int. J. Solids Struct.},
keywords = {3D fracture criterion,Characteristic fracture length,Mean stress,Mixed-mode loading},
pages = {142--154},
title = {{Maximum mean principal stress criterion for three-dimensional brittle fracture}},
volume = {102-103},
year = {2016}
}
@article{Gu2002,
author = {Gu, Minyi and Die, Lynda and Frank, R C and Mark, I D},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2012{\_}Trijselaar{\_}KNOCK PREDICTION IN GAS FIRED RECIPROCATING ENGINES.pdf:pdf},
pages = {8--15},
title = {{A N ew Vec t or f or H i gh - Throughpu t , L i ga t i on - I ndependen t C l on i ng E ncod i ng a Tobacco E t ch V i rus Pro t e ase C l e avage S i t e}},
volume = {15},
year = {2002}
}
@article{Arbeitsumgebungc,
author = {Arbeitsumgebung, Die},
journal = {Pro-Engineer Prakt.},
title = {{6 Baugruppenmodellierung}}
}
@article{Clement,
author = {Clement, Steffen and Informationstechnik, Elektro- and Klein, Bernd and Engelken, Gerhard and Konstruktion, Maschinenelemente and Czichos, Horst and Theumert, Hans and Maschinenbau, Grundlagen and Hei, Bernd and Ersoy, Metin and Isermann, Rolf and Schabacker, Michael and Fiala, Ernst and Klette, Guido},
isbn = {9783528331245},
journal = {Konstruktion},
title = {{Aus dem Programm}}
}
@article{Zhao2008,
abstract = {Extensive fatigue experiments were conducted using 7075-T651 aluminum alloy under uniaxial, torsion, and axial-torsion loading. Detailed fatigue results were reported. Different mean stresses were applied in the experiments and the mean stress was found to have a significant influence on the fatigue strength of the material. A tensile mean stress decreased the fatigue strength dramatically. Fatigue damage was found to occur under compression-compression loading. In addition, axial-torsion experiments using tubular specimens were conducted under different loading paths to study the multiaxial fatigue behavior. Fatigue cracking behavior was found to be dependent on the loading path as well as the loading magnitude. When the loading magnitude was high, the material displayed shear cracking. When the loading stress was below a certain level, the material exhibited tensile cracking. For most loading cases under investigation, the material displayed a mixed cracking behavior. A kink was found in the shear strain versus fatigue life curve from the pure torsion experiments, and it was associated with a distinctive transition of cracking behavior. The Smith-Watson-Topper (SWT) parameter with a critical plane interpretation was found to correlate well with most of the experiments conducted in terms of fatigue lives. However, the SWT parameter cannot deal with the uniaxial fatigue conditions where the maximum stress is low or negative. More importantly, the model fails to correctly predict the cracking behavior observed experimentally on the material. A critical plane criterion based on a combination of the normal and shear components of the stresses and strains on material planes was found to better correlate the fatigue experiments in terms of both fatigue life and cracking behavior. The characteristics of the multiaxial fatigue criterion were discussed based on the experimental observations on 7075-T651 aluminum alloy. ?? 2007 Elsevier Ltd. All rights reserved.},
author = {Zhao, Tianwen and Jiang, Yanyao},
doi = {10.1016/j.ijfatigue.2007.07.005},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Empirical Fatigue Models + Validation/2007{\_}Jiang{\_}Fatigue of 7075-T651 aluminum alloy VALIDATION+MODEL.pdf:pdf},
isbn = {0142-1123},
issn = {01421123},
journal = {Int. J. Fatigue},
keywords = {7075-T651 aluminum alloy,Axial-torsion,Compression-compression fatigue,Multiaxial criterion,Multiaxial fatigue},
number = {5},
pages = {834--849},
title = {{Fatigue of 7075-T651 aluminum alloy}},
volume = {30},
year = {2008}
}
@article{Kress2004,
author = {Kress, Gerald},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/{\_}skripte/Kress 2004 - Strukturanalyse mit FEM.pdf:pdf},
journal = {Cent. Struct. Technol. ETHZ},
pages = {1--124},
title = {{Strukturanalyse mit FEM}},
url = {http://www.structures.ethz.ch/education/master/analysis/Skript/FEM{\_}D{\_}Main{\_}2009.pdf},
year = {2004}
}
@misc{Mura1982a,
author = {Mura, Toshio},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/Strukturmechanik MMS/Literatur/Mikromechanik{\_}B{\"{u}}cher{\_}Literaturvorschlag{\_}MMS/Mura 1987 Micromechanics of defects in solids.pdf:pdf},
title = {{Mechanics of elastic and inelastic solids}},
year = {1982}
}
@article{Zienkiewicz2000,
abstract = {We have so far dealt with one possible approach to the approximate solution of the particular problem of linear elasticity. Many other continuum problems arise in engineering and physics and usually these problems are posed by appropriate differ- ential equations and boundary conditions to be imposed on the unknown function or functions. It is the object of this chapter to show that all such problems can be dealt with by the finite element method.},
author = {Zienkiewicz, O.C. and Taylor, R.L.},
doi = {http://dx.doi.org/10.1016/B978-075066431-8.50171-5},
isbn = {0 7506 5049 4},
journal = {Finite Elem. Method Vol. 1 Basis},
pages = {39--60},
title = {{Generalization of the finite element concepts. Galerkin-weighted residual and variational approaches}},
url = {http://freeit.free.fr/Finite Element/Zienkiewicz/Volume 1 The Basis/},
year = {2000}
}
@article{Sharma2002,
abstract = {This paper illustrates the micromechanics approach to cyclic creep-fatigue damage of Pb-Sn, developed by the authors with the help of a simple case study. It is demonstrated that durability predictions can be made based solely on monotonic test data. Various parametric studies of practical interest are conducted to obtain mechanistic insights into various aspects of damage in solders e.g., effect of hydrostatic stresses, grain size, ramp rate, etc.},
author = {Sharma, Pradeep and Dasgupta, Abhijit},
doi = {10.1115/1.1493203},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Kriechen{\_}Spannungsrelaxation/2002{\_}Sharma Pradeep{\_}Micro-Mechanics of Creep-Fatigue Damage in PB-SN Solder Due to Thermal Cycling PartOne.pdf:pdf},
issn = {1043-7398},
journal = {J. Electron. Packag.},
number = {3},
pages = {298--304},
title = {{Micro-Mechanics of Creep-Fatigue Damage in PB-SN Solder Due to Thermal Cycling—Part II: Mechanistic Insights and Cyclic Durability Predictions From Monotonic Data}},
url = {http://dx.doi.org/10.1115/1.1493203{\%}7B{\%}25{\%}7D5Cnhttp://electronicpackaging.asmedigitalcollection.asme.org/data/Journals/JEPAE4/26206/298{\%}7B{\_}{\%}7D1.pdf},
volume = {124},
year = {2002}
}
@article{Lin1969a,
abstract = {The mechanics of the build-up of large local plastic strains at the free surface of a polycrystal under fatigue loading is shown. Two closely located thin slices in a most-favourably-oriented crystal located at a free surface of the polycrystal are assumed to have an initial resolved shear stress of a few psi of opposite sign. Under cyclic loading, the two thin slices slide in opposite directions, one during the forward loading and the other during the reversed loading. Based on the dependency of slip on the resolved shear stress, the increase of local plastic strain in the slices with cycles of loading is calculated by applying the analogy between plastic strain and external force. The calculated local plastic shear strain in both slices (one positive and the other negative) reaches 100 per cent at the free surface in a few hundred cycles. These large plastic shear strains clearly cause the start of an extrusion or intrusion and the nucleation of a fatigue crack.},
author = {Lin, TH and Ito, YM},
doi = {doi: DOI: 10.1016/0022-5096(69)90006-4},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/1969{\_}Lin{\_}Mechanics of a fatigue crack nucleation mechanism.pdf:pdf},
isbn = {0022-5096},
issn = {0022-5096},
journal = {J. Mech. Phys. Solids},
pages = {511--523},
title = {{Mechanics of a Fatigue Crack Nucleation Mechanism}},
url = {http://www.sciencedirect.com/science/article/pii/0022509669900064},
volume = {17},
year = {1969}
}
@article{Antriebe2005,
author = {Antriebe, Hydrostatische},
pages = {1--53},
title = {{Hydrostatische Antriebe}},
year = {2005}
}
@article{Simulation,
author = {Simulation, Eine and Simulationsprozess, Dieser and Reifenmodelle, Diese and Simulationsergebnisse, Diese and Prozess, Dieser and Simulation, Die and Gesamtprozess, Der},
journal = {Simulation},
title = {{12 Simulation}}
}
@article{Santus2009,
abstract = {In metals, during high cycle fatigue on plain specimens, almost the entire fatigue life is spent as short crack initiation and propagation. The fatigue short crack life can be schematically divided into two subsequent phases: microstructurally short crack and physically short crack. Recently, Chapetti proposed a physically short crack threshold and propagation driving force model [Chapetti MD. Fatigue propagation threshold of short cracks under constant amplitude loading. Int J Fatigue 2003;25(12):1319-1326]. In his model the physically short crack behavior is obtained from the long crack propagation, just introducing the reduced threshold due to unsaturated closure. In the present paper the physically short crack propagation is similarly modeled by means of a driving force equation, but independent from the long crack propagation. In this way, a better description of the short crack behavior is provided, however short crack propagation data is required. Physically short crack propagation model parameters were obtained, by fitting experimental data drawn from the literature, for two aluminum alloys and a titanium alloy at two different heat treatment conditions and load ratios. By calculating the physically short crack plus long crack propagation, and assuming microstructurally short crack as part of the initiation stage, a purer information about crack initiation can be drawn from the S-N curves, and it is shown in the paper for the investigated materials. A precise crack initiation size and the number of cycles just for initiation are then provided. This information is useful to accurately predict fatigue life for blunt notched and for thick components, where the propagation is much higher than in the small plain specimen. A validation of the model was obtained by predicting the fatigue life of a notched specimen. An accurate prediction was obtained both when the initiation was much smaller than propagation and when almost the entire fatigue life was initiation. ?? 2009 Elsevier Ltd. All rights reserved.},
author = {Santus, C. and Taylor, D.},
doi = {10.1016/j.ijfatigue.2009.03.002},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/2009{\_}SantusAndTaylor{\_}Physically short crack propagation in metals during high cycle fatigue.pdf:pdf},
isbn = {01421123},
issn = {01421123},
journal = {Int. J. Fatigue},
keywords = {Fatigue crack initiation,Fatigue crack propagation,Microstructurally short cracks,Notched component fatigue life,Physically short cracks},
number = {8-9},
pages = {1356--1365},
publisher = {Elsevier Ltd},
title = {{Physically short crack propagation in metals during high cycle fatigue}},
url = {http://dx.doi.org/10.1016/j.ijfatigue.2009.03.002},
volume = {31},
year = {2009}
}
@article{Menny2006,
author = {Menny, Klaus},
isbn = {103-519-46317-2},
title = {{1.Pdf}},
year = {2006}
}
@article{Elasticity2003,
author = {Elasticity, Linear},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Nicholson 2003 - Finite Element Analysis Thermomechanics of Solids/0749{\_}C06.pdf:pdf},
pages = {95--106},
title = {{Stress-Strain Relation and the Tangent-Modulus Tensor 6.1}},
year = {2003}
}
@article{Nenngro,
author = {Nenngro, Mit Den},
pages = {118--124},
title = {{16 Riementriebe}}
}
@inproceedings{Karnik2015,
abstract = {Numerous studies describe the fuel consumption benefits of changing the powertrain temperature based on vehicle operating conditions. Actuators such as electric water pumps and active thermostats now provide more flexibility to change powertrain operating temperature than traditional mechanical-only systems did.Various control strategies have been proposed for powertrain temperature set-point regulation. A characteristic of powertrain thermal management systems is that the operating conditions (speed, load etc) change continuously to meet the driver demand and in most cases, the optimal conditions lie on the edge of the constraint envelope. Control strategies for set-point regulation which rely purely on feedback for disturbance rejection, without knowledge of future disturbances, might not provide the full fuel consumption benefits due to the slow thermal inertia of the system.A solution to this problem is to design a control strategy that utilizes an estimate of variability of future disturbances. In this work, we consider the design of a controller for direct optimization of fuel consumption which allows for improved handling of constraints on temperatures and actuators. We propose a robust Model Predictive Control (MPC) formulation to optimize fuel consumption. The controller formulation guarantees that temperature constraints are met for future load and speed profile within specified bounds. The performance of the proposed controller is demonstrated through simulations on a system that uses an electric water pump, active thermostat and radiator fan, to control engine oil and metal (lumped block/head mass) temperature during regular driving so that fuel consumption is minimized.},
author = {Karnik, Amey and Pachner, Daniel and Fuxman, Adrian M and Germann, David and Jankovic, Mrdjan and House, Christopher},
booktitle = {SAE 2015 World Congr. Exhib.},
doi = {https://doi.org/10.4271/2015-01-0336},
file = {:C$\backslash$:/Users/p327208/Desktop/Promotion/Literature/Motorspezifisch/Thermal Coating + Water Heat Transfer + Applikation/2015{\_}Karnik{\_}Model Predictive Control for Engine Powertrain Thermal Management Applications.pdf:pdf},
month = {apr},
publisher = {SAE International},
title = {{Model Predictive Control for Engine Powertrain Thermal Management Applications}},
year = {2015}
}
@article{Normen1997,
author = {Normen, Deutsche},
title = {{Normen und Richtlinien f{\"{u}}r Verbrennungsmotoren}},
year = {1997}
}
@article{Gurtin1967a,
author = {Gurtin, Morton E. and Williams, William O.},
doi = {10.1007/BF00285676},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Thermodynamik/An Axiomatic Foundation for Continuum Thermodynamics{\_}CommunicatedByNoll.pdf:pdf},
issn = {00039527},
journal = {Arch. Ration. Mech. Anal.},
number = {2},
pages = {83--117},
title = {{An axiomatic foundation for continuum thermodynamics}},
volume = {26},
year = {1967}
}
@article{The2003,
author = {The, S Olving and Lement, F Inite and Tatic, E Quations S},
pages = {153--165},
title = {{Solution Methods for Linear Problems 11.1}},
year = {2003}
}
@article{Vektor,
author = {Vektor, Ein},
doi = {10.1007/3-540-28067-7_13},
isbn = {978-3-540-25782-0},
pages = {80--87},
title = {{EIGENWERTE und EIGENVEKTOREN}},
volume = {0}
}
@article{Martin2003,
abstract = {We study a family of "classical" orthogonal polynomials which satisfy (apart from a 3-term recurrence relation) an eigenvalue problem with a differential operator of Dunkl-type. These polynomials can be obtained from the little {\$}q{\$}-Jacobi polynomials in the limit {\$}q=-1{\$}. We also show that these polynomials provide a nontrivial realization of the Askey-Wilson algebra for {\$}q=-1{\$}.},
archivePrefix = {arXiv},
arxivId = {10.1007/978-3-662-49677-0},
author = {Martin, Holger},
doi = {10.1002/cite.200303280},
eprint = {978-3-662-49677-0},
isbn = {978-3-642-05500-3},
issn = {0009286X},
journal = {Chemie-Ingenieur-Technik},
number = {10},
pages = {1472--1475},
pmid = {589023500},
primaryClass = {10.1007},
title = {{W??rme- und Stoff??bertragung}},
volume = {75},
year = {2003}
}
@article{Wallentowitz2006d,
author = {Wallentowitz, Henning and Reif, Konrad},
doi = {10.1007/978-3-8348-9121-1_10},
journal = {Handb. Kraftfahrzeugelektronik - Grundlagen, Kompon. Syst. Anwendungen},
title = {{Telematik}},
url = {http://www.springerlink.com/index/10.1007/978-3-8348-9121-1{\%}7B{\_}{\%}7D10},
year = {2006}
}
@article{Planck2006,
author = {Planck, Max and Bahnen, Neue},
journal = {Gerthsen Phys.},
pages = {569--606},
title = {{11 - Strahlungsfelder}},
year = {2006}
}
@article{Azzouz2010,
author = {Azzouz, F and Cailletaud, G and Quilici, S},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Kriechen{\_}Spannungsrelaxation/xxx{\_}Chaboche+Azzouz{\_}Cyclic calculations and life estimation in thermomechanical fatigue.pdf:pdf},
pages = {785--793},
title = {{Cyclic calculations and life estimation in thermomechanical fatigue}},
year = {2010}
}
@article{Seyedia,
author = {Seyedi, M and Desmorat, R},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/2 scale models papers/Seyedi+Desmorat+Sermage{\_}A TWO SCALE DAMAGE MODEL FOR THERMOMECHANICAL HIGH CYCLE FATIQUE FAILURE.pdf:pdf},
title = {{Two Scale Damage Model for Thermomechanical High Cycle Fatigue Failure}}
}
@article{Band,
author = {Band, Begriff Der Ortskurve},
pages = {124--126},
title = {{5 Ortskurven}}
}
@article{Brecq2005b,
abstract = {High frequency pressure oscillations are generated under knocking conditions within the combustion chamber of Spark Ignition engines. Although acoustic-oscillation model can give the natural frequencies of these oscillations, very few mathematical models are today available, in scientific literature, to describe the oscillation deadening effect. An analytical formulation of the deadening has been highlighted. Analytical solution has been established for future ECU implementation. Coupling this new concept and an existing high-frequency model, an achieved model of the knocking pressure high frequencies is compared to experimental data. Good behavior is obtained on a natural gas fuelled spark ignition engine.},
author = {Brecq, G and {Le Corre}, O},
doi = {10.4271/2005-01-1126},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2005{\_}Brecq{\_}Modeling of In-cylinder Pressure Oscillations under Knocking conditions - Intro to Pressure Envelope Curve.pdf:pdf},
isbn = {2005011126},
issn = {0148-7191},
title = {{Modeling of In-cylinder Pressure Oscillations under Knocking Conditions: Introduction to Pressure Envelope Curve}},
url = {http://papers.sae.org/2005-01-1126/},
year = {2005}
}
@article{Entropy2003,
author = {Entropy, O F},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Nicholson 2003 - Finite Element Analysis Thermomechanics of Solids/0749{\_}C07.pdf:pdf},
journal = {Energy},
pages = {107--116},
title = {{Thermal and Thermomechanical Response}},
year = {2003}
}
@inproceedings{Wimmer2000,
abstract = {This paper summarizes the results of several investigations on in-cylinder heat transfer during high-pressure and gas exchange phases as well as heat transfer in the inlet and outlet ports for a number of different engine types (DI Diesel, SI and gaseous fueled engine). The paper contains a comparision of simulation results and experimental data derived from heat flux measurements. Numerical results were obtained from zero-, one- and three-dimensional simulation methods. Time and spatially resolved heat fluxes were measured applying the surface temperature method and special heat flux sensors. The paper also includes an assessment of different sensor types with respect to accuracy and applicability.ER -},
author = {Wimmer, Andreas and Pivec, Robert and Sams, Theodor},
booktitle = {SAE Tech. Pap. Ser. 2000-01-0568},
doi = {https://doi.org/10.4271/2000-01-0568},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2000{\_}Wimmer{\_}Heat Transfer to the Combustion Cahmber and Port Walls of IC Engines - Measurement and Prediction.pdf:pdf},
publisher = {SAE international},
title = {{Heat Transfer to the Combustion Chamber and Port Walls of IC Engines - Measurement and Prediction}},
year = {2000}
}
@article{Baaser2010,
author = {Baaser, Herbert},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/{\_}skripte/TU Darmstadt 2010 - ABAQUS Materialsimulation beispiele.pdf:pdf},
title = {{FEM–Kurs - FEM-Simulationen mit ABAQUS}},
year = {2010}
}
@article{Tong2013,
abstract = {Ratchetting deformation has significant implications on material damage and fatigue life of components under service loading conditions. In this work, we explore the concept of ratchetting strain as a driving force in controlling crack growth, both time-independent and time-dependent, utilising elasto-plastic, visco-plastic and crystal-plasticity constitutive models. Characteristics of crack tip deformation were examined for both stationary and growing cracks using the finite element method. Whilst the strain range and the stress range remained largely unchanged throughout the loading cycles, distinctive strain ratchetting behaviour near the crack tip occurred in all cases, leading to progressive accumulation of tensile strain normal to the crack growth plane. It seems plausible that this tensile strain, or ratchetting strain, may be responsible for material separation leading to crack growth. The effects of material constitutive model, grain orientation and loading frequency on the development of ratchetting strain were also examined. Ratchetting strain was found to be related to accumulated plastic strain; and both were used in a crack growth criterion with which the crack growth rates of a nickel alloy were predicted. The preliminary results seem to be encouraging. ?? 2012 Elsevier Ltd. All rights reserved.},
author = {Tong, J and Zhao, L G and Lin, B},
doi = {10.1016/j.ijfatigue.2012.01.003},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/2013{\_}Tong+Zhao+Lin{\_}Ratchetting strain as a driving force for fatigue crack growth.pdf:pdf},
isbn = {01421123},
issn = {01421123},
journal = {Int. J. Fatigue},
keywords = {Constitutive model,Crack tip,Fatigue crack growth,Ratchetting},
pages = {49--57},
publisher = {Elsevier Ltd},
title = {{Ratchetting strain as a driving force for fatigue crack growth}},
url = {http://dx.doi.org/10.1016/j.ijfatigue.2012.01.003},
volume = {46},
year = {2013}
}
@book{Flaceliere2007a,
author = {Flaceliere, L and Morel, F and Dragon, A},
booktitle = {Int. J. Damage Mech.},
doi = {10.1177/1056789506067935},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/2 scale models papers/2007{\_} Flaceliere+Morel+Dragon{\_}Coupling Between Mesoplasticity and Damage in HCF{\_}MitViskoEffekte.pdf:pdf},
isbn = {1056789506},
issn = {1056-7895},
keywords = {author to whom correspondence,damage model,e-mail,ensma,experiment,flaceliere,fr,lmpm,mesoplasticity,multiaxial fatigue,should be addressed},
number = {4},
pages = {473--509},
title = {{Coupling Between Mesoplasticity and Damage in High-cycle Fatigue}},
volume = {16},
year = {2007}
}
@article{Papula2009,
abstract = {Kennzeichen der B nde des erfahrenen Hochschullehrers und erfolgreichen Autors ist die anschauliche und leicht verst ndliche Darstellungsform des mathematischen Stoffes. Mit seiner un bertroffenen didaktischen Konzeption erm glicht das Buch einen nahtlosen bergang von der Schul- zur anwendungsorientierten Hochschulmathematik. Die leicht verst ndliche und anschauliche Art der Darstellung hat das Buch zum Standardwerk der Ingenieurmathematik werden lassen.Die aktuelle Auflage enth lt ein neues Kapitel Fourier-Transformationen.},
author = {Papula, Lothar},
isbn = {3834805645},
pages = {795},
title = {{Mathematik f{\{}{\"{u}}{\}}r Ingenieure und Naturwissenschaftler 2: Ein Lehr- und Arbeitsbuch f{\{}{\"{u}}{\}}r das Grundstudium. Mit zahlreichen Beispielen aus Naturwissenschaft und Technik, 310 {\{}{\"{U}}{\}}bungsaufgaben mit ausf{\{}{\"{u}}{\}}hrlichen L{\{}{\"{o}}{\}}sungen. Mit zahlreichen Beispielen aus Nat}},
url = {http://books.google.com/books?id=vQgR9GR8nYEC{\%}7B{\&}{\%}7Dpgis=1},
year = {2009}
}
@article{Grandin2000a,
abstract = {It is generally accepted that knocking combustion influences the heat transfer in SI engines. However, the effects of heat transfer on the onset of knock is still not clear due to lack of experimental data of the thermal boundary layer close to the combustion chamber wall. This paper presents measurements of the temperature in the thermal boundary layer under knocking and non-knocking conditions. The temperature was measured using dual-broadband rotational Coherent anti-Stokes Raman Spectroscopy (CARS). Simultaneous time-resolved measurements of the cylinder pressure, at three different locations, and the heat flux to the wall were carried out. Optical access to the region near the combustion chamber wall was achieved by using a horseshoe-shaped combustion chamber with windows installed in the rectangular part of the chamber. This arrangement made CARS temperature measurements close to the wall possible and results are presented in the range 0.1-5 mm from the wall. The engine was run with constant fuel flow under near stoichiometric conditions. Knocking and non-knocking conditions were achieved by using different mixtures of n-heptane and iso-octane.},
author = {Grandin, B{\"{o}}rje and Denbratt, Ingemar and Bood, Joakim and Brackmann, Christian and Bengtsson, Per-Erik},
doi = {10.4271/2000-01-2831},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Heat transfer intake+exhaust system/2000{\_}Bood{\_}The Effect of Knock on the Heat Transfer in an SI Engine.pdf:pdf},
journal = {SAE Tech. Pap.},
number = {2000-01-2831},
title = {{The Effect of Knock on the Heat Transfer in an SI Engine: Thermal Boundary Layer Investigation using CARS Temperature Measurements and Heat Flux Measurements}},
url = {http://dx.doi.org/10.4271/2000-01-2831},
year = {2000}
}
@article{Horstemeyer1999,
abstract = {A phenomenological void–crack nucleation model for ductile metals with secondphases is described which is motivated from fracture mechanics and microscale physicalobservations. The void–crack nucleation model is a function of the fracture toughness of theaggregate material, length scale parameter (taken to be the average size of the second phaseparticles in the examples shown in this writing) , the volume fraction of the second phase, strainlevel, and stress state. These parameters are varied to explore their effects upon the nucleationand damage rates. Examples of correlating the void–crack nucleation model to tension data in theliterature illustrate the utility of the model for several ductile metals. Furthermore, compression,tension, and torsion experiments on a cast Al–Si–Mg alloy were conducted to determinevoid–crack nucleation rates under different loading conditions. The nucleation model was thencorrelated to the cast Al–Si–Mg data as well.},
author = {Horstemeyer, Mark F. and Gokhale, Arun M.},
doi = {10.1016/S0020-7683(98)00239-X},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Plasticity models/A void crack nucleation model for ductile metals with or without inclusions{\_}HorstemeyerAndGokhale.pdf:pdf},
isbn = {00207683 (ISSN)},
issn = {00207683},
journal = {Int. J. Solids Struct.},
pages = {5029--5055},
pmid = {111},
title = {{A Void-Crack Nucleation Model for Ductile Metals}},
volume = {36},
year = {1999}
}
@article{Thornton2002,
author = {Thornton, Colin and I, David Kafui},
pages = {178--182},
title = {{Discrete Element Methods}},
year = {2002}
}
@article{Wirkrichtungswinkel1836,
author = {Wirkrichtungswinkel, K},
pages = {329--372},
title = {{Drehen und Grundbegriffe der Zerspantechnik}},
year = {1836}
}
@article{Essmann1979a,
abstract = {It is proposed that, during dislocation glide at low temperatures, both screw and non-screw dislocations annihilate mutually with dislocations of opposite sign approaching on closely neighbouring glide planes. The experimental evidence is summarized and possible mechanisms are discussed. Phenomenological models of dislocation accumulation during deformation, taking into account the annihilation of dislocations, are formulated. The analysis of selected examples of tensile and cyclic deformation of f. c. c. and b. c. c. metal crystals demonstrates that annihilation of edge and/or screw dislocations occurs during strain hardening and can lead to steady-state deformation. It follows that the dislocation densities introduced during deformation cannot exceed well-defined upper limits that are distinctly lower than the hypothetical upper limits estimated for the static case. The observations suggest that the critical spacings of dislocation pairs that annihilate are similar 50-500 nm for screw and similar 1. 6 nm for edge dislocations (in copper). The atomic concentration of point defects formed by the annihilation of non-screw dislocations is found to be low in most cases. However, it is concluded that, in the dislocation-rich walls of persistent slip bands in fatigued copper, a rather high concentration of point defects prevails.},
author = {Essmann, U. and Mughrabi, H.},
doi = {10.1080/01418617908234871},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/2006{\_}Mughrabi + Essmann{\_}Annihilation of dislocations   during tensile and cyclic deformation and limits of dislocation   densities.pdf:pdf},
isbn = {0141-8610},
issn = {0141-8610},
journal = {Philos. Mag. A},
number = {6},
pages = {731--756},
title = {{Annihilation of dislocations during tensile and cyclic deformation and limits of dislocation densities}},
url = {http://www.tandfonline.com/doi/abs/10.1080/01418617908234871},
volume = {40},
year = {1979}
}
@article{Zienkiewicz2013c,
abstract = {This chapter describes the use of a patch of one or more elements to assess convergence of a finite element solution to that of the differential equation it approximates. The requirements are presented by a consistency and stability test on the resulting matrix problem. For elements which are numerically integrated or otherwise explicitly stated the stability test requires that the stiffness matrix of a structural problem or the conductivity matrix of a quasi-harmonic problem has proper rank. This requires the number of quadrature points to be equal or larger to some minimum value. Use of less than the minimum number is called reduced integration. Consistency requires the finite element solution to exactly represent all the derivatives up to the highest order that exists in a weak or variational expression for the problem. The chapter presents alternative methods to asses the two requirements. The patch test is an essential test to both test accuracy of the computer program used to solve problems as well as to validate formulations that violate the standard rules described in previous chapters. One such case of a non-conforming element is presented in the chapter.},
author = {Zienkiewicz, O.C. and Taylor, R.L. and Zhu, J.Z.},
doi = {10.1016/B978-1-85617-633-0.00008-3},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Zienkiewicz FEM - Vol 1 Basics Fundamentals/63205{\_}09.pdf:pdf},
isbn = {9781856176330},
issn = {00295981},
journal = {Finite Elem. Method its Basis Fundam.},
pages = {257--284},
title = {{The Patch Test, Reduced Integration, and Nonconforming Elements}},
url = {http://linkinghub.elsevier.com/retrieve/pii/B9781856176330000083},
year = {2013}
}
@article{Geologie2009,
author = {Geologie, Allgemeine},
doi = {10.1007/978-3-540-92940-6},
isbn = {9783540929406},
pages = {1--36},
title = {{Kapitel 10}},
year = {2009}
}
@article{Tabellenb,
author = {Tabellen, Die and Zahlenwerte, Tabelle and Gau{\ss}, Der},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Empirical Fatigue Models + Validation/Betriebsfestigkeit{\_}ErwinHaibach/Kap5 Anhang.pdf:pdf},
title = {{5 Anhang Daten zu statistischen Verfahren}}
}
@article{Gleichstromkreis,
author = {Gleichstromkreis, Leistungsmessung and Ui, P},
doi = {10.1007/978-3-642-22609-0},
isbn = {9783642226090},
title = {{Messung der elektrischen Leistung}}
}
@article{Seidl1998,
author = {Seidl, Anton L},
journal = {Compos. Struct.},
title = {{Adhesively Bonded Aircraft Structures}},
year = {1998}
}
@article{Schweißen1990,
author = {Schwei{\ss}en, Das F{\"{u}}geverfahren},
title = {{3 F{\{}{\"{u}}{\}}gen 3.1}},
year = {1990}
}
@book{Course2006,
author = {Course, First},
booktitle = {Engineering},
doi = {10.1002/9780470510858},
isbn = {9780470035801},
title = {{First Course in Finite Elements}},
year = {2006}
}
@article{Battjes2001,
author = {Battjes, Jurjen A.},
issn = {02748096},
title = {{Short Waves}},
year = {2001}
}
@article{Hettinger2009,
abstract = {It is a well known fact that indicated efficiency of a SI engine at WOT is predominantly limited by knock occurrence. Therefore many investigations have been carried out to avoid knocking. Considering the further development of downsized engines knocking will also pose a greater challenge. Not only knocking but also irregular combustion in general will require further investigation in supercharged SI eingines. Premature ignition, for instance, hasn't yet been completely understood and therefore limits the low end torque of supercharged SI engines.The purpose of this paper is to introduce different analysis methods which allow to identify the knock onset and the knocking zones in the combustion chamber. In addition to established methods new techniques have been developed to account for the complex nature of pressure oscillation during knocking combustion.Experimental data was acquired on a single cylinder research engine to validate the methodology using six pressure transducers.},
author = {Hettinger, Alexander and Kulzer, Andr{\'{e}}},
doi = {10.4271/2009-01-0698},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2009{\_}Hettinger+Kulzer{\_}A new method to detect Knocking Zones.pdf:pdf},
isbn = {2009010698},
issn = {1946-3944},
journal = {SAE Int. J. Engines},
number = {1},
pages = {2009--01--0698},
title = {{A New Method to Detect Knocking Zones}},
url = {http://papers.sae.org/2009-01-0698/},
volume = {2},
year = {2009}
}
@book{Wishington2012,
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Wishington, D C},
booktitle = {Bioinforma. Biomed. Eng. 2008. ICBBE 2008. 2nd Int. Conf.},
doi = {10.1002/ejoc.201200111},
eprint = {arXiv:1011.1669v3},
isbn = {3082342418},
issn = {0196-6553},
pages = {7--58},
pmid = {26840611},
title = {{Table of of contents}},
year = {2012}
}
@book{Fox1918a,
author = {Fox, P J},
booktitle = {Science (80-. ).},
doi = {10.1126/science.49.1254.44},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Thermodynamik/M{\"{u}}llerAndNoll{\_}Thermodynamik/Noll 1974 Mechanics and Thermodynamics{\_}SelectedPapers.pdf:pdf},
isbn = {9783642658198},
issn = {0036-8075},
number = {1240},
pages = {343--345},
pmid = {17811888},
title = {{the Foundations of Mechanics.}},
volume = {48},
year = {1918}
}
@article{Bohlke2012,
author = {B{\"{o}}hlke, Prof Thomas},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/{\_}skripte/Boehlke 2011 p{\_}skript{\_}htf{\_}ws{\_}2011{\_}2012{\_}Endversion.pdf:pdf},
journal = {Mechanik},
number = {September},
title = {{Skript zur Vorlesung H{\"{o}}here Technische Festigkeitslehre}},
year = {2012}
}
@book{Riccardella1992a,
author = {Riccardella, P C and Deardorff, A F and Griesbach, T J},
booktitle = {Adv. Fatigue Lifetime Predict. Tech.},
doi = {10.1520/STP1122-EB},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Neuer Ordner/Advances in fatigue lifetime predictive techniques Part1.pdf:pdf},
isbn = {978-0-8031-1423-4},
issn = {00660558},
keywords = {FATIGUE,MONITORING,POWER PLANTS,PRESSURE VESSELS AND PIPING,THERMAL STRESSES},
pages = {460--473},
pmid = {11439068},
title = {{Advances in Fatigue Lifetime Predictive Techniques}},
url = {https://apps.webofknowledge.com/full{\%}7B{\_}{\%}7Drecord.do?product=UA{\%}7B{\&}{\%}7Dsearch{\%}7B{\_}{\%}7Dmode=GeneralSearch{\%}7B{\&}{\%}7Dqid=11{\%}7B{\&}{\%}7DSID=Z1UxbH6jtsqo8n9kPQr{\%}7B{\&}{\%}7Dpage=1{\%}7B{\&}{\%}7Ddoc=1},
volume = {1122},
year = {1992}
}
@article{Pahl2007a,
author = {Pahl, Gerhard and Beitz†, Wolfgang and Feldhusen, J{\"{o}}rg and Grote, Karl-H.},
journal = {Pahl/Beitz Konstr. - Grundlagen},
title = {{Rechnerunterst{\"{u}}tzung}},
year = {2007}
}
@article{Metallplastizit2013,
author = {Metallplastizit, Hrungdie and Helm, Dirk},
number = {November},
pages = {1--29},
title = {{Prozesssimulation in Der Umformtechnik}},
year = {2013}
}
@article{Weertman1955,
abstract = {A theory of steady-state creep is developed using Mott's mechanism of dislocation climb. It is assumed in the analysis that the rate-controlling process is the diffusion of vacancies between dislocations which are creating vacancies and those which are destroying them. The concentration of vacancies along a dislocation line is determined by setting the change in the free energy caused by a decrease or increase in the number of vacancies equal to the change in the elastic energy occuring during dislocation climb. The creep equation that results from the analysis is creep rate=const (o-{\textless}Y./kT)exp(-Q/kT) where" is a constant ("",3 to 4), Q is the activation energy of self-diffusion, kT has its usual meaning, and 0- to 108 is the stress. This equation is valid in the stress range from the critical shear stress to a stress about equal to 10' dynes/cm'. At larger stresses the creep rate increases much more rapidly with stress.},
author = {Weertman, J.},
doi = {10.1063/1.1721875},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Kriechen{\_}Spannungsrelaxation/1955{\_}Weertman{\_}Theory of Steady-State Creep Based on Dislocation Climb.pdf:pdf},
isbn = {0021-8979},
issn = {00218979},
journal = {J. Appl. Phys.},
number = {10},
pages = {1213--1217},
title = {{Theory of steady-state creep based on dislocation climb}},
volume = {26},
year = {1955}
}
@article{Energie1997,
author = {Energie, Mit Der Beherrschung Der},
pages = {2--4},
title = {{1 Einleitung}},
year = {1997}
}
@inproceedings{Burkhard2014,
author = {Burkhard, James F},
booktitle = {SAE Tech. Pap. 2014-01-1167},
doi = {10.4271/2014-01-1167},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Thermal Coating + Water Heat Transfer + Applikation/2014{\_}Burkhard{\_}Individual Cylinder Fuel Control for a Turbocharged Engine.pdf:pdf},
publisher = {SAE International},
title = {{Individual Cylinder Fuel Control for a Turbocharged Engine}},
year = {2014}
}
@article{Lin1969b,
abstract = {The mechanics of the build-up of large local plastic strains at the free surface of a polycrystal under fatigue loading is shown. Two closely located thin slices in a most-favourably-oriented crystal located at a free surface of the polycrystal are assumed to have an initial resolved shear stress of a few psi of opposite sign. Under cyclic loading, the two thin slices slide in opposite directions, one during the forward loading and the other during the reversed loading. Based on the dependency of slip on the resolved shear stress, the increase of local plastic strain in the slices with cycles of loading is calculated by applying the analogy between plastic strain and external force. The calculated local plastic shear strain in both slices (one positive and the other negative) reaches 100 per cent at the free surface in a few hundred cycles. These large plastic shear strains clearly cause the start of an extrusion or intrusion and the nucleation of a fatigue crack.},
author = {Lin, T H and Ito, Y M},
doi = {doi: DOI: 10.1016/0022-5096(69)90006-4},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/1969{\_}Lin{\_}Mechanics of a fatigue crack nucleation mechanism.pdf:pdf},
isbn = {0022-5096},
issn = {0022-5096},
journal = {J. Mech. Phys. Solids},
pages = {511--523},
title = {{Mechanics of a Fatigue Crack Nucleation Mechanism}},
url = {http://www.sciencedirect.com/science/article/pii/0022509669900064},
volume = {17},
year = {1969}
}
@article{Journal2008a,
author = {Journal, American and Sciences, Applied and Publications, Science},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Heat transfer intake+exhaust system/2008{\_}Semin+Ismail{\_}Heat Transfer Investigation of Intake Port Engine Based on Steady-State and Transient Simulation.pdf:pdf},
keywords = {compression ignition engine,computational model,heat transfer,intake port,simulation},
number = {11},
pages = {1572--1579},
title = {{Heat Transfer Investigation of Intake Port Engine Based on Steady-State and Transient Simulation Semin , 2 Abdul Rahim Ismail , 2 Rosli Abu Bakar and 2 Ismail Ali Institute of Technology Sepuluh Nopember , Surabaya 60111 , Indonesia Faculty of Mechanical }},
volume = {5},
year = {2008}
}
@article{Popping2012a,
author = {P{\"{o}}pping, K},
isbn = {9783844021653},
issn = {1861-0595},
journal = {D-Nb.Info},
title = {{Diese Dissertation ist auf den Internetseiten der Hochschulbibliothek online verf{\{}{\"{u}}{\}}gbar.}},
url = {http://d-nb.info/985390468/34},
year = {2012}
}
@article{Growth1988,
author = {Growth, Part},
number = {March},
title = {{Continuum Damage Mechanics :}},
volume = {55165},
year = {1988}
}
@article{Verbrennungsvorgang,
author = {Verbrennungsvorgang, Jeder},
journal = {Betrieb},
pages = {213--242},
title = {{9 Abgasemissionen und Schadstoffreduzierung}}
}
@article{Stresses1988,
author = {Stresses, Residual and Energy, Stored Elastic},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/1990{\_}Kreher{\_}Residual stresses and stored elastic energy of composites and polycrystals.pdf:pdf},
title = {{RESIDUAL STRESSES AND STORED ELASTIC ENERGY Of: {\~{}}U{\~{}}P{\~{}}S{\~{}}TES AND PULYCRYSTALS}},
year = {1988}
}
@article{Dynamics,
author = {Dynamics, Computational Fluid},
pages = {443--482},
title = {{12 Dreidimensionale Str{\"{o}}mungsfelder}}
}
@article{Agarwal2006,
abstract = {Thermal loading of diesel engine pistons has increased dramatically in recent years owing to applications of various technologies to meet low emission and high power density requirements. Control of piston temperatures by cooling of these pistons has become one of the determining factors in a successful engine design. The pistons are cooled by oil jets fired at the underside from the crankcase. Any excessive piston temperature rise may lead to engine seizure because of piston warping. However, if the temperature at the underside of the piston, where the oil jet strikes the piston, is above the boiling range of the oil being used, it may contribute to the generation of mist. This mist significantly contributes to the non-tailpipe emissions in the form of unburnt hydrocarbons (UBHCs). The problem of non-tailpipe emissions has unfortunately not been looked into so seriously, as the current stress of all automobile manufacturers is to meet the tailpipe emission legislative limits.A numerical model has been developed using finite element methods for studying the oil jet cooling of pistons and has been validated experimentally on a flat plate cooled by oil jet. Using numerical modelling, the heat transfer coefficient (h) at the underside of the piston is predicted. This predicted value of heat transfer coefficient significantly helps in selecting the correct oil type, oil jet velocity, oil jet diameter, and distance of oil nozzle from the underside of the piston. It also helps to predict whether the selected grade of oil will contribute to mist generation. Isotherms of the predicted temperature profiles in a production grade piston have been plotted.},
author = {Agarwal, A K and Varghese, M B},
doi = {10.1243/14680874JER01804},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/W{\"{a}}rme-RBen Kolben/2004{\_}Varghese{\_}Numerical investigation of piston cooling using oil jet.pdf:pdf},
issn = {1468-0874},
journal = {Int. J. Engine Res.},
number = {5},
pages = {411--421},
title = {{Numerical investigations of piston cooling using oil jet in heavy duty diesel engines}},
url = {http://journals.sagepub.com/doi/10.1243/14680874JER01804},
volume = {7},
year = {2006}
}
@article{Lin1989,
author = {Lin, T H and Lin, S R and Wu, X Q},
doi = {10.1080/01418618908221174},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/1989{\_}Lin{\_}Micromechanics of an extrusion in high-cycle fatigue.pdf:pdf},
issn = {0141-8610},
journal = {Philos. Mag. A},
number = {6},
pages = {1263--1276},
title = {{Micromechanics of an extrusion in high-cycle fatigue}},
url = {http://www.tandfonline.com/doi/abs/10.1080/01418618908221174},
volume = {59},
year = {1989}
}
@book{Flaceliere2007a,
author = {Flaceliere, L. and Morel, F. and Dragon, A.},
booktitle = {Int. J. Damage Mech.},
doi = {10.1177/1056789506067935},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/2 scale models papers/2007{\_} Flaceliere+Morel+Dragon{\_}Coupling Between Mesoplasticity and Damage in HCF{\_}MitViskoEffekte.pdf:pdf},
isbn = {1056789506},
issn = {1056-7895},
keywords = {author to whom correspondence,damage model,e-mail,ensma,experiment,flaceliere,fr,lmpm,mesoplasticity,multiaxial fatigue,should be addressed},
number = {4},
pages = {473--509},
title = {{Coupling Between Mesoplasticity and Damage in High-cycle Fatigue}},
volume = {16},
year = {2007}
}
@article{Hartmann1997,
abstract = {This paper deals with two main topics. The first one concerns the equivalence of stress algorithms, based on a Backward-Euler-step applied on viscoplastic models of Chaboche-type, and their elastoplastic counter- part. Generally, the stress algorithm yields a system of non-linear algebraic equations and the corresponding consistent tangent operator, occurring in the principle of virtual displacements, leads to a system of linear equations. This procedure can be obtained utilizing only numerical methods. The second topic concerns a special constitutive relation based on a kinematic hardening model using a sum of Armstrong/Frederick terms, which is equivalent to a multi-surface plasticity model. Applying this model a so-called problem- adapted stress algorithm is derived, where only one non-linear equation must be solved. This result is independent of the number of terms in the hardening model. Furthermore, only the viscoplastic algorithm must be implemented, since it includes the elastoplastic constitutive model as a special case.},
author = {Hartmann, Stefan and L{\"{u}}hrs, Georg and Haupt, Peter},
doi = {10.1002/(SICI)1097-0207(19970330)40:6<991::AID-NME98>3.0.CO;2-H},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Numerik UMATS FE-Codes/1997{\_}Hartmann{\_}AN EFFICIENT STRESS ALGORITHM WITH APPLICATIONS IN VISCOPLASTICITY AND PLASTICITY.pdf:pdf},
issn = {0029-5981},
journal = {Int. J. Numer. Methods Eng.},
keywords = {finite elements,kinematic hardening,plasticity,stress algorithm,viscoplasticity},
number = {6},
pages = {991--1013},
title = {{an Efficient Stress Algorithm With Applications in Viscoplasticity and Plasticity}},
url = {http://doi.wiley.com/10.1002/(SICI)1097-0207(19970330)40:6{\%}3C991::AID-NME98{\%}3E3.0.CO;2-H{\%}5Cnhttp://doi.wiley.com/10.1002/(SICI)1097-0207(19970330)40:6{\%}3C991::AID-NME98{\%}3E3.0.CO;2-H},
volume = {40},
year = {1997}
}
@article{Arnold,
author = {Arnold, J{\"{o}}rg},
pages = {793--800},
title = {{C6 C6 Gl{\"{u}}hlampen C6 Untersuchungen von Gl{\"{u}}hlampen}}
}
@article{Energiewandlung,
author = {Energiewandlung, Einzelprozesse},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/Motoren/Golloch{\_}Downsizing/chp{\_}10.1007{\_}3-540-27490-1{\_}2.pdf:pdf},
title = {{2 Energieumsetzung im Verbrennungsmotor}}
}
@article{Verbrennungsgase,
author = {Verbrennungsgase, Die and Gasturbinen, Mit and Abgasturbolader, Als},
title = {{4 Gasturbinen}}
}
@article{Chaboche1989,
abstract = {The cyclic constitutive equations developed and used at ONERA and LMT-Cachan are presented in detail in terms of a hierarchy of various models. Both the time-independent and the viscoplasticity versions of the equations are discussed, as well as their ability to describe correctly most of the experimentally observed effects under monotonic or cyclic loading, constant or variable temperature, including strain hardening and time recovery effects. The reported experimental data concerns stainless steels and have been published previously. Four other theories are then presented and compared in a systematic way. They include the Ohno-Kachi time-independent plasticity theory, two unified viscoplastic models by Walker and by Krempl and Yao, the new developments of the endochronic theory by Watanabe and Atluri. All these approaches show some similarities with the first one, especially in that concerns the non.linearity of kinematic hardening, which represents the key for describing the cyclic behav- iour of metallic materials.},
author = {Chaboche, J L},
doi = {http://dx.doi.org/10.1016/0749-6419(89)90015-6},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/Hardening Recovery Creep/1989{\_}Chaboche{\_}Constitutive equations for cyclic plasticity and cyclic viscoplasticity.pdf:pdf},
isbn = {1111111111},
issn = {0749-6419},
journal = {Int. J. Plast.},
pages = {247--302},
title = {{Constitutive equations for cyclic plasticty and cyclic viscoplasticity}},
volume = {5},
year = {1989}
}
@article{Fourier-transformation,
author = {Fourier-transformation, Technik Der},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Mathematik/fourier{\_}{\_}transformation{\_}{\_}university{\_}muenster.pdf:pdf},
title = {{Technik der Fourier-Transformation}}
}
@article{Zusammenh,
author = {Zusammenh, Die and Entwicklung, Die},
journal = {Auslegung A Grad. J. Philos.},
pages = {117--150},
title = {{4 Einspritzsysteme und System{\{}{\"{u}}{\}}bersicht}}
}
@book{Zheng-Ping2013,
abstract = {In this paper, the Turing instability in reaction-diffusion models defined on complex networks is studied. Here, we focus on three types of models which generate complex networks, i.e. the Erd{\$}\backslash{\$}H{\{}{\{}{\}}o{\{}{\}}{\}}s-R{\$}\backslash{\$}'enyi, the Watts-Strogatz and the threshold network models. From analysis of the Laplacian matrices of graphs generated by these models, we reveal that the stable-unstable regions of a spatially homogeneous solution completely differ, depending on network structures. In particular, we approximately argue the existence of the stable-unstable regions in the cases of regular enhanced ring lattices which include regular circles, and networks generated by the threshold network model when the number of vertices is large enough.},
archivePrefix = {arXiv},
arxivId = {1406.6401},
author = {Zheng-Ping, Fu and Xin-Hang, Xu and Hong-Li, Wang and Qi, Ouyang and Yang, Lingfa and Zhabotinsky, Anatol M and Epstein, Irving R and Wiggins, L Sirovich S and Toole, Gregory and Hurdal, Monica K and Cogan, Nick and Shi, Junping and Search, Home and Journals, Collections and Contact, About and Iopscience, My and Rozhnova, G and Nunes, a. and McKane, Alan J and Page, Karen and Maini, Philip K and a.M. Monk, Nicholas and Li, Qian Shu and Ji, Lin and Levine, Herbert and Rappel, Wouter Jan and Kumar, Niraj and Horsthemke, Werner and Kov{\'{a}}cs, S{\'{a}}ndor and Judd, Stephen L and Silber, Mary and Ide, Yusuke and Izuhara, Hirofumi and Machida, Takuya and Hori, Yutaka and Guiu-Souto, Jacobo and Carballido-Landeira, Jorge and P{\'{e}}rez-Villar, Vicente and Mu{\~{n}}uzuri, Alberto P and Gambino, G and Lombardo, M C C and Sammartino, M and Fanelli, Duccio and Cianci, Claudia and {Di Patti}, Francesca and Cao, Yang and Erban, Radek and Cantini, Laura and Massi, Emma and Barletti, Luigi and Biancalani, Tommaso and Bhattacharyay, a. and Berenstein, Igal and Dolnik, Milos and Asslani, Malbor and Asllani, Malbor and Busiello, Daniel M and Carletti, Timoteo and Planchon, Gwendoline and Access, Open},
booktitle = {Phys. Rev. E - Stat. Nonlinear, Soft Matter Phys.},
doi = {10.1016/j.camwa.2013.03.019},
eprint = {1406.6401},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/Strukturmechanik MMS/Literatur/Mikromechanik{\_}B{\"{u}}cher{\_}Literaturvorschlag{\_}MMS/Torquato 2002 RHM.pdf:pdf},
isbn = {4420767936},
issn = {1539-3755},
keywords = {05c82,1,2010 msc,35k57,60g05,60j60,70k50,92c15,92c40,Amplitude equation,Cortical folding,Cross diffusion,Ginzburg-Landau equation,Growing domain,Linearised stability,Morphology,Nonlinear diffusion,Pattern formation,Quintic Stuart-Landau equation,Reaction-diffusion system,Turing bifurcation,Turing system,activator,ams subject classifications,and another for inhibitor,and diffusion,approaches to the mathematical,based,clo,compartment-based models,complex network,cross-diffusion,cross-diffusion systems,deterministic models which are,diffusion models,diffusion system,epstein,growing domain,holling type-ii functional response,i,instability,introduction,le,lengyel,model,modelling of chemical reactions,non-constant positive steady state,pattern,pattern formation,reaction,reaction-diffusion,reaction-diffusion models on networks,reaction-diffusion processes,reaction-diffusion systems,self-organised spatial pattern,stationary patterns,stochastic processes,stochastic simulations,stochastic turing patterns,systems,there are two fundamental,turing instability,turing pattern,turing reaction,turing system},
number = {4},
pages = {476},
pmid = {15267983},
title = {{Interdisciplinary Applied Mathematics}},
url = {http://link.springer.com/10.1140/epjb/e2013-40570-8{\%}7B{\%}25{\%}7D5Cnhttp://arxiv.org/abs/1406.6401{\%}7B{\%}25{\%}7D5Cnhttp://arxiv.org/abs/1204.1475{\%}7B{\%}25{\%}7D5Cnhttp://link.aps.org/doi/10.1103/PhysRevLett.91.058302{\%}7B{\%}25{\%}7D5Cnhttp://arxiv.org/abs/nlin/0111059{\%}7B{\%}25{\%}7D5},
volume = {82},
year = {2013}
}
@article{Spannungszustand,
author = {Spannungszustand, Einachsiger and Spannungszustand, Ebener},
pages = {215--246},
title = {{A a a a}}
}
@article{Verbrennungsmotoren2012,
author = {Verbrennungsmotoren, Grundlagen},
doi = {10.1007/978-3-8348-1988-8},
isbn = {9783834819888},
pages = {453--478},
title = {{Ph{\"{a}}nomenologische Verbrennungsmodelle}},
year = {2012}
}
@article{SMA2000,
author = {SMA},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fatigue{\_}Folien{\_}Ueberblick{\_}Standardgesetze.pdf:pdf},
pages = {35},
title = {{Fatigue: Total Life Approaches}},
year = {2000}
}
@article{Rothe2006,
abstract = {A general definition and an index for the assessment of different engine knock behavior have been developed. The knock onset locations have been determined by piezoresistive pressure actuators and optical fiber probes in full load engine operation mode. The thermodynamic conditions at the knock onset locations have been quantified by CFD-calculations. Therefore the local fuel concentration, mixture temperature and residual gas concentration have been considered. These calculated thermodynamic conditions were further used to calculate the necessary volume of an exothermal center for the generation of the maximal measured pressure amplitudes.},
author = {Rothe, M. and Heidenreich, T. and Spicher, U. and Schubert, Alexander},
doi = {10.4271/2006-01-0225},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Klopfen{\_}Ottomotor/2006{\_}Rothe{\_}Knock Behavior of SI-Engines - Thermodynamic Analysis of Knock Onset Locations and Knock Intensitiespdf.pdf:pdf},
issn = {0148-7191},
title = {{Knock Behavior of SI-Engines: Thermodynamic Analysis of Knock Onset Locations and Knock Intensities}},
url = {http://papers.sae.org/2006-01-0225/},
year = {2006}
}
@article{Jammoussi2017,
author = {Jammoussi, Hassene and Makki, Imad and Kluzner, Michael and Jentz, Robert},
doi = {10.4271/2017-01-1684},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Thermal Coating + Water Heat Transfer + Applikation/2017{\_}Jammoussi+Makki{\_}Diagnostics of Individual Air Fuel Ratio Cylinder Imbalance.pdf:pdf},
journal = {SAE Int. J. Passeng. Cars -Electron. Electr. Syst.},
number = {2},
pages = {400--404},
title = {{Diagnostics of Individual Air Fuel Ratio Cylinder Imbalance}},
volume = {10},
year = {2017}
}
@article{Ermittlung,
author = {Ermittlung, Die and Charakterisierung, Die and Charakterisierung, Zur},
title = {{5 Me{\ss}fehler}}
}
@article{Soyhan2009a,
abstract = {Combustion in HCCI engines is a controlled auto-ignition of well-mixed fuel, air and residual gas. The thermal conditions of the combustion chamber are governed by chemical kinetics strongly coupled with heat transfer from the hot gas to the walls. The heat losses have a critical effect on HCCI ignition timing and burning rate, so it is essential to understand heat transfer process in the combustion chamber in the modeling of HCCI engines. In the present paper, a comparative analysis is performed to investigate the performance of well-known heat transfer correlations in an HCCI engine. The results from the existing correlations are compared with the experimental results obtained in a single-cylinder engine. Significant differences are observed between the heat transfer results obtained by using Woschni, Assanis and Hohenberg correlations. {\textcopyright} 2008 Elsevier Ltd. All rights reserved.},
author = {Soyhan, H. S. and Yasar, H. and Walmsley, H. and Head, B. and Kalghatgi, G. T. and Sorusbay, C.},
doi = {10.1016/j.applthermaleng.2008.03.014},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Heat Transfer Combustion Chamber/2008{\_}Soyhan{\_}Evaluation of heat transfer correlations for HCCI engine modeling.pdf:pdf},
isbn = {1359-4311},
issn = {13594311},
journal = {Appl. Therm. Eng.},
keywords = {HCCI,Heat transfer correlations,Modeling,Ricardo Hydra engine},
number = {2-3},
pages = {541--549},
publisher = {Elsevier Ltd},
title = {{Evaluation of heat transfer correlations for HCCI engine modeling}},
url = {http://dx.doi.org/10.1016/j.applthermaleng.2008.03.014},
volume = {29},
year = {2009}
}
@article{Pr,
author = {Pr, Diese and Ermitteln, Das},
title = {{7 Reifenpr{\"{u}}fungen}}
}
@article{Tanaka1981,
abstract = {The effects of grain size and crack length on the threshold condition of fatigue growth of small cracks are analysed both theoretically and experimentally. The theoretical model is based on the assumption that the threshold condition is determined by whether the crack-tip slip band blocked by the grain boundary propagates into an adjacent grain or not. By comparing the model analysis with the experiments of mild steel, it was found that the threshold stress estimated from the fatigue limit of the smooth specimen gave the effective components of the applied stress. When the threshold stress normalized by the fatigue limit of the smooth specimen was correlated to the crack length normalized by a certain crack length, the theoretical relation was found to agree well with the experimental data. From a further analysis of the published data of various materials, the theoretical normalized relation was found to give a lower bound of the threshold values of the stress and the stress intensity factor. A deviation from the theoretical relation seen in the cases of hard metals was explained through an extension of the model by regarding that hard metals contained initial, inherent flaws even in the smooth specimen.},
author = {Tanaka, K and Nakai, Y and Yamashita, M},
doi = {10.1007/BF00033345},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/1981{\_}Tanaka{\_}Fatigue growth threshold of small cracks.pdf:pdf},
isbn = {0376-9429},
issn = {03769429},
journal = {Int. J. Fract.},
number = {5},
pages = {519--533},
title = {{Fatigue growth threshold of small cracks}},
volume = {17},
year = {1981}
}
@article{Haslam2013b,
author = {Haslam, Antony and Laskaridis, Panos},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2010{\_}Jaroslav Pokluda+Pavel {\v{S}}andera{\_}Micromechanisms of fracture and fatigue{\_}Buch/Kap4{\_}FatigueFracture.pdf:pdf},
title = {{Fatigue {\{}{\&}{\}} Fracture}},
year = {2013}
}
@article{Wallentowitz2006b,
author = {Wallentowitz, Henning and Reif, Konrad},
doi = {10.1007/978-3-8348-9121-1},
isbn = {978-3-528-03971-4},
journal = {Handb. Kraftfahrzeugelektronik},
pages = {40},
title = {{15 Elektromagnetische Vertr{\"{a}}glichkeit}},
url = {http://www.springerlink.com/index/10.1007/978-3-322-82991-7{\%}5Cnhttp://www.springerlink.com/index/10.1007/978-3-8348-9121-1},
year = {2006}
}
@misc{Qi1999a,
author = {Qi, W and Bertram, A},
booktitle = {Int. J. Plast.},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Plasticity models/Anisotropic continuum damage modeling for single crystals at high temperatures{\_}QiAndBertram.pdf:pdf},
pages = {1197--1215},
title = {{Anisotropic continuum damage modeling for single crystals at high temperatures}},
volume = {15},
year = {1999}
}
@article{Mousavi2016,
abstract = {{\textcopyright} 2016 Springer Science+Business Media DordrechtThe in-plane classical dislocation-based linear elastic fracture mechanics analysis is extended to the case of strain gradient elasticity. Nonsingular stress and smooth-closure crack profiles are derived. As in the classical treatment, the crack is represented by a distribution of climb edge dislocations (for Mode I) or glide edge dislocations (for mode II). These distributions are determined through the solution of corresponding integral equations based on variationally consistent boundary conditions. An incompatible framework is used and the nonsingular full-field plastic distortion tensor components are calculated. Numerical results and related graphs are provided illustrating the nonsingular behaviour of the stress/strain components and the smooth cusp-like closure of the crack faces at the crack tip. The work provides an alternative approach to celebrated “Barenblatt's treatment” of cracks, without the introduction of a cohesive zone and related to intermolecular forces ahead of the physical crack tip. It also supplements a recent paper by the authors in which the mode III crack, represented by an array of screw dislocations, was solved within the present gradient elasticity framework.},
author = {Mousavi, S. Mahmoud and Aifantis, Elias C.},
doi = {10.1007/s10704-016-0143-5},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/2016{\_}Mousavi{\_}Dislocation-based gradient elastic fracture mechanics.pdf:pdf},
issn = {15732673},
journal = {Int. J. Fract.},
keywords = {Crack tip plasticity,Gradient elasticity,Nonsingular cracks,Nonsingular dislocations},
number = {1},
pages = {93--110},
title = {{Dislocation-based gradient elastic fracture mechanics for in-plane analysis of cracks}},
volume = {202},
year = {2016}
}
@article{Konzepte,
author = {Konzepte, Downsizing- and Steigerung, Eine and Gegensatz, Im and Geschwindigkeit, Die},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/Motoren/Golloch{\_}Downsizing/chp{\_}10.1007{\_}3-540-27490-1{\_}3.pdf:pdf},
title = {{3 Downsizing}}
}
@article{Hill1931,
author = {Hill, Constraint},
doi = {http://dx.doi.org/10.1016/B978-012566251-2/50019-8},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Atomistic and Continuum Modeling of Nanocrystalline Materials/back-matter.pdf:pdf},
isbn = {978-0-12-566251-2},
issn = {1076-1608},
journal = {J. Physiol.},
pages = {1--58},
title = {{Subject Index}},
volume = {71},
year = {1931}
}
@book{Chakrabarty2006,
abstract = {During recent years, there has been considerable interest in the application of the macroscopic theory of plasticity to engineering problems associated with structural designs and the technological forming of metals. The need for a comprehensive text book on plasticity, incorporating the most recent developments of the subject, has been strongly felt for some years. This book has been written primarily to meet the needs of graduate and research students of Mechanical, Civil, and Metallurgical Engineering, although some of the material in the book is also suitable for under- graduate students and practicing engineers. In order to discuss the various topics as fully as possible, it has been found necessary to treat the subject matter in two volumes, of which the first one is now presented to the reader. The},
author = {Chakrabarty, J},
doi = {10.1016/B978-0-7506-6638-1.50006-6},
isbn = {0750666382},
issn = {02321300},
pages = {896},
title = {{Theory of plasticity}},
url = {http://books.google.com/books?hl=en{\&}lr={\&}id=uMcID-tu-8YC{\&}oi=fnd{\&}pg=PP2{\&}dq=Theory+of+plasticity{\&}ots=dAGJbq6QUZ{\&}sig=-d4jjjFGmrIIlUe1p1XNq63z59s},
year = {2006}
}
@article{Payne2010a,
abstract = {This paper reports the results of a study of the initial stages of fatigue crack formation in the commercial aluminum alloy 7075-T651. Direct observations were made of the evolution of cracking in a notch under moderately high fatigue loads in a scanning electron microscope. The experimental conditions were designed to mimic the behavior of fastener holes in the lower wing covers of military attack aircraft, thus the loading parameters were such that local plasticity was expected. Constituent particle cracking was observed to be the sole cause of fatigue crack initiation in these experiments; particle debonding was not a factor. The iron-bearing constituent particles were the sites of nearly all of the cracks initiated by fatigue. Mg2Si particles were not effective crack initiation sites. This was attributed to the difference in the moduli of the particles: the iron-bearing particles were harder than the matrix while the Mg2Si particles were softer. A large fraction of the cracks in the constituent particles were present before any loading was applied, but a certain amount of additional constituent particle cracking was caused by the fatigue loading. A cracked constituent particle eventually gave rise to a crack in the surrounding matrix, but this process required the application of fatigue loads. No matrix cracks were observed prior to fatigue loading. Subsequent propagation of the matrix cracks also required additional fatigue cycling. These observations are being used in the development of detailed computer models of the fatigue process in 7075-T651. ?? 2009 Elsevier Ltd.},
author = {Payne, Joel and Welsh, Greg and Christ, Robert J and Nardiello, Jerrell and Papazian, John M},
doi = {10.1016/j.ijfatigue.2009.06.003},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/2 scale models papers/2010{\_}Papazian{\_}Observations of fatigue crack initiation in 7075-T651.pdf:pdf},
isbn = {0142-1123},
issn = {01421123},
journal = {Int. J. Fatigue},
keywords = {7075-T651,Aluminum alloy 7075,Crack initiation,Fatigue,Scanning electron microscopy},
number = {2},
pages = {247--255},
publisher = {Elsevier Ltd},
title = {{Observations of fatigue crack initiation in 7075-T651}},
url = {http://dx.doi.org/10.1016/j.ijfatigue.2009.06.003},
volume = {32},
year = {2010}
}
@article{Niedrig,
author = {Niedrig, H and Sternberg, M},
journal = {H{\{}{\"{u}}{\}}tte},
pages = {1--289},
title = {{B-Physik}}
}
@article{Skrotzki,
author = {Skrotzki, B and Simon, F and Materialkreislauf, Der},
journal = {H{\{}{\"{u}}{\}}tte},
pages = {1--110},
title = {{D-Werkstoffe}}
}
@article{Unsymmetrie,
author = {Unsymmetrie, Das Naturgesetz Der},
title = {{5. Die Entropiebilanz}}
}
@article{Begriffe2010,
author = {Begriffe, Die},
doi = {10.1007/978-3-540-89315-8},
isbn = {9783540893158},
title = {{2 Mathematische und kinematische Grundlagen}},
year = {2010}
}
@article{Eindhoven2005,
author = {Eindhoven, Uni and Polystyrene, Isotactic and Press, Academic and Verlag, Shaker},
pages = {272--282},
title = {{Quellennachweis}},
year = {2005}
}
@article{Rostampour2015a,
abstract = {This investigation deals with the EF7 (TC) engine, a dual fuel engine equipped with a turbocharger system, consequently with a high probability of knock inception. In this study, an operating cycle of the engine was simulated using KIVA-3V code. Some modifications were carried out on the KIVA method of calculating pressure in the intake port in order to simulate turbocharger pressure correctly. Auto-ignition and knock were then simulated using the auto-ignition integral model. The modified code and the simulation were verified using three different methods; in-cylinder average pressure, gas temperature of the exhaust port, and auto-ignition timing. The simulation results using the auto-ignition integral model, as compared with the experimental data, proved to be reasonably accurate. Following this validation, the effect of the knock phenomenon on the engine heat transfer through the walls was investigated. The simulations showed that the rate of heat transfer through the walls under knocking conditions is about 2.2 times higher than that under normal conditions. However, it was also shown that the total heat transfer increases about 15{\%}.},
author = {Rostampour, Arman and Toosi, Ali Nassiri},
doi = {10.1115/1.4030517},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2015{\_}Rostampour{\_}Numerical Investigation of the effect of knock on heat transfer in a turbo si engine.pdf:pdf},
issn = {0742-4795},
journal = {J. Eng. Gas Turbines Power},
number = {12},
pages = {121502},
title = {{Numerical Investigation of the Effect of Knock on Heat Transfer in a Turbocharged Spark Ignition Engine}},
url = {http://www.scopus.com/inward/record.url?eid=2-s2.0-84930634240{\&}partnerID=tZOtx3y1},
volume = {137},
year = {2015}
}
@article{Transporteigenschaft,
author = {Transporteigenschaft, Eine},
journal = {Dimens. Contemp. Ger. Arts Lett.},
pages = {47--201},
title = {{Grundlagen der Stromungsmechanik}}
}
@article{Cassis1998,
abstract = {2.1 INTRODUCTION AND HISTORY sored production of styrene-butadiene rubber. Organic polymers are divided into two types, reinforced-thermoplastic and thermoset. With thermoset polymers such as unsaturated poly-esters and vinyl esters, a chemical reaction cross links the material so that it cannot be returned to liquid form. Other common ther-mosetting polymers include epoxy and phenolic resins. Thermoset plastics made with polyester and vinyl ester resins represent the major portion of the reinforced plastic com-posites industry today. Early workers on unsaturated polyesters soon learned that despite the possession of reactive double bonds, these resins were slug-gish in reacting with themselves. Even with effective catalysts, they still required high tem-peratures and lengthy cure times to complete the cross linking reaction. The key to modern day application of unsaturated polyesters was the discovery by Carlton Ellis in 1937l that the addition of reactive monomers, such as styrene, gave mixtures that would copolymerize many times faster than homopolymerization. The styrene addition produced the added benefit of an easily handled liquid material that could be pumped, transported and fabricated into a fin-ished plastic by a myriad of molding processes. Developments during the 1940s accelerated the commercial applicability of unsaturated polyesters to the position they hold today. Styrene became readily available and lower in cost as a result of the US Government's spon-Handbook of Composites. Edited by S.T. Peters. Published in 1998 by Chapman {\&} Hall, London. ISBN 0 412 54020 7 At the same time, scientists found that styre-nated polyesters could yield high strength, light weight structures when reinforced with glass fibers. They also learned that fiberglass-reinforced polyesters had excellent electrical properties and that large structures could be molded at low pressures with low cost tooling. As a result, commercial development pro-ceeded rapidly after World War I1 with materials and molding research moving in many directions. In the 20 years that followed, polyester and vinyl ester resins matured rapidly and by the mid-l970s, the composites fabricator and end user had numerous options with these matrix systems to achieve the desired properties in the finished part. 2.2 POLYESTER RESINS},
author = {Cassis, Frank A. and Talbot, Robert C.},
doi = {10.1007/978-1-4615-6389-1_3},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/{\_}buecherSong/HandbookofComposites/I/02{\_}PolyesterandVinylEsterResin.pdf:pdf},
isbn = {978-1-4615-6389-1},
issn = {07230192},
journal = {Handb. Compos.},
pages = {34--47},
title = {{Polyester and Vinyl Ester Resins}},
url = {http://link.springer.com/10.1007/978-1-4615-6389-1{\_}3},
year = {1998}
}
@article{Esfahanian2006,
abstract = {In this study, the heat transfer to an engine piston crown is calculated. Three different methods for the combustion boundary condition are used. The results of different combustion side boundary condition treatments are compared and their effects on the thermal behavior of the piston are investigated. It has been shown that using spatial and time averaged combustion side boundary condition is a suitable treatment method within engineering approximations. An interface between KIVA-3V and NASTRAN codes is developed. ?? 2005 Elsevier Ltd. All rights reserved.},
author = {Esfahanian, V and Javaheri, A and Ghaffarpour, M},
doi = {10.1016/j.applthermaleng.2005.05.002},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2006{\_}Esfahanian{\_}Thermal analysis of an SI engine piston using different combustion boundary condition treatements.pdf:pdf},
issn = {13594311},
journal = {Appl. Therm. Eng.},
keywords = {Boundary Condition Treatment,Combustion,Heat transfer,Piston},
number = {2-3},
pages = {277--287},
title = {{Thermal analysis of an SI engine piston using different combustion boundary condition treatments}},
volume = {26},
year = {2006}
}
@article{Reglern,
author = {Reglern, Synthese Von},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Vorlesungen/Messtechnik+Regelungstechnik/gmrt05.pdf:pdf},
pages = {1--21},
title = {{Forderungen an die Regelung}}
}
@article{Dieselmotors1893,
author = {Dieselmotors, Historie},
title = {{Geschichte und Grundlagen des Dieselmotors}},
year = {1893}
}
@article{Morris1979,
author = {Morris, W. L.},
doi = {10.1007/BF02686400},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/1979{\_}Morris{\_}Microcrack closure phenomena for AL2219-T851.pdf:pdf},
issn = {03602133},
journal = {Metall. Trans. A},
number = {1},
pages = {5--11},
title = {{Microcrack closure phenomena for AI 2219-T851}},
volume = {10},
year = {1979}
}
@article{Haslam2013,
author = {Haslam, Antony and Laskaridis, Panos},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2010{\_}Jaroslav Pokluda+Pavel {\v{S}}andera{\_}Micromechanisms of fracture and fatigue{\_}Buch/Kap4{\_}FatigueFracture.pdf:pdf},
journal = {Adv. Mater. Process.},
number = {April},
title = {{Fatigue {\&} Fracture}},
year = {2013}
}
@article{Zielsetzung2008,
author = {Zielsetzung, Einleitung and Verbrennungsmotor, Der and Generatoren, Schiffe},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/Motoren/Golloch{\_}Downsizing/chp{\_}10.1007{\_}3-540-27490-1{\_}1.pdf:pdf},
pages = {1--2},
title = {{1 Einleitung und Zielsetzung}},
year = {2008}
}
@article{Berg1998a,
author = {Berg, Kenneth R},
title = {{Typical Properties for Advanced Composites}},
year = {1998}
}
@article{Chen1999,
author = {Chen, Ang and Zhi, Yu and Bao, Yahua},
doi = {10.1088/0953-8984/6/39/012},
issn = {0953-8984},
journal = {J. Phys. Condens. Matter},
number = {39},
pages = {7921--7925},
title = {{Ceramic Composites}},
volume = {6},
year = {1999}
}
@inproceedings{Kenningley2012a,
author = {Kenningley, Scott and Morgenstern, Roman},
booktitle = {SAE Tech. Pap. 2012-01-1330},
doi = {https://doi.org/10.4271/2012-01-1330},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/W{\"{a}}rme-RBen Kolben/2012{\_}Kenningley+Morgenstern{\_}Thermal and Mechanical Loading in the Combustion Bowl Region of LVD Pistons.pdf:pdf},
publisher = {SAE International},
title = {{Thermal and Mechanical Loading in the Combustion Bowl Region of Light Vehicle Diesel AlSiCuNiMg Pistons; Reviewed with Emphasis on Advanced Finite Element Analysis and Instrumented Engine Testing Techniques}},
year = {2012}
}
@article{Schnittstelle,
author = {Schnittstelle, Serielle},
title = {{5 Projekte mit Assembler gel{\"{o}}st}}
}
@article{Misdariis2015,
abstract = {Large Eddy Simulation of knocking in piston engines requires high-fidelity physical models and numerical techniques. The need to capture temperature fields with high precision to predict autoignition is an additional critical constraint compared to existing LES in engines. The present work presents advances for LES of knocking in two fields: (1) a Conjugate Heat Transfer (CHT) technique is implemented to compute the flow within the engine over successive cycles with LES together with the temperature field within the cylinder head walls and the valves and (2) a reduced two-step scheme is used to predict both propagating premixed flames as well as autoignition times over a wide range of equivalence ratios, pressures and temperatures. The paper focuses on CHT which is critical for knocking because the gas temperature field is controlled by the wall temperature field and knocking is sensitive to small temperature changes. The CHT LES is compared to classical LES where the temperatures of the head and the valves are supposed to be homogeneous and imposed empirically. Results show that the skin temperature field (which is a result of the CHT LES while it is a user input for classical LES) is complex and controls knocking events. While the results of the CHT LES are obviously better because they suppress a large part of the empirical specification of the wall temperatures, this study also reveals a difficult and crucial element of the CHT approach: the description of exhaust valves cooling which are in contact with the engine head for part of the cycle and not in the rest of the cycle, leading to difficulties for heat transfer descriptions between valves and head. The CHT method is successfully applied to an engine studied at IFP Energies Nouvelles where knocking characteristics have been studied over a wide range of conditions.},
author = {Misdariis, Antony and Vermorel, Olivier and Poinsot, Thierry},
doi = {10.1016/j.combustflame.2015.07.023},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Klopfen{\_}Ottomotor/2015{\_}Misdariis{\_}LES of knocking in engines using dual heat transfer and two-step reduced schemes{\_}ModelForHeatConductionBetweenValveAndRing.pdf:pdf},
issn = {00102180},
journal = {Combust. Flame},
keywords = {Autoignition,Heat transfert,Internal combustion engine,Knock,LES},
number = {11},
pages = {4304--4312},
publisher = {Elsevier Ltd.},
title = {{LES of knocking in engines using dual heat transfer and two-step reduced schemes}},
url = {http://dx.doi.org/10.1016/j.combustflame.2015.07.023},
volume = {162},
year = {2015}
}
@article{Lechner2007,
author = {Lechner, Gisbert and Naunheimer, Harald},
doi = {10.1007/978-3-540-30670-2_7},
isbn = {978-3-540-30670-2},
journal = {Fahrzeuggetriebe},
pages = {238--279},
title = {{Auslegung von Zahnradgetrieben f{\"{u}}r Fahrzeuge}},
url = {http://link.springer.com/10.1007/978-3-540-30670-2{\_}7},
year = {2007}
}
@article{Reuter2008,
author = {Reuter, Manfred and Zacher, Serge},
doi = {10.1007/978-3-8348-9273-7},
isbn = {978-3-8348-0018-3},
journal = {Anal. Simul. und Entwurf von Regelkreisen},
title = {{Aus dem Programm}},
year = {2008}
}
@article{Szabo1991,
author = {Szabo, B A and Babuska, I},
isbn = {084930749X},
title = {{Finite element analysis}},
year = {1991}
}
@book{Streicher-abel,
author = {Streicher-abel, Christian Demant Bernd},
booktitle = {Media},
doi = {10.1007/s10531-008-9469-2},
isbn = {9783642130960},
title = {{1 C}}
}
@article{Soyhan2009,
abstract = {Combustion in HCCI engines is a controlled auto-ignition of well-mixed fuel, air and residual gas. The thermal conditions of the combustion chamber are governed by chemical kinetics strongly coupled with heat transfer from the hot gas to the walls. The heat losses have a critical effect on HCCI ignition timing and burning rate, so it is essential to understand heat transfer process in the combustion chamber in the modeling of HCCI engines. In the present paper, a comparative analysis is performed to investigate the performance of well-known heat transfer correlations in an HCCI engine. The results from the existing correlations are compared with the experimental results obtained in a single-cylinder engine. Significant differences are observed between the heat transfer results obtained by using Woschni, Assanis and Hohenberg correlations. ?? 2008 Elsevier Ltd. All rights reserved.},
author = {Soyhan, H. S. and Yasar, H. and Walmsley, H. and Head, B. and Kalghatgi, G. T. and Sorusbay, C.},
doi = {https://doi.org/10.1016/j.applthermaleng.2008.03.014},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2008{\_}Soyhan{\_}Evaluation of heat transfer correlations for HCCI engine modeling.pdf:pdf},
journal = {Appl. Therm. Eng.},
keywords = {HCCI,Heat transfer correlations,Modeling,Ricardo Hydra engine},
number = {2-3},
pages = {541--549},
publisher = {Elsevier Ltd},
title = {{Evaluation of heat transfer correlations for HCCI engine modeling}},
volume = {29},
year = {2009}
}
@article{Hbs,
author = {Hbs, Bezeichnung},
pages = {93--113},
title = {( 0 , 204}
}
@article{Spur2008,
author = {Spur, G},
journal = {H{\{}{\"{u}}{\}}tte - Das Ingenieurwissen},
pages = {1746--1801},
title = {{Produktion}},
year = {2008}
}
@article{Brettschneider1979,
author = {Brettschneider, J},
journal = {Bosch Tech. Berichte Tech. Mitteilungen aus Forschung, Entwicklung und Fert. des Bosch-Firmenverbandes},
number = {1979},
title = {{Berechnung des Luftverh{\"{a}}ltnisses Lambda von Luft-Kraftstoff-Gemischen und des Einflusses von Messfehler auf Lambda}},
year = {1979}
}
@article{Von,
author = {Von, Fourierreihenentwicklung},
title = {{Wechselgr{\{}{\"{o}}{\}}{\{}{\ss}{\}}en und nichtperiodische Gr{\{}{\"{o}}{\}}{\{}{\ss}{\}}en}}
}
@article{Shimada2004a,
abstract = {The effect of local lubricant viscosity on the temperature and thickness of oil film on a piston ring in a diesel engine is analyzed by using the Reynolds equation, and unsteady and two-dimensional energy equation with heat generated from viscous dissipation. The oil film viscosity for a multi-grade oil is then estimated by using the local oil film temperature and the local shear rate. Moreover, the heat transfer between ring and liner surfaces is examined. The oil film thickness calculated from this method is lesser than that of the case where the viscosity is based on the liner temperature and the mean shear rate. Maximum values of heat transfer at the ring and liner surfaces are obtained at the vicinity of crank angle where the oil film thickness is at a minimum.ER -},
author = {Shimada, Akiko and Harigaya, Yasuo and Suzuki, Michiyoshi and Takiguchi, Masaaki},
doi = {10.4271/2004-32-0024},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Heat Transfer Combustion Chamber/2004{\_}Shimada{\_}An Analysis of Oil Film Temperature - Oil Film Thickness and Heat Transfer on a piston ring of internal combustion engine.pdf:pdf},
isbn = {0791846628},
issn = {07424795},
number = {724},
title = {{An Analysis of Oil Film Temperature, Oil Film Thickness and Heat Transfer on a Piston Ring of Internal Combustion Engine: The Effect of Local Lubricant Viscosity}},
url = {http://papers.sae.org/2004-32-0024/},
year = {2004}
}
@article{Sauer,
author = {Sauer, Bernd and Schraube, Wirkprinzip Der},
title = {{Kapitel 6}}
}
@article{Prileschajew1947,
author = {Prileschajew, N and Greenlee, S O},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/{\_}buecherSong/HandbookofComposites/I/03{\_}EpoxyResins.pdf:pdf},
title = {{Epoxy Resins}},
year = {1947}
}
@article{Vorgang,
author = {Vorgang, Experimenteller},
pages = {217--232},
title = {{1.1 Begriffe}}
}
@article{Robinson2003a,
author = {Robinson, J. S. and Cudd, R. L. and Evans, J. T.},
doi = {https://doi.org/10.1179/026708303225009373},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Empirical Fatigue Models + Validation/2003{\_}Robinson{\_}Creep resistant aluminium alloys - experiments overview with different alloys - Al2618T6.pdf:pdf},
journal = {Mater. Sci. Technol.},
number = {2},
pages = {143--155},
title = {{Creep resistant aluminium alloys and their applications}},
volume = {19},
year = {2003}
}
@article{Trachtler2006,
author = {Tr{\"{a}}chtler, Ansgar and Niewels, Frank},
journal = {Fahrdynamik-Regelung},
pages = {237--251},
title = {{Integrierte Querdynamikregelung mit ESP, AFS und aktiven Fahrwerksystemen}},
year = {2006}
}
@article{Cherkaoui2009c,
author = {Cherkaoui, Mohammed and Capolungo, Laurent},
doi = {10.1007/978-0-387-46771-9},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Atomistic and Continuum Modeling of Nanocrystalline Materials/Chapter 01.pdf:pdf},
isbn = {978-0-387-46765-8},
pages = {1--27},
title = {{Atomistic and Continuum Modeling of Nanocrystalline Materials}},
url = {http://link.springer.com/10.1007/978-0-387-46771-9},
volume = {112},
year = {2009}
}
@article{Ma2016,
abstract = {High-purity single crystal tungsten nanowire was prepared by the metal-catalyzed vapor-phase reaction method, which was firstly proposed by our research group. Its tensile stress-strain curves and microscopic deformed structures at different temperatures were simulated by molecular dynamics method, in order to study the effects of temperature on its tensile mechanical properties and failure mechanisms. Research results show that the stress-strain curves can be all divided into five stages: elastic, damage, phase transition (dominant), hardening and failure stages. Elastic modulus, tensile strength and strain of phase transition are decreased with increase of temperature, while hardening peak stress is first increased and then decreased. There exists a critical temperature Tc for its phase transition mechanism. When T ??? Tc, the phase transition occurs in one direction and leads to less damage and random failure in its damage zone. When T {\{}{\textgreater}{\}} Tc, the phase transition occurs in two directions and leads to more damage (twin plane) and failure in its twin plane. That is quite different from FCC metal, where there is only one direction of phase transition.},
author = {Ma, Bin and Rao, Qiuhua and He, Yuehui},
doi = {10.1016/j.commatsci.2016.01.001},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Thermodynamik/2016{\_}Ma+Rao{\_}Molecular dynamics simulation of temperature effect on tensile mechanical properties of single crystal tungsten nanowire.pdf:pdf},
issn = {09270256},
journal = {Comput. Mater. Sci.},
keywords = {Mechanical property,Microscopic deformation mechanism,Molecular dynamics,Single crystal tungsten nanowire,Temperature},
pages = {40--44},
publisher = {Elsevier B.V.},
title = {{Molecular dynamics simulation of temperature effect on tensile mechanical properties of single crystal tungsten nanowire}},
url = {http://dx.doi.org/10.1016/j.commatsci.2016.01.001},
volume = {117},
year = {2016}
}
@article{Hilfe,
author = {Hilfe, Mit and Kenntnisstand, Sie Ihren and Sie, Hilfe and Detail-, Das and Sie, Falls and Aufgabe, Die and Unterlagen, Ihren and Aufgaben, Die and Sie, Schreiben and Aus-, Nach and Sie, Skizzieren and Sie, Schreiben and Sie, Schreiben and Programm, Das and Sie, Beschreiben},
title = {{10 {\"{U}}bungsaufgaben}}
}
@article{Pahl2007,
author = {Pahl, Gerhard and Beitz†, Wolfgang and Feldhusen, J{\"{o}}rg and Grote, Karl-H.},
doi = {10.1007/b137606},
isbn = {3-540-22048-8},
journal = {Pahl/Beitz Konstr. - Grundlagen},
title = {{Methoden zur qualit{\"{a}}tssichernden Produktentwicklung}},
year = {2007}
}
@article{Dampf1916,
author = {Dampf, Kommt},
title = {{Kondensation}},
year = {1916}
}
@article{Remy2002a,
abstract = {The purpose of the paper is to show the successive steps of a numerical method for the predic-tion of crack initiation in industrial components submitted to thermo-mechanical fatigue. Finite element computations using realistic constitutive equations are first used to determine the stress and strain fields in the component. The constitutive equations account for cyclic viscoplasticity, creep, and aging effect. The industrial use of such theories requires robust integration techniques to reach the mechanical steady state. Since the real meshes have 10{\{}{\^{}}{\}}-10{\{}{\^{}}{\}} degrees of freedom, parallel computers are also needed. Damage models with creep-fatigue interaction are finally applied to determine crack initiation. The example of aluminum cylinder heads is chosen to illustrate the demonstration.},
author = {Remy, L and Petit, J and Nicouleau, E and Feyel, F and Quilici, S and Cailletaud, G},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/2002{\_}Nicouleau+Feyel{\_}STRUCTURAL CALCULATION AND LIFETIME-PREDICTION IN THERMOMECHANICAL FATIGUE OF ENGINE COMPONENTS.pdf:pdf},
keywords = {FE struc-tural calculation Cycle skip,Parallel computations,Thermomechanical fatigue,Viscoplastic modeling Aging effect Aluminum alloys},
title = {{Temperature-Fatigue Interaction STRUCTURAL CALCULATION AND LIFETIME- PREDICTION IN THERMOMECHANICAL FATIGUE OF ENGINE COMPONENTS}},
year = {2002}
}
@article{Liu1972b,
author = {Liu, I. Shih and M{\"{u}}ller, Ingo},
doi = {10.1007/BF00250689},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Thermodynamik/Liu{\_}Entropieprinzip{\_}Lagrange/On the Thermodynamics and Thermostatics of Fluid in Electromagnetic Fields {\_}Liu.pdf:pdf},
issn = {00039527},
journal = {Arch. Ration. Mech. Anal.},
number = {2},
pages = {149--176},
title = {{On the thermodynamics and thermostatics of fluids in electromagnetic fields}},
volume = {46},
year = {1972}
}
@article{Lubarda2002,
abstract = {In this chapter we briefly summarize the fundamental relations of$\backslash$nthe kinematics of large deformations, restricting ourselves to the$\backslash$napplications we have in mind. For concise treatments we advise the$\backslash$nliterature on continuum mechanics},
author = {Lubarda, Vlado a.},
isbn = {0849311381},
journal = {Elastoplast. Theory},
pages = {51--71},
title = {{Kinematics of deformation}},
year = {2002}
}
@article{Mandadapu2012a,
abstract = {This article proposes a continuum thermomechanical homogenization method inspired by the Irving-Kirkwood procedure relating the atomistic equations of motion to the balance laws of continuum mechanics. This method yields expressions for the macroscopic stress and heat flux in terms of microscopic kinematic and kinetic quantities. The resulting equation for macroscopic stress affords a rational comparison with the widely used Hill-Mandel stress-deformation condition, while the one for heat flux reduces, under certain assumptions, to a Hill-Mandel-like condition involving heat flux and the gradient of temperature.},
archivePrefix = {arXiv},
arxivId = {84862181137},
author = {Mandadapu, K. K. and Sengupta, A. and Papadopoulos, P.},
doi = {10.1098/rspa.2011.0578},
eprint = {84862181137},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/A homogenization method for thermomechanical continua using extensive physical quantities.pdf:pdf},
isbn = {1364-5021$\backslash$r1471-2946},
issn = {1364-5021},
journal = {Proc. R. Soc. A Math. Phys. Eng. Sci.},
keywords = {hill,homogenization,irving,kirkwood procedure,mandel condition,thermomechanics},
number = {2142},
pages = {1696--1715},
title = {{A homogenization method for thermomechanical continua using extensive physical quantities}},
url = {http://rspa.royalsocietypublishing.org/content/early/2012/02/16/rspa.2011.0578.full},
volume = {468},
year = {2012}
}
@article{Zienkiewicz2013d,
abstract = {The set of differential equations from which we start the discretization process will determine whether we refer to the formulation as mixed or irreducible. Thus if we consider an equation system with several dependent variables u written as [see Eqs (3.1) and (3.2)] A ( u ) = 0 in domain $\Omega$ (10.1a) and ℬ ( u ) = 0 on boundary $\Gamma$ (10.1b) in which none of the components of u can be eliminated still leaving a well-defined problem, then the formulation will be termed irreducible. If this is not the case the formulation will be called mixed. These definitions were given in Chapter 3 (p. 56). Publisher Summary The aim of this chapter is to discuss mixed formulation and constraints. The set of differential equations from which the discretization process is started determines whether the formulation is referred to as mixed or as irreducible. This chapter demonstrates how elasticity problems can be dealt with in mixed form and shows how such formulations are essential in certain problems. If the operator specifying the mixed form is symmetric or self-adjoint, the formulation can proceed from the basis of a variational principle that can be directly obtained for linear problems. This chapter essentially outlines the mixed form of finite element formulation, which opens a new range of possibilities, many with potentially higher accuracy and robustness than those offered by irreducible forms. However, an additional advantage arises even in situations where, by the principle of limitation, the irreducible and mixed forms yield identical results. Therefore, the study of the behavior of the mixed form can frequently reveal weaknesses or lack of robustness in the irreducible form that otherwise would be difficult to determine. The mixed approximation expands the potential of the finite element method and presents almost limitless possibilities of detailed improvement.},
author = {Zienkiewicz, O.C. and Taylor, R.L. and Zhu, J.Z.},
doi = {10.1016/B978-1-85617-633-0.00009-5},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Zienkiewicz FEM - Vol 1 Basics Fundamentals/63205{\_}10.pdf:pdf},
isbn = {978-0-7506-6431-8},
issn = {00295981},
journal = {Finite Elem. Method its Basis Fundam.},
pages = {285--314},
title = {{Mixed Formulation and Constraints: Complete Field Methods}},
url = {http://linkinghub.elsevier.com/retrieve/pii/B9781856176330000095},
year = {2013}
}
@article{Gurson1977c,
abstract = {Widely used constitutive laws for engineering materials assume plastic incompressibility, and no effect on yield of the hydrostatic component of stress. However, void nucleation and growth (and thus bulk dilatancy) are commonly observed is some processes which are characterized by large local plastic flow, such as ductile fracture.},
author = {Gurson, A L},
doi = {10.1115/1.3443401},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Plasticity models/Continuum Theory of Ductile Rupture by Void Nucleation and  Growth-PartI{\_}ByGurson.pdf:pdf},
isbn = {0094-4289},
issn = {00944289},
journal = {J. Eng. Mater. Technol.},
number = {1},
pages = {2},
title = {{Continuum Theory of Ductile Rupture by Void Nucleation and Growth: Part I—Yield Criteria and Flow Rules for Porous Ductile Media}},
url = {http://materialstechnology.asmedigitalcollection.asme.org/article.aspx?articleid=1422194},
volume = {99},
year = {1977}
}
@article{Motion,
author = {Motion, Thermally Assisted and Obstacles, Penetrable and Stre, D-solut I O N and Ng, Ngtheni},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Surface effects + Frequency effects/Bulatov - 2006 - Computer simulations of dislocations.pdf:pdf},
title = {{Series Editors Adrian P . Sutton , FRS Department of Physics , Imperial College London Robert E . Rudd}}
}
@book{Naumenko2016,
author = {Naumenko, Konstantin},
doi = {10.1007/978-3-319-31629-1},
isbn = {9783319316277},
title = {{Modeling High Temperature Materials Behavior for Structural Analysis Part I : Continuum Mechanics}},
year = {2016}
}
@article{Probleme2012,
author = {Probleme, Fem-ansatz and Elastostatik, Der Finite-element-methode Der},
doi = {10.1007/978-3-8348-2134-8},
isbn = {9783834821348},
pages = {202--246},
title = {{9 FEM-Ansatz f{\"{u}}r dynamische Probleme}},
volume = {0},
year = {2012}
}
@article{Haslam2013,
author = {Haslam, Antony and Laskaridis, Panos},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2010{\_}Jaroslav Pokluda+Pavel {\v{S}}andera{\_}Micromechanisms of fracture and fatigue{\_}Buch/Kap4{\_}FatigueFracture.pdf:pdf},
title = {{Fatigue {\&} Fracture}},
year = {2013}
}
@article{Lcmaitrca,
author = {Lcmaitrc, Cordchois},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Plasticity models/On Energy based coupled elastoplastic damage theories{\_}Ju1988.pdf:pdf},
title = {{1989-Ju{\{}{\_}{\}} On energy-based coupled elastoplastic damage theories{\{}{\_}{\}}constitutive modeling and computational aspects.pdf}}
}
@article{Bohlke2012,
author = {B{\"{o}}hlke, Prof Thomas},
journal = {Mechanik},
number = {September},
title = {{Skript zur Vorlesung H{\{}{\"{o}}{\}}here Technische Festigkeitslehre}},
year = {2012}
}
@article{Sietsmaa,
author = {Sietsma, J},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/Hardening Recovery Creep/KocksMecking{\_}Annihilation of dislocation in plastic deformation.pdf:pdf},
pages = {1--24},
title = {{Dislocation annihilation in plastic deformation}}
}
@article{Wortmann2010,
author = {Wortmann, Hendrik},
doi = {10.1515/9783111376363.1},
isbn = {9783867642644},
pages = {7--9},
title = {{0 Einleitung}},
year = {2010}
}
@article{Caton1981a,
abstract = {Because of the increasing need for precise information on engine processes, this study developed and experimentally verified models for the instantaneous heat transfer in an engine exhaust port. Experimental measurements were made of the instantaneous cylinder pressure and instantaneous exhaust gas temperature for a range of engine operating conditions. The pressure measurements were used to obtain the instantaneous cylinder gas state and the temperature measurements were used to validate the heat transfer models. The exhaust port heat transfer was dominated by jet induced large-scale fluid motion as opposed to wallshear generated fluid motion. An analysis based on the jet velocity through the valve opening correctly estimated the heat transfer due to this large-scale motion. Models for the instantaneous exhaust port heat transfer provided excellent agreement with measurements as a function of engine operating conditions. A cause d'un besoin croissant d'information pr{\'{e}}cise sur le fonctionnement d'un moteur, on d{\'{e}}veloppe une {\'{e}}tude et on v{\'{e}}rifie exp{\'{e}}rimentalement des mod{\`{e}}les sur le transfert de chaleur instantan{\'{e}} {\`{a}} l'{\'{e}}chappement d'un cylindre. Des mesures de la pression instantan{\'{e}}e dans le cylindre et de la temp{\'{e}}rature instantan{\'{e}}e {\`{a}} l'{\'{e}}chappement sont effectu{\'{e}}es pour un domaine de conditions de fonctionnement d'un moteur. Les mesures de pression permettent d'atteindre l'{\'{e}}tat instantan{\'{e}} du gaz dans le cylindre et les mesures de temp{\'{e}}rature permettent de valider les mod{\`{e}}les de transfert thermique. Le transfert {\`{a}} l'{\'{e}}chappement est domin{\'{e}} par un mouvement de jet {\`{a}} large {\'{e}}chelle au contraire du mouvement de fluide {\`{a}} frottement pari{\'{e}}tal. Une analyse bas{\'{e}}e sur la vitesse du jet {\`{a}} travers l'ouverture de la soupape pr{\'{e}}dit correctement le transfert de chaleur d{\^{u}} {\`{a}} ce mouvement {\`{a}} grande {\'{e}}chelle. Des mod{\`{e}}les pour l'{\'{e}}chappement instantan{\'{e}} fournissent un accord excellent avec des mesures pour les conditions de fonctionnement du moteur. Wegen des zunehmenden Bedarfs an genauer Information {\"{u}}ber Verbrennungsmotoren-Prozesse wurden in dieser Studie Modelle f{\"{u}}r den momentanen W{\"{a}}rme{\"{u}}bergang in einer Motor-Ausla$\beta$-{\"{O}}ffnung entwickelt und experimentell best{\"{a}}tigt. Die Momentanwerte des Zylinderdrucks und der Abgastemperatur wurden in Versuchen f{\"{u}}r einen ausgedehnten Betriebsbereich gemessen. Druckmessungen wurden verwendet, um den momentanen Gaszustand im Zylinder zu bestimmenn und Temperaturmessungen dienten zur Best{\"{a}}tigung der W{\"{a}}rme{\"{u}}bergangs-Modelle. Der W{\"{a}}rme{\"{u}}bergang in der Ausla$\beta$-{\"{O}}ffnung wurde im wesentlichen durch die strahlinduzierte Makro-Bewegung des Fluides entgegen der durch Wandschubspannung erzeugten Fluidbewegung bestimmt. Eine theoretische Untersuchung, die sich auf die Strahlgeschwindigkeit durch die Ventil{\"{o}}ffnung st{\"{u}}tzt, liefert korrekt den W{\"{a}}rme{\"{u}}bergang, hervorgerufen durch diese Makro-Bewegung. Die Modelle f{\"{u}}r den momentanen W{\"{a}}rme{\"{u}}bergang in der Ausla$\beta$-{\"{O}}ffnung als Funktion der Arbeitsbedingungen des Motors zeigten vorz{\"{u}}gliche {\"{U}}bereinstimmung mit den Messungen. B cвязи c вce бoлee вoзpacтaющeй нeoбчoдимocтью в тoчнoй инфopмaции o пpoцeccaч, пpoиcчoдящич в двигaтeляч, пpeдлoзeны мoдeди тeплoпepeнoca в вычлoпнoм oтвepcтии двигaтeля. Измepялиcь дaвлeниe в цилиндpe и тeмпepaтypa вычлoпнoгo гaзa пpи paздичныч peзимaч paбoты двигaтeля. Дaнныe пo дaвлeнию иcпoльзoвaлиcь для oпpeдeлeния cocтoяния гaзa в цилиндpe, a пo тeмпepaтype — для пpoвepки cпpaвeдливocти пpeдлoзeнныч мoдeлeй. Teплoпepeнoc в вычлoпнoм oтвepcтии oпpeдeляeтcя кpyпнoмacштaбными пepeмeщeниями зидкocти, вoзникaющими пpи cтpyйнoм иcтeчeнии, кoтopыe cyщecтвeннo oтличaютcя oт пepeмeщeний, вызывaeмыч нaпpязeниeм cдвигa нa cтeнкe. Aнaлиз, ocнoвaный нa cкopocти иcтeчeния cтpyи чepeз oтвepcтиe клaпaнa, пoзвoляeт кoppeктнo oцeнить вeличинy тeплoвoгo пoтoкa пpи тaкич кpyпнoмacщтaбпыч пepeмeщeнияч. Moдeли тeплoпepeнoca в вычлoпнoм oтвepcтии чopoшo coглacyютcя c peзyльтaтaми измepeний пpи paзличныч peзимaч paбoты двигaтeдя.},
author = {Caton, J.A. and Heywood, J.B.},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/1981{\_}An experimental and analytical study of heat transfer in an engine exhaust port{\_}Caton.pdf:pdf},
journal = {Int. J. Heat Mass Transf.},
number = {4},
pages = {581--595},
title = {{An experimental and analytical study of heat transfer in an engine exhaust port}},
volume = {24},
year = {1981}
}
@article{Gurson1977,
abstract = {Widely used constitutive laws for engineering materials assume plastic incompressibility, and no effect on yield of the hydrostatic component of stress. However, void nucleation and growth (and thus bulk dilatancy) are commonly observed is some processes which are characterized by large local plastic flow, such as ductile fracture.},
author = {Gurson, A L},
doi = {10.1115/1.3443401},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Plasticity models/Continuum Theory of Ductile Rupture by Void Nucleation and  Growth-PartI{\_}ByGurson.pdf:pdf},
isbn = {0094-4289},
issn = {00944289},
journal = {J. Eng. Mater. Technol.},
number = {1},
pages = {2},
title = {{Continuum Theory of Ductile Rupture by Void Nucleation and Growth: Part I—Yield Criteria and Flow Rules for Porous Ductile Media}},
url = {http://materialstechnology.asmedigitalcollection.asme.org/article.aspx?articleid=1422194},
volume = {99},
year = {1977}
}
@article{Teilaufgabenb,
author = {Teilaufgaben, Abzuhandelnde},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Empirical Fatigue Models + Validation/Betriebsfestigkeit{\_}ErwinHaibach/Kap4 Praktische Umsetzung des Betriebsfestigkeits-Konzepts.pdf:pdf},
title = {{des Betriebsfestigkeits-Konzeptes}}
}
@article{Werdich2011,
author = {Werdich, Martin},
doi = {10.1007/978-3-8348-9951-4_6},
isbn = {978-3-8348-1433-3},
journal = {FMEA – Einf{\{}{\"{u}}{\}}hrung und Moderation},
pages = {101--108},
title = {{6 Software}},
url = {http://www.springerlink.com/index/10.1007/978-3-8348-9951-4},
year = {2011}
}
@article{Burgg,
author = {Burg, Heinz},
pages = {705--714},
title = {{B9 B9 Unf{\{}{\"{a}}{\}}lle mit Schienenfahrzeugen B9}}
}
@book{Riccardella1992c,
author = {Riccardella, P C and Deardorff, A F and Griesbach, T J},
booktitle = {Adv. Fatigue Lifetime Predict. Tech.},
doi = {10.1520/STP1122-EB},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Neuer Ordner/Advances in fatigue lifetime predictive techniques Part1.pdf:pdf},
isbn = {978-0-8031-1423-4},
issn = {00660558},
keywords = {FATIGUE,MONITORING,POWER PLANTS,PRESSURE VESSELS AND PIPING,THERMAL STRESSES},
pages = {460--473},
pmid = {11439068},
title = {{Advances in Fatigue Lifetime Predictive Techniques}},
url = {https://apps.webofknowledge.com/full{\%}7B{\_}{\%}7Drecord.do?product=UA{\%}7B{\&}{\%}7Dsearch{\%}7B{\_}{\%}7Dmode=GeneralSearch{\%}7B{\&}{\%}7Dqid=11{\%}7B{\&}{\%}7DSID=Z1UxbH6jtsqo8n9kPQr{\%}7B{\&}{\%}7Dpage=1{\%}7B{\&}{\%}7Ddoc=1},
volume = {1122},
year = {1992}
}
@article{Sun2016c,
abstract = {A multi-scale model is developed in this study for linking collective behavior of short and long cracks to continuous average fatigue damage. By using the developed model, the average fatigue damage evolution can be evaluated through some parameters that reflect collective behavior of short and long cracks, while collective behavior of short and long cracks can be reflected from the measured continuous average fatigue damage evolution based on the effective stress concept. The effectiveness of the model is verified by comparing numerical results with experimental data. The comparative results show that the developed model can be used to study the metal fatigue failure mechanisms from both macro- and micro-scale viewpoint.},
author = {Sun, Bin and Xu, You Lin and Li, Zhaoxia},
doi = {10.1016/j.engfracmech.2016.02.013},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/2 scale models papers/2016{\_}Sun+Lu{\_}Multi-scale model for linking collective behavior of short.pdf:pdf},
issn = {00137944},
journal = {Eng. Fract. Mech.},
keywords = {Crack,Effective stress,Fatigue damage,Multi-scale},
pages = {141--153},
publisher = {Elsevier Ltd},
title = {{Multi-scale model for linking collective behavior of short and long cracks to continuous average fatigue damage}},
url = {http://dx.doi.org/10.1016/j.engfracmech.2016.02.013},
volume = {157},
year = {2016}
}
@article{Papula,
author = {Papula, L},
doi = {10.1007/978-3-8348-8643-9},
isbn = {9783834886439},
journal = {Math. f{\"{u}}r Ingenieure und Naturwissenschaftler Band 2},
number = {1},
title = {{I Lineare Algebra 1}},
volume = {1}
}
@article{Dynamik2006,
author = {Dynamik, Nichtlineare},
journal = {Gerthsen Phys.},
pages = {1085--1130},
title = {{20 - Nichtlineare Dynamik}},
year = {2006}
}
@book{Tobergte2013a,
abstract = {applicability for this approach.},
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Tobergte, David R. and Curtis, Shirley},
booktitle = {J. Chem. Inf. Model.},
doi = {10.1017/CBO9781107415324.004},
eprint = {arXiv:1011.1669v3},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Thermodynamik/M{\"{u}}llerAndNoll{\_}Thermodynamik/M{\"{u}}ller 2007 Energy and Entropy.pdf:pdf},
isbn = {9788578110796},
issn = {1098-6596},
keywords = {icle},
number = {9},
pages = {1689--1699},
pmid = {25246403},
title = {{A History of Thermodynamics}},
volume = {53},
year = {2013}
}
@article{Block1994,
author = {Block, I and Esslinger, T and Eigler, D M and Gimzewski, J and Rapaport, D C and Meyer, M and Toschek, P E and Neuhauser, W and Vogel, H and Walz, J},
journal = {Museum},
pages = {1--11},
title = {{Quellennachweis f{\"{u}}r die Einleitungs- und Ausblickabbildungen Sach- und Namenverzeichnis}},
volume = {7},
year = {1994}
}
@article{Eekoye1996b,
abstract = {Heat-transfer rates present in an engine cylinder undergoing knock are known to be larger than the rates associated with normal engine operation. Further, at the time of knock, the largest heat fluxes are associated with locations on the cylinder wall where the flame is locally quenching. In this study, heat-transfer processes at the flame-wall interface during a knock event are investigated computationally and analytically. Computationally, the governing equations for a one-dimensional, flame-quenching event are solved using a reduced chemical reaction mechanism. Analytically, scaling relations for the flame heat-release rates are used in the governing equations to determine the heat-transfer rates. It is found that while pressure transients modify the wall heat flux, the absolute value of the pressure is the most significant parameter in predicting the maximum heat flux. The wall heat flux profiles are predicted for both the analytical and computational models. In the range of pressures examined, a linear relationship was found between the peak flux and pressure, both for the computational and analytical models. The linear relationship between the pressure and peak flux was found to be invalid when the flame-quenching process was disrupted by the pressure fluctuations for pressure oscillations with a characteristic time on the order of the quenching process. ?? 1996 Combustion Institute.},
author = {Eekoye, O. A.},
doi = {10.1016/S0082-0784(96)80101-9},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Klopfen{\_}Ottomotor/1996{\_}Ezekoye{\_}Heat transfer modeling during knock and flame quenching in an engine chamber.pdf:pdf},
isbn = {0082-0784},
issn = {00820784},
journal = {Symp. Combust.},
number = {2},
pages = {2661--2668},
title = {{Heat transfer modeling during knock and flame quenching in an engine chamber}},
volume = {26},
year = {1996}
}
@article{Morris1980,
author = {Morris, W. L.},
doi = {10.1007/BF02668135},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/1980{\_}Morris{\_}The noncontinuum crack tip defo behavior of surface microcracks.pdf:pdf},
issn = {03602133},
journal = {Metall. Trans. A},
number = {7},
pages = {1117--1123},
title = {{The noncontinuum crack tip deformation behavior of surface microcracks}},
volume = {11},
year = {1980}
}
@article{Results1994,
abstract = {As a concluding comment, I should like to return to the point raised by Ayres, that it is not enough simply to tell a better version of the fourth-century history in the expectation that modern theologians will finally get it straight! This is a valid point: if we want to have Christianity's fourth-century heritage taken seriously, we need to be in dialogue with modern writers. But, if there is to be a dialogue, both sides must be allowed to speak, and so we are also responsible for expounding the historical material on its own terms. As Heidegger put it, “[O]nly when we think through what has been thought will we be of any use for what must still be thought.” Perhaps studying the figures from a distant era will open up for us possibilities we would never have dreamed of within our own modern presuppositions, so that we can recognize differences even beyond those which lie within our own horizon or tradition. If I am right in affirming that there is a different style of doing theology prior to Augustine and after him in the East than that which we find in the theological and scholarly tradition in which Ayres's book stands, then we must ask whether we need to address the question of the legitimacy of each (and ponder how one might even answer that) or whether a plurality of approaches is possible without reducing one to the other. In a way, this would be a further step toward deconstructing monolithic notions of “Orthodoxy” in recognition of genuine and legitimate diversity within early Christianity and among modern Christians. Might it be better not to speak of Nicaea and its legacy, but of the legacies of Nicaea—or better—“Christ and him crucified” (2 Cor 2:2) and the ways in which Nicaea and its interpreters affirm the true divinity of this one?},
author = {Results, Useful},
doi = {10.1007/BF02600226},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2010{\_}Jaroslav Pokluda+Pavel {\v{S}}andera{\_}Micromechanisms of fracture and fatigue{\_}Buch/Kap5{\_}FinalReflection.pdf:pdf},
isbn = {9780470434673},
issn = {08848734},
journal = {J. Gen. Intern. Med.},
number = {3 Supplement},
pages = {243--247},
title = {{Final reflections}},
volume = {9},
year = {1994}
}
@article{Tanguy2013,
author = {Tanguy, Jean-Michel},
doi = {10.1002/9781118557877.ch7},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Nicholson 2003 - Finite Element Analysis Thermomechanics of Solids/0749{\_}C08.pdf:pdf},
journal = {Numer. Methods},
pages = {109--159},
title = {{Introduction to the Finite Element Method}},
url = {http://doi.wiley.com/10.1002/9781118557877.ch7},
year = {2013}
}
@article{Kreher1985,
author = {Kreher, W and Pompe, W},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Probabilistic Aspects/1985{\_}Kreher{\_}Field Fluctuations in a heterogeneous elastic material - an info theory approach.pdf:pdf},
journal = {J. Mech. Phys. Solids},
number = {5},
pages = {419--445},
title = {{Field fluctuations in a heterogeneous elastic material: An information theory approach}},
volume = {33},
year = {1985}
}
@article{Funktionen,
author = {Funktionen, Zuordnung Von},
journal = {Area},
pages = {53--84},
title = {{Klima / Heizung}}
}
@article{Beck2007a,
abstract = {Out-of-phase thermal-mechanical fatigue (TMF) tests with superimposed higher frequency mechanical fatigue (HCF) loading were performed at three cast Al-Si cylinder head alloys. All materials show for maximum temperatures of the TMF cycle between 200 and 250 ??C a threshold of the amplitude of the superimposed HCF loading below of which the number of TMF cycles to failure is not significantly affected by the superimposed HCF loading. Above this threshold the TMF life shows a strong decrease with increasing HCF loading. Extensive microscopic analyses revealed that independent from the HCF loading first cracks are initiated at eutectic Si-particles detached from the surrounding ??-Al matrix. Crack propagation occurs at small HCF amplitudes along the eutectic regions. At higher superimposed HCF loadings an accelerated crack propagation along slip bands within the ??-Al matrix is observed. ?? 2007 Elsevier B.V. All rights reserved.},
author = {Beck, Tilmann and L??he, Detlef and Luft, Jochen and Henne, Ingo},
doi = {10.1016/j.msea.2006.05.177},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Empirical Fatigue Models + Validation/2006{\_}Beck{\_}Damage mechanisms of cast Al–Si–Mg alloys under superimposed TMF and HCF.pdf:pdf},
isbn = {09215093 (ISSN)},
issn = {09215093},
journal = {Mater. Sci. Eng. A},
keywords = {Cast aluminium alloys,Damage behaviour,High-cycle fatigue,Thermal-mechanical fatigue},
number = {SPEC. ISS.},
pages = {184--192},
title = {{Damage mechanisms of cast Al-Si-Mg alloys under superimposed thermal-mechanical fatigue and high-cycle fatigue loading}},
volume = {468-470},
year = {2007}
}
@article{Prebil,
author = {Prebil, Ivan},
pages = {803--820},
title = {{C11 C11 Biomechanische Daten C11}}
}
@article{Wei2007a,
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Wei, Wilfried},
doi = {10.1007/978-3-8348-0353-5},
eprint = {arXiv:1011.1669v3},
isbn = {978-3-8348-0058-9},
issn = {0717-6163},
pmid = {15003161},
title = {{Elektrotechnik f{\"{u}}r Ingenieure 1}},
year = {2007}
}
@article{Morris1981,
author = {Morris, W. L. and James, M. R. and Buck, O.},
doi = {10.1007/BF02648508},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/1981{\_}Morris+James{\_}Growth rate models for short surface cracks in Al 2219-T851.pdf:pdf},
issn = {0360-2133},
journal = {Metall. Trans. A},
number = {January},
pages = {57--64},
title = {{Growth rate models for short surface cracks in AI 2219-T851}},
volume = {12},
year = {1981}
}
@article{Embers2003,
author = {Embers, O N E Imensional M},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Nicholson 2003 - Finite Element Analysis Thermomechanics of Solids/0749{\_}C09.pdf:pdf},
journal = {Dimens. Contemp. Ger. Arts Lett.},
pages = {121--138},
title = {{Element Fields in Linear Problems}},
volume = {1},
year = {2003}
}
@article{Bozek2008a,
abstract = {Microstructurally small fatigue crack (MSFC) formation includes stages of incubation, nucleation and microstructurally small propagation. In AA 7075-T651, the fracture of Al 7 Cu 2 Fe constituent particles is the major incubation source. In experiments, it has been observed that only a small percentage of these Fe-bearing particles crack in a highly stressed volume. The work presented here addresses the identification of the particles prone to cracking and the prediction of particle cracking frequency, given a distribution of particles and crystallographic texture in such a volume. Three-dimensional elasto-viscoplastic finite element analyses are performed to develop a response surface for the tensile stress in the particle as a function of the strain level surrounding the particle, parent grain orientation and particle aspect ratio. A technique for estimating particle strength from fracture toughness, particle size and intrinsic flaw size is developed. Particle cracking is then determined by comparing particle stress and strength. The frequency of particle cracking is then predicted from sampling measured distributions of grain orientation, particle aspect ratio and size. Good agreement is found between the predicted frequency of particle cracking and two preliminary validation experiments. An estimate of particle cracking frequency is important for simulating the next stages of MSFC formation: inserting all particles into a microstructural model for these stages is computationally intractable and physically unnecessary.},
author = {Bozek, J E and Hochhalter, J D and Veilleux, M G and Liu, M and Heber, G and Sintay, S D and Rollett, A D and Littlewood, D J and Maniatty, A M and Weiland, H and Christ, R J and Payne, J and Welsh, G and Harlow, D G and Wawrzynek, P A and Ingraffea, A R},
doi = {10.1088/0965-0393/16/6/065007},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/2008{\_}Hochhalter{\_}AL7075AgeometricapproachI{\_}ParticeleCracking.pdf:pdf},
isbn = {09650393 (ISSN)},
issn = {0965-0393},
journal = {Model. Simul. Mater. Sci. Eng.},
number = {6},
pages = {065007},
title = {{A geometric approach to modeling microstructurally small fatigue crack formation: I. Probabilistic simulation of constituent particle cracking in AA 7075-T651}},
url = {http://stacks.iop.org/0965-0393/16/i=6/a=065007?key=crossref.c2c7fddb48a7b52013977b4d25c503c4},
volume = {16},
year = {2008}
}
@article{Gingrich2016b,
abstract = {An experimental investigation was conducted to explore the impact in-cylinder pressure oscillations have on piston heat transfer. Two fast-response surface thermocouples embedded in the piston top measured transient temperature and a commercial wireless telemetry system was used to transmit thermocouple signals from the moving piston. Measurements were made in a light-duty single-cylinder research engine operated under low temperature combustion regimes including Homogeneous Charge Compression Ignition (HCCI) and Reactivity Controlled Compression Ignition (RCCI) and Conventional Diesel (CDC). The HCCI data showed a correlated trend of higher heat transfer with increased pressure oscillation strength, while the RCCI and CDC data did not. An extensive HCCI data set was acquired. The heat transfer rate - when corrected for differences in cylinder pressure and gas temperature - was found to positively correlate with increased pressure oscillations. It is important to normalize the data before drawing conclusions as the magnitude of the effect was diminished significantly by the normalization procedure.},
author = {Gingrich, Eric and Janecek, Daniel and Ghandhi, Jaal},
doi = {10.4271/2016-01-9044},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2016{\_}Gingrich{\_}Experimental Investigation of the Impact of In-Cylinder Pressure Oscillations on Piston Heat Transfer.pdf:pdf},
issn = {1946-3944},
journal = {SAE Int. J. Engines},
number = {3},
pages = {2016--9044},
title = {{Experimental Investigation of the Impact of In-Cylinder Pressure Oscillations on Piston Heat Transfer}},
url = {http://papers.sae.org/2016-01-9044/},
volume = {9},
year = {2016}
}
@inproceedings{Setlur2003,
author = {Setlur, P and Wagner, J and Dawson, D and Chen, J},
booktitle = {Am. Control Conf.},
doi = {10.1109/ACC.2003.1242465},
file = {:C$\backslash$:/Users/p327208/Desktop/Promotion/Literature/Motorspezifisch/Thermal Coating + Water Heat Transfer + Applikation/2003{\_}Setlur{\_}Nonlinear Controller for Automotive Thermal Management Systems.pdf:pdf},
publisher = {IEEE},
title = {{Nonlinear controller for automotive thermal management systems}},
year = {2003}
}
@article{Filipi2011,
author = {Lee, T.-K and Filipi, Z. S},
doi = {https://doi.org/10.1007/s12239-011-0001-4},
file = {:C$\backslash$:/Users/p327208/Desktop/Promotion/Literature/Motorspezifisch/Heat Transfer Combustion Chamber/2011{\_}Lee+Filip{\_}IMPROVING THE PREDICTIVENESS OF THE QUASI-D COMBUSTION MODEL FOR SI ENGINES WITH FLEXIBLE INTAKE SYSTEMS.pdf:pdf},
journal = {Int. J. Automot. Technol.},
number = {1},
pages = {1--9},
title = {{Improving the Predictiveness of the Quasi-D Combustion Model for Spark Ignition Engines with Flexibles Intake Systems}},
volume = {12},
year = {2011}
}
@article{Zhen2012,
abstract = {Knocking combustion in spark-ignition (SI) engines is an abnormal combustion phenomenon which can constrain the engine performance and thermal efficiency. It can also result in severe permanent engine damage under certain operating conditions. This paper systematically reviews the engine knock phenomenon, including the mechanisms, influencing factors, consequences and detection methods etc. It introduces the visualization researches, simulations and some judging indexes of engine knock. Three mathematical models which can predict the engine knock, and various kinds of methods of suppressing knock are summarized. Finally, this paper puts forward some new suggestions on the weakness in the researches of knocking combustion. {\textcopyright} 2011 Elsevier Ltd.},
author = {Zhen, Xudong and Wang, Yang and Xu, Shuaiqing and Zhu, Yongsheng and Tao, Chengjun and Xu, Tao and Song, Mingzhi},
doi = {10.1016/j.apenergy.2011.11.079},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Klopfen{\_}Ottomotor/2012{\_}Zhen{\_}The engine knock analysis - an overview about models and index.pdf:pdf},
isbn = {0306-2619},
issn = {03062619},
journal = {Appl. Energy},
keywords = {Detection methods,Knock,Models,Simulations,Suppressing methods,Visualization researches},
pages = {628--636},
publisher = {Elsevier Ltd},
title = {{The engine knock analysis - An overview}},
url = {http://dx.doi.org/10.1016/j.apenergy.2011.11.079},
volume = {92},
year = {2012}
}
@article{Ritchie1985a,
abstract = {Relationships between crack initiation and crack growth toughness are reviewed by examining the crack tip fields and microscopic (local) and macroscopic (continuum) fracture criteria for the onset and continued quasi-static extension of cracks in ductile materials. By comparison of the micromechanisms of crack initiation via transgranular cleavage and crack initiation and subsequent growth via microvoid coalescence, expressions are shown for the fracture toughness of materials in terms of microstructural parameters. Utilizing the exact asymptotic crack tip deformation fields for the nonstationary plane strain Mode I crack and evoking various microscopic failure criteria for such stable crack growth, a relationship between the tearing modulus TR and the nondimensionalized crack initiation fracture toughness Jlc is described and shown to yield a good fit to experimental toughness data for a wide range of steels},
author = {Ritchie, R O and Thompson, A W},
doi = {10.1007/BF02815305},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/1985{\_}RichtieAndThompson{\_}On Macroscopic and Microscopic Analyses for Crack Initiation and Crack Groth Toughness in Ductile Alloys.pdf:pdf},
isbn = {0360-2133},
issn = {03602133},
journal = {Met. Trans. A},
number = {1},
pages = {233--248},
title = {{On macroscopic and microscopic analyses for crack initiation and crack growth toughness in ductile alloys}},
volume = {16},
year = {1985}
}
@article{Darstellungb,
author = {Darstellung, Zur and Hilfe, Mit and Geschwindigkeit, Position and Verbindungsreaktion, Beschleunigung and Impuls, Lastenreaktion},
pages = {70--92},
title = {{7 Bewegungssimulation}}
}
@article{Wallentowitz2006o,
author = {Wallentowitz, Henning and Reif, Konrad},
doi = {10.1007/978-3-8348-9121-1_7},
journal = {Handb. Kraftfahrzeugelektronik - Grundlagen, Kompon. Syst. Anwendungen},
title = {{Komfortsysteme}},
url = {http://www.springerlink.com/index/10.1007/978-3-8348-9121-1{\_}7},
year = {2006}
}
@article{Schumacher2013a,
author = {Schumacher, Axel},
doi = {10.1007/978-3-642-34700-9},
isbn = {9783642347009},
journal = {Optimierung Mech. Strukt.},
title = {{Mathematische Grundlagen der Optimierung 3}},
year = {2013}
}
@article{Demuynck2011a,
abstract = {Hydrogen-fueled internal combustion engines are a possible solution to make transportation more ecological. Only emissions of oxides of nitrogen (NOx) occur at high loads, being a constraint for power and efficiency optimization. A thermodynamic model of the engine cycle enables a cheap and fast optimization of engine settings. It needs to accurately predict the heat transfer in the engine because the NOxemissions are influenced by the maximum gas temperature. However, the existing engine heat transfer models in the literature are developed for fossil fuels and they have been cited to be inaccurate for hydrogen. We have measured the heat transfer inside a spark ignited engine with a thermopile to investigate the heat transfer process of hydrogen and to find the differences with a fossil fuel. This paper describes the effects of the compression ratio, ignition timing and mixture richness on the heat transfer process, comparing hydrogen with methane. A convection coefficient is used to separate the effect of the temperature difference between the gas and the wall from the influence of the gas movement and combustion. The paper shows that the convection coefficient gives more insight in the heat transfer process in a combustion engine despite the assumptions involved in its definition. The comparison between hydrogen and methane demonstrates, in contrast to what is believed, that the heat loss of hydrogen can be lower. {\textcopyright} 2010 Elsevier Ltd. All rights reserved.},
author = {Demuynck, Joachim and {De Paepe}, Michel and Huisseune, Henk and Sierens, Roger and Vancoillie, Jeroen and Verhelst, Sebastian},
doi = {10.1016/j.applthermaleng.2010.12.023},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Heat Transfer Combustion Chamber/2011{\_}Demuynck{\_}Investigation of the inflence of engine settings on the heat flux in a hydrogen- and methane-fueled SI engine.pdf:pdf},
isbn = {1359-4311},
issn = {13594311},
journal = {Appl. Therm. Eng.},
keywords = {Experimental,Heat transfer,Hydrogen,Internal combustion engine,Methane,Thermopile},
number = {6-7},
pages = {1220--1228},
publisher = {Elsevier Ltd},
title = {{Investigation of the influence of engine settings on the heat flux in a hydrogen- and methane-fueled spark ignition engine}},
url = {http://dx.doi.org/10.1016/j.applthermaleng.2010.12.023},
volume = {31},
year = {2011}
}
@article{Strecke2004,
abstract = {Bevor wir einige Grundbegriffe der Thermodynamik einf{\"{u}}hren, gehen wir kurz auf ihre geschichtliche Entwicklung ein und versuchen dann, die Frage zu beantworten: Was ist Thermodynamik? In den darauf folgenden Ab- schnitten definieren wir das thermodynamische System und behandeln seine Beschreibung durch Zustandsgr{\"{o}}{\ss}en. Dabei f{\"{u}}hren wir den f{\"{u}}r die klassische Thermodynamik grundlegenden Begriff der Phase ein. Bei der daran anschlie{\ss}enden Behandlung der thermodynamischen Prozesse erhalten wir mit dem Prinzip der Irreversibilit{\"{a}}t eine erste Formulierung des 2. Hauptsatzes der Thermodynamik. Schlie{\ss}lich f¨ uhren wir die Temperatur als die erste typisch thermodynamische Zustandsgr{\"{o}}{\ss}e ein.},
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Strecke, Ab and Formataufbaus, G Des and Blattgr{\"{o}}{\ss}en, Din},
doi = {10.1055/s-2004-834544},
eprint = {arXiv:1011.1669v3},
isbn = {9783834882851},
issn = {0302-4350},
journal = {Springer},
number = {August 1832},
pages = {1--25},
pmid = {25246403},
title = {{1 Allgemeine Grundlagen}},
url = {http://www.springerlink.com/index/w26t7673r61611tj.pdf},
year = {2004}
}
@article{Bockh2006a,
author = {B{\"{o}}ckh, P V},
doi = {10.1007/978-3-642-15959-6},
isbn = {9783642159596},
journal = {Springer},
title = {{Warmeleitung in ruhenden stoffen}},
year = {2006}
}
@article{Gibbs1998,
author = {Gibbs, Hugh H.},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/{\_}buecherSong/HandbookofComposites/I/04{\_}HighTemperatureResins.pdf:pdf},
isbn = {1859573894},
journal = {Handb. Compos.},
pages = {75--98},
title = {{High Temperature Resins}},
year = {1998}
}
@article{Randbedingungen,
author = {Randbedingungen, Die},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Mathematik/Funktionale{\_}Konvexitaet{\_}UniKoeln.pdf:pdf},
title = {{Variationsrechnung Kapitel 4 Die zweite Variation und Konvexit ¨ at}}
}
@article{Soyhan2009,
abstract = {Combustion in HCCI engines is a controlled auto-ignition of well-mixed fuel, air and residual gas. The thermal conditions of the combustion chamber are governed by chemical kinetics strongly coupled with heat transfer from the hot gas to the walls. The heat losses have a critical effect on HCCI ignition timing and burning rate, so it is essential to understand heat transfer process in the combustion chamber in the modeling of HCCI engines. In the present paper, a comparative analysis is performed to investigate the performance of well-known heat transfer correlations in an HCCI engine. The results from the existing correlations are compared with the experimental results obtained in a single-cylinder engine. Significant differences are observed between the heat transfer results obtained by using Woschni, Assanis and Hohenberg correlations. ?? 2008 Elsevier Ltd. All rights reserved.},
author = {Soyhan, H S and Yasar, H and Walmsley, H and Head, B and Kalghatgi, G T and Sorusbay, C},
doi = {https://doi.org/10.1016/j.applthermaleng.2008.03.014},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2008{\_}Soyhan{\_}Evaluation of heat transfer correlations for HCCI engine modeling.pdf:pdf},
journal = {Appl. Therm. Eng.},
keywords = {HCCI,Heat transfer correlations,Modeling,Ricardo Hydra engine},
number = {2-3},
pages = {541--549},
publisher = {Elsevier Ltd},
title = {{Evaluation of heat transfer correlations for HCCI engine modeling}},
volume = {29},
year = {2009}
}
@article{Negi2015,
author = {Negi, Anjna},
doi = {10.1016/j.pedn.2008},
isbn = {0514190450},
issn = {1095-9203},
number = {2},
pages = {464--467},
pmid = {12399572},
title = {{References 1.}},
volume = {6},
year = {2015}
}
@article{Stanley1999a,
abstract = {This paper presents a simplified piston ring assembly (PRA) friction model of the piston ring pack and the piston skirt. The ring model considers both mixed and hydrodynamic lubrication; the skirt model considers hydrodynamic lubrication only. The Reynold's equation is used as a governing equation for the hydrodynamic regimes of both models. Simplified assumptions are used to include mixed lubrication in the ring model. The ring model generates unique Stribeck curves for a given ring's geometry; the skirt model generates generic relationships between the friction force and skirt geometry, piston speed, oil viscosity, and assumed boundary conditions. Inter-ring starvation effects are introduced by varying the boundary conditions, as appropriate. The models are compared to measurements made on a motored and fired single-cylinder diesel engine; the theoretical calculations provide a reasonable estimate of the measured data. .},
author = {Stanley, Richard and Taraza, Dinu and Henein, Naeim and Bryzik, Walter},
doi = {10.4271/1999-01-0974},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Mechanik+Reibung/1999{\_}Stanley{\_}A Simplified Friction Model of the Piston Ring Assembly.pdf:pdf},
isbn = {SAE 1999-01-0974},
number = {724},
title = {{A Simplified Friction Model of the Piston Ring Assembly}},
url = {http://papers.sae.org/1999-01-0974/},
year = {1999}
}
@article{Gegensatz,
author = {Gegensatz, Im and Anteil, Der and Aufladung, Die and Lau-, Im and Konzepte, Downsizing- and Auf-, Andere},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/Motoren/Golloch{\_}Downsizing/chp{\_}10.1007{\_}3-540-27490-1{\_}4.pdf:pdf},
title = {{4 Relevante Subsysteme und Prozesse}}
}
@article{Cherkaoui2009d,
author = {Cherkaoui, Mohammed and Capolungo, Laurent},
doi = {10.1007/978-0-387-46771-9},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Atomistic and Continuum Modeling of Nanocrystalline Materials/Chapter 02.pdf:pdf},
isbn = {978-0-387-46765-8},
pages = {29--52},
title = {{Atomistic and Continuum Modeling of Nanocrystalline Materials}},
url = {http://link.springer.com/10.1007/978-0-387-46771-9},
volume = {112},
year = {2009}
}
@article{Kapitele,
author = {Kapitel, Dieses and Zeitsignale, Derartige and Faltung, Die and Erinnerung, Zur and Entwicklung, Potenzreihen-},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Mathematik/Fourier Faltung Overview{\_}ETHZ.pdf:pdf},
title = {{Fourier-Transformation 6.1}}
}
@article{Crashlastfallen,
author = {Crashlastf{\"{a}}llen, Optimierung},
journal = {Auslegung A Grad. J. Philos.},
title = {{9 Weitere exemplarische Anwendungen der Strukturoptimierung}}
}
@article{Gestaltoptimierung1992,
author = {Gestaltoptimierung, Methoden},
number = {c},
title = {{7 Methoden zur Gestaltoptimierung}},
year = {1992}
}
@article{Kerbwirkunga,
author = {Kerbwirkung, Bedeutung Der},
doi = {10.1007/978-3-540-71459-0},
isbn = {978-3-540-71458-3},
title = {{4 Kerbwirkung 4.1}}
}
@article{Kochmann2009a,
author = {Kochmann, D. M. and Hackl, Klaus. and Le, K. C.},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/2009{\_}Le{\_}A continuum dislocation theory for modeling dislocation microstructures in crystal plasticity.pdf:pdf},
journal = {Conf. Pap.},
keywords = {abstract,and pile up near,anisms related to the,continuum mechanics,dislocation,dislocation network,high degree on the,in order to accommodate,material moderling,mech-,microstructure,new dislocations are nucleated,plastic deformation and,plastic deformation of crystalline,plasticity,s energy,solids depends to a,the grain or,to reduce the crystal},
number = {September},
pages = {7--11},
title = {{a Continuum-Dislocation Theory for Modeling Dislocation Microstructures and Size Effects in Crystal Plastiticy}},
year = {2009}
}
@article{Mroz2003a,
author = {Mr{\'{o}}z, Z. and Maciejewski, J.},
doi = {10.1007/978-3-540-36418-4_3},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Anisotropic Behaviouir of Damaged Materials{\_}Skrzypek{\_}ARTICEL/Kap3{\_}Failure Criteria and Compliance Variation of Anisotropically Damaged Materials.pdf:pdf},
isbn = {9783642055874},
issn = {16137736},
journal = {Lect. Notes Appl. Comput. Mech.},
keywords = {Failure condition,anisotropic damage,critical plane,strength variation},
pages = {75--112},
title = {{Failure Criteria and Compliance Variation of Anisotropically Damaged Materials}},
volume = {9},
year = {2003}
}
@article{Mughrabi2010,
abstract = {In the first part, some fundamental issues that have been under discussion for a long time will be revisited, namely the effect of the cyclic slip mode on the fatigue-induced dislocation distributions, the origin and effect of cyclic slip irreversibilities and their relation to fatigue life and, finally, cyclic strain localization and fatigue crack initiation in persistent slip bands. In the second part, some topics that have recently found increasing interest will be discussed such as the cyclic deformation and fatigue behaviour of ultrafine-grained and nanostructured materials and the microstructural mechanisms that govern fatigue life of ductile and high-strength materials in the range of ultrahigh cycle fatigue. Some general conclusions will be drawn. ?? 2010 Published by Elsevier Ltd.},
author = {Mughrabi, Hael},
doi = {10.1016/j.proeng.2010.03.003},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2010{\_}Mughrabi{\_}Fatigue, an everlasting materials problem-still en vogue{\_}FatigueSlipBands-Overview.pdf:pdf},
isbn = {1877-7058},
issn = {18777058},
journal = {Procedia Eng.},
keywords = {Cyclic slip irreversibilities,Cyclic slip mode,Fatigue lives,Microstructural effects,Ultrafine-grained metals,Ultrahigh Cycle Fatigue (UHCF)},
number = {1},
pages = {3--26},
publisher = {Elsevier},
title = {{Fatigue, an everlasting materials problem - Still en vogue}},
url = {http://dx.doi.org/10.1016/j.proeng.2010.03.003},
volume = {2},
year = {2010}
}
@article{Haslam2013b,
author = {Haslam, Antony and Laskaridis, Panos},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2010{\_}Jaroslav Pokluda+Pavel {\v{S}}andera{\_}Micromechanisms of fracture and fatigue{\_}Buch/Kap4{\_}FatigueFracture.pdf:pdf},
title = {{Fatigue {\&} Fracture}},
year = {2013}
}
@article{Haque,
author = {Haque, Enarnul and Leach, Burr Bud L},
journal = {Composites},
title = {{Matched Metal Compression Molding of Polymer Composites}}
}
@article{Borg2006,
author = {Borg, Jm and Alkidas, Ac},
doi = {10.4271/2006-01-3341},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2006{\_}Borg{\_}Characterisation of autoignition in a knocking si engine using heat release analysis.pdf:pdf},
journal = {SAE Tech. Pap.},
number = {724},
pages = {776--790},
title = {{Characterization of autoignition in a knocking SI engine using heat release analysis}},
url = {http://papers.sae.org/2006-01-3341/},
volume = {2006-01-33},
year = {2006}
}
@article{Method,
author = {Method, Finite Element and Method, Boundary Element and Analysis, Transformation Field and Tanaka, Mori},
title = {{3 Elastoplastic Problems}}
}
@article{Erma,
author = {Erm, Unter and Beanspruchungsablauf, Der and Versagenskriterium, Als and Vorgehensweise, Diese and Vorgaben, Den and Erweiterungen, Notwendige},
title = {{2 Schwingfestigkeit 2.1}}
}
@article{Stoßfanger,
author = {Sto{\ss}f{\"{a}}nger, Vordere},
pages = {164--169},
title = {{24 Vorderwagen}}
}
@article{Unsymmetrie,
author = {Unsymmetrie, Das Naturgesetz Der},
title = {{5. Die Entropiebilanz}}
}
@article{Berdichevsky2006,
abstract = {hepapercontinuesthediscussionofcontinuumtheoryofdislocationssuggestedbyBerdichevsky and Sedov (PMM 31(6): 981--1000, 1967). The major new points are: the choice of energy, the variational form of the governing dynamical equations, the variational principle for the final plastic state.},
author = {Berdichevsky, Victor L.},
doi = {10.1007/s00161-006-0024-7},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/2006{\_}Berdichevsky{\_}Continuum theory of dislocations revisited.pdf:pdf},
issn = {09351175},
journal = {Contin. Mech. Thermodyn.},
keywords = {Continuum theory of dislocations,Plastic spin,Strain gradient plasticity},
number = {3-4},
pages = {195--222},
title = {{Continuum theory of dislocations revisited}},
volume = {18},
year = {2006}
}
@article{Linear2014,
author = {Linear, D},
doi = {10.1016/B978-1-85617-635-4.00029-7},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Zienkiewicz FEM - Vol 3 Fluid Dynamics/63229{\_}apdxd.pdf:pdf},
isbn = {9781856176354},
journal = {Finite Elem. Method Fluid Dyn.},
pages = {509--510},
title = {{Integration Formulae}},
url = {http://linkinghub.elsevier.com/retrieve/pii/B9781856176354000297},
year = {2014}
}
@article{Forest2004a,
abstract = {The modeling of damage processes at the material point scale through a specific constitutive law addresses a wide variety of constitutive behaviors, for instance brittle elasticity where the evolution of damage degrades the elastic stiffness, or ductile plasticity where both dissipative mechanisms (plasticity and damage) are intimately coupled. In spite of their obvious differences, all these laws possess a common feature: beyond some load level, the domain of reversibility expressed in the stress space shrinks. This phenomenon is called strain-softening. This essential property, characteristic of damage mechanisms, is responsible for the localization of the mechanical fields (strain, damage, plastic strain, . . .) inside narrow bands, an experimental fact observed on many degrading materials such as soils, concrete, metals, etc., see for instance Desrues and Chambon (1985). Despite twenty years of intensive research, numerical modeling of the localization phenomenon remains a challenging objective which has not yet been given a fully satisfactory answer. This is in contrast with the great progresses that have been achieved regarding the local description of damage mechanisms for various materials, on the basis of micro–macro derivations as well as phenomenological intuitions. Unfortunately, localization partially hinders predictive computations of propagating damaged zones in real-life structures submitted to a given load history. The difficulty originates from the fact that the equations that describe the structural behavior (including not only the constitutive law but also the equilibrium and compat-ibility equations) result in an ill-posed problem which manifests itself by a spurious mesh-dependency when making use of finite element solutions. After a first insight into the localization phenomena, the problem of loss of uniqueness and loss of ellipticity is addressed for elastoplastic solids. General (diffuse) and localized bifurcation modes are distinguished. The existence of jumps of the velocity gradient is explored in the dynamic (acceleration waves) and static cases (stationary waves). Critical values of hardening moduli for loss of uniqueness or loss of ellipticity are derived. A link between the notion of material stability and acceleration waves is also presented. The collected strain localization criteria are summarized in section 1.2.6. Note that the derivations and formula are presented in the case of elastoplastic ma-terials. However the results can be extended to damaging materials in a straightforward 311 312 Local approach to fracture manner. In fact it deals with all incremental models involving a fourth–rank tangent operator L ∼ ∼ .},
author = {Forest, S and Lorentz, E},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/xxx{\_}Forst+Lorentz{\_}Localization{\_}phenomena{\_}and{\_}regularization{\_}methods-damage.pdf:pdf},
journal = {Local Approach to Fract.},
pages = {311--371},
title = {{Localization phenomena and regularization methods}},
volume = {1},
year = {2004}
}
@article{Stromkreis,
author = {Stromkreis, Der},
pages = {4--26},
title = {{2 Gleichstromtechnik}}
}
@article{Essmann1981a,
abstract = {Based on recent experimental observations a realistic model of the evolution of the surface profile of persistent slip bands (PSBs) in fatigued metals is proposed. An essential feature of the model is the production of vacancies by the annihilation of edge dislocations which, combined with irreversible slip processes, leads to an elongation of the PSB parallel to the active slip vector. It is shown that a net extrusion forms rather rapidly. The growth processes and their dependence on temperature are discussed in detail. It is proposed that cracks initiate at the surface steps at the PSB{\&}ndash;matrix interface and, at a later stage, also at the notch-peak profile from the random slip processes.},
author = {Essmann, U. and G{\"{o}}sele, U. and Mughrabi, H.},
doi = {10.1080/01418618108239541},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2016{\_}Mughrabi{\_}A model of extrusions and intrusions in fatigued metals I  Point defect production and the growth of extrusions.pdf:pdf},
isbn = {0141-8610},
issn = {0141-8610},
journal = {Philos. Mag. A},
number = {2},
pages = {405--426},
title = {{A model of extrusions and intrusions in fatigued metals I. Point-defect production and the growth of extrusions}},
url = {http://www.tandfonline.com/doi/abs/10.1080/01418618108239541},
volume = {44},
year = {1981}
}
@article{Mizuno2009,
abstract = {This study examined a method of predicting the piston temperature in reciprocating internal combustion engines with the aim of developing lightweight pistons. Since the piston temperature is strongly affected by the in-cylinder temperature distribution and turbulence, it is necessary to consider the effects of flame propagation, cooling by the intake air, temperature rise due to combustion, in-cylinder flow and the combustion chamber shape. A three-dimensional combustion simulation that can take these effects into consideration was run to calculate the heat transfer coefficient from the piston crown surface and the gas temperature. The results were used as the boundary conditions for an analysis of heat transfer from the piston, and a method was thus developed for analyzing the piston temperature. The hardness method was used to obtain the piston temperature distribution and maximum temperature during engine operation, and a comparison was made with the analytical results to examine the effects of flame propagation.},
author = {Mizuno, Hideaki and Ashida, Koichi and Teraji, Atsushi and Ushijima, Kenshi and Takemura, Shinichi},
doi = {10.4271/2009-01-0187},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2009{\_}Mizuno{\_}Transient Analysis of the Piston Temperature with Measurement and Simulation.pdf:pdf},
isbn = {9200901018},
issn = {1946-3944},
journal = {SAE Int. J. Engines},
number = {1},
pages = {2009--01--0187},
title = {{Transient Analysis of the Piston Temperature with Consideration of In-cylinder Phenomena Using Engine Measurement and Heat Transfer Simulation Coupled with Three-dimensional Combustion Simulation}},
url = {http://papers.sae.org/2009-01-0187/},
volume = {2},
year = {2009}
}
@article{Cherkaoui2009,
author = {Cherkaoui, Mohammed and Capolungo, Laurent},
doi = {10.1007/978-0-387-46771-9},
isbn = {978-0-387-46765-8},
pages = {117--142},
title = {{Atomistic and Continuum Modeling of Nanocrystalline Materials}},
url = {http://link.springer.com/10.1007/978-0-387-46771-9},
volume = {112},
year = {2009}
}
@article{Luk????1968a,
abstract = {Persistent slip bands in fatigued copper single crystals are studied by means of transmission electron microscopy of surface thin foils, both parallel and nonparallel to the surface. Comparing the observations from the different nonparallel sections a three-dimensional model of the internal structure may be constructed. Dislocations with all six possible Burgers vectors of the type 1/2 〈0011〉 are found in the structure. This demonstrates the microscopic action of the secondary slip systems during the low stress fatigue. The macroscopic action of the secondary systems, which is connected with the cell structure formation, is typical for the high stress fatigue. Surface extrusions are found to be related to the dislocation structure below the surface.},
author = {Luk????, P and Klesnil, M and Krej????, J},
doi = {10.1002/pssb.19680270212},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/1968{\_}Luka{\_}Dislocations and persistent slip bands in copper single crystals fatigued at low stress amplitude.pdf:pdf},
isbn = {0031-8957},
issn = {15213951},
journal = {Phys. Status Solidi},
number = {2},
pages = {545--558},
title = {{Dislocations and Persistent Slip Bands in Copper Single Crystals Fatigued at Low Stress Amplitude}},
volume = {27},
year = {1968}
}
@article{Kettemrades,
author = {Kettemrades, Teilkreisdurchmesser},
pages = {215--220},
title = {{17 Kettentriebe}},
volume = {8152}
}
@article{Verbindungen2007,
author = {Verbindungen, Wechselnde},
journal = {Fahrzeuggetriebe},
title = {{9 Schalteinrichtungen}},
year = {2007}
}
@article{Saugmotor,
author = {Saugmotor, Ein and Gegensatz, Im and Motoren, Aufgeladene and Drehmomentverlauf, Der},
pages = {161--187},
title = {{6 Aufladung}}
}
@article{Brosdorf2005,
author = {Br{\"{o}}sdorf, Klaus-dieter and Moser, Andreas and Burg, J{\"{u}}rgen},
pages = {27--57},
title = {{A2 A2 Unfallaufnahme und Datenerhebung A2}},
year = {2005}
}
@article{Dieselmotora,
author = {Dieselmotor, Der and Gewinn, Der and Direkteinspritzung, Die and Eingang, Verfahren},
pages = {1--2},
title = {{1 Einleitung}}
}
@article{Tanaka1982a,
abstract = {The fatigue crack initiation along the slip banks emanating from notches is analyzed theoretically with the use of the dislocation dipole accumulation model proposed previously by the authors. The complex function analysis for an elliptical notch under the anti-plane shear gives a quantitative method for assessment of the reduction of fatigue strength as a function of the notch tip radius, the notch size and the elastic stress concentration factor. Special cases of this theoretical analysis yield several semi-empirical formulae commonly used by engineers for data collection. In the derivation, the limitations for each engineering approach are clarified. The material properties are included in the present micromechanical theory as the slip band length and the dislocation frictional stress. ?? 1982.},
author = {Tanaka, K. and Mura, T.},
doi = {10.1016/0167-6636(82)90024-2},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/1981{\_}Mura+Tanaka{\_}A micromechanical theory of fatigue crack initiation from notches.pdf:pdf},
isbn = {0921-5093},
issn = {01676636},
journal = {Mech. Mater.},
number = {1},
pages = {63--73},
title = {{A micromechanical theory of fatique crack initiation from notches}},
volume = {1},
year = {1982}
}
@article{Papula2009,
abstract = {Kennzeichen der B nde des erfahrenen Hochschullehrers und erfolgreichen Autors ist die anschauliche und leicht verst ndliche Darstellungsform des mathematischen Stoffes. Mit seiner un bertroffenen didaktischen Konzeption erm glicht das Buch einen nahtlosen bergang von der Schul- zur anwendungsorientierten Hochschulmathematik. Die leicht verst ndliche und anschauliche Art der Darstellung hat das Buch zum Standardwerk der Ingenieurmathematik werden lassen.Die aktuelle Auflage enth lt ein neues Kapitel Fourier-Transformationen.},
author = {Papula, Lothar},
isbn = {3834805645},
pages = {795},
title = {{Mathematik f{\"{u}}r Ingenieure und Naturwissenschaftler 2: Ein Lehr- und Arbeitsbuch f{\"{u}}r das Grundstudium. Mit zahlreichen Beispielen aus Naturwissenschaft und Technik, 310 {\"{U}}bungsaufgaben mit ausf{\"{u}}hrlichen L{\"{o}}sungen. Mit zahlreichen Beispielen aus Naturwissensc}},
url = {http://books.google.com/books?id=vQgR9GR8nYEC{\&}pgis=1},
year = {2009}
}
@article{2015Huegel+Koch,
abstract = {In this work, heat loss was investigated in homogeneous and stratified DI-SI operation mode in a single cylinder research engine. Several thermocouples were adapted to the combustion chamber surfaces. The crank angle resolved temperature oscillations at the cylinder head and piston surface could thereby be measured in homogeneous and stratified operation mode. A grasshopper linkage was designed and adapted to the engine, to transfer the piston signals to the data acquisition device. The design of the experimental apparatus is described briefly.For both operation modes the average steady-state temperatures of the combustion chamber surfaces were compared. The temperature distribution along the individual sensor positions at the cylinder head and piston surface are shown. Furthermore, the curves of the crank angle resolved temperature oscillations in stratified and homogeneous operation mode were compared. It is shown that the local temperature curves show large variations, depending on the operation mode.Using these oscillations, the heat flux profiles were calculated and compared with each other. To calculate the heat flux at the surface of deposits and the deposit thickness, an approach was used, that allows consideration of multiple layers with different material properties and thicknesses.The differences in the heat transfer characteristics are demonstrated for a variation of spark timing in stratified operation mode. For comparison the heat transfer characteristic in homogeneous operation mode is shown at reference spark timing. Finally, the determined heat losses were compared with the predictions of existing models for instantaneous wall heat transfer and rated.},
author = {Huegel, Philipp and Kubach, Heiko and Koch, Thomas and Velji, Amin},
doi = {https://doi.org/10.4271/2015-01-0782},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Heat Transfer Combustion Chamber/2015{\_}Huegel{\_}Koch{\_}Investigations on the Heat Transfer in a Single Cylinder Research SI Engine with Gasoline DI.pdf:pdf},
journal = {SAE Int. J. Engines},
month = {apr},
number = {2},
pages = {557--569},
title = {{Investigations on the Heat Transfer in a Single Cylinder Research SI Engine with Gasoline Direct Injection}},
volume = {8},
year = {2015}
}
@article{Staubgehalt,
author = {Staubgehalt, Der and Vergleich, Zum and Daten, Diese and Abrieb, Systemen and Stellen, Kritische and Verschlei, Der and Staubkon-, Die and Luftfilter, Ein},
title = {{Ansaug- und Abgasanlagen}}
}
@article{Narasimhamurthy1957,
abstract = {BISPLINGHOFF has given a comparative graph showing the relative importance of the parameters of design at various Mach numbers. At Mach numbers above five, i.e. in the range of missile flight, creep becomes the critical design factor. Even though the time of flight of the missile is very short, and not enough to cause any considerable amount of creep, the deflexions caused will be enough to disturb the stability of compression members. Also the aerodynamic shape can be distorted with serious effects on the flow characteristics of the profile.},
author = {Narasimhamurthy, P},
doi = {10.1108/eb032892},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Kriechen{\_}Spannungsrelaxation/1957{\_}Narasimhamurthy{\_}An Analytical Investigation of creep under combined loadings.pdf:pdf},
issn = {0002-2667},
journal = {Aircr. Eng. Aerosp. Technol.},
number = {11},
pages = {346--349},
title = {{An Analytical Investigation of Creep under Combined Loadings}},
url = {http://www.emeraldinsight.com/doi/abs/10.1108/eb032892},
volume = {29},
year = {1957}
}
@article{Ekh2004a,
abstract = {We develop a model framework for anisotropic damage coupled to crystal (visco)plasticity, which is based on the concept of a fictitious (undamaged) configuration. The theoretical setting is that of finite strains, which is natural when studying crystal inelasticity even in the case of actual small strains. It turns out that the evolution law for damage, which reflects degradation in the slip planes and which is the key new relation, bears strong resemblance with the inelastic flow rule. Some numerical results showing qualitatively the anisotropic development of damage concludes the paper. ?? 2004 Elsevier Ltd. All rights reserved.},
author = {Ekh, Magnus and Lillbacka, Robert and Runesson, Kenneth},
doi = {10.1016/j.ijplas.2004.04.007},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2004{\_}Ekh{\_}A model framework for anisotropic damage coupled to crystal visco plasticity.pdf:pdf},
isbn = {0749-6419},
issn = {07496419},
journal = {Int. J. Plast.},
keywords = {Anisotropy,Crystal plasticity,Damage,Finite deformations},
number = {12},
pages = {2143--2159},
title = {{A model framework for anisotropic damage coupled to crystal (visco)plasticity}},
volume = {20},
year = {2004}
}
@article{Gurtsysteme1985,
author = {Gurtsysteme, A Technik Der and Kramer, Florian},
pages = {761--774},
title = {{C2 C2 Sicherheitsgurte C2}},
year = {1985}
}
@article{Wirsching1983,
abstract = {Two methods are discussed for constructing a design curve on the safe side of fatigue data. Both the tolerance interval and equivalent prediction interval (EPI) concepts provide such a curve while accounting for both the distribution of the estimators in small samples and the data scatter. The EPI is also useful as a mechanism for providing necessary statistics on S-N data for a full reliability analysis which includes uncertainty in all fatigue design factors. Examples of statistical analyses of the general strain life relationship are presented. The tolerance limit and EPI techniques for defining a design curve are demonstrated. Examples usng WASPALOY B and RQC-100 data demonstrate that a reliability model could be constructed by considering the fatigue strength and fatigue ductility coefficients as two independent random variables. A technique given for establishing the fatigue strength for high cycle lives relies on an extrapolation technique and also accounts for "runners." A reliability model or design value can be specified.},
author = {Wirsching, P. H.},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Probabilistic Aspects/1983{\_}Wirsching{\_}Statistical summaries of fatigue data for design purposes.pdf:pdf},
issn = {05657059},
journal = {Nasa Cr 3697},
number = {July},
title = {{Statistical Summaries of Fatigue Data for Design Purposes}},
year = {1983}
}
@article{Work2003,
author = {Work, O F Virtual},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Nicholson 2003 - Finite Element Analysis Thermomechanics of Solids/0749{\_}C10.pdf:pdf},
journal = {Work},
pages = {139--151},
title = {{Element and Global Stiffness and Mass Matrices 10.1}},
year = {2003}
}
@article{Silitonga2013a,
abstract = {Engineering methods to predict the fatigue life of structures have been available since the beginning of the 20th century. However, a practical problem arises from complex loading conditions and a significant concern is the accuracy of the methods under variable amplitude loading. This paper provides an overview of existing fatigue damage models with emphasis on relatively new alternative models and computational strategies to predict fatigue life. These models are compared and promising new capabilities are discussed.},
author = {Silitonga, S and Maljaars, J and Soetens, F and Snijder, H H},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/2013{\_} Silitonga{\_}Maljaars{\_}Soetens{\_}Snijder{\_}Survey on damage mechanics models for fatique life prediction.pdf:pdf},
issn = {15744078},
journal = {Heron},
keywords = {Cohesive zone,Continuum damage mechanics,Fatigue damage},
number = {1},
pages = {25--60},
title = {{Survey on damage mechanics models for fatigue life prediction}},
volume = {58},
year = {2013}
}
@inproceedings{Choi1997,
abstract = {Cylinder head and piston temperatures and heat fluxes were measured in a DOHC engine. Measurements for the combustion chamber were made at different engine speeds and engine loads. Twenty-one instantaneous temperature probes were totally embedded in a cylinder head and a piston. Major conclusions of this research include; 1) the instantaneous temperature on the cylinder head was affected by flame traveling distance, gas flow characteristics, and cooling passage; 2) all temperatures at the exhaust valve heads with different engine loads are much higher than those at the intake valve heads; 3) the instantaneous surface temperature at around exhaust valve pocket is higher than that at piston crown center; 4) the instantaneous temperatures of the top-ring groove and the second land are also varied; and 5) heat flux in the piston crown is largely occurred during the expansion stroke and the heat flux has dissimilar trend to the temperature distribution.},
author = {Choi, G H and Choi, K H and Lee, J T and Song, Y S and Ryu, Y and Cho, J W},
booktitle = {SAE Tech. Pap. 970895},
doi = {10.4271/970895},
file = {:C$\backslash$:/Users/p327208/Desktop/Promotion/Literature/Motorspezifisch/Heat Transfer Combustion Chamber/1997{\_}Choi{\_}Analysisi of Combustion Chamber Temperature and Heat Flux in a DOHC Engine.pdf:pdf},
publisher = {SAE International},
title = {{Analysis of Combustion Chamber Temperature and Heat Flux in a DOHC Engine}},
year = {1997}
}
@article{RajuP2011,
abstract = {This paper presents the details of method of sample size determination to estimate the characteristic fatigue life of aluminum alloy, A356.2-T6. The characteristic fatigue life of the alloy has been estimated by assuming log normal distribution model. A step wise procedure is outlined to determine the number of specimens required at predetermined stress amplitude to estimate the fatigue life with an acceptable error at 50{\{}{\%}{\}} probability and various confidence levels, 90{\{}{\%}{\}}, 95{\{}{\%}{\}} and 99{\{}{\%}{\}}. Maximum percentage of errors has also been calculated for the above probability and confidence levels. Details of generation of S-N curve for aluminum alloy A356.2-T6 using regression analysis have been explained. From this study, the adequate sample size required for evaluating the average fatigue life of A356.2-T6 with an acceptable error at 50{\{}{\%}{\}} probability and 90{\{}{\%}{\}} confidence level using log normal distribution is established. In order to check the significance of regression equation, analysis of variance (ANOVA) is performed. Copyright 2011 Tech Science Press.},
author = {{Raju P}, R and Rajesh, S and Satyanarayana, B and Ramji, K},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Probabilistic Aspects/2011{\_}Ramamurty{\_}Statistical Analysis of Fatigue Life Data of A356.2-T6 Aluminium Alloy.pdf:pdf},
journal = {Struct. Durab. Heal. Monit.},
keywords = {aluminum alloy,fatigue life,log normal distribution,s n curve},
number = {1-2},
pages = {139--152},
title = {{Statistical analysis of fatigue life data of A356.2-T6 aluminum alloy}},
url = {http://www.scopus.com/inward/record.url?eid=2-s2.0-79957943262{\%}7B{\&}{\%}7DpartnerID=40{\%}7B{\&}{\%}7Dmd5=a5890475316795056516da22de2c7672},
volume = {7},
year = {2011}
}
@article{Messtechnik,
author = {Messtechnik, Grundbegriffe Der},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Vorlesungen/Messtechnik+Regelungstechnik/gmrt06.pdf:pdf},
pages = {1--17},
title = {{6 Grundbegriffe der Messtechnik}}
}
@article{Shimp1971,
author = {Shimp, David A},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/{\_}buecherSong/HandbookofComposites/I/05{\_}SpecialityMatrixResins.pdf:pdf},
title = {{Speciality matrix resins}},
year = {1971}
}
@misc{Boeff,
author = {Boeff, Martin and Gutknecht, Florian and Engels, Philipp S and Ma, Anxin},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/2015{\_}Boeff{\_}Formulation of nonlocal damag models based on spectral methods for application to complex micostructures.pdf:pdf},
keywords = {nonlocal damage modelling,plasticity,rve,spectral solver},
title = {{Formulation of nonlocal damage models based on spectral methods for application to complex microstructures}}
}
@article{Tensors1968a,
author = {Tensors, Flux},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/Folien CISM Summer School Mai2017 - Mesoscale Models/courses{\%}2FC1703{\%}2Fgroma{\%}2Fcontinuum (1).pdf:pdf},
title = {{Continuum Theory of Dislocations and Plastleity'}},
year = {1968}
}
@article{Priester,
author = {Priester, Johannes and Kasanicky, Gustav},
pages = {383--410},
title = {{A11 A11 Unf{\{}{\"{a}}{\}}lle mit Zweir{\{}{\"{a}}{\}}dern A11 Einteilung der Zweir{\{}{\"{a}}{\}}der}}
}
@article{Cassis1998,
abstract = {2.1 INTRODUCTION AND HISTORY sored production of styrene-butadiene rubber. Organic polymers are divided into two types, reinforced-thermoplastic and thermoset. With thermoset polymers such as unsaturated poly-esters and vinyl esters, a chemical reaction cross links the material so that it cannot be returned to liquid form. Other common ther-mosetting polymers include epoxy and phenolic resins. Thermoset plastics made with polyester and vinyl ester resins represent the major portion of the reinforced plastic com-posites industry today. Early workers on unsaturated polyesters soon learned that despite the possession of reactive double bonds, these resins were slug-gish in reacting with themselves. Even with effective catalysts, they still required high tem-peratures and lengthy cure times to complete the cross linking reaction. The key to modern day application of unsaturated polyesters was the discovery by Carlton Ellis in 1937l that the addition of reactive monomers, such as styrene, gave mixtures that would copolymerize many times faster than homopolymerization. The styrene addition produced the added benefit of an easily handled liquid material that could be pumped, transported and fabricated into a fin-ished plastic by a myriad of molding processes. Developments during the 1940s accelerated the commercial applicability of unsaturated polyesters to the position they hold today. Styrene became readily available and lower in cost as a result of the US Government's spon-Handbook of Composites. Edited by S.T. Peters. Published in 1998 by Chapman {\&} Hall, London. ISBN 0 412 54020 7 At the same time, scientists found that styre-nated polyesters could yield high strength, light weight structures when reinforced with glass fibers. They also learned that fiberglass-reinforced polyesters had excellent electrical properties and that large structures could be molded at low pressures with low cost tooling. As a result, commercial development pro-ceeded rapidly after World War I1 with materials and molding research moving in many directions. In the 20 years that followed, polyester and vinyl ester resins matured rapidly and by the mid-l970s, the composites fabricator and end user had numerous options with these matrix systems to achieve the desired properties in the finished part. 2.2 POLYESTER RESINS},
author = {Cassis, Frank A. and Talbot, Robert C.},
doi = {10.1007/978-1-4615-6389-1_3},
isbn = {978-1-4615-6389-1},
issn = {07230192},
journal = {Handb. Compos.},
pages = {34--47},
title = {{Polyester and Vinyl Ester Resins}},
url = {http://link.springer.com/10.1007/978-1-4615-6389-1{\_}3},
year = {1998}
}
@article{Vikram2013,
author = {Vikram, Nirpesh and Kumar, Raghuvir},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/2013{\_}Vikram+Kumar{\_}Review-on-Fatigue-Crack-Growth-and-Finite-Element-Method.pdf:pdf},
journal = {Int. J. Sci. Eng. Res.},
number = {4},
pages = {833--843},
title = {{Review on Fatigue-Crack Growth and Finite Element Method}},
url = {http://www.ijser.org/researchpaper{\%}7B{\%}25{\%}7D5CReview-on-Fatigue-Crack-Growth-and-Finite-Element-Method.pdf},
volume = {4},
year = {2013}
}
@article{Produkt,
author = {Produkt, Das},
journal = {Differentiation},
pages = {116--133},
title = {{6 Zustandsgleichungen Idealer Gase}}
}
@article{Taylor1957,
author = {Taylor, C F and Toong, T Y},
journal = {ASME Pap. 57-HT-17},
title = {{Heat Transfer in Internal-combustion Engines}},
volume = {(1957)}
}
@book{Cherkaoui2009b,
author = {Cherkaoui, Mohammed and Capolungo, Laurent},
doi = {10.1007/978-0-387-46771-9},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Atomistic and Continuum Modeling of Nanocrystalline Materials/Chapter 04.pdf:pdf},
isbn = {978-0-387-46765-8},
title = {{Atomistic and Continuum Modeling of Nanocrystalline Materials}},
url = {http://link.springer.com/10.1007/978-0-387-46771-9},
volume = {112},
year = {2009}
}
@article{McDowell2007,
abstract = {Further efforts to provide more direct dependence of fatigue life estimation methods on microstructure of alloy systems must consider various factors that are not explicitly addressed by conventional fatigue design tools such as the strain-life curve, the stress-life curve, the modified Goodman diagram, or fatigue limit concepts, or by traditional linear elastic fracture mechanics approaches. In this work, we offer insight from micromechanical perspectives on tradeoffs of fatigue crack formation and growth regimes in low cycle and high cycle fatigue, including considerations of effects of notches of various scales. Relations between remote loading conditions and microstructure-scale cyclic plasticity/crack behavior are considered as a function of stress amplitude and microstructure to support assessment of intrinsic microstructure fatigue resistance (percolation limits for connected microplasticity) as well as effects of extrinsic features such as non-metallic inclusions. Algorithms are summarized for computing nonlocal cyclic plastic shear strain and inferring fatigue resistance, both in terms of mean behavior and variability with microstructure. Several applications are presented, including intrinsic and extrinsic fatigue resistance of Ni-base superalloys, fatigue of polycrystals, cast A356-T6 Al alloy, and fretting fatigue of Ti-6Al-4V. {\{}{\textcopyright}{\}} 2007 Elsevier B.V. All rights reserved.},
author = {McDowell, David L},
doi = {10.1016/j.msea.2006.08.129},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/2006{\_}McDowell{\_}Simulation-based strategies for microstructure-sensitive fatigue modeling.pdf:pdf},
isbn = {0921-5093},
issn = {09215093},
journal = {Mater. Sci. Eng. A},
keywords = {Computational fatigue,Hierarchical microstructure,Microstructure,Simulation-based fatigue},
number = {SPEC. ISS.},
pages = {4--14},
title = {{Simulation-based strategies for microstructure-sensitive fatigue modeling}},
volume = {468-470},
year = {2007}
}
@article{Rostampour2015,
abstract = {This investigation deals with the EF7 (TC) engine, a dual fuel engine equipped with a turbocharger system, consequently with a high probability of knock inception. In this study, an operating cycle of the engine was simulated using KIVA-3V code. Some modifications were carried out on the KIVA method of calculating pressure in the intake port in order to simulate turbocharger pressure correctly. Auto-ignition and knock were then simulated using the auto-ignition integral model. The modified code and the simulation were verified using three different methods; in-cylinder average pressure, gas temperature of the exhaust port, and auto-ignition timing. The simulation results using the auto-ignition integral model, as compared with the experimental data, proved to be reasonably accurate. Following this validation, the effect of the knock phenomenon on the engine heat transfer through the walls was investigated. The simulations showed that the rate of heat transfer through the walls under knocking conditions is about 2.2 times higher than that under normal conditions. However, it was also shown that the total heat transfer increases about 15{\{}{\%}{\}}.},
author = {Rostampour, Arman and Toosi, Ali Nassiri},
doi = {10.1115/1.4030517},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2015{\_}Rostampour{\_}Numerical Investigation of the effect of knock on heat transfer in a turbo si engine.pdf:pdf},
issn = {0742-4795},
journal = {J. Eng. Gas Turbines Power},
number = {12},
pages = {121502},
title = {{Numerical Investigation of the Effect of Knock on Heat Transfer in a Turbocharged Spark Ignition Engine}},
url = {http://www.scopus.com/inward/record.url?eid=2-s2.0-84930634240{\%}7B{\&}{\%}7DpartnerID=tZOtx3y1},
volume = {137},
year = {2015}
}
@article{Rousselier1987a,
abstract = {Since the pioneering studies conducted by McClintock, Rice and Tracey on the growth of cavities, many studies have covered modelling of ductile fracture; a non-exhaustive list is given of these studies. In the local approach of fracture, the models are used at the tip of cracks, and in the present state, only relatively simple models can be used to solve fracture problems in a complete manner, from material characterization to the analysis of cracked structures. The paper presents two types of models based on a critical ratio of cavity growth or on continuum damage mechanics. In the framework of the local approach of fracture, their possibilities are presented with constant references to experimental validation studies. This allows conclusions to be drawn regarding the effectiveness of the methods proposed and their undeniable contribution to fracture mechanics. ?? 1987.},
author = {Rousselier, G},
doi = {10.1016/0029-5493(87)90234-2},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Plasticity models/Ductile fracture models and their potential in local approach of fracture{\_}Rousselier.pdf:pdf},
isbn = {00295493},
issn = {00295493},
journal = {Nucl. Eng. Des.},
number = {1},
pages = {97--111},
title = {{Ductile fracture models and their potential in local approach of fracture}},
volume = {105},
year = {1987}
}
@article{Sangid2011a,
abstract = {In many engineering applications, fatigue is the dominant failure mechanism governing the life of a component. Thus, many studies have focused on this phenomenon, although there is a need for a model that addresses fatigue based on the material's microstructure, specifically the energetics of the grain boundaries (GBs) and persistent slip bands (PSBs). Our approach is to model the energy of a PSB structure and use its stability with respect to dislocation motion as our failure criterion for fatigue crack initiation. The components that contribute to the energy of the PSB are identified, namely the stress field resulting from the applied external forces, dislocation pile-ups and work-hardening of the material is calculated at the continuum scale. Further, energies for dislocations creating slip in the matrix/precipitates, interacting with the GBs and nucleating/agglomerating within the PSB are computed via molecular dynamics. The results of our simulations on the stability of a PSB produce the correct fatigue crack initiation trends for the grain size, grain orientation, character of the GB, precipitate volume fraction and applied strain. From this information, we see that distinct GBs act as strong barriers to slip and increase the fatigue strength of the material. ?? 2010 Acta Materialia Inc. Published by Elsevier Ltd. All rights reserved.},
author = {Sangid, Michael D and Maier, Hans J and Sehitoglu, Huseyin},
doi = {10.1016/j.actamat.2010.09.036},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2010{\_}Sehitoglu{\_}A physically based fatigue model for prediction of crack initiation from persistent slip bands in polycrystals.pdf:pdf},
isbn = {1359-6454},
issn = {13596454},
journal = {Acta Mater.},
keywords = {Coincidence site lattice (CSL),Crack initiation,Fatigue,Grain boundaries,Persistent slip bands},
number = {1},
pages = {328--341},
publisher = {Acta Materialia Inc.},
title = {{A physically based fatigue model for prediction of crack initiation from persistent slip bands in polycrystals}},
url = {http://dx.doi.org/10.1016/j.actamat.2010.09.036},
volume = {59},
year = {2011}
}
@article{Objekte,
author = {Objekte, Ue and Anzahl, Die and Untersuchungsobjekte, Die and Unter, Grundgesamtheit and Grundge-, Die and Auswahl, Die and Elemente, Ue and Stichprobenwerte, Ben and Elemen-, Ue},
title = {{XVI Grundlagen der mathematischen Statistik}}
}
@article{Yahya2005,
author = {Yahya, S M},
doi = {10.1016/j.ijantimicag.2012.06.019},
isbn = {0132592010},
number = {6},
pages = {22--24},
title = {{References [1]}},
volume = {76},
year = {2005}
}
@article{Clement,
author = {Clement, Steffen and Informationstechnik, Elektro- and Klein, Bernd and Engelken, Gerhard and Konstruktion, Maschinenelemente and Czichos, Horst and Theumert, Hans and Maschinenbau, Grundlagen and Hei, Bernd and Ersoy, Metin and Isermann, Rolf and Schabacker, Michael and Fiala, Ernst and Klette, Guido},
isbn = {9783528331245},
journal = {Konstruktion},
title = {{Aus dem Programm}}
}
@article{Gurson1977,
abstract = {Widely used constitutive laws for engineering materials assume plastic incompressibility, and no effect on yield of the hydrostatic component of stress. However, void nucleation and growth (and thus bulk dilatancy) are commonly observed is some processes which are characterized by large local plastic flow, such as ductile fracture.},
author = {Gurson, A. L.},
doi = {10.1115/1.3443401},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Plasticity models/Continuum Theory of Ductile Rupture by Void Nucleation and  Growth-PartI{\_}ByGurson.pdf:pdf},
isbn = {0094-4289},
issn = {00944289},
journal = {J. Eng. Mater. Technol.},
number = {1},
pages = {2},
title = {{Continuum Theory of Ductile Rupture by Void Nucleation and Growth: Part I—Yield Criteria and Flow Rules for Porous Ductile Media}},
url = {http://materialstechnology.asmedigitalcollection.asme.org/article.aspx?articleid=1422194},
volume = {99},
year = {1977}
}
@article{Gross2011h,
author = {Gross, Dietmar and Seelig, Thomas},
doi = {10.1007/978-3-642-10196-0},
isbn = {978-3-642-10195-3},
title = {{Bruchmechanik}},
url = {http://link.springer.com/10.1007/978-3-642-10196-0},
year = {2011}
}
@article{Vorl1908,
author = {Vorl, Als},
number = {1829},
title = {{2 Wasserturbinen}},
year = {1908}
}
@article{Bestimmung,
author = {Bestimmung, Die},
title = {{3. Geschwindigkeitsmessung}}
}
@article{Taylor--galerkin,
author = {Taylor--galerkin, E The},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Zienkiewicz FEM - Vol 3 Fluid Dynamics/63229{\_}apdxe.pdf:pdf},
journal = {Order A J. Theory Ordered Sets Its Appl.},
title = {{Convection--diffusion equations : vector-valued variables and differentiating}}
}
@article{Mcdowell2017,
author = {Mcdowell, David L},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/Folien CISM Summer School Mai2017 - Mesoscale Models/courses{\%}2FC1703{\%}2Fmcdowell{\%}2FCISM.multiscale+crystal+plasticity.mcdowell.lecture1.final.pdf:pdf},
title = {{Multilevel Crystal Plasticity From nm to mm}},
year = {2017}
}
@article{Mroz2003,
author = {Mr{\'{o}}z, Z and Maciejewski, J},
doi = {10.1007/978-3-540-36418-4_3},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Anisotropic Behaviouir of Damaged Materials{\_}Skrzypek{\_}ARTICEL/Kap3{\_}Failure Criteria and Compliance Variation of Anisotropically Damaged Materials.pdf:pdf},
isbn = {9783642055874},
issn = {16137736},
journal = {Lect. Notes Appl. Comput. Mech.},
keywords = {Failure condition,anisotropic damage,critical plane,strength variation},
pages = {75--112},
title = {{Failure Criteria and Compliance Variation of Anisotropically Damaged Materials}},
volume = {9},
year = {2003}
}
@article{Kress2004,
author = {Kress, Gerald},
journal = {Cent. Struct. Technol. ETHZ},
pages = {1--124},
title = {{Strukturanalyse mit FEM}},
url = {http://www.structures.ethz.ch/education/master/analysis/Skript/FEM{\%}7B{\_}{\%}7DD{\%}7B{\_}{\%}7DMain{\%}7B{\_}{\%}7D2009.pdf},
year = {2004}
}
@article{Peerlings2002,
abstract = {Continuum approaches to fracture regard crack initiation and growth as the ultimate consequences of a gradual, local loss of material integrity. The material models which are traditionally used to describe the degradation process, however, may predict premature crack initiation and instantaneous, perfectly brittle crack growth. This nonphysical response is caused by localisation instabilities due to loss of ellipticity of the governing equations and - more importantly - singularity of the damage rate at the crack tip. It is argued that this singularity results in instantaneous failure in a vanishing volume, even if ellipticity is not first lost. Adding strong nonlocality to the modelling is shown to preclude localisation instabilities and remove damage rate singularities. As a result, premature crack initiation is avoided and crack growth rates remain finite. Weak nonlocality, as provided by explicit gradient models, does not suffice for this purpose. In implementing the enhanced modelling, the crack must be excluded from the equilibrium problem and the nonlocal interactions in order to avoid unrealistic damage growth. ?? 2002 ??ditions scientifiques et m??dicales Elsevier SAS. All rights reserved.},
author = {Peerlings, R. H J and {De Borst}, R. and Brekelmans, W. A M and Geers, M. G D},
doi = {10.1016/S0997-7538(02)01211-1},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/2002{\_}Peerlings{\_}Localisation issues in local and nonlocal continuum approaches to fracture.pdf:pdf},
issn = {09977538},
journal = {Eur. J. Mech. A/Solids},
number = {2},
pages = {175--189},
title = {{Localisation issues in local and nonlocal continuum approaches to fracture}},
volume = {21},
year = {2002}
}
@article{Tschirschwitz,
author = {Tschirschwitz, Christian},
pages = {665--694},
title = {{B7 B7 Unf{\"{a}}lle mit Nutzfahrzeugen Reisebus kippt beim Abbiegen auf linke Seite B7}}
}
@article{Cherkaoui2009e,
author = {Cherkaoui, Mohammed and Capolungo, Laurent},
doi = {10.1007/978-0-387-46771-9},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Atomistic and Continuum Modeling of Nanocrystalline Materials/Chapter 03.pdf:pdf},
isbn = {978-0-387-46765-8},
title = {{Atomistic and Continuum Modeling of Nanocrystalline Materials}},
url = {http://link.springer.com/10.1007/978-0-387-46771-9},
volume = {112},
year = {2009}
}
@article{Saad2003,
abstract = {Tremendous progress has been made in the scientific and engineering disciplines regarding the use of iterative methods for linear systems. The size and complexity of linear and nonlinear systems arising in typical applications has grown, meaning that using direct solvers for the three-dimensional models of these problems is no longer effective. At the same time, parallel computing, becoming less expensive and standardized, has penetrated these application areas. Iterative methods are easier than direct solvers to implement on parallel computers but require approaches and solution algorithms that are different from classical methods. This second edition gives an in-depth, up-to-date view of practical algorithms for solving large-scale linear systems of equations, including a wide range of the best methods available today. A new chapter on multigrid techniques has been added, whilst material throughout has been updated, removed or shortened. Numerous exercises have been added, as well as an updated and expanded bibliography.},
archivePrefix = {arXiv},
arxivId = {0806.3802},
author = {Saad, Yousef},
doi = {10.2113/gsjfr.6.1.30},
eprint = {0806.3802},
isbn = {0898715342},
issn = {1570579X},
journal = {Notes},
number = {2nd Edition},
pages = {xviii+528},
pmid = {15237199},
title = {{Iterative Methods for Sparse Linear Systems}},
url = {http://www.stanford.edu/class/cme324/saad.pdf},
volume = {3},
year = {2003}
}
@article{Endokrinologie,
author = {Endokrinologie, Das Forschungsgebiet Der},
pages = {1--2},
title = {{1 Einf{\"{u}}hrung}}
}
@article{Brosdorf,
author = {Br{\"{o}}sdorf, Klaus-dieter and Depr{\'{e}}, Klaus and G{\"{o}}ritz, J{\"{o}}rg},
pages = {471--558},
title = {{A17 A17 Schadenaufkl{\"{a}}rung A17}}
}
@article{Verbrennungsmotor2007,
author = {Verbrennungsmotor, Der and Anfahren, Zum},
journal = {Fahrzeuggetriebe},
title = {{10 Anfahrelemente}},
volume = {1},
year = {2007}
}
@inproceedings{Seifert2009,
author = {Seifert, Thomas and Riedel, Hermann},
booktitle = {Proc. 4Th EASC},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/2009{\_}Seifert{\_}Fatigue Life of high temperature in combustion engines and exhaust systems.pdf:pdf},
title = {{Fatigue Life Prediction of High Temperature Components in Combustion Engines and Exhaust Systems}},
year = {2009}
}
@article{Analogien2010,
author = {Analogien, Der},
doi = {10.1007/978-3-642-10194-6},
isbn = {9783642101946},
title = {{W ¨ armeleitung und Diffusion}},
year = {2010}
}
@article{Nitsche,
author = {Nitsche, W. and Brunn, A.},
isbn = {10 3-540-20990-5},
title = {{Str{\"{o}}mungsmesstechnik}}
}
@article{Tensors1968a,
author = {Tensors, Flux},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/Folien CISM Summer School Mai2017 - Mesoscale Models/courses{\%}2FC1703{\%}2Fgroma{\%}2Fcontinuum (1).pdf:pdf},
title = {{Continuum Theory of Dislocations and Plastleity'}},
year = {1968}
}
@article{Zienkiewicz2005c,
author = {Zienkiewicz, O C and Taylor, R L and Zhu, J Z},
doi = {http://dx.doi.org/10.1016/B978-075066431-8.50180-6},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Zienkiewicz FEM - Vol 1 Basics Fundamentals/63205{\_}12.pdf:pdf},
isbn = {978-0-7506-6431-8},
journal = {Finite Elem. Method - Its Basis Fundam.},
pages = {27},
title = {{12-Multidomain mixed approximations – domain decomposition and ‘frame' methods}},
year = {2005}
}
@article{Beispiel2005,
author = {Beispiel, Als},
pages = {4--6},
title = {{B CAD-Konstruktion Konstruktion mit CATIA V5 17 Grunds{\{}{\"{a}}{\}}tzliches zu CATIA V5}},
year = {2005}
}
@article{Gibbs1998,
author = {Gibbs, Hugh H.},
isbn = {1859573894},
journal = {Handb. Compos.},
pages = {75--98},
title = {{High Temperature Resins}},
year = {1998}
}
@article{Tsurushima2002b,
author = {Tsurushima, Tadashi and Kunishima, Eiji and Asaumi, Yasuo and Aoyagi, Yuzo and Enomoto, Yoshiteru},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2002{\_}Tsurushima{\_}The Effect of Knock on Heat Loss in HCCI Engines-Modified Woschni.pdf:pdf},
journal = {Sae},
number = {108},
title = {{The Effect of Knock on Heat Loss in Homogeneous Charge Compression Ignition Engines}},
volume = {1},
year = {2002}
}
@article{Hartmann1997,
abstract = {This paper deals with two main topics. The first one concerns the equivalence of stress algorithms, based on a Backward-Euler-step applied on viscoplastic models of Chaboche-type, and their elastoplastic counter- part. Generally, the stress algorithm yields a system of non-linear algebraic equations and the corresponding consistent tangent operator, occurring in the principle of virtual displacements, leads to a system of linear equations. This procedure can be obtained utilizing only numerical methods. The second topic concerns a special constitutive relation based on a kinematic hardening model using a sum of Armstrong/Frederick terms, which is equivalent to a multi-surface plasticity model. Applying this model a so-called problem- adapted stress algorithm is derived, where only one non-linear equation must be solved. This result is independent of the number of terms in the hardening model. Furthermore, only the viscoplastic algorithm must be implemented, since it includes the elastoplastic constitutive model as a special case.},
author = {Hartmann, Stefan and L{\"{u}}hrs, Georg and Haupt, Peter},
doi = {10.1002/(SICI)1097-0207(19970330)40:6<991::AID-NME98>3.0.CO;2-H},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Numerik UMATS FE-Codes/1997{\_}Hartmann{\_}AN EFFICIENT STRESS ALGORITHM WITH APPLICATIONS IN VISCOPLASTICITY AND PLASTICITY.pdf:pdf},
issn = {0029-5981},
journal = {Int. J. Numer. Methods Eng.},
keywords = {finite elements,kinematic hardening,plasticity,stress algorithm,viscoplasticity},
number = {6},
pages = {991--1013},
title = {{an Efficient Stress Algorithm With Applications in Viscoplasticity and Plasticity}},
url = {http://doi.wiley.com/10.1002/(SICI)1097-0207(19970330)40:6{\%}7B{\%}25{\%}7D3C991::AID-NME98{\%}7B{\%}25{\%}7D3E3.0.CO;2-H{\%}7B{\%}25{\%}7D5Cnhttp://doi.wiley.com/10.1002/(SICI)1097-0207(19970330)40:6{\%}7B{\%}25{\%}7D3C991::AID-NME98{\%}7B{\%}25{\%}7D3E3.0.CO;2-H},
volume = {40},
year = {1997}
}
@article{Stiller2006,
author = {Stiller, Christoph},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Vorlesungen/Messtechnik+Regelungstechnik/gmrt01.pdf:pdf},
issn = {02731177},
journal = {Adv. Sp. Res.},
number = {12},
pages = {2820--2823},
title = {{Grundlagen der Mess- und Regelungstechnik}},
volume = {38},
year = {2006}
}
@article{Wang2007,
author = {Wang, X and Price, P and Stone, C R and Richardson, D},
doi = {10.1243/09544070JAUTO586},
file = {:C$\backslash$:/Users/p327208/Desktop/Promotion/Literature/Motorspezifisch/Heat Transfer Combustion Chamber/2007{\_}Wang{\_}Heat release and heat flux in a spray-guided direct-injection gasoline engine.pdf:pdf},
journal = {Proc Inst Mech Eng Part D J Automob Eng},
keywords = {direct-injection spark ignition,heat release,heat transfer},
pages = {1441--1452},
title = {{Heat release and heat flux in a spray-guided direct-injection gasoline engine}},
volume = {221},
year = {2007}
}
@inproceedings{Woschni1967,
author = {Woschni, G.},
booktitle = {SAE Tech. Pap. 670931},
doi = {https://doi.org/10.4271/670931},
title = {{A Universally Applicable Equation for the Instantaneous Heat Transfer Coefficient in the Internal Combustion Engine}},
year = {1967}
}
@article{Groma2015,
abstract = {According to recent experimental and numerical investigations if the characteristic size of a specimen is in the submicron size regime several new interesting phenomena emerge during the deformation of the samples. Since in such a systems the boundaries play a crucial role, to model the plastic response of submicron sized crystals it is crucial to determine the dislocation distribution near the boundaries. In this paper a phase field type of continuum theory of the time evolution of an ensemble of parallel edge dislocations with identical Burgers vectors, corresponding to the dislocation geometry near boundaries, is presented. Since the dislocation-dislocation interaction is scale free ({\$}1/r{\$}), apart from the average dislocation spacing the theory cannot contain any length scale parameter. As shown, the continuum theory suggested is able to recover the dislocation distribution near boundaries obtained by discrete dislocation dynamics simulations.},
archivePrefix = {arXiv},
arxivId = {1404.6344},
author = {Groma, Istv??n and Vandrus, Zolt??n and Isp??novity, P??ter Dus??n},
doi = {10.1103/PhysRevLett.114.015503},
eprint = {1404.6344},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/2015{\_}Groma{\_}Scale-Free Phase Field Theory of Dislocations.pdf:pdf},
issn = {10797114},
journal = {Phys. Rev. Lett.},
number = {1},
pages = {1--5},
title = {{Scale-free phase field theory of dislocations}},
volume = {114},
year = {2015}
}
@article{Piero2005,
author = {Piero, D E L},
number = {1967},
title = {{10 Plasticity}},
year = {2005}
}
@article{Talbot1987,
abstract = {Bounds of Hashin-Shtrikman type and self-consistent estimates for the overall properties of composites, which may be anisotropic, are developed. Bodies containing aligned ellipsoidal inclusions are considered particularly, generalizing previously known results. The overall thermal conductivity of a body containing aligned spheroidal inclusions is discussed as an example including, as limiting cases, bodies containing highly-conducting aligned needles and bodies containing aligned pennyshaped cracks. ?? 1977.},
author = {Talbot, D R S and Willis, J R},
doi = {10.1093/imamat/39.3.215},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/Strukturmechanik MMS/Literatur/Willis 1977.pdf:pdf},
isbn = {0022-5096},
issn = {02724960},
journal = {IMA J. Appl. Math. (Institute Math. Its Appl.},
number = {3},
pages = {215--240},
title = {{Bounds and self-consistent estimates for the overall properties of nonlinear composites}},
volume = {39},
year = {1987}
}
@article{Entleermethode,
author = {Entleermethode, Bei Der F{\"{u}}ll- and Prozess-, Der},
doi = {10.1007/978-3-8348-1988-8},
isbn = {9783834819888},
pages = {223--305},
title = {{Reale Arbeitsprozessrechnung Ein-Zonen-Zylinder-Modell}}
}
@article{Kim2012,
abstract = {This study examines the cold performance of biodiesel blends in a passenger car and a light duty truck at −16 °C and −20 °C. Six different types of biodiesels derived from soybean oil, waste cooking oil, rapeseed oil, cottonseed oil, palm oil and jatropha oil were blended with different volume ratios (B5 (5 vol. {\%} biodiesel — 95 vol. {\%} diesel), B10 and B20). The cold filter plugging point (CFPP) and the cloud point had an effect on the startability and driveability of both the passenger car and the light duty truck. The startability and driveability of the passenger car with all biodiesel blends (B5) were generally good at −20 °C. In the light duty truck, biodiesel blends (B10 and B20) of soybean, waste cooking, rapeseed and jatropha tended to be good at −20 °C in the startability and driveability tests than the biodiesel blends (B10 and B20) of cottonseed and palm. In particular, the palm biodiesel blend (B10) failed at −20 °C, and the palm biodiesel blend (B20) also failed at −16 °C in the startability test. The cold flow properties of biodiesel dictate that the length of the hydrocarbon chains and the presence of unsaturated structures significantly affect the low temperature properties of biodiesel.},
author = {Kim, Jk and Yim, Es and Jeon, Ch and Jung, Cs and Han, Bh},
doi = {10.1007/s12239},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Heat Transfer Combustion Chamber/2011{\_}Lee+Filip{\_}IMPROVING THE PREDICTIVENESS OF THE QUASI-D COMBUSTION MODEL FOR SI ENGINES WITH FLEXIBLE INTAKE SYSTEMS.pdf:pdf},
isbn = {1229-9138},
issn = {1229-9138},
journal = {Int. J. {\ldots}},
keywords = {biodiesel,cold filter plugging point,cold performance,driveability,startability},
number = {2},
pages = {293--300},
pmid = {1592335},
title = {{Cold performance of various biodiesel fuel blends at low temperature}},
url = {http://link.springer.com/article/10.1007/s12239-012-0027-2},
volume = {13},
year = {2012}
}
@article{Lange2002a,
abstract = {Ein Grundkurs zur Theorie des Systems Atmosph{\{}{\"{a}}{\}}re},
author = {Lange, Hans-Joachim},
doi = {10.1007/978-3-8348-9781-7},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/xxx{\_}Herzog{\_}Kolbenmaschinen{\_}2{\_}ThermodynamischeGrundlagen.pdf:pdf},
isbn = {978-3-8348-1404-3},
journal = {Die Phys. des Wetters und des Klimas},
pages = {1--64},
title = {{Thermodynamische Grundlagen}},
year = {2002}
}
@article{Wallentowitza,
author = {Wallentowitz, Henning and Reif, Konrad},
doi = {10.1007/978-3-8348-8195-3},
isbn = {9783834802576},
title = {{Aus dem Programm}}
}
@article{Rothe2015,
abstract = {In this article we investigate a fully, thermo-mechanically coupled viscoplasticity model in view of various numerical aspects. First, we develop the entire system of differential–algebraic equations resulting from the spatially discretized principle of virtual displacements, the principle of virtual temperatures, and the evolution equations of the internal variables provided by the constitutive model. In the time-integration step this system is solved both using a fully monolithic approach based on a Backward–Euler scheme in combination with the Multilevel-Newton algorithm as well as a partitioned approach solving the fully coupled system. The latter is treated by means of a combination of a Backward–Euler method and an accelerated Gauss–Seidel/Multilevel-Newton scheme to solve the resulting system of algebraic equations within each time-integration step. Additionally, we consider a specific treatment of the interpolation between different meshes within the partitioned approach. This is shown for p-version finite elements based on hierarchical shape functions. Finally, it turns out that the specific constitutive model of small-strain thermo-viscoplasticity, which is based on the decomposition into kinematic hardening and energy storing strains, yields a problem-adapted stress algorithm. This allows to reduce the stress algorithm on Gauss-point level to the solution of one scalar equation. Numerical examples serve to elucidate the behavior and properties of the proposed methods.},
author = {Rothe, Steffen and Erbts, Patrick and D{\"{u}}ster, Alexander and Hartmann, Stefan},
doi = {10.1016/j.cma.2015.05.002},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Numerik UMATS FE-Codes/2015{\_}Hartmann{\_}Monolithic and partitioned coupling schemes for thermo-viscoplasticity.pdf:pdf},
issn = {00457825},
journal = {Comput. Methods Appl. Mech. Eng.},
keywords = {algebraic equations,differential,fully coupled finite elements,monolithic approach,partitioned approach,thermo-viscoplasticity},
pages = {375--410},
publisher = {Elsevier B.V.},
title = {{Monolithic and partitioned coupling schemes for thermo-viscoplasticity}},
url = {http://linkinghub.elsevier.com/retrieve/pii/S0045782515001681},
volume = {293},
year = {2015}
}
@article{Rodi2017,
abstract = {The paper reviews in condensed form and from a historical perspective the various methods for treating and simulating turbulence and its effects in hydraulic flows. After highlighting the main characteristic features of turbulence and the role it plays in hydraulics, a necessarily brief overview is given of the main methods used in hydraulic flow calculations for dealing with turbulence and its effects. These are (1) empirical relations, (2) methods solving the Reynolds-averaged Navier-Stokes (RANS) equations with the aid of statistical turbulence models, (3) direct numerical simulations (DNS), and (4) large-eddy simulations (LES). Brief comments are made on the historical development of the different methods, and for RANS, DNS, and LES methods some application examples are presented. For details on the individual methods and further application examples, the reader is directed to the very extensive literature. DOI:},
author = {Rodi, Wolfgang},
doi = {10.1061/(ASCE)HY.1943-7900.0001288.},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Boiling/Turbulence/2017{\_}Rodi{\_}Turbulence Modeling and Simulation in Hydraulics - a historical Review.pdf:pdf},
journal = {J. Hydraul. Eng.},
keywords = {turbulence},
number = {5},
pages = {1--20},
title = {{Turbulence Modeling and Simulation in Hydraulics : A Historical Review}},
volume = {143},
year = {2017}
}
@article{Klein2009b,
author = {Klein, Bernd},
journal = {Leichtbau-Konstruktion},
pages = {232--258},
title = {{Beulen von Blechfeldern und Rohren}},
year = {2009}
}
@article{Deutscher,
author = {Deutscher, Allgemeiner and Club, Automobil and Scale, Abbreviated Injury and Device, Anthropomorphic Test and Servey, Co-operative Crash Injury and Scale, Collision Deformation and Committee, European Enhanced Vehicle-safety and Transport, European and Council, Safety and Motor, Federal and Safety, Vehicle and Versicherungswirtschaft, Gesamtverband Der Deutschen and Criteria, Head Injury and Criteria, Head Performance and Assessment, Injury and Value, Reference and Criteria, Injury and Level, Protection and Harmonized, International and Score, Injury Severity and Barrier, Mobile Deformable},
pages = {967--969},
title = {{D2 D2 Begriffe und Abk{\"{u}}rzungen D2 Firmen und Institutionen}}
}
@article{Schmitt2006,
author = {Schmitt, J{\"{u}}rgen and Isermann, Ralf},
journal = {Fahrdynamik-Regelung},
pages = {365--375},
title = {{Entwicklungsumgebung mit echtzeitf{\"{a}}higen Gesamtfahrzeugmodellen f{\"{u}}r sicherheitsrelevante Fahrerassistenzsysteme}},
year = {2006}
}
@article{The2003,
author = {The, S Olving and Lement, F Inite and Tatic, E Quations S},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Nicholson 2003 - Finite Element Analysis Thermomechanics of Solids/0749{\_}C11.pdf:pdf},
pages = {153--165},
title = {{Solution Methods for Linear Problems 11.1}},
year = {2003}
}
@article{Cherkaoui2009h,
author = {Cherkaoui, Mohammed and Capolungo, Laurent},
doi = {10.1007/978-0-387-46771-9},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Atomistic and Continuum Modeling of Nanocrystalline Materials/Chapter 05.pdf:pdf},
isbn = {978-0-387-46765-8},
pages = {117--142},
title = {{Atomistic and Continuum Modeling of Nanocrystalline Materials}},
url = {http://link.springer.com/10.1007/978-0-387-46771-9},
volume = {112},
year = {2009}
}
@book{Fallis2013a,
abstract = {Predicting the binding mode of flexible polypeptides to proteins is an important task that falls outside the domain of applicability of most small molecule and protein−protein docking tools. Here, we test the small molecule flexible ligand docking program Glide on a set of 19 non-$\alpha$-helical peptides and systematically improve pose prediction accuracy by enhancing Glide sampling for flexible polypeptides. In addition, scoring of the poses was improved by post-processing with physics-based implicit solvent MM- GBSA calculations. Using the best RMSD among the top 10 scoring poses as a metric, the success rate (RMSD ≤ 2.0 {\AA} for the interface backbone atoms) increased from 21{\%} with default Glide SP settings to 58{\%} with the enhanced peptide sampling and scoring protocol in the case of redocking to the native protein structure. This approaches the accuracy of the recently developed Rosetta FlexPepDock method (63{\%} success for these 19 peptides) while being over 100 times faster. Cross-docking was performed for a subset of cases where an unbound receptor structure was available, and in that case, 40{\%} of peptides were docked successfully. We analyze the results and find that the optimized polypeptide protocol is most accurate for extended peptides of limited size and number of formal charges, defining a domain of applicability for this approach.},
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Fallis, A.G},
booktitle = {J. Chem. Inf. Model.},
doi = {10.1017/CBO9781107415324.004},
eprint = {arXiv:1011.1669v3},
isbn = {9788578110796},
issn = {1098-6596},
keywords = {icle},
number = {9},
pages = {1689--1699},
pmid = {25246403},
title = {{ComputationalMethods forMicrostructure-Property Relationships}},
volume = {53},
year = {2013}
}
@article{Stiller2006a,
author = {Stiller, Christoph},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Vorlesungen/Messtechnik+Regelungstechnik/gmrt01.pdf:pdf},
issn = {02731177},
journal = {Adv. Sp. Res.},
number = {12},
pages = {2820--2823},
title = {{Grundlagen der Mess- und Regelungstechnik}},
volume = {38},
year = {2006}
}
@article{Ahnlichkeitstheorie,
author = {Ahnlichkeitstheorie, Die and Ahnlichkeitstheorie, Der},
title = {{¨ 7 Ahnlichkeitstheorie 7.1}}
}
@article{Technologya,
author = {Technology, O F},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Heat Transfer Combustion Chamber/2013{\_}Oleg{\_}Spitsov{\_}HEAT TRANSFER INSIDE INTERNAL COMBUSTION ENGINE - Modelling and comparison with experimental data{\_}Masters{\_}thesis.pdf:pdf},
keywords = {combustion engine,degree program in energy,faculty of technology,heat transfer inside internal,peenranta university of technology,technology},
title = {{Heat Transfer Inside Internal Combustion Engine :}}
}
@article{Kanchanomai2007,
abstract = {Fatigue cracking due to traffic load is a major factor in road damage. Therefore, durability and lifetime prediction of roads plays a substantial role for road maintenance and cost planning. This paper reports a study of fatigue crack performance of solid asphalt and asphalt-asphalt interfaces by means of the wedge-splitting test. Instead of beams and the three- or four-point bending test, the wedge splitting method was used for the first time to observe crack growth on bituminous drilling cores. Samples of solid asphalt and samples with asphalt-interfaces were tested. One group of asphalt interfaces was untreated and the other was sandblasted before spreading the top layer during manufacturing. Due to the temperature dependency of material properties of asphalt, the tests were performed in a compact climate chamber at -10, 0 and + 10(' The challenge of determining the crack length and the crack tip were detected with an optical measurement system and picture analysis after testing. The results prove that the wedge splitting method is a highly practicable and repeatable method for crack growth testing of bituminous materials.},
author = {Kanchanomai, C and Mutoh, Y},
doi = {10.1111/j.1460-2695.2006.01088.x},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/1979{\_}Kung+Fine{\_}Fatigue crack initiation and microcrack growth in 2024-T4 and 2124-T4 Alu alloy.pdf:pdf},
issn = {8756758X},
journal = {Eng. Fract. Mech.},
keywords = {fatigue crack growth,fatigue crack initiation,lead free,low cycle fatigue},
number = {5},
pages = {443--457},
title = {{Fatigue crack initiation and growth in solder alloys}},
url = {http://doi.wiley.com/10.1111/j.1460-2695.2006.01088.x},
volume = {30},
year = {2007}
}
@article{Arbeitsumgebunga,
author = {Arbeitsumgebung, Die},
journal = {Pro-Engineer Prakt.},
title = {{5 Bauteilmodellierung}}
}
@article{Kaune,
author = {Kaune, Vanessa and Janda, Daniel and Schliephake, Daniel},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Werkstoffkunde/Ueberblick{\_}Ausscheidungshaertung{\_}AluminiumLegierungen{\_}TUDarmstadt.pdf:pdf},
journal = {TU Darmstadt},
pages = {6},
title = {{Aush{\"{a}}rtung von Aluminiumlegierungen}},
url = {http://www.mawi.tu-darmstadt.de/media/phm/5semester/ausscheidungshrtungiv.pdf}
}
@book{Fox1918a,
author = {Fox, P J},
booktitle = {Science},
doi = {10.1126/science.49.1254.44},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Thermodynamik/M{\"{u}}llerAndNoll{\_}Thermodynamik/Noll 1974 Mechanics and Thermodynamics{\_}SelectedPapers.pdf:pdf},
isbn = {9783642658198},
issn = {0036-8075},
number = {1240},
pages = {343--345},
pmid = {17811888},
title = {{the Foundations of Mechanics.}},
volume = {48},
year = {1918}
}
@article{Burg2005,
author = {Burg, Heinz},
number = {559},
pages = {443--450},
title = {{A14 A14 Unf{\"{a}}lle mit land- oder forstwirtschaftlichen Fahrzeugen A14}},
year = {2005}
}
@article{Man2009a,
abstract = {Current state and historical progress in experimental and theoretical studies of surface relief appertaining to persistent slip bands (PSBs) and leading to fatigue crack initiation in cyclically deformed metals is presented as a thorough critical overview. A comprehensive inventory of microscopic techniques used for this study is tabulated chronologically with emphasis to their applicability to polycrystals. The most relevant experimental characteristics concerning surface relief evolution, namely the form of extrusions and intrusions in single- and polycrystalline materials, are surveyed. Theoretical models and computational simulations of extrusion and intrusion formation and fatigue crack initiation are critically reviewed.},
author = {Man, J. and Obrtl{\'{i}}k, K. and Pol{\'{a}}k, J.},
doi = {10.1080/14786430902917616},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/2009{\_}Man + Polak{\_}Extrusions and intrusions in fatigued metals Part 1 State of the art and history.pdf:pdf},
isbn = {1478-6435},
issn = {1478-6435},
journal = {Philos. Mag.},
number = {16},
pages = {1295--1336},
title = {{Extrusions and intrusions in fatigued metals. Part 1. State of the art and history†}},
url = {http://www.tandfonline.com/doi/abs/10.1080/14786430902917616},
volume = {89},
year = {2009}
}
@article{Finite2014,
author = {Finite, The and Method, Element and Basis, Its},
doi = {10.1016/B978-1-85617-635-4.00032-7},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Zienkiewicz FEM - Vol 3 Fluid Dynamics/63229{\_}apdxg.pdf:pdf},
journal = {Finite Elem. Method Fluid Dyn.},
pages = {519--520},
title = {{Multigrid Method}},
url = {http://linkinghub.elsevier.com/retrieve/pii/B9781856176354000327},
year = {2014}
}
@article{Wulfinghoff2010a,
author = {Wulfinghoff, Stephan and B{\"{o}}hlke, Thomas},
doi = {10.1002/pamm.201010168},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2010{\_}Wulfinghoff{\_}Gradient Plasticity for Single Crystals.pdf:pdf},
issn = {16177061},
pages = {351--352},
title = {{Gradient Plasticity for Single Crystals}},
volume = {352},
year = {2010}
}
@article{Bockh2006,
author = {B{\"{o}}ckh, Peter},
doi = {10.1007/978-3-662-44477-1},
isbn = {978-3-662-44476-4},
title = {{W{\"{a}}rme{\"{u}}bertragung}},
url = {http://link.springer.com/10.1007/978-3-662-44477-1},
year = {2006}
}
@article{Weißgerber2013,
author = {Wei{\ss}gerber, Wilfried},
doi = {10.1007/978-3-8348-2088-4},
isbn = {978-3-8348-1339-8},
title = {{Elektrotechnik f{\"{u}}r Ingenieure 3}},
url = {http://link.springer.com/10.1007/978-3-8348-2088-4},
year = {2013}
}
@book{Melorose2015,
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Melorose, J and Perroy, R and Careas, S},
booktitle = {Statew. Agric. L. Use Baseline 2015},
doi = {10.1017/CBO9781107415324.004},
eprint = {arXiv:1011.1669v3},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/Crystall Plasticity Basics/Hull 2011 - Introduction to Dislocation.pdf:pdf},
isbn = {9788578110796},
issn = {1098-6596},
keywords = {icle},
pmid = {25246403},
title = {{Introduction to dislocations}},
volume = {1},
year = {2015}
}
@book{DanielGhebru2013,
author = {{Daniel Ghebru}, Dipl-Ing and {Ulrich Spicher Korreferent}, Dr-Ing and {techn Andreas Wimmer Korreferent} and {sc techn Thomas Koch}},
isbn = {9783832534325},
keywords = {Co-Simulation,Instation{\{}{\"{a}}{\}}res Thermomanagement,Modellbildung,Thermische Gesamtfahrzeugsimulation,Thermisches Motormodell},
number = {April},
title = {{Modellierung und Analyse des instation{\{}{\"{a}}{\}}ren thermischen Verhaltens von Verbrennungsmotor und Gesamtfahrzeug}},
year = {2013}
}
@article{Metzger2014,
abstract = {This paper reports on the evolution of cracks in the cylinder heads of a large V8 Diesel engine during cyclic engine tests. The observations are compared with the predictions of a lifetime model for combined thermo-mechanical (TMF) and high cycle fatigue (HCF) loading, which is based on a fracture mechanics analysis of microcrack growth in viscoplastic solids and assumes that the crack advance per cycle is proportional to the cyclic crack tip opening displacement. Since the material of the cylinder heads, the cast iron EN-GJV450, exhibits the typical features of cast iron, namely pressure dependence of the yield stress, dilatancy and tension-compression asymmetry, the Gurson model is applied and combined with the viscoplastic Chaboche model. This constitutive model together with the lifetime model is implemented into a finite element code as a user defined material routine. Published model parameters for the considered cast iron are used to carry out the simulation of the engine test. This simulation comprises a CFD analysis to determine the heat transfer coefficients, a thermal analysis of the load cycle and the mechanical analysis. The thermal analysis reproduces the temperatures at various measuring points sufficiently accurately. Finally, the mechanical analysis predicts the location and orientation of the cracks in the valve bridges correctly in all cases. However, the lifetime predictions are rather conservative compared to the tests (by a factor of 1 to 5 in lifetime). This is discussed and explained by the fact that the cracks were detected in the tests only when they had already spread over a substantial fraction of the valve bridge width. To describe this situation a long-crack analysis would be necessary, which is not yet included in the applied lifetime model},
author = {Metzger, Mario and Leidenfrost, Marc and Werner, Ewald and Riedel, Hermann and Seifert, Thomas},
doi = {10.4271/2014-01-9047},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2014{\_}Metzger{\_}Lifetime prediction of EN-GJV 450 Cast Iron Cylinder Heads und combined thermo-mechanical and hcf loading.pdf:pdf},
journal = {SAE Int. J. Engines},
number = {2},
pages = {2014--9047},
title = {{Lifetime Prediction of EN-GJV 450 Cast Iron Cylinder Heads under Combined Thermo-Mechanical and High Cycle Fatigue Loading}},
volume = {7},
year = {2014}
}
@article{Ubersetzungen2007,
author = {{\"{U}}bersetzungen, Kennungswandler Wahl Der},
journal = {Fahrzeuggetriebe},
title = {{4 Kennungswandler – Wahl der {\"{U}}bersetzungen}},
year = {2007}
}
@book{Zybell2016,
author = {Zybell, Lutz},
doi = {10.1007/978-3-319-21467-2},
isbn = {978-3-319-21466-5},
title = {{Recent Trends in Fracture and Damage Mechanics}},
url = {http://link.springer.com/10.1007/978-3-319-21467-2},
year = {2016}
}
@article{Aslan2011,
abstract = {Proper life-time prediction modeling of single crystalline components is of increasing importance due to their common use in turbine industry. Viscoplastic damage approaches are of great interest in that context. However, mechanical properties of single crystals are strongly anisotropic and nonlinear in service conditions, bringing certain complexity into constitutive and numerical modeling. The aim of this work is to develop a thermodynamically consistent constitutive model based on generalized continua in order to simulate fatigue crack initiation and growth in single crystals. For that purpose, a standard crystal plasticity model is taken as a basis and coupled with the continuous damage model developed by Marchal et al. (2006a) [Marchal, N., Forest, S., Remy, L. and Duvinage, S. (2006a). Simulation of Fatigue Crack Growth in Single Crystal Superalloys Using Local Approach to Fracture, In: Moinereau, D., Steglich, D. and Besson, J. (eds.), Local Approach to Fracture, 9th European Mechanics of Materials Conference, Euromech–Mechamat, Moret–Sur–Loing, France, Presses de l'Ecole des mines de Paris, pp. 353–358]. As a variant of micromorphic theory, microdamage approach is applied to the model in order to obtain a regularized continuum damage formulation which solves mesh dependency problem by introducing an intrinsic length scale. A detailed finite element implementation procedure and its validation for monotonic crack growth areshown. Fatigue crack growth analyses have been performed on a single edge notched geometry and a comparison between numerical and experimental results is presented.},
author = {Aslan, Ozgur and Quilici, St{\'{e}}phane and Forest, Samuel},
doi = {10.1177/1056789510395738},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/2011{\_}Aslan{\_}Numerical Modeling of Fatigue Crack Growth in Single Crystals Based on micodamage theory.pdf:pdf},
issn = {1056-7895},
journal = {Int. J. Damage Mech.},
number = {5},
pages = {681--705},
title = {{Numerical Modeling of Fatigue Crack Growth in Single Crystals Based on Microdamage Theory}},
url = {http://journals.sagepub.com/doi/10.1177/1056789510395738},
volume = {20},
year = {2011}
}
@book{Tobergte2013a,
abstract = {applicability for this approach.},
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Tobergte, David R and Curtis, Shirley},
booktitle = {J. Chem. Inf. Model.},
doi = {10.1017/CBO9781107415324.004},
eprint = {arXiv:1011.1669v3},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Thermodynamik/M{\"{u}}llerAndNoll{\_}Thermodynamik/M{\"{u}}ller 2007 Energy and Entropy.pdf:pdf},
isbn = {9788578110796},
issn = {1098-6596},
keywords = {icle},
number = {9},
pages = {1689--1699},
pmid = {25246403},
title = {{A History of Thermodynamics}},
volume = {53},
year = {2013}
}
@article{Stabilitat,
author = {Stabilit{\"{a}}t, {\"{U}}bertragungsverhalten and Stabilit{\"{a}}t, Bestimmuing Der},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Vorlesungen/Messtechnik+Regelungstechnik/gmrt04.pdf:pdf},
pages = {1--20},
title = {{Stabilit{\{}{\"{a}}{\}}t im Zeitbereich}}
}
@article{Drehmoment,
author = {Drehmoment, Das and Leis-, Die and Kolbenfl, Zylinderdruck and Kolbenweg, Kurbelwinkel},
pages = {151--159},
title = {{5 Leistung und Drehmoment 5 Leistung und Drehmoment}}
}
@article{Nallasamy1987,
abstract = {The paper presents a brief account of various turbulence models employed in the computation of turbulent flows, and evaluates the application of these models to internal flows by examining the predictions of various turbulence models in selected important flow configurations. The main conclusions of this analysis are: (a) The $\kappa$-$\epsilon$ model is used in a majority of all the 2-D flow calculations reported in the literature. (b) Modified forms of the $\kappa$-$\epsilon$ model improve the performance for flows with streamline curvature and heat transfer. (c) For flows with swirl, the $\kappa$-$\epsilon$ model performs rather poorly; the algebraic stress model performs better in this case. (d) For flows with regions of secondary flow (noncircular duct flows), the algebraic stress model performs fairly well. Two important factors in the numerical solution of the model equations, namely false diffusion and inlet boundary conditions, are discussed. The existence of countergradient transport and its implications in turbulence modeling are examined. Finally, some recommendations for improving the model performance are made. The need for detailed experimental data in flows with strong curvature is emphasized. {\textcopyright} 1987, Pergamon Journals Ltd. All rights reserved.},
author = {Nallasamy, M.},
doi = {10.1016/S0045-7930(87)80003-8},
file = {:C$\backslash$:/Users/p327208/Desktop/Promotion/Literature/Motorspezifisch/Boiling/Turbulence/1985{\_}Nallasamy{\_}Turbulence models and therir applications to the prediciton of internal flows - a review.pdf:pdf},
isbn = {0045-7930},
issn = {00457930},
journal = {Comput. Fluids},
number = {2},
pages = {151--194},
title = {{Turbulence models and their applications to the prediction of internal flows: A review}},
volume = {15},
year = {1987}
}
@article{Endokrinologie,
author = {Endokrinologie, Das Forschungsgebiet Der},
pages = {1--2},
title = {{1 Einf{\{}{\"{u}}{\}}hrung}}
}
@article{Lejsek+Kulzer2010,
abstract = {The introduction of CO2-reduction technologies like Start--Stop or the Hybrid-Powertrain and the worldwide stringent emission legislation require a detailed optimization of the engine start-up. The combustion concept development as well as the calibration of the engine control unit makes an explicit thermodynamic analysis of the combustion process during the start-up necessary. Initially, the well-known thermodynamic analysis of in-cylinder pressure at stationary condition was transmitted to the highly non-stationary engine start-up. For this running mode of the engine the current models for calculation of the transient wall heat fluxes were found to be misleading. With a fraction of nearly 45{\{}{\%}{\}} of the burned fuel energy, the wall heat is very important for the calculation of energy balance and for the combustion process analysis. Based on the measurements of transient wall heat transfer densities during the start-up presented in a former work (Lejsek and Kulzer in Investigations on the transient wall heat transfer at start-up for SI engines with gasoline direct injection. SAE Paper), the paper describes the development of adaptations to the known correlations by Woschni (MTZ 31:491, 1970), Hohenberg (Experimentelle Erfassung der Wandw{\{}{\"{a}}{\}}rme von Kolbenmotoren. TU Graz, Habil., 1980) and Bargende (Ein Gleichungsansatz zur Berechnung der instation{\{}{\"{a}}{\}}ren Wandw{\{}{\"{a}}{\}}rmeverluste im Hochdruckteil von Ottomotoren. TH Darmstadt, PhD-Thesis, 1991) for the application during engine start-up. To demonstrate the high accuracy of the model, the results of the cyclic resolved thermodynamic analysis using the presented novel approaches were compared with the results of the measurements. It is shown, that the novel heat flux models for the engine start-up process gives a cyclic resolved thermodynamic analysis to optimize the engine start-up pretty efficient.},
author = {Lejsek, David and Kulzer, Andr{\'{e}} and Hammer, J{\"{u}}rgen},
doi = {10.1007/s00231-010-0712-5},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Heat Transfer Combustion Chamber/2010{\_}Kulzer{\_}Novel Transient Wall Heat Transfer Approach for the Start-up of SI Engines with Gasoline DI.pdf:pdf},
journal = {Heat Mass Transf.},
month = {nov},
number = {10},
pages = {1053--1067},
title = {{A novel transient wall heat transfer approach for the start-up of SI engines with gasoline direct injection}},
volume = {46},
year = {2010}
}
@article{Hochhalter2010,
abstract = {The objective of this paper is to develop further a framework for computationally modeling$\backslash$nmicrostructurally small fatigue crack growth in AA 7075-T651 (Bozek et al 2008 Modelling Simul.$\backslash$nMater. Sci. [/0965-0393/16] 16 065007 ). The focus is on the nucleation event, when a crack extends$\backslash$nfrom within a second-phase particle into a surrounding grain, since this has been observed to be an$\backslash$ninitiating mechanism for fatigue crack growth in this alloy. It is hypothesized that nucleation can$\backslash$nbe predicted by computing a non-local nucleation metric near the crack front. The hypothesis is$\backslash$ntested by employing a combination of experimentation and finite element modeling in which various$\backslash$nslip-based and energy-based nucleation metrics are tested for validity, where each metric is derived$\backslash$nfrom a continuum crystal plasticity formulation. To investigate each metric, a non-local procedure$\backslash$nis developed for the calculation of nucleation metrics in the neighborhood of a crack front.$\backslash$nInitially, an idealized baseline model consisting of a single grain containing a semi-ellipsoidal$\backslash$nsurface particle is studied to investigate the dependence of each nucleation metric on lattice$\backslash$norientation, number of load cycles and non-local regularization method. This is followed by a$\backslash$ncomparison of experimental observations and computational results for microstructural models$\backslash$nconstructed by replicating the observed microstructural geometry near second-phase particles in$\backslash$nfatigue specimens. It is found that orientation strongly influences the direction of slip$\backslash$nlocalization and, as a result, influences the nucleation mechanism. Also, the baseline models,$\backslash$nreplication models and past experimental observation consistently suggest that a set of particular$\backslash$ngrain orientations is most likely to nucleate fatigue cracks. It is found that a continuum crystal$\backslash$nplasticity model and a non-local nucleation metric can be used to predict the nucleation event in AA$\backslash$n7075-T651. However, nucleation metric threshold values that correspond to various nucleation$\backslash$ngoverning mechanisms must be calibrated.},
author = {Hochhalter, J D and Littlewood, D J and Christ, R J and Veilleux, M G and Bozek, J E and Ingraffea, A R and Maniatty, A M},
doi = {10.1088/0965-0393/18/4/045004},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/2010{\_}Hochhalter{\_}AL7075AgeometricapproachII{\_}SlipAndNucleation.pdf:pdf},
isbn = {0965-0393},
issn = {0965-0393},
journal = {Model. Simul. Mater. Sci. Eng.},
number = {4},
pages = {045004},
title = {{A geometric approach to modeling microstructurally small fatigue crack formation: II. Physically based modeling of microstructure-dependent slip localization and actuation of the crack nucleation mechanism in AA 7075-T651}},
url = {http://stacks.iop.org/0965-0393/18/i=4/a=045004?key=crossref.ef8bc48536790be47a24f27989602c36},
volume = {18},
year = {2010}
}
@article{Mesarovic2017a,
author = {Mesarovic, S},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/Folien CISM Summer School Mai2017 - Mesoscale Models/courses{\_}C1703{\_}Mesarovic+Lecture+4+CORR+2.pdf:pdf},
title = {{Physical foundations of meso-scale continua Part 2 : ( Thermo- ) Dynamics}},
year = {2017}
}
@article{Burgc,
author = {Burg, Heinz and Geigl, Bertram C and Kramer, Florian and Moser, Andreas and Steffan, Hermann},
journal = {Injury},
pages = {569--584},
title = {{A19 A19 Biomechanik A19}}
}
@article{Desmorat2015a,
author = {Desmorat, Rodrigue and {Du Tertre}, Alban and Gaborit, Pierre},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/2 scale models papers/2015{\_}Desmorat{\_}Multiaxial Haigh Diagrams from incremental two scale damage analysis.pdf:pdf},
journal = {Aerosp. Lab J.},
number = {9},
pages = {1--15},
title = {{Multiaxial Haigh diagrams from incremental two scale damage analysis}},
volume = {en review},
year = {2015}
}
@article{Steering,
author = {Steering, Active Front and Kapitel, Dieses},
pages = {213--236},
title = {{9 Mechatronische Lenksysteme : Modellbildung und Funktionalit{\{}{\"{a}}{\}}t des Active Front Steering}}
}
@article{Essmann1979a,
abstract = {It is proposed that, during dislocation glide at low temperatures, both screw and non-screw dislocations annihilate mutually with dislocations of opposite sign approaching on closely neighbouring glide planes. The experimental evidence is summarized and possible mechanisms are discussed. Phenomenological models of dislocation accumulation during deformation, taking into account the annihilation of dislocations, are formulated. The analysis of selected examples of tensile and cyclic deformation of f. c. c. and b. c. c. metal crystals demonstrates that annihilation of edge and/or screw dislocations occurs during strain hardening and can lead to steady-state deformation. It follows that the dislocation densities introduced during deformation cannot exceed well-defined upper limits that are distinctly lower than the hypothetical upper limits estimated for the static case. The observations suggest that the critical spacings of dislocation pairs that annihilate are similar 50-500 nm for screw and similar 1. 6 nm for edge dislocations (in copper). The atomic concentration of point defects formed by the annihilation of non-screw dislocations is found to be low in most cases. However, it is concluded that, in the dislocation-rich walls of persistent slip bands in fatigued copper, a rather high concentration of point defects prevails.},
author = {Essmann, U and Mughrabi, H},
doi = {10.1080/01418617908234871},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/2006{\_}Mughrabi + Essmann{\_}Annihilation of dislocations   during tensile and cyclic deformation and limits of dislocation   densities.pdf:pdf},
isbn = {0141-8610},
issn = {0141-8610},
journal = {Philos. Mag. A},
number = {6},
pages = {731--756},
title = {{Annihilation of dislocations during tensile and cyclic deformation and limits of dislocation densities}},
url = {http://www.tandfonline.com/doi/abs/10.1080/01418617908234871},
volume = {40},
year = {1979}
}
@article{Torrilhon2007a,
author = {Torrilhon, Manuel},
doi = {10.1002/theDOIsuffix},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Thermodynamik/PhasenFeld/Nestler{\_}Crack{\_}propagation{\_}on{\_}mesoscopic{\_}length{\_}scale.pdf:pdf},
journal = {Pamm},
keywords = {chemo-mechanical coupling,crack propagation,multiphase-field,phase-field},
pages = {1--2},
title = {{Stability of reduced electric arc models}},
url = {http://onlinelibrary.wiley.com/doi/10.1002/pamm.200700318/abstract},
volume = {2},
year = {2007}
}
@article{Thomson2006,
author = {Thomson, J J},
journal = {Gerthsen Phys.},
pages = {447--482},
title = {{08 - Freie Elektronen und Ionen}},
year = {2006}
}
@article{Tsurushima2002b,
author = {Tsurushima, Tadashi and Kunishima, Eiji and Asaumi, Yasuo and Aoyagi, Yuzo and Enomoto, Yoshiteru},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Klopfen{\_}Ottomotor/2002{\_}Tsurushima{\_}The Effect of Knock on Heat Loss in HCCI Engines-Modified Woschni.pdf:pdf},
journal = {Sae},
number = {108},
title = {{The Effect of Knock on Heat Loss in Homogeneous Charge Compression Ignition Engines}},
volume = {1},
year = {2002}
}
@article{Variationsrechnung,
author = {Variationsrechnung, Gegenstand Der},
title = {{10 Variationsrechnung}}
}
@article{Rhouma2011,
author = {Rhouma, W. Ben and Deschanel, S. and Weiss, J.},
doi = {10.1063/1.3637920},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2011{\_}Weiss{\_}Collective Dislocation Dynamics and avalanches during fatigue of aluminium.pdf:pdf},
isbn = {9780735409569},
issn = {0094243X},
journal = {AIP Conf. Proc.},
keywords = {acoustic emission,damage,dislocations,fatigue,microstructure},
number = {May},
pages = {1536--1539},
title = {{Collective dislocation dynamics and avalanches during fatigue of aluminum}},
volume = {1389},
year = {2011}
}
@article{Voraussetzungen1936,
author = {Voraussetzungen, Die and Rail-einspritztechnologie, Common},
title = {{Fahrzeugdieselmotoren}},
year = {1936}
}
@article{Frage2007,
author = {Frage, Die and Wirkungen, Den and Hilfen, Den},
doi = {10.1007/978-3-531-19320-5},
isbn = {9783531193199},
journal = {Arbeit},
pages = {17--20},
title = {{1 Einleitung}},
year = {2007}
}
@article{Perez2003,
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {P{\'{e}}rez, Mara{\~{n}}a and Strictest, In and Confidence, Commercial and One, Part and Strictest, In and Confidence, Commercial},
doi = {10.1002/ejoc.201200111},
eprint = {arXiv:1011.1669v3},
isbn = {9781107671812},
issn = {0196-6553},
journal = {Eng. Med. Biol. Soc. 2008. EMBS 2008. 30th Annu. Int. Conf. IEEE},
number = {January},
pages = {2004},
pmid = {26840611},
title = {{Table of of contents}},
year = {2003}
}
@article{Teilaufgabenc,
author = {Teilaufgaben, Abzuhandelnde},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Empirical Fatigue Models + Validation/Betriebsfestigkeit{\_}ErwinHaibach/Kap4 Praktische Umsetzung des Betriebsfestigkeits-Konzepts.pdf:pdf},
title = {{des Betriebsfestigkeits-Konzeptes}}
}
@article{Mcdowell2017a,
author = {Mcdowell, David L},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/Folien CISM Summer School Mai2017 - Mesoscale Models/courses{\_}C1703{\_}mcdowell{\_}CISM.atomistic.mcdowell.lecture+2.final.pdf:pdf},
title = {{Atomistic Modeling for Crystalline Nanostructures}},
year = {2017}
}
@article{Caton1981,
abstract = {Because of the increasing need for precise information on engine processes, this study developed and experimentally verified models for the instantaneous heat transfer in an engine exhaust port. Experimental measurements were made of the instantaneous cylinder pressure and instantaneous exhaust gas temperature for a range of engine operating conditions. The pressure measurements were used to obtain the instantaneous cylinder gas state and the temperature measurements were used to validate the heat transfer models. The exhaust port heat transfer was dominated by jet induced large-scale fluid motion as opposed to wallshear generated fluid motion. An analysis based on the jet velocity through the valve opening correctly estimated the heat transfer due to this large-scale motion. Models for the instantaneous exhaust port heat transfer provided excellent agreement with measurements as a function of engine operating conditions. A cause d'un besoin croissant d'information pr{\{}{\'{e}}{\}}cise sur le fonctionnement d'un moteur, on d{\{}{\'{e}}{\}}veloppe une {\{}{\'{e}}{\}}tude et on v{\{}{\'{e}}{\}}rifie exp{\{}{\'{e}}{\}}rimentalement des mod{\{}{\`{e}}{\}}les sur le transfert de chaleur instantan{\{}{\'{e}}{\}} {\{}{\`{a}}{\}} l'{\{}{\'{e}}{\}}chappement d'un cylindre. Des mesures de la pression instantan{\{}{\'{e}}{\}}e dans le cylindre et de la temp{\{}{\'{e}}{\}}rature instantan{\{}{\'{e}}{\}}e {\{}{\`{a}}{\}} l'{\{}{\'{e}}{\}}chappement sont effectu{\{}{\'{e}}{\}}es pour un domaine de conditions de fonctionnement d'un moteur. Les mesures de pression permettent d'atteindre l'{\{}{\'{e}}{\}}tat instantan{\{}{\'{e}}{\}} du gaz dans le cylindre et les mesures de temp{\{}{\'{e}}{\}}rature permettent de valider les mod{\{}{\`{e}}{\}}les de transfert thermique. Le transfert {\{}{\`{a}}{\}} l'{\{}{\'{e}}{\}}chappement est domin{\{}{\'{e}}{\}} par un mouvement de jet {\{}{\`{a}}{\}} large {\{}{\'{e}}{\}}chelle au contraire du mouvement de fluide {\{}{\`{a}}{\}} frottement pari{\{}{\'{e}}{\}}tal. Une analyse bas{\{}{\'{e}}{\}}e sur la vitesse du jet {\{}{\`{a}}{\}} travers l'ouverture de la soupape pr{\{}{\'{e}}{\}}dit correctement le transfert de chaleur d{\{}{\^{u}}{\}} {\{}{\`{a}}{\}} ce mouvement {\{}{\`{a}}{\}} grande {\{}{\'{e}}{\}}chelle. Des mod{\{}{\`{e}}{\}}les pour l'{\{}{\'{e}}{\}}chappement instantan{\{}{\'{e}}{\}} fournissent un accord excellent avec des mesures pour les conditions de fonctionnement du moteur. Wegen des zunehmenden Bedarfs an genauer Information {\{}{\"{u}}{\}}ber Verbrennungsmotoren-Prozesse wurden in dieser Studie Modelle f{\{}{\"{u}}{\}}r den momentanen W{\{}{\"{a}}{\}}rme{\{}{\"{u}}{\}}bergang in einer Motor-Ausla{\$}\beta{\$}-{\{}{\"{O}}{\}}ffnung entwickelt und experimentell best{\{}{\"{a}}{\}}tigt. Die Momentanwerte des Zylinderdrucks und der Abgastemperatur wurden in Versuchen f{\{}{\"{u}}{\}}r einen ausgedehnten Betriebsbereich gemessen. Druckmessungen wurden verwendet, um den momentanen Gaszustand im Zylinder zu bestimmenn und Temperaturmessungen dienten zur Best{\{}{\"{a}}{\}}tigung der W{\{}{\"{a}}{\}}rme{\{}{\"{u}}{\}}bergangs-Modelle. Der W{\{}{\"{a}}{\}}rme{\{}{\"{u}}{\}}bergang in der Ausla{\$}\beta{\$}-{\{}{\"{O}}{\}}ffnung wurde im wesentlichen durch die strahlinduzierte Makro-Bewegung des Fluides entgegen der durch Wandschubspannung erzeugten Fluidbewegung bestimmt. Eine theoretische Untersuchung, die sich auf die Strahlgeschwindigkeit durch die Ventil{\{}{\"{o}}{\}}ffnung st{\{}{\"{u}}{\}}tzt, liefert korrekt den W{\{}{\"{a}}{\}}rme{\{}{\"{u}}{\}}bergang, hervorgerufen durch diese Makro-Bewegung. Die Modelle f{\{}{\"{u}}{\}}r den momentanen W{\{}{\"{a}}{\}}rme{\{}{\"{u}}{\}}bergang in der Ausla{\$}\beta{\$}-{\{}{\"{O}}{\}}ffnung als Funktion der Arbeitsbedingungen des Motors zeigten vorz{\{}{\"{u}}{\}}gliche {\{}{\"{U}}{\}}bereinstimmung mit den Messungen. B cвязи c вce бoлee вoзpacтaющeй нeoбчoдимocтью в тoчнoй инфopмaции o пpoцeccaч, пpoиcчoдящич в двигaтeляч, пpeдлoзeны мoдeди тeплoпepeнoca в вычлoпнoм oтвepcтии двигaтeля. Измepялиcь дaвлeниe в цилиндpe и тeмпepaтypa вычлoпнoгo гaзa пpи paздичныч peзимaч paбoты двигaтeля. Дaнныe пo дaвлeнию иcпoльзoвaлиcь для oпpeдeлeния cocтoяния гaзa в цилиндpe, a пo тeмпepaтype — для пpoвepки cпpaвeдливocти пpeдлoзeнныч мoдeлeй. Teплoпepeнoc в вычлoпнoм oтвepcтии oпpeдeляeтcя кpyпнoмacштaбными пepeмeщeниями зидкocти, вoзникaющими пpи cтpyйнoм иcтeчeнии, кoтopыe cyщecтвeннo oтличaютcя oт пepeмeщeний, вызывaeмыч нaпpязeниeм cдвигa нa cтeнкe. Aнaлиз, ocнoвaный нa cкopocти иcтeчeния cтpyи чepeз oтвepcтиe клaпaнa, пoзвoляeт кoppeктнo oцeнить вeличинy тeплoвoгo пoтoкa пpи тaкич кpyпнoмacщтaбпыч пepeмeщeнияч. Moдeли тeплoпepeнoca в вычлoпнoм oтвepcтии чopoшo coглacyютcя c peзyльтaтaми измepeний пpи paзличныч peзимaч paбoты двигaтeдя.},
author = {Caton, J A and Heywood, J B},
doi = {https://doi.org/10.1016/0017-9310(81)90003-X},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/1981{\_}An experimental and analytical study of heat transfer in an engine exhaust port{\_}Caton.pdf:pdf},
journal = {Int. J. Heat Mass Transf.},
number = {4},
pages = {581--595},
title = {{An experimental and analytical study of heat transfer in an engine exhaust port}},
volume = {24},
year = {1981}
}
@article{Chemie1806b,
author = {Chemie, Organische},
pages = {1--16},
title = {{1 Einf{\{}{\"{u}}{\}}hrung}},
year = {1806}
}
@inproceedings{972938,
abstract = {The purpose of this study is to outline the effects of aerodynamics on the heat losses of a S.I. multivalve engine and to link these results with the energetic efficiency of the engine. For that aim, we measured the local and instantaneous heat transfer in a 1.6 1 spark-ignited engine with several heat flux probes inserted in the cylinder head and in the liner of the combustion chamber. Two different cylinder heads were instrumented. They allowed to create distinct air motion configurations (baseline without structured flow, swirl and two levels of tumble). Furthermore, the pressure history was determined in the same cylinder than the heat transfer measurements. For all these configurations, we used a large range of operating conditions including several part loads, distinct equivalence ratios and two different engine speeds.Local heat transfer measurements on firing conditions showed clearly that the cycle by cycle and spatial variations, are directly linked to the flame propagation and that local heat losses increase with swirl and tumble. Moreover, the fuel consumption of the S.I. engine increases with air motion at low loads and under lean-burn conditions. The tendency is more significant for a tumble configuration.},
author = {Saulnier, Jean-Luc and Dupont, Alain and Rivere, Jean-Pierre and Jullien, Jacques},
booktitle = {Int. Fuels Lubr. Meet. Expo.},
doi = {https://doi.org/10.4271/972938},
issn = {0148-7191},
publisher = {SAE International},
title = {{Effects of Aerodynamics on Fuel Consumption of a Multivalve S-I Engine. Investigation of the Instantaneous Local Heat Transfer at Part Loads and Distinct Equivalence Ratios}},
url = {https://doi.org/10.4271/972938},
year = {1997}
}
@article{Horstemeyer1999,
abstract = {A phenomenological void–crack nucleation model for ductile metals with secondphases is described which is motivated from fracture mechanics and microscale physicalobservations. The void–crack nucleation model is a function of the fracture toughness of theaggregate material, length scale parameter (taken to be the average size of the second phaseparticles in the examples shown in this writing) , the volume fraction of the second phase, strainlevel, and stress state. These parameters are varied to explore their effects upon the nucleationand damage rates. Examples of correlating the void–crack nucleation model to tension data in theliterature illustrate the utility of the model for several ductile metals. Furthermore, compression,tension, and torsion experiments on a cast Al–Si–Mg alloy were conducted to determinevoid–crack nucleation rates under different loading conditions. The nucleation model was thencorrelated to the cast Al–Si–Mg data as well.},
author = {Horstemeyer, Mark F and Gokhale, Arun M},
doi = {10.1016/S0020-7683(98)00239-X},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Plasticity models/A void crack nucleation model for ductile metals with or without inclusions{\_}HorstemeyerAndGokhale.pdf:pdf},
isbn = {00207683 (ISSN)},
issn = {00207683},
journal = {Int. J. Solids Struct.},
pages = {5029--5055},
pmid = {111},
title = {{A Void-Crack Nucleation Model for Ductile Metals}},
volume = {36},
year = {1999}
}
@article{Burkhard2014,
author = {Burkhard, James F},
doi = {10.4271/2014-01-1167},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Thermal Coating + Water Heat Transfer + Applikation/2014{\_}Burkhard{\_}Individual Cylinder Fuel Control for a Turbocharged Engine.pdf:pdf},
journal = {SAE Tech. Pap. 2014-01-1167},
number = {2014},
title = {{Individual Cylinder Fuel Control for a Turbocharged Engine}},
year = {2014}
}
@article{Hilfe,
author = {Hilfe, Mit and Kenntnisstand, Sie Ihren and Sie, Hilfe and Detail-, Das and Sie, Falls and Aufgabe, Die and Unterlagen, Ihren and Aufgaben, Die and Sie, Schreiben and Aus-, Nach and Sie, Skizzieren and Sie, Schreiben and Sie, Schreiben and Programm, Das and Sie, Beschreiben},
title = {{10 {\{}{\"{U}}{\}}bungsaufgaben}}
}
@article{Betrachtungeng,
author = {Betrachtungen, Allgemeine},
title = {{Omungen}}
}
@article{Irimescu2013,
abstract = {An equation developed for the case of turbulent flow in tubes was applied for the study of convective heat transfer in internal combustion engines. Calculated average heat flux values under motored conditions were compared to measurements, results available in the literature obtained by using a computational fluid dynamics (CFD) code and the correlations of Woschni and Annand. Cumulative heat flux values for the four models were also compared to measurements at the end of the compression stroke and start of expansion. Average heat transfer rates were found to be predicted with reasonable accuracy by the proposed model. The major advantage of this equation compared to the correlations of Woschni and Annand is that it does not require any corrections for specific engine characteristics or working conditions. The proposed model was found to correctly predict higher heat transfer rates as engine speed, load and compression ratio were increased. Accuracy at the end of the compression stroke was found to be within acceptable limits for the cumulative heat flux, comparable to that of the CFD code, except for one case of the seven different engines investigated. Therefore, this model can be used to predict spatial average convective heat flux values with fairly good accuracy under motored conditions, when limited information on engine geometry is available, or when computing resources are required to be minimal. {\textcopyright} 2012 Elsevier Ltd. All rights reserved.},
author = {Irimescu, Adrian},
doi = {10.1016/j.applthermaleng.2012.06.051},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Heat Transfer Combustion Chamber/2013{\_}Irimescu{\_}Convective heat transfer equation for turbulent flow in tubes applied to ICE operated under motored conditions.pdf:pdf},
isbn = {1359-4311},
issn = {13594311},
journal = {Appl. Therm. Eng.},
keywords = {CFD modeling,Convective heat transfer,Empirical equation,Internal combustion engines,Motored operation,Turbulent flow},
number = {1},
pages = {536--545},
publisher = {Elsevier Ltd},
title = {{Convective heat transfer equation for turbulent flow in tubes applied to internal combustion engines operated under motored conditions}},
url = {http://dx.doi.org/10.1016/j.applthermaleng.2012.06.051},
volume = {50},
year = {2013}
}
@article{Aslan2010,
author = {Aslan, Ozgur},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/2010{\_}Aslan{\_}Numerical modeling of fatigue crack growth in single crystal nickel based superalloys.pdf:pdf},
title = {{Numerical modeling of fatigue crack growth in single crystal nickel based superalloys Ozgur Aslan l ' {\'{E}}cole nationale sup{\'{e}}rieure des mines de Paris Sp{\'{e}}cialit{\'{e}} « Sciences et G{\'{e}}nie des Mat{\'{e}}riaux » Simulation num{\'{e}}rique de la fissuration par fatigue dans les }},
year = {2010}
}
@article{Arnoldb,
author = {Arnold, J{\"{o}}rg},
pages = {787--792},
title = {{C5 C5 Reifen und R{\{}{\"{a}}{\}}der C5 Reifensch{\{}{\"{a}}{\}}den als Unfallfolgen}}
}
@article{Mehrphasensysteme,
author = {Mehrphasensysteme, Verkettete and Stern, Der and Polygon, Der},
title = {{7 Mehrphasensysteme 7.1}}
}
@article{Hashin1962a,
abstract = {Variational principles for anisotropic and nonhomogeneous elasticity, established by the authors in a previous paper, have been applied to the derivation of lower and upper bounds for the elastic moduli of polycrystals in terms of the moduli of the constituting crystals. The results hold for arbitrary crystal shapes. Explicit results tor cubic polycrystals showed that the present bounds are a considerable improvement of the well-known Voigt and Reuss bounds. Good agreement with experimental results has been obtained.},
author = {Hashin, Z. and Shtrikman, S.},
doi = {10.1016/0022-5096(62)90005-4},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/Strukturmechanik MMS/Literatur/Hashin Shtrikman 1962.pdf:pdf},
issn = {00225096},
journal = {J. Mech. Phys. Solids},
number = {4},
pages = {343--352},
title = {{A variational approach to the theory of the elastic behaviour of polycrystals}},
url = {http://linkinghub.elsevier.com/retrieve/pii/0022509662900054},
volume = {10},
year = {1962}
}
@article{Ansatz,
author = {Ansatz, Ein},
journal = {Sein},
pages = {71--91},
title = {{4 Objektorientierte Modellbildung des fahrdynamischen Verhaltens mit M ODELICA}}
}
@article{Roman2009,
author = {Roman, Kenneth},
isbn = {9783540718512},
journal = {David Ogilvy - Ein Leb. f{\"{u}}r die Werbung},
title = {{Literatur und Quellen}},
year = {2009}
}
@article{Gratzera,
author = {Gratzer, Werner and Becke, Manfred},
pages = {89--169},
title = {{A5 A5 Kinematik A5}}
}
@article{Pahl2007g,
author = {Pahl, Gerhard and Beitz†, Wolfgang and Feldhusen, J{\"{o}}rg and Grote, Karl-H.},
journal = {Pahl/Beitz Konstr. - Grundlagen},
title = {{L{\"{o}}sungsfelder}},
year = {2007}
}
@article{Svendsen1995,
abstract = {This work is concerned with the formulation of a constitutive model for a saturated or unsaturated, single-temperature mixture of n (???2) heat-conducting, isotropic viscous materials, the first m ??? n of which possess a variable true mass density. To do this, we extend the M??ller-Liu approach to the formulation and exploitation of the mixture entropy inequality. This approach yields, among other things, a generalized Gibbs' relation for such a mixture, as well as integrability conditions for the mixture entropy, and "extra" entropy flux, densities. Reduction of these general results to results comparable to those obtained in the standard approach necessitates two further constitutive assumptions: (1) the constraint field ("Lagrange multiplier") associated with the mixture reduced energy balance in the entropy inequality is equal to the mixture absolute coldness, and (2) that associated with the constituent momentum balance in the entropy inequality is equal to the negative of the mixture absolute coldness times the corresponding diffusion velocity. On this basis, for example, the inner parts of the mixture specific internal and Helmholtz free energies, as well as the mixture specific entropy, depend only on the mixture absolute temperature, the constituent true mass densities of the m "compressible" constituents, the volume densities of the first v constituents (with v = m in the unsaturated, and v = n - 1 in the saturated, case), and the constituent left Cauchy-Green deformation tensors. In the context of thermodynamic equilibrium, the entropy inequality yields, among other things, the interesting result that the constituent equilibrium thermodynamic pressure depends in a saturated mixture directly on the mixture saturation constraint field, but not on that associated with the evolution relations for the constituent (infinitesimal) volume fractions. As such, the so-called "closure problem" in volume-fraction-based mixture theory does not arise in the current formulation. ?? 1995.},
author = {Svendsen, Bob and Hutter, Kolumban},
doi = {10.1016/0020-7225(95)00044-X},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Thermodynamik/Liu-Entropieprinzip{\_}Lukas{\_}Fraunhofer/Liu-Entropieprinzip/Svendsen{\_}Hutter{\_}mixture{\_}with{\_}constraints{\_}1995.pdf:pdf},
issn = {00207225},
journal = {Int. J. Eng. Sci.},
number = {14},
pages = {2021--2054},
title = {{On the thermodynamics of a mixture of isotropic materials with constraints}},
volume = {33},
year = {1995}
}
@article{Winkler2014a,
author = {Winkler, N.},
doi = {10.1177/1468087414544899},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2015{\_}Winkler{\_}Effect of pressure oscillations on in-cylinder heat transfer  - through LES Simulation.pdf:pdf},
isbn = {1468087414544},
issn = {1468-0874},
journal = {Int. J. Engine Res.},
keywords = {24 june 2014,6 march 2014,accepted,computational fluid dynamics,date received,heat transfer,internal combustion engines,large eddy simulation,pressure oscillations},
number = {6},
pages = {705--715},
title = {{Effect of pressure oscillations on in-cylinder heat transfer - through large eddy simulation}},
url = {http://jer.sagepub.com/lookup/doi/10.1177/1468087414544899},
volume = {16},
year = {2014}
}
@article{Arnold1998,
author = {Arnold, J{\"{o}}rg and Verkehrsunf{\"{a}}llen, Bei},
pages = {781--786},
title = {{C4 C4 Schutzhelme Erste Untersuchungen am Helm C4 Besch{\{}{\"{a}}{\}}digungen am Helm}},
year = {1998}
}
@article{Burgb,
author = {Burg, Heinz},
pages = {595--611},
title = {{B1 B1 Unf{\"{a}}lle mit Tieren B1}}
}
@article{Mesarovic2017,
author = {Mesarovic, S},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/Folien CISM Summer School Mai2017 - Mesoscale Models/courses{\_}C1703{\_}Mesarovic+Lecture+5+CORR+2.pdf:pdf},
title = {{Physical foundations of meso-scale continua Part 2 : ( Thermo- ) Dynamics}},
year = {2017}
}
@article{Zienkiewicz2013b,
abstract = {In this chapter we present matrix differential equations governing transient problems for a variety of physical situations. A finite element discretization in the space dimension is used and a semi-discretization process followed (as introducled in Chapters 3 and 5). For structural problems the result is a set of equations involving a mass, damping and stiffness matrix. The second order equation in time may be solved formally using analytical methods in which time is represented by exponential functions. For undamped systems this leads to a classical eigen-problem in which the natural frequencies and mode shapes for a system may be identified. Including damping makes the solution feasible in complex arithmetic. General transient solutions are obtained from modal representations. A second form is forced periodic response in which applied force is represented in periodic form.},
author = {Zienkiewicz, O.C. and Taylor, R.L. and Zhu, J.Z.},
doi = {10.1016/B978-1-85617-633-0.00012-5},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Zienkiewicz FEM - Vol 1 Basics Fundamentals/63205{\_}16.pdf:pdf},
isbn = {9781856176330},
issn = {00295981},
journal = {Finite Elem. Method its Basis Fundam.},
pages = {379--405},
title = {{The Time Dimension: Semi-Discretization of Field and Dynamic Problems}},
url = {http://linkinghub.elsevier.com/retrieve/pii/B9781856176330000125},
year = {2013}
}
@article{Mandadapu2012,
abstract = {This article proposes a continuum thermomechanical homogenization method inspired by the Irving-Kirkwood procedure relating the atomistic equations of motion to the balance laws of continuum mechanics. This method yields expressions for the macroscopic stress and heat flux in terms of microscopic kinematic and kinetic quantities. The resulting equation for macroscopic stress affords a rational comparison with the widely used Hill-Mandel stress-deformation condition, while the one for heat flux reduces, under certain assumptions, to a Hill-Mandel-like condition involving heat flux and the gradient of temperature.},
archivePrefix = {arXiv},
arxivId = {84862181137},
author = {Mandadapu, K. K. and Sengupta, A. and Papadopoulos, P.},
doi = {10.1098/rspa.2011.0578},
eprint = {84862181137},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/A homogenization method for thermomechanical continua using extensive physical quantities.pdf:pdf},
isbn = {1364-5021$\backslash$r1471-2946},
issn = {1364-5021},
journal = {Proc. R. Soc. A Math. Phys. Eng. Sci.},
keywords = {hill,homogenization,irving,kirkwood procedure,mandel condition,thermomechanics},
number = {2142},
pages = {1696--1715},
title = {{A homogenization method for thermomechanical continua using extensive physical quantities}},
url = {http://rspa.royalsocietypublishing.org/content/early/2012/02/16/rspa.2011.0578.full},
volume = {468},
year = {2012}
}
@article{Einheit,
author = {Einheit, Die and Signale, Analoge},
journal = {Pulse},
title = {{Antworten und L{\"{o}}sungen zu den Kontrollfragen und {\"{U}}bungsaufgaben}}
}
@article{Bodies2003,
author = {Bodies, Elastic},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Nicholson 2003 - Finite Element Analysis Thermomechanics of Solids/0749{\_}C12.pdf:pdf},
journal = {Elements},
pages = {167--172},
title = {{Rotating and Unrestrained Elastic Bodies 12.1}},
year = {2003}
}
@article{Softwareergonomie,
author = {Softwareergonomie, Angewandte and Liskowsky, R{\"{u}}diger and W{\"{u}}nschmann, Wolfgang and R{\"{u}}diger, Prof and Prof, Liskowsky},
pages = {1},
title = {{1 Vorbemerkung}}
}
@article{Robinson2003a,
author = {Robinson, J S and Cudd, R L and Evans, J T},
doi = {https://doi.org/10.1179/026708303225009373},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Empirical Fatigue Models + Validation/2003{\_}Robinson{\_}Creep resistant aluminium alloys - experiments overview with different alloys - Al2618T6.pdf:pdf},
journal = {Mater. Sci. Technol.},
number = {2},
pages = {143--155},
title = {{Creep resistant aluminium alloys and their applications}},
volume = {19},
year = {2003}
}
@article{Zustandsgr,
author = {Zustandsgr, Kritische and Acetylen, Stoff and Argon, Ammoniak and Ethan, Butan and Ethylen, Ethanol and Kohlendioxid, Helium and Methan, Kohlenmonoxid and Propan, Oktan and Schwefeldioxid, Sauerstoff and Wasser, Stickstoff and Co, He and Ch, C O},
title = {{Anhang}}
}
@article{Shiling1979,
author = {Sihling, K. and Woschni, G.},
doi = {https://doi.org/10.4271/790833},
journal = {SAE Pap.},
number = {790833},
title = {{Experimental Investigation of the Instantaneous Heat Transfer in the Cylinder of a High Speed Diesel Engine}},
year = {1979}
}
@article{Sangid2010,
abstract = {In many engineering alloys, there exists a wide distribution of grain sizes; we investigate the role of grain boundaries as a strengthening mechanism in such a material. The coincidental site lattice (CSL) model is a powerful mathematical tool to characterize grain boundaries (GBs) and identify 'special' boundaries, which display beneficial mechanical behavior. We define the CSL and describe a detailed procedure to obtain this information from the grain orientation mapping via electron back scattering diffraction (EBSD). From this information, we show the evolution of the CSL for a nickel-based superalloy, Udimet 720 (U720), throughout various stages of processing (billet and forging) and experiments (tension, compression, and fatigue). A deeper level of understanding the GB's role in the mechanical behavior of the material is investigated through atomic simulations using molecular dynamics (MD) as the GB energy is determined for the most prevalent GBs within this material. The spatial map of the orientation and grain sizes measured from EBSD is linked to the GB energies calculated from MD. Based upon the large number of boundaries analyzed (29,035), there is a strong inverse correlation between GB energy and grain size for every specimen examined during the various processing and testing conditions. ?? 2010 Elsevier B.V.},
author = {Sangid, Michael D. and Sehitoglu, Huseyin and Maier, Hans J. and Niendorf, Thomas},
doi = {10.1016/j.msea.2010.07.062},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/2010{\_}Sangid{\_}Grain boundary characterization and energetics of superalloys.pdf:pdf},
isbn = {0921-5093},
issn = {09215093},
journal = {Mater. Sci. Eng. A},
keywords = {Coincidence site lattice (CSL),Electron back scattering diffraction (EBSD),Grain boundary energy,Molecular dynamics simulations,Nickel-based superalloys},
number = {26},
pages = {7115--7125},
publisher = {Elsevier B.V.},
title = {{Grain boundary characterization and energetics of superalloys}},
url = {http://dx.doi.org/10.1016/j.msea.2010.07.062},
volume = {527},
year = {2010}
}
@article{Finite2014,
author = {Finite, The and Method, Element and Basis, Its},
doi = {10.1016/B978-1-85617-635-4.00032-7},
journal = {Finite Elem. Method Fluid Dyn.},
pages = {519--520},
title = {{Multigrid Method}},
url = {http://linkinghub.elsevier.com/retrieve/pii/B9781856176354000327},
year = {2014}
}
@article{Hill1952a,
abstract = {The connection between the elastic behaviour of an aggregate and a single crystal is considered, with special reference to the theories of Voigt, Reuss, and Huber and Schmid. The elastic limit under various stress systems is also considered, in particular, it is shown that the tensile elastic limit of a face-centred aggregate cannot exceed two-thirds of the stress at which pronounced plastic distortion occurs.},
author = {Hill, R},
doi = {10.1088/0370-1298/65/5/307},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/Strukturmechanik MMS/Literatur/Hill 1952.pdf:pdf},
isbn = {0370-1298},
issn = {0370-1298},
journal = {Proc. Phys. Soc. Sect. A},
number = {5},
pages = {349--354},
title = {{The Elastic Behaviour of a Crystalline Aggregate}},
url = {http://stacks.iop.org/0370-1298/65/i=5/a=307?key=crossref.630b67f122246b4defcc5fda55c7bf20},
volume = {65},
year = {1952}
}
@article{Beanspruchungsablaufa,
author = {Beanspruchungsablauf, Der},
title = {{5 Betriebsfestigkeit 5.1}}
}
@article{Schumacher2013,
author = {Schumacher, Axel},
doi = {10.1007/978-3-642-34700-9},
isbn = {9783642347009},
journal = {Optimierung Mech. Strukt.},
pages = {9--44},
title = {{Grundwissen zur Entwicklung mechanischer Systeme 2}},
year = {2013}
}
@inproceedings{Fontanesi2011,
abstract = {The paper presents a combined experimental and numerical activity carried out to improve the accuracy of conjugate heat transfer CFD simulations of a high-performance S.I. engine water cooling jacket.Due to the complexity of the computational domain, which covers both the coolant jacket and the surrounding metal cast (both head and block), particular care is required in order to find a tradeoff between the accuracy and the cost-effectiveness of the numerical procedure. In view of the presence of many complex physical phenomena, the contribution of some relevant CFD parameters and sub-models is separately evaluated and discussed.Among the formers, the extent of the computational domain, the choice of a proper set of boundary conditions and the detailed representation of the physical properties of the involved materials are separately considered. Among the latters, the choice between a simplified single-phase approach and a more complex two-phase approach taking into account the effects of phase transition within the engine coolant is discussed.The predictive capability of the CFD-CHT methodology is assessed by means of the comparison between CFD results and experimental measurements provided by the engine manufacturer for different engine operating conditions.At the end of the validation process, a methodology for the correct and cost-effective characterization of conjugate heat transfer is proposed, showing a reasonable trade-off between the predictive capability and the computational effort of the simulations.},
author = {Fontanesi, Stefano and Cicalese, Giuseppe and D'Adamo, Alessandro and Pivetti, Gianluca},
booktitle = {10th Int. Conf. Engines Veh.},
doi = {10.4271/2011-24-0132},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Boiling/2011{\_}Fontanesi{\_}Validation of a CFD Methodology for the Analysis of CHT in a high performance SI engine{\_}No Boling used.pdf:pdf},
month = {sep},
publisher = {SAE International},
title = {{Validation of a CFD Methodology for the Analysis of Conjugate Heat Transfer in a High Performance SI Engine}},
year = {2011}
}
@article{Festk2006,
author = {Festk, Makromolekulare},
journal = {Gerthsen Phys.},
pages = {883--967},
title = {{17 - Festk{\{}{\"{o}}{\}}rperphysik}},
year = {2006}
}
@article{Hartey,
author = {Hartey, Beispiel and Motorrad, B M W},
pages = {391--414},
title = {{Individualisierung 13 Zubeh{\{}{\"{o}}{\}}r , Spezialteile und technische Verfeinerung}}
}
@book{Riccardella1992,
author = {Riccardella, P C and Deardorff, A F and Griesbach, T J},
booktitle = {Adv. Fatigue Lifetime Predict. Tech.},
doi = {10.1520/STP1122-EB},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Neuer Ordner/Advances in fatigue lifetime predictive techniques Part1.pdf:pdf},
isbn = {978-0-8031-1423-4},
issn = {00660558},
keywords = {FATIGUE,MONITORING,POWER PLANTS,PRESSURE VESSELS AND PIPING,THERMAL STRESSES},
pages = {460--473},
pmid = {11439068},
title = {{Advances in Fatigue Lifetime Predictive Techniques}},
url = {https://apps.webofknowledge.com/full{\%}7B{\_}{\%}7Drecord.do?product=UA{\%}7B{\&}{\%}7Dsearch{\%}7B{\_}{\%}7Dmode=GeneralSearch{\%}7B{\&}{\%}7Dqid=11{\%}7B{\&}{\%}7DSID=Z1UxbH6jtsqo8n9kPQr{\%}7B{\&}{\%}7Dpage=1{\%}7B{\&}{\%}7Ddoc=1},
volume = {1122},
year = {1992}
}
@article{Schneider2016c,
abstract = {{\textcopyright} 2016 Elsevier B.V.Modeling of crack propagation in materials has long been a challenge in solid-state physics and materials science. The phase-field method has now established as one of the tools for the description of crack propagation. The applied models are thermodynamically consistent and predict crack propagation in homogeneous materials under the consideration of different loading types, multiple physical fields and geometrical nonlinearities. Even dynamic loading processes are studied, including plastic effects. A multiphase-field model for crack propagation, which is indispensable to describe crack propagation on a mesoscopic length scale, is still missing. In this work, we overcome this deficiency and combine a crack propagation approach, which is based on Griffith's theory, with an established multiphase-field model for phase transformation.},
author = {Schneider, D. and Schoof, E. and Huang, Y. and Selzer, M. and Nestler, B.},
doi = {10.1016/j.cma.2016.04.009},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Thermodynamik/PhasenFeld/Schneider{\_}Crack{\_}propagation{\_}multiphase{\_}systems-Dez2015.pdf:pdf},
issn = {00457825},
journal = {Comput. Methods Appl. Mech. Eng.},
keywords = {crack propagation,multiphase-field,phase-field,polycrystalline material},
title = {{Phase-field modeling of crack propagation in multiphase systems}},
url = {http://dx.doi.org/10.1016/j.cma.2016.04.009},
year = {2016}
}
@phdthesis{Bargende1991Original,
author = {Bargende, Michael},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Injection+Combustion+Ignitionsystems/1992{\_}Bargende{\_}Gleichungsansatz{\_}instationäre{\_}Wandwärmeverluste{\_}Otto{\_}kl.pdf:pdf},
school = {Technische Hochschule Darmstadt},
title = {{Ein Gleichungssatz zur Berechnung der instation{\"{a}}ren Wandw{\"{a}}rmeverluste im Hochdruckteil von Ottomotoren}},
year = {1991}
}
@article{Ab,
author = {Ab, Strecke},
journal = {Delta},
pages = {1--53},
title = {{Mathematik Mathematische Zeichen 1.1}}
}
@article{Logue,
author = {Logue, Steve},
pages = {52--131},
title = {{19 Beispiele V5}}
}
@article{Cherkaoui2009f,
author = {Cherkaoui, Mohammed and Capolungo, Laurent},
doi = {10.1007/978-0-387-46771-9},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Atomistic and Continuum Modeling of Nanocrystalline Materials/Chapter 06.pdf:pdf},
isbn = {978-0-387-46765-8},
title = {{Atomistic and Continuum Modeling of Nanocrystalline Materials}},
url = {http://link.springer.com/10.1007/978-0-387-46771-9},
volume = {112},
year = {2009}
}
@article{Interaction2012,
author = {Interaction, Creep-fatigue},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Kriechen{\_}Spannungsrelaxation/2012{\_}Weaver{\_}Creep-Fatigue Interaction - An overview.pdf:pdf},
pages = {1--13},
title = {{Module {\{}{\#}{\}} 40 Creep- Creep- Let ' s review our basic fracture mechanisms before}},
year = {2012}
}
@article{Loubar2005,
abstract = {This paper deals with the transient thermal signal around an engine cylinder in order to propose a new and nonintrusive method of knock detection. Numerical simulations of unsteady heat transfer through the cylinder and inside the coolant flow are carried out to account for heat flux variations due to normal and knocking combustion. The effect of rib roughened surfaces on thermal signal amplification is investigated. The geometric parameters are fixed at Pi/h=70 and w/h=1 with a Reynolds number based on hydraulic diameter of 12,000. The results reveal that square ribs give better performance in term of thermal signal amplification within the fluid. An amplification of the temperature variation up to 20 times higher is found. Finally, flow analysis shows that amplification depends on the position where the thermal signal is collected.},
author = {Loubar, Khaled and Bellettre, Jérôme and Tazerout, Mohand},
doi = {10.1115/1.1857943},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2005{\_}Loubar{\_}Unsteady Heat Transfer enhancement around an engine cylinder in order to detect knockpdf.pdf:pdf},
isbn = {0022-1481},
issn = {00221481},
journal = {J. Heat Transf.},
number = {3},
pages = {278},
title = {{Unsteady Heat Transfer Enhancement Around an Engine Cylinder in Order to Detect Knock}},
url = {http://heattransfer.asmedigitalcollection.asme.org/article.aspx?articleid=1447711},
volume = {127},
year = {2005}
}
@article{Sachverhalt,
author = {Sachverhalt, Diesen and Wissen, Das and Erstellung, Die and Entwicklungsschritt, Dieser and Burntest, Verarbeitungsunterlagen and Verf, Liste and Checkliste, Verbesserungen Diese and Vdi, V D E Richtlinien},
title = {{Entwicklung von µ-Computer-Hardware}}
}
@article{Lerch2016,
abstract = {Dieses Lehrbuch bietet eine umfassende Einf{\{}{\"{u}}{\}}hrung in die moderne Elektrische Messtechnik. Behandelt werden: die Fehlerrechnung systematischer und zuf{\{}{\"{a}}{\}}lliger Fehler, die Erfassung von dynamischen Messfehlern und ihren Korrekturen, Ger{\{}{\"{a}}{\}}te und Verfahren der analogen Messtechnik, wie z.B. Standard-Messger{\{}{\"{a}}{\}}te, elektronische Messverst{\{}{\"{a}}{\}}rker, Messbr{\{}{\"{u}}{\}}cken. Anschlie{\{}{\ss}{\}}end werden Analog-Digital- und Digital-Analog-Umsetzer sowie digitale Messger{\{}{\"{a}}{\}}te beschrieben. Ein weiterer Schwerpunkt des Buches ist die ausf{\{}{\"{u}}{\}}hrliche Behandlung der modernen computerunterst{\{}{\"{u}}{\}}tzten Messdatenerfassung und Messsignalverarbeitung bez{\{}{\"{u}}{\}}glich Hard- und Software. In der 4. Auflage wurden die Kapitel zur rechnergest{\{}{\"{u}}{\}}tzten Messdatenerfassung dem allerneuesten Stand der Technik angepasst und die Abschnitte zur Messsignalverarbeitung erheblich erweitert. Es ist eine DVD mit {\{}{\"{U}}{\}}bungsaufgaben zur rechnergest{\{}{\"{u}}{\}}tzten Messdatenerfassung und Messsignalverarbeitung sowie zur Programmierung von Speicherprogrammierbaren Steuerungen (SPS) enthalten. Via Internet kann der Leser eine am Lehrstuhl f{\{}{\"{u}}{\}}r Sensorik aufgebaute SPS programmieren sowie weitere {\{}{\"{U}}{\}}bungsaufgaben und L{\{}{\"{o}}{\}}sungen zu den Programmieraufgaben von der DVD herunterladen. Die DVD enth{\{}{\"{a}}{\}}lt au{\{}{\ss}{\}}erdem eine Studentenversion von LabVIEW 8.2.1. Das Buch eignet sich in Verbindung mit dem Werk Elektrische Messtechnik/{\{}{\"{U}}{\}}bungsbuch f{\{}{\"{u}}{\}}r Studierende der Ingenieur- und Naturwissenschaften sowie f{\{}{\"{u}}{\}}r den in der Praxis t{\{}{\"{a}}{\}}tigen Ingenieur auch zum Selbststudium.},
author = {Lerch, R},
doi = {10.1007/978-3-8348-8304-9_3},
isbn = {978-3-8348-1374-9},
issn = {0937-7433},
journal = {Elektrische Messtechnik},
title = {{Geb{\{}{\"{a}}{\}}udeautomatisierung (Smart Home)}},
url = {http://dx.doi.org/10.1007/978-3-8348-8304-9{\%}7B{\_}{\%}7D3},
year = {2016}
}
@article{Fahrwerk,
author = {Fahrwerk, Das and Methoden, Folgenden and Aktor, Dieser and Hydraulikzylinder, Dieser and An-, Diese},
journal = {Praxis (Bern. 1994).},
pages = {431--451},
title = {{20 Diagnose und Sensor-Fehlertoleranz aktiver}}
}
@article{Foundations2003,
author = {Foundations, Mathematical},
pages = {1--23},
title = {and},
year = {2003}
}
@article{Apparaten,
author = {Apparaten, Berechnung Von},
title = {{Verdampfung}}
}
@article{Papulad,
author = {Papula, Lothar},
pages = {470--540},
title = {{Integraltafel}}
}
@article{Theoreme1964,
author = {Theoreme, Kohn},
doi = {10.1007/978-3-540-72637-1},
isbn = {9783642054952},
pages = {139--150},
title = {{Kapitel 9}},
year = {1964}
}
@article{Verbrennungsmotor2007,
author = {Verbrennungsmotor, Der and Anfahren, Zum},
journal = {Fahrzeuggetriebe},
title = {{10 Anfahrelemente}},
volume = {1},
year = {2007}
}
@inproceedings{Hohenberg1979,
author = {Hohenberg, G. F.},
booktitle = {SAE Tech. Pap. 790825},
doi = {https://doi.org/10.4271/790825},
title = {{Advance approaches for heat transfer calculation}},
year = {1979}
}
@article{Hochhalter2010a,
abstract = {The objective of this paper is to develop further a framework for computationally modeling$\backslash$nmicrostructurally small fatigue crack growth in AA 7075-T651 (Bozek et al 2008 Modelling Simul.$\backslash$nMater. Sci. [/0965-0393/16] 16 065007 ). The focus is on the nucleation event, when a crack extends$\backslash$nfrom within a second-phase particle into a surrounding grain, since this has been observed to be an$\backslash$ninitiating mechanism for fatigue crack growth in this alloy. It is hypothesized that nucleation can$\backslash$nbe predicted by computing a non-local nucleation metric near the crack front. The hypothesis is$\backslash$ntested by employing a combination of experimentation and finite element modeling in which various$\backslash$nslip-based and energy-based nucleation metrics are tested for validity, where each metric is derived$\backslash$nfrom a continuum crystal plasticity formulation. To investigate each metric, a non-local procedure$\backslash$nis developed for the calculation of nucleation metrics in the neighborhood of a crack front.$\backslash$nInitially, an idealized baseline model consisting of a single grain containing a semi-ellipsoidal$\backslash$nsurface particle is studied to investigate the dependence of each nucleation metric on lattice$\backslash$norientation, number of load cycles and non-local regularization method. This is followed by a$\backslash$ncomparison of experimental observations and computational results for microstructural models$\backslash$nconstructed by replicating the observed microstructural geometry near second-phase particles in$\backslash$nfatigue specimens. It is found that orientation strongly influences the direction of slip$\backslash$nlocalization and, as a result, influences the nucleation mechanism. Also, the baseline models,$\backslash$nreplication models and past experimental observation consistently suggest that a set of particular$\backslash$ngrain orientations is most likely to nucleate fatigue cracks. It is found that a continuum crystal$\backslash$nplasticity model and a non-local nucleation metric can be used to predict the nucleation event in AA$\backslash$n7075-T651. However, nucleation metric threshold values that correspond to various nucleation$\backslash$ngoverning mechanisms must be calibrated.},
author = {Hochhalter, J D and Littlewood, D J and Christ, R J and Veilleux, M G and Bozek, J E and Ingraffea, A R and Maniatty, A M},
doi = {10.1088/0965-0393/18/4/045004},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/2010{\_}Hochhalter{\_}AL7075AgeometricapproachII{\_}SlipAndNucleation.pdf:pdf},
isbn = {0965-0393},
issn = {0965-0393},
journal = {Model. Simul. Mater. Sci. Eng.},
number = {4},
pages = {045004},
title = {{A geometric approach to modeling microstructurally small fatigue crack formation: II. Physically based modeling of microstructure-dependent slip localization and actuation of the crack nucleation mechanism in AA 7075-T651}},
url = {http://stacks.iop.org/0965-0393/18/i=4/a=045004?key=crossref.ef8bc48536790be47a24f27989602c36},
volume = {18},
year = {2010}
}
@inproceedings{Borgnakke1980_Turbulence,
abstract = {The heat transfer and turbulence are modeled for a spark-ignition engine. The heat transfer is described in terms of unsteady boundary layers for both the burned and unburned gas regions. These boundary layers are influenced by both the free stream turbulence level and the rate of flame propagation. Turbulence levels are characterized by a K-$\epsilon$ model which includes the effects of compressibility and anisotropic behavior of the flow field. The flame propagation process is modeled using current entrainment model philosophy.The results of the modeling are illustrated for an engine having a simple pancake geometry. The major accomplishments are the development of an unsteady, compressible turbulence model and the development of an instantaneous heat transfer model. The influence of the turbulent field on the heat transfer rate is given via the turbulent Reynolds number and the integral length scale. The averaged heat transfer rate is compared with the correlations of Annand and Woschni and the shortcomings of these simpler correlations are discussed.},
author = {Borgnakke, Claus and Arpaci, Vedat S and Tabaczynski, Rodney J},
booktitle = {Automot. Eng. Congr. Expo.},
doi = {https://doi.org/10.4271/800287},
publisher = {SAE International},
title = {{A Model for the Instantaneous Heat Transfer and Turbulence in a Spark Ignition Engine}},
year = {1980}
}
@article{Einsicht,
author = {ergibt sich die Einsicht, D},
journal = {Springer},
title = {{1 Physikalische und mathematische Hilfsmittel}},
url = {http://link.springer.com/chapter/10.1007/978-3-8351-9095-5{\_}1}
}
@article{Wellen,
author = {Wellen, Elektromagnetische},
title = {{Strahlung}}
}
@article{Cheong2007a,
abstract = {The influence of individual grain orientation on early fatigue crack initiation in a four-point bend fatigue test was investigated numerically and experimentally. The 99.99{\{}{\%}{\}} aluminium test sample was subjected to high cycle fatigue (HCF) and the top surface microstructure within the inner span of the sample was characterized using electron-beam backscattering diffraction (EBSD). Applying a finite-element submodelling approach, the microstructure was digitally reconstructed and refined studies carried out in regions where fatigue damage was observed. The constitutive behaviour of aluminium was described by a crystal plasticity model which considers the evolution of dislocations and accumulation of edge dislocation dipoles. Using an energy-based approach to quantify fatigue damage, the model correctly predicts regions in grains where early fatigue crack initiation was observed. The tendency for fatigue cracks to initiate in these grains appears to be strongly linked to the orientations of the grains relative to the direction of loading - grains less favourably aligned with respect to the loading direction appear more susceptible to fatigue crack initiation. The limitations of this modelling approach are also highlighted and discussed, as some grains predicted to initiate cracks did not show any visible signs of fatigue cracking in the same locations during testing. ?? 2006 Acta Materialia Inc.},
author = {Cheong, Ke Shen and Smillie, Matthew J and Knowles, David M},
doi = {10.1016/j.actamat.2006.10.038},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2006{\_}Cheong{\_}Predicting fatigue crack initiation through image-based micromechanical modeling.pdf:pdf},
isbn = {1359-6454},
issn = {13596454},
journal = {Acta Mater.},
keywords = {Crystal plasticity,Dislocations,Electron backscatter diffraction,Image analysis,Micromechanical modelling},
number = {5},
pages = {1757--1768},
title = {{Predicting fatigue crack initiation through image-based micromechanical modeling}},
volume = {55},
year = {2007}
}
@article{Einf1999,
author = {Einf, Seit and Reaktion, Als},
number = {C},
pages = {238--270},
title = {{7 Kraftstoff und Schmier{\{}{\"{o}}{\}}l}},
year = {1999}
}
@article{Aerostatik2006,
author = {Aerostatik, Hydro-},
journal = {Gerthsen Phys.},
pages = {93--140},
title = {{03 - Mechanik deformierbarer K{\{}{\"{o}}{\}}rper}},
year = {2006}
}
@article{Barrett1995,
abstract = {Which of the following statements is true? • Users want “black box” software that they can use with complete confidence for general problem classes without having to understand the fine algorithmic details. • Users want to be able to tune data structures for a particular application, even if the software is not as reliable as that provided for general methods. It turns out both are true, for different groups of users. Traditionally, users have asked for and been provided with black box software in the form of mathematical libraries such as LAPACK, LINPACK, NAG, and IMSL. More recently, the high performance community has discovered that they must write custom software for their problem. Their reasons include inadequate functionality of existing software libraries, data structures that are not natural or convenient for a particular problem, and overly general software that sacrifices too much performance when applied to a special case of interest. Can we meet the needs of both groups of users? We believe we can. Accordingly, in this book, we introduce the use of templates. A template is a description of a general algorithm rather than the executable object code or the source code more commonly found in a conventional software library. Nevertheless, although templates are general descriptions of key algorithms, they offer whatever degree of customization the user may desire. For example, they can be configured for the specific data structure of a problem or for the specific computing system on which the problem is to run. We focus on the use of iterative methods for solving large sparse systems of linear equations. Many methods exist for solving such problems. The trick is to find the most effective method for the problem at hand. Unfortunately, a method that works well for one problem type may not work as well for another. Indeed, it may not work at all. Thus, besides providing templates, we suggest how to choose and implement an effective method, and how to specialize a method to specific matrix types. We restrict ourselves to iter ative methods, which work by repeatedly improving an approximate solution until it is accurate enough. These methods access the coefficient matrix A of the linear system only via the matrix vector product y = A {\textperiodcentered} x (and perhaps z = A T {\textperiodcentered} x). Thus the user need only supply a subroutine for computing y (and perhaps z) given x, which permits full exploitation of the sparsity or other special structure of A. We believe that after reading this book, applications developers will be able to use templates to get their program running on a parallel machine quickly. Nonspecialists will know how to choose and implement an approach to solve a particular problem. Specialists will be able to assemble and modify their codes—without having to make the huge investment that has, up to now, been required to tune large-scale applications for each particular machine. Finally, we hope that all users will gain a better understanding of the algorithms employed. While education has not been one of 1 the traditional goals of mathematical software, we believe that our approach will go a long way in providing such a valuable service.},
author = {Barrett, Richard and Berry, Michael and Chan, Tony F. and Demmel, James and Donato, June M and Dongarra, Jack and Eijkhout, Victor and Pozo, Roldan and Romine, Charles and S., G. W. and van der Vorst, Henk},
doi = {10.2307/2153507},
isbn = {978-0-89871-328-2},
issn = {00255718},
journal = {Math. Comput.},
keywords = {Linear Systems,iterative methods},
number = {211},
pages = {1349},
title = {{Templates for the Solution of Linear Systems: Building Blocks for Iterative Methods.}},
url = {http://www.jstor.org/stable/2153507?origin=crossref},
volume = {64},
year = {1995}
}
@article{Pr,
author = {Pr, Diese and Ermitteln, Das},
title = {{7 Reifenpr{\{}{\"{u}}{\}}fungen}}
}
@article{Essmann1981,
abstract = {Based on recent experimental observations a realistic model of the evolution of the surface profile of persistent slip bands (PSBs) in fatigued metals is proposed. An essential feature of the model is the production of vacancies by the annihilation of edge dislocations which, combined with irreversible slip processes, leads to an elongation of the PSB parallel to the active slip vector. It is shown that a net extrusion forms rather rapidly. The growth processes and their dependence on temperature are discussed in detail. It is proposed that cracks initiate at the surface steps at the PSB{\{}{\&}{\}}ndash;matrix interface and, at a later stage, also at the notch-peak profile from the random slip processes.},
author = {Essmann, U and G{\"{o}}sele, U and Mughrabi, H},
doi = {10.1080/01418618108239541},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2016{\_}Mughrabi{\_}A model of extrusions and intrusions in fatigued metals I  Point defect production and the growth of extrusions.pdf:pdf},
isbn = {0141-8610},
issn = {0141-8610},
journal = {Philos. Mag. A},
number = {2},
pages = {405--426},
title = {{A model of extrusions and intrusions in fatigued metals I. Point-defect production and the growth of extrusions}},
url = {http://www.tandfonline.com/doi/abs/10.1080/01418618108239541},
volume = {44},
year = {1981}
}
@article{BERNI2017,
author = {Berni, Fabio and Cicalese, Giuseppe and Fontanesi, Stefano},
doi = {https://doi.org/10.1016/j.applthermaleng.2017.01.055},
journal = {Appl. Therm. Eng.},
keywords = {CFD,Conjugate heat transfer,Engine thermal survey,Heat transfer,Law of the wall,Thermal wall function},
pages = {1045--1062},
title = {{A modified thermal wall function for the estimation of gas-to-wall heat fluxes in CFD in-cylinder simulations of high performance spark-ignition engines}},
volume = {115},
year = {2017}
}
@article{Untersuchung,
author = {Untersuchung, Die and Konstanten, Der},
pages = {34--46},
title = {{5 Messeinrichtung}}
}
@book{Cherkaoui2009a,
author = {Cherkaoui, Mohammed and Capolungo, Laurent},
doi = {10.1007/978-0-387-46771-9},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Atomistic and Continuum Modeling of Nanocrystalline Materials/Chapter 08.pdf:pdf},
isbn = {978-0-387-46765-8},
title = {{Atomistic and Continuum Modeling of Nanocrystalline Materials}},
url = {http://link.springer.com/10.1007/978-0-387-46771-9},
volume = {112},
year = {2009}
}
@article{Schie??l2003,
abstract = {We investigate spatial temperature fluctuations in the unburned endgas of a spark-ignited (SI) engine. Our approach exploits the fact that the quantities (species concentrations, temperature) comprising the state of the combustion chamber gases are not independent, but often correlate sharply. Information about spatial temperature variations is obtained indirectly by observing two complementary quantities that sensitively reflect the local temperature. Spatial formaldehyde (H2CO) concentration variations in the endgas are converted to temperature fluctuations using calculated correlations between temperature and [H2CO]. Additionally, the geometrical size of inhomogeneities is deduced from LIF-images displaying the locally varying formation of temperature-sensitive intermediate species. The results indicate that temperature fluctuations exceeding 20 K are present in the nominally homogeneous endgas. The geometrical size of these fluctuations ranges from ???1 mm to ???1 cm. ?? 2003 The Combustion Institute. All rights reserved.},
author = {Schie??l, R and Maas, U},
doi = {10.1016/S0010-2180(02)00538-2},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Klopfen{\_}Ottomotor/2003{\_}Schiessl{\_}Analysis of endgas temperture fluctuations in an si engine by LIF.pdf:pdf},
isbn = {4907116855653},
issn = {00102180},
journal = {Combust. Flame},
keywords = {Endgas,IC engines,Laser-induced fluorescence,Temperature fluctuations},
number = {1-2},
pages = {19--27},
title = {{Analysis of endgas temperature fluctuations in an SI engine by laser-induced fluorescence}},
volume = {133},
year = {2003}
}
@article{Berger2003,
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Berger},
doi = {10.1002/ejoc.201200111},
eprint = {arXiv:1011.1669v3},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Vortraege/Book-of-Abstracts{\_}2016-03-04{\_}GAMM.pdf:pdf},
isbn = {9781107671812},
issn = {0196-6553},
journal = {Eng. Med. Biol. Soc. 2008. EMBS 2008. 30th Annu. Int. Conf. IEEE},
pages = {2004},
pmid = {26840611},
title = {{Table of of contents}},
volume = {24},
year = {2003}
}
@article{Druck2014,
author = {Druck, Der and Presse, Hydraulische and Schwerkraft, Der},
doi = {10.1007/978-3-642-38891-0},
isbn = {978-3-642-38890-3},
journal = {Maschinenelemente},
number = {3},
pages = {48--49},
title = {{Statik der Fl{\{}{\"{u}}{\}}ssigkeiten}},
url = {http://link.springer.com/10.1007/978-3-642-38891-0},
year = {2014}
}
@article{Konstruktion1997,
author = {Konstruktion, Bei Der},
pages = {1--6},
title = {{1 Einf{\"{u}}hrung}},
year = {1997}
}
@article{August2001,
author = {August, Auflage},
keywords = {Physik},
number = {August},
pages = {25},
title = {{Physik-Formelsammlung}},
year = {2001}
}
@article{Bozza2011a,
abstract = {In the present paper a combined procedure for the quasi-dimensional modelling of heat transfer, combustion and knock phenomena in a "downsized" Spark Ignition two-cylinder turbocharged engine is presented. The procedure is extended to also include the effects consequent the Cyclic Variability. Heat transfer is modelled by means of a Finite Elements model. Combustion simulation is based on a fractal description of the flame front area. Cyclic Variability (CV) is characterized through the introduction of a random variation on a number of parameters controlling the rate of heat release (air/fuel ratio, initial flame kernel duration and radius, laminar flame speed, turbulence intensity). The intensity of the random variation is specified in order to realize a Coefficient Of Variation (COV) of the Indicated Mean Effective Pressure (IMEP) similar to the one measured during an experimental campaign. Moreover, the relative importance of the various concurring effects is established on the overall COV. A kinetic scheme is then solved within the unburned gas zone, characterized by different thermodynamic conditions occurring cycle-by-cycle. In this way, an optimal choice of the "knock-limited" spark advance is effected and compared with experimental data. Finally, the CV effects on the occurrence of individual knocking cycles are assessed and discussed. {\textcopyright} 2011 Global Science Press.},
author = {Bozza, Fabio and Siano, Daniela and Costa, Michela},
doi = {10.4208/aamm.10-10s2-04},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2011{\_}Bozza{\_}heat-transfer-knock-modeling-and-cyclic-variability-in-a-downsized-spark-ignition-turbocharged-engine.pdf:pdf},
issn = {20700733},
journal = {Adv. Appl. Math. Mech.},
keywords = {Cyclic variability,Finite elements in heat transfer,Internal combustion engines modelling,Knock},
number = {3},
pages = {310--326},
title = {{Heat transfer, knock modeling and cyclic variability in a "Downsized" spark-ignition turbocharged engine}},
volume = {3},
year = {2011}
}
@inproceedings{Fontanesi2013Comb,
abstract = {The paper describes an integrated methodology for the accurate characterization of the thermal behavior of internal combustion engines, with particular reference to a high performance direct injected SI engine for sport car applications. The engine is operated at full load and maximum power revving speed, which is known to be critical from the point of view of thermal stresses on the engine components.In particular, two different sets of 3D-CFD calculations are adopted: on one side, full-cycle in-cylinder analyses are carried out to estimate the point wise thermal heat flux due to combustion on the engine components facing the combustion chamber. On the other side, full-engine multi-region CHT calculations covering the engine coolant jacket and the surrounding metal components are used to compute the point wise temperature distribution within the engine head, liner and block.An iterative procedure is then implemented in order to exchange relevant thermal data between the two modeling frameworks: at first, local gas temperatures and heat transfer coefficients from the in-cylinder simulations are applied as thermal loads to the CHT calculations; then, the resulting surface temperature maps are re-applied to the combustion chamber walls for the subsequent in-cylinder CFD analysis. The procedure is iteratively repeated until convergence is met in terms of thermal characterization of the engine.The procedure takes into account the non-uniform spatial distribution of both thermal loads from the combustion process and resulting temperature distribution on the combustion chamber walls, which are known to be particularly evident when considering direct injected stratified charged engines. The resulting thermal fields are compared to those deriving from a traditional approach for both the in-cylinder and CHT calculations, i.e. the application of uniform heat fluxes on the CHT side and the use of uniform wall temperatures on the in-cylinder side. The resulting differences are highlighted and critically discussed, with particular emphasis on those which could have a relevant impact on both the fatigue strength evaluation of the engine and the arising of local undesired phenomena such as surface ignition and knocking.},
author = {Fontanesi, Stefano and Cicalese, Giuseppe and Tiberi, Alessandro},
booktitle = {SAE 2013 World Congr. Exhib.},
doi = {10.4271/2013-01-1088},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/W{\"{a}}rme-RBen Kolben/2013{\_}Fontanesi{\_}Combined In-cylinder - CHT Analyses for the accurate estimation of the thermal flow field of a high performance engine for sport car applications.pdf:pdf},
month = {apr},
publisher = {SAE International},
title = {{Combined In-cylinder / CHT Analyses for the Accurate Estimation of the Thermal Flow Field of a High Performance Engine for Sport Car Applications}},
year = {2013}
}
@article{Brecq2005b,
abstract = {High frequency pressure oscillations are generated under knocking conditions within the combustion chamber of Spark Ignition engines. Although acoustic-oscillation model can give the natural frequencies of these oscillations, very few mathematical models are today available, in scientific literature, to describe the oscillation deadening effect. An analytical formulation of the deadening has been highlighted. Analytical solution has been established for future ECU implementation. Coupling this new concept and an existing high-frequency model, an achieved model of the knocking pressure high frequencies is compared to experimental data. Good behavior is obtained on a natural gas fuelled spark ignition engine.},
author = {Brecq, G. and {Le Corre}, O.},
doi = {10.4271/2005-01-1126},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Klopfen{\_}Ottomotor/2005{\_}Brecq{\_}Modeling of In-cylinder Pressure Oscillations under Knocking conditions - Intro to Pressure Envelope Curve.pdf:pdf},
isbn = {2005011126},
issn = {0148-7191},
title = {{Modeling of In-cylinder Pressure Oscillations under Knocking Conditions: Introduction to Pressure Envelope Curve}},
url = {http://papers.sae.org/2005-01-1126/},
year = {2005}
}
@article{Lauf-,
author = {Lauf-, Die and Fluid, Dem and Energie, Laufschaufeln},
title = {{5 Kreiselpumpen}}
}
@book{Riccardella1992d,
author = {Riccardella, P C and Deardorff, A F and Griesbach, T J},
booktitle = {Adv. Fatigue Lifetime Predict. Tech.},
doi = {10.1520/STP1122-EB},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Neuer Ordner/Advances in fatigue lifetime predictive techniques Part1.pdf:pdf},
isbn = {978-0-8031-1423-4},
issn = {00660558},
keywords = {FATIGUE,MONITORING,POWER PLANTS,PRESSURE VESSELS AND PIPING,THERMAL STRESSES},
pages = {460--473},
pmid = {11439068},
title = {{Advances in Fatigue Lifetime Predictive Techniques}},
url = {https://apps.webofknowledge.com/full{\%}7B{\_}{\%}7Drecord.do?product=UA{\%}7B{\&}{\%}7Dsearch{\%}7B{\_}{\%}7Dmode=GeneralSearch{\%}7B{\&}{\%}7Dqid=11{\%}7B{\&}{\%}7DSID=Z1UxbH6jtsqo8n9kPQr{\%}7B{\&}{\%}7Dpage=1{\%}7B{\&}{\%}7Ddoc=1},
volume = {1122},
year = {1992}
}
@article{Morris1979a,
author = {Morris, W L},
doi = {10.1007/BF02686400},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/1979{\_}Morris{\_}Microcrack closure phenomena for AL2219-T851.pdf:pdf},
issn = {03602133},
journal = {Met. Trans. A},
number = {1},
pages = {5--11},
title = {{Microcrack closure phenomena for AI 2219-T851}},
volume = {10},
year = {1979}
}
@article{McEvily1991,
abstract = {The behavior of short fatigue cracks cannot be analysed by linear elastic methods because of large scale plasticity effects as well as a breakdown in the stress intensity factor correlation of fatigue crack growth rates for crack sizes less than a millimeter in length. In the present paper a number of modifications are introduced to the linear elastic approach to establish a new parameter which is capable of correlating both long crack and short crack fatigue crack growth data. These modifications include the use of a material constant, re; an allowance for large scale plasticity effects; allowance for the development of crack closure; and the incorporation of the fatigue crack growth threshold. The new parameter is used with reasonable success in calculating fatigue crack growth behavior of short cracks in notched and unnotched specimens, and comparing with experimental data. In addition the analysis leads to a rationale for the dependence of the stress amplitude at the endurance level on the mean stress in a manner consistent with Gerber's parabolic relationship.},
author = {McEvily, A.J. and Eifler, D. and Macherauch, E.},
doi = {10.1016/0013-7944(91)90151-P},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/1991{\_}McEvily{\_}An analysis of the growth of short fatigue cracks.pdf:pdf},
issn = {00137944},
journal = {Eng. Fract. Mech.},
number = {3},
pages = {571--584},
title = {{An analysis of the growth of short fatigue cracks}},
url = {http://www.sciencedirect.com/science/article/pii/001379449190151P},
volume = {40},
year = {1991}
}
@article{Essmann1981,
abstract = {Based on recent experimental observations a realistic model of the evolution of the surface profile of persistent slip bands (PSBs) in fatigued metals is proposed. An essential feature of the model is the production of vacancies by the annihilation of edge dislocations which, combined with irreversible slip processes, leads to an elongation of the PSB parallel to the active slip vector. It is shown that a net extrusion forms rather rapidly. The growth processes and their dependence on temperature are discussed in detail. It is proposed that cracks initiate at the surface steps at the PSB{\&}ndash;matrix interface and, at a later stage, also at the notch-peak profile from the random slip processes.},
author = {Essmann, U. and G{\"{o}}sele, U. and Mughrabi, H.},
doi = {10.1080/01418618108239541},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2016{\_}Mughrabi{\_}A model of extrusions and intrusions in fatigued metals I  Point defect production and the growth of extrusions.pdf:pdf},
isbn = {0141-8610},
issn = {0141-8610},
journal = {Philos. Mag. A},
number = {2},
pages = {405--426},
title = {{A model of extrusions and intrusions in fatigued metals I. Point-defect production and the growth of extrusions}},
url = {http://www.tandfonline.com/doi/abs/10.1080/01418618108239541},
volume = {44},
year = {1981}
}
@article{Quation2003,
author = {Quation, F Inite Lement E},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Nicholson 2003 - Finite Element Analysis Thermomechanics of Solids/0749{\_}C13.pdf:pdf},
title = {{By the}},
volume = {2},
year = {2003}
}
@book{Heywood,
author = {Heywood, John B.},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/Motoren/Internal Combustion Engine Fundamentals - J Heywood (Mcraw-Hill, 1988) Ww+Kommentare.pdf:pdf},
isbn = {0-07-028637-X},
publisher = {Mcraw-Hill, Inc.},
title = {{Internal Combustion Engine Fundamentals}},
year = {1988}
}
@book{Cherkaoui2009g,
author = {Cherkaoui, Mohammed and Capolungo, Laurent},
doi = {10.1007/978-0-387-46771-9},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Atomistic and Continuum Modeling of Nanocrystalline Materials/Chapter 07.pdf:pdf},
isbn = {978-0-387-46765-8},
title = {{Atomistic and Continuum Modeling of Nanocrystalline Materials}},
url = {http://link.springer.com/10.1007/978-0-387-46771-9},
volume = {112},
year = {2009}
}
@article{Lubliner2006,
abstract = {This self-contained text for advanced undergraduate and graduate students is devoted to classical quasistatic problems of rate-independent plasticity theory. It discusses the finite element method for both viscoplastic and rate-independent plastic solids, in addition to large deformation plasticity numerical methods for rate-based formulations and hyperelastic methods.},
author = {Lubliner, Jacob},
doi = {10.1115/1.2899459},
isbn = {0023721618},
issn = {00218936},
journal = {J. Appl. Mech.},
number = {1},
pages = {540},
pmid = {15010233},
title = {{PLASTICITY Revised Edition ( PDF )}},
url = {http://www.getcited.org/pub/102800120},
volume = {59},
year = {2006}
}
@article{Gingrich2016,
abstract = {An experimental investigation was conducted to explore the impact in-cylinder pressure oscillations have on piston heat transfer. Two fast-response surface thermocouples embedded in the piston top measured transient temperature and a commercial wireless telemetry system was used to transmit thermocouple signals from the moving piston. Measurements were made in a light-duty single-cylinder research engine operated under low temperature combustion regimes including Homogeneous Charge Compression Ignition (HCCI) and Reactivity Controlled Compression Ignition (RCCI) and Conventional Diesel (CDC). The HCCI data showed a correlated trend of higher heat transfer with increased pressure oscillation strength, while the RCCI and CDC data did not. An extensive HCCI data set was acquired. The heat transfer rate - when corrected for differences in cylinder pressure and gas temperature - was found to positively correlate with increased pressure oscillations. It is important to normalize the data before drawing conclusions as the magnitude of the effect was diminished significantly by the normalization procedure.},
author = {Gingrich, Eric and Janecek, Daniel and Ghandhi, Jaal},
doi = {10.4271/2016-01-9044},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2016{\_}Gingrich{\_}Experimental Investigation of the Impact of In-Cylinder Pressure Oscillations on Piston Heat Transfer.pdf:pdf},
issn = {1946-3944},
journal = {SAE Int. J. Engines},
number = {3},
pages = {2016--9044},
title = {{Experimental Investigation of the Impact of In-Cylinder Pressure Oscillations on Piston Heat Transfer}},
url = {http://papers.sae.org/2016-01-9044/},
volume = {9},
year = {2016}
}
@article{Motor1892,
author = {Motor, Diesel Den and Pkw, Der},
pages = {27--52},
title = {{3 Beispiel Elektronische Dieselsteuerung ( EDC )}},
year = {1892}
}
@article{Findeisen,
author = {Findeisen, Dietmar},
isbn = {9783540238805},
journal = {New York},
title = {{Dietmar Findeisen}}
}
@article{Drucka,
author = {Druck, Der},
doi = {10.1007/978-3-8348-2230-7},
isbn = {9783834822307},
pages = {204--284},
title = {{Grundgleichungen der Str{\"{o}}mungsmechanik}}
}
@article{Helmholtz1969,
author = {Helmholtz, The},
title = {{Long and medium waves ∗}},
year = {1969}
}
@article{Metallplastizit2013d,
author = {Metallplastizit, Hrungdie and Helm, Dirk},
number = {November},
pages = {1--29},
title = {{Prozesssimulation in Der Umformtechnik}},
year = {2013}
}
@article{Bohlke2011,
author = {B{\"{o}}hlke, Thomas},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Vorlesungen/MMF{\_}Skript.pdf:pdf},
journal = {Mechanik},
keywords = {skript},
title = {{Skript zur Vorlesung Mathematische Methoden der Festigkeitslehre}},
year = {2011}
}
@article{Eichelberg1939,
author = {Eichelberg, G.},
journal = {Engineering},
pages = {463--466, 547--550},
title = {{Some investigations on old combustion-engine problems. Parts I and II.}},
volume = {148},
year = {1939}
}
@article{Hamilton2014,
abstract = {The continuous growth of the worldwide vehicle fleet is leading to many private initiatives and governmental policies for the achievement of lower pollutant and greenhouse gas emissions through energetic efficiency improvement. The in-cylinder heat transfer has been generally recognised as a major factor influencing internal combustion engines efficiency and exhaust emissions. Therefore, the analysis of in-cylinder heat transfer is of importance for fuel economy, as well as for environmental preservation. In the present paper, the use of particle filters applied on the time-dependent heat transfer coefficient estimation of a combustion process in a spark-ignition internal combustion engine is presented. The combustion process was modelled as a transient zero-dimensional process based on the First Law of Thermodynamics for a perfect gas, and the fuel burned fraction was modelled through a Wiebe's function model. Results with different measurement frequencies and errors are available, using a sample importance resampling filter, showing a very good estimate, even for initial guesses far away from the real value of the unknown function. {\textcopyright} 2013 Taylor {\&} Francis.},
author = {Hamilton, F.C.a and Cola{\c{c}}o, M.J.a and Carvalho, R.N.a B and Leiroz, A.J.K.a},
doi = {10.1080/17415977.2013.797411},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2013{\_}Hamilton{\_}Heat transfer coefficient estimation of an internal combustion engine using particle filters.pdf:pdf},
issn = {1741-5977},
journal = {Inverse Probl. Sci. Eng.},
keywords = {1741-5977,1741-5985,and engineering,com,combustion engine using particle,erse problems in science,filters,gipe20,heat transfer coefficient estimation,http,issn,journal homepage,loi,of an internal,online,print,tandfonline,www},
number = {3},
pages = {483--506},
title = {{Heat transfer coefficient estimation of an internal combustion engine using particle filters}},
url = {http://www.scopus.com/inward/record.url?eid=2-s2.0-84892543088{\&}partnerID=40{\&}md5=b4dec32ec5b338e03414a6e59567e78d},
volume = {22},
year = {2014}
}
@article{Finite2000,
author = {Finite, The and Method, Element and Mechanics, Continuum and Basis, The and Basis, Its},
title = {{It is thirty-eight years since the}},
year = {2000}
}
@article{Gleichgewicht,
author = {Gleichgewicht, Chemisches},
pages = {167--188},
title = {{Reaktionskinetik}},
volume = {1}
}
@article{Wei1974,
author = {Wei, K P},
pages = {19--32},
title = {{Study of in}},
volume = {6},
year = {1974}
}
@article{Sensorik,
author = {Sensorik, Die and Sensorik, Bauteile and Sensorik, Beschleunigungssensorik and Sensorik, Drucksensorik and Sensoren, Matrixdarstellung},
journal = {Glass},
title = {{5 Sensorik}}
}
@article{Alphabet,
author = {Alphabet, Tabelle Griechisches and Z, Realteil Von and Z, Imagin{\"{a}}rteil Von},
title = {{Tabellenanhang}}
}
@article{Papula2008,
author = {Papula, Lothar},
isbn = {3-658-11924-1},
journal = {Math. fur Ingenieure und Naturwissenschaftler},
number = {Teil 3},
title = {{Fehler- und Ausgleichsrechnug}},
volume = {1319},
year = {2008}
}
@article{Konstruktionc,
author = {Konstruktion, C Manuelle},
pages = {160--163},
title = {{23 Karosserie allgemein}}
}
@article{Donnet1998,
author = {Donnet, JB},
doi = {10.1361/asmhba0003354},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/{\_}buecherSong/HandbookofComposites/I/09{\_}CarbonFibers.pdf:pdf},
pages = {35--40},
title = {{Carbon fibers}},
url = {http://books.google.com/books?hl=en{\&}lr={\&}id=YkN8xIwL0dsC{\&}oi=fnd{\&}pg=PR7{\&}dq=Carbon+Fibers{\&}ots=TSZQ3MkZPG{\&}sig=PRk4Wzq5SDVhtEJ4e1z7FG8j2ek},
volume = {21},
year = {1998}
}
@article{McEvily1991a,
abstract = {The behavior of short fatigue cracks cannot be analysed by linear elastic methods because of large scale plasticity effects as well as a breakdown in the stress intensity factor correlation of fatigue crack growth rates for crack sizes less than a millimeter in length. In the present paper a number of modifications are introduced to the linear elastic approach to establish a new parameter which is capable of correlating both long crack and short crack fatigue crack growth data. These modifications include the use of a material constant, re; an allowance for large scale plasticity effects; allowance for the development of crack closure; and the incorporation of the fatigue crack growth threshold. The new parameter is used with reasonable success in calculating fatigue crack growth behavior of short cracks in notched and unnotched specimens, and comparing with experimental data. In addition the analysis leads to a rationale for the dependence of the stress amplitude at the endurance level on the mean stress in a manner consistent with Gerber's parabolic relationship.},
author = {McEvily, A J and Eifler, D and Macherauch, E},
doi = {10.1016/0013-7944(91)90151-P},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/1991{\_}McEvily{\_}An analysis of the growth of short fatigue cracks.pdf:pdf},
issn = {00137944},
journal = {Eng. Fract. Mech.},
number = {3},
pages = {571--584},
title = {{An analysis of the growth of short fatigue cracks}},
url = {http://www.sciencedirect.com/science/article/pii/001379449190151P},
volume = {40},
year = {1991}
}
@article{Models1992,
author = {Models, Mathematical},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Anisotropic Behaviouir of Damaged Materials{\_}Skrzypek{\_}ARTICEL/Kap1{\_}Applications of Tensor Functions in Damage Mechanics of Anisotropic Materials.pdf:pdf},
keywords = {anisotropy,canonical form,constitutive equations,continuum damage,creep,creep rupture,creep rupture time,damage tensor,evolutional equa-,irreducible invariants,material,material behaviour,mechanics,monkman-grant relationship,net-stress concept,tensor,tensor function,tensor generator,tensorial interpolation,ter-,tions},
number = {January},
pages = {47--59},
title = {{Applications of Tensor Functions in Continuum Damage Mechanics}},
year = {1992}
}

@article{Eslami2015a,
abstract = {An approach for prediction of high cycle fatigue (HCF) at a length scale of 5-100 ??m is established, which evaluates the accumulated plastic shear strain in slip bands of grains. Damage mechanisms initiated by dislocations and the grain microstructure are the key factors that influence the fatigue of metals in small dimensions. For this reason the HCF model considers the elasto-plastic behavior of metals at the grain level and microstructural parameters, specifically grain size and grain orientation. The HCF model can be applied either as a criterion for deterministic predictions of the failure in individual grains, or as a failure function in probabilistic studies on aggregates of grains, if the input parameters are given by specific distributions. This is addressed in a parameter study and a sensitivity analysis of the failure function with respect to different parameters. For model verification, the predicted results of the failure function are compared with the observed micro-damage in individual grains of nickel micro-samples. It is shown that the overall predictive power of the HCF model is fairly good. Nevertheless, some misclassifications occur as some grains are damaged, which were predicted to be safe. Those misclassifications are addressed in post-fatigue investigations on individual grains.},
author = {Eslami, R. and Riesch-Oppermann, H. and Kraft, O.},
doi = {10.1016/j.ijfatigue.2015.03.029},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2015{\_}Eslami+Kraft{\_}Prediction of multiaxial high cycle fatigue at small scales based on an micro-mecahnical model{\_}IAM{\_}KIT{\_}KRAFT.pdf:pdf},
issn = {01421123},
journal = {Int. J. Fatigue},
keywords = {Accumulated plastic shear strain,Micro electro mechanical systems (MEMS),Multiaxial high cycle fatigue (HCF),Probability methods,Surface damage},
pages = {66--74},
publisher = {Elsevier Ltd},
title = {{Prediction of multiaxial high cycle fatigue at small scales based on a micro-mechanical model}},
url = {http://dx.doi.org/10.1016/j.ijfatigue.2015.03.029},
volume = {83},
year = {2015}
}
@article{Aslan2011a,
abstract = {Proper life-time prediction modeling of single crystalline components is of increasing importance due to their common use in turbine industry. Viscoplastic damage approaches are of great interest in that context. However, mechanical properties of single crystals are strongly anisotropic and nonlinear in service conditions, bringing certain complexity into constitutive and numerical modeling. The aim of this work is to develop a thermodynamically consistent constitutive model based on generalized continua in order to simulate fatigue crack initiation and growth in single crystals. For that purpose, a standard crystal plasticity model is taken as a basis and coupled with the continuous damage model developed by Marchal et al. (2006a) [Marchal, N., Forest, S., Remy, L. and Duvinage, S. (2006a). Simulation of Fatigue Crack Growth in Single Crystal Superalloys Using Local Approach to Fracture, In: Moinereau, D., Steglich, D. and Besson, J. (eds.), Local Approach to Fracture, 9th European Mechanics of Materials Conference, Euromech–Mechamat, Moret–Sur–Loing, France, Presses de l'Ecole des mines de Paris, pp. 353–358]. As a variant of micromorphic theory, microdamage approach is applied to the model in order to obtain a regularized continuum damage formulation which solves mesh dependency problem by introducing an intrinsic length scale. A detailed finite element implementation procedure and its validation for monotonic crack growth areshown. Fatigue crack growth analyses have been performed on a single edge notched geometry and a comparison between numerical and experimental results is presented.},
author = {Aslan, Ozgur and Quilici, St{\'{e}}phane and Forest, Samuel},
doi = {10.1177/1056789510395738},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/2011{\_}Aslan{\_}Numerical Modeling of Fatigue Crack Growth in Single Crystals Based on micodamage theory.pdf:pdf},
issn = {1056-7895},
journal = {Int. J. Damage Mech.},
number = {5},
pages = {681--705},
title = {{Numerical Modeling of Fatigue Crack Growth in Single Crystals Based on Microdamage Theory}},
url = {http://journals.sagepub.com/doi/10.1177/1056789510395738},
volume = {20},
year = {2011}
}
@article{Svoboda2008,
abstract = {An extremal principle is formulated for thermodynamic systems near equi- librium subjected to various external conditions. It is shown that the principle describes un- ambiguously the kinetics of the thermodynamic system and replaces classical phenomeno- logical equations. Thus the principle can be considered as an effective tool for the treatment of non-equilibrium thermodynamic systems. In two examples the principle is used for the description of Dufour and Soret effects and plasticity. 1.},
author = {Svoboda, Jiř{\'{i}} and Fischer, Franz Dieter and Vala, Jiř{\'{i}}},
doi = {10.1478/C1S0801022},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Thermodynamik/2008{\_}Svoboda+Fischer{\_}Thermodynamic extremal principle and its application to Dufour and Soret effects and Plasticity.pdf:pdf},
issn = {03650359},
journal = {AAPP Atti della Accad. Peloritana dei Pericolanti, Cl. di Sci. Fis. Mat. e Nat.},
number = {SUPPL.1},
pages = {1--11},
title = {{Thermodynamic extremal principle and its application to dufour and soret effects and plasticity}},
volume = {86},
year = {2008}
}
@article{Bozza2011c,
abstract = {In the present paper a combined procedure for the quasi-dimensional modelling of heat transfer, combustion and knock phenomena in a "downsized" Spark Ignition two-cylinder turbocharged engine is presented. The procedure is extended to also include the effects consequent the Cyclic Variability. Heat transfer is modelled by means of a Finite Elements model. Combustion simulation is based on a fractal description of the flame front area. Cyclic Variability (CV) is characterized through the introduction of a random variation on a number of parameters controlling the rate of heat release (air/fuel ratio, initial flame kernel duration and radius, laminar flame speed, turbulence intensity). The intensity of the random variation is specified in order to realize a Coefficient Of Variation (COV) of the Indicated Mean Effective Pressure (IMEP) similar to the one measured during an experimental campaign. Moreover, the relative importance of the various concurring effects is established on the overall COV. A kinetic scheme is then solved within the unburned gas zone, characterized by different thermodynamic conditions occurring cycle-by-cycle. In this way, an optimal choice of the "knock-limited" spark advance is effected and compared with experimental data. Finally, the CV effects on the occurrence of individual knocking cycles are assessed and discussed. {\{}{\textcopyright}{\}} 2011 Global Science Press.},
author = {Bozza, Fabio and Siano, Daniela and Costa, Michela},
doi = {10.4208/aamm.10-10s2-04},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2011{\_}Bozza{\_}heat-transfer-knock-modeling-and-cyclic-variability-in-a-downsized-spark-ignition-turbocharged-engine.pdf:pdf},
issn = {20700733},
journal = {Adv. Appl. Math. Mech.},
keywords = {Cyclic variability,Finite elements in heat transfer,Internal combustion engines modelling,Knock},
number = {3},
pages = {310--326},
title = {{Heat transfer, knock modeling and cyclic variability in a "Downsized" spark-ignition turbocharged engine}},
volume = {3},
year = {2011}
}
@article{Banvillet2003a,
abstract = {A reliable design of industrial parts against high-cycle multiaxial fatigue requires a fatigue criterion capable of predicting both the stress gradient and the load-type effects. These effects are very important in the transfer of fatigue data from specimen to component. By using the concept of volume influencing fatigue crack initiation proposed by Palin-Luc and Lasserre with an energy based approach, a new criterion is presented. Based on the strain-work density given to the material, this proposal is usable whatever the constant amplitude loading is: in and out-of-phase combined loadings, with or without mean stress. Its predictions are compared both with a total of 38 experiments on four materials (a mild steel, two high strength steels and a spheroidal graphite cast iron) and with the predictions of local criteria (Crossland, Dang Van, Papadopoulos and Morel). The comparison shows that the predictions of the volumetric proposal are very good and less scattered than those of the local approaches, especially for loadings with mean stresses or under non-proportional loadings. ?? 2003 Elsevier Science Ltd. All rights reserved.},
author = {Banvillet, A and Palin-Luc, T and Lasserre, S},
doi = {10.1016/S0142-1123(03)00048-3},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Empirical Fatigue Models + Validation/Energy based models/A volumetric energy based high  cycle multiaxial fatigue criterion.pdf:pdf},
issn = {01421123},
journal = {Int. J. Fatigue},
keywords = {Criterion,Energy,Gradient,High cycle fatigue,Multiaxial,Volume},
number = {8},
pages = {755--769},
title = {{A volumetric energy based high cycle multiaxial fatigue citerion}},
volume = {25},
year = {2003}
}
@inproceedings{Gilaber1988,
abstract = {The computational fluid dynamics codes, which help to predict the behaviour of combusting gas in reciprocating engines, need, as boundary conditions for the momentum and energy equations, to approximate wall frictions and heat transfer between gas and walls. The purpose of this work is to outline the physical parameters which affect the heat transfer in spark ignited engines, and then to validate a multidimensional model which takes these parameters into account.In an experimental study, measurements were made on a test-engine instrumented with fast-response surface heat flux gages. Each gage was made of a steel cylinder, containing two thermocouples. A laser doppler velocimeter was used to analyze the influence of fluid dynamics on heat transfer. Up to ten data inputs could be simultaneously recorded at each crank — angle, including the heat flux at four locations of the combustion chamber, two velocity components and the cylinder pressure.A parametric analysis of the engine conditions including spark timing, volumetric efficiency, engine speed, equivalence ratio and swirl number was carried out. It revealed that: the gas density variation greatly affects the heat transfer when the spark timing or the load are changed. It also plays a role when the equivalence ratio is varied. turbulence intensity is the main parameter influencing the heat transfer during variations of the engine speed.In a computational study, a heat transfer model was introduced in a 3-dimensionai code. Because of prohibitive computing time, the boundary layer could not be meshed, so the model relies on a wall function. Coupled with a k-$\epsilon$ formulation of the turbulence, the response of this mode! to the density and turbulence was studied, analysing the influence of spark timing and engine speed. A comparison between measurements and computational predictions was done, showing as good agreement in terms of instantaneous and local heat-flux as in terms of global heat balance.},
author = {Gilaber, P and Pinchon, P},
booktitle = {SAE Int. Congr. Expo.},
doi = {https://doi.org/10.4271/880516},
month = {feb},
publisher = {SAE International},
title = {{Measurements and Multidimensional Modeling of Gas-Wall Heat Transfer in a S.I. Engine}},
year = {1988}
}
@article{Morgan1993,
abstract = {During prenatal and postnatal development of the mammalian brain, new neurons are generated by precursor cells that are located in the germinal zones. Subsequently newborn neurons migrate to their destined location in the brain. On the migrational route immature neurons interact via a series of recognition molecules with a plethora of extracellular cues. Stimuli that are conveyed by extracellular cues are translated into complex intracellular signaling networks that eventually enable neuronal migration. In this Focused Review we discuss signaling networks underlying neuronal migration emphasizing molecules and pathways that appear to be neuron-specific.},
author = {Morgan, Ken and Swansea, Wales},
journal = {Plant Soil},
number = {March},
pages = {39--47},
title = {{Plate 1 Analysis of subsonic flow around an aircraft ( Dassault Falkon )}},
url = {http://www.pubmedcentral.nih.gov/articlerender.fcgi?artid=3096852{\&}tool=pmcentrez{\&}rendertype=abstract},
volume = {250},
year = {1993}
}
@article{Schwingbeanspruchungb,
author = {Schwingbeanspruchung, Kennzeichnung Der},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Empirical Fatigue Models + Validation/Betriebsfestigkeit{\_}ErwinHaibach/Kap2 Experimentelle Grundlagen und Betriebsfestigkeit.pdf:pdf},
title = {{2 Experimentelle Grundlagen der Betriebsfestigkeit}}
}
@article{Wilson1951,
author = {Wilson, Brian A},
journal = {Processing},
title = {{A. Wilson 23}},
year = {1951}
}
@article{Evert2006,
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Evert, Ray F},
doi = {10.1002/0470047380.indauth},
eprint = {arXiv:1011.1669v3},
isbn = {9780470047385},
issn = {15672719},
journal = {Esau's Plant Anat.},
pages = {541--566},
pmid = {20348824},
title = {{Author Index}},
url = {http://dx.doi.org/10.1002/0470047380.indauth},
year = {2006}
}
@book{Tobergte2013,
abstract = {applicability for this approach.},
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Tobergte, David R and Curtis, Shirley},
booktitle = {J. Chem. Inf. Model.},
doi = {10.1017/CBO9781107415324.004},
eprint = {arXiv:1011.1669v3},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Thermodynamik/M{\"{u}}llerAndNoll{\_}Thermodynamik/M{\"{u}}ller 2007 Energy and Entropy.pdf:pdf},
isbn = {9788578110796},
issn = {1098-6596},
keywords = {icle},
number = {9},
pages = {1689--1699},
pmid = {25246403},
title = {{A History of Thermodynamics}},
volume = {53},
year = {2013}
}
@article{Leichtbau,
author = {Leichtbau, Gestaltungsprinzipien},
title = {{7 Gestaltungsprinzipien im Leichtbau}}
}
@article{Olmeda2015a,
abstract = {In the last years, a growing interest about increasing the engine efficiency has led to the development of new engine technologies. The accurate determination of the heat transfer across the combustion chamber walls is highly relevant to perform a valid thermal balance while evaluating the potential of new engine concepts. Several works dealing with heat transfer correlations that consider the swirl motion are found in the literature; however, there is a lack of works dealing with heat transfer correlations which take into account the effect of the tumble movement. In this work, a heat transfer model accounting for the tumble motion is presented. A two stroke HSDI Diesel engine with high tumble and no swirl is used to perform the theoretical study, the model development and its final calibration. Initially, a theoretical analysis of the gas movement phenomena is carried out based on CFD results and then, a model is developed and calibrated based on a skip-fire testing technique. Finally, a sensitivity study focused on evaluating the model robustness is performed. The results confirm an average RMSE reduction of 70{\%} with respect to the Woschni model, being this consistent improvement qualitatively evidenced in the instantaneous heat transfer evolution.},
author = {Olmeda, Pablo and Mart{\'{i}}n, Jaime and Novella, Ricardo and Carre{\~{n}}o, Ricardo},
doi = {10.1016/j.apenergy.2015.08.051},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Heat Transfer Combustion Chamber/2015{\_}Olmeda{\_}An adapted heat transfer model for engines with tumble motion.pdf:pdf},
issn = {03062619},
journal = {Appl. Energy},
keywords = {Combustion diagnosis,Engine heat transfer,Tumble},
pages = {190--202},
publisher = {Elsevier Ltd},
title = {{An adapted heat transfer model for engines with tumble motion}},
url = {http://dx.doi.org/10.1016/j.apenergy.2015.08.051},
volume = {158},
year = {2015}
}
@article{Grandin2002,
abstract = {SI Engine knock is caused by autoignition in the unburnt part of the mixture (end-gas) ahead of the propagating flame. Autoignition of the end-gas occurs when the temperature and pressure exceeds a critical limit when comparatively slow reactions-releasing moderate amounts of heat-transform into ignition and rapid heat release.In this paper the difference in the heat released in the end-gas-by low temperature chemistry-between lean, rich, stochiometric, and stoichiometric mixtures diluted with cooled EGR was examined by measuring the temperature in the end-gas with Dual Broadband Rotational CARS. The measured temperature history was compared with an isentropic temperature calculated from the cylinder pressure trace. The experimentally obtained values for knock onset were compared with results from a two-zone thermodynamic model including detailed chemistry modeling of the end-gas reactions.},
author = {Grandin, B{\"{o}}rje and Denbratt, Ingemar and Bood, Joakim and Brackmann, Christian and Bengtsson, Per-Erik and Gogan, Adina and Mauss, Fabian and Sund{\'{e}}n, Bengt},
doi = {10.4271/2002-01-0239},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2002{\_}Grandin{\_}Heat Release in the End-Gas Prior to Knock in lean-rich-stoichiometric mixtures.pdf:pdf},
journal = {SAE Tech. Pap.},
number = {724},
title = {{Heat Release in the End-Gas Prior to Knock in Lean, Rich and Stoichiometric Mixtures With and Without EGR}},
url = {http://dx.doi.org/10.4271/2002-01-0239},
volume = {2002-01-02},
year = {2002}
}
@article{Marzullo1998,
author = {Marzullo, A},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/{\_}buecherSong/HandbookofComposites/I/08{\_}BoronHighSilicaQuartzCeramicFibers.pdf:pdf},
isbn = {9780412540202},
journal = {Handb. Compos.},
pages = {156--168},
title = {{Boron, High Silica, Quartz and Ceramic Fibers}},
year = {1998}
}
@article{Papulad,
author = {Papula, Lothar},
pages = {470--540},
title = {{Integraltafel}}
}
@article{Konstruktiona,
author = {Konstruktion, C Manuelle},
pages = {184--188},
title = {{26 Hinterwagen}}
}
@article{Huang2004a,
abstract = {For a fine grained pure copper (grain size, 3.8 ??m) with a weak initial texture, the flow stress and the microstructure have been examined. The stress-strain curve has been compared with that of a coarse grained copper with a weak texture and a similar curve shape has been found, indicating no change in the strain hardening behavior as the grain size is decreased. The validity of the Hall-Petch relationship has been demonstrated down to a grain size of 3.8 ??m. Careful microstructural characterization of deformed specimens has shown that the microstructural evolution in the fine grained copper follows the same pattern previously established for larger grain sizes, which is characterized by the formation of three types of microstructures depending on the grain orientation. This observation suggests that the slip patterns in the fine grained and coarse grained copper are comparable, which underpin the observation of a comparable stress-strain behavior. ?? 2004 Elsevier B.V. All rights reserved.},
author = {Huang, Xiaoxu and Hansen, N.},
doi = {10.1016/j.msea.2004.02.081},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2005{\_}Huang{\_}Hansen Flow stress and microstructures of fine grained copper.pdf:pdf},
isbn = {0921-5093},
issn = {09215093},
journal = {Mater. Sci. Eng. A},
keywords = {Copper,Deformation microstructure,Flow stress,Grain orientation,Hall-Petch relationship,Slip pattern},
number = {1-2 SPEC. ISS.},
pages = {186--190},
title = {{Flow stress and microstructures of fine grained copper}},
volume = {387-389},
year = {2004}
}
@article{Hashin1962,
abstract = {IN PREVIOUS papers (HASHIN and SHTRIKMAN 1961a, b) the authors have established some new variational principles in the linear theory of elasticity for isotropic nonhomogeneous bodies with prescribed surface displacements. These have been applied to the theory of the elastic behaviour of multiphase materials. The present work is concerned with the generalization of these principles to anisotropic and nonhomogeneous e1asticity.j and the establishn-ent of similar variational principles for a body with prescribed surface tractions. An accompanying paper deals with the application of these variational principles to the theory of the elastic behaviour of polycrystals.},
author = {Hashin, Z and Shtrikman, S},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/Strukturmechanik MMS/Literatur/HS Schranken Methodik MMS Vorlesung Details/Hashin, Shtrikman - 1962.pdf:pdf},
number = {42},
title = {{Some Principles in and}},
volume = {10},
year = {1962}
}
@article{Loubar2005b,
abstract = {This paper deals with the transient thermal signal around an engine cylinder in order to propose a new and nonintrusive method of knock detection. Numerical simulations of unsteady heat transfer through the cylinder and inside the coolant flow are carried out to account for heat flux variations due to normal and knocking combustion. The effect of rib roughened surfaces on thermal signal amplification is investigated. The geometric parameters are fixed at Pi/h=70 and w/h=1 with a Reynolds number based on hydraulic diameter of 12,000. The results reveal that square ribs give better performance in term of thermal signal amplification within the fluid. An amplification of the temperature variation up to 20 times higher is found. Finally, flow analysis shows that amplification depends on the position where the thermal signal is collected.},
author = {Loubar, Khaled and Bellettre, Jérôme and Tazerout, Mohand},
doi = {10.1115/1.1857943},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Klopfen{\_}Ottomotor/2005{\_}Loubar{\_}Unsteady Heat Transfer enhancement around an engine cylinder in order to detect knockpdf.pdf:pdf},
isbn = {0022-1481},
issn = {00221481},
journal = {J. Heat Transfer},
number = {3},
pages = {278},
title = {{Unsteady Heat Transfer Enhancement Around an Engine Cylinder in Order to Detect Knock}},
url = {http://heattransfer.asmedigitalcollection.asme.org/article.aspx?articleid=1447711},
volume = {127},
year = {2005}
}
@article{Pebzy1998,
author = {Pebzy, Harry E},
journal = {Perspective},
keywords = {treated waste wood, disposal, reuse, recycle, inci},
title = {{Reuse and disposal}},
year = {1998}
}
@article{Tsurushima2002a,
author = {Tsurushima, Tadashi and Kunishima, Eiji and Asaumi, Yasuo and Aoyagi, Yuzo and Enomoto, Yoshiteru},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2002{\_}Tsurushima{\_}The Effect of Knock on Heat Loss in HCCI Engines-Modified Woschni.pdf:pdf},
journal = {Sae},
number = {108},
title = {{The Effect of Knock on Heat Loss in Homogeneous Charge Compression Ignition Engines}},
volume = {1},
year = {2002}
}
@article{Betrachtungeni,
author = {Betrachtungen, Allgemeine},
title = {{4 Grundlagen der Str¨ omungskinematik 4.1}}
}
@article{Buryachenko1995,
abstract = {We consider a linearly elastic composite medium, which consists of a homogeneous matrix containing a homogeneous and statistically uniform random set of ellipsoidal inclusions. Because of the differential thermal expansion, a microstructural residual stress state arises. By means of the "multiparticle effective field" method we first derive the functional relation between the stored elastic energy and the thermoelastic constants of the components. Using this result an exact estimation of all components of the statistical second moment tensor of the stress fields is given. Furthermore, an expression for the second moment of the stress in the matrix in the vicinity of the ellipsoidal inclusion and a correlation function of internal stresses is obtained. The application of the theory is demonstrated by some numerical results for a WC-Co composite. ?? 1995.},
author = {Buryachenko, Valeriy A. and Kreher, Wolfgang S.},
doi = {10.1016/0022-5096(95)00029-I},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Probabilistic Aspects/1995{\_}Kreher{\_}Internal residual stresses in heterogeneous solids - a statistical theory for particulate composites.pdf:pdf},
isbn = {0022-5096},
issn = {00225096},
journal = {J. Mech. Phys. Solids},
number = {7},
pages = {1105--1125},
title = {{Internal residual stresses in heterogeneous solids-A statistical theory for particulate composites}},
volume = {43},
year = {1995}
}
@article{Menter1994,
author = {Menter, F R},
doi = {https://doi.org/10.2514/3.12149},
journal = {AIAA J.},
number = {8},
pages = {1598--1605},
title = {{Two-Equation Eddy-Viscosity Turbulence Models for Engineering Applications}},
volume = {32},
year = {1994}
}
@article{Burgj,
author = {Burg, Heinz and Gratzer, Werner and Moser, Andreas and Steffan, Hermann},
journal = {Energy},
title = {{A9 A9 Kollisionsmechanik A9}}
}
@article{Chemie1806,
author = {Chemie, Organische},
title = {{1 Einf{\"{u}}hrung}},
year = {1806}
}
@article{Zahoransky2013a,
author = {Zahoransky, Richard a. and Allelein, Hans-Josef and Schelling, Udo and Schwarz, Harald and Bollin, Elmar and Oehler, Helmut},
doi = {10.1007/978-3-8348-2279-6},
isbn = {978-3-8348-1869-0},
journal = {Energietechnik - Syst. zur Energieumwandlung},
pages = {286--326},
title = {{12 Solartechnik}},
url = {http://www.springerlink.com/index/10.1007/978-3-8348-2279-6},
year = {2013}
}
@article{Problems2003,
author = {Problems, Contact},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Nicholson 2003 - Finite Element Analysis Thermomechanics of Solids/0749{\_}C15.pdf:pdf},
journal = {Springs},
pages = {195--200},
title = {{Introduction to Contact Problems 15.1}},
year = {2003}
}
@article{Morgan1993,
abstract = {During prenatal and postnatal development of the mammalian brain, new neurons are generated by precursor cells that are located in the germinal zones. Subsequently newborn neurons migrate to their destined location in the brain. On the migrational route immature neurons interact via a series of recognition molecules with a plethora of extracellular cues. Stimuli that are conveyed by extracellular cues are translated into complex intracellular signaling networks that eventually enable neuronal migration. In this Focused Review we discuss signaling networks underlying neuronal migration emphasizing molecules and pathways that appear to be neuron-specific.},
author = {Morgan, Ken and Swansea, Wales},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Zienkiewicz FEM - Vol 3 Fluid Dynamics/63229{\_}clrplate.pdf:pdf},
journal = {Plant Soil},
number = {March},
pages = {39--47},
title = {{Plate 1 Analysis of subsonic flow around an aircraft ( Dassault Falkon )}},
url = {http://www.pubmedcentral.nih.gov/articlerender.fcgi?artid=3096852{\&}tool=pmcentrez{\&}rendertype=abstract},
volume = {250},
year = {1993}
}
@article{Cherkaoui2009g,
author = {Cherkaoui, Mohammed and Capolungo, Laurent},
doi = {10.1007/978-0-387-46771-9},
isbn = {978-0-387-46765-8},
title = {{Atomistic and Continuum Modeling of Nanocrystalline Materials}},
url = {http://link.springer.com/10.1007/978-0-387-46771-9},
volume = {112},
year = {2009}
}
@article{Popping2012,
author = {P{\"{o}}pping, K},
isbn = {9783844021653},
issn = {1861-0595},
journal = {D-Nb.Info},
title = {{Diese Dissertation ist auf den Internetseiten der Hochschulbibliothek online verf{\{}{\"{u}}{\}}gbar.}},
url = {http://d-nb.info/985390468/34},
year = {2012}
}
@article{Voraussetzungen1936,
author = {Voraussetzungen, Die and Rail-einspritztechnologie, Common},
title = {{Fahrzeugdieselmotoren}},
year = {1936}
}
@article{Modellbildung,
author = {Modellbildung, Methodik Der},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Vorlesungen/Messtechnik+Regelungstechnik/gmrt03.pdf:pdf},
pages = {1--31},
title = {{3.1 Methodik der Modellbildung}}
}
@article{Caton1981,
abstract = {Because of the increasing need for precise information on engine processes, this study developed and experimentally verified models for the instantaneous heat transfer in an engine exhaust port. Experimental measurements were made of the instantaneous cylinder pressure and instantaneous exhaust gas temperature for a range of engine operating conditions. The pressure measurements were used to obtain the instantaneous cylinder gas state and the temperature measurements were used to validate the heat transfer models. The exhaust port heat transfer was dominated by jet induced large-scale fluid motion as opposed to wallshear generated fluid motion. An analysis based on the jet velocity through the valve opening correctly estimated the heat transfer due to this large-scale motion. Models for the instantaneous exhaust port heat transfer provided excellent agreement with measurements as a function of engine operating conditions. A cause d'un besoin croissant d'information pr{\'{e}}cise sur le fonctionnement d'un moteur, on d{\'{e}}veloppe une {\'{e}}tude et on v{\'{e}}rifie exp{\'{e}}rimentalement des mod{\`{e}}les sur le transfert de chaleur instantan{\'{e}} {\`{a}} l'{\'{e}}chappement d'un cylindre. Des mesures de la pression instantan{\'{e}}e dans le cylindre et de la temp{\'{e}}rature instantan{\'{e}}e {\`{a}} l'{\'{e}}chappement sont effectu{\'{e}}es pour un domaine de conditions de fonctionnement d'un moteur. Les mesures de pression permettent d'atteindre l'{\'{e}}tat instantan{\'{e}} du gaz dans le cylindre et les mesures de temp{\'{e}}rature permettent de valider les mod{\`{e}}les de transfert thermique. Le transfert {\`{a}} l'{\'{e}}chappement est domin{\'{e}} par un mouvement de jet {\`{a}} large {\'{e}}chelle au contraire du mouvement de fluide {\`{a}} frottement pari{\'{e}}tal. Une analyse bas{\'{e}}e sur la vitesse du jet {\`{a}} travers l'ouverture de la soupape pr{\'{e}}dit correctement le transfert de chaleur d{\^{u}} {\`{a}} ce mouvement {\`{a}} grande {\'{e}}chelle. Des mod{\`{e}}les pour l'{\'{e}}chappement instantan{\'{e}} fournissent un accord excellent avec des mesures pour les conditions de fonctionnement du moteur. Wegen des zunehmenden Bedarfs an genauer Information {\"{u}}ber Verbrennungsmotoren-Prozesse wurden in dieser Studie Modelle f{\"{u}}r den momentanen W{\"{a}}rme{\"{u}}bergang in einer Motor-Ausla$\beta$-{\"{O}}ffnung entwickelt und experimentell best{\"{a}}tigt. Die Momentanwerte des Zylinderdrucks und der Abgastemperatur wurden in Versuchen f{\"{u}}r einen ausgedehnten Betriebsbereich gemessen. Druckmessungen wurden verwendet, um den momentanen Gaszustand im Zylinder zu bestimmenn und Temperaturmessungen dienten zur Best{\"{a}}tigung der W{\"{a}}rme{\"{u}}bergangs-Modelle. Der W{\"{a}}rme{\"{u}}bergang in der Ausla$\beta$-{\"{O}}ffnung wurde im wesentlichen durch die strahlinduzierte Makro-Bewegung des Fluides entgegen der durch Wandschubspannung erzeugten Fluidbewegung bestimmt. Eine theoretische Untersuchung, die sich auf die Strahlgeschwindigkeit durch die Ventil{\"{o}}ffnung st{\"{u}}tzt, liefert korrekt den W{\"{a}}rme{\"{u}}bergang, hervorgerufen durch diese Makro-Bewegung. Die Modelle f{\"{u}}r den momentanen W{\"{a}}rme{\"{u}}bergang in der Ausla$\beta$-{\"{O}}ffnung als Funktion der Arbeitsbedingungen des Motors zeigten vorz{\"{u}}gliche {\"{U}}bereinstimmung mit den Messungen. B cвязи c вce бoлee вoзpacтaющeй нeoбчoдимocтью в тoчнoй инфopмaции o пpoцeccaч, пpoиcчoдящич в двигaтeляч, пpeдлoзeны мoдeди тeплoпepeнoca в вычлoпнoм oтвepcтии двигaтeля. Измepялиcь дaвлeниe в цилиндpe и тeмпepaтypa вычлoпнoгo гaзa пpи paздичныч peзимaч paбoты двигaтeля. Дaнныe пo дaвлeнию иcпoльзoвaлиcь для oпpeдeлeния cocтoяния гaзa в цилиндpe, a пo тeмпepaтype — для пpoвepки cпpaвeдливocти пpeдлoзeнныч мoдeлeй. Teплoпepeнoc в вычлoпнoм oтвepcтии oпpeдeляeтcя кpyпнoмacштaбными пepeмeщeниями зидкocти, вoзникaющими пpи cтpyйнoм иcтeчeнии, кoтopыe cyщecтвeннo oтличaютcя oт пepeмeщeний, вызывaeмыч нaпpязeниeм cдвигa нa cтeнкe. Aнaлиз, ocнoвaный нa cкopocти иcтeчeния cтpyи чepeз oтвepcтиe клaпaнa, пoзвoляeт кoppeктнo oцeнить вeличинy тeплoвoгo пoтoкa пpи тaкич кpyпнoмacщтaбпыч пepeмeщeнияч. Moдeли тeплoпepeнoca в вычлoпнoм oтвepcтии чopoшo coглacyютcя c peзyльтaтaми измepeний пpи paзличныч peзимaч paбoты двигaтeдя.},
author = {Caton, J.A. and Heywood, J.B.},
doi = {https://doi.org/10.1016/0017-9310(81)90003-X},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/1981{\_}An experimental and analytical study of heat transfer in an engine exhaust port{\_}Caton.pdf:pdf},
journal = {Int. J. Heat Mass Transf.},
number = {4},
pages = {581--595},
title = {{An experimental and analytical study of heat transfer in an engine exhaust port}},
volume = {24},
year = {1981}
}
@article{Colburn1964,
author = {Colburn, A. P.},
doi = {http://dx.doi.org/10.1016/0017-9310(64)90125-5},
journal = {Int. J. Heat Mass Transf.},
number = {12},
pages = {1359--1384},
title = {{A method of correlating forced convection heat transfer data and a comparison with fluid friction}},
volume = {7},
year = {1964}
}
@article{Sharief2008,
abstract = {Heat transfer in reciprocating combustion engine is an intricate phenomenon involving rapid cyclic variation of cylinder pressure temperature density and area of contacting surfaces. Rate of heat transfer in internal combustion engine is further complicated greatly due to the gas turbulence and flame radiation effects, the magnitudes of which depend on the engine type and operating conditions. It is necessary to calculate the heat flow, the temperature distribution and the temperature stresses. Hence, an accurate model for estimation of heat transfer in various phases of the cycle is an important factor which influences the accuracy of all parameters in the cycle analysis. Nearly more than twenty correlations have been proposed to find the heat transfer coefficient in the combustion chamber wall among which some of theoretical concepts. The large disagreement among the various proposed formulae for reciprocating engine heat transfer made it hard to choose any adequate e formula for universal application to various combustion engines. This paper proposes a modified heat transfer correlation based on experiments conducted in motored diesel engine with natural aspiration of hot air at around 150°C-300°C. The author considered the Intake jet velocity in place of mean piston speed in Reynold parameter in proposed heat transfer coefficient equation. The Intake jet velocity is better representative of gas velocity than the mean piston speed since it takes into account the diameter of inlet port of an engine and diameter of piston. Further, the proposed heat transfer correlation for Compression Ignition engine is validated by conducting experiments on a direct injection, four-stroke, single-cylinder, water-cooled diesel engine under fired conditions at different loads and different speeds. The formulated new heat transfer correlation is finally compared with other earlier correlations proposed by other researchers.ER -},
author = {Sharief, Abdul and Chandrashekar, T K and Antony.A.J and Samaga, B S},
doi = {10.4271/2008-01-1816},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2008.{\_}Sharief{\_}Study on Heat Transfer Correlation in IC Enginespdf.pdf:pdf},
journal = {SAE Pap.},
number = {724},
title = {{Study on Heat Transfer Correlation in IC Engines}},
volume = {2008-01-18},
year = {2008}
}
@book{Borbely2006a,
abstract = {Loss of cortical gray matter is accompanied by a commensurate increase in the sulcal and intraventricular cerebrospinal fluid volume. On diffusion-weighted magnetic resonance imaging, this would be reflected as a higher apparent diffusion coefficient in affected brain regions. On the basis of the above premise, we suggest that the apparent diffusion coefficient may be used as a surrogate marker for the assessment of regional brain volume deficits. We demonstrate this approach by voxelwise analysis of registered apparent diffusion coefficient images from a group of 15 patients with schizophrenia and 15 age-matched healthy controls. We found widespread regional apparent diffusion coefficient increases in patients. Affected areas included the bilateral insular cortex, hippocampus, temporal lobe, and occipital areas. These results largely concur with previous findings of cortical volume deficits in schizophrenia.},
author = {Borbely, Anne-marie and Kreider, Jan F and Bejan, Adrian and Cundiff, John S and Davis, Lorin R},
booktitle = {Mech. Compos. Mater.},
doi = {10.1021/ja00116a001},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Plasticity models/Elastoplasticity Theory{\_}Lubarda{\_}2002.pdf:pdf},
isbn = {9780849391392},
issn = {9780849391378},
pages = {1455--1459},
title = {{Distributed Generation : The Power Paradigm for the New Millennium Fluid Power Circuits and Controls : Fundamentals and Applications}},
url = {http://www.ncbi.nlm.nih.gov/pubmed/16110271},
volume = {23},
year = {2006}
}
@article{Verbundwerkstoff,
author = {Verbundwerkstoff, Ein and Verbundwerkstoff, Der and Problem, Das},
pages = {79--101},
title = {{2 Polymere Verbundwerkstoffe}}
}
@inproceedings{Grill2006_QuasiDim,
abstract = {A quasidimensional combustion model for homogenous spark ignition combustion processes with variable valve timing is proposed which is able to compute a complete engine map in advance and can be calibrated rapidly. In the engine map there are not only load and speed that do change considerably, the residual gas mass does so as well. This paper exposes the models' potential and limits by both simulation and measurement on two different engines with port-injection. Methods for model adjustment as well as the implementation in the commercial one-dimensional flow simulation software “GT-Power” will be shown. Furthermore a knock control is introduced and resulting errors are discussed.},
author = {Grill, M and Billinger, T and Bargende, M},
booktitle = {SAE 2006 World Congr. Exhib.},
doi = {https://doi.org/10.4271/2006-01-1107},
month = {apr},
publisher = {SAE International},
title = {{Quasi-Dimensional Modeling of Spark Ignition Engine Combustion with Variable Valve Train}},
year = {2006}
}
@article{Broekaert2016,
abstract = {The heat transfer from the combustion gases to the cylinder walls inside a spark ignition engine is a key factor in an engine's design, due to its influence on the engine's efficiency, power and emissions. Therefore a lot of research has been conducted in order to accurately model the heat transfer, for engine design and optimization purposes. These models have been found to provide inaccurate predictions for fuels which have significantly different gas properties compared to traditional fossil fuels. This indicates that the models either do not properly include gas properties, or are missing some important properties in their formulation. In order to construct a general (“fuel-independent”) heat transfer model, new measurements need to be executed, with multiple fuels that have different properties. Designing such an experiment requires a thorough understanding of the factors influencing the heat transfer and their interactions. In this paper a literature review is presented of heat transfer measurements in spark ignition engines in order to investigate the effect of the engine factors on the heat transfer. Based on this review, a root cause analysis is conducted to identify the independent factors that affect heat transfer. These factors are then used to set up two experiments according to a Design of Experiments methodology that allows the investigation of the effect of different gas properties and engine settings on the heat transfer in a consistent way. The results of these measurements for motored operation are discussed in [1] and for fired operation in a companion paper [2].},
author = {Broekaert, Stijn and Demuynck, Joachim and {De Cuyper}, Thomas and {De Paepe}, Michel and Verhelst, Sebastian},
doi = {10.1016/j.energy.2016.08.065},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Heat Transfer Combustion Chamber/2016{\_}Broekaert{\_}Heat transfer in premixed spark ignition engines part I - Identification of the factors inflencing heat transfer.pdf:pdf},
issn = {03605442},
journal = {Energy},
keywords = {Experimental,Heat transfer,Internal combustion engine,Review},
pages = {380--391},
publisher = {Elsevier Ltd},
title = {{Heat transfer in premixed spark ignition engines part I: Identification of the factors influencing heat transfer}},
volume = {116},
year = {2016}
}
@article{Technologien2004,
author = {Technologien, Seminar Neue and Wintersemester, W W W and Langguth, Christoph},
journal = {Publish},
title = {{RSS - Nachrichtendienste f u ¨ r Jedermann}},
year = {2004}
}
@article{Schabacker2011a,
author = {Schabacker, M},
doi = {10.1007/978-3-8348-8161-8},
isbn = {9783834881618},
pages = {39--60},
title = {{4 Geometriemodellierung}},
year = {2011}
}
@article{To2013,
author = {To, Nswers},
doi = {10.1007/978-3-642-22346-4},
isbn = {9783642223464},
pages = {1--6},
title = {{Kapitel 8}},
year = {2013}
}
@phdthesis{Oehrby2014,
author = {Oehrby, Frederik},
school = {Chalmers University of Technology},
title = {{Numerical modeling of subcooled nucleate flow boiling in engine cooling systems}},
year = {2014}
}
@article{Papulac,
author = {Papula, L},
doi = {10.1007/978-3-8348-8643-9},
isbn = {3834805645},
journal = {Math. f{\"{u}}r Ingenieure und Naturwissenschaftler Band 2},
title = {{VI Laplace-Transformationen 1}}
}
@article{Fea2003,
author = {Fea, Nonlinear},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Nicholson 2003 - Finite Element Analysis Thermomechanics of Solids/0749{\_}C16.pdf:pdf},
pages = {201--213},
title = {{Introduction to Nonlinear FEA 16.1}},
year = {2003}
}
@article{Wei1974a,
author = {Wei, K P},
pages = {19--32},
title = {{Study of in}},
volume = {6},
year = {1974}
}
@article{Grandin2002b,
abstract = {SI Engine knock is caused by autoignition in the unburnt part of the mixture (end-gas) ahead of the propagating flame. Autoignition of the end-gas occurs when the temperature and pressure exceeds a critical limit when comparatively slow reactions-releasing moderate amounts of heat-transform into ignition and rapid heat release.In this paper the difference in the heat released in the end-gas-by low temperature chemistry-between lean, rich, stochiometric, and stoichiometric mixtures diluted with cooled EGR was examined by measuring the temperature in the end-gas with Dual Broadband Rotational CARS. The measured temperature history was compared with an isentropic temperature calculated from the cylinder pressure trace. The experimentally obtained values for knock onset were compared with results from a two-zone thermodynamic model including detailed chemistry modeling of the end-gas reactions.},
author = {Grandin, B{\"{o}}rje and Denbratt, Ingemar and Bood, Joakim and Brackmann, Christian and Bengtsson, Per-Erik and Gogan, Adina and Mauss, Fabian and Sund{\'{e}}n, Bengt},
doi = {10.4271/2002-01-0239},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2002{\_}Grandin{\_}Heat Release in the End-Gas Prior to Knock in lean-rich-stoichiometric mixtures.pdf:pdf},
journal = {SAE Tech. Pap.},
number = {724},
title = {{Heat Release in the End-Gas Prior to Knock in Lean, Rich and Stoichiometric Mixtures With and Without EGR}},
url = {http://dx.doi.org/10.4271/2002-01-0239},
volume = {2002-01-02},
year = {2002}
}
@misc{Mura1982,
author = {Mura, Toshio},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/Strukturmechanik MMS/Literatur/Mikromechanik{\_}B{\"{u}}cher{\_}Literaturvorschlag{\_}MMS/Mura 1987 Micromechanics of defects in solids.pdf:pdf},
title = {{Mechanics of elastic and inelastic solids}},
year = {1982}
}
@article{Meneghetti2016,
abstract = {Fatigue crack initiation and propagation involve plastic strains that require some work to be done on the material. Most part of this irreversible energy is dissipated as heat and consequently the material temperature increases. The heat being an indicator of the intense plastic strains occurring at the tip of a propagating fatigue crack, the hypothesis is formed that it can be used to assess the fatigue damage accumulation rate of cracked components. Moreover, the heat energy at the crack tip is averaged according to Neuber's finite particle concept. The aim of the present paper is to present the theoretical framework and the corresponding experimental technique to evaluate the heat energy dissipated in a structural volume surrounding the crack tip. The shape and size of the structural volume have been assumed according to the literature, even though the definition of the structural volume size of the analysed material in a fatigue sense is not the scope of the present paper. The proposed experimental technique to evaluate the averaged heat energy is based on the radial temperature profiles measured around the crack tip by means of an infrared camera. The temperature fields measured within few millimetres from the crack tip have been compared successfully with existing analytical solutions.},
author = {Meneghetti, G and Ricotta, M},
doi = {10.1016/j.ijfatigue.2016.04.001},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2016{\_}Meneghetti{\_}Evaluating the heat energy dissipated in a small volume surrounding the tip of a fatigue crack.pdf:pdf},
issn = {01421123},
journal = {Int. J. Fatigue},
keywords = {AISI 304L,Averaging approaches,Crack propagation,Crack tip,Critical distance mechanics,Energy approaches,Fatigue assessment},
pages = {605--615},
publisher = {Elsevier Ltd},
title = {{Evaluating the heat energy dissipated in a small volume surrounding the tip of a fatigue crack}},
url = {http://dx.doi.org/10.1016/j.ijfatigue.2016.04.001},
volume = {92},
year = {2016}
}
@article{Xiaoming2004,
author = {Xiaoming, Ye and Guohua, Chen and Yankun, Jiang and Yunchuan, Zou},
doi = {10.4271/2004-01-0778},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2004{\_}Xiaoming{\_}Numerical Investigation of the EHL performance and friction heat transfer in pistopn and cylinder liner system.pdf:pdf},
isbn = {0768013194},
number = {724},
title = {{Numerical Investigation of the EHL Performance and Friction Heat Transfer in Piston and Cylinder Liner System}},
year = {2004}
}
@article{Schneider2016b,
abstract = {{\textcopyright} 2016 Elsevier B.V.Modeling of crack propagation in materials has long been a challenge in solid-state physics and materials science. The phase-field method has now established as one of the tools for the description of crack propagation. The applied models are thermodynamically consistent and predict crack propagation in homogeneous materials under the consideration of different loading types, multiple physical fields and geometrical nonlinearities. Even dynamic loading processes are studied, including plastic effects. A multiphase-field model for crack propagation, which is indispensable to describe crack propagation on a mesoscopic length scale, is still missing. In this work, we overcome this deficiency and combine a crack propagation approach, which is based on Griffith's theory, with an established multiphase-field model for phase transformation.},
author = {Schneider, D. and Schoof, E. and Huang, Y. and Selzer, M. and Nestler, B.},
doi = {10.1016/j.cma.2016.04.009},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Thermodynamik/PhasenFeld/Schneider{\_}Crack{\_}propagation{\_}multiphase{\_}systems-Feb2016.pdf:pdf},
issn = {00457825},
journal = {Comput. Methods Appl. Mech. Eng.},
keywords = {crack propagation,multiphase-field,phase-field,polycrystalline material},
title = {{Phase-field modeling of crack propagation in multiphase systems}},
url = {http://dx.doi.org/10.1016/j.cma.2016.04.009},
year = {2016}
}
@inproceedings{LiuJiang2000,
abstract = {A simplified turbulence model for predicating the in-cylinder turbulence parameters during combustion in a spark-ignition engine is investigated in this study. It is based on the standard k - $\epsilon$ model with the assumptions that no influence of squish and swirl is considered and that turbulence is in equilibrium. Hence it has a simplified form that meets the requirements for a two-zone quasi-dimensional combustion model.The proposed sub-model is implemented in a quasi-dimensional entrainment combustion model for spark-ignition engines. With this combustion model as the core system, a complete thermodynamics simulation system for a turbo-charged spark-ignition engine is programmed to simulate the working process and engine performance characteristics. After calibration against experimental date taken from a 4-cylinder turbocharged spark-ignition engine, some adjustable constants for the proposed turbulence model are fixed, and successful validation is thus made under variable engine operating conditions. The results show that the proposed turbulence model could present correct predication results for the turbulence parameters during combustion, and hence make this thermodynamics model more reasonable in calculating engine performance and working process.Finally, parametric studies are performed to analyze the sensitivity of the adjustable constants used in the proposed model to provide guidance for future study.},
author = {LIU, Chuanli and JIANG, Deming and OBOKATA, Tomio},
booktitle = {Int. Fuels Lubr. Meet. Expo.},
doi = {https://doi.org/10.4271/2000-01-2803},
publisher = {SAE International},
title = {{A Simplified Turbulence Model for In-cylinder Gas Flow in Quasi-dimensional Turbulence Combustion Model for Spark-ignition Engines}},
year = {2000}
}
@article{Problembereiche,
author = {Problembereiche, Beide and Ziele, Beide},
title = {{Abw{\"{a}}rmeverwertung}}
}
@article{Hochrainer2009a,
abstract = {Crystal plasticity is the result of the motion and interaction of dislocations. There is, however, still a major gap between microscopic and mesoscopic simulations and continuum crystal plasticity models. Only recently a higher dimensional dislocation density tensor was defined which overcomes some drawbacks of earlier dislocation density measures. The evolution equation for this tensor can be considered as a continuum version of dislocation dynamics. We use this evolution equation to develop evolution equations for the total dislocation density and an average curvature which together govern a faithful representation of the dislocation kinematics without having to use extra dimensions.},
archivePrefix = {arXiv},
arxivId = {1010.2884},
author = {Hochrainer, T and Zaiser, M and Gumbsch, P},
doi = {10.1063/1.3241258},
eprint = {1010.2884},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2010{\_}Hochrainer{\_}Dislocation transport and line length increase in averageddescription of dislocations.pdf:pdf},
isbn = {9780735407091},
issn = {0094243X},
journal = {AIP Conf. Proc.},
keywords = {Continuum tlieory of dislocations,Dislocations dynamics},
pages = {1133--1136},
title = {{Dislocation transport and line length increase in averaged descriptions of dislocations}},
volume = {1168},
year = {2009}
}
@article{Pkw-pkw-unfalle2005,
author = {Pkw-pkw-unf{\"{a}}lle, A and Br{\"{o}}sdorf, Klaus-dieter and Burg, Heinz and Moser, Andreas and Hauptumfang, Den Pkw-pkw-unf{\"{a}}llen Der},
journal = {Sierra},
pages = {411--437},
title = {{A12 Zum Stra{\{}{\ss}{\}}enverkehr in Deutschland und in Europa A12}},
year = {2005}
}
@article{Deutscher,
author = {Deutscher, Allgemeiner and Club, Automobil and Scale, Abbreviated Injury and Device, Anthropomorphic Test and Servey, Co-operative Crash Injury and Scale, Collision Deformation and Committee, European Enhanced Vehicle-safety and Transport, European and Council, Safety and Motor, Federal and Safety, Vehicle and Versicherungswirtschaft, Gesamtverband Der Deutschen and Criteria, Head Injury and Criteria, Head Performance and Assessment, Injury and Value, Reference and Criteria, Injury and Level, Protection and Harmonized, International and Score, Injury Severity and Barrier, Mobile Deformable},
pages = {967--969},
title = {{D2 D2 Begriffe und Abk{\{}{\"{u}}{\}}rzungen D2 Firmen und Institutionen}}
}
@article{Interaction2012,
author = {Interaction, Creep-fatigue},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Kriechen{\_}Spannungsrelaxation/2012{\_}Weaver{\_}Creep-Fatigue Interaction - An overview.pdf:pdf},
pages = {1--13},
title = {{Module {\#} 40 Creep- Creep- Let ' s review our basic fracture mechanisms before}},
year = {2012}
}
@article{Bohlke2012a,
author = {B{\"{o}}hlke, Prof Thomas},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Vorlesungen/HTF{\_}Skript.pdf:pdf},
journal = {Mechanik},
number = {September},
title = {{Skript zur Vorlesung H{\"{o}}here Technische Festigkeitslehre}},
year = {2012}
}
@article{Ausf,
author = {Ausf, Die and Bewertung, Die and Reihenfolge, Die and Schaltkomfort, Der and Abschnitt, Mit},
title = {{Komfortaspekte}}
}
@article{Differt1986,
abstract = {A mdoel of the evolution of the surface roughness of persistent slip bands (PSBs) is presented. The physical background of the model is the existence of a dynamic equilibrium between dislocation multiplication and annihilation in PSBs which leads to irreversible microscopic positive and negative slip steps at the surface. The fluctuation of a random distribution of these slip line segments leads to a surface roughness which increases with the square root of the cycle number. The relation between the parameters which characterize the surface relief and the microscopic parameters which contol the dislocation glide in PSBs is investigated by computer simulations. Fair agreement is obtained between observed and simulated surface reliefs where such a comparison is possible.},
author = {Differt, K. and Esmann, U. and Mughrabi, H.},
doi = {10.1080/01418618608242897},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2016{\_}Mughrabi{\_}A model of extrusions and intrusions in fatigued metals II  Surface roughening by random irreversible slip.pdf:pdf},
isbn = {0141-8610},
issn = {0141-8610},
journal = {Philos. Mag. A},
number = {2},
pages = {237--258},
title = {{A model of extrusions and intrusions in fatigued metals II. Surface roughening by random irreversible slip}},
url = {http://www.tandfonline.com/doi/abs/10.1080/01418618608242897},
volume = {54},
year = {1986}
}
@article{Of2003,
author = {Of, Torsion and Bars, Prismatic},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Nicholson 2003 - Finite Element Analysis Thermomechanics of Solids/0749{\_}C14.pdf:pdf},
pages = {181--194},
title = {{Torsion and Buckling 14.1}},
year = {2003}
}
@misc{Holzapfel2000,
abstract = {Nonlinear Solid Mechanics a Continuum Approach for Engineering Gerhard A. Holzapfel Graz University of Technology, Austria With a modern, comprehensive approach directed towards computational mechanics, this book covers a unique combination of subjects at present unavailable in any other text. It includes vital information on 'variational principles' constituting the cornerstone of the finite element method. In fact this is the only method by which Nonlinear Solid Mechanics is utilized in engineering practice. The book opens with a fundamental chapter on vectors and tensors. The following chapters are based on nonlinear continuum mechanics - an inevitable prerequisite for computational mechanicians. In addition, continuum field theory (applied to a representative sample of hyperelastic materials currently used in nonlinear computations such as incompressible and compressible materials) is presented, as are transversely isotropic materials, composite materials, viscoelastic materials and hyperelastic materials with isotropic damage. Another central chapter is devoted to the thermodynamics of materials, covering both finite thermoelasticity and finite thermoviscoelasticity. Also included are: an up-to-date list of almost 300 references and a comprehensive index useful examples and exercises for the student selected topics of statistical and continuum thermodynamics. Furthermore, the principle of virtual work (in both the material and spatial descriptions) is compared with two and three-field variational principles particularly designed to capture kinematic constraints such as incompressibility. All of the features combined result in an essential text for final year undergraduates, postgraduates and researchers in mechanical, civil and aerospace engineering and applied maths and physics.},
author = {Holzapfel, G},
booktitle = {Work},
doi = {10.1023/A:1020843529530},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/nonlinear{\_}solid{\_}mechanics{\_}holzapfel.pdf:pdf},
isbn = {0471823198},
issn = {1572-9648},
pages = {455},
title = {{Nonlinear solid mechanics: A continuum approach for engineering}},
url = {http://www.citeulike.org/group/2006/article/1044720},
volume = {First Edit},
year = {2000}
}
@article{Gross2011f,
author = {Gross, Dietmar and Seelig, Thomas},
doi = {10.1007/978-3-642-10196-0},
isbn = {978-3-642-10195-3},
title = {{Bruchmechanik}},
url = {http://link.springer.com/10.1007/978-3-642-10196-0},
year = {2011}
}
@article{Moscatelli2017,
author = {Moscatelli, D and Sponchioni, M},
doi = {10.1016/B978-0-08-100262-9.00012-4},
isbn = {9780081002629},
title = {12 12.1},
year = {2017}
}
@article{Anlagen,
author = {Anlagen, Bauliche and Muster-bauordnung, Die and Funktionalit, Die},
journal = {System},
pages = {227--242},
title = {{14 Bauliche Anlagen}}
}
@article{Nitsche2006a,
author = {Nitsche, Wolfgang},
journal = {Str{\"{o}}mungsmesstechnik},
pages = {189--202},
title = {{Signalanalyse}},
year = {2006}
}
@article{Zienkiewicz2005f,
author = {Zienkiewicz, O.C.},
journal = {finite Elem. method fluid Dyn.},
pages = {2--3},
title = {{Incom- Pressible or Almost Incompressible}},
year = {2005}
}
@article{Dell2003,
author = {Dell, Trues-},
number = {2000},
pages = {91--110},
title = {{Placements of Bodies}},
year = {2003}
}
@article{Santus2009,
abstract = {In metals, during high cycle fatigue on plain specimens, almost the entire fatigue life is spent as short crack initiation and propagation. The fatigue short crack life can be schematically divided into two subsequent phases: microstructurally short crack and physically short crack. Recently, Chapetti proposed a physically short crack threshold and propagation driving force model [Chapetti MD. Fatigue propagation threshold of short cracks under constant amplitude loading. Int J Fatigue 2003;25(12):1319-1326]. In his model the physically short crack behavior is obtained from the long crack propagation, just introducing the reduced threshold due to unsaturated closure. In the present paper the physically short crack propagation is similarly modeled by means of a driving force equation, but independent from the long crack propagation. In this way, a better description of the short crack behavior is provided, however short crack propagation data is required. Physically short crack propagation model parameters were obtained, by fitting experimental data drawn from the literature, for two aluminum alloys and a titanium alloy at two different heat treatment conditions and load ratios. By calculating the physically short crack plus long crack propagation, and assuming microstructurally short crack as part of the initiation stage, a purer information about crack initiation can be drawn from the S-N curves, and it is shown in the paper for the investigated materials. A precise crack initiation size and the number of cycles just for initiation are then provided. This information is useful to accurately predict fatigue life for blunt notched and for thick components, where the propagation is much higher than in the small plain specimen. A validation of the model was obtained by predicting the fatigue life of a notched specimen. An accurate prediction was obtained both when the initiation was much smaller than propagation and when almost the entire fatigue life was initiation. ?? 2009 Elsevier Ltd. All rights reserved.},
author = {Santus, C and Taylor, D},
doi = {10.1016/j.ijfatigue.2009.03.002},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/2009{\_}SantusAndTaylor{\_}Physically short crack propagation in metals during high cycle fatigue.pdf:pdf},
isbn = {01421123},
issn = {01421123},
journal = {Int. J. Fatigue},
keywords = {Fatigue crack initiation,Fatigue crack propagation,Microstructurally short cracks,Notched component fatigue life,Physically short cracks},
number = {8-9},
pages = {1356--1365},
publisher = {Elsevier Ltd},
title = {{Physically short crack propagation in metals during high cycle fatigue}},
url = {http://dx.doi.org/10.1016/j.ijfatigue.2009.03.002},
volume = {31},
year = {2009}
}
@article{Chaboche2008a,
abstract = {The purpose of the present review article is twofold:???recall elementary notions as well as the main ingredients and assumptions of developing macroscopic inelastic constitutive equations, mainly for metals and low strain cyclic conditions. The explicit models considered have been essentially developed by the author and co-workers, along the past 30 years;???summarize and discuss a certain number of alternative theoretical frameworks, with some comparisons made with the previous ones, including more recent developments that offer potential new capabilities. ?? 2008 Elsevier Ltd. All rights reserved.},
author = {Chaboche, J. L.},
doi = {10.1016/j.ijplas.2008.03.009},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/Hardening Recovery Creep/2008{\_}Chaboche{\_}A-review-of-some-plasticity-and-viscoplasticity-constitutive-theories.pdf:pdf},
isbn = {0749-6419},
issn = {07496419},
journal = {Int. J. Plast.},
keywords = {Continuum mechanics,Plasticity,Ratchetting,Strain hardening,Viscoplasticity},
number = {10},
pages = {1642--1693},
title = {{A review of some plasticity and viscoplasticity constitutive theories}},
volume = {24},
year = {2008}
}
@article{Differenzialgleichung,
author = {Differenzialgleichung, Diese and Erhaltungssatz, Der and Finite-volumen-verfahren, Das},
doi = {10.1007/978-3-642-24335-6},
isbn = {9783642243356},
title = {{8 Finite-Volumen-Verfahren}}
}
@article{Universit2001a,
author = {Universit, Technischen},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Kolben FEM/Kolbenberechnung{\_}FEM{\_}TemperaturWaermeuebergang.pdf:pdf},
title = {{Technische Universit{\"{a}}t M{\"{u}}nchen Institut f{\"{u}}r Werkstoffe und Verarbeitung Forschungsgruppe Prof . Schmitt-Thomas Werkstoffgerechte Auslegung und Festigkeitsnachweis f{\"{u}}r Verbrennungsmotorkolben aus Mesophasenkohlenstoff}},
year = {2001}
}
@article{EnomotoTemperature1986,
author = {Enomoto, Yoshiteru and Furuhama, Shoichi},
doi = {10.1299/jsme1958.29.3434},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Heat Transfer Combustion Chamber/1986{\_}Enomoto{\_}Study on thin film thermocouple measuring instan temperature on surface of combustion chamber wall in ICE - Part2.pdf:pdf},
journal = {Bull. JSME},
number = {256},
pages = {3434--3441},
title = {{Study on Thin Film Thermocouple Measuring Instantaneous Temperature on Surface of Combustion Chamber Wall In Internal Combustion Engine - 2nd Report, Study on Thin Film Thermocouples Embedded in Combustion Chamber Wall}},
volume = {29},
year = {1986}
}
@article{Verfahren1984,
author = {Verfahren, Berechnung Von and Prozessen, Von},
number = {um 1900},
pages = {186--237},
title = {{9 Energieumwandlung, thermische Maschinen}},
year = {1984}
}
@article{Einzelteile,
author = {Einzelteile, Der},
title = {{8 Methodisches Ausarbeiten Detail design}}
}
@article{LeeFilipi2011,
abstract = {Fast and predictive simulation tools are prerequisites for pursuing simulation based engine control development. A particularly attractive tradeoff between speed and fidelity is achieved with a co-simulation approach that marries a commercial gas dynamic code WAVE{\{}$\backslash$texttrademark{\}} with an in-house quasi-dimensional combustion model. Gas dynamics are critical for predicting the effect of wave action in intake and exhaust systems, while the quasi-D turbulent flame entrainment model provides sensitivity to variations of composition and turbulence in the cylinder. This paper proposes a calibration procedure for such a tool that maximizes its range of validity and therefore achieves a fully predictive combustion model for the analysis of a high degree of freedom (HDOF) engines. Inclusion of a charge motion control device in the intake runner presented a particular challenge, since anything altering the flow upstream of the intake valve remains ``invisible'' to the zero-D turbulence model applied to the cylinder control volume. The solution is based on the use of turbulence multiplier and scheduling of its value. Consequently, proposed calibration procedure considers two scalar variables (dissipation constant C {\$}\beta{\$} and turbulence multiplier C M ), and the refinements of flame front area maps to capture details of the spark-plug design, i.e. the actual distance between the spark and the surface of the cylinder head. The procedure is demonstrated using an SI engine system with dual-independent cam phasing and charge motion control valves (CMCV) in the intake runner. A limited number of iterations led to convergence, thanks to a small number of adjustable constants. After calibrating constants at the reference operating point, the predictions are validated for a range of engine speeds, loads and residual fractions.},
author = {Lee, T -K. and Filipi, Z S},
doi = {10.1007/s12239-011-0001-4},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Injection+Combustion+Ignitionsystems/2011{\_}Lee+Filip{\_}IMPROVING THE PREDICTIVENESS OF THE QUASI-D COMBUSTION MODEL FOR SI ENGINES WITH FLEXIBLE INTAKE SYSTEMS.pdf:pdf},
journal = {Int. J. Automot. Technol.},
month = {feb},
number = {1},
pages = {1--9},
title = {{Improving the predictiveness of the quasi-d combustion model for spark ignition engines with flexible intake systems}},
volume = {12},
year = {2011}
}
@article{Wallentowitz2006e,
author = {Wallentowitz, Henning and Reif, Konrad},
doi = {10.1007/978-3-8348-9121-1_12},
isbn = {978-3-528-03971-4},
journal = {Handb. Kraftfahrzeugelektronik - Grundlagen, Kompon. Syst. Anwendungen},
title = {{Elektrische Aktorik}},
url = {http://www.springerlink.com/index/10.1007/978-3-8348-9121-1{\_}12},
year = {2006}
}
@article{Tobergte2013a,
abstract = {applicability for this approach.},
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Tobergte, David R. and Curtis, Shirley},
doi = {10.1017/CBO9781107415324.004},
eprint = {arXiv:1011.1669v3},
isbn = {9788578110796},
issn = {1098-6596},
journal = {J. Chem. Inf. Model.},
keywords = {icle},
number = {9},
pages = {1689--1699},
pmid = {25246403},
title = {{Technische Thermodynamik}},
volume = {53},
year = {2013}
}
@article{Lotsch,
author = {Lotsch, H K V and Rhodes, Editor-in-chief W T and Adibi, Editorial Board A and Asakura, T and H{\"{a}}nsch, T W and Kamiya, T and Krausz, F and Monemar, B and Venghaus, H and Weber, H and Weinfurter, H and Rhodes, William T},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Atomistic and Continuum Modeling of Nanocrystalline Materials/front-matter.pdf:pdf},
isbn = {9780387300696},
title = {{Springer Series in Springer Series in}}
}
@article{Clements1998,
author = {Clements, Linda L.},
doi = {10.1007/978-1-4615-6389-1_11},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/{\_}buecherSong/HandbookofComposites/I/10{\_}OrganicFibers.pdf:pdf},
isbn = {978-0-412-54020-2},
pages = {202--241},
title = {{Organic Fibers}},
year = {1998}
}
@article{Tensors2003,
author = {Tensors, Tangent-modulus},
pages = {227--241},
title = {{for Thermomechanical Response of Elastomers}},
year = {2003}
}
@misc{Eshelby1951a,
abstract = {The parallel between the classical theory of elasticity and the modern physical theory of the solid state is incomplete; the former has nothing analogous to the concept of the force acting on an imperfection (dislocation, foreign atom, etc.) in a stressed crystal lattice. To remedy this a general theory of the forces on singularities in a Hookean elastic continuum is developed. The singularity is taken to be any state of internal stress satisfying the equilibrium equations but not the compatibility conditions. The force on a singularity can be given as an integral over a surface enclosing it. The integral contains the elastic field quantities which would surround the singularity in an infinite medium, multiplied by the difference between these quantities and those actually present. The expression for the force is thus of essentially the same form whether the force is due to applied surface tractions, other singularities or the presence of the free surface of the body ({\{}{\{}{\}}'{\{}{\}}{\}}image force{\{}{\{}{\}}'{\{}{\}}{\}}). A region of inhomogeneity in the elastic constants modifies the stress field; if it is mobile one can define and calculate the force on it. The total force on the singularities and inhomogeneities inside a surface can be expressed in terms of the integral of a {\{}{\{}{\}}'{\{}{\}}{\}}Maxwell tensor of elasticity{\{}{\{}{\}}'{\{}{\}}{\}} taken over the surface. Possible extensions to the dynamical case are discussed.},
author = {Eshelby, J D},
booktitle = {Philos. Trans. R. Soc. A Math. Phys. Eng. Sci.},
doi = {10.1098/rsta.1951.0016},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/1951{\_}Eshelby{\_}The force oo an elastic singularity.pdf:pdf},
isbn = {00804614},
issn = {1364-503X},
number = {877},
pages = {87--112},
title = {{The Force on an Elastic Singularity}},
url = {http://rsta.royalsocietypublishing.org/cgi/doi/10.1098/rsta.1951.0016},
volume = {244},
year = {1951}
}
@article{Guo2013,
author = {Guo, Junhang},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Plasticity models/An experimental and numerical investigation on damage evolution and ductile fracture mechanism of aluminium alloy{\_}MitRousselierHerleitung.pdf:pdf},
number = {June},
title = {{Junhang Guo The University of Tokushima June 2013}},
year = {2013}
}
@article{Xu1993a,
abstract = {In a numerical micromechanical study of void nucleation, a framework is used where
constitutive relations are specified independently for the matrix, the void-nucleating particles and the interface. Plane strain analyses are carried out for a doubly periodic array of circular cylindrical particles. The particles are taken to be rigid and the elastic-plastic deformations of the matrix are decribed in terms of continuum crystalline plasticity, using a planar crystal model that allows for three slip systems. Comparison is made with void-nucleation predictions based on a corresponding flow theory of plasticity with isotropic hardening. The crystal model on give rise to shear localization at the particle-matrix interface and shear localization, which leads to large localized strains in the matrix. is found to inhibit decohesion. The role of the triaxiality of the stress state in determining whether decohesion or localization occurs first is investigated. A parametric study is also carried out for a crystal matrix using two descriptions of the interface shear behaviour; one is periodic in the shear displacement across the interface while the other allows for shear decohesion.},
author = {Xu, X -P and Needleman, A},
doi = {10.1088/0965-0393/1/2/001},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/1993{\_}Needleman{\_}Void nucleation by inclusion debonding in a crystal matrix.pdf:pdf},
issn = {0965-0393},
journal = {Model. Simul. Mater. Sci. Eng.},
number = {2},
pages = {111--132},
title = {{Void nucleation by inclusion debonding in a crystal matrix}},
url = {http://stacks.iop.org/0965-0393/1/i=2/a=001?key=crossref.0ad72f94185990833a445936aea2f0ba},
volume = {1},
year = {1993}
}
@article{Guo2013,
author = {Guo, Junhang},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Plasticity models/An experimental and numerical investigation on damage evolution and ductile fracture mechanism of aluminium alloy{\_}MitRousselierHerleitung.pdf:pdf},
number = {June},
title = {{Junhang Guo The University of Tokushima June 2013}},
year = {2013}
}
@article{Arnolda,
author = {Arnold, J{\"{o}}rg},
pages = {811--821},
title = {{C8 Mikrospurenauswertung C8 Arten von Mikrospuren}}
}
@article{Principle2003,
author = {Principle, Incremental},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Nicholson 2003 - Finite Element Analysis Thermomechanics of Solids/0749{\_}C17.pdf:pdf},
pages = {215--226},
title = {{Incremental Principle of Virtual Work 17.1}},
volume = {2},
year = {2003}
}
@article{Entropy2003,
author = {Entropy, O F},
journal = {Energy},
pages = {107--116},
title = {{Thermal and Thermomechanical Response}},
year = {2003}
}
@article{Arbeitsumgebungc,
author = {Arbeitsumgebung, Die},
journal = {Pro-Engineer Prakt.},
title = {{6 Baugruppenmodellierung}}
}
@book{Schade2006,
author = {Schade, Heinz and Neemann, Klaus},
isbn = {3110147416},
pages = {398},
title = {{Tensoranalysis}},
url = {http://www.amazon.de/dp/3110147416},
year = {2006}
}
@article{Wasserwellen2006,
author = {Wasserwellen, Den},
journal = {Gerthsen Phys.},
pages = {519--568},
title = {{10 - Wellenoptik}},
year = {2006}
}
@inproceedings{Wang1985,
author = {Wang, C S and Berry, G F},
booktitle = {ASME Winter Annu. Meet.},
file = {:C$\backslash$:/Users/p327208/Desktop/Promotion/Literature/Motorspezifisch/1985{\_}Wang{\_}Heat Transfer in Internal Combustion Engines.pdf:pdf},
pages = {1--7},
title = {{Heat Transfer in Internal Combustion Engines}},
year = {1985}
}
@article{Tress2003,
author = {Tress, C Auchy S},
pages = {73--93},
title = {{Mechanical Equilibrium and the Principle of Virtual Work 5.1}},
year = {2003}
}
@inproceedings{Malbec2011,
author = {Malbec, Louis Marie and Picket, Lyle M. and Payri, Raul and Manin, Julien and Bardi, Michele and Bazin, Tim and Kastengren, Alan and Meijer, Maarten and Somers, L M T},
booktitle = {ECN Work. 13-14 May},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Heat Transfer Combustion Chamber/2011{\_}Malbec{\_}Spray{\_}NozzleTipTemperatureMeasurements.pdf:pdf},
title = {{Nozzle tip and injectors body temperature measurements}},
year = {2011}
}
@article{Bewegungsgleichungen,
author = {Bewegungsgleichungen, Die and Bewegungsgleichungen, Die},
title = {{13 Schleichende Str o ¨ mungen}}
}
@article{AntonT.2006,
author = {{Anton T.}, van Zanten},
doi = {10.1007/978-3-8348-9049-8_8},
isbn = {978-3-8348-0109-8},
journal = {Fahrdynamik Regelung},
pages = {169--211},
title = {{8 Elektronisches Stabilit{\{}{\"{a}}{\}}tsprogramm (ESP)}},
url = {http://link.springer.com/chapter/10.1007/978-3-8348-9049-8{\%}7B{\_}{\%}7D8},
year = {2006}
}
@article{Fallbeispiele2005,
author = {Fallbeispiele, Die},
doi = {10.1007/3-7985-1528-X_7},
isbn = {3-7985-1465-8},
pages = {25--125},
title = {{Fallbeispiele}},
year = {2005}
}
@article{Lal1977,
abstract = {This paper reviews and compares the various approaches for finding monotonic and cyclic plastic zone sizes for elastic-perfectly plastic and strain hardening materials. All through the analysis Ramberg-Osgood relationship has been used representing the monotonic and cyclic stress-strain curves. The results for elastic-perfectly plastic materials are compared with those available using finite-element technique. The ratio of monotonic plastic zone sizes strain hardening and elastic perfectly plastic materials are found to be related to the Ramberg-Osgood index n. The values of cyclic plastic zone size are found to depend upon factors like crack opening stress, material properties and specimen geometry. The cyclic plastic zone size obtained in this paper compare well with those given by Antolovich. ?? 1977.},
author = {Lal, K. M. and Garg, S. B L},
doi = {10.1016/0013-7944(77)90036-4},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/1977{\_}LAL+GARG{\_}On the evaluation of monotonic and cyclic plastic zones.pdf:pdf},
issn = {00137944},
journal = {Eng. Fract. Mech.},
number = {2},
pages = {433--442},
title = {{On the evaluation of monotonic and cyclic plastic zones}},
volume = {9},
year = {1977}
}
@article{To2013,
author = {To, Nswers},
doi = {10.1007/978-3-642-22346-4},
isbn = {9783642223464},
pages = {1--6},
title = {{Kapitel 8}},
year = {2013}
}
@article{Fillers,
author = {Fillers, Particulate},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/{\_}buecherSong/HandbookofComposites/I/11{\_}ParticulateFillers.pdf:pdf},
journal = {New York},
title = {{Particulate fillers}}
}
@article{Konzepte,
author = {Konzepte, Downsizing- and Steigerung, Eine and Gegensatz, Im and Geschwindigkeit, Die},
title = {{3 Downsizing}}
}
@inproceedings{Wang1985,
author = {Wang, C S and Berry, G F},
booktitle = {ASME Winter Annu. Meet.},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/1985{\_}Wang{\_}Heat Transfer in Internal Combustion Engines.pdf:pdf},
pages = {1--7},
title = {{Heat Transfer in Internal Combustion Engines}},
year = {1985}
}
@article{Mohammadi2011_Boiling,
abstract = {Basic understanding of the process of coolant heat transfer inside an engine is an indispensable prerequisite to devise an infallible cooling strategy. Coolant flow and its heat transfer affect the cooling efficiency, thermal load of heated components, and thermal efficiency of a diesel engine. An efficient approach to studying cooling system for diesel engine is a 3D computational fluid dynamics (CFD) calculation for coolant jacket. Therefore, computer simulation can analyze and consequently optimize cooling system performance, including complex cooling jacket. In this paper a computational model for boiling heat transfer based on two-phase Mixture model flow is established. Furthermore, the phenomenon of nucleate boiling, its mathematical modeling, and its effect on heat transfer is discussed. Besides, the static, total pressure, velocity and stream lines of the flow field, heat flux, heat transfer coefficient and volume fraction of vapor distribution in the coolant jacket of a four-cylinder diesel engine is computed. Also, comparison between experimental equation (Pflaum/Mollenhauer) and two-phase Mixture model for boiling heat transfer coefficient is done and good agreement is seen. In conclusion, it is observed that at high operating temperatures, nucleate boiling occurs in regions around the exhaust ports. Numerical simulation of boiling heat transfer process of cooling water jacket and temperature field in the cylinder head of the diesel engine is compared with the data measured on the engine test bench. The calculated results indicate that this method can reflect the impact of boiling heat transfer on water jacket more accurately. Therefore, this method is beneficial to improve the computational precision in the temperature field computation of a cylinder head.},
author = {Mohammadi, A and Yaghoubi, M},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Boiling/2011{\_}Mohammadi{\_}Two Phase Flow Simulation for Subcooled Nucleat  Boiling Heat Transfer Calculation in Water Jacket of Diesel Engine.pdf:pdf},
journal = {J. Engine Res.},
number = {22},
pages = {50--61},
title = {{Two Phase Flow Simulation for Subcooled Nucleat Boiling Heat Transfer Calculation in Water Jacket of Diesel Engine}},
volume = {22},
year = {2011}
}
@article{Fs2013b,
author = {Fs},
doi = {10.1007/978-1-4614-0502-3},
isbn = {2009004043},
number = {1},
pages = {0--10},
title = {{Chapter 0}},
year = {2013}
}
@article{Ubersetzungen2007,
author = {{\"{U}}bersetzungen, Kennungswandler Wahl Der},
journal = {Fahrzeuggetriebe},
title = {{4 Kennungswandler – Wahl der {\{}{\"{U}}{\}}bersetzungen}},
year = {2007}
}
@article{Sanli2009b,
author = {Sanli, A and Sayin, C and Gumus, M and Kilicaslan, I and Canakci, M},
journal = {Numer. Heat Transf. Part A Appl.},
number = {5},
pages = {444--458},
title = {{Numerical Evaluation by Models of Load and Spark Timing Effects on the In-Cylinder Heat Transfer of a SI Engine}},
volume = {56},
year = {2009}
}
@article{Rothe2015a,
abstract = {In this article we investigate a fully, thermo-mechanically coupled viscoplasticity model in view of various numerical aspects. First, we develop the entire system of differential–algebraic equations resulting from the spatially discretized principle of virtual displacements, the principle of virtual temperatures, and the evolution equations of the internal variables provided by the constitutive model. In the time-integration step this system is solved both using a fully monolithic approach based on a Backward–Euler scheme in combination with the Multilevel-Newton algorithm as well as a partitioned approach solving the fully coupled system. The latter is treated by means of a combination of a Backward–Euler method and an accelerated Gauss–Seidel/Multilevel-Newton scheme to solve the resulting system of algebraic equations within each time-integration step. Additionally, we consider a specific treatment of the interpolation between different meshes within the partitioned approach. This is shown for p-version finite elements based on hierarchical shape functions. Finally, it turns out that the specific constitutive model of small-strain thermo-viscoplasticity, which is based on the decomposition into kinematic hardening and energy storing strains, yields a problem-adapted stress algorithm. This allows to reduce the stress algorithm on Gauss-point level to the solution of one scalar equation. Numerical examples serve to elucidate the behavior and properties of the proposed methods.},
author = {Rothe, Steffen and Erbts, Patrick and D{\"{u}}ster, Alexander and Hartmann, Stefan},
doi = {10.1016/j.cma.2015.05.002},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Numerik UMATS FE-Codes/2015{\_}Hartmann{\_}Monolithic and partitioned coupling schemes for thermo-viscoplasticity.pdf:pdf},
issn = {00457825},
journal = {Comput. Methods Appl. Mech. Eng.},
keywords = {algebraic equations,differential,fully coupled finite elements,monolithic approach,partitioned approach,thermo-viscoplasticity},
pages = {375--410},
publisher = {Elsevier B.V.},
title = {{Monolithic and partitioned coupling schemes for thermo-viscoplasticity}},
url = {http://linkinghub.elsevier.com/retrieve/pii/S0045782515001681},
volume = {293},
year = {2015}
}
@article{Kraftstoffverbrauch,
author = {Kraftstoffverbrauch, Der and Pra-, Der},
pages = {189--204},
title = {{7 Kraftstoffverbrauch}}
}
@article{Fertigungsverfahren,
author = {Fertigungsverfahren, Fertigungsverfahren and Folgenden, Im},
pages = {172--227},
title = {{4 Verarbeitungsmethoden}}
}
@article{Teil2011,
author = {Teil, Solidworks and Einzelteile, Modellierung and Baugruppen, Modellierung and Baugruppe, Solidworks and Zeichnung, Solidworks and Drehen, Dynamisches},
doi = {10.1007/978-3-8348-8161-8},
isbn = {9783834881618},
pages = {134--141},
title = {{Musterl{\"{o}}sungen zu Kontrollfragen in Kapitel 1 Musterl{\"{o}}sungen zu Kontrollfragen in Kapitel 2 Musterl{\"{o}}sungen zu Kontrollfragen in Kapitel 3}},
year = {2011}
}
@article{Mughrabi2013,
abstract = {Depending on material and details of cyclic loading conditions, fatigue damage develops and spreads by various modes of crack initiation and subsequent crack growth. In order to gain a deeper understanding of the underlying microstructural mechanisms, many details must be considered. The present study focuses on just a few specific aspects, namely the role of cyclic slip irreversibilities, the significance of fatigue crack initiation in high and ultrahigh cycle fatigue (HCF, UHCF) and, finally the analysis of non-linear effects of elasticity and compliance of fatigued specimens, as a promising non-destructive in situ fatigue damage diagnosis tool. Selected experimental data obtained on different materials will be considered to illustrate the issues named above. ?? 2012 Elsevier B.V. All rights reserved.},
author = {Mughrabi, Hael},
doi = {10.1016/j.ijfatigue.2012.06.007},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/2013{\_}Mughrabi{\_}Microstructural fatigue mechanisms - Cyclic slip irreversibility - crack initiation - non-linear elastic damage analysis.pdf:pdf},
isbn = {01421123},
issn = {01421123},
journal = {Int. J. Fatigue},
keywords = {(Ultra) High cycle fatigue,Cyclic slip irreversibility,Fatigue crack initiation,Fatigue lives,Non-linear elasticity},
pages = {2--8},
publisher = {Elsevier Ltd},
title = {{Microstructural fatigue mechanisms: Cyclic slip irreversibility, crack initiation, non-linear elastic damage analysis}},
url = {http://dx.doi.org/10.1016/j.ijfatigue.2012.06.007},
volume = {57},
year = {2013}
}
@article{Variablesa,
author = {Variables, Biowin State},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Probabilistic Aspects/A Unified Statistical Methodology for Modeling Fatigue Damage{\_}Castillo/Backmatter{\_}MitModelle.pdf:pdf},
pages = {1--72},
title = {{Models Used In BioWin}}
}
@article{Hochhalter2011a,
abstract = {It has been observed during fatigue cracking of AA 7075-T651 that a small percentage of Al 7 Cu 2 Fe particles crack during manufacturing or very early in their life. Some of the cracked particles eventually nucleate cracks into the surrounding microstructure, and among these the number of cycles required for nucleation varies widely. It is important to comprehend the mechanics underpinning the observed variation so that the subsequent propagation stage can be accurately modeled. To this end, finite element models of replicated grain and particle geometry are used to compute mechanical fields near monitored cracked particles using an elastic–viscoplastic crystal plasticity model that captures the effect of the orientation of the grains near each monitored particle. Nonlocal, slip-based metrics are used to study the localization and cyclic accumulation of slip near the cracked particles providing mechanics-based insight into the actuation of the nucleation event. A high slip localization and cyclic accumulation rate are found to be a necessary, but not sufficient, condition for nucleation from cracked particles. A sufficient local driving stress must also be present, which is strongly dependent on the local microstructure and accumulated slip. Furthermore, the simulation results elucidate a quantitative relationship between the slip accumulated during fatigue loading and a consequential reduction of the critical local driving stress for nucleation, providing a physical basis for the fatigue damage concept. The observed nucleation direction is orthogonal to the computed local maximum tangential stress direction, as expected for this alloy. The main result is a semi-empirical model for the number of cycles required for nucleation, which is dependent on the maximum tangential stress and cyclic slip-accumulation rate near a cracked particle.},
author = {Hochhalter, J D and Littlewood, D J and Veilleux, M G and Bozek, J E and Maniatty, A M and Rollett, A D and Ingraffea, A R},
doi = {10.1088/0965-0393/19/3/035008},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/2011{\_}Hochhalter{\_}AL7075AgeometricapproachIII{\_}SemiempiricalApproachNucleation.pdf:pdf},
isbn = {09650393 (ISSN)},
issn = {0965-0393},
journal = {Model. Simul. Mater. Sci. Eng.},
number = {3},
pages = {35008},
title = {{A geometric approach to modeling microstructurally small fatigue crack formation: III. Development of a semi-empirical model for nucleation}},
url = {http://stacks.iop.org/0965-0393/19/i=3/a=035008?key=crossref.8640954c7485639bf37ab73e6f2eb0ad},
volume = {19},
year = {2011}
}
@article{Chaboche1989a,
abstract = {The cyclic constitutive equations developed and used at ONERA and LMT-Cachan are presented in detail in terms of a hierarchy of various models. Both the time-independent and the viscoplasticity versions of the equations are discussed, as well as their ability to describe correctly most of the experimentally observed effects under monotonic or cyclic loading, constant or variable temperature, including strain hardening and time recovery effects. The reported experimental data concerns stainless steels and have been published previously. Four other theories are then presented and compared in a systematic way. They include the Ohno-Kachi time-independent plasticity theory, two unified viscoplastic models by Walker and by Krempl and Yao, the new developments of the endochronic theory by Watanabe and Atluri. All these approaches show some similarities with the first one, especially in that concerns the non.linearity of kinematic hardening, which represents the key for describing the cyclic behav- iour of metallic materials.},
author = {Chaboche, J.L.},
doi = {http://dx.doi.org/10.1016/0749-6419(89)90015-6},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/Hardening Recovery Creep/1989{\_}Chaboche{\_}Constitutive equations for cyclic plasticity and cyclic viscoplasticity.pdf:pdf},
isbn = {1111111111},
issn = {0749-6419},
journal = {Int. J. Plast.},
pages = {247--302},
title = {{Constitutive equations for cyclic plasticty and cyclic viscoplasticity}},
volume = {5},
year = {1989}
}
@article{Chemie1806a,
author = {Chemie, Organische},
pages = {1--3},
title = {{1 Einf{\{}{\"{u}}{\}}hrung}},
year = {1806}
}
@book{Riccardella1992c,
author = {Riccardella, PC and Deardorff, AF and Griesbach, TJ},
booktitle = {Adv. Fatigue Lifetime Predict. Tech.},
doi = {10.1520/STP1122-EB},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Neuer Ordner/Advances in fatigue lifetime predictive techniques Part1.pdf:pdf},
isbn = {978-0-8031-1423-4},
issn = {00660558},
keywords = {FATIGUE,MONITORING,POWER PLANTS,PRESSURE VESSELS AND PIPING,THERMAL STRESSES},
pages = {460--473},
pmid = {11439068},
title = {{Advances in Fatigue Lifetime Predictive Techniques}},
url = {https://apps.webofknowledge.com/full{\_}record.do?product=UA{\&}search{\_}mode=GeneralSearch{\&}qid=11{\&}SID=Z1UxbH6jtsqo8n9kPQr{\&}page=1{\&}doc=1},
volume = {1122},
year = {1992}
}
@article{Lankford1973,
abstract = {Electron microscopy of surface replicas has been employed to determine the metallurgical micromechanics of fatigue crack initiation at surface and shallow subsurface inclusions in 4340 steel. The experimental results are considered in terms of current theoretical anal- yses of elastic stress distributions around hard inclusions imbedded in soft matrices. A model for crack nucleation at surface inclusions is suggested, based upon debonding of the inclusion/matrix interface at the tensile pole of the inclusion, followed by growth of the debond seam toward the inclusion "equator". Subsequent generation of a matrix crack is associated with the initiation of "point" surface defects some distance from the inclusion/ma- trix boundary, but in the plane of the inclusion "equator". Surface slip plays no discernible role in nucleation of surface inclusions, but slip bands are formed at crack sites above sub- surface inclusions. However, the microcracks continue to form through the link-up of point surface defects.},
author = {Lankford, James and Kusenberger, F. N.},
doi = {10.1007/BF02648709},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/1973{\_}Lankford{\_}Initiation of fatigue cracks in 4340 steel.pdf:pdf},
issn = {0360-2133},
journal = {Metall. Trans.},
number = {February},
pages = {553--559},
title = {{Initiation of fatigue cracks in 4340 steel}},
volume = {4},
year = {1973}
}
@article{Wallentowitz2006a,
author = {Wallentowitz, Henning and Reif, Konrad},
doi = {10.1007/978-3-8348-9121-1_11},
journal = {Handb. Kraftfahrzeugelektronik - Grundlagen, Kompon. Syst. Anwendungen},
title = {{Sensorik}},
url = {http://www.springerlink.com/index/10.1007/978-3-8348-9121-1{\_}11},
year = {2006}
}
@article{Borg2006b,
author = {Borg, Jm and Alkidas, Ac},
doi = {10.4271/2006-01-3341},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Klopfen{\_}Ottomotor/2006{\_}Borg{\_}Characterisation of autoignition in a knocking si engine using heat release analysis.pdf:pdf},
journal = {SAE Tech. Pap.},
number = {724},
pages = {776--790},
title = {{Characterization of autoignition in a knocking SI engine using heat release analysis}},
url = {http://papers.sae.org/2006-01-3341/},
volume = {2006-01-33},
year = {2006}
}
@article{Klein1990,
author = {Klein, Bernd},
doi = {10.1007/978-3-322-85604-3_3},
isbn = {9783528051259},
pages = {11--32},
title = {{Grundgleichungen der Linearen Finite-Element-Methode}},
year = {1990}
}
@article{Betrachtungeng,
author = {Betrachtungen, Allgemeine},
title = {{Omungen}}
}
@article{Meister2011d,
abstract = {Die wichtigsten Verfahren zur numerischen L{\"{o}}sung von linearen Gleichungssystemen in einer umfassenden Einf{\"{u}}hrung, die zum Verst{\"{a}}ndnis nur geringe mathematische Vorkenntnisse ben{\"{o}}tigt. Behandelt werden sowohl die direkten als auch die iterativen Verfahren, wobei der Autor gro{\ss}en Wert auf eine sorgf{\"{a}}ltige Herleitung dieser Verfahren legt. Au{\ss}erdem sind sehr detaillierte Pseudocodes enthalten, mit deren Hilfe sich die jeweiligen Verfahren in einer beliebigen Programmiersprache sofort auf dem Computer realisieren lassen. Das Lehrbuch ist auch f{\"{u}}r Natur- und Ingenieurwissenschaftler geeignet, die in vielen praktischen Anwendungen mit der L{\"{o}}sung von linearen Gleichungssystemen konfrontiert sind.},
archivePrefix = {arXiv},
arxivId = {1011.1669v3},
author = {Meister, Andreas},
doi = {10.1007/978-3-8348-8100-7},
eprint = {1011.1669v3},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/Numerik linearer Gleichungssysteme{\_}Andreas Meister/Frontmatter.pdf:pdf},
isbn = {978-3-8348-1550-7},
issn = {1098-6596},
journal = {Matrix},
pages = {36--68},
pmid = {25246403},
title = {{Numerik linearer Gleichungssysteme}},
url = {http://link.springer.com/10.1007/978-3-8348-8100-7},
year = {2011}
}
@misc{Banabic2000,
abstract = {After a brief introduction into crystal plasticity, the fun- damentals of crystallographic textures and plastic anisotro- py, a main topic of this book, are outlined. A large chapter is devoted to formability testing both for bulk metal and sheet metal forming. For the first time testing methods for plastic anisotropy of round bars and tubes are included. A profound survey is given of literature about yield criteria for anisotropic materials up to most recent developments and the calculation of forming limits of anisotropic sheet me- tal. Other chapters are concerned with properties of workpieces after metal forming as well as the fundamentals of the theory of plasticity and finite element simulation of metal forming processes. The book is completed by a collection of tables of international standards for formability testing and of flow curves of metals which are most commonly used in metal forming. It is addressed both to university and industrial readers.},
author = {Banabic, Dorel},
doi = {\url{10.1007/978-3-662-04013-3}},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Banabic et al. - 2000 - Formability Topics-Metallic Materials.pdf:pdf},
isbn = {3540679065},
title = {{Formability of metallic materials: plastic anisotropy, formability testing, forming limits}},
year = {2000}
}
@inproceedings{Konigsson2012,
author = {K{\"{o}}nigsson, Fredrik and Stalhammar, Per and Angstrom, Hans-Erik},
booktitle = {SAE Tech. Pap. 2012-01-0826},
doi = {10.4271/2012-01-0826},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Heat Transfer Combustion Chamber/2012{\_}Koenigsson{\_}Controlling the Injector Tip Temperature in a Diesel Dual Fuel Engine.pdf:pdf},
publisher = {SAE international},
title = {{Controlling the Injector Tip Temperature in a Diesel Dual Fuel Engine}},
year = {2012}
}
@article{Cherkaoui2009e,
author = {Cherkaoui, Mohammed and Capolungo, Laurent},
doi = {10.1007/978-0-387-46771-9},
isbn = {978-0-387-46765-8},
pages = {29--52},
title = {{Atomistic and Continuum Modeling of Nanocrystalline Materials}},
url = {http://link.springer.com/10.1007/978-0-387-46771-9},
volume = {112},
year = {2009}
}
@article{Murakami2012h,
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Murakami, Sumio},
doi = {10.1007/978-94-007-2666-6},
eprint = {arXiv:1011.1669v3},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/Continuum Damage Mechanics - SumioMurakami/Kap1{\_}Material Damage and Continuum Damage Mechanics.pdf:pdf},
isbn = {978-94-007-2665-9},
issn = {09250042},
pages = {3--13},
pmid = {25246403},
title = {{Continuum Damage Mechanics}},
url = {http://link.springer.com/10.1007/978-94-007-2666-6},
volume = {185},
year = {2012}
}
@article{Borg2006a,
author = {Borg, Jm and Alkidas, Ac},
doi = {10.4271/2006-01-3341},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2006{\_}Borg{\_}Characterisation of autoignition in a knocking si engine using heat release analysis.pdf:pdf},
journal = {SAE Tech. Pap.},
number = {724},
pages = {776--790},
title = {{Characterization of autoignition in a knocking SI engine using heat release analysis}},
url = {http://papers.sae.org/2006-01-3341/},
volume = {2006-01-33},
year = {2006}
}
@article{Steering,
author = {Steering, Active Front and Kapitel, Dieses},
pages = {213--236},
title = {{9 Mechatronische Lenksysteme : Modellbildung und Funktionalit{\"{a}}t des Active Front Steering}}
}
@article{Hochhalter2011a,
abstract = {It has been observed during fatigue cracking of AA 7075-T651 that a small percentage of Al 7 Cu 2 Fe particles crack during manufacturing or very early in their life. Some of the cracked particles eventually nucleate cracks into the surrounding microstructure, and among these the number of cycles required for nucleation varies widely. It is important to comprehend the mechanics underpinning the observed variation so that the subsequent propagation stage can be accurately modeled. To this end, finite element models of replicated grain and particle geometry are used to compute mechanical fields near monitored cracked particles using an elastic–viscoplastic crystal plasticity model that captures the effect of the orientation of the grains near each monitored particle. Nonlocal, slip-based metrics are used to study the localization and cyclic accumulation of slip near the cracked particles providing mechanics-based insight into the actuation of the nucleation event. A high slip localization and cyclic accumulation rate are found to be a necessary, but not sufficient, condition for nucleation from cracked particles. A sufficient local driving stress must also be present, which is strongly dependent on the local microstructure and accumulated slip. Furthermore, the simulation results elucidate a quantitative relationship between the slip accumulated during fatigue loading and a consequential reduction of the critical local driving stress for nucleation, providing a physical basis for the fatigue damage concept. The observed nucleation direction is orthogonal to the computed local maximum tangential stress direction, as expected for this alloy. The main result is a semi-empirical model for the number of cycles required for nucleation, which is dependent on the maximum tangential stress and cyclic slip-accumulation rate near a cracked particle.},
author = {Hochhalter, J D and Littlewood, D J and Veilleux, M G and Bozek, J E and Maniatty, A M and Rollett, A D and Ingraffea, A R},
doi = {10.1088/0965-0393/19/3/035008},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/2011{\_}Hochhalter{\_}AL7075AgeometricapproachIII{\_}SemiempiricalApproachNucleation.pdf:pdf},
isbn = {09650393 (ISSN)},
issn = {0965-0393},
journal = {Model. Simul. Mater. Sci. Eng.},
number = {3},
pages = {035008},
title = {{A geometric approach to modeling microstructurally small fatigue crack formation: III. Development of a semi-empirical model for nucleation}},
url = {http://stacks.iop.org/0965-0393/19/i=3/a=035008?key=crossref.8640954c7485639bf37ab73e6f2eb0ad},
volume = {19},
year = {2011}
}
@article{Zienkiewicz,
author = {Zienkiewicz, O C},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Zienkiewicz FEM - Vol 3 Fluid Dynamics/63229{\_}fm.pdf:pdf},
title = {{Method for Fluid Dynamics}}
}
@article{Element2002,
abstract = {Three Botrytis-susceptible mutants bos2, bos3, and bos4 which define independent and novel genetic loci required for Arabidopsis resistance to Botrytis cinerea were isolated. The bos2 mutant is susceptible to B. cinerea but retains wild-type levels of resistance to other pathogens tested, indicative of a defect in a response pathway more specific to B. cinerea. The bos3 and bos4 mutants also show increased susceptibility to Alternaria brassicicola, another necrotrophic pathogen, suggesting a broader role for these loci in resistance. bos4 shows the broadest range of effects on resistance, being more susceptible to avirulent strain of Pseudomonas syringae pv. tomato. Interestingly, bos3 is more resistant than wild-type plants to virulent strains of the biotrophic pathogen Peronospora parasitica and the bacterial pathogen P. syringae pv. tomato. The Pathogenesis Related gene 1 (PR-1), a molecular marker of the salicylic acid (SA)-dependent resistance pathway, shows a wild-type pattern of expression in bos2, while in bos3 this gene was expressed at elevated levels, both constitutively and in response to pathogen challenge. In bos4 plants, PR-1 expression was reduced compared with wild type in response to B. cinerea and SA. In bos3, the mutant most susceptible to B. cinerea and with the highest expression of PR-1, removal of SA resulted in reduced PR-1 expression but no change to the B. cinerea response. Expression of the plant defensin gene PDF1-2 was generally lower in bos mutants compared with wild-type plants, with a particularly strong reduction in bos3. Production of the phytoalexin camalexin is another well-characterized plant defense response. The bos2 and bos4 mutants accumulate reduced levels of camalexin whereas bos3 accumulates significantly higher levels of camalexin than wild-type plants in response to B. cinerea. The BOS2, BOS3, and BOS4 loci may affect camalexin levels and responsiveness to ethylene and jasmonate. The three new mutants appear to mediate disease responses through mechanisms independent of the previously described BOS1 gene. Based on the differences in the phenotypes of the bos mutants, it appears that they affect different points in defense response pathways.},
author = {Element, Finite and Program, Analysis and Fortran, Compac},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Zienkiewicz FEM - Vol 1 Basics Fundamentals/63205{\_}19.pdf:pdf},
journal = {Program},
number = {1},
pages = {2--5},
title = {{Computer procedures for finite}},
url = {http://www.ncbi.nlm.nih.gov/pubmed/15500471},
volume = {1},
year = {2002}
}
@article{Haarlem1999,
author = {van Haarlem, M.P.},
doi = {10.1007/BFb0104276},
isbn = {978-3-540-65737-8},
journal = {Physics (College. Park. Md).},
title = {{Scientific Applications of Neural Nets}},
url = {http://www.springerlink.com/index/10.1007/BFb0104276},
volume = {522},
year = {1999}
}
@article{Space1996a,
author = {Space, On},
journal = {Imagine},
keywords = {component fit,model functions,normal distribution,odf analysis},
number = {C},
pages = {77--96},
title = {{On Space}},
volume = {10},
year = {1996}
}
@phdthesis{Kraus2007,
author = {Kraus, Eberhard},
file = {:C$\backslash$:/Users/p327208/Desktop/Promotion/FEM{\_}Simulationen{\_}andereLeute/Diplomarbeit Jaberg Brennraumstroemung/Literatur/Dissertation{\_}Kraus.PDF:PDF},
school = {Eberhard-Karls-University Tuebingen},
title = {{Simulation der vorgemischten Verbrennung in einem realen Motor mit dem Level-Set-Ansatz}},
year = {2007}
}
@article{Seifert2010c,
abstract = {In the present paper, predictions of mechanism-based models for cast iron are compared to experimental results obtained for the nodular cast iron EN-GJS-700, the vermicular cast iron EN-GJV-450 and the lamellar cast iron EN-GJL-250. A strategy is proposed to efficiently identify the model parameters based on isothermal experiments. In particular, complex low cycle fatigue (LCF) tests, tension tests and compression tests are used to adjust the time and temperature dependent cyclic plasticity model. The time and temperature dependent fatigue life prediction model is adjusted to LCF tests. For all investigated cast iron materials, good predictions of thermomechanical fatigue (TMF) tests are possible with the models. Additionally, the location of failure and fatigue life of a thermomechanically loaded double-sided notched specimen are predicted with high accuracy. ?? 2010 Elsevier Ltd. All rights reserved.},
author = {Seifert, T and Maier, G and Uihlein, A and Lang, K H and Riedel, H},
doi = {10.1016/j.ijfatigue.2010.02.005},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/2010{\_}Seiffert+Riedel{\_}Mechanism-based thermomechanical fatigue life prediction of cast iron PartTwo Comparison of model with experiment.pdf:pdf},
isbn = {01421123},
issn = {01421123},
journal = {Int. J. Fatigue},
keywords = {Cast iron,Experimental data,Life prediction,Thermomechanical fatigue},
number = {8},
pages = {1368--1377},
publisher = {Elsevier Ltd},
title = {{Mechanism-based thermomechanical fatigue life prediction of cast iron. Part II: Comparison of model predictions with experiments}},
url = {http://dx.doi.org/10.1016/j.ijfatigue.2010.02.005},
volume = {32},
year = {2010}
}
@misc{Oppenheim1989,
author = {Oppenheim, A V and Schafer, R W and Buck, J R},
booktitle = {Discret. signal Process.},
keywords = {FFT,Hilbert,Signal processing,filtering},
pages = {870},
title = {{1 -Introduction.Pdf}},
year = {1989}
}
@article{Science1979,
author = {Science, Greek and Imagery, Social},
journal = {Text},
title = {{Kapitel 3}},
year = {1979}
}
@article{Hufunktionen,
author = {Hufunktionen, Den and Pyramidenfunktionen, Der},
doi = {10.1007/978-3-642-24335-6},
isbn = {9783642243356},
title = {{7 Finite-Elemente-Methode}}
}
@book{Melorose2015a,
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Melorose, J and Perroy, R and Careas, S},
booktitle = {Statew. Agric. L. Use Baseline 2015},
doi = {10.1017/CBO9781107415324.004},
eprint = {arXiv:1011.1669v3},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/Crystall Plasticity Basics/Hull 2011 - Introduction to Dislocation.pdf:pdf},
isbn = {9788578110796},
issn = {1098-6596},
keywords = {icle},
pmid = {25246403},
title = {{Introduction to dislocations}},
volume = {1},
year = {2015}
}
@article{Pahl2007c,
author = {Pahl, Gerhard and Beitz, Wolfgang},
journal = {Konstruktionslehre},
title = {{14 Begriffs{\"{u}}bersicht}},
year = {2007}
}
@article{Ermittlunga,
author = {Ermittlung, Die and Sum-, Die and Vor-, Die},
pages = {38--39},
title = {{16 Gep{\"{a}}ckraum und Volumenermittlung nach VDA ( DIN70020 )}}
}
@article{DeCuyper2016,
abstract = {The heat transfer is a keystone sub-model for engine simulation tools since it affects all targeting parameters (power output, efficiency and emissions. Part I of this work [1] reported a thorough review of heat transfer measurements from literature. Using Design of Experiments (DoE) two measurement matrices were constructed, one for motored and one for fired operation. The present paper focuses on the measurements under fired operation and analyses the heat transfer phenomena in a systematic way. First, the effect of the dependent engine settings on the heat flux is analyzed in a consistent way using ANOVA (Analysis of Variance). Second, it also discusses the influence of the gas properties on the heat flux, which has been overlooked by many authors. Third, the validity of the Reynolds analogy modelling approach is checked, and several improvements are proposed.},
author = {{De Cuyper}, Thomas and Demuynck, Joachim and Broekaert, Stijn and {De Paepe}, Michel and Verhelst, Sebastian},
doi = {10.1016/j.energy.2016.10.032},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Heat Transfer Combustion Chamber/2016{\_}Broekaert{\_}Heat transfer in premixed spark ignition engines part II - Systematicanalysis of the heat transfer phenomena.pdf:pdf},
issn = {03605442},
journal = {Energy},
keywords = {Heat transfer,Internal combustion engine,Model},
pages = {851--860},
publisher = {Elsevier Ltd},
title = {{Heat transfer in premixed spark ignition engines part II: Systematic analysis of the heat transfer phenomena}},
volume = {116},
year = {2016}
}
@article{Yahya2005,
author = {Yahya, S M},
doi = {10.1016/j.ijantimicag.2012.06.019},
isbn = {0132592010},
number = {6},
pages = {22--24},
title = {{References [1]}},
volume = {76},
year = {2005}
}
@article{Kasaba1998,
author = {Kasaba, Koichi and Sano, Takahiro and Kudo, Souichi and Shoji, Tetsuo and Katagiri, Kazumune and Sato, Tadashi},
doi = {10.1016/S0022-3115(98)00343-2},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/1998{\_}Kasaba+Sano{\_}Fatigue crack growth under compressive loading.pdf:pdf},
issn = {00223115},
journal = {J. Nucl. Mater.},
pages = {2059--2063},
title = {{Fatigue crack growth under compressive loading}},
volume = {258-263},
year = {1998}
}
@article{Festigkeit,
author = {Festigkeit, Die and Verformung, Die and Zug, Im and Aktivierung, Die and Po-, Ein},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Werkstoffkunde/Quantitative Verfestigungsmechanismen.pdf:pdf},
title = {{13.1 Verformung und Verfestigung von Polykristallen}}
}
@article{Bauer1998a,
abstract = {Entry flow heat transfer experiments are reported in steady and pulsating flows of air at mean Reynolds numbers of 3000-35 000. THe ducts are chosen to match typical spark-ignition engine manifolds: a highly curved and a straight pipe, which together bracket most practical geometries. The pulsating engine intake flow encompasses an approximate half sine wave followed by a stagnant phase three itmes as long, all at a repetition rate of 16-50 Hz. Heat flow is imposed through electric heating of the outsides of the manifolds. Heat transfer in the curved pipe is closely comparable to the straight geometry, and it is concluded that entrance effects dominate. Time-averaged axially resolved and axially averaged Nusselt numbers are reported. The unsteady nature of the intake flow enhances heat transfer significantly, between 50{\{}{\%}{\}} and 100{\{}{\%}{\}}. Time-resolved wall heat flux measurements at a location close to the exit of the system show that heat transfer is delayed relative to the onset of the flow. During the stagnant flow phase, heat transfer and turbulence decay slowly from their high levels during the induction flow phase. Heat transfer enhancement in the pulsating flow case is caused by the contribution of the stagnant phase.},
author = {Bauer, Wolf D and Wenisch, Joseph and Heywood, John B},
doi = {https://doi.org/10.1016/S0142-727X(97)10001-7},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/1998{\_}Bauer{\_}Averaged and time-resolved heat transfer of steady and pulsating entry flow in intake manifold of a SI engine.pdf:pdf},
journal = {Int. J. Heat Fluid Flow},
keywords = {intake manifold,internal combustion engine,ow,pulsating,transient heat,ux measurements},
number = {1},
pages = {1--9},
title = {{Averaged and time-resolved heat transfer of steady and pulsating entry flow in intake manifold of a spark-ignition engine}},
volume = {19},
year = {1998}
}
@phdthesis{Kunkelmann2011,
author = {Kunkelmann, Christian},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Boiling/2011{\_}Kunkelmann{\_}Numerical Modeling and Investigation of Boiling Phenomena .pdf:pdf},
school = {Technical University Darmstadt},
title = {{Numerical Modeling and Investigation of Boiling Phenomena}},
year = {2011}
}
@article{Ocko1998,
author = {Ocko, B M and Sirota, E B and Sinha, S K and Deutsch, M and Cao, B H and Wu, X Z and Flagan, R C and Vortisch, H and Leisner, T and Schwell, M and Ruehl, E},
doi = {10.1007/978-3-540-89141-3},
isbn = {0446512516},
journal = {Interface},
number = {14},
pages = {127--133},
title = {{Literaturverzeichnis [1]}},
volume = {91},
year = {1998}
}
@article{Sharma2002,
abstract = {This paper illustrates the micromechanics approach to cyclic creep-fatigue damage of Pb-Sn, developed by the authors with the help of a simple case study. It is demonstrated that durability predictions can be made based solely on monotonic test data. Various parametric studies of practical interest are conducted to obtain mechanistic insights into various aspects of damage in solders e.g., effect of hydrostatic stresses, grain size, ramp rate, etc.},
author = {Sharma, Pradeep and Dasgupta, Abhijit},
doi = {10.1115/1.1493203},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Kriechen{\_}Spannungsrelaxation/2002{\_}Sharma Pradeep{\_}Micro-Mechanics of Creep-Fatigue Damage in PB-SN Solder Due to Thermal Cycling PartOne.pdf:pdf},
issn = {1043-7398},
journal = {J. Electron. Packag.},
number = {3},
pages = {298--304},
title = {{Micro-Mechanics of Creep-Fatigue Damage in PB-SN Solder Due to Thermal Cycling—Part II: Mechanistic Insights and Cyclic Durability Predictions From Monotonic Data}},
url = {http://dx.doi.org/10.1115/1.1493203{\%}5Cnhttp://electronicpackaging.asmedigitalcollection.asme.org/data/Journals/JEPAE4/26206/298{\_}1.pdf},
volume = {124},
year = {2002}
}
@article{Brown2005,
abstract = {The classic theories of dislocation pile-ups, initiated by Eshelby, Frank and Nabarro, and by Leibfried, can be greatly simplified if it is recognised that the dislocations in the pile-up will experience uniform stress if they are lodged in an ellipsoidal interface. Elementary algebra then produces the familiar results from continuum theory. It seems possible that the ellipsoid construction may represent physical reality if it is taken to represent a three-dimensional slip-band. If so, there are concentrated forces spreading the band perpendicular to the slip band as well as parallel to it. Such ellipsoids also represent Mode II and Mode III cracks, and give a method for dealing with the more complicated Mode I cracks. ?? 2005 Elsevier B.V. All rights reserved.},
author = {Brown, Lawrence M.},
doi = {10.1016/j.msea.2005.03.043},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/2005{\_}Brown{\_}Dislocation pile-ups slip-bands ellipsoids and cracks.pdf:pdf},
isbn = {0921-5093},
issn = {09215093},
journal = {Mater. Sci. Eng. A},
keywords = {Dislocations,Ellipsoids,Pile-ups,Slip-bands},
number = {1-2 SUPPL.},
pages = {2--6},
title = {{Dislocation pile-ups, slip-bands, ellipsoids, and cracks}},
volume = {400-401},
year = {2005}
}
@article{Meister2011f,
abstract = {Die wichtigsten Verfahren zur numerischen L{\"{o}}sung von linearen Gleichungssystemen in einer umfassenden Einf{\"{u}}hrung, die zum Verst{\"{a}}ndnis nur geringe mathematische Vorkenntnisse ben{\"{o}}tigt. Behandelt werden sowohl die direkten als auch die iterativen Verfahren, wobei der Autor gro{\ss}en Wert auf eine sorgf{\"{a}}ltige Herleitung dieser Verfahren legt. Au{\ss}erdem sind sehr detaillierte Pseudocodes enthalten, mit deren Hilfe sich die jeweiligen Verfahren in einer beliebigen Programmiersprache sofort auf dem Computer realisieren lassen. Das Lehrbuch ist auch f{\"{u}}r Natur- und Ingenieurwissenschaftler geeignet, die in vielen praktischen Anwendungen mit der L{\"{o}}sung von linearen Gleichungssystemen konfrontiert sind.},
archivePrefix = {arXiv},
arxivId = {1011.1669v3},
author = {Meister, Andreas},
doi = {10.1007/978-3-8348-8100-7},
eprint = {1011.1669v3},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/Numerik linearer Gleichungssysteme{\_}Andreas Meister/Kapitel1-Bsp fuer das Auftreten LGS.pdf:pdf},
isbn = {978-3-8348-1550-7},
issn = {1098-6596},
journal = {Matrix},
pages = {36--68},
pmid = {25246403},
title = {{Numerik linearer Gleichungssysteme}},
url = {http://link.springer.com/10.1007/978-3-8348-8100-7},
year = {2011}
}
@article{Barrett1995,
abstract = {Which of the following statements is true? • Users want “black box” software that they can use with complete confidence for general problem classes without having to understand the fine algorithmic details. • Users want to be able to tune data structures for a particular application, even if the software is not as reliable as that provided for general methods. It turns out both are true, for different groups of users. Traditionally, users have asked for and been provided with black box software in the form of mathematical libraries such as LAPACK, LINPACK, NAG, and IMSL. More recently, the high performance community has discovered that they must write custom software for their problem. Their reasons include inadequate functionality of existing software libraries, data structures that are not natural or convenient for a particular problem, and overly general software that sacrifices too much performance when applied to a special case of interest. Can we meet the needs of both groups of users? We believe we can. Accordingly, in this book, we introduce the use of templates. A template is a description of a general algorithm rather than the executable object code or the source code more commonly found in a conventional software library. Nevertheless, although templates are general descriptions of key algorithms, they offer whatever degree of customization the user may desire. For example, they can be configured for the specific data structure of a problem or for the specific computing system on which the problem is to run. We focus on the use of iterative methods for solving large sparse systems of linear equations. Many methods exist for solving such problems. The trick is to find the most effective method for the problem at hand. Unfortunately, a method that works well for one problem type may not work as well for another. Indeed, it may not work at all. Thus, besides providing templates, we suggest how to choose and implement an effective method, and how to specialize a method to specific matrix types. We restrict ourselves to iter ative methods, which work by repeatedly improving an approximate solution until it is accurate enough. These methods access the coefficient matrix A of the linear system only via the matrix vector product y = A {\textperiodcentered} x (and perhaps z = A T {\textperiodcentered} x). Thus the user need only supply a subroutine for computing y (and perhaps z) given x, which permits full exploitation of the sparsity or other special structure of A. We believe that after reading this book, applications developers will be able to use templates to get their program running on a parallel machine quickly. Nonspecialists will know how to choose and implement an approach to solve a particular problem. Specialists will be able to assemble and modify their codes—without having to make the huge investment that has, up to now, been required to tune large-scale applications for each particular machine. Finally, we hope that all users will gain a better understanding of the algorithms employed. While education has not been one of 1 the traditional goals of mathematical software, we believe that our approach will go a long way in providing such a valuable service.},
author = {Barrett, Richard and Berry, Michael and Chan, Tony F. and Demmel, James and Donato, June M and Dongarra, Jack and Eijkhout, Victor and Pozo, Roldan and Romine, Charles and S., G. W. and van der Vorst, Henk},
doi = {10.2307/2153507},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Barrett 1994 - Templates for the Solution of Linear Systems.pdf:pdf},
isbn = {978-0-89871-328-2},
issn = {00255718},
journal = {Math. Comput.},
keywords = {Linear Systems,iterative methods},
number = {211},
pages = {1349},
title = {{Templates for the Solution of Linear Systems: Building Blocks for Iterative Methods.}},
url = {http://www.jstor.org/stable/2153507?origin=crossref},
volume = {64},
year = {1995}
}
@article{Wallentowitz2006i,
author = {Wallentowitz, Henning and Reif, Konrad},
doi = {10.1007/978-3-8348-9121-1_3},
isbn = {978-3-528-03971-4},
journal = {Handb. Kraftfahrzeugelektronik - Grundlagen, Kompon. Syst. Anwendungen},
title = {{Fahrwerksysteme}},
url = {http://www.springerlink.com/index/10.1007/978-3-8348-9121-1{\%}7B{\_}{\%}7D3},
year = {2006}
}
@article{Fem,
author = {Fem, Engineering},
title = {{{\textless}Fracture and Fatigue Models for Composites.pdf{\textgreater}}}
}
@book{Murakami2012d,
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Murakami, Sumio},
doi = {10.1007/978-94-007-2666-6},
eprint = {arXiv:1011.1669v3},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/Continuum Damage Mechanics - SumioMurakami/Kap2{\_}Mechanical Representation of Damage and Damage Variables.pdf:pdf},
isbn = {978-94-007-2665-9},
issn = {09250042},
number = {2},
pages = {15--55},
pmid = {25246403},
title = {{Continuum Damage Mechanics}},
url = {http://link.springer.com/10.1007/978-94-007-2666-6},
volume = {185},
year = {2012}
}
@article{Carlo,
author = {Carlo, Monte},
title = {{2 Elasticity 2.1}}
}
@book{Milton2002,
abstract = {Some of the greatest scientists including Poisson, Faraday, Maxwell, Rayleigh, and Einstein have contributed to the theory of composite materials. Mathematically, it is the study of partial differential equations with rapid oscillations in their coefficients. Although extensively studied for more than a hundred years, an explosion of ideas in the last four decades (and particularly in the last two decades) has dramatically increased our understanding of the relationship between the properties of the constituent materials, the underlying microstructure of a composite, and the overall effective (electrical, thermal, elastic) moduli which govern the macroscopic behavior. This book surveys these exciting developments at the frontier of mathematics and presents many new results.},
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Milton, Graeme W},
doi = {10.1017/CBO9780511613357},
eprint = {arXiv:1011.1669v3},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/Strukturmechanik MMS/Literatur/Mikromechanik{\_}B{\"{u}}cher{\_}Literaturvorschlag{\_}MMS/Milton 2004 Composites.pdf:pdf},
isbn = {9780511613357},
issn = {1098-6596},
pmid = {12215489},
title = {{The Theory of Composites}},
url = {http://ebooks.cambridge.org/ref/id/CBO9780511613357},
year = {2002}
}
@article{Rousselier1987a,
abstract = {Since the pioneering studies conducted by McClintock, Rice and Tracey on the growth of cavities, many studies have covered modelling of ductile fracture; a non-exhaustive list is given of these studies. In the local approach of fracture, the models are used at the tip of cracks, and in the present state, only relatively simple models can be used to solve fracture problems in a complete manner, from material characterization to the analysis of cracked structures. The paper presents two types of models based on a critical ratio of cavity growth or on continuum damage mechanics. In the framework of the local approach of fracture, their possibilities are presented with constant references to experimental validation studies. This allows conclusions to be drawn regarding the effectiveness of the methods proposed and their undeniable contribution to fracture mechanics. ?? 1987.},
author = {Rousselier, G.},
doi = {10.1016/0029-5493(87)90234-2},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Plasticity models/Ductile fracture models and their potential in local approach of fracture{\_}Rousselier.pdf:pdf},
isbn = {00295493},
issn = {00295493},
journal = {Nucl. Eng. Des.},
number = {1},
pages = {97--111},
title = {{Ductile fracture models and their potential in local approach of fracture}},
volume = {105},
year = {1987}
}
@article{Grandin2000,
abstract = {It is generally accepted that knocking combustion influences the heat transfer in SI engines. However, the effects of heat transfer on the onset of knock is still not clear due to lack of experimental data of the thermal boundary layer close to the combustion chamber wall. This paper presents measurements of the temperature in the thermal boundary layer under knocking and non-knocking conditions. The temperature was measured using dual-broadband rotational Coherent anti-Stokes Raman Spectroscopy (CARS). Simultaneous time-resolved measurements of the cylinder pressure, at three different locations, and the heat flux to the wall were carried out. Optical access to the region near the combustion chamber wall was achieved by using a horseshoe-shaped combustion chamber with windows installed in the rectangular part of the chamber. This arrangement made CARS temperature measurements close to the wall possible and results are presented in the range 0.1-5 mm from the wall. The engine was run with constant fuel flow under near stoichiometric conditions. Knocking and non-knocking conditions were achieved by using different mixtures of n-heptane and iso-octane.},
author = {Grandin, B{\"{o}}rje and Denbratt, Ingemar and Bood, Joakim and Brackmann, Christian and Bengtsson, Per-Erik},
doi = {10.4271/2000-01-2831},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Heat transfer intake+exhaust system/2000{\_}Bood{\_}The Effect of Knock on the Heat Transfer in an SI Engine.pdf:pdf},
journal = {SAE Tech. Pap.},
number = {2000-01-2831},
title = {{The Effect of Knock on the Heat Transfer in an SI Engine: Thermal Boundary Layer Investigation using CARS Temperature Measurements and Heat Flux Measurements}},
url = {http://dx.doi.org/10.4271/2000-01-2831},
year = {2000}
}
@article{Menny2006,
author = {Menny, Klaus},
isbn = {103-519-46317-2},
title = {{1.Pdf}},
year = {2006}
}
@article{Analysis,
author = {Analysis, Finite Element and Boundary, Contact},
journal = {Analysis},
title = {{Finite Element Analysis of Contact Boundary Layers}}
}
@article{Index2004,
author = {Index, Subject},
doi = {10.1016/B978-0-444-53238-1.00018-1},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Zienkiewicz FEM - Vol 3 Fluid Dynamics/63229{\_}sindx.pdf:pdf},
isbn = {0065-2458},
issn = {0196-0644},
number = {12},
pages = {1104--1110},
pmid = {25160461},
title = {{Subject Index}},
volume = {11},
year = {2004}
}
@article{Boshers2001,
author = {Boshers, Chris},
doi = {10.1361/asmhba0003393},
journal = {Composites},
pages = {360--365},
title = {{Design Allowables}},
volume = {21},
year = {2001}
}
@article{Evert2006,
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Evert, Ray F},
doi = {10.1002/0470047380.indauth},
eprint = {arXiv:1011.1669v3},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Zienkiewicz FEM - Vol 1 Basics Fundamentals/63205{\_}aindx.pdf:pdf},
isbn = {9780470047385},
issn = {15672719},
journal = {Esau's Plant Anat.},
pages = {541--566},
pmid = {20348824},
title = {{Author Index}},
url = {http://dx.doi.org/10.1002/0470047380.indauth},
year = {2006}
}
@article{Space1996,
author = {Space, On},
journal = {Imagine},
keywords = {component fit,model functions,normal distribution,odf analysis},
number = {C},
pages = {77--96},
title = {{On Space}},
volume = {10},
year = {1996}
}
@article{Liu1972a,
author = {Liu, I Shih and M{\"{u}}ller, Ingo},
doi = {10.1007/BF00250689},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Thermodynamik/Liu{\_}Entropieprinzip{\_}Lagrange/On the Thermodynamics and Thermostatics of Fluid in Electromagnetic Fields {\_}Liu.pdf:pdf},
issn = {00039527},
journal = {Arch. Ration. Mech. Anal.},
number = {2},
pages = {149--176},
title = {{On the thermodynamics and thermostatics of fluids in electromagnetic fields}},
volume = {46},
year = {1972}
}
@article{Guerra-Rosa1984,
abstract = {Monotonic and cyclic plastic zone sizes were measured in a medium strength ferrite-pearlite steel (BM 45) tested in fatigue at 25 Hz at room temperature. Two methods were applied: microhardness and the recently developed 'fatigue in compression' technique. The results obtained are discussed in terms of accuracy and reliability. The retardation effect due to overloads was also studied in the same material and is illustrated experimentally as a da dN vs $\Delta$K curve. This effect emphasizes the importance of an accurate evaluation of both the size and shape of the overall plastic zone. The shape and dimensions of the cyclic plastic zones seem to indicate that in ductile metals the steady state of fatigue crack growth occurs under plane strain conditions. {\textcopyright} 1984.},
author = {Guerra-Rosa, L. and {Moura Branco}, C. and Radon, J. C.},
doi = {10.1016/0142-1123(84)90004-5},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/1984{\_}Guerra-Rosa{\_}Monotonic and cyclic crack tip plasticity - a theory for a combination of HCF and load peaks.pdf:pdf},
issn = {01421123},
journal = {Int. J. Fatigue},
keywords = {fatigue,fatigue in compression,ferrite-pearlite steels,microhardness,plastic zone characteristics},
number = {1},
pages = {17--24},
title = {{Monotonic and cyclic crack tip plasticity}},
volume = {6},
year = {1984}
}
@article{Hauptteil,
author = {Hauptteil, Der and Technik, Rem-kl and Mikroskopie, Rem-kl and Vordergrund, Im and Mikroskopie, Kl- and Untersuchungen, Dynamische Rem-kl and Cdte, Mit and Bestandteil, Wichtiger and Versetzungen, Material},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/Crystall Plasticity Basics/Beitrag{\_}zur{\_}Versetzungsdynamik.pdf:pdf},
pages = {59--89},
title = {{Untersuchungen zur Versetzungsdynamik}}
}
@article{McEvily1991,
abstract = {The behavior of short fatigue cracks cannot be analysed by linear elastic methods because of large scale plasticity effects as well as a breakdown in the stress intensity factor correlation of fatigue crack growth rates for crack sizes less than a millimeter in length. In the present paper a number of modifications are introduced to the linear elastic approach to establish a new parameter which is capable of correlating both long crack and short crack fatigue crack growth data. These modifications include the use of a material constant, re; an allowance for large scale plasticity effects; allowance for the development of crack closure; and the incorporation of the fatigue crack growth threshold. The new parameter is used with reasonable success in calculating fatigue crack growth behavior of short cracks in notched and unnotched specimens, and comparing with experimental data. In addition the analysis leads to a rationale for the dependence of the stress amplitude at the endurance level on the mean stress in a manner consistent with Gerber's parabolic relationship.},
author = {McEvily, A J and Eifler, D and Macherauch, E},
doi = {10.1016/0013-7944(91)90151-P},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/1991{\_}McEvily{\_}An analysis of the growth of short fatigue cracks.pdf:pdf},
issn = {00137944},
journal = {Eng. Fract. Mech.},
number = {3},
pages = {571--584},
title = {{An analysis of the growth of short fatigue cracks}},
url = {http://www.sciencedirect.com/science/article/pii/001379449190151P},
volume = {40},
year = {1991}
}
@article{Wang2014,
author = {Wang, Cong and Shang, De Guang and Wang, Xiao Wei},
doi = {10.1007/s11665-014-1335-7},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Empirical Fatigue Models + Validation/2014{\_}Wang{\_}7075-T651 Models and validation.pdf:pdf},
isbn = {1059-9495},
issn = {15441024},
journal = {J. Mater. Eng. Perform.},
keywords = {critical plane,high-cycle fatigue,life prediction,maximum shear stress (MSS),multsiaxial fatigue},
number = {2},
pages = {816--824},
title = {{A New Multiaxial High-Cycle Fatigue Criterion Based on the Critical Plane for Ductile and Brittle Materials}},
volume = {24},
year = {2014}
}
@article{Temperaturgradienten,
author = {Temperaturgradienten, Nicht and Wellenl, Diese and Auffinden, Das and Abschnitt, Im},
title = {{W ¨ armestrahlung}}
}
@article{Zeit,
author = {Zeit, Zur and Gegensatz, Im and Anteil, Der and Unit, Electronic Control},
pages = {307--322},
title = {{14 Parkassistent}}
}
@article{Winkler2014c,
author = {Winkler, N},
doi = {10.1177/1468087414544899},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2015{\_}Winkler{\_}Effect of pressure oscillations on in-cylinder heat transfer  - through LES Simulation.pdf:pdf},
isbn = {1468087414544},
issn = {1468-0874},
journal = {Int. J. Engine Res.},
keywords = {24 june 2014,6 march 2014,accepted,computational fluid dynamics,date received,heat transfer,internal combustion engines,large eddy simulation,pressure oscillations},
number = {6},
pages = {705--715},
title = {{Effect of pressure oscillations on in-cylinder heat transfer - through large eddy simulation}},
url = {http://jer.sagepub.com/lookup/doi/10.1177/1468087414544899},
volume = {16},
year = {2014}
}
@article{Funktion,
author = {Funktion, Die and Wie, Beispiele and Ausdruck, Der},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Mathematik/Differentation im Komplexen{\_}Quelle TU Darmstadt.pdf:pdf},
pages = {3--9},
title = {{1 1.1 Differentiation im Komplexen}}
}
@article{Rojas2016,
abstract = {? 2016 by the authors; licensee MDPI, Basel, Switzerland.The viscoelastic response of pure Al and 7075 (AlZnMg) and 2024 (AlCuMg) alloys, obtained with a dynamic-mechanical analyzer (DMA), is studied. The purpose is to identify relationships between the viscoelasticity and fatigue response of these materials, of great interest for structural applications, in view of their mutual dependence on intrinsic microstructural effects associated with internal friction. The objective is to investigate the influence of dynamic loading frequency and temperature on fatigue, based on their effect on the viscoelastic behavior. This research suggests that the decrease of yield and fatigue behavior reported for Al alloys as temperature increases may be associated with the increase of internal friction. Furthermore, materials subjected to dynamic loading below a given threshold frequency exhibit a static-like response, such that creep mechanisms dominate and fatigue effects are negligible. In this work, an alternative procedure to the time-consuming fatigue tests is proposed to estimate this threshold frequency, based on the frequency dependence of the initial decrease of the storage modulus with temperature, obtained from the relatively short DMA tests. This allows for a fast estimation of the threshold frequency. The frequencies obtained for pure Al and 2024 and 7075 alloys are 0.001-0.005, 0.006 and 0.075-0.350 Hz, respectively.},
author = {Rojas, J.I. and Crespo, D.},
doi = {10.3390/met6030050},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Surface effects + Frequency effects/Frequency effect regarding EModulus and fatigue of some aluminium alloys .pdf:pdf},
issn = {20754701},
journal = {Metals (Basel).},
keywords = {[AlCuMg, Aluminum alloys, AlZnMg, Dynamic-mechanic},
number = {3},
pages = {1--13},
title = {{Onset frequency of fatigue effects in pure aluminum and 7075 (AlznMg) and 2024 (AlCuMg) alloys}},
volume = {6},
year = {2016}
}
@article{DeBellis2016,
abstract = {It is widely recognized that spatial and temporal evolution of both macro- and micro- turbulent scales inside internal combustion engines affect air-fuel mixing, combustion and pollutants formation. Particularly, in spark ignition engines, tumbling macro-structure induces the generation of a proper turbulence level to sustain the development and propagation of the flame front.As known, 3D-CFD codes are able to describe the evolution of the in-cylinder flow and turbulence fields with good accuracy, although a high computational effort is required. For this reason, only a limited set of operating conditions is usually investigated. On the other hand, thanks to a lower computational burden, 1D codes can be employed to study engine performance in the whole operating domain, despite of a less detailed description of in-cylinder processes. The integration of 1D and 3D approaches appears hence a promising path to combine the advantages of both.In the present paper, a 0D phenomenological mean flow and turbulence model belonging to the K-k model family is presented in detail. The latter is implemented in the GT-Power™ software under the form of “user routine”. The model is tuned against in-cylinder results provided by 3D-CFD analyses carried out by the Star-CD™ code at two engine speeds under motored operation. In particular, a currently produced twin-cylinder turbocharged VVA engine is analyzed. The 0D model is then validated against further 3D results at various engine speeds and intake valve lifts, including early closure strategies, both under motored and fired operation.The proposed 0D mean flow and turbulence model shows the capability to accurately estimate the temporal evolution of the incylinder turbulence for all the considered operating conditions, without requiring any case-dependent tuning, proving its generality and reliability.},
author = {{De Bellis}, Vincenzo and Bozza, Fabio and Fontanesi, Stefano and Severi, Elena and Berni, Fabio},
doi = {https://doi.org/10.4271/2016-01-0545},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Injection+Combustion+Ignitionsystems/2016{\_}DeBellis{\_}Development of a Phenomenological Turbulence Model through a hierarchical 1D-3D approach applied to a VVA Turbocharged engine.pdf:pdf},
journal = {SAE Int. J. Engines},
month = {apr},
number = {1},
pages = {506--519},
title = {{Development of a Phenomenological Turbulence Model through a Hierarchical 1D/3D Approach Applied to a VVA Turbocharged Engine}},
volume = {9},
year = {2016}
}
@article{Nitsche2006,
author = {Nitsche, Wolfgang and Brunn, Andr{\'{e}}},
isbn = {3540209905},
journal = {Str{\"{o}}mungsmesstechnik},
pages = {7--40},
title = {{Druckmessung}},
volume = {6},
year = {2006}
}
@article{Jammoussi2017,
author = {Jammoussi, Hassene and Makki, Imad and Kluzner, Michael and Jentz, Robert},
doi = {10.4271/2017-01-1684},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Thermal Coating + Water Heat Transfer + Applikation/2017{\_}Jammoussi+Makki{\_}Diagnostics of Individual Air Fuel Ratio Cylinder Imbalance.pdf:pdf},
journal = {SAE Int. J. Passeng. Cars},
number = {2},
title = {{Diagnostics of Individual Air Fuel Ratio Cylinder Imbalance}},
volume = {10},
year = {2017}
}
@article{Ashby1979,
author = {Ashby, M F and Gandhi, C and Taplin, D M R},
doi = {https://doi.org/10.1016/0001-6160(79)90105-6},
issn = {0001-6160},
journal = {Acta Metall.},
number = {5},
pages = {699--729},
title = {{Overview No. 3 Fracture-mechanism maps and their construction for f.c.c. metals and alloys}},
url = {http://www.sciencedirect.com/science/article/pii/0001616079901056},
volume = {27},
year = {1979}
}
@article{Chemisky2013,
author = {Chemisky, Yves and Meraghni, Fodil},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/Micromechanics formulas{\_}Overview{\_}EshelbyHillAndMore.pdf:pdf},
journal = {Presentations},
title = {{Micromechanics based on the Eshelby solution : Concepts and formulas}},
year = {2013}
}
@article{Tanaka1982,
abstract = {The dislocation dipole accumulation model for fatigue crack initiation previously proposed by the authors is extended to an analysis of the fatigue strength reduction due to inclusions in high strength alloys. The initiation of a fatigue crack is determined by an energy criterion under the assumption that the crack initiation takes place when the self strain energy of dislocation dipoles accumulated at the damaged part in the material reaches a critical value. Explicit formulae for the crack initiation criterion in several cases are derived as functions of the applied stress, the inclusion size, the slip band shape, and the shear moduli of the inclusion and matrix. The following three types of fatigue crack initiation at inclusions are considered: the slip-band crack emanating from a debonded inclusion, the inclusion cracking due to impinging of slip bands, and the slip-band crack emanating from an uncracked inclusion. The first mechanism was reported to be operative in high strength steels, while the last two mechanisms were reported in high strength aluminum alloys. The present theoretical results are in good agreement with the experimental data published for each case of fatigue crack initiation at inclusions.},
author = {Tanaka, K and Mura, T},
doi = {10.1007/BF02642422},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/1981{\_}Mura+Tanaka{\_}A Theory of fatigue crack initiation at inclusions.pdf:pdf},
isbn = {0360-2133},
issn = {03602133},
journal = {Met. Trans. A},
number = {1},
pages = {117--123},
title = {{A theory of fatigue crack initiation at inclusions}},
volume = {13},
year = {1982}
}
@article{Hild2015a,
abstract = {{\{}{\textcopyright}{\}} Springer Science+Business Media New York 2015.This chapter is devoted to the evaluation of damage with digital image correlation (DIC). This measurement technique provides displacement fields that can be used to tune material parameters of damage models. The potential of DIC for identification purposes is illustrated hereafter for simple 1D-type geometries in the context of quasi-brittle and ductile behaviors. Beams and frames as encountered in civil engineering application can be described through damage laws. The localization of damage at single points (lumped damage mechanics) and the resulting damage law can be determined very precisely based on dedicated versions of DIC incorporating the descriptive language of beam theory. At smaller scale, plasterboards (plaster core lined with paper) constitute another example of a structure (rather than a material), which can be described as damageable. Those cases will be analyzed in details.},
author = {Hild, Fran{\c{c}}ois and Roux, St{\'{e}}phane},
doi = {10.1007/978-1-4614-5589-9},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/2015{\_}Sun+Liu{\_}Particel-Debonding modeling of metal-matrix composites.pdf:pdf},
isbn = {9781461455899},
journal = {Handb. Damage Mech. Nano to Macro Scale Mater. Struct.},
pages = {1277--1299},
title = {{Evaluating damage with digital image correlation: b. from physical to mechanical damage}},
year = {2015}
}
@article{Vergleich,
author = {Vergleich, Im},
title = {{2 2.1 Urformen}}
}
@article{Mehrphasensysteme,
author = {Mehrphasensysteme, Verkettete and Stern, Der and Polygon, Der},
title = {{7 Mehrphasensysteme 7.1}}
}
@article{Tensors2003,
author = {Tensors, Tangent-modulus},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Nicholson 2003 - Finite Element Analysis Thermomechanics of Solids/0749{\_}C18.pdf:pdf},
pages = {227--241},
title = {{for Thermomechanical Response of Elastomers}},
year = {2003}
}
@article{Verbrennungsmotoren2012,
author = {Verbrennungsmotoren, Grundlagen},
doi = {10.1007/978-3-8348-1988-8},
isbn = {9783834819888},
pages = {453--478},
title = {{Ph{\{}{\"{a}}{\}}nomenologische Verbrennungsmodelle}},
year = {2012}
}
@article{Wimmer2000d,
abstract = {This paper summarizes the results of several investigations on in-cylinder heat transfer during high-pressure and gas exchange phases as well as heat transfer in the inlet and outlet ports for a number of different engine types (DI Diesel, SI and gaseous fueled engine). The paper contains a comparision of simulation results and experimental data derived from heat flux measurements. Numerical results were obtained from zero-, one- and three-dimensional simulation methods. Time and spatially resolved heat fluxes were measured applying the surface temperature method and special heat flux sensors. The paper also includes an assessment of different sensor types with respect to accuracy and applicability.ER -},
author = {Wimmer, Andreas and Pivec, Robert and Sams, Theodor},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2000{\_}Wimmer{\_}Heat Transfer to the Combustion Cahmber and Port Walls of IC Engines - Measurement and Prediction.pdf:pdf},
number = {724},
title = {{Heat Transfer to the Combustion Chamber and Port Walls of IC Engines - Measurement and Prediction}},
year = {2000}
}
@article{Gurson1977a,
abstract = {Widely used constitutive laws for engineering materials assume plastic incompressibility, and no effect on yield of the hydrostatic component of stress. However, void nucleation and growth (and thus bulk dilatancy) are commonly observed is some processes which are characterized by large local plastic flow, such as ductile fracture.},
author = {Gurson, A L},
doi = {10.1115/1.3443401},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Plasticity models/Continuum Theory of Ductile Rupture by Void Nucleation and  Growth-PartI{\_}ByGurson.pdf:pdf},
isbn = {0094-4289},
issn = {00944289},
journal = {J. Eng. Mater. Technol.},
number = {1},
pages = {2},
title = {{Continuum Theory of Ductile Rupture by Void Nucleation and Growth: Part I—Yield Criteria and Flow Rules for Porous Ductile Media}},
url = {http://materialstechnology.asmedigitalcollection.asme.org/article.aspx?articleid=1422194},
volume = {99},
year = {1977}
}
@article{Darstellunga,
author = {Darstellung, Vektorielle},
title = {{XIV Vektoranalysis}}
}
@article{Niedrig,
author = {Niedrig, H and Sternberg, M},
journal = {H{\"{u}}tte},
pages = {1--289},
title = {{B-Physik}}
}
@article{Systeme2007,
author = {Systeme, Vernetzte},
journal = {Fahrzeuggetriebe},
title = {{13 Elektronische Getriebesteuerung}},
year = {2007}
}
@book{Melorose2015a,
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Melorose, J. and Perroy, R. and Careas, S.},
booktitle = {Statew. Agric. L. Use Baseline 2015},
doi = {10.1017/CBO9781107415324.004},
eprint = {arXiv:1011.1669v3},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/Crystall Plasticity Basics/Hull 2011 - Introduction to Dislocation.pdf:pdf},
isbn = {9788578110796},
issn = {1098-6596},
keywords = {icle},
pmid = {25246403},
title = {{Introduction to dislocations}},
volume = {1},
year = {2015}
}
@article{Zienkiewicz2005,
author = {Zienkiewicz, O.C.},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Zienkiewicz FEM - Vol 3 Fluid Dynamics/63229{\_}pref.pdf:pdf},
journal = {finite Elem. method fluid Dyn.},
pages = {2--3},
title = {{Incom- Pressible or Almost Incompressible}},
year = {2005}
}
@article{Gross2011c,
author = {Gross, Dietmar and Seelig, Thomas},
doi = {10.1007/978-3-642-10196-0},
isbn = {978-3-642-10195-3},
title = {{Bruchmechanik}},
url = {http://link.springer.com/10.1007/978-3-642-10196-0},
year = {2011}
}
@article{Bridier2008a,
abstract = {The purpose of this experimental study is to investigate the micromechanical fatigue behavior, in terms of slip nature and preferential cracking sites, of a commercial ??/??-forged Ti-6Al-4V alloy. Electron backscattering diffraction is extensively used to identify the deformation (prismatic, basal, pyramidal slip) and crack formation modes activated by fatigue at the surface of several hundred primary ?? nodules. Some fatal crack formation sites are also characterized. Cracking in basal planes is identified as the most critical damage mode leading to fracture. An explanation is proposed which involves the resolved shear stress, taking into account the Schmid factor and the normal stress in relation to the elastic anisotropy of the ??-phase. Finally, the spatial distribution of the secondary cracks is analyzed according to the crystallographic textures (macrozones) present on a mesoscopic scale in the Ti-6Al-4V alloy. ?? 2008 Acta Materialia Inc.},
author = {Bridier, F and Villechaise, P and Mendez, J},
doi = {10.1016/j.actamat.2008.04.036},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2008{\_}Villechaise{\_}Slip and fatigue crack formation processes in an titanium alloy in relation to crystallographic texture on different scales.pdf:pdf},
isbn = {1359-6454},
issn = {13596454},
journal = {Acta Mater.},
keywords = {Electron backscattering diffraction,Fatigue,Slip,Texture,Titanium alloys},
number = {15},
pages = {3951--3962},
title = {{Slip and fatigue crack formation processes in an ??/?? titanium alloy in relation to crystallographic texture on different scales}},
volume = {56},
year = {2008}
}
@article{Macha1999a,
abstract = {At present there are several approaches to the prediction of fatigue life of machine elements and structures. create complex states of stress and under such loadings the assumed criteria of multiaxial fatigue play a very important role in the algorithm used for the prediction of fatigue life. From a review of the literature on multiaxial cyclic fatigue it appears that there is no single universal cri- terion for different loading conditions. New mathemat- ical models are sought. Presently, special attention is being paid to energy criteria.1–14 From some uniaxial and multiaxial cyclic fatigue tests it has been concluded that the energy approach appears promising. The aims of this paper are: (i) to review current energy criteria ofmultiaxial fatigue and their proposed algorithms; (ii) to determine the kind of energy which is assumed to control the fatigue process; (iii) to describe simple exper- imental verifications of the theoretical assumptions of the criteria; and (iv) to present those parameters which domi- nate multiaxial fatigue behaviour. A recommendation for the practical use of the procedures by industry will not be given because of a lack of experimental verification on complex shaped and loaded components.},
author = {Macha, E and Sonsino, C M},
doi = {10.1046/j.1460-2695.1999.00220.x},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Empirical Fatigue Models + Validation/Energy based models/Energy criteria of multiaxial  fatigue failure.pdf:pdf},
issn = {8756758X},
journal = {Fatigue Fract. Eng. Mater. Struct.},
keywords = {and low-cycle fatigue,critical plane,effect of mean stresses,high-,hysteresis loops,proportional and non-proportional loading,strain energy density},
number = {12},
pages = {1053--1070},
title = {{Energy criteria of multiaxial fatigue failure}},
volume = {22},
year = {1999}
}
@article{Morris1978,
author = {Morris, W. L.},
doi = {10.1007/BF02652263},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/1978{\_}Morris{\_}The effect of IMP and microstructure on fatigue crack initiation in AL2219.pdf:pdf},
issn = {03602133},
journal = {Metall. Trans. A},
number = {9},
pages = {1345--1348},
title = {{The effect of intermetallics composition and microstructure on fatigue crack initiation in AI 2219-T851}},
volume = {9},
year = {1978}
}
@article{Toninel2009,
abstract = {The G-equation model was implemented in the commercial code ANSYS CFX and validated against experimental data in order to successfully simulate turbulent premixed combustion in internal combustion engines. The model is based on the level-set approach. Two transport equations are solved respectively for the G-scalar mean value, representing the local distance function from the time-averaged mean flame front, and its variance, correlated to the turbulent flame brush thickness. The model closure for tracking the flame front is based on an algebraic expression for the turbulent burning velocity.The composition of the reacted mixture is evaluated by coupling the code with flamelet libraries generated with the ANSYS CFX-RIF package by means of a reaction progress variable computed as a function of the G-related quantities. An innovative technique for periodically re-initializing the G-scalar field, in order to enforce geometrical consistency and avoid numerical instabilities, was developed, consisting of a least-square-based interface reconstruction and a minimization of the distance from the discretized flame front.In order to make the code suitable for spark-ignition engine applications the combustion model was coupled with a spark kernel model that simulates the early stages of the ignition process at sub-grid scales. The robustness and accuracy of the level-set approach with moving structured and unstructured meshes were assessed and the parallel performance of the combustion model was optimized in order to deal with large meshes in industrial applications.Validation was carried out by comparing simulations against experimental data for three different test-cases: a steady flame in a slot-burner, a transient spark-ignited premixed combustion in a cylinder with fixed walls and optical access and a spark-ignition research engine with flat head and flat piston.The results show good numerical properties and other attractive features in terms of geometrical description of the flame front and coupling with sub-models for detailed chemistry and spark-ignition.},
author = {Toninel, Stefano and Forkel, Hendrik and Frank, Thomas and Durst, Bodo and Hasse, Christian and Linse, Dirk},
doi = {https://doi.org/10.4271/2009-01-0709},
journal = {SAE Int. J. Engines},
month = {apr},
number = {1},
pages = {674--690},
title = {{Implementation and Validation of the G-equation Model Coupled with Flamelet Libraries for Simulating Premixed Combustion in I.C. Engines}},
volume = {2},
year = {2009}
}
@article{Shudo2000,
author = {Shudo, Toshio and Nakajima, Yasuo and Futakuchi, Takayuki},
doi = {https://doi.org/10.1016/S0389-4304(99)00091-0},
file = {:C$\backslash$:/Users/p327208/Desktop/Promotion/Literature/Motorspezifisch/Heat Transfer Combustion Chamber/2007{\_}Shudo{\_}Thermal efficiency analysis in a hydrogen premixed combustion engine.pdf:pdf},
journal = {JSAE Rev.},
number = {2},
pages = {177--182},
title = {{Thermal efficiency analysis in a hydrogen premixed combustion engine}},
volume = {21},
year = {2000}
}
@article{Stiller2006b,
author = {Stiller, Christoph},
file = {:C$\backslash$:/Users/p327208/Desktop/Promotion/Literature/Vorlesungen/Messtechnik+Regelungstechnik/gmrt{\_}buch0801.pdf:pdf},
issn = {02731177},
journal = {Adv. Sp. Res.},
number = {12},
pages = {2820--2823},
title = {{Grundlagen der Mess- und Regelungstechnik}},
volume = {38},
year = {2006}
}
@article{Leichtbaustruktur,
author = {Leichtbaustruktur, Eine and Zuverl, Forderung and Bewertung, Zur and Bewertung, Die and Weiteren, Im},
pages = {370--378},
title = {{25 Strukturzuverl{\"{a}}ssigkeit}}
}
@article{Depcik2002b,
abstract = {In this paper, the available correlations proposed in the literature for the gas-side heat transfer in the intake and exhaust system of a spark-ignition internal combustion engine were surveyed. It was noticed that theseAB - {\textless}inline-graphic xlink:href="2002-01-0372{\_}fig0001" xmlns:xlink="http://www.w3.org/1999/xlink"/{\textgreater}AB - only by empirically fitted constants. This similarity provided the impetus for the authors to explore if a universal correlation could be developed. Based on a scaling approach using microscales of turbulence, the authors have fixed the exponential factor on the Reynolds number and thus reduced the number of adjustable coefficients to just one; the latter can be determined from a least squares curve-fit of available experimental data. Using intake and exhaust side data, it was shown that the universal correlationAB - {\textless}inline-graphic xlink:href="2002-01-0372{\_}fig0002" xmlns:xlink="http://www.w3.org/1999/xlink"/{\textgreater}AB - The correlation coefficient of this proposed heat transfer model with all available experimental data is 0.845 for the intake side and 0.800 for the exhaust side.ER -},
author = {Depcik, Christopher and Assanis, Dennis},
doi = {10.4271/2002-01-0372},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2002{\_}Depcik{\_}A Universal Heat Transfer Correlation for intake and exhaust flows in an SI internal combustion engine.pdf:pdf},
journal = {SAE Pap.},
number = {January 2016},
title = {{A Universal Heat Transfer Correlation for Intake and Exhaust Flows in an Spark-Ignition Internal Combustion Engine}},
url = {http://papers.sae.org/2002-01-0372},
volume = {2002-01-03},
year = {2002}
}
@inproceedings{Anantharaman2015,
author = {Anantharaman, Srinivas and Baskaran, Manoj},
booktitle = {SAE Tech. Pap. 2015-01-2791},
doi = {10.4271/2015-01-2791},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Heat Transfer Combustion Chamber/2015{\_}Anantharaman{\_}A Research on Factors Affecting Nozzle Tip Temperature in Diesel Engines.pdf:pdf},
publisher = {SAE international},
title = {{A Research on Factors Affecting Nozzle Tip Temperature in Diesel Engines}},
year = {2015}
}
@article{Hauptteila,
author = {Hauptteil, Der and Technik, Rem-kl and Mikroskopie, Rem-kl and Vordergrund, Im and Mikroskopie, Kl- and Untersuchungen, Dynamische Rem-kl and Cdte, Mit and Bestandteil, Wichtiger and Versetzungen, Material},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/Crystall Plasticity Basics/Beitrag{\_}zur{\_}Versetzungsdynamik.pdf:pdf},
pages = {59--89},
title = {{Untersuchungen zur Versetzungsdynamik}}
}
@article{Leichtbaus,
author = {Leichtbaus, Problemstruktur},
journal = {Design},
pages = {3--9},
title = {{2 Problemstruktur des Leichtbaus}}
}
@article{Str,
author = {Str, Ohne},
pages = {1--16},
title = {{1 Einleitung: Bedeutung und Entwicklung der Str¨ omungsmechanik 1.1}}
}
@article{Michl2016a,
abstract = {Due to marked differences of material properties and combustion characteristics between hydrogen and carbon-based fuels, an increased heat flux inside the cylinder of hydrogen-fuelled internal combustion engines occurs. The present study aims for a simulation model that describes the wall heat transfer within the entire range of engine calibration possibilities. Conducted experiments on a hydrogen engine equipped with temperature sensors provide the base for the present study. Using the surface temperature method, highly resolved instantaneous surface heat fluxes can be identified. These measurements are compared with results from published heat transfer models that are originally developed for conventional fuels. As no satisfying result with these models can be obtained for the hydrogen engine, a modified heat transfer model is derived and validated based on the experimental data. Necessary developments on characteristic model features lead to a distinctive model for a hydrogen engine. It is demonstrated that the proposed model attains a consistently high prediction quality for a broad range of engine calibration variabilities.},
author = {Michl, Johannes and Neumann, Jens and Rottengruber, Hermann and Wensing, Michael},
doi = {10.1016/j.applthermaleng.2015.12.062},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Heat Transfer Combustion Chamber/2016{\_}Michl+Neumann{\_}Derivation and validation of a heat transfer model in a hydrogen combustion egnine.pdf:pdf},
issn = {13594311},
journal = {Appl. Therm. Eng.},
keywords = {Heat transfer,Hydrogen,Internal combustion engine,Simulation},
pages = {502--512},
publisher = {Elsevier Ltd},
title = {{Derivation and validation of a heat transfer model in a hydrogen combustion engine}},
volume = {98},
year = {2016}
}
@article{Verwendung,
author = {Verwendung, Funktion},
doi = {10.1007/978-3-8348-8279-0},
isbn = {9783834882790},
pages = {744--764},
title = {{¨ der und Kegelradgetriebe}}
}
@article{Ladungswechsela,
author = {Ladungswechsel, Der},
journal = {Auslegung A Grad. J. Philos.},
pages = {273--295},
title = {{5 Berechnung und Auslegung von Baugruppen}}
}
@article{Chawla2012,
author = {Chawla, Krishan K.},
doi = {10.1007/978-0-387-74365-3_6},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/{\_}buecherSong/HandbookofComposites/I/13{\_}MMC.pdf:pdf},
isbn = {978-0-412-58260-8},
issn = {1531-7331},
journal = {Compos. Mater.},
pages = {197--248},
pmid = {20355882},
title = {{Metal Matrix Composites}},
url = {http://link.springer.com/10.1007/978-0-387-74365-3{\_}6},
year = {2012}
}
@article{Wallentowitz2006a,
author = {Wallentowitz, Henning and Reif, Konrad},
doi = {10.1007/978-3-8348-9121-1_11},
journal = {Handb. Kraftfahrzeugelektronik - Grundlagen, Kompon. Syst. Anwendungen},
title = {{Sensorik}},
url = {http://www.springerlink.com/index/10.1007/978-3-8348-9121-1{\%}7B{\_}{\%}7D11},
year = {2006}
}
@misc{AshbyDefo,
author = {Frost, Harold J and Ashby, Michael F},
title = {{Deformation-Mechanism Maps - The Plasticity and Creep of Metals and Ceramics}},
url = {http://engineering.dartmouth.edu/defmech/},
urldate = {2017-06-10}
}
@article{Motion,
author = {Motion, Thermally Assisted and Obstacles, Penetrable and Stre, D-solut I O N and Ng, Ngtheni},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Surface effects + Frequency effects/Bulatov - 2006 - Computer simulations of dislocations.pdf:pdf},
title = {{Series Editors Adrian P . Sutton , FRS Department of Physics , Imperial College London Robert E . Rudd}}
}
@article{Haarlem1999,
author = {van Haarlem, M P},
doi = {10.1007/BFb0104276},
isbn = {978-3-540-65737-8},
journal = {Phys. (College. Park. Md).},
title = {{Scientific Applications of Neural Nets}},
url = {http://www.springerlink.com/index/10.1007/BFb0104276},
volume = {522},
year = {1999}
}
@article{Rousselier1987,
abstract = {Since the pioneering studies conducted by McClintock, Rice and Tracey on the growth of cavities, many studies have covered modelling of ductile fracture; a non-exhaustive list is given of these studies. In the local approach of fracture, the models are used at the tip of cracks, and in the present state, only relatively simple models can be used to solve fracture problems in a complete manner, from material characterization to the analysis of cracked structures. The paper presents two types of models based on a critical ratio of cavity growth or on continuum damage mechanics. In the framework of the local approach of fracture, their possibilities are presented with constant references to experimental validation studies. This allows conclusions to be drawn regarding the effectiveness of the methods proposed and their undeniable contribution to fracture mechanics. ?? 1987.},
author = {Rousselier, G.},
doi = {10.1016/0029-5493(87)90234-2},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Plasticity models/Ductile fracture models and their potential in local approach of fracture{\_}Rousselier.pdf:pdf},
isbn = {00295493},
issn = {00295493},
journal = {Nucl. Eng. Des.},
number = {1},
pages = {97--111},
title = {{Ductile fracture models and their potential in local approach of fracture}},
volume = {105},
year = {1987}
}
@article{EnomotoTemperature1985,
author = {Enomoto, Yoshiteru and Furuhama, Shoichi},
doi = {10.1299/jsme1958.28.108},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Heat Transfer Combustion Chamber/1985{\_}Enomoto{\_}Study on thin film thermocouple measuring instan temperature on surface of combustion chamber wall in ICE - Part1.pdf:pdf},
journal = {Bull. JSME},
number = {235},
pages = {108--116},
title = {{Study on Thin Film Thermocouple for Measuring Instantaneous Temperature on Surface of Combustion Chamber Wall in Internal Combustion Engine}},
volume = {28},
year = {1985}
}
@article{Verbraucher,
author = {Verbraucher, Dem and Gase, Fluide Brennstoffe and Energietransport-, Leitungsgebundene and Wirkungsgrad, Entfernungsspezifischer and Investitionskosten, Spezifische and Betriebskosten, Spezifische and Leckagen, Die and Roh, Die and Tal, Transalpine-pipeline and Druckverlust, Der and Druckabfall, Der},
pages = {311--324},
title = {{17 Energieverteilung, Energiespeicherung 17.1}}
}
@article{Murakami2012c,
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Murakami, Sumio},
doi = {10.1007/978-94-007-2666-6},
eprint = {arXiv:1011.1669v3},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/Continuum Damage Mechanics - SumioMurakami/Kap3{\_}Thermodynamics of Damaged Material.pdf:pdf},
isbn = {978-94-007-2665-9},
issn = {09250042},
pages = {57--76},
pmid = {25246403},
title = {{Continuum Damage Mechanics}},
url = {http://link.springer.com/10.1007/978-94-007-2666-6},
volume = {185},
year = {2012}
}
@article{Reuter2008,
author = {Reuter, Manfred and Zacher, Serge},
doi = {10.1007/978-3-8348-9273-7},
isbn = {978-3-8348-0018-3},
journal = {Anal. Simul. und Entwurf von Regelkreisen},
title = {{Aus dem Programm}},
year = {2008}
}
@article{Germain1983,
abstract = {cp},
author = {Germain, P and Nguyen, Q S and Suquet, P},
doi = {10.1115/1.3167184},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Thermodynamik/1983{\_}Germain{\_}Continuum Thermodynamics.pdf:pdf},
isbn = {9789812835567},
issn = {00218936},
journal = {J. Appl. Mech.},
number = {4b},
pages = {1010},
title = {{Continuum Thermodynamics}},
url = {http://appliedmechanics.asmedigitalcollection.asme.org/article.aspx?articleid=1407311},
volume = {50},
year = {1983}
}
@inproceedings{Uchida2005,
author = {Uchida, Keisuke and Suzuki, Takashi and Oguri, Yasufumi and Yoshida, Masatake},
booktitle = {SAE Tech. Pap. 2005-01-0999},
doi = {https://doi.org/10.4271/2005-01-0999},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Heat transfer intake+exhaust system/2005{\_}Uchida{\_}Precise Measurement of Heat Transfer to the Inlet Air unsing Intake Port Model.pdf:pdf},
publisher = {SAE International},
title = {{Precise Measurement of Heat Transfer to the Inlet Air using Intake Port Model}},
year = {2005}
}
@inproceedings{DeBellis20188II,
author = {Bozza, Fabio and Teodosio, Luigi and {De Bellis}, Vincenzo and Fontanesi, Stefano and Iorio, Agostino},
booktitle = {SAE Tech. Pap. 2018-01-0856},
doi = {10.4271/2018-01-0856},
title = {{Refinement of a 0D Turbulence Model to Predict Tumble and Turbulent Intensity in SI Engines. Part II: Model Concept, Validation and Discussion}},
year = {2018}
}
@article{Gratzer,
author = {Gratzer, Werner and Unfallrekonstruktion, Der},
journal = {Computer (Long. Beach. Calif).},
pages = {193--208},
title = {{A7 A7 Informationsaufnahme beim Kraftfahrer Definitionen A7}}
}
@article{Seifert2010a,
abstract = {In the present paper, predictions of mechanism-based models for cast iron are compared to experimental results obtained for the nodular cast iron EN-GJS-700, the vermicular cast iron EN-GJV-450 and the lamellar cast iron EN-GJL-250. A strategy is proposed to efficiently identify the model parameters based on isothermal experiments. In particular, complex low cycle fatigue (LCF) tests, tension tests and compression tests are used to adjust the time and temperature dependent cyclic plasticity model. The time and temperature dependent fatigue life prediction model is adjusted to LCF tests. For all investigated cast iron materials, good predictions of thermomechanical fatigue (TMF) tests are possible with the models. Additionally, the location of failure and fatigue life of a thermomechanically loaded double-sided notched specimen are predicted with high accuracy. ?? 2010 Elsevier Ltd. All rights reserved.},
author = {Seifert, T. and Maier, G. and Uihlein, A. and Lang, K. H. and Riedel, H.},
doi = {10.1016/j.ijfatigue.2010.02.005},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/2010{\_}Seiffert+Riedel{\_}Mechanism-based thermomechanical fatigue life prediction of cast iron PartTwo Comparison of model with experiment.pdf:pdf},
isbn = {01421123},
issn = {01421123},
journal = {Int. J. Fatigue},
keywords = {Cast iron,Experimental data,Life prediction,Thermomechanical fatigue},
number = {8},
pages = {1368--1377},
publisher = {Elsevier Ltd},
title = {{Mechanism-based thermomechanical fatigue life prediction of cast iron. Part II: Comparison of model predictions with experiments}},
url = {http://dx.doi.org/10.1016/j.ijfatigue.2010.02.005},
volume = {32},
year = {2010}
}
@article{Nutzen,
author = {Nutzen, Hoher},
pages = {335--348},
title = {{13 Ausblick}}
}
@article{Eq2015,
author = {Eq, Hence and Eqs, Comparing},
pages = {1--5},
title = {{Appendix H}},
year = {2015}
}
@article{Merker,
author = {Merker, G{\"{u}}nter and Schwarz, Christian},
pages = {189--219},
title = {{Schadstoffbildung}}
}
@article{Wallentowitz2006l,
author = {Wallentowitz, Henning and Reif, Konrad},
doi = {10.1007/978-3-8348-9121-1_4},
isbn = {978-3-528-03971-4},
journal = {Handb. Kraftfahrzeugelektronik - Grundlagen, Kompon. Syst. Anwendungen},
title = {{Bordnetz und Vernetzung}},
url = {http://www.springerlink.com/index/10.1007/978-3-8348-9121-1{\_}4},
year = {2006}
}
@book{Rech-,
author = {Rech-, Vorzeichen and Befehle, Diese},
booktitle = {Matrix},
isbn = {4586286322785},
title = {{9 L¨ osung der Aufgaben 9.1}}
}
@book{Murakami2012c,
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Murakami, Sumio},
doi = {10.1007/978-94-007-2666-6},
eprint = {arXiv:1011.1669v3},
isbn = {978-94-007-2665-9},
issn = {09250042},
number = {2},
pages = {15--55},
pmid = {25246403},
title = {{Continuum Damage Mechanics}},
url = {http://link.springer.com/10.1007/978-94-007-2666-6},
volume = {185},
year = {2012}
}
@article{Sangid2011,
abstract = {In this paper, we construct a model for prediction of fatigue crack initiation based on the material's microstructure. In order to do so, the energy of a persistent slip band (PSB) is monitored and an energy balance approach is taken, in which cracks initiate and the material fails due to stress concentration from a PSB (with respect to dislocation motion). These PSBs are able to traverse low-angle grain boundaries (GB), thus belonging to clusters of grains. As a consequence of the ongoing cyclic slip process, the PSBs evolve and interact with high-angle GBs, the result of which leads to dislocation pile-ups, static extrusions in the form of ledges/steps at the GB, stress concentration, and ultimately crack initiation. Hence, this fatigue model is driven by the microstructure, i.e. grain orientations, widely distributed grain sizes, precipitates, PSB-GB interactions, as well as the affect of neighboring grains. The results predict that cracks initiate near twin boundaries from PSBs spanning a single large grain with a favorable orientation or multiple grains connected by low-angle GBs. Excellent agreement is shown between model predictions and experimental data. ?? 2010 Elsevier Ltd. All rights reserved.},
author = {Sangid, Michael D. and Maier, Hans J. and Sehitoglu, Huseyin},
doi = {10.1016/j.ijplas.2010.09.009},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/2011{\_}Sangid{\_}The role of grain boundaries on fatigue crack initiation - An energy approach.pdf:pdf},
isbn = {0749-6419},
issn = {07496419},
journal = {Int. J. Plast.},
keywords = {Energy methods,Fatigue,Grain boundaries,Persistent slip bands,Polycrystalline material},
number = {5},
pages = {801--821},
publisher = {Elsevier Ltd},
title = {{The role of grain boundaries on fatigue crack initiation - An energy approach}},
url = {http://dx.doi.org/10.1016/j.ijplas.2010.09.009},
volume = {27},
year = {2011}
}
@article{Mughrabi2010a,
abstract = {In the first part, some fundamental issues that have been under discussion for a long time will be revisited, namely the effect of the cyclic slip mode on the fatigue-induced dislocation distributions, the origin and effect of cyclic slip irreversibilities and their relation to fatigue life and, finally, cyclic strain localization and fatigue crack initiation in persistent slip bands. In the second part, some topics that have recently found increasing interest will be discussed such as the cyclic deformation and fatigue behaviour of ultrafine-grained and nanostructured materials and the microstructural mechanisms that govern fatigue life of ductile and high-strength materials in the range of ultrahigh cycle fatigue. Some general conclusions will be drawn. ?? 2010 Published by Elsevier Ltd.},
author = {Mughrabi, Hael},
doi = {10.1016/j.proeng.2010.03.003},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2010{\_}Mughrabi{\_}Fatigue, an everlasting materials problem-still en vogue{\_}FatigueSlipBands-Overview.pdf:pdf},
isbn = {1877-7058},
issn = {18777058},
journal = {Procedia Eng.},
keywords = {Cyclic slip irreversibilities,Cyclic slip mode,Fatigue lives,Microstructural effects,Ultrafine-grained metals,Ultrahigh Cycle Fatigue (UHCF)},
number = {1},
pages = {3--26},
publisher = {Elsevier},
title = {{Fatigue, an everlasting materials problem - Still en vogue}},
url = {http://dx.doi.org/10.1016/j.proeng.2010.03.003},
volume = {2},
year = {2010}
}
@article{Castillo2009,
author = {Castillo, E},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Probabilistic Aspects/A Unified Statistical Methodology for Modeling Fatigue Damage{\_}Castillo/Kap2{\_}S-N or W{\"{o}}hler Field Models.pdf:pdf},
title = {{S-N or W ¨ ohler Field}},
year = {2009}
}
@book{Qu2007a,
abstract = {The complete primer to micromechanics{\$}\backslash{\$}n{\$}\backslash{\$}n{\$}\backslash{\$}nFundamentals of Micromechanics of Solids is the first book integrating various approaches in micromechanics into a unified mathematical framework, complete with coverage of both linear and nonlinear behaviors. Based on this unified framework, results from the authors' own research, as well as existing results in the literature are re-derived in a logical, pedagogical, and understandable approach. It enables readers to follow the various developments of micromechanics theories and quickly understand its wide range of applications of micromechanics.{\$}\backslash{\$}n{\$}\backslash{\$}nThis helpful guide is a powerful tool for learning the most fundamental ideas and approaches, basic concepts, principles, and methodologies of micromechanics. Readers will find:{\$}\backslash{\$}n* Vigorous derivations of the mathematical framework{\$}\backslash{\$}n* Introductions to both linear and nonlinear material behavior{\$}\backslash{\$}n* Unique coverage of brittle damage, shape memory alloys, and TRIP steels{\$}\backslash{\$}n* Large numbers of problems and exercises to support teaching and learning the concepts{\$}\backslash{\$}n* Lists of references and suggested readings in each chapter},
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Qu, Jianmin and Cherkaoui, Mohammed},
booktitle = {Fundam. Micromechanics Solids},
doi = {10.1002/9780470117835},
eprint = {arXiv:1011.1669v3},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/Strukturmechanik MMS/Literatur/Mikromechanik{\_}B{\"{u}}cher{\_}Literaturvorschlag{\_}MMS/Qu 2006 Micromechanics.pdf:pdf},
isbn = {0471464511},
issn = {16137736},
pages = {1--386},
pmid = {21972053},
title = {{Fundamentals of Micromechanics of Solidss}},
year = {2007}
}
@article{Moscatelli2017,
author = {Moscatelli, D and Sponchioni, M},
doi = {10.1016/B978-0-08-100262-9.00012-4},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/{\_}buecherSong/HandbookofComposites/I/12{\_}SandwichConstruction.pdf:pdf},
isbn = {9780081002629},
title = {12 12.1},
year = {2017}
}
@article{Aslan2010a,
author = {Aslan, Ozgur},
title = {{Numerical modeling of fatigue crack growth in single crystal nickel based superalloys Ozgur Aslan l ' {\{}{\'{E}}{\}}cole nationale sup{\{}{\'{e}}{\}}rieure des mines de Paris Sp{\{}{\'{e}}{\}}cialit{\{}{\'{e}}{\}} « Sciences et G{\{}{\'{e}}{\}}nie des Mat{\{}{\'{e}}{\}}riaux » Simulation num{\{}{\'{e}}{\}}rique de la fissuration par fat}},
year = {2010}
}
@article{Amara1994a,
abstract = {LES VARIATIONS RAPIDES DE PRESSION ET DE TEMPERATURE INFLUENT CONSIDERABLEMENT SUR LES ECHANGES THERMIQUES INSTANTANES ENTRE LE GAZ ET LES PAROIS DE LA CHAMBRE DE COMBUSTION. UNE ETUDE EXPERIMENTALE DE LA DENSITE SURFACIQUE DU FLUX DE CHALEUR ECHANGE EN DEUX POINTS DE LA PAROI DE LA CULASSE A PERMIS EN EFFET DE METTRE EN EVIDENCE L'ACCUMULATION D'ENERGIE DANS LA COUCHE LIMITE THERMIQUE QUI SE MANIFESTE PAR UN DEPHASAGE TEMPOREL ENTRE LE FLUX ET L'ECART DE TEMPERATURE GLOBAL GAZ-PAROI. EN REGIME LAMINAIRE INSTATIONNAIRE, UNE SIMULATION DE CES ECHANGES FAIT BIEN APPARAITRE DES EXTREMA LOCAUX DE TEMPERATURE DANS LA COUCHE LIMITE THERMIQUE. UNE INTERPRETATION DU MECANISME DE FORMATION ET DE DEPLACEMENT DE CES EXTREMA EST DONNEE. LES ECHANGES THERMIQUES EN REGIME TURBULENT SONT DECRITS A L'AIDE DU MODELE MONODIMENSIONNEL DE YANG ET MARTIN OU L'EFFET DE LA TURBULENCE EST PRIS EN COMPTE PAR LE BIAIS DE LA CONDUCTIVITE THERMIQUE TURBULENTE. CE MODELE A ETE MODIFIE POUR LIMITER L'AUGMENTATION DE LA CONDUCTIVITE THERMIQUE TURBULENTE AVEC LA DISTANCE A LA PAROI. LE PARAMETRE DE LIMITATION EST LIE A LA VALEUR LOCALE DE LA VISCOSITE TURBULENTE. LE MODELE AINSI OBTENU PERMET UNE MEILLEURE DETERMINATION DE L'EPAISSEUR DE LA COUCHE LIMITE THERMIQUE ET S'ADAPTE DE LUI-MEME A TOUTE SITUATION INTERMEDIAIRE ENTRE LE REGIME LAMINAIRE ET LES REGIMES FORTEMENT TURBULENTS, LA DENSITE DU FLUX DE CHALEUR ETANT MODULEE EN CONSEQUENCE. L'IMPLANTATION DE CE MODELE DANS LE CODE DE SIMULATION KIVA2 A MONTRE QUE LA PRISE EN COMPTE DES INSTATIONNARITES DE TEMPERATURE ET DE PRESSION CONSTITUE UNE AMELIORATION PAR RAPPORT AUX LOIS DE PAROI LOGARITHMIQUES MAIS SE REVELE INSUFFISANTE. UNE SUPERPOSITION DU MODELE MONODIMENSIONNEL ET D'UNE LOI DE PAROI LOGARITHMIQUE RENDANT COMPTE DE L'EFFET DE LA VITESSE TANGENTIELLE DONNE DES RESULTATS SE RAPPROCHANT AU MIEUX DES EVOLUTIONS EXPERIMENTALES ET CECI POUR DIFFERENTES VITESSES DE ROTATION. UNE ETUDE PARAMETRIQUE COMPARATIVE EST ENSUITE REALISEE POUR MONTRER L'IMPACT DU CHOIX D'UN MODELE DE CALCUL DU FLUX DE CHALEUR PARIETAL SUR LA DETERMINATION DES CHAMPS DE VITESSE, DE TEMPERATURE, D'ENERGIE CINETIQUE TURBULENTE ET DE SON TAUX DE DISSIPATION A LA FIN DE LA COURSE DE COMPRESSION.},
author = {Amara, S},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Heat Transfer Combustion Chamber/1994{\_}Amara{\_}Elaboration et validation dun modele de transferts thermiques dun moteur{\_}UebersichtWaermeuebergangsmodelle.pdf:pdf},
keywords = {Chambre de combustion,Cin{\{}{\'{e}}{\}}tique turbulente,R{\{}{\'{e}}{\}}gime laminaire},
publisher = {{\{}{\'{E}}{\}}cole centrale de Lyon},
title = {{Elaboration et validation d'un mod{\{}{\`{e}}{\}}le de transferts thermiques instationnaires gaz paroi dans la chambre de combustion d'un moteur}},
url = {http://cat.inist.fr/?aModele=afficheN{\%}7B{\&}{\%}7Dcpsidt=162697},
year = {1994}
}
@article{Forster2013,
author = {Forster, Caroline},
doi = {10.1007/978-3-642-24303-5},
isbn = {9783642243035},
pages = {1--8},
title = {{Kapitel 16:}},
year = {2013}
}
@misc{Mura1982,
author = {Mura, Toshio},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/Strukturmechanik MMS/Literatur/Mikromechanik{\_}B{\"{u}}cher{\_}Literaturvorschlag{\_}MMS/Mura 1987 Micromechanics of defects in solids.pdf:pdf},
title = {{Mechanics of elastic and inelastic solids}},
year = {1982}
}
@article{Grosskreutz1971a,
abstract = {Fatigue crack initiation Fatigue crack growth},
author = {Grosskreutz, J. G.},
doi = {10.1002/pssb.2220470202},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/1971{\_}Grosskreutz{\_}The Mechanisms of metal fatigue.pdf:pdf},
isbn = {0370-1972},
issn = {15213951},
journal = {Phys. Status Solidi},
number = {2},
pages = {359--396},
title = {{The mechanisms of metal fatigue (II)}},
volume = {47},
year = {1971}
}
@article{Protons2006,
author = {Protons, Ruhmasse and Neutrons, Ruhmasse and Elektrons, Ruhmasse and Ladung, Spezifische and Elektrons, Ruhenergie and Masseneinheit, Atomare},
doi = {10.1007/3-540-29973-4},
isbn = {3-540-25421-8},
journal = {Gerthsen Phys.},
title = {{Front Matter}},
year = {2006}
}
@article{Meister2011e,
abstract = {Die wichtigsten Verfahren zur numerischen L{\{}{\"{o}}{\}}sung von linearen Gleichungssystemen in einer umfassenden Einf{\{}{\"{u}}{\}}hrung, die zum Verst{\{}{\"{a}}{\}}ndnis nur geringe mathematische Vorkenntnisse ben{\{}{\"{o}}{\}}tigt. Behandelt werden sowohl die direkten als auch die iterativen Verfahren, wobei der Autor gro{\{}{\ss}{\}}en Wert auf eine sorgf{\{}{\"{a}}{\}}ltige Herleitung dieser Verfahren legt. Au{\{}{\ss}{\}}erdem sind sehr detaillierte Pseudocodes enthalten, mit deren Hilfe sich die jeweiligen Verfahren in einer beliebigen Programmiersprache sofort auf dem Computer realisieren lassen. Das Lehrbuch ist auch f{\{}{\"{u}}{\}}r Natur- und Ingenieurwissenschaftler geeignet, die in vielen praktischen Anwendungen mit der L{\{}{\"{o}}{\}}sung von linearen Gleichungssystemen konfrontiert sind.},
archivePrefix = {arXiv},
arxivId = {1011.1669v3},
author = {Meister, Andreas},
doi = {10.1007/978-3-8348-8100-7},
eprint = {1011.1669v3},
isbn = {978-3-8348-1550-7},
issn = {1098-6596},
journal = {Matrix},
pages = {36--68},
pmid = {25246403},
title = {{Numerik linearer Gleichungssysteme}},
url = {http://link.springer.com/10.1007/978-3-8348-8100-7},
year = {2011}
}
@article{Pan2014c,
abstract = {Knocking combustion in spark-ignition (SI) engines is a typical abnormal combustion phenomenon that severely limits engine performance and thermal efficiency. However, its mechanism has not so far been completely revealed, such as the origin of pressure oscillation with tremendous amplitude and broken mechanisms of the engine body when knock occurs. This article systematically reviews the series of physical and chemical phenomena involved in knocking combustion, including auto-ignition, gas-dynamic waves, cavity resonance, and auto-ignited flame propagation. Significant research has shown that the rapid heat release of end-gas auto-ignition and subsequent strong pressure waves play a crucial role during knocking combustion. A methodology of the interaction of flame propagation and pressure waves has been proposed to reveal knock formation in terms of positive feedback between strengthened pressure waves and auto-ignited flame propagation. Also, new suggestions on the weakness in prior research of knocking combustion have also been discussed in the present article. {\{}{\textcopyright}{\}} 2014 Copyright Taylor and Francis Group, LLC.},
author = {Pan, Jiaying and Shu, Gequn and Wei, Haiqiao},
doi = {10.1080/00102202.2013.857665},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2014{\_}Pan+Wei{\_}Interaction of Flame Propagation and Pressure Waves During Knocking Combustion in Spark-Ignition Engines.pdf:pdf},
issn = {0010-2202},
journal = {Combust. Sci. Technol.},
number = {2},
pages = {192--209},
title = {{Interaction of Flame Propagation and Pressure Waves During Knocking Combustion in Spark-Ignition Engines}},
url = {http://www.tandfonline.com/doi/abs/10.1080/00102202.2013.857665},
volume = {186},
year = {2014}
}
@article{Burgg,
author = {Burg, Heinz},
pages = {705--714},
title = {{B9 B9 Unf{\"{a}}lle mit Schienenfahrzeugen B9}}
}
@article{Borgeest2010,
author = {Borgeest, Kai},
doi = {10.1007/978-3-8348-9337-6},
isbn = {978-3-8348-0548-5},
journal = {Elektron. der Fahrzeugtechnik},
pages = {18},
title = {{2 Bordelektrik}},
url = {http://www.springerlink.com/index/10.1007/978-3-8348-9337-6},
year = {2010}
}
@article{Numerical2003,
author = {Numerical, Advanced},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Nicholson 2003 - Finite Element Analysis Thermomechanics of Solids/0749{\_}C20.pdf:pdf},
number = {4},
pages = {257--263},
title = {{Advanced Numerical Methods}},
year = {2003}
}
@article{Morris2007,
author = {Morris, J W},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/Crystall Plasticity Basics/Morris{\_}Dislocation plasticity-AnOverview.pdf:pdf},
journal = {Introd. to Mater. Sci.},
pages = {1--36},
title = {{Dislocation Plasticity : Overview}},
url = {http://www.mse.berkeley.edu/groups/morris/MSE205/Extras/dislocation plasticity.pdf},
volume = {i},
year = {2007}
}
@article{Skerrett1991,
author = {Skerrett, P},
doi = {10.1126/science.252.5009.1064},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Zienkiewicz FEM - Vol 1 Basics Fundamentals/63205{\_}apdxa.pdf:pdf},
isbn = {0521822890},
issn = {0036-8075},
journal = {Science},
number = {5009},
pages = {1064--6},
pmid = {17797900},
title = {{"Matrix algebra" heals life's wounds.}},
url = {http://www.ncbi.nlm.nih.gov/pubmed/20866130},
volume = {252},
year = {1991}
}
@book{Antman2007,
abstract = {This book has been written for undergraduate and graduate students in various areas of mathematics and its applications. It is for students who are willing to get acquainted with Bayesian approach to computational science but not necessarily to go through the full immerson into the statistical analysis. It has also been written for researchers working in areas where mathematical and statistical modeling are of central importance, such as biology and engineering.},
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Antman, S S and Marsden, J E and Sirovich, L},
booktitle = {Uquedusa},
doi = {10.1007/978-4-431-54177-6},
eprint = {arXiv:1011.1669v3},
isbn = {9780387733937},
issn = {1098-6596},
pages = {202},
pmid = {25246403},
title = {{Surveys and Tutorials in the}},
url = {http://books.google.com/books?id=HIG0CRf6msoC},
volume = {2},
year = {2007}
}
@article{Liu1996,
author = {Liu, I S},
doi = {10.1007/s001610050042},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Thermodynamik/Liu{\_}Entropieprinzip{\_}Lagrange/On Entropy Flux Heat Flux Relation in Thermodynamic with Lagrange Multipliers {\_} Liu.pdf:pdf},
issn = {0935-1175},
journal = {Contin. Mech. Thermodyn.},
number = {4},
pages = {247--256},
title = {{On entropy flux heat flux relation in thermodynamics with Lagrange multipliers}},
volume = {8},
year = {1996}
}
@article{Singer1977,
abstract = {The aluminum alloy investigated contained about 2. 7{\{}{\%}{\}} Cu, 1. 6{\{}{\%}{\}} Mg, 1. 1{\{}{\%}{\}} Fe, 1{\{}{\%}{\}} Ni, and small amounts of Si, Zn, and Ti. Creep at 473 K resulted in deformation-induced softening because of microstructural instability. Creep tests at varied stresses and temperatures were performed to explore the dislocation mechanisms during creep in specimens subjected to 13 different thermomechanical treatments. It was found that the room temperature yield stress and creep resistance after prolonged creep stressing can be improved by preliminary deformation, whereas the initial creep resistance is decreased. This is explained in terms of the effect of deformation on the structure and its stability.},
author = {Singer, Robert and Blum, Wolfgang},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Empirical Fatigue Models + Validation/1975{\_}Blum{\_}The influence of thermomechanical treatment on the creep resistance of RR58 - Al2618.pdf:pdf},
issn = {00443093},
journal = {Zeitschrift fuer Met. Res. Adv. Tech.},
number = {5},
title = {{Influence of Thermomechanical Treatments on the Creep Resistance of Rr 58 At Elevated Temperature.}},
volume = {68},
year = {1977}
}
@article{Sanli2008,
author = {Sanli, Ali and Ozsezen, Ahmet N and Kilicaslan, Ibrahim and Canekci, Mustafa},
doi = {https://doi.org/10.1016/j.applthermaleng.2007.10.005},
file = {:C$\backslash$:/Users/p327208/Desktop/Promotion/Literature/Motorspezifisch/Heat Transfer Combustion Chamber/2008{\_}Sanli{\_}The influence of engine speed and load on the heat transfer between gases an incylinder walls at firted and motored conditions.pdf:pdf},
journal = {Appl. Therm. Eng.},
keywords = {heat flux,heat transfer coefficient,idi diesel engine},
pages = {1395--1404},
title = {{The influence of engine speed and load on the heat transfer between gases and in-cylinder walls at fired and motored conditions of an IDI diesel engine}},
volume = {28},
year = {2008}
}
@article{Bungartz2010a,
abstract = {Stra{\ss}enverkehr geht uns alle an, jeder ist davon betroffen. Unsere W{\"{u}}nsche und Vorstellungen bez{\"{u}}glich des Stra{\ss}enverkehrs sind jedoch in der Regel etwas widerspr{\"{u}}chlich: Einerseits wollen wir m{\"{o}}glichst viel davon. Wir wollen mobil sein und so schnell und angenehm wie m{\"{o}}glich von der Wohnung zur Uni oder Arbeit, vom Heimatort zum Ferienziel oder vom Einkaufen zur Freizeitbesch{\"{a}}ftigung gelangen. Wir w{\"{u}}nschen uns dazu gut ausgebaute Stra{\ss}en und Parkpl{\"{a}}tze oder h{\"{a}}ufig fahrenden Personennahverkehr. Andererseits wollen wir m{\"{o}}glichst wenig davon. Stra{\ss}enverkehr soll uns nicht bel{\"{a}}stigen. Wir m{\"{o}}chten nicht im Berufsverkehr oder in den kilometerlangen Mammutstaus zu Ferienbeginn und -ende stehen, w{\"{u}}nschen uns, von L{\"{a}}rm- und Abgasemissionen unbehelligt zu bleiben, und bevorzugen Gr{\"{u}}nstreifen anstelle von Stra{\ss}enasphalt.},
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Bungartz and Zimmer and Buchholz and Pfl{\"{u}}ger},
doi = {10.1515/bmt.2010.712},
eprint = {arXiv:1011.1669v3},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Vorlesungen/Modellbildung{\_}und{\_}Simulation/Skript{\_}Modellbildung{\_}und{\_}Simulation.pdf:pdf},
isbn = {9783642054600},
issn = {0013-5585},
journal = {Biomed. Tech. Eng.},
keywords = {Stichw䣏rter des Dokuments},
number = {s1},
pages = {1--237},
pmid = {14685750},
title = {{Modellbildung und Simulation}},
volume = {55},
year = {2010}
}
@article{Baehr2009,
abstract = {All living beings are, from the thermodynamic point of view, open, well regulated, and optimized systems with considerable internal irreversibilities. However scientific research is mainly based on closed systems. The theory of open systems is very well developed in engineering thermodynamics. Here the concept of "exergy"--the thermodynamic potential related to given surroundings--clearly distinguishes between the two concepts of the word "energy".},
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Baehr, Hans Dieter and Kabelac, Stephan},
doi = {10.1007/978-3-642-00556-5},
eprint = {arXiv:1011.1669v3},
isbn = {9783540325130},
issn = {0028-1042},
journal = {Naturwissenschaften},
keywords = {Animals,Biological,Energy Metabolism,Energy Transfer,Mathematics,Models,Temperature,Thermodynamics},
pages = {335--41},
pmid = {6482977},
title = {{Thermodynamik: Grundlagen und technische Anwendungen}},
url = {http://www.ncbi.nlm.nih.gov/pubmed/1776310{\%}5Cnhttp://www.springerlink.com/index/10.1007/978-3-642-00556-5},
volume = {71},
year = {2009}
}
@article{Polak2014a,
abstract = {Experimental data on the formation of persistent slip markings (PSMs) at the egressing persistent slip bands (PSBs) and physically based models of surface relief formation and fatigue crack initiation are surveyed. The original Pol{\'{a}}k's model of fatigue crack initiation based on the formation, migration and annihilation of vacancy-type defects in PSBs is further refined and extended by taking into consideration the annihilation of vacancies in the matrix and the formation of internal stresses. The proposed mechanisms of surface relief formation are based on the plastic relaxation of internal compression stresses in PSBs and internal tensile stresses in the matrix. By solving the migration of vacancies from the PSB and their annihilation in the matrix, the shapes of extrusion and parallel intrusions are derived analytically under some simplifying assumptions. {\textcopyright} 2013 Elsevier B.V.},
author = {Pol{\'{a}}k, J. and Man, J.},
doi = {10.1016/j.msea.2013.12.005},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/2014{\_}Polak+Man{\_}Mechanisms of extrusion and intrusion formation in fatigued crystalline materials.htm.pdf:pdf},
issn = {09215093},
journal = {Mater. Sci. Eng. A},
keywords = {Crack initiation,Extrusion,Fatigue,Intrusion,Persistent slip band (PSB)},
pages = {15--24},
publisher = {Elsevier},
title = {{Mechanisms of extrusion and intrusion formation in fatigued crystalline materials}},
url = {http://dx.doi.org/10.1016/j.msea.2013.12.005},
volume = {596},
year = {2014}
}
@inproceedings{Fontanesi2013Comb,
abstract = {The paper describes an integrated methodology for the accurate characterization of the thermal behavior of internal combustion engines, with particular reference to a high performance direct injected SI engine for sport car applications. The engine is operated at full load and maximum power revving speed, which is known to be critical from the point of view of thermal stresses on the engine components.In particular, two different sets of 3D-CFD calculations are adopted: on one side, full-cycle in-cylinder analyses are carried out to estimate the point wise thermal heat flux due to combustion on the engine components facing the combustion chamber. On the other side, full-engine multi-region CHT calculations covering the engine coolant jacket and the surrounding metal components are used to compute the point wise temperature distribution within the engine head, liner and block.An iterative procedure is then implemented in order to exchange relevant thermal data between the two modeling frameworks: at first, local gas temperatures and heat transfer coefficients from the in-cylinder simulations are applied as thermal loads to the CHT calculations; then, the resulting surface temperature maps are re-applied to the combustion chamber walls for the subsequent in-cylinder CFD analysis. The procedure is iteratively repeated until convergence is met in terms of thermal characterization of the engine.The procedure takes into account the non-uniform spatial distribution of both thermal loads from the combustion process and resulting temperature distribution on the combustion chamber walls, which are known to be particularly evident when considering direct injected stratified charged engines. The resulting thermal fields are compared to those deriving from a traditional approach for both the in-cylinder and CHT calculations, i.e. the application of uniform heat fluxes on the CHT side and the use of uniform wall temperatures on the in-cylinder side. The resulting differences are highlighted and critically discussed, with particular emphasis on those which could have a relevant impact on both the fatigue strength evaluation of the engine and the arising of local undesired phenomena such as surface ignition and knocking.},
author = {Fontanesi, Stefano and Cicalese, Giuseppe and Tiberi, Alessandro},
booktitle = {SAE 2013 World Congr. Exhib.},
doi = {10.4271/2013-01-1088},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/W{\"{a}}rme-RBen Kolben/2013{\_}Fontanesi{\_}Combined In-cylinder - CHT Analyses for the accurate estimation of the thermal flow field of a high performance engine for sport car applications.pdf:pdf},
month = {apr},
publisher = {SAE International},
title = {{Combined In-cylinder / CHT Analyses for the Accurate Estimation of the Thermal Flow Field of a High Performance Engine for Sport Car Applications}},
year = {2013}
}

@article{Tornau1998,
author = {Tornau, Christian},
doi = {10.1515/9783110934540.261},
isbn = {9783110934540},
pages = {1--10},
title = {{Kapitel 14}},
year = {1998}
}
@article{Fertigungskontrolle,
author = {Fertigungskontrolle, Der},
journal = {Konstruktion},
title = {{11 Synthese und Konstruktion 11.1}}
}

@article{Chen1999,
author = {Chen, Ang and Zhi, Yu and Bao, Yahua},
doi = {10.1088/0953-8984/6/39/012},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/{\_}buecherSong/HandbookofComposites/I/14{\_}CeramicComposites.pdf:pdf},
issn = {0953-8984},
journal = {J. Phys. Condens. Matter},
number = {39},
pages = {7921--7925},
title = {{Ceramic Composites}},
volume = {6},
year = {1999}
}
@article{Motorverhalten,
author = {Motorverhalten, Thermisches},
title = {{8 Gesamtprozessanalyse 8.1}}
}
@article{Carta2013,
abstract = {This paper describes the propagation of an edge crack in a structured thermoelastic solid. A rapid change of temperature, represented by a time-periodic series of high-gradient temperature pulses, is applied at the boundary of the structured solid. A lattice approximation is employed in the model analysis discussed here. In order to describe the crack advance through the lattice a failure criterion is imposed, whereby the links break as soon as they attain a critical elastic elongation. The elongations of the links are produced both by a variation in temperature and by elastic waves generated at the boundary due to thermal shocks, as well as waves created by the propagating crack through the breakage of the elastic ligaments. The analysis is compared to the quasi-static and dynamic models of thermal striping in thermally loaded solids containing edge cracks. The emphasis is on the effect of the structure on the crack trapping. The nonlinear simulations presented in this paper show that the average speed of crack propagation can be estimated from the analysis of the dispersion properties of waves initiated by the crack. Temperature and inertia contributions to crack propagation are also investigated. It is found that inertia amplifies the elongations of the links, and thus influences the crack advance through the structured solid. ?? 2013 Elsevier Ltd. All rights reserved.},
author = {Carta, G and Jones, I S and Brun, M and Movchan, N V and Movchan, A B},
doi = {10.1016/j.ijsolstr.2013.05.001},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/2013{\_}Carta+Jones{\_}Crack propagation induced by thermal shocks in structured media.pdf:pdf},
issn = {00207683},
journal = {Int. J. Solids Struct.},
keywords = {Crack propagation,Elastic lattice,Fracture,Microstructure,Nonlinear dynamic problem,Thermal shock,Thermal striping},
number = {18},
pages = {2725--2736},
publisher = {Elsevier Ltd},
title = {{Crack propagation induced by thermal shocks in structured media}},
url = {http://dx.doi.org/10.1016/j.ijsolstr.2013.05.001},
volume = {50},
year = {2013}
}

@article{Sanli2009,
author = {Sanli, A. and Sayin, C. and Gumus, M. and Kilicaslan, I. and Canakci, M.},
doi = {https://doi.org/10.1080/10407780903244312},
file = {:C$\backslash$:/Users/p327208/Desktop/Promotion/Literature/Motorspezifisch/2009{\_}Sanli{\_}Numerical evaluation by models of load and spark timing effects on the in-cylinder heat transfer of a si engine.pdf:pdf},
journal = {Numer. Heat Transf. Part A Appl.},
number = {5},
pages = {444--458},
title = {{Numerical Evaluation by Models of Load and Spark Timing Effects on the In-Cylinder Heat Transfer of a SI Engine}},
volume = {56},
year = {2009}
}
@article{Rest,
author = {Rest, Der and Zwangskr, Ladungstrennung and Ladungen, Energiezufuhr and Spannung, Elektrische and Spannung, Die and Stromst, Elektrische},
journal = {System},
title = {{2 Gleichstromkreis 2.1}}
}

@book{Murakami2012f,
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Murakami, Sumio},
doi = {10.1007/978-94-007-2666-6},
eprint = {arXiv:1011.1669v3},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/Continuum Damage Mechanics - SumioMurakami/Kap4{\_}Inelastic Constitutive Equation and Damage Evolution Equation of Material with Isotropic Damage.pdf:pdf},
isbn = {978-94-007-2665-9},
issn = {09250042},
pages = {77--110},
pmid = {25246403},
title = {{Continuum Damage Mechanics}},
url = {http://link.springer.com/10.1007/978-94-007-2666-6},
volume = {185},
year = {2012}
}

@article{Microbiol2001,
author = {Microbiol, Food and Prot, Food and Vet, Trinidad J},
isbn = {3870701854},
number = {1991},
pages = {1174--1181},
title = {{9. Literaturverzeichnis}},
volume = {60},
year = {2001}
}
@article{Torsion,
author = {Torsion, Abscheren},
title = {{Sachwortverzeichnis}}
}
@book{HuseyinSehitoglu2000a,
author = {{Huseyin Sehitoglu} and {Hans J. Maier}},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/2000{\_}Huseyin Sehitoglu{\_}Thermo-mechanical Fatigue Behavior of  Materials{\_}OverviewDifferentPapers.pdf:pdf},
isbn = {0803128533},
pages = {151},
title = {{Thermo-mechanical Fatigue Behavior of Materials: Third volume}},
url = {https://books.google.se/books?id=ZY84rIMG82sC{\&}pg=PA150{\&}lpg=PA150{\&}dq=thermomechanical+fatigue+behavior+of+materials{\&}source=bl{\&}ots=93h1yoyJVR{\&}sig=YTp4LbQdi6Kms-Ys06yBsW5LnPU{\&}hl=sv{\&}sa=X{\&}ved=0ahUKEwidx4jg27rKAhVGqHIKHfYeBXoQ6AEIMjAC{\#}v=onepage{\&}q{\&}f=false},
year = {2000}
}
@article{Gingrich2016a,
abstract = {An experimental investigation was conducted to explore the impact in-cylinder pressure oscillations have on piston heat transfer. Two fast-response surface thermocouples embedded in the piston top measured transient temperature and a commercial wireless telemetry system was used to transmit thermocouple signals from the moving piston. Measurements were made in a light-duty single-cylinder research engine operated under low temperature combustion regimes including Homogeneous Charge Compression Ignition (HCCI) and Reactivity Controlled Compression Ignition (RCCI) and Conventional Diesel (CDC). The HCCI data showed a correlated trend of higher heat transfer with increased pressure oscillation strength, while the RCCI and CDC data did not. An extensive HCCI data set was acquired. The heat transfer rate - when corrected for differences in cylinder pressure and gas temperature - was found to positively correlate with increased pressure oscillations. It is important to normalize the data before drawing conclusions as the magnitude of the effect was diminished significantly by the normalization procedure.},
author = {Gingrich, Eric and Janecek, Daniel and Ghandhi, Jaal},
doi = {10.4271/2016-01-9044},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2016{\_}Gingrich{\_}Experimental Investigation of the Impact of In-Cylinder Pressure Oscillations on Piston Heat Transfer.pdf:pdf},
issn = {1946-3944},
journal = {SAE Int. J. Engines},
number = {3},
pages = {2016--01--9044},
title = {{Experimental Investigation of the Impact of In-Cylinder Pressure Oscillations on Piston Heat Transfer}},
url = {http://papers.sae.org/2016-01-9044/},
volume = {9},
year = {2016}
}
@article{Reimer2003,
abstract = {It's sometimes difficult to observe combustion in situ — inside, say, a porous material or an industrial reactor. But with the help of nuclear magnetic resonance, a new vista has opened up.},
author = {Reimer, Jeffrey},
doi = {10.1038/426508a},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Klopfen{\_}Ottomotor/2009{\_}Forte+Corti+Bianchi{\_}Combined experimental and numerical analysis of knock in SI engines.pdf:pdf},
isbn = {9789535108566},
issn = {1476-4687},
journal = {Nature},
number = {December},
pages = {508--509},
pmid = {14654825},
title = {{Internal combustion}},
volume = {426},
year = {2003}
}
@article{Frenz2008,
author = {Frenz, Walter},
doi = {10.1007/978-3-540-71852-9_16},
isbn = {978-3-540-71851-2},
journal = {H{\"{u}}tte},
pages = {P1--P26},
title = {{P-Recht}},
year = {2008}
}
@article{Strc,
author = {Str, Sammelbezeichnung and Energie, Fluid and Wirkungsweise, Die and Bei, Arbeit and Merkmal, Dieses and Beispiel, Am and Fluid, Das and Laufrad, Im and Energie, Laufrad and Leitschaufeln, Die},
pages = {1--41},
title = {{1 Gemeinsame Grundlagen der Str{\"{o}}mungsmaschinen}}
}
@article{Turner1999,
author = {Turner, I M},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Zienkiewicz FEM - Vol 3 Fluid Dynamics/63229{\_}toc.pdf:pdf},
isbn = {0521801834},
journal = {Rain},
pages = {13--16},
title = {{Preface Acknowledgements 1}},
year = {1999}
}
@article{Kreher1996,
author = {Kreher, Wolfgang S.},
doi = {10.1016/S0927-0256(96)00073-0},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Probabilistic Aspects/1996{\_}Kreher{\_}Modeling of random microstructural stresses and grain boundary damage in polycrystals.pdf:pdf},
issn = {09270256},
journal = {Comput. Mater. Sci.},
keywords = {damage,internal stresses,polycrystals,randomness},
number = {1-2},
pages = {147--153},
title = {{Modeling of random microstructural stresses and grain boundary damage in polycrystals}},
url = {http://linkinghub.elsevier.com/retrieve/pii/S0927025696000730},
volume = {7},
year = {1996}
}

@article{Berger2003,
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Berger},
doi = {10.1002/ejoc.201200111},
eprint = {arXiv:1011.1669v3},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Vortraege/Book-of-Abstracts{\_}2016-03-04{\_}GAMM.pdf:pdf},
isbn = {9781107671812},
issn = {0196-6553},
journal = {Eng. Med. Biol. Soc. 2008. EMBS 2008. 30th Annu. Int. Conf. IEEE},
pages = {2004},
pmid = {26840611},
title = {{Table of of contents}},
volume = {24},
year = {2003}
}
@article{Case,
author = {Case, The General and Case, General and Example, Above},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Mathematik/Transformation pdfs.pdf:pdf},
pages = {1--11},
title = {{11 — Transforming Density Functions}},
url = {https://www.cl.cam.ac.uk/teaching/2003/Probability/prob11.pdf}
}
@article{Papulab,
author = {Papula, L},
doi = {10.1007/978-3-8348-8643-9},
isbn = {9783834886439},
journal = {Math. f{\"{u}}r Ingenieure und Naturwissenschaftler Band 2},
title = {{V Fourier-Transformationen 1}}
}
@article{Materials2003,
author = {Materials, Thermoinelastic},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Nicholson 2003 - Finite Element Analysis Thermomechanics of Solids/0749{\_}C19.pdf:pdf},
pages = {243--256},
title = {{Inelastic and Thermoinelastic Materials 19.1}},
volume = {22},
year = {2003}
}
@article{Meister2011e,
abstract = {Die wichtigsten Verfahren zur numerischen L{\"{o}}sung von linearen Gleichungssystemen in einer umfassenden Einf{\"{u}}hrung, die zum Verst{\"{a}}ndnis nur geringe mathematische Vorkenntnisse ben{\"{o}}tigt. Behandelt werden sowohl die direkten als auch die iterativen Verfahren, wobei der Autor gro{\ss}en Wert auf eine sorgf{\"{a}}ltige Herleitung dieser Verfahren legt. Au{\ss}erdem sind sehr detaillierte Pseudocodes enthalten, mit deren Hilfe sich die jeweiligen Verfahren in einer beliebigen Programmiersprache sofort auf dem Computer realisieren lassen. Das Lehrbuch ist auch f{\"{u}}r Natur- und Ingenieurwissenschaftler geeignet, die in vielen praktischen Anwendungen mit der L{\"{o}}sung von linearen Gleichungssystemen konfrontiert sind.},
archivePrefix = {arXiv},
arxivId = {1011.1669v3},
author = {Meister, Andreas},
doi = {10.1007/978-3-8348-8100-7},
eprint = {1011.1669v3},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/Numerik linearer Gleichungssysteme{\_}Andreas Meister/Kapitel2-Grundlagen lineare Algebra.pdf:pdf},
isbn = {978-3-8348-1550-7},
issn = {1098-6596},
journal = {Matrix},
pages = {36--68},
pmid = {25246403},
title = {{Numerik linearer Gleichungssysteme}},
url = {http://link.springer.com/10.1007/978-3-8348-8100-7},
year = {2011}
}
@article{Arnold2000,
author = {Arnold, J{\"{o}}rg and Alleinunf{\"{a}}llen, Bei},
pages = {715--729},
title = {{B10 B10 Alleinunf{\{}{\"{a}}{\}}lle B10}},
year = {2000}
}
@article{Skeist1959,
author = {Skeist, Irving},
doi = {10.1097/00010694-195903000-00018},
isbn = {978-1-4615-7141-4},
journal = {Soil Sci.},
number = {3},
pages = {181},
title = {{Epoxy Resins}},
volume = {87},
year = {1959}
}
@article{Wimmer2000b,
abstract = {This paper summarizes the results of several investigations on in-cylinder heat transfer during high-pressure and gas exchange phases as well as heat transfer in the inlet and outlet ports for a number of different engine types (DI Diesel, SI and gaseous fueled engine). The paper contains a comparision of simulation results and experimental data derived from heat flux measurements. Numerical results were obtained from zero-, one- and three-dimensional simulation methods. Time and spatially resolved heat fluxes were measured applying the surface temperature method and special heat flux sensors. The paper also includes an assessment of different sensor types with respect to accuracy and applicability.ER -},
author = {Wimmer, Andreas and Pivec, Robert and Sams, Theodor},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2000{\_}Wimmer{\_}Heat Transfer to the Combustion Cahmber and Port Walls of IC Engines - Measurement and Prediction.pdf:pdf},
number = {724},
title = {{Heat Transfer to the Combustion Chamber and Port Walls of IC Engines - Measurement and Prediction}},
year = {2000}
}
@article{Hettinger2009a,
abstract = {It is a well known fact that indicated efficiency of a SI engine at WOT is predominantly limited by knock occurrence. Therefore many investigations have been carried out to avoid knocking. Considering the further development of downsized engines knocking will also pose a greater challenge. Not only knocking but also irregular combustion in general will require further investigation in supercharged SI eingines. Premature ignition, for instance, hasn't yet been completely understood and therefore limits the low end torque of supercharged SI engines.The purpose of this paper is to introduce different analysis methods which allow to identify the knock onset and the knocking zones in the combustion chamber. In addition to established methods new techniques have been developed to account for the complex nature of pressure oscillation during knocking combustion.Experimental data was acquired on a single cylinder research engine to validate the methodology using six pressure transducers.},
author = {Hettinger, Alexander and Kulzer, Andr{\'{e}}},
doi = {10.4271/2009-01-0698},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2009{\_}Hettinger+Kulzer{\_}A new method to detect Knocking Zones.pdf:pdf},
isbn = {2009010698},
issn = {1946-3944},
journal = {SAE Int. J. Engines},
number = {1},
pages = {2009--01--0698},
title = {{A New Method to Detect Knocking Zones}},
url = {http://papers.sae.org/2009-01-0698/},
volume = {2},
year = {2009}
}
@article{Ley2012,
author = {Ley, F and Regelungs-, Einordnung Der},
doi = {10.1007/978-3-642-22850-6},
isbn = {9783642228506},
pages = {1--123},
title = {{Regelungs- und Steuerungstechnik}},
year = {2012}
}
@article{Fachausdr,
author = {Fachausdr, Medizinische},
pages = {971--1016},
title = {{D3 Medizinische Fachausdr{\"{u}}cke D3}}
}
@article{Airbag-systeme,
author = {Airbag-systeme, C and Kramer, Florian},
journal = {Thorax},
pages = {775--779},
title = {{C3 Der Airbag als Sicherheitsbestandteil heutiger Automobile C3}}
}
@article{Arbeitsumgebunga,
author = {Arbeitsumgebung, Die},
journal = {Pro-Engineer Prakt.},
title = {{5 Bauteilmodellierung}}
}
@misc{Oppenheim1989,
author = {Oppenheim, A.V. and Schafer, R.W. and Buck, J. R.},
booktitle = {Discret. signal Process.},
keywords = {FFT,Hilbert,Signal processing,filtering},
pages = {870},
title = {{1 -Introduction.Pdf}},
year = {1989}
}
@book{Murakami2012e,
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Murakami, Sumio},
doi = {10.1007/978-94-007-2666-6},
eprint = {arXiv:1011.1669v3},
isbn = {978-94-007-2665-9},
issn = {09250042},
pages = {77--110},
pmid = {25246403},
title = {{Continuum Damage Mechanics}},
url = {http://link.springer.com/10.1007/978-94-007-2666-6},
volume = {185},
year = {2012}
}
@article{Energietechnik,
author = {Energietechnik, Die and Umwandlungswirkungsgrad, Der and Energieinhalt, Gesamter and Energieform, Energieform and Grundlage, Energieform},
doi = {10.1007/978-3-8348-2279-6},
isbn = {9783834822796},
pages = {15--22},
title = {{3 {\{}{\"{U}}{\}}berblick}}
}
@article{Barber,
author = {Barber, Ever J},
journal = {Concrete},
title = {{Chemical Resistance Guide for their molded fiberglass}}
}
@book{Merker2000,
author = {Merker, G{\"{u}}nter and Baumgarten, Carsten},
publisher = {Vieweg+Teubner Verlag},
title = {{Fluid- und W{\"{a}}rmetransport Str{\"{o}}mungslehre}},
year = {2000}
}
@article{Broekaert2017,
abstract = {The heat transfer from the bulk gases to the combustion chamber walls has a strong effect on the combustion and emission formation process in an HCCI engine. In this work, the empirical heat transfer models of Annand, Woschni, Hohenberg, Bargende, Chang et al. and Hensel et al. are evaluated at various engine operating conditions. The modelled heat flux is compared to the measured heat flux in a CFR engine with a thermopile sensor. The shape of the heat flux trace, the maximum heat flux and the total heat loss are evaluated and different model calibration procedures are investigated. It is found that all models require calibration and need to be recalibrated if the fuel type and certain engine settings are changed. A better model fit can be obtained if different model coefficients are applied for the compression and the expansion phase.},
author = {Broekaert, Stijn and {De Cuyper}, Thomas and {De Paepe}, Michel and Verhelst, Sebastian},
doi = {10.1016/j.apenergy.2017.08.100},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Heat Transfer Combustion Chamber/2017{\_}Broekaert{\_}Evaluation of empirical heat transfer models for HCCI combustion in a CFR engine.pdf:pdf},
issn = {03062619},
journal = {Appl. Energy},
keywords = {Experimental,Heat transfer,Homogeneous charge compression ignition,Internal combustion engine},
number = {May},
pages = {1141--1150},
publisher = {Elsevier},
title = {{Evaluation of empirical heat transfer models for HCCI combustion in a CFR engine}},
volume = {205},
year = {2017}
}
@article{Tsurushima2002,
abstract = {One of the problems in HCCI combustion is a knocking in higher load conditions. It governs the high load limit, and it is suggested that the knock increases heat loss[1], because it breaks the thermal boundary layer. But it is not clear how much knock affects on heat loss in the HCCI combustion in various conditions, such as ignition timing and load. The motivation of this study is to clarify the ratio of heat loss caused by knock in HCCI engines. The heat loss from zero-dimensional calculations with modified heat transfer coefficient, which is considering the effect of knock by adding a term of cylinder pressure rising rate dp/dt, agreed well with the results from the thermodynamic analysis in various conditions. And the results show that it is possible to avoid heat loss by knock by controlling the ignition timing at appropriate timing after T.D.C. and it will be possible to expand the load range if knock can be avoided. Copyright {\textcopyright} 2002 Society of Automotive Engineers, Inc.},
author = {Tsurushima, T. and Kunishima, E. and Asaumi, Y. and Aoyagi, Y. and Enomoto, Y.},
doi = {10.4271/2002-01-0108},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2002{\_}Tsurushima{\_}The Effect of Knock on Heat Loss in HCCI Engines-Modified Woschni.pdf:pdf},
journal = {SAE Tech. Pap.},
number = {724},
title = {{The effect of knock on heat loss in homogeneous charge compression ignition engines}},
volume = {2002},
year = {2002}
}
@article{Geometrie,
author = {Geometrie, Die and Innendurchmesser, Der},
title = {{3 Geometrie und Tragf{\{}{\"{a}}{\}}higkeit}}
}
@article{Fu,
author = {Fu, Fertigungsverfahren and Din, Nach and Druckbeha, Im},
doi = {10.1007/978-3-8348-8279-0},
isbn = {9783834882790},
pages = {186--216},
title = {{7 Nietverbindungen 7.1}}
}
@article{Tornau1998,
author = {Tornau, Christian},
doi = {10.1515/9783110934540.261},
isbn = {9783110934540},
pages = {1--10},
title = {{Kapitel 14}},
year = {1998}
}
@article{Forest,
author = {Forest, Samuel},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/Folien CISM Summer School Mai2017 - Mesoscale Models/courses{\_}C1703{\_}forest{\_}Forest1-Micromorphic.pdf:pdf},
title = {{Micromorphic media}}
}
@article{Sun2016b,
abstract = {Multi-scale fatigue model and image-based simulation method are developed in this study to describe collective short cracks evolution process in micro-scale and continuous fatigue damage evolution in macro-scale based on the concept of continuum damage mechanics (CDM). The relationship between the micro-scale and macro-scale fatigue is explored to enhance the understanding the nature of fatigue phenomenon. A case study is carried out to verify the developed multi-scale fatigue model and image-based simulation method. The results show that it is more effective and clear to reveal metal fatigue failure mechanisms from the viewpoint of multi-scale.},
author = {Sun, Bin and Xu, You Lin and Li, Zhaoxia},
doi = {10.1016/j.commatsci.2016.01.021},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/2 scale models papers/2016{\_}Sun+Lu{\_}Multi-scale fatigue model and image-based simulation of collective short cracks evolution process.pdf:pdf},
issn = {09270256},
journal = {Comput. Mater. Sci.},
keywords = {Damage,Fatigue,Image-based,Multi-scale,Short crack},
pages = {24--32},
publisher = {Elsevier B.V.},
title = {{Multi-scale fatigue model and image-based simulation of collective short cracks evolution process}},
url = {http://dx.doi.org/10.1016/j.commatsci.2016.01.021},
volume = {117},
year = {2016}
}
@article{Abbrennstumpfschwei,
author = {Abbrennstumpfschwei, A-stabelektrode and Prototyping, Rapid and Abk, Abkantpresse and Abschr, Abschmelzleistung and Abstreckziehen, Sintern and Abtrennen, Erodieren and Acetylen, Acc-regelung Aceton and Acetylenzerfall, Verbrennungsstufe and Aktivkraft, Aco-regelung Aggregat and Aluminiumlegierung, Aluminiumbasislot and Anschmelzung, Anodenfall and Anschnittsystem, Anschnittquerschnitt and Arbeitsbedarf, Apfelsinenhaut and Arbeitsebene, Walzen and Arbeitstemperatur, Arbeitseingriff and Aufschmelzgrad, Aufbauschneide Aufheizgeschwindigkeit},
title = {{6 Sachwortverzeichnis}}
}
@article{Lemaitre1999a,
abstract = {The ductile type of damage is a phenomenon now well understood. Once the fully coupled set of constitutive equations is identified, Damage Mechanics is a powerful tool to predict failure. Brittle materials do not exhibit such a damageable macroscopic behavior. Nevertheless, they still fail. On the idea that damage is localized at the microscopic scale, a scale smaller than the mesoscopic one of the Representative Volume Element (RVE), we propose a three-dimensional failure modeling for monotonic as well as for fatigue loading. We develop a two scale model of what we shall call brittle damage: at the microscopic scale, micro-cracks or micro-voids exhibit a damageable plastic-like behavior with no effect on the global (mesoscopic) elastic behavior. Microscopic failure is assumed to coincide with the RVE failure. This model turns out to represent quite well physical phenomena related to high cycle fatigue such as the mean stress effect, the nonlinear accumulation of damage, initial strain hardening or damage effect and the nonproportional loading effect for bi-axial fatigue. The model has been implemented as a post-processor computer code. A simplified identification procedure for the determination of the material properties is given.},
author = {Lemaitre, J and Sermage, J P and Desmorat, Rodrigue},
doi = {10.1023/A:1018641414428},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/2 scale models papers/1999{\_}Lemaitre+Sermage+Desmorat{\_}A two scale damage concept applied to fatigue{\_}AnalyticalApproachForDamageEvolution.pdf:pdf},
isbn = {0376-9429},
issn = {0376-9429},
journal = {Int. J. Fract.},
keywords = {Chemistry},
number = {1},
pages = {67--81},
title = {{A two scale damage concept applied to fatigue}},
url = {http://www.springerlink.com/content/xw24115jm0166154/},
volume = {97},
year = {1999}
}
@article{Papula2009c,
author = {Papula, Lothar},
doi = {10.1007/978-3-8348-8285-1},
isbn = {9783834882851},
journal = {Math. Formelsammlung},
pages = {308--397},
title = {{Differentialrechnung 1}},
year = {2009}
}
@article{Corti2009b,
abstract = {Specific power and efficiency of gasoline engines are influenced by factors such as compression ratio and Spark Advance (SA) regulation. These factors influence the combustion development over the crank angle: the trade-off between performance and the risk of irreversible damages is still a key element in the design of both high-performance (racing) and low-consumption engines. This paper presents a novel approach to the problem, with the objective of defining a damage-related and operating conditions-independent index. The methodology is based on the combined analysis of indicating parameters, such as Cumulated Heat Release (CHR), Indicated Mean Effective Pressure (IMEP) and 50{\%} Mass Fraction Burned (MFB50), and typical knock detection parameters, estimated by means of the in-cylinder pressure sensor signal. Knocking combustions have several consequences, therefore they can be detected in many ways. As it is well known, knock excites the combustion chamber resonant frequencies, rising high frequency components in the in-cylinder pressure signal. Additionally, knocking combustions cause a higher heat flux through the combustion chamber walls, increasing the heat losses and lowering the IMEP: this effect can be observed by evaluating IMEP or CHR, that are based on the low-frequency content of the in-cylinder signal spectrum. A knock detection index can then be based on the crossed-observation of two phenomena, one set in the low-frequencies range and the other one on the high frequencies range of the in-cylinder pressure signal. Knock-related parameters have been analyzed with a statistical approach, in order to define a detection strategy based on one single threshold value, to be used for all the engines, independently of engine speed and load: IMEP and CHR have been related to a typical high-frequency knock index, based on the Maximum Amplitude of Pressure Oscillations (MAPO) evaluated over the combustion angular window. It can be observed that, as knock intensity increases, the relationships between these parameters change. This change can be seized by evaluating the correlation coefficient between the parameters distributions and observing its trend as a function of SA (Spark Advance). The correlation coefficient is intrinsically normalized, therefore the index range is the same for every engine operating condition, and the paper shows that the threshold level, too, is constant. The same approach can be applied to determine SA corresponding to the best combustion phase, simply by evaluating the correlation coefficient for IMEP and MFB50 distributions. The methodology has been successfully applied to different engines running in different speed and load conditions.},
author = {Corti, Enrico and Forte, Claudio},
doi = {10.4271/2009-24-0019},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Klopfen{\_}Ottomotor/2009{\_}Forte+Corti{\_}Statistical Analysis of Indicating Parameters for Knock Detection Purposes.pdf:pdf},
issn = {19463936},
journal = {SAE Tech. Pap.},
number = {2009-01-0237},
title = {{Statistical Analysis of Indicating Parameters for Knock Detection Purposes}},
url = {http://papers.sae.org/2009-01-0237/},
year = {2009}
}
@article{Dieselmotor,
author = {Dieselmotor, Der},
title = {{11 Schmierstoffe und Schmiersystem 11.1}}
}

@book{Reuter2008a,
author = {Reuter, Manfred and Zacher, Serge},
booktitle = {Anal. Simul. und Entwurf von Regelkreisen},
doi = {10.1007/978-3-8348-9273-7},
isbn = {978-3-8348-0018-3},
title = {{Aus dem Programm}},
year = {2008}
}
@article{La,
author = {La, Die and Zahl, Reelle},
pages = {224--238},
title = {{VIII Komplexe Zahlen und Funktionen 1 Darstellungsformen einer komplexen Zahl}}
}
@article{Mathematik,
author = {Mathematik, Zentrum and Funktion, Eine},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Mathematik/Laplacetrafo{\_}Uebersicht.pdf:pdf},
pages = {1--2},
title = {{Laplace-Transformation – Definition und Rechenregeln}}
}
@article{Szabo1991,
author = {Szabo, B A and Babuska, I},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Nicholson 2003 - Finite Element Analysis Thermomechanics of Solids/Nicholson - 2003 - Finite element analysis thermomechanics of solids.pdf:pdf},
isbn = {084930749X},
title = {{Finite element analysis}},
year = {1991}
}

@book{Meister2011b,
abstract = {Die wichtigsten Verfahren zur numerischen L{\"{o}}sung von linearen Gleichungssystemen in einer umfassenden Einf{\"{u}}hrung, die zum Verst{\"{a}}ndnis nur geringe mathematische Vorkenntnisse ben{\"{o}}tigt. Behandelt werden sowohl die direkten als auch die iterativen Verfahren, wobei der Autor gro{\ss}en Wert auf eine sorgf{\"{a}}ltige Herleitung dieser Verfahren legt. Au{\ss}erdem sind sehr detaillierte Pseudocodes enthalten, mit deren Hilfe sich die jeweiligen Verfahren in einer beliebigen Programmiersprache sofort auf dem Computer realisieren lassen. Das Lehrbuch ist auch f{\"{u}}r Natur- und Ingenieurwissenschaftler geeignet, die in vielen praktischen Anwendungen mit der L{\"{o}}sung von linearen Gleichungssystemen konfrontiert sind.},
archivePrefix = {arXiv},
arxivId = {1011.1669v3},
author = {Meister, Andreas},
booktitle = {Matrix},
doi = {10.1007/978-3-8348-8100-7},
eprint = {1011.1669v3},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/Numerik linearer Gleichungssysteme{\_}Andreas Meister/Kapitel3-Direkte Verfahren.pdf:pdf},
isbn = {978-3-8348-1550-7},
issn = {1098-6596},
pages = {36--68},
pmid = {25246403},
title = {{Numerik linearer Gleichungssysteme}},
url = {http://link.springer.com/10.1007/978-3-8348-8100-7},
year = {2011}
}
@article{Merker2004,
author = {Merker, G{\"{u}}nter and Schwarz, Christian and Stiesch, Gunnar and Otto, Frank},
journal = {Simul. der Verbrennung und Schadstoffbildung},
number = {2002},
pages = {152--160},
title = {{Literatur}},
year = {2004}
}
@article{Verst,
author = {Verst, Elektronische},
title = {{Arker}}
}
@article{McEvily1987,
abstract = {A method for determining the fatigue notch-size-effect is presented based upon the development of closure in the wake of a newly formed crack growing from a notch. A comparison with experimental results is in accord with predictions. The effect of crack closure on the formation of non-propagating cracks at notches and on notch sensitivity is also discussed. ?? 1987.},
author = {McEvily, A J and Minakawa, K},
doi = {10.1016/0013-7944(87)90049-X},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/1987{\_}McEvily{\_}ON CRACK CLOSURE AND THE NOTCH SIZE EFFECT IN FATIGUE.pdf:pdf},
isbn = {0013794418},
issn = {00137944},
journal = {Eng. Fract. Mech.},
number = {5-6},
pages = {519--527},
title = {{On crack closure and the notch size effect in fatigue}},
volume = {28},
year = {1987}
}
@article{James1983,
author = {James, M. R. and Morris, W. L.},
doi = {10.1007/BF02643749},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Surface effects + Frequency effects/1983{\_}Morris{\_}Effect of fracture surface roughness on growth of short fatigue cracks.pdf:pdf},
issn = {0360-2133},
journal = {Metall. Trans. A},
number = {1},
pages = {153--155},
title = {{Effect of Fracture Surface Roughness on Growth of Short Fatigue Cracks}},
url = {http://link.springer.com/10.1007/BF02643749},
volume = {14},
year = {1983}
}

@article{Menny2000,
author = {Menny, Klaus},
doi = {10.1007/978-3-322-96796-1_6},
isbn = {978-3-519-26317-3},
pages = {250--277},
title = {{Ventilatoren und Verdichter}},
year = {2000}
}
@article{Zienkiewicz2014c,
author = {Zienkiewicz, O.C. and Taylor, R.L. and Fox, David},
doi = {10.1016/B978-1-85617-634-7.00005-3},
journal = {Finite Elem. Method Solid Struct. Mech.},
pages = {147--177},
title = {{Geometrically Nonlinear Problems: Finite Deformation}},
url = {http://linkinghub.elsevier.com/retrieve/pii/B9781856176347000053},
year = {2014}
}
@article{Strd,
author = {Str, Methoden},
title = {{Omungssichtbarmachung}}
}
@article{Tabellen,
author = {Tabellen, Die and Zahlenwerte, Tabelle and Gau{\ss}, Der},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Empirical Fatigue Models + Validation/Betriebsfestigkeit{\_}ErwinHaibach/Kap5 Anhang.pdf:pdf},
title = {{5 Anhang Daten zu statistischen Verfahren}}
}
@article{Functions2003,
author = {Functions, Mathematical and Wiley, John},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Nicholson 2003 - Finite Element Analysis Thermomechanics of Solids/0749{\_}References.pdf:pdf},
title = {{Articles and Other Sources}},
volume = {2},
year = {2003}
}
@article{Zienkiewicz2005e,
abstract = {Publisher Summary Plates and shells are a particular form of three-dimensional solid, the treatment of which presents no theoretical difficulties in the case of elasticity. The thickness of such structures is very small when compared with other dimensions. Their complete three-dimensional numerical treatment is costly and often leads to serious numerical ill-conditioning problems. To ease the solution, even long before numerical approaches became possible, several classical assumptions regarding the behavior of such structures were introduced. Such assumptions result in a series of approximations. Therefore, numerical treatment concerns itself with the approximation to an already approximate theory, the validity of which is restricted. The shape functions for rectangular elements are the simplest to form for thin plates. The thick-plate theory is simpler to implement in the finite element method; however, in the early days of analytical treatment, it presented more difficulties. This chapter discusses non-conforming shape functions. The solution with conforming shape functions give bounds to the energy of the correct solution; however, on many occasions, yields inferior accuracy to that achieved with non-conforming elements. },
author = {Zienkiewicz, O C and Taylor, R L and Zhu, J Z},
doi = {http://dx.doi.org/10.1016/B978-075066431-8.50198-3},
isbn = {978-0-7506-6431-8},
journal = {Finite Elem. Method Set (Sixth Ed.},
pages = {323--381},
title = {{11 - Plate bending approximation: Thin (Kirchhoff) plates and {\{}C1{\}} continuity requirements}},
url = {http://www.sciencedirect.com/science/article/pii/B9780750664318501983},
year = {2005}
}
@inproceedings{Hoermann2005,
abstract = {The present paper is part of a more comprehensive study concerning the surface flow in the engine compartment and focuses on the fluid flow of a cooling system in a modern vehicle. The complexity of this field needs to further optimization in the integration of 3D CFD (Computational Fluid Dynamics) methods. An important focus lies on the modeling of radiators and fans. A new simulation method needs to be validated. For this purpose a component test bench was built.This paper shows the results oft the simulation on the test bench and the CFD analysis. All the fan and radiator model configurations have been studied by means of a commercial CFD package. The comparison of the results gives a better understanding of the total system performance for a faster and more reliable preliminary design.},
author = {H{\"{o}}rmann, T and Lechner, B and Puntigam, W and Moshammer, T and Almbauer, R},
booktitle = {Veh. Therm. Manag. Syst. Conf. Expo.},
doi = {10.4271/2005-01-2006},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Thermal Coating + Water Heat Transfer + Applikation/2005{\_}Hoerman{\_}Numerical and Experimental Investigation of Flow and Temperature Fields around Automotive Cooling Systems.pdf:pdf},
publisher = {SAE International},
title = {{Numerical and Experimental Investigation of Flow and Temperature Fields around Automotive Cooling Systems}},
year = {2005}
}
@article{Fs2013b,
author = {Fs},
doi = {10.1007/978-1-4614-0502-3},
isbn = {2009004043},
number = {1},
pages = {0--10},
title = {{Chapter 0}},
year = {2013}
}
@article{Markers2009,
author = {Markers, Tissue Tumor},
journal = {Surg. Clin. North Am.},
pages = {427--448},
title = {10 10.1.1},
year = {2009}
}

@article{Mohammadi2010,
abstract = {Optimizing heat transfer for internal combustion engines requires application of advanced development tools. In addition to experimental method, numerical 3D-CFD calculations are needed in order to obtain an insight into the complex phenomenas in-cylinder processes. In this context, fluid flow and heat transfer inside a four-valve engine cylinder is modeled and effects of changing engine speed on dimensionless parameters, instantaneous local Nusselt number and Reynolds number near the surface of combustion chamber are studied. Based on the numerical simulation new correlations for instantaneous local heat transfer on the combustion chamber of SI engines are derived. Results for several engine speeds are compared for total heat transfer coefficient of the cylinder engine with available correlation proposed by experimental measurements and a close agreement is observed. It is found that the local value of heat transfer coefficient varies considerably in different parts of the cylinder, but it has equivalent trend with crank angle position. ?? 2010 Elsevier Masson SAS. All rights reserved.},
author = {Mohammadi, A and Yaghoubi, M},
doi = {10.1016/j.ijthermalsci.2009.12.010},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2010{\_}Mohammadi{\_}Estimation of instantaneous local heat transfer coefficient.pdf:pdf},
isbn = {12900729 (ISSN)},
issn = {12900729},
journal = {Int. J. Therm. Sci.},
keywords = {CFD,Combustion,Cylinder head,Heat transfer coefficient,Nusselt number,SI engine,Turbulence},
number = {7},
pages = {1309--1317},
publisher = {Elsevier Masson SAS},
title = {{Estimation of instantaneous local heat transfer coefficient in spark-ignition engines}},
url = {http://dx.doi.org/10.1016/j.ijthermalsci.2009.12.010},
volume = {49},
year = {2010}
}
@article{Zheng2001a,
abstract = {Research on the basic fatigue formula, the criterion for omitting small loads, the rule for cumulative fatigue damage, and models for predicting the fatigue crack initiation (FCI) life and probability distribution under variable-amplitude loading are comprehensively studied and summarized in the present paper. First, the formula for FCI life is given as a function of the equivalent stress amplitude, and the procedures for investigating overload effects are introduced. Using the above formula to analyze test results of the overload effect on FCI life yields the formula for FCI life containing the overload effect factor, z, which can be adopted to characterize the load interaction effect when Miner's rule is used to compute the cumulative fatigue damage. Fatigue test results and analysis of the underload effect show that the FCI threshold in the FCI life formula can be taken as the criterion for omitting small loads in life prediction and in compilation of the load spectrum. Then, the fatigue damage functi on is defined, the cumulative fatigue damage can be computed and the FCI life of structure members under variable-amplitude loading can be obtained by using Miner's rule. Procedures for predicting the probability distribution of FCI life or fatigue life are described and examples are introduced. Furthermore, factors affecting the value of z and the applicability of Miner's rule are briefly discussed. Finally, further areas for fatigue research are tentatively proposed. Most interest should be focused on research into generally applicable life prediction models and the approach for fatigue reliability assessment of structure details made of the metals with continuous strain-hardening characteristics, which have been widely adopted in aeronautical engineering, under service load and environments. ?? 2001 Elsevier Science Ltd. All rights reserved.},
author = {Zheng, Xiulin},
doi = {10.1016/S0142-1123(01)00040-8},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Empirical Fatigue Models + Validation/2001{\_}Zheng{\_}On some basic problems of fatigue research in engineering{\_}ModelsAccumulationProbabilityOverloadeffect.pdf:pdf},
issn = {01421123},
journal = {Int. J. Fatigue},
keywords = {Criterion for omitting small load,Fatigue crack initiation,Fatigue damage function,Fatigue formula,Joints,Life prediction,Miner's rule,Overload effect,Strain-hardening characteristics},
number = {9},
pages = {751--766},
title = {{On some basic problems of fatigue research in engineering}},
volume = {23},
year = {2001}
}

@article{Chang2004c,
abstract = {An experimental study has been carried out to provide qualitative and quantitative insight into gas to wall heat transfer in a gasoline fueled Homogeneous Charge Compression Ignition (HCCI) engine. Fast response thermocouples are embedded in the piston top and cylinder head surface to measure instantaneous wall temperature and heat flux. Heat flux measurements obtained at multiple locations show small spatial variations, thus confirming relative uniformity of incylinder conditions in a HCCI engine operating with premixed charge. Consequently, the spatially-averaged heat flux represents well the global heat transfer from the gas to the combustion chamber walls in the premixed HCCI engine, as confirmed through the gross heat release analysis. Heat flux measurements were used for assessing several existing heat transfer correlations. One of the most popular models, the Woschni expression, was shown to be inadequate for the HCCI engine. The problem is traced back to the flame propagation term which is not appropriate for the HCCI combustion. Subsequently, a modified model is proposed which significantly improves the prediction of heat transfer in a gasoline HCCI engine and shows very good agreement over a range of conditions},
author = {Chang, Junseok and G{\"{u}}ralp, Orgun and Filipi, Zoran and Assanis, Dennis N and Kuo, Tang-Wei and Najt, Paul and Rask, Rod},
doi = {10.4271/2004-01-2996},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2004{\_}Chang{\_}New Heat Transfer Correlation for an HCCI Engine Derived from Measurements of Instantaneous Surface Heat Flux.pdf:pdf},
isbn = {0148-7191},
issn = {0148-7191},
number = {724},
title = {{New Heat Transfer Correlation for an HCCI Engine Derived from Measurements of Instantaneous Surface Heat Flux}},
url = {http://papers.sae.org/2004-01-2996/},
year = {2004}
}
@article{Grafenhorst2016,
author = {Grafenhorst, Matthias and Hartmann, Stefan and Rang, Joachim},
doi = {10.1002/pamm.201610210},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Numerik UMATS FE-Codes/2016{\_}Hartmann{\_}Time-adaptive non-linear ﬁnite-element computa tions for thermo-mechanically coupled analysis in elastic dynamical systems.pdf:pdf},
issn = {16177061},
journal = {Pamm},
number = {1},
pages = {443--444},
title = {{Time-adaptive non-linear finite-element computations for thermo-mechanically coupled analysis in inelastic dynamical systems}},
url = {http://doi.wiley.com/10.1002/pamm.201610210},
volume = {16},
year = {2016}
}
@article{Koalitionsfreiheit1971,
author = {Koalitionsfreiheit, I Grundfunktionen Der},
number = {N 1},
pages = {410--443},
title = {{A . Allgemeine Grundlagen}},
year = {1971}
}
@article{Contentsa,
author = {Contents, Chapter},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Zienkiewicz FEM - Vol 1 Basics Fundamentals/63205{\_}apdxc.pdf:pdf},
title = {{Solution of Simultaneous Linear Algebraic Equations 3.1}}
}
@article{Metallurgy,
author = {Metallurgy, Physical},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/Folien CISM Summer School Mai2017 - Mesoscale Models/courses{\_}C1703{\_}roux+{\_}lect5-behaviour.pdf:pdf},
number = {I},
pages = {1--22},
title = {{Stress-strain behaviour}}
}
@article{Foundations2003,
author = {Foundations, Mathematical},
pages = {1--23},
title = {and},
year = {2003}
}
@article{Behandlung,
author = {Behandlung, Bei Der and Emv, Der},
journal = {System},
title = {{A1 Elektrische Felder von Stabanordnungen}}
}

@inproceedings{Taler2017,
author = {Taler, Dawid and Taler, Jan},
booktitle = {E3S Web Conf.},
doi = {https://doi.org/10.1051/e3sconf/20171302008},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Heat transfer intake+exhaust system/2017{\_}Taler{\_}Simple heat transfer correlations for turbulent tube flow.pdf:pdf},
title = {{Simple heat transfer correlations for turbulent tube flow}},
volume = {13},
year = {2017}
}
@article{Zahoransky2013f,
author = {Zahoransky, Richard a. and Allelein, Hans-Josef and Schelling, Udo and Schwarz, Harald and Bollin, Elmar and Oehler, Helmut},
doi = {10.1007/978-3-8348-2279-6},
isbn = {978-3-8348-1869-0},
journal = {Energietechnik - Syst. zur Energieumwandlung},
pages = {32},
title = {{8 Station{\"{a}}re Kolbenmotoren f{\"{u}}r energetischen Einsatz}},
url = {http://www.springerlink.com/index/10.1007/978-3-8348-2279-6},
year = {2013}
}
@book{Johna,
author = {John, F and Marsden, J E and Sirovich, L and Golubitsky, M},
isbn = {9781475743401},
title = {{Texts in Applied Mathematics 15}}
}

@article{Adair1972b,
abstract = {This study first reviews, discusses, and compares existing correlations{\$}\backslash{\$}nfor heat transfer in reciprocating compressors and engines. Then{\$}\backslash{\$}nafter a discussion of the significance of obtaining accurate instantaneous{\$}\backslash{\$}nheat transfer data, the authors describe an experimental investigation{\$}\backslash{\$}nof the instantaneous heat transfer rates to the cylinder wall of{\$}\backslash{\$}na reciprocating refrigerating compressor. Finally, this report presents{\$}\backslash{\$}nan expression which correlates the time averaged data within 20{\{}{\%}{\}}.},
author = {Adair, R P and Qvale, E B and Pearson, J T},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/1972{\_}Adair{\_}Instantaneous Heat Transfer to the Cylinder Wall in Reciprocating compressors and engines.pdf:pdf},
journal = {Int. Compress. Eng. Conf.},
pages = {521--526},
title = {{Instantaneous heat transfer to cylinder wall in reciprocating compressors}},
year = {1972}
}
@article{Wimmer2000a,
abstract = {This paper summarizes the results of several investigations on in-cylinder heat transfer during high-pressure and gas exchange phases as well as heat transfer in the inlet and outlet ports for a number of different engine types (DI Diesel, SI and gaseous fueled engine). The paper contains a comparision of simulation results and experimental data derived from heat flux measurements. Numerical results were obtained from zero-, one- and three-dimensional simulation methods. Time and spatially resolved heat fluxes were measured applying the surface temperature method and special heat flux sensors. The paper also includes an assessment of different sensor types with respect to accuracy and applicability.ER -},
author = {Wimmer, Andreas and Pivec, Robert and Sams, Theodor},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2000{\_}Wimmer{\_}Heat Transfer to the Combustion Cahmber and Port Walls of IC Engines - Measurement and Prediction.pdf:pdf},
number = {724},
title = {{Heat Transfer to the Combustion Chamber and Port Walls of IC Engines - Measurement and Prediction}},
year = {2000}
}
@article{Polak2014b,
abstract = {The role of point defects in the formation of surface relief and in the initiation of a fatigue crack in crystalline materials is analyzed. The dislocation interactions in the bands of intensive cyclic slip (persistent slip bands - PSBs) are specified and relations describing the formation and annihilation of interstitial and vacancy type defects in the channels of the ladder-like PSB are derived. The continuous formation, annihilation and primarily the migration of point defects are proposed to be responsible for the mass redistribution within PSB and between PSB and the PSB/matrix boundary. The redistribution of the matter results in local tensile and compressive stresses that are the sources of the principal irreversibility of slip within PSB. Local tensile and compressive stresses are relaxed by dislocation movement within PSB in the direction of the active Burgers vector and lead to the formation of characteristic surface relief in the form of extrusions and intrusions. The intrusions represent crack-like defects and fatigue cracks initiate in the tip of intrusions. {\{}{\textcopyright}{\}} 2013 Elsevier Ltd. All rights reserved.},
author = {Pol{\'{a}}k, Jaroslav and Man, Jiř{\'{i}}},
doi = {10.1016/j.ijfatigue.2013.10.016},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Kriechen{\_}Spannungsrelaxation/2014{\_}Polak+Man{\_}Fatigue crack initiation – The role of point defects.pdf:pdf},
isbn = {0142-1123},
issn = {01421123},
journal = {Int. J. Fatigue},
keywords = {Extrusion,Fatigue crack initiation,Intrusion,Persistent slip band (PSB),Point defects},
number = {July},
pages = {18--27},
title = {{Fatigue crack initiation - The role of point defects}},
volume = {65},
year = {2014}
}
@article{Kr??mer2013a,
author = {Kr??mer, Stephan and Rothe, Steffen and Hartmann, Stefan},
doi = {10.1007/s00366-013-0337-7},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Parametersch{\"{a}}tzung/2013{\_}Hartmann{\_}Homogeneous stress–strain states computed by 3D-stress algorithms of FE-codes - application to material parameter identification.pdf:pdf},
issn = {14355663},
journal = {Eng. Comput.},
keywords = {DAE-systems,Finite elements,Material parameter identification,Plane stress,Stress algorithms},
number = {1},
pages = {141--159},
title = {{Homogeneous stress???strain states computed by 3D-stress algorithms of FE-codes: application to material parameter identification}},
volume = {31},
year = {2013}
}
@article{Thon2015a,
author = {Thon, M},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Vorlesungen/p{\_}script{\_}em1{\_}ws1516.pdf:pdf},
pages = {2--4},
title = {{Engineering Mechanics I}},
volume = {2},
year = {2015}
}
@article{Mesarovic2017,
author = {Mesarovic, S},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/Folien CISM Summer School Mai2017 - Mesoscale Models/courses{\_}C1703{\_}Mesarovic+Lecture+3+CORR+2.pdf:pdf},
title = {{Physical foundations of meso-scale continua Part 2 : ( Thermo- ) Dynamics}},
year = {2017}
}

@inproceedings{Fontanesi2011,
abstract = {The paper presents a combined experimental and numerical activity carried out to improve the accuracy of conjugate heat transfer CFD simulations of a high-performance S.I. engine water cooling jacket.Due to the complexity of the computational domain, which covers both the coolant jacket and the surrounding metal cast (both head and block), particular care is required in order to find a tradeoff between the accuracy and the cost-effectiveness of the numerical procedure. In view of the presence of many complex physical phenomena, the contribution of some relevant CFD parameters and sub-models is separately evaluated and discussed.Among the formers, the extent of the computational domain, the choice of a proper set of boundary conditions and the detailed representation of the physical properties of the involved materials are separately considered. Among the latters, the choice between a simplified single-phase approach and a more complex two-phase approach taking into account the effects of phase transition within the engine coolant is discussed.The predictive capability of the CFD-CHT methodology is assessed by means of the comparison between CFD results and experimental measurements provided by the engine manufacturer for different engine operating conditions.At the end of the validation process, a methodology for the correct and cost-effective characterization of conjugate heat transfer is proposed, showing a reasonable trade-off between the predictive capability and the computational effort of the simulations.},
author = {Fontanesi, Stefano and Cicalese, Giuseppe and D'Adamo, Alessandro and Pivetti, Gianluca},
booktitle = {10th Int. Conf. Engines Veh.},
doi = {10.4271/2011-24-0132},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Boiling/2011{\_}Fontanesi{\_}Validation of a CFD Methodology for the Analysis of CHT in a high performance SI engine{\_}No Boling used.pdf:pdf},
month = {sep},
publisher = {SAE International},
title = {{Validation of a CFD Methodology for the Analysis of Conjugate Heat Transfer in a High Performance SI Engine}},
year = {2011}
}
@article{Principle2003,
author = {Principle, Incremental},
pages = {215--226},
title = {{Incremental Principle of Virtual Work 17.1}},
volume = {2},
year = {2003}
}

@article{Grandin2002a,
abstract = {Heat transfer to the walls of the combustion chamber is increased by engine knock. In this study the influence of knock onset and knock intensity on the heat flux is investigated by examining over 10 000 individual engine cycles with a varying degree of knock. The heat transfer to the walls was estimated by measuring the combustion chamber wall temperature in an SI engine under knocking conditions. The influence of the air-fuel ratio and the orientation of the oscillating cylinder pressure-relative to the combustion chamber wall-were also investigated.It was found that knock intensities above 0.2 Mpa influenced the heat flux. At knock intensities above 0.6 Mpa, the peak heat flux was 2.5 times higher than for a non-knocking cycle. The direction of the oscillations did not affect the heat transfer.ER -},
author = {Grandin, B{\"{o}}rje and Denbratt, Ingemar},
doi = {10.4271/2002-01-0238},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Klopfen{\_}Ottomotor/2002{\_}Grandin{\_}The Effect of Knock on Heat Transfer in SI Engines-Experimental Results.pdf:pdf},
journal = {Sae Tech. Pap. Ser.},
number = {724},
title = {{The Effect of Knock on Heat Transfer in SI Engines}},
url = {http://papers.sae.org/2002-01-0238},
year = {2002}
}
@article{Bauer1998b,
abstract = {Entry flow heat transfer experiments are reported in steady and pulsating flows of air at mean Reynolds numbers of 3000-35 000. THe ducts are chosen to match typical spark-ignition engine manifolds: a highly curved and a straight pipe, which together bracket most practical geometries. The pulsating engine intake flow encompasses an approximate half sine wave followed by a stagnant phase three itmes as long, all at a repetition rate of 16-50 Hz. Heat flow is imposed through electric heating of the outsides of the manifolds. Heat transfer in the curved pipe is closely comparable to the straight geometry, and it is concluded that entrance effects dominate. Time-averaged axially resolved and axially averaged Nusselt numbers are reported. The unsteady nature of the intake flow enhances heat transfer significantly, between 50{\%} and 100{\%}. Time-resolved wall heat flux measurements at a location close to the exit of the system show that heat transfer is delayed relative to the onset of the flow. During the stagnant flow phase, heat transfer and turbulence decay slowly from their high levels during the induction flow phase. Heat transfer enhancement in the pulsating flow case is caused by the contribution of the stagnant phase.},
author = {Bauer, Wolf D. and Wenisch, Joseph and Heywood, John B.},
doi = {10.1016/S0142-727X(97)10001-7},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Heat transfer intake+exhaust system/1998{\_}Bauer{\_}Averaged and time-resolved heat transfer of steady and pulsating entry flow in intake manifold of a SI engine.pdf:pdf},
isbn = {0142-727x},
issn = {0142727X},
journal = {Int. J. Heat Fluid Flow},
keywords = {intake manifold,internal combustion engine,ow,pulsating,transient heat,ux measurements},
number = {1},
pages = {1--9},
title = {{Averaged and time-resolved heat transfer of steady and pulsating entry flow in intake manifold of a spark-ignition engine}},
volume = {19},
year = {1998}
}
@article{Bedienung2008,
author = {Bedienung, Die and Wunsch, Der and Eingabem, Alternative and Umsetzung, Die and Sprachsteuerung, Die and Mmi, Audi and Comand, Mercedes},
journal = {Haut},
pages = {115--145},
title = {{4 Haptische Bedienschnittstellen}},
year = {2008}
}
@article{Svendsen1999,
author = {Svendsen, B},
doi = {10.1007/s001610050114},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Thermodynamik/Liu-Entropieprinzip{\_}Lukas{\_}Fraunhofer/Liu-Entropieprinzip/Svendsen{\_}thermoelasticity{\_}with{\_}additional{\_}DOF{\_}1999.pdf:pdf},
issn = {0935-1175},
journal = {Contin. Mech. Therm.},
pages = {247--262},
title = {{On the thermodynamics of thermoelastic materials with additional scalar degrees of freedom}},
volume = {4},
year = {1999}
}
@article{Fahrzeugsystemen1987,
author = {Fahrzeugsystemen, Der Ausfall Von},
journal = {Prax. (Bern. 1994).},
title = {{8 Sicherheit und Zuverl{\{}{\"{a}}{\}}ssigkeit}},
year = {1987}
}
@article{Fitton1992,
author = {Fitton, J C and Nates, R J},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Klopfen{\_}Ottomotor/1992{\_}Fitton{\_}and{\_}Nates{\_}Investigation into the relationship between knock intensity and piston seizure.pdf:pdf},
journal = {N{\{}{\&}{\}}O J.},
title = {{Investigation into the relationship between knock intensity and piston Seizure}},
year = {1992}
}
@article{Brown2005,
abstract = {The classic theories of dislocation pile-ups, initiated by Eshelby, Frank and Nabarro, and by Leibfried, can be greatly simplified if it is recognised that the dislocations in the pile-up will experience uniform stress if they are lodged in an ellipsoidal interface. Elementary algebra then produces the familiar results from continuum theory. It seems possible that the ellipsoid construction may represent physical reality if it is taken to represent a three-dimensional slip-band. If so, there are concentrated forces spreading the band perpendicular to the slip band as well as parallel to it. Such ellipsoids also represent Mode II and Mode III cracks, and give a method for dealing with the more complicated Mode I cracks. ?? 2005 Elsevier B.V. All rights reserved.},
author = {Brown, Lawrence M},
doi = {10.1016/j.msea.2005.03.043},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/2005{\_}Brown{\_}Dislocation pile-ups slip-bands ellipsoids and cracks.pdf:pdf},
isbn = {0921-5093},
issn = {09215093},
journal = {Mater. Sci. Eng. A},
keywords = {Dislocations,Ellipsoids,Pile-ups,Slip-bands},
number = {1-2 SUPPL.},
pages = {2--6},
title = {{Dislocation pile-ups, slip-bands, ellipsoids, and cracks}},
volume = {400-401},
year = {2005}
}
@article{Haupt1995,
author = {Haupt, P and Lion, A},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Kriechen{\_}Spannungsrelaxation/1995{\_}Haupt+Lion{\_}Experimental identification and mathematical modeling of viscoplastic material behavior.pdf:pdf},
pages = {73--96},
title = {{C0ntinuum Mechanics Experimental identification and mathematical modeling of viscoplastic material behavior}},
volume = {7},
year = {1995}
}
@article{Leichtbautheorie,
author = {Leichtbautheorie, Der},
journal = {Mechanik},
pages = {74--105},
title = {{8 Elastizit{\"{a}}tstheoretische Grundlagen}}
}
@inproceedings{Klein2004,
abstract = {The objective is to investigate models of the specific heat ratio for the single-zone heat release model, and find a model accurate enough to introduce a modeling error less than or in the order of the cylinder pressure measurement noise, while keeping the computational complexity at a minimum. Based on assumptions of frozen mixture for the unburned mixture and chemical equilibrium for the burned mixture, the specific heat ratio is calculated using a full equilibrium program for an unburned and a burned air-fuel mixture, and compared to already existing and newly proposed approximative models of $\gamma$.A two-zone mean temperature model, Matekunas pressure ratio management and the Vibe function are used to parameterize the mass fraction burned. The mass fraction burned is used to interpolate the specific heats for the unburned and burned mixture, and then form the specific heat ratio, which renders a small enough modeling error in $\gamma$. The specific heats for the unburned mixture is captured within 0.2 {\%} by a linear function, and the specific heats for the burned mixture is captured within 1 {\%} by a higher-order polynomial for the major operating range of a spark ignited (SI) engine.},
author = {Klein, Marcus and Eriksson, Lars},
booktitle = {SAE 2004 World Congr. Exhib.},
doi = {https://doi.org/10.4271/2004-01-1464},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Injection+Combustion+Ignitionsystems/2004{\_}Klein{\_}A Specific Heat Ratio Model for Single-Zone Heat Release Models.pdf:pdf},
publisher = {SAE International},
title = {{A Specific Heat Ratio Model for Single-Zone Heat Release Models}},
year = {2004}
}
@article{Flik,
author = {Flik, H. and Th., Liebig and M{\"{o}}ssenb{\"{o}}ck, P. and H., Rechenberg},
journal = {H{\"{u}}tte},
pages = {1--172},
title = {{J-Technische Informatik}}
}
@book{Schade2006,
author = {Schade, Heinz and Neemann, Klaus},
isbn = {3110147416},
pages = {398},
title = {{Tensoranalysis}},
url = {http://www.amazon.de/dp/3110147416},
year = {2006}
}
@article{Reichardt1951,
author = {Reichardt, H},
doi = {10.1002/zamm.19510310704},
journal = {Z. Angew. Math. Mech},
number = {7},
pages = {208--219},
title = {{Vollst{\"{a}}ndige Darstellung der turbulenten Geschwindigkeitsverteilung in glatten Leitungen}},
volume = {31},
year = {1951}
}
@article{Allianz2003c,
author = {Allianz, Von M Pfender and Berlin, M{\"{u}}nchen},
isbn = {3540440631},
number = {2},
title = {{6 Schrifttumshinweise}},
volume = {6},
year = {2003}
}

@article{Murakami2012e,
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Murakami, Sumio},
doi = {10.1007/978-94-007-2666-6},
eprint = {arXiv:1011.1669v3},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/Continuum Damage Mechanics - SumioMurakami/Kap5{\_}Inelastic Constitutive Equation and Damage Evolution Equation of Material with Anisotropic Damage.pdf:pdf},
isbn = {978-94-007-2665-9},
issn = {09250042},
pmid = {25246403},
title = {{Continuum Damage Mechanics}},
url = {http://link.springer.com/10.1007/978-94-007-2666-6},
volume = {185},
year = {2012}
}
@article{Mehrzahl,
author = {Mehrzahl, Die and Umwelt, Der Der},
pages = {111--124},
title = {{9 Messung nichtelektrischer physikalischer Gr{\"{o}}{\ss}en}}
}
@inproceedings{Payri2005,
abstract = {In this paper the heat transfer of the hot gases to the cylinder walls of DI Diesel engines is analyzed using Computational Fluid Dynamics (CFD) and compared to the predictions obtained with a zero-dimensional thermodynamic model based on a variant of the Woschni equation. The final objective is to improve the simple model by modifying the original equations to better take into account the influence of important parameters, such as swirl, on the heat transfer.CFD calculations of the compression and expansion strokes have been made for two real DI Diesel engine geometries, a small one with a displacement of 0.4 l. and a heavy duty one of 2.0 l., and for different working points.The total heat transfer rate to the cylinder surfaces is highly dependent on the mean flow behavior and turbulence levels. Hence, starting from initial conditions at Inlet Valve Closing (IVC), various parametric studies have been performed to take into account the influence on the heat transfer of the level of swirl on the one hand, of engine speed on another, and of modifying the clearance height on another.Solutions obtained with both the CFD simulation and the diagnosis model are compared. They show that there are some important differences due to the assumptions made in the thermodynamic model concerning these parameters. Interesting conclusions are drawn from the more accurate CFD results and a simple modification of the terms included in the Woschni-like equation of the thermodynamic model is proposed to better take into account the significant influence of the swirl on the heat transfer.},
author = {Payri, F and Margot, X and Gil, A and Martin, J},
booktitle = {SAE Tech. Pap. 2005-01-0210},
doi = {10.4271/2005-01-0210},
publisher = {SAE International},
title = {{Computational Study of Heat Transfer to the Walls of a DI Diesel Engine}},
year = {2005}
}
@book{Eifler2009,
address = {Wiesbaden},
author = {Eifler, Wolfgang and Schl{\"{u}}cker, Eberhard and Spicher, Ulrich and Will, Gotthard},
edition = {7},
isbn = {978-3-8348-9302-4},
publisher = {Vieweg+Teubner},
title = {{K{\"{u}}ttner Kolbenmaschinen}},
year = {2009}
}
@article{Kametani1980,
author = {Kametani, T. and Umezawa, O.},
doi = {10.1248/cpb.37.3229},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/1985{\_}Enomoto{\_}Heat Loss to Combustion Chamber Wall of 4-Stroke Gasoline Engine - Heat Loss to Piston and Cylinder.pdf:pdf},
issn = {09168451},
journal = {Chem. Pharm. Bull.},
number = {6},
pages = {369--375},
pmid = {8987871},
title = {{NII-Electronic Library Service}},
volume = {28},
year = {1980}
}
@book{Bridgman1932,
author = {Bridgman, P. W.},
publisher = {Teubner Verlag Berlin},
title = {{Theorie der physikalischen Dimensionen}},
year = {1932}
}
@misc{Vagera1971,
author = {Vagera, I},
booktitle = {Scr. Met.},
doi = {10.1016/0036-9748(71)90036-6},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/1971{\_}Vagera{\_}A PileUp or a dislocation model of crack in an interface between two isotropic or anisotropic media.pdf:pdf},
issn = {00369748},
number = {2},
pages = {93--96},
title = {{A pile-up or a dislocation model of crack in an interface between two isotropic or anisotropic media}},
volume = {5},
year = {1971}
}
@article{Popov2009,
author = {Popov, Valentin and Schargott, Martin},
title = {{Materialtheorie}},
year = {2009}
}


@article{Gingrich2016,
abstract = {An experimental investigation was conducted to explore the impact in-cylinder pressure oscillations have on piston heat transfer. Two fast-response surface thermocouples embedded in the piston top measured transient temperature and a commercial wireless telemetry system was used to transmit thermocouple signals from the moving piston. Measurements were made in a light-duty single-cylinder research engine operated under low temperature combustion regimes including Homogeneous Charge Compression Ignition (HCCI) and Reactivity Controlled Compression Ignition (RCCI) and Conventional Diesel (CDC). The HCCI data showed a correlated trend of higher heat transfer with increased pressure oscillation strength, while the RCCI and CDC data did not. An extensive HCCI data set was acquired. The heat transfer rate - when corrected for differences in cylinder pressure and gas temperature - was found to positively correlate with increased pressure oscillations. It is important to normalize the data before drawing conclusions as the magnitude of the effect was diminished significantly by the normalization procedure.},
author = {Gingrich, Eric and Janecek, Daniel and Ghandhi, Jaal},
doi = {10.4271/2016-01-9044},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2016{\_}Gingrich{\_}Experimental Investigation of the Impact of In-Cylinder Pressure Oscillations on Piston Heat Transfer.pdf:pdf},
issn = {1946-3944},
journal = {SAE Int. J. Engines},
number = {3},
pages = {2016--01--9044},
title = {{Experimental Investigation of the Impact of In-Cylinder Pressure Oscillations on Piston Heat Transfer}},
url = {http://papers.sae.org/2016-01-9044/},
volume = {9},
year = {2016}
}
@article{Tensors1968,
author = {Tensors, Flux},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/Folien CISM Summer School Mai2017 - Mesoscale Models/courses{\_}C1703{\_}groma{\_}continuum.pdf:pdf},
title = {{Continuum Theory of Dislocations and Plastleity'}},
year = {1968}
}
@article{Gesellschaft2004,
author = {Gesellschaft, Deutsche},
journal = {Tagungsbericht},
keywords = {eu-wrrl,ffh-richtlinie,flie{\{}{\ss}{\}}gew{\{}{\"{a}}{\}}s-,makrophyten,nordrhein-westfalen,seen},
pages = {1--5},
title = {{1 Einleitung}},
year = {2004}
}
@article{Merker2004,
author = {Merker, G{\"{u}}nter and Schwarz, Christian and Stiesch, Gunnar and Otto, Frank},
journal = {Simul. der Verbrennung und Schadstoffbildung},
number = {2002},
pages = {152--160},
title = {{Literatur}},
year = {2004}
}
@article{Opitz1959a,
author = {Opitz, Herwart},
doi = {10.1007/978-3-663-05002-5_6},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Empirical Fatigue Models + Validation/Betriebsfestigkeit{\_}ErwinHaibach/Backmatter.pdf:pdf},
isbn = {978-3-663-03813-9},
pages = {33},
title = {{Verwendete Formelzeichen}},
year = {1959}
}
@article{Vektors,
author = {Vektors, Definition},
keywords = {gesetze der,vektor,vektoraddition},
title = {{II Vektoralgebra}}
}
@article{V,
author = {V, Von Catia},
pages = {44--51},
title = {{18 Begleittext zu den Anwendungsbeispielen}}
}
@article{Hernandez2010,
author = {Hern{\'{a}}ndez, Abarca},
doi = {10.1002/cbdv.201090012},
issn = {1612-1880},
journal = {Chem. Biodivers.},
number = {12},
pages = {2963--80},
pmid = {21162009},
title = {{Author index.}},
url = {http://www.ncbi.nlm.nih.gov/pubmed/21162009},
volume = {7},
year = {2010}
}
@article{Burgi,
author = {Burg, Heinz and Moser, Andreas and Taschenbuch, Kraftfahrtechnischen and Firma, Von Der and Bosch, Robert},
pages = {73--88},
title = {{A4 Systematik der Fahrzeugtechnik A4}}
}
@book{Besson2010,
author = {Besson, Jacques and Cailletaud, Georges and Chaboche, Jean-Louis and Forest, Samuel},
booktitle = {Solid Mech. its Appl.},
doi = {10.1007/978-90-481-3356-7},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Besson 2009 - Non-linear Mechanics of Materials.pdf:pdf},
isbn = {978-90-481-3355-0},
keywords = {emergency,luation of non-urgent visits,to a busy urban},
pages = {1--450},
title = {{Non-Linear Mechanics of Materials}},
volume = {33},
year = {2010}
}

@article{Wang2014a,
author = {Wang, Cong and Shang, De Guang and Wang, Xiao Wei},
doi = {10.1007/s11665-014-1335-7},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Empirical Fatigue Models + Validation/2014{\_}Wang{\_}7075-T651 Models and validation.pdf:pdf},
issn = {15441024},
journal = {J. Mater. Eng. Perform.},
keywords = {critical plane,high-cycle fatigue,life prediction,maximum shear stress (MSS),multsiaxial fatigue},
number = {2},
pages = {816--824},
title = {{A New Multiaxial High-Cycle Fatigue Criterion Based on the Critical Plane for Ductile and Brittle Materials}},
volume = {24},
year = {2014}
}
@misc{GTPower75,
author = {Technologies, Gamma},
title = {{GT-Power User Manual, v7.5}}
}
@article{Fourier-transformation,
author = {Fourier-transformation, Technik Der},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Mathematik/fourier{\_}{\_}transformation{\_}{\_}university{\_}muenster.pdf:pdf},
title = {{Technik der Fourier-Transformation}}
}
@article{Eq2015,
author = {Eq, Hence and Eqs, Comparing},
pages = {1--5},
title = {{Appendix H}},
year = {2015}
}

@phdthesis{BargendeDis1991,
author = {Bargende, Michael},
school = {Technical University Darmstadt},
title = {{Ein Gleichungsansatz zur Berechnung der instation{\"{a}}ren Wandw{\"{a}}rmeverluste im Hochdruckteil von Ottomotoren}},
year = {1991}
}
@article{Hettinger2009b,
abstract = {It is a well known fact that indicated efficiency of a SI engine at WOT is predominantly limited by knock occurrence. Therefore many investigations have been carried out to avoid knocking. Considering the further development of downsized engines knocking will also pose a greater challenge. Not only knocking but also irregular combustion in general will require further investigation in supercharged SI eingines. Premature ignition, for instance, hasn't yet been completely understood and therefore limits the low end torque of supercharged SI engines.The purpose of this paper is to introduce different analysis methods which allow to identify the knock onset and the knocking zones in the combustion chamber. In addition to established methods new techniques have been developed to account for the complex nature of pressure oscillation during knocking combustion.Experimental data was acquired on a single cylinder research engine to validate the methodology using six pressure transducers.},
author = {Hettinger, Alexander and Kulzer, Andr{\'{e}}},
doi = {10.4271/2009-01-0698},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Klopfen{\_}Ottomotor/2009{\_}Hettinger+Kulzer{\_}A new method to detect Knocking Zones.pdf:pdf},
isbn = {2009010698},
issn = {1946-3944},
journal = {SAE Int. J. Engines},
number = {1},
pages = {2009--01--0698},
title = {{A New Method to Detect Knocking Zones}},
url = {http://papers.sae.org/2009-01-0698/},
volume = {2},
year = {2009}
}
@article{Vii-,
author = {Vii-, Bild},
doi = {10.1007/978-3-8348-8285-1},
isbn = {9783834882851},
pages = {640--720},
title = {{VII Komplexe Zahlen und Funktionen}}
}
@article{Kapitel,
author = {Kapitel, Dieses and Simulation, Der and Einspritzprozessen, Von},
pages = {483--533},
title = {{13 Simulation von Einspritzprozessen}}
}
@article{Gegensatz,
author = {Gegensatz, Im and Anteil, Der and Aufladung, Die and Lau-, Im and Konzepte, Downsizing- and Auf-, Andere},
title = {{4 Relevante Subsysteme und Prozesse}}
}
@article{Raillard2015,
author = {Raillard, B and Mu, F},
doi = {10.1016/B978-1-78242-074-3.00024-6},
isbn = {9781782420743},
title = {24 24.1},
year = {2015}
}
@article{Results1994a,
abstract = {As a concluding comment, I should like to return to the point raised by Ayres, that it is not enough simply to tell a better version of the fourth-century history in the expectation that modern theologians will finally get it straight! This is a valid point: if we want to have Christianity's fourth-century heritage taken seriously, we need to be in dialogue with modern writers. But, if there is to be a dialogue, both sides must be allowed to speak, and so we are also responsible for expounding the historical material on its own terms. As Heidegger put it, “[O]nly when we think through what has been thought will we be of any use for what must still be thought.” Perhaps studying the figures from a distant era will open up for us possibilities we would never have dreamed of within our own modern presuppositions, so that we can recognize differences even beyond those which lie within our own horizon or tradition. If I am right in affirming that there is a different style of doing theology prior to Augustine and after him in the East than that which we find in the theological and scholarly tradition in which Ayres's book stands, then we must ask whether we need to address the question of the legitimacy of each (and ponder how one might even answer that) or whether a plurality of approaches is possible without reducing one to the other. In a way, this would be a further step toward deconstructing monolithic notions of “Orthodoxy” in recognition of genuine and legitimate diversity within early Christianity and among modern Christians. Might it be better not to speak of Nicaea and its legacy, but of the legacies of Nicaea—or better—“Christ and him crucified” (2 Cor 2:2) and the ways in which Nicaea and its interpreters affirm the true divinity of this one?},
author = {Results, Useful},
doi = {10.1007/BF02600226},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/Micromechanisms of fracture and fatigue/Kap5{\_}FinalReflection.pdf:pdf},
isbn = {9780470434673},
issn = {08848734},
journal = {J. Gen. Intern. Med.},
number = {3 Supplement},
pages = {243--247},
title = {{Final reflections}},
volume = {9},
year = {1994}
}
@article{Plan,
author = {Plan, Dieser and Ecie-plan, Auch and Carmanufactures, European},
pages = {103--105},
title = {{12 Ableitung von Fahrzeug-Hauptabmessungen}}
}
@article{Demu2012_Properties,
abstract = {Models for the convective heat transfer from the combustion gases to the walls inside a spark ignition engine are an important keystone in the simulation tools which are being developed to aid engine optimization. The existing models have, however, been cited to be inaccurate for hydrogen, one of the alternative fuels currently investigated. One possible explanation for this inaccuracy is that the models do not adequately capture the effect of the gas properties. These have never been varied in a wide range because air and ‘classical' fossil fuels have similar values, but they are significantly different in the case of hydrogen. As a first step towards a fuel independent heat transfer model, we have investigated the effect of the gas properties on the heat flux in a spark ignition engine. The effect of the gas properties was decoupled from that of combustion, by injecting different inert gases (helium, argon, carbon dioxide) into the intake air flow of the engine under motored operation. This paper presents the results of the experiment, which was designed with DoE techniques. The paper shows that the three investigated effects (throttle position, compression ratio and gas) and the interaction between the throttle and the compression ratio are significant with a significance level of 1{\%}. Both the individual and combined effects of the gas properties are investigated. The most remarkable effect observed in the data was that the dynamic viscosity influences the heat flux in two contrasting ways. At the one hand, it increases the heat flux by increasing the gas temperature, at the other hand, it reduces the heat flux through the convection coefficient. A preliminary test shows that modeling under motored operation could be based on classical concepts. However, some scatter occurs in the data which needs further investigation.},
author = {Demuynck, Joachim and {De Paepe}, Michel and Sileghem, Louis and Vancoillie, Jeroen and Verhelst, Sebastian and Chana, Kam},
doi = {https://doi.org/10.4271/2012-01-1209},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Heat Transfer Combustion Chamber/2012{\_}Demuynck{\_}Applying Design of Experiments to Determine the Effect of Gas Properties on In Cylinder Heat Flux in a Motored SI Engine.pdf:pdf},
journal = {SAE Int. J. Engines},
month = {apr},
number = {3},
pages = {1286--1299},
title = {{Applying Design of Experiments to Determine the Effect of Gas Properties on In-Cylinder Heat Flux in a Motored SI Engine}},
volume = {5},
year = {2012}
}
@article{Verbindungstechnologien,
author = {Verbindungstechnologien, Die and Von, Leichtbau},
title = {{22 Verbindungstechnik}}
}
@article{Heinisch1994a,
author = {Heinisch, Rudolf},
doi = {10.1007/BF02600863},
isbn = {3-540-23870-0},
journal = {Forsch. im Ingenieurwes.},
number = {Nr. 718},
pages = {11/12--35},
title = {{Der 1. Hauptsatz der Thermodynamik}},
volume = {59},
year = {1994}
}
@misc{Draper1935a,
author = {Draper, C S},
booktitle = {NACA Rep.},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/xxx{\_}Draper{\_}The physical effects of detonation in a closed cylindrical chamber - analytical solutions.pdf:pdf},
number = {493},
title = {{The physical effects of detonation in a closed cylindrical chamber}},
year = {1935}
}
@article{Temperatur,
author = {Temperatur, Die},
title = {{W{\{}{\"{a}}{\}}rme{\{}{\"{u}}{\}}bertrager}}
}
@article{FONTANESI_Boiling,
author = {Fontanesi, Stefano and Giacopini, Matteo},
doi = {https://doi.org/10.1016/j.applthermaleng.2012.12.005},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Boiling/2013{\_}Fontanesi{\_}Multiphase CFD-CHT optimization of the cooling jacket and FEM analysis of the engine head of a V6 Diesel engine.pdf:pdf},
journal = {Appl. Therm. Eng.},
number = {2},
pages = {293--303},
title = {{Multiphase CFD-CHT optimization of the cooling jacket and FEM analysis of the engine head of a V6 diesel engine}},
volume = {52},
year = {2013}
}
@article{Produktion,
author = {Produktion, Die},
journal = {Elektronik},
number = {1},
pages = {171--182},
title = {{9 Produktionstechnik}}
}
@article{Wimmer2000a,
abstract = {This paper summarizes the results of several investigations on in-cylinder heat transfer during high-pressure and gas exchange phases as well as heat transfer in the inlet and outlet ports for a number of different engine types (DI Diesel, SI and gaseous fueled engine). The paper contains a comparision of simulation results and experimental data derived from heat flux measurements. Numerical results were obtained from zero-, one- and three-dimensional simulation methods. Time and spatially resolved heat fluxes were measured applying the surface temperature method and special heat flux sensors. The paper also includes an assessment of different sensor types with respect to accuracy and applicability.ER -},
author = {Wimmer, Andreas and Pivec, Robert and Sams, Theodor},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2000{\_}Wimmer{\_}Heat Transfer to the Combustion Cahmber and Port Walls of IC Engines - Measurement and Prediction.pdf:pdf},
number = {724},
title = {{Heat Transfer to the Combustion Chamber and Port Walls of IC Engines - Measurement and Prediction}},
year = {2000}
}
@article{Burge,
author = {Burg, Heinz},
pages = {695--703},
title = {{B8 B8 Unf{\{}{\"{a}}{\}}lle mit land- oder forstwirtschaftlichen Fahrzeugen {\{}{\"{U}}{\}}berholender Pkw kollidiert mit nach links abbiegendem Traktor B8}}
}

@article{Ubertragung,
author = {{\"{U}}bertragung, Die},
journal = {Frequenz},
pages = {6--13},
title = {{2 Messsignale}}
}
@book{Riccardella1992b,
author = {Riccardella, P C and Deardorff, A F and Griesbach, T J},
booktitle = {Adv. Fatigue Lifetime Predict. Tech.},
doi = {10.1520/STP1122-EB},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Neuer Ordner/Advances in fatigue lifetime predictive techniques Part1.pdf:pdf},
isbn = {978-0-8031-1423-4},
issn = {00660558},
keywords = {FATIGUE,MONITORING,POWER PLANTS,PRESSURE VESSELS AND PIPING,THERMAL STRESSES},
pages = {460--473},
pmid = {11439068},
title = {{Advances in Fatigue Lifetime Predictive Techniques}},
url = {https://apps.webofknowledge.com/full{\%}7B{\_}{\%}7Drecord.do?product=UA{\%}7B{\&}{\%}7Dsearch{\%}7B{\_}{\%}7Dmode=GeneralSearch{\%}7B{\&}{\%}7Dqid=11{\%}7B{\&}{\%}7DSID=Z1UxbH6jtsqo8n9kPQr{\%}7B{\&}{\%}7Dpage=1{\%}7B{\&}{\%}7Ddoc=1},
volume = {1122},
year = {1992}
}
@book{Dobrinski1984,
author = {Dobrinski, Professor Dr. rer. nat. Paul and Krakau, Professor Dr. phil. nat. Gunter and Vogel, Professor Dr. rer. nat. Aneselm},
isbn = {3-519-06501-0},
title = {{Physik f{\"{u}}r Ingenieure}},
year = {1984}
}
@article{Metallurgy,
author = {Metallurgy, Physical},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/Folien CISM Summer School Mai2017 - Mesoscale Models/courses{\_}C1703{\_}roux+{\_}lect5-behaviour.pdf:pdf},
number = {I},
pages = {1--22},
title = {{Stress-strain behaviour}}
}
@article{Pahl2007e,
author = {Pahl, Gerhard and Beitz, Wolfgang and Feldhusen, J{\"{o}}rg and Grote, Karl-Heinrich},
journal = {Konstr. Grundlagen erfolgreicher Produktentwicklung, Methoden und Anwendung},
pages = {189--211},
title = {{Product Development Process}},
year = {2007}
}
@article{General1971,
author = {General, The and Model, Linear},
doi = {10.1016/B978-0-12-627865-1.00015-5},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/{\_}buecherSong/HandbookofComposites/I/15{\_}CCComposites.pdf:pdf},
isbn = {9780126278651},
title = {15 15.1},
year = {1971}
}
@article{Pineau2016,
abstract = {In this interpretive review, fatigue in metallic systems is considered primarily from the perspective of interactions between the microstructure, the deformation mode and the mechanical state at both low and high temperatures. In Part 1 the development and early propagation of cracks is considered in terms of the basic damage mechanisms and the relative size of the crack with respect to applicable microstructural feature(s). In this section, a multistage grain scale approach to microstructure-sensitive fatigue crack formation and growth is presented which uses Fatigue Indicator Parameters (FIPs) to correlate these processes. Various FIPs parameters are discussed in terms of their indication of the state of fatigue. The development and early crack propagation is considered in the context of microstructure and notches, and probabilistic aspects of the notch fatigue problem are discussed. These features are integrated into a systematic approach for the selection of fatigue resistant microstructures for given applications. In Part 2, attention is focused on Ni-base superalloys and the interaction between oxidation, creep and microstructure (including coatings) in the formation and propagation of cracks. This part of the overview addresses both experimental and modelling aspects. Methodologies based upon fundamental physical processes are presented for understanding and predicting the development and propagation of fatigue cracks, including effects of sequential oxide type formation and of creep on either restraining or accelerating damage by oxidation. The variable fatigue resistance of discs in jet engines is seen to depend upon the variability of microstructure and its influence on the severity of creep/oxidation interactions. All of these factors are considered in the practical case where both temperature and loading parameters vary simultaneously (thermomechanical fatigue). A physics-based life prediction model considering the interactions of deformation and environmental damage is reviewed in terms of its applicability to life prediction of components.},
author = {Pineau, Andr?? and McDowell, David L and Busso, Esteban P and Antolovich, Stephen D},
doi = {10.1016/j.actamat.2015.05.050},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/2016{\_}Pineau + McDowell{\_}Failure of metals II Fatigue.pdf:pdf},
isbn = {13596454},
issn = {13596454},
journal = {Acta Mater.},
keywords = {Environment-microstructure interaction,Fatigue in metallic alloys,Intergranular cracking,Local and global fatigue approaches,Multistage fatigue,Oxidation,Superalloys,thermomechanical fatigue},
pages = {484--507},
title = {{Failure of metals II: Fatigue}},
volume = {107},
year = {2016}
}
@article{Bungartz2010,
abstract = {Stra{\ss}enverkehr geht uns alle an, jeder ist davon betroffen. Unsere W{\"{u}}nsche und Vorstellungen bez{\"{u}}glich des Stra{\ss}enverkehrs sind jedoch in der Regel etwas widerspr{\"{u}}chlich: Einerseits wollen wir m{\"{o}}glichst viel davon. Wir wollen mobil sein und so schnell und angenehm wie m{\"{o}}glich von der Wohnung zur Uni oder Arbeit, vom Heimatort zum Ferienziel oder vom Einkaufen zur Freizeitbesch{\"{a}}ftigung gelangen. Wir w{\"{u}}nschen uns dazu gut ausgebaute Stra{\ss}en und Parkpl{\"{a}}tze oder h{\"{a}}ufig fahrenden Personennahverkehr. Andererseits wollen wir m{\"{o}}glichst wenig davon. Stra{\ss}enverkehr soll uns nicht bel{\"{a}}stigen. Wir m{\"{o}}chten nicht im Berufsverkehr oder in den kilometerlangen Mammutstaus zu Ferienbeginn und -ende stehen, w{\"{u}}nschen uns, von L{\"{a}}rm- und Abgasemissionen unbehelligt zu bleiben, und bevorzugen Gr{\"{u}}nstreifen anstelle von Stra{\ss}enasphalt.},
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Bungartz and Zimmer and Buchholz and Pfl{\"{u}}ger},
doi = {10.1515/bmt.2010.712},
eprint = {arXiv:1011.1669v3},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Vorlesungen/Modellbildung{\_}und{\_}Simulation/Skript{\_}Modellbildung{\_}und{\_}Simulation.pdf:pdf},
isbn = {9783642054600},
issn = {0013-5585},
journal = {Biomed. Tech. Eng.},
keywords = {Stichw䣏rter des Dokuments},
number = {s1},
pages = {1--237},
pmid = {14685750},
title = {{Modellbildung und Simulation}},
volume = {55},
year = {2010}
}
@article{Chemisky2013a,
author = {Chemisky, Yves and Meraghni, Fodil},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/Micromechanics formulas{\_}Overview{\_}EshelbyHillAndMore.pdf:pdf},
journal = {Presentations},
title = {{Micromechanics based on the Eshelby solution : Concepts and formulas}},
year = {2013}
}
@article{Kasaba1998,
author = {Kasaba, Koichi and Sano, Takahiro and Kudo, Souichi and Shoji, Tetsuo and Katagiri, Kazumune and Sato, Tadashi},
doi = {10.1016/S0022-3115(98)00343-2},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/1998{\_}Kasaba+Sano{\_}Fatigue crack growth under compressive loading.pdf:pdf},
issn = {00223115},
journal = {J. Nucl. Mater.},
pages = {2059--2063},
title = {{Fatigue crack growth under compressive loading}},
volume = {258-263},
year = {1998}
}
@article{Sauerstoff,
author = {Sauerstoff, Komponenten and Gegensatz, Im},
number = {x},
title = {{6 Schadstoffbildung 6.1}}
}
@article{Bozza2011c,
abstract = {In the present paper a combined procedure for the quasi-dimensional modelling of heat transfer, combustion and knock phenomena in a "downsized" Spark Ignition two-cylinder turbocharged engine is presented. The procedure is extended to also include the effects consequent the Cyclic Variability. Heat transfer is modelled by means of a Finite Elements model. Combustion simulation is based on a fractal description of the flame front area. Cyclic Variability (CV) is characterized through the introduction of a random variation on a number of parameters controlling the rate of heat release (air/fuel ratio, initial flame kernel duration and radius, laminar flame speed, turbulence intensity). The intensity of the random variation is specified in order to realize a Coefficient Of Variation (COV) of the Indicated Mean Effective Pressure (IMEP) similar to the one measured during an experimental campaign. Moreover, the relative importance of the various concurring effects is established on the overall COV. A kinetic scheme is then solved within the unburned gas zone, characterized by different thermodynamic conditions occurring cycle-by-cycle. In this way, an optimal choice of the "knock-limited" spark advance is effected and compared with experimental data. Finally, the CV effects on the occurrence of individual knocking cycles are assessed and discussed. {\textcopyright} 2011 Global Science Press.},
author = {Bozza, Fabio and Siano, Daniela and Costa, Michela},
doi = {10.4208/aamm.10-10s2-04},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Klopfen{\_}Ottomotor/2011{\_}Bozza{\_}heat-transfer-knock-modeling-and-cyclic-variability-in-a-downsized-spark-ignition-turbocharged-engine.pdf:pdf},
issn = {20700733},
journal = {Adv. Appl. Math. Mech.},
keywords = {Cyclic variability,Finite elements in heat transfer,Internal combustion engines modelling,Knock},
number = {3},
pages = {310--326},
title = {{Heat transfer, knock modeling and cyclic variability in a "Downsized" spark-ignition turbocharged engine}},
volume = {3},
year = {2011}
}
@article{Burgc,
author = {Burg, Heinz and Geigl, Bertram C and Kramer, Florian and Moser, Andreas and Steffan, Hermann},
journal = {Injury},
pages = {569--584},
title = {{A19 A19 Biomechanik A19}}
}
@article{Saad2003,
abstract = {Tremendous progress has been made in the scientific and engineering disciplines regarding the use of iterative methods for linear systems. The size and complexity of linear and nonlinear systems arising in typical applications has grown, meaning that using direct solvers for the three-dimensional models of these problems is no longer effective. At the same time, parallel computing, becoming less expensive and standardized, has penetrated these application areas. Iterative methods are easier than direct solvers to implement on parallel computers but require approaches and solution algorithms that are different from classical methods. This second edition gives an in-depth, up-to-date view of practical algorithms for solving large-scale linear systems of equations, including a wide range of the best methods available today. A new chapter on multigrid techniques has been added, whilst material throughout has been updated, removed or shortened. Numerous exercises have been added, as well as an updated and expanded bibliography.},
archivePrefix = {arXiv},
arxivId = {0806.3802},
author = {Saad, Yousef},
doi = {10.2113/gsjfr.6.1.30},
eprint = {0806.3802},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Saad 1996 - Iterative Methods for Sparse Linear Systems.pdf:pdf},
isbn = {0898715342},
issn = {1570579X},
journal = {Notes},
number = {2nd Edition},
pages = {xviii+528},
pmid = {15237199},
title = {{Iterative Methods for Sparse Linear Systems}},
url = {http://www.stanford.edu/class/cme324/saad.pdf},
volume = {3},
year = {2003}
}
@article{Forte2014,
abstract = {A methodology for the evaluation of the effects of twin spark ignition system on CCV (Cycle by Cycle Variability) and knocking combustions is here presented, based on both the use of Computation Fluid Dynamics (CFD) tools and experimental information. The focus of the numerical methodology is the statistical evaluation of the local air-to-fuel distribution at the spark plugs and its correlation with the variability of the initial stages of combustion. A detailed analysis of knocking events can help improving engine performance and diagnosis strategies. The use of twin spark ignition system can enhance the probability that the initial kernel could come across a zone with the correct air-to-fuel ratio, thus lowering the initial combustion instabilities. Moreover the lower distance swept from the flame fronts can considerably reduce the time for the unburnt mixture to auto-ignite, thus reducing the risk of knocking combustion. CFD simulations have been used to reproduce knock effect on the in-cylinder pressure trace. The pressure signal holds information about waves propagation and heat losses: it is crucial to relate local pressure oscillations to knock severity. For this purpose, a CFD model has been implemented, able to predict the combustion evolution with respect to Spark Advance, from non-knocking up to heavy knocking conditions. The CFD model validation phase is essential for a correct representation of both regular and knocking combustions: the operation has been carried out by means of an accurate statistical analysis of experimental in-cylinder pressure data. ?? 2013 The Authors.},
author = {Forte, Claudio and Bianchi, Gian Marco and Corti, Enrico and Fantoni, Stefano and Costa, Marco},
doi = {10.1016/j.egypro.2014.01.091},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Klopfen{\_}Ottomotor/2014{\_}Forte+Corti+Bianchi{\_}CFD Methodology for the evaluation of knock of a PFI Twin Spark Engine.pdf:pdf},
isbn = {3905120933},
issn = {18766102},
journal = {Energy Procedia},
keywords = {Cycle by Cycle Variability,High performance engine,Knock,Twin spark},
pages = {859--868},
publisher = {Elsevier B.V.},
title = {{CFD methodology for the evaluation of knock of a PFI Twin spark engine}},
url = {http://dx.doi.org/10.1016/j.egypro.2014.01.091},
volume = {45},
year = {2014}
}

@article{Eiamsa-Ard2010a,
abstract = {The article presents an investigation of the effect of twisted tape with serrated-edge insert on heat transfer and pressure loss behaviors in a constant heat-fluxed tube. In the experiments, the serrated twisted tape (STT) was inserted into the entire test tube with a constant twist ratio in order to generate a continuous swirling airflow. Two geometry parameters of the STT to be considered in the present work are the serration width ratio and the serration depth ratio. The measurements have been conducted for the airflow rate based on Reynolds numbers in the turbulent regime from 4000 to 20,000. The experimental results of the STT inserted tube are compared with those of the plain tube fitted with typical twisted tape (TT). The results show that the heat transfer rate in terms of Nusselt number, Nu increases with the rise in the depth ratio but decreases with raising the width ratio. The heat transfer rate is up to 72.2{\%} and 27{\%} relative to the plain tube and the TT inserted tube, respectively. The use of the STT leads to higher heat transfer rate and friction factor than that of the TT for all cases. The thermal performance factor of the STT tube under constant pumping power is evaluated and found to be above unity indicating that using the STT tube is advantageous over the TT tube or the plain tube. In addition, the empirical correlations developed by relating the serration width ratio, serration depth ratio and Reynolds number are determined. {\textcopyright} 2010 Elsevier Ltd. All rights reserved.},
author = {Eiamsa-Ard, Smith and Promvonge, Pongjet},
doi = {10.1016/j.applthermaleng.2010.03.026},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Heat transfer intake+exhaust system/2010{\_}Eiamsa-ard+Promvonge{\_}Thermal characteristics in round tube fitted with serrated twisted tape.pdf:pdf},
issn = {13594311},
journal = {Appl. Therm. Eng.},
keywords = {Friction factor,Heat transfer,Serrated twisted tape,Swirl flow,Typical twisted tape},
number = {13},
pages = {1673--1682},
publisher = {Elsevier Ltd},
title = {{Thermal characteristics in round tube fitted with serrated twisted tape}},
url = {http://dx.doi.org/10.1016/j.applthermaleng.2010.03.026},
volume = {30},
year = {2010}
}
@article{Clementa,
author = {Clement, Steffen and Informationstechnik, Elektro- and Klein, Bernd and Engelken, Gerhard and Konstruktion, Maschinenelemente and Czichos, Horst and Theumert, Hans and Maschinenbau, Grundlagen and Hei, Bernd and Ersoy, Metin and Isermann, Rolf and Schabacker, Michael and Fiala, Ernst and Klette, Guido},
isbn = {9783528331245},
journal = {Konstruktion},
title = {{Aus dem Programm}}
}
@article{Page1998,
author = {Page, Previous},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/{\_}buecherSong/HandbookofComposites/II/16{\_}HandLay-upandBagMolding.pdf:pdf},
journal = {Practice},
pages = {372--377},
title = {{372 Hand lay-up and bag molding}},
year = {1998}
}
@article{Dynamics,
author = {Dynamics, Computational Fluid},
pages = {443--482},
title = {{12 Dreidimensionale Str{\{}{\"{o}}{\}}mungsfelder}}
}
@article{Pan2014b,
abstract = {Knocking combustion in spark-ignition (SI) engines is a typical abnormal combustion phenomenon that severely limits engine performance and thermal efficiency. However, its mechanism has not so far been completely revealed, such as the origin of pressure oscillation with tremendous amplitude and broken mechanisms of the engine body when knock occurs. This article systematically reviews the series of physical and chemical phenomena involved in knocking combustion, including auto-ignition, gas-dynamic waves, cavity resonance, and auto-ignited flame propagation. Significant research has shown that the rapid heat release of end-gas auto-ignition and subsequent strong pressure waves play a crucial role during knocking combustion. A methodology of the interaction of flame propagation and pressure waves has been proposed to reveal knock formation in terms of positive feedback between strengthened pressure waves and auto-ignited flame propagation. Also, new suggestions on the weakness in prior research of knocking combustion have also been discussed in the present article. {\{}{\textcopyright}{\}} 2014 Copyright Taylor and Francis Group, LLC.},
author = {Pan, Jiaying and Shu, Gequn and Wei, Haiqiao},
doi = {10.1080/00102202.2013.857665},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2014{\_}Pan+Wei{\_}Interaction of Flame Propagation and Pressure Waves During Knocking Combustion in Spark-Ignition Engines.pdf:pdf},
issn = {0010-2202},
journal = {Combust. Sci. Technol.},
number = {2},
pages = {192--209},
title = {{Interaction of Flame Propagation and Pressure Waves During Knocking Combustion in Spark-Ignition Engines}},
url = {http://www.tandfonline.com/doi/abs/10.1080/00102202.2013.857665},
volume = {186},
year = {2014}
}
@article{Strb,
author = {Str, Die},
pages = {1--6},
title = {{¨ Hrung}}
}

@book{John,
author = {John, F and Marsden, J E and Sirovich, L and Golubitsky, M},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Brenner Susanne C. Scott - 2008 - The mathematical theory of finite element methods.pdf:pdf},
isbn = {9781475743401},
title = {{Texts in Applied Mathematics 15}}
}
@article{Meister2011a,
abstract = {Die wichtigsten Verfahren zur numerischen L{\"{o}}sung von linearen Gleichungssystemen in einer umfassenden Einf{\"{u}}hrung, die zum Verst{\"{a}}ndnis nur geringe mathematische Vorkenntnisse ben{\"{o}}tigt. Behandelt werden sowohl die direkten als auch die iterativen Verfahren, wobei der Autor gro{\ss}en Wert auf eine sorgf{\"{a}}ltige Herleitung dieser Verfahren legt. Au{\ss}erdem sind sehr detaillierte Pseudocodes enthalten, mit deren Hilfe sich die jeweiligen Verfahren in einer beliebigen Programmiersprache sofort auf dem Computer realisieren lassen. Das Lehrbuch ist auch f{\"{u}}r Natur- und Ingenieurwissenschaftler geeignet, die in vielen praktischen Anwendungen mit der L{\"{o}}sung von linearen Gleichungssystemen konfrontiert sind.},
archivePrefix = {arXiv},
arxivId = {1011.1669v3},
author = {Meister, Andreas},
doi = {10.1007/978-3-8348-8100-7},
eprint = {1011.1669v3},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/Numerik linearer Gleichungssysteme{\_}Andreas Meister/Kapitel5-Pr{\"{a}}konditionierer.pdf:pdf},
isbn = {978-3-8348-1550-7},
issn = {1098-6596},
journal = {Matrix},
pages = {36--68},
pmid = {25246403},
title = {{Numerik linearer Gleichungssysteme}},
url = {http://link.springer.com/10.1007/978-3-8348-8100-7},
year = {2011}
}
@article{Trend,
author = {Trend, Der and Forderungen, Diese and Strips, Tailored and Erl, Zur},
journal = {Stahlbau},
pages = {152--158},
title = {{12 Schubwandtr{\{}{\"{a}}{\}}ger-Profile}}
}
@article{Devulder2010a,
author = {Devulder, Anne and Aubry, Denis and Puel, Guillaume},
doi = {10.1007/s00466-010-0476-2},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/2 scale models papers/2010{\_}Devulder+Aubrypouel{\_}Two time scale fatigue modelling-application to damage.pdf:pdf},
issn = {01787675},
journal = {Comput. Mech.},
keywords = {Bone,Damage,Fatigue,Time homogenization},
number = {6},
pages = {637--646},
title = {{Two-time scale fatigue modelling: Application to damage}},
volume = {45},
year = {2010}
}
@article{Terms2014,
author = {Terms, Index},
doi = {10.1016/B978-0-12-416677-6.00029-9},
isbn = {978-0-08-043408-7},
issn = {00220248},
journal = {Seeds},
pages = {1573--1586},
pmid = {24263858},
title = {{Subject Index}},
url = {http://linkinghub.elsevier.com/retrieve/pii/B9780124166776000299},
year = {2014}
}
@article{Lemaitre1999a,
abstract = {The ductile type of damage is a phenomenon now well understood. Once the fully coupled set of constitutive equations is identified, Damage Mechanics is a powerful tool to predict failure. Brittle materials do not exhibit such a damageable macroscopic behavior. Nevertheless, they still fail. On the idea that damage is localized at the microscopic scale, a scale smaller than the mesoscopic one of the Representative Volume Element (RVE), we propose a three-dimensional failure modeling for monotonic as well as for fatigue loading. We develop a two scale model of what we shall call brittle damage: at the microscopic scale, micro-cracks or micro-voids exhibit a damageable plastic-like behavior with no effect on the global (mesoscopic) elastic behavior. Microscopic failure is assumed to coincide with the RVE failure. This model turns out to represent quite well physical phenomena related to high cycle fatigue such as the mean stress effect, the nonlinear accumulation of damage, initial strain hardening or damage effect and the nonproportional loading effect for bi-axial fatigue. The model has been implemented as a post-processor computer code. A simplified identification procedure for the determination of the material properties is given.},
author = {Lemaitre, J. and Sermage, J.P. and Desmorat, Rodrigue},
doi = {10.1023/A:1018641414428},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/2 scale models papers/1999{\_}Lemaitre+Sermage+Desmorat{\_}A two scale damage concept applied to fatigue{\_}AnalyticalApproachForDamageEvolution.pdf:pdf},
isbn = {0376-9429},
issn = {0376-9429},
journal = {Int. J. Fract.},
keywords = {Chemistry},
number = {1},
pages = {67--81--81},
title = {{A two scale damage concept applied to fatigue}},
url = {http://www.springerlink.com/content/xw24115jm0166154/},
volume = {97},
year = {1999}
}
@article{Narasimhamurthy1957,
abstract = {BISPLINGHOFF has given a comparative graph showing the relative importance of the parameters of design at various Mach numbers. At Mach numbers above five, i.e. in the range of missile flight, creep becomes the critical design factor. Even though the time of flight of the missile is very short, and not enough to cause any considerable amount of creep, the deflexions caused will be enough to disturb the stability of compression members. Also the aerodynamic shape can be distorted with serious effects on the flow characteristics of the profile.},
author = {Narasimhamurthy, P.},
doi = {10.1108/eb032892},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Kriechen{\_}Spannungsrelaxation/1957{\_}Narasimhamurthy{\_}An Analytical Investigation of creep under combined loadings.pdf:pdf},
issn = {0002-2667},
journal = {Aircr. Eng. Aerosp. Technol.},
number = {11},
pages = {346--349},
title = {{An Analytical Investigation of Creep under Combined Loadings}},
url = {http://www.emeraldinsight.com/doi/abs/10.1108/eb032892},
volume = {29},
year = {1957}
}
@article{Lerch2016,
abstract = {Dieses Lehrbuch bietet eine umfassende Einf{\"{u}}hrung in die moderne Elektrische Messtechnik. Behandelt werden: die Fehlerrechnung systematischer und zuf{\"{a}}lliger Fehler, die Erfassung von dynamischen Messfehlern und ihren Korrekturen, Ger{\"{a}}te und Verfahren der analogen Messtechnik, wie z.B. Standard-Messger{\"{a}}te, elektronische Messverst{\"{a}}rker, Messbr{\"{u}}cken. Anschlie{\ss}end werden Analog-Digital- und Digital-Analog-Umsetzer sowie digitale Messger{\"{a}}te beschrieben. Ein weiterer Schwerpunkt des Buches ist die ausf{\"{u}}hrliche Behandlung der modernen computerunterst{\"{u}}tzten Messdatenerfassung und Messsignalverarbeitung bez{\"{u}}glich Hard- und Software. In der 4. Auflage wurden die Kapitel zur rechnergest{\"{u}}tzten Messdatenerfassung dem allerneuesten Stand der Technik angepasst und die Abschnitte zur Messsignalverarbeitung erheblich erweitert. Es ist eine DVD mit {\"{U}}bungsaufgaben zur rechnergest{\"{u}}tzten Messdatenerfassung und Messsignalverarbeitung sowie zur Programmierung von Speicherprogrammierbaren Steuerungen (SPS) enthalten. Via Internet kann der Leser eine am Lehrstuhl f{\"{u}}r Sensorik aufgebaute SPS programmieren sowie weitere {\"{U}}bungsaufgaben und L{\"{o}}sungen zu den Programmieraufgaben von der DVD herunterladen. Die DVD enth{\"{a}}lt au{\ss}erdem eine Studentenversion von LabVIEW 8.2.1. Das Buch eignet sich in Verbindung mit dem Werk Elektrische Messtechnik/{\"{U}}bungsbuch f{\"{u}}r Studierende der Ingenieur- und Naturwissenschaften sowie f{\"{u}}r den in der Praxis t{\"{a}}tigen Ingenieur auch zum Selbststudium.},
author = {Lerch, R.},
doi = {10.1007/978-3-8348-8304-9_3},
isbn = {978-3-8348-1374-9},
issn = {0937-7433},
journal = {Elektrische Messtechnik},
title = {{Geb{\"{a}}udeautomatisierung (Smart Home)}},
url = {http://dx.doi.org/10.1007/978-3-8348-8304-9{\_}3},
year = {2016}
}
@article{Seng,
author = {Seng, Jocelyn M},
journal = {Production},
title = {{Laminate design}}
}
@article{Papula2011f,
author = {Papula, Lothar},
doi = {10.1007/978-3-8348-8285-1},
isbn = {9783834882851},
journal = {Math. f{\{}{\"{u}}{\}}r Ingenieure und Naturwissenschaftler Band 1},
pages = {422--569},
title = {{V Integralrechnung 1}},
year = {2011}
}
@article{Pahl2007f,
author = {Pahl, Gerhard and Beitz†, Wolfgang and Feldhusen, J{\"{o}}rg and Grote, Karl-H.},
journal = {Pahl/Beitz Konstr. - Grundlagen},
title = {{Inhaltsverzeichnis}},
year = {2007}
}
@article{Bahke2008,
author = {Bahke, T},
journal = {H{\"{u}}tte},
pages = {1--21},
title = {{O-Normung}},
year = {2008}
}
@article{Kapitel2004,
author = {Kapitel, Dieses and Prius, Toyota and Ausblick, Ein and Hybrid, Two Mode and Kapitel, Das},
title = {{Leistungs u ¨ bertragung in Hybridfahrzeugen}},
year = {2004}
}
@book{Merker2014,
address = {Wiesbaden},
author = {Merker, G{\"{u}}nter P. and Teichmann, R{\"{u}}diger},
publisher = {Springer Fachmedien},
title = {{Grundlagen Verbrennungsmotoren}},
year = {2014}
}
@article{Akustik1989,
author = {Akustik, Technischen},
pages = {401--432},
title = {{6 Motorger{\{}{\"{a}}{\}}usch}},
year = {1989}
}
@article{Schie??l2003a,
abstract = {We investigate spatial temperature fluctuations in the unburned endgas of a spark-ignited (SI) engine. Our approach exploits the fact that the quantities (species concentrations, temperature) comprising the state of the combustion chamber gases are not independent, but often correlate sharply. Information about spatial temperature variations is obtained indirectly by observing two complementary quantities that sensitively reflect the local temperature. Spatial formaldehyde (H2CO) concentration variations in the endgas are converted to temperature fluctuations using calculated correlations between temperature and [H2CO]. Additionally, the geometrical size of inhomogeneities is deduced from LIF-images displaying the locally varying formation of temperature-sensitive intermediate species. The results indicate that temperature fluctuations exceeding 20 K are present in the nominally homogeneous endgas. The geometrical size of these fluctuations ranges from ???1 mm to ???1 cm. ?? 2003 The Combustion Institute. All rights reserved.},
author = {Schie??l, R and Maas, U},
doi = {10.1016/S0010-2180(02)00538-2},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Klopfen{\_}Ottomotor/2003{\_}Schiessl{\_}Analysis of endgas temperture fluctuations in an si engine by LIF.pdf:pdf},
isbn = {4907116855653},
issn = {00102180},
journal = {Combust. Flame},
keywords = {Endgas,IC engines,Laser-induced fluorescence,Temperature fluctuations},
number = {1-2},
pages = {19--27},
title = {{Analysis of endgas temperature fluctuations in an SI engine by laser-induced fluorescence}},
volume = {133},
year = {2003}
}
@article{WoschniCsallnerFieger1979,
author = {Woschni, G and Csallner, P and Fieger, J},
journal = {FVV – Vor. Nr. 190, H. Nr. 260 1. Teilabschlussbericht},
number = {190},
title = {{W{\{}{\"{a}}{\}}rme{\{}{\"{u}}{\}}bergang und Brennverlauf im Ottomotor}},
volume = {304},
year = {1979}
}
@article{Chang2004a,
abstract = {An experimental study has been carried out to provide qualitative and quantitative insight into gas to wall heat transfer in a gasoline fueled Homogeneous Charge Compression Ignition (HCCI) engine. Fast response thermocouples are embedded in the piston top and cylinder head surface to measure instantaneous wall temperature and heat flux. Heat flux measurements obtained at multiple locations show small spatial variations, thus confirming relative uniformity of incylinder conditions in a HCCI engine operating with premixed charge. Consequently, the spatially-averaged heat flux represents well the global heat transfer from the gas to the combustion chamber walls in the premixed HCCI engine, as confirmed through the gross heat release analysis. Heat flux measurements were used for assessing several existing heat transfer correlations. One of the most popular models, the Woschni expression, was shown to be inadequate for the HCCI engine. The problem is traced back to the flame propagation term which is not appropriate for the HCCI combustion. Subsequently, a modified model is proposed which significantly improves the prediction of heat transfer in a gasoline HCCI engine and shows very good agreement over a range of conditions},
author = {Chang, Junseok and G{\"{u}}ralp, Orgun and Filipi, Zoran and Assanis, Dennis N. and Kuo, Tang-Wei and Najt, Paul and Rask, Rod},
doi = {10.4271/2004-01-2996},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2004{\_}Chang{\_}New Heat Transfer Correlation for an HCCI Engine Derived from Measurements of Instantaneous Surface Heat Flux.pdf:pdf},
isbn = {0148-7191},
issn = {0148-7191},
number = {724},
title = {{New Heat Transfer Correlation for an HCCI Engine Derived from Measurements of Instantaneous Surface Heat Flux}},
url = {http://papers.sae.org/2004-01-2996/},
year = {2004}
}
@article{Approximation,
author = {Approximation, Die and Integral, Das},
doi = {10.1007/978-3-642-24335-6},
isbn = {9783642243356},
title = {{1 Numerische Integration und Differenziation}}
}
@article{Burg1925,
author = {Burg, Heinz and Arnold, J{\"{o}}rg},
pages = {461--469},
title = {{A16 Schienenfahrzeuge / Stra{\ss}enbahnen A16}},
year = {1925}
}
@article{Yahya2005a,
archivePrefix = {arXiv},
arxivId = {arXiv:1208.3922},
author = {Yahya, S M},
doi = {10.1016/j.ijantimicag.2012.06.019},
eprint = {arXiv:1208.3922},
isbn = {0132592010},
issn = {1540-5834},
number = {6},
pages = {22--24},
pmid = {23425417},
title = {{References [1]}},
volume = {76},
year = {2005}
}
@article{Geh,
author = {Geh, Die and Differential, Das},
title = {{Allgemeine Komponenten der Fahrzeuggetriebe}}
}
@article{Kre2006,
author = {Kre, Der and Gl, Zum and Betrag, Der},
journal = {Gerthsen Phys.},
pages = {71--92},
title = {{02 - Mechanik des starren K{\"{o}}rpers}},
year = {2006}
}
@article{Krank2008a,
author = {Krank, Lothar and Streit, Andreas},
doi = {10.1007/978-3-8348-9430-4},
isbn = {978-3-8348-9430-4},
journal = {Vieweg Praxiswissen},
pages = {209--266},
title = {{Infotainmentsysteme im Kraftfahrzeug}},
year = {2008}
}
@article{Reifenbeurteilung,
author = {Reifenbeurteilung, Die},
title = {{11 Reifenbeurteilung}}
}
@article{Gem2006,
author = {Gem, Gubelin and Opt, Erweiterungen},
number = {2251},
pages = {1--8},
title = {{1 {\{}{\"{U}}{\}}bersicht}},
year = {2006}
}

@article{Murakami2012,
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Murakami, Sumio},
doi = {10.1007/978-94-007-2666-6},
eprint = {arXiv:1011.1669v3},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/Continuum Damage Mechanics - SumioMurakami/Kap7{\_}Fatigue Damage.pdf:pdf},
isbn = {978-94-007-2665-9},
issn = {09250042},
number = {1995},
pages = {201--215},
pmid = {25246403},
title = {{Continuum Damage Mechanics}},
url = {http://link.springer.com/10.1007/978-94-007-2666-6},
volume = {185},
year = {2012}
}
@article{Mughrabi2013,
abstract = {Depending on material and details of cyclic loading conditions, fatigue damage develops and spreads by various modes of crack initiation and subsequent crack growth. In order to gain a deeper understanding of the underlying microstructural mechanisms, many details must be considered. The present study focuses on just a few specific aspects, namely the role of cyclic slip irreversibilities, the significance of fatigue crack initiation in high and ultrahigh cycle fatigue (HCF, UHCF) and, finally the analysis of non-linear effects of elasticity and compliance of fatigued specimens, as a promising non-destructive in situ fatigue damage diagnosis tool. Selected experimental data obtained on different materials will be considered to illustrate the issues named above. ?? 2012 Elsevier B.V. All rights reserved.},
author = {Mughrabi, Hael},
doi = {10.1016/j.ijfatigue.2012.06.007},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/2013{\_}Mughrabi{\_}Microstructural fatigue mechanisms - Cyclic slip irreversibility - crack initiation - non-linear elastic damage analysis.pdf:pdf},
isbn = {01421123},
issn = {01421123},
journal = {Int. J. Fatigue},
keywords = {(Ultra) High cycle fatigue,Cyclic slip irreversibility,Fatigue crack initiation,Fatigue lives,Non-linear elasticity},
pages = {2--8},
publisher = {Elsevier Ltd},
title = {{Microstructural fatigue mechanisms: Cyclic slip irreversibility, crack initiation, non-linear elastic damage analysis}},
url = {http://dx.doi.org/10.1016/j.ijfatigue.2012.06.007},
volume = {57},
year = {2013}
}
@misc{Draper1935,
author = {Draper, C.S.},
booktitle = {NACA Rep.},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/xxx{\_}Draper{\_}The physical effects of detonation in a closed cylindrical chamber - analytical solutions.pdf:pdf},
number = {493},
title = {{The physical effects of detonation in a closed cylindrical chamber}},
year = {1935}
}
@article{Motorauslegung,
author = {Motorauslegung, Kriterien Der and Motorkenndaten, Zur Ver{\"{a}}nderlichkeit Von},
title = {{3 Kriterien bei der Motorauslegung 3.1}}
}
@article{Litewka2008,
author = {Litewka, Andrzej},
doi = {10.1080/01495730802199465},
isbn = {9783540742999},
issn = {0149-5739},
journal = {J. Therm. Stress.},
number = {8},
pages = {788--790},
title = {{Advanced Materials and Structures for Extreme Operating Conditions}},
url = {http://www.informaworld.com/openurl?genre=article{\&}doi=10.1080/01495730802199465{\&}magic=crossref{\%}7C{\%}7CD404A21C5BB053405B1A640AFFD44AE3},
volume = {31},
year = {2008}
}
@article{Tanaka1982b,
abstract = {The fatigue crack initiation along the slip banks emanating from notches is analyzed theoretically with the use of the dislocation dipole accumulation model proposed previously by the authors. The complex function analysis for an elliptical notch under the anti-plane shear gives a quantitative method for assessment of the reduction of fatigue strength as a function of the notch tip radius, the notch size and the elastic stress concentration factor. Special cases of this theoretical analysis yield several semi-empirical formulae commonly used by engineers for data collection. In the derivation, the limitations for each engineering approach are clarified. The material properties are included in the present micromechanical theory as the slip band length and the dislocation frictional stress. ?? 1982.},
author = {Tanaka, K and Mura, T},
doi = {10.1016/0167-6636(82)90024-2},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/1981{\_}Mura+Tanaka{\_}A micromechanical theory of fatigue crack initiation from notches.pdf:pdf},
isbn = {0921-5093},
issn = {01676636},
journal = {Mech. Mater.},
number = {1},
pages = {63--73},
title = {{A micromechanical theory of fatique crack initiation from notches}},
volume = {1},
year = {1982}
}
@article{Hild2015c,
abstract = {{\textcopyright} Springer Science+Business Media New York 2015.This chapter is devoted to the evaluation of damage with digital image correlation (DIC). This measurement technique provides displacement fields that can be used to tune material parameters of damage models. The potential of DIC for identification purposes is illustrated hereafter for simple 1D-type geometries in the context of quasi-brittle and ductile behaviors. Beams and frames as encountered in civil engineering application can be described through damage laws. The localization of damage at single points (lumped damage mechanics) and the resulting damage law can be determined very precisely based on dedicated versions of DIC incorporating the descriptive language of beam theory. At smaller scale, plasterboards (plaster core lined with paper) constitute another example of a structure (rather than a material), which can be described as damageable. Those cases will be analyzed in details.},
author = {Hild, Fran{\c{c}}ois and Roux, St{\'{e}}phane},
doi = {10.1007/978-1-4614-5589-9},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/2015{\_}Sun+Liu{\_}Particle-Cracking modeling of metal matrix composites.pdf:pdf},
isbn = {9781461455899},
journal = {Handb. Damage Mech. Nano to Macro Scale Mater. Struct.},
pages = {1277--1299},
title = {{Evaluating damage with digital image correlation: b. from physical to mechanical damage}},
year = {2015}
}
@article{Algebra2013,
author = {Algebra, Some Vector},
doi = {10.1016/B978-1-85617-633-0.00028-9},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Zienkiewicz FEM - Vol 1 Basics Fundamentals/63205{\_}apdxf.pdf:pdf},
isbn = {9781856176330},
pages = {655--659},
title = {{Some Vector Algebra}},
volume = {1},
year = {2013}
}
@article{Wilhelm2001,
author = {Wilhelm, Mark and Commercial, Boeing and Company, Airplane},
doi = {10.1361/asmhba0003477},
isbn = {9781467399395},
title = {{Aircraft Applications}},
volume = {21},
year = {2001}
}
@article{Enomoto1986,
author = {Enomoto, Yoshiteru and Furuhama, Shoichi},
doi = {10.1299/jsme1958.29.2196},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Heat Transfer Combustion Chamber/1986{\_}Enomoto{\_}Heat Loss to Combustion Chamber Wall of 4-Stroke Gasoline Engine - Heat Loss to Head and Valves.pdf:pdf},
journal = {Bull. JSME},
number = {253},
pages = {2196--2203},
title = {{Heat Loss into Combustion Chamber Wall of 4-stroke Gasoline Engine : 2nd Report, Heat Loss into Cylinder Head, Intake and Exhaust Valves}},
volume = {29},
year = {1986}
}

@article{Leis-1894,
author = {Leis-, Fahrstufen and Theorie, Die and Hertz, Heinrich},
title = {{Erweiterungen der elementaren Festigkeitslehre f{\"{u}}r die Auslegung betriebsfester Fahrzeuggetriebe}},
year = {1894}
}
@book{JANAF1971,
edition = {2},
publisher = {NSRDS-NB537, U.S. National Bureau of Standards},
title = {{JANAF Thermomechanical Tables}}
}
@article{Zienkiewicz2014,
abstract = {Summary In Chapter 2 we presented a framework for solving general problems in solid mechanics. In this chapter we consider several classical models for describing the behaviour of engineering materials. Each model we describe is given in a strain-driven form in which a strain or strain increment obtained from each finite element solution step is used to compute the stress needed to evaluate the internal force, [sigma] BT[sigma] d[Omega], as well as a tangent modulus matrix, or its approximation, for use in constructing the tangent stiffness matrix. Quite generally in the study of small deformation and inelastic materials (and indeed in some forms applied to large deformation) the strain (or strain rate) or the stress is assumed to split into an additive sum of parts. We can write this as [epsilon]=[epsilon]e+[epsilon]i (4.1) or [sigma]=[sigma]e+[sigma]i (4.2) in which we shall generally assume that the elastic part is given by the linear model [epsilon]e=D-1[sigma] (4.3) in which D is the matrix of elastic moduli.},
author = {Zienkiewicz, O.C. and Taylor, R.L. and Fox, David},
doi = {10.1016/B978-1-85617-634-7.00004-1},
isbn = {978-0-75-066431-8},
issn = {0733-9399},
journal = {Finite Elem. Method Solid Struct. Mech.},
pages = {75--145},
pmid = {24603084},
title = {{Inelastic and Nonlinear Materials}},
url = {http://linkinghub.elsevier.com/retrieve/pii/B9781856176347000041},
year = {2014}
}
@article{Nitsche,
author = {Nitsche, W and Brunn, A},
isbn = {10 3-540-20990-5},
title = {{Str{\{}{\"{o}}{\}}mungsmesstechnik}}
}
@article{Walgraef1985,
abstract = {The nucleation of persistent slip bands (PSBs) in stressed metals may be interpreted as a cooperative phenomenon for dislocation populations. The competition between their mobility and nonlinear interaction (creation, annihilation, pinning) induces an instability of uniform dislocation distributions vs inhomogeneous ones and leads to the formation and persistence of spatial patterns. In particular, we have shown in preceding publications that the nucleation and coexistence of the layered structure of PSBs and the rodlike structure of the surrounding matrix can be described by a system of coupled partial differential equations of the reaction-diffusion type for immobile and mobile dislocations. Here we consider explicitly the motion and interaction of positive and negative mobile dislocations and derive an expression for their effective diffusivity. Moreover we show how these effects together with secondary slip activity may trigger the formation of walls in different directions in analogy with observations of labyrinth structures. ?? 1986.},
author = {Walgraef, Daniel and Aifantis, Elias C},
doi = {10.1063/1.336183},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/1985{\_}WalgraefAndAifantis{\_}Dislocation patterning in fatigued metals as a result of dynamical instabilities.pdf:pdf},
issn = {00218979},
journal = {J. Appl. Phys.},
number = {2},
pages = {688--691},
title = {{Dislocation patterning in fatigued metals as a result of dynamical instabilities}},
volume = {58},
year = {1985}
}
@article{Vhwoxu2003a,
author = {Vhwoxu, S and Zdjqhu, M and Gdzvrq, G},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Thermal Coating + Water Heat Transfer + Applikation/2003{\_}Setlur{\_}Nonlinear Controller for Automotive Thermal Management Systems.pdf:pdf},
isbn = {0780378962},
pages = {4699--4704},
title = {{Qrqolqhdu Frqwuroohu iru Dxwrprwlyh Wkhupdo Pdqdjhphqw V | vwhpv}},
year = {2003}
}
@article{Za,
author = {Za, Die and Za, Der},
pages = {696--743},
title = {{21 Stirnra ¨ der mit Evolventenverzahnung 21.1}}
}
@article{Hild2015,
abstract = {{\{}{\textcopyright}{\}} Springer Science+Business Media New York 2015.This chapter is devoted to the evaluation of damage with digital image correlation (DIC). This measurement technique provides displacement fields that can be used to tune material parameters of damage models. The potential of DIC for identification purposes is illustrated hereafter for simple 1D-type geometries in the context of quasi-brittle and ductile behaviors. Beams and frames as encountered in civil engineering application can be described through damage laws. The localization of damage at single points (lumped damage mechanics) and the resulting damage law can be determined very precisely based on dedicated versions of DIC incorporating the descriptive language of beam theory. At smaller scale, plasterboards (plaster core lined with paper) constitute another example of a structure (rather than a material), which can be described as damageable. Those cases will be analyzed in details.},
author = {Hild, Fran{\c{c}}ois and Roux, St{\'{e}}phane},
doi = {10.1007/978-1-4614-5589-9},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/2015{\_}Sun+Liu{\_}Particel-Debonding modeling of metal-matrix composites.pdf:pdf},
isbn = {9781461455899},
journal = {Handb. Damage Mech. Nano to Macro Scale Mater. Struct.},
pages = {1277--1299},
title = {{Evaluating damage with digital image correlation: b. from physical to mechanical damage}},
year = {2015}
}
@article{Tschirschwitzb,
author = {Tschirschwitz, Christian and Dre{\ss}ler, Jan},
pages = {741--754},
title = {{B12 B12 Beispiele zu Insassenverletzungen Beweissicherung und Rekonstruktion von Stra{\{}{\ss}{\}}enverkehrsunf{\{}{\"{a}}{\}}llen mit unklarer Sitzposition B12}}
}
@article{Vorgehensweise,
author = {Vorgehensweise, Verst{\"{a}}ndnis Der},
doi = {10.1007/978-3-8348-2134-8},
isbn = {9783834821348},
journal = {Elements},
pages = {34--40},
title = {{4 Die Matrix-Steifigkeitsmethode}}
}
@article{Zustandsgr,
author = {Zustandsgr, Kritische and Acetylen, Stoff and Argon, Ammoniak and Ethan, Butan and Ethylen, Ethanol and Kohlendioxid, Helium and Methan, Kohlenmonoxid and Propan, Oktan and Schwefeldioxid, Sauerstoff and Wasser, Stickstoff and Co, He and Ch, C O},
title = {{Anhang}}
}

@article{Svoboda2008a,
abstract = {An extremal principle is formulated for thermodynamic systems near equi- librium subjected to various external conditions. It is shown that the principle describes un- ambiguously the kinetics of the thermodynamic system and replaces classical phenomeno- logical equations. Thus the principle can be considered as an effective tool for the treatment of non-equilibrium thermodynamic systems. In two examples the principle is used for the description of Dufour and Soret effects and plasticity. 1.},
author = {Svoboda, Jiř{\'{i}} and Fischer, Franz Dieter and Vala, Jiř{\'{i}}},
doi = {10.1478/C1S0801022},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Thermodynamik/2008{\_}Svoboda+Fischer{\_}Thermodynamic extremal principle and its application to Dufour and Soret effects and Plasticity.pdf:pdf},
issn = {03650359},
journal = {AAPP Atti della Accad. Peloritana dei Pericolanti, Cl. di Sci. Fis. Mat. e Nat.},
number = {SUPPL.1},
pages = {1--11},
title = {{Thermodynamic extremal principle and its application to dufour and soret effects and plasticity}},
volume = {86},
year = {2008}
}
@article{Sauzay2000a,
author = {Sauzay, M. and Gilormini, P.},
doi = {10.1046/j.1460-2695.2000.00307.x},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2000{\_}Sauzay{\_}Surface and cyclic microplasticity{\_}SurfaceAndPlasticityInMicro.pdf:pdf},
issn = {8756758X},
journal = {Fatigue Fract. Eng. Mater. Struct.},
keywords = {crystallographic glide,fatigue,free surface,microplasticity},
number = {7},
pages = {573--579},
title = {{Surface and cyclic microplasticity}},
volume = {23},
year = {2000}
}
@article{Ma2016,
abstract = {High-purity single crystal tungsten nanowire was prepared by the metal-catalyzed vapor-phase reaction method, which was firstly proposed by our research group. Its tensile stress-strain curves and microscopic deformed structures at different temperatures were simulated by molecular dynamics method, in order to study the effects of temperature on its tensile mechanical properties and failure mechanisms. Research results show that the stress-strain curves can be all divided into five stages: elastic, damage, phase transition (dominant), hardening and failure stages. Elastic modulus, tensile strength and strain of phase transition are decreased with increase of temperature, while hardening peak stress is first increased and then decreased. There exists a critical temperature Tc for its phase transition mechanism. When T ??? Tc, the phase transition occurs in one direction and leads to less damage and random failure in its damage zone. When T {\textgreater} Tc, the phase transition occurs in two directions and leads to more damage (twin plane) and failure in its twin plane. That is quite different from FCC metal, where there is only one direction of phase transition.},
author = {Ma, Bin and Rao, Qiuhua and He, Yuehui},
doi = {10.1016/j.commatsci.2016.01.001},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Thermodynamik/2016{\_}Ma+Rao{\_}Molecular dynamics simulation of temperature effect on tensile mechanical properties of single crystal tungsten nanowire.pdf:pdf},
issn = {09270256},
journal = {Comput. Mater. Sci.},
keywords = {Mechanical property,Microscopic deformation mechanism,Molecular dynamics,Single crystal tungsten nanowire,Temperature},
pages = {40--44},
publisher = {Elsevier B.V.},
title = {{Molecular dynamics simulation of temperature effect on tensile mechanical properties of single crystal tungsten nanowire}},
url = {http://dx.doi.org/10.1016/j.commatsci.2016.01.001},
volume = {117},
year = {2016}
}
@article{Notation,
author = {Notation, Matrix},
title = {{Micro-Macro Transit ion Relations for Simple}}
}
@article{Pineau2016a,
abstract = {In this interpretive review, fatigue in metallic systems is considered primarily from the perspective of interactions between the microstructure, the deformation mode and the mechanical state at both low and high temperatures. In Part 1 the development and early propagation of cracks is considered in terms of the basic damage mechanisms and the relative size of the crack with respect to applicable microstructural feature(s). In this section, a multistage grain scale approach to microstructure-sensitive fatigue crack formation and growth is presented which uses Fatigue Indicator Parameters (FIPs) to correlate these processes. Various FIPs parameters are discussed in terms of their indication of the state of fatigue. The development and early crack propagation is considered in the context of microstructure and notches, and probabilistic aspects of the notch fatigue problem are discussed. These features are integrated into a systematic approach for the selection of fatigue resistant microstructures for given applications. In Part 2, attention is focused on Ni-base superalloys and the interaction between oxidation, creep and microstructure (including coatings) in the formation and propagation of cracks. This part of the overview addresses both experimental and modelling aspects. Methodologies based upon fundamental physical processes are presented for understanding and predicting the development and propagation of fatigue cracks, including effects of sequential oxide type formation and of creep on either restraining or accelerating damage by oxidation. The variable fatigue resistance of discs in jet engines is seen to depend upon the variability of microstructure and its influence on the severity of creep/oxidation interactions. All of these factors are considered in the practical case where both temperature and loading parameters vary simultaneously (thermomechanical fatigue). A physics-based life prediction model considering the interactions of deformation and environmental damage is reviewed in terms of its applicability to life prediction of components.},
author = {Pineau, Andr?? and McDowell, David L. and Busso, Esteban P. and Antolovich, Stephen D.},
doi = {10.1016/j.actamat.2015.05.050},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/2016{\_}Pineau + McDowell{\_}Failure of metals II Fatigue.pdf:pdf},
isbn = {13596454},
issn = {13596454},
journal = {Acta Mater.},
keywords = {Environment-microstructure interaction,Fatigue in metallic alloys,Intergranular cracking, thermomechanical fatigue,Local and global fatigue approaches,Multistage fatigue,Oxidation,Superalloys},
pages = {484--507},
title = {{Failure of metals II: Fatigue}},
volume = {107},
year = {2016}
}
@article{Wirkung,
author = {Wirkung, Funktion},
number = {Lagerschale 2},
pages = {522--576},
title = {15 15.1.2},
volume = {0}
}
@article{Enomoto1989,
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Heat Transfer Combustion Chamber/1989{\_}Enomoto{\_}A study of the local HTC on the Cmb CHamber Wall of a four stroke gasoline engine.pdf:pdf},
title = {{NII-Electronic Library Service}}
}
@article{Schweizer2011,
abstract = {In this paper a mechanism-based model is presented, which is able to describe the evolution of microcracks under pure low cycle fatigue (LCF) and combined LCF and high cycle fatigue (HCF) loading conditions. In order to verify the model and to calibrate the model parameters, the crack length evolution of microcracks is followed at room temperature for pure LCF and combined LCF/HCF loading in a 10{\%}-chromium steel. These studies reveal accelerated crack growth rates under LCF/HCF interaction as soon as a critical crack length is reached. The model is capable of accounting for this effect and needs only few parameters, including the threshold for fatigue crack growth, whose knowledge is crucial for the accuracy of the model. ?? 2010 Elsevier Ltd. All rights reserved.},
author = {Schweizer, C. and Seifert, T. and Nieweg, B. and {Von Hartrott}, P. and Riedel, H.},
doi = {10.1016/j.ijfatigue.2010.08.008},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/2010{\_}Schweizer+Seifert{\_}Mechanisms+Modelling of fatigue crack growth under combined low and high cycle fatigue loading.pdf:pdf},
issn = {01421123},
journal = {Int. J. Fatigue},
keywords = {Crack-tip opening displacement (CTOD),Fatigue crack growth,High cycle fatigue,Low cycle fatigue,Threshold stress intensity factor},
number = {2},
pages = {194--202},
publisher = {Elsevier Ltd},
title = {{Mechanisms and modelling of fatigue crack growth under combined low and high cycle fatigue loading}},
url = {http://dx.doi.org/10.1016/j.ijfatigue.2010.08.008},
volume = {33},
year = {2011}
}
@article{Kernphysik,
author = {Kernphysik, Anwendungen Der},
pages = {264--302},
title = {{9. Anwendungen der Kernphysik}},
volume = {120}
}
@article{Morris1976a,
abstract = {Abstract  Fatigue crack initiation in Al 2219-T851 for fully reversed loading(R = $\sigma$/$\sigma$max =−1) parallel to the material rolling direction is found to occur at intermetallic inclusions at the specimen surface. The inclusions are not involved in crack initiation for fatigue perpendicular to the rolling direction, and for this orientation crack initiation is at grain boundaries and specimens have an increased fatigue life. Except for fatigue at low peak stress, multiple numbers of microcracks are formed and for selected failed specimens the number of cracks has been determined as a function of crack length. Such crack length distribution measurements show that there is significant retardation of microcracks by interaction with grain boundaries. Furthermore it is found that the coalescence of microcracks provides a mechanism for cracking to “jump“ grain boundaries and reduce fatigue lifetime. The effect of relative humidity on this process is to increase the observed mean crack length, and decrease the number of crack initiations apparently due to weakening of the matrix-intermetallic interface at potential initiation sites. The overall result is that no significant dependence of fatigue life on relative humidity is found.},
author = {Morris, W. L. and Buck, O. and Marcus, H. L.},
doi = {10.1007/BF02656599},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/1976{\_}Morris{\_}Fatigue crack initiation and early propagation in Al 2219-T851.pdf:pdf},
isbn = {0360-2133$\backslash$r1543-1940},
issn = {03602133},
journal = {Metall. Trans. A},
number = {7},
pages = {1161--1165},
title = {{Fatigue crack initiation and early propagation in Al 2219-T851}},
volume = {7},
year = {1976}
}
@article{Isermann2006,
author = {Isermann, Rolf},
doi = {10.1007/978-3-8348-9049-8\_18},
isbn = {978-3-8348-0109-8},
journal = {Fahrdynamik-Regelung},
pages = {377--406},
title = {{Modellgest{\"{u}}tzte {\"{U}}berwachung und Fehlerdiagnose f{\"{u}}r Kraftfahrzeuge}},
year = {2006}
}
@article{Implantable,
author = {Implantable, Active and Devices, Medical},
pages = {435--465},
title = {{Index terms A}}
}
@article{Kontinuumsmechanik2013,
author = {Kontinuumsmechanik, Grundlagen D E R},
number = {November},
pages = {1--46},
title = {{Prozesssimulation in Der Einf{\{}{\"{u}}{\}}hrung in Die Mathematischen}},
year = {2013}
}
@article{Robinson2003,
author = {Robinson, J S and Cudd, R L and Evans, J T},
doi = {10.1179/026708303225009373},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Empirical Fatigue Models + Validation/2003{\_}Robinson{\_}Creep resistant aluminium alloys - experiments overview with different alloys - Al2618T6.pdf:pdf},
issn = {0267-0836},
journal = {Mater. Sci. Technol.},
number = {2},
pages = {143--155},
title = {{Creep resistant aluminium alloys and their applications}},
url = {http://www.tandfonline.com/doi/full/10.1179/026708303225009373},
volume = {19},
year = {2003}
}
@article{Energieb,
author = {Energie, Thermische and Energie, Mechanische and Energie, Elektrische},
title = {{2 Einf{\{}{\"{u}}{\}}hrung in die Funktionsweise von Verbren- nungsmotoren}}
}
@article{Bergmann2008,
abstract = {Allgemeine Grundlagen; Elektrische Hilfsmittel und Messverfahren; Elektronische Hifsmittel und Messger{\"{a}}te; Elektrische Messung nichtelektrischer Gr{\"{o}}{\ss}en; Elektrische Messanlagen; Systemtheorie der Messtechnik;},
author = {Bergmann, Kurt},
doi = {10.1007/978-3-663-01616-8},
isbn = {978-3-528-54080-7},
issn = {0937-7433},
title = {{Elektrische Messtechnik}},
url = {http://link.springer.com/10.1007/978-3-663-01616-8},
year = {2008}
}
@article{Brennraum,
author = {Brennraum, Der},
title = {{7 Reale Arbeitsprozessrechnung}}
}
@article{Tragfliigelstromung,
author = {Tragfliigelstromung, B},
title = {{4 Numerische Losungsmethoden}}
}
@article{Starten,
author = {Starten, Das},
title = {{Start- und Z{\{}{\"{u}}{\}}ndhilfesysteme}}
}
@article{Burgd,
author = {Burg, Heinz and Moser, Andreas and Steffan, Hermann},
journal = {Messtechnik},
pages = {59--71},
title = {{A3 A3 Messtechnik A3}}
}
@article{Garbe,
author = {Garbe, Juergen and Martinsohn, Matthias},
pages = {801--810},
title = {{C7 C7 Fahrzeugschl{\{}{\"{u}}{\}}ssel C7}}
}
@article{Dietmann1973,
author = {Dietmann, H},
doi = {10.1002/mawe.19730040608},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Empirical Fatigue Models + Validation/1973{\_}Dietmann Materialwissenschaft{\_}und{\_}Werkstofftechnik{\_}ExperimentelleUntersuchungenZuFatigue.pdf:pdf},
issn = {15214052},
journal = {Materwiss. Werksttech.},
number = {6},
pages = {322--333},
title = {{Werkstoffverhalten unter mehrachsiger schwingender Beanspruchung. Teil 2: Experimentelle Untersuchungen}},
volume = {4},
year = {1973}
}
@article{Sangid2013a,
abstract = {The fatigue life of a component can be expressed as the sum of two segments of life: (a) the number of loading cycles required to initiate a crack and (b) the number of cycles it takes that crack to propagate to failure. In this review, the primary emphasis is relating the fatigue crack initiation to the microstructure of the material. Many studies have focused on this phenomenon over the years and the goal of this paper is to put this work in perspective and encourage future work of fatigue in polycrystals based on the material's microstructure. In order to address fatigue, it is necessary to understand the mechanisms that facilitate crack initiation. Slip irreversibilities exist in a material and accumulate during fatigue loading. At the defect level, irreversibilities are a result of dislocations: annihilating, cross-slipping, penetrating precipitates, transmitting through grain boundaries, and piling-up. These slip irreversibilities are the early signs of damage during cyclic loading. The dislocations subsequently form low-energy, stable structures as a means to accommodate the irreversible slip processes and increasing dislocation density during cyclic forward and reverse loading. The result is strain localizing in a small region within the materials, i.e. persistent slip bands and dislocation cells/bundles. Strain localization is a precursor to crack initiation. This review paper will focus on experimental observations of strain localization and the theory and numerical analysis of both slip irreversibilities and low energy configuration defect structures. This fundamental understanding is necessary to study persistent slip bands in FCC metals and alloys including the appropriate characterization, theory, and modeling. From this fundamental knowledge both micromechanical and crystal plasticity models can be used to predict crack initiation, which are also reviewed. Finally, this review ends with a discussion of the future of fatigue modeling and experiments. ?? 2012 Elsevier B.V. All rights reserved.},
author = {Sangid, Michael D.},
doi = {10.1016/j.ijfatigue.2012.10.009},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2012{\_}Sangid{\_}The physics of fatigue crack initiation.pdf:pdf},
isbn = {01421123},
issn = {01421123},
journal = {Int. J. Fatigue},
keywords = {Crack initiation,Fatigue,Microstructure,Persistent slip bands,Slip irreversibility},
pages = {58--72},
publisher = {Elsevier Ltd},
title = {{The physics of fatigue crack initiation}},
url = {http://dx.doi.org/10.1016/j.ijfatigue.2012.10.009},
volume = {57},
year = {2013}
}
@article{Haque,
author = {Haque, Enarnul and Leach, Burr Bud L},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/{\_}buecherSong/HandbookofComposites/II/17{\_}MatchedMetalCompressionMoldingofPolymerComposites.pdf:pdf},
journal = {Composites},
title = {{Matched Metal Compression Molding of Polymer Composites}}
}
@article{Gross2011c,
author = {Gross, Dietmar and Seelig, Thomas},
doi = {10.1007/978-3-642-10196-0},
isbn = {978-3-642-10195-3},
title = {{Bruchmechanik}},
url = {http://link.springer.com/10.1007/978-3-642-10196-0},
year = {2011}
}
@article{Drucka,
author = {Druck, Der},
doi = {10.1007/978-3-8348-2230-7},
isbn = {9783834822307},
pages = {204--284},
title = {{Grundgleichungen der Str{\{}{\"{o}}{\}}mungsmechanik}}
}
@article{Sauzay2000a,
author = {Sauzay, M and Gilormini, P},
doi = {10.1046/j.1460-2695.2000.00307.x},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2000{\_}Sauzay{\_}Surface and cyclic microplasticity{\_}SurfaceAndPlasticityInMicro.pdf:pdf},
issn = {8756758X},
journal = {Fatigue Fract. Eng. Mater. Struct.},
keywords = {crystallographic glide,fatigue,free surface,microplasticity},
number = {7},
pages = {573--579},
title = {{Surface and cyclic microplasticity}},
volume = {23},
year = {2000}
}
@article{Anteil2008,
author = {Anteil, Der},
doi = {10.1007/978-3-642-14470-7},
isbn = {9783540688877},
pages = {431--439},
title = {{Kapitel 12}},
year = {2008}
}
@article{Forestd,
author = {Forest, Samuel},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/Folien CISM Summer School Mai2017 - Mesoscale Models/courses{\_}C1703{\_}forest{\_}Forest1-Micromorphic.pdf:pdf},
title = {{Micromorphic media}}
}
@article{Verbesserung,
author = {Verbesserung, Durch},
journal = {Stand},
pages = {261--334},
title = {{11 Einfl{\"{u}}sse der Benzin-Direkteinspritzung auf weitere Motor-Einzelsysteme}}
}
@article{Moto,
author = {Moto, Das and Motorrad, Beim and Bremsen, Die and Karo, Die and Lese, Der and Verst, Zum and Fahrdynamik, Kapitel and Radstand, Der},
pages = {259--326},
title = {{Fahrwerk 8 Konstruktive Auslegung von Motorradfahrwerken}}
}
@article{Wallentowitz2006n,
author = {Wallentowitz, Henning and Reif, Konrad},
journal = {Handb. Kraftfahrzeugelektronik - Grundlagen, Kompon. Syst. Anwendungen},
title = {{Back Matter}},
url = {http://www.springerlink.com/index/10.1007/978-3-8348-9121-1},
year = {2006}
}
@article{Evans1998,
abstract = {Today, fiber reinforced composites are in use in a variety of structures, ranging from spacecraft to aircraft to buildings and bridges. This wide use of composites has been facilitated by the introduction of new materials, improvements in manufacturing processes and developments of new analytical and testing methods. Unfortunately, information on these topics is scattered in journal articles, in conference and symposium proceedings, in workshop notes, and in government and company reports. This proliferation of the source material, coupled with the fact that some of the relevant publications are hard to find or are restricted, makes it difficult to identify and obtain the up-to-date knowledge needed to utilize composites to their full advantage. This book intends to overcome these difficulties by presenting in a single volume, many of the recent advances in the field of composite materials.},
author = {Evans, Don O.},
doi = {10.1007/978-1-4615-6389-1_23},
isbn = {0412540207},
journal = {Handb. Compos.},
pages = {476--487},
title = {{Fiber Placement}},
url = {http://link.springer.com/10.1007/978-1-4615-6389-1{\_}23},
volume = {21},
year = {1998}
}
@article{Ocko1998,
author = {Ocko, B M and Sirota, E B and Sinha, S K and Deutsch, M and Cao, B H and Wu, X Z and Flagan, R C and Vortisch, H and Leisner, T and Schwell, M and Ruehl, E},
doi = {10.1007/978-3-540-89141-3},
isbn = {0446512516},
journal = {Interface},
number = {14},
pages = {127--133},
title = {{Literaturverzeichnis [1]}},
volume = {91},
year = {1998}
}
@article{Table,
author = {Table, Truth and Table, Function},
number = {1},
title = {{2 Die Peripherie des µ-Controllers}}
}
@book{Schade2006,
author = {Schade, Heinz and Neemann, Klaus},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Schade, Neemann 2006 - Tensoranalysis.pdf:pdf},
isbn = {3110147416},
pages = {398},
title = {{Tensoranalysis}},
url = {http://www.amazon.de/dp/3110147416},
year = {2006}
}
@article{Dell2003,
author = {Dell, Trues-},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/B{\"{u}}cher{\_}Sammlung{\_}ITM/Elasticity and Plasticity of large deformations - Bertram/fulltext1.pdf:pdf},
number = {2000},
pages = {91--110},
title = {{Placements of Bodies}},
year = {2003}
}
@article{Berg1998,
author = {Berg, Kenneth R},
title = {{Typical Properties for Advanced Composites}},
year = {1998}
}
@article{Zahoransky2013e,
author = {Zahoransky, Richard A and Allelein, Hans-Josef and Schelling, Udo and Schwarz, Harald and Bollin, Elmar and Oehler, Helmut},
doi = {10.1007/978-3-8348-2279-6},
isbn = {978-3-8348-1869-0},
journal = {Energietechnik - Syst. zur Energieumwandlung},
pages = {30},
title = {{9 Brennstoffzellen}},
url = {http://www.springerlink.com/index/10.1007/978-3-8348-2279-6},
year = {2013}
}
@article{Forte2014a,
abstract = {A methodology for the evaluation of the effects of twin spark ignition system on CCV (Cycle by Cycle Variability) and knocking combustions is here presented, based on both the use of Computation Fluid Dynamics (CFD) tools and experimental information. The focus of the numerical methodology is the statistical evaluation of the local air-to-fuel distribution at the spark plugs and its correlation with the variability of the initial stages of combustion. A detailed analysis of knocking events can help improving engine performance and diagnosis strategies. The use of twin spark ignition system can enhance the probability that the initial kernel could come across a zone with the correct air-to-fuel ratio, thus lowering the initial combustion instabilities. Moreover the lower distance swept from the flame fronts can considerably reduce the time for the unburnt mixture to auto-ignite, thus reducing the risk of knocking combustion. CFD simulations have been used to reproduce knock effect on the in-cylinder pressure trace. The pressure signal holds information about waves propagation and heat losses: it is crucial to relate local pressure oscillations to knock severity. For this purpose, a CFD model has been implemented, able to predict the combustion evolution with respect to Spark Advance, from non-knocking up to heavy knocking conditions. The CFD model validation phase is essential for a correct representation of both regular and knocking combustions: the operation has been carried out by means of an accurate statistical analysis of experimental in-cylinder pressure data. ?? 2013 The Authors.},
author = {Forte, Claudio and Bianchi, Gian Marco and Corti, Enrico and Fantoni, Stefano and Costa, Marco},
doi = {10.1016/j.egypro.2014.01.091},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Klopfen{\_}Ottomotor/2014{\_}Forte+Corti+Bianchi{\_}CFD Methodology for the evaluation of knock of a PFI Twin Spark Engine.pdf:pdf},
isbn = {3905120933},
issn = {18766102},
journal = {Energy Procedia},
keywords = {Cycle by Cycle Variability,High performance engine,Knock,Twin spark},
pages = {859--868},
publisher = {Elsevier B.V.},
title = {{CFD methodology for the evaluation of knock of a PFI Twin spark engine}},
url = {http://dx.doi.org/10.1016/j.egypro.2014.01.091},
volume = {45},
year = {2014}
}
@article{Aufbaua,
author = {Aufbau, Vom and Technik, Diese and Anwendungen, Neuere and Kraftaufteilung, Die and Bauprinzip, Das and St, Die and Schubfeld, Rechteckiges and Belastung, Nutzfahrzeug Als},
title = {{13 Schubfeld-Konstruktionen}}
}
@book{Boelter1965,
address = {New York},
author = {Boelter, L. M. K. and Cherry, V. H. and Johnson, H. A. and Martinelli, R.C.},
publisher = {McGraw-Hill Book Company},
title = {{Heat Transfer Notes}},
year = {1965}
}
@article{Murakami2012g,
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Murakami, Sumio},
doi = {10.1007/978-94-007-2666-6},
eprint = {arXiv:1011.1669v3},
isbn = {978-94-007-2665-9},
issn = {09250042},
number = {1986},
pmid = {25246403},
title = {{Continuum Damage Mechanics}},
url = {http://link.springer.com/10.1007/978-94-007-2666-6},
volume = {185},
year = {2012}
}
@article{Zienkiewicz2005d,
author = {Zienkiewicz, O C and Taylor, R L},
doi = {http://dx.doi.org/10.1016/B978-075066431-8.50203-4},
isbn = {978-0-7506-6431-8},
journal = {Finite Elem. Method Solid Struct. Mech.},
pages = {498--516},
title = {{Semi-analytical finite element processes – use of orthogonal functions and ‘ finite strip ' methods}},
year = {2005}
}
@article{Wallentowitz2006b,
author = {Wallentowitz, Henning and Reif, Konrad},
doi = {10.1007/978-3-8348-9121-1},
isbn = {978-3-528-03971-4},
journal = {Handb. Kraftfahrzeugelektronik},
pages = {40},
title = {{15 Elektromagnetische Vertr{\{}{\"{a}}{\}}glichkeit}},
url = {http://www.springerlink.com/index/10.1007/978-3-322-82991-7{\%}7B{\%}25{\%}7D5Cnhttp://www.springerlink.com/index/10.1007/978-3-8348-9121-1},
year = {2006}
}
@inproceedings{Wisniewski1998,
abstract = {An experimental study was conducted in order to determine some heat transfer coefficients and to measure temperatures and heat fluxes in exhaust valves of 4C90 diesel engine. Measurements were performed both on a model stand and on a firing engine.The experimental stand for model studies was built with use of 4C90 engine parts. The thermal contact conductance between a valve face and a seat as a function of mechanical load was determined. Heat transfer between valve face and seat and between valve stem and guide was measured in some range of valve gear speed.The temperatures and heat fluxes, measured in exhaust valves and valve seat of firing 4C90 diesel engine, were presented as a function of its torque and speed.},
author = {Wisniewski, Tomasz S},
booktitle = {Int. Congr. Expo.},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Heat transfer intake+exhaust system/1998{\_}Wisniewski{\_}Experimental Study of Heat Transfer on Exhaust Valves of 4C90 Diesel Engine.pdf:pdf},
month = {feb},
publisher = {SAE International},
title = {{Experimental Study of Heat Transfer on Exhaust Valves of 4C90 Diesel Engine}},
year = {1998}
}
@article{Eekoye1996,
abstract = {Heat-transfer rates present in an engine cylinder undergoing knock are known to be larger than the rates associated with normal engine operation. Further, at the time of knock, the largest heat fluxes are associated with locations on the cylinder wall where the flame is locally quenching. In this study, heat-transfer processes at the flame-wall interface during a knock event are investigated computationally and analytically. Computationally, the governing equations for a one-dimensional, flame-quenching event are solved using a reduced chemical reaction mechanism. Analytically, scaling relations for the flame heat-release rates are used in the governing equations to determine the heat-transfer rates. It is found that while pressure transients modify the wall heat flux, the absolute value of the pressure is the most significant parameter in predicting the maximum heat flux. The wall heat flux profiles are predicted for both the analytical and computational models. In the range of pressures examined, a linear relationship was found between the peak flux and pressure, both for the computational and analytical models. The linear relationship between the pressure and peak flux was found to be invalid when the flame-quenching process was disrupted by the pressure fluctuations for pressure oscillations with a characteristic time on the order of the quenching process. ?? 1996 Combustion Institute.},
author = {Eekoye, O A},
doi = {10.1016/S0082-0784(96)80101-9},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/1996{\_}Ezekoye{\_}Heat transfer modeling during knock and flame quenching in an engine chamber.pdf:pdf},
isbn = {0082-0784},
issn = {00820784},
journal = {Symp. Combust.},
number = {2},
pages = {2661--2668},
title = {{Heat transfer modeling during knock and flame quenching in an engine chamber}},
volume = {26},
year = {1996}
}
@inproceedings{Tillock1996,
author = {Tillock, Brad R and Martin, Jay K},
booktitle = {SAE Tech. Pap. 961731},
file = {:C$\backslash$:/Users/p327208/Desktop/Promotion/Literature/Motorspezifisch/Heat Transfer Combustion Chamber/1996{\_}Tillock{\_}Meausrement and Modeling of Thermal Flows in an Air-Cooled Engine.pdf:pdf},
publisher = {SAE international},
title = {{Measurement and Modeling of Thermal Flows in an Air-Cooled Engine}},
year = {1996}
}
@article{Luftschall,
author = {Luftschall, Direkter and Biegeschwin-, Allgemeinen and Ger, Das and Lokalisierung, Zur and Motor-, Quellen and Anschl, Linearantriebe and Bild, Rohrleitungen and Betriebskr, Typische and Schaffung, Die},
title = {{26 Strukturakustik}}
}
@misc{Boeff,
author = {Boeff, Martin and Gutknecht, Florian and Engels, Philipp S and Ma, Anxin},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/2015{\_}Boeff{\_}Formulation of nonlocal damag models based on spectral methods for application to complex micostructures.pdf:pdf},
keywords = {nonlocal damage modelling,plasticity,rve,spectral solver},
title = {{Formulation of nonlocal damage models based on spectral methods for application to complex microstructures}}
}
@article{Reifenh,
author = {Reifenh, Die and Zugriff, Anwender},
pages = {169--184},
title = {{25 Fahrgastzelle 25.1}}
}
@misc{Vagera1971a,
author = {Vagera, I},
booktitle = {Scr. Met.},
doi = {10.1016/0036-9748(71)90036-6},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/1971{\_}Vagera{\_}A PileUp or a dislocation model of crack in an interface between two isotropic or anisotropic media.pdf:pdf},
issn = {00369748},
number = {2},
pages = {93--96},
title = {{A pile-up or a dislocation model of crack in an interface between two isotropic or anisotropic media}},
volume = {5},
year = {1971}
}
@article{Verbindungstechnologien,
author = {Verbindungstechnologien, Die and Von, Leichtbau},
title = {{22 Verbindungstechnik}}
}
@article{Fan1992,
author = {Fan, H and Keer, L M},
doi = {10.1016/0013-7944(92)90059-N},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/1977{\_}Morris{\_}The early stage of fatigue crack propagation in al 2048.pdf:pdf},
issn = {00137944},
journal = {Eng. Fract. Mech.},
number = {5},
pages = {789--796},
title = {{The early stage of fatigue crack propagation}},
volume = {42},
year = {1992}
}
@article{Cimmelli2014,
abstract = {We present the state of the art on the modern mathematical methods of exploiting the entropy principle in thermomechanics of continuous media. A survey of recent results and conceptual discussions of this topic in some well-known non-equilibrium theories (Classical irreversible thermodynamics CIT, Rational thermodynamics RT, Thermodynamics of irreversible processes TIP, Extended irreversible thermodynamics EIT, Rational Extended thermodynamics RET) is also summarized.},
author = {Cimmelli, Vito Antonio and Jou, David and Ruggeri, Tommaso and V??n, P??ter},
doi = {10.3390/e16031756},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Thermodynamik/Entropy Principle and Recent Results in Non Equilibrium Theories{\_}Cimmelli .pdf:pdf},
issn = {10994300},
journal = {Entropy},
keywords = {Classical irreversible thermodynamics,Continuum thermodynamics,Entropy principle,Exploitation of second law,Extended irreversible thermodynamics,Rational extended thermodynamics,Rational thermodynamics},
number = {3},
pages = {1756--1807},
title = {{Entropy principle and recent results in non-equilibrium theories}},
volume = {16},
year = {2014}
}
@article{Sanli2009a,
author = {Sanli, A. and Sayin, C. and Gumus, M. and Kilicaslan, I. and Canakci, M.},
file = {:C$\backslash$:/Users/p327208/Desktop/Promotion/Literature/Motorspezifisch/2009{\_}Sanli{\_}Numerical evaluation by models of load and spark timing effects on the in-cylinder heat transfer of a si engine.pdf:pdf},
journal = {Numer. Heat Transf. Part A Appl.},
number = {5},
pages = {444--458},
title = {{Numerical Evaluation by Models of Load and Spark Timing Effects on the In-Cylinder Heat Transfer of a SI Engine}},
volume = {56},
year = {2009}
}
@article{Laser2006,
author = {Laser, Das Licht Der},
journal = {Gerthsen Phys.},
pages = {823--882},
title = {{15 - Laserphysik}},
year = {2006}
}
@article{Zienkiewicz2000,
author = {Zienkiewicz, O C and Taylor, R L},
doi = {10.1016/B978-1-85617-633-0.00034-4},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Zienkiewicz FEM - Vol 1 Basics Fundamentals/63205{\_}apdxi.pdf:pdf},
isbn = {9781856176330},
journal = {finite Elem. method Vol. 1 basis},
pages = {648--653},
title = {{Matrix diagonalization or lumping}},
year = {2000}
}
@article{Aslan2011,
abstract = {Proper life-time prediction modeling of single crystalline components is of increasing importance due to their common use in turbine industry. Viscoplastic damage approaches are of great interest in that context. However, mechanical properties of single crystals are strongly anisotropic and nonlinear in service conditions, bringing certain complexity into constitutive and numerical modeling. The aim of this work is to develop a thermodynamically consistent constitutive model based on generalized continua in order to simulate fatigue crack initiation and growth in single crystals. For that purpose, a standard crystal plasticity model is taken as a basis and coupled with the continuous damage model developed by Marchal et al. (2006a) [Marchal, N., Forest, S., Remy, L. and Duvinage, S. (2006a). Simulation of Fatigue Crack Growth in Single Crystal Superalloys Using Local Approach to Fracture, In: Moinereau, D., Steglich, D. and Besson, J. (eds.), Local Approach to Fracture, 9th European Mechanics of Materials Conference, Euromech–Mechamat, Moret–Sur–Loing, France, Presses de l'Ecole des mines de Paris, pp. 353–358]. As a variant of micromorphic theory, microdamage approach is applied to the model in order to obtain a regularized continuum damage formulation which solves mesh dependency problem by introducing an intrinsic length scale. A detailed finite element implementation procedure and its validation for monotonic crack growth areshown. Fatigue crack growth analyses have been performed on a single edge notched geometry and a comparison between numerical and experimental results is presented.},
author = {Aslan, Ozgur and Quilici, St{\'{e}}phane and Forest, Samuel},
doi = {10.1177/1056789510395738},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/2011{\_}Aslan{\_}Numerical Modeling of Fatigue Crack Growth in Single Crystals Based on micodamage theory.pdf:pdf},
issn = {1056-7895},
journal = {Int. J. Damage Mech.},
number = {5},
pages = {681--705},
title = {{Numerical Modeling of Fatigue Crack Growth in Single Crystals Based on Microdamage Theory}},
url = {http://journals.sagepub.com/doi/10.1177/1056789510395738},
volume = {20},
year = {2011}
}
@article{Dimensionierung2011,
author = {Dimensionierung, Die},
doi = {10.1007/978-3-8348-8279-0},
isbn = {9783834882790},
title = {{3 Festigkeitsberechnung 3 3.1}},
year = {2011}
}
@article{Le2012a,
author = {Le, K C},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2012{\_}Le{\_}Continuum dislocation theory-size effects and formation of microstructure{\_}Lecture Bad Herrenalb.pdf:pdf},
title = {{Continuum dislocation theory : size effects and formation of microstructure}},
year = {2012}
}
@article{M1959,
author = {M, M Grundlagen Der Elektrotechnik},
doi = {10.1002/prop.19590071309},
journal = {Fortschritte der Phys.},
number = {S1},
pages = {162--167},
title = {{Literaturverzeichnis}},
volume = {7},
year = {1959}
}
@article{Mughrabi2013a,
abstract = {The primary cause of fatigue damage is usually intimately related to some form of cyclic slip irreversibilities. Depending on material and details of the loading conditions, various types of fatigue crack initiation are observed. Here, typical examples of fatigue damage evolution in low and high cycle fatigue (LCF, HCF) and ultrahigh cycle fatigue (UHCF) will be discussed. Various forms of fatigue damage and life-controlling microstructural mechanisms in different metals and alloys will be illustrated. In particular, the fatigue properties of ultrafine-grained (UFG) materials will be discussed, and the microstructural mechanisms and the question of the existence of a fatigue limit in the UHCF regime will be considered. ?? 2013 The Authors.},
author = {Mughrabi, Hael},
doi = {10.1016/j.proeng.2013.03.307},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2013{\_}Mughrabi{\_}Damage mechanisms and fatigue lives - From the low to the very high cycle regime.pdf:pdf},
isbn = {9781627486361},
issn = {18777058},
journal = {Procedia Eng.},
keywords = {Fatigue crack initiation,Fatigue limit,Fatigue lives,HCF,LCF,UHCF},
pages = {636--644},
publisher = {Elsevier B.V.},
title = {{Damage mechanisms and fatigue lives: From the low to the very high cycle regime}},
url = {http://dx.doi.org/10.1016/j.proeng.2013.03.307},
volume = {55},
year = {2013}
}
@article{Models1992a,
author = {Models, Mathematical},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Anisotropic Behaviouir of Damaged Materials{\_}Skrzypek{\_}ARTICEL/Kap1{\_}Applications of Tensor Functions in Damage Mechanics of Anisotropic Materials.pdf:pdf},
keywords = {anisotropy,canonical form,constitutive equations,continuum damage,creep,creep rupture,creep rupture time,damage tensor,evolutional equa-,irreducible invariants,material,material behaviour,mechanics,monkman-grant relationship,net-stress concept,tensor,tensor function,tensor generator,tensorial interpolation,ter-,tions},
number = {January},
pages = {47--59},
title = {{Applications of Tensor Functions in Continuum Damage Mechanics}},
year = {1992}
}
@article{Rangarajan2012,
abstract = {We describe a method for discretizing planar C2-regular domains immersed in non-conforming triangulations. The method consists in constructing mappings from triangles in a background mesh to curvilinear ones that conform exactly to the immersed domain. Constructing such a map relies on a novel way of parameterizing the immersed boundary over a collection of nearby edges with its closest point projection. By interpolating the mappings to curvilinear triangles at select points, we recover isoparametric mappings for the immersed domain defined over the background mesh. Indeed, interpolating the constructed mappings just at the vertices of the background mesh yields a fast meshing algorithm that involves only perturbing a few vertices near the boundary. For the discretization of a curved domain to be robust, we have to impose restrictions on the background mesh. Conversely, these restrictions define a family of domains that can be discretized with a given background mesh. We then say that the background mesh is a universal mesh for such a family of domains. The notion of universal meshes is particularly useful in free/moving boundary problems because the same background mesh can serve as the universal mesh for the evolving domain for time intervals that are independent of the time step. Hence it facilitates a framework for finite element calculations over evolving domains while using a fixed background mesh. Furthermore, since the evolving geometry can be approximated with any desired order, numerical solutions can be computed with high-order accuracy. We demonstrate these ideas with various numerical examples.},
archivePrefix = {arXiv},
arxivId = {1201.4903},
author = {Rangarajan, Ramsharan and Lew, Adrian J.},
doi = {10.1002/nme},
eprint = {1201.4903},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/2010{\_}Miehe{\_}Thermodynamically consistent phase-field models of fracture-Variational principles and multi field FE implementations.pdf:pdf},
keywords = {coupled multi-field problems,crack propagation,finite elements,fracture,gradient-type damage,incremental variational,phase-fields,principles},
number = {March},
pages = {1273--1311},
title = {{Universal Meshes: A new paradigm for computing with nonconforming triangulations}},
url = {http://arxiv.org/abs/1201.4903},
year = {2012}
}
@article{Anwendungsfelder,
author = {Anwendungsfelder, Bevorzugte and Versteifungen, Schalenartige and Herstellung, Die and Blechdicke, Die},
title = {{20 Konstruktive Versteifungen}}
}
@article{Kommunalbereich1897,
author = {Kommunalbereich, Der},
title = {18.1.1},
year = {1897}
}
@article{Felder,
author = {Felder, Formen},
number = {Din 42401},
title = {{8 Mehrphasiger Wechselstrom}}
}
@article{Crisfield1996,
abstract = {applicability for this approach.},
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Crisfield, Mike a},
doi = {10.1017/CBO9781107415324.004},
eprint = {arXiv:1011.1669v3},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Crisfield 2000 - Non-Linear Finite Element Analysis Of Solids And Structures Advanced Topics.pdf:pdf},
isbn = {978-0-470-66644-9},
issn = {1098-6596},
journal = {John Wiley Sons, Inc.},
keywords = {icle},
pages = {31--62},
pmid = {25246403},
title = {{Nonlinear Finite Element Analysis of Solids and Structures}},
url = {http://eu.wiley.com/WileyCDA/WileyTitle/productCd-0470666447.html},
year = {1996}
}
@article{Meister2011,
abstract = {Die wichtigsten Verfahren zur numerischen L{\"{o}}sung von linearen Gleichungssystemen in einer umfassenden Einf{\"{u}}hrung, die zum Verst{\"{a}}ndnis nur geringe mathematische Vorkenntnisse ben{\"{o}}tigt. Behandelt werden sowohl die direkten als auch die iterativen Verfahren, wobei der Autor gro{\ss}en Wert auf eine sorgf{\"{a}}ltige Herleitung dieser Verfahren legt. Au{\ss}erdem sind sehr detaillierte Pseudocodes enthalten, mit deren Hilfe sich die jeweiligen Verfahren in einer beliebigen Programmiersprache sofort auf dem Computer realisieren lassen. Das Lehrbuch ist auch f{\"{u}}r Natur- und Ingenieurwissenschaftler geeignet, die in vielen praktischen Anwendungen mit der L{\"{o}}sung von linearen Gleichungssystemen konfrontiert sind.},
archivePrefix = {arXiv},
arxivId = {1011.1669v3},
author = {Meister, Andreas},
doi = {10.1007/978-3-8348-8100-7},
eprint = {1011.1669v3},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/Numerik linearer Gleichungssysteme{\_}Andreas Meister/Kapitel6-Implementierung MATLAB.pdf:pdf},
isbn = {978-3-8348-1550-7},
issn = {1098-6596},
journal = {Matrix},
pages = {36--68},
pmid = {25246403},
title = {{Numerik linearer Gleichungssysteme}},
url = {http://link.springer.com/10.1007/978-3-8348-8100-7},
year = {2011}
}
@article{Timoshenko,
author = {Timoshenko, The},
title = {{Structural mechanics problems in one dimension – rods}}
}
@book{Elshahawy2008a,
author = {Elshahawy, Waleed},
isbn = {0120020211},
title = {{Advances i}},
year = {2008}
}
@article{Results1994,
abstract = {As a concluding comment, I should like to return to the point raised by Ayres, that it is not enough simply to tell a better version of the fourth-century history in the expectation that modern theologians will finally get it straight! This is a valid point: if we want to have Christianity's fourth-century heritage taken seriously, we need to be in dialogue with modern writers. But, if there is to be a dialogue, both sides must be allowed to speak, and so we are also responsible for expounding the historical material on its own terms. As Heidegger put it, “[O]nly when we think through what has been thought will we be of any use for what must still be thought.” Perhaps studying the figures from a distant era will open up for us possibilities we would never have dreamed of within our own modern presuppositions, so that we can recognize differences even beyond those which lie within our own horizon or tradition. If I am right in affirming that there is a different style of doing theology prior to Augustine and after him in the East than that which we find in the theological and scholarly tradition in which Ayres's book stands, then we must ask whether we need to address the question of the legitimacy of each (and ponder how one might even answer that) or whether a plurality of approaches is possible without reducing one to the other. In a way, this would be a further step toward deconstructing monolithic notions of “Orthodoxy” in recognition of genuine and legitimate diversity within early Christianity and among modern Christians. Might it be better not to speak of Nicaea and its legacy, but of the legacies of Nicaea—or better—“Christ and him crucified” (2 Cor 2:2) and the ways in which Nicaea and its interpreters affirm the true divinity of this one?},
author = {Results, Useful},
doi = {10.1007/BF02600226},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2010{\_}Jaroslav Pokluda+Pavel {\v{S}}andera{\_}Micromechanisms of fracture and fatigue{\_}Buch/Kap5{\_}FinalReflection.pdf:pdf},
isbn = {9780470434673},
issn = {08848734},
journal = {J. Gen. Intern. Med.},
number = {3 Supplement},
pages = {243--247},
title = {{Final reflections}},
volume = {9},
year = {1994}
}
@article{Ableitung,
author = {Ableitung, Die and Gleichungen, Reynoldsschen and Gleichungen, Navier-stokesschen and Messungen, Solche},
title = {{21 Einf u omungsmesstechnik ¨ hrung in die Str ¨}}
}
@article{Weng1987a,
abstract = {Based on the dislocation structures developed during plastic deformation, an anisotropic hardening law is developed to describe the latent hardening behavior of slip systems under multislip. This theory incorporates the concept of isotropic hardening, kinematic hardening, and the two-parameter representation; it automatically includes the strength differential between the forward and reversed slips and between the acute and obtuse cross slips. The self-hardening modulus of a slip system is found to be "associated" with the latent hardening law involved, and, based on some experimental evidence, two specific sets of self-hardening modulus are suggested. An important feature of this associated modulus is that the slip system with a soft latent hardening (e.g., the reversed system with a Bauschinge effect) will have an enhanced self-hardening modulus. This newly developed hardening law, together with its associated latent hardening moduli, is then applied to examine the strain-hardening behavior of a polycrystal. Although crystals with a stronger latent hardening will, in general, also lead to a stranger strain-hardening for the polycrystal, the stress-strain behavior of the polycrystal using the kinematic hardening law of single crystals is found to be not necessarily softer than that using the isotropic hardening law. Within the range of experimentally measured latent hardening ratio of slip systems, the anisotropic theory is also used to calculate the motion of yield surface of a polycrystal. The general results, employing four selected types of anisotropic hardening, all show the essential features of experimental observations by Phillips and his co-workers. The application is highlighted with a reasonably successful quantitative modeling of initial and subsequent yield surfaces of an aluminum. ?? 1987.},
author = {Weng, G J},
doi = {10.1016/0749-6419(87)90007-6},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/Hardening Recovery Creep/1987{\_}Weng{\_} IJP Anisotropic hardening of crystalls.pdf:pdf},
issn = {07496419},
journal = {Int. J. Plast.},
number = {4},
pages = {315--339},
title = {{Anisotropic hardening in single crystals and the plasticity of polycrystals}},
volume = {3},
year = {1987}
}
@article{Wallentowitz2006c,
author = {Wallentowitz, Henning and Reif, Konrad},
doi = {10.1007/978-3-8348-9121-1},
isbn = {978-3-528-03971-4},
journal = {Handb. Kraftfahrzeugelektronik},
pages = {23},
title = {{14 Mechatronische Systeme}},
url = {http://www.springerlink.com/index/10.1007/978-3-8348-9121-1},
year = {2006}
}
@article{Arnoldc,
author = {Arnold, J{\"{o}}rg and Braun, Marcel},
pages = {835--847},
title = {{C10 C10 Zuk{\"{u}}nftige Methoden bei der Spurensicherung C10 Neue M{\"{o}}glichkeiten und Bed{\"{u}}rfnisse}}
}
@article{Gallusa,
author = {Gallus, J{\"{u}}rgen and Gut, Thomas and Wolfer, Bernd and Wendevorg{\"{a}}ngen, Passier- and Verursachers, Feststellen},
journal = {Haut},
pages = {867--873},
title = {{C12 C12 Bemerkbarkeit von Kleinkollisionen C12}}
}
@article{Dimensionierung2011,
author = {Dimensionierung, Die},
doi = {10.1007/978-3-8348-8279-0},
isbn = {9783834882790},
title = {{3 Festigkeitsberechnung 3 3.1}},
year = {2011}
}
@article{Haslam2013a,
author = {Haslam, Antony and Laskaridis, Panos},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2010{\_}Jaroslav Pokluda+Pavel {\v{S}}andera{\_}Micromechanisms of fracture and fatigue{\_}Buch/Kap4{\_}FatigueFracture.pdf:pdf},
journal = {Adv. Mater. Process.},
number = {April},
title = {{Fatigue {\{}{\&}{\}} Fracture}},
year = {2013}
}
@article{Zienkiewicz2005e,
author = {Zienkiewicz, O},
doi = {10.1016/B978-075066431-8/50226-5},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Zienkiewicz FEM - Vol 1 Basics Fundamentals/63205{\_}apdxg.pdf:pdf},
isbn = {9780750664318},
pages = {699--700},
title = {{Integration by parts in two or three dimensions (Green}},
year = {2005}
}
@article{Forestd,
author = {Forest, Samuel},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/Folien CISM Summer School Mai2017 - Mesoscale Models/Slides{\_}CISM{\_}SummerSchool2017.pdf:pdf},
title = {{Micromorphic media}}
}
@phdthesis{Hadzic1999,
author = {Hadzic, Ibrahim},
school = {Technical University of Delft},
title = {{Second-moment closure modeling of transitional and unsteady turbulent flows}},
year = {1999}
}
@article{Gross2011a,
author = {Gross, Dietmar and Seelig, Thomas},
doi = {10.1007/978-3-642-10196-0},
isbn = {978-3-642-10195-3},
title = {{Bruchmechanik}},
url = {http://link.springer.com/10.1007/978-3-642-10196-0},
year = {2011}
}
@article{Erfolg,
author = {Erfolg, Neutraler},
pages = {2--6},
title = {{Teil a}}
}
@article{Haslam2013a,
author = {Haslam, Antony and Laskaridis, Panos},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/Micromechanisms of fracture and fatigue/Kap4{\_}FatigueFracture.pdf:pdf},
journal = {Adv. Mater. Process.},
number = {April},
title = {{Fatigue {\&} Fracture}},
year = {2013}
}
@article{Vorl1908,
author = {Vorl, Als},
number = {1829},
title = {{2 Wasserturbinen}},
year = {1908}
}
@article{Papula2011c,
author = {Papula, Lothar},
isbn = {978-3-38348-1227-8},
pages = {795},
title = {{Lothar Papula Mathematik f{\"{u}}r Ingenieure und Naturwissenschaftler Band 2}},
year = {2011}
}
@article{Meroth2008,
abstract = {Das Wort Infotainment ist ein Kunstwort, das sich aus den Begriffen Information und Unterhaltung (Entertainment) zusammensetzt. 75 Jahre nach Einf{\{}{\"{u}}{\}}hrung des ersten Autoradios hat sich Infotainment einen wertbestimmenden Rang im Automobil erobert. Sp{\{}{\"{a}}{\}}testens mit den Fahrerassistenzsystemen sind Fahrzeugfunktionen und Infotainment zu einer Einheit verschmolzen. Die Mindmap in Abbildung 1.1 zeigt einige Aspekte, die im Folgenden n{\{}{\"{a}}{\}}her erl{\{}{\"{a}}{\}}utert werden sollen.},
author = {Meroth, Ansgar and Tolg, Boris and Plappert, Christian},
isbn = {978-3-8348-9430-4},
journal = {Infotainmentsysteme im Kraftfahrzeug},
pages = {1--6},
title = {{Einf{\{}{\"{u}}{\}}hrung}},
url = {http://dx.doi.org/10.1007/978-3-8348-9430-4{\%}7B{\_}{\%}7D1},
year = {2008}
}
@article{Gerhard2005,
author = {Gerhard, Pahl.},
journal = {Konstr. Grundlagen erfolgreicher Produktentwicklung Methoden und Anwendung},
pages = {93--187},
title = {{3 Methoden zur Produktplanung, L{\{}{\"{o}}{\}}sungssuche und Beurteilung}},
year = {2005}
}
@article{Fr,
author = {Fr, Beim and Tiefe, Die and Beobachtung, Diese and Nach, U A},
title = {{Ergebnisse der Untersuchungen bearbeiteter Werkst{\{}{\"{u}}{\}}cke}}
}
@article{Jungbluth2007,
author = {Jungbluth, Niels and Spielmann, Michael and Dones, Roberto and Heck, Thomas and Emmenegger, Mireille Faist and Frischknecht, Rolf},
pages = {537},
title = {{Teil IV}},
year = {2007}
}
@article{Stromfunktion,
author = {Stromfunktion, Potential-},
title = {{Omungen}}
}
@article{Verger2002,
abstract = {This paper presents a global approach of thermomechanical design in the automotive industry. The three steps of the method are the following: the loading definition, the modelling of the constitutive law, a failure criterion. Cracked area and lifetime prediction are described in the case of aluminium alloy cylinder heads submitted to transient thermal loadings. The main hypothesis and modelling choices are presented and results are illustrated by a series of computations on real 3D structures. {\textcopyright} 2002 Elsevier Ltd. All rights reserved.},
author = {Verger, L. and Constantinescu, A. and Charkaluk, E.},
doi = {10.1016/S1566-1369(02)80087-5},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Kriechen{\_}Spannungsrelaxation/2002{\_}Verger{\_}THERMOMECHANICAL FATIGUE DESIGN OF ALUMINIUM COMPONENTS.pdf:pdf},
issn = {15661369},
journal = {Eur. Struct. Integr. Soc.},
number = {C},
pages = {309--318},
title = {{Thermomechanical fatigue design of aluminium components}},
volume = {29},
year = {2002}
}
@article{Buryachenko1995,
abstract = {We consider a linearly elastic composite medium, which consists of a homogeneous matrix containing a homogeneous and statistically uniform random set of ellipsoidal inclusions. Because of the differential thermal expansion, a microstructural residual stress state arises. By means of the "multiparticle effective field" method we first derive the functional relation between the stored elastic energy and the thermoelastic constants of the components. Using this result an exact estimation of all components of the statistical second moment tensor of the stress fields is given. Furthermore, an expression for the second moment of the stress in the matrix in the vicinity of the ellipsoidal inclusion and a correlation function of internal stresses is obtained. The application of the theory is demonstrated by some numerical results for a WC-Co composite. ?? 1995.},
author = {Buryachenko, Valeriy A and Kreher, Wolfgang S},
doi = {10.1016/0022-5096(95)00029-I},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Probabilistic Aspects/1995{\_}Kreher{\_}Internal residual stresses in heterogeneous solids - a statistical theory for particulate composites.pdf:pdf},
isbn = {0022-5096},
issn = {00225096},
journal = {J. Mech. Phys. Solids},
number = {7},
pages = {1105--1125},
title = {{Internal residual stresses in heterogeneous solids-A statistical theory for particulate composites}},
volume = {43},
year = {1995}
}
@article{Down1977,
author = {Down, Claverton},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/Strukturmechanik MMS/Literatur/HS Schranken Methodik MMS Vorlesung Details/Willis - 1977{\_}Uberblick{\_}Methodik{\_}HS{\_}Schranken.pdf:pdf},
pages = {185--202},
title = {{Bounds and Self-Consistent Estimates for the}},
volume = {25},
year = {1977}
}
@article{Oberbegriff,
author = {Oberbegriff, Emv-intrasystemma{\ss}nahmen Der},
title = {{7 Intrasystemma{\ss}nahmen}}
}
@book{Streicher-abel,
author = {Streicher-abel, Christian Demant Bernd},
booktitle = {Media},
doi = {10.1007/s10531-008-9469-2},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Schier 2011 - Finite Elemente Modelle der Statik und Festigkeitslehre.pdf:pdf},
isbn = {9783642130960},
title = {{1 C}}
}
@article{Bauer1998,
abstract = {Entry flow heat transfer experiments are reported in steady and pulsating flows of air at mean Reynolds numbers of 3000-35 000. THe ducts are chosen to match typical spark-ignition engine manifolds: a highly curved and a straight pipe, which together bracket most practical geometries. The pulsating engine intake flow encompasses an approximate half sine wave followed by a stagnant phase three itmes as long, all at a repetition rate of 16-50 Hz. Heat flow is imposed through electric heating of the outsides of the manifolds. Heat transfer in the curved pipe is closely comparable to the straight geometry, and it is concluded that entrance effects dominate. Time-averaged axially resolved and axially averaged Nusselt numbers are reported. The unsteady nature of the intake flow enhances heat transfer significantly, between 50{\%} and 100{\%}. Time-resolved wall heat flux measurements at a location close to the exit of the system show that heat transfer is delayed relative to the onset of the flow. During the stagnant flow phase, heat transfer and turbulence decay slowly from their high levels during the induction flow phase. Heat transfer enhancement in the pulsating flow case is caused by the contribution of the stagnant phase.},
author = {Bauer, Wolf D. and Wenisch, Joseph and Heywood, John B.},
doi = {https://doi.org/10.1016/S0142-727X(97)10001-7},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/1998{\_}Bauer{\_}Averaged and time-resolved heat transfer of steady and pulsating entry flow in intake manifold of a SI engine.pdf:pdf},
journal = {Int. J. Heat Fluid Flow},
keywords = {intake manifold,internal combustion engine,ow,pulsating,transient heat,ux measurements},
number = {1},
pages = {1--9},
title = {{Averaged and time-resolved heat transfer of steady and pulsating entry flow in intake manifold of a spark-ignition engine}},
volume = {19},
year = {1998}
}
@article{Muhs2007,
author = {Muhs, Dieter and Wittel, Herbert and Jannasch, Dieter and Vo{\ss}iek, Joachim},
doi = {10.1007/978-3-8348-9406-9},
isbn = {978-3-8348-0262-0},
journal = {Roloff / Matek Maschinenelemente},
pages = {21--36},
title = {{Toleranzen, Passungen, Oberfl{\"{a}}chenbeschaffenheit}},
url = {http://www.springerlink.com/index/10.1007/978-3-8348-9406-9},
year = {2007}
}
@article{Eq2015,
author = {Eq, Hence and Eqs, Comparing},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Zienkiewicz FEM - Vol 1 Basics Fundamentals/63205{\_}apdxh.pdf:pdf},
pages = {1--5},
title = {{Appendix H}},
year = {2015}
}
@article{Forest2004a,
abstract = {The modeling of damage processes at the material point scale through a specific constitutive law addresses a wide variety of constitutive behaviors, for instance brittle elasticity where the evolution of damage degrades the elastic stiffness, or ductile plasticity where both dissipative mechanisms (plasticity and damage) are intimately coupled. In spite of their obvious differences, all these laws possess a common feature: beyond some load level, the domain of reversibility expressed in the stress space shrinks. This phenomenon is called strain-softening. This essential property, characteristic of damage mechanisms, is responsible for the localization of the mechanical fields (strain, damage, plastic strain, . . .) inside narrow bands, an experimental fact observed on many degrading materials such as soils, concrete, metals, etc., see for instance Desrues and Chambon (1985). Despite twenty years of intensive research, numerical modeling of the localization phenomenon remains a challenging objective which has not yet been given a fully satisfactory answer. This is in contrast with the great progresses that have been achieved regarding the local description of damage mechanisms for various materials, on the basis of micro–macro derivations as well as phenomenological intuitions. Unfortunately, localization partially hinders predictive computations of propagating damaged zones in real-life structures submitted to a given load history. The difficulty originates from the fact that the equations that describe the structural behavior (including not only the constitutive law but also the equilibrium and compat-ibility equations) result in an ill-posed problem which manifests itself by a spurious mesh-dependency when making use of finite element solutions. After a first insight into the localization phenomena, the problem of loss of uniqueness and loss of ellipticity is addressed for elastoplastic solids. General (diffuse) and localized bifurcation modes are distinguished. The existence of jumps of the velocity gradient is explored in the dynamic (acceleration waves) and static cases (stationary waves). Critical values of hardening moduli for loss of uniqueness or loss of ellipticity are derived. A link between the notion of material stability and acceleration waves is also presented. The collected strain localization criteria are summarized in section 1.2.6. Note that the derivations and formula are presented in the case of elastoplastic ma-terials. However the results can be extended to damaging materials in a straightforward 311 312 Local approach to fracture manner. In fact it deals with all incremental models involving a fourth–rank tangent operator L ∼ ∼ .},
author = {Forest, S and Lorentz, E},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/xxx{\_}Forst+Lorentz{\_}Localization{\_}phenomena{\_}and{\_}regularization{\_}methods-damage.pdf:pdf},
journal = {Local Approach to Fract.},
pages = {311--371},
title = {{Localization phenomena and regularization methods}},
volume = {1},
year = {2004}
}
@article{Lotsch,
author = {Lotsch, H K V and Rhodes, Editor-in-chief W T and Adibi, Editorial Board A and Asakura, T and H{\"{a}}nsch, T W and Kamiya, T and Krausz, F and Monemar, B and Venghaus, H and Weber, H and Weinfurter, H and Rhodes, William T},
isbn = {9780387300696},
title = {{Springer Series in Springer Series in}}
}
@article{Hild2015b,
abstract = {{\{}{\textcopyright}{\}} Springer Science+Business Media New York 2015.This chapter is devoted to the evaluation of damage with digital image correlation (DIC). This measurement technique provides displacement fields that can be used to tune material parameters of damage models. The potential of DIC for identification purposes is illustrated hereafter for simple 1D-type geometries in the context of quasi-brittle and ductile behaviors. Beams and frames as encountered in civil engineering application can be described through damage laws. The localization of damage at single points (lumped damage mechanics) and the resulting damage law can be determined very precisely based on dedicated versions of DIC incorporating the descriptive language of beam theory. At smaller scale, plasterboards (plaster core lined with paper) constitute another example of a structure (rather than a material), which can be described as damageable. Those cases will be analyzed in details.},
author = {Hild, Fran{\c{c}}ois and Roux, St{\'{e}}phane},
doi = {10.1007/978-1-4614-5589-9},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/2015{\_}Sun+Liu{\_}Particel-Debonding modeling of metal-matrix composites.pdf:pdf},
isbn = {9781461455899},
journal = {Handb. Damage Mech. Nano to Macro Scale Mater. Struct.},
pages = {1277--1299},
title = {{Evaluating damage with digital image correlation: b. from physical to mechanical damage}},
year = {2015}
}
@article{Na,
author = {Na, Meoy},
title = {{12 Mehrk{\{}{\"{o}}{\}}rpersysteme}}
}
@article{Of2003,
author = {Of, Torsion and Bars, Prismatic},
pages = {181--194},
title = {{Torsion and Buckling 14.1}},
year = {2003}
}
@article{Turner1999,
author = {Turner, I M},
isbn = {0521801834},
journal = {Rain},
pages = {13--16},
title = {{Preface Acknowledgements 1}},
year = {1999}
}
@article{Hansen2005c,
abstract = {The strengthening effect of grain boundaries and dislocation boundaries is a traditional metallurgical theme, which at the present time is being revived. The reason is the scientific and industrial interest in strength obtained through a structural refinement. Such a refinement is found in nanocrystalline metals subdivided by grain boundaries and in heavily deformed metals subdivided by a mixture of dislocation boundaries and high angle boundaries. The structural dimension of these materials covers a scale form the nanometre range to the hundreds micrometers level i.e. five length scales. Consequently, a multiscale analysis has been applied to the relationship between strength and the boundary parameters. As an example this analysis suggests that the yield stress/grain size relationship follows the Hall-Petch relationship down to a grain size of about 15-20 nm showing large potential for strengthening of a metal through a structural refinement. {\textcopyright} 2005 WILEY-VCH Verlag GmbH {\&} Co. KGaA, Weinheim.},
author = {Hansen, Niels},
doi = {10.1002/adem.200500102},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2005{\_}Hansen Boundary Strengthing over 5 length scales.pdf:pdf},
isbn = {14381656 (ISSN)},
issn = {14381656},
journal = {Adv. Eng. Mater.},
number = {9},
pages = {815--821},
title = {{Boundary strengthening over five length scales}},
volume = {7},
year = {2005}
}
@article{Pang2004a,
abstract = {The performance of the conventional engine-cooling system has always been constrained by the passive nature of the system and the need to provide the required heat-rejection capability at high-power conditions. This leads to considerable losses in the cooling system at part-load conditions where vehicles operate most of the time. A set of design and operating features from advanced enginecooling systems is reviewed and evaluated for their potential to provide improved engine protection while improving fuel efficiency and emissions output. Although these features demonstrate significant potential to improve engine performance, their full potential is limited by the need to balance between satisfying the engine-cooling requirement under all operating ambient conditions and the system effectiveness, as with any conventional engine-cooling system. The introduction of controllable elements allows limits to be placed on the operating envelope of the cooling system without restricting the benefits offered by adopting these features. The integration of split cooling and precision cooling with controllable elements has been identified as the most promising set of concepts to be adopted in a modern engine-cooling system. C1 Univ Bath, Dept Mech Engn, Bath BA2 7AY, Avon, England},
author = {Pang, H. H. and Brace, C. J.},
doi = {10.1243/0954407042580110},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Thermal Coating + Water Heat Transfer + Applikation/2004{\_}Pang+Brace{\_}Review of engine cooling technologies for modern engines.pdf:pdf},
journal = {Proc. Inst. Mech. Eng. Part D J. Automob. Eng.},
keywords = {Emissions reduction,Engine cooling,Fuel efficiency},
number = {11},
pages = {1209--1215},
title = {{Review of engine cooling technologies for modern engines}},
volume = {218},
year = {2004}
}
@article{Energietechnik,
author = {Energietechnik, Die and Umwandlungswirkungsgrad, Der and Energieinhalt, Gesamter and Energieform, Energieform and Grundlage, Energieform},
doi = {10.1007/978-3-8348-2279-6},
isbn = {9783834822796},
pages = {15--22},
title = {{3 {\"{U}}berblick}}
}
@article{Allianz2003b,
author = {Allianz, Von M Pfender and Berlin, M{\"{u}}nchen},
isbn = {3540440631},
number = {2},
title = {{6 Schrifttumshinweise}},
volume = {6},
year = {2003}
}
@article{Wallentowitz2006k,
author = {Wallentowitz, Henning and Reif, Konrad},
doi = {10.1007/978-3-8348-9121-1_6},
journal = {Handb. Kraftfahrzeugelektronik - Grundlagen, Kompon. Syst. Anwendungen},
title = {{Sicherheitssysteme}},
url = {http://www.springerlink.com/index/10.1007/978-3-8348-9121-1{\_}6},
year = {2006}
}
@article{Feuer,
author = {Feuer, Kein},
title = {{Kraftanlagen}}
}
@article{Pan2014,
abstract = {Knocking combustion in spark-ignition (SI) engines is a typical abnormal combustion phenomenon that severely limits engine performance and thermal efficiency. However, its mechanism has not so far been completely revealed, such as the origin of pressure oscillation with tremendous amplitude and broken mechanisms of the engine body when knock occurs. This article systematically reviews the series of physical and chemical phenomena involved in knocking combustion, including auto-ignition, gas-dynamic waves, cavity resonance, and auto-ignited flame propagation. Significant research has shown that the rapid heat release of end-gas auto-ignition and subsequent strong pressure waves play a crucial role during knocking combustion. A methodology of the interaction of flame propagation and pressure waves has been proposed to reveal knock formation in terms of positive feedback between strengthened pressure waves and auto-ignited flame propagation. Also, new suggestions on the weakness in prior research of knocking combustion have also been discussed in the present article. {\textcopyright} 2014 Copyright Taylor and Francis Group, LLC.},
author = {Pan, Jiaying and Shu, Gequn and Wei, Haiqiao},
doi = {10.1080/00102202.2013.857665},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2014{\_}Pan+Wei{\_}Interaction of Flame Propagation and Pressure Waves During Knocking Combustion in Spark-Ignition Engines.pdf:pdf},
issn = {0010-2202},
journal = {Combust. Sci. Technol.},
number = {2},
pages = {192--209},
title = {{Interaction of Flame Propagation and Pressure Waves During Knocking Combustion in Spark-Ignition Engines}},
url = {http://www.tandfonline.com/doi/abs/10.1080/00102202.2013.857665},
volume = {186},
year = {2014}
}
@article{Lal1977,
abstract = {This paper reviews and compares the various approaches for finding monotonic and cyclic plastic zone sizes for elastic-perfectly plastic and strain hardening materials. All through the analysis Ramberg-Osgood relationship has been used representing the monotonic and cyclic stress-strain curves. The results for elastic-perfectly plastic materials are compared with those available using finite-element technique. The ratio of monotonic plastic zone sizes strain hardening and elastic perfectly plastic materials are found to be related to the Ramberg-Osgood index n. The values of cyclic plastic zone size are found to depend upon factors like crack opening stress, material properties and specimen geometry. The cyclic plastic zone size obtained in this paper compare well with those given by Antolovich. ?? 1977.},
author = {Lal, K M and Garg, S B L},
doi = {10.1016/0013-7944(77)90036-4},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/1977{\_}LAL+GARG{\_}On the evaluation of monotonic and cyclic plastic zones.pdf:pdf},
issn = {00137944},
journal = {Eng. Fract. Mech.},
number = {2},
pages = {433--442},
title = {{On the evaluation of monotonic and cyclic plastic zones}},
volume = {9},
year = {1977}
}
@article{Fitton1992a,
author = {Fitton, J. C. and Nates, R. J.},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Klopfen{\_}Ottomotor/1992{\_}Fitton{\_}and{\_}Nates{\_}Investigation into the relationship between knock intensity and piston seizure.pdf:pdf},
journal = {N{\&}O J.},
title = {{Investigation into the relationship between knock intensity and piston Seizure}},
year = {1992}
}
@article{Chawla2012,
author = {Chawla, Krishan K},
doi = {10.1007/978-0-387-74365-3_6},
isbn = {978-0-412-58260-8},
issn = {1531-7331},
journal = {Compos. Mater.},
pages = {197--248},
pmid = {20355882},
title = {{Metal Matrix Composites}},
url = {http://link.springer.com/10.1007/978-0-387-74365-3{\%}7B{\_}{\%}7D6},
year = {2012}
}
@article{Geschwindigkeit,
author = {Geschwindigkeit, Beispiel},
doi = {10.1007/978-3-642-24335-6},
isbn = {9783642243356},
title = {{4 Grundlagen der partiellen}}
}
@book{Schurmann2007,
author = {Sch{\"{u}}rmann, H.},
booktitle = {New York},
doi = {10.1007/b137636},
isbn = {9783540721895},
keywords = {Bolzenverbindung,CFK-Welle,Konstruieren mit FKV,Laminate,Leichtbau,Pin},
pages = {1--679},
title = {{Konstruieren mit Faser-Kunststoff- Verbunden}},
year = {2007}
}
@article{Variables,
author = {Variables, Biowin State},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Probabilistic Aspects/A Unified Statistical Methodology for Modeling Fatigue Damage{\_}Castillo/Backmatter{\_}MitModelle.pdf:pdf},
pages = {1--72},
title = {{Models Used In BioWin}}
}
@article{Auflosungsgrenze,
author = {Aufl{\"{o}}sungsgrenze, Abbe and Zahl, Abbe and Mikroskoptheorie, Abbe},
journal = {H{\"{u}}tte},
pages = {1--62},
title = {{S-Sachverzeichnis}}
}
@article{Fu,
author = {Fu, Fertigungsverfahren and Din, Nach and Druckbeha, Im},
doi = {10.1007/978-3-8348-8279-0},
isbn = {9783834882790},
pages = {186--216},
title = {{7 Nietverbindungen 7.1}}
}
@article{Chemisky2013a,
author = {Chemisky, Yves and Meraghni, Fodil},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/Micromechanics formulas{\_}Overview{\_}EshelbyHillAndMore.pdf:pdf},
journal = {Presentations},
title = {{Micromechanics based on the Eshelby solution : Concepts and formulas}},
year = {2013}
}
@article{Winkler2014b,
author = {Winkler, N},
doi = {10.1177/1468087414544899},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2015{\_}Winkler{\_}Effect of pressure oscillations on in-cylinder heat transfer  - through LES Simulation.pdf:pdf},
isbn = {1468087414544},
issn = {1468-0874},
journal = {Int. J. Engine Res.},
keywords = {24 june 2014,6 march 2014,accepted,computational fluid dynamics,date received,heat transfer,internal combustion engines,large eddy simulation,pressure oscillations},
number = {6},
pages = {705--715},
title = {{Effect of pressure oscillations on in-cylinder heat transfer - through large eddy simulation}},
url = {http://jer.sagepub.com/lookup/doi/10.1177/1468087414544899},
volume = {16},
year = {2014}
}
@article{Sommitsch2007,
abstract = {During hot extrusion of aluminium alloys, extrusion dies experience cyclic temperature changes as well as multiaxial loadings. To improve the service life of the dies, cleaner and high hot strength materials are designed as well as an optimised process control is performed. For the improvement of the process guiding and a comparison of lifetime behaviour of different hot work tool steels, modelling and simulation are appropriate means. The extrusion process has been simulated using the FE-program Deform to find the stress and temperature history at the inner diameter of the liner, i.e. the boundary conditions for the subsequent cyclic simulation of the container during service. Inelastic constitutive equations have been implemented into Abaqus Standard to describe strain hardening and time recovery effects. They include the Norton viscoplastic flow rule, thermo-mechanical isotropic hardening and two non-linear kinematic hardening laws. A damage-rate model predicts failure and thus the lifetime of the container. The procedure for the identification of material parameters for both the constitutive and the damage model is described in detail for the hot work tool steel B{\"{o}}hler W400 VMR (EN 1.2343). {\textcopyright} 2006 Elsevier B.V. All rights reserved.},
author = {Sommitsch, C. and Sievert, R. and Wlanis, T. and G{\"{u}}nther, B. and Wieser, V.},
doi = {10.1016/j.commatsci.2006.03.024},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Kriechen{\_}Spannungsrelaxation/2007{\_}Sommitsch{\_}Modelling of creep-fatigue in containers during aluminium and copper extrusion.pdf:pdf},
isbn = {09270256},
issn = {09270256},
journal = {Comput. Mater. Sci.},
keywords = {Creep-fatigue,Damage,Extrusion,Hot work tool steels,Lifetime},
number = {1 SPEC. ISS.},
pages = {55--64},
title = {{Modelling of creep-fatigue in containers during aluminium and copper extrusion}},
volume = {39},
year = {2007}
}
@article{Vektors,
author = {Vektors, Definition},
keywords = {gesetze der,vektor,vektoraddition},
title = {{II Vektoralgebra}}
}
@article{Wallentowitz2006f,
author = {Wallentowitz, Henning and Reif, Konrad},
doi = {10.1007/978-3-8348-9121-1_13},
isbn = {978-3-528-03971-4},
journal = {Handb. Kraftfahrzeugelektronik - Grundlagen, Kompon. Syst. Anwendungen},
title = {{Elektronik Hardware}},
url = {http://www.springerlink.com/index/10.1007/978-3-8348-9121-1{\_}13},
year = {2006}
}
@article{Cadden1998,
author = {Cadden, Jerry L and Sadesky, Paul F},
journal = {Handb. Compos.},
title = {{Tooling for composites}},
year = {1998}
}
@article{Sensorik,
author = {Sensorik, Die and Sensorik, Bauteile and Sensorik, Beschleunigungssensorik and Sensorik, Drucksensorik and Sensoren, Matrixdarstellung},
journal = {Glass},
title = {{5 Sensorik}}
}
@article{Differentialgleichung2008,
author = {Differentialgleichung, Eine},
doi = {10.1007/978-3-642-18424-6},
isbn = {9783642184246},
journal = {System},
title = {{ohnliche Differentialgleichungen}},
year = {2008}
}
@article{Johnson2004a,
author = {Johnson, Ws and Hillberry, Bm},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Probabilistic Aspects/2004{\_}StevenJohnson{\_}Probabilistic Aspects of Life Prediction.pdf:pdf},
journal = {Book},
title = {{Probabilistic aspects of life prediction}},
url = {http://books.google.com/books?hl=en{\%}7B{\&}{\%}7Dlr={\%}7B{\&}{\%}7Did=pDtb-CJLVbYC{\%}7B{\&}{\%}7Doi=fnd{\%}7B{\&}{\%}7Dpg=PP7{\%}7B{\&}{\%}7Ddq=Probabilistic+Aspects+of+Life+Prediction{\%}7B{\&}{\%}7Dots=fII0k-XR1K{\%}7B{\&}{\%}7Dsig=qyo{\%}7B{\_}{\%}7D6w{\%}7B{\_}{\%}7DnT7cN1tqI8pird5rUdts},
year = {2004}
}
@article{Depcik2002,
abstract = {In this paper, the available correlations proposed in the literature for the gas-side heat transfer in the intake and exhaust system of a spark-ignition internal combustion engine were surveyed. It was noticed that theseAB - {\{}{\textless}{\}}inline-graphic xlink:href="2002-01-0372{\{}{\_}{\}}fig0001" xmlns:xlink="http://www.w3.org/1999/xlink"/{\{}{\textgreater}{\}}AB - only by empirically fitted constants. This similarity provided the impetus for the authors to explore if a universal correlation could be developed. Based on a scaling approach using microscales of turbulence, the authors have fixed the exponential factor on the Reynolds number and thus reduced the number of adjustable coefficients to just one; the latter can be determined from a least squares curve-fit of available experimental data. Using intake and exhaust side data, it was shown that the universal correlationAB - {\{}{\textless}{\}}inline-graphic xlink:href="2002-01-0372{\{}{\_}{\}}fig0002" xmlns:xlink="http://www.w3.org/1999/xlink"/{\{}{\textgreater}{\}}AB - The correlation coefficient of this proposed heat transfer model with all available experimental data is 0.845 for the intake side and 0.800 for the exhaust side.ER -},
author = {Depcik, Christopher and Assanis, Dennis},
doi = {10.4271/2002-01-0372},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2002{\_}Assanis{\_}A Universal Heat Transfer Correlation for Intake and Exhaust flows in an SI INternal Combustion Engine.pdf:pdf},
journal = {SAE Pap.},
number = {January 2016},
title = {{A Universal Heat Transfer Correlation for Intake and Exhaust Flows in an Spark-Ignition Internal Combustion Engine}},
url = {http://papers.sae.org/2002-01-0372},
volume = {2002-01-03},
year = {2002}
}
@article{Chaboche1986a,
author = {Chaboche, J L},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/Hardening Recovery Creep/1986{\_}Chaboche{\_}Time-independent-constitutive-theories-for-cyclic-plasticity.pdf:pdf},
journal = {Int. J. Plast.},
number = {2},
pages = {149--188},
title = {{Time-independent constitutive theorems for cyclic plasticity}},
volume = {2},
year = {1986}
}
@article{Enomoto19892,
author = {Enomoto, Yoshiteru and Furuhama, Shoichi},
doi = {10.1299/jsmeb1988.32.1_107},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Heat Transfer Combustion Chamber/1989{\_}Enomoto{\_}A study of the local HTC on the Cmb CHamber Wall of a four stroke gasoline engine.pdf:pdf},
journal = {JSME Int. Journal. Ser. 2},
number = {1},
pages = {107--114},
title = {{A Study of the Local Heat Transfer Coefficient on the Combustion Chamber Walls of a Four-Stroke Gasoline Engine}},
volume = {32},
year = {1989}
}
@article{James1983,
author = {James, M R and Morris, W L},
doi = {10.1007/BF02643749},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Surface effects + Frequency effects/1983{\_}Morris{\_}Effect of fracture surface roughness on growth of short fatigue cracks.pdf:pdf},
issn = {0360-2133},
journal = {Met. Trans. A},
number = {1},
pages = {153--155},
title = {{Effect of Fracture Surface Roughness on Growth of Short Fatigue Cracks}},
url = {http://link.springer.com/10.1007/BF02643749},
volume = {14},
year = {1983}
}
@article{Gesellschaft2004,
author = {Gesellschaft, Deutsche},
journal = {Tagungsbericht},
keywords = {eu-wrrl,ffh-richtlinie,flie{\ss}gew{\"{a}}s-,makrophyten,nordrhein-westfalen,seen},
pages = {1--5},
title = {{1 Einleitung}},
year = {2004}
}
@article{Hettinger2009a,
abstract = {It is a well known fact that indicated efficiency of a SI engine at WOT is predominantly limited by knock occurrence. Therefore many investigations have been carried out to avoid knocking. Considering the further development of downsized engines knocking will also pose a greater challenge. Not only knocking but also irregular combustion in general will require further investigation in supercharged SI eingines. Premature ignition, for instance, hasn't yet been completely understood and therefore limits the low end torque of supercharged SI engines.The purpose of this paper is to introduce different analysis methods which allow to identify the knock onset and the knocking zones in the combustion chamber. In addition to established methods new techniques have been developed to account for the complex nature of pressure oscillation during knocking combustion.Experimental data was acquired on a single cylinder research engine to validate the methodology using six pressure transducers.},
author = {Hettinger, Alexander and Kulzer, Andr{\'{e}}},
doi = {10.4271/2009-01-0698},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2009{\_}Hettinger+Kulzer{\_}A new method to detect Knocking Zones.pdf:pdf},
isbn = {2009010698},
issn = {1946-3944},
journal = {SAE Int. J. Engines},
number = {1},
pages = {698--2009},
title = {{A New Method to Detect Knocking Zones}},
url = {http://papers.sae.org/2009-01-0698/},
volume = {2},
year = {2009}
}
@article{Guennec2013a,
abstract = {Ultrasonic testing method has allowed some impressive improvements in order to better grasp fatigue properties of various metallic materials the latest 20 years. It is particularly the case in the very high cycle regime since ultrasonic fatigue tests are conducted at very high stressing frequencies. However, the question of a potential difference of fatigue strengths due to huge frequency gap between ultrasonic method (usually carried out at 20 kHz) and servo-hydraulic one (usually in the range of 1?100 Hz) is still unclear and needs to be studied for a various kind of metallic materials. The case of low carbon steels presents a singularity, as fatigue properties are significantly different between these two fatigue tests methods. It seems particularly interesting to study this kind of materials in order to get a better overview of frequency effect in metallic materials fatigue. Aim of the present work, which consists of a general survey of JIS S15C steel (0.15{\{}{\%}{\}} C) fatigue properties, is firstly to reconfirm such a frequency effect. Secondly, based on several experiments related to micro-plasticity behavior, some discussions will be held in order to explain this frequency effect in the case of low carbon steels.},
author = {Guennec, B and Ueno, A and Sakai, T and Takanashi, M and Itabashi, Y},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Surface effects + Frequency effects/Frequency effects on high cycle fatigue of low carbon steel.PDF:PDF},
journal = {13th Int. Conf. Fract.},
keywords = {cyclic hardening,ebsd observations,frequency effect,low carbon steel,ultrasonic test},
pages = {1--10},
title = {{Effect of Loading Frequency in Fatigue Properties and Micro-Plasticity Behavior of JIS S15C Low Carbon Steel}},
year = {2013}
}
@article{Habib2004,
author = {Habib, M A and Attya, A M and Said, S A M and Eid, A I and Aly, A Z},
doi = {10.1007/s00231-003-0456-6},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Thermal Coating + Water Heat Transfer/2004{\_}Habib+Attya{\_}Heat transfer characteristics and Nusselt number correlation of turbulent pulsating pipe air flows.pdf:pdf},
journal = {Heat Mass Transf.},
pages = {307--318},
title = {{Heat transfer characteristics and Nusselt number correlation of turbulent pulsating pipe air flows}},
volume = {40},
year = {2004}
}
@article{Kreher1985,
author = {Kreher, W and Pompe, W},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Probabilistic Aspects/1985{\_}Kreher{\_}Field Fluctuations in a heterogeneous elastic material - an info theory approach.pdf:pdf},
journal = {J. Mech. Phys. Solids},
number = {5},
pages = {419--445},
title = {{Field fluctuations in a heterogeneous elastic material: An information theory approach}},
volume = {33},
year = {1985}
}
@article{Habenicht2012g,
author = {Habenicht, Gerd},
isbn = {9783834802958},
title = {{Aus dem Programm Fertigungstechnik}},
year = {2012}
}
@article{Chemicals2005,
author = {Chemicals, Thermoset},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/{\_}buecherSong/HandbookofComposites/II/20{\_}ResinTransferMolding.pdf:pdf},
number = {May},
title = {{Resin Transfer Molding}},
year = {2005}
}
@article{Vanderbilt1989,
author = {Vanderbilt, David},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/Folien CISM Summer School Mai2017 - Mesoscale Models/courses{\_}C1703{\_}roux+{\_}lect4-elast1.pdf:pdf},
number = {8},
pages = {77--89},
title = {{Elastic Properties}},
volume = {40},
year = {1989}
}
@book{Zaefferer2009,
author = {Zaefferer, Stefan and Wright, Stuart I},
doi = {10.1007/978-0-387-88136-2},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Schwartz 2009 - Electron{\_}Backscatter{\_}Diffraction{\_}in{\_}Materials{\_}Science.pdf:pdf},
isbn = {978-0-387-88135-5},
pages = {109--122},
title = {{Electron Backscatter Diffraction in Materials Science}},
url = {http://www.springerlink.com/index/10.1007/978-0-387-88136-2},
year = {2009}
}
@article{Wang1985a,
author = {Wang, C S and Berry, G F},
file = {:C$\backslash$:/Users/p327208/Desktop/Promotion/Literature/Motorspezifisch/1985{\_}Wang{\_}Heat Transfer in Internal Combustion Engines.pdf:pdf},
journal = {Asme},
number = {Ic},
pages = {1--7},
title = {{Heat Transfer in Internal Combustion Engines}},
year = {1985}
}
@article{Popping2012,
author = {P{\"{o}}pping, K},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/Hardening Recovery Creep/2001{\_}M{\"{u}}lders{\_}Modellierung der Verfestigung technischer Aluminiumlegierungen.pdf:pdf},
isbn = {9783844021653},
issn = {1861-0595},
journal = {D-Nb.Info},
title = {{Diese Dissertation ist auf den Internetseiten der Hochschulbibliothek online verf{\"{u}}gbar.}},
url = {http://d-nb.info/985390468/34},
year = {2012}
}
@article{Steigerungen,
author = {Steigerungen, Weitere and Jahr, Jedes and Erkennt, Die and Ausweitung, Eine},
pages = {415--422},
title = {{Zukunftsentwicklungen 14 Trends und zuk{\"{u}}nftige Anforder ungen im Motor radbau}}
}
@article{Fischerauer,
author = {Fischerauer, G and Tr{\"{a}}nkler, H},
journal = {H{\{}{\"{u}}{\}}tte},
pages = {1--96},
title = {{H-Messtechnik}}
}
@article{Mcdowell2017,
author = {Mcdowell, David L},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/Folien CISM Summer School Mai2017 - Mesoscale Models/courses{\_}C1703{\_}mcdowell{\_}CISM.multiscale+crystal+plasticity.mcdowell.lecture+2.final.pdf:pdf},
title = {{Multilevel Crystal Plasticity From nm to mm}},
year = {2017}
}
@article{Warrier2006,
abstract = {In this paper we provide a review of heat transfer and wall heat flux partitioning models/correlations applicable to subcooled forced flow nucleate boiling. Details of both empirical and mechanistic models that have been proposed in the literature are provided. A comparison of the experimental data with predictions from selected models is also included.},
annote = {10.1115/1.2349510},
author = {Warrier, Gopinath R and Dhir, Vijay K},
doi = {10.1115/1.2349510},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Boiling/2006{\_}WarrierHeat Transfer and Wall Heat Flux partitioning during subcooled flow nucelate boiling-a review.pdf:pdf},
journal = {J. Heat Transfer},
month = {feb},
number = {12},
pages = {1243--1256},
publisher = {ASME},
title = {{Heat Transfer and Wall Heat Flux Partitioning During Subcooled Flow Nucleate Boiling - A Review}},
volume = {128},
year = {2006}
}
@article{Morris1976,
abstract = {Abstract Fatigue crack initiation in Al 2219-T851 for fully reversed loading(R = {\$}\sigma{\$}/{\$}\sigma{\$}max =−1) parallel to the material rolling direction is found to occur at intermetallic inclusions at the specimen surface. The inclusions are not involved in crack initiation for fatigue perpendicular to the rolling direction, and for this orientation crack initiation is at grain boundaries and specimens have an increased fatigue life. Except for fatigue at low peak stress, multiple numbers of microcracks are formed and for selected failed specimens the number of cracks has been determined as a function of crack length. Such crack length distribution measurements show that there is significant retardation of microcracks by interaction with grain boundaries. Furthermore it is found that the coalescence of microcracks provides a mechanism for cracking to “jump“ grain boundaries and reduce fatigue lifetime. The effect of relative humidity on this process is to increase the observed mean crack length, and decrease the number of crack initiations apparently due to weakening of the matrix-intermetallic interface at potential initiation sites. The overall result is that no significant dependence of fatigue life on relative humidity is found.},
author = {Morris, W L and Buck, O and Marcus, H L},
doi = {10.1007/BF02656599},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/1976{\_}Morris{\_}Fatigue crack initiation and early propagation in Al 2219-T851.pdf:pdf},
isbn = {0360-2133{\$}\backslash{\$}r1543-1940},
issn = {03602133},
journal = {Met. Trans. A},
number = {7},
pages = {1161--1165},
title = {{Fatigue crack initiation and early propagation in Al 2219-T851}},
volume = {7},
year = {1976}
}
@article{Pan2014c,
abstract = {Knocking combustion in spark-ignition (SI) engines is a typical abnormal combustion phenomenon that severely limits engine performance and thermal efficiency. However, its mechanism has not so far been completely revealed, such as the origin of pressure oscillation with tremendous amplitude and broken mechanisms of the engine body when knock occurs. This article systematically reviews the series of physical and chemical phenomena involved in knocking combustion, including auto-ignition, gas-dynamic waves, cavity resonance, and auto-ignited flame propagation. Significant research has shown that the rapid heat release of end-gas auto-ignition and subsequent strong pressure waves play a crucial role during knocking combustion. A methodology of the interaction of flame propagation and pressure waves has been proposed to reveal knock formation in terms of positive feedback between strengthened pressure waves and auto-ignited flame propagation. Also, new suggestions on the weakness in prior research of knocking combustion have also been discussed in the present article. {\textcopyright} 2014 Copyright Taylor and Francis Group, LLC.},
author = {Pan, Jiaying and Shu, Gequn and Wei, Haiqiao},
doi = {10.1080/00102202.2013.857665},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Klopfen{\_}Ottomotor/2014{\_}Pan+Wei{\_}Interaction of Flame Propagation and Pressure Waves During Knocking Combustion in Spark-Ignition Engines.pdf:pdf},
issn = {0010-2202},
journal = {Combust. Sci. Technol.},
number = {2},
pages = {192--209},
title = {{Interaction of Flame Propagation and Pressure Waves During Knocking Combustion in Spark-Ignition Engines}},
url = {http://www.tandfonline.com/doi/abs/10.1080/00102202.2013.857665},
volume = {186},
year = {2014}
}
@article{Zeita,
author = {Zeit, Der and Frequenz, Der and Frequenz, Der and Frequenz, Der and Zeit, Der and Frequenz, Der and Frequenz, Der and Verwechslungs-, Wegen},
pages = {313--329},
title = {{Signal- und Systemtheorie}},
volume = {1}
}
@article{Saugmotor,
author = {Saugmotor, Ein and Gegensatz, Im and Motoren, Aufgeladene and Drehmomentverlauf, Der},
pages = {161--187},
title = {{6 Aufladung}}
}
@article{Muhs2007a,
author = {Muhs, Dieter and Wittel, Herbert and Jannasch, Dieter and Vo{\ss}iek, Joachim},
doi = {10.1007/978-3-8348-9406-9},
isbn = {9783834802620},
pages = {1068},
title = {{Roloff / Matek Maschinenelemente}},
year = {2007}
}
@article{Finite2000,
author = {Finite, The and Method, Element and Mechanics, Continuum and Basis, The and Basis, Its},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Zienkiewicz FEM - Vol 1 Basics Fundamentals/63205{\_}pref.pdf:pdf},
title = {{It is thirty-eight years since the}},
year = {2000}
}
@article{Mindlin,
author = {Mindlin, Reissner-},
title = {{'Thick' Reissner-Mindlin plates- irreducible and mixed formulations ': ',}},
volume = {0}
}
@article{Stiller2006a,
author = {Stiller, Christoph},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Vorlesungen/Messtechnik+Regelungstechnik/gmrt01.pdf:pdf},
issn = {02731177},
journal = {Adv. Sp. Res.},
number = {12},
pages = {2820--2823},
title = {{Grundlagen der Mess- und Regelungstechnik}},
volume = {38},
year = {2006}
}
@inproceedings{Punekar2013,
abstract = {There has been a change in the thermal management of IC engines where engineers now like to harness the superior heat transfer rates available when limited and controlled nucleate boiling is used to remove heat from high temperature zones. Any flaws in the design of such systems, such as uncontrolled boiling that leads to Dry Out situation, can have an adverse effect on the cooling performance. A detailed engineering model of this process would allow engineers to weed out flawed designs early in the design process. In this paper, we proposed and validated a CFD model for this process.A CFD model is built using the commercial CFD solver ANSYS FLUENT. The mixture multiphase model is used to study subcooled nucleate boiling in IC engine cooling jackets. The departure of bubbles enhances heat transfer at walls, which is captured using the empirical correlation. Volumetric mass transfer is modeled using the inbuilt evaporation-condensation model. Results obtained from heat transfer in channels are compared with experimental results available in the literature for a range of operating pressures, different inlet sub-cooling and different inlet flow velocities. The predicted heat fluxes are in good agreement with experimental data. Results from a typical I.C. engine cooling jacket geometry are also presented.},
author = {Punekar, Hemant and Das, Saurish},
booktitle = {SAE 2013 World Congr. Exhib.},
doi = {10.4271/2013-01-1651},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Boiling/2013{\_}Punekar{\_}Numerical Simulation of Subcooled Nucleate Bpoiling in Cooling Jacket of IC Engine.pdf:pdf},
month = {apr},
publisher = {SAE International},
title = {{Numerical Simulation of Subcooled Nucleate Boiling in Cooling Jacket of IC Engine}},
year = {2013}
}
@article{Xue2005,
author = {Xue, Yibin and Jordon, Brian and Horstemeyer, Stephen and Horstemeyer, Mark F},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Empirical Fatigue Models + Validation/Xue{\_}Fatigue-Experiments-Damage-Evaluation-Multiscale-Modeling-AA-7075{\_}Ansatz ueber Modellierung verschiedener Rissstadien.pdf:pdf},
isbn = {0912053909},
journal = {Proc. 2005 SEM Annu. Conf. Expo. Exp. Appl. Mech.},
pages = {1443--1450},
title = {{Fatigue Experiments , Damage Evaluation and Multiscale Modeling for AA 7075-T651}},
year = {2005}
}
@article{Verschleißteile,
author = {Verschlei{\ss}teile, Reifen},
title = {{5 Mobilit{\"{a}}tsstrategie}}
}
@article{Feldhusen2012,
author = {Feldhusen, J{\"{o}}rg},
doi = {10.1007/978-3-642-24301-1},
isbn = {9783642243011},
title = {{4 Gestaltung von Elementen und Systemen}},
year = {2012}
}
@article{Coulombsche,
author = {Coulombsche, Das},
pages = {4--6},
title = {{1 Physikalische Grundbegriffe der Elektrotechnik}}
}
@book{Dhondt2004,
author = {Dhondt, G.},
booktitle = {Wiley},
doi = {10.1002/0470021217},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Dhondt 2004 - The Finite Element Method for Three-dimensional Thermomechanical Applications.pdf:pdf},
isbn = {0470857528},
pages = {340},
title = {{The Finite Element Method for Three-dimensional Thermo- mechanical Applications}},
year = {2004}
}
@article{Guennec2013,
abstract = {Ultrasonic testing method has allowed some impressive improvements in order to better grasp fatigue properties of various metallic materials the latest 20 years. It is particularly the case in the very high cycle regime since ultrasonic fatigue tests are conducted at very high stressing frequencies. However, the question of a potential difference of fatigue strengths due to huge frequency gap between ultrasonic method (usually carried out at 20 kHz) and servo-hydraulic one (usually in the range of 1?100 Hz) is still unclear and needs to be studied for a various kind of metallic materials. The case of low carbon steels presents a singularity, as fatigue properties are significantly different between these two fatigue tests methods. It seems particularly interesting to study this kind of materials in order to get a better overview of frequency effect in metallic materials fatigue. Aim of the present work, which consists of a general survey of JIS S15C steel (0.15{\{}{\%}{\}} C) fatigue properties, is firstly to reconfirm such a frequency effect. Secondly, based on several experiments related to micro-plasticity behavior, some discussions will be held in order to explain this frequency effect in the case of low carbon steels.},
author = {Guennec, B and Ueno, A and Sakai, T and Takanashi, M and Itabashi, Y},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Surface effects + Frequency effects/Frequency effects on high cycle fatigue of low carbon steel.PDF:PDF},
journal = {13th Int. Conf. Fract.},
keywords = {cyclic hardening,ebsd observations,frequency effect,low carbon steel,ultrasonic test},
pages = {1--10},
title = {{Effect of Loading Frequency in Fatigue Properties and Micro-Plasticity Behavior of JIS S15C Low Carbon Steel}},
year = {2013}
}
@article{Gross2010,
author = {Gross, Dietmar},
doi = {10.1007/978-3-642-11264-5_3},
isbn = {978-3-642-11263-8},
issn = {0937-7433},
pages = {81--117},
title = {{Kinetik eines Systems von Massenpunkten}},
year = {2010}
}
@article{Petukhov1970,
author = {Petukhov, B S},
doi = {https://doi.org/10.1016/S0065-2717(08)70153-9},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Heat transfer intake+exhaust system/1970{\_}Petukhov{\_}Heat Transfer and Friction in Turbulent Pipe Flow with Variable Physical Properties.pdf:pdf},
journal = {Adv. Heat Transf.},
pages = {504--564},
title = {{Heat Transfer and Friction in Turbulent Pipe Flow with Variable Physical Properties}},
volume = {6},
year = {1970}
}
@article{Mughrabi2009,
abstract = {In this article, the physical origin of fatigue crack initiation in ductile metals is discussed from a historical perspective. The main focus is to assess those cyclic slip irreversibilities in a microstructural sense that occur not only at the surface but also in the bulk at the dislocation scale and to show how they contribute to surface fatigue damage. The evolution of early fatigue damage, as evidenced experimentally in the last decades, is reviewed. The phenomenon of cyclic strain localization in persistent slip bands (PSBs) and models of the formation of extrusions, intrusions, and microcracks are discussed in detail. The predictions of these models are compared with experimental evidence obtained on mono- and polycrystalline face-centered-cubic (fcc) metals. In addition, examples of the evolution of fatigue damage in selected fcc solid solution alloys and precipitation-hardened alloys and in body-centered-cubic (bcc) metals are analyzed. Where possible, the cyclic slip irreversibilities p, defined as the fraction of plastic shear strain that is microstructurally irreversible, have been estimated quantitatively. Broadly speaking, p has been found to vary over orders of magnitude (0 p 1), being almost negligible at low loading amplitudes (high fatigue lives) and substantial at larger loading amplitudes (low fatigue lives). 2009 The Minerals, Metals Materials Society and ASM International.},
author = {Mughrabi, Hael},
doi = {10.1007/s11663-009-9240-4},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/2008{\_}Mughrabi{\_}Cyclic Slip Irreversibilities and the Evolution of Fatigue Damage.pdf:pdf},
isbn = {10735615},
issn = {10735615},
journal = {Metall. Mater. Trans. B Process Metall. Mater. Process. Sci.},
number = {4},
pages = {431--453},
title = {{Cyclic slip irreversibilities and the evolution of fatigue damage}},
volume = {40},
year = {2009}
}
@article{Stebbins1967a,
author = {Stebbins, Jeun},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Empirical Fatigue Models + Validation/1965{\_}NASA+Hudson{\_}Studies of fatigue crack growth in alloys suitable for elevated temperature-Al2618.pdf:pdf},
number = {May},
title = {{Nasa Technical N O T E}},
year = {1967}
}
@book{Meister2011c,
abstract = {Die wichtigsten Verfahren zur numerischen L{\{}{\"{o}}{\}}sung von linearen Gleichungssystemen in einer umfassenden Einf{\{}{\"{u}}{\}}hrung, die zum Verst{\{}{\"{a}}{\}}ndnis nur geringe mathematische Vorkenntnisse ben{\{}{\"{o}}{\}}tigt. Behandelt werden sowohl die direkten als auch die iterativen Verfahren, wobei der Autor gro{\{}{\ss}{\}}en Wert auf eine sorgf{\{}{\"{a}}{\}}ltige Herleitung dieser Verfahren legt. Au{\{}{\ss}{\}}erdem sind sehr detaillierte Pseudocodes enthalten, mit deren Hilfe sich die jeweiligen Verfahren in einer beliebigen Programmiersprache sofort auf dem Computer realisieren lassen. Das Lehrbuch ist auch f{\{}{\"{u}}{\}}r Natur- und Ingenieurwissenschaftler geeignet, die in vielen praktischen Anwendungen mit der L{\{}{\"{o}}{\}}sung von linearen Gleichungssystemen konfrontiert sind.},
archivePrefix = {arXiv},
arxivId = {1011.1669v3},
author = {Meister, Andreas},
booktitle = {Matrix},
doi = {10.1007/978-3-8348-8100-7},
eprint = {1011.1669v3},
isbn = {978-3-8348-1550-7},
issn = {1098-6596},
pages = {36--68},
pmid = {25246403},
title = {{Numerik linearer Gleichungssysteme}},
url = {http://link.springer.com/10.1007/978-3-8348-8100-7},
year = {2011}
}
@article{Amara1994a,
abstract = {LES VARIATIONS RAPIDES DE PRESSION ET DE TEMPERATURE INFLUENT CONSIDERABLEMENT SUR LES ECHANGES THERMIQUES INSTANTANES ENTRE LE GAZ ET LES PAROIS DE LA CHAMBRE DE COMBUSTION. UNE ETUDE EXPERIMENTALE DE LA DENSITE SURFACIQUE DU FLUX DE CHALEUR ECHANGE EN DEUX POINTS DE LA PAROI DE LA CULASSE A PERMIS EN EFFET DE METTRE EN EVIDENCE L'ACCUMULATION D'ENERGIE DANS LA COUCHE LIMITE THERMIQUE QUI SE MANIFESTE PAR UN DEPHASAGE TEMPOREL ENTRE LE FLUX ET L'ECART DE TEMPERATURE GLOBAL GAZ-PAROI. EN REGIME LAMINAIRE INSTATIONNAIRE, UNE SIMULATION DE CES ECHANGES FAIT BIEN APPARAITRE DES EXTREMA LOCAUX DE TEMPERATURE DANS LA COUCHE LIMITE THERMIQUE. UNE INTERPRETATION DU MECANISME DE FORMATION ET DE DEPLACEMENT DE CES EXTREMA EST DONNEE. LES ECHANGES THERMIQUES EN REGIME TURBULENT SONT DECRITS A L'AIDE DU MODELE MONODIMENSIONNEL DE YANG ET MARTIN OU L'EFFET DE LA TURBULENCE EST PRIS EN COMPTE PAR LE BIAIS DE LA CONDUCTIVITE THERMIQUE TURBULENTE. CE MODELE A ETE MODIFIE POUR LIMITER L'AUGMENTATION DE LA CONDUCTIVITE THERMIQUE TURBULENTE AVEC LA DISTANCE A LA PAROI. LE PARAMETRE DE LIMITATION EST LIE A LA VALEUR LOCALE DE LA VISCOSITE TURBULENTE. LE MODELE AINSI OBTENU PERMET UNE MEILLEURE DETERMINATION DE L'EPAISSEUR DE LA COUCHE LIMITE THERMIQUE ET S'ADAPTE DE LUI-MEME A TOUTE SITUATION INTERMEDIAIRE ENTRE LE REGIME LAMINAIRE ET LES REGIMES FORTEMENT TURBULENTS, LA DENSITE DU FLUX DE CHALEUR ETANT MODULEE EN CONSEQUENCE. L'IMPLANTATION DE CE MODELE DANS LE CODE DE SIMULATION KIVA2 A MONTRE QUE LA PRISE EN COMPTE DES INSTATIONNARITES DE TEMPERATURE ET DE PRESSION CONSTITUE UNE AMELIORATION PAR RAPPORT AUX LOIS DE PAROI LOGARITHMIQUES MAIS SE REVELE INSUFFISANTE. UNE SUPERPOSITION DU MODELE MONODIMENSIONNEL ET D'UNE LOI DE PAROI LOGARITHMIQUE RENDANT COMPTE DE L'EFFET DE LA VITESSE TANGENTIELLE DONNE DES RESULTATS SE RAPPROCHANT AU MIEUX DES EVOLUTIONS EXPERIMENTALES ET CECI POUR DIFFERENTES VITESSES DE ROTATION. UNE ETUDE PARAMETRIQUE COMPARATIVE EST ENSUITE REALISEE POUR MONTRER L'IMPACT DU CHOIX D'UN MODELE DE CALCUL DU FLUX DE CHALEUR PARIETAL SUR LA DETERMINATION DES CHAMPS DE VITESSE, DE TEMPERATURE, D'ENERGIE CINETIQUE TURBULENTE ET DE SON TAUX DE DISSIPATION A LA FIN DE LA COURSE DE COMPRESSION.},
author = {Amara, S},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Heat Transfer Combustion Chamber/1994{\_}Amara{\_}Elaboration et validation dun modele de transferts thermiques dun moteur{\_}UebersichtWaermeuebergangsmodelle.pdf:pdf},
keywords = {Chambre de combustion,Cin{\'{e}}tique turbulente,R{\'{e}}gime laminaire},
publisher = {{\'{E}}cole centrale de Lyon},
title = {{Elaboration et validation d'un mod{\`{e}}le de transferts thermiques instationnaires gaz paroi dans la chambre de combustion d'un moteur}},
url = {http://cat.inist.fr/?aModele=afficheN{\&}cpsidt=162697},
year = {1994}
}
@article{Wahrnehmung,
author = {Wahrnehmung, Deren and Augen, Die and Generation, Von and Reifen, Schnittstelle and Reifen, Der and Reifen, Beim and Fahrzeugen, Bei and Ph, Dieses and Resonanzlage, Die and Felge-seitenwand-stahlg, Resonanzsystem},
title = {{9 Ger{\{}{\"{a}}{\}}usche und Schwingungen}}
}
@article{Doquet1997,
abstract = {The development of fatigue damage in Co45Ni specimens during push-pull and reversed torsion tests, performed inside a scanning electron microscope, was observed and the different stress states compared. It appeared that transgranular crack initiation and development is delayed and intergranular crack initiation promoted under torsional loading. This was explained in terms of reduced surface distortion at the emergence of persistent slip bands (PSBs) and smaller compatibility stresses at the PSB-matrix interfaces. The influence of the mechanical strength of grain boundaries on the difference between tensile and torsional fatigue lives is discussed.},
author = {Doquet, V},
doi = {10.1111/j.1460-2695.1997.tb00280.x},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/1996{\_}Doquet{\_}CRACK INITIATION MECHANISMS IN TORSIONAL FATIGUE.pdf:pdf},
issn = {8756758X},
journal = {Fatigue Fract. Eng. Mater. Struct.},
keywords = {-torsional fatigue,intergranular crack initiation},
number = {2},
pages = {227--235},
title = {{Crack Initiation Mechanisms in Torsional Fatigue}},
url = {http://doi.wiley.com/10.1111/j.1460-2695.1997.tb00280.x},
volume = {20},
year = {1997}
}
@article{Schumacher2005,
author = {Schumacher, Axel},
doi = {10.1007/978-3-642-34700-9},
isbn = {3-540-21887-4},
title = {{Optimierung mechanischer Strukturen : Grundlagen und industrielle Anwendungen / Axel Schumacher}},
url = {https://portal.dnb.de/opac.htm;jsessionid=F23EC21423D793C1D8FF7679BCFF886F.prod-worker4?method=showFullRecord{\&}currentResultId=optimierung+mechanischer+strukturen{\%}26any{\&}currentPosition=2},
year = {2005}
}
@article{Kr??mer2013,
author = {Kr??mer, Stephan and Rothe, Steffen and Hartmann, Stefan},
doi = {10.1007/s00366-013-0337-7},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Parametersch{\"{a}}tzung/2013{\_}Hartmann{\_}Homogeneous stress–strain states computed by 3D-stress algorithms of FE-codes - application to material parameter identification.pdf:pdf},
issn = {14355663},
journal = {Eng. Comput.},
keywords = {DAE-systems,Finite elements,Material parameter identification,Plane stress,Stress algorithms},
number = {1},
pages = {141--159},
title = {{Homogeneous stress???strain states computed by 3D-stress algorithms of FE-codes: application to material parameter identification}},
volume = {31},
year = {2013}
}
@article{gnielinski1976new,
author = {Gnielinski, V},
journal = {Int. Chem. Eng},
keywords = {1976 channel flow heat-transfer pipe turbulent},
number = {2},
pages = {359--368},
title = {{New equations for heat and mass transfer in turbulent pipe and channel flow}},
volume = {16},
year = {1976}
}
@article{Johna,
author = {John, T K and Berg, Jerome S},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/{\_}buecherSong/HandbookofComposites/II/19{\_}TableRollingofCompositeTubes.pdf:pdf},
journal = {Design},
title = {{Table rolling of composite tubes}}
}
@article{Hochhalter2010a,
abstract = {The objective of this paper is to develop further a framework for computationally modeling{\$}\backslash{\$}nmicrostructurally small fatigue crack growth in AA 7075-T651 (Bozek et al 2008 Modelling Simul.{\$}\backslash{\$}nMater. Sci. [/0965-0393/16] 16 065007 ). The focus is on the nucleation event, when a crack extends{\$}\backslash{\$}nfrom within a second-phase particle into a surrounding grain, since this has been observed to be an{\$}\backslash{\$}ninitiating mechanism for fatigue crack growth in this alloy. It is hypothesized that nucleation can{\$}\backslash{\$}nbe predicted by computing a non-local nucleation metric near the crack front. The hypothesis is{\$}\backslash{\$}ntested by employing a combination of experimentation and finite element modeling in which various{\$}\backslash{\$}nslip-based and energy-based nucleation metrics are tested for validity, where each metric is derived{\$}\backslash{\$}nfrom a continuum crystal plasticity formulation. To investigate each metric, a non-local procedure{\$}\backslash{\$}nis developed for the calculation of nucleation metrics in the neighborhood of a crack front.{\$}\backslash{\$}nInitially, an idealized baseline model consisting of a single grain containing a semi-ellipsoidal{\$}\backslash{\$}nsurface particle is studied to investigate the dependence of each nucleation metric on lattice{\$}\backslash{\$}norientation, number of load cycles and non-local regularization method. This is followed by a{\$}\backslash{\$}ncomparison of experimental observations and computational results for microstructural models{\$}\backslash{\$}nconstructed by replicating the observed microstructural geometry near second-phase particles in{\$}\backslash{\$}nfatigue specimens. It is found that orientation strongly influences the direction of slip{\$}\backslash{\$}nlocalization and, as a result, influences the nucleation mechanism. Also, the baseline models,{\$}\backslash{\$}nreplication models and past experimental observation consistently suggest that a set of particular{\$}\backslash{\$}ngrain orientations is most likely to nucleate fatigue cracks. It is found that a continuum crystal{\$}\backslash{\$}nplasticity model and a non-local nucleation metric can be used to predict the nucleation event in AA{\$}\backslash{\$}n7075-T651. However, nucleation metric threshold values that correspond to various nucleation{\$}\backslash{\$}ngoverning mechanisms must be calibrated.},
author = {Hochhalter, J D and Littlewood, D J and Christ, R J and Veilleux, M G and Bozek, J E and Ingraffea, A R and Maniatty, A M},
doi = {10.1088/0965-0393/18/4/045004},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/2010{\_}Hochhalter{\_}AL7075AgeometricapproachII{\_}SlipAndNucleation.pdf:pdf},
isbn = {0965-0393},
issn = {0965-0393},
journal = {Model. Simul. Mater. Sci. Eng.},
number = {4},
pages = {45004},
title = {{A geometric approach to modeling microstructurally small fatigue crack formation: II. Physically based modeling of microstructure-dependent slip localization and actuation of the crack nucleation mechanism in AA 7075-T651}},
url = {http://stacks.iop.org/0965-0393/18/i=4/a=045004?key=crossref.ef8bc48536790be47a24f27989602c36},
volume = {18},
year = {2010}
}
@article{Rostampour2015c,
abstract = {This investigation deals with the EF7 (TC) engine, a dual fuel engine equipped with a turbocharger system, consequently with a high probability of knock inception. In this study, an operating cycle of the engine was simulated using KIVA-3V code. Some modifications were carried out on the KIVA method of calculating pressure in the intake port in order to simulate turbocharger pressure correctly. Auto-ignition and knock were then simulated using the auto-ignition integral model. The modified code and the simulation were verified using three different methods; in-cylinder average pressure, gas temperature of the exhaust port, and auto-ignition timing. The simulation results using the auto-ignition integral model, as compared with the experimental data, proved to be reasonably accurate. Following this validation, the effect of the knock phenomenon on the engine heat transfer through the walls was investigated. The simulations showed that the rate of heat transfer through the walls under knocking conditions is about 2.2 times higher than that under normal conditions. However, it was also shown that the total heat transfer increases about 15{\{}{\%}{\}}.},
author = {Rostampour, Arman and Toosi, Ali Nassiri},
doi = {10.1115/1.4030517},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2015{\_}Rostampour{\_}Numerical Investigation of the effect of knock on heat transfer in a turbo si engine.pdf:pdf},
issn = {0742-4795},
journal = {J. Eng. Gas Turbines Power},
number = {12},
pages = {121502},
title = {{Numerical Investigation of the Effect of Knock on Heat Transfer in a Turbocharged Spark Ignition Engine}},
url = {http://www.scopus.com/inward/record.url?eid=2-s2.0-84930634240{\%}7B{\&}{\%}7DpartnerID=tZOtx3y1},
volume = {137},
year = {2015}
}
@article{Proakis1996,
abstract = {The author and publisher of this book have used their best efforts in preparing this book. These efforts include the development, research, and testing of the theories and programs to determine their effectiveness. The author and publisher make no warranty of any kind, expressed or implied, with regard to these programs or the documentation contained in this book. The author and publisher shall not be liable in any event for incidental or consequential damages in connection with, or arising out of. the furnishing, performance, or use of these programs.},
author = {Proakis, John G. and Monolakis, Dimitri G.},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/Signal Verarbeitung/1996{\_}ProakisandManolakis{\_}Digital{\_}Signal{\_}Processing{\_}Principles{\_}Algorithms{\_}and{\_}Applications{\_}Third{\_}Edition.pdf:pdf},
isbn = {0-13-394338-9},
journal = {Pentice Hall},
pages = {1--42},
title = {{Digital signal processing: principles, algorithms, and applications}},
year = {1996}
}
@article{Sturz-,
author = {Sturz-, Die},
title = {{7 Kurvenfahrt 7.1}}
}
@article{Fs2013b,
author = {Fs},
doi = {10.1007/978-1-4614-0502-3},
isbn = {2009004043},
number = {1},
pages = {0--10},
title = {{Chapter 0}},
year = {2013}
}
@article{Bridier2009a,
abstract = {Deformation micromechanisms of a Ti-6Al-4V alloy under fatigue loading at room temperature are studied using a three-dimensional crystal plasticity constitutive model. The model employs a minimum set of fitting parameters based on experimental data for Ti-6Al-4V. Single slip is strongly favored through a softening law that affects mainly the driving force for slip on the first activated slip system. Cyclic deformation behavior at the macroscopic scale and at the local scale of grains is analyzed through the simulation of 20 cycles of fatigue on a polycrystalline structure of 900 randomly oriented grains. The progressive activation of slip (basal, prismatic, and pyramidal) is analyzed and compared to experimental observations. {\{}{\textcopyright}{\}} 2008 Elsevier Ltd. All rights reserved.},
author = {Bridier, Florent and McDowell, David L and Villechaise, Patrick and Mendez, Jos{\'{e}}},
doi = {10.1016/j.ijplas.2008.08.004},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2008{\_}Bridier{\_}Crystal plasticity modeling of slip activity in Ti–6Al–4V under high cycle fatigue loading.pdf:pdf},
isbn = {0749-6419},
issn = {07496419},
journal = {Int. J. Plast.},
keywords = {A. Microstructures,B. Anisotropic material,B. Crystal plasticity,B. Polycrystalline material,C. Finite elements},
number = {6},
pages = {1066--1082},
publisher = {Elsevier Ltd},
title = {{Crystal plasticity modeling of slip activity in Ti-6Al-4V under high cycle fatigue loading}},
url = {http://dx.doi.org/10.1016/j.ijplas.2008.08.004},
volume = {25},
year = {2009}
}
@article{Zhao2008a,
abstract = {Extensive fatigue experiments were conducted using 7075-T651 aluminum alloy under uniaxial, torsion, and axial-torsion loading. Detailed fatigue results were reported. Different mean stresses were applied in the experiments and the mean stress was found to have a significant influence on the fatigue strength of the material. A tensile mean stress decreased the fatigue strength dramatically. Fatigue damage was found to occur under compression-compression loading. In addition, axial-torsion experiments using tubular specimens were conducted under different loading paths to study the multiaxial fatigue behavior. Fatigue cracking behavior was found to be dependent on the loading path as well as the loading magnitude. When the loading magnitude was high, the material displayed shear cracking. When the loading stress was below a certain level, the material exhibited tensile cracking. For most loading cases under investigation, the material displayed a mixed cracking behavior. A kink was found in the shear strain versus fatigue life curve from the pure torsion experiments, and it was associated with a distinctive transition of cracking behavior. The Smith-Watson-Topper (SWT) parameter with a critical plane interpretation was found to correlate well with most of the experiments conducted in terms of fatigue lives. However, the SWT parameter cannot deal with the uniaxial fatigue conditions where the maximum stress is low or negative. More importantly, the model fails to correctly predict the cracking behavior observed experimentally on the material. A critical plane criterion based on a combination of the normal and shear components of the stresses and strains on material planes was found to better correlate the fatigue experiments in terms of both fatigue life and cracking behavior. The characteristics of the multiaxial fatigue criterion were discussed based on the experimental observations on 7075-T651 aluminum alloy. ?? 2007 Elsevier Ltd. All rights reserved.},
author = {Zhao, Tianwen and Jiang, Yanyao},
doi = {10.1016/j.ijfatigue.2007.07.005},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Empirical Fatigue Models + Validation/2007{\_}Jiang{\_}Fatigue of 7075-T651 aluminum alloy VALIDATION+MODEL.pdf:pdf},
isbn = {0142-1123},
issn = {01421123},
journal = {Int. J. Fatigue},
keywords = {7075-T651 aluminum alloy,Axial-torsion,Compression-compression fatigue,Multiaxial criterion,Multiaxial fatigue},
number = {5},
pages = {834--849},
title = {{Fatigue of 7075-T651 aluminum alloy}},
volume = {30},
year = {2008}
}
@article{Arnoldb,
author = {Arnold, J{\"{o}}rg},
pages = {787--792},
title = {{C5 C5 Reifen und R{\"{a}}der C5 Reifensch{\"{a}}den als Unfallfolgen}}
}
@article{Embers2003,
author = {Embers, O N E Imensional M},
journal = {Dimens. Contemp. Ger. Arts Lett.},
pages = {121--138},
title = {{Element Fields in Linear Problems}},
volume = {1},
year = {2003}
}
@article{Zienkiewicz1971,
author = {Zienkiewicz, O C},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Zienkiewicz FEM - Vol 1 Basics Fundamentals/63205{\_}fm.pdf:pdf},
title = {{Method : Its Basis and Fundamentals UNESCO Professor of Numerical Methods in Engineering}},
year = {1971}
}
@article{Zuge2001,
author = {Zuge, Im and Deutschland, Bundesrepublik},
keywords = {gebieten},
number = {1993},
pages = {1--94},
title = {{1 Allgemeine Einleitung}},
year = {2001}
}
@article{Krause2000,
author = {Krause, Prof Klaus},
number = {Eg I},
pages = {1--5},
title = {{Grundlagen der Elektrotechnik Grundlagen der Elektrotechnik}},
year = {2000}
}
@article{Apparate,
author = {Apparate, Gebilde and Ger, Gebilde and Wiener, Norbert and Kennzeichen, Die and Systemelemente, Die and Funktion, Die and Input, Jeder and Drucker, Peter},
journal = {Mechanik},
pages = {9--20},
title = {{2 Einf{\{}{\"{u}}{\}}hrung in die systemtechnische Methodik}}
}
@article{Principal,
author = {Principal, A},
pages = {1--5},
title = {{Invariants of second-order tensors}},
volume = {13}
}
@article{Wallentowitz2006k,
author = {Wallentowitz, Henning and Reif, Konrad},
doi = {10.1007/978-3-8348-9121-1_6},
journal = {Handb. Kraftfahrzeugelektronik - Grundlagen, Kompon. Syst. Anwendungen},
title = {{Sicherheitssysteme}},
url = {http://www.springerlink.com/index/10.1007/978-3-8348-9121-1{\%}7B{\_}{\%}7D6},
year = {2006}
}
@article{Beispielc,
author = {Beispiel, Am and Beispiel, Dieses and Iso, D I N E N and Datei, Neue},
pages = {36--42},
title = {{4 Zylinderschraube}}
}
@article{Variables,
author = {Variables, Biowin State},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Probabilistic Aspects/A Unified Statistical Methodology for Modeling Fatigue Damage{\_}Castillo/Backmatter{\_}MitModelle.pdf:pdf},
pages = {1--72},
title = {{Models Used In BioWin}}
}
@article{Fertigungstechnik,
author = {Fertigungstechnik, Der and Unfallsicherheit, Der and Konstrukteur, Den},
title = {{C Manuelle Konstruktion 22}}
}
@article{Schlupfregelsysteme,
author = {Schlupfregelsysteme, Antriebs- and Bereits, Kurvenleger and Beispiele, Drei and Fahrzeugkarosserie, Die},
title = {{10 Servo- und Regelsysteme am Fahrwerk}}
}
@article{Evans1998,
abstract = {Today, fiber reinforced composites are in use in a variety of structures, ranging from spacecraft to aircraft to buildings and bridges. This wide use of composites has been facilitated by the introduction of new materials, improvements in manufacturing processes and developments of new analytical and testing methods. Unfortunately, information on these topics is scattered in journal articles, in conference and symposium proceedings, in workshop notes, and in government and company reports. This proliferation of the source material, coupled with the fact that some of the relevant publications are hard to find or are restricted, makes it difficult to identify and obtain the up-to-date knowledge needed to utilize composites to their full advantage. This book intends to overcome these difficulties by presenting in a single volume, many of the recent advances in the field of composite materials.},
author = {Evans, Don O.},
doi = {10.1007/978-1-4615-6389-1_23},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/{\_}buecherSong/HandbookofComposites/II/22{\_}FiberPlacement.pdf:pdf},
isbn = {0412540207},
journal = {Handb. Compos.},
pages = {476--487},
title = {{Fiber Placement}},
url = {http://link.springer.com/10.1007/978-1-4615-6389-1{\_}23},
volume = {21},
year = {1998}
}
@article{Getriebe2007,
author = {Getriebe, Gesamtsystems and Einsparung, Durch},
journal = {Fahrzeuggetriebe},
title = {{14 Rechnerunterst{\{}{\"{u}}{\}}tzte Getriebeentwicklung}},
year = {2007}
}
@article{Liu1972,
abstract = {1. Introduction In thermodynamics, whenever a material is subject to investigation of its properties, the entropy principle is used to impose restrictions on the constitutive relations for the material. There is not, so far, any simple method by which restrictions from the entropy ... },
author = {Liu, I Shih},
doi = {10.1007/BF00250688},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Thermodynamik/Liu{\_}Entropieprinzip{\_}Lagrange/Method of LAgrange Multipliers for Exploitation of the Entropy Principle {\_} Liu.pdf:pdf},
issn = {00039527},
journal = {Arch. Ration. Mech. Anal.},
number = {2},
pages = {131--148},
title = {{Method of Lagrange multipliers for exploitation of the entropy principle}},
volume = {46},
year = {1972}
}
@article{Negi2015,
author = {Negi, Anjna},
doi = {10.1016/j.pedn.2008},
isbn = {0514190450},
issn = {1095-9203},
number = {2},
pages = {464--467},
pmid = {12399572},
title = {{References 1.}},
volume = {6},
year = {2015}
}
@article{Schaltgetriebe2006,
author = {Schaltgetriebe, Bezeichnung Automatisiertes and Transmission, Dual Clutch},
journal = {Network},
title = {{5 Architektur, Komponenten und Baugruppen automatisch schaltender PKW-Getriebe}},
year = {2006}
}
@article{Sandoval2003,
abstract = {A spark-ignition engine friction model developed by Patton et al. in the late 1980s was evaluated against current engine friction data, and improved. The model, which was based on a combination of fundamental scaling laws and empirical results, includes predictions of rubbing losses from the crankshaft, reciprocating, and valvetrain components, auxiliary losses from engine accessories, and pumping losses from the intake and exhaust systems. These predictions were based on engine friction data collected between 1980 and 1988. Some of the terms are derived from lubrication theory. Other terms were derived empirically from measurements of individual friction components from engine teardown experiments. Recent engine developments (e.g., improved oils, surface finish on piston liners, valve train mechanisms) suggested that the model needed updating. So modifications were made to the piston ring tension and gas pressure loading contributions to piston assembly friction, the impact of liner roughness, and to the valvetrain mechanism friction. Lubricant viscosity scaling was added to the hydrodynamic terms in the rubbing friction component models. The improved model now gives reasonable estimates of individual friction component and total spark-ignition engine friction mean effective pressure. The inclusion of oil viscosity scaling with temperature results in cold engine friction predictions about twice the value for warmed up engines. This agrees with the limited cold engine friction data available in the literature.},
archivePrefix = {arXiv},
arxivId = {2003-01-0725},
author = {Sandoval, Daniel and Heywood, John B.},
doi = {10.4271/2003-01-0725},
eprint = {2003-01-0725},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2003{\_}Sandoval{\_}An Imporved Friction Model for Spark{\_}Ign Engines.pdf:pdf},
isbn = {0148-7191},
title = {{An Improved Friction Model for Spark-Ignition Engines}},
url = {http://papers.sae.org/2003-01-0725/},
year = {2003}
}
@book{ONeal1972,
abstract = {This book provides an applications-oriented introduction to digital signal processing written primarily for electrical engineering undergraduates. Practicing engineers and graduate students may also find it useful as a first text on the subject. Digital signal processing is everywhere. Today's college students hear “DSP” all the time in their everyday life—from their CD players, to their electronic music synthesizers, to the sound cards in their PCs. They hear all about “DSP chips”, “oversampling digital filters”, “1-bit A/D and D/A converters”, “wavetable sound synthesis”, “audio effects processors”, “all-digital audio studios”. By the time they reach their junior year, they are already very eager to learn more about DSP. Approach},
author = {O'Neal, J.},
booktitle = {IEEE Trans. Commun.},
doi = {10.1109/TCOM.1972.1091274},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/Signal Verarbeitung/1996{\_}S. J. Orfanidis{\_}Introduction To Signal Processing.pdf:pdf},
isbn = {0-13-209172-0.},
issn = {0090-6778},
number = {5},
pages = {1046--1047},
pmid = {22203662},
title = {{Introduction to Signal Transmission}},
url = {http://ieeexplore.ieee.org/document/1091274/},
volume = {20},
year = {1972}
}
@article{Manonukul2004,
abstract = {A polycrystal plasticity finite–element model has been developed for nickel–base alloy C263. That is, a representative region of the material, containing about 60 grains, has been modelled using crystal plasticity, taking account of grain morphology and crystallographic orientation. With just a single material property (in addition to standard elastic properties), namely, the critical resolved shear stress, the model is shown to be capable of predicting correctly a wide range of cyclic plasticity behaviour in face–centred cubic nickel alloy C263. A fatigue crack initiation criterion is proposed, based simply on a critical accumulated slip. When this critical slip is achieved within the microstructure, crack initiation is taken to have occurred. The model predicts the development of persistent slip bands within individual grains with a width of ca. 10 {\$}\mu{\$}m. The model also predicts that crack initiation can occur preferentially at grain triple points under both low– (LCF) and high–cycle fatigue (HCF). For the case of HCF, this also corresponds to a free surface. The polycrystal plasticity model combined with the fatigue crack initiation criterion are shown to predict correctly the standard Basquin and Goodman correlations in HCF, and the Coffin–Manson correlation in LCF. The model predictions are based on just two material properties: the critical resolved shear stress and the critical accumulated slip. Just one experimental test is required to determine these properties, for a given temperature, which have been obtained for nickel alloy C263. Predictions of life for nickel alloy C263 are then made over a broad range of loading conditions covering both LCF and HCF. Good agreement with experiments is achieved, despite the simplicity of the proposed ‘two–parameter' model. A simple three–dimensional form of the model has provided an estimate of the fatigue limit for HCF crack initiation in C263.},
author = {Manonukul, A and Dunne, F P E},
doi = {10.1098/rspa.2003.1258},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2003{\_}Manonukul+Dunne{\_}High- and low-cycle fatigue crack initiation using polcrystal plasticity.pdf:pdf},
isbn = {1364-5021},
issn = {1364-5021},
journal = {Proc. R. Soc. A Math. Phys. Eng. Sci.},
keywords = {crack initiation,hcf,high-cycle fatigue,lcf,low-cycle fatigue,polycrystal plasticity},
number = {2047},
pages = {1881--1903},
title = {{High- and low-cycle fatigue crack initiation using polycrystal plasticity}},
url = {http://rspa.royalsocietypublishing.org/cgi/doi/10.1098/rspa.2003.1258},
volume = {460},
year = {2004}
}
@article{Worlds2016,
author = {Worlds, Small and Attachment, Preferential and Models, Voter and Distributions, Fixed Degree and Laws, Power},
isbn = {9780511546594},
pages = {5--6},
title = {{Preface 1.}},
year = {2016}
}
@article{Rousselier1987b,
abstract = {Since the pioneering studies conducted by McClintock, Rice and Tracey on the growth of cavities, many studies have covered modelling of ductile fracture; a non-exhaustive list is given of these studies. In the local approach of fracture, the models are used at the tip of cracks, and in the present state, only relatively simple models can be used to solve fracture problems in a complete manner, from material characterization to the analysis of cracked structures. The paper presents two types of models based on a critical ratio of cavity growth or on continuum damage mechanics. In the framework of the local approach of fracture, their possibilities are presented with constant references to experimental validation studies. This allows conclusions to be drawn regarding the effectiveness of the methods proposed and their undeniable contribution to fracture mechanics. ?? 1987.},
author = {Rousselier, G},
doi = {10.1016/0029-5493(87)90234-2},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Plasticity models/Ductile fracture models and their potential in local approach of fracture{\_}Rousselier.pdf:pdf},
isbn = {00295493},
issn = {00295493},
journal = {Nucl. Eng. Des.},
number = {1},
pages = {97--111},
title = {{Ductile fracture models and their potential in local approach of fracture}},
volume = {105},
year = {1987}
}
@article{Berger2003a,
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Berger},
doi = {10.1002/ejoc.201200111},
eprint = {arXiv:1011.1669v3},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Vortraege/Book-of-Abstracts{\_}2016-03-04{\_}GAMM.pdf:pdf},
isbn = {9781107671812},
issn = {0196-6553},
journal = {Eng. Med. Biol. Soc. 2008. EMBS 2008. 30th Annu. Int. Conf. IEEE},
pages = {2004},
pmid = {26840611},
title = {{Table of of contents}},
volume = {24},
year = {2003}
}
@article{Leichtbausa,
author = {Leichtbaus, Zielsetzung and Hauptforderung, Eine},
pages = {1--2},
title = {{1 Zielsetzung des Leichtbaus}}
}
@article{RajuP2011,
abstract = {This paper presents the details of method of sample size determination to estimate the characteristic fatigue life of aluminum alloy, A356.2-T6. The characteristic fatigue life of the alloy has been estimated by assuming log normal distribution model. A step wise procedure is outlined to determine the number of specimens required at predetermined stress amplitude to estimate the fatigue life with an acceptable error at 50{\%} probability and various confidence levels, 90{\%}, 95{\%} and 99{\%}. Maximum percentage of errors has also been calculated for the above probability and confidence levels. Details of generation of S-N curve for aluminum alloy A356.2-T6 using regression analysis have been explained. From this study, the adequate sample size required for evaluating the average fatigue life of A356.2-T6 with an acceptable error at 50{\%} probability and 90{\%} confidence level using log normal distribution is established. In order to check the significance of regression equation, analysis of variance (ANOVA) is performed. Copyright 2011 Tech Science Press.},
author = {{Raju P}, R and Rajesh, S and Satyanarayana, B and Ramji, K},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Probabilistic Aspects/2011{\_}Ramamurty{\_}Statistical Analysis of Fatigue Life Data of A356.2-T6 Aluminium Alloy.pdf:pdf},
journal = {Struct. Durab. Heal. Monit.},
keywords = {aluminum alloy,fatigue life,log normal distribution,s n curve},
number = {1-2},
pages = {139--152},
title = {{Statistical analysis of fatigue life data of A356.2-T6 aluminum alloy}},
url = {http://www.scopus.com/inward/record.url?eid=2-s2.0-79957943262{\&}partnerID=40{\&}md5=a5890475316795056516da22de2c7672},
volume = {7},
year = {2011}
}
@article{Anwendungb,
author = {Anwendung, Wirkprinzip},
pages = {112--185},
title = {{6 Schwei{\{}{\ss}{\}}verbindungen 6 6.1}}
}
@article{Desmorat2007a,
abstract = {On the idea that fatigue damage is localized at the microscopic scale, a scale smaller than the mesoscopic one of the Representative Volume Element (RVE), a three-dimensional two scale damage model has been proposed for High Cycle Fatigue applications. It is extended here to anisothermal cases and then to thermo-mechanical fatigue. The modeling consists in the micromechanics analysis of a weak micro-inclusion subjected to plasticity and damage embedded in an elastic meso-element (the RVE of continuum mechanics). The consideration of plasticity coupled with damage equations at microscale, altogether with Eshelby-Kr{\"{o}}ner localization law, allows to compute the value of microscopic damage up to failure for any kind of loading, 1D or 3D, cyclic or random, isothermal or anisothermal, mechanical, thermal or thermo-mechanical. A robust numerical scheme is proposed in order to make the computations fast. A post-processor for damage and fatigue (DAMAGE{\_}2005) has been developed. It applies to complex thermo-mechanical loadings. Examples of the representation by the two scale damage model of physical phenomena related to High Cycle Fatigue are given such as the mean stress effect, the non-linear accumulation of damage. Examples of thermal and thermo-mechanical fatigue as well as complex applications on real size testing structure subjected to thermo-mechanical fatigue are detailed. {\textcopyright} 2007 Elsevier Masson SAS. All rights reserved.},
author = {Desmorat, R. and Kane, A. and Seyedi, M. and Sermage, J. P.},
doi = {10.1016/j.euromechsol.2007.01.002},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/2 scale models papers/2007{\_}Desmorat+Kane+Seyedi+Sermage{\_}Two scale damage model and related numerical issues.pdf:pdf},
isbn = {09977538},
issn = {09977538},
journal = {Eur. J. Mech. A/Solids},
keywords = {Damage,Fatigue,Post-processing,Thermomechanical loading},
number = {6},
pages = {909--935},
title = {{Two scale damage model and related numerical issues for thermo-mechanical High Cycle Fatigue}},
volume = {26},
year = {2007}
}
@article{Rostampour2015c,
abstract = {This investigation deals with the EF7 (TC) engine, a dual fuel engine equipped with a turbocharger system, consequently with a high probability of knock inception. In this study, an operating cycle of the engine was simulated using KIVA-3V code. Some modifications were carried out on the KIVA method of calculating pressure in the intake port in order to simulate turbocharger pressure correctly. Auto-ignition and knock were then simulated using the auto-ignition integral model. The modified code and the simulation were verified using three different methods; in-cylinder average pressure, gas temperature of the exhaust port, and auto-ignition timing. The simulation results using the auto-ignition integral model, as compared with the experimental data, proved to be reasonably accurate. Following this validation, the effect of the knock phenomenon on the engine heat transfer through the walls was investigated. The simulations showed that the rate of heat transfer through the walls under knocking conditions is about 2.2 times higher than that under normal conditions. However, it was also shown that the total heat transfer increases about 15{\%}.},
author = {Rostampour, Arman and Toosi, Ali Nassiri},
doi = {10.1115/1.4030517},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Klopfen{\_}Ottomotor/2015{\_}Rostampour{\_}Numerical Investigation of the effect of knock on heat transfer in a turbo si engine.pdf:pdf},
issn = {0742-4795},
journal = {J. Eng. Gas Turbines Power},
number = {12},
pages = {121502},
title = {{Numerical Investigation of the Effect of Knock on Heat Transfer in a Turbocharged Spark Ignition Engine}},
url = {http://www.scopus.com/inward/record.url?eid=2-s2.0-84930634240{\&}partnerID=tZOtx3y1},
volume = {137},
year = {2015}
}
@article{Karnik2015a,
author = {Karnik, Amey and Pachner, Daniel and Fuxman, Adrian M and Germann, David and Jankovic, Mrdjan and House, Christopher},
doi = {10.4271/2015-01-0336},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Thermal Coating + Water Heat Transfer + Applikation/2015{\_}Karnik{\_}Model Predictive Control for Engine Powertrain Thermal Management Applications.pdf:pdf},
journal = {SAE 2015 World Congr. Exhib.},
title = {{Model Predictive Control for Engine Powertrain Thermal Management Applications}},
url = {http://papers.sae.org/2015-01-0336/},
year = {2015}
}
@article{Beispiela,
author = {Beispiel, Am and Problembereiche, Mittellagen and Vorgang, Dieser and Durch-, Ein},
pages = {4--7},
title = {{4 CA-Systeme und deren Einsatz im Karosseriebau}}
}
@article{2012,
author = {Ε$\pi$$\iota$$\tau$$\rho$ο$\pi$ά$\kappa$$\eta$ς, Ι},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/{\_}buecherSong/HandbookofComposites/II/21{\_}FilamentWinding.pdf:pdf},
title = {{Χ$\alpha$$\rho$$\alpha$$\kappa$$\tau$$\eta$$\rho$$\iota$$\sigma$$\mu$ός $\Sigma$ύ$\nu$$\theta$$\epsilon$$\tau$$\omega$$\nu$ $\Upsilon$$\lambda$$\iota$$\kappa$ώ$\nu$ Α$\nu$$\theta$$\rho$$\alpha$$\kappa$ο$\nu$$\eta$$\mu$ά$\tau$$\omega$$\nu$ Κ$\alpha$$\tau$$\alpha$$\sigma$$\kappa$$\epsilon$$\upsilon$$\alpha$$\sigma$$\mu$έ$\nu$$\omega$$\nu$ Μ$\epsilon$ Τ$\eta$ Μέ$\theta$ο$\delta$ο $\Pi$$\epsilon$$\rho$$\iota$έ$\lambda$$\iota$$\xi$$\eta$ς Τ$\omega$$\nu$ Ι$\nu$ώ$\nu$ (Filament Winding)}},
year = {2012}
}
@article{Forest2009a,
abstract = {A unifying thermomechanical framework is presented that reconciles several classes of gradient elastoviscoplasticity and damage models proposed in the literature during the last 40 years. It is based on the introduction of the micromorphic counterpart ϕ $\chi$ of a selected ... $\backslash$n},
author = {Forest, Samuel},
doi = {10.1061/(ASCE)0733-9399(2009)135:3(117)},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/2009{\_}Forest{\_}Micromorphic Approach for Gradient Elasticity Viscoplasticity and Damage.pdf:pdf},
isbn = {0733-9399},
issn = {0733-9399},
journal = {J. Eng. Mech.},
number = {3},
pages = {117--131},
title = {{Micromorphic Approach for Gradient Elasticity, Viscoplasticity, and Damage}},
volume = {135},
year = {2009}
}
@article{Cheong2007a,
abstract = {The influence of individual grain orientation on early fatigue crack initiation in a four-point bend fatigue test was investigated numerically and experimentally. The 99.99{\%} aluminium test sample was subjected to high cycle fatigue (HCF) and the top surface microstructure within the inner span of the sample was characterized using electron-beam backscattering diffraction (EBSD). Applying a finite-element submodelling approach, the microstructure was digitally reconstructed and refined studies carried out in regions where fatigue damage was observed. The constitutive behaviour of aluminium was described by a crystal plasticity model which considers the evolution of dislocations and accumulation of edge dislocation dipoles. Using an energy-based approach to quantify fatigue damage, the model correctly predicts regions in grains where early fatigue crack initiation was observed. The tendency for fatigue cracks to initiate in these grains appears to be strongly linked to the orientations of the grains relative to the direction of loading - grains less favourably aligned with respect to the loading direction appear more susceptible to fatigue crack initiation. The limitations of this modelling approach are also highlighted and discussed, as some grains predicted to initiate cracks did not show any visible signs of fatigue cracking in the same locations during testing. ?? 2006 Acta Materialia Inc.},
author = {Cheong, Ke Shen and Smillie, Matthew J. and Knowles, David M.},
doi = {10.1016/j.actamat.2006.10.038},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2006{\_}Cheong{\_}Predicting fatigue crack initiation through image-based micromechanical modeling.pdf:pdf},
isbn = {1359-6454},
issn = {13596454},
journal = {Acta Mater.},
keywords = {Crystal plasticity,Dislocations,Electron backscatter diffraction,Image analysis,Micromechanical modelling},
number = {5},
pages = {1757--1768},
title = {{Predicting fatigue crack initiation through image-based micromechanical modeling}},
volume = {55},
year = {2007}
}
@article{Atherosklerose2000,
author = {Atherosklerose, Die},
pages = {7--19},
title = {{1. Einleitung}},
year = {2000}
}
@article{Tschirschwitza,
author = {Tschirschwitz, Christian},
journal = {Asphalt},
pages = {653--663},
title = {{B6 B6 Unf{\"{a}}lle mit Kleintransportern B6}}
}
@article{Klein2012a,
author = {Klein, B},
doi = {10.1007/978-3-8348-2134-8},
isbn = {9783834821348},
title = {{5 Das Konzept der Finite-Element-Methode}},
year = {2012}
}
@book{Shclick2013,
abstract = {In this paper, the Turing instability in reaction-diffusion models defined on complex networks is studied. Here, we focus on three types of models which generate complex networks, i.e. the Erd$\backslash$H{\{}o{\}}s-R$\backslash$'enyi, the Watts-Strogatz and the threshold network models. From analysis of the Laplacian matrices of graphs generated by these models, we reveal that the stable-unstable regions of a spatially homogeneous solution completely differ, depending on network structures. In particular, we approximately argue the existence of the stable-unstable regions in the cases of regular enhanced ring lattices which include regular circles, and networks generated by the threshold network model when the number of vertices is large enough.},
archivePrefix = {arXiv},
arxivId = {1406.6401},
author = {Shclick, Tamra and Torquato, Salvatore},
booktitle = {Phys. Rev. E - Stat. Nonlinear, Soft Matter Phys.},
doi = {10.1016/j.camwa.2013.03.019},
eprint = {1406.6401},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Simu, Hughes 1998 - Computational Inelasticity.pdf:pdf},
isbn = {4420767936},
issn = {1539-3755},
keywords = {05c82,1,2010 msc,35k57,60g05,60j60,70k50,92c15,92c40,Amplitude equation,Cortical folding,Cross diffusion,Ginzburg-Landau equation,Growing domain,Linearised stability,Morphology,Nonlinear diffusion,Pattern formation,Quintic Stuart-Landau equation,Reaction-diffusion system,Turing bifurcation,Turing system,activator,ams subject classifications,and another for inhibitor,and diffusion,approaches to the mathematical,based,clo,compartment-based models,complex network,cross-diffusion,cross-diffusion systems,deterministic models which are,diffusion models,diffusion system,epstein,growing domain,holling type-ii functional response,i,instability,introduction,le,lengyel,model,modelling of chemical reactions,non-constant positive steady state,pattern,pattern formation,reaction,reaction-diffusion,reaction-diffusion models on networks,reaction-diffusion processes,reaction-diffusion systems,self-organised spatial pattern,stationary patterns,stochastic processes,stochastic simulations,stochastic turing patterns,systems,there are two fundamental,turing instability,turing pattern,turing reaction,turing system},
number = {4},
pages = {476},
pmid = {15267983},
title = {{Interdisciplinary Applied Mathematics}},
url = {http://link.springer.com/10.1140/epjb/e2013-40570-8{\%}5Cnhttp://arxiv.org/abs/1406.6401{\%}5Cnhttp://arxiv.org/abs/1204.1475{\%}5Cnhttp://link.aps.org/doi/10.1103/PhysRevLett.91.058302{\%}5Cnhttp://arxiv.org/abs/nlin/0111059{\%}5Cnhttp://link.aps.org/doi/10.1103/PhysRe},
volume = {82},
year = {2013}
}
@article{Contents,
author = {Contents, Chapter},
pages = {48--140},
title = {{Solution of Nonlinear}},
volume = {1}
}
@article{Eekoye1996c,
abstract = {Heat-transfer rates present in an engine cylinder undergoing knock are known to be larger than the rates associated with normal engine operation. Further, at the time of knock, the largest heat fluxes are associated with locations on the cylinder wall where the flame is locally quenching. In this study, heat-transfer processes at the flame-wall interface during a knock event are investigated computationally and analytically. Computationally, the governing equations for a one-dimensional, flame-quenching event are solved using a reduced chemical reaction mechanism. Analytically, scaling relations for the flame heat-release rates are used in the governing equations to determine the heat-transfer rates. It is found that while pressure transients modify the wall heat flux, the absolute value of the pressure is the most significant parameter in predicting the maximum heat flux. The wall heat flux profiles are predicted for both the analytical and computational models. In the range of pressures examined, a linear relationship was found between the peak flux and pressure, both for the computational and analytical models. The linear relationship between the pressure and peak flux was found to be invalid when the flame-quenching process was disrupted by the pressure fluctuations for pressure oscillations with a characteristic time on the order of the quenching process. ?? 1996 Combustion Institute.},
author = {Eekoye, O A},
doi = {10.1016/S0082-0784(96)80101-9},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/1996{\_}Ezekoye{\_}Heat transfer modeling during knock and flame quenching in an engine chamber.pdf:pdf},
isbn = {0082-0784},
issn = {00820784},
journal = {Symp. Combust.},
number = {2},
pages = {2661--2668},
title = {{Heat transfer modeling during knock and flame quenching in an engine chamber}},
volume = {26},
year = {1996}
}
@article{Metallplastizit2013c,
author = {Metallplastizit, Hrungdie and Helm, Dirk},
number = {November},
pages = {1--29},
title = {{Prozesssimulation in Der Umformtechnik}},
year = {2013}
}
@book{Warnatz2006,
author = {Warnatz, J and Maas, U and Dibble, R W},
booktitle = {New York},
edition = {4},
isbn = {9783540259923},
publisher = {Springer Berlin Heidelberg New York},
title = {{Combustion}},
year = {2006}
}
@book{Rieger,
author = {Rieger, Florian},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Plasticity models/2015{\_}Rieger{\_}Work-hardening of dual-phase steel.pdf:pdf},
isbn = {9783731505136},
title = {{Florian Rieger Work-hardening of dual-phase steel}}
}
@article{Skrotzki,
author = {Skrotzki, B and Simon, F and Materialkreislauf, Der},
journal = {H{\"{u}}tte},
pages = {1--110},
title = {{D-Werkstoffe}}
}
@article{Paul1994,
author = {Paul, Reinhold},
doi = {10.1007/978-3-322-96651-3_6},
isbn = {978-3-519-02126-1},
journal = {Elektrotechnik und Elektron. f{\"{u}}r Inform. SE - 6},
pages = {435--520},
title = {{Das elektromagnetische Feld}},
url = {http://dx.doi.org/10.1007/978-3-322-96651-3{\_}6},
year = {1994}
}
@article{Schraubradgetriebe,
author = {Schraubradgetriebe, Einheit Benennung},
pages = {278--292},
title = {{23 Sdiraubrad- und Schneckengetriebe}}
}
@article{Rinato1995,
author = {Rinato, Infrastruktur-},
pages = {619},
title = {{Teil V}},
year = {1995}
}
@article{Kametani1980a,
author = {Kametani, T. and Umezawa, O.},
doi = {10.1248/cpb.37.3229},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/1994{\_}Enomoto{\_}Heat Losses during Knocking in a Four-Stroke Gasoline Engine.pdf:pdf},
issn = {09168451},
journal = {Chem. Pharm. Bull.},
number = {6},
pages = {369--375},
pmid = {8987871},
title = {{NII-Electronic Library Service}},
volume = {28},
year = {1980}
}
@article{Crisfield1996,
abstract = {applicability for this approach.},
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Crisfield, Mike a},
doi = {10.1017/CBO9781107415324.004},
eprint = {arXiv:1011.1669v3},
isbn = {978-0-470-66644-9},
issn = {1098-6596},
journal = {John Wiley Sons, Inc.},
keywords = {icle},
pages = {31--62},
pmid = {25246403},
title = {{Nonlinear Finite Element Analysis of Solids and Structures}},
url = {http://eu.wiley.com/WileyCDA/WileyTitle/productCd-0470666447.html},
year = {1996}
}
@article{Vorbemerkungen2010,
author = {Vorbemerkungen, A Motivierende},
doi = {10.1007/978-3-642-05185-2},
isbn = {9783642051852},
pages = {37--65},
title = {{Kapitel 15}},
year = {2010}
}
@article{Fs2013a,
author = {Fs},
doi = {10.1007/978-1-4614-0502-3},
isbn = {2009004043},
number = {1},
pages = {0--10},
title = {{Chapter 0}},
year = {2013}
}
@article{Sellars1954,
author = {Sellars, John and Tribus, Myron and Klein, John},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Heat transfer intake+exhaust system/1954{\_}Sellars{\_}Heat transfer to laminar flow on a round tube or flat conduit - the graetz  problem extended.pdf:pdf},
journal = {WADC Tech. Rep. 54-255},
pages = {1--23},
title = {{Heat Transfer To Laminar Flow In A Round Tube Or Flat Conduit: The Graetz Problem Extended}},
year = {1954}
}
@article{Pan2014,
abstract = {Knocking combustion in spark-ignition (SI) engines is a typical abnormal combustion phenomenon that severely limits engine performance and thermal efficiency. However, its mechanism has not so far been completely revealed, such as the origin of pressure oscillation with tremendous amplitude and broken mechanisms of the engine body when knock occurs. This article systematically reviews the series of physical and chemical phenomena involved in knocking combustion, including auto-ignition, gas-dynamic waves, cavity resonance, and auto-ignited flame propagation. Significant research has shown that the rapid heat release of end-gas auto-ignition and subsequent strong pressure waves play a crucial role during knocking combustion. A methodology of the interaction of flame propagation and pressure waves has been proposed to reveal knock formation in terms of positive feedback between strengthened pressure waves and auto-ignited flame propagation. Also, new suggestions on the weakness in prior research of knocking combustion have also been discussed in the present article. {\{}{\textcopyright}{\}} 2014 Copyright Taylor and Francis Group, LLC.},
author = {Pan, Jiaying and Shu, Gequn and Wei, Haiqiao},
doi = {10.1080/00102202.2013.857665},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2014{\_}Pan+Wei{\_}Interaction of Flame Propagation and Pressure Waves During Knocking Combustion in Spark-Ignition Engines.pdf:pdf},
issn = {0010-2202},
journal = {Combust. Sci. Technol.},
number = {2},
pages = {192--209},
title = {{Interaction of Flame Propagation and Pressure Waves During Knocking Combustion in Spark-Ignition Engines}},
url = {http://www.tandfonline.com/doi/abs/10.1080/00102202.2013.857665},
volume = {186},
year = {2014}
}
@article{Zienkiewicz2005a,
author = {Zienkiewicz, O C and Taylor, R L and Zhu, J Z},
doi = {http://dx.doi.org/10.1016/B978-075066431-8.50180-6},
isbn = {978-0-7506-6431-8},
journal = {Finite Elem. Method - Its Basis Fundam.},
pages = {27},
title = {{12-Multidomain mixed approximations – domain decomposition and ‘frame' methods}},
year = {2005}
}
@article{Bockh2006,
author = {B{\"{o}}ckh, Peter},
doi = {10.1007/978-3-662-44477-1},
isbn = {978-3-662-44476-4},
title = {{W{\{}{\"{a}}{\}}rme{\{}{\"{u}}{\}}bertragung}},
url = {http://link.springer.com/10.1007/978-3-662-44477-1},
year = {2006}
}
@article{Burg,
author = {Burg, Heinz and {\"{A}}ein, Buch and Sanner, Gegenwart Von},
pages = {3--25},
title = {{A1 A1 Allgemeine Anmerkungen zum Sachverst{\{}{\"{a}}{\}}ndigenwesen A1}}
}
@article{Bozek2008a,
abstract = {Microstructurally small fatigue crack (MSFC) formation includes stages of incubation, nucleation and microstructurally small propagation. In AA 7075-T651, the fracture of Al 7 Cu 2 Fe constituent particles is the major incubation source. In experiments, it has been observed that only a small percentage of these Fe-bearing particles crack in a highly stressed volume. The work presented here addresses the identification of the particles prone to cracking and the prediction of particle cracking frequency, given a distribution of particles and crystallographic texture in such a volume. Three-dimensional elasto-viscoplastic finite element analyses are performed to develop a response surface for the tensile stress in the particle as a function of the strain level surrounding the particle, parent grain orientation and particle aspect ratio. A technique for estimating particle strength from fracture toughness, particle size and intrinsic flaw size is developed. Particle cracking is then determined by comparing particle stress and strength. The frequency of particle cracking is then predicted from sampling measured distributions of grain orientation, particle aspect ratio and size. Good agreement is found between the predicted frequency of particle cracking and two preliminary validation experiments. An estimate of particle cracking frequency is important for simulating the next stages of MSFC formation: inserting all particles into a microstructural model for these stages is computationally intractable and physically unnecessary.},
author = {Bozek, J E and Hochhalter, J D and Veilleux, M G and Liu, M and Heber, G and Sintay, S D and Rollett, A D and Littlewood, D J and Maniatty, A M and Weiland, H and Christ, R J and Payne, J and Welsh, G and Harlow, D G and Wawrzynek, P A and Ingraffea, A R},
doi = {10.1088/0965-0393/16/6/065007},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/2008{\_}Hochhalter{\_}AL7075AgeometricapproachI{\_}ParticeleCracking.pdf:pdf},
isbn = {09650393 (ISSN)},
issn = {0965-0393},
journal = {Model. Simul. Mater. Sci. Eng.},
number = {6},
pages = {65007},
title = {{A geometric approach to modeling microstructurally small fatigue crack formation: I. Probabilistic simulation of constituent particle cracking in AA 7075-T651}},
url = {http://stacks.iop.org/0965-0393/16/i=6/a=065007?key=crossref.c2c7fddb48a7b52013977b4d25c503c4},
volume = {16},
year = {2008}
}
@article{Desmorat2006a,
abstract = {Application of damage mechanics to fatigue is addressed in the present paper. The ability of Lemaitre's damage law to describe low and high cycle fatigue failure of metals is illustrated. Its generalization into an evolution law modeling a damage rate governed by the main dissipative mechanics applies to concrete, elastomers, rocks and to probably other materials. The importance of rate written laws is emphasized.},
author = {Desmorat, Rodrigue},
doi = {10.1080/17747120.2006.9692859},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/2006{\_}Desmorat{\_}SummerSchool{\_}Damage and Fatigue Overview Evolution Equation.pdf:pdf},
isbn = {9780387739052},
issn = {1774-7120},
journal = {Rev. Eur. G{\'{e}}nie Civ.},
keywords = {concrete,damage,elastomers,fatigue,metals,rocks},
number = {6-7},
pages = {849--877},
title = {{Damage and Fatigue: Continuum damage mechanics modeling for fatigue of materials and structures}},
volume = {10},
year = {2006}
}
@article{Burg,
author = {Burg, Heinz and {\"{A}}ein, Buch and Sanner, Gegenwart Von},
pages = {3--25},
title = {{A1 A1 Allgemeine Anmerkungen zum Sachverst{\"{a}}ndigenwesen A1}}
}
@article{Betrachtungene,
author = {Betrachtungen, Allgemeine},
title = {{omungen gro{\ss}er Reynoldszahlen ( Grenzschichtstr ¨ omungen )}}
}
@article{Skizzierers2011,
author = {Skizzierers, Aufruf},
doi = {10.1007/978-3-8348-8161-8},
isbn = {9783834881618},
pages = {28--38},
title = {{3 Volumenmodellierung im Skizzier-Modus}},
year = {2011}
}
@article{Voraussetzung,
author = {Voraussetzung, Die},
pages = {144--151},
title = {{11 Biegung offener Profilst{\"{a}}be}}
}
@article{Gratzera,
author = {Gratzer, Werner and Becke, Manfred},
pages = {89--169},
title = {{A5 A5 Kinematik A5}}
}
@book{Hartley2006,
abstract = {This book gives an introduction to computational plasticity and includes the kinematics of large deformations, together with relevant continuum mechanics. Central to the book is its focus on computational plasticity, and we cover an introduction to the finite element method which includes both quasi-static and dynamic problems. We then go on to describe explicit and implicit implementations of plasticity models in to finite element software. Throughout the book, we describe thegeneral, multiaxial form of the theory but uniquely, wherever possible, reduce the equations to their simplest, uniaxial form to develop understanding of the general theory and, we hope, physical insight. We provide several examples of implicit and explicit implementations of von Mises time-independentand visco-plasticity in to the commercial code ABAQUS (including the fortran coding), which should prove invaluable to research students and practising engineers developing ABAQUS 'UMATs'. The book bridges the gap between undergraduate material on plasticity and existing advanced texts on nonlinear computational mechanics, which makes it ideal for students and practising engineers alike. It introduces a range of engineering applications, including superplasticity, porous plasticity, cyclicplasticity and thermo-mechanical fatigue, to emphasize the subject's relevance and importance.},
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Hartley, P},
booktitle = {J. Phys. A. Math. Gen.},
doi = {10.1088/0305-4470/39/14/B02},
eprint = {arXiv:1011.1669v3},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Dunne, Petrinic 2006 - Introduction to Computational Plasticity.pdf:pdf},
isbn = {9780198568261},
issn = {0305-4470},
number = {14},
pages = {3850--3851},
pmid = {25246403},
title = {{Introduction to Computational Plasticity}},
url = {http://stacks.iop.org/0305-4470/39/i=14/a=B02?key=crossref.df6043dc7dee1ea3fe9a75a1094a108d},
volume = {39},
year = {2006}
}
@article{Sietsma,
author = {Sietsma, J},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/Hardening Recovery Creep/KocksMecking{\_}Annihilation of dislocation in plastic deformation.pdf:pdf},
pages = {1--24},
title = {{Dislocation annihilation in plastic deformation}}
}
@inproceedings{Hoermann2005,
abstract = {The present paper is part of a more comprehensive study concerning the surface flow in the engine compartment and focuses on the fluid flow of a cooling system in a modern vehicle. The complexity of this field needs to further optimization in the integration of 3D CFD (Computational Fluid Dynamics) methods. An important focus lies on the modeling of radiators and fans. A new simulation method needs to be validated. For this purpose a component test bench was built.This paper shows the results oft the simulation on the test bench and the CFD analysis. All the fan and radiator model configurations have been studied by means of a commercial CFD package. The comparison of the results gives a better understanding of the total system performance for a faster and more reliable preliminary design.},
author = {H{\"{o}}rmann, T and Lechner, B and Puntigam, W and Moshammer, T and Almbauer, R},
booktitle = {Veh. Therm. Manag. Syst. Conf. Expo.},
doi = {10.4271/2005-01-2006},
publisher = {SAE International},
title = {{Numerical and Experimental Investigation of Flow and Temperature Fields around Automotive Cooling Systems}},
year = {2005}
}
@article{Ingenieur,
author = {Ingenieur, Ein and Erfolg, Der and Unix, Betriebssystems},
title = {{6 C f{\"{u}}r die 8051-Familie}}
}
@article{Lal1977a,
abstract = {This paper reviews and compares the various approaches for finding monotonic and cyclic plastic zone sizes for elastic-perfectly plastic and strain hardening materials. All through the analysis Ramberg-Osgood relationship has been used representing the monotonic and cyclic stress-strain curves. The results for elastic-perfectly plastic materials are compared with those available using finite-element technique. The ratio of monotonic plastic zone sizes strain hardening and elastic perfectly plastic materials are found to be related to the Ramberg-Osgood index n. The values of cyclic plastic zone size are found to depend upon factors like crack opening stress, material properties and specimen geometry. The cyclic plastic zone size obtained in this paper compare well with those given by Antolovich. ?? 1977.},
author = {Lal, K M and Garg, S B L},
doi = {10.1016/0013-7944(77)90036-4},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/1977{\_}LAL+GARG{\_}On the evaluation of monotonic and cyclic plastic zones.pdf:pdf},
issn = {00137944},
journal = {Eng. Fract. Mech.},
number = {2},
pages = {433--442},
title = {{On the evaluation of monotonic and cyclic plastic zones}},
volume = {9},
year = {1977}
}
@article{Forte2014,
abstract = {A methodology for the evaluation of the effects of twin spark ignition system on CCV (Cycle by Cycle Variability) and knocking combustions is here presented, based on both the use of Computation Fluid Dynamics (CFD) tools and experimental information. The focus of the numerical methodology is the statistical evaluation of the local air-to-fuel distribution at the spark plugs and its correlation with the variability of the initial stages of combustion. A detailed analysis of knocking events can help improving engine performance and diagnosis strategies. The use of twin spark ignition system can enhance the probability that the initial kernel could come across a zone with the correct air-to-fuel ratio, thus lowering the initial combustion instabilities. Moreover the lower distance swept from the flame fronts can considerably reduce the time for the unburnt mixture to auto-ignite, thus reducing the risk of knocking combustion. CFD simulations have been used to reproduce knock effect on the in-cylinder pressure trace. The pressure signal holds information about waves propagation and heat losses: it is crucial to relate local pressure oscillations to knock severity. For this purpose, a CFD model has been implemented, able to predict the combustion evolution with respect to Spark Advance, from non-knocking up to heavy knocking conditions. The CFD model validation phase is essential for a correct representation of both regular and knocking combustions: the operation has been carried out by means of an accurate statistical analysis of experimental in-cylinder pressure data. ?? 2013 The Authors.},
author = {Forte, Claudio and Bianchi, Gian Marco and Corti, Enrico and Fantoni, Stefano and Costa, Marco},
doi = {10.1016/j.egypro.2014.01.091},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Klopfen{\_}Ottomotor/2014{\_}Forte+Corti+Bianchi{\_}CFD Methodology for the evaluation of knock of a PFI Twin Spark Engine.pdf:pdf},
isbn = {3905120933},
issn = {18766102},
journal = {Energy Procedia},
keywords = {Cycle by Cycle Variability,High performance engine,Knock,Twin spark},
pages = {859--868},
publisher = {Elsevier B.V.},
title = {{CFD methodology for the evaluation of knock of a PFI Twin spark engine}},
url = {http://dx.doi.org/10.1016/j.egypro.2014.01.091},
volume = {45},
year = {2014}
}
@article{Pla,
author = {Pla, Wilfried},
isbn = {9783528039738},
keywords = {fgang b{\"{o}}ge,formeln und tabellen,hrsg,wilfried pla{\ss}mann},
title = {{Wolfgang B{\"{o}}ge , Wilfried Pla{\ss}mann ( Hrsg .) Formeln und Tabellen Elektrotechnik}}
}
@article{Terms2003,
abstract = {SUBJECT INDEX Absorption, intestinal Effect of Inborn Errors of Bile A.. Absorption; fat Highly Effective Enteral Treatmen., . intestinal-specific deletion of m, . . Altered MetabolLsm of Postprandia... Effect of Glucagon-fike Peptide-1.. 5-HT3 receptors are essential for...},
author = {Terms, Index},
doi = {10.1016/S0016-5085(03)84188-4},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Zienkiewicz FEM - Vol 1 Basics Fundamentals/63205{\_}sindx.pdf:pdf},
issn = {00165085},
journal = {Gastroenterology},
number = {4},
pages = {AA60--AA102},
title = {{Subject index}},
url = {http://www.sciencedirect.com/science?{\_}ob=GatewayURL{\&}{\_}origin=ScienceSearch{\&}{\_}method=citationSearch{\&}{\_}piikey=S0016508503841884{\&}{\_}version=1{\&}{\_}returnURL={\&}md5=47aa5121dbf61e18d5fcb18eefe1bd2e},
volume = {124},
year = {2003}
}
@article{Heth1998,
author = {Heth, Jennifer A},
title = {{Safety and health issues}},
year = {1998}
}
@article{Esfahanian2006b,
abstract = {In this study, the heat transfer to an engine piston crown is calculated. Three different methods for the combustion boundary condition are used. The results of different combustion side boundary condition treatments are compared and their effects on the thermal behavior of the piston are investigated. It has been shown that using spatial and time averaged combustion side boundary condition is a suitable treatment method within engineering approximations. An interface between KIVA-3V and NASTRAN codes is developed. {\textcopyright} 2005 Elsevier Ltd. All rights reserved.},
author = {Esfahanian, V. and Javaheri, A. and Ghaffarpour, M.},
doi = {10.1016/j.applthermaleng.2005.05.002},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/W{\"{a}}rme-RBen Kolben/2006{\_}Esfahanian{\_}Thermal analysis of an SI engine piston using different combustion boundary condition treatements.pdf:pdf},
issn = {13594311},
journal = {Appl. Therm. Eng.},
keywords = {Boundary Condition Treatment,Combustion,Heat transfer,Piston},
number = {2-3},
pages = {277--287},
title = {{Thermal analysis of an SI engine piston using different combustion boundary condition treatments}},
volume = {26},
year = {2006}
}
@article{Getriebe2007,
author = {Getriebe, Gesamtsystems and Einsparung, Durch},
journal = {Fahrzeuggetriebe},
title = {{14 Rechnerunterst{\"{u}}tzte Getriebeentwicklung}},
year = {2007}
}
@article{McDowell2007,
abstract = {Further efforts to provide more direct dependence of fatigue life estimation methods on microstructure of alloy systems must consider various factors that are not explicitly addressed by conventional fatigue design tools such as the strain-life curve, the stress-life curve, the modified Goodman diagram, or fatigue limit concepts, or by traditional linear elastic fracture mechanics approaches. In this work, we offer insight from micromechanical perspectives on tradeoffs of fatigue crack formation and growth regimes in low cycle and high cycle fatigue, including considerations of effects of notches of various scales. Relations between remote loading conditions and microstructure-scale cyclic plasticity/crack behavior are considered as a function of stress amplitude and microstructure to support assessment of intrinsic microstructure fatigue resistance (percolation limits for connected microplasticity) as well as effects of extrinsic features such as non-metallic inclusions. Algorithms are summarized for computing nonlocal cyclic plastic shear strain and inferring fatigue resistance, both in terms of mean behavior and variability with microstructure. Several applications are presented, including intrinsic and extrinsic fatigue resistance of Ni-base superalloys, fatigue of polycrystals, cast A356-T6 Al alloy, and fretting fatigue of Ti-6Al-4V. {\textcopyright} 2007 Elsevier B.V. All rights reserved.},
author = {McDowell, David L.},
doi = {10.1016/j.msea.2006.08.129},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/2006{\_}McDowell{\_}Simulation-based strategies for microstructure-sensitive fatigue modeling.pdf:pdf},
isbn = {0921-5093},
issn = {09215093},
journal = {Mater. Sci. Eng. A},
keywords = {Computational fatigue,Hierarchical microstructure,Microstructure,Simulation-based fatigue},
number = {SPEC. ISS.},
pages = {4--14},
title = {{Simulation-based strategies for microstructure-sensitive fatigue modeling}},
volume = {468-470},
year = {2007}
}
@article{Winkel,
author = {Winkel, Machschen},
title = {{Omungen ¨}}
}
@article{Federung,
author = {Federung, Aufgaben Der},
title = {{5 Federung und D{\"{a}}mpfung}}
}
@article{Depcik2002,
abstract = {In this paper, the available correlations proposed in the literature for the gas-side heat transfer in the intake and exhaust system of a spark-ignition internal combustion engine were surveyed. It was noticed that theseAB - {\textless}inline-graphic xlink:href="2002-01-0372{\_}fig0001" xmlns:xlink="http://www.w3.org/1999/xlink"/{\textgreater}AB - only by empirically fitted constants. This similarity provided the impetus for the authors to explore if a universal correlation could be developed. Based on a scaling approach using microscales of turbulence, the authors have fixed the exponential factor on the Reynolds number and thus reduced the number of adjustable coefficients to just one; the latter can be determined from a least squares curve-fit of available experimental data. Using intake and exhaust side data, it was shown that the universal correlationAB - {\textless}inline-graphic xlink:href="2002-01-0372{\_}fig0002" xmlns:xlink="http://www.w3.org/1999/xlink"/{\textgreater}AB - The correlation coefficient of this proposed heat transfer model with all available experimental data is 0.845 for the intake side and 0.800 for the exhaust side.ER -},
author = {Depcik, Christopher and Assanis, Dennis},
doi = {10.4271/2002-01-0372},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2002{\_}Depcik{\_}A Universal Heat Transfer Correlation for intake and exhaust flows in an SI internal combustion engine.pdf:pdf},
journal = {SAE Pap.},
number = {January 2016},
title = {{A Universal Heat Transfer Correlation for Intake and Exhaust Flows in an Spark-Ignition Internal Combustion Engine}},
url = {http://papers.sae.org/2002-01-0372},
volume = {2002-01-03},
year = {2002}
}
@article{Und1999,
author = {Und, Inleitung},
pages = {1--9},
title = {{1 Einleitung und Zielsetzung}},
year = {1999}
}
@book{Bonnet2009a,
abstract = {Ein Verbundwerkstoff ist ein Werkstoff aus zwei oder mehr verbundenen Materialien. Der Verbundwerkstoff besitzt andere Werkstoffeigenschaften als seine einzelnen Komponenten.},
author = {Bonnet, Martin},
doi = {10.1007/978-3-8348-9303-1},
isbn = {978-3-8348-0349-8},
issn = {00182001},
pages = {79},
title = {{Kunststoffe in der Ingenieuranwendung}},
url = {http://link.springer.com/10.1007/978-3-8348-9303-1},
year = {2009}
}
@article{Pahl2005,
author = {Pahl, Gerhard},
journal = {Konstr. Grundlagen erfolgreicher Produktentwicklung Methoden und Anwendung},
pages = {231--303},
title = {{6. Methodisches Konzipieren Methods for conceptual design}},
year = {2005}
}
@article{Liu1972,
abstract = {1. Introduction In thermodynamics, whenever a material is subject to investigation of its properties, the entropy principle is used to impose restrictions on the constitutive relations for the material. There is not, so far, any simple method by which restrictions from the entropy ... },
author = {Liu, I. Shih},
doi = {10.1007/BF00250688},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Thermodynamik/Liu{\_}Entropieprinzip{\_}Lagrange/Method of LAgrange Multipliers for Exploitation of the Entropy Principle {\_} Liu.pdf:pdf},
issn = {00039527},
journal = {Arch. Ration. Mech. Anal.},
number = {2},
pages = {131--148},
title = {{Method of Lagrange multipliers for exploitation of the entropy principle}},
volume = {46},
year = {1972}
}
@book{HuseyinSehitoglu2000,
author = {{Huseyin Sehitoglu} and {Hans J. Maier}},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/2000{\_}Huseyin Sehitoglu{\_}Thermo-mechanical Fatigue Behavior of  Materials{\_}OverviewDifferentPapers.pdf:pdf},
isbn = {0803128533},
pages = {151},
title = {{Thermo-mechanical Fatigue Behavior of Materials: Third volume}},
url = {https://books.google.se/books?id=ZY84rIMG82sC{\%}7B{\&}{\%}7Dpg=PA150{\%}7B{\&}{\%}7Dlpg=PA150{\%}7B{\&}{\%}7Ddq=thermomechanical+fatigue+behavior+of+materials{\%}7B{\&}{\%}7Dsource=bl{\%}7B{\&}{\%}7Dots=93h1yoyJVR{\%}7B{\&}{\%}7Dsig=YTp4LbQdi6Kms-Ys06yBsW5LnPU{\%}7B{\&}{\%}7Dhl=sv{\%}7B{\&}{\%}7Dsa=X{\%}7B{\&}{\%}7Dved=0ahUKEwidx4jg2},
year = {2000}
}
@article{Plewinsky,
author = {Plewinsky, B and Hennecke, M and Oppermann, W},
journal = {H{\"{u}}tte},
pages = {1--114},
title = {{C-Chemie}}
}
@article{Liberalisierung1998,
author = {Liberalisierung, Thema and Schwankungen, Wettbewerbs and Folgenden, Im and Struktur, Die and Zeit, Die and Strompreise, Die},
doi = {10.1007/978-3-8348-2279-6},
isbn = {9783834822796},
number = {Ka V},
pages = {325--336},
title = {{18 Liberalisierung der Energiem{\{}{\"{a}}{\}}rkte}},
year = {1998}
}
@article{Zurek1983,
abstract = {The influence of alloy grain size on growth rates of surface cracks 20 to 500 {\$}\mu{\$}m in length was studied in Al 7075-T6 specimens prepared in 12 and 130 {\$}\mu{\$}n grain sizes. Grain boundaries temporarily interrupt the propagation of cracks shorter than several grain diameters in length. Linear elastic fracture mechanics is inadequate to describe resulting average growth rates which must instead be characterized as a function of cyclic stress amplitude, {\$}\sigma{\$}a, and alloy grain size as well as stress intensity range, {\$}\sigma{\$}K. These observations are rationalized using two models, one that relates crack closure stress to alloy grain size, and a second that relates the development of microplasticity in a new grain in the crack path to grain size. In addition, growth rates were found to be faster in fully reversed loading than in tension-tension loading, especially in the large grained material. Evidence is presented to demonstrate that this is a consequence of the fatigue induced development of a compressive residual surface stress during tension-tension loading. These complex effects, and the role of grain size in determining short crack growth, are discussed.},
author = {Zurek, A K and James, M R and Morris, W L},
doi = {10.1007/BF02654397},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/1983{\_}Morris{\_}The effect of grain size on fatigue growth of short cracks.pdf:pdf},
isbn = {03602133},
issn = {03602133},
journal = {Met. Trans. A},
number = {8},
pages = {1697--1705},
title = {{The Effect of Grain Size on Fatigue Growth of Short Cracks}},
volume = {14},
year = {1983}
}
@article{Castillo2009a,
author = {Castillo, E},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Probabilistic Aspects/A Unified Statistical Methodology for Modeling Fatigue Damage{\_}Castillo/Kap1{\_}Presentation of the Book. An Integrated Overview of the Fatigue Problem.pdf:pdf},
journal = {Stress Int. J. Biol. Stress},
title = {{Presentation of the Book . An Integrated Overview of}},
year = {2009}
}
@article{Strahlung2006,
author = {Strahlung, Kosmische},
journal = {Gerthsen Phys.},
pages = {969--1044},
title = {{18 - Kerne und Elementarteilchen}},
year = {2006}
}
@article{Klein,
author = {Klein, Bernd},
isbn = {9783834802965},
title = {{Aus dem Programm Maschinenelemente und}}
}
@article{Zienkiewicz2005,
abstract = {Publisher Summary Some general families of finite elements can be obtained for C0 interpolations. A progressively increasing number of nodes, and hence improved accuracy characterizes each new member of the family and presumably the number of such elements required to obtain an adequate solution decreases rapidly. To ensure that a small number of elements can represent a relatively complex form of the type that is liable to occur in real, rather than academic, problems, simple rectangles, and triangles no longer suffice. This chapter is concerned with the subject of distorting such simple forms into others of more arbitrary shape. Elements of the basic one-, two-, or three-dimensional types are mapped into distorted forms. Not only can two-dimensional elements be distorted into others in two dimensions but the mapping of these can be taken into three dimensions also as indicated by the flat sheet elements distorting into a three-dimensional space. This principle applies generally, providing a one-to-one correspondence between Cartesian and curvilinear coordinates can be established. Once such coordinate relationships are known, shape functions can be specified in local coordinates and by suitable transformations the element properties established in the global coordinate system.},
author = {Zienkiewicz, O C and Taylor, R L and Zhu, J Z},
doi = {http://dx.doi.org/10.1016/B978-075066431-8.50173-9},
isbn = {978-0-7506-6431-8},
journal = {Finite Elem. Method Set (Sixth Ed.},
pages = {138--186},
title = {{5 - Mapped elements and numerical integration — ‘infinite' and ‘singularity elements'}},
url = {http://www.sciencedirect.com/science/article/pii/B9780750664318501739},
year = {2005}
}
@article{Doquet1997a,
abstract = {The development of fatigue damage in Co45Ni specimens during push-pull and reversed torsion tests, performed inside a scanning electron microscope, was observed and the different stress states compared. It appeared that transgranular crack initiation and development is delayed and intergranular crack initiation promoted under torsional loading. This was explained in terms of reduced surface distortion at the emergence of persistent slip bands (PSBs) and smaller compatibility stresses at the PSB-matrix interfaces. The influence of the mechanical strength of grain boundaries on the difference between tensile and torsional fatigue lives is discussed.},
author = {Doquet, V.},
doi = {10.1111/j.1460-2695.1997.tb00280.x},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/1996{\_}Doquet{\_}CRACK INITIATION MECHANISMS IN TORSIONAL FATIGUE.pdf:pdf},
issn = {8756758X},
journal = {Fatigue Fract. Eng. Mater. Struct.},
keywords = {-torsional fatigue,intergranular crack initiation},
number = {2},
pages = {227--235},
title = {{Crack Initiation Mechanisms in Torsional Fatigue}},
url = {http://doi.wiley.com/10.1111/j.1460-2695.1997.tb00280.x},
volume = {20},
year = {1997}
}
@article{CARPINTERI2001a,
abstract = {Some multiaxial high-cycle fatigue criteria based on the so-called critical plane approach are reviewed. According to such an approach, the critical plane where the fatigue life assessment should be performed can be determined by maximising the amplitudes and/or values of some stress components. In the present paper, the critical plane orientation is correlated with the averaged principal stress directions deduced through the weight function method, and a new fatigue failure criterion is proposed. The results derived by applying the present criterion and the other critical plane criteria analysed are compared with experimental data related to different brittle (hard) metals under in-phase or out-of-phase sinusoidal biaxial normal and shear stress states. 0},
author = {CARPINTERI, A and SPAGNOLI, A},
doi = {10.1016/S0142-1123(00)00075-X},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Empirical Fatigue Models + Validation/2000{\_}Carpinteri{\_}Multiaxial high cycle fatigue criterion for hard metals.pdf:pdf},
isbn = {0142-1123},
issn = {01421123},
journal = {Int. J. Fatigue},
keywords = {multiaxial},
number = {2},
pages = {135--145},
title = {{Multiaxial high-cycle fatigue criterion for hard metals}},
url = {http://linkinghub.elsevier.com/retrieve/pii/S014211230000075X},
volume = {23},
year = {2001}
}
@article{I,
author = {I, U R M I},
doi = {10.1007/978-3-642-22609-0},
isbn = {9783642226090},
journal = {Praxis (Bern. 1994).},
title = {{Messung von elektrischen Impedanzen}}
}
@article{Herleitunga,
author = {Herleitung, Zur and Bilanzgleichungen, Der},
doi = {10.1007/978-3-642-10194-6},
isbn = {9783642101946},
journal = {Differentiation},
title = {{Anhang A : Erg ¨ anzungen A . 1 Einf u}}
}
@article{Sangid2010,
abstract = {In many engineering alloys, there exists a wide distribution of grain sizes; we investigate the role of grain boundaries as a strengthening mechanism in such a material. The coincidental site lattice (CSL) model is a powerful mathematical tool to characterize grain boundaries (GBs) and identify 'special' boundaries, which display beneficial mechanical behavior. We define the CSL and describe a detailed procedure to obtain this information from the grain orientation mapping via electron back scattering diffraction (EBSD). From this information, we show the evolution of the CSL for a nickel-based superalloy, Udimet 720 (U720), throughout various stages of processing (billet and forging) and experiments (tension, compression, and fatigue). A deeper level of understanding the GB's role in the mechanical behavior of the material is investigated through atomic simulations using molecular dynamics (MD) as the GB energy is determined for the most prevalent GBs within this material. The spatial map of the orientation and grain sizes measured from EBSD is linked to the GB energies calculated from MD. Based upon the large number of boundaries analyzed (29,035), there is a strong inverse correlation between GB energy and grain size for every specimen examined during the various processing and testing conditions. ?? 2010 Elsevier B.V.},
author = {Sangid, Michael D and Sehitoglu, Huseyin and Maier, Hans J and Niendorf, Thomas},
doi = {10.1016/j.msea.2010.07.062},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/2010{\_}Sangid{\_}Grain boundary characterization and energetics of superalloys.pdf:pdf},
isbn = {0921-5093},
issn = {09215093},
journal = {Mater. Sci. Eng. A},
keywords = {Coincidence site lattice (CSL),Electron back scattering diffraction (EBSD),Grain boundary energy,Molecular dynamics simulations,Nickel-based superalloys},
number = {26},
pages = {7115--7125},
publisher = {Elsevier B.V.},
title = {{Grain boundary characterization and energetics of superalloys}},
url = {http://dx.doi.org/10.1016/j.msea.2010.07.062},
volume = {527},
year = {2010}
}
@article{Bohlke2001a,
author = {B{\"{o}}hlke, Thomas and Br{\"{u}}ggemann, C},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/Strukturmechanik MMS/Literatur/Graphical Representation of the Generalized Hooke's Law{\_}SingleCrystals{\_}B{\"{o}}hlke{\_}Kommentar.pdf:pdf},
journal = {Techn,sche Mech.},
number = {2},
pages = {145--158},
title = {{Graphical Representation of the Generalized Hooke's Law}},
volume = {21},
year = {2001}
}
@article{Garikipati2001,
abstract = {This work represents a first step toward the development of a continuum field formulation for the coupled phenomena of diffusion and mechanics in polycrystalline solids. The basis of the formulation lies in lattice-level mechanisms, from which a continuum thermodynamic description of processes at micron length scales is developed. Considering self-diffusion, the composition problem is posed in terms of a binary vacancy-atom mixture. For mechanics, isotropic linear elasticity and isothermal conditions are assumed. The coupled constitutive relations for composition and mechanics are formally derived from the underlying thermodynamic principles. When applied to governing partial differential equations for each subproblem, the coupled nature is realized. Under applied tractions or intrinsic stress, the atoms diffuse - in general from surfaces with compressive normal traction to those with relatively tensile normal traction. The flow is mediated by electric fields via the mechanism of electromigration. In the case of metal interconnect lines in integrated circuit devices, the results of these microscopic processes are manifested in phenomena such as diffusional creep, hillock formation, grain growth, grain boundary motion, void formation and void evolution. These phenomena have a significant impact on the function, performance and failure of interconnect lines. A computational framework based on the finite element method has been developed to solve the coupled equations. Several numerical examples are presented and comparisons with analytical results are provided where the latter are available. ?? 2001 Elsevier Science Ltd.},
author = {Garikipati, Krishna and Bassman, Lori and Deal, Michael},
doi = {10.1016/S0022-5096(00)00081-8},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Kriechen{\_}Spannungsrelaxation/2001{\_}Garikipati+Bassman+Deal{\_}A lattice-based micromechanical continuum formulation for stress-driven mass transport in polycrystalline solids.pdf:pdf},
issn = {00225096},
journal = {J. Mech. Phys. Solids},
keywords = {C. Finite elements,Coupling,Diffusion,Stress,Thermodynamics},
number = {6},
pages = {1209--1237},
title = {{A lattice-based micromechanical continuum formulation for stress-driven mass transport in polycrystalline solids}},
volume = {49},
year = {2001}
}
@article{Eekoye1996c,
abstract = {Heat-transfer rates present in an engine cylinder undergoing knock are known to be larger than the rates associated with normal engine operation. Further, at the time of knock, the largest heat fluxes are associated with locations on the cylinder wall where the flame is locally quenching. In this study, heat-transfer processes at the flame-wall interface during a knock event are investigated computationally and analytically. Computationally, the governing equations for a one-dimensional, flame-quenching event are solved using a reduced chemical reaction mechanism. Analytically, scaling relations for the flame heat-release rates are used in the governing equations to determine the heat-transfer rates. It is found that while pressure transients modify the wall heat flux, the absolute value of the pressure is the most significant parameter in predicting the maximum heat flux. The wall heat flux profiles are predicted for both the analytical and computational models. In the range of pressures examined, a linear relationship was found between the peak flux and pressure, both for the computational and analytical models. The linear relationship between the pressure and peak flux was found to be invalid when the flame-quenching process was disrupted by the pressure fluctuations for pressure oscillations with a characteristic time on the order of the quenching process. ?? 1996 Combustion Institute.},
author = {Eekoye, O. A.},
doi = {10.1016/S0082-0784(96)80101-9},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/1996{\_}Ezekoye{\_}Heat transfer modeling during knock and flame quenching in an engine chamber.pdf:pdf},
isbn = {0082-0784},
issn = {00820784},
journal = {Symp. Combust.},
number = {2},
pages = {2661--2668},
title = {{Heat transfer modeling during knock and flame quenching in an engine chamber}},
volume = {26},
year = {1996}
}
@article{Chan2010a,
abstract = {Fatigue failure in the high-cycle and ultrahigh-cycle regimes is often dominated by the crack initiation processes, which are strongly influenced by the salient features and defects in the microstructure. Competing fatigue mechanisms involving crack initiation at persistent slipbands, grain boundaries, pores, and non-metallic inclusions or particles, have been reported to occur at surface sites in the high-cycle fatigue regime (106-107 cycles), but shift to interior sites in the ultrahigh-cycle fatigue regime (109-1010 cycles). The changes in fatigue mechanism and crack initiation site result in large variations in fatigue life. This overview article examines the roles of microstructural features such as grain size, texture, porosity, non-metallic inclusion in the fatigue crack initiation process and the manners by which these microstructural effects affect the shape of the stress-life curves. ?? 2010 Elsevier Ltd. All rights reserved.},
author = {Chan, Kwai S.},
doi = {10.1016/j.ijfatigue.2009.10.005},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2010{\_}Chan{\_}Roles of microstructure in fatigue crack initiation.pdf:pdf},
isbn = {01421123},
issn = {01421123},
journal = {Int. J. Fatigue},
keywords = {Crack initiation,Double fatigue limits,Fatigue mechanism,High-cycle fatigue,Microstructure,Ultrahigh-cycle fatigue},
number = {9},
pages = {1428--1447},
publisher = {Elsevier Ltd},
title = {{Roles of microstructure in fatigue crack initiation}},
url = {http://dx.doi.org/10.1016/j.ijfatigue.2009.10.005},
volume = {32},
year = {2010}
}
@article{Easter2014,
abstract = {Laboratory tests were performed to measure cooling rates of an impinging oil-jet on the underside of an automotive piston as functions of oil nozzle-to-piston surface spacing, oil pressure, oil temperature, and piston temperature. Based on these results, area-average Nusselt number correlations were derived for a Reynolds number range of 100–4500, a Prandtl number range of 90–750, and a nozzle-to-piston surface spacing range over 73–160 mm, which are within the ranges expected for oil-jet cooling of automotive pistons.},
annote = {10.1115/1.4027835},
author = {Easter, J and Jarrett, C and Pespisa, C and Liu, Y C and Alkidas, A C and Guessous, L and Sangeorzan, B P},
doi = {10.1115/1.4027835},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/W{\"{a}}rme-RBen Kolben/2014{\_}Easter+Jarret{\_}An Area Average Correlation for Oil-Jet Cooling of Automotive Pistons .pdf:pdf},
journal = {J. Heat Transfer},
month = {sep},
number = {12},
pages = {124501--124504},
publisher = {ASME},
title = {{An Area-Average Correlation for Oil-Jet Cooling of Automotive Pistons}},
volume = {136},
year = {2014}
}
@article{Block2010,
author = {Block, Katharina},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Mathematik/green.function.university.berlin.pdf:pdf},
number = {April},
pages = {2--5},
title = {{Green ' sche Funktionen als Hilfsmittel zur Konstruktion klassischer L{\"{o}}sungen von partiellen Di erentialgleichungen 2 Mathematische Grundlagen}},
volume = {0},
year = {2010}
}
@article{Theoreme1964,
author = {Theoreme, Kohn},
doi = {10.1007/978-3-540-72637-1},
isbn = {9783642054952},
pages = {139--150},
title = {{Kapitel 9}},
year = {1964}
}
@article{Hochhalter2011,
abstract = {It has been observed during fatigue cracking of AA 7075-T651 that a small percentage of Al 7 Cu 2 Fe particles crack during manufacturing or very early in their life. Some of the cracked particles eventually nucleate cracks into the surrounding microstructure, and among these the number of cycles required for nucleation varies widely. It is important to comprehend the mechanics underpinning the observed variation so that the subsequent propagation stage can be accurately modeled. To this end, finite element models of replicated grain and particle geometry are used to compute mechanical fields near monitored cracked particles using an elastic–viscoplastic crystal plasticity model that captures the effect of the orientation of the grains near each monitored particle. Nonlocal, slip-based metrics are used to study the localization and cyclic accumulation of slip near the cracked particles providing mechanics-based insight into the actuation of the nucleation event. A high slip localization and cyclic accumulation rate are found to be a necessary, but not sufficient, condition for nucleation from cracked particles. A sufficient local driving stress must also be present, which is strongly dependent on the local microstructure and accumulated slip. Furthermore, the simulation results elucidate a quantitative relationship between the slip accumulated during fatigue loading and a consequential reduction of the critical local driving stress for nucleation, providing a physical basis for the fatigue damage concept. The observed nucleation direction is orthogonal to the computed local maximum tangential stress direction, as expected for this alloy. The main result is a semi-empirical model for the number of cycles required for nucleation, which is dependent on the maximum tangential stress and cyclic slip-accumulation rate near a cracked particle.},
author = {Hochhalter, J D and Littlewood, D J and Veilleux, M G and Bozek, J E and Maniatty, A M and Rollett, A D and Ingraffea, A R},
doi = {10.1088/0965-0393/19/3/035008},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/2011{\_}Hochhalter{\_}AL7075AgeometricapproachIII{\_}SemiempiricalApproachNucleation.pdf:pdf},
isbn = {09650393 (ISSN)},
issn = {0965-0393},
journal = {Model. Simul. Mater. Sci. Eng.},
number = {3},
pages = {035008},
title = {{A geometric approach to modeling microstructurally small fatigue crack formation: III. Development of a semi-empirical model for nucleation}},
url = {http://stacks.iop.org/0965-0393/19/i=3/a=035008?key=crossref.8640954c7485639bf37ab73e6f2eb0ad},
volume = {19},
year = {2011}
}
@article{ConferenceonFatigueMechanisms:AdvancesinQuantitativeMeasurementofPhysicalDamage1983,
author = {{Conference on Fatigue Mechanisms: Advances in Quantitative Measurement of Physical Damage}},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/1983{\_}Lankford{\_}Fatigue Mechanisms Advances in quantitative   meausrements of physical damage.pdf:pdf},
issn = {10403094},
journal = {Stp 811},
keywords = {An{\{}{\'{a}}{\}}lise quantitativa,Congresso,Dano f{\{}{\'{i}}{\}}sico,Fadiga de materiais},
pages = {496},
title = {{Fatigue mechanisms advances in quantitative measurement of physical damage {\{}{\textless}{\}}{\{}{\textless}{\}}a{\{}{\textgreater}{\}}{\{}{\textgreater}{\}} conference}},
year = {1983}
}
@article{Gross2011e,
author = {Gross, Dietmar and Seelig, Thomas},
doi = {10.1007/978-3-642-10196-0},
isbn = {978-3-642-10195-3},
title = {{Bruchmechanik}},
url = {http://link.springer.com/10.1007/978-3-642-10196-0},
year = {2011}
}
@article{Wang2016a,
abstract = {Cracks encountered in engineering structures are typically three dimensional, and the fracture mechanism remains unclear because of the superimposed stresses induced by mixed-mode I/II/III loading. This paper introduces a general 3D mixed-mode fracture criterion based on the maximum mean principal stress (MMPS) by introducing the concept of a characteristic fracture length that is related to the material tensile strength. This criterion has clear physical significance, a systematic mathematical expression and a wide scope of applications to estimate both the in- and out-of-plane fracture angles and fracture strength. The proposed criterion is validated for all mixed-mode conditions (I/II, I/III and II/III) and is compared with several widely used criteria based on experimental results reported in previous studies. Good agreement is achieved in terms of the fracture angles and, in particular, the fracture strength between the results predicted by the new criterion and the experimental results of various brittle materials.},
author = {Wang, J and Ren, L and Xie, L Z and Xie, H P and Ai, T},
doi = {10.1016/j.ijsolstr.2016.10.009},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/2016{\_}Wang{\_}Maximum mean principal stress criterion for 3D brittle fracture.pdf:pdf},
issn = {00207683},
journal = {Int. J. Solids Struct.},
keywords = {3D fracture criterion,Characteristic fracture length,Mean stress,Mixed-mode loading},
pages = {142--154},
title = {{Maximum mean principal stress criterion for three-dimensional brittle fracture}},
volume = {102-103},
year = {2016}
}
@article{Vorschriften,
author = {Vorschriften, Gesetzliche},
journal = {Betrieb},
pages = {243--259},
title = {{10 Ger{\"{a}}uschemissionen}}
}
@article{Beispiele,
author = {Beispiele, Konstruktive},
pages = {132--140},
title = {{Konstruktion mit CATIA V4 20 Rohbau}}
}
@article{Voß2005,
author = {Vo{\ss}, H},
pages = {1--204},
title = {{Numerische Simulation}},
year = {2005}
}
@article{Forestb,
author = {Forest, Samuel},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/Folien CISM Summer School Mai2017 - Mesoscale Models/courses{\_}C1703{\_}forest{\_}Forest1-Micromorphic.pdf:pdf},
title = {{Micromorphic media}}
}
@article{Bahke2008,
author = {Bahke, T},
journal = {H{\{}{\"{u}}{\}}tte},
pages = {1--21},
title = {{O-Normung}},
year = {2008}
}
@article{Adair1972,
abstract = {This study first reviews, discusses, and compares existing correlations{\$}\backslash{\$}nfor heat transfer in reciprocating compressors and engines. Then{\$}\backslash{\$}nafter a discussion of the significance of obtaining accurate instantaneous{\$}\backslash{\$}nheat transfer data, the authors describe an experimental investigation{\$}\backslash{\$}nof the instantaneous heat transfer rates to the cylinder wall of{\$}\backslash{\$}na reciprocating refrigerating compressor. Finally, this report presents{\$}\backslash{\$}nan expression which correlates the time averaged data within 20{\{}{\%}{\}}.},
author = {Adair, R P and Qvale, E B and Pearson, J T},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/1972{\_}Adair{\_}Instantaneous Heat Transfer to the Cylinder Wall in Reciprocating compressors and engines.pdf:pdf},
journal = {Int. Compress. Eng. Conf.},
pages = {521--526},
title = {{Instantaneous heat transfer to cylinder wall in reciprocating compressors}},
year = {1972}
}
@misc{Qi1999,
author = {Qi, Weidong and Bertram, Albrecht},
booktitle = {Int. J. Plast.},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Plasticity models/Anisotropic continuum damage modeling for single crystals at high temperatures{\_}QiAndBertram.pdf:pdf},
pages = {1197--1215},
title = {{Anisotropic continuum damage modeling for single crystals at high temperatures}},
volume = {15},
year = {1999}
}
@misc{Oppenheim1989,
author = {Oppenheim, A.V. and Schafer, R.W. and Buck, J. R.},
booktitle = {Discret. signal Process.},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/statistical analysis of microstructures/1 Introduction.pdf:pdf},
keywords = {FFT,Hilbert,Signal processing,filtering},
pages = {870},
title = {{1 -Introduction.Pdf}},
year = {1989}
}
@article{Betrachtungenk,
author = {Betrachtungen, Allgemeine},
journal = {Integr. Vlsi J.},
title = {{9 Stromfadentheorie 9.1}}
}
@article{Druck,
author = {Druck, Der},
journal = {Hand, The},
pages = {30--33},
title = {{4 Messmethoden}}
}
@article{Markers2009,
author = {Markers, Tissue Tumor},
journal = {Surg. Clin. North Am.},
pages = {427--448},
title = {10 10.1.1},
year = {2009}
}
@article{Technology,
author = {Technology, O F},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Heat Transfer Combustion Chamber/2013{\_}Oleg{\_}Spitsov{\_}HEAT TRANSFER INSIDE INTERNAL COMBUSTION ENGINE - Modelling and comparison with experimental data{\_}Masters{\_}thesis.pdf:pdf},
keywords = {combustion engine,degree program in energy,faculty of technology,heat transfer inside internal,peenranta university of technology,technology},
title = {{Heat Transfer Inside Internal Combustion Engine :}}
}
@article{Winkler2014c,
author = {Winkler, N.},
doi = {10.1177/1468087414544899},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Klopfen{\_}Ottomotor/2015{\_}Winkler{\_}Effect of pressure oscillations on in-cylinder heat transfer  - through LES Simulation.pdf:pdf},
isbn = {1468087414544},
issn = {1468-0874},
journal = {Int. J. Engine Res.},
keywords = {24 june 2014,6 march 2014,accepted,computational fluid dynamics,date received,heat transfer,internal combustion engines,large eddy simulation,pressure oscillations},
number = {6},
pages = {705--715},
title = {{Effect of pressure oscillations on in-cylinder heat transfer - through large eddy simulation}},
url = {http://jer.sagepub.com/lookup/doi/10.1177/1468087414544899},
volume = {16},
year = {2014}
}
@article{Background,
author = {Background, General},
journal = {Mathematica},
pages = {1--207},
title = {{1.0 Remarks}}
}
@article{Kadija1993,
author = {Kadija, K. and Martinis, M.},
doi = {10.1103/PhysRevD.48.2027},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/B{\"{u}}cher{\_}Sammlung{\_}ITM/Elasticity and Plasticity of large deformations - Bertram/fulltext8.pdf:pdf},
isbn = {1550-7998},
issn = {05562821},
journal = {Phys. Rev. D},
number = {5},
pages = {2027--2034},
pmid = {10016439},
title = {{Inelasticity distribution and relationship between e+e- and pp hadron-production mechanisms}},
volume = {48},
year = {1993}
}
@article{Hashin1962b,
abstract = {Variational principles for anisotropic and nonhomogeneous elasticity, established by the authors in a previous paper, have been applied to the derivation of lower and upper bounds for the elastic moduli of polycrystals in terms of the moduli of the constituting crystals. The results hold for arbitrary crystal shapes. Explicit results tor cubic polycrystals showed that the present bounds are a considerable improvement of the well-known Voigt and Reuss bounds. Good agreement with experimental results has been obtained.},
author = {Hashin, Z. and Shtrikman, S.},
doi = {10.1016/0022-5096(62)90005-4},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/Strukturmechanik MMS/Literatur/Hashin Shtrikman 1962.pdf:pdf},
issn = {00225096},
journal = {J. Mech. Phys. Solids},
number = {4},
pages = {343--352},
title = {{A variational approach to the theory of the elastic behaviour of polycrystals}},
url = {http://linkinghub.elsevier.com/retrieve/pii/0022509662900054},
volume = {10},
year = {1962}
}
@article{Stebbins1967,
author = {Stebbins, Jeun},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Empirical Fatigue Models + Validation/1965{\_}NASA+Hudson{\_}Studies of fatigue crack growth in alloys suitable for elevated temperature-Al2618.pdf:pdf},
number = {May},
title = {{Nasa Technical N O T E}},
year = {1967}
}
@article{Loud1998,
author = {Loud, Stewart N},
journal = {Rev. Lit. Arts Am.},
pages = {1--11},
title = {{Commercial and Industrial Applications of Composites}},
year = {1998}
}
@inproceedings{Varghese2004,
abstract = {AbstractThermal loading of diesel engine pistons has increased dramatically in recent years due to applications of various technologies to meet low emission and high power requirements. Control of piston temperatures by cooling of these pistons has become one of the determining factors in a successful engine design. The pistons are cooled by oil jets fired at the underside from the crankcase. Any undesirable piston temperature rise may lead to engine seizure due to piston warping. However, if the temperature at the underside of the piston, where the oil jet strikes the piston, is above the boiling point of the oil being used, it may contribute to the mist generation. This mist may significantly contribute to the non-tail pipe emissions in the form of unburnt hydrocarbons (UBHC). The problem of non-tail pipe emissions has unfortunately not been looked into so seriously, as the current stress of all the automobile manufacturers is on meeting the tail -pipe emission legislative limits.A numerical model has been developed using computational fluid dynamics (CFD) tools, such as finite elements methods for studying the oil jet cooling of pistons. Using the numerical model developed by Stevens and Webb (1991), the heat transfer coefficient (h) required at the underside of the piston is predicted. This predicted value of heat transfer coefficient significantly helps in selecting right oil type, jet velocity, jet diameter and distance of the jet from the underside of the piston. It also helps to predict whether the oil selected will contribute to mist generation or not and if it contributes to mist generation then it helps in selecting the oil which does not contribute to mist generation. Grid generation for a production grade M {\&} M DI 2500 engine piston has been done using GNUPLOT. Isotherms of the predicted temperature profiles in the piston have been plotted using TECPLOT.},
author = {Varghese, Mani Bijoy and Agarwal, Avinash Kumar},
booktitle = {SAE Tech. Pap.},
doi = {10.4271/2004-28-0061},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/W{\"{a}}rme-RBen Kolben/2004{\_}Varghese{\_}Numerical investigation of piston cooling using oil jet.pdf:pdf},
publisher = {The Automotive Research Association of India},
title = {{Numerical Investigations Of Piston Cooling Using Oil Jet}},
year = {2004}
}
@article{Macha1999a,
abstract = {At present there are several approaches to the prediction of fatigue life of machine elements and structures. create complex states of stress and under such loadings the assumed criteria of multiaxial fatigue play a very important role in the algorithm used for the prediction of fatigue life. From a review of the literature on multiaxial cyclic fatigue it appears that there is no single universal cri- terion for different loading conditions. New mathemat- ical models are sought. Presently, special attention is being paid to energy criteria.1–14 From some uniaxial and multiaxial cyclic fatigue tests it has been concluded that the energy approach appears promising. The aims of this paper are: (i) to review current energy criteria ofmultiaxial fatigue and their proposed algorithms; (ii) to determine the kind of energy which is assumed to control the fatigue process; (iii) to describe simple exper- imental verifications of the theoretical assumptions of the criteria; and (iv) to present those parameters which domi- nate multiaxial fatigue behaviour. A recommendation for the practical use of the procedures by industry will not be given because of a lack of experimental verification on complex shaped and loaded components.},
author = {Macha, E. and Sonsino, C. M.},
doi = {10.1046/j.1460-2695.1999.00220.x},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Empirical Fatigue Models + Validation/Energy based models/Energy criteria of multiaxial  fatigue failure.pdf:pdf},
issn = {8756758X},
journal = {Fatigue Fract. Eng. Mater. Struct.},
keywords = {and low-cycle fatigue,critical plane,effect of mean stresses,high-,hysteresis loops,proportional and non-proportional loading,strain energy density},
number = {12},
pages = {1053--1070},
title = {{Energy criteria of multiaxial fatigue failure}},
volume = {22},
year = {1999}
}
@article{2012,
author = {Ε$\pi$$\iota$$\tau$$\rho$ο$\pi$ά$\kappa$$\eta$ς, Ι},
title = {{Χ$\alpha$$\rho$$\alpha$$\kappa$$\tau$$\eta$$\rho$$\iota$$\sigma$$\mu$ός $\Sigma$ύ$\nu$$\theta$$\epsilon$$\tau$$\omega$$\nu$ $\Upsilon$$\lambda$$\iota$$\kappa$ώ$\nu$ Α$\nu$$\theta$$\rho$$\alpha$$\kappa$ο$\nu$$\eta$$\mu$ά$\tau$$\omega$$\nu$ Κ$\alpha$$\tau$$\alpha$$\sigma$$\kappa$$\epsilon$$\upsilon$$\alpha$$\sigma$$\mu$έ$\nu$$\omega$$\nu$ Μ$\epsilon$ Τ$\eta$ Μέ$\theta$ο$\delta$ο $\Pi$$\epsilon$$\rho$$\iota$έ$\lambda$$\iota$$\xi$$\eta$ς Τ$\omega$$\nu$ Ι$\nu$ώ$\nu$ (Filament Winding)}},
year = {2012}
}
@article{Wei1970,
abstract = {Metal fatigue as an engineering problem has been well recognized. Many experiments have been carried out in recent years to assess the effects of load amplitude, mean load, load range and test frequency on the rate of fatigue-crack growth to characterize material response to different load profiles and to develop methods for estimating the service behavior of structural components. Recent studies have shown that fatigue-crack growth can be influenced strongly by the test environment; the effect being dependent on the particular material-environment involved. These results suggest that careful reassessments of the data of previous studies and of the proper direction for future fatigue research will be required. Hence, a critical review and analysis of existing fatigue-crack-growth data on high-strength aluminum and titanium alloys and high-strength steels has been made. The influences of load profile, test frequency, temperature, test environment and state-of-stress on fatigue-crack growth are discussed. Correlation with environment-enhanced crack growth under sustained loads and the associated changes in material response are examined. Possible mechanisms, synergistic effects and implications regarding methods for service-life estimation are considered. ?? 1970.},
author = {Wei, R P},
doi = {10.1016/0013-7944(70)90004-4},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/1970{\_}Wei{\_}Some aspects of environment-enhanced fatigue crack growth{\_}For example frequency in Al7075.pdf:pdf},
issn = {00137944},
journal = {Eng. Fract. Mech.},
number = {4},
pages = {633--651},
title = {{Some aspects of environment-enhanced fatigue-crack growth}},
volume = {1},
year = {1970}
}
@article{Stoßfanger,
author = {Sto{\ss}f{\"{a}}nger, Vordere},
pages = {164--169},
title = {{24 Vorderwagen}}
}
@article{Pan2014a,
abstract = {Knocking combustion in spark-ignition (SI) engines is a typical abnormal combustion phenomenon that severely limits engine performance and thermal efficiency. However, its mechanism has not so far been completely revealed, such as the origin of pressure oscillation with tremendous amplitude and broken mechanisms of the engine body when knock occurs. This article systematically reviews the series of physical and chemical phenomena involved in knocking combustion, including auto-ignition, gas-dynamic waves, cavity resonance, and auto-ignited flame propagation. Significant research has shown that the rapid heat release of end-gas auto-ignition and subsequent strong pressure waves play a crucial role during knocking combustion. A methodology of the interaction of flame propagation and pressure waves has been proposed to reveal knock formation in terms of positive feedback between strengthened pressure waves and auto-ignited flame propagation. Also, new suggestions on the weakness in prior research of knocking combustion have also been discussed in the present article. {\{}{\textcopyright}{\}} 2014 Copyright Taylor and Francis Group, LLC.},
author = {Pan, Jiaying and Shu, Gequn and Wei, Haiqiao},
doi = {10.1080/00102202.2013.857665},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2014{\_}Pan+Wei{\_}Interaction of Flame Propagation and Pressure Waves During Knocking Combustion in Spark-Ignition Engines.pdf:pdf},
issn = {0010-2202},
journal = {Combust. Sci. Technol.},
number = {2},
pages = {192--209},
title = {{Interaction of Flame Propagation and Pressure Waves During Knocking Combustion in Spark-Ignition Engines}},
url = {http://www.tandfonline.com/doi/abs/10.1080/00102202.2013.857665},
volume = {186},
year = {2014}
}
@article{LIU2017195,
annote = {Signal Processing and Control challenges for Smart Vehicles},
author = {Liu, Lei and Li, Zhijun and Liu, Shiyu and Shen, Boxi},
doi = {https://doi.org/10.1016/j.ymssp.2015.12.029},
journal = {Mech. Syst. Signal Process.},
keywords = {Exhaust Gas Recirculation,Lean NOx trap,Lean-burn gasoline engine,Mechanism,Nitrogen oxides},
pages = {195--213},
title = {{Effect of exhaust gases of Exhaust Gas Recirculation (EGR) coupling lean-burn gasoline engine on NOx purification of Lean NOx trap (LNT)}},
volume = {87},
year = {2017}
}
@article{Arnold2000,
author = {Arnold, J{\"{o}}rg and Alleinunf{\"{a}}llen, Bei},
pages = {715--729},
title = {{B10 B10 Alleinunf{\"{a}}lle B10}},
year = {2000}
}
@article{Softwareergonomie,
author = {Softwareergonomie, Angewandte and Liskowsky, R{\"{u}}diger and W{\"{u}}nschmann, Wolfgang and R{\"{u}}diger, Prof and Prof, Liskowsky},
pages = {1},
title = {{1 Vorbemerkung}}
}
@article{Rothe2015,
abstract = {In this article we investigate a fully, thermo-mechanically coupled viscoplasticity model in view of various numerical aspects. First, we develop the entire system of differential–algebraic equations resulting from the spatially discretized principle of virtual displacements, the principle of virtual temperatures, and the evolution equations of the internal variables provided by the constitutive model. In the time-integration step this system is solved both using a fully monolithic approach based on a Backward–Euler scheme in combination with the Multilevel-Newton algorithm as well as a partitioned approach solving the fully coupled system. The latter is treated by means of a combination of a Backward–Euler method and an accelerated Gauss–Seidel/Multilevel-Newton scheme to solve the resulting system of algebraic equations within each time-integration step. Additionally, we consider a specific treatment of the interpolation between different meshes within the partitioned approach. This is shown for p-version finite elements based on hierarchical shape functions. Finally, it turns out that the specific constitutive model of small-strain thermo-viscoplasticity, which is based on the decomposition into kinematic hardening and energy storing strains, yields a problem-adapted stress algorithm. This allows to reduce the stress algorithm on Gauss-point level to the solution of one scalar equation. Numerical examples serve to elucidate the behavior and properties of the proposed methods.},
author = {Rothe, Steffen and Erbts, Patrick and D{\"{u}}ster, Alexander and Hartmann, Stefan},
doi = {10.1016/j.cma.2015.05.002},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Numerik UMATS FE-Codes/2015{\_}Hartmann{\_}Monolithic and partitioned coupling schemes for thermo-viscoplasticity.pdf:pdf},
issn = {00457825},
journal = {Comput. Methods Appl. Mech. Eng.},
keywords = {algebraic equations,differential,fully coupled finite elements,monolithic approach,partitioned approach,thermo-viscoplasticity},
pages = {375--410},
publisher = {Elsevier B.V.},
title = {{Monolithic and partitioned coupling schemes for thermo-viscoplasticity}},
url = {http://linkinghub.elsevier.com/retrieve/pii/S0045782515001681},
volume = {293},
year = {2015}
}
@article{Pro-,
author = {Pro-, Mathematischen and Search, Line},
title = {{4 Optimierungsverfahren}}
}
@techreport{NASA1993,
author = {McBride, B.J. and Gordon, S. and Reno, M.A.},
institution = {NASA Report TM-4513},
title = {{Coefficients for Calculating Thermodynamic and Transport Properties of Individual Species}},
year = {1993}
}
@article{Wilson1951,
author = {Wilson, Brian A},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/{\_}buecherSong/HandbookofComposites/II/23{\_}Pultrusion.pdf:pdf},
journal = {Processing},
title = {{A. Wilson 23}},
year = {1951}
}
@article{Dietmann1973,
author = {Dietmann, H.},
doi = {10.1002/mawe.19730040608},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Empirical Fatigue Models + Validation/1973{\_}Dietmann Materialwissenschaft{\_}und{\_}Werkstofftechnik{\_}ExperimentelleUntersuchungenZuFatigue.pdf:pdf},
issn = {15214052},
journal = {Materwiss. Werksttech.},
number = {6},
pages = {322--333},
title = {{Werkstoffverhalten unter mehrachsiger schwingender Beanspruchung. Teil 2: Experimentelle Untersuchungen}},
volume = {4},
year = {1973}
}
@article{Liu1972b,
author = {Liu, I Shih and M{\"{u}}ller, Ingo},
doi = {10.1007/BF00250689},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Thermodynamik/Liu{\_}Entropieprinzip{\_}Lagrange/On the Thermodynamics and Thermostatics of Fluid in Electromagnetic Fields {\_}Liu.pdf:pdf},
issn = {00039527},
journal = {Arch. Ration. Mech. Anal.},
number = {2},
pages = {149--176},
title = {{On the thermodynamics and thermostatics of fluids in electromagnetic fields}},
volume = {46},
year = {1972}
}
@article{Pahl2007d,
abstract = {Kap. 5},
author = {Pahl, Gerhard and Beitz, Wolfgang and Feldhusen, J{\"{o}}rg and Grote, Karl-Heinz},
isbn = {9783540340607},
pages = {213--230},
title = {{Konstruktionslehre}},
year = {2007}
}
@article{Beispielc,
author = {Beispiel, Am and Beispiel, Dieses and Iso, D I N E N and Datei, Neue},
pages = {36--42},
title = {{4 Zylinderschraube}}
}
@misc{Vagera1971,
author = {Vagera, I.},
booktitle = {Scr. Metall.},
doi = {10.1016/0036-9748(71)90036-6},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/1971{\_}Vagera{\_}A PileUp or a dislocation model of crack in an interface between two isotropic or anisotropic media.pdf:pdf},
issn = {00369748},
number = {2},
pages = {93--96},
title = {{A pile-up or a dislocation model of crack in an interface between two isotropic or anisotropic media}},
volume = {5},
year = {1971}
}
@article{Gesetz2012,
author = {Gesetz, Ohmsches},
doi = {10.1007/978-3-8348-8643-9},
isbn = {9783834886439},
pages = {194--342},
title = {{III Differential- und Integralrechnung fu ¨ r Funktionen von mehreren Variablen 1}},
year = {2012}
}
@article{Jungbluth2007,
author = {Jungbluth, Niels and Spielmann, Michael and Dones, Roberto and Heck, Thomas and Emmenegger, Mireille Faist and Frischknecht, Rolf},
pages = {537},
title = {{Teil IV}},
year = {2007}
}
@article{Systems2009,
author = {Systems, Linear Shift-invariant},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/Signal Verarbeitung/2001{\_}Selesnick{\_}The Discrete Fourier Transform.PDF:PDF},
number = {x},
pages = {407--418},
title = {{The Discrete Fourier Transform}},
year = {2009}
}
@article{Stiller2006b,
author = {Stiller, Christoph},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Vorlesungen/Messtechnik+Regelungstechnik/gmrt01.pdf:pdf},
issn = {02731177},
journal = {Adv. Sp. Res.},
number = {12},
pages = {2820--2823},
title = {{Grundlagen der Mess- und Regelungstechnik}},
volume = {38},
year = {2006}
}
@article{Desmorat2006a,
abstract = {Application of damage mechanics to fatigue is addressed in the present paper. The ability of Lemaitre's damage law to describe low and high cycle fatigue failure of metals is illustrated. Its generalization into an evolution law modeling a damage rate governed by the main dissipative mechanics applies to concrete, elastomers, rocks and to probably other materials. The importance of rate written laws is emphasized.},
author = {Desmorat, Rodrigue},
doi = {10.1080/17747120.2006.9692859},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/2006{\_}Desmorat{\_}SummerSchool{\_}Damage and Fatigue Overview Evolution Equation.pdf:pdf},
isbn = {9780387739052},
issn = {1774-7120},
journal = {Rev. Eur. G{\{}{\'{e}}{\}}nie Civ.},
keywords = {concrete,damage,elastomers,fatigue,metals,rocks},
number = {6-7},
pages = {849--877},
title = {{Damage and Fatigue: Continuum damage mechanics modeling for fatigue of materials and structures}},
volume = {10},
year = {2006}
}
@article{Differt1986a,
abstract = {A mdoel of the evolution of the surface roughness of persistent slip bands (PSBs) is presented. The physical background of the model is the existence of a dynamic equilibrium between dislocation multiplication and annihilation in PSBs which leads to irreversible microscopic positive and negative slip steps at the surface. The fluctuation of a random distribution of these slip line segments leads to a surface roughness which increases with the square root of the cycle number. The relation between the parameters which characterize the surface relief and the microscopic parameters which contol the dislocation glide in PSBs is investigated by computer simulations. Fair agreement is obtained between observed and simulated surface reliefs where such a comparison is possible.},
author = {Differt, K and Esmann, U and Mughrabi, H},
doi = {10.1080/01418618608242897},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2016{\_}Mughrabi{\_}A model of extrusions and intrusions in fatigued metals II  Surface roughening by random irreversible slip.pdf:pdf},
isbn = {0141-8610},
issn = {0141-8610},
journal = {Philos. Mag. A},
number = {2},
pages = {237--258},
title = {{A model of extrusions and intrusions in fatigued metals II. Surface roughening by random irreversible slip}},
url = {http://www.tandfonline.com/doi/abs/10.1080/01418618608242897},
volume = {54},
year = {1986}
}
@article{Modellbildung,
author = {Modellbildung, Methodik Der},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Vorlesungen/Messtechnik+Regelungstechnik/gmrt03.pdf:pdf},
pages = {1--31},
title = {{3.1 Methodik der Modellbildung}}
}
@article{Apparate,
author = {Apparate, Gebilde and Ger, Gebilde and Wiener, Norbert and Kennzeichen, Die and Systemelemente, Die and Funktion, Die and Input, Jeder and Drucker, Peter},
journal = {Mechanik},
pages = {9--20},
title = {{2 Einf{\"{u}}hrung in die systemtechnische Methodik}}
}
@article{Zhao2008a,
abstract = {Extensive fatigue experiments were conducted using 7075-T651 aluminum alloy under uniaxial, torsion, and axial-torsion loading. Detailed fatigue results were reported. Different mean stresses were applied in the experiments and the mean stress was found to have a significant influence on the fatigue strength of the material. A tensile mean stress decreased the fatigue strength dramatically. Fatigue damage was found to occur under compression-compression loading. In addition, axial-torsion experiments using tubular specimens were conducted under different loading paths to study the multiaxial fatigue behavior. Fatigue cracking behavior was found to be dependent on the loading path as well as the loading magnitude. When the loading magnitude was high, the material displayed shear cracking. When the loading stress was below a certain level, the material exhibited tensile cracking. For most loading cases under investigation, the material displayed a mixed cracking behavior. A kink was found in the shear strain versus fatigue life curve from the pure torsion experiments, and it was associated with a distinctive transition of cracking behavior. The Smith-Watson-Topper (SWT) parameter with a critical plane interpretation was found to correlate well with most of the experiments conducted in terms of fatigue lives. However, the SWT parameter cannot deal with the uniaxial fatigue conditions where the maximum stress is low or negative. More importantly, the model fails to correctly predict the cracking behavior observed experimentally on the material. A critical plane criterion based on a combination of the normal and shear components of the stresses and strains on material planes was found to better correlate the fatigue experiments in terms of both fatigue life and cracking behavior. The characteristics of the multiaxial fatigue criterion were discussed based on the experimental observations on 7075-T651 aluminum alloy. ?? 2007 Elsevier Ltd. All rights reserved.},
author = {Zhao, Tianwen and Jiang, Yanyao},
doi = {10.1016/j.ijfatigue.2007.07.005},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Empirical Fatigue Models + Validation/2007{\_}Jiang{\_}Fatigue of 7075-T651 aluminum alloy VALIDATION+MODEL.pdf:pdf},
isbn = {0142-1123},
issn = {01421123},
journal = {Int. J. Fatigue},
keywords = {7075-T651 aluminum alloy,Axial-torsion,Compression-compression fatigue,Multiaxial criterion,Multiaxial fatigue},
number = {5},
pages = {834--849},
title = {{Fatigue of 7075-T651 aluminum alloy}},
volume = {30},
year = {2008}
}
@article{Ince2014a,
abstract = {In this paper, two different forms of an original multiaxial fatigue damage parameter related to the maximum fatigue damage plane are proposed for performing fatigue life prediction under various loading conditions loadings. The proposed fatigue damage parameters have been applied to uniaxial and multiaxial loading conditions for geometrically different bodies. Both the damage parameters are correlated to sets of experimental data published in the literature to verify the prediction accuracy of the damage parameters. The damage parameter in the form of the GSA, when applied to the uniaxial loading, provides very good correlations with four sets of experimental mean stress fatigue data for Incoloy 901 super alloy, ASTM A723 steel, 7075-T561 aluminum alloy and 1045 HRC 55 steel. In the case of multiaxial loadings, both the GSE and GSA parameters are found to correlate well with fatigue data of 1045 steel and Inconel 718 tubular specimens under proportional and non-proportional loadings. In addition, the damage parameters show reasonably acceptable correlations with experimental fatigue data of SAE 1045 steel notched shafts subjected to proportional and non-proportional loadings. ?? 2013 Elsevier Ltd. All rights reserved.},
author = {Ince, Ayhan and Glinka, Grzegorz},
doi = {10.1016/j.ijfatigue.2013.10.007},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Empirical Fatigue Models + Validation/Energy based models/A generalized fatigue damage  parameter for multiaxial fatigue life prediction under proportional  loadings.pdf:pdf},
issn = {01421123},
journal = {Int. J. Fatigue},
keywords = {Critical plane,Fatigue damage parameter,Mean stress,Multiaxial fatigue life},
pages = {34--41},
publisher = {Elsevier Ltd},
title = {{A generalized fatigue damage parameter for multiaxial fatigue life prediction under proportional and non-proportional loadings}},
url = {http://dx.doi.org/10.1016/j.ijfatigue.2013.10.007},
volume = {62},
year = {2014}
}
@book{Fox1918,
author = {Fox, P J},
booktitle = {Science},
doi = {10.1126/science.49.1254.44},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Thermodynamik/M{\"{u}}llerAndNoll{\_}Thermodynamik/Noll 1974 Mechanics and Thermodynamics{\_}SelectedPapers.pdf:pdf},
isbn = {9783642658198},
issn = {0036-8075},
number = {1240},
pages = {343--345},
pmid = {17811888},
title = {{the Foundations of Mechanics.}},
volume = {48},
year = {1918}
}
@article{Models1992a,
author = {Models, Mathematical},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Anisotropic Behaviouir of Damaged Materials{\_}Skrzypek{\_}ARTICEL/Kap1{\_}Applications of Tensor Functions in Damage Mechanics of Anisotropic Materials.pdf:pdf},
keywords = {anisotropy,canonical form,constitutive equations,continuum damage,creep,creep rupture,creep rupture time,damage tensor,evolutional equa-,irreducible invariants,material,material behaviour,mechanics,monkman-grant relationship,net-stress concept,tensor,tensor function,tensor generator,tensorial interpolation,ter-,tions},
number = {January},
pages = {47--59},
title = {{Applications of Tensor Functions in Continuum Damage Mechanics}},
year = {1992}
}
@article{Grandin2000,
abstract = {It is generally accepted that knocking combustion influences the heat transfer in SI engines. However, the effects of heat transfer on the onset of knock is still not clear due to lack of experimental data of the thermal boundary layer close to the combustion chamber wall. This paper presents measurements of the temperature in the thermal boundary layer under knocking and non-knocking conditions. The temperature was measured using dual-broadband rotational Coherent anti-Stokes Raman Spectroscopy (CARS). Simultaneous time-resolved measurements of the cylinder pressure, at three different locations, and the heat flux to the wall were carried out. Optical access to the region near the combustion chamber wall was achieved by using a horseshoe-shaped combustion chamber with windows installed in the rectangular part of the chamber. This arrangement made CARS temperature measurements close to the wall possible and results are presented in the range 0.1-5 mm from the wall. The engine was run with constant fuel flow under near stoichiometric conditions. Knocking and non-knocking conditions were achieved by using different mixtures of n-heptane and iso-octane.},
author = {Grandin, B{\"{o}}rje and Denbratt, Ingemar and Bood, Joakim and Brackmann, Christian and Bengtsson, Per-Erik},
doi = {10.4271/2000-01-2831},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2000{\_}Grandin{\_}The Effect of Knock on the Heat Transfer in an SI Engine.pdf:pdf},
journal = {SAE Tech. Pap.},
number = {2000-01-2831},
title = {{The Effect of Knock on the Heat Transfer in an SI Engine: Thermal Boundary Layer Investigation using CARS Temperature Measurements and Heat Flux Measurements}},
url = {http://dx.doi.org/10.4271/2000-01-2831},
year = {2000}
}
@article{Buck,
author = {Buck, H and Leyh, J and Ohlhausen, P and Richter, M and Spath, D and Warschat, J},
journal = {H{\{}{\"{u}}{\}}tte},
pages = {1--41},
title = {{N-Management}}
}
@article{Tarnopolskii1998,
author = {Tarnopol'skii, Yu.M. and Kulakov, V L},
isbn = {0-412-54020-7},
journal = {Handb. Compos.},
pages = {778--793},
title = {{Mechanical tests}},
year = {1998}
}
@article{Buryachenko1995a,
abstract = {We consider a linearly elastic composite medium, which consists of a homogeneous matrix containing a homogeneous and statistically uniform random set of ellipsoidal inclusions. Because of the differential thermal expansion, a microstructural residual stress state arises. By means of the "multiparticle effective field" method we first derive the functional relation between the stored elastic energy and the thermoelastic constants of the components. Using this result an exact estimation of all components of the statistical second moment tensor of the stress fields is given. Furthermore, an expression for the second moment of the stress in the matrix in the vicinity of the ellipsoidal inclusion and a correlation function of internal stresses is obtained. The application of the theory is demonstrated by some numerical results for a WC-Co composite. ?? 1995.},
author = {Buryachenko, Valeriy A and Kreher, Wolfgang S},
doi = {10.1016/0022-5096(95)00029-I},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Probabilistic Aspects/1995{\_}Kreher{\_}Internal residual stresses in heterogeneous solids - a statistical theory for particulate composites.pdf:pdf},
isbn = {0022-5096},
issn = {00225096},
journal = {J. Mech. Phys. Solids},
number = {7},
pages = {1105--1125},
title = {{Internal residual stresses in heterogeneous solids-A statistical theory for particulate composites}},
volume = {43},
year = {1995}
}
@article{Torrilhon2007,
author = {Torrilhon, Manuel},
doi = {10.1002/theDOIsuffix},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Thermodynamik/PhasenFeld/Nestler{\_}Crack{\_}propagation{\_}on{\_}mesoscopic{\_}length{\_}scale.pdf:pdf},
journal = {Pamm},
keywords = {chemo-mechanical coupling,crack propagation,multiphase-field,phase-field},
pages = {1--2},
title = {{Stability of reduced electric arc models}},
url = {http://onlinelibrary.wiley.com/doi/10.1002/pamm.200700318/abstract},
volume = {2},
year = {2007}
}
@article{Ubungsaufgaben,
author = {{\"{U}}bungsaufgaben, A L{\"{o}}sungen Der},
title = {{A.1 L{\"{o}}sungen der {\"{U}}bungsaufgaben}}
}
@article{Hans,
author = {Hans, Von A and Horner, B and Moosmann, F},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Vorlesungen/Messtechnik+Regelungstechnik/D{\_}Reglersynthese.pdf:pdf},
pages = {1--35},
title = {{Reglersynthese und Simulation}}
}
@article{Frontlangs-allradantrieb1910,
author = {Frontl{\"{a}}ngs-allradantrieb, F L A and Heckl{\"{a}}ngs-antrieb, H L and Heckquer-antrieb, H Q},
journal = {Erkenntnis},
title = {{12 Beispiele ausgef{\"{u}}hrter Konstruktionen von Fahrzeuggetrieben}},
year = {1910}
}
@article{Raillard2015,
author = {Raillard, B and Mu, F},
doi = {10.1016/B978-1-78242-074-3.00024-6},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/{\_}buecherSong/HandbookofComposites/II/24{\_}ProcessingThermoplasticComposites.pdf:pdf},
isbn = {9781782420743},
title = {24 24.1},
year = {2015}
}
@article{Mizuno2009a,
abstract = {This study examined a method of predicting the piston temperature in reciprocating internal combustion engines with the aim of developing lightweight pistons. Since the piston temperature is strongly affected by the in-cylinder temperature distribution and turbulence, it is necessary to consider the effects of flame propagation, cooling by the intake air, temperature rise due to combustion, in-cylinder flow and the combustion chamber shape. A three-dimensional combustion simulation that can take these effects into consideration was run to calculate the heat transfer coefficient from the piston crown surface and the gas temperature. The results were used as the boundary conditions for an analysis of heat transfer from the piston, and a method was thus developed for analyzing the piston temperature. The hardness method was used to obtain the piston temperature distribution and maximum temperature during engine operation, and a comparison was made with the analytical results to examine the effects of flame propagation.},
author = {Mizuno, Hideaki and Ashida, Koichi and Teraji, Atsushi and Ushijima, Kenshi and Takemura, Shinichi},
doi = {10.4271/2009-01-0187},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2009{\_}Mizuno{\_}Transient Analysis of the Piston Temperature with Measurement and Simulation.pdf:pdf},
isbn = {9200901018},
issn = {1946-3944},
journal = {SAE Int. J. Engines},
number = {1},
pages = {187--2009},
title = {{Transient Analysis of the Piston Temperature with Consideration of In-cylinder Phenomena Using Engine Measurement and Heat Transfer Simulation Coupled with Three-dimensional Combustion Simulation}},
url = {http://papers.sae.org/2009-01-0187/},
volume = {2},
year = {2009}
}
@article{Case,
author = {Case, The General and Case, General and Example, Above},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Mathematik/Transformation pdfs.pdf:pdf},
pages = {1--11},
title = {{11 — Transforming Density Functions}},
url = {https://www.cl.cam.ac.uk/teaching/2003/Probability/prob11.pdf}
}
@article{Weise2017,
author = {Weise, Martina and Arnold, Thomas and Ambrosius, Volker and Neukirchner, Heiko},
doi = {https://doi.org/10.1007/s35146-017-0108-x},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Thermal Coating + Water Heat Transfer + Applikation/2017{\_}Weise+Arnold{\_}Innovatives Thermomanagement{\_}Blasensieden im Motor.pdf:pdf},
journal = {MTZ - Mot. Zeitschrift},
number = {10},
pages = {50--55},
title = {{Innovatives Thermomanagement}},
volume = {78},
year = {2017}
}
@article{Hild2015,
abstract = {{\textcopyright} Springer Science+Business Media New York 2015.This chapter is devoted to the evaluation of damage with digital image correlation (DIC). This measurement technique provides displacement fields that can be used to tune material parameters of damage models. The potential of DIC for identification purposes is illustrated hereafter for simple 1D-type geometries in the context of quasi-brittle and ductile behaviors. Beams and frames as encountered in civil engineering application can be described through damage laws. The localization of damage at single points (lumped damage mechanics) and the resulting damage law can be determined very precisely based on dedicated versions of DIC incorporating the descriptive language of beam theory. At smaller scale, plasterboards (plaster core lined with paper) constitute another example of a structure (rather than a material), which can be described as damageable. Those cases will be analyzed in details.},
author = {Hild, Fran{\c{c}}ois and Roux, St{\'{e}}phane},
doi = {10.1007/978-1-4614-5589-9},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/2015{\_}Sun+Liu{\_}Particel-Debonding modeling of metal-matrix composites.pdf:pdf},
isbn = {9781461455899},
journal = {Handb. Damage Mech. Nano to Macro Scale Mater. Struct.},
pages = {1277--1299},
title = {{Evaluating damage with digital image correlation: b. from physical to mechanical damage}},
year = {2015}
}
@book{mollenhauer2010handbook,
author = {Mollenhauer, K and Johnson, K G E and Tsch{\"{o}}ke, H},
isbn = {9783540890836},
publisher = {Springer Berlin Heidelberg},
title = {{Handbook of Diesel Engines}},
url = {https://books.google.de/books?id=1zykqE-UN2QC},
year = {2010}
}
@book{Oerteljr.2011,
author = {Oertel jr., Herbert and B{\"{o}}hle, Martin and Reviol, Thomas},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/Str{\"{o}}mungsmechanik{\_}Oertel{\_}KurzeVersion.pdf:pdf},
isbn = {9783834813978},
pages = {479},
title = {{Str{\"{o}}mungs- mechanik}},
year = {2011}
}
@article{Rostampour2015b,
abstract = {This investigation deals with the EF7 (TC) engine, a dual fuel engine equipped with a turbocharger system, consequently with a high probability of knock inception. In this study, an operating cycle of the engine was simulated using KIVA-3V code. Some modifications were carried out on the KIVA method of calculating pressure in the intake port in order to simulate turbocharger pressure correctly. Auto-ignition and knock were then simulated using the auto-ignition integral model. The modified code and the simulation were verified using three different methods; in-cylinder average pressure, gas temperature of the exhaust port, and auto-ignition timing. The simulation results using the auto-ignition integral model, as compared with the experimental data, proved to be reasonably accurate. Following this validation, the effect of the knock phenomenon on the engine heat transfer through the walls was investigated. The simulations showed that the rate of heat transfer through the walls under knocking conditions is about 2.2 times higher than that under normal conditions. However, it was also shown that the total heat transfer increases about 15{\{}{\%}{\}}.},
author = {Rostampour, Arman and Toosi, Ali Nassiri},
doi = {10.1115/1.4030517},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2015{\_}Rostampour{\_}Numerical Investigation of the effect of knock on heat transfer in a turbo si engine.pdf:pdf},
issn = {0742-4795},
journal = {J. Eng. Gas Turbines Power},
number = {12},
pages = {121502},
title = {{Numerical Investigation of the Effect of Knock on Heat Transfer in a Turbocharged Spark Ignition Engine}},
url = {http://www.scopus.com/inward/record.url?eid=2-s2.0-84930634240{\%}7B{\&}{\%}7DpartnerID=tZOtx3y1},
volume = {137},
year = {2015}
}
@article{Sozialisation1999,
author = {Sozialisation, Organisationale},
journal = {Forschung},
pages = {8--9},
title = {{Teil III :}},
year = {1999}
}
@article{2012,
author = {Ε{\$}\pi{\$}{\$}\iota{\$}{\$}\tau{\$}{\$}\rho{\$}ο{\$}\pi{\$}ά{\$}\kappa{\$}{\$}\eta{\$}ς, Ι},
title = {{Χ{\$}\alpha{\$}{\$}\rho{\$}{\$}\alpha{\$}{\$}\kappa{\$}{\$}\tau{\$}{\$}\eta{\$}{\$}\rho{\$}{\$}\iota{\$}{\$}\sigma{\$}{\$}\mu{\$}ός {\$}\Sigma{\$}ύ{\$}\nu{\$}{\$}\theta{\$}{\$}\epsilon{\$}{\$}\tau{\$}{\$}\omega{\$}{\$}\nu{\$} {\$}\Upsilon{\$}{\$}\lambda{\$}{\$}\iota{\$}{\$}\kappa{\$}ώ{\$}\nu{\$} Α{\$}\nu{\$}{\$}\theta{\$}{\$}\rho{\$}{\$}\alpha{\$}{\$}\kappa{\$}ο{\$}\nu{\$}{\$}\eta{\$}{\$}\mu{\$}ά{\$}\tau{\$}{\$}\omega{\$}{\$}\nu{\$} Κ{\$}\alpha{\$}{\$}\tau{\$}{\$}\alpha{\$}{\$}\sigma{\$}{\$}\kappa{\$}{\$}\epsilon{\$}{\$}\upsilon{\$}{\$}\alpha{\$}{\$}\sigma{\$}{\$}\mu{\$}έ{\$}\nu{\$}{\$}\omega{\$}{\$}\nu{\$} Μ{\$}\epsilon{\$} Τ{\$}\eta{\$} Μέ{\$}\theta{\$}ο{\$}\delta{\$}ο {\$}\Pi{\$}{\$}\epsilon{\$}{\$}\rho{\$}{\$}\iota{\$}έ{\$}\lambda{\$}{\$}\iota{\$}{\$}\xi{\$}{\$}\eta{\$}ς Τ{\$}\omega{\$}{\$}\nu{\$} Ι{\$}\nu{\$}ώ{\$}\nu{\$} (Filament Winding)}},
year = {2012}
}
@article{Differenzen-,
author = {Differenzen-, Die},
title = {{5 Grundlagen der numerischen Verfahren f u ¨ r partielle Differenzialgleichungen}}
}
@article{Rousselier1987,
abstract = {Since the pioneering studies conducted by McClintock, Rice and Tracey on the growth of cavities, many studies have covered modelling of ductile fracture; a non-exhaustive list is given of these studies. In the local approach of fracture, the models are used at the tip of cracks, and in the present state, only relatively simple models can be used to solve fracture problems in a complete manner, from material characterization to the analysis of cracked structures. The paper presents two types of models based on a critical ratio of cavity growth or on continuum damage mechanics. In the framework of the local approach of fracture, their possibilities are presented with constant references to experimental validation studies. This allows conclusions to be drawn regarding the effectiveness of the methods proposed and their undeniable contribution to fracture mechanics. ?? 1987.},
author = {Rousselier, G},
doi = {10.1016/0029-5493(87)90234-2},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Plasticity models/Ductile fracture models and their potential in local approach of fracture{\_}Rousselier.pdf:pdf},
isbn = {00295493},
issn = {00295493},
journal = {Nucl. Eng. Des.},
number = {1},
pages = {97--111},
title = {{Ductile fracture models and their potential in local approach of fracture}},
volume = {105},
year = {1987}
}
@book{Gross2011j,
author = {Gross, Dietmar and Seelig, Thomas},
doi = {10.1007/978-3-642-10196-0},
isbn = {978-3-642-10195-3},
title = {{Bruchmechanik}},
url = {http://link.springer.com/10.1007/978-3-642-10196-0},
year = {2011}
}
@article{Gingrich2016b,
abstract = {An experimental investigation was conducted to explore the impact in-cylinder pressure oscillations have on piston heat transfer. Two fast-response surface thermocouples embedded in the piston top measured transient temperature and a commercial wireless telemetry system was used to transmit thermocouple signals from the moving piston. Measurements were made in a light-duty single-cylinder research engine operated under low temperature combustion regimes including Homogeneous Charge Compression Ignition (HCCI) and Reactivity Controlled Compression Ignition (RCCI) and Conventional Diesel (CDC). The HCCI data showed a correlated trend of higher heat transfer with increased pressure oscillation strength, while the RCCI and CDC data did not. An extensive HCCI data set was acquired. The heat transfer rate - when corrected for differences in cylinder pressure and gas temperature - was found to positively correlate with increased pressure oscillations. It is important to normalize the data before drawing conclusions as the magnitude of the effect was diminished significantly by the normalization procedure.},
author = {Gingrich, Eric and Janecek, Daniel and Ghandhi, Jaal},
doi = {10.4271/2016-01-9044},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Klopfen{\_}Ottomotor/2016{\_}Gingrich{\_}Experimental Investigation of the Impact of In-Cylinder Pressure Oscillations on Piston Heat Transfer.pdf:pdf},
issn = {1946-3944},
journal = {SAE Int. J. Engines},
number = {3},
pages = {2016--01--9044},
title = {{Experimental Investigation of the Impact of In-Cylinder Pressure Oscillations on Piston Heat Transfer}},
url = {http://papers.sae.org/2016-01-9044/},
volume = {9},
year = {2016}
}
@article{Cetin2013,
abstract = {The most relevant aspects of material fatigue, i.e., the size of fatigue initiating defects, the fatigue limit, and the fatigue life can be characterized by means of extreme value distributions. The present work introduces a new physically based extreme value distribution. This new distribution function is derived by assuming that the size of the fatigue initiating defects in a component are log-normally distributed. It is demonstrated how the different aspects of material fatigue can be related to each other and consistently characterized with a single type of distribution function. {\textcopyright} 2012 Elsevier Ltd. All rights reserved.},
author = {Cetin, A. and Naess, A. and H{\"{a}}rkeg{\aa}rd, G.},
doi = {10.1016/j.ijfatigue.2012.09.003},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Probabilistic Aspects/2013{\_}Cetin+Naess{\_}A physically based extreme value characterization of material fatigue.pdf:pdf},
issn = {01421123},
journal = {Int. J. Fatigue},
keywords = {Defects,Extreme value distributions,Fatigue life,Fatigue limit,Weakest link},
pages = {216--221},
publisher = {Elsevier Ltd},
title = {{A physically based extreme value characterization of material fatigue}},
url = {http://dx.doi.org/10.1016/j.ijfatigue.2012.09.003},
volume = {47},
year = {2013}
}
@article{Vergleicha,
author = {Vergleich, Im},
title = {{9. Versuchsanlagen}}
}
@inproceedings{Elmqvist2003,
abstract = {The objective of this paper is to present a simulation model for controlling combustion phasing in order to avoid knock in turbocharged SI engines. An empirically based knock model was integrated in a one-dimensional simulation tool. The empirical knock model was optimized and validated against engine tests for a variety of speeds and $\lambda$. This model can be used to optimize control strategies as well as design of new engine concepts.The model is able to predict knock onset with an accuracy of a few crank angle degrees. The phasing of the combustion provides information about optimal engine operating conditions.},
author = {Elmqvist, Christel and Lindstr{\"{o}}m, Fredrik and Angstr{\"{o}}m, Hans-Erik and Grandin, B{\"{o}}rje and Kalghatgi, Gautam},
booktitle = {SAE Powertrain Fluid Syst. Conf. Exhib.},
doi = {10.4271/2003-01-3123},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Klopfen{\_}Ottomotor/2003{\_}Elmqvist{\_}Optimizing Engine Concepts by Using a Simple Model for Knock Prediction.pdf:pdf},
publisher = {SAE International},
title = {{Optimizing Engine Concepts by Using a Simple Model for Knock Prediction}},
year = {2003}
}
@article{Statik,
author = {Statik, Band},
doi = {10.1007/978-3-642-19984-4},
isbn = {9783642199844},
pages = {2--4},
title = {{Uhrung}}
}
@article{Meschede2006,
author = {Meschede, D},
journal = {Gerthsen Phys.},
pages = {677--730},
title = {{13 - Teilchen, Wellen, mikroskopische Physik}},
url = {http://www.springerlink.com/index/TU4R8J43253155M3.pdf},
year = {2006}
}
@article{Mutzke2016b,
abstract = {{\textcopyright} 2016 SAE International.Knocking combustion places a major limit on the performance and efficiency of spark ignition engines. Spontaneous ignition of the unburned air-fuel mixture ahead of the flame front leads to a rapid release of energy, which produces pressure waves that cause the engine structure to vibrate at its natural frequencies and produce an audible 'pinging' sound. In extreme cases of knock, increased temperatures and pressures in the cylinder can cause severe engine damage. Damage is thought to be caused by thermal strain effects that are directly related to the heat flux. Since it will be the maximum values that are potentially the most damaging, then the heat flux needs to be measured on a cycle-by-cycle basis. Previous work has correlated heat flux with the pressure fluctuations on an average basis, but the work here shows a correlation on a cycle-by-cycle basis. The in-cylinder pressure and surface temperature were measured using a pressure transducer and eroding-type thermocouple. These sensors were installed side-by-side at the surface of the cylinder in order to investigate the relationship between knock and heat flux on a cycle-by-cycle basis. A finite difference method was implemented to solve the one-dimensional unsteady heat conduction equation and calculate the temperature distribution away from the surface of the combustion chamber, and thus the instantaneous heat flux. The knock intensity was varied by controlling the fuel quality, compression ratio, ignition timing and air-fuel ratio. The measured heat flux was compared with pressure-based knock indices and it was found that as knock intensity increases, the correlation with peak heat flux became stronger. Results from different fuels and engine operating conditions did not collapse onto the same trend line. At higher speeds and higher compression ratios the heat flux was higher at a given level of knock intensity. The co-location of the pressure transducer and heat flux sensor meant that a correlation was found on a cycle-by-cycle basis.},
author = {Mutzke, J. and Scott, B. and Stone, R. and Williams, J.},
doi = {10.4271/2016-01-0700},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Klopfen{\_}Ottomotor/2016{\_}Mutzke{\_}The Effect of Combustion Knock on the Instantaneous Heat Flux in Spark Ignition Engines.pdf:pdf},
journal = {SAE Tech. Pap.},
title = {{The Effect of Combustion Knock on the Instantaneous Heat Flux in Spark Ignition Engines}},
volume = {2016-April},
year = {2016}
}
@article{Herleitung,
author = {Herleitung, Die and Grundlage, Eine and Zusammenstel-, Durch and Be-, Zur and Annahme, Unter and Modellbildung, Zur and Vereinfachen, Das and Untersuchung, Zur and Er-, Diese},
journal = {Simulation},
pages = {47--70},
title = {{3 Modellierung , Analyse und Simulation der}}
}
@book{Antman2007,
abstract = {This book has been written for undergraduate and graduate students in various areas of mathematics and its applications. It is for students who are willing to get acquainted with Bayesian approach to computational science but not necessarily to go through the full immerson into the statistical analysis. It has also been written for researchers working in areas where mathematical and statistical modeling are of central importance, such as biology and engineering.},
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Antman, S S and Marsden, J E and Sirovich, L},
booktitle = {Uquedusa},
doi = {10.1007/978-4-431-54177-6},
eprint = {arXiv:1011.1669v3},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Efendiev, Hou 2009 - Multiscale Finite Element Methods.pdf:pdf},
isbn = {9780387733937},
issn = {1098-6596},
pages = {202},
pmid = {25246403},
title = {{Surveys and Tutorials in the}},
url = {http://books.google.com/books?id=HIG0CRf6msoC},
volume = {2},
year = {2007}
}
@article{Fillers,
author = {Fillers, Particulate},
journal = {New York},
title = {{Particulate fillers}}
}
@article{Wirsching1983a,
abstract = {Two methods are discussed for constructing a design curve on the safe side of fatigue data. Both the tolerance interval and equivalent prediction interval (EPI) concepts provide such a curve while accounting for both the distribution of the estimators in small samples and the data scatter. The EPI is also useful as a mechanism for providing necessary statistics on S-N data for a full reliability analysis which includes uncertainty in all fatigue design factors. Examples of statistical analyses of the general strain life relationship are presented. The tolerance limit and EPI techniques for defining a design curve are demonstrated. Examples usng WASPALOY B and RQC-100 data demonstrate that a reliability model could be constructed by considering the fatigue strength and fatigue ductility coefficients as two independent random variables. A technique given for establishing the fatigue strength for high cycle lives relies on an extrapolation technique and also accounts for "runners." A reliability model or design value can be specified.},
author = {Wirsching, P. H.},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Probabilistic Aspects/1983{\_}Wirsching{\_}Statistical summaries of fatigue data for design purposes.pdf:pdf},
issn = {05657059},
journal = {Nasa Cr 3697},
number = {July},
title = {{Statistical Summaries of Fatigue Data for Design Purposes}},
year = {1983}
}
@article{Magneten,
author = {Magneten, Feldlinien Von},
pages = {1--29},
title = {{5 Magnetisches Feld}}
}
@article{Baker2009,
author = {B{\"{a}}ker, Martin},
isbn = {3-936148-08-2},
journal = {Braunschweiger Schriften zum Maschinenbau},
title = {{Numerische Methoden in der Materialwissenschaft}},
volume = {8},
year = {2009}
}
@article{Maschinenelemente2011,
author = {Maschinenelemente, Einteilung Der},
doi = {10.1007/978-3-8348-8279-0},
isbn = {9783834882790},
title = {{1 Allgemeine und konstruktive Grundlagen}},
year = {2011}
}
@article{Worlds2016,
author = {Worlds, Small and Attachment, Preferential and Models, Voter and Distributions, Fixed Degree and Laws, Power},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Zienkiewicz FEM - Vol 1 Basics Fundamentals/63205{\_}toc.pdf:pdf},
isbn = {9780511546594},
pages = {5--6},
title = {{Preface 1.}},
year = {2016}
}
@article{Cherkaoui2009d,
author = {Cherkaoui, Mohammed and Capolungo, Laurent},
doi = {10.1007/978-0-387-46771-9},
isbn = {978-0-387-46765-8},
pages = {1--27},
title = {{Atomistic and Continuum Modeling of Nanocrystalline Materials}},
url = {http://link.springer.com/10.1007/978-0-387-46771-9},
volume = {112},
year = {2009}
}
@article{Merhy2013,
abstract = {This paper presents results and interpretations of several long crack thermo-mechanical fatigue tests on A356-T7 cast aluminum alloy used in automotive cylinder heads. These tests were conducted on CT16 and SEN specimens for different positive and negative load ratios, temperatures, frequencies and stress intensity factor values in order to establish the contribution of each parameter governing the fatigue crack propagation. It was shown that the decrease of the frequency causes significant increase of the crack growth rate especially at high temperatures and load ratios. The performing of negative load ratio tests had shown a primordial importance of the compressive load part of fatigue on the crack advance. In addition, SEM, optical microscopy and other metallographic techniques were used to examine fracture surfaces and to analyze particles cracking. For positive load ratios tests, it was shown that in stage II (Paris regime) and stage III (high crack growth rates) the number of cracked particles increases with Kmax and gradual changes in fracture surface appearance occur. These changes were associated with different crack growth mechanisms at the microstructural scale. The amplitude of the inelastic deformations and the extent of the plastic zone ahead of the crack tip were used to explain the observed changes in crack growth mechanisms. The crack growth under negative load ratio loads is especially analyzed, and a way of deriving this rate is given and shown to be relevant even for nonisothermal loading. ?? 2013 Elsevier Ltd.},
author = {Merhy, E and R??my, L and Maitournam, H and Augustins, L},
doi = {10.1016/j.engfracmech.2013.03.019},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/2013{\_}Merhy{\_}Crack growth characterisation of A356-T7 aluminium alloy under TMF.pdf:pdf},
issn = {00137944},
journal = {Eng. Fract. Mech.},
keywords = {A356 cast alloy,Crack growth rate,Damage tolerant design,Life time prediction,Thermal-mechanical fatigue},
pages = {99--112},
publisher = {Elsevier Ltd},
title = {{Crack growth characterisation of A356-T7 aluminum alloy under thermo-mechanical fatigue loading}},
url = {http://dx.doi.org/10.1016/j.engfracmech.2013.03.019},
volume = {110},
year = {2013}
}
@article{Langeheinecke,
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Langeheinecke, Klaus},
doi = {10.1017/CBO9781107415324.004},
eprint = {arXiv:1011.1669v3},
isbn = {9783658031688},
issn = {1098-6596},
pmid = {25246403},
title = {{Thermodynamik f{\"{u}}r Ingenieure}}
}
@article{Shimada2004,
abstract = {The effect of local lubricant viscosity on the temperature and thickness of oil film on a piston ring in a diesel engine is analyzed by using the Reynolds equation, and unsteady and two-dimensional energy equation with heat generated from viscous dissipation. The oil film viscosity for a multi-grade oil is then estimated by using the local oil film temperature and the local shear rate. Moreover, the heat transfer between ring and liner surfaces is examined. The oil film thickness calculated from this method is lesser than that of the case where the viscosity is based on the liner temperature and the mean shear rate. Maximum values of heat transfer at the ring and liner surfaces are obtained at the vicinity of crank angle where the oil film thickness is at a minimum.ER -},
author = {Shimada, Akiko and Harigaya, Yasuo and Suzuki, Michiyoshi and Takiguchi, Masaaki},
doi = {10.4271/2004-32-0024},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Heat Transfer Combustion Chamber/2004{\_}Shimada{\_}An Analysis of Oil Film Temperature - Oil Film Thickness and Heat Transfer on a piston ring of internal combustion engine.pdf:pdf},
isbn = {0791846628},
issn = {07424795},
number = {724},
title = {{An Analysis of Oil Film Temperature, Oil Film Thickness and Heat Transfer on a Piston Ring of Internal Combustion Engine: The Effect of Local Lubricant Viscosity}},
url = {http://papers.sae.org/2004-32-0024/},
year = {2004}
}
@article{1967MolPh..12..569M,
author = {Mathur, S and Tondon, P.{\~{}}K. and Saxena, S.{\~{}}C.},
doi = {https://doi.org/10.1080/00268976700100731},
journal = {Mol. Phys.},
pages = {569--579},
title = {{Thermal conductivity of binary, ternary and quaternary mixtures of rare gases}},
volume = {12},
year = {1967}
}
@article{MacCamhaoil1989a,
author = {MacCamhaoil, Macdara},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Dynamics/Static and dynamic balancing of rigid rotors.pdf:pdf},
pages = {2},
title = {{Static and Dynamic Balancing of Rigid Rotors}},
year = {1989}
}
@article{Darstellung,
author = {Darstellung, Vektorielle},
journal = {Differentiation},
title = {{I Vektoranalysis 1}}
}
@article{Lange2002,
abstract = {Ein Grundkurs zur Theorie des Systems Atmosph{\{}{\"{a}}{\}}re},
author = {Lange, Hans-Joachim},
doi = {10.1007/978-3-8348-9781-7},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/xxx{\_}Herzog{\_}Kolbenmaschinen{\_}2{\_}ThermodynamischeGrundlagen.pdf:pdf},
isbn = {978-3-8348-1404-3},
journal = {Die Phys. des Wetters und des Klimas},
pages = {1--64},
title = {{Thermodynamische Grundlagen}},
year = {2002}
}
@article{Carlo,
author = {Carlo, Monte},
title = {{2 Elasticity 2.1}}
}
@article{Leichtbaua,
author = {Leichtbau, Im},
pages = {38--64},
title = {{6 Leichtbauwerkstoffe}}
}
@article{Beitz2006,
abstract = {Kap 7},
author = {Beitz and Pahl},
isbn = {9783540340607},
journal = {Konstruktionslehre},
pages = {629 -- 688},
title = {{Entwickeln von Baureihen und Bauk{\"{a}}sten - Developing size ranges and modular products}},
year = {2006}
}
@article{Werkstoffkennwertea,
author = {Werkstoffkennwerte, Werkstoffs},
title = {{Einfl{\{}{\"{u}}{\}}sse auf die Schwingfestigkeit}}
}
@article{Aluminium,
author = {Aluminium, Schaum- and Bild, Rechtecke},
pages = {192--214},
title = {{17 Sandwichelemente}}
}
@article{Man2009,
abstract = {Current state and historical progress in experimental and theoretical studies of surface relief appertaining to persistent slip bands (PSBs) and leading to fatigue crack initiation in cyclically deformed metals is presented as a thorough critical overview. A comprehensive inventory of microscopic techniques used for this study is tabulated chronologically with emphasis to their applicability to polycrystals. The most relevant experimental characteristics concerning surface relief evolution, namely the form of extrusions and intrusions in single- and polycrystalline materials, are surveyed. Theoretical models and computational simulations of extrusion and intrusion formation and fatigue crack initiation are critically reviewed.},
author = {Man, J. and Obrtl{\'{i}}k, K. and Pol{\'{a}}k, J.},
doi = {10.1080/14786430902917616},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/2009{\_}Man + Polak{\_}Extrusions and intrusions in fatigued metals Part 1 State of the art and history.pdf:pdf},
isbn = {1478-6435},
issn = {1478-6435},
journal = {Philos. Mag.},
number = {16},
pages = {1295--1336},
title = {{Extrusions and intrusions in fatigued metals. Part 1. State of the art and history†}},
url = {http://www.tandfonline.com/doi/abs/10.1080/14786430902917616},
volume = {89},
year = {2009}
}
@article{Mohammadi2008a,
abstract = {A computational fluid dynamics (CFD) code is applied to simulate fluid flow, heat transfer and combustion in a four-stroke single cylinder engine with pent roof combustion chamber geometry, having two inlet valves and two exhaust valves. Heat flux and heat transfer coefficient on the cylinder head, cylinder wall, piston, intake and exhaust valves are determined with respect to crank angle position. Results for a certain condition are compared for total heat transfer coefficient of the cylinder engine with available correlation proposed by experimental measurement in the literature and close agreement are observed. It was found that the local value of heat transfer coefficient varies considerably in different parts of the cylinder, but they have equivalent trend with crank angle. Based on the results, new correlations are suggested to predict maximum and minimum convective heat transfer coefficient in the combustion chamber of a SI engine. ?? 2007 Elsevier Ltd. All rights reserved.},
author = {Mohammadi, A and Yaghoubi, M and Rashidi, M},
doi = {https://doi.org/10.1016/j.icheatmasstransfer.2007.06.008},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2008{\_}Mohammadi{\_}Analysis of local convective heat transfer in a spark ignition engine.pdf:pdf},
journal = {Int. Commun. Heat Mass Transf.},
keywords = {Combustion chamber,Heat flux,Heat transfer coefficient,SI engine},
number = {2},
pages = {215--224},
title = {{Analysis of local convective heat transfer in a spark ignition engine}},
volume = {35},
year = {2008}
}
@article{Beck2007a,
abstract = {Out-of-phase thermal-mechanical fatigue (TMF) tests with superimposed higher frequency mechanical fatigue (HCF) loading were performed at three cast Al-Si cylinder head alloys. All materials show for maximum temperatures of the TMF cycle between 200 and 250 ??C a threshold of the amplitude of the superimposed HCF loading below of which the number of TMF cycles to failure is not significantly affected by the superimposed HCF loading. Above this threshold the TMF life shows a strong decrease with increasing HCF loading. Extensive microscopic analyses revealed that independent from the HCF loading first cracks are initiated at eutectic Si-particles detached from the surrounding ??-Al matrix. Crack propagation occurs at small HCF amplitudes along the eutectic regions. At higher superimposed HCF loadings an accelerated crack propagation along slip bands within the ??-Al matrix is observed. ?? 2007 Elsevier B.V. All rights reserved.},
author = {Beck, Tilmann and L??he, Detlef and Luft, Jochen and Henne, Ingo},
doi = {10.1016/j.msea.2006.05.177},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Empirical Fatigue Models + Validation/2006{\_}Beck{\_}Damage mechanisms of cast Al–Si–Mg alloys under superimposed TMF and HCF.pdf:pdf},
isbn = {09215093 (ISSN)},
issn = {09215093},
journal = {Mater. Sci. Eng. A},
keywords = {Cast aluminium alloys,Damage behaviour,High-cycle fatigue,Thermal-mechanical fatigue},
number = {SPEC. ISS.},
pages = {184--192},
title = {{Damage mechanisms of cast Al-Si-Mg alloys under superimposed thermal-mechanical fatigue and high-cycle fatigue loading}},
volume = {468-470},
year = {2007}
}
@article{Vektoren,
author = {Vektoren, Spezielle},
pages = {46--66},
title = {{II Vektorrechnung}},
volume = {0}
}
@article{Papadopoulos1997a,
abstract = {The aim of this paper is firstly, to provide a concise assessment of some commonly used high-cycle fatigue criteria and secondly, to check their predictive capabilities against synchronous sinusoidal out-of-phase bending and torsion experimental results (i.e. sinusoidal stress signals of the same frequency but with a phase difference). This bending-torsion stress system does not closely represent real load conditions undergone by a machine part. However, it is complex enough to differentiate the various fatigue criteria and to permit a first classification of the approaches examined, according to the accuracy of their predictions. A fatigue criterion recently formulated by the first of the authors is also included in this comparative study. According to this criterion the phase difference in out-of-phase bending and torsion does not affect the fatigue strength corresponding to a very high (theoretically infinite) fatigue life. It is pointed out that this theoretical finding is valid for the category of hard metals for which the ratio of the fully re-versed torsion fatigue limit over the fully reversed bending fatigue limit lies in the interval from 1√3 o approx. 0.8. Experimental results collected from the relevant literature, concerning precisely lard metals, fully support this theoretical finding.},
author = {Papadopoulos, I},
doi = {10.1016/S0142-1123(96)00064-3},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Empirical Fatigue Models + Validation/1996{\_}Papadopoulos{\_}A comparative study of multiaxial high cycle fatigue criteria for metals .pdf:pdf},
isbn = {0142-1123},
issn = {01421123},
journal = {Int. J. Fatigue},
keywords = {cycle fatigue,high,loading,metals,multiaxial fatigue,n o n -,o n a l,o r t i,p r o p},
number = {3},
pages = {219--235},
title = {{A comparative study of multiaxial high-cycle fatigue criteria for metals}},
url = {http://linkinghub.elsevier.com/retrieve/pii/S0142112396000643},
volume = {19},
year = {1997}
}
@article{Christiaens,
author = {Christiaens, Dirk},
pages = {731--740},
title = {{B11 B11 {\"{U}}berschlagunf{\"{a}}lle Pkw kollidiert mit einem Gel{\"{a}}ndewagen B11}}
}
@article{Notwendigkeit,
author = {Notwendigkeit, Die and Umfang, Der and Ger, Beim},
title = {{9 EMV-Planung und Analysen}}
}
@article{Hashin1963a,
abstract = {Variational principles in the linear theory of elasticity, involving the elastic polarization tensor, have been applied to the derivation of upper and lower bounds for the effective elastic moduli of quasi-isotropic and quasi-homogeneous multiphase materials of arbitrary phase geometry. When the ratios between the different phase moduli are not too large the bounds derived are close enough to provide a good estimate for the effective moduli. Comparison of theoretical and experimental results for a two-phase alloy showed good agreement.},
author = {Hashin, Zvi and Shtrikman, Shmuel},
doi = {10.1016/0022-5096(63)90060-7},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/Strukturmechanik MMS/Literatur/Hashin Shtrikman 1963.pdf:pdf},
isbn = {0022-5096},
issn = {00225096},
journal = {J. Mech. Phys. Solids},
number = {2},
pages = {127--140},
title = {{A variational approach to the theory of the elastic behaviour of multiphase materials}},
url = {http://linkinghub.elsevier.com/retrieve/pii/0022509663900607},
volume = {11},
year = {1963}
}
@article{Erm,
author = {Erm, Unter and Beanspruchungsablauf, Der and Versagenskriterium, Als and Vorgehensweise, Diese and Vorgaben, Den and Erweiterungen, Notwendige},
title = {{2 Schwingfestigkeit 2.1}}
}
@article{Priester,
author = {Priester, Johannes and Kasanicky, Gustav},
pages = {383--410},
title = {{A11 A11 Unf{\"{a}}lle mit Zweir{\"{a}}dern A11 Einteilung der Zweir{\"{a}}der}}
}
@article{Massenkraft,
author = {Massenkraft, Der and Massenkraft, Der and Dichte, Der and Dichte, Der},
journal = {Entropie},
title = {{5 Hydrostatik 5.1}}
}
@article{Piero2005,
author = {Piero, D E L},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/B{\"{u}}cher{\_}Sammlung{\_}ITM/Elasticity and Plasticity of large deformations - Bertram/fulltext9.pdf:pdf},
number = {1967},
title = {{10 Plasticity}},
year = {2005}
}
@article{Hill1966a,
abstract = {A general, type of cross-coupling between glide and hardening on different slip-systems is proposed. Its implications in regard to the character of the connexion between the overall stress-rate and strain-rate in multislip are investigated. Uniqueness theorems and extremal properties are established in respect both of the overall constitutive law itself and any boundary-value problem for non-uniform deformation of a single crystal or aggregate.},
author = {Hill, R.},
doi = {10.1016/0022-5096(66)90040-8},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/1966{\_}Hill{\_}Generalized consititutive relations for incremental defo of metal crystals by multislip.pdf:pdf},
isbn = {0022-5096},
issn = {00225096},
journal = {J. Mech. Phys. Solids},
number = {2},
pages = {95--102},
title = {{Generalized constitutive relations for incremental deformation of metal crystals by multislip}},
volume = {14},
year = {1966}
}
@book{Habenicht2012c,
author = {Habenicht, Gerd},
isbn = {9783834802958},
title = {{Aus dem Programm Fertigungstechnik}},
year = {2012}
}
@article{Schwingbeanspruchungb,
author = {Schwingbeanspruchung, Kennzeichnung Der},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Empirical Fatigue Models + Validation/Betriebsfestigkeit{\_}ErwinHaibach/Kap2 Experimentelle Grundlagen und Betriebsfestigkeit.pdf:pdf},
title = {{2 Experimentelle Grundlagen der Betriebsfestigkeit}}
}
@article{Seifert2010,
abstract = {In the present paper, mechanism-based models are developed to describe the time and temperature dependent cyclic plasticity and damage of cast iron materials. The cyclic plasticity model is a combination of a viscoplastic model with kinematic hardening and a porous plasticity model to take the effect of graphite inclusions into account. Thus, the model can describe creep, relaxation and the Bauschinger-effect as well as the tension-compression asymmetry often observed for cast iron. The model for thermomechanical fatigue life prediction is based on a crack growth law, which assumes that the crack growth per cycle, da/dN, is correlated with the cyclic crack-tip opening displacement, ?? CTOD. The effect of the graphite inclusions on crack growth is incorporated with a scalar factor into the crack growth law. Both models can describe the essential phenomena which are relevant for cast iron materials. ?? 2010 Elsevier Ltd. All rights reserved.},
author = {Seifert, T. and Riedel, H.},
doi = {10.1016/j.ijfatigue.2010.02.004},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/2010{\_}Seifert+Riedel{\_}Mechanism-based thermomechanical fatigue life prediction of cast iron PartOne Models.pdf:pdf},
isbn = {01421123},
issn = {01421123},
journal = {Int. J. Fatigue},
keywords = {Cast iron,Fatigue crack growth,Life prediction,Plasticity,Thermomechanical fatigue},
number = {8},
pages = {1358--1367},
publisher = {Elsevier Ltd},
title = {{Mechanism-based thermomechanical fatigue life prediction of cast iron. Part I: Models}},
url = {http://dx.doi.org/10.1016/j.ijfatigue.2010.02.004},
volume = {32},
year = {2010}
}
@article{Stiller2006c,
author = {Stiller, Christoph},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Vorlesungen/Messtechnik+Regelungstechnik/gmrt{\_}buch0801.pdf:pdf},
isbn = {3-8322-5582-6; 978-3-8322-5582-4},
issn = {02731177},
journal = {Adv. Sp. Res.},
number = {12},
pages = {2820--2823},
title = {{Grundlagen der Mess- und Regelungstechnik}},
volume = {38},
year = {2006}
}
@article{Merkera,
author = {Merker, G{\"{u}}nter and Schwarz, Christian and Stiesch, Gunnar and Otto, Frank},
journal = {Simul. der Verbrennung und Schadstoffbildung},
title = {{9 Str{\"{o}}mungsmechanische Simulation}}
}
@article{Kennametal2011,
author = {Kennametal},
pages = {34--55},
title = {{Composite machining}},
url = {www.kennametal.com},
year = {2011}
}
@article{Stromfunktion,
author = {Stromfunktion, Potential-},
title = {{Omungen}}
}
@article{Murakami2012a,
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Murakami, Sumio},
doi = {10.1007/978-94-007-2666-6},
eprint = {arXiv:1011.1669v3},
isbn = {978-94-007-2665-9},
issn = {09250042},
pages = {305--323},
pmid = {25246403},
title = {{Continuum Damage Mechanics}},
url = {http://link.springer.com/10.1007/978-94-007-2666-6},
volume = {185},
year = {2012}
}
@article{Prozesse,
author = {Prozesse, Aussagen and Hauptsatz, Zweiter},
journal = {Arbeit},
pages = {84--115},
title = {{5 Prozesse 5.1}}
}
@article{Bungartz2010a,
abstract = {Stra{\{}{\ss}{\}}enverkehr geht uns alle an, jeder ist davon betroffen. Unsere W{\{}{\"{u}}{\}}nsche und Vorstellungen bez{\{}{\"{u}}{\}}glich des Stra{\{}{\ss}{\}}enverkehrs sind jedoch in der Regel etwas widerspr{\{}{\"{u}}{\}}chlich: Einerseits wollen wir m{\{}{\"{o}}{\}}glichst viel davon. Wir wollen mobil sein und so schnell und angenehm wie m{\{}{\"{o}}{\}}glich von der Wohnung zur Uni oder Arbeit, vom Heimatort zum Ferienziel oder vom Einkaufen zur Freizeitbesch{\{}{\"{a}}{\}}ftigung gelangen. Wir w{\{}{\"{u}}{\}}nschen uns dazu gut ausgebaute Stra{\{}{\ss}{\}}en und Parkpl{\{}{\"{a}}{\}}tze oder h{\{}{\"{a}}{\}}ufig fahrenden Personennahverkehr. Andererseits wollen wir m{\{}{\"{o}}{\}}glichst wenig davon. Stra{\{}{\ss}{\}}enverkehr soll uns nicht bel{\{}{\"{a}}{\}}stigen. Wir m{\{}{\"{o}}{\}}chten nicht im Berufsverkehr oder in den kilometerlangen Mammutstaus zu Ferienbeginn und -ende stehen, w{\{}{\"{u}}{\}}nschen uns, von L{\{}{\"{a}}{\}}rm- und Abgasemissionen unbehelligt zu bleiben, und bevorzugen Gr{\{}{\"{u}}{\}}nstreifen anstelle von Stra{\{}{\ss}{\}}enasphalt.},
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Bungartz and Zimmer and Buchholz and Pfl{\"{u}}ger},
doi = {10.1515/bmt.2010.712},
eprint = {arXiv:1011.1669v3},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Vorlesungen/Modellbildung{\_}und{\_}Simulation/Skript{\_}Modellbildung{\_}und{\_}Simulation.pdf:pdf},
isbn = {9783642054600},
issn = {0013-5585},
journal = {Biomed. Tech. Eng.},
keywords = {Stichw䣏rter des Dokuments},
number = {s1},
pages = {1--237},
pmid = {14685750},
title = {{Modellbildung und Simulation}},
volume = {55},
year = {2010}
}
@article{Stanley1999a,
abstract = {This paper presents a simplified piston ring assembly (PRA) friction model of the piston ring pack and the piston skirt. The ring model considers both mixed and hydrodynamic lubrication; the skirt model considers hydrodynamic lubrication only. The Reynold's equation is used as a governing equation for the hydrodynamic regimes of both models. Simplified assumptions are used to include mixed lubrication in the ring model. The ring model generates unique Stribeck curves for a given ring's geometry; the skirt model generates generic relationships between the friction force and skirt geometry, piston speed, oil viscosity, and assumed boundary conditions. Inter-ring starvation effects are introduced by varying the boundary conditions, as appropriate. The models are compared to measurements made on a motored and fired single-cylinder diesel engine; the theoretical calculations provide a reasonable estimate of the measured data. .},
author = {Stanley, Richard and Taraza, Dinu and Henein, Naeim and Bryzik, Walter},
doi = {10.4271/1999-01-0974},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Mechanik+Reibung/1999{\_}Stanley{\_}A Simplified Friction Model of the Piston Ring Assembly.pdf:pdf},
isbn = {SAE 1999-01-0974},
number = {724},
title = {{A Simplified Friction Model of the Piston Ring Assembly}},
url = {http://papers.sae.org/1999-01-0974/},
year = {1999}
}
@article{Veranschaulichung,
author = {Veranschaulichung, Zur},
pages = {43--58},
title = {{5 Salzstreuer}}
}
@article{Meister2011,
abstract = {Die wichtigsten Verfahren zur numerischen L{\{}{\"{o}}{\}}sung von linearen Gleichungssystemen in einer umfassenden Einf{\{}{\"{u}}{\}}hrung, die zum Verst{\{}{\"{a}}{\}}ndnis nur geringe mathematische Vorkenntnisse ben{\{}{\"{o}}{\}}tigt. Behandelt werden sowohl die direkten als auch die iterativen Verfahren, wobei der Autor gro{\{}{\ss}{\}}en Wert auf eine sorgf{\{}{\"{a}}{\}}ltige Herleitung dieser Verfahren legt. Au{\{}{\ss}{\}}erdem sind sehr detaillierte Pseudocodes enthalten, mit deren Hilfe sich die jeweiligen Verfahren in einer beliebigen Programmiersprache sofort auf dem Computer realisieren lassen. Das Lehrbuch ist auch f{\{}{\"{u}}{\}}r Natur- und Ingenieurwissenschaftler geeignet, die in vielen praktischen Anwendungen mit der L{\{}{\"{o}}{\}}sung von linearen Gleichungssystemen konfrontiert sind.},
archivePrefix = {arXiv},
arxivId = {1011.1669v3},
author = {Meister, Andreas},
doi = {10.1007/978-3-8348-8100-7},
eprint = {1011.1669v3},
isbn = {978-3-8348-1550-7},
issn = {1098-6596},
journal = {Matrix},
pages = {36--68},
pmid = {25246403},
title = {{Numerik linearer Gleichungssysteme}},
url = {http://link.springer.com/10.1007/978-3-8348-8100-7},
year = {2011}
}
@book{Mullera,
author = {M{\"{u}}ller, Rolf},
booktitle = {Antriebstechnik},
isbn = {9783834800183},
title = {{Aus dem Programm Automatisierungstechnik}}
}
@article{Hansen2005b,
abstract = {The Hall-Petch relation is discussed separately for the yield stress of undeformed polycrystalline metals and the flow stress of deformed metals. The strength contributions for grain boundaries and from dislocation boundaries are given special attention. An experimental analysis supports the Hall-Petch relation for undeformed metals over a grain size range from about 20 nm to hundred of micrometres. For deformed metals the strengthening effect of low angle dislocation boundaries evolves with increasing strain in parallel with a change in their spacing. An application of the Hall-Petch relation must therefore be based on a detailed structural characterization. ?? 2005 Elsevier B.V. All rights reserved.},
author = {Hansen, Niels},
doi = {10.1016/j.msea.2005.04.061},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2005{\_}Hansen Boundary strengthening in undeformed and deformed polycrystals.pdf:pdf},
isbn = {0921-5093},
issn = {09215093},
journal = {Mater. Sci. Eng. A},
keywords = {Dislocation boundaries,Grain boundaries,Hall-Petch relation,Nanostructures},
number = {1-2},
pages = {39--45},
title = {{Boundary strengthening in undeformed and deformed polycrystals}},
volume = {409},
year = {2005}
}
@article{Lauf-,
author = {Lauf-, Die and Fluid, Dem and Energie, Laufschaufeln},
title = {{5 Kreiselpumpen}}
}
@article{Kerbwirkung,
author = {Kerbwirkung, Bedeutung Der},
doi = {10.1007/978-3-540-71459-0},
isbn = {978-3-540-71458-3},
title = {{4 Kerbwirkung 4.1}}
}
@article{Castillo2009,
author = {Castillo, E},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Probabilistic Aspects/A Unified Statistical Methodology for Modeling Fatigue Damage{\_}Castillo/Kap2{\_}S-N or W{\"{o}}hler Field Models.pdf:pdf},
title = {{S-N or W ¨ ohler Field}},
year = {2009}
}
@misc{Oppenheim1989,
author = {Oppenheim, A V and Schafer, R W and Buck, J R},
booktitle = {Discret. signal Process.},
keywords = {FFT,Hilbert,Signal processing,filtering},
pages = {870},
title = {{1 -Introduction.Pdf}},
year = {1989}
}
@article{Zienkiewicz2014d,
abstract = {In this chapter the weak (variational) form for problems in nonlinear solid mechanics in which strains remain small is used to construct approximate solutions based on the finite element method. This results in a Galerkin method for which general properties are well known. Both irreducible (displacement) and mixed form approaches are considered. In particular, we consider a mixed form based on the Hu-Washizu variational theorem that is appropriate for use in problems in which near incompressible behavior can occur. An isoparametric form for finite element approximation is used along with quadrature to evaluate integrals that appear in the variational form. The chapter also applies the methods developed for the equations of solid mechanics to that for thermal analysis based on a nonlinear form of the quasi-harmonic equation.},
author = {Zienkiewicz, O.C. and Taylor, R.L. and Fox, David},
doi = {10.1016/B978-1-85617-634-7.00002-8},
isbn = {9781856176347},
issn = {0733-9399},
journal = {Finite Elem. Method Solid Struct. Mech.},
pages = {21--55},
title = {{Galerkin Method of Approximation: Irreducible and Mixed Forms}},
url = {http://linkinghub.elsevier.com/retrieve/pii/B9781856176347000028},
year = {2014}
}
@article{Pla,
author = {Pla, Wilfried},
isbn = {9783528039738},
keywords = {fgang b{\{}{\"{o}}{\}}ge,formeln und tabellen,hrsg,wilfried pla{\{}{\ss}{\}}mann},
title = {{Wolfgang B{\{}{\"{o}}{\}}ge , Wilfried Pla{\{}{\ss}{\}}mann ( Hrsg .) Formeln und Tabellen Elektrotechnik}}
}
@article{Lange2002,
abstract = {Ein Grundkurs zur Theorie des Systems Atmosph{\"{a}}re},
author = {Lange, Hans-Joachim},
doi = {10.1007/978-3-8348-9781-7},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/xxx{\_}Herzog{\_}Kolbenmaschinen{\_}2{\_}ThermodynamischeGrundlagen.pdf:pdf},
isbn = {978-3-8348-1404-3},
journal = {Die Phys. des Wetters und des Klimas},
pages = {1--64},
title = {{Thermodynamische Grundlagen}},
year = {2002}
}
@article{Reifenh,
author = {Reifenh, Die and Zugriff, Anwender},
pages = {169--184},
title = {{25 Fahrgastzelle 25.1}}
}
@article{Anfangb,
author = {Anfang, Den and Hauptansicht, Aspekte and Drafting-umgebung, Die and Edge, Solid and Zeichnungen, Plotten Din-gerechter and Zeichnungsdatei, Eine and Blatt, Neues and Auswahl, Schen Die and Grundblatt, Hinter- and Definition, Registerkarte and Zeichnen, Button and Zeichnen, Symbolleiste},
pages = {88--106},
title = {{6 Zeichnungserstellung (Drafting)}}
}
@article{Hochspan-,
author = {Hochspan-, Die Aufgabe Der},
title = {{3 Elektrische Festigkeit}}
}
@misc{Zacher2014,
abstract = {Das Buch behandelt klassische und moderne Methoden zur Untersuchung dynamischer Systeme. Es bietet eine ausf{\"{u}}hrliche und verst{\"{a}}ndliche Darstellung des Stoffes unter Ber{\"{u}}cksichtigung der Laplace-Transformation, der Verfahren der z-Transformation, sowie der digitalen Regelung mittels Mikrorechner. Zahlreiche Beispiele und Aufgaben dienen der Vertiefung des dargebotenen Stoffes. Die Regelkreisanalyse mittels MATLAB/SIMULINK sowie modell- und wissensbasierte Verfahren wie Neuro-Fuzzy werden ebenso behandelt. Aufgrund der ausf{\"{u}}hrlichen Darstellung und der zahlreichen Beispiele und Aufgaben ist das Buch zum Selbststudium besonders gut geeignet. Es wendet sich an die mehr praxisbezogenen Studieng{\"{a}}nge der Elektrotechnik und des Maschinenbaus.},
author = {Zacher, Serge and Reuter, Manfred},
doi = {10.1007/978-3-8348-2216-1},
isbn = {3834822167},
pages = {515},
title = {{Regelungstechnik f{\"{u}}r Ingenieure: Analyse, Simulation und Entwurf von Regelkreisen}},
url = {https://books.google.com/books?id=VLnEBAAAQBAJ{\&}pgis=1},
year = {2014}
}
@article{Fallbeispiele2005,
author = {Fallbeispiele, Die},
doi = {10.1007/3-7985-1528-X_7},
isbn = {3-7985-1465-8},
pages = {25--125},
title = {{Fallbeispiele}},
year = {2005}
}
@article{Zienkiewicz2014d,
abstract = {Abstract In this chapter we review the general equations for analysis of solids in which deformations remain “small” but material behavior includes effects of a nonlinear kind. We present the theory in both an indicial (or tensorial) form as well as in the matrix form commonly used in finite element developments. We also reformulate the equations of solids in a variational (Galerkin) form. The chapter also presents the notation and the methodology which we shall adopt throughout this book. The reader will note how simply the transition between forms for linear and nonlinear problems occurs. },
author = {Zienkiewicz, O.C. and Taylor, R.L. and Fox, David},
doi = {10.1016/B978-1-85617-634-7.00001-6},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Zienkiewicz FEM - Vol 2 Solid Structural Mechanics/63212{\_}01.pdf:pdf},
isbn = {978-1-85617-634-7},
issn = {0733-9399},
journal = {Finite Elem. Method Solid Struct. Mech.},
pages = {1--20},
title = {{General Problems in Solid Mechanics and Nonlinearity}},
url = {http://linkinghub.elsevier.com/retrieve/pii/B9781856176347000016},
year = {2014}
}
@article{Grandin2000b,
abstract = {It is generally accepted that knocking combustion influences the heat transfer in SI engines. However, the effects of heat transfer on the onset of knock is still not clear due to lack of experimental data of the thermal boundary layer close to the combustion chamber wall. This paper presents measurements of the temperature in the thermal boundary layer under knocking and non-knocking conditions. The temperature was measured using dual-broadband rotational Coherent anti-Stokes Raman Spectroscopy (CARS). Simultaneous time-resolved measurements of the cylinder pressure, at three different locations, and the heat flux to the wall were carried out. Optical access to the region near the combustion chamber wall was achieved by using a horseshoe-shaped combustion chamber with windows installed in the rectangular part of the chamber. This arrangement made CARS temperature measurements close to the wall possible and results are presented in the range 0.1-5 mm from the wall. The engine was run with constant fuel flow under near stoichiometric conditions. Knocking and non-knocking conditions were achieved by using different mixtures of n-heptane and iso-octane.},
author = {Grandin, B{\"{o}}rje and Denbratt, Ingemar and Bood, Joakim and Brackmann, Christian and Bengtsson, Per-Erik},
doi = {10.4271/2000-01-2831},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Heat transfer intake+exhaust system/2000{\_}Bood{\_}The Effect of Knock on the Heat Transfer in an SI Engine.pdf:pdf},
journal = {SAE Tech. Pap.},
number = {2000-01-2831},
title = {{The Effect of Knock on the Heat Transfer in an SI Engine: Thermal Boundary Layer Investigation using CARS Temperature Measurements and Heat Flux Measurements}},
url = {http://dx.doi.org/10.4271/2000-01-2831},
year = {2000}
}
@book{Tobergte2013,
abstract = {applicability for this approach.},
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Tobergte, David R. and Curtis, Shirley},
booktitle = {J. Chem. Inf. Model.},
doi = {10.1017/CBO9781107415324.004},
eprint = {arXiv:1011.1669v3},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Thermodynamik/M{\"{u}}llerAndNoll{\_}Thermodynamik/M{\"{u}}ller 2007 Energy and Entropy.pdf:pdf},
isbn = {9788578110796},
issn = {1098-6596},
keywords = {icle},
number = {9},
pages = {1689--1699},
pmid = {25246403},
title = {{A History of Thermodynamics}},
volume = {53},
year = {2013}
}
@inproceedings{Allmendinger2001,
abstract = {Coming along with the present movement towards the ultimately variable engine, the need for clear and simple models for complex engine systems is rapidly increasing. In this context Common-Rail-Systems cause a special kind of problem due to of the high amount of parameters which cannot be taken into consideration with simple map-based models. For this reason models with a higher amount of complexity are necessary to realize a representative behavior of the simulation. The high computational time of the simulation, which is caused by the increased complexity, makes it nearly impossible to implement this type of model in software in closed loop applications or simulations for control purposes. In this paper a method for decreasing the complexity and accelerating the computing time of automotive engine models is being evaluated which uses an optimized method for each stage of the diesel engine process. Except for the gas exchange phase, this approach works analytically and independent of engine maps. Investigations result in the capability of the above mentioned approach to perform engine simulations while reducing the computing time.},
author = {Allmendinger, Klaus and Guzzella, Lino and Seiler, Adrian and Loffeld, Otmar},
booktitle = {SAE 2001 World Congr.},
doi = {10.4271/2001-01-0574},
publisher = {SAE International},
title = {{A Method to Reduce the Calculation Time for an Internal Combustion Engine Model}},
year = {2001}
}
@article{Eekoye1996a,
abstract = {Heat-transfer rates present in an engine cylinder undergoing knock are known to be larger than the rates associated with normal engine operation. Further, at the time of knock, the largest heat fluxes are associated with locations on the cylinder wall where the flame is locally quenching. In this study, heat-transfer processes at the flame-wall interface during a knock event are investigated computationally and analytically. Computationally, the governing equations for a one-dimensional, flame-quenching event are solved using a reduced chemical reaction mechanism. Analytically, scaling relations for the flame heat-release rates are used in the governing equations to determine the heat-transfer rates. It is found that while pressure transients modify the wall heat flux, the absolute value of the pressure is the most significant parameter in predicting the maximum heat flux. The wall heat flux profiles are predicted for both the analytical and computational models. In the range of pressures examined, a linear relationship was found between the peak flux and pressure, both for the computational and analytical models. The linear relationship between the pressure and peak flux was found to be invalid when the flame-quenching process was disrupted by the pressure fluctuations for pressure oscillations with a characteristic time on the order of the quenching process. ?? 1996 Combustion Institute.},
author = {Eekoye, O A},
doi = {10.1016/S0082-0784(96)80101-9},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/1996{\_}Ezekoye{\_}Heat transfer modeling during knock and flame quenching in an engine chamber.pdf:pdf},
isbn = {0082-0784},
issn = {00820784},
journal = {Symp. Combust.},
number = {2},
pages = {2661--2668},
title = {{Heat transfer modeling during knock and flame quenching in an engine chamber}},
volume = {26},
year = {1996}
}
@article{Pokluda2010a,
author = {Pokluda, Jaroslav and Andera, Pavel},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/Micromechanisms of fracture and fatigue/Kap3{\_}BrittleAndDuctileFracture.pdf:pdf},
journal = {Micromechanisms Fract. Fatigue},
pages = {69--123},
title = {{Brittle and Ductile Fracture}},
year = {2010}
}
@article{Borgeest2010,
author = {Borgeest, Kai},
doi = {10.1007/978-3-8348-9337-6},
isbn = {978-3-8348-0548-5},
journal = {Elektron. der Fahrzeugtechnik},
pages = {18},
title = {{2 Bordelektrik}},
url = {http://www.springerlink.com/index/10.1007/978-3-8348-9337-6},
year = {2010}
}
@article{Merker2003,
author = {Merker, G{\"{u}}nter and Schwarz, Christian and Stiesch, Gunnar and Otto, Frank},
journal = {Simul. der Verbrennung und Schadstoffbildung},
title = {{5 Ph{\"{a}}nomenologische Verbrennungsmodelle}},
year = {2003}
}
@article{Strd,
author = {Str, Methoden},
title = {{Omungssichtbarmachung}}
}
@article{Mizuno2009,
abstract = {This study examined a method of predicting the piston temperature in reciprocating internal combustion engines with the aim of developing lightweight pistons. Since the piston temperature is strongly affected by the in-cylinder temperature distribution and turbulence, it is necessary to consider the effects of flame propagation, cooling by the intake air, temperature rise due to combustion, in-cylinder flow and the combustion chamber shape. A three-dimensional combustion simulation that can take these effects into consideration was run to calculate the heat transfer coefficient from the piston crown surface and the gas temperature. The results were used as the boundary conditions for an analysis of heat transfer from the piston, and a method was thus developed for analyzing the piston temperature. The hardness method was used to obtain the piston temperature distribution and maximum temperature during engine operation, and a comparison was made with the analytical results to examine the effects of flame propagation.},
author = {Mizuno, Hideaki and Ashida, Koichi and Teraji, Atsushi and Ushijima, Kenshi and Takemura, Shinichi},
doi = {10.4271/2009-01-0187},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2009{\_}Mizuno{\_}Transient Analysis of the Piston Temperature with Measurement and Simulation.pdf:pdf},
isbn = {9200901018},
issn = {1946-3944},
journal = {SAE Int. J. Engines},
number = {1},
pages = {187--2009},
title = {{Transient Analysis of the Piston Temperature with Consideration of In-cylinder Phenomena Using Engine Measurement and Heat Transfer Simulation Coupled with Three-dimensional Combustion Simulation}},
url = {http://papers.sae.org/2009-01-0187/},
volume = {2},
year = {2009}
}
@article{Begriff,
author = {Begriff, Der},
pages = {144--162},
title = {{8 Ausgleichsvorg{\{}{\"{a}}{\}}nge in linearen Netzen}}
}
@article{Ottomotor1989,
author = {Ottomotor, Den},
pages = {29--115},
title = {{3 Gemischbildungs- und Verbrennungsverfahren}},
year = {1989}
}
@article{Betrachtungen,
author = {Betrachtungen, Allgemeine},
title = {{in viskosit ¨ atsfreien Fluiden}}
}
@article{Nenngro,
author = {Nenngro, Mit Den},
pages = {118--124},
title = {{16 Riementriebe}}
}
@article{Steffan1988,
author = {Steffan, Hermann and Moser, Andreas and Burg, Heinz and Dynamik, Die and Mechanik, Der},
journal = {Comput. (Long. Beach. Calif).},
pages = {171--216},
title = {{A6 A6 Kinetik A6}},
year = {1988}
}
@article{Bueno2005,
abstract = {The strain relaxation behaviour after full stress removals during creep of RR-58 Hiduminium alloy has been observed. Creep tests were carried out at 180 ??C, with stresses of 120, 170 and 230 MPa. Tests involved a series of unloading cycles after different creep periods involving the primary and secondary creep stages. The results were interpreted according to a model based on the thermally activated unbowing of dislocation segments. Activation parameters were calculated and an interpretation of the phenomena is made in terms of microstructural details of the material. The appearance of the fast and slow anelastic creep stages may be just a consequence of the high non-linearity existing between the line tension and the area swept by the segments during their unbowing movement. ?? 2005 Elsevier B.V. All rights reserved.},
author = {Bueno, Levi O and Bell, R L},
doi = {10.1016/j.msea.2005.08.055},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Kriechen{\_}Spannungsrelaxation/2005{\_}Bueno{\_}Anelastic creep behaviour of RR-58 aluminum alloy at 180-Phenomenological aspects and analysis based on dislocations.pdf:pdf},
isbn = {0921-5093},
issn = {09215093},
journal = {Mater. Sci. Eng. A},
keywords = {Anelastic creep,Creep recovery,Dislocation unbowing,RR-58 aluminium alloy},
pages = {72--78},
title = {{Anelastic creep behaviour of RR-58 aluminum alloy at 180 ??C: Phenomenological aspects and analysis based on the unbowing of dislocation segments}},
volume = {410-411},
year = {2005}
}
@article{Verger2002a,
abstract = {This paper presents a global approach of thermomechanical design in the automotive industry. The three steps of the method are the following: the loading definition, the modelling of the constitutive law, a failure criterion. Cracked area and lifetime prediction are described in the case of aluminium alloy cylinder heads submitted to transient thermal loadings. The main hypothesis and modelling choices are presented and results are illustrated by a series of computations on real 3D structures. {\{}{\textcopyright}{\}} 2002 Elsevier Ltd. All rights reserved.},
author = {Verger, L and Constantinescu, A and Charkaluk, E},
doi = {10.1016/S1566-1369(02)80087-5},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Kriechen{\_}Spannungsrelaxation/2002{\_}Verger{\_}THERMOMECHANICAL FATIGUE DESIGN OF ALUMINIUM COMPONENTS.pdf:pdf},
issn = {15661369},
journal = {Eur. Struct. Integr. Soc.},
number = {C},
pages = {309--318},
title = {{Thermomechanical fatigue design of aluminium components}},
volume = {29},
year = {2002}
}
@article{Forest2009,
abstract = {A unifying thermomechanical framework is presented that reconciles several classes of gradient elastoviscoplasticity and damage models proposed in the literature during the last 40 years. It is based on the introduction of the micromorphic counterpart ϕ $\chi$ of a selected ... $\backslash$n},
author = {Forest, Samuel},
doi = {10.1061/(ASCE)0733-9399(2009)135:3(117)},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/2009{\_}Forest{\_}Micromorphic Approach for Gradient Elasticity Viscoplasticity and Damage.pdf:pdf},
isbn = {0733-9399},
issn = {0733-9399},
journal = {J. Eng. Mech.},
number = {3},
pages = {117--131},
title = {{Micromorphic Approach for Gradient Elasticity, Viscoplasticity, and Damage}},
volume = {135},
year = {2009}
}
@article{Papula2011a,
author = {Papula, Lothar},
doi = {10.1007/978-3-8348-8285-1},
isbn = {9783834882851},
journal = {Math. f{\"{u}}r Ingenieure und Naturwissenschaftler Band 1},
pages = {422--569},
title = {{V Integralrechnung 1}},
year = {2011}
}
@article{Journal2008,
author = {Journal, American and Sciences, Applied and Publications, Science},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Heat transfer intake+exhaust system/2008{\_}Semin+Ismail{\_}Heat Transfer Investigation of Intake Port Engine Based on Steady-State and Transient Simulation.pdf:pdf},
keywords = {compression ignition engine,computational model,heat transfer,intake port,simulation},
number = {11},
pages = {1572--1579},
title = {{Heat Transfer Investigation of Intake Port Engine Based on Steady-State and Transient Simulation Semin , 2 Abdul Rahim Ismail , 2 Rosli Abu Bakar and 2 Ismail Ali Institute of Technology Sepuluh Nopember , Surabaya 60111 , Indonesia Faculty of Mechanical }},
volume = {5},
year = {2008}
}
@article{Singer1977,
abstract = {The aluminum alloy investigated contained about 2. 7{\%} Cu, 1. 6{\%} Mg, 1. 1{\%} Fe, 1{\%} Ni, and small amounts of Si, Zn, and Ti. Creep at 473 K resulted in deformation-induced softening because of microstructural instability. Creep tests at varied stresses and temperatures were performed to explore the dislocation mechanisms during creep in specimens subjected to 13 different thermomechanical treatments. It was found that the room temperature yield stress and creep resistance after prolonged creep stressing can be improved by preliminary deformation, whereas the initial creep resistance is decreased. This is explained in terms of the effect of deformation on the structure and its stability.},
author = {Singer, Robert and Blum, Wolfgang},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Empirical Fatigue Models + Validation/1975{\_}Blum{\_}The influence of thermomechanical treatment on the creep resistance of RR58 - Al2618.pdf:pdf},
issn = {00443093},
journal = {Zeitschrift fuer Met. Res. Adv. Tech.},
number = {5},
title = {{Influence of Thermomechanical Treatments on the Creep Resistance of Rr 58 At Elevated Temperature.}},
volume = {68},
year = {1977}
}
@article{Modell,
author = {Modell, Diskretes and Modell, Kontinuierliches and Vorgehensweise, Von Der},
journal = {Mechanik},
pages = {1--10},
title = {{1 Einf{\{}{\"{u}}{\}}hrung}}
}
@article{Polak2014,
abstract = {Experimental data on the formation of persistent slip markings (PSMs) at the egressing persistent slip bands (PSBs) and physically based models of surface relief formation and fatigue crack initiation are surveyed. The original Pol{\{}{\'{a}}{\}}k's model of fatigue crack initiation based on the formation, migration and annihilation of vacancy-type defects in PSBs is further refined and extended by taking into consideration the annihilation of vacancies in the matrix and the formation of internal stresses. The proposed mechanisms of surface relief formation are based on the plastic relaxation of internal compression stresses in PSBs and internal tensile stresses in the matrix. By solving the migration of vacancies from the PSB and their annihilation in the matrix, the shapes of extrusion and parallel intrusions are derived analytically under some simplifying assumptions. {\{}{\textcopyright}{\}} 2013 Elsevier B.V.},
author = {Pol{\'{a}}k, J and Man, J},
doi = {10.1016/j.msea.2013.12.005},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/2014{\_}Polak+Man{\_}Mechanisms of extrusion and intrusion formation in fatigued crystalline materials.htm.pdf:pdf},
issn = {09215093},
journal = {Mater. Sci. Eng. A},
keywords = {Crack initiation,Extrusion,Fatigue,Intrusion,Persistent slip band (PSB)},
pages = {15--24},
publisher = {Elsevier},
title = {{Mechanisms of extrusion and intrusion formation in fatigued crystalline materials}},
url = {http://dx.doi.org/10.1016/j.msea.2013.12.005},
volume = {596},
year = {2014}
}
@article{Fs2013,
author = {Fs},
doi = {10.1007/978-1-4614-0502-3},
isbn = {2009004043},
number = {1},
pages = {0--10},
title = {{Chapter 0}},
year = {2013}
}
@article{Festigkeit,
author = {Festigkeit, Die and Verformung, Die and Zug, Im and Aktivierung, Die and Po-, Ein},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Werkstoffkunde/Quantitative Verfestigungsmechanismen.pdf:pdf},
title = {{13.1 Verformung und Verfestigung von Polykristallen}}
}
@article{Hinblick2000,
author = {Hinblick, Im},
pages = {3--8},
title = {{Einleitung}},
year = {2000}
}
@article{Clausert,
author = {Clausert, H. and Mathis, W. and Hoffmann, K. and Wiesemann, G. and Z{\"{u}}rneck, H.},
journal = {H{\"{u}}tte},
pages = {1--180},
title = {{G-Elektrotechnik}}
}
@article{Cadden1998,
author = {Cadden, Jerry L and Sadesky, Paul F},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/{\_}buecherSong/HandbookofComposites/II/25{\_}ToolingforComposites.pdf:pdf},
journal = {Handb. Compos.},
title = {{Tooling for composites}},
year = {1998}
}
@article{Getriebelehre,
author = {Getriebelehre, Der},
title = {{3 Kinematische Analyse der Radf{\"{u}}hrungen}}
}
@article{Hill1952a,
abstract = {The connection between the elastic behaviour of an aggregate and a single crystal is considered, with special reference to the theories of Voigt, Reuss, and Huber and Schmid. The elastic limit under various stress systems is also considered, in particular, it is shown that the tensile elastic limit of a face-centred aggregate cannot exceed two-thirds of the stress at which pronounced plastic distortion occurs.},
author = {Hill, R},
doi = {10.1088/0370-1298/65/5/307},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/Strukturmechanik MMS/Literatur/Hill 1952.pdf:pdf},
isbn = {0370-1298},
issn = {0370-1298},
journal = {Proc. Phys. Soc. Sect. A},
number = {5},
pages = {349--354},
title = {{The Elastic Behaviour of a Crystalline Aggregate}},
url = {http://stacks.iop.org/0370-1298/65/i=5/a=307?key=crossref.630b67f122246b4defcc5fda55c7bf20},
volume = {65},
year = {1952}
}
@article{Wasserenergie,
author = {Wasserenergie, Nutzbare},
doi = {10.1007/978-3-8348-2279-6},
isbn = {9783834822796},
pages = {215--235},
title = {{11 Wasserkraftwerke}}
}
@article{Berger2003a,
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Berger},
doi = {10.1002/ejoc.201200111},
eprint = {arXiv:1011.1669v3},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Vortraege/Book-of-Abstracts{\_}2016-03-04{\_}GAMM.pdf:pdf},
isbn = {9781107671812},
issn = {0196-6553},
journal = {Eng. Med. Biol. Soc. 2008. EMBS 2008. 30th Annu. Int. Conf. IEEE},
pages = {2004},
pmid = {26840611},
title = {{Table of of contents}},
volume = {24},
year = {2003}
}
@book{Davies2008,
abstract = {Texture analysis is one of the fundamental aspects of human vision by which we discriminate between surfaces and objects. In a similar manner, computer vision can take advantage of the cues provided by surface texture to distinguish and recognize objects. In computer vision, texture analysis may be used alone or in combination with other sensed features (e.g. color, shape, or motion) to perform the task of recognition. Either way, it is a feature of paramount importance and boasts a tremendous body of work in terms of both research and applications. Currently, the main approaches to texture analysis must be sought out through a variety of research papers. This collection of chapters brings together in one handy volume the major topics of importance, and categorizes the various techniques into comprehensible concepts. The methods covered will not only be relevant to those working in computer vision, but will also be of benefit to the computer graphics, psychophysics, and pattern recognition communities, academic or industrial.},
author = {Davies, E. R.},
booktitle = {Handb. Texture Anal.},
doi = {interface shear stre},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Engler, Randle - 2010 - Introduction to texture analysis.pdf:pdf},
isbn = {978-1-84816-115-3},
issn = {04515994},
pages = {1--31},
pmid = {15680927},
title = {{Introduction to Texture Analysis}},
year = {2008}
}
@article{Fara-2006,
author = {Fara-, Michael and Maxwell, James Clerk},
journal = {Gerthsen Phys.},
pages = {379--445},
title = {{07 - Elektrodynamik}},
year = {2006}
}
@book{Meister2011b,
abstract = {Die wichtigsten Verfahren zur numerischen L{\{}{\"{o}}{\}}sung von linearen Gleichungssystemen in einer umfassenden Einf{\{}{\"{u}}{\}}hrung, die zum Verst{\{}{\"{a}}{\}}ndnis nur geringe mathematische Vorkenntnisse ben{\{}{\"{o}}{\}}tigt. Behandelt werden sowohl die direkten als auch die iterativen Verfahren, wobei der Autor gro{\{}{\ss}{\}}en Wert auf eine sorgf{\{}{\"{a}}{\}}ltige Herleitung dieser Verfahren legt. Au{\{}{\ss}{\}}erdem sind sehr detaillierte Pseudocodes enthalten, mit deren Hilfe sich die jeweiligen Verfahren in einer beliebigen Programmiersprache sofort auf dem Computer realisieren lassen. Das Lehrbuch ist auch f{\{}{\"{u}}{\}}r Natur- und Ingenieurwissenschaftler geeignet, die in vielen praktischen Anwendungen mit der L{\{}{\"{o}}{\}}sung von linearen Gleichungssystemen konfrontiert sind.},
archivePrefix = {arXiv},
arxivId = {1011.1669v3},
author = {Meister, Andreas},
booktitle = {Matrix},
doi = {10.1007/978-3-8348-8100-7},
eprint = {1011.1669v3},
isbn = {978-3-8348-1550-7},
issn = {1098-6596},
pages = {36--68},
pmid = {25246403},
title = {{Numerik linearer Gleichungssysteme}},
url = {http://link.springer.com/10.1007/978-3-8348-8100-7},
year = {2011}
}
@article{Papula2009e,
author = {Papula, Lothar},
journal = {Math. Formelsammlung},
pages = {24},
title = {{XIII Laplace-Transformationen 1}},
year = {2009}
}
@article{Uberschlagsunfalle,
author = {{\"{U}}berschlagsunf{\"{a}}lle, A},
pages = {451--460},
title = {{A15 A15 {\"{U}}berschlagsunf{\"{a}}lle}}
}
@inproceedings{Taler2017,
author = {Taler, Dawid and Taler, Jan},
booktitle = {E3S Web Conf.},
doi = {https://doi.org/10.1051/e3sconf/20171302008},
file = {:C$\backslash$:/Users/p327208/Desktop/Promotion/Literature/Motorspezifisch/Heat transfer intake+exhaust system/2017{\_}Taler{\_}Simple heat transfer correlations for turbulent tube flow.pdf:pdf},
title = {{Simple heat transfer correlations for turbulent tube flow}},
volume = {13},
year = {2017}
}
@article{Schmitt2006,
author = {Schmitt, J{\"{u}}rgen and Isermann, Ralf},
journal = {Fahrdynamik-Regelung},
pages = {365--375},
title = {{Entwicklungsumgebung mit echtzeitf{\{}{\"{a}}{\}}higen Gesamtfahrzeugmodellen f{\{}{\"{u}}{\}}r sicherheitsrelevante Fahrerassistenzsysteme}},
year = {2006}
}
@article{Federung,
author = {Federung, Aufgaben Der},
title = {{5 Federung und D{\{}{\"{a}}{\}}mpfung}}
}
@article{Brecq2005,
abstract = {High frequency pressure oscillations are generated under knocking conditions within the combustion chamber of Spark Ignition engines. Although acoustic-oscillation model can give the natural frequencies of these oscillations, very few mathematical models are today available, in scientific literature, to describe the oscillation deadening effect. An analytical formulation of the deadening has been highlighted. Analytical solution has been established for future ECU implementation. Coupling this new concept and an existing high-frequency model, an achieved model of the knocking pressure high frequencies is compared to experimental data. Good behavior is obtained on a natural gas fuelled spark ignition engine.},
author = {Brecq, G and {Le Corre}, O},
doi = {10.4271/2005-01-1126},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2005{\_}Brecq{\_}Modeling of In-cylinder Pressure Oscillations under Knocking conditions - Intro to Pressure Envelope Curve.pdf:pdf},
isbn = {2005011126},
issn = {0148-7191},
title = {{Modeling of In-cylinder Pressure Oscillations under Knocking Conditions: Introduction to Pressure Envelope Curve}},
url = {http://papers.sae.org/2005-01-1126/},
year = {2005}
}
@article{Wimmer2000c,
abstract = {This paper summarizes the results of several investigations on in-cylinder heat transfer during high-pressure and gas exchange phases as well as heat transfer in the inlet and outlet ports for a number of different engine types (DI Diesel, SI and gaseous fueled engine). The paper contains a comparision of simulation results and experimental data derived from heat flux measurements. Numerical results were obtained from zero-, one- and three-dimensional simulation methods. Time and spatially resolved heat fluxes were measured applying the surface temperature method and special heat flux sensors. The paper also includes an assessment of different sensor types with respect to accuracy and applicability.ER -},
author = {Wimmer, Andreas and Pivec, Robert and Sams, Theodor},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2000{\_}Wimmer{\_}Heat Transfer to the Combustion Cahmber and Port Walls of IC Engines - Measurement and Prediction.pdf:pdf},
number = {724},
title = {{Heat Transfer to the Combustion Chamber and Port Walls of IC Engines - Measurement and Prediction}},
year = {2000}
}
@article{Le2012a,
author = {Le, K C},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2012{\_}Le{\_}Continuum dislocation theory-size effects and formation of microstructure{\_}Lecture Bad Herrenalb.pdf:pdf},
title = {{Continuum dislocation theory : size effects and formation of microstructure}},
year = {2012}
}
@article{Eekoye1996,
abstract = {Heat-transfer rates present in an engine cylinder undergoing knock are known to be larger than the rates associated with normal engine operation. Further, at the time of knock, the largest heat fluxes are associated with locations on the cylinder wall where the flame is locally quenching. In this study, heat-transfer processes at the flame-wall interface during a knock event are investigated computationally and analytically. Computationally, the governing equations for a one-dimensional, flame-quenching event are solved using a reduced chemical reaction mechanism. Analytically, scaling relations for the flame heat-release rates are used in the governing equations to determine the heat-transfer rates. It is found that while pressure transients modify the wall heat flux, the absolute value of the pressure is the most significant parameter in predicting the maximum heat flux. The wall heat flux profiles are predicted for both the analytical and computational models. In the range of pressures examined, a linear relationship was found between the peak flux and pressure, both for the computational and analytical models. The linear relationship between the pressure and peak flux was found to be invalid when the flame-quenching process was disrupted by the pressure fluctuations for pressure oscillations with a characteristic time on the order of the quenching process. ?? 1996 Combustion Institute.},
author = {Eekoye, O. A.},
doi = {10.1016/S0082-0784(96)80101-9},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/1996{\_}Ezekoye{\_}Heat transfer modeling during knock and flame quenching in an engine chamber.pdf:pdf},
isbn = {0082-0784},
issn = {00820784},
journal = {Symp. Combust.},
number = {2},
pages = {2661--2668},
title = {{Heat transfer modeling during knock and flame quenching in an engine chamber}},
volume = {26},
year = {1996}
}
@article{Bradley1996,
abstract = {Net chemical heat-release rates have been estimated experimentally, throughout the combustion, from a single-cylinder gasoline engine, running on paraffinic and aromatic fuels. These rates are compared for autoigniting and nonautoigniting cycles and, by means of a differencing procedure, the heat release rate due to autoignition found. Comparison of heat release rates in the propagating flame and in autoignition show that in knocking combustion, almost half the total energy release can occur in autoignition. Pressures were measured with transducers and gas temperatures prior to autoignition by the CARS technique. The measurements enabled volumetric autoignition heat release rates to be obtained. When plotted against the reciprocal temperature of the unburned gas just prior to autoignition, an activation temperature and Arrhenius constant were obtained for each fuel in a single global expression for the autoignition heat release rate. These constants are reexpressed in terms of the actual temperature and fuel concentration to give a more accurate kinetic representation. This is used in an analysis of the conditions necessary for the pressure wave generated at autoignition to couple with the chemical kinetics sufficiently to lead to a developing detonation. At the inception of knock, for the same temperatures and pressures, the maximum autoignition heat release rates for the paraffinic fuel are two to three times those for the aromatic fuel. Because of this, the paraffinic fuel is more prone to developing detonation than is the aromatic fuel. ?? 1996 Combustion Institute.},
author = {Bradley, D. and Kalghatgi, G. T. and Golombok, M. and Yeo, Jinku},
doi = {10.1016/S0082-0784(96)80100-7},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Klopfen{\_}Ottomotor/1996{\_}Bradley{\_}HEAT RELEASE RATES DUE TO AUTOIGNITION AND THEIR RELATIONSHIP TO KNOCK INTENSITY IN SI ENGINES.pdf:pdf},
isbn = {00820784},
issn = {00820784},
journal = {Symp. Combust.},
number = {2},
pages = {2653--2660},
title = {{Heat release rates due to autoignition, and their relationship to knock intensity in spark ignition engines}},
volume = {26},
year = {1996}
}
@article{Cantrell2009a,
author = {Cantrell, John H},
doi = {10.1063/1.3254223},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2009{\_}Cantrell{\_}Ultrasonic harmonic generation from fatigue-induced dislocation substructures in planar slip metals and assessment of remaining fatigue life.pdf:pdf},
issn = {00218979},
journal = {J. Appl. Phys.},
number = {9},
title = {{Ultrasonic harmonic generation from fatigue-induced dislocation substructures in planar slip metals and assessment of remaining fatigue life}},
volume = {106},
year = {2009}
}
@article{Wirkung2011,
author = {Wirkung, Funktion},
doi = {10.1007/978-3-8348-8279-0},
isbn = {9783834882790},
pages = {653--672},
title = {{19 Dichtungen 19.1}},
year = {2011}
}
@article{Sangid2011,
abstract = {In this paper, we construct a model for prediction of fatigue crack initiation based on the material's microstructure. In order to do so, the energy of a persistent slip band (PSB) is monitored and an energy balance approach is taken, in which cracks initiate and the material fails due to stress concentration from a PSB (with respect to dislocation motion). These PSBs are able to traverse low-angle grain boundaries (GB), thus belonging to clusters of grains. As a consequence of the ongoing cyclic slip process, the PSBs evolve and interact with high-angle GBs, the result of which leads to dislocation pile-ups, static extrusions in the form of ledges/steps at the GB, stress concentration, and ultimately crack initiation. Hence, this fatigue model is driven by the microstructure, i.e. grain orientations, widely distributed grain sizes, precipitates, PSB-GB interactions, as well as the affect of neighboring grains. The results predict that cracks initiate near twin boundaries from PSBs spanning a single large grain with a favorable orientation or multiple grains connected by low-angle GBs. Excellent agreement is shown between model predictions and experimental data. ?? 2010 Elsevier Ltd. All rights reserved.},
author = {Sangid, Michael D and Maier, Hans J and Sehitoglu, Huseyin},
doi = {10.1016/j.ijplas.2010.09.009},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/2011{\_}Sangid{\_}The role of grain boundaries on fatigue crack initiation - An energy approach.pdf:pdf},
isbn = {0749-6419},
issn = {07496419},
journal = {Int. J. Plast.},
keywords = {Energy methods,Fatigue,Grain boundaries,Persistent slip bands,Polycrystalline material},
number = {5},
pages = {801--821},
publisher = {Elsevier Ltd},
title = {{The role of grain boundaries on fatigue crack initiation - An energy approach}},
url = {http://dx.doi.org/10.1016/j.ijplas.2010.09.009},
volume = {27},
year = {2011}
}
@article{Vergleicha,
author = {Vergleich, Im},
title = {{9. Versuchsanlagen}}
}
@article{Mutzke2016a,
abstract = {{\textcopyright} 2016 SAE International.Knocking combustion places a major limit on the performance and efficiency of spark ignition engines. Spontaneous ignition of the unburned air-fuel mixture ahead of the flame front leads to a rapid release of energy, which produces pressure waves that cause the engine structure to vibrate at its natural frequencies and produce an audible 'pinging' sound. In extreme cases of knock, increased temperatures and pressures in the cylinder can cause severe engine damage. Damage is thought to be caused by thermal strain effects that are directly related to the heat flux. Since it will be the maximum values that are potentially the most damaging, then the heat flux needs to be measured on a cycle-by-cycle basis. Previous work has correlated heat flux with the pressure fluctuations on an average basis, but the work here shows a correlation on a cycle-by-cycle basis. The in-cylinder pressure and surface temperature were measured using a pressure transducer and eroding-type thermocouple. These sensors were installed side-by-side at the surface of the cylinder in order to investigate the relationship between knock and heat flux on a cycle-by-cycle basis. A finite difference method was implemented to solve the one-dimensional unsteady heat conduction equation and calculate the temperature distribution away from the surface of the combustion chamber, and thus the instantaneous heat flux. The knock intensity was varied by controlling the fuel quality, compression ratio, ignition timing and air-fuel ratio. The measured heat flux was compared with pressure-based knock indices and it was found that as knock intensity increases, the correlation with peak heat flux became stronger. Results from different fuels and engine operating conditions did not collapse onto the same trend line. At higher speeds and higher compression ratios the heat flux was higher at a given level of knock intensity. The co-location of the pressure transducer and heat flux sensor meant that a correlation was found on a cycle-by-cycle basis.},
author = {Mutzke, J. and Scott, B. and Stone, R. and Williams, J.},
doi = {10.4271/2016-01-0700},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2016{\_}Mutzke{\_}The Effect of Combustion Knock on the Instantaneous Heat Flux in Spark Ignition Engines.pdf:pdf},
journal = {SAE Tech. Pap.},
title = {{The Effect of Combustion Knock on the Instantaneous Heat Flux in Spark Ignition Engines}},
volume = {2016-April},
year = {2016}
}
@article{Anforderungen,
author = {Anforderungen, Fahrzeuggetriebetypische},
journal = {Auslegung A Grad. J. Philos.},
title = {{8 Auslegung und Gestaltung von Wellen}}
}
@article{Muller,
author = {M{\"{u}}ller, Rolf},
isbn = {9783834800183},
journal = {Antriebstechnik},
title = {{Aus dem Programm Automatisierungstechnik}}
}
@inproceedings{Shayler2005,
abstract = {The paper reports the design of a model and HIL system produced to support the development and testing of Electronic Control Unit/Engine Management System (ECU/EMS) software for a V6 turbo-charged automotive diesel engine. The engine model, developed in Simulink, is compiled to execute on a dSpace platform and interacts with the ECU/EMS module in real time. The main features of the engine model are outlined. The configuration of the model and HIL components are described, and the performance of the system is illustrated and discussed. Practical decisions on the inclusion of real or virtual sensors and actuators, and other implementation issues, are explained. Recent and potential future applications of the system are described.},
author = {Shayler, P J and Allen, A J and Roberts, A L},
booktitle = {SAE 2005 World Congr. Exhib.},
doi = {10.4271/2005-01-0056},
month = {apr},
publisher = {SAE International},
title = {{Running Real-Time Engine Model Simulation with Hardware-in-the-Loop for Diesel Engine Development}},
year = {2005}
}
@book{Haberhauer2014,
abstract = {Dieses bew{\"{a}}hrte Lehrbuch gibt einen fundierten {\"{U}}berblick {\"{u}}ber die wichtigsten Maschinenelemente. Der Leser lernt, die Funktionsweise moderner Maschinenteile zu verstehen, sie auszulegen und sicher anzuwenden. Das Buch enth{\"{a}}lt die aktuellen Berechnungsverfahren; es ist auf das Wesentliche konzentriert, gleichzeitig aber anwendungs- und praxisorientiert. F{\"{u}}r diese aktualisierte 17. Auflage wurden Normen aktualisiert und Beispiele erweitert. Insbesondere wurde das Kapitel „Schrauben“ {\"{u}}berarbeitet. Eine Formelsammlung und weitere Beispielaufgaben k{\"{o}}nnen aus dem Internet heruntergeladen werden.},
author = {Haberhauer, Horst and Bodenstein, Ferdinand},
doi = {10.1007/978-3-540-68612-5},
isbn = {9783642374166},
pages = {662},
title = {{Maschinenelemente: Gestaltung, Berechnung, Anwendung (Springer-Lehrbuch)}},
year = {2014}
}
@article{Mende2013,
author = {Mende},
isbn = {9192631770},
journal = {Phys. Gleichungen und Tabellen},
pages = {177--204},
title = {{Mechanik fester K{\"{o}}rper}},
year = {2013}
}
@article{Kratzsch2013b,
author = {Kratzsch, Matthias and G{\"{u}}nther, Michael},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Klopfen{\_}Ottomotor/4. Internationale Tagung Ottomotorisches Klopfen - Berlin 12{\_}2013/Knocking+in+Gasoline+Engines.pdf:pdf},
pages = {445},
title = {{Knocking in Gasoline Engines}},
year = {2013}
}
@article{Polak2014c,
abstract = {The role of point defects in the formation of surface relief and in the initiation of a fatigue crack in crystalline materials is analyzed. The dislocation interactions in the bands of intensive cyclic slip (persistent slip bands - PSBs) are specified and relations describing the formation and annihilation of interstitial and vacancy type defects in the channels of the ladder-like PSB are derived. The continuous formation, annihilation and primarily the migration of point defects are proposed to be responsible for the mass redistribution within PSB and between PSB and the PSB/matrix boundary. The redistribution of the matter results in local tensile and compressive stresses that are the sources of the principal irreversibility of slip within PSB. Local tensile and compressive stresses are relaxed by dislocation movement within PSB in the direction of the active Burgers vector and lead to the formation of characteristic surface relief in the form of extrusions and intrusions. The intrusions represent crack-like defects and fatigue cracks initiate in the tip of intrusions. {\textcopyright} 2013 Elsevier Ltd. All rights reserved.},
author = {Pol{\'{a}}k, Jaroslav and Man, Jiř{\'{i}}},
doi = {10.1016/j.ijfatigue.2013.10.016},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Kriechen{\_}Spannungsrelaxation/2014{\_}Polak+Man{\_}Fatigue crack initiation – The role of point defects.pdf:pdf},
isbn = {0142-1123},
issn = {01421123},
journal = {Int. J. Fatigue},
keywords = {Extrusion,Fatigue crack initiation,Intrusion,Persistent slip band (PSB),Point defects},
number = {July},
pages = {18--27},
title = {{Fatigue crack initiation - The role of point defects}},
volume = {65},
year = {2014}
}
@article{Marzullo1998,
author = {Marzullo, A},
isbn = {9780412540202},
journal = {Handb. Compos.},
pages = {156--168},
title = {{Boron, High Silica, Quartz and Ceramic Fibers}},
year = {1998}
}
@article{Sun2016b,
abstract = {Multi-scale fatigue model and image-based simulation method are developed in this study to describe collective short cracks evolution process in micro-scale and continuous fatigue damage evolution in macro-scale based on the concept of continuum damage mechanics (CDM). The relationship between the micro-scale and macro-scale fatigue is explored to enhance the understanding the nature of fatigue phenomenon. A case study is carried out to verify the developed multi-scale fatigue model and image-based simulation method. The results show that it is more effective and clear to reveal metal fatigue failure mechanisms from the viewpoint of multi-scale.},
author = {Sun, Bin and Xu, You Lin and Li, Zhaoxia},
doi = {10.1016/j.commatsci.2016.01.021},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/2 scale models papers/2016{\_}Sun+Lu{\_}Multi-scale fatigue model and image-based simulation of collective short cracks evolution process.pdf:pdf},
issn = {09270256},
journal = {Comput. Mater. Sci.},
keywords = {Damage,Fatigue,Image-based,Multi-scale,Short crack},
pages = {24--32},
publisher = {Elsevier B.V.},
title = {{Multi-scale fatigue model and image-based simulation of collective short cracks evolution process}},
url = {http://dx.doi.org/10.1016/j.commatsci.2016.01.021},
volume = {117},
year = {2016}
}
@book{Gross2011d,
author = {Gross, Dietmar and Seelig, Thomas},
doi = {10.1007/978-3-642-10196-0},
isbn = {978-3-642-10195-3},
title = {{Bruchmechanik}},
url = {http://link.springer.com/10.1007/978-3-642-10196-0},
year = {2011}
}
@article{Morris2007a,
author = {Morris, J W},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/Crystall Plasticity Basics/Morris{\_}Dislocation plasticity-AnOverview.pdf:pdf},
journal = {Introd. to Mater. Sci.},
pages = {1--36},
title = {{Dislocation Plasticity : Overview}},
url = {http://www.mse.berkeley.edu/groups/morris/MSE205/Extras/dislocation plasticity.pdf},
volume = {i},
year = {2007}
}
@article{L,
author = {L, Bei Der},
doi = {10.1007/978-3-642-24335-6},
isbn = {9783642243356},
title = {{6 Differenzenverfahren}}
}
@article{AntonT.2006,
author = {{Anton T.}, van Zanten},
doi = {10.1007/978-3-8348-9049-8_8},
isbn = {978-3-8348-0109-8},
journal = {Fahrdynamik Regelung},
pages = {169 -- 211},
title = {{8 Elektronisches Stabilit{\"{a}}tsprogramm (ESP)}},
url = {http://link.springer.com/chapter/10.1007/978-3-8348-9049-8{\_}8},
year = {2006}
}
@article{Kennametal2011,
author = {Kennametal},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/{\_}buecherSong/HandbookofComposites/II/27{\_}CompositeMachining.pdf:pdf},
pages = {34--55},
title = {{Composite machining}},
url = {www.kennametal.com},
year = {2011}
}
@article{Vorschriften,
author = {Vorschriften, Gesetzliche},
journal = {Betrieb},
pages = {243--259},
title = {{10 Ger{\{}{\"{a}}{\}}uschemissionen}}
}
@article{Corti2016,
abstract = {Recent trends in gasoline engines, such as downsizing, downspeeding and the increase of the compression ratio make knocking combustions a serious limiting factor for engine performance. A detailed analysis of knocking events can help improving the engine performance and diagnostic strategies. An effective way is to use advanced 3D Computational Fluid Dynamics (CFD) simulation for the analysis and prediction of the combustion process. The effects of Cycle to Cycle Variation (CCV) on knocking combustions are taken into account, maintaining a RANS (Reynolds Averaged Navier-Stokes) CFD approach, while representing a complex running condition, where knock intensity changes from cycle to cycle. The focus of the numerical methodology is the statistical evaluation of the local air-to-fuel and turbulence distribution at the spark plugs and their correlation with the variability of the initial stages of combustion. CFD simulations have been used to reproduce knock effect on the cylinder pressure trace. For this purpose, the CFD model has been validated, proving its ability to predict the combustion evolution with respect to SA variations, from non-knocking up to heavy knocking conditions. The pressure traces simulated by the CFD model are then used to evaluate cylinder pressure-based knock indexes. Since the model is able to output other knock intensity tracers, such as the mass of fuel burned in knocking mode, or the local heat transferred to the piston, knock indexes based on the cylinder pressure trace can be related to parameters only available in a simulation environment, that are likely to be more representative of the actual knock intensity, with respect to the local pressure trace for the sensor position. The possibility of simulating hundredths of engine cycle allows using the methodology to compare the indexes quality (correlation with actual knock intensity) on a statistical base.},
author = {Corti, Enrico and Forte, Claudio and Cazzoli, Giulio and Moro, Davide and Falfari, Stefania and Ravaglioli, Vittorio},
doi = {10.1016/j.egypro.2016.11.116},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Klopfen{\_}Ottomotor/2016{\_}Corti{\_}Comparison of knock indexes based on CFD analysis.pdf:pdf},
issn = {18766102},
journal = {Energy Procedia},
keywords = {CFD,Knock,Sensor position,Simulation},
number = {September},
pages = {917--924},
publisher = {The Author(s)},
title = {{Comparison of Knock Indexes Based on CFD Analysis}},
url = {http://dx.doi.org/10.1016/j.egypro.2016.11.116},
volume = {101},
year = {2016}
}
@book{Gross2011,
author = {Gross, Dietmar and Seelig, Thomas},
doi = {10.1007/978-3-642-10196-0},
isbn = {978-3-642-10195-3},
title = {{Bruchmechanik}},
url = {http://link.springer.com/10.1007/978-3-642-10196-0},
year = {2011}
}
@article{Winkler2014,
author = {Winkler, N},
doi = {10.1177/1468087414544899},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2015{\_}Winkler{\_}Effect of pressure oscillations on in-cylinder heat transfer  - through LES Simulation.pdf:pdf},
isbn = {1468087414544},
issn = {1468-0874},
journal = {Int. J. Engine Res.},
keywords = {24 june 2014,6 march 2014,accepted,computational fluid dynamics,date received,heat transfer,internal combustion engines,large eddy simulation,pressure oscillations},
number = {6},
pages = {705--715},
title = {{Effect of pressure oscillations on in-cylinder heat transfer - through large eddy simulation}},
url = {http://jer.sagepub.com/lookup/doi/10.1177/1468087414544899},
volume = {16},
year = {2014}
}
@article{Zech2005,
author = {Zech, Michael},
doi = {10.1002/best.200590286},
journal = {Beton- und Stahlbetonbau},
number = {2},
pages = {81--246},
title = {{Krafteinleitung }},
volume = {100},
year = {2005}
}
@article{Hernandez2010a,
author = {Hern{\'{a}}ndez, Abarca},
doi = {10.1002/cbdv.201090012},
issn = {1612-1880},
journal = {Chem. Biodivers.},
number = {12},
pages = {2963--80},
pmid = {21162009},
title = {{Author index.}},
url = {http://www.ncbi.nlm.nih.gov/pubmed/21162009},
volume = {7},
year = {2010}
}
@article{Polyacrylic,
author = {Polyacrylic, A C M},
title = {{Index Terms A}}
}
@article{Gurtin1967,
author = {Gurtin, Morton E and Williams, William O},
doi = {10.1007/BF00285676},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Thermodynamik/An Axiomatic Foundation for Continuum Thermodynamics{\_}CommunicatedByNoll.pdf:pdf},
issn = {00039527},
journal = {Arch. Ration. Mech. Anal.},
number = {2},
pages = {83--117},
title = {{An axiomatic foundation for continuum thermodynamics}},
volume = {26},
year = {1967}
}
@article{Einf1999,
author = {Einf, Seit and Reaktion, Als},
number = {C},
pages = {238--270},
title = {{7 Kraftstoff und Schmier{\"{o}}l}},
year = {1999}
}
@article{Finol2006a,
abstract = {Over the last 40 years, several empirical correlations have been developed to estimate heat fluxes from the combustion chambers of internal combustion engines. Some of these expressions are based on correlations to compute the Nusselt number for forced convection in turbulent flow inside circular tubes. The fundamental suitability of this kind of empirical model in representing the highly complex processes of in-cylinder heat transfer is questionable, but in practice the models have steadily improved owing to contributions from numerous investigators. Other correlations have a less theoretical basis than those of the Nusselt number form. Formulae of this type have been obtained from the application of simple statistical techniques to large datasets, taking into account several engine operational parameters and engine types. The resulting correlations provide reasonable estimates but perform poorly when extrapolated or applied to novel concepts. In this paper, the most important correlations are reviewed against the features of a modern diesel engine, and research requirements for future modelling developments are identified and discussed. {\textcopyright} IMechE 2006.},
author = {Finol, C A and Robinson, K},
doi = {https://doi.org/10.1243/09544070JAUTO202},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2006{\_}Finol{\_}Thermal modelling of modern engines - A review of empirical correlations to estimate the in-cylinder heat transfer coefficient .pdf:pdf},
journal = {Proc. Inst. Mech. Eng. Part D J. Automob. Eng.},
keywords = {cient,heat flux,heat transfer coe ffi,in-cylinder heat transfer models},
number = {12},
pages = {1765--1781},
title = {{Thermal modelling of modern engines: a review of empirical correlations to estimate the in-cylinder heat transfer coefficient}},
volume = {220},
year = {2006}
}
@article{Albers,
author = {Albers, Albert and Grundlagen, Allgemeine},
title = {{Kapitel 5}}
}
@article{Kaunea,
author = {Kaune, Vanessa and Janda, Daniel and Schliephake, Daniel},
journal = {TU Darmstadt},
pages = {6},
title = {{Aush{\{}{\"{a}}{\}}rtung von Aluminiumlegierungen}},
url = {http://www.mawi.tu-darmstadt.de/media/phm/5semester/ausscheidungshrtungiv.pdf}
}
@article{McKelvey2012,
abstract = {The process of prevention of failure from structural fatigue is a process that should take place during the early development and design phases of a structure. In the ground vehicle industry, for example, the durability specifications of a new product are directly interweaved with the desired perfor-mance characteristics, materials selection, manufacturing methods, and safety characteristics of the vehicle. In the field of fatigue and durability analysis of materials, three main tech-niques have emerged: nominal stress-based analysis, local strain-based analysis, and fracture mechanics analysis. Each of these methods has their own strengths and domain of applica-bility—for example, if an initial crack or flaw size is known to exist in a structure, a fracture mechanics approach can give a meaningful estimate of the number of cycles it takes to prop-agate the initial flaw to failure. The development of the local strain-based fatigue analysis approach has been used to great success in the automotive industry, particularly for the analysis of measured strain time histories gathered during proving ground testing or customer usage. However, the strain life approach is dependent on specific material properties data and the ability to measure (or calculate) a local strain history. His-torically, the stress-based fatigue analysis approach was developed first—and is sometimes considered an ''old'' approach—but the stress-based fatigue analysis methods have been continued to be developed. The major strengths of this approach include the ability to give both quantitative and qualitative estimates of fatigue life with minimal estimates on stress levels and material properties, thus making the stress-based approach very relevant in the early design phase of structures where uncertainties regarding material selection, manufacturing processes, and final design specifications may cause numerous design iterations. This article explains the FKM-Guideline approach to stress-based uniaxial fatigue analysis. The Forschungskuratorium Maschinenbau (FKM) was developed in 1994 in Germany and has since continued to be updated. The guideline was developed for the use of the mechanical engineering community involved in the design of machine components, welded joints, and related areas. It is our desire to make the failure prevention and design community aware of these guidelines through a thorough explanation of the method and the application of the method to detailed examples.},
author = {McKelvey, Sean A. and Lee, Yung Li and Barkey, Mark E.},
doi = {10.1007/s11668-012-9599-4},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Werkstoffkunde/2012{\_}McKelvey-Lee-Barkey{\_}Stress-Based Uniaxial Fatigue Analysis Using Methods Described in FKM.pdf:pdf},
issn = {15477029},
journal = {J. Fail. Anal. Prev.},
keywords = {Durability analysis,Failure prevention,Stress-based fatigue analysis,Structural fatigue,Surface finish effect},
number = {5},
pages = {445--484},
title = {{Stress-based uniaxial fatigue analysis using methods described in FKM-guideline}},
volume = {12},
year = {2012}
}
@book{Taylor2005,
author = {Taylor, R.L. and Zienkiewicz, O.C.},
booktitle = {Int. J. Numer. Methods Eng.},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/B{\"{u}}cher{\_}Sammlung{\_}ITM/The Finite Element Method - O.C. Zienkiewicz {\&} R.L. Taylor/The-Finite-Element-Method.pdf:pdf},
isbn = {9780750663212},
pages = {1863},
title = {{The Finite Element Method for Solid and Structural Mechanics}},
year = {2005}
}
@article{Carta2013,
abstract = {This paper describes the propagation of an edge crack in a structured thermoelastic solid. A rapid change of temperature, represented by a time-periodic series of high-gradient temperature pulses, is applied at the boundary of the structured solid. A lattice approximation is employed in the model analysis discussed here. In order to describe the crack advance through the lattice a failure criterion is imposed, whereby the links break as soon as they attain a critical elastic elongation. The elongations of the links are produced both by a variation in temperature and by elastic waves generated at the boundary due to thermal shocks, as well as waves created by the propagating crack through the breakage of the elastic ligaments. The analysis is compared to the quasi-static and dynamic models of thermal striping in thermally loaded solids containing edge cracks. The emphasis is on the effect of the structure on the crack trapping. The nonlinear simulations presented in this paper show that the average speed of crack propagation can be estimated from the analysis of the dispersion properties of waves initiated by the crack. Temperature and inertia contributions to crack propagation are also investigated. It is found that inertia amplifies the elongations of the links, and thus influences the crack advance through the structured solid. ?? 2013 Elsevier Ltd. All rights reserved.},
author = {Carta, G. and Jones, I. S. and Brun, M. and Movchan, N. V. and Movchan, A. B.},
doi = {10.1016/j.ijsolstr.2013.05.001},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/2013{\_}Carta+Jones{\_}Crack propagation induced by thermal shocks in structured media.pdf:pdf},
issn = {00207683},
journal = {Int. J. Solids Struct.},
keywords = {Crack propagation,Elastic lattice,Fracture,Microstructure,Nonlinear dynamic problem,Thermal shock,Thermal striping},
number = {18},
pages = {2725--2736},
publisher = {Elsevier Ltd},
title = {{Crack propagation induced by thermal shocks in structured media}},
url = {http://dx.doi.org/10.1016/j.ijsolstr.2013.05.001},
volume = {50},
year = {2013}
}
@article{Perez2003,
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {P{\'{e}}rez, Mara{\~{n}}a and Strictest, In and Confidence, Commercial and One, Part and Strictest, In and Confidence, Commercial},
doi = {10.1002/ejoc.201200111},
eprint = {arXiv:1011.1669v3},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Fellippa 2007 - AdvancedFEM.pdf:pdf},
isbn = {9781107671812},
issn = {0196-6553},
journal = {Eng. Med. Biol. Soc. 2008. EMBS 2008. 30th Annu. Int. Conf. IEEE},
number = {January},
pages = {2004},
pmid = {26840611},
title = {{Table of of contents}},
year = {2003}
}
@article{Graner1982,
author = {Graner, William R.},
journal = {Handb. Compos.},
pages = {699--722},
title = {{Marine Applications}},
year = {1982}
}
@article{Potirniche2006b,
abstract = {Void growth and coalescence in fcc single crystals were studied using crystal plasticity under uniaxial and biaxial loading conditions and various orientations of the crystalline lattice. A 2D plane strain unit cell with one and two cylindrical voids was employed using three-dimensional 12 potentially active slip systems. The results were compared to five representative orientations of the tensile axis on the stereographic triangle. For uniaxial tension conditions, the void volume fraction increase under the applied load is strongly dependent on the crystallographic orientation with respect to the tensile axis. For some orientations of the tensile axis, such as [1 0 0] or [1 1 0], the voids exhibited a growth rate twice as fast compared with other orientations ([1 0 0], [2 1 1]). Void growth and coalescence simulations under uniaxial loading indicated that during deformation along some orientations with asymmetry of the slip systems, the voids experienced rotation and shape distortion, due mainly to lattice reorientation. Coalescence effects are shown to diminish the influence of lattice orientation on the void volume fraction increase, but noteworthy differences are still present. Under biaxial loading conditions, practically all differences in the void volume fraction for different orientations of the tensile axes during void growth vanish. These results lead to the conclusion that at microstructural length scales in regions under intense biaxiality/triaxiality conditions, such as crack tip or notched regions, the plastic anisotropy due to the initial lattice orientation has only a minor role in influencing the void growth rate. In such situations, void growth and coalescence are mainly determined by the stress triaxiality, the magnitude of accumulated strain, and the spatial localization of such plastic strains.},
author = {Potirniche, G P and Hearndon, J L and Horstemeyer, M F and Ling, X W},
doi = {10.1016/j.ijplas.2005.06.003},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2005{\_}Horstemeyer{\_}Lattice-orientation-effects-on-void-growth-and-coalescence-in-fcc-single-crystals.pdf:pdf},
isbn = {07496419},
issn = {07496419},
journal = {Int. J. Plast.},
keywords = {Fcc Single crystal,Finite element method,Void coalescence,Void growth},
number = {5},
pages = {921--942},
title = {{Lattice orientation effects on void growth and coalescence in fcc single crystals}},
volume = {22},
year = {2006}
}
@article{Terms2003,
abstract = {SUBJECT INDEX Absorption, intestinal Effect of Inborn Errors of Bile A.. Absorption; fat Highly Effective Enteral Treatmen., . intestinal-specific deletion of m, . . Altered MetabolLsm of Postprandia... Effect of Glucagon-fike Peptide-1.. 5-HT3 receptors are essential for...},
author = {Terms, Index},
doi = {10.1016/S0016-5085(03)84188-4},
issn = {00165085},
journal = {Gastroenterology},
number = {4},
pages = {AA60--AA102},
title = {{Subject index}},
url = {http://www.sciencedirect.com/science?{\_}ob=GatewayURL{\&}{\_}origin=ScienceSearch{\&}{\_}method=citationSearch{\&}{\_}piikey=S0016508503841884{\&}{\_}version=1{\&}{\_}returnURL={\&}md5=47aa5121dbf61e18d5fcb18eefe1bd2e},
volume = {124},
year = {2003}
}
@article{Anti-blockier-system,
author = {Anti-blockier-system, Die Bremsenregelungssysteme A B S},
pages = {352--373},
title = {{11 Physikalische Grundlagen der Bremsung und Bremsenregelungssysteme}},
volume = {2}
}
@article{Weng1987,
abstract = {Based on the dislocation structures developed during plastic deformation, an anisotropic hardening law is developed to describe the latent hardening behavior of slip systems under multislip. This theory incorporates the concept of isotropic hardening, kinematic hardening, and the two-parameter representation; it automatically includes the strength differential between the forward and reversed slips and between the acute and obtuse cross slips. The self-hardening modulus of a slip system is found to be "associated" with the latent hardening law involved, and, based on some experimental evidence, two specific sets of self-hardening modulus are suggested. An important feature of this associated modulus is that the slip system with a soft latent hardening (e.g., the reversed system with a Bauschinge effect) will have an enhanced self-hardening modulus. This newly developed hardening law, together with its associated latent hardening moduli, is then applied to examine the strain-hardening behavior of a polycrystal. Although crystals with a stronger latent hardening will, in general, also lead to a stranger strain-hardening for the polycrystal, the stress-strain behavior of the polycrystal using the kinematic hardening law of single crystals is found to be not necessarily softer than that using the isotropic hardening law. Within the range of experimentally measured latent hardening ratio of slip systems, the anisotropic theory is also used to calculate the motion of yield surface of a polycrystal. The general results, employing four selected types of anisotropic hardening, all show the essential features of experimental observations by Phillips and his co-workers. The application is highlighted with a reasonably successful quantitative modeling of initial and subsequent yield surfaces of an aluminum. ?? 1987.},
author = {Weng, G J},
doi = {10.1016/0749-6419(87)90007-6},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/Hardening Recovery Creep/1987{\_}Weng{\_} IJP Anisotropic hardening of crystalls.pdf:pdf},
issn = {07496419},
journal = {Int. J. Plast.},
number = {4},
pages = {315--339},
title = {{Anisotropic hardening in single crystals and the plasticity of polycrystals}},
volume = {3},
year = {1987}
}
@article{Werkstoff,
author = {Werkstoff, Der},
journal = {Optik (Stuttg).},
pages = {305--308},
title = {{11 Zukunftstechnologien im Fahrzeug}}
}
@book{Melorose2015,
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Melorose, J. and Perroy, R. and Careas, S.},
booktitle = {Statew. Agric. L. Use Baseline 2015},
doi = {10.1017/CBO9781107415324.004},
eprint = {arXiv:1011.1669v3},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/Crystall Plasticity Basics/Hull 2011 - Introduction to Dislocation.pdf:pdf},
isbn = {9788578110796},
issn = {1098-6596},
keywords = {icle},
pmid = {25246403},
title = {{Introduction to dislocations}},
volume = {1},
year = {2015}
}
@article{Cantrell2009,
author = {Cantrell, John H},
doi = {10.1063/1.3254223},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2009{\_}Cantrell{\_}Ultrasonic harmonic generation from fatigue-induced dislocation substructures in planar slip metals and assessment of remaining fatigue life.pdf:pdf},
issn = {00218979},
journal = {J. Appl. Phys.},
number = {9},
title = {{Ultrasonic harmonic generation from fatigue-induced dislocation substructures in planar slip metals and assessment of remaining fatigue life}},
volume = {106},
year = {2009}
}
@book{Wishington2012,
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Wishington, D.C},
booktitle = {Bioinforma. Biomed. Eng. 2008. ICBBE 2008. 2nd Int. Conf.},
doi = {10.1002/ejoc.201200111},
eprint = {arXiv:1011.1669v3},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/B{\"{u}}cher{\_}Sammlung{\_}ITM/gnu{\_}make{\_}joined.pdf:pdf},
isbn = {3082342418},
issn = {0196-6553},
pages = {7--58},
pmid = {26840611},
title = {{Table of of contents}},
year = {2012}
}
@article{Zienkiewicz2014f,
abstract = {In this chapter the weak (variational) form for problems in nonlinear solid mechanics in which strains remain small is used to construct approximate solutions based on the finite element method. This results in a Galerkin method for which general properties are well known. Both irreducible (displacement) and mixed form approaches are considered. In particular, we consider a mixed form based on the Hu-Washizu variational theorem that is appropriate for use in problems in which near incompressible behavior can occur. An isoparametric form for finite element approximation is used along with quadrature to evaluate integrals that appear in the variational form. The chapter also applies the methods developed for the equations of solid mechanics to that for thermal analysis based on a nonlinear form of the quasi-harmonic equation.},
author = {Zienkiewicz, O.C. and Taylor, R.L. and Fox, David},
doi = {10.1016/B978-1-85617-634-7.00002-8},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Zienkiewicz FEM - Vol 2 Solid Structural Mechanics/63212{\_}02.pdf:pdf},
isbn = {9781856176347},
issn = {0733-9399},
journal = {Finite Elem. Method Solid Struct. Mech.},
pages = {21--55},
title = {{Galerkin Method of Approximation: Irreducible and Mixed Forms}},
url = {http://linkinghub.elsevier.com/retrieve/pii/B9781856176347000028},
year = {2014}
}
@article{Morris1976a,
abstract = {Abstract Fatigue crack initiation in Al 2219-T851 for fully reversed loading(R = {\$}\sigma{\$}/{\$}\sigma{\$}max =−1) parallel to the material rolling direction is found to occur at intermetallic inclusions at the specimen surface. The inclusions are not involved in crack initiation for fatigue perpendicular to the rolling direction, and for this orientation crack initiation is at grain boundaries and specimens have an increased fatigue life. Except for fatigue at low peak stress, multiple numbers of microcracks are formed and for selected failed specimens the number of cracks has been determined as a function of crack length. Such crack length distribution measurements show that there is significant retardation of microcracks by interaction with grain boundaries. Furthermore it is found that the coalescence of microcracks provides a mechanism for cracking to “jump“ grain boundaries and reduce fatigue lifetime. The effect of relative humidity on this process is to increase the observed mean crack length, and decrease the number of crack initiations apparently due to weakening of the matrix-intermetallic interface at potential initiation sites. The overall result is that no significant dependence of fatigue life on relative humidity is found.},
author = {Morris, W L and Buck, O and Marcus, H L},
doi = {10.1007/BF02656599},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/1976{\_}Morris{\_}Fatigue crack initiation and early propagation in Al 2219-T851.pdf:pdf},
isbn = {0360-2133{\$}\backslash{\$}r1543-1940},
issn = {03602133},
journal = {Met. Trans. A},
number = {7},
pages = {1161--1165},
title = {{Fatigue crack initiation and early propagation in Al 2219-T851}},
volume = {7},
year = {1976}
}
@article{Burgh,
author = {Burg, Heinz and Reaktionspunktes, Festlegung},
pages = {251--260},
title = {{A8 A8 Vermeidbarkeitsbetrachtungen A8}}
}
@article{Anwendunga,
author = {Anwendung, Als and Einsatzgebiete, Typische and Unterschied, Im and Viergurtmodell, Das and Biegesteifigkeit, Die},
pages = {167--176},
title = {{14 Ausgesteifte Kastenprofile}},
volume = {6}
}
@article{Wallentowitz2006o,
author = {Wallentowitz, Henning and Reif, Konrad},
doi = {10.1007/978-3-8348-9121-1_7},
journal = {Handb. Kraftfahrzeugelektronik - Grundlagen, Kompon. Syst. Anwendungen},
title = {{Komfortsysteme}},
url = {http://www.springerlink.com/index/10.1007/978-3-8348-9121-1{\%}7B{\_}{\%}7D7},
year = {2006}
}
@article{Liu1973,
author = {Liu, I Shih},
doi = {10.1007/BF00251292},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Thermodynamik/Liu-Entropieprinzip{\_}Lukas{\_}Fraunhofer/Liu-Entropieprinzip/Liu{\_}heat-conducting{\_}fluid{\_}1973.pdf:pdf},
issn = {00039527},
journal = {Arch. Ration. Mech. Anal.},
number = {1},
pages = {26--33},
title = {{A non-simple heat-conducting fluid}},
volume = {50},
year = {1973}
}
@article{Betrachtungenl,
author = {Betrachtungen, Allgemeine},
journal = {Integr. Vlsi J.},
title = {{9 Stromfadentheorie 9.1}}
}
@article{Ergonomie,
author = {Ergonomie, Die and Arbeitsplatzgestal-, Bereiche and Auslegung, Die and Modelle, Rechner-mensch- and Konzeptvarianten, Diese and Bedienkonzepte, Die and Designmodelle, Die and Aktivit, Diese and Erkenntnisse, Die},
pages = {10--15},
title = {{7 Ergonomie}}
}
@article{Zahoransky2013,
author = {Zahoransky, Richard A and Allelein, Hans-Josef and Schelling, Udo and Schwarz, Harald and Bollin, Elmar and Oehler, Helmut},
doi = {10.1007/978-3-8348-2279-6},
isbn = {978-3-8348-1869-0},
journal = {Energietechnik - Syst. zur Energieumwandlung},
pages = {23},
title = {{10 Kraft-W{\{}{\"{a}}{\}}rmekopplung und Blockheiz-Kraftwerke}},
url = {http://www.springerlink.com/index/10.1007/978-3-8348-2279-6},
year = {2013}
}
@article{Mollenhauer2007,
abstract = {Kapitel 16 des Springer Buchs Handbuch Dieselmotoren; Ger{\"{a}}uschemissionen von Dieselmotoren; Ganzes Buch siehe Ordner B{\"{u}}cher},
author = {Mollenhauer, Klaus and Tsch{\"{o}}ke, Helmut},
title = {{Handbuch Dieselmotoren; Kapitel 16}},
year = {2007}
}
@article{Eslami2015,
abstract = {An approach for prediction of high cycle fatigue (HCF) at a length scale of 5-100 ??m is established, which evaluates the accumulated plastic shear strain in slip bands of grains. Damage mechanisms initiated by dislocations and the grain microstructure are the key factors that influence the fatigue of metals in small dimensions. For this reason the HCF model considers the elasto-plastic behavior of metals at the grain level and microstructural parameters, specifically grain size and grain orientation. The HCF model can be applied either as a criterion for deterministic predictions of the failure in individual grains, or as a failure function in probabilistic studies on aggregates of grains, if the input parameters are given by specific distributions. This is addressed in a parameter study and a sensitivity analysis of the failure function with respect to different parameters. For model verification, the predicted results of the failure function are compared with the observed micro-damage in individual grains of nickel micro-samples. It is shown that the overall predictive power of the HCF model is fairly good. Nevertheless, some misclassifications occur as some grains are damaged, which were predicted to be safe. Those misclassifications are addressed in post-fatigue investigations on individual grains.},
author = {Eslami, R and Riesch-Oppermann, H and Kraft, O},
doi = {10.1016/j.ijfatigue.2015.03.029},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2015{\_}Eslami+Kraft{\_}Prediction of multiaxial high cycle fatigue at small scales based on an micro-mecahnical model{\_}IAM{\_}KIT{\_}KRAFT.pdf:pdf},
isbn = {0142-1123},
issn = {01421123},
journal = {Int. J. Fatigue},
keywords = {Accumulated plastic shear strain,Micro electro mechanical systems (MEMS),Multiaxial high cycle fatigue (HCF),Probability methods,Surface damage},
pages = {66--74},
publisher = {Elsevier Ltd},
title = {{Prediction of multiaxial high cycle fatigue at small scales based on a micro-mechanical model}},
url = {http://dx.doi.org/10.1016/j.ijfatigue.2015.03.029},
volume = {83},
year = {2015}
}
@article{Eekoye1996a,
abstract = {Heat-transfer rates present in an engine cylinder undergoing knock are known to be larger than the rates associated with normal engine operation. Further, at the time of knock, the largest heat fluxes are associated with locations on the cylinder wall where the flame is locally quenching. In this study, heat-transfer processes at the flame-wall interface during a knock event are investigated computationally and analytically. Computationally, the governing equations for a one-dimensional, flame-quenching event are solved using a reduced chemical reaction mechanism. Analytically, scaling relations for the flame heat-release rates are used in the governing equations to determine the heat-transfer rates. It is found that while pressure transients modify the wall heat flux, the absolute value of the pressure is the most significant parameter in predicting the maximum heat flux. The wall heat flux profiles are predicted for both the analytical and computational models. In the range of pressures examined, a linear relationship was found between the peak flux and pressure, both for the computational and analytical models. The linear relationship between the pressure and peak flux was found to be invalid when the flame-quenching process was disrupted by the pressure fluctuations for pressure oscillations with a characteristic time on the order of the quenching process. ?? 1996 Combustion Institute.},
author = {Eekoye, O. A.},
doi = {10.1016/S0082-0784(96)80101-9},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/1996{\_}Ezekoye{\_}Heat transfer modeling during knock and flame quenching in an engine chamber.pdf:pdf},
isbn = {0082-0784},
issn = {00820784},
journal = {Symp. Combust.},
number = {2},
pages = {2661--2668},
title = {{Heat transfer modeling during knock and flame quenching in an engine chamber}},
volume = {26},
year = {1996}
}
@article{Wishington2012a,
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Wishington, D.C},
doi = {10.1002/ejoc.201200111},
eprint = {arXiv:1011.1669v3},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Fellippa 2007 - IntroductionToFEM.pdf:pdf},
isbn = {3082342418},
issn = {0196-6553},
journal = {Bioinforma. Biomed. Eng. 2008. ICBBE 2008. 2nd Int. Conf.},
pages = {7--58},
pmid = {26840611},
title = {{Table of of contents}},
year = {2012}
}
@article{Papadopoulos1997,
abstract = {The aim of this paper is firstly, to provide a concise assessment of some commonly used high-cycle fatigue criteria and secondly, to check their predictive capabilities against synchronous sinusoidal out-of-phase bending and torsion experimental results (i.e. sinusoidal stress signals of the same frequency but with a phase difference). This bending-torsion stress system does not closely represent real load conditions undergone by a machine part. However, it is complex enough to differentiate the various fatigue criteria and to permit a first classification of the approaches examined, according to the accuracy of their predictions. A fatigue criterion recently formulated by the first of the authors is also included in this comparative study. According to this criterion the phase difference in out-of-phase bending and torsion does not affect the fatigue strength corresponding to a very high (theoretically infinite) fatigue life. It is pointed out that this theoretical finding is valid for the category of hard metals for which the ratio of the fully re-versed torsion fatigue limit over the fully reversed bending fatigue limit lies in the interval from 1√3 o approx. 0.8. Experimental results collected from the relevant literature, concerning precisely lard metals, fully support this theoretical finding.},
author = {Papadopoulos, I},
doi = {10.1016/S0142-1123(96)00064-3},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Empirical Fatigue Models + Validation/1996{\_}Papadopoulos{\_}A comparative study of multiaxial high cycle fatigue criteria for metals .pdf:pdf},
isbn = {0142-1123},
issn = {01421123},
journal = {Int. J. Fatigue},
keywords = {cycle fatigue,high,loading,metals,multiaxial fatigue,n o n -,o n a l,o r t i,p r o p},
number = {3},
pages = {219--235},
title = {{A comparative study of multiaxial high-cycle fatigue criteria for metals}},
url = {http://linkinghub.elsevier.com/retrieve/pii/S0142112396000643},
volume = {19},
year = {1997}
}
@inproceedings{Sugihara2007,
author = {Sugihara, T and Suzuki, Y and Shimano, K and Enomoto, Y and Emi, M},
booktitle = {SAE Tech. Pap. 2007-24-0006},
doi = {https://doi.org/10.4271/2007-24-0006},
file = {:C$\backslash$:/Users/p327208/Desktop/Promotion/Literature/Motorspezifisch/Heat Transfer Combustion Chamber/2007{\_}Shimano{\_}Direct Heat Loss to Combustion Chamber Walls in a D.I. Diesel Engine-Development of Measurement Technique and Evaluation of Direct Heat Loss to Cylinder Liner Wall.pdf:pdf},
publisher = {SAE international},
title = {{Direct Heat Loss to Combustion Chamber Walls in a D.I. Diesel Engine}},
year = {2007}
}
@article{Fan1992a,
author = {Fan, H and Keer, L M},
doi = {10.1016/0013-7944(92)90059-N},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/1977{\_}Morris{\_}The early stage of fatigue crack propagation in al 2048.pdf:pdf},
issn = {00137944},
journal = {Eng. Fract. Mech.},
number = {5},
pages = {789--796},
title = {{The early stage of fatigue crack propagation}},
volume = {42},
year = {1992}
}
@book{Morawiec2001,
author = {Morawiec, Adam},
isbn = {9783642073861},
title = {{Springer-Verlag Berlin Heidelberg GmbH}},
url = {http://download.springer.com/static/pdf/185/bfm{\%}253A978-3-642-56668-4{\%}252F1.pdf?auth66=1401995374{\_}4d363c462609ae19e3de18b0ee51ef07{\&}ext=.pdf},
year = {2001}
}
@article{Weiteren,
author = {Weiteren, Im},
journal = {Integr. Vlsi J.},
pages = {106--122},
title = {{9 D{\{}{\"{u}}{\}}nnwandige Profilst{\{}{\"{a}}{\}}be}}
}
@article{Takeuchi1982a,
abstract = {Plastic behavior of single crystals of Cu52Zn48 alloy with the CsCl structure has been examined over a temperature range between 2 K and room temperature. Both at 4.2 K and 77 K, the operative slip plane is the twinning {\{}112{\}} plane in most orientations and it is the anti-twinning {\{}112{\}} plane only in orientations with the maximum shear stress plane close to the anti-twinning {\{}112{\}} plane. Orientation dependence of the yield stress ??mssp showed a maximum near the orientation of the slip plane transition. These results agree well with those of computer simulation of superlattice screw dislocation motion [S. Takeuchi, Phil. Mag. A 41, 541 (1980)]. Temperature and strain-rate dependences of yield stress below {\~{}}130K are essentially similar to those in bcc metals. The above results together with in situ TEM observation indicate that low temperature deformation in ??-CuZn is governed by motion of screw dislocations overcoming the Peierls potential. Activation analyses revealed that the value of exponent in the Arrhenius rate equation, ??H kT, decreases rapidly below 10 K toward zero at 0 K, showing discrepancy of the classical rate theory in the very low temperature range. ?? 1982.},
author = {Takeuchi, S. and Hashimoto, T. and Suzuki, K. and Ichihara, M.},
doi = {10.1016/0001-6160(82)90232-2},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/1958{\_}Haasen{\_}Plastic deformation of nickel single crystals at low temperatures.pdf:pdf},
isbn = {1478-6435 {\%}[ July 29, 2008},
issn = {00016160},
journal = {Acta Metall.},
number = {2},
pages = {513--521},
title = {{Plastic deformation of ??-CuZn single crystals at low temperatures}},
volume = {30},
year = {1982}
}
@article{Tensors1968,
author = {Tensors, Flux},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/Folien CISM Summer School Mai2017 - Mesoscale Models/courses{\%}2FC1703{\%}2Fgroma{\%}2Fcontinuum (1).pdf:pdf},
title = {{Continuum Theory of Dislocations and Plastleity'}},
year = {1968}
}
@article{Package,
author = {Package, Das and Entwicklungsphasen, Diese and Unter-, Hersteller},
pages = {22--26},
title = {{10 Beschreibung eines Package 11 Aufgaben innerhalb der einzelnen}}
}
@article{Schneider2016,
abstract = {{\textcopyright} 2016 Elsevier B.V.Modeling of crack propagation in materials has long been a challenge in solid-state physics and materials science. The phase-field method has now established as one of the tools for the description of crack propagation. The applied models are thermodynamically consistent and predict crack propagation in homogeneous materials under the consideration of different loading types, multiple physical fields and geometrical nonlinearities. Even dynamic loading processes are studied, including plastic effects. A multiphase-field model for crack propagation, which is indispensable to describe crack propagation on a mesoscopic length scale, is still missing. In this work, we overcome this deficiency and combine a crack propagation approach, which is based on Griffith's theory, with an established multiphase-field model for phase transformation.},
author = {Schneider, D. and Schoof, E. and Huang, Y. and Selzer, M. and Nestler, B.},
doi = {10.1016/j.cma.2016.04.009},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Thermodynamik/PhasenFeld/Schneider{\_}Crack{\_}propagation{\_}multiphase{\_}systems-Dez2015.pdf:pdf},
issn = {00457825},
journal = {Comput. Methods Appl. Mech. Eng.},
keywords = {crack propagation,multiphase-field,phase-field,polycrystalline material},
title = {{Phase-field modeling of crack propagation in multiphase systems}},
url = {http://dx.doi.org/10.1016/j.cma.2016.04.009},
year = {2016}
}
@article{Richard,
author = {Richard, H A and Zierep, J and B{\"{u}}hler, K},
journal = {H{\"{u}}tte},
pages = {1--225},
title = {{E-Technische Mechanik}}
}
@article{Lados2006,
abstract = {Linear elastic fracture mechanics describes the fracture behavior of materials and components that respond elastically under loading. This approach is valuable and accurate for the continuum analysis of crack growth in brittle and high strength materials; however it introduces increasing inaccuracies for low-strength/high-ductility alloys (particularly low-carbon steels and light metal alloys). In the case of ductile alloys, different degrees of plastic deformation precede and accompany crack initiation and propagation, and a non-linear ductile fracture mechanics approach better characterizes the fatigue and fracture behavior under elastic-plastic conditions. To delineate plasticity effects in upper Region II and Region III of crack growth an analysis comparing linear elastic stress intensity factor ranges (??Kel) with crack tip plasticity adjusted linear elastic stress intensity factor ranges (??Kpl) is presented. To compute plasticity corrected stress intensity factor ranges (??Kpl), a new relationship for plastic zone size determination was developed taking into account effects of plane-strain and plane-stress conditions ("combo plastic zone"). In addition, for the upper part of the fatigue crack growth curve, elastic-plastic (cyclic J based) stress intensity factor (??KJ) were computed from load-displacement records and compared to plasticity corrected stress intensity factor ranges (??Kpl). A new cyclic J analysis was designed to compute elastic-plastic stress intensity factor ranges (??KJ) by determining cumulative plastic damage from load-displacement records captured in load-control (K-control) fatigue crack growth tests. The cyclic J analysis provides the true fatigue crack growth behavior of the material. A methodology to evaluate the lower and upper bound fracture toughness of the material (JIC and Jmax) directly from fatigue crack growth test data (??KFT(JIC) and ??KFT(Jmax) was developed and validated using static fracture toughness test results. The value of ??KFT(JIC) (and implicitly JIC) is determined by comparing the plasticity corrected elastic fatigue crack growth curve with the elastic-plastic fatigue crack growth curve. A most relevant finding is that plasticity adjusted linear elastic stress intensity factor ranges (??Kpl) are in remarkably good agreement with cyclic J analysis results (??KJ), and provide accurate plasticity corrections up to a ??K corresponding to JIC(i.e. ??KFT(JIC). Towards the end of the fatigue crack growth test (above ??KFT(JIC) when plasticity is accompanied by significant tearing, the cyclic J analysis provides a more accurate way to capture the true behavior of the material and determine ??KFT(Jmax). A procedure to decouple and partition plasticity and tearing effects on crack growth rates is given. Three ca st Al-Si-Mg alloys with different levels of ductility, provided by different Si contents and heat treatments (T61 and T4) are evaluated, and the effects of crack tip plasticity on fatigue crack growth are assessed. Fatigue crack growth tests were conducted at a constant stress ratio, R = 0.1, using compact tension specimens. ?? 2005 Elsevier Ltd. All rights reserved.},
author = {Lados, Diana A. and Apelian, Diran},
doi = {10.1016/j.engfracmech.2005.08.010},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/2004{\_}Lados{\_}Limitations of elastic definitions in Al–Si–Mg cast alloys with enhanced plasticity{\_}LEFM vs Elastic-plastic fracture mechan.pdf:pdf},
isbn = {0013-7944},
issn = {00137944},
journal = {Eng. Fract. Mech.},
keywords = {Elastic-plastic fracture mechanics (EPFM),Linear elastic fracture mechanics (LEFM),Lower and upper bound fracture toughness,Plane-strain/plane-stress ("combo") crack tip plas,Plasticity and tearing,Plasticity corrected linear elastic fracture mecha},
number = {4},
pages = {435--455},
title = {{Limitations of elastic definitions in Al-Si-Mg cast alloys with enhanced plasticity: Linear elastic fracture mechanics versus elastic-plastic fracture mechanics}},
volume = {73},
year = {2006}
}
@article{Haraldsson2004,
author = {Haraldsson, G{\"{o}}ran and Tunestal, Per and Johansson, Bengt and Hyvoenen, Jari},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Thermal Coating + Water Heat Transfer + Applikation/2004{\_}Haraldsson{\_}HCCI Closed-Loop Combustion Control Using Fast Thermal Management.pdf:pdf},
journal = {SAE Trans. J. Engines},
number = {3},
pages = {599--610},
title = {{HCCI Closed-Loop Combustion Control Using Fast Thermal Management}},
volume = {113},
year = {2004}
}
@article{Gross2007,
author = {Gross, Dietmar},
doi = {10.1007/978-3-540-70763-9_7},
isbn = {978-3-540-70762-2},
pages = {205--258},
title = {{Der Arbeitsbegriff in der Elastostatik}},
year = {2007}
}
@article{Leiss2009,
author = {Leiss, Elisabeth},
doi = {10.1515/9783110217001.276},
isbn = {9783110217001},
issn = {9783110217001},
pages = {362--365},
title = {{7. Zusammenfassung und Ausblick}},
url = {file:///C:/Users/Verena/Dropbox/Diplomarbeit{\_}Marketing/Zollenkop{\_}2006{\_}Gesch{\"{a}}ftsmodellinnovation/Zusammenfassung und Ausblick.pdf},
year = {2009}
}
@article{Gross2011b,
author = {Gross, Dietmar and Seelig, Thomas},
doi = {10.1007/978-3-642-10196-0},
isbn = {978-3-642-10195-3},
title = {{Bruchmechanik}},
url = {http://link.springer.com/10.1007/978-3-642-10196-0},
year = {2011}
}
@book{Pope2003,
author = {Pope, S B},
edition = {7},
isbn = {978-0-521-59886-6},
pages = {34--82},
publisher = {Cambridge University Press},
title = {{Turbulent Flows}},
year = {2010}
}
@article{Hauptsatz2011,
author = {Hauptsatz, Erster},
doi = {10.1007/978-3-8348-9903-3},
isbn = {9783834899033},
pages = {60--84},
title = {{4 Energien 4.1}},
year = {2011}
}
@article{Murakami2012j,
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Murakami, Sumio},
doi = {10.1007/978-94-007-2666-6},
eprint = {arXiv:1011.1669v3},
isbn = {978-94-007-2665-9},
issn = {09250042},
pmid = {25246403},
title = {{Continuum Damage Mechanics}},
url = {http://link.springer.com/10.1007/978-94-007-2666-6},
volume = {185},
year = {2012}
}
@article{Haslam2013,
author = {Haslam, Antony and Laskaridis, Panos},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2010{\_}Jaroslav Pokluda+Pavel {\v{S}}andera{\_}Micromechanisms of fracture and fatigue{\_}Buch/Kap4{\_}FatigueFracture.pdf:pdf},
journal = {Adv. Mater. Process.},
number = {April},
title = {{Fatigue {\{}{\&}{\}} Fracture}},
year = {2013}
}
@article{Wimmer2000d,
abstract = {This paper summarizes the results of several investigations on in-cylinder heat transfer during high-pressure and gas exchange phases as well as heat transfer in the inlet and outlet ports for a number of different engine types (DI Diesel, SI and gaseous fueled engine). The paper contains a comparision of simulation results and experimental data derived from heat flux measurements. Numerical results were obtained from zero-, one- and three-dimensional simulation methods. Time and spatially resolved heat fluxes were measured applying the surface temperature method and special heat flux sensors. The paper also includes an assessment of different sensor types with respect to accuracy and applicability.ER -},
author = {Wimmer, Andreas and Pivec, Robert and Sams, Theodor},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2000{\_}Wimmer{\_}Heat Transfer to the Combustion Chamber and Port Walls of IC Engines - A very good overview.pdf:pdf},
number = {724},
title = {{Heat Transfer to the Combustion Chamber and Port Walls of IC Engines - Measurement and Prediction}},
year = {2000}
}
@article{Reglern,
author = {Reglern, Synthese Von},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Vorlesungen/Messtechnik+Regelungstechnik/gmrt05.pdf:pdf},
pages = {1--21},
title = {{Forderungen an die Regelung}}
}
@article{Assistent1999,
author = {Assistent, Wissenschaftlicher and Hannover, Uni and Simulation, Abteilungen and Gmbh, Der Luk},
pages = {1996 -- 1999},
title = {{Dr.-Ing. Dr. h.c. Albert Albers}},
year = {1999}
}
@article{Kratzsch2013b,
author = {Kratzsch, Matthias and G{\"{u}}nther, Michael},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Klopfen{\_}Ottomotor/4. Internationale Tagung Ottomotorisches Klopfen - Berlin 12{\_}2013/Knocking+in+Gasoline+Engines.pdf:pdf},
pages = {445},
title = {{Knocking in Gasoline Engines}},
year = {2013}
}
@article{Kapitela,
author = {Kapitel, Dieses and Anschluss, Im and Sammlung, Assembly and Komponenten, Unterbaugruppe and Komponente, Jede and Bottom, Komponente and Verkn, Up Modelling},
pages = {65--87},
title = {{5 Zusammenbau ( Assemblies )}}
}
@article{Oplinger1998,
author = {Oplinger, D W},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/{\_}buecherSong/HandbookofComposites/II/28{\_}MechanicalFasteningandAdhesiveBonding.pdf:pdf},
journal = {Handb. Compos.},
pages = {57},
title = {{Mechanical Fastening and Adhesive Bonding}},
year = {1998}
}
@article{Kroner1977,
abstract = {Recently P.H. Dederichs and R. Zeller (1973) have developed a formal theory of the bounds of odd order n for the effective elastic moduli of linearly elastic, disordered materials. The bounds are established by use of statistical information given in terms of correlation functions up to order n (= 1, 3, 5,...). This theory is extended to include the bounds of even order n. It is indicated how these bounds can be made optimum under the given statistical information. The results for bounds of even and odd order are obtained in forms which resemble Neumann series, containing multiple integrals up to order (n-1). These integrals can be calculated for certain materials which are classified in terms of a gradual statistical homogeneity, isotropy and disorder. Materials which possess these properties up to the correlation functions of nth order are called overall grade n materials. The optimum bounds for overall grade 2 and grade 3 materials are given explicitly. Optimum bounds for materials which are of grade ∞ in homogeneity and isotropy (i.e. (statistically) perfectly homogeneous and isotropic) and, at the same time, disordered of grade 2 or 3 are also derived. Those for grade 2 in disorder are the Z. Hashin and S. Shtrikman's (1963) bounds. Those for grade 3 are the narrowest, explicit bounds so far derived for random elastic materials. They contain within themselves the so-called self-consistent elastic moduli. {\{}{\textcopyright}{\}} 1977.},
author = {Kr{\"{o}}ner, E},
doi = {10.1016/0022-5096(77)90009-6},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/Strukturmechanik MMS/Literatur/Kr{\"{o}}ner 1977.pdf:pdf},
isbn = {0022-5096},
issn = {00225096},
journal = {J. Mech. Phys. Solids},
number = {2},
pages = {137--155},
title = {{Bounds for effective elastic moduli of disordered materials}},
volume = {25},
year = {1977}
}
@article{Fritz2008,
author = {Fritz, Alfred Herbert and Schulze, G{\"{u}}nter},
doi = {10.1007/978-3-540-76696-4},
isbn = {978-3-540-76695-7},
pages = {494},
title = {{Fertigungstechnik}},
year = {2008}
}
@article{Meneghetti2016b,
abstract = {Fatigue crack initiation and propagation involve plastic strains that require some work to be done on the material. Most part of this irreversible energy is dissipated as heat and consequently the material temperature increases. The heat being an indicator of the intense plastic strains occurring at the tip of a propagating fatigue crack, the hypothesis is formed that it can be used to assess the fatigue damage accumulation rate of cracked components. Moreover, the heat energy at the crack tip is averaged according to Neuber's finite particle concept. The aim of the present paper is to present the theoretical framework and the corresponding experimental technique to evaluate the heat energy dissipated in a structural volume surrounding the crack tip. The shape and size of the structural volume have been assumed according to the literature, even though the definition of the structural volume size of the analysed material in a fatigue sense is not the scope of the present paper. The proposed experimental technique to evaluate the averaged heat energy is based on the radial temperature profiles measured around the crack tip by means of an infrared camera. The temperature fields measured within few millimetres from the crack tip have been compared successfully with existing analytical solutions.},
author = {Meneghetti, G and Ricotta, M},
doi = {10.1016/j.ijfatigue.2016.04.001},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2016{\_}Meneghetti{\_}Evaluating the heat energy dissipated in a small volume surrounding the tip of a fatigue crack.pdf:pdf},
issn = {01421123},
journal = {Int. J. Fatigue},
keywords = {AISI 304L,Averaging approaches,Crack propagation,Crack tip,Critical distance mechanics,Energy approaches,Fatigue assessment},
pages = {605--615},
publisher = {Elsevier Ltd},
title = {{Evaluating the heat energy dissipated in a small volume surrounding the tip of a fatigue crack}},
url = {http://dx.doi.org/10.1016/j.ijfatigue.2016.04.001},
volume = {92},
year = {2016}
}
@article{To2013a,
author = {To, Nswers},
doi = {http://dx.doi.org/10.1016/B978-343722790-5.50023-3},
isbn = {978-3-437-22790-5},
number = {450},
pages = {96--99},
title = {{Kapitel 17}},
volume = {5975},
year = {2013}
}
@article{Motoren,
author = {Motoren, Tuning Von},
pages = {200--211},
title = {{5 Motorentuning}}
}
@article{Leichtbautheorie,
author = {Leichtbautheorie, Der},
journal = {Mechanik},
pages = {74--105},
title = {{8 Elastizit{\{}{\"{a}}{\}}tstheoretische Grundlagen}}
}
@article{Bueno2005,
abstract = {The strain relaxation behaviour after full stress removals during creep of RR-58 Hiduminium alloy has been observed. Creep tests were carried out at 180 ??C, with stresses of 120, 170 and 230 MPa. Tests involved a series of unloading cycles after different creep periods involving the primary and secondary creep stages. The results were interpreted according to a model based on the thermally activated unbowing of dislocation segments. Activation parameters were calculated and an interpretation of the phenomena is made in terms of microstructural details of the material. The appearance of the fast and slow anelastic creep stages may be just a consequence of the high non-linearity existing between the line tension and the area swept by the segments during their unbowing movement. ?? 2005 Elsevier B.V. All rights reserved.},
author = {Bueno, Levi O. and Bell, R. L.},
doi = {10.1016/j.msea.2005.08.055},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Kriechen{\_}Spannungsrelaxation/2005{\_}Bueno{\_}Anelastic creep behaviour of RR-58 aluminum alloy at 180-Phenomenological aspects and analysis based on dislocations.pdf:pdf},
isbn = {0921-5093},
issn = {09215093},
journal = {Mater. Sci. Eng. A},
keywords = {Anelastic creep,Creep recovery,Dislocation unbowing,RR-58 aluminium alloy},
pages = {72--78},
title = {{Anelastic creep behaviour of RR-58 aluminum alloy at 180 ??C: Phenomenological aspects and analysis based on the unbowing of dislocation segments}},
volume = {410-411},
year = {2005}
}
@article{Rudolf2007,
author = {Rudolf, Als and Ende, Diesel},
title = {{Kraftstoffe}},
year = {2007}
}
@misc{Draper1935a,
author = {Draper, C.S.},
booktitle = {NACA Rep.},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/xxx{\_}Draper{\_}The physical effects of detonation in a closed cylindrical chamber - analytical solutions.pdf:pdf},
number = {493},
title = {{The physical effects of detonation in a closed cylindrical chamber}},
year = {1935}
}
@article{Ture1980,
author = {Ture, Nomencla},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/1980{\_}Singh{\_}Effect of prior treatement on LCF of AL alloy 2618 at 432K.pdf:pdf},
number = {January},
pages = {12--22},
title = {{Effect of ior alloy mmst oa at 423K cycle alumini l mm amr of}},
year = {1980}
}
@article{Meroth2008c,
abstract = {Die Entwicklung eines Infotainmentsystems f{\"{u}}r ein Kraftfahrzeug erfordert ein hohes Ma{\ss} an interdisziplin{\"{a}}rem Fachwissen. Zum einen muss die Software verschiedene Multimediaapplikationen, wie Radio, Video oder Navigation, bereitstellen. Zum anderen handelt es sich um ein Softwaresystem, das auf einem eingebetteten System innerhalb eines Kraftfahrzeugs entwickelt wird, sodass ein erh{\"{o}}htes Ma{\ss} an Zuverl{\"{a}}ssigkeit und Korrektheit der Software erforderlich ist. Die Erstellung einer umfangreichen Softwarearchitektur f{\"{u}}r die Planung des Systems ist eine M{\"{o}}glichkeit, um der Komplexit{\"{a}}t der Problemstellung Rechnung zu tragen. In diesem Kapitel wird auf die Besonderheiten eingegangen, die bei der Entwicklung einer Softwarearchitektur f{\"{u}}r ein Infotainmentsystem beachtet werden sollten. Abschnitt 7.1.1 gibt einen {\"{U}}berblick {\"{u}}ber die Historie der Unified Modelling Language (UML) sowie eine kurze Einf{\"{u}}hrung der Modellierungselemente.},
author = {Meroth, Ansgar and Tolg, Boris},
isbn = {978-3-8348-9430-4},
journal = {Infotainmentsysteme im Kraftfahrzeug},
pages = {267--320},
title = {{Plattform-Software}},
url = {http://dx.doi.org/10.1007/978-3-8348-9430-4{\_}7},
year = {2008}
}
@article{Felderb,
author = {Felder, Magnetische},
title = {( ) (4.1)}
}
@article{Mechanismen,
author = {Mechanismen, Die},
title = {{8 Kr{\"{a}}fte und Momente}}
}
@article{Arminger2007,
author = {Arminger, Gerhard and Bommert, Karl},
journal = {Geographie},
title = {{Skriptum f{\"{u}}r die Vorlesungen Statistik I und II 2006/2007}},
year = {2007}
}
@article{Anhang1995,
author = {Anhang, Der},
isbn = {0688011411},
pages = {104--111},
title = {{9 Anhang}},
year = {1995}
}
@article{Lo,
author = {Lo, Kleb- and Wirkung, Funktion},
doi = {10.1007/978-3-8348-8279-0},
isbn = {9783834882790},
pages = {89--111},
title = {{5 Kleb- und Lo ¨ tverbindungen 5 5.1}}
}
@article{Contents,
author = {Contents, Chapter},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Zienkiewicz FEM - Vol 2 Solid Structural Mechanics/63212{\_}03.pdf:pdf},
pages = {48--140},
title = {{Solution of Nonlinear}},
volume = {1}
}
@article{Wilson1951,
author = {Wilson, Brian A},
journal = {Processing},
title = {{A. Wilson 23}},
year = {1951}
}
@article{Rako1996,
author = {Rakopoulos, C.D. and Mavropoulos, G.C.},
doi = {10.1002/(SICI)1099-114X(199605)20:5<437::AID-ER169>3.0.CO;2-J},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Heat Transfer Combustion Chamber/1996{\_}Rakopoulos{\_}Study of the steady and transient temperature field and heat flow{\_}Diesel{\_}FEM.pdf:pdf},
journal = {Int. J. Energy Res.},
keywords = {diesel engine components transient,temperature field finite elements},
pages = {437--464},
title = {{Study of the steady and transient temperature field and heat flow in the combustion chamber components of a medium speed diesel engine using finite element analyses}},
volume = {20},
year = {1996}
}
@inproceedings{Su2002,
abstract = {Thermal fatigue presents a new challenge in cast aluminum engine design. Accurate thermomechanical stress analysis and reliable failure criterion are the keys to a successful life prediction. It is shown that the material stress and strain behavior of cast aluminum is strongly temperature and strain rate sensitive. A unified viscoplasticity constitutive relation is thus proposed to simultaneously describe the plasticity and creep of cast aluminum components deforming at high temperatures. A fatigue failure criterion based on a damage accumulation model is introduced. Damages due to mechanical fatigue, environmental impact and creep are accounted for. The material stress and strain model and thermal fatigue model are shown to be effective in accurately capturing features of thermal fatigue by simulating a component thermal fatigue test using 3D FEA with ABAQUS and comparing the results with measured data. Copyright {\textcopyright} 2002 Society of Automotive Engineers, Inc.},
author = {Su, X and Zubeck, M and Lasecki, J and Jr, C C Engler-pinto and Tang, C and Allison, J},
booktitle = {SAE Tech. Pap. 2002-01-0657},
doi = {https://doi.org/10.4271/2002-01-0657.},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Kriechen{\_}Spannungsrelaxation/2002{\_}Su+Zubeck{\_}Thermal fatigue analysis of cast aluminium cyclinder heads.pdf:pdf},
publisher = {SAE International},
title = {{Thermal Fatigue Analysis of Cast Aluminum Cylinder Heads}},
year = {2002}
}
@article{Park2013,
author = {Park, Minje and Jung, Daebong and Kim, Minjae and Min, Kyoungdoug},
doi = {10.1016/j.applthermaleng.2013.07.032},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Thermal Coating + Water Heat Transfer + Applikation/2013{\_}Park{\_}Study on the improvement in continuously variable transmission efficiency with a thermal management system.pdf:pdf},
journal = {Appl. Therm. Eng.},
keywords = {continuously variable transmission,thermal management system},
number = {2},
pages = {11--19},
publisher = {Elsevier Ltd},
title = {{Study on the improvement in continuously variable transmission efficiency with a thermal management system}},
volume = {61},
year = {2013}
}
@article{Matrizen,
author = {Matrizen, Reelle},
doi = {10.1007/978-3-8348-2129-4},
isbn = {9783834821294},
pages = {194--223},
title = {{VII Lineare Algebra}}
}
@article{Essmann1981b,
abstract = {Based on recent experimental observations a realistic model of the evolution of the surface profile of persistent slip bands (PSBs) in fatigued metals is proposed. An essential feature of the model is the production of vacancies by the annihilation of edge dislocations which, combined with irreversible slip processes, leads to an elongation of the PSB parallel to the active slip vector. It is shown that a net extrusion forms rather rapidly. The growth processes and their dependence on temperature are discussed in detail. It is proposed that cracks initiate at the surface steps at the PSB{\&}ndash;matrix interface and, at a later stage, also at the notch-peak profile from the random slip processes.},
author = {Essmann, U. and G{\"{o}}sele, U. and Mughrabi, H.},
doi = {10.1080/01418618108239541},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2016{\_}Mughrabi{\_}A model of extrusions and intrusions in fatigued metals I  Point defect production and the growth of extrusions.pdf:pdf},
isbn = {0141-8610},
issn = {0141-8610},
journal = {Philos. Mag. A},
number = {2},
pages = {405--426},
title = {{A model of extrusions and intrusions in fatigued metals I. Point-defect production and the growth of extrusions}},
url = {http://www.tandfonline.com/doi/abs/10.1080/01418618108239541},
volume = {44},
year = {1981}
}
@article{Finol2006,
abstract = {Over the last 40 years, several empirical correlations have been developed to estimate heat fluxes from the combustion chambers of internal combustion engines. Some of these expressions are based on correlations to compute the Nusselt number for forced convection in turbulent flow inside circular tubes. The fundamental suitability of this kind of empirical model in representing the highly complex processes of in-cylinder heat transfer is questionable, but in practice the models have steadily improved owing to contributions from numerous investigators. Other correlations have a less theoretical basis than those of the Nusselt number form. Formulae of this type have been obtained from the application of simple statistical techniques to large datasets, taking into account several engine operational parameters and engine types. The resulting correlations provide reasonable estimates but perform poorly when extrapolated or applied to novel concepts. In this paper, the most important correlations are reviewed against the features of a modern diesel engine, and research requirements for future modelling developments are identified and discussed. {\textcopyright} IMechE 2006.},
author = {Finol, C A and Robinson, K},
doi = {https://doi.org/10.1243/09544070JAUTO202},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2006{\_}Finol{\_}Thermal modelling of modern engines - A review of empirical correlations to estimate the in-cylinder heat transfer coefficient .pdf:pdf},
journal = {Proc. Inst. Mech. Eng. Part D J. Automob. Eng.},
keywords = {cient,heat flux,heat transfer coe ffi,in-cylinder heat transfer models},
number = {12},
pages = {1765--1781},
title = {{Thermal modelling of modern engines: a review of empirical correlations to estimate the in-cylinder heat transfer coefficient}},
volume = {220},
year = {2006}
}
@article{Rice1969a,
abstract = {The fracture of ductile solids has frequently been observed to result from the large growth and coalescence of microscopic voids, a process enhanced by the superposition of hydrostatic tensile stresses on a plastic deformation field. The ductile growth of voids is treated here as a problem in continuum plasticity. First, a variational principle is established to characterize the flow field in an elastically rigid and incompressible plastic material containing an internal void or voids, and subjected to a remotely uniform stress and strain rate field. Then an approximate Rayleigh-Ritz procedure is developed and applied to the enlargement of an isolated spherical void in a nonhardening material. Growth is studied in some detail for the case of a remote tensile extension field with superposed hydrostatic stresses. The volume changing contribution to void growth is found to overwhelm the shape changing part when the mean remote normal stress is large, so that growth is essentially spherical. Further, it is found that for any remote strain rate field, the void enlargement rate is amplified over the remote strain rate by a factor rising exponentially with the ratio of mean normal stress to yield stress. Some related results are discussed, including the long cylindrical void considered by F.A. McClintock (1968, J. appl. Mech. 35, 363), and an approximate relation is given to describe growth of a spherical void in a general remote field. The results suggest a rapidly decreasing fracture ductility with increasing hydrostatic tension.},
author = {Rice, J R and Tracey, D M},
doi = {10.1016/0022-5096(69)90033-7},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Plasticity models/On the ductile enlargement of voids in triaxial stress fields {\_}RiceAndTracey.pdf:pdf},
isbn = {0022-5096},
issn = {00225096},
journal = {J. Mech. Phys. Solids},
number = {3},
pages = {201--217},
title = {{On the ductile enlargement of voids in triaxial stress fields∗}},
url = {http://linkinghub.elsevier.com/retrieve/pii/0022509669900337},
volume = {17},
year = {1969}
}
@article{Lin1989a,
author = {Lin, T H and Lin, S R and Wu, X Q},
doi = {10.1080/01418618908221174},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/1989{\_}Lin{\_}Micromechanics of an extrusion in high-cycle fatigue.pdf:pdf},
issn = {0141-8610},
journal = {Philos. Mag. A},
number = {6},
pages = {1263--1276},
title = {{Micromechanics of an extrusion in high-cycle fatigue}},
url = {http://www.tandfonline.com/doi/abs/10.1080/01418618908221174},
volume = {59},
year = {1989}
}
@article{Sauerstoff,
author = {Sauerstoff, Komponenten and Gegensatz, Im},
number = {x},
title = {{6 Schadstoffbildung 6.1}}
}
@article{Modelle,
author = {Modelle, Response Surface},
title = {{6 Optimierungsstrategien}}
}
@article{Shitsu,
author = {Shitsu, H I N and No, K a and Kai, T E N},
pages = {2--3},
title = {{Quality – Function – Deployment ( QFD )}}
}
@inproceedings{Wagner2003SAE,
abstract = {The introduction of mechatronic components into thermal-mechanical systems provides an opportunity to apply real time control strategies for enhanced engine performance. The traditional automotive thermal management system contains the engine, thermostat, air cooled radiator, and centrifugal pump driven by the crankshaft belt. A servo-motor valve and pump may be inserted into the vehicle's heating/cooling system to regulate the coolant flow with the engine control unit. To study these dual actuators, a scale experimental cooling system has been investigated. This automotive inspired thermal system contains a heater, smart thermostat valve, radiator, and variable speed electric pump. A lumped parameter model has been developed to describe the system's behavioral response and establish the basis for temperature regulation. Real time control algorithms are introduced for the synchronous regulation of the valve and pump. Representative numerical results are presented and discussed to demonstrate the thermal management system concept.},
author = {Wagner, John R and Srinivasan, Venkat and Dawson, Darren M and Marotta, Egidio E},
booktitle = {SAE 2003 World Congr. Exhib.},
doi = {https://doi.org/10.4271/2003-01-0272},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Thermal Coating + Water Heat Transfer + Applikation/2003{\_}Wagner{\_}Smart Thermostat and Coolant Pump Control for Engine Thermal Management Systems.pdf:pdf},
publisher = {SAE International},
title = {{Smart Thermostat and Coolant Pump Control for Engine Thermal Management Systems}},
year = {2003}
}
@article{Mechatronik,
author = {Mechatronik, Der and Bewegungen, Prozesse},
journal = {Sensors (Peterborough, NH)},
pages = {103--122},
title = {{6 Aktorik}}
}
@article{Endokrinologiea,
author = {Endokrinologie, Das Forschungsgebiet Der},
pages = {1--2},
title = {{1 Einf{\"{u}}hrung}}
}
@article{Dietmann1973a,
author = {Dietmann, H.},
doi = {10.1002/mawe.19730040608},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Empirical Fatigue Models + Validation/1973{\_}Dietmann Materialwissenschaft{\_}und{\_}Werkstofftechnik{\_}ExperimentelleUntersuchungenZuFatigue.pdf:pdf},
issn = {15214052},
journal = {Materwiss. Werksttech.},
number = {6},
pages = {322--333},
title = {{Werkstoffverhalten unter mehrachsiger schwingender Beanspruchung. Teil 2: Experimentelle Untersuchungen}},
volume = {4},
year = {1973}
}
@book{Flaceliere2007,
author = {Flaceliere, L. and Morel, F. and Dragon, A.},
booktitle = {Int. J. Damage Mech.},
doi = {10.1177/1056789506067935},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/2 scale models papers/2007{\_} Flaceliere+Morel+Dragon{\_}Coupling Between Mesoplasticity and Damage in HCF{\_}MitViskoEffekte.pdf:pdf},
isbn = {1056789506},
issn = {1056-7895},
keywords = {author to whom correspondence,damage model,e-mail,ensma,experiment,flaceliere,fr,lmpm,mesoplasticity,multiaxial fatigue,should be addressed},
number = {4},
pages = {473--509},
title = {{Coupling Between Mesoplasticity and Damage in High-cycle Fatigue}},
volume = {16},
year = {2007}
}
@article{CARPINTERI2001,
abstract = {Some multiaxial high-cycle fatigue criteria based on the so-called critical plane approach are reviewed. According to such an approach, the critical plane where the fatigue life assessment should be performed can be determined by maximising the amplitudes and/or values of some stress components. In the present paper, the critical plane orientation is correlated with the averaged principal stress directions deduced through the weight function method, and a new fatigue failure criterion is proposed. The results derived by applying the present criterion and the other critical plane criteria analysed are compared with experimental data related to different brittle (hard) metals under in-phase or out-of-phase sinusoidal biaxial normal and shear stress states. 0},
author = {CARPINTERI, A and SPAGNOLI, A},
doi = {10.1016/S0142-1123(00)00075-X},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Empirical Fatigue Models + Validation/2000{\_}Carpinteri{\_}Multiaxial high cycle fatigue criterion for hard metals.pdf:pdf},
isbn = {0142-1123},
issn = {01421123},
journal = {Int. J. Fatigue},
keywords = {multiaxial},
number = {2},
pages = {135--145},
title = {{Multiaxial high-cycle fatigue criterion for hard metals}},
url = {http://linkinghub.elsevier.com/retrieve/pii/S014211230000075X},
volume = {23},
year = {2001}
}
@article{Zahoransky2013f,
author = {Zahoransky, Richard a. and Allelein, Hans-Josef and Schelling, Udo and Schwarz, Harald and Bollin, Elmar and Oehler, Helmut},
doi = {10.1007/978-3-8348-2279-6},
isbn = {978-3-8348-1869-0},
journal = {Energietechnik - Syst. zur Energieumwandlung},
pages = {32},
title = {{8 Station{\{}{\"{a}}{\}}re Kolbenmotoren f{\{}{\"{u}}{\}}r energetischen Einsatz}},
url = {http://www.springerlink.com/index/10.1007/978-3-8348-2279-6},
year = {2013}
}
@article{Roters2000a,
abstract = {A new work-hardening model for homogeneous and heterogeneous cell-forming alloys is introduced. It distinguishes three internal state variables in terms of three categories of dislocations: mobile dislocations, immobile dislocations in the cell interiors and immobile dislocations in the cell walls. For each dislocation population an evolution law is derived taking into account dislocation generation, annihilation and storage by dipole and lock formation. In particular, these rate equations take into account the number of active glide systems and, thus, introduce texture in the model in addition to the Taylor factor. Microstructure is represented by the dislocation cell structure as well as second-phase particles, which may undergo changes by precipitation and Ostwald ripening. Interaction of mobile dislocations with the microstructure is taken into account through an effective slip length of the mobile dislocations. For the same set of parameters, the predictions are in excellent agreement with measured stress–strain curves of both a precipitation-hardened aluminium alloy (Al–4.16 wt{\{}{\%}{\}} Cu–1.37 wt{\{}{\%}{\}} Mg, AlCuMg2) and a precipitation-free model alloy (Al–0.35 wt{\{}{\%}{\}} Cu–0.25 wt{\{}{\%}{\}} Mg), the composition of which corresponds to the matrix of the two-phase alloy. Ein neues Verfestigungsmodell f{\{}{\"{u}}{\}}r homogene und heterogene Legierungen wird vorgestellt. Es werden drei innere Zustandsvariablen in Form von drei Versetzungsklassen unterschieden, mobile Versetzungen, immobile Versetzungen im Zellinnern und immobile Versetzungen in den Zellw{\{}{\"{a}}{\}}nden der Substruktur. F{\{}{\"{u}}{\}}r die Dichte jeder dieser Versetzungsklassen wird eine Evolutionsgleichung hergeleitet, die Versetzungsproduktion, -annihilation und -speicherung durch Bildung von Dipolen und se{\{}{\ss}{\}}haften Versetzungsreaktionsprodukten ber{\{}{\"{u}}{\}}cksichtigt. Insbesondere wird dabei die Zahl der aktiven Gleitsysteme ber{\{}{\"{u}}{\}}cksichtigt, wodurch die Textur zus{\{}{\"{a}}{\}}tzlich zum Taylorfaktor in das Modell einflie{\{}{\ss}{\}}t. Die Mikrostruktur wird durch die Versetzungszellstruktur und Sekund{\{}{\"{a}}{\}}rphasen repr{\{}{\"{a}}{\}}sentiert, wobei letztere Ausscheidungs- und Reifungsprozessen unterworfen sind. Die Wechselwirkung der mobilen Versetzungen mit der Mikrostruktur wird durch eine effektive freie Wegl{\{}{\"{a}}{\}}nge der mobilen Versetzungen ber{\{}{\"{u}}{\}}cksichtigt. Die Modellvorhersagen stimmen bei gleichem Parametersatz sehr gut mit gemessenen Spannungs-Dehnungs-Kurven einer ausscheidungsh{\{}{\"{a}}{\}}rtbaren Aluminiumlegierung (Al–4.16 wt{\{}{\%}{\}} Cu–1.37 wt{\{}{\%}{\}} Mg, AlCuMg2) und einer ausscheidungsfreien Modellegierung (Al–0.35 wt{\{}{\%}{\}} Cu–0.25 wt{\{}{\%}{\}} Mg), die der Matrix des zweiphasigen Werkstoffs entspricht, {\{}{\"{u}}{\}}berein.},
author = {Roters, F and Raabe, D and Gottstein, G},
doi = {10.1016/S1359-6454(00)00289-5},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/Hardening Recovery Creep/2000{\_}GOTTSTEIN{\_}Work hardening in heterogeneous alloys - a microstructural approach based on three internal state variables.pdf:pdf},
isbn = {1359-6454},
issn = {13596454},
journal = {Acta Mater.},
keywords = {Alloys,Dislocations,Dislocations-theory,Mechanical properties,aluminium,mobility,plastic},
number = {17},
pages = {4181--4189},
title = {{Work hardening in heterogeneous alloys—a microstructural approach based on three internal state variables}},
url = {http://www.sciencedirect.com/science/article/pii/S1359645400002895},
volume = {48},
year = {2000}
}
@article{Balken,
author = {Balken, Aufgelegter},
doi = {10.1007/978-3-642-24335-6},
isbn = {9783642243356},
title = {{3 Rand- und Eigenwertprobleme gew¨ ohnlicher Differenzialgleichungen}}
}
@article{Ladungstrager,
author = {Ladungstr{\"{a}}ger, Driftbewegung Der},
title = {{3 Elektrisches Str{\{}{\"{o}}{\}}mungsfeld}}
}
@article{Moschandreou1997,
author = {Moschandreou, T and Zamir, M},
doi = {https://doi.org/10.1016/S0017-9310(96)00266-9},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Thermal Coating + Water Heat Transfer + Applikation/1996{\_}Zamir+Moschandreau{\_}Heat Transfer in a tube with pulsating flow and constant heat flux.pdf:pdf},
journal = {Int. J. Heat Mass Transf.},
number = {10},
pages = {2461--2466},
title = {{Heat transfer in a tube with pulsating flow and constant heat flux}},
volume = {40},
year = {1997}
}
@article{Hansen2004a,
abstract = {The Hall-Petch relation is discussed separately for the yield stress of undeformed polycrystalline metals and for the flow stress of deformed metals. Key structural parameters are the boundary spacing, between grain boundaries in the former case and between dislocation boundaries and high angle boundaries in the latter. An analysis of experimental data supports the Hall-Petch relation for undeformed metals over a grain size range from about 20 nm to hundreds of micrometers. For deformed metals, boundary strengthening is not a constant and the Hall-Petch relation must be modified. ?? 2004 Acta Materialia Inc. Published by Elsevier Ltd. All rights reserved.},
author = {Hansen, Niels},
doi = {10.1016/j.scriptamat.2004.06.002},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2004{\_}Hansen Hall–Petch relation and boundary strengthening.pdf:pdf},
isbn = {1359-6462},
issn = {13596462},
journal = {Scr. Mater.},
keywords = {Dislocation boundaries,Flow stress,Grain size,Nanostructure,Yield stress},
number = {8 SPEC. ISS.},
pages = {801--806},
title = {{Hall-petch relation and boundary strengthening}},
volume = {51},
year = {2004}
}
@article{Spannungszustand,
author = {Spannungszustand, Einachsiger and Spannungszustand, Ebener},
pages = {215--246},
title = {{A a a a}}
}
@article{Kratzsch2013c,
author = {Kratzsch, Matthias and G{\"{u}}nther, Michael},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Klopfen{\_}Ottomotor/Knocking+in+Gasoline+Engines{\_}ExtremdetailierterUeberblick{\_}445Seiten.pdf:pdf},
pages = {445},
title = {{Knocking in Gasoline Engines}},
year = {2013}
}
@book{Chakrabarty2006,
abstract = {During recent years, there has been considerable interest in the application of the macroscopic theory of plasticity to engineering problems associated with structural designs and the technological forming of metals. The need for a comprehensive text book on plasticity, incorporating the most recent developments of the subject, has been strongly felt for some years. This book has been written primarily to meet the needs of graduate and research students of Mechanical, Civil, and Metallurgical Engineering, although some of the material in the book is also suitable for under- graduate students and practicing engineers. In order to discuss the various topics as fully as possible, it has been found necessary to treat the subject matter in two volumes, of which the first one is now presented to the reader. The},
author = {Chakrabarty, J},
doi = {10.1016/B978-0-7506-6638-1.50006-6},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/B{\"{u}}cher{\_}Sammlung{\_}ITM/Theory of Plasticity - J. Chakrabarty/Theory-of-Plasticity-Chakrabarty.pdf:pdf},
isbn = {0750666382},
issn = {02321300},
pages = {896},
title = {{Theory of plasticity}},
url = {http://books.google.com/books?hl=en{\&}lr={\&}id=uMcID-tu-8YC{\&}oi=fnd{\&}pg=PP2{\&}dq=Theory+of+plasticity{\&}ots=dAGJbq6QUZ{\&}sig=-d4jjjFGmrIIlUe1p1XNq63z59s},
year = {2006}
}
@article{Hart-Smith1998,
author = {Hart-Smith, L J and Brown, D and Wong, S},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/{\_}buecherSong/HandbookofComposites/II/29{\_}SurfacePreparationsforEnsuringThattheGlueWillStickinBondedComposite.pdf:pdf},
isbn = {0412540207},
journal = {Handb. Compos.},
pages = {667--685},
title = {{Surface preparations for ensuring that the glue will stick in bonded composite structures}},
year = {1998}
}
@article{Popov2009,
author = {Popov, Valentin and Schargott, Martin},
title = {{Materialtheorie}},
year = {2009}
}
@inproceedings{Woschnithermal1979,
abstract = {Experimental investigations were carried out on a high speed Diesel engine, where the heat fluxes to the different components piston, cylinder head, and liner were seperately determined by evaluating heat balances and measured steady state temperature fields. A comparison with the results of cycle simulations carried out with the equation for the local mean heat transfer coefficient suggested by the author around 15 years ago shows, that this equation is applicable to predict the heat losses to the cylinder walls and their influence on the process data as well as the steady state temperature fields occuring in the components during operation.},
author = {Woschni, Gerhard},
booktitle = {SAE Tech. Pap.},
doi = {10.4271/790821},
publisher = {SAE International},
title = {{Prediction of Thermal Loading of Supercharged Diesel Engines}},
year = {1979}
}
@article{McDowell2003,
abstract = {High cycle fatigue (HCF) life in cast Al-Mg-Si alloys is particularly sensitive to the combination of microstructural inclusions and stress concentrations. Inclusions can range from large-scale shrinkage porosity with a tortuous surface profile to entrapped oxides introduced during the pour. When shrinkage porosity is controlled, the relevant microstructural initiation sites are often the larger Si particles within eutectic regions. In this paper, a HCF model is introduced which recognizes multiple inclusion severity scales for crack formation. The model addresses the role of constrained microplasticity around debonded particles or shrinkage pores in forming and growing microstructurally small fatigue cracks and is based on the cyclic crack tip displacement rather than linear elastic fracture mechanics stress intensity factor. Conditions for transitioning to long crack fatigue crack growth behavior are introduced. The model is applied to a cast A356-T6 Al alloy over a range of inclusion severities. ?? 2002 Elsevier Science Ltd. All rights reserved.},
author = {McDowell, D. L. and Gall, K. and Horstemeyer, M. F. and Fan, J.},
doi = {10.1016/S0013-7944(02)00021-8},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/2003{\_}McDowell{\_}Microstructure-based fatigue modeling of cast A356-T6 alloy.pdf:pdf},
isbn = {0013-7944},
issn = {00137944},
journal = {Eng. Fract. Mech.},
keywords = {A356,Cast alloys,High cycle fatigue,Microstructure},
number = {1},
pages = {49--80},
pmid = {119},
title = {{Microstructure-based fatigue modeling of cast A356-T6 alloy}},
volume = {70},
year = {2003}
}
@article{Nachgang2012,
author = {Nachgang, Im},
doi = {10.1007/978-3-8348-2134-8},
isbn = {9783834821348},
pages = {306--323},
title = {{14 Grundregeln der FEM-Anwendung}},
year = {2012}
}
@article{Warmeubertragung2011,
author = {W{\"{a}}rme{\"{u}}bertragung, Die and W{\"{a}}rmelehre, Teilgebiet Der},
doi = {10.1007/978-3-642-15959-6},
isbn = {9783642159596},
pages = {1--16},
title = {{Einleitung und Definitionen}},
year = {2011}
}
@article{Senga,
author = {Seng, Jocelyn M},
journal = {Production},
title = {{Laminate design}}
}
@article{Zienkiewicz2013d,
author = {Zienkiewicz, O.C. and Taylor, R.L. and Zhu, J.Z.},
doi = {10.1016/B978-1-85617-633-0.00014-9},
isbn = {9781856176330},
issn = {00295981},
journal = {Finite Elem. Method its Basis Fundam.},
pages = {467--491},
title = {{Shells as a Special Case of Three-Dimensional Analysis}},
url = {http://linkinghub.elsevier.com/retrieve/pii/B9781856176330000149},
year = {2013}
}
@book{Hartley2006,
abstract = {This book gives an introduction to computational plasticity and includes the kinematics of large deformations, together with relevant continuum mechanics. Central to the book is its focus on computational plasticity, and we cover an introduction to the finite element method which includes both quasi-static and dynamic problems. We then go on to describe explicit and implicit implementations of plasticity models in to finite element software. Throughout the book, we describe thegeneral, multiaxial form of the theory but uniquely, wherever possible, reduce the equations to their simplest, uniaxial form to develop understanding of the general theory and, we hope, physical insight. We provide several examples of implicit and explicit implementations of von Mises time-independentand visco-plasticity in to the commercial code ABAQUS (including the fortran coding), which should prove invaluable to research students and practising engineers developing ABAQUS 'UMATs'. The book bridges the gap between undergraduate material on plasticity and existing advanced texts on nonlinear computational mechanics, which makes it ideal for students and practising engineers alike. It introduces a range of engineering applications, including superplasticity, porous plasticity, cyclicplasticity and thermo-mechanical fatigue, to emphasize the subject's relevance and importance.},
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Hartley, P},
booktitle = {J. Phys. A. Math. Gen.},
doi = {10.1088/0305-4470/39/14/B02},
eprint = {arXiv:1011.1669v3},
isbn = {9780198568261},
issn = {0305-4470},
number = {14},
pages = {3850--3851},
pmid = {25246403},
title = {{Introduction to Computational Plasticity}},
url = {http://stacks.iop.org/0305-4470/39/i=14/a=B02?key=crossref.df6043dc7dee1ea3fe9a75a1094a108d},
volume = {39},
year = {2006}
}
@article{Zech2005,
author = {Zech, Michael},
doi = {10.1002/best.200590286},
journal = {Beton- und Stahlbetonbau},
number = {2},
pages = {81--246},
title = {{Krafteinleitung }},
volume = {100},
year = {2005}
}
@article{Mechatronik,
author = {Mechatronik, Der and Bewegungen, Prozesse},
journal = {Sensors (Peterborough, NH)},
pages = {103--122},
title = {{6 Aktorik}}
}
@article{Burg2006,
author = {Burg, Heinz and Rekonstruktion, Die and Nutzfahrzeugunf{\"{a}}llen, Von},
pages = {439--442},
title = {{A13 A13 Unf{\"{a}}lle mit Nutzfahrzeugen A13}},
year = {2006}
}
@article{Polak2014b,
abstract = {The role of point defects in the formation of surface relief and in the initiation of a fatigue crack in crystalline materials is analyzed. The dislocation interactions in the bands of intensive cyclic slip (persistent slip bands - PSBs) are specified and relations describing the formation and annihilation of interstitial and vacancy type defects in the channels of the ladder-like PSB are derived. The continuous formation, annihilation and primarily the migration of point defects are proposed to be responsible for the mass redistribution within PSB and between PSB and the PSB/matrix boundary. The redistribution of the matter results in local tensile and compressive stresses that are the sources of the principal irreversibility of slip within PSB. Local tensile and compressive stresses are relaxed by dislocation movement within PSB in the direction of the active Burgers vector and lead to the formation of characteristic surface relief in the form of extrusions and intrusions. The intrusions represent crack-like defects and fatigue cracks initiate in the tip of intrusions. {\textcopyright} 2013 Elsevier Ltd. All rights reserved.},
author = {Pol{\'{a}}k, Jaroslav and Man, Jiř{\'{i}}},
doi = {10.1016/j.ijfatigue.2013.10.016},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/2014{\_}Polak+Man{\_}Fatigue crack initiation – The role of point defects.pdf:pdf},
isbn = {0142-1123},
issn = {01421123},
journal = {Int. J. Fatigue},
keywords = {Extrusion,Fatigue crack initiation,Intrusion,Persistent slip band (PSB),Point defects},
number = {July},
pages = {18--27},
title = {{Fatigue crack initiation - The role of point defects}},
volume = {65},
year = {2014}
}
@article{Results1994b,
abstract = {As a concluding comment, I should like to return to the point raised by Ayres, that it is not enough simply to tell a better version of the fourth-century history in the expectation that modern theologians will finally get it straight! This is a valid point: if we want to have Christianity's fourth-century heritage taken seriously, we need to be in dialogue with modern writers. But, if there is to be a dialogue, both sides must be allowed to speak, and so we are also responsible for expounding the historical material on its own terms. As Heidegger put it, “[O]nly when we think through what has been thought will we be of any use for what must still be thought.” Perhaps studying the figures from a distant era will open up for us possibilities we would never have dreamed of within our own modern presuppositions, so that we can recognize differences even beyond those which lie within our own horizon or tradition. If I am right in affirming that there is a different style of doing theology prior to Augustine and after him in the East than that which we find in the theological and scholarly tradition in which Ayres's book stands, then we must ask whether we need to address the question of the legitimacy of each (and ponder how one might even answer that) or whether a plurality of approaches is possible without reducing one to the other. In a way, this would be a further step toward deconstructing monolithic notions of “Orthodoxy” in recognition of genuine and legitimate diversity within early Christianity and among modern Christians. Might it be better not to speak of Nicaea and its legacy, but of the legacies of Nicaea—or better—“Christ and him crucified” (2 Cor 2:2) and the ways in which Nicaea and its interpreters affirm the true divinity of this one?},
author = {Results, Useful},
doi = {10.1007/BF02600226},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2010{\_}Jaroslav Pokluda+Pavel {\v{S}}andera{\_}Micromechanisms of fracture and fatigue{\_}Buch/Kap5{\_}FinalReflection.pdf:pdf},
isbn = {9780470434673},
issn = {08848734},
journal = {J. Gen. Intern. Med.},
number = {3 Supplement},
pages = {243--247},
title = {{Final reflections}},
volume = {9},
year = {1994}
}
@article{Sandoval2003,
abstract = {A spark-ignition engine friction model developed by Patton et al. in the late 1980s was evaluated against current engine friction data, and improved. The model, which was based on a combination of fundamental scaling laws and empirical results, includes predictions of rubbing losses from the crankshaft, reciprocating, and valvetrain components, auxiliary losses from engine accessories, and pumping losses from the intake and exhaust systems. These predictions were based on engine friction data collected between 1980 and 1988. Some of the terms are derived from lubrication theory. Other terms were derived empirically from measurements of individual friction components from engine teardown experiments. Recent engine developments (e.g., improved oils, surface finish on piston liners, valve train mechanisms) suggested that the model needed updating. So modifications were made to the piston ring tension and gas pressure loading contributions to piston assembly friction, the impact of liner roughness, and to the valvetrain mechanism friction. Lubricant viscosity scaling was added to the hydrodynamic terms in the rubbing friction component models. The improved model now gives reasonable estimates of individual friction component and total spark-ignition engine friction mean effective pressure. The inclusion of oil viscosity scaling with temperature results in cold engine friction predictions about twice the value for warmed up engines. This agrees with the limited cold engine friction data available in the literature.},
archivePrefix = {arXiv},
arxivId = {2003-01-0725},
author = {Sandoval, Daniel and Heywood, John B},
doi = {10.4271/2003-01-0725},
eprint = {2003-01-0725},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2003{\_}Sandoval{\_}An Imporved Friction Model for Spark{\_}Ign Engines.pdf:pdf},
isbn = {0148-7191},
title = {{An Improved Friction Model for Spark-Ignition Engines}},
url = {http://papers.sae.org/2003-01-0725/},
year = {2003}
}
@article{Wirsching1983,
abstract = {Two methods are discussed for constructing a design curve on the safe side of fatigue data. Both the tolerance interval and equivalent prediction interval (EPI) concepts provide such a curve while accounting for both the distribution of the estimators in small samples and the data scatter. The EPI is also useful as a mechanism for providing necessary statistics on S-N data for a full reliability analysis which includes uncertainty in all fatigue design factors. Examples of statistical analyses of the general strain life relationship are presented. The tolerance limit and EPI techniques for defining a design curve are demonstrated. Examples usng WASPALOY B and RQC-100 data demonstrate that a reliability model could be constructed by considering the fatigue strength and fatigue ductility coefficients as two independent random variables. A technique given for establishing the fatigue strength for high cycle lives relies on an extrapolation technique and also accounts for "runners." A reliability model or design value can be specified.},
author = {Wirsching, P H},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Probabilistic Aspects/1983{\_}Wirsching{\_}Statistical summaries of fatigue data for design purposes.pdf:pdf},
issn = {05657059},
journal = {Nasa Cr 3697},
number = {July},
title = {{Statistical Summaries of Fatigue Data for Design Purposes}},
year = {1983}
}
@article{Rhouma2011a,
author = {Rhouma, W Ben and Deschanel, S and Weiss, J},
doi = {10.1063/1.3637920},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2011{\_}Weiss{\_}Collective Dislocation Dynamics and avalanches during fatigue of aluminium.pdf:pdf},
isbn = {9780735409569},
issn = {0094243X},
journal = {AIP Conf. Proc.},
keywords = {acoustic emission,damage,dislocations,fatigue,microstructure},
number = {May},
pages = {1536--1539},
title = {{Collective dislocation dynamics and avalanches during fatigue of aluminum}},
volume = {1389},
year = {2011}
}
@article{Depcik2002d,
abstract = {In this paper, the available correlations proposed in the literature for the gas-side heat transfer in the intake and exhaust system of a spark-ignition internal combustion engine were surveyed. It was noticed that theseAB - {\textless}inline-graphic xlink:href="2002-01-0372{\_}fig0001" xmlns:xlink="http://www.w3.org/1999/xlink"/{\textgreater}AB - only by empirically fitted constants. This similarity provided the impetus for the authors to explore if a universal correlation could be developed. Based on a scaling approach using microscales of turbulence, the authors have fixed the exponential factor on the Reynolds number and thus reduced the number of adjustable coefficients to just one; the latter can be determined from a least squares curve-fit of available experimental data. Using intake and exhaust side data, it was shown that the universal correlationAB - {\textless}inline-graphic xlink:href="2002-01-0372{\_}fig0002" xmlns:xlink="http://www.w3.org/1999/xlink"/{\textgreater}AB - The correlation coefficient of this proposed heat transfer model with all available experimental data is 0.845 for the intake side and 0.800 for the exhaust side.ER -},
author = {Depcik, Christopher and Assanis, Dennis},
doi = {10.4271/2002-01-0372},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2002{\_}Assanis{\_}A Universal Heat Transfer Correlation for Intake and Exhaust flows in an SI INternal Combustion Engine.pdf:pdf},
journal = {SAE Pap.},
number = {January 2016},
title = {{A Universal Heat Transfer Correlation for Intake and Exhaust Flows in an Spark-Ignition Internal Combustion Engine}},
url = {http://papers.sae.org/2002-01-0372},
volume = {2002-01-03},
year = {2002}
}
@article{Robinson2003,
author = {Robinson, J. S. and Cudd, R. L. and Evans, J. T.},
doi = {10.1179/026708303225009373},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Empirical Fatigue Models + Validation/2003{\_}Robinson{\_}Creep resistant aluminium alloys - experiments overview with different alloys - Al2618T6.pdf:pdf},
issn = {0267-0836},
journal = {Mater. Sci. Technol.},
number = {2},
pages = {143--155},
title = {{Creep resistant aluminium alloys and their applications}},
url = {http://www.tandfonline.com/doi/full/10.1179/026708303225009373},
volume = {19},
year = {2003}
}
@article{Kommunalbereich1897,
author = {Kommunalbereich, Der},
title = {18.1.1},
year = {1897}
}
@inbook{Eifler2009,
abstract = {Aufgaben der Hauptbauteile des Motors sind die Steuerung des Ladungswechsels, die Realisierung der Verbrennung, die Aufnahme der entstehenden Gaskr{\{}{\"{a}}{\}}fte und die Umwandlung dieser Kr{\{}{\"{a}}{\}}fte in ein nutzbares Drehmoment. Zylinderkopf und Kurbelgeh{\{}{\"{a}}{\}}use dienen dabei als Lagerung und F{\{}{\"{u}}{\}}hrung der bewegten Bauteile des Kurbel- und Ventiltriebes.},
address = {Wiesbaden},
booktitle = {K{\"{u}}ttner Kolbenmaschinen},
doi = {10.1007/978-3-8348-9302-4_4},
pages = {231--522},
publisher = {Vieweg+Teubner},
title = {{Brennkraftmaschinen}},
year = {2009}
}
@article{Topologieoptimierung1980,
author = {Topologieoptimierung, Methoden and Topologie, Die},
title = {{8 Methoden zur Topologieoptimierung}},
year = {1980}
}
@article{Mizuno2009b,
abstract = {This study examined a method of predicting the piston temperature in reciprocating internal combustion engines with the aim of developing lightweight pistons. Since the piston temperature is strongly affected by the in-cylinder temperature distribution and turbulence, it is necessary to consider the effects of flame propagation, cooling by the intake air, temperature rise due to combustion, in-cylinder flow and the combustion chamber shape. A three-dimensional combustion simulation that can take these effects into consideration was run to calculate the heat transfer coefficient from the piston crown surface and the gas temperature. The results were used as the boundary conditions for an analysis of heat transfer from the piston, and a method was thus developed for analyzing the piston temperature. The hardness method was used to obtain the piston temperature distribution and maximum temperature during engine operation, and a comparison was made with the analytical results to examine the effects of flame propagation.},
author = {Mizuno, Hideaki and Ashida, Koichi and Teraji, Atsushi and Ushijima, Kenshi and Takemura, Shinichi},
doi = {10.4271/2009-01-0187},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2009{\_}Mizuno{\_}Transient Analysis of the Piston Temperature with Measurement and Simulation.pdf:pdf},
journal = {SAE Int. J. Engines},
number = {1},
pages = {2009--01--0187},
title = {{Transient Analysis of the Piston Temperature with Consideration of In-cylinder Phenomena Using Engine Measurement and Heat Transfer Simulation Coupled with Three-dimensional Combustion Simulation}},
volume = {2},
year = {2009}
}
@article{Ekh2004a,
abstract = {We develop a model framework for anisotropic damage coupled to crystal (visco)plasticity, which is based on the concept of a fictitious (undamaged) configuration. The theoretical setting is that of finite strains, which is natural when studying crystal inelasticity even in the case of actual small strains. It turns out that the evolution law for damage, which reflects degradation in the slip planes and which is the key new relation, bears strong resemblance with the inelastic flow rule. Some numerical results showing qualitatively the anisotropic development of damage concludes the paper. ?? 2004 Elsevier Ltd. All rights reserved.},
author = {Ekh, Magnus and Lillbacka, Robert and Runesson, Kenneth},
doi = {10.1016/j.ijplas.2004.04.007},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2004{\_}Ekh{\_}A model framework for anisotropic damage coupled to crystal visco plasticity.pdf:pdf},
isbn = {0749-6419},
issn = {07496419},
journal = {Int. J. Plast.},
keywords = {Anisotropy,Crystal plasticity,Damage,Finite deformations},
number = {12},
pages = {2143--2159},
title = {{A model framework for anisotropic damage coupled to crystal (visco)plasticity}},
volume = {20},
year = {2004}
}
@article{Konstruktiona,
author = {Konstruktion, C Manuelle},
pages = {184--188},
title = {{26 Hinterwagen}}
}
@article{Kramer2012,
abstract = {Material parameter identification is the necessary link between constitutive modeling and application of material models in complex simulations of real world problems. We present an approach to make use of already developed stress algorithms for three-dimensional finite-element computations in terms of a reduction to uniaxial tensile tests for material parameter identification. Strain-driven stress algorithms lead to the approach of solving differential-algebraic equations. ({\textcopyright} 2012 Wiley-VCH Verlag GmbH {\&} Co. KGaA, Weinheim)},
author = {Kr{\"{a}}mer, Stephan and Rothe, Steffen and Hartmann, Stefan},
doi = {10.1002/pamm.201210147},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Parametersch{\"{a}}tzung/2012{\_}Hartmann{\_}Material parameter identification using model reduction to uniaxial tensile test.pdf:pdf},
issn = {1617-7061},
journal = {Pamm},
number = {1},
pages = {315--316},
title = {{Material parameter identification using model reduction to uniaxial tensile test}},
url = {http://dx.doi.org/10.1002/pamm.201210147},
volume = {12},
year = {2012}
}
@article{Garbe,
author = {Garbe, Juergen and Martinsohn, Matthias},
pages = {801--810},
title = {{C7 C7 Fahrzeugschl{\"{u}}ssel C7}}
}
@article{Zienkiewicz2014b,
abstract = {Summary In Chapter 2 we presented a framework for solving general problems in solid mechanics. In this chapter we consider several classical models for describing the behaviour of engineering materials. Each model we describe is given in a strain-driven form in which a strain or strain increment obtained from each finite element solution step is used to compute the stress needed to evaluate the internal force, [sigma] BT[sigma] d[Omega], as well as a tangent modulus matrix, or its approximation, for use in constructing the tangent stiffness matrix. Quite generally in the study of small deformation and inelastic materials (and indeed in some forms applied to large deformation) the strain (or strain rate) or the stress is assumed to split into an additive sum of parts. We can write this as [epsilon]=[epsilon]e+[epsilon]i (4.1) or [sigma]=[sigma]e+[sigma]i (4.2) in which we shall generally assume that the elastic part is given by the linear model [epsilon]e=D-1[sigma] (4.3) in which D is the matrix of elastic moduli.},
author = {Zienkiewicz, O.C. and Taylor, R.L. and Fox, David},
doi = {10.1016/B978-1-85617-634-7.00004-1},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Zienkiewicz FEM - Vol 2 Solid Structural Mechanics/63212{\_}04.pdf:pdf},
isbn = {978-0-75-066431-8},
issn = {0733-9399},
journal = {Finite Elem. Method Solid Struct. Mech.},
pages = {75--145},
pmid = {24603084},
title = {{Inelastic and Nonlinear Materials}},
url = {http://linkinghub.elsevier.com/retrieve/pii/B9781856176347000041},
year = {2014}
}
@book{Elshahawy2008a,
author = {Elshahawy, Waleed},
file = {:C$\backslash$:/Users/p327208/Desktop/Promotion/Literature/Homogenisierung Und Lokalisierung/Strukturmechanik MMS/Literatur/HS Schranken Methodik MMS Vorlesung Details/Yih 1981 Advances in Applied Mechanics Vol. 21{\_}WilliBeitragZumThemaHSSchranken{\_}SehrDetailliert.pdf:pdf},
isbn = {0120020211},
title = {{Advances i}},
year = {2008}
}
@article{Papula2009f,
author = {Papula, Lothar},
doi = {10.1007/978-3-8348-9598-1_15},
isbn = {978-3-8348-0757-1},
journal = {Math. Formelsammlung f{\"{u}}r Ingenieure und Naturwissenschaftler},
pages = {398--430},
title = {{XV Wahrscheinlichkeitsrechnung}},
year = {2009}
}
@article{Anforderungena,
author = {Anforderungen, Die and Sicherheitsaspekte, Die and Komfort, Beim and Handling-, Beim and Schr, Reifeneigenschaften and Winterreifen, Bei},
title = {{4 Reifenlastenheft}}
}
@article{Forest2004,
abstract = {The modeling of damage processes at the material point scale through a specific constitutive law addresses a wide variety of constitutive behaviors, for instance brittle elasticity where the evolution of damage degrades the elastic stiffness, or ductile plasticity where both dissipative mechanisms (plasticity and damage) are intimately coupled. In spite of their obvious differences, all these laws possess a common feature: beyond some load level, the domain of reversibility expressed in the stress space shrinks. This phenomenon is called strain-softening. This essential property, characteristic of damage mechanisms, is responsible for the localization of the mechanical fields (strain, damage, plastic strain, . . .) inside narrow bands, an experimental fact observed on many degrading materials such as soils, concrete, metals, etc., see for instance Desrues and Chambon (1985). Despite twenty years of intensive research, numerical modeling of the localization phenomenon remains a challenging objective which has not yet been given a fully satisfactory answer. This is in contrast with the great progresses that have been achieved regarding the local description of damage mechanisms for various materials, on the basis of micro–macro derivations as well as phenomenological intuitions. Unfortunately, localization partially hinders predictive computations of propagating damaged zones in real-life structures submitted to a given load history. The difficulty originates from the fact that the equations that describe the structural behavior (including not only the constitutive law but also the equilibrium and compat-ibility equations) result in an ill-posed problem which manifests itself by a spurious mesh-dependency when making use of finite element solutions. After a first insight into the localization phenomena, the problem of loss of uniqueness and loss of ellipticity is addressed for elastoplastic solids. General (diffuse) and localized bifurcation modes are distinguished. The existence of jumps of the velocity gradient is explored in the dynamic (acceleration waves) and static cases (stationary waves). Critical values of hardening moduli for loss of uniqueness or loss of ellipticity are derived. A link between the notion of material stability and acceleration waves is also presented. The collected strain localization criteria are summarized in section 1.2.6. Note that the derivations and formula are presented in the case of elastoplastic ma-terials. However the results can be extended to damaging materials in a straightforward 311 312 Local approach to fracture manner. In fact it deals with all incremental models involving a fourth–rank tangent operator L ∼ ∼ .},
author = {Forest, S and Lorentz, E},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/xxx{\_}Forst+Lorentz{\_}Localization{\_}phenomena{\_}and{\_}regularization{\_}methods-damage.pdf:pdf},
journal = {Local Approach to Fract.},
pages = {311--371},
title = {{Localization phenomena and regularization methods}},
volume = {1},
year = {2004}
}
@article{Weertman1956a,
abstract = {Polycrystalline samples of high purity aluminium have been tested in a strain rate machine over a wide temperature range. The relationship which exists between the maximum stress, strain rate, and temperature is strain rate = A (stress)4.4exp( — QRT) where A is a constant, R is the gas constant, T is the absolute temperature, Q is an activation energy equal to 36,000 cal/mole. The results are compared with those of Servi and Grant on constant stress creep tests and shown to be almost identical.},
author = {Weertman, J},
doi = {10.1016/0022-5096(56)90031-X},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Kriechen{\_}Spannungsrelaxation/1956{\_}Weertman{\_}Creep of polycrystalline aluminium as determined from strain rate tests.pdf:pdf},
isbn = {0022-5096},
issn = {00225096},
journal = {J. Mech. Phys. Solids},
number = {4},
pages = {230--234},
title = {{Creep of polycrystalline aluminium as determined from strain rate tests}},
url = {http://www.sciencedirect.com/science/article/pii/002250965690031X},
volume = {4},
year = {1956}
}
@article{Popov2009a,
author = {Popov, Valentin and Schargott, Martin},
file = {:C$\backslash$:/Users/p327208/Desktop/Promotion/Literature/Werkstoffkunde/Materialtheorie{\_}Versetzungen.pdf:pdf},
title = {{Materialtheorie}},
year = {2009}
}
@article{Murakami2012i,
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Murakami, Sumio},
doi = {10.1007/978-94-007-2666-6},
eprint = {arXiv:1011.1669v3},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/Continuum Damage Mechanics - SumioMurakami/Backmatter.pdf:pdf},
isbn = {978-94-007-2665-9},
issn = {09250042},
number = {1986},
pmid = {25246403},
title = {{Continuum Damage Mechanics}},
url = {http://link.springer.com/10.1007/978-94-007-2666-6},
volume = {185},
year = {2012}
}
@article{Ruzzene2009a,
abstract = {This article presents an overview of damage measures proposed in the area of structural health monitoring. This is an extremely active, open, and vast research field, as demonstrated by the variety of topics presented in this encyclopedia. The direction taken in this article is to present some examples of techniques that have been proposed, or that are promising tools for the estimation of location and extent of structural damage. All of the techniques considered are based on the analysis of the dynamic response of the structure under consideration. The organization of the article is based on the frequency range of analysis, which spans the low-frequency range, and correspondingly long response times, associated with the modal analysis of the structure, to frequencies associated with the propagation of guided ultrasonic waves. Hence, the methods presented belong to the classes of vibration-based and guided waves-based techniques. The damage measures discussed rely on the estimation of changes in modal parameters of the structure (natural frequencies, mode shapes, and strain energy distributions), or on features associated with the signal corresponding to the measured dynamic response. This overview is not meant to be exhaustive, but rather it provides examples of interesting solutions and approaches proposed in this area.},
author = {Ruzzene, M},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Probabilistic Aspects/A Unified Statistical Methodology for Modeling Fatigue Damage{\_}Castillo/Kap6{\_}Damage Measures.pdf:pdf},
isbn = {978-0-470-05822-0},
journal = {Encycl. Struct. Heal. Monit.},
keywords = {damage measures,guided ultrasonic waves,vibration-based technique},
number = {48},
pages = {----},
title = {{Damage measures}},
year = {2009}
}
@article{Tabellen,
author = {Tabellen, Die and Zahlenwerte, Tabelle and Gau{\ss}, Der},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Empirical Fatigue Models + Validation/Betriebsfestigkeit{\_}ErwinHaibach/Kap5 Anhang.pdf:pdf},
title = {{5 Anhang Daten zu statistischen Verfahren}}
}
@article{Papula2009f,
author = {Papula, Lothar},
doi = {10.1007/978-3-8348-9598-1_15},
isbn = {978-3-8348-0757-1},
journal = {Math. Formelsammlung f{\{}{\"{u}}{\}}r Ingenieure und Naturwissenschaftler},
pages = {398--430},
title = {{XV Wahrscheinlichkeitsrechnung}},
year = {2009}
}
@article{Wirkprinzip,
author = {Wirkprinzip, Aufgaben},
title = {8 8.1.2}
}
@article{Senga,
author = {Seng, Jocelyn M},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/{\_}buecherSong/HandbookofComposites/III/30{\_}LaminateDesign.pdf:pdf},
journal = {Production},
title = {{Laminate design}}
}
@article{Aufgabea,
author = {Aufgabe, Die and Fol, Eine and Vielzahl, Die and Din, Die Norm},
pages = {1--3},
title = {{Einf{\{}{\"{u}}{\}}hrung}}
}
@article{Sanli2009b,
author = {Sanli, A. and Sayin, C. and Gumus, M. and Kilicaslan, I. and Canakci, M.},
file = {:C$\backslash$:/Users/p327208/Desktop/Promotion/Literature/Motorspezifisch/2009{\_}Sanli{\_}Numerical evaluation by models of load and spark timing effects on the in-cylinder heat transfer of a si engine.pdf:pdf},
journal = {Numer. Heat Transf. Part A Appl.},
number = {5},
pages = {444--458},
title = {{Numerical Evaluation by Models of Load and Spark Timing Effects on the In-Cylinder Heat Transfer of a SI Engine}},
volume = {56},
year = {2009}
}
@article{Nicoletto1989,
author = {Nicoletto, G},
keywords = {alumi-,cyclic plastic zone,effective stress intensity factor,fatigue crack growth,moir6 interferometry,monotonic plastic zone,nium alloy,overload,range,steels},
number = {2},
pages = {107--115},
title = {{P l a s t i c z o n e s a b o u t f a t i g u e c r a c k s in metals}},
volume = {2},
year = {1989}
}
@article{Klein2009,
author = {Klein, Bernd},
isbn = {9783834802965},
title = {{Leichtbau Konstruktionen}},
year = {2009}
}
@article{Corti2016,
abstract = {Recent trends in gasoline engines, such as downsizing, downspeeding and the increase of the compression ratio make knocking combustions a serious limiting factor for engine performance. A detailed analysis of knocking events can help improving the engine performance and diagnostic strategies. An effective way is to use advanced 3D Computational Fluid Dynamics (CFD) simulation for the analysis and prediction of the combustion process. The effects of Cycle to Cycle Variation (CCV) on knocking combustions are taken into account, maintaining a RANS (Reynolds Averaged Navier-Stokes) CFD approach, while representing a complex running condition, where knock intensity changes from cycle to cycle. The focus of the numerical methodology is the statistical evaluation of the local air-to-fuel and turbulence distribution at the spark plugs and their correlation with the variability of the initial stages of combustion. CFD simulations have been used to reproduce knock effect on the cylinder pressure trace. For this purpose, the CFD model has been validated, proving its ability to predict the combustion evolution with respect to SA variations, from non-knocking up to heavy knocking conditions. The pressure traces simulated by the CFD model are then used to evaluate cylinder pressure-based knock indexes. Since the model is able to output other knock intensity tracers, such as the mass of fuel burned in knocking mode, or the local heat transferred to the piston, knock indexes based on the cylinder pressure trace can be related to parameters only available in a simulation environment, that are likely to be more representative of the actual knock intensity, with respect to the local pressure trace for the sensor position. The possibility of simulating hundredths of engine cycle allows using the methodology to compare the indexes quality (correlation with actual knock intensity) on a statistical base.},
author = {Corti, Enrico and Forte, Claudio and Cazzoli, Giulio and Moro, Davide and Falfari, Stefania and Ravaglioli, Vittorio},
doi = {10.1016/j.egypro.2016.11.116},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Klopfen{\_}Ottomotor/2016{\_}Corti{\_}Comparison of knock indexes based on CFD analysis.pdf:pdf},
issn = {18766102},
journal = {Energy Procedia},
keywords = {CFD,Knock,Sensor position,Simulation},
number = {September},
pages = {917--924},
publisher = {The Author(s)},
title = {{Comparison of Knock Indexes Based on CFD Analysis}},
url = {http://dx.doi.org/10.1016/j.egypro.2016.11.116},
volume = {101},
year = {2016}
}
@article{Tsurushima2002a,
author = {Tsurushima, Tadashi and Kunishima, Eiji and Asaumi, Yasuo and Aoyagi, Yuzo and Enomoto, Yoshiteru},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2002{\_}Tsurushima{\_}The Effect of Knock on Heat Loss in HCCI Engines-Modified Woschni.pdf:pdf},
journal = {Sae},
number = {108},
title = {{The Effect of Knock on Heat Loss in Homogeneous Charge Compression Ignition Engines}},
volume = {1},
year = {2002}
}
@article{Peerlings2002,
abstract = {Continuum approaches to fracture regard crack initiation and growth as the ultimate consequences of a gradual, local loss of material integrity. The material models which are traditionally used to describe the degradation process, however, may predict premature crack initiation and instantaneous, perfectly brittle crack growth. This nonphysical response is caused by localisation instabilities due to loss of ellipticity of the governing equations and - more importantly - singularity of the damage rate at the crack tip. It is argued that this singularity results in instantaneous failure in a vanishing volume, even if ellipticity is not first lost. Adding strong nonlocality to the modelling is shown to preclude localisation instabilities and remove damage rate singularities. As a result, premature crack initiation is avoided and crack growth rates remain finite. Weak nonlocality, as provided by explicit gradient models, does not suffice for this purpose. In implementing the enhanced modelling, the crack must be excluded from the equilibrium problem and the nonlocal interactions in order to avoid unrealistic damage growth. ?? 2002 ??ditions scientifiques et m??dicales Elsevier SAS. All rights reserved.},
author = {Peerlings, R H J and {De Borst}, R and Brekelmans, W A M and Geers, M G D},
doi = {10.1016/S0997-7538(02)01211-1},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/2002{\_}Peerlings{\_}Localisation issues in local and nonlocal continuum approaches to fracture.pdf:pdf},
issn = {09977538},
journal = {Eur. J. Mech. A/Solids},
number = {2},
pages = {175--189},
title = {{Localisation issues in local and nonlocal continuum approaches to fracture}},
volume = {21},
year = {2002}
}
@article{Druckindizierung2008,
author = {Druckindizierung, Grundlagen Der},
pages = {39--114},
title = {{Verbrennungsdiagnostik}},
volume = {1},
year = {2008}
}
@article{Mroz2003a,
author = {Mr{\'{o}}z, Z and Maciejewski, J},
doi = {10.1007/978-3-540-36418-4_3},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Anisotropic Behaviouir of Damaged Materials{\_}Skrzypek{\_}ARTICEL/Kap3{\_}Failure Criteria and Compliance Variation of Anisotropically Damaged Materials.pdf:pdf},
isbn = {9783642055874},
issn = {16137736},
journal = {Lect. Notes Appl. Comput. Mech.},
keywords = {Failure condition,anisotropic damage,critical plane,strength variation},
pages = {75--112},
title = {{Failure Criteria and Compliance Variation of Anisotropically Damaged Materials}},
volume = {9},
year = {2003}
}
@article{Kaunea,
author = {Kaune, Vanessa and Janda, Daniel and Schliephake, Daniel},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Werkstoffkunde/Ueberblick{\_}Ausscheidungshaertung{\_}AluminiumLegierungen{\_}TUDarmstadt.pdf:pdf},
journal = {TU Darmstadt},
pages = {6},
title = {{Aush{\"{a}}rtung von Aluminiumlegierungen}},
url = {http://www.mawi.tu-darmstadt.de/media/phm/5semester/ausscheidungshrtungiv.pdf}
}
@article{Nutzfahrzeugen2007,
author = {Nutzfahrzeugen, Bei and Komponenten, Die and Anwendung, Baugruppen},
journal = {Direct},
title = {{7 Leistungs u ¨ bertragung in Nutzfahrzeuggetrieben}},
year = {2007}
}
@article{Zahoransky2013c,
author = {Zahoransky, Richard a. and Allelein, Hans-Josef and Schelling, Udo and Schwarz, Harald and Bollin, Elmar and Oehler, Helmut},
doi = {10.1007/978-3-8348-2279-6},
isbn = {978-3-8348-1869-0},
journal = {Energietechnik - Syst. zur Energieumwandlung},
pages = {327--349},
title = {{13 Windenergie}},
url = {http://www.springerlink.com/index/10.1007/978-3-8348-2279-6},
year = {2013}
}
@article{Felippa2008,
author = {Felippa, Carlos A},
doi = {10.1007/978-3-540-71001-1},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Fellippa 2007 - NonlinearFEM.pdf:pdf},
isbn = {978-3-540-71000-4},
issn = {0003-5599},
number = {August},
title = {{Nonlinear Finite Element Methods}},
url = {http://link.springer.com/10.1007/978-3-540-71001-1},
year = {2008}
}
@article{Zienkiewicz2000a,
author = {Zienkiewicz, O C and Taylor, R L},
doi = {10.1016/B978-1-85617-633-0.00034-4},
isbn = {9781856176330},
journal = {finite Elem. method Vol. 1 basis},
pages = {648--653},
title = {{Matrix diagonalization or lumping}},
year = {2000}
}
@article{Doquet1997a,
abstract = {The development of fatigue damage in Co45Ni specimens during push-pull and reversed torsion tests, performed inside a scanning electron microscope, was observed and the different stress states compared. It appeared that transgranular crack initiation and development is delayed and intergranular crack initiation promoted under torsional loading. This was explained in terms of reduced surface distortion at the emergence of persistent slip bands (PSBs) and smaller compatibility stresses at the PSB-matrix interfaces. The influence of the mechanical strength of grain boundaries on the difference between tensile and torsional fatigue lives is discussed.},
author = {Doquet, V},
doi = {10.1111/j.1460-2695.1997.tb00280.x},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/1996{\_}Doquet{\_}CRACK INITIATION MECHANISMS IN TORSIONAL FATIGUE.pdf:pdf},
issn = {8756758X},
journal = {Fatigue Fract. Eng. Mater. Struct.},
keywords = {-torsional fatigue,intergranular crack initiation},
number = {2},
pages = {227--235},
title = {{Crack Initiation Mechanisms in Torsional Fatigue}},
url = {http://doi.wiley.com/10.1111/j.1460-2695.1997.tb00280.x},
volume = {20},
year = {1997}
}
@article{Massenzahl,
author = {Massenzahl, Ein Atomkern Der and Kernladungszahl, Die},
doi = {10.1007/978-3-8348-9912-5},
isbn = {9783834899125},
journal = {Elektron},
pages = {19--30},
title = {{3 Physikalische Grundlagen}}
}
@article{Erfolg,
author = {Erfolg, Neutraler},
pages = {2--6},
title = {{Teil a}}
}
@article{Beispiel,
author = {Beispiel, Als and Feldgleichungen, Maxwellschen and Din, Nach},
title = {{6 Elektromagnetische Wechselwirkungen}}
}
@book{DeSouzaNeto2008,
abstract = {Two integration algorithms, namely the implicit return mapping and explicit sub-stepping schemes, are adopted in the anisotropic bounding surface plasticity model for cyclic behaviours of saturated clay and are implemented into finite element code. The model is a representative of a series of bounding surface models that have typical characteristics, including isotropic and kinematic hardening rules and a rotational bounding surface to capture complex but important cyclic behaviours of soils, such as cyclic shakedown and degradation. However, there is no explicit current yield surface in the model to which the conventional implicit algorithm returns the stress state back or the sub-stepping integration corrects the drift of the stress state. Hence, necessary modifications have been made for both of the integration schemes. First, the image stress point is mapped or corrected to the bounding surface instead of mapping back or correcting the stress state to the yield surface. Second, the unloading–loading criterion is checked to determine the image stress point rather than checking the yield criterion after giving the trial stress state in a conventional way. Comparative studies on the accuracy, stability and efficiency of the two integration schemes are conducted not only at the element level but also in solving boundary value problems of monotonic and cyclic bearing behaviours of rigid footings on saturated clay. For smaller strain increments, there is no significant difference in the accuracy between the two integration schemes, but the explicit integration shows a higher efficiency and accuracy. For relatively larger increments, the implicit return mapping algorithm presents good accuracy and more robustness, while the sub-stepping algorithm shows deteriorating accuracy and suffers the convergence problem. With the tolerance used in the present model, the bearing capacity of the rigid footing predicted by the return mapping algorithm is closer to the available analytical and numerical solutions, while the bearing capacity predicted by the sub-stepping algorithm shows a marginal increase.},
author = {{de Souza Neto}, E. A. and Peri, D. and Owen, D. R. J.},
doi = {10.1002/9780470694626},
isbn = {9780470694626},
issn = {0266352X},
title = {{Computational Methods for Plasticity}},
url = {http://doi.wiley.com/10.1002/9780470694626},
year = {2008}
}
@article{Voraussetzung,
author = {Voraussetzung, Die},
pages = {144--151},
title = {{11 Biegung offener Profilst{\{}{\"{a}}{\}}be}}
}
@article{Index2004,
author = {Index, Subject},
doi = {10.1016/B978-0-444-53238-1.00018-1},
isbn = {0065-2458},
issn = {0196-0644},
number = {12},
pages = {1104--1110},
pmid = {25160461},
title = {{Subject Index}},
volume = {11},
year = {2004}
}
@article{Clausert,
author = {Clausert, H and Mathis, W and Hoffmann, K and Wiesemann, G and Z{\"{u}}rneck, H},
journal = {H{\{}{\"{u}}{\}}tte},
pages = {1--180},
title = {{G-Elektrotechnik}}
}
@article{Bozza2011a,
abstract = {In the present paper a combined procedure for the quasi-dimensional modelling of heat transfer, combustion and knock phenomena in a "downsized" Spark Ignition two-cylinder turbocharged engine is presented. The procedure is extended to also include the effects consequent the Cyclic Variability. Heat transfer is modelled by means of a Finite Elements model. Combustion simulation is based on a fractal description of the flame front area. Cyclic Variability (CV) is characterized through the introduction of a random variation on a number of parameters controlling the rate of heat release (air/fuel ratio, initial flame kernel duration and radius, laminar flame speed, turbulence intensity). The intensity of the random variation is specified in order to realize a Coefficient Of Variation (COV) of the Indicated Mean Effective Pressure (IMEP) similar to the one measured during an experimental campaign. Moreover, the relative importance of the various concurring effects is established on the overall COV. A kinetic scheme is then solved within the unburned gas zone, characterized by different thermodynamic conditions occurring cycle-by-cycle. In this way, an optimal choice of the "knock-limited" spark advance is effected and compared with experimental data. Finally, the CV effects on the occurrence of individual knocking cycles are assessed and discussed. {\{}{\textcopyright}{\}} 2011 Global Science Press.},
author = {Bozza, Fabio and Siano, Daniela and Costa, Michela},
doi = {10.4208/aamm.10-10s2-04},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2011{\_}Bozza{\_}heat-transfer-knock-modeling-and-cyclic-variability-in-a-downsized-spark-ignition-turbocharged-engine.pdf:pdf},
issn = {20700733},
journal = {Adv. Appl. Math. Mech.},
keywords = {Cyclic variability,Finite elements in heat transfer,Internal combustion engines modelling,Knock},
number = {3},
pages = {310--326},
title = {{Heat transfer, knock modeling and cyclic variability in a "Downsized" spark-ignition turbocharged engine}},
volume = {3},
year = {2011}
}
@article{Grandin2002b,
abstract = {SI Engine knock is caused by autoignition in the unburnt part of the mixture (end-gas) ahead of the propagating flame. Autoignition of the end-gas occurs when the temperature and pressure exceeds a critical limit when comparatively slow reactions-releasing moderate amounts of heat-transform into ignition and rapid heat release.In this paper the difference in the heat released in the end-gas-by low temperature chemistry-between lean, rich, stochiometric, and stoichiometric mixtures diluted with cooled EGR was examined by measuring the temperature in the end-gas with Dual Broadband Rotational CARS. The measured temperature history was compared with an isentropic temperature calculated from the cylinder pressure trace. The experimentally obtained values for knock onset were compared with results from a two-zone thermodynamic model including detailed chemistry modeling of the end-gas reactions.},
author = {Grandin, B{\"{o}}rje and Denbratt, Ingemar and Bood, Joakim and Brackmann, Christian and Bengtsson, Per-Erik and Gogan, Adina and Mauss, Fabian and Sund{\'{e}}n, Bengt},
doi = {10.4271/2002-01-0239},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2002{\_}Grandin{\_}Heat Release in the End-Gas Prior to Knock in lean-rich-stoichiometric mixtures.pdf:pdf},
journal = {SAE Tech. Pap.},
number = {724},
title = {{Heat Release in the End-Gas Prior to Knock in Lean, Rich and Stoichiometric Mixtures With and Without EGR}},
url = {http://dx.doi.org/10.4271/2002-01-0239},
volume = {2002-01-02},
year = {2002}
}
@article{Schwan1998,
author = {Schwan, F J},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/{\_}buecherSong/HandbookofComposites/III/31{\_}DesignofStructurewithComposites.pdf:pdf},
journal = {Design},
title = {{Design of structure with composites 31}},
year = {1998}
}
@article{Schalenbauweise,
author = {Schalenbauweise, Die},
pages = {140--146},
title = {{21 Ausstattung 21.1}}
}
@article{Benjac2014Wurzenberger,
author = {Banjac, Titina and Wurzenberger, Johann C and Katrasnik, Tomaz},
doi = {10.1016/j.advengsoft.2014.01.016},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Thermal Coating + Water Heat Transfer + Applikation/2014{\_}Banjac{\_}Assessment of engine thermal management through advanced system engineering modeling.pdf:pdf},
journal = {Adv. Eng. Softw.},
keywords = {electrically driven coolant pump,engine thermal management,system level vehicle model},
pages = {19--33},
title = {{Assessment of engine thermal management through advanced system engineering modeling}},
volume = {71},
year = {2014}
}
@article{Svendsen1995,
abstract = {This work is concerned with the formulation of a constitutive model for a saturated or unsaturated, single-temperature mixture of n (???2) heat-conducting, isotropic viscous materials, the first m ??? n of which possess a variable true mass density. To do this, we extend the M??ller-Liu approach to the formulation and exploitation of the mixture entropy inequality. This approach yields, among other things, a generalized Gibbs' relation for such a mixture, as well as integrability conditions for the mixture entropy, and "extra" entropy flux, densities. Reduction of these general results to results comparable to those obtained in the standard approach necessitates two further constitutive assumptions: (1) the constraint field ("Lagrange multiplier") associated with the mixture reduced energy balance in the entropy inequality is equal to the mixture absolute coldness, and (2) that associated with the constituent momentum balance in the entropy inequality is equal to the negative of the mixture absolute coldness times the corresponding diffusion velocity. On this basis, for example, the inner parts of the mixture specific internal and Helmholtz free energies, as well as the mixture specific entropy, depend only on the mixture absolute temperature, the constituent true mass densities of the m "compressible" constituents, the volume densities of the first v constituents (with v = m in the unsaturated, and v = n - 1 in the saturated, case), and the constituent left Cauchy-Green deformation tensors. In the context of thermodynamic equilibrium, the entropy inequality yields, among other things, the interesting result that the constituent equilibrium thermodynamic pressure depends in a saturated mixture directly on the mixture saturation constraint field, but not on that associated with the evolution relations for the constituent (infinitesimal) volume fractions. As such, the so-called "closure problem" in volume-fraction-based mixture theory does not arise in the current formulation. ?? 1995.},
author = {Svendsen, Bob and Hutter, Kolumban},
doi = {10.1016/0020-7225(95)00044-X},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Thermodynamik/Liu-Entropieprinzip{\_}Lukas{\_}Fraunhofer/Liu-Entropieprinzip/Svendsen{\_}Hutter{\_}mixture{\_}with{\_}constraints{\_}1995.pdf:pdf},
issn = {00207225},
journal = {Int. J. Eng. Sci.},
number = {14},
pages = {2021--2054},
title = {{On the thermodynamics of a mixture of isotropic materials with constraints}},
volume = {33},
year = {1995}
}
@article{MOHAMED20161352,
author = {Mohamed, Eid S},
doi = {https://doi.org/10.1016/j.applthermaleng.2016.06.123},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Thermal Coating + Water Heat Transfer + Applikation/2016{\_}Mohamed{\_}Experimental study on the effect of active engine thermal management on a bi-fuel engine performance combustion and exhaust emissions.pdf:pdf},
journal = {Appl. Therm. Eng.},
keywords = {Active engine thermal management,Bi-fuel engine,Combustion characteristics,Emissions,Engine performance},
pages = {1352--1365},
title = {{Experimental study on the effect of active engine thermal management on a bi-fuel engine performance, combustion and exhaust emissions}},
volume = {106},
year = {2016}
}
@article{Allianz2003c,
author = {Allianz, Von M Pfender and Berlin, M{\"{u}}nchen},
isbn = {3540440631},
number = {2},
title = {{6 Schrifttumshinweise}},
volume = {6},
year = {2003}
}
@book{Riccardella1992e,
author = {Riccardella, P C and Deardorff, A F and Griesbach, T J},
booktitle = {Adv. Fatigue Lifetime Predict. Tech.},
doi = {10.1520/STP1122-EB},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Neuer Ordner/Advances in fatigue lifetime predictive techniques Part1.pdf:pdf},
isbn = {978-0-8031-1423-4},
issn = {00660558},
keywords = {FATIGUE,MONITORING,POWER PLANTS,PRESSURE VESSELS AND PIPING,THERMAL STRESSES},
pages = {460--473},
pmid = {11439068},
title = {{Advances in Fatigue Lifetime Predictive Techniques}},
url = {https://apps.webofknowledge.com/full{\%}7B{\_}{\%}7Drecord.do?product=UA{\%}7B{\&}{\%}7Dsearch{\%}7B{\_}{\%}7Dmode=GeneralSearch{\%}7B{\&}{\%}7Dqid=11{\%}7B{\&}{\%}7DSID=Z1UxbH6jtsqo8n9kPQr{\%}7B{\&}{\%}7Dpage=1{\%}7B{\&}{\%}7Ddoc=1},
volume = {1122},
year = {1992}
}
@article{Albers,
author = {Albers, Albert and Grundlagen, Allgemeine},
title = {{Kapitel 5}}
}
@article{Forest2009,
abstract = {A unifying thermomechanical framework is presented that reconciles several classes of gradient elastoviscoplasticity and damage models proposed in the literature during the last 40 years. It is based on the introduction of the micromorphic counterpart ϕ {\$}\chi{\$} of a selected ... {\$}\backslash{\$}n},
author = {Forest, Samuel},
doi = {10.1061/(ASCE)0733-9399(2009)135:3(117)},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/2009{\_}Forest{\_}Micromorphic Approach for Gradient Elasticity Viscoplasticity and Damage.pdf:pdf},
isbn = {0733-9399},
issn = {0733-9399},
journal = {J. Eng. Mech.},
number = {3},
pages = {117--131},
title = {{Micromorphic Approach for Gradient Elasticity, Viscoplasticity, and Damage}},
volume = {135},
year = {2009}
}
@article{Corti2009,
abstract = {Specific power and efficiency of gasoline engines are influenced by factors such as compression ratio and Spark Advance (SA) regulation. These factors influence the combustion development over the crank angle: the trade-off between performance and the risk of irreversible damages is still a key element in the design of both high-performance (racing) and low-consumption engines. This paper presents a novel approach to the problem, with the objective of defining a damage-related and operating conditions-independent index. The methodology is based on the combined analysis of indicating parameters, such as Cumulated Heat Release (CHR), Indicated Mean Effective Pressure (IMEP) and 50{\{}{\%}{\}} Mass Fraction Burned (MFB50), and typical knock detection parameters, estimated by means of the in-cylinder pressure sensor signal. Knocking combustions have several consequences, therefore they can be detected in many ways. As it is well known, knock excites the combustion chamber resonant frequencies, rising high frequency components in the in-cylinder pressure signal. Additionally, knocking combustions cause a higher heat flux through the combustion chamber walls, increasing the heat losses and lowering the IMEP: this effect can be observed by evaluating IMEP or CHR, that are based on the low-frequency content of the in-cylinder signal spectrum. A knock detection index can then be based on the crossed-observation of two phenomena, one set in the low-frequencies range and the other one on the high frequencies range of the in-cylinder pressure signal. Knock-related parameters have been analyzed with a statistical approach, in order to define a detection strategy based on one single threshold value, to be used for all the engines, independently of engine speed and load: IMEP and CHR have been related to a typical high-frequency knock index, based on the Maximum Amplitude of Pressure Oscillations (MAPO) evaluated over the combustion angular window. It can be observed that, as knock intensity increases, the relationships between these parameters change. This change can be seized by evaluating the correlation coefficient between the parameters distributions and observing its trend as a function of SA (Spark Advance). The correlation coefficient is intrinsically normalized, therefore the index range is the same for every engine operating condition, and the paper shows that the threshold level, too, is constant. The same approach can be applied to determine SA corresponding to the best combustion phase, simply by evaluating the correlation coefficient for IMEP and MFB50 distributions. The methodology has been successfully applied to different engines running in different speed and load conditions.},
author = {Corti, Enrico and Forte, Claudio},
doi = {10.4271/2009-24-0019},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Klopfen{\_}Ottomotor/2009{\_}Forte+Corti{\_}Statistical Analysis of Indicating Parameters for Knock Detection Purposes.pdf:pdf},
issn = {19463936},
journal = {SAE Tech. Pap.},
number = {2009-01-0237},
title = {{Statistical Analysis of Indicating Parameters for Knock Detection Purposes}},
url = {http://papers.sae.org/2009-01-0237/},
year = {2009}
}
@article{Eigenschaftsprofil,
author = {Eigenschaftsprofil, Das and Datenbanken, Diese and Best, Thema and Medien-, Bereichen and Tabellen, Kunststoff and Kunststoffe, Die},
pages = {228--239},
title = {{5 Werkstoffauswahl – Kunststoffe}}
}
@article{Desmorat2015a,
author = {Desmorat, Rodrigue and {Du Tertre}, Alban and Gaborit, Pierre},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/2 scale models papers/2015{\_}Desmorat{\_}Multiaxial Haigh Diagrams from incremental two scale damage analysis.pdf:pdf},
journal = {Aerosp. Lab J.},
number = {9},
pages = {1--15},
title = {{Multiaxial Haigh diagrams from incremental two scale damage analysis}},
volume = {en review},
year = {2015}
}
@article{Standardnormalverteilung,
author = {Standardnormalverteilung, Der},
title = {{Teil A: Tabellen zur Wahrscheinlichkeitsrechnung und Statistik}}
}
@article{Sozialisation1999,
author = {Sozialisation, Organisationale},
journal = {Forschung},
pages = {8--9},
title = {{Teil III :}},
year = {1999}
}
@article{Forestc,
author = {Forest, Samuel},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/Folien CISM Summer School Mai2017 - Mesoscale Models/courses{\_}C1703{\_}forest{\_}Forest1-Micromorphic.pdf:pdf},
title = {{Micromorphic media}}
}
@article{Roters2000,
abstract = {A new work-hardening model for homogeneous and heterogeneous cell-forming alloys is introduced. It distinguishes three internal state variables in terms of three categories of dislocations: mobile dislocations, immobile dislocations in the cell interiors and immobile dislocations in the cell walls. For each dislocation population an evolution law is derived taking into account dislocation generation, annihilation and storage by dipole and lock formation. In particular, these rate equations take into account the number of active glide systems and, thus, introduce texture in the model in addition to the Taylor factor. Microstructure is represented by the dislocation cell structure as well as second-phase particles, which may undergo changes by precipitation and Ostwald ripening. Interaction of mobile dislocations with the microstructure is taken into account through an effective slip length of the mobile dislocations. For the same set of parameters, the predictions are in excellent agreement with measured stress–strain curves of both a precipitation-hardened aluminium alloy (Al–4.16 wt{\{}{\%}{\}} Cu–1.37 wt{\{}{\%}{\}} Mg, AlCuMg2) and a precipitation-free model alloy (Al–0.35 wt{\{}{\%}{\}} Cu–0.25 wt{\{}{\%}{\}} Mg), the composition of which corresponds to the matrix of the two-phase alloy. Ein neues Verfestigungsmodell f{\{}{\"{u}}{\}}r homogene und heterogene Legierungen wird vorgestellt. Es werden drei innere Zustandsvariablen in Form von drei Versetzungsklassen unterschieden, mobile Versetzungen, immobile Versetzungen im Zellinnern und immobile Versetzungen in den Zellw{\{}{\"{a}}{\}}nden der Substruktur. F{\{}{\"{u}}{\}}r die Dichte jeder dieser Versetzungsklassen wird eine Evolutionsgleichung hergeleitet, die Versetzungsproduktion, -annihilation und -speicherung durch Bildung von Dipolen und se{\{}{\ss}{\}}haften Versetzungsreaktionsprodukten ber{\{}{\"{u}}{\}}cksichtigt. Insbesondere wird dabei die Zahl der aktiven Gleitsysteme ber{\{}{\"{u}}{\}}cksichtigt, wodurch die Textur zus{\{}{\"{a}}{\}}tzlich zum Taylorfaktor in das Modell einflie{\{}{\ss}{\}}t. Die Mikrostruktur wird durch die Versetzungszellstruktur und Sekund{\{}{\"{a}}{\}}rphasen repr{\{}{\"{a}}{\}}sentiert, wobei letztere Ausscheidungs- und Reifungsprozessen unterworfen sind. Die Wechselwirkung der mobilen Versetzungen mit der Mikrostruktur wird durch eine effektive freie Wegl{\{}{\"{a}}{\}}nge der mobilen Versetzungen ber{\{}{\"{u}}{\}}cksichtigt. Die Modellvorhersagen stimmen bei gleichem Parametersatz sehr gut mit gemessenen Spannungs-Dehnungs-Kurven einer ausscheidungsh{\{}{\"{a}}{\}}rtbaren Aluminiumlegierung (Al–4.16 wt{\{}{\%}{\}} Cu–1.37 wt{\{}{\%}{\}} Mg, AlCuMg2) und einer ausscheidungsfreien Modellegierung (Al–0.35 wt{\{}{\%}{\}} Cu–0.25 wt{\{}{\%}{\}} Mg), die der Matrix des zweiphasigen Werkstoffs entspricht, {\{}{\"{u}}{\}}berein.},
author = {Roters, F and Raabe, D and Gottstein, G},
doi = {10.1016/S1359-6454(00)00289-5},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/Hardening Recovery Creep/2000{\_}GOTTSTEIN{\_}Work hardening in heterogeneous alloys - a microstructural approach based on three internal state variables.pdf:pdf},
isbn = {1359-6454},
issn = {13596454},
journal = {Acta Mater.},
keywords = {Alloys,Dislocations,Dislocations-theory,Mechanical properties,aluminium,mobility,plastic},
number = {17},
pages = {4181--4189},
title = {{Work hardening in heterogeneous alloys—a microstructural approach based on three internal state variables}},
url = {http://www.sciencedirect.com/science/article/pii/S1359645400002895},
volume = {48},
year = {2000}
}
@article{V.Winterfeldt,
author = {V.Winterfeldt, J Schade},
journal = {H{\{}{\"{u}}{\}}tte},
pages = {1--21},
title = {{Q-Patente}}
}
@article{Wahrnehmung,
author = {Wahrnehmung, Deren and Augen, Die and Generation, Von and Reifen, Schnittstelle and Reifen, Der and Reifen, Beim and Fahrzeugen, Bei and Ph, Dieses and Resonanzlage, Die and Felge-seitenwand-stahlg, Resonanzsystem},
title = {{9 Ger{\"{a}}usche und Schwingungen}}
}
@book{Course2006,
author = {Course, First},
booktitle = {Engineering},
doi = {10.1002/9780470510858},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Fish, Belytschko 2007 - A First Course In Finite Elements.pdf:pdf},
isbn = {9780470035801},
title = {{First Course in Finite Elements}},
year = {2006}
}
@article{Space1996a,
author = {Space, On},
file = {:C$\backslash$:/Users/p327208/Desktop/Promotion/Literature/Homogenisierung Und Lokalisierung/Strukturmechanik MMS/Literatur/Matthies, Muller, Vinel - 1988.pdf:pdf},
journal = {Imagine},
keywords = {component fit,model functions,normal distribution,odf analysis},
number = {C},
pages = {77--96},
title = {{On Space}},
volume = {10},
year = {1996}
}
@article{Zienkiewicz2014c,
author = {Zienkiewicz, O.C. and Taylor, R.L. and Fox, David},
doi = {10.1016/B978-1-85617-634-7.00005-3},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Zienkiewicz FEM - Vol 2 Solid Structural Mechanics/63212{\_}05.pdf:pdf},
journal = {Finite Elem. Method Solid Struct. Mech.},
pages = {147--177},
title = {{Geometrically Nonlinear Problems: Finite Deformation}},
url = {http://linkinghub.elsevier.com/retrieve/pii/B9781856176347000053},
year = {2014}
}
@article{Petukhov1970,
author = {Petukhov, B S},
doi = {https://doi.org/10.1016/S0065-2717(08)70153-9},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Heat transfer intake+exhaust system/1970{\_}Petukhov{\_}Heat Transfer and Friction in Turbulent Pipe Flow with Variable Physical Properties.pdf:pdf},
journal = {Adv. Heat Transf.},
pages = {504--564},
title = {{Heat Transfer and Friction in Turbulent Pipe Flow with Variable Physical Properties}},
volume = {6},
year = {1970}
}
@article{Gem2006,
author = {Gem, Gubelin and Opt, Erweiterungen},
number = {2251},
pages = {1--8},
title = {{1 {\"{U}}bersicht}},
year = {2006}
}
@article{Gleichgewicht,
author = {Gleichgewicht, Chemisches},
pages = {167--188},
title = {{Reaktionskinetik}},
volume = {1}
}
@article{Frenz2008,
author = {Frenz, Walter},
doi = {10.1007/978-3-540-71852-9_16},
isbn = {978-3-540-71851-2},
journal = {H{\{}{\"{u}}{\}}tte},
pages = {P1----P26},
title = {{P-Recht}},
year = {2008}
}
@article{Merker,
author = {Merker, G{\"{u}}nter and Schwarz, Christian},
pages = {189--219},
title = {{Schadstoffbildung}}
}
@article{Universit2001b,
author = {Universit, Technischen},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Kolben FEM/Werkstoffgerechte Auslegung und Festigkeitsnachweis f{\"{u}}r Verbrennungsmotorkolben.pdf:pdf},
title = {{Technische Universit{\"{a}}t M{\"{u}}nchen Institut f{\"{u}}r Werkstoffe und Verarbeitung Forschungsgruppe Prof . Schmitt-Thomas Werkstoffgerechte Auslegung und Festigkeitsnachweis f{\"{u}}r Verbrennungsmotorkolben aus Mesophasenkohlenstoff}},
year = {2001}
}
@article{Boshers2001,
author = {Boshers, Chris},
doi = {10.1361/asmhba0003393},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/{\_}buecherSong/HandbookofComposites/III/33{\_}DesignAllowablesSubstantiation.pdf:pdf},
journal = {Composites},
pages = {360--365},
title = {{Design Allowables}},
volume = {21},
year = {2001}
}
@article{Ergonomie,
author = {Ergonomie, Die and Arbeitsplatzgestal-, Bereiche and Auslegung, Die and Modelle, Rechner-mensch- and Konzeptvarianten, Diese and Bedienkonzepte, Die and Designmodelle, Die and Aktivit, Diese and Erkenntnisse, Die},
pages = {10--15},
title = {{7 Ergonomie}}
}
@article{Pineau2016a,
abstract = {In this interpretive review, fatigue in metallic systems is considered primarily from the perspective of interactions between the microstructure, the deformation mode and the mechanical state at both low and high temperatures. In Part 1 the development and early propagation of cracks is considered in terms of the basic damage mechanisms and the relative size of the crack with respect to applicable microstructural feature(s). In this section, a multistage grain scale approach to microstructure-sensitive fatigue crack formation and growth is presented which uses Fatigue Indicator Parameters (FIPs) to correlate these processes. Various FIPs parameters are discussed in terms of their indication of the state of fatigue. The development and early crack propagation is considered in the context of microstructure and notches, and probabilistic aspects of the notch fatigue problem are discussed. These features are integrated into a systematic approach for the selection of fatigue resistant microstructures for given applications. In Part 2, attention is focused on Ni-base superalloys and the interaction between oxidation, creep and microstructure (including coatings) in the formation and propagation of cracks. This part of the overview addresses both experimental and modelling aspects. Methodologies based upon fundamental physical processes are presented for understanding and predicting the development and propagation of fatigue cracks, including effects of sequential oxide type formation and of creep on either restraining or accelerating damage by oxidation. The variable fatigue resistance of discs in jet engines is seen to depend upon the variability of microstructure and its influence on the severity of creep/oxidation interactions. All of these factors are considered in the practical case where both temperature and loading parameters vary simultaneously (thermomechanical fatigue). A physics-based life prediction model considering the interactions of deformation and environmental damage is reviewed in terms of its applicability to life prediction of components.},
author = {Pineau, Andr?? and McDowell, David L and Busso, Esteban P and Antolovich, Stephen D},
doi = {10.1016/j.actamat.2015.05.050},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/2016{\_}Pineau + McDowell{\_}Failure of metals II Fatigue.pdf:pdf},
isbn = {13596454},
issn = {13596454},
journal = {Acta Mater.},
keywords = {Environment-microstructure interaction,Fatigue in metallic alloys,Intergranular cracking,Local and global fatigue approaches,Multistage fatigue,Oxidation,Superalloys,thermomechanical fatigue},
pages = {484--507},
title = {{Failure of metals II: Fatigue}},
volume = {107},
year = {2016}
}
@article{Caresana2011Num,
author = {Caresana, F and Bilancia, M and Bartolini, C M},
doi = {https://doi.org/10.1016/j.applthermaleng.2011.07.017},
journal = {Appl. Therm. Eng.},
keywords = {Cooling system,Engine thermal management,Fuel consumption reduction,Heat transfer coefficient,nucleate boiling},
number = {16},
pages = {3559--3568},
title = {{Numerical method for assessing the potential of smart engine thermal management: Application to a medium-upper segment passenger car}},
volume = {31},
year = {2011}
}
@article{Brookfield2008,
abstract = {This chapter contains section titled: * Age equivalence * Relative ages * Numerical methods (ages in years) * Calibration of relative and numerical dates},
author = {Brookfield, Michael E},
doi = {10.1002/9780470694015.ch7},
isbn = {9780470694015},
issn = {0015900X},
journal = {Princ. Stratigr.},
keywords = {crucifixion,geologic time,geologists,planets,relative ages},
pages = {140--170},
title = {{The Time Dimension}},
url = {http://dx.doi.org/10.1002/9780470694015.ch7{\%}0Ahttp://onlinelibrary.wiley.com/doi/10.1002/9780470694015.ch7/summary},
year = {2008}
}
@article{Berger2003a,
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Berger},
doi = {10.1002/ejoc.201200111},
eprint = {arXiv:1011.1669v3},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Vortraege/Book-of-Abstracts{\_}2016-03-04{\_}GAMM.pdf:pdf},
isbn = {9781107671812},
issn = {0196-6553},
journal = {Eng. Med. Biol. Soc. 2008. EMBS 2008. 30th Annu. Int. Conf. IEEE},
pages = {2004},
pmid = {26840611},
title = {{Table of of contents}},
volume = {24},
year = {2003}
}
@article{Bauer1998,
abstract = {Entry flow heat transfer experiments are reported in steady and pulsating flows of air at mean Reynolds numbers of 3000-35 000. THe ducts are chosen to match typical spark-ignition engine manifolds: a highly curved and a straight pipe, which together bracket most practical geometries. The pulsating engine intake flow encompasses an approximate half sine wave followed by a stagnant phase three itmes as long, all at a repetition rate of 16-50 Hz. Heat flow is imposed through electric heating of the outsides of the manifolds. Heat transfer in the curved pipe is closely comparable to the straight geometry, and it is concluded that entrance effects dominate. Time-averaged axially resolved and axially averaged Nusselt numbers are reported. The unsteady nature of the intake flow enhances heat transfer significantly, between 50{\{}{\%}{\}} and 100{\{}{\%}{\}}. Time-resolved wall heat flux measurements at a location close to the exit of the system show that heat transfer is delayed relative to the onset of the flow. During the stagnant flow phase, heat transfer and turbulence decay slowly from their high levels during the induction flow phase. Heat transfer enhancement in the pulsating flow case is caused by the contribution of the stagnant phase.},
author = {Bauer, Wolf D and Wenisch, Joseph and Heywood, John B},
doi = {https://doi.org/10.1016/S0142-727X(97)10001-7},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/1998{\_}Bauer{\_}Averaged and time-resolved heat transfer of steady and pulsating entry flow in intake manifold of a SI engine.pdf:pdf},
journal = {Int. J. Heat Fluid Flow},
keywords = {intake manifold,internal combustion engine,ow,pulsating,transient heat,ux measurements},
number = {1},
pages = {1--9},
title = {{Averaged and time-resolved heat transfer of steady and pulsating entry flow in intake manifold of a spark-ignition engine}},
volume = {19},
year = {1998}
}
@article{Spur2008,
author = {Spur, G},
journal = {H{\"{u}}tte - Das Ingenieurwissen},
pages = {1746 -- 1801},
title = {{Produktion}},
year = {2008}
}
@article{Klein2009a,
author = {Klein, Bernd},
doi = {10.1007/978-3-8348-9965-1_18},
isbn = {978-3-8348-0701-4},
journal = {Leichtbau-Konstruktion},
pages = {215--231},
title = {{Stabilit{\"{a}}t von St{\"{a}}ben und Balken}},
year = {2009}
}
@article{Industrie,
author = {Industrie, Die and Bem, Viele and Gewichts-, Die and Schwerpunkt, Der and Grenzbedingungen, Als},
pages = {297--305},
title = {{13 Bauteiloptimierung}}
}
@article{Pol??k2016,
abstract = {Results of the study of the early fatigue damage in a number of model and structural crystalline materials using modern experimental techniques are presented. The dislocation structure of the persistent slip bands and the evolution of the surface relief resulting in the formation of persistent slip markings during cyclic loading are documented. The dislocation mechanisms leading to production of point defects in cyclic loading are described and point defect production and annihilation rates are derived. The kinetics of point defect migration is characterized. The physically based models of the surface relief formation describing the formation of extrusions and intrusions are presented. The models are confronted with experimental evidence. It is concluded that intrusions representing sharp surface crack-like defects play the principal role in the initiation of fatigue cracks.},
author = {Pol??k, Jaroslav and Man, Ji????},
doi = {10.1016/j.ijfatigue.2016.02.021},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/2016{\_}Polak+Man{\_}Experimental evidence and physical models of fatigue crack initiation.pdf:pdf},
issn = {01421123},
journal = {Int. J. Fatigue},
keywords = {Crack initiation,Extrusions,Intrusions,Persistent slip band,Point defects},
pages = {294--303},
title = {{Experimental evidence and physical models of fatigue crack initiation}},
volume = {91},
year = {2016}
}
@inproceedings{Sharief2008,
abstract = {Heat transfer in reciprocating combustion engine is an intricate phenomenon involving rapid cyclic variation of cylinder pressure temperature density and area of contacting surfaces. Rate of heat transfer in internal combustion engine is further complicated greatly due to the gas turbulence and flame radiation effects, the magnitudes of which depend on the engine type and operating conditions. It is necessary to calculate the heat flow, the temperature distribution and the temperature stresses. Hence, an accurate model for estimation of heat transfer in various phases of the cycle is an important factor which influences the accuracy of all parameters in the cycle analysis. Nearly more than twenty correlations have been proposed to find the heat transfer coefficient in the combustion chamber wall among which some of theoretical concepts. The large disagreement among the various proposed formulae for reciprocating engine heat transfer made it hard to choose any adequate e formula for universal application to various combustion engines. This paper proposes a modified heat transfer correlation based on experiments conducted in motored diesel engine with natural aspiration of hot air at around 150°C-300°C. The author considered the Intake jet velocity in place of mean piston speed in Reynold parameter in proposed heat transfer coefficient equation. The Intake jet velocity is better representative of gas velocity than the mean piston speed since it takes into account the diameter of inlet port of an engine and diameter of piston. Further, the proposed heat transfer correlation for Compression Ignition engine is validated by conducting experiments on a direct injection, four-stroke, single-cylinder, water-cooled diesel engine under fired conditions at different loads and different speeds. The formulated new heat transfer correlation is finally compared with other earlier correlations proposed by other researchers.ER -},
author = {Sharief, Abdul and Chandrashekar, T K and Antony.A.J and Samaga, B S},
booktitle = {SAE Tech. Pap. 2008-01-1816},
doi = {10.4271/2008-01-1816},
file = {:C$\backslash$:/Users/p327208/Desktop/Promotion/Literature/Motorspezifisch/2008.{\_}Sharief{\_}Study on Heat Transfer Correlation in IC Enginespdf.pdf:pdf},
publisher = {SAE international},
title = {{Study on Heat Transfer Correlation in IC Engines}},
year = {2008}
}
@article{CARPINTERI2001a,
abstract = {Some multiaxial high-cycle fatigue criteria based on the so-called critical plane approach are reviewed. According to such an approach, the critical plane where the fatigue life assessment should be performed can be determined by maximising the amplitudes and/or values of some stress components. In the present paper, the critical plane orientation is correlated with the averaged principal stress directions deduced through the weight function method, and a new fatigue failure criterion is proposed. The results derived by applying the present criterion and the other critical plane criteria analysed are compared with experimental data related to different brittle (hard) metals under in-phase or out-of-phase sinusoidal biaxial normal and shear stress states. 0},
author = {CARPINTERI, A and SPAGNOLI, A},
doi = {10.1016/S0142-1123(00)00075-X},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Empirical Fatigue Models + Validation/2000{\_}Carpinteri{\_}Multiaxial high cycle fatigue criterion for hard metals.pdf:pdf},
isbn = {0142-1123},
issn = {01421123},
journal = {Int. J. Fatigue},
keywords = {multiaxial},
number = {2},
pages = {135--145},
title = {{Multiaxial high-cycle fatigue criterion for hard metals}},
url = {http://linkinghub.elsevier.com/retrieve/pii/S014211230000075X},
volume = {23},
year = {2001}
}
@article{Mughrabi2010a,
abstract = {In the first part, some fundamental issues that have been under discussion for a long time will be revisited, namely the effect of the cyclic slip mode on the fatigue-induced dislocation distributions, the origin and effect of cyclic slip irreversibilities and their relation to fatigue life and, finally, cyclic strain localization and fatigue crack initiation in persistent slip bands. In the second part, some topics that have recently found increasing interest will be discussed such as the cyclic deformation and fatigue behaviour of ultrafine-grained and nanostructured materials and the microstructural mechanisms that govern fatigue life of ductile and high-strength materials in the range of ultrahigh cycle fatigue. Some general conclusions will be drawn. ?? 2010 Published by Elsevier Ltd.},
author = {Mughrabi, Hael},
doi = {10.1016/j.proeng.2010.03.003},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2010{\_}Mughrabi{\_}Fatigue, an everlasting materials problem-still en vogue{\_}FatigueSlipBands-Overview.pdf:pdf},
isbn = {1877-7058},
issn = {18777058},
journal = {Procedia Eng.},
keywords = {Cyclic slip irreversibilities,Cyclic slip mode,Fatigue lives,Microstructural effects,Ultrafine-grained metals,Ultrahigh Cycle Fatigue (UHCF)},
number = {1},
pages = {3--26},
publisher = {Elsevier},
title = {{Fatigue, an everlasting materials problem - Still en vogue}},
url = {http://dx.doi.org/10.1016/j.proeng.2010.03.003},
volume = {2},
year = {2010}
}
@inproceedings{Yang1996Coolant,
author = {Yang, J},
booktitle = {SAE Int. Off-highw. Powerpl. Congr. Expo.},
doi = {https://doi.org/10.4271/961813},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Thermal Coating + Water Heat Transfer + Applikation/1996{\_}Yang{\_}Coolant Pump Throttling - A simple method to improve the control over SI engine cooling system.pdf:pdf},
publisher = {SAE International},
title = {{Coolant Pump Throttling - A Simple Method to Improve the Control Over SI Engine Cooling System}},
year = {1996}
}
@article{Sanli2009c,
author = {Sanli, A and Sayin, C and Gumus, M and Kilicaslan, I and Canakci, M},
journal = {Numer. Heat Transf. Part A Appl.},
number = {5},
pages = {444--458},
title = {{Numerical Evaluation by Models of Load and Spark Timing Effects on the In-Cylinder Heat Transfer of a SI Engine}},
volume = {56},
year = {2009}
}
@article{Variationsrechnunga,
author = {Variationsrechnung, Gegenstand Der},
file = {:C$\backslash$:/Users/p327208/Desktop/Promotion/Literature/Homogenisierung Und Lokalisierung/Strukturmechanik MMS/Literatur/variationen.pdf:pdf},
title = {{10 Variationsrechnung}}
}
@book{Schneider2013,
abstract = {Predicting the binding mode of flexible polypeptides to proteins is an important task that falls outside the domain of applicability of most small molecule and protein−protein docking tools. Here, we test the small molecule flexible ligand docking program Glide on a set of 19 non-$\alpha$-helical peptides and systematically improve pose prediction accuracy by enhancing Glide sampling for flexible polypeptides. In addition, scoring of the poses was improved by post-processing with physics-based implicit solvent MM- GBSA calculations. Using the best RMSD among the top 10 scoring poses as a metric, the success rate (RMSD ≤ 2.0 {\AA} for the interface backbone atoms) increased from 21{\%} with default Glide SP settings to 58{\%} with the enhanced peptide sampling and scoring protocol in the case of redocking to the native protein structure. This approaches the accuracy of the recently developed Rosetta FlexPepDock method (63{\%} success for these 19 peptides) while being over 100 times faster. Cross-docking was performed for a subset of cases where an unbound receptor structure was available, and in that case, 40{\%} of peptides were docked successfully. We analyze the results and find that the optimized polypeptide protocol is most accurate for extended peptides of limited size and number of formal charges, defining a domain of applicability for this approach.},
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Schneider, Wolfgang},
booktitle = {J. Chem. Inf. Model.},
doi = {10.1017/CBO9781107415324.004},
eprint = {arXiv:1011.1669v3},
isbn = {9788578110796},
issn = {1098-6596},
keywords = {icle},
number = {9},
pages = {1689--1699},
pmid = {25246403},
title = {{Praktische Regelungstechnik}},
volume = {53},
year = {2013}
}
@article{Yin2016,
abstract = {In this study, industrial 2524 aluminium alloy plates with various grain sizes (0.8-298 ??m) were prepared by cold rolling and heat treatment. The fatigue-crack-growth rate was studied as a function of grain size through fatigue tests and microstructural observations. The results showed that grain refinement led to a decrease in the resistance against fatigue-crack growth. Besides, the levels of crack closure in coarse-grained samples were higher than those in fine-grained ones at low values of the range of the stress intensity factor K, ??K. This phenomenon was predicted and explained well by the crack-deflection model.},
author = {Yin, Deyan and Liu, Huiqun and Chen, Yuqiang and Yi, Danqing and Wang, Bo and Wang, Bin and Shen, Fanghua and Fu, Shang and Tang, Cong and Pan, Suping},
doi = {10.1016/j.ijfatigue.2015.11.011},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/2015{\_}Yin+Liu{\_}Effect of grain size on fatigue crack growth in 2524 aluminium alloy.pdf:pdf},
isbn = {0142-1123},
issn = {01421123},
journal = {Int. J. Fatigue},
keywords = {2524 aluminium alloy,Fatigue-crack growth,Grain-size tailoring},
pages = {9--16},
publisher = {Elsevier Ltd},
title = {{Effect of grain size on fatigue-crack growth in 2524 aluminium alloy}},
url = {http://dx.doi.org/10.1016/j.ijfatigue.2015.11.011},
volume = {84},
year = {2016}
}
@article{Hansen1998b,
abstract = {The relation between polycrystal deformation and single crystal deformation has been studied in this work. A pure aluminium polycrystal having an average grain size of 300 [mu]m has been strained in tension at room temperature. The flow stress has been determined at four different strains (0.05, 0.14, 0.22 and 0.34) and deformation microstructures have been characterized qualitatively and quantitatively by transmission electron microscopy. Improved experimental techniques have allowed large foil areas to be characterized and in total 89 grains have been examined. At the four strains examined a classification of the deformation microstructures into three different types has shown a correlation between the grain orientation and the type of deformation microstructure which develops during straining. The dislocation density has been calculated at each strain and by assuming that the shear stress is proportional to the square root of the dislocation density the shear stress-strain relationship has been derived for each of the three groups of grains showing different deformation microstructures. The stress-strain curves show a strain hardening behaviour which depends on the orientation of the grain. The behaviour of the grains embedded in the polycrystal is compared with the behaviour of single crystals and the stress-strain curve of the polycrystal is estimated with good accuracy from single crystal data, which are weighted based on a quantitative texture analysis of the polycrystal.},
author = {Hansen, N. and Huang, X.},
doi = {10.1016/S1359-6454(97)00365-0},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/1998{\_}Hansen{\_}Huang MICROSTRUCTURE AND FLOW STRESS OF.pdf:pdf},
isbn = {1359-6454},
issn = {13596454},
journal = {Acta Mater.},
number = {5},
pages = {1827--1836},
title = {{Microstructure and flow stress of polycrystals and single crystals}},
url = {http://linkinghub.elsevier.com/retrieve/pii/S1359645497003650},
volume = {46},
year = {1998}
}
@article{Menge,
author = {Menge, Endliche and Menge, Unendliche},
doi = {10.1007/978-3-8348-8285-1},
isbn = {9783834882851},
number = {4},
title = {{I Allgemeine Grundlagen}}
}
@article{Desmorat2015,
author = {Desmorat, Rodrigue and {Du Tertre}, Alban and Gaborit, Pierre},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/2 scale models papers/2015{\_}Desmorat{\_}Multiaxial Haigh Diagrams from incremental two scale damage analysis.pdf:pdf},
journal = {Aerosp. Lab J.},
number = {9},
pages = {1--15},
title = {{Multiaxial Haigh diagrams from incremental two scale damage analysis}},
volume = {en review},
year = {2015}
}
@article{Gutbrod1954,
author = {Gutbrod, Firmen and Zweitaktmotoren, Bosch and Superior, Gutbrod and Fahr-, Beide},
journal = {Transport},
title = {{14 Motorkonzepte}},
year = {1954}
}
@article{Habenicht2012,
author = {Habenicht, Gerd},
isbn = {9783834802958},
title = {{Aus dem Programm Fertigungstechnik}},
year = {2012}
}
@article{McEvily1987,
abstract = {A method for determining the fatigue notch-size-effect is presented based upon the development of closure in the wake of a newly formed crack growing from a notch. A comparison with experimental results is in accord with predictions. The effect of crack closure on the formation of non-propagating cracks at notches and on notch sensitivity is also discussed. ?? 1987.},
author = {McEvily, A. J. and Minakawa, K.},
doi = {10.1016/0013-7944(87)90049-X},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/1987{\_}McEvily{\_}ON CRACK CLOSURE AND THE NOTCH SIZE EFFECT IN FATIGUE.pdf:pdf},
isbn = {0013794418},
issn = {00137944},
journal = {Eng. Fract. Mech.},
number = {5-6},
pages = {519--527},
title = {{On crack closure and the notch size effect in fatigue}},
volume = {28},
year = {1987}
}
@article{Zienkiewicz2005b,
author = {Zienkiewicz, O},
doi = {10.1016/B978-075066431-8/50204-6},
isbn = {9780750664318},
pages = {517--546},
title = {{Non-linear structural problems }},
volume = {2},
year = {2005}
}
@article{Grandin2002c,
abstract = {Heat transfer to the walls of the combustion chamber is increased by engine knock. In this study the influence of knock onset and knock intensity on the heat flux is investigated by examining over 10 000 individual engine cycles with a varying degree of knock. The heat transfer to the walls was estimated by measuring the combustion chamber wall temperature in an SI engine under knocking conditions. The influence of the air-fuel ratio and the orientation of the oscillating cylinder pressure-relative to the combustion chamber wall-were also investigated.It was found that knock intensities above 0.2 Mpa influenced the heat flux. At knock intensities above 0.6 Mpa, the peak heat flux was 2.5 times higher than for a non-knocking cycle. The direction of the oscillations did not affect the heat transfer.ER -},
author = {Grandin, B{\"{o}}rje and Denbratt, Ingemar},
doi = {10.4271/2002-01-0238},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Klopfen{\_}Ottomotor/2002{\_}Grandin{\_}The Effect of Knock on Heat Transfer in SI Engines-Experimental Results.pdf:pdf},
journal = {Sae Tech. Pap. Ser.},
number = {724},
title = {{The Effect of Knock on Heat Transfer in SI Engines}},
url = {http://papers.sae.org/2002-01-0238},
year = {2002}
}
@article{Thorium,
author = {Thorium, Elemente},
doi = {10.1007/978-3-8348-2279-6},
isbn = {9783834822796},
journal = {Arbeit},
pages = {326--341},
title = {{15 Geothermie}}
}
@inproceedings{961813,
abstract = {Pump throttling at light engine loads can reduce the heat-transfer coefficients in both the water jacket and the radiator, reducing HC emissions and friction/heat-transfer losses. Pump throttling can also accelerates engine warm-up. Pump driving power under pump throttling is predicted using measured flow parameters of a production-engine cooling system. The lower pump driving power due to pump throttling results in a 0.5{\%} decrease in predicted BSFC. Engine BSFC can decrease by more than 0.5{\%} due to reduced friction and heat-transfer losses as a result of the increased engine temperature.},
author = {Yang, Jialin},
booktitle = {SAE Int. Off-highw. Powerpl. Congr. Expo.},
doi = {https://doi.org/10.4271/961813},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Thermal Coating + Water Heat Transfer + Applikation/1996{\_}Yang{\_}Coolant Pump Throttling - A simple method to improve the control over SI engine cooling system.pdf:pdf},
issn = {0148-7191},
month = {aug},
publisher = {SAE International},
title = {{Coolant Pump Throttling - A Simple Method to Improve the Control Over SI Engine Cooling System}},
url = {https://doi.org/10.4271/961813},
year = {1996}
}
@article{Annand1963,
annote = {doi: 10.1243/PIME{\_}PROC{\_}1963{\_}177{\_}069{\_}02},
author = {Annand, W J D},
doi = {https://doi.org/10.1243/PIME_PROC_1963_177_069_02},
journal = {Proc. Inst. Mech. Eng.},
number = {1},
pages = {973--996},
publisher = {SAGE Publications},
title = {{Heat Transfer in the Cylinders of Reciprocating Internal Combustion Engines}},
volume = {177},
year = {1963}
}
@article{Hansen1998b,
abstract = {The relation between polycrystal deformation and single crystal deformation has been studied in this work. A pure aluminium polycrystal having an average grain size of 300 [mu]m has been strained in tension at room temperature. The flow stress has been determined at four different strains (0.05, 0.14, 0.22 and 0.34) and deformation microstructures have been characterized qualitatively and quantitatively by transmission electron microscopy. Improved experimental techniques have allowed large foil areas to be characterized and in total 89 grains have been examined. At the four strains examined a classification of the deformation microstructures into three different types has shown a correlation between the grain orientation and the type of deformation microstructure which develops during straining. The dislocation density has been calculated at each strain and by assuming that the shear stress is proportional to the square root of the dislocation density the shear stress-strain relationship has been derived for each of the three groups of grains showing different deformation microstructures. The stress-strain curves show a strain hardening behaviour which depends on the orientation of the grain. The behaviour of the grains embedded in the polycrystal is compared with the behaviour of single crystals and the stress-strain curve of the polycrystal is estimated with good accuracy from single crystal data, which are weighted based on a quantitative texture analysis of the polycrystal.},
author = {Hansen, N and Huang, X},
doi = {10.1016/S1359-6454(97)00365-0},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/1998{\_}Hansen{\_}Huang MICROSTRUCTURE AND FLOW STRESS OF.pdf:pdf},
isbn = {1359-6454},
issn = {13596454},
journal = {Acta Mater.},
number = {5},
pages = {1827--1836},
title = {{Microstructure and flow stress of polycrystals and single crystals}},
url = {http://linkinghub.elsevier.com/retrieve/pii/S1359645497003650},
volume = {46},
year = {1998}
}
@article{Ermudungsfestigkeit,
author = {Erm{\"{u}}dungsfestigkeit, Nachweises Der},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Empirical Fatigue Models + Validation/Erm{\"{u}}dungsfestigkeit{\_}Radaj/Kap8{\_}Rechnerischer Nachweis der Erm{\"{u}}dungsfestigkeit.pdf:pdf},
title = {{8 Rechnerischer Nachweis der Erm{\{}{\"{u}}{\}}dungsfestigkeit}}
}
@article{Depcik2002a,
abstract = {In this paper, the available correlations proposed in the literature for the gas-side heat transfer in the intake and exhaust system of a spark-ignition internal combustion engine were surveyed. It was noticed that theseAB - {\textless}inline-graphic xlink:href="2002-01-0372{\_}fig0001" xmlns:xlink="http://www.w3.org/1999/xlink"/{\textgreater}AB - only by empirically fitted constants. This similarity provided the impetus for the authors to explore if a universal correlation could be developed. Based on a scaling approach using microscales of turbulence, the authors have fixed the exponential factor on the Reynolds number and thus reduced the number of adjustable coefficients to just one; the latter can be determined from a least squares curve-fit of available experimental data. Using intake and exhaust side data, it was shown that the universal correlationAB - {\textless}inline-graphic xlink:href="2002-01-0372{\_}fig0002" xmlns:xlink="http://www.w3.org/1999/xlink"/{\textgreater}AB - The correlation coefficient of this proposed heat transfer model with all available experimental data is 0.845 for the intake side and 0.800 for the exhaust side.ER -},
author = {Depcik, Christopher and Assanis, Dennis},
doi = {10.4271/2002-01-0372},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2002{\_}Depcik{\_}A Universal Heat Transfer Correlation for intake and exhaust flows in an SI internal combustion engine.pdf:pdf},
journal = {SAE Pap.},
number = {January 2016},
title = {{A Universal Heat Transfer Correlation for Intake and Exhaust Flows in an Spark-Ignition Internal Combustion Engine}},
url = {http://papers.sae.org/2002-01-0372},
volume = {2002-01-03},
year = {2002}
}
@article{Controller1981,
author = {Controller, Jeder and Entwicklung, Die and Intel, Firma},
title = {{Prozessorarchitekturen im {\{}{\"{U}}{\}}berblick}},
year = {1981}
}
@article{Meroth2008b,
abstract = {Der Begriff Audio kommt vom lateinischen „audire“, „h{\"{o}}ren“ und bezieht sich auf alle akustischen Signale im Bereich der menschlichen Wahrnehmung. Ziel jeder Audiosignalverarbeitung ist es, dem Geh{\"{o}}r genau das Signal zu bieten, das der H{\"{o}}rer erwartet („nat{\"{u}}rliche Wiedergabe“[Has06]), daf{\"{u}}r muss der Weg des Signals von der Umwandlung {\"{u}}ber die Abstrahlung und Ausbreitung verstanden werden.},
author = {Meroth, Ansgar and Tolg, Boris},
isbn = {978-3-8348-9430-4},
journal = {Infotainmentsysteme im Kraftfahrzeug},
pages = {7--77},
title = {{Akustik und Audiotechnik}},
url = {http://dx.doi.org/10.1007/978-3-8348-9430-4{\_}2},
year = {2008}
}
@article{ZhouLan2015,
author = {Zhou, Bing and Lan, Xudong and Xu, Xianghua and Liang, Xingang},
doi = {10.1016/j.applthermaleng.2015.03.005},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Thermal Coating + Water Heat Transfer + Applikation/2015{\_}Zhou{\_}Numerical model and control strategies for the advanced therma management system of Diesel Engine.pdf:pdf},
journal = {Appl. Therm. Eng.},
pages = {368--379},
publisher = {Elsevier Ltd},
title = {{Numerical model and control strategies for the advanced thermal management system of diesel engine}},
volume = {82},
year = {2015}
}
@article{Liberalisierung1998,
author = {Liberalisierung, Thema and Schwankungen, Wettbewerbs and Folgenden, Im and Struktur, Die and Zeit, Die and Strompreise, Die},
doi = {10.1007/978-3-8348-2279-6},
isbn = {9783834822796},
number = {Ka V},
pages = {325--336},
title = {{18 Liberalisierung der Energiem{\"{a}}rkte}},
year = {1998}
}
@article{Burgj,
author = {Burg, Heinz and Gratzer, Werner and Moser, Andreas and Steffan, Hermann},
journal = {Energy},
title = {{A9 A9 Kollisionsmechanik A9}}
}
@article{Bozza2011b,
abstract = {In the present paper a combined procedure for the quasi-dimensional modelling of heat transfer, combustion and knock phenomena in a "downsized" Spark Ignition two-cylinder turbocharged engine is presented. The procedure is extended to also include the effects consequent the Cyclic Variability. Heat transfer is modelled by means of a Finite Elements model. Combustion simulation is based on a fractal description of the flame front area. Cyclic Variability (CV) is characterized through the introduction of a random variation on a number of parameters controlling the rate of heat release (air/fuel ratio, initial flame kernel duration and radius, laminar flame speed, turbulence intensity). The intensity of the random variation is specified in order to realize a Coefficient Of Variation (COV) of the Indicated Mean Effective Pressure (IMEP) similar to the one measured during an experimental campaign. Moreover, the relative importance of the various concurring effects is established on the overall COV. A kinetic scheme is then solved within the unburned gas zone, characterized by different thermodynamic conditions occurring cycle-by-cycle. In this way, an optimal choice of the "knock-limited" spark advance is effected and compared with experimental data. Finally, the CV effects on the occurrence of individual knocking cycles are assessed and discussed. {\{}{\textcopyright}{\}} 2011 Global Science Press.},
author = {Bozza, Fabio and Siano, Daniela and Costa, Michela},
doi = {10.4208/aamm.10-10s2-04},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2011{\_}Bozza{\_}heat-transfer-knock-modeling-and-cyclic-variability-in-a-downsized-spark-ignition-turbocharged-engine.pdf:pdf},
issn = {20700733},
journal = {Adv. Appl. Math. Mech.},
keywords = {Cyclic variability,Finite elements in heat transfer,Internal combustion engines modelling,Knock},
number = {3},
pages = {310--326},
title = {{Heat transfer, knock modeling and cyclic variability in a "Downsized" spark-ignition turbocharged engine}},
volume = {3},
year = {2011}
}
@article{Pineau2016,
abstract = {In this interpretive review, fatigue in metallic systems is considered primarily from the perspective of interactions between the microstructure, the deformation mode and the mechanical state at both low and high temperatures. In Part 1 the development and early propagation of cracks is considered in terms of the basic damage mechanisms and the relative size of the crack with respect to applicable microstructural feature(s). In this section, a multistage grain scale approach to microstructure-sensitive fatigue crack formation and growth is presented which uses Fatigue Indicator Parameters (FIPs) to correlate these processes. Various FIPs parameters are discussed in terms of their indication of the state of fatigue. The development and early crack propagation is considered in the context of microstructure and notches, and probabilistic aspects of the notch fatigue problem are discussed. These features are integrated into a systematic approach for the selection of fatigue resistant microstructures for given applications. In Part 2, attention is focused on Ni-base superalloys and the interaction between oxidation, creep and microstructure (including coatings) in the formation and propagation of cracks. This part of the overview addresses both experimental and modelling aspects. Methodologies based upon fundamental physical processes are presented for understanding and predicting the development and propagation of fatigue cracks, including effects of sequential oxide type formation and of creep on either restraining or accelerating damage by oxidation. The variable fatigue resistance of discs in jet engines is seen to depend upon the variability of microstructure and its influence on the severity of creep/oxidation interactions. All of these factors are considered in the practical case where both temperature and loading parameters vary simultaneously (thermomechanical fatigue). A physics-based life prediction model considering the interactions of deformation and environmental damage is reviewed in terms of its applicability to life prediction of components.},
author = {Pineau, Andr?? and McDowell, David L. and Busso, Esteban P. and Antolovich, Stephen D.},
doi = {10.1016/j.actamat.2015.05.050},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/2016{\_}Pineau + McDowell{\_}Failure of metals II Fatigue.pdf:pdf},
isbn = {13596454},
issn = {13596454},
journal = {Acta Mater.},
keywords = {Environment-microstructure interaction,Fatigue in metallic alloys,Intergranular cracking, thermomechanical fatigue,Local and global fatigue approaches,Multistage fatigue,Oxidation,Superalloys},
pages = {484--507},
title = {{Failure of metals II: Fatigue}},
volume = {107},
year = {2016}
}
@article{Beispield,
author = {Beispiel, Dieses},
pages = {59--69},
title = {{6 Welle}}
}
@article{Esfahanian2006a,
abstract = {In this study, the heat transfer to an engine piston crown is calculated. Three different methods for the combustion boundary condition are used. The results of different combustion side boundary condition treatments are compared and their effects on the thermal behavior of the piston are investigated. It has been shown that using spatial and time averaged combustion side boundary condition is a suitable treatment method within engineering approximations. An interface between KIVA-3V and NASTRAN codes is developed. ?? 2005 Elsevier Ltd. All rights reserved.},
author = {Esfahanian, V. and Javaheri, A. and Ghaffarpour, M.},
doi = {10.1016/j.applthermaleng.2005.05.002},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2006{\_}Esfahanian{\_}Thermal analysis of an SI engine piston using different combustion boundary condition treatements.pdf:pdf},
issn = {13594311},
journal = {Appl. Therm. Eng.},
keywords = {Boundary Condition Treatment,Combustion,Heat transfer,Piston},
number = {2-3},
pages = {277--287},
title = {{Thermal analysis of an SI engine piston using different combustion boundary condition treatments}},
volume = {26},
year = {2006}
}
@article{Rothe2015a,
abstract = {In this article we investigate a fully, thermo-mechanically coupled viscoplasticity model in view of various numerical aspects. First, we develop the entire system of differential–algebraic equations resulting from the spatially discretized principle of virtual displacements, the principle of virtual temperatures, and the evolution equations of the internal variables provided by the constitutive model. In the time-integration step this system is solved both using a fully monolithic approach based on a Backward–Euler scheme in combination with the Multilevel-Newton algorithm as well as a partitioned approach solving the fully coupled system. The latter is treated by means of a combination of a Backward–Euler method and an accelerated Gauss–Seidel/Multilevel-Newton scheme to solve the resulting system of algebraic equations within each time-integration step. Additionally, we consider a specific treatment of the interpolation between different meshes within the partitioned approach. This is shown for p-version finite elements based on hierarchical shape functions. Finally, it turns out that the specific constitutive model of small-strain thermo-viscoplasticity, which is based on the decomposition into kinematic hardening and energy storing strains, yields a problem-adapted stress algorithm. This allows to reduce the stress algorithm on Gauss-point level to the solution of one scalar equation. Numerical examples serve to elucidate the behavior and properties of the proposed methods.},
author = {Rothe, Steffen and Erbts, Patrick and D{\"{u}}ster, Alexander and Hartmann, Stefan},
doi = {10.1016/j.cma.2015.05.002},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Numerik UMATS FE-Codes/2015{\_}Hartmann{\_}Monolithic and partitioned coupling schemes for thermo-viscoplasticity.pdf:pdf},
issn = {00457825},
journal = {Comput. Methods Appl. Mech. Eng.},
keywords = {algebraic equations,differential,fully coupled finite elements,monolithic approach,partitioned approach,thermo-viscoplasticity},
pages = {375--410},
publisher = {Elsevier B.V.},
title = {{Monolithic and partitioned coupling schemes for thermo-viscoplasticity}},
url = {http://linkinghub.elsevier.com/retrieve/pii/S0045782515001681},
volume = {293},
year = {2015}
}
@article{Pkw-pkw-unfalle2005,
author = {Pkw-pkw-unf{\"{a}}lle, A and Br{\"{o}}sdorf, Klaus-dieter and Burg, Heinz and Moser, Andreas and Hauptumfang, Den Pkw-pkw-unf{\"{a}}llen Der},
journal = {Sierra},
pages = {411--437},
title = {{A12 Zum Stra{\ss}enverkehr in Deutschland und in Europa A12}},
year = {2005}
}
@article{Fea2003,
author = {Fea, Nonlinear},
pages = {201--213},
title = {{Introduction to Nonlinear FEA 16.1}},
year = {2003}
}
@article{Morris2007a,
author = {Morris, J W},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/Crystall Plasticity Basics/Morris{\_}Dislocation plasticity-AnOverview.pdf:pdf},
journal = {Introd. to Mater. Sci.},
pages = {1--36},
title = {{Dislocation Plasticity : Overview}},
url = {http://www.mse.berkeley.edu/groups/morris/MSE205/Extras/dislocation plasticity.pdf},
volume = {i},
year = {2007}
}
@article{Thornton2002,
author = {Thornton, Colin and I, David Kafui},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Zienkiewicz FEM - Vol 2 Solid Structural Mechanics/63212{\_}09.pdf:pdf},
pages = {178--182},
title = {{Discrete Element Methods}},
year = {2002}
}
@article{Tarnopolskii1998,
author = {Tarnopol'skii, Yu.M. and Kulakov, V.L.},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/{\_}buecherSong/HandbookofComposites/III/34{\_}MechanicalTests.pdf:pdf},
isbn = {0-412-54020-7},
journal = {Handb. Compos.},
pages = {778--793},
title = {{Mechanical tests}},
year = {1998}
}
@article{Down1977,
author = {Down, Claverton},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/Strukturmechanik MMS/Literatur/HS Schranken Methodik MMS Vorlesung Details/Willis - 1977{\_}Uberblick{\_}Methodik{\_}HS{\_}Schranken.pdf:pdf},
pages = {185--202},
title = {{Bounds and Self-Consistent Estimates for the}},
volume = {25},
year = {1977}
}
@article{Zahoransky2013d,
author = {Zahoransky, Richard a. and Allelein, Hans-Josef and Schelling, Udo and Schwarz, Harald and Bollin, Elmar and Oehler, Helmut},
doi = {10.1007/978-3-8348-2279-6},
isbn = {978-3-8348-1869-0},
journal = {Energietechnik - Syst. zur Energieumwandlung},
pages = {378--386},
title = {{16 Energetische M{\"{u}}llverwertung}},
url = {http://www.springerlink.com/index/10.1007/978-3-8348-2279-6},
year = {2013}
}
@article{Wilson1951,
author = {Wilson, Brian A},
journal = {Processing},
title = {{A. Wilson 23}},
year = {1951}
}
@article{Gross2011h,
author = {Gross, Dietmar and Seelig, Thomas},
doi = {10.1007/978-3-642-10196-0},
isbn = {978-3-642-10195-3},
title = {{Bruchmechanik}},
url = {http://link.springer.com/10.1007/978-3-642-10196-0},
year = {2011}
}
@article{Forest2009a,
abstract = {A unifying thermomechanical framework is presented that reconciles several classes of gradient elastoviscoplasticity and damage models proposed in the literature during the last 40 years. It is based on the introduction of the micromorphic counterpart ϕ {\$}\chi{\$} of a selected ... {\$}\backslash{\$}n},
author = {Forest, Samuel},
doi = {10.1061/(ASCE)0733-9399(2009)135:3(117)},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/2009{\_}Forest{\_}Micromorphic Approach for Gradient Elasticity Viscoplasticity and Damage.pdf:pdf},
isbn = {0733-9399},
issn = {0733-9399},
journal = {J. Eng. Mech.},
number = {3},
pages = {117--131},
title = {{Micromorphic Approach for Gradient Elasticity, Viscoplasticity, and Damage}},
volume = {135},
year = {2009}
}
@article{Grandin2000b,
abstract = {It is generally accepted that knocking combustion influences the heat transfer in SI engines. However, the effects of heat transfer on the onset of knock is still not clear due to lack of experimental data of the thermal boundary layer close to the combustion chamber wall. This paper presents measurements of the temperature in the thermal boundary layer under knocking and non-knocking conditions. The temperature was measured using dual-broadband rotational Coherent anti-Stokes Raman Spectroscopy (CARS). Simultaneous time-resolved measurements of the cylinder pressure, at three different locations, and the heat flux to the wall were carried out. Optical access to the region near the combustion chamber wall was achieved by using a horseshoe-shaped combustion chamber with windows installed in the rectangular part of the chamber. This arrangement made CARS temperature measurements close to the wall possible and results are presented in the range 0.1-5 mm from the wall. The engine was run with constant fuel flow under near stoichiometric conditions. Knocking and non-knocking conditions were achieved by using different mixtures of n-heptane and iso-octane.},
author = {Grandin, B{\"{o}}rje and Denbratt, Ingemar and Bood, Joakim and Brackmann, Christian and Bengtsson, Per-Erik},
doi = {10.4271/2000-01-2831},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Heat transfer intake+exhaust system/2000{\_}Bood{\_}The Effect of Knock on the Heat Transfer in an SI Engine.pdf:pdf},
journal = {SAE Tech. Pap.},
number = {2000-01-2831},
title = {{The Effect of Knock on the Heat Transfer in an SI Engine: Thermal Boundary Layer Investigation using CARS Temperature Measurements and Heat Flux Measurements}},
url = {http://dx.doi.org/10.4271/2000-01-2831},
year = {2000}
}
@article{Mohammadi2010a,
abstract = {Optimizing heat transfer for internal combustion engines requires application of advanced development tools. In addition to experimental method, numerical 3D-CFD calculations are needed in order to obtain an insight into the complex phenomenas in-cylinder processes. In this context, fluid flow and heat transfer inside a four-valve engine cylinder is modeled and effects of changing engine speed on dimensionless parameters, instantaneous local Nusselt number and Reynolds number near the surface of combustion chamber are studied. Based on the numerical simulation new correlations for instantaneous local heat transfer on the combustion chamber of SI engines are derived. Results for several engine speeds are compared for total heat transfer coefficient of the cylinder engine with available correlation proposed by experimental measurements and a close agreement is observed. It is found that the local value of heat transfer coefficient varies considerably in different parts of the cylinder, but it has equivalent trend with crank angle position. ?? 2010 Elsevier Masson SAS. All rights reserved.},
author = {Mohammadi, A. and Yaghoubi, M.},
doi = {10.1016/j.ijthermalsci.2009.12.010},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2010{\_}Mohammadi{\_}Estimation of instantaneous local heat transfer coefficient.pdf:pdf},
journal = {Int. J. Therm. Sci.},
keywords = {CFD,Combustion,Cylinder head,Heat transfer coefficient,Nusselt number,SI engine,Turbulence},
number = {7},
pages = {1309--1317},
title = {{Estimation of instantaneous local heat transfer coefficient in spark-ignition engines}},
volume = {49},
year = {2010}
}
@article{Cimmelli2014,
abstract = {We present the state of the art on the modern mathematical methods of exploiting the entropy principle in thermomechanics of continuous media. A survey of recent results and conceptual discussions of this topic in some well-known non-equilibrium theories (Classical irreversible thermodynamics CIT, Rational thermodynamics RT, Thermodynamics of irreversible processes TIP, Extended irreversible thermodynamics EIT, Rational Extended thermodynamics RET) is also summarized.},
author = {Cimmelli, Vito Antonio and Jou, David and Ruggeri, Tommaso and V??n, P??ter},
doi = {10.3390/e16031756},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Thermodynamik/Entropy Principle and Recent Results in Non Equilibrium Theories{\_}Cimmelli .pdf:pdf},
issn = {10994300},
journal = {Entropy},
keywords = {Classical irreversible thermodynamics,Continuum thermodynamics,Entropy principle,Exploitation of second law,Extended irreversible thermodynamics,Rational extended thermodynamics,Rational thermodynamics},
number = {3},
pages = {1756--1807},
title = {{Entropy principle and recent results in non-equilibrium theories}},
volume = {16},
year = {2014}
}
@article{Schabacker2011,
author = {Schabacker, M},
doi = {10.1007/978-3-8348-8161-8},
isbn = {9783834881618},
pages = {98--108},
title = {{7 Blechteilmodellierung (Sheet Metal)}},
year = {2011}
}
@article{Problems2003,
author = {Problems, Contact},
journal = {Springs},
pages = {195--200},
title = {{Introduction to Contact Problems 15.1}},
year = {2003}
}
@article{Logue,
author = {Logue, Steve},
pages = {52--131},
title = {{19 Beispiele V5}}
}
@article{Eiamsa-Ard2010,
abstract = {The article presents an investigation of the effect of twisted tape with serrated-edge insert on heat transfer and pressure loss behaviors in a constant heat-fluxed tube. In the experiments, the serrated twisted tape (STT) was inserted into the entire test tube with a constant twist ratio in order to generate a continuous swirling airflow. Two geometry parameters of the STT to be considered in the present work are the serration width ratio and the serration depth ratio. The measurements have been conducted for the airflow rate based on Reynolds numbers in the turbulent regime from 4000 to 20,000. The experimental results of the STT inserted tube are compared with those of the plain tube fitted with typical twisted tape (TT). The results show that the heat transfer rate in terms of Nusselt number, Nu increases with the rise in the depth ratio but decreases with raising the width ratio. The heat transfer rate is up to 72.2{\%} and 27{\%} relative to the plain tube and the TT inserted tube, respectively. The use of the STT leads to higher heat transfer rate and friction factor than that of the TT for all cases. The thermal performance factor of the STT tube under constant pumping power is evaluated and found to be above unity indicating that using the STT tube is advantageous over the TT tube or the plain tube. In addition, the empirical correlations developed by relating the serration width ratio, serration depth ratio and Reynolds number are determined. ?? 2010 Elsevier Ltd. All rights reserved.},
author = {Eiamsa-Ard, Smith and Promvonge, Pongjet},
doi = {10.1016/j.applthermaleng.2010.03.026},
file = {:C$\backslash$:/Users/p327208/Desktop/Promotion/Literature/Motorspezifisch/Heat transfer intake+exhaust system/2010{\_}Eiamsa-ard+Promvonge{\_}Thermal characteristics in round tube fitted with serrated twisted tape.pdf:pdf},
journal = {Appl. Therm. Eng.},
keywords = {Friction factor,Heat transfer,Serrated twisted tape,Swirl flow,Typical twisted tape},
number = {13},
pages = {1673--1682},
title = {{Thermal characteristics in round tube fitted with serrated twisted tape}},
volume = {30},
year = {2010}
}
@inproceedings{Schubert2005,
abstract = {A realistic simulation of the wall heat transfer is an imperative condition for the accurate analysis and simulation of the working process of IC engines. Due to its simplicity in application, zero-dimensional wall heat transfer models dominate engine cycle simulation in practice. However, experience shows that existing zero-dimensional models for wall heat transfer do not yield satisfactory results in certain applications. This is mainly due to a lack of consideration of the actual flow field in the cylinder.In this paper a quasi-dimensional heat transfer model, which is based on a detailed description of the turbulent flow field in the combustion chamber, is described. The model presents a consistent approach for the high pressure as well as the low pressure part of the cycle. The results of the heat transfer model are compared with results from the correlation by Woschni/Huber and with experimental results from various DI Diesel engines.},
author = {Schubert, Claudia and Wimmer, Andreas and Chmela, Franz},
booktitle = {SAE Tech. Pap. 2005-01-0695},
doi = {10.4271/2005-01-0695},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2005{\_}Schubert{\_}Advanced Heat Transfer Model for CI Engines.pdf:pdf},
publisher = {SAE international},
title = {{Advanced Heat Transfer Model for CI Engines}},
year = {2005}
}
@article{Sandoval2003a,
abstract = {A spark-ignition engine friction model developed by Patton et al. in the late 1980s was evaluated against current engine friction data, and improved. The model, which was based on a combination of fundamental scaling laws and empirical results, includes predictions of rubbing losses from the crankshaft, reciprocating, and valvetrain components, auxiliary losses from engine accessories, and pumping losses from the intake and exhaust systems. These predictions were based on engine friction data collected between 1980 and 1988. Some of the terms are derived from lubrication theory. Other terms were derived empirically from measurements of individual friction components from engine teardown experiments. Recent engine developments (e.g., improved oils, surface finish on piston liners, valve train mechanisms) suggested that the model needed updating. So modifications were made to the piston ring tension and gas pressure loading contributions to piston assembly friction, the impact of liner roughness, and to the valvetrain mechanism friction. Lubricant viscosity scaling was added to the hydrodynamic terms in the rubbing friction component models. The improved model now gives reasonable estimates of individual friction component and total spark-ignition engine friction mean effective pressure. The inclusion of oil viscosity scaling with temperature results in cold engine friction predictions about twice the value for warmed up engines. This agrees with the limited cold engine friction data available in the literature.},
archivePrefix = {arXiv},
arxivId = {2003-01-0725},
author = {Sandoval, Daniel and Heywood, John B.},
doi = {10.4271/2003-01-0725},
eprint = {2003-01-0725},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2003{\_}Sandoval{\_}An Imporved Friction Model for Spark{\_}Ign Engines.pdf:pdf},
isbn = {0148-7191},
title = {{An Improved Friction Model for Spark-Ignition Engines}},
url = {http://papers.sae.org/2003-01-0725/},
year = {2003}
}
@article{KangAhnMin2015,
author = {Kang, Hyungmook and Ahn, Hyunchul and Min, Kyoungdoug},
doi = {10.1016/j.applthermaleng.2014.12.042},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Thermal Coating + Water Heat Transfer + Applikation/2016{\_}Kang{\_}Smart cooling system of the double loop coolant structure with engine thermal management modeling.pdf:pdf},
journal = {Appl. Therm. Eng.},
keywords = {double loop coolant structure,engine thermal management},
pages = {124--131},
publisher = {Elsevier Ltd},
title = {{Smart cooling system of the double loop coolant structure with engine thermal management modeling}},
volume = {79},
year = {2015}
}
@article{Steffen,
author = {Steffen, Horst and Bausch, Hansj{\"{u}}rgen},
isbn = {9783835100145},
title = {{Horst Steffen, Hansj{\{}{\"{u}}{\}}rgen Bausch}}
}
@article{Ubungsaufgaben,
author = {{\"{U}}bungsaufgaben, A L{\"{o}}sungen Der},
title = {{A.1 L{\{}{\"{o}}{\}}sungen der {\{}{\"{U}}{\}}bungsaufgaben}}
}
@misc{Draper1935,
author = {Draper, C S},
booktitle = {NACA Rep.},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/xxx{\_}Draper{\_}The physical effects of detonation in a closed cylindrical chamber - analytical solutions.pdf:pdf},
number = {493},
title = {{The physical effects of detonation in a closed cylindrical chamber}},
year = {1935}
}
@article{Simulation,
author = {Simulation, Eine and Simulationsprozess, Dieser and Reifenmodelle, Diese and Simulationsergebnisse, Diese and Prozess, Dieser and Simulation, Die and Gesamtprozess, Der},
journal = {Simulation},
title = {{12 Simulation}}
}
@article{Sharma2002a,
abstract = {This paper illustrates the micromechanics approach to cyclic creep-fatigue damage of Pb-Sn, developed by the authors with the help of a simple case study. It is demonstrated that durability predictions can be made based solely on monotonic test data. Various parametric studies of practical interest are conducted to obtain mechanistic insights into various aspects of damage in solders e.g., effect of hydrostatic stresses, grain size, ramp rate, etc.},
author = {Sharma, Pradeep and Dasgupta, Abhijit},
doi = {10.1115/1.1493203},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Kriechen{\_}Spannungsrelaxation/2002{\_}Sharma Pradeep{\_}Micro-Mechanics of Creep-Fatigue Damage in PB-SN Solder Due to Thermal Cycling PartOne.pdf:pdf},
issn = {1043-7398},
journal = {J. Electron. Packag.},
number = {3},
pages = {298--304},
title = {{Micro-Mechanics of Creep-Fatigue Damage in PB-SN Solder Due to Thermal Cycling—Part II: Mechanistic Insights and Cyclic Durability Predictions From Monotonic Data}},
url = {http://dx.doi.org/10.1115/1.1493203{\%}7B{\%}25{\%}7D5Cnhttp://electronicpackaging.asmedigitalcollection.asme.org/data/Journals/JEPAE4/26206/298{\%}7B{\_}{\%}7D1.pdf},
volume = {124},
year = {2002}
}
@article{Vierpoltheorie,
author = {Vierpoltheorie, Grundlegende Zusammenh{\"{a}}nge Der},
pages = {180--200},
title = {{10 Vierpoltheorie 10.1}},
volume = {1}
}
@article{Eslami2015,
abstract = {An approach for prediction of high cycle fatigue (HCF) at a length scale of 5-100 ??m is established, which evaluates the accumulated plastic shear strain in slip bands of grains. Damage mechanisms initiated by dislocations and the grain microstructure are the key factors that influence the fatigue of metals in small dimensions. For this reason the HCF model considers the elasto-plastic behavior of metals at the grain level and microstructural parameters, specifically grain size and grain orientation. The HCF model can be applied either as a criterion for deterministic predictions of the failure in individual grains, or as a failure function in probabilistic studies on aggregates of grains, if the input parameters are given by specific distributions. This is addressed in a parameter study and a sensitivity analysis of the failure function with respect to different parameters. For model verification, the predicted results of the failure function are compared with the observed micro-damage in individual grains of nickel micro-samples. It is shown that the overall predictive power of the HCF model is fairly good. Nevertheless, some misclassifications occur as some grains are damaged, which were predicted to be safe. Those misclassifications are addressed in post-fatigue investigations on individual grains.},
author = {Eslami, R. and Riesch-Oppermann, H. and Kraft, O.},
doi = {10.1016/j.ijfatigue.2015.03.029},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2015{\_}Eslami+Kraft{\_}Prediction of multiaxial high cycle fatigue at small scales based on an micro-mecahnical model{\_}IAM{\_}KIT{\_}KRAFT.pdf:pdf},
isbn = {0142-1123},
issn = {01421123},
journal = {Int. J. Fatigue},
keywords = {Accumulated plastic shear strain,Micro electro mechanical systems (MEMS),Multiaxial high cycle fatigue (HCF),Probability methods,Surface damage},
pages = {66--74},
publisher = {Elsevier Ltd},
title = {{Prediction of multiaxial high cycle fatigue at small scales based on a micro-mechanical model}},
url = {http://dx.doi.org/10.1016/j.ijfatigue.2015.03.029},
volume = {83},
year = {2015}
}
@article{Bohlke2012a,
author = {B{\"{o}}hlke, Prof Thomas},
journal = {Mechanik},
title = {{Skript zur Vorlesung H{\{}{\"{o}}{\}}here Technische Festigkeitslehre}},
year = {2012}
}
@article{Faktoren,
author = {Faktoren, Alle},
title = {{Motor und Antrieb 3 Arbeitsweise , Bauformen und konstruktive Ausf{\"{u}}hrung von Motorradmotoren}}
}
@article{Den,
author = {Den, Zu},
journal = {Frequenz},
pages = {87--110},
title = {{8 Messung elektrischer Gr{\"{o}}{\ss}en}}
}
@article{Aufgabea,
author = {Aufgabe, Die and Fol, Eine and Vielzahl, Die and Din, Die Norm},
pages = {1--3},
title = {{Einf{\"{u}}hrung}}
}
@article{Baehr2006,
abstract = {Bevor wir einige Grundbegriffe der Thermodynamik einf{\"{u}}hren, gehen wir kurz auf ihre geschichtliche Entwicklung ein und versuchen dann, die Frage zu beantworten: Was ist Thermodynamik? In den darauf folgenden Ab- schnitten definieren wir das thermodynamische System und behandeln seine Beschreibung durch Zustandsgr{\"{o}}{\ss}en. Dabei f{\"{u}}hren wir den f{\"{u}}r die klassische Thermodynamik grundlegenden Begriff der Phase ein. Bei der daran anschlie{\ss}enden Behandlung der thermodynamischen Prozesse erhalten wir mit dem Prinzip der Irreversibilit{\"{a}}t eine erste Formulierung des 2. Hauptsatzes der Thermodynamik. Schlie{\ss}lich f¨ uhren wir die Temperatur als die erste typisch thermodynamische Zustandsgr{\"{o}}{\ss}e ein.},
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Baehr, Hans Dieter and Kabelac, Stephan},
doi = {10.1017/CBO9781107415324.004},
eprint = {arXiv:1011.1669v3},
isbn = {9783834882851},
issn = {0302-4350},
journal = {Springer},
keywords = {Grundlagen,Thermodynamik,Verbrennung},
pages = {1--42},
pmid = {25246403},
title = {{Thermodynamik}},
url = {http://www.springerlink.com/index/w26t7673r61611tj.pdf},
volume = {1},
year = {2006}
}
@article{Radaufhangungen,
author = {Radaufh{\"{a}}ngungen, Freiheitsgrade Der},
journal = {Sein},
number = {Beispiel c},
title = {{2 Bauarten und Freiheitsgrade}}
}
@article{Growth1988,
author = {Growth, Part},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/Continuum Damage Mechanics - SumioMurakami/FrontMatter.pdf:pdf},
number = {March},
title = {{Continuum Damage Mechanics :}},
volume = {55165},
year = {1988}
}
@article{Zhao2008,
abstract = {Extensive fatigue experiments were conducted using 7075-T651 aluminum alloy under uniaxial, torsion, and axial-torsion loading. Detailed fatigue results were reported. Different mean stresses were applied in the experiments and the mean stress was found to have a significant influence on the fatigue strength of the material. A tensile mean stress decreased the fatigue strength dramatically. Fatigue damage was found to occur under compression-compression loading. In addition, axial-torsion experiments using tubular specimens were conducted under different loading paths to study the multiaxial fatigue behavior. Fatigue cracking behavior was found to be dependent on the loading path as well as the loading magnitude. When the loading magnitude was high, the material displayed shear cracking. When the loading stress was below a certain level, the material exhibited tensile cracking. For most loading cases under investigation, the material displayed a mixed cracking behavior. A kink was found in the shear strain versus fatigue life curve from the pure torsion experiments, and it was associated with a distinctive transition of cracking behavior. The Smith-Watson-Topper (SWT) parameter with a critical plane interpretation was found to correlate well with most of the experiments conducted in terms of fatigue lives. However, the SWT parameter cannot deal with the uniaxial fatigue conditions where the maximum stress is low or negative. More importantly, the model fails to correctly predict the cracking behavior observed experimentally on the material. A critical plane criterion based on a combination of the normal and shear components of the stresses and strains on material planes was found to better correlate the fatigue experiments in terms of both fatigue life and cracking behavior. The characteristics of the multiaxial fatigue criterion were discussed based on the experimental observations on 7075-T651 aluminum alloy. ?? 2007 Elsevier Ltd. All rights reserved.},
author = {Zhao, Tianwen and Jiang, Yanyao},
doi = {10.1016/j.ijfatigue.2007.07.005},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Empirical Fatigue Models + Validation/2007{\_}Jiang{\_}Fatigue of 7075-T651 aluminum alloy VALIDATION+MODEL.pdf:pdf},
isbn = {0142-1123},
issn = {01421123},
journal = {Int. J. Fatigue},
keywords = {7075-T651 aluminum alloy,Axial-torsion,Compression-compression fatigue,Multiaxial criterion,Multiaxial fatigue},
number = {5},
pages = {834--849},
title = {{Fatigue of 7075-T651 aluminum alloy}},
volume = {30},
year = {2008}
}
@article{Eq2015,
author = {Eq, Hence and Eqs, Comparing},
pages = {1--5},
title = {{Appendix H}},
year = {2015}
}
@article{Computertechnik1947,
author = {Computertechnik, In Der},
journal = {System},
pages = {205--210},
title = {{12 Computertechnik}},
volume = {1947},
year = {1947}
}
@article{Grosskreutz1971,
abstract = {Fatigue crack initiation Fatigue crack growth},
author = {Grosskreutz, J. G.},
doi = {10.1002/pssb.2220470202},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/1971{\_}Grosskreutz{\_}The Mechanisms of metal fatigue.pdf:pdf},
isbn = {0370-1972},
issn = {15213951},
journal = {Phys. Status Solidi},
number = {2},
pages = {359--396},
title = {{The mechanisms of metal fatigue (II)}},
volume = {47},
year = {1971}
}
@article{Hashin1963,
abstract = {Variational principles in the linear theory of elasticity, involving the elastic polarization tensor, have been applied to the derivation of upper and lower bounds for the effective elastic moduli of quasi-isotropic and quasi-homogeneous multiphase materials of arbitrary phase geometry. When the ratios between the different phase moduli are not too large the bounds derived are close enough to provide a good estimate for the effective moduli. Comparison of theoretical and experimental results for a two-phase alloy showed good agreement.},
author = {Hashin, Zvi and Shtrikman, Shmuel},
doi = {10.1016/0022-5096(63)90060-7},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/Strukturmechanik MMS/Literatur/Hashin Shtrikman 1963.pdf:pdf},
isbn = {0022-5096},
issn = {00225096},
journal = {J. Mech. Phys. Solids},
number = {2},
pages = {127--140},
title = {{A variational approach to the theory of the elastic behaviour of multiphase materials}},
url = {http://linkinghub.elsevier.com/retrieve/pii/0022509663900607},
volume = {11},
year = {1963}
}
@article{Mohamed2016ETM,
author = {Mohamed, Eid S},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Thermal Coating + Water Heat Transfer + Applikation/2016{\_}Mohamed{\_}Experimental study on the effect of active engine thermal management on a bi-fuel engine performance combustion and exhaust emissions.pdf:pdf},
journal = {Appl. Therm. Eng.},
pages = {1352--1365},
title = {{Experimental study on the effect of active engine thermal management on a bi-fuel engine performance combustion and exhaust emissions}},
volume = {106},
year = {2016}
}
@article{Gleichunga,
author = {Gleichung, Reynoldssche and Gleichung, Reynoldssche},
title = {{8 Hydrodynamische Schmierung 8.1}}
}
@article{Mohammadi2010,
abstract = {Optimizing heat transfer for internal combustion engines requires application of advanced development tools. In addition to experimental method, numerical 3D-CFD calculations are needed in order to obtain an insight into the complex phenomenas in-cylinder processes. In this context, fluid flow and heat transfer inside a four-valve engine cylinder is modeled and effects of changing engine speed on dimensionless parameters, instantaneous local Nusselt number and Reynolds number near the surface of combustion chamber are studied. Based on the numerical simulation new correlations for instantaneous local heat transfer on the combustion chamber of SI engines are derived. Results for several engine speeds are compared for total heat transfer coefficient of the cylinder engine with available correlation proposed by experimental measurements and a close agreement is observed. It is found that the local value of heat transfer coefficient varies considerably in different parts of the cylinder, but it has equivalent trend with crank angle position. ?? 2010 Elsevier Masson SAS. All rights reserved.},
author = {Mohammadi, A. and Yaghoubi, M.},
doi = {10.1016/j.ijthermalsci.2009.12.010},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2010{\_}Mohammadi{\_}Estimation of instantaneous local heat transfer coefficient.pdf:pdf},
isbn = {12900729 (ISSN)},
issn = {12900729},
journal = {Int. J. Therm. Sci.},
keywords = {CFD,Combustion,Cylinder head,Heat transfer coefficient,Nusselt number,SI engine,Turbulence},
number = {7},
pages = {1309--1317},
publisher = {Elsevier Masson SAS},
title = {{Estimation of instantaneous local heat transfer coefficient in spark-ignition engines}},
url = {http://dx.doi.org/10.1016/j.ijthermalsci.2009.12.010},
volume = {49},
year = {2010}
}
@article{Murakami2012k,
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Murakami, Sumio},
doi = {10.1007/978-94-007-2666-6},
eprint = {arXiv:1011.1669v3},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/Continuum Damage Mechanics - SumioMurakami/KAp10{\_}Continuum Damage Mechanics of Composite Materials.pdf:pdf},
isbn = {978-94-007-2665-9},
issn = {09250042},
pages = {277--303},
pmid = {25246403},
title = {{Continuum Damage Mechanics}},
url = {http://link.springer.com/10.1007/978-94-007-2666-6},
volume = {185},
year = {2012}
}
@article{Shimp1971,
author = {Shimp, David A},
title = {{Speciality matrix resins}},
year = {1971}
}
@article{PeterThermalManagement2018,
author = {H{\"{o}}lz, Peter and B{\"{o}}hlke, Thomas and Kr{\"{a}}mer, Thomas},
number = {Submitted},
title = {{Two-stage calculation method for optimized thermal management}}
}
@article{Poisson-gleichung,
author = {Poisson-gleichung, Die and Operator, Laplace- and Symbol, Das},
title = {{Numerische Verfahren f u ¨ r}}
}
@article{Kramer2012,
abstract = {Material parameter identification is the necessary link between constitutive modeling and application of material models in complex simulations of real world problems. We present an approach to make use of already developed stress algorithms for three-dimensional finite-element computations in terms of a reduction to uniaxial tensile tests for material parameter identification. Strain-driven stress algorithms lead to the approach of solving differential-algebraic equations. ({\{}{\textcopyright}{\}} 2012 Wiley-VCH Verlag GmbH {\{}{\&}{\}} Co. KGaA, Weinheim)},
author = {Kr{\"{a}}mer, Stephan and Rothe, Steffen and Hartmann, Stefan},
doi = {10.1002/pamm.201210147},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Parametersch{\"{a}}tzung/2012{\_}Hartmann{\_}Material parameter identification using model reduction to uniaxial tensile test.pdf:pdf},
issn = {1617-7061},
journal = {Pamm},
number = {1},
pages = {315--316},
title = {{Material parameter identification using model reduction to uniaxial tensile test}},
url = {http://dx.doi.org/10.1002/pamm.201210147},
volume = {12},
year = {2012}
}
@article{Einheit,
author = {Einheit, Die and Signale, Analoge},
journal = {Pulse},
title = {{Antworten und L{\{}{\"{o}}{\}}sungen zu den Kontrollfragen und {\{}{\"{U}}{\}}bungsaufgaben}}
}
@article{Burg1925,
author = {Burg, Heinz and Arnold, J{\"{o}}rg},
pages = {461--469},
title = {{A16 Schienenfahrzeuge / Stra{\{}{\ss}{\}}enbahnen A16}},
year = {1925}
}
@article{Veranschaulichung,
author = {Veranschaulichung, Zur},
pages = {43--58},
title = {{5 Salzstreuer}}
}
@article{Wei1970a,
abstract = {Metal fatigue as an engineering problem has been well recognized. Many experiments have been carried out in recent years to assess the effects of load amplitude, mean load, load range and test frequency on the rate of fatigue-crack growth to characterize material response to different load profiles and to develop methods for estimating the service behavior of structural components. Recent studies have shown that fatigue-crack growth can be influenced strongly by the test environment; the effect being dependent on the particular material-environment involved. These results suggest that careful reassessments of the data of previous studies and of the proper direction for future fatigue research will be required. Hence, a critical review and analysis of existing fatigue-crack-growth data on high-strength aluminum and titanium alloys and high-strength steels has been made. The influences of load profile, test frequency, temperature, test environment and state-of-stress on fatigue-crack growth are discussed. Correlation with environment-enhanced crack growth under sustained loads and the associated changes in material response are examined. Possible mechanisms, synergistic effects and implications regarding methods for service-life estimation are considered. ?? 1970.},
author = {Wei, R P},
doi = {10.1016/0013-7944(70)90004-4},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/1970{\_}Wei{\_}Some aspects of environment-enhanced fatigue crack growth{\_}For example frequency in Al7075.pdf:pdf},
issn = {00137944},
journal = {Eng. Fract. Mech.},
number = {4},
pages = {633--651},
title = {{Some aspects of environment-enhanced fatigue-crack growth}},
volume = {1},
year = {1970}
}
@article{Pahl2007h,
author = {Pahl, Gerhard and Beitz†, Wolfgang and Feldhusen, J{\"{o}}rg and Grote, Karl-H.},
journal = {Pahl/Beitz Konstr. - Grundlagen},
title = {{Methodisches Entwerfen}},
year = {2007}
}
@article{Steward1938,
author = {Steward, G. C. and Caratheodory, C.},
doi = {10.2307/3607286},
isbn = {9783110351439},
issn = {00255572},
journal = {Math. Gaz.},
number = {252},
pages = {509},
title = {{Geometrische Optik}},
url = {http://www.jstor.org/stable/3607286?origin=crossref},
volume = {22},
year = {1938}
}
@article{Kr??mer2013a,
author = {Kr??mer, Stephan and Rothe, Steffen and Hartmann, Stefan},
doi = {10.1007/s00366-013-0337-7},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Parametersch{\"{a}}tzung/2013{\_}Hartmann{\_}Homogeneous stress–strain states computed by 3D-stress algorithms of FE-codes - application to material parameter identification.pdf:pdf},
issn = {14355663},
journal = {Eng. Comput.},
keywords = {DAE-systems,Finite elements,Material parameter identification,Plane stress,Stress algorithms},
number = {1},
pages = {141--159},
title = {{Homogeneous stress???strain states computed by 3D-stress algorithms of FE-codes: application to material parameter identification}},
volume = {31},
year = {2013}
}
@article{Seng,
author = {Seng, Jocelyn M},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/{\_}buecherSong/HandbookofComposites/III/Mechanics.pdf:pdf},
journal = {Production},
title = {{Laminate design}}
}
@article{Luk????1968a,
abstract = {Persistent slip bands in fatigued copper single crystals are studied by means of transmission electron microscopy of surface thin foils, both parallel and nonparallel to the surface. Comparing the observations from the different nonparallel sections a three-dimensional model of the internal structure may be constructed. Dislocations with all six possible Burgers vectors of the type 1/2 〈0011〉 are found in the structure. This demonstrates the microscopic action of the secondary slip systems during the low stress fatigue. The macroscopic action of the secondary systems, which is connected with the cell structure formation, is typical for the high stress fatigue. Surface extrusions are found to be related to the dislocation structure below the surface.},
author = {Luk????, P. and Klesnil, M. and Krej????, J.},
doi = {10.1002/pssb.19680270212},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/1968{\_}Luka{\_}Dislocations and persistent slip bands in copper single crystals fatigued at low stress amplitude.pdf:pdf},
isbn = {0031-8957},
issn = {15213951},
journal = {Phys. Status Solidi},
number = {2},
pages = {545--558},
title = {{Dislocations and Persistent Slip Bands in Copper Single Crystals Fatigued at Low Stress Amplitude}},
volume = {27},
year = {1968}
}
@article{Singer1977a,
abstract = {The aluminum alloy investigated contained about 2. 7{\{}{\%}{\}} Cu, 1. 6{\{}{\%}{\}} Mg, 1. 1{\{}{\%}{\}} Fe, 1{\{}{\%}{\}} Ni, and small amounts of Si, Zn, and Ti. Creep at 473 K resulted in deformation-induced softening because of microstructural instability. Creep tests at varied stresses and temperatures were performed to explore the dislocation mechanisms during creep in specimens subjected to 13 different thermomechanical treatments. It was found that the room temperature yield stress and creep resistance after prolonged creep stressing can be improved by preliminary deformation, whereas the initial creep resistance is decreased. This is explained in terms of the effect of deformation on the structure and its stability.},
author = {Singer, Robert and Blum, Wolfgang},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Empirical Fatigue Models + Validation/1975{\_}Blum{\_}The influence of thermomechanical treatment on the creep resistance of RR58 - Al2618.pdf:pdf},
issn = {00443093},
journal = {Zeitschrift fuer Met. Res. Adv. Tech.},
number = {5},
title = {{Influence of Thermomechanical Treatments on the Creep Resistance of Rr 58 At Elevated Temperature.}},
volume = {68},
year = {1977}
}
@article{Leidich,
author = {Leidich, Erhard and Deters, Ludger},
doi = {10.1007/978-3-540-76647-6},
isbn = {978-3-540-76647-6},
issn = {0937-7433},
journal = {Konstr. des Maschinenbaus},
pages = {13--69},
title = {{Normen, Toleranzen, Passungen und Technische Oberfl{\"{a}}chen}},
url = {http://www.springerlink.com/content/k3qk85404263063q/}
}
@article{Software,
author = {Software, Kommerzielle and Methode, Die and Schwerpunkt, Der and Mks, Kreiselbewegung and Sch, Emks Schmierfilm and Elektrotechnik, Temperaturfelder and Schalldruckverteilung, Wellenfelder},
pages = {11--15},
title = {{2 Anwendungsfelder und Software}}
}
@article{Ritchie1985,
abstract = {Relationships between crack initiation and crack growth toughness are reviewed by examining the crack tip fields and microscopic (local) and macroscopic (continuum) fracture criteria for the onset and continued quasi-static extension of cracks in ductile materials. By comparison of the micromechanisms of crack initiation via transgranular cleavage and crack initiation and subsequent growth via microvoid coalescence, expressions are shown for the fracture toughness of materials in terms of microstructural parameters. Utilizing the exact asymptotic crack tip deformation fields for the nonstationary plane strain Mode I crack and evoking various microscopic failure criteria for such stable crack growth, a relationship between the tearing modulus TR and the nondimensionalized crack initiation fracture toughness Jlc is described and shown to yield a good fit to experimental toughness data for a wide range of steels},
author = {Ritchie, R. O. and Thompson, A. W.},
doi = {10.1007/BF02815305},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/1985{\_}RichtieAndThompson{\_}On Macroscopic and Microscopic Analyses for Crack Initiation and Crack Groth Toughness in Ductile Alloys.pdf:pdf},
isbn = {0360-2133},
issn = {03602133},
journal = {Metall. Trans. A},
number = {1},
pages = {233--248},
title = {{On macroscopic and microscopic analyses for crack initiation and crack growth toughness in ductile alloys}},
volume = {16},
year = {1985}
}
@article{Oo1962,
author = {Oчирoв, У. У.},
journal = {Записки Калмыцкого Научно-Исследовательского Института Языка, Литературы И Истории},
pages = {167--192},
title = {{Придатoчныe Прeдлo{\v{z}}eния Врeмeни}},
volume = {Выпуск 2},
year = {1962}
}
@article{Zahoransky2013d,
author = {Zahoransky, Richard a. and Allelein, Hans-Josef and Schelling, Udo and Schwarz, Harald and Bollin, Elmar and Oehler, Helmut},
doi = {10.1007/978-3-8348-2279-6},
isbn = {978-3-8348-1869-0},
journal = {Energietechnik - Syst. zur Energieumwandlung},
pages = {378--386},
title = {{16 Energetische M{\{}{\"{u}}{\}}llverwertung}},
url = {http://www.springerlink.com/index/10.1007/978-3-8348-2279-6},
year = {2013}
}
@book{Steinbach2008,
author = {Steinbach, Olaf},
booktitle = {English},
doi = {10.1007/978-0-387-68805-3},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Steinbach 2000 - Numerical Approximation Methods for Elliptic Boundary Value Problems.pdf:pdf},
isbn = {978-0-387-31312-2},
title = {{Numerical Approximation Methods for Elliptic Boundary Value Problems}},
url = {http://www.springerlink.com/index/10.1007/978-0-387-68805-3},
year = {2008}
}
@book{Fallis2013,
abstract = {Predicting the binding mode of flexible polypeptides to proteins is an important task that falls outside the domain of applicability of most small molecule and protein−protein docking tools. Here, we test the small molecule flexible ligand docking program Glide on a set of 19 non-$\alpha$-helical peptides and systematically improve pose prediction accuracy by enhancing Glide sampling for flexible polypeptides. In addition, scoring of the poses was improved by post-processing with physics-based implicit solvent MM- GBSA calculations. Using the best RMSD among the top 10 scoring poses as a metric, the success rate (RMSD ≤ 2.0 {\AA} for the interface backbone atoms) increased from 21{\%} with default Glide SP settings to 58{\%} with the enhanced peptide sampling and scoring protocol in the case of redocking to the native protein structure. This approaches the accuracy of the recently developed Rosetta FlexPepDock method (63{\%} success for these 19 peptides) while being over 100 times faster. Cross-docking was performed for a subset of cases where an unbound receptor structure was available, and in that case, 40{\%} of peptides were docked successfully. We analyze the results and find that the optimized polypeptide protocol is most accurate for extended peptides of limited size and number of formal charges, defining a domain of applicability for this approach.},
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Fallis, A.G},
booktitle = {J. Chem. Inf. Model.},
doi = {10.1017/CBO9781107415324.004},
eprint = {arXiv:1011.1669v3},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Ghosh 2012 - Computational Methods for Microstructure-Property Relationships.pdf:pdf},
isbn = {9788578110796},
issn = {1098-6596},
keywords = {icle},
number = {9},
pages = {1689--1699},
pmid = {25246403},
title = {{ComputationalMethods forMicrostructure-Property Relationships}},
volume = {53},
year = {2013}
}
@article{Nitsche2006a,
author = {Nitsche, Wolfgang},
journal = {Str{\{}{\"{o}}{\}}mungsmesstechnik},
pages = {189--202},
title = {{Signalanalyse}},
year = {2006}
}
@article{Lin1969,
abstract = {The mechanics of the build-up of large local plastic strains at the free surface of a polycrystal under fatigue loading is shown. Two closely located thin slices in a most-favourably-oriented crystal located at a free surface of the polycrystal are assumed to have an initial resolved shear stress of a few psi of opposite sign. Under cyclic loading, the two thin slices slide in opposite directions, one during the forward loading and the other during the reversed loading. Based on the dependency of slip on the resolved shear stress, the increase of local plastic strain in the slices with cycles of loading is calculated by applying the analogy between plastic strain and external force. The calculated local plastic shear strain in both slices (one positive and the other negative) reaches 100 per cent at the free surface in a few hundred cycles. These large plastic shear strains clearly cause the start of an extrusion or intrusion and the nucleation of a fatigue crack.},
author = {Lin, T H and Ito, Y M},
doi = {doi: DOI: 10.1016/0022-5096(69)90006-4},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/1969{\_}Lin{\_}Mechanics of a fatigue crack nucleation mechanism.pdf:pdf},
isbn = {0022-5096},
issn = {0022-5096},
journal = {J. Mech. Phys. Solids},
pages = {511--523},
title = {{Mechanics of a Fatigue Crack Nucleation Mechanism}},
url = {http://www.sciencedirect.com/science/article/pii/0022509669900064},
volume = {17},
year = {1969}
}
@article{Pol??k2016,
abstract = {Results of the study of the early fatigue damage in a number of model and structural crystalline materials using modern experimental techniques are presented. The dislocation structure of the persistent slip bands and the evolution of the surface relief resulting in the formation of persistent slip markings during cyclic loading are documented. The dislocation mechanisms leading to production of point defects in cyclic loading are described and point defect production and annihilation rates are derived. The kinetics of point defect migration is characterized. The physically based models of the surface relief formation describing the formation of extrusions and intrusions are presented. The models are confronted with experimental evidence. It is concluded that intrusions representing sharp surface crack-like defects play the principal role in the initiation of fatigue cracks.},
author = {Pol??k, Jaroslav and Man, Ji????},
doi = {10.1016/j.ijfatigue.2016.02.021},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/2016{\_}Polak+Man{\_}Experimental evidence and physical models of fatigue crack initiation.pdf:pdf},
issn = {01421123},
journal = {Int. J. Fatigue},
keywords = {Crack initiation,Extrusions,Intrusions,Persistent slip band,Point defects},
pages = {294--303},
title = {{Experimental evidence and physical models of fatigue crack initiation}},
volume = {91},
year = {2016}
}
@book{Besson2010,
author = {Besson, Jacques and Cailletaud, Georges and Chaboche, Jean-Louis and Forest, Samuel},
booktitle = {Solid Mech. its Appl.},
doi = {10.1007/978-90-481-3356-7},
isbn = {978-90-481-3355-0},
keywords = {emergency,luation of non-urgent visits,to a busy urban},
pages = {1--450},
title = {{Non-Linear Mechanics of Materials}},
volume = {33},
year = {2010}
}
@article{Eigenschaften,
author = {Eigenschaften, Aufbau},
title = {{4 Der Reifen}}
}
@article{Bozza2011b,
abstract = {In the present paper a combined procedure for the quasi-dimensional modelling of heat transfer, combustion and knock phenomena in a "downsized" Spark Ignition two-cylinder turbocharged engine is presented. The procedure is extended to also include the effects consequent the Cyclic Variability. Heat transfer is modelled by means of a Finite Elements model. Combustion simulation is based on a fractal description of the flame front area. Cyclic Variability (CV) is characterized through the introduction of a random variation on a number of parameters controlling the rate of heat release (air/fuel ratio, initial flame kernel duration and radius, laminar flame speed, turbulence intensity). The intensity of the random variation is specified in order to realize a Coefficient Of Variation (COV) of the Indicated Mean Effective Pressure (IMEP) similar to the one measured during an experimental campaign. Moreover, the relative importance of the various concurring effects is established on the overall COV. A kinetic scheme is then solved within the unburned gas zone, characterized by different thermodynamic conditions occurring cycle-by-cycle. In this way, an optimal choice of the "knock-limited" spark advance is effected and compared with experimental data. Finally, the CV effects on the occurrence of individual knocking cycles are assessed and discussed. {\textcopyright} 2011 Global Science Press.},
author = {Bozza, Fabio and Siano, Daniela and Costa, Michela},
doi = {10.4208/aamm.10-10s2-04},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2011{\_}Bozza{\_}heat-transfer-knock-modeling-and-cyclic-variability-in-a-downsized-spark-ignition-turbocharged-engine.pdf:pdf},
issn = {20700733},
journal = {Adv. Appl. Math. Mech.},
keywords = {Cyclic variability,Finite elements in heat transfer,Internal combustion engines modelling,Knock},
number = {3},
pages = {310--326},
title = {{Heat transfer, knock modeling and cyclic variability in a "Downsized" spark-ignition turbocharged engine}},
volume = {3},
year = {2011}
}
@book{Berger2003b,
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Berger},
booktitle = {Eng. Med. Biol. Soc. 2008. EMBS 2008. 30th Annu. Int. Conf. IEEE},
doi = {10.1002/ejoc.201200111},
eprint = {arXiv:1011.1669v3},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Vortraege/Book-of-Abstracts{\_}2016-03-04{\_}GAMM.pdf:pdf},
isbn = {9781107671812},
issn = {0196-6553},
pages = {2004},
pmid = {26840611},
title = {{Table of of contents}},
volume = {24},
year = {2003}
}
@article{Foreste,
author = {Forest, Samuel},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/xxx{\_}Forest{\_}Micromorphic Media.pdf:pdf},
title = {{Micromorphic media}}
}
@article{Schneider2016b,
abstract = {{\{}{\textcopyright}{\}} 2016 Elsevier B.V.Modeling of crack propagation in materials has long been a challenge in solid-state physics and materials science. The phase-field method has now established as one of the tools for the description of crack propagation. The applied models are thermodynamically consistent and predict crack propagation in homogeneous materials under the consideration of different loading types, multiple physical fields and geometrical nonlinearities. Even dynamic loading processes are studied, including plastic effects. A multiphase-field model for crack propagation, which is indispensable to describe crack propagation on a mesoscopic length scale, is still missing. In this work, we overcome this deficiency and combine a crack propagation approach, which is based on Griffith's theory, with an established multiphase-field model for phase transformation.},
author = {Schneider, D and Schoof, E and Huang, Y and Selzer, M and Nestler, B},
doi = {10.1016/j.cma.2016.04.009},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Thermodynamik/PhasenFeld/Schneider{\_}Crack{\_}propagation{\_}multiphase{\_}systems-Dez2015.pdf:pdf},
issn = {00457825},
journal = {Comput. Methods Appl. Mech. Eng.},
keywords = {crack propagation,multiphase-field,phase-field,polycrystalline material},
title = {{Phase-field modeling of crack propagation in multiphase systems}},
url = {http://dx.doi.org/10.1016/j.cma.2016.04.009},
year = {2016}
}
@article{Ieee,
author = {Ieee, Recent and Dae, The},
title = {{4 Sensitivity Analysis for Voltage Stability}}
}
@article{Burgb,
author = {Burg, Heinz},
pages = {595--611},
title = {{B1 B1 Unf{\{}{\"{a}}{\}}lle mit Tieren B1}}
}
@article{Bouaziz2012a,
abstract = {The current work extends the well established approach of Kocks and Mecking by a more realistic description of strain-hardening using an original dislocation density law with a revisited physical understanding of dynamic recovery, without new material parameters and keeping only one internal variable. The current work extends the well established approach of Kocks and Mecking by a more realistic description of strain-hardening using an original dislocation density law with a revisited physical understanding of dynamic recovery, without new material parameters and keeping only one internal variable. First validation shows that the new approach is more consistent with experiments than the common Kocks-Mecking modeling with the same number of parameters. Copyright {\textcopyright} 2012 WILEY-VCH Verlag GmbH {\&} Co. KGaA, Weinheim.},
author = {Bouaziz, O.},
doi = {10.1002/adem.201200083},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/Hardening Recovery Creep/2012{\_}BouazizRevisited Storage and Dynamic Recovery of Dislocation Density Evolution Law- Toward a Generalized Kocks–Mecking Model of Strain-Hardening.pdf:pdf},
issn = {14381656},
journal = {Adv. Eng. Mater.},
number = {9},
pages = {759--761},
title = {{Revisited storage and dynamic recovery of dislocation density evolution law: Toward a generalized kocks-mecking model of strain-hardening}},
volume = {14},
year = {2012}
}
@article{Tribologie2000,
author = {Tribologie, Fachgebiet},
doi = {10.1007/978-3-8348-8279-0},
isbn = {9783834882790},
pages = {2000},
title = {{4 Tribologie 4 4.1}},
year = {2000}
}
@article{Misdariis2015,
abstract = {Large Eddy Simulation of knocking in piston engines requires high-fidelity physical models and numerical techniques. The need to capture temperature fields with high precision to predict autoignition is an additional critical constraint compared to existing LES in engines. The present work presents advances for LES of knocking in two fields: (1) a Conjugate Heat Transfer (CHT) technique is implemented to compute the flow within the engine over successive cycles with LES together with the temperature field within the cylinder head walls and the valves and (2) a reduced two-step scheme is used to predict both propagating premixed flames as well as autoignition times over a wide range of equivalence ratios, pressures and temperatures. The paper focuses on CHT which is critical for knocking because the gas temperature field is controlled by the wall temperature field and knocking is sensitive to small temperature changes. The CHT LES is compared to classical LES where the temperatures of the head and the valves are supposed to be homogeneous and imposed empirically. Results show that the skin temperature field (which is a result of the CHT LES while it is a user input for classical LES) is complex and controls knocking events. While the results of the CHT LES are obviously better because they suppress a large part of the empirical specification of the wall temperatures, this study also reveals a difficult and crucial element of the CHT approach: the description of exhaust valves cooling which are in contact with the engine head for part of the cycle and not in the rest of the cycle, leading to difficulties for heat transfer descriptions between valves and head. The CHT method is successfully applied to an engine studied at IFP Energies Nouvelles where knocking characteristics have been studied over a wide range of conditions.},
author = {Misdariis, Antony and Vermorel, Olivier and Poinsot, Thierry},
doi = {10.1016/j.combustflame.2015.07.023},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Klopfen{\_}Ottomotor/2015{\_}Misdariis{\_}LES of knocking in engines using dual heat transfer and two-step reduced schemes{\_}ModelForHeatConductionBetweenValveAndRing.pdf:pdf},
issn = {00102180},
journal = {Combust. Flame},
keywords = {Autoignition,Heat transfert,Internal combustion engine,Knock,LES},
number = {11},
pages = {4304--4312},
publisher = {Elsevier Ltd.},
title = {{LES of knocking in engines using dual heat transfer and two-step reduced schemes}},
url = {http://dx.doi.org/10.1016/j.combustflame.2015.07.023},
volume = {162},
year = {2015}
}
@article{Januszka2015,
author = {Januszka, Marcin and Panfil, Wawrzyniec},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2016{\_}Lasocki{\_}ENGINE KNOCK DETECTION AND EVALUATION - A REVIEW.pdf:pdf},
number = {102},
pages = {37--48},
title = {{Proceedings of the institute of vehicles 2(102)/2015}},
volume = {2},
year = {2015}
}
@article{Leichtbaua,
author = {Leichtbau, Im},
pages = {38--64},
title = {{6 Leichtbauwerkstoffe}}
}
@article{Mutzke2016b,
abstract = {{\{}{\textcopyright}{\}} 2016 SAE International.Knocking combustion places a major limit on the performance and efficiency of spark ignition engines. Spontaneous ignition of the unburned air-fuel mixture ahead of the flame front leads to a rapid release of energy, which produces pressure waves that cause the engine structure to vibrate at its natural frequencies and produce an audible 'pinging' sound. In extreme cases of knock, increased temperatures and pressures in the cylinder can cause severe engine damage. Damage is thought to be caused by thermal strain effects that are directly related to the heat flux. Since it will be the maximum values that are potentially the most damaging, then the heat flux needs to be measured on a cycle-by-cycle basis. Previous work has correlated heat flux with the pressure fluctuations on an average basis, but the work here shows a correlation on a cycle-by-cycle basis. The in-cylinder pressure and surface temperature were measured using a pressure transducer and eroding-type thermocouple. These sensors were installed side-by-side at the surface of the cylinder in order to investigate the relationship between knock and heat flux on a cycle-by-cycle basis. A finite difference method was implemented to solve the one-dimensional unsteady heat conduction equation and calculate the temperature distribution away from the surface of the combustion chamber, and thus the instantaneous heat flux. The knock intensity was varied by controlling the fuel quality, compression ratio, ignition timing and air-fuel ratio. The measured heat flux was compared with pressure-based knock indices and it was found that as knock intensity increases, the correlation with peak heat flux became stronger. Results from different fuels and engine operating conditions did not collapse onto the same trend line. At higher speeds and higher compression ratios the heat flux was higher at a given level of knock intensity. The co-location of the pressure transducer and heat flux sensor meant that a correlation was found on a cycle-by-cycle basis.},
author = {Mutzke, J and Scott, B and Stone, R and Williams, J},
doi = {10.4271/2016-01-0700},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2016{\_}Mutzke{\_}The Effect of Combustion Knock on the Instantaneous Heat Flux in Spark Ignition Engines.pdf:pdf},
journal = {SAE Tech. Pap.},
title = {{The Effect of Combustion Knock on the Instantaneous Heat Flux in Spark Ignition Engines}},
volume = {2016-April},
year = {2016}
}
@article{Stresses1988,
author = {Stresses, Residual and Energy, Stored Elastic},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/1990{\_}Kreher{\_}Residual stresses and stored elastic energy of composites and polycrystals.pdf:pdf},
title = {{RESIDUAL STRESSES AND STORED ELASTIC ENERGY Of: {\{}{\~{}}{\}}U{\{}{\~{}}{\}}P{\{}{\~{}}{\}}S{\{}{\~{}}{\}}TES AND PULYCRYSTALS}},
year = {1988}
}
@article{Computertechnik1947,
author = {Computertechnik, In Der},
journal = {System},
pages = {205--210},
title = {{12 Computertechnik}},
volume = {1947},
year = {1947}
}
@article{Seyedi,
author = {Seyedi, M and Desmorat, R},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/2 scale models papers/Seyedi+Desmorat+Sermage{\_}A TWO SCALE DAMAGE MODEL FOR THERMOMECHANICAL HIGH CYCLE FATIQUE FAILURE.pdf:pdf},
title = {{Two Scale Damage Model for Thermomechanical High Cycle Fatigue Failure}}
}
@article{Verbindungslinie,
author = {Verbindungslinie, Die and Stab, Der and Kraft, Dimension},
doi = {10.1007/978-3-642-19984-4},
isbn = {9783642199844},
journal = {Dimens. Contemp. Ger. Arts Lett.},
title = {{1 Zug und Druck in St ¨ aben}},
volume = {2}
}
@article{Weertman1955a,
abstract = {A theory of steady-state creep is developed using Mott's mechanism of dislocation climb. It is assumed in the analysis that the rate-controlling process is the diffusion of vacancies between dislocations which are creating vacancies and those which are destroying them. The concentration of vacancies along a dislocation line is determined by setting the change in the free energy caused by a decrease or increase in the number of vacancies equal to the change in the elastic energy occuring during dislocation climb. The creep equation that results from the analysis is creep rate=const (o-{\textless}Y./kT)exp(-Q/kT) where" is a constant ("",3 to 4), Q is the activation energy of self-diffusion, kT has its usual meaning, and 0- to 108 is the stress. This equation is valid in the stress range from the critical shear stress to a stress about equal to 10' dynes/cm'. At larger stresses the creep rate increases much more rapidly with stress.},
author = {Weertman, J.},
doi = {10.1063/1.1721875},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Kriechen{\_}Spannungsrelaxation/1955{\_}Weertman{\_}Theory of Steady-State Creep Based on Dislocation Climb.pdf:pdf},
isbn = {0021-8979},
issn = {00218979},
journal = {J. Appl. Phys.},
number = {10},
pages = {1213--1217},
title = {{Theory of steady-state creep based on dislocation climb}},
volume = {26},
year = {1955}
}
@article{Timoshenko,
author = {Timoshenko, The},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Zienkiewicz FEM - Vol 2 Solid Structural Mechanics/63212{\_}10.pdf:pdf},
title = {{Structural mechanics problems in one dimension – rods}}
}
@article{Mandadapu2012,
abstract = {This article proposes a continuum thermomechanical homogenization method inspired by the Irving-Kirkwood procedure relating the atomistic equations of motion to the balance laws of continuum mechanics. This method yields expressions for the macroscopic stress and heat flux in terms of microscopic kinematic and kinetic quantities. The resulting equation for macroscopic stress affords a rational comparison with the widely used Hill-Mandel stress-deformation condition, while the one for heat flux reduces, under certain assumptions, to a Hill-Mandel-like condition involving heat flux and the gradient of temperature.},
archivePrefix = {arXiv},
arxivId = {84862181137},
author = {Mandadapu, K K and Sengupta, A and Papadopoulos, P},
doi = {10.1098/rspa.2011.0578},
eprint = {84862181137},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/A homogenization method for thermomechanical continua using extensive physical quantities.pdf:pdf},
isbn = {1364-5021{\$}\backslash{\$}r1471-2946},
issn = {1364-5021},
journal = {Proc. R. Soc. A Math. Phys. Eng. Sci.},
keywords = {hill,homogenization,irving,kirkwood procedure,mandel condition,thermomechanics},
number = {2142},
pages = {1696--1715},
title = {{A homogenization method for thermomechanical continua using extensive physical quantities}},
url = {http://rspa.royalsocietypublishing.org/content/early/2012/02/16/rspa.2011.0578.full},
volume = {468},
year = {2012}
}
@article{Bindeglied,
author = {Bindeglied, Das and Beginn, Zu and Auswahl, Die and Bemerkung, Die},
journal = {Sensors (Peterborough, NH)},
title = {{10 Sensoren}}
}
@article{Funktiona,
author = {Funktion, Definitionsbereich Der},
pages = {67--128},
title = {{III Funktionen und Kurven 2 Allgemeine Funktionseigenschaften}}
}
@article{Chen2014,
abstract = {A predictive knock model is crucial for one dimensional (1-D) engine cycle simulation that has been proven to be a powerful tool in both optimization of the conceptual design and reduction of calibration efforts in development of spark-ignition (SI) engines. With application of advanced technologies such as exhaust gas recirculation (EGR) in modern SI engines, update of knock model is needed to give an acceptable prediction of knock onset. In this study, bench tests of a turbocharged gasoline SI engine with cooled EGR system operated under knocking conditions were conducted, the cylinder pressure traces were analyzed by the band-pass filtering technique, and the crank angle of knock onset was determined by the signal energy ratio (SER) and image processing method. A knock model considering multi-variable effects including pressure, temperature, EGR ratio and excess air ratio (??) is formulated and calibrated with the experimental data using the multi-island genetic algorithm (GA). The calculation method of the end gas temperature, the impacts of the ratio of specific heats as well as the temperature at the intake valve closure on the end gas temperature are discussed. The performance of the new model is compared with the widely-used phenomenological knock models such as Douaud-Eyzat model and Hoepke model. While the widely-used knock models fail to give acceptable predictions when increasing EGR with fuel enrichment operations, the new model predicts the knock onset with high accuracy under the fuel enrichment conditions both with and without EGR. Performance of the newly developed model is also examined in a different engine and a higher predictive accuracy of the new model than other models is obtained. ?? 2014 Elsevier Ltd. All rights reserved.},
author = {Chen, Longhua and Li, Tie and Yin, Tao and Zheng, Bin},
doi = {10.1016/j.enconman.2014.08.002},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2014{\_}Chen+Li{\_}A predictive model for knock onset in spark-ignition engines with cooled EGR.pdf:pdf},
issn = {01968904},
journal = {Energy Convers. Manag.},
keywords = {Excess air ratio,Exhaust gas recirculation,Knock modeling,Knock onset,Spark ignition engines},
pages = {946--955},
publisher = {Elsevier Ltd},
title = {{A predictive model for knock onset in spark-ignition engines with cooled EGR}},
url = {http://dx.doi.org/10.1016/j.enconman.2014.08.002},
volume = {87},
year = {2014}
}
@article{Merkera,
author = {Merker, G{\"{u}}nter and Schwarz, Christian and Stiesch, Gunnar and Otto, Frank},
journal = {Simul. der Verbrennung und Schadstoffbildung},
title = {{9 Str{\{}{\"{o}}{\}}mungsmechanische Simulation}}
}
@article{Krank2008,
author = {Krank, Lothar and Meroth, Ansgar and Streit, Andreas and Tolg, Boris},
pages = {147--207},
title = {{5 Netzwerke im Fahrzeug}},
year = {2008}
}
@article{Eds,
author = {Eds, Firma},
pages = {322--403},
title = {{Fallstudien *)}}
}
@book{Taylor2005,
author = {Taylor, R.L. and Zienkiewicz, O.C.},
booktitle = {Int. J. Numer. Methods Eng.},
isbn = {9780750663212},
pages = {1863},
title = {{The Finite Element Method for Solid and Structural Mechanics}},
year = {2005}
}
@article{Murakami2012g,
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Murakami, Sumio},
doi = {10.1007/978-94-007-2666-6},
eprint = {arXiv:1011.1669v3},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/Continuum Damage Mechanics - SumioMurakami/Kap11{\_}Local Approach to Damage and Fracture.pdf:pdf},
isbn = {978-94-007-2665-9},
issn = {09250042},
pages = {305--323},
pmid = {25246403},
title = {{Continuum Damage Mechanics}},
url = {http://link.springer.com/10.1007/978-94-007-2666-6},
volume = {185},
year = {2012}
}
@article{Zienkiewicz2013b,
abstract = {The set of differential equations from which we start the discretization process will determine whether we refer to the formulation as mixed or irreducible. Thus if we consider an equation system with several dependent variables u written as [see Eqs (3.1) and (3.2)] A ( u ) = 0 in domain $\Omega$ (10.1a) and ℬ ( u ) = 0 on boundary $\Gamma$ (10.1b) in which none of the components of u can be eliminated still leaving a well-defined problem, then the formulation will be termed irreducible. If this is not the case the formulation will be called mixed. These definitions were given in Chapter 3 (p. 56). Publisher Summary The aim of this chapter is to discuss mixed formulation and constraints. The set of differential equations from which the discretization process is started determines whether the formulation is referred to as mixed or as irreducible. This chapter demonstrates how elasticity problems can be dealt with in mixed form and shows how such formulations are essential in certain problems. If the operator specifying the mixed form is symmetric or self-adjoint, the formulation can proceed from the basis of a variational principle that can be directly obtained for linear problems. This chapter essentially outlines the mixed form of finite element formulation, which opens a new range of possibilities, many with potentially higher accuracy and robustness than those offered by irreducible forms. However, an additional advantage arises even in situations where, by the principle of limitation, the irreducible and mixed forms yield identical results. Therefore, the study of the behavior of the mixed form can frequently reveal weaknesses or lack of robustness in the irreducible form that otherwise would be difficult to determine. The mixed approximation expands the potential of the finite element method and presents almost limitless possibilities of detailed improvement.},
author = {Zienkiewicz, O.C. and Taylor, R.L. and Zhu, J.Z.},
doi = {10.1016/B978-1-85617-633-0.00009-5},
isbn = {978-0-7506-6431-8},
issn = {00295981},
journal = {Finite Elem. Method its Basis Fundam.},
pages = {285--314},
title = {{Mixed Formulation and Constraints: Complete Field Methods}},
url = {http://linkinghub.elsevier.com/retrieve/pii/B9781856176330000095},
year = {2013}
}
@article{Teilaufgabenc,
author = {Teilaufgaben, Abzuhandelnde},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Empirical Fatigue Models + Validation/Betriebsfestigkeit{\_}ErwinHaibach/Kap4 Praktische Umsetzung des Betriebsfestigkeits-Konzepts.pdf:pdf},
title = {{des Betriebsfestigkeits-Konzeptes}}
}
@article{Wallentowitz2006g,
author = {Wallentowitz, Henning and Reif, Konrad},
doi = {10.1007/978-3-8348-9121-1_16},
isbn = {978-3-528-03971-4},
journal = {Handb. Kraftfahrzeugelektronik},
pages = {609--650},
title = {{Handbuch Kraftfahrzeugelektronik}},
url = {http://www.springerlink.com/index/10.1007/978-3-8348-9121-1{\_}16},
year = {2006}
}
@article{Unfallrekonstruktion,
author = {Unfallrekonstruktion, Begriffe Der},
pages = {937--965},
title = {{D1 D1 Fachbegriffe nach DIN 75204 Stra{\ss}enfahrzeuge D1}}
}
@article{Validierung,
author = {Validierung, Unter and Gliederung, Die and Aspekte, Einige and Abschnitt, Mit and Entwicklungsmethodik, Die and Fahrzeugvalidierung, Die},
title = {{Validierung : M ¨ oglichkeiten und Konzepte}}
}
@book{Reuter2008b,
author = {Reuter, Manfred and Zacher, Serge},
booktitle = {Anal. Simul. und Entwurf von Regelkreisen},
doi = {10.1007/978-3-8348-9273-7},
isbn = {978-3-8348-0018-3},
title = {{Aus dem Programm}},
year = {2008}
}
@article{Polak2014a,
abstract = {Experimental data on the formation of persistent slip markings (PSMs) at the egressing persistent slip bands (PSBs) and physically based models of surface relief formation and fatigue crack initiation are surveyed. The original Pol{\{}{\'{a}}{\}}k's model of fatigue crack initiation based on the formation, migration and annihilation of vacancy-type defects in PSBs is further refined and extended by taking into consideration the annihilation of vacancies in the matrix and the formation of internal stresses. The proposed mechanisms of surface relief formation are based on the plastic relaxation of internal compression stresses in PSBs and internal tensile stresses in the matrix. By solving the migration of vacancies from the PSB and their annihilation in the matrix, the shapes of extrusion and parallel intrusions are derived analytically under some simplifying assumptions. {\{}{\textcopyright}{\}} 2013 Elsevier B.V.},
author = {Pol{\'{a}}k, J and Man, J},
doi = {10.1016/j.msea.2013.12.005},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/2014{\_}Polak+Man{\_}Mechanisms of extrusion and intrusion formation in fatigued crystalline materials.htm.pdf:pdf},
issn = {09215093},
journal = {Mater. Sci. Eng. A},
keywords = {Crack initiation,Extrusion,Fatigue,Intrusion,Persistent slip band (PSB)},
pages = {15--24},
publisher = {Elsevier},
title = {{Mechanisms of extrusion and intrusion formation in fatigued crystalline materials}},
url = {http://dx.doi.org/10.1016/j.msea.2013.12.005},
volume = {596},
year = {2014}
}
@article{Einsicht,
author = {ergibt sich die Einsicht, D},
journal = {Springer},
title = {{1 Physikalische und mathematische Hilfsmittel}},
url = {http://link.springer.com/chapter/10.1007/978-3-8351-9095-5{\%}7B{\_}{\%}7D1}
}
@article{Sanli2009a,
author = {Sanli, A and Sayin, C and Gumus, M and Kilicaslan, I and Canakci, M},
journal = {Numer. Heat Transf. Part A Appl.},
number = {5},
pages = {444--458},
title = {{Numerical Evaluation by Models of Load and Spark Timing Effects on the In-Cylinder Heat Transfer of a SI Engine}},
volume = {56},
year = {2009}
}
@article{Zavala2011a,
author = {Zavala, Jos{\'{e}} Carlos and Folkerts, Charles},
doi = {10.4271/2011-01-1409},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2011{\_}Zavala{\_}Knock Detection and Estimation Based on Heat Release Startegies.pdf:pdf},
title = {{Knock Detection and Estimation Based on Heat Release Strategies}},
url = {http://papers.sae.org/2011-01-1409/},
year = {2011}
}
@article{Chemie1806b,
author = {Chemie, Organische},
pages = {1--16},
title = {{1 Einf{\"{u}}hrung}},
year = {1806}
}
@article{Eindhoven2005,
author = {Eindhoven, Uni and Polystyrene, Isotactic and Press, Academic and Verlag, Shaker},
pages = {272--282},
title = {{Quellennachweis}},
year = {2005}
}
@inproceedings{Kleinschmidt1993,
address = {Graz},
author = {Kleinschmidt, W.},
booktitle = {4. Tagung "Der Arbeitsprozess des Verbrennungsmotors"},
title = {{Zur Theorie und Berechnung der instation{\"{a}}ren W{\"{a}}rme{\"{u}}bertragung in Verbrennungsmotoren}},
year = {1993}
}
@article{Liu1996,
author = {Liu, I S},
doi = {10.1007/s001610050042},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Thermodynamik/Liu{\_}Entropieprinzip{\_}Lagrange/On Entropy Flux Heat Flux Relation in Thermodynamic with Lagrange Multipliers {\_} Liu.pdf:pdf},
issn = {0935-1175},
journal = {Contin. Mech. Thermodyn.},
number = {4},
pages = {247--256},
title = {{On entropy flux heat flux relation in thermodynamics with Lagrange multipliers}},
volume = {8},
year = {1996}
}
@article{Schie??l2003a,
abstract = {We investigate spatial temperature fluctuations in the unburned endgas of a spark-ignited (SI) engine. Our approach exploits the fact that the quantities (species concentrations, temperature) comprising the state of the combustion chamber gases are not independent, but often correlate sharply. Information about spatial temperature variations is obtained indirectly by observing two complementary quantities that sensitively reflect the local temperature. Spatial formaldehyde (H2CO) concentration variations in the endgas are converted to temperature fluctuations using calculated correlations between temperature and [H2CO]. Additionally, the geometrical size of inhomogeneities is deduced from LIF-images displaying the locally varying formation of temperature-sensitive intermediate species. The results indicate that temperature fluctuations exceeding 20 K are present in the nominally homogeneous endgas. The geometrical size of these fluctuations ranges from ???1 mm to ???1 cm. ?? 2003 The Combustion Institute. All rights reserved.},
author = {Schie??l, R. and Maas, U.},
doi = {10.1016/S0010-2180(02)00538-2},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Klopfen{\_}Ottomotor/2003{\_}Schiessl{\_}Analysis of endgas temperture fluctuations in an si engine by LIF.pdf:pdf},
isbn = {4907116855653},
issn = {00102180},
journal = {Combust. Flame},
keywords = {Endgas,IC engines,Laser-induced fluorescence,Temperature fluctuations},
number = {1-2},
pages = {19--27},
title = {{Analysis of endgas temperature fluctuations in an SI engine by laser-induced fluorescence}},
volume = {133},
year = {2003}
}
@article{Hashin1962b,
abstract = {Variational principles for anisotropic and nonhomogeneous elasticity, established by the authors in a previous paper, have been applied to the derivation of lower and upper bounds for the elastic moduli of polycrystals in terms of the moduli of the constituting crystals. The results hold for arbitrary crystal shapes. Explicit results tor cubic polycrystals showed that the present bounds are a considerable improvement of the well-known Voigt and Reuss bounds. Good agreement with experimental results has been obtained.},
author = {Hashin, Z and Shtrikman, S},
doi = {10.1016/0022-5096(62)90005-4},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/Strukturmechanik MMS/Literatur/Hashin Shtrikman 1962.pdf:pdf},
issn = {00225096},
journal = {J. Mech. Phys. Solids},
number = {4},
pages = {343--352},
title = {{A variational approach to the theory of the elastic behaviour of polycrystals}},
url = {http://linkinghub.elsevier.com/retrieve/pii/0022509662900054},
volume = {10},
year = {1962}
}
@article{Walgraef1985a,
abstract = {The nucleation of persistent slip bands (PSBs) in stressed metals may be interpreted as a cooperative phenomenon for dislocation populations. The competition between their mobility and nonlinear interaction (creation, annihilation, pinning) induces an instability of uniform dislocation distributions vs inhomogeneous ones and leads to the formation and persistence of spatial patterns. In particular, we have shown in preceding publications that the nucleation and coexistence of the layered structure of PSBs and the rodlike structure of the surrounding matrix can be described by a system of coupled partial differential equations of the reaction-diffusion type for immobile and mobile dislocations. Here we consider explicitly the motion and interaction of positive and negative mobile dislocations and derive an expression for their effective diffusivity. Moreover we show how these effects together with secondary slip activity may trigger the formation of walls in different directions in analogy with observations of labyrinth structures. ?? 1986.},
author = {Walgraef, Daniel and Aifantis, Elias C},
doi = {10.1063/1.336183},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/1985{\_}WalgraefAndAifantis{\_}Dislocation patterning in fatigued metals as a result of dynamical instabilities.pdf:pdf},
issn = {00218979},
journal = {J. Appl. Phys.},
number = {2},
pages = {688--691},
title = {{Dislocation patterning in fatigued metals as a result of dynamical instabilities}},
volume = {58},
year = {1985}
}
@article{Depcik2002d,
abstract = {In this paper, the available correlations proposed in the literature for the gas-side heat transfer in the intake and exhaust system of a spark-ignition internal combustion engine were surveyed. It was noticed that theseAB - {\{}{\textless}{\}}inline-graphic xlink:href="2002-01-0372{\{}{\_}{\}}fig0001" xmlns:xlink="http://www.w3.org/1999/xlink"/{\{}{\textgreater}{\}}AB - only by empirically fitted constants. This similarity provided the impetus for the authors to explore if a universal correlation could be developed. Based on a scaling approach using microscales of turbulence, the authors have fixed the exponential factor on the Reynolds number and thus reduced the number of adjustable coefficients to just one; the latter can be determined from a least squares curve-fit of available experimental data. Using intake and exhaust side data, it was shown that the universal correlationAB - {\{}{\textless}{\}}inline-graphic xlink:href="2002-01-0372{\{}{\_}{\}}fig0002" xmlns:xlink="http://www.w3.org/1999/xlink"/{\{}{\textgreater}{\}}AB - The correlation coefficient of this proposed heat transfer model with all available experimental data is 0.845 for the intake side and 0.800 for the exhaust side.ER -},
author = {Depcik, Christopher and Assanis, Dennis},
doi = {10.4271/2002-01-0372},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2002{\_}Assanis{\_}A Universal Heat Transfer Correlation for Intake and Exhaust flows in an SI INternal Combustion Engine.pdf:pdf},
journal = {SAE Pap.},
number = {January 2016},
title = {{A Universal Heat Transfer Correlation for Intake and Exhaust Flows in an Spark-Ignition Internal Combustion Engine}},
url = {http://papers.sae.org/2002-01-0372},
volume = {2002-01-03},
year = {2002}
}
@article{Chan2010a,
abstract = {Fatigue failure in the high-cycle and ultrahigh-cycle regimes is often dominated by the crack initiation processes, which are strongly influenced by the salient features and defects in the microstructure. Competing fatigue mechanisms involving crack initiation at persistent slipbands, grain boundaries, pores, and non-metallic inclusions or particles, have been reported to occur at surface sites in the high-cycle fatigue regime (106-107 cycles), but shift to interior sites in the ultrahigh-cycle fatigue regime (109-1010 cycles). The changes in fatigue mechanism and crack initiation site result in large variations in fatigue life. This overview article examines the roles of microstructural features such as grain size, texture, porosity, non-metallic inclusion in the fatigue crack initiation process and the manners by which these microstructural effects affect the shape of the stress-life curves. ?? 2010 Elsevier Ltd. All rights reserved.},
author = {Chan, Kwai S},
doi = {10.1016/j.ijfatigue.2009.10.005},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2010{\_}Chan{\_}Roles of microstructure in fatigue crack initiation.pdf:pdf},
isbn = {01421123},
issn = {01421123},
journal = {Int. J. Fatigue},
keywords = {Crack initiation,Double fatigue limits,Fatigue mechanism,High-cycle fatigue,Microstructure,Ultrahigh-cycle fatigue},
number = {9},
pages = {1428--1447},
publisher = {Elsevier Ltd},
title = {{Roles of microstructure in fatigue crack initiation}},
url = {http://dx.doi.org/10.1016/j.ijfatigue.2009.10.005},
volume = {32},
year = {2010}
}
@article{Christiaens,
author = {Christiaens, Dirk},
pages = {731--740},
title = {{B11 B11 {\{}{\"{U}}{\}}berschlagunf{\{}{\"{a}}{\}}lle Pkw kollidiert mit einem Gel{\{}{\"{a}}{\}}ndewagen B11}}
}
@article{Papula2011f,
author = {Papula, Lothar},
doi = {10.1007/978-3-8348-8285-1},
isbn = {9783834882851},
journal = {Math. f{\"{u}}r Ingenieure und Naturwissenschaftler Band 1},
pages = {422--569},
title = {{V Integralrechnung 1}},
year = {2011}
}
@article{Vielfalt,
author = {Vielfalt, Diese},
title = {{und Impedanzen}}
}
@article{Habenicht2012b,
author = {Habenicht, Gerd},
isbn = {9783834802958},
title = {{Aus dem Programm Fertigungstechnik}},
year = {2012}
}
@article{Nicoletto1989,
author = {Nicoletto, G},
keywords = {alumi-,cyclic plastic zone,effective stress intensity factor,fatigue crack growth,moir6 interferometry,monotonic plastic zone,nium alloy,overload,range,steels},
number = {2},
pages = {107--115},
title = {{P l a s t i c z o n e s a b o u t f a t i g u e c r a c k s in metals}},
volume = {2},
year = {1989}
}
@article{Whitaker1998,
author = {Whitaker, Ann F. and Finckenor, Miria M. and Dursch, Harry W. and Tennyson, R. C. and Young, Philip R.},
doi = {10.1007/978-1-4615-6389-1_37},
isbn = {978-0-412-54020-2},
journal = {Handb. Compos.},
pages = {810--821},
title = {{Environmental Effects on Composites}},
url = {http://link.springer.com/10.1007/978-1-4615-6389-1{\_}37},
year = {1998}
}
@article{Zahoransky2007,
author = {Zahoransky, Richard A},
isbn = {9783834804884},
pages = {337--346},
title = {{Energietechnik}},
url = {d:{\%}7B{\$}{\%}7D{\%}7B{\%}25{\%}7D5C{\%}7B{\$}{\%}7D00{\%}7B{\%}25{\%}7D7B{\%}7B{\_}{\%}7D{\%}7B{\%}25{\%}7D7DDATA{\%}7B{\$}{\%}7D{\%}7B{\%}25{\%}7D5C{\%}7B{\$}{\%}7D90{\%}7B{\%}25{\%}7D5CnLiteratur{\%}7B{\$}{\%}7D{\%}7B{\%}25{\%}7D5C{\%}7B{\$}{\%}7D30{\%}7B{\%}25{\%}7D5CnDateien{\%}7B{\$}{\%}7D{\%}7B{\%}25{\%}7D5C{\%}7B{\$}{\%}7D(Zahoransky-2007)Kyoto-Protokoll.pdf{\%}7B{\%}25{\%}7D5Cnhttp://www.springerlink.co},
volume = {3},
year = {2007}
}
@article{Buque2001a,
abstract = {The influence of the plastic strain amplitude (??pa) and the crystallographic grain orientation on the occurrence of the ladder-like dislocation substructure characteristic of persistent slip bands (PSBs) was studied by scanning electron microscopy (SEM) on individual grains of cycled nickel polycrystals. The ladder substructures were found to occur in the range of plastic strain amplitudes of 1??10-4?????pa???1??10-3 on grains having considerable different axial orientations. Studies of the slip activity show that all ladder dislocation patterns are correlated with the well-known PSBs. Apart from projection effects, the ladder-like dislocation configuration of PSBs remains unchanged for all grain orientations. The effect of crystallographic orientation concerns only the matrix surrounding the PSBs which is determined by the axial grain orientation. An increase of ??pa results in a reduction of the mean PSB wall spacing and in higher effective PSB volume fractions. The mean shear plastic strain amplitude of primary PSBs in polycrystals is estimated to be about 2??10-3. ?? 2001 Elsevier Science Ltd.},
author = {Buque, C.},
doi = {10.1016/S0142-1123(01)00013-5},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2001{\_}Buque{\_}Persistent slip bands in cyclically deformed nickel polycrystals.pdf:pdf},
issn = {01421123},
journal = {Int. J. Fatigue},
keywords = {Dislocation structure,Grain orientation,Low cycle fatigue,Nickel polycrystals,Persistent slip bands},
number = {6},
pages = {459--466},
title = {{Persistent slip bands in cyclically deformed nickel polycrystals}},
volume = {23},
year = {2001}
}
@article{Systeme,
author = {Systeme, Mechatronische},
journal = {Mechanik},
pages = {21--50},
title = {{3 Modellbildung mechatronischer Systeme}}
}
@article{Sources1995,
author = {Sources, A Neutron},
title = {{Appendix : European Sources of Neutrons and X-ray Synchrotron Radiation and their Main}},
year = {1995}
}
@article{Kunzli1999,
author = {K{\"{u}}nzli, Benjamin},
isbn = {3928034804},
journal = {Soziol. Aufkl{\"{a}}rung der Erziehungswissenschaften?},
pages = {11--20 T4  -- Anmerkungen zur Rezeption und Themenfi},
title = {{2. Einleitung}},
year = {1999}
}
@article{Wang2014,
author = {Wang, Cong and Shang, De Guang and Wang, Xiao Wei},
doi = {10.1007/s11665-014-1335-7},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Empirical Fatigue Models + Validation/2014{\_}Wang{\_}7075-T651 Models and validation.pdf:pdf},
isbn = {1059-9495},
issn = {15441024},
journal = {J. Mater. Eng. Perform.},
keywords = {critical plane,high-cycle fatigue,life prediction,maximum shear stress (MSS),multsiaxial fatigue},
number = {2},
pages = {816--824},
title = {{A New Multiaxial High-Cycle Fatigue Criterion Based on the Critical Plane for Ductile and Brittle Materials}},
volume = {24},
year = {2014}
}
@article{Koutiri2013,
abstract = {This article is dedicated to the high cycle fatigue behaviour of cast hypo-eutectic Al–Si alloys and in particular the AlSi7Cu05Mg03 alloy. In a vast experimental campaign undertaken to investigate the fatigue damage mechanisms operating in this alloy, subject to complex loading conditions, it was shown that two different coexisting fatigue damage mechanisms occur in this materials, depending on the presence of different microstructural heterogeneities (i.e. micro-shrinkage pores, Si particles, Fe-rich intermetallic phases, DAS of the Al-matrix, etc.). In order to take into account both of these damage mechanisms, a probabilistic approach using the weakest link concept is introduced to model the competition between the two mechanisms. This approach leads naturally to a probabilistic Kitagawa type diagram, which explains the relationship between the fatigue behaviour of the material and the different casting processes or post-treatments (e.g. gravity casting and HIP). It is shown that the sensitivity to the different loading modes (i.e. uniaxial with and without mean stress, torsion and equibiaxial tension) depends on the microstructural heterogeneities responsible for crack initiation. For a porosity-free alloy, the predictions are very good for combined tension–torsion loading modes. When pores are present and control the fatigue strength, the predictions are very satisfactory for the uniaxial loads with different R-ratios and slightly conservative for multiaxial loads (i.e. torsion and equibiaxial tension). Never-the-less, they are much better than the predictions of the Dang Van criterion [1].},
author = {Koutiri, I and Bellett, D and Morel, F and Pessard, E},
doi = {10.1016/j.ijfatigue.2012.08.004},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Probabilistic Aspects/xxxx{\_}Koutiri{\_}A probabilistic model for the high cycle fatigue behaviour of cast aluminium alloys subject to complex loads.pdf:pdf},
issn = {01421123},
journal = {Int. J. Fatigue},
keywords = {AlSi7Cu05Mg03-T7,Fatigue damage mechanisms,High cycle fatigue,Multiaxial loads,Probabilistic model},
pages = {137--147},
title = {{A probabilistic model for the high cycle fatigue behaviour of cast aluminium alloys subject to complex loads}},
url = {http://www.sciencedirect.com/science/article/pii/S0142112312002472},
volume = {47},
year = {2013}
}
@book{Gross2011e,
author = {Gross, Dietmar and Seelig, Thomas},
doi = {10.1007/978-3-642-10196-0},
isbn = {978-3-642-10195-3},
title = {{Bruchmechanik}},
url = {http://link.springer.com/10.1007/978-3-642-10196-0},
year = {2011}
}
@article{Strc,
author = {Str, Sammelbezeichnung and Energie, Fluid and Wirkungsweise, Die and Bei, Arbeit and Merkmal, Dieses and Beispiel, Am and Fluid, Das and Laufrad, Im and Energie, Laufrad and Leitschaufeln, Die},
pages = {1--41},
title = {{1 Gemeinsame Grundlagen der Str{\{}{\"{o}}{\}}mungsmaschinen}}
}
@article{Schneider2016a,
abstract = {{\textcopyright} 2016 Elsevier B.V.Modeling of crack propagation in materials has long been a challenge in solid-state physics and materials science. The phase-field method has now established as one of the tools for the description of crack propagation. The applied models are thermodynamically consistent and predict crack propagation in homogeneous materials under the consideration of different loading types, multiple physical fields and geometrical nonlinearities. Even dynamic loading processes are studied, including plastic effects. A multiphase-field model for crack propagation, which is indispensable to describe crack propagation on a mesoscopic length scale, is still missing. In this work, we overcome this deficiency and combine a crack propagation approach, which is based on Griffith's theory, with an established multiphase-field model for phase transformation.},
author = {Schneider, D. and Schoof, E. and Huang, Y. and Selzer, M. and Nestler, B.},
doi = {10.1016/j.cma.2016.04.009},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Thermodynamik/PhasenFeld/Schneider{\_}Crack{\_}propagation{\_}multiphase{\_}systems-Dez2015.pdf:pdf},
issn = {00457825},
journal = {Comput. Methods Appl. Mech. Eng.},
keywords = {crack propagation,multiphase-field,phase-field,polycrystalline material},
title = {{Phase-field modeling of crack propagation in multiphase systems}},
url = {http://dx.doi.org/10.1016/j.cma.2016.04.009},
year = {2016}
}
@article{Roters2000a,
abstract = {A new work-hardening model for homogeneous and heterogeneous cell-forming alloys is introduced. It distinguishes three internal state variables in terms of three categories of dislocations: mobile dislocations, immobile dislocations in the cell interiors and immobile dislocations in the cell walls. For each dislocation population an evolution law is derived taking into account dislocation generation, annihilation and storage by dipole and lock formation. In particular, these rate equations take into account the number of active glide systems and, thus, introduce texture in the model in addition to the Taylor factor. Microstructure is represented by the dislocation cell structure as well as second-phase particles, which may undergo changes by precipitation and Ostwald ripening. Interaction of mobile dislocations with the microstructure is taken into account through an effective slip length of the mobile dislocations. For the same set of parameters, the predictions are in excellent agreement with measured stress–strain curves of both a precipitation-hardened aluminium alloy (Al–4.16 wt{\%} Cu–1.37 wt{\%} Mg, AlCuMg2) and a precipitation-free model alloy (Al–0.35 wt{\%} Cu–0.25 wt{\%} Mg), the composition of which corresponds to the matrix of the two-phase alloy. Ein neues Verfestigungsmodell f{\"{u}}r homogene und heterogene Legierungen wird vorgestellt. Es werden drei innere Zustandsvariablen in Form von drei Versetzungsklassen unterschieden, mobile Versetzungen, immobile Versetzungen im Zellinnern und immobile Versetzungen in den Zellw{\"{a}}nden der Substruktur. F{\"{u}}r die Dichte jeder dieser Versetzungsklassen wird eine Evolutionsgleichung hergeleitet, die Versetzungsproduktion, -annihilation und -speicherung durch Bildung von Dipolen und se{\ss}haften Versetzungsreaktionsprodukten ber{\"{u}}cksichtigt. Insbesondere wird dabei die Zahl der aktiven Gleitsysteme ber{\"{u}}cksichtigt, wodurch die Textur zus{\"{a}}tzlich zum Taylorfaktor in das Modell einflie{\ss}t. Die Mikrostruktur wird durch die Versetzungszellstruktur und Sekund{\"{a}}rphasen repr{\"{a}}sentiert, wobei letztere Ausscheidungs- und Reifungsprozessen unterworfen sind. Die Wechselwirkung der mobilen Versetzungen mit der Mikrostruktur wird durch eine effektive freie Wegl{\"{a}}nge der mobilen Versetzungen ber{\"{u}}cksichtigt. Die Modellvorhersagen stimmen bei gleichem Parametersatz sehr gut mit gemessenen Spannungs-Dehnungs-Kurven einer ausscheidungsh{\"{a}}rtbaren Aluminiumlegierung (Al–4.16 wt{\%} Cu–1.37 wt{\%} Mg, AlCuMg2) und einer ausscheidungsfreien Modellegierung (Al–0.35 wt{\%} Cu–0.25 wt{\%} Mg), die der Matrix des zweiphasigen Werkstoffs entspricht, {\"{u}}berein.},
author = {Roters, F. and Raabe, D. and Gottstein, G.},
doi = {10.1016/S1359-6454(00)00289-5},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/Hardening Recovery Creep/2000{\_}GOTTSTEIN{\_}Work hardening in heterogeneous alloys - a microstructural approach based on three internal state variables.pdf:pdf},
isbn = {1359-6454},
issn = {13596454},
journal = {Acta Mater.},
keywords = {Alloys,Dislocations,Dislocations-theory,Mechanical properties,aluminium,mobility,plastic},
number = {17},
pages = {4181--4189},
title = {{Work hardening in heterogeneous alloys—a microstructural approach based on three internal state variables}},
url = {http://www.sciencedirect.com/science/article/pii/S1359645400002895},
volume = {48},
year = {2000}
}
@article{Universit2001,
author = {Universit, Technischen},
title = {{Technische Universit{\{}{\"{a}}{\}}t M{\{}{\"{u}}{\}}nchen Institut f{\{}{\"{u}}{\}}r Werkstoffe und Verarbeitung Forschungsgruppe Prof . Schmitt-Thomas Werkstoffgerechte Auslegung und Festigkeitsnachweis f{\{}{\"{u}}{\}}r Verbrennungsmotorkolben aus Mesophasenkohlenstoff}},
year = {2001}
}
@article{Zienkiewicz1971,
author = {Zienkiewicz, O C},
title = {{Method : Its Basis and Fundamentals UNESCO Professor of Numerical Methods in Engineering}},
year = {1971}
}
@article{Seyedi,
author = {Seyedi, M and Desmorat, R},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/2 scale models papers/Seyedi+Desmorat+Sermage{\_}A TWO SCALE DAMAGE MODEL FOR THERMOMECHANICAL HIGH CYCLE FATIQUE FAILURE.pdf:pdf},
title = {{Two Scale Damage Model for Thermomechanical High Cycle Fatigue Failure}}
}
@article{Gross2011b,
author = {Gross, Dietmar and Seelig, Thomas},
doi = {10.1007/978-3-642-10196-0},
isbn = {978-3-642-10195-3},
title = {{Bruchmechanik}},
url = {http://link.springer.com/10.1007/978-3-642-10196-0},
year = {2011}
}
@article{Fr,
author = {Fr, Beim and Tiefe, Die and Beobachtung, Diese and Nach, U A},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Surface effects + Frequency effects/Erm{\"{u}}dungsversuche gefr{\"{a}}ster Bauteile.pdf:pdf},
title = {{Ergebnisse der Untersuchungen bearbeiteter Werkst{\"{u}}cke}}
}
@article{Gruyter1996,
author = {Gruyter, Walter De and Cliffs, Englewwood},
number = {1974},
pages = {348--378},
title = {{12 Einf u ¨ hrung in die Gasdynamik}},
volume = {1},
year = {1996}
}
@article{Vick,
author = {Vick, Prof Ralf},
title = {{11 Modellierung und Bewertung von St{\{}{\"{o}}{\}}rfestigkeitsnachweisen}}
}
@article{Stromkreis,
author = {Stromkreis, Der},
pages = {4--26},
title = {{2 Gleichstromtechnik}}
}
@article{Universit2001,
author = {Universit, Technischen},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Kolben FEM/Kolbenberechnung{\_}FEM{\_}TemperaturWaermeuebergang.pdf:pdf},
title = {{Technische Universit{\"{a}}t M{\"{u}}nchen Institut f{\"{u}}r Werkstoffe und Verarbeitung Forschungsgruppe Prof . Schmitt-Thomas Werkstoffgerechte Auslegung und Festigkeitsnachweis f{\"{u}}r Verbrennungsmotorkolben aus Mesophasenkohlenstoff}},
year = {2001}
}
@article{Schorn2006,
author = {Schorn, Matthias},
journal = {Fahrdynamik-Regelung},
pages = {27--46},
title = {{Modelle zur Beschreibung des Fahrverhaltens}},
year = {2006}
}
@article{Santner1976,
author = {Santner, J S and Fine, M E},
doi = {10.1007/BF02643972},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/1976{\_}Morris+Buck{\_}Fatigue crack propagation in AL-base copper alloys.pdf:pdf},
issn = {03602133},
journal = {Met. Trans. A},
number = {3},
pages = {583--593},
title = {{Fatigue crack propagation in aluminum-base copper alloys}},
volume = {7},
year = {1976}
}
@article{Energieb,
author = {Energie, Thermische and Energie, Mechanische and Energie, Elektrische},
title = {{2 Einf{\"{u}}hrung in die Funktionsweise von Verbren- nungsmotoren}}
}
@article{Reifenbeurteilung,
author = {Reifenbeurteilung, Die},
title = {{11 Reifenbeurteilung}}
}
@article{Anteil2008,
author = {Anteil, Der},
doi = {10.1007/978-3-642-14470-7},
isbn = {9783540688877},
pages = {431--439},
title = {{Kapitel 12}},
year = {2008}
}
@article{Energiea,
author = {Energie, Thermische and Energie, Mechanische and Energie, Elektrische},
title = {{Der Hubkolbenmotor}}
}
@article{Forest2009b,
abstract = {A unifying thermomechanical framework is presented that reconciles several classes of gradient elastoviscoplasticity and damage models proposed in the literature during the last 40 years. It is based on the introduction of the micromorphic counterpart ϕ $\chi$ of a selected ... $\backslash$n},
author = {Forest, Samuel},
doi = {10.1061/(ASCE)0733-9399(2009)135:3(117)},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Plasticity models/2009{\_}Forest{\_}Micromorphic Approach for Gradient Elasticity Viscoplasticity and Damage.pdf:pdf},
isbn = {0733-9399},
issn = {0733-9399},
journal = {J. Eng. Mech.},
number = {3},
pages = {117--131},
title = {{Micromorphic Approach for Gradient Elasticity, Viscoplasticity, and Damage}},
volume = {135},
year = {2009}
}
@article{Teilchen,
author = {Teilchen, Elementar- and Proton, Name and Elektron, Neutron and Masse, Relative and Kugel, Atomkern and Verh, Das},
journal = {Elektron},
pages = {63--92},
title = {{Atombau und Periodensystem 3.1}}
}
@article{Sturz-,
author = {Sturz-, Die},
title = {{7 Kurvenfahrt 7.1}}
}
@article{Weertman1956a,
abstract = {Polycrystalline samples of high purity aluminium have been tested in a strain rate machine over a wide temperature range. The relationship which exists between the maximum stress, strain rate, and temperature is strain rate = A (stress)4.4exp( — QRT) where A is a constant, R is the gas constant, T is the absolute temperature, Q is an activation energy equal to 36,000 cal/mole. The results are compared with those of Servi and Grant on constant stress creep tests and shown to be almost identical.},
author = {Weertman, J.},
doi = {10.1016/0022-5096(56)90031-X},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Kriechen{\_}Spannungsrelaxation/1956{\_}Weertman{\_}Creep of polycrystalline aluminium as determined from strain rate tests.pdf:pdf},
isbn = {0022-5096},
issn = {00225096},
journal = {J. Mech. Phys. Solids},
number = {4},
pages = {230--234},
title = {{Creep of polycrystalline aluminium as determined from strain rate tests}},
url = {http://www.sciencedirect.com/science/article/pii/002250965690031X},
volume = {4},
year = {1956}
}
@article{Mindlin,
author = {Mindlin, Reissner-},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Zienkiewicz FEM - Vol 2 Solid Structural Mechanics/63212{\_}12.pdf:pdf},
title = {{'Thick' Reissner-Mindlin plates- irreducible and mixed formulations ': ',}},
volume = {0}
}
@article{Chemicals2005,
author = {Chemicals, Thermoset},
number = {May},
title = {{Resin Transfer Molding}},
year = {2005}
}
@article{Whitaker1998,
author = {Whitaker, Ann F. and Finckenor, Miria M. and Dursch, Harry W. and Tennyson, R. C. and Young, Philip R.},
doi = {10.1007/978-1-4615-6389-1_37},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/{\_}buecherSong/HandbookofComposites/IV/36{\_}EnvironmentalEffectsonComposites.pdf:pdf},
isbn = {978-0-412-54020-2},
journal = {Handb. Compos.},
pages = {810--821},
title = {{Environmental Effects on Composites}},
url = {http://link.springer.com/10.1007/978-1-4615-6389-1{\_}37},
year = {1998}
}
@article{Zurek1983,
abstract = {The influence of alloy grain size on growth rates of surface cracks 20 to 500 $\mu$m in length was studied in Al 7075-T6 specimens prepared in 12 and 130 $\mu$n grain sizes. Grain boundaries temporarily interrupt the propagation of cracks shorter than several grain diameters in length. Linear elastic fracture mechanics is inadequate to describe resulting average growth rates which must instead be characterized as a function of cyclic stress amplitude, $\sigma$a, and alloy grain size as well as stress intensity range, $\sigma$K. These observations are rationalized using two models, one that relates crack closure stress to alloy grain size, and a second that relates the development of microplasticity in a new grain in the crack path to grain size. In addition, growth rates were found to be faster in fully reversed loading than in tension-tension loading, especially in the large grained material. Evidence is presented to demonstrate that this is a consequence of the fatigue induced development of a compressive residual surface stress during tension-tension loading. These complex effects, and the role of grain size in determining short crack growth, are discussed.},
author = {Zurek, A. K. and James, M. R. and Morris, W. L.},
doi = {10.1007/BF02654397},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/1983{\_}Morris{\_}The effect of grain size on fatigue growth of short cracks.pdf:pdf},
isbn = {03602133},
issn = {03602133},
journal = {Metall. Trans. A},
number = {8},
pages = {1697--1705},
title = {{The Effect of Grain Size on Fatigue Growth of Short Cracks}},
volume = {14},
year = {1983}
}
@inproceedings{BargendeAdditional2011,
address = {Graz},
author = {Bargende, Michael and Heinle, Moritz and Berner, Hans-J{\"{u}}rgen},
booktitle = {13th Symp. Work. Process Intern. Combust. Engine},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Heat Transfer Combustion Chamber/2011{\_}Heinle{\_}Einige Ergaenzung zur Berechnung der Wandwaermeverluste in der Prozessrechnung.pdf:pdf},
pages = {45--63},
title = {{Einige Erg{\"{a}}nzungen zur Berechnung der Wandw{\"{a}}rmeverluste in der Prozessrechnung}},
year = {2011}
}
@article{Wasserenergie,
author = {Wasserenergie, Nutzbare},
doi = {10.1007/978-3-8348-2279-6},
isbn = {9783834822796},
pages = {215--235},
title = {{11 Wasserkraftwerke}}
}
@article{Zienkiewicz2013,
abstract = {Abstract This chapter describes discrete systems and their mathematical representation by what we define as a standard discrete system. The system is defined by components we call elements which are joined together at discrete points we call nodes. Today, discrete problems can generally be solved using computers even if the number of elements is very large. Systems which are continuous are often defined using differential equations or equivalent statements which imply an infinite number of elements. Engineering solutions to continuous problems can be attained using discretization methods. This volume presents a view of the finite element method as a general discretization procedure of continuous systems. Finite element analyses follow a standard pattern which is universally adaptable to all discrete systems. The goal of this volume is to show how finite element methods lead to a standard discrete system. This chapter is primarily concerned with establishing the processes applicable to such systems.},
author = {Zienkiewicz, O.C. and Taylor, R.L. and Zhu, J.Z.},
doi = {10.1016/B978-1-85617-633-0.00001-0},
isbn = {978-1-85617-633-0},
issn = {00295981},
journal = {Finite Elem. Method its Basis Fundam.},
pages = {1--20},
pmid = {21333062},
title = {{The Standard Discrete System and Origins of the Finite Element Method}},
url = {http://linkinghub.elsevier.com/retrieve/pii/B9781856176330000010},
year = {2013}
}
@article{Differt1986,
abstract = {A mdoel of the evolution of the surface roughness of persistent slip bands (PSBs) is presented. The physical background of the model is the existence of a dynamic equilibrium between dislocation multiplication and annihilation in PSBs which leads to irreversible microscopic positive and negative slip steps at the surface. The fluctuation of a random distribution of these slip line segments leads to a surface roughness which increases with the square root of the cycle number. The relation between the parameters which characterize the surface relief and the microscopic parameters which contol the dislocation glide in PSBs is investigated by computer simulations. Fair agreement is obtained between observed and simulated surface reliefs where such a comparison is possible.},
author = {Differt, K and Esmann, U and Mughrabi, H},
doi = {10.1080/01418618608242897},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2016{\_}Mughrabi{\_}A model of extrusions and intrusions in fatigued metals II  Surface roughening by random irreversible slip.pdf:pdf},
isbn = {0141-8610},
issn = {0141-8610},
journal = {Philos. Mag. A},
number = {2},
pages = {237--258},
title = {{A model of extrusions and intrusions in fatigued metals II. Surface roughening by random irreversible slip}},
url = {http://www.tandfonline.com/doi/abs/10.1080/01418618608242897},
volume = {54},
year = {1986}
}
@article{Kratzsch2013c,
author = {Kratzsch, Matthias and G{\"{u}}nther, Michael},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Klopfen{\_}Ottomotor/4. Internationale Tagung Ottomotorisches Klopfen - Berlin 12{\_}2013/Knocking+in+Gasoline+Engines.pdf:pdf},
pages = {445},
title = {{Knocking in Gasoline Engines}},
year = {2013}
}
@article{Pizzonia2016,
author = {Pizzonia, Francesco and Castiglione, Teresa and Bova, Sergio},
doi = {10.1016/j.apenergy.2016.02.063},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Thermal Coating + Water Heat Transfer + Applikation/2016{\_}Pizzonia{\_}A Robust Model Predictive Control for efficient thermal management of ICE.pdf:pdf},
journal = {Appl. Energy},
pages = {555--566},
publisher = {Elsevier Ltd},
title = {{A Robust Model Predictive Control for efficient thermal management of internal combustion engines}},
volume = {169},
year = {2016}
}
@book{Kloninger2012,
abstract = {Das Tool MECHANICA ist eine bekannte und verbreitete Software von Para-metric Technology Corporation (PTC). Heutzutage benutzt man die Funktionalit{\"{a}}t {\"{u}}berwiegend in Verbindung mit Pro/ENGINEER, einem der weltweit f{\"{u}}hrenden CAD-Programme (CAD = Computer Aided Design). Das war nicht immer so, da MECHANICA urspr{\"{u}}nglich unabh{\"{a}}ngig von Pro/ENGINEER entwickelt und sp{\"{a}}-ter in die CAD-Umgebung integriert wurde. Dennoch gibt es noch immer einige Spezialisten, die MECHANICA losgel{\"{o}}st von CAD einsetzen. Diese Arbeitsweise geh{\"{o}}rt keineswegs zum Schwerpunkt der Abhandlung, denn die Zielgruppe ent-spricht nicht dem Buchkonzept.},
author = {Kloninger, Paul},
doi = {10.1007/978-3-642-24841-2},
isbn = {9783540890171},
keywords = {Computer Aided Design,Computer science,Engineering,Engineering design,Mechanical engineering},
pages = {255},
title = {{Pro/MECHANICA{\textregistered} verstehen lernen}},
url = {http://www.springerlink.com/content/t64q367388614t74/},
year = {2012}
}
@article{Xiaoming2004,
author = {Xiaoming, Ye and Guohua, Chen and Yankun, Jiang and Yunchuan, Zou},
doi = {10.4271/2004-01-0778},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2004{\_}Xiaoming{\_}Numerical Investigation of the EHL performance and friction heat transfer in pistopn and cylinder liner system.pdf:pdf},
isbn = {0768013194},
number = {724},
title = {{Numerical Investigation of the EHL Performance and Friction Heat Transfer in Piston and Cylinder Liner System}},
year = {2004}
}
@article{Papula2011a,
author = {Papula, Lothar},
doi = {10.1007/978-3-8348-8285-1},
isbn = {9783834882851},
journal = {Math. f{\{}{\"{u}}{\}}r Ingenieure und Naturwissenschaftler Band 1},
pages = {422--569},
title = {{V Integralrechnung 1}},
year = {2011}
}
@book{Qu2007,
abstract = {The complete primer to micromechanics{\$}\backslash{\$}n{\$}\backslash{\$}n{\$}\backslash{\$}nFundamentals of Micromechanics of Solids is the first book integrating various approaches in micromechanics into a unified mathematical framework, complete with coverage of both linear and nonlinear behaviors. Based on this unified framework, results from the authors' own research, as well as existing results in the literature are re-derived in a logical, pedagogical, and understandable approach. It enables readers to follow the various developments of micromechanics theories and quickly understand its wide range of applications of micromechanics.{\$}\backslash{\$}n{\$}\backslash{\$}nThis helpful guide is a powerful tool for learning the most fundamental ideas and approaches, basic concepts, principles, and methodologies of micromechanics. Readers will find:{\$}\backslash{\$}n* Vigorous derivations of the mathematical framework{\$}\backslash{\$}n* Introductions to both linear and nonlinear material behavior{\$}\backslash{\$}n* Unique coverage of brittle damage, shape memory alloys, and TRIP steels{\$}\backslash{\$}n* Large numbers of problems and exercises to support teaching and learning the concepts{\$}\backslash{\$}n* Lists of references and suggested readings in each chapter},
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Qu, Jianmin and Cherkaoui, Mohammed},
booktitle = {Fundam. Micromechanics Solids},
doi = {10.1002/9780470117835},
eprint = {arXiv:1011.1669v3},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/Strukturmechanik MMS/Literatur/Mikromechanik{\_}B{\"{u}}cher{\_}Literaturvorschlag{\_}MMS/Qu 2006 Micromechanics.pdf:pdf},
isbn = {0471464511},
issn = {16137736},
pages = {1--386},
pmid = {21972053},
title = {{Fundamentals of Micromechanics of Solidss}},
year = {2007}
}
@article{Chang2004c,
abstract = {An experimental study has been carried out to provide qualitative and quantitative insight into gas to wall heat transfer in a gasoline fueled Homogeneous Charge Compression Ignition (HCCI) engine. Fast response thermocouples are embedded in the piston top and cylinder head surface to measure instantaneous wall temperature and heat flux. Heat flux measurements obtained at multiple locations show small spatial variations, thus confirming relative uniformity of incylinder conditions in a HCCI engine operating with premixed charge. Consequently, the spatially-averaged heat flux represents well the global heat transfer from the gas to the combustion chamber walls in the premixed HCCI engine, as confirmed through the gross heat release analysis. Heat flux measurements were used for assessing several existing heat transfer correlations. One of the most popular models, the Woschni expression, was shown to be inadequate for the HCCI engine. The problem is traced back to the flame propagation term which is not appropriate for the HCCI combustion. Subsequently, a modified model is proposed which significantly improves the prediction of heat transfer in a gasoline HCCI engine and shows very good agreement over a range of conditions},
author = {Chang, Junseok and G{\"{u}}ralp, Orgun and Filipi, Zoran and Assanis, Dennis N. and Kuo, Tang-Wei and Najt, Paul and Rask, Rod},
doi = {10.4271/2004-01-2996},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2004{\_}Chang{\_}New Heat Transfer Correlation for an HCCI Engine Derived from Measurements of Instantaneous Surface Heat Flux.pdf:pdf},
isbn = {0148-7191},
issn = {0148-7191},
number = {724},
title = {{New Heat Transfer Correlation for an HCCI Engine Derived from Measurements of Instantaneous Surface Heat Flux}},
url = {http://papers.sae.org/2004-01-2996/},
year = {2004}
}
@article{Baehr1956,
author = {Baehr, H D},
doi = {10.1007/978-3-642-24161-1},
isbn = {9783642241611},
journal = {Thermodyn. Baehr},
pages = {605--626},
title = {{10 Mengenma{\{}{\ss}{\}}e, Einheiten, Stoffdaten}},
year = {1956}
}
@article{Rojas2016a,
abstract = {? 2016 by the authors; licensee MDPI, Basel, Switzerland.The viscoelastic response of pure Al and 7075 (AlZnMg) and 2024 (AlCuMg) alloys, obtained with a dynamic-mechanical analyzer (DMA), is studied. The purpose is to identify relationships between the viscoelasticity and fatigue response of these materials, of great interest for structural applications, in view of their mutual dependence on intrinsic microstructural effects associated with internal friction. The objective is to investigate the influence of dynamic loading frequency and temperature on fatigue, based on their effect on the viscoelastic behavior. This research suggests that the decrease of yield and fatigue behavior reported for Al alloys as temperature increases may be associated with the increase of internal friction. Furthermore, materials subjected to dynamic loading below a given threshold frequency exhibit a static-like response, such that creep mechanisms dominate and fatigue effects are negligible. In this work, an alternative procedure to the time-consuming fatigue tests is proposed to estimate this threshold frequency, based on the frequency dependence of the initial decrease of the storage modulus with temperature, obtained from the relatively short DMA tests. This allows for a fast estimation of the threshold frequency. The frequencies obtained for pure Al and 2024 and 7075 alloys are 0.001-0.005, 0.006 and 0.075-0.350 Hz, respectively.},
author = {Rojas, J I and Crespo, D},
doi = {10.3390/met6030050},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Surface effects + Frequency effects/Frequency effect regarding EModulus and fatigue of some aluminium alloys .pdf:pdf},
issn = {20754701},
journal = {Met. (Basel).},
keywords = {AlZnMg,Aluminum alloys,Dynamic-mechanic,[AlCuMg},
number = {3},
pages = {1--13},
title = {{Onset frequency of fatigue effects in pure aluminum and 7075 (AlznMg) and 2024 (AlCuMg) alloys}},
volume = {6},
year = {2016}
}
@article{Fitton1992,
author = {Fitton, J. C. and Nates, R. J.},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Klopfen{\_}Ottomotor/1992{\_}Fitton{\_}and{\_}Nates{\_}Investigation into the relationship between knock intensity and piston seizure.pdf:pdf},
journal = {N{\&}O J.},
title = {{Investigation into the relationship between knock intensity and piston Seizure}},
year = {1992}
}
@article{Opitz1959,
author = {Opitz, Herwart},
doi = {10.1007/978-3-663-05002-5_6},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Empirical Fatigue Models + Validation/Betriebsfestigkeit{\_}ErwinHaibach/Backmatter.pdf:pdf},
isbn = {978-3-663-03813-9},
pages = {33--33},
title = {{Verwendete Formelzeichen}},
year = {1959}
}
@article{G,
author = {G, Lutering and Williams, J C},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2010{\_}Jaroslav Pokluda+Pavel {\v{S}}andera{\_}Micromechanisms of fracture and fatigue{\_}Buch/Front.pdf:pdf},
isbn = {9781848825062},
journal = {New York},
title = {{Engineering Materials and Processes}}
}
@article{Nutzen,
author = {Nutzen, Hoher},
pages = {335--348},
title = {{13 Ausblick}}
}
@article{Bouaziz2012a,
abstract = {The current work extends the well established approach of Kocks and Mecking by a more realistic description of strain-hardening using an original dislocation density law with a revisited physical understanding of dynamic recovery, without new material parameters and keeping only one internal variable. The current work extends the well established approach of Kocks and Mecking by a more realistic description of strain-hardening using an original dislocation density law with a revisited physical understanding of dynamic recovery, without new material parameters and keeping only one internal variable. First validation shows that the new approach is more consistent with experiments than the common Kocks-Mecking modeling with the same number of parameters. Copyright {\{}{\textcopyright}{\}} 2012 WILEY-VCH Verlag GmbH {\{}{\&}{\}} Co. KGaA, Weinheim.},
author = {Bouaziz, O},
doi = {10.1002/adem.201200083},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/Hardening Recovery Creep/2012{\_}BouazizRevisited Storage and Dynamic Recovery of Dislocation Density Evolution Law- Toward a Generalized Kocks–Mecking Model of Strain-Hardening.pdf:pdf},
issn = {14381656},
journal = {Adv. Eng. Mater.},
number = {9},
pages = {759--761},
title = {{Revisited storage and dynamic recovery of dislocation density evolution law: Toward a generalized kocks-mecking model of strain-hardening}},
volume = {14},
year = {2012}
}
@article{Spektrum,
author = {Spektrum, Das and Vordergrund, Im and En, D I N and Heran-, Unter},
journal = {Matrix},
title = {{5 Kriterien f{\"{u}}r die Werkstoffauswahl}}
}
@article{Le2016,
abstract = {A continuum model of dislocation pileups that takes the self-energy of dislocations into account is proposed. An analytical solution describing the distribution of dislocations in equilibrium is found from the energy minimization. Based on this solution we show (i) the existence of a critical threshold stress for the equilibrium of dislocations within a double pileup, and (ii) the existence of a non-linear regime in which the number of dislocations in a double pileup does not scale linearly with the resolved external shear stress, contrary to the classical double pileup model.},
archivePrefix = {arXiv},
arxivId = {1506.03572},
author = {Le, Khanh Chau},
doi = {10.1016/j.ijengsci.2015.11.008},
eprint = {1506.03572},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/2015{\_}Le{\_}Self-energy of dislocations and dislocation pileups.pdf:pdf},
issn = {00207225},
journal = {Int. J. Eng. Sci.},
keywords = {Dislocation nucleation,Dislocations,Self-energy,Yield stress},
pages = {1--7},
title = {{Self-energy of dislocations and dislocation pileups}},
volume = {100},
year = {2016}
}
@article{Energien,
author = {Energien, Systeme},
journal = {Transport},
pages = {8--31},
title = {{2 Die Systeme und ihre Beschreibung}}
}
@article{Procedure,
author = {Procedure, Accounting and Mass, Air and Gemisch, Ammoniak-wasser and Industrie, Deutschen},
title = {{Sachwortverzeichnis}}
}
@article{Horstemeyer1999a,
abstract = {A phenomenological void–crack nucleation model for ductile metals with secondphases is described which is motivated from fracture mechanics and microscale physicalobservations. The void–crack nucleation model is a function of the fracture toughness of theaggregate material, length scale parameter (taken to be the average size of the second phaseparticles in the examples shown in this writing) , the volume fraction of the second phase, strainlevel, and stress state. These parameters are varied to explore their effects upon the nucleationand damage rates. Examples of correlating the void–crack nucleation model to tension data in theliterature illustrate the utility of the model for several ductile metals. Furthermore, compression,tension, and torsion experiments on a cast Al–Si–Mg alloy were conducted to determinevoid–crack nucleation rates under different loading conditions. The nucleation model was thencorrelated to the cast Al–Si–Mg data as well.},
author = {Horstemeyer, Mark F. and Gokhale, Arun M.},
doi = {10.1016/S0020-7683(98)00239-X},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Plasticity models/A void crack nucleation model for ductile metals with or without inclusions{\_}HorstemeyerAndGokhale.pdf:pdf},
isbn = {00207683 (ISSN)},
issn = {00207683},
journal = {Int. J. Solids Struct.},
pages = {5029--5055},
pmid = {111},
title = {{A Void-Crack Nucleation Model for Ductile Metals}},
volume = {36},
year = {1999}
}
@article{Triebwerks,
author = {Triebwerks, Eigenschaften},
title = {{G des Triebwerks}}
}
@book{HuseyinSehitoglu2000,
author = {{Huseyin Sehitoglu} and {Hans J. Maier}},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/2000{\_}Huseyin Sehitoglu{\_}Thermo-mechanical Fatigue Behavior of  Materials{\_}OverviewDifferentPapers.pdf:pdf},
isbn = {0803128533},
pages = {151},
title = {{Thermo-mechanical Fatigue Behavior of Materials: Third volume}},
url = {https://books.google.se/books?id=ZY84rIMG82sC{\&}pg=PA150{\&}lpg=PA150{\&}dq=thermomechanical+fatigue+behavior+of+materials{\&}source=bl{\&}ots=93h1yoyJVR{\&}sig=YTp4LbQdi6Kms-Ys06yBsW5LnPU{\&}hl=sv{\&}sa=X{\&}ved=0ahUKEwidx4jg27rKAhVGqHIKHfYeBXoQ6AEIMjAC{\#}v=onepage{\&}q{\&}f=false},
year = {2000}
}
@article{Ausf,
author = {Ausf, Die and Bewertung, Die and Reihenfolge, Die and Schaltkomfort, Der and Abschnitt, Mit},
title = {{Komfortaspekte}}
}
@article{Papula2009d,
author = {Papula, Lothar},
journal = {Math. Formelsammlung},
title = {{Fourier-Transformationen}},
year = {2009}
}
@book{Elshahawy2008,
author = {Elshahawy, Waleed},
isbn = {0120020211},
title = {{Advances i}},
year = {2008}
}
@article{Castillo2009a,
author = {Castillo, E},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Probabilistic Aspects/A Unified Statistical Methodology for Modeling Fatigue Damage{\_}Castillo/Kap1{\_}Presentation of the Book. An Integrated Overview of the Fatigue Problem.pdf:pdf},
journal = {Stress Int. J. Biol. Stress},
title = {{Presentation of the Book . An Integrated Overview of}},
year = {2009}
}
@article{Fahrzeugsystemen1987,
author = {Fahrzeugsystemen, Der Ausfall Von},
journal = {Praxis (Bern. 1994).},
title = {{8 Sicherheit und Zuverl{\"{a}}ssigkeit}},
year = {1987}
}
@article{Fischer2016,
author = {Fischer, Carl and Schweizer, Christoph and Seifert, Thomas},
doi = {10.1016/j.ijfatigue.2016.03.011},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/2016{\_}Seifert+Schweizer{\_}A crack opening stress equation for in phase and out of phase thermomechanical fatigue loading.pdf:pdf},
issn = {01421123},
journal = {Int. J. Fatigue},
keywords = {fatigue crack closure,thermomechanical fatigue},
pages = {178--184},
publisher = {Elsevier Ltd},
title = {{A crack opening stress equation for in-phase and out-of-phase thermomechanical fatigue loading}},
url = {http://linkinghub.elsevier.com/retrieve/pii/S0142112316300160},
volume = {88},
year = {2016}
}
@article{Baehr1956,
author = {Baehr, H.D.},
doi = {10.1007/978-3-642-24161-1},
isbn = {9783642241611},
journal = {Thermodyn. Baehr},
pages = {605--626},
title = {{10 Mengenma{\ss}e, Einheiten, Stoffdaten}},
year = {1956}
}
@article{Zienkiewicz2005d,
abstract = {Publisher Summary Plates and shells are a particular form of three-dimensional solid, the treatment of which presents no theoretical difficulties in the case of elasticity. The thickness of such structures is very small when compared with other dimensions. Their complete three-dimensional numerical treatment is costly and often leads to serious numerical ill-conditioning problems. To ease the solution, even long before numerical approaches became possible, several classical assumptions regarding the behavior of such structures were introduced. Such assumptions result in a series of approximations. Therefore, numerical treatment concerns itself with the approximation to an already approximate theory, the validity of which is restricted. The shape functions for rectangular elements are the simplest to form for thin plates. The thick-plate theory is simpler to implement in the finite element method; however, in the early days of analytical treatment, it presented more difficulties. This chapter discusses non-conforming shape functions. The solution with conforming shape functions give bounds to the energy of the correct solution; however, on many occasions, yields inferior accuracy to that achieved with non-conforming elements. },
author = {Zienkiewicz, O C and Taylor, R L and Zhu, J Z},
doi = {http://dx.doi.org/10.1016/B978-075066431-8.50198-3},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Zienkiewicz FEM - Vol 2 Solid Structural Mechanics/63212{\_}11.pdf:pdf},
isbn = {978-0-7506-6431-8},
journal = {Finite Elem. Method Set (Sixth Ed.},
pages = {323--381},
title = {{11 - Plate bending approximation: Thin (Kirchhoff) plates and {\{}C1{\}} continuity requirements}},
url = {http://www.sciencedirect.com/science/article/pii/B9780750664318501983},
year = {2005}
}
@article{Cherkaoui2009a,
author = {Cherkaoui, Mohammed and Capolungo, Laurent},
doi = {10.1007/978-0-387-46771-9},
isbn = {978-0-387-46765-8},
title = {{Atomistic and Continuum Modeling of Nanocrystalline Materials}},
url = {http://link.springer.com/10.1007/978-0-387-46771-9},
volume = {112},
year = {2009}
}
@article{Weertman1955a,
abstract = {A theory of steady-state creep is developed using Mott's mechanism of dislocation climb. It is assumed in the analysis that the rate-controlling process is the diffusion of vacancies between dislocations which are creating vacancies and those which are destroying them. The concentration of vacancies along a dislocation line is determined by setting the change in the free energy caused by a decrease or increase in the number of vacancies equal to the change in the elastic energy occuring during dislocation climb. The creep equation that results from the analysis is creep rate=const (o-{\{}{\textless}{\}}Y./kT)exp(-Q/kT) where" is a constant ("",3 to 4), Q is the activation energy of self-diffusion, kT has its usual meaning, and 0- to 108 is the stress. This equation is valid in the stress range from the critical shear stress to a stress about equal to 10' dynes/cm'. At larger stresses the creep rate increases much more rapidly with stress.},
author = {Weertman, J},
doi = {10.1063/1.1721875},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Kriechen{\_}Spannungsrelaxation/1955{\_}Weertman{\_}Theory of Steady-State Creep Based on Dislocation Climb.pdf:pdf},
isbn = {0021-8979},
issn = {00218979},
journal = {J. Appl. Phys.},
number = {10},
pages = {1213--1217},
title = {{Theory of steady-state creep based on dislocation climb}},
volume = {26},
year = {1955}
}
@book{Qu2007,
abstract = {The complete primer to micromechanics$\backslash$n$\backslash$n$\backslash$nFundamentals of Micromechanics of Solids is the first book integrating various approaches in micromechanics into a unified mathematical framework, complete with coverage of both linear and nonlinear behaviors. Based on this unified framework, results from the authors' own research, as well as existing results in the literature are re-derived in a logical, pedagogical, and understandable approach. It enables readers to follow the various developments of micromechanics theories and quickly understand its wide range of applications of micromechanics.$\backslash$n$\backslash$nThis helpful guide is a powerful tool for learning the most fundamental ideas and approaches, basic concepts, principles, and methodologies of micromechanics. Readers will find:$\backslash$n* Vigorous derivations of the mathematical framework$\backslash$n* Introductions to both linear and nonlinear material behavior$\backslash$n* Unique coverage of brittle damage, shape memory alloys, and TRIP steels$\backslash$n* Large numbers of problems and exercises to support teaching and learning the concepts$\backslash$n* Lists of references and suggested readings in each chapter},
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Qu, Jianmin and Cherkaoui, Mohammed},
booktitle = {Fundam. Micromechanics Solids},
doi = {10.1002/9780470117835},
eprint = {arXiv:1011.1669v3},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/Strukturmechanik MMS/Literatur/Mikromechanik{\_}B{\"{u}}cher{\_}Literaturvorschlag{\_}MMS/Qu 2006 Micromechanics.pdf:pdf},
isbn = {0471464511},
issn = {16137736},
pages = {1--386},
pmid = {21972053},
title = {{Fundamentals of Micromechanics of Solidss}},
year = {2007}
}
@article{LuWang2016,
author = {Lu, Pengyu and Gao, Qing and Wang, Yan},
doi = {10.1016/j.applthermaleng.2016.05.047},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Thermal Coating + Water Heat Transfer + Applikation/2016{\_}Wang{\_}The simulation methods based on 1D-3D collaborative computing for the vehicle integrated thermal management.pdf:pdf},
journal = {Appl. Therm. Eng.},
pages = {42--53},
publisher = {Elsevier Ltd},
title = {{The simulation methods based on 1D-3D collaborative computing for the vehicle integrated thermal management}},
volume = {104},
year = {2016}
}
@book{Voyiadjis2021,
author = {Voyiadjis, George Z},
doi = {10.1007/978-1-4614-8968-9},
isbn = {978-1-4614-8968-9},
title = {{Handbook of Damage Mechanics}},
url = {http://link.springer.com/10.1007/978-1-4614-8968-9},
year = {2021}
}
@article{Anfanga,
author = {Anfang, Am},
journal = {Chart},
pages = {93--116},
title = {{5 Anwendungsorientierte {\{}{\"{U}}{\}}bersicht kommerzieller}}
}
@article{Zienkiewicz2013a,
abstract = {This chapter describes the use of a patch of one or more elements to assess convergence of a finite element solution to that of the differential equation it approximates. The requirements are presented by a consistency and stability test on the resulting matrix problem. For elements which are numerically integrated or otherwise explicitly stated the stability test requires that the stiffness matrix of a structural problem or the conductivity matrix of a quasi-harmonic problem has proper rank. This requires the number of quadrature points to be equal or larger to some minimum value. Use of less than the minimum number is called reduced integration. Consistency requires the finite element solution to exactly represent all the derivatives up to the highest order that exists in a weak or variational expression for the problem. The chapter presents alternative methods to asses the two requirements. The patch test is an essential test to both test accuracy of the computer program used to solve problems as well as to validate formulations that violate the standard rules described in previous chapters. One such case of a non-conforming element is presented in the chapter.},
author = {Zienkiewicz, O.C. and Taylor, R.L. and Zhu, J.Z.},
doi = {10.1016/B978-1-85617-633-0.00008-3},
isbn = {9781856176330},
issn = {00295981},
journal = {Finite Elem. Method its Basis Fundam.},
pages = {257--284},
title = {{The Patch Test, Reduced Integration, and Nonconforming Elements}},
url = {http://linkinghub.elsevier.com/retrieve/pii/B9781856176330000083},
year = {2013}
}
@article{Bohlke2011,
author = {B{\"{o}}hlke, Thomas},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Vorlesungen/MMF{\_}Skript.pdf:pdf},
journal = {Mechanik},
keywords = {skript},
title = {{Skript zur Vorlesung Mathematische Methoden der Festigkeitslehre}},
year = {2011}
}
@article{Buck,
author = {Buck, H and Leyh, J and Ohlhausen, P and Richter, M and Spath, D and Warschat, J},
journal = {H{\"{u}}tte},
pages = {1--41},
title = {{N-Management}}
}
@article{Teilaufgabenb,
author = {Teilaufgaben, Abzuhandelnde},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Empirical Fatigue Models + Validation/Betriebsfestigkeit{\_}ErwinHaibach/Kap4 Praktische Umsetzung des Betriebsfestigkeits-Konzepts.pdf:pdf},
title = {{des Betriebsfestigkeits-Konzeptes}}
}
@phdthesis{Koch2002_Diss,
author = {Koch, Thomas},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Injection+Combustion+Ignitionsystems/2002{\_}Koch{\_}Thomas{\_}Numerischer Beitrag zur Charakterisierung und Vorausberchnung der Gemischbildung und Verbrennung in einenem DI Ottomotor.pdf:pdf},
school = {ETH Z{\"{u}}rich},
title = {{Numerischer Beitrag zur Charakterisierung und Vorausberechnung der Gemischbildung und Verbrennung in einem direkteingespritzten, strahlgef{\"{u}}hrten Ottomotor}},
year = {2002}
}
@article{Vierpoltheorie,
author = {Vierpoltheorie, Grundlegende Zusammenh{\"{a}}nge Der},
pages = {180--200},
title = {{10 Vierpoltheorie 10.1}},
volume = {1}
}
@article{Groma2016,
author = {Groma, Istv??n and Zaiser, Michael and Isp??novity, P??ter Dus??n},
doi = {10.1103/PhysRevB.93.214110},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2016{\_}Groma{\_}Dislocation patterning in a two-dimensional continuum theory of dislocations.pdf:pdf},
issn = {1550235X},
journal = {Phys. Rev. B - Condens. Matter Mater. Phys.},
number = {21},
pages = {1--10},
title = {{Dislocation patterning in a two-dimensional continuum theory of dislocations}},
volume = {93},
year = {2016}
}
@article{Gu2002a,
author = {Gu, Minyi and Die, Lynda and Frank, R C and Mark, I D},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2012{\_}Trijselaar{\_}KNOCK PREDICTION IN GAS FIRED RECIPROCATING ENGINES.pdf:pdf},
pages = {8--15},
title = {{A N ew Vec t or f or H i gh - Throughpu t , L i ga t i on - I ndependen t C l on i ng E ncod i ng a Tobacco E t ch V i rus Pro t e ase C l e avage S i t e}},
volume = {15},
year = {2002}
}
@article{WangGaoZhang2016,
author = {Wang, Guohua and Gao, Qing and Zhang, Tianshi and Wang, Yan},
doi = {10.1016/j.advengsoft.2016.06.010},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Thermal Coating + Water Heat Transfer + Applikation/2016{\_}Wang{\_}A simulation approach of under-hood thermal management.pdf:pdf},
journal = {Adv. Eng. Softw.},
keywords = {1D/3D,Integrated simulation,Multip,Under-hood,VTMS},
pages = {43--52},
publisher = {Elsevier Ltd},
title = {{A simulation approach of under-hood thermal management}},
volume = {100},
year = {2016}
}
@article{Desmorat2006,
abstract = {Application of damage mechanics to fatigue is addressed in the present paper. The ability of Lemaitre's damage law to describe low and high cycle fatigue failure of metals is illustrated. Its generalization into an evolution law modeling a damage rate governed by the main dissipative mechanics applies to concrete, elastomers, rocks and to probably other materials. The importance of rate written laws is emphasized.},
author = {Desmorat, Rodrigue},
doi = {10.1080/17747120.2006.9692859},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/2006{\_}Desmorat{\_}SummerSchool{\_}Damage and Fatigue Overview Evolution Equation.pdf:pdf},
isbn = {9780387739052},
issn = {1774-7120},
journal = {Rev. Eur. G{\'{e}}nie Civ.},
keywords = {concrete,damage,elastomers,fatigue,metals,rocks},
number = {6-7},
pages = {849--877},
title = {{Damage and Fatigue: Continuum damage mechanics modeling for fatigue of materials and structures}},
volume = {10},
year = {2006}
}
@article{Zienkiewicz2014f,
author = {Zienkiewicz, O.C. and Taylor, R.L. and Nithiarasu, P.},
doi = {10.1016/B978-1-85617-635-4.00007-8},
isbn = {9781856176354},
journal = {Finite Elem. Method Fluid Dyn.},
pages = {225--281},
title = {{Compressible High-Speed Gas Flow}},
url = {http://linkinghub.elsevier.com/retrieve/pii/B9781856176354000078},
year = {2014}
}
@article{Pokluda2010,
author = {Pokluda, Jaroslav and Andera, Pavel},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2010{\_}Jaroslav Pokluda+Pavel {\v{S}}andera{\_}Micromechanisms of fracture and fatigue{\_}Buch/Kap3{\_}BrittleAndDuctileFracture.pdf:pdf},
journal = {Micromechanisms Fract. Fatigue},
pages = {69--123},
title = {{Brittle and Ductile Fracture}},
year = {2010}
}
@article{Papula2011d,
author = {Papula, L},
doi = {10.1007/978-3-8348-8133-5},
isbn = {9783834881335},
title = {{III Grundlagen der mathematischen Statistik 1}},
year = {2011}
}
@article{Bestimmung,
author = {Bestimmung, Die},
title = {{3. Geschwindigkeitsmessung}}
}
@article{Endo2007,
abstract = {A modified linear-elastic fracture mechanics approach has been proposed and developed by McEvily and co-workers, with which the fatigue crack growth rates of both small cracks and large cracks can be quantitatively evaluated. This paper reviews the recent results of applications of this approach to the following fatigue problems involving the prediction of the behavior of small fatigue cracks: (1) in an examination of the use of Miner's rule in fatigue life estimation under variable amplitude loading, (2) in the verification of the sqrt(a r e a) parameter model, and (3) in the prediction of the fatigue life and strength of defect-containing components subjected to multiaxial stress. ?? 2006 Elsevier B.V. All rights reserved.},
author = {Endo, M and McEvily, A J},
doi = {10.1016/j.msea.2006.09.084},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/2007{\_}Endo+McEvily{\_}Prediction of the behavior of small fatigue cracks.pdf:pdf},
issn = {09215093},
journal = {Mater. Sci. Eng. A},
keywords = {Crack closure,Elastic-plastic behavior,Fatigue crack growth,Fatigue lifetime estimate,Fatigue thresholds,Multiaxial stress},
number = {SPEC. ISS.},
pages = {51--58},
title = {{Prediction of the behavior of small fatigue cracks}},
volume = {468-470},
year = {2007}
}
@article{Loubar2005a,
abstract = {This paper deals with the transient thermal signal around an engine cylinder in order to propose a new and nonintrusive method of knock detection. Numerical simulations of unsteady heat transfer through the cylinder and inside the coolant flow are carried out to account for heat flux variations due to normal and knocking combustion. The effect of rib roughened surfaces on thermal signal amplification is investigated. The geometric parameters are fixed at Pi/h=70 and w/h=1 with a Reynolds number based on hydraulic diameter of 12,000. The results reveal that square ribs give better performance in term of thermal signal amplification within the fluid. An amplification of the temperature variation up to 20 times higher is found. Finally, flow analysis shows that amplification depends on the position where the thermal signal is collected.},
author = {Loubar, Khaled and Bellettre, Jérôme and Tazerout, Mohand},
doi = {10.1115/1.1857943},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2005{\_}Loubar{\_}Unsteady Heat Transfer enhancement around an engine cylinder in order to detect knockpdf.pdf:pdf},
isbn = {0022-1481},
issn = {00221481},
journal = {J. Heat Transfer},
number = {3},
pages = {278},
title = {{Unsteady Heat Transfer Enhancement Around an Engine Cylinder in Order to Detect Knock}},
url = {http://heattransfer.asmedigitalcollection.asme.org/article.aspx?articleid=1447711},
volume = {127},
year = {2005}
}
@book{Bazant1992a,
abstract = {Elasticity, plasticity, damage mechanics and cracking are all phenomena that determine the resistance of solids to deformation and fracture. The authors of this book discuss a modern method of mathematically modeling the behavior of macroscopic volume elements. The first three chapters review physical mechanisms at the microstructural level, thermodynamics of irreversible processes, mechanics of continuous media, and the classification of the behavior of solids. The rest of the book is devoted to the modeling of different types of material behavior. In each case the authors present characteristic data for numerous materials, and discuss the physics underlying the phenomena together with methods for the numerical analysis of the resulting equations.},
author = {Ba{\v{z}}ant, Z. P.},
booktitle = {Can. J. Civ. Eng.},
doi = {10.1139/l92-025},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Kriechen{\_}Spannungsrelaxation/1985{\_}Jean{\_}Lemaitre+Jean-Louis+Chaboche{\_}Mechanics{\_}of{\_}Solid{\_}Materials.pdf:pdf},
isbn = {0521477581},
issn = {0315-1468},
number = {1},
pages = {197--197},
title = {{Mechanics of solid materials}},
url = {http://www.nrcresearchpress.com/doi/abs/10.1139/l92-025},
volume = {19},
year = {1992}
}
@article{Arnold,
author = {Arnold, J{\"{o}}rg},
pages = {793--800},
title = {{C6 C6 Gl{\{}{\"{u}}{\}}hlampen C6 Untersuchungen von Gl{\{}{\"{u}}{\}}hlampen}}
}
@article{Wallentowitz2006,
author = {Wallentowitz, Henning and Reif, Konrad},
doi = {10.1007/978-3-8348-9121-1_1},
isbn = {978-3-528-03971-4},
journal = {Handb. Kraftfahrzeugelektronik - Grundlagen, Kompon. Syst. Anwendungen},
pages = {1--4},
title = {{Einleitung}},
url = {http://www.springerlink.com/index/10.1007/978-3-8348-9121-1{\%}7B{\_}{\%}7D1},
year = {2006}
}
@article{Bohlke2001,
author = {B{\"{o}}hlke, Thomas and Br{\"{u}}ggemann, C},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/Strukturmechanik MMS/Literatur/Graphical Representation of the Generalized Hooke's Law{\_}SingleCrystals{\_}B{\"{o}}hlke{\_}Kommentar.pdf:pdf},
journal = {Techn,sche Mech.},
number = {2},
pages = {145--158},
title = {{Graphical Representation of the Generalized Hooke's Law}},
volume = {21},
year = {2001}
}
@book{Gross2011j,
author = {Gross, Dietmar and Seelig, Thomas},
doi = {10.1007/978-3-642-10196-0},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Gross, Selig 2011 - Bruchmechanik/Gross, Seelig - 2011 - BruchmechanikKap1.pdf:pdf},
isbn = {978-3-642-10195-3},
title = {{Bruchmechanik}},
url = {http://link.springer.com/10.1007/978-3-642-10196-0},
year = {2011}
}
@article{Element2002,
abstract = {Three Botrytis-susceptible mutants bos2, bos3, and bos4 which define independent and novel genetic loci required for Arabidopsis resistance to Botrytis cinerea were isolated. The bos2 mutant is susceptible to B. cinerea but retains wild-type levels of resistance to other pathogens tested, indicative of a defect in a response pathway more specific to B. cinerea. The bos3 and bos4 mutants also show increased susceptibility to Alternaria brassicicola, another necrotrophic pathogen, suggesting a broader role for these loci in resistance. bos4 shows the broadest range of effects on resistance, being more susceptible to avirulent strain of Pseudomonas syringae pv. tomato. Interestingly, bos3 is more resistant than wild-type plants to virulent strains of the biotrophic pathogen Peronospora parasitica and the bacterial pathogen P. syringae pv. tomato. The Pathogenesis Related gene 1 (PR-1), a molecular marker of the salicylic acid (SA)-dependent resistance pathway, shows a wild-type pattern of expression in bos2, while in bos3 this gene was expressed at elevated levels, both constitutively and in response to pathogen challenge. In bos4 plants, PR-1 expression was reduced compared with wild type in response to B. cinerea and SA. In bos3, the mutant most susceptible to B. cinerea and with the highest expression of PR-1, removal of SA resulted in reduced PR-1 expression but no change to the B. cinerea response. Expression of the plant defensin gene PDF1-2 was generally lower in bos mutants compared with wild-type plants, with a particularly strong reduction in bos3. Production of the phytoalexin camalexin is another well-characterized plant defense response. The bos2 and bos4 mutants accumulate reduced levels of camalexin whereas bos3 accumulates significantly higher levels of camalexin than wild-type plants in response to B. cinerea. The BOS2, BOS3, and BOS4 loci may affect camalexin levels and responsiveness to ethylene and jasmonate. The three new mutants appear to mediate disease responses through mechanisms independent of the previously described BOS1 gene. Based on the differences in the phenotypes of the bos mutants, it appears that they affect different points in defense response pathways.},
author = {Element, Finite and Program, Analysis and Fortran, Compac},
journal = {Program},
number = {1},
pages = {2--5},
title = {{Computer procedures for finite}},
url = {http://www.ncbi.nlm.nih.gov/pubmed/15500471},
volume = {1},
year = {2002}
}
@article{Tatsache,
author = {Tatsache, Ausgehend Von Der},
journal = {Messtechnik},
title = {{6 Bewertung von Messergebnissen}}
}
@article{Le2016,
abstract = {A continuum model of dislocation pileups that takes the self-energy of dislocations into account is proposed. An analytical solution describing the distribution of dislocations in equilibrium is found from the energy minimization. Based on this solution we show (i) the existence of a critical threshold stress for the equilibrium of dislocations within a double pileup, and (ii) the existence of a non-linear regime in which the number of dislocations in a double pileup does not scale linearly with the resolved external shear stress, contrary to the classical double pileup model.},
archivePrefix = {arXiv},
arxivId = {1506.03572},
author = {Le, Khanh Chau},
doi = {10.1016/j.ijengsci.2015.11.008},
eprint = {1506.03572},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/2015{\_}Le{\_}Self-energy of dislocations and dislocation pileups.pdf:pdf},
issn = {00207225},
journal = {Int. J. Eng. Sci.},
keywords = {Dislocation nucleation,Dislocations,Self-energy,Yield stress},
pages = {1--7},
title = {{Self-energy of dislocations and dislocation pileups}},
volume = {100},
year = {2016}
}
@article{Pan2014b,
abstract = {Knocking combustion in spark-ignition (SI) engines is a typical abnormal combustion phenomenon that severely limits engine performance and thermal efficiency. However, its mechanism has not so far been completely revealed, such as the origin of pressure oscillation with tremendous amplitude and broken mechanisms of the engine body when knock occurs. This article systematically reviews the series of physical and chemical phenomena involved in knocking combustion, including auto-ignition, gas-dynamic waves, cavity resonance, and auto-ignited flame propagation. Significant research has shown that the rapid heat release of end-gas auto-ignition and subsequent strong pressure waves play a crucial role during knocking combustion. A methodology of the interaction of flame propagation and pressure waves has been proposed to reveal knock formation in terms of positive feedback between strengthened pressure waves and auto-ignited flame propagation. Also, new suggestions on the weakness in prior research of knocking combustion have also been discussed in the present article. {\textcopyright} 2014 Copyright Taylor and Francis Group, LLC.},
author = {Pan, Jiaying and Shu, Gequn and Wei, Haiqiao},
doi = {10.1080/00102202.2013.857665},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2014{\_}Pan+Wei{\_}Interaction of Flame Propagation and Pressure Waves During Knocking Combustion in Spark-Ignition Engines.pdf:pdf},
issn = {0010-2202},
journal = {Combust. Sci. Technol.},
number = {2},
pages = {192--209},
title = {{Interaction of Flame Propagation and Pressure Waves During Knocking Combustion in Spark-Ignition Engines}},
url = {http://www.tandfonline.com/doi/abs/10.1080/00102202.2013.857665},
volume = {186},
year = {2014}
}
@article{Gurtsysteme1985,
author = {Gurtsysteme, A Technik Der and Kramer, Florian},
pages = {761--774},
title = {{C2 C2 Sicherheitsgurte C2}},
year = {1985}
}
@article{Stupkiewicz2007a,
author = {Stupkiewicz, Stanis{\l}aw},
doi = {10.1007/978-3-540-49717-2_4},
isbn = {3540497161},
issn = {16137736},
journal = {Lect. Notes Appl. Comput. Mech.},
number = {30},
pages = {37--57},
title = {{Boundary layers induced by micro-inhomogeneous boundary conditions}},
volume = {2006},
year = {2007}
}
@article{Meroth2008a,
abstract = {Der visuelle Kanal besitzt die h{\{}{\"{o}}{\}}chste Informationsdichte im Fahrzeug. Anzeigen im Fahrzeug liefern Informationen zum Betriebszustand des Fahrzeugs, warnen bei kritischen Zust{\{}{\"{a}}{\}}nden, informieren {\{}{\"{u}}{\}}ber den Zustand der Entertainmentkomponenten, geben empfangene Nachrichten wieder, unterst{\{}{\"{u}}{\}}tzen bei der Navigation (Abbiegehinweise, Karten) oder der Fahrzeugf{\{}{\"{u}}{\}}hrung (Abstand zu Hindernissen und zu Fahrbahnbegrenzungen) oder dienen der Unterhaltung (Videoentertainment). Entsprechend ihrer Funktion sind Anzeigen an verschiedenen Stellen im Fahrzeug verteilt und beruhen auf unterschiedlichen Technologien.},
author = {Meroth, Ansgar and Tolg, Boris},
isbn = {978-3-8348-9430-4},
journal = {Infotainmentsysteme im Kraftfahrzeug},
pages = {79--114},
title = {{Anzeigetechnik}},
url = {http://dx.doi.org/10.1007/978-3-8348-9430-4{\%}7B{\_}{\%}7D3},
year = {2008}
}
@article{Corti2009a,
abstract = {A detailed analysis of knocking events can help improving engine performance and diagnosis strategies. The paper aim is a better understanding of the phenomena involved in knocking combustions through the combination of CFD and signals analysis tools. CFD simulations have been used in order to reproduce knock effect on the in-cylinder pressure trace. In fact, the in-cylinder pressure signal holds information about waves propagation and heat losses: for the sake of the diagnosis it is important to relate knock severity to knock indexes values. For this purpose, a CFD model has been implemented, able to predict the combustion evolution with respect to Spark Advance, from non-knocking up to heavy knocking conditions. The CFD model validation phase is crucial for a correct representation of both regular and knocking combustions: the operation has been carried out by means of an accurate statistical analysis of experimental in-cylinder pressure data. The simulation results allow relating the combustion characteristics to their effect on the in-cylinder pressure signal. It is then possible to highlight critical issues regarding typical knock detection methodologies, while disclosing novel approaches. One of the main results is the validation of knock detection strategies based on the low-frequency content of the pressure signal. These strategies can be used together with standard high-frequency based techniques in order to improve the detection robustness.},
author = {Corti, Enrico and Forte, Claudio},
doi = {10.4271/2009-24-0019},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Klopfen{\_}Ottomotor/2009{\_}Forte+Corti+Bianchi{\_}Combination on In-Cylinder Pressure Signal Analysis and CFD Simulation for Knock Detection Purposes.pdf:pdf},
issn = {1946-3944},
journal = {SAE Int. J. Engines},
number = {2},
pages = {19--2009},
title = {{Combination of In-Cylinder Pressure Signal Analysis and CFD Simulation for Knock Detection Purposes}},
url = {http://papers.sae.org/2009-24-0019/},
volume = {2},
year = {2009}
}
@article{Felippa2008,
author = {Felippa, Carlos A},
doi = {10.1007/978-3-540-71001-1},
isbn = {978-3-540-71000-4},
issn = {0003-5599},
number = {August},
title = {{Nonlinear Finite Element Methods}},
url = {http://link.springer.com/10.1007/978-3-540-71001-1},
year = {2008}
}
@article{Heth1998,
author = {Heth, Jennifer A},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/{\_}buecherSong/HandbookofComposites/IV/37{\_}SafetyandHealthIssues.pdf:pdf},
title = {{Safety and health issues}},
year = {1998}
}
@article{Pro-,
author = {Pro-, Mathematischen and Search, Line},
title = {{4 Optimierungsverfahren}}
}
@article{Rhouma2011a,
author = {Rhouma, W. Ben and Deschanel, S. and Weiss, J.},
doi = {10.1063/1.3637920},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2011{\_}Weiss{\_}Collective Dislocation Dynamics and avalanches during fatigue of aluminium.pdf:pdf},
isbn = {9780735409569},
issn = {0094243X},
journal = {AIP Conf. Proc.},
keywords = {acoustic emission,damage,dislocations,fatigue,microstructure},
number = {May},
pages = {1536--1539},
title = {{Collective dislocation dynamics and avalanches during fatigue of aluminum}},
volume = {1389},
year = {2011}
}
@article{Kirchner2007,
abstract = {Vorwort{\$}\backslash{\$}r{\$}\backslash{\$}n{\$}\backslash{\$}r{\$}\backslash{\$}nEigentlich sollte man annehmen, dass nach mehr als 100 Jahren Automobilbau{\$}\backslash{\$}r{\$}\backslash{\$}n{\$}\backslash{\$}r{\$}\backslash{\$}nalles ¨uber die Leistungs¨ubertragung in Fahrzeuggetrieben in schriftlicher{\$}\backslash{\$}r{\$}\backslash{\$}n{\$}\backslash{\$}r{\$}\backslash{\$}nForm dokumentiert ist. Aber weit gefehlt: Das Fahrzeuggetriebe besch¨aftigt{\$}\backslash{\$}r{\$}\backslash{\$}n{\$}\backslash{\$}r{\$}\backslash{\$}nmehr denn je die Ingenieure in Forschung und Entwicklung, um unter dem{\$}\backslash{\$}r{\$}\backslash{\$}n{\$}\backslash{\$}r{\$}\backslash{\$}nDruck der Selbstverpflichtung der Automobilindustrie das technisch und ¨okonomisch{\$}\backslash{\$}r{\$}\backslash{\$}n{\$}\backslash{\$}r{\$}\backslash{\$}nM¨ogliche zur Senkung von Kraftstoffverbrauch und CO2-Aussto{\{}{\ss}{\}} bei{\$}\backslash{\$}r{\$}\backslash{\$}n{\$}\backslash{\$}r{\$}\backslash{\$}ngleichzeitiger Steigerung der Tragf¨ahigkeit zu leisten.{\$}\backslash{\$}r{\$}\backslash{\$}n{\$}\backslash{\$}r{\$}\backslash{\$}nDas Manuskript zu diesem Buch entsteht also mitten in einer Zeit, in der die{\$}\backslash{\$}r{\$}\backslash{\$}n{\$}\backslash{\$}r{\$}\backslash{\$}nAutomobilwirtschaft mit gro{\{}{\ss}{\}}em technischen Ehrgeiz nach neuen technischen{\$}\backslash{\$}r{\$}\backslash{\$}n{\$}\backslash{\$}r{\$}\backslash{\$}nM¨oglichkeiten zur Reduktion des Kraftstoffverbrauchs bei gleichzeitiger Beibehaltung{\$}\backslash{\$}r{\$}\backslash{\$}n{\$}\backslash{\$}r{\$}\backslash{\$}nder ¨ublichen Fahrleistungen sucht. Zeitgleich haben Kostendruck{\$}\backslash{\$}r{\$}\backslash{\$}n{\$}\backslash{\$}r{\$}\backslash{\$}nund Aufgabenteilung in der Entwicklung ein bisher noch nicht bekanntes Niveau{\$}\backslash{\$}r{\$}\backslash{\$}n{\$}\backslash{\$}r{\$}\backslash{\$}nerreicht. Hinzu kommen die Anforderungen des Kunden nach immer{\$}\backslash{\$}r{\$}\backslash{\$}n{\$}\backslash{\$}r{\$}\backslash{\$}nkomfortableren, robusten Getrieben, die ihn begeistern und nicht nur zufriedenstellen.{\$}\backslash{\$}r{\$}\backslash{\$}n{\$}\backslash{\$}r{\$}\backslash{\$}nDer Aspekt der Kundensicht und mit ihm die vielf¨altigen Fragestellungen{\$}\backslash{\$}r{\$}\backslash{\$}n{\$}\backslash{\$}r{\$}\backslash{\$}nnach komfortrelevanten Ph¨anomenen verbunden mit einem soliden ¨Uberblick{\$}\backslash{\$}r{\$}\backslash{\$}n{\$}\backslash{\$}r{\$}\backslash{\$}n¨uber konstruktive und entwicklungsmethodische Grundz¨uge der Fahrzeuggetriebe{\$}\backslash{\$}r{\$}\backslash{\$}n{\$}\backslash{\$}r{\$}\backslash{\$}nwar meine urspr¨ungliche Motivation f¨ur dieses Buch. Es entstand auf{\$}\backslash{\$}r{\$}\backslash{\$}n{\$}\backslash{\$}r{\$}\backslash{\$}nder Grundlage einer Vorlesung, die ich f¨ur Studierende des Maschinenbaus{\$}\backslash{\$}r{\$}\backslash{\$}n{\$}\backslash{\$}r{\$}\backslash{\$}nhalte; die positiven R¨uckmeldungen zum Inhalt der Vorlesung haben das Entstehen{\$}\backslash{\$}r{\$}\backslash{\$}n{\$}\backslash{\$}r{\$}\backslash{\$}ndieses Buches vorangetrieben.{\$}\backslash{\$}r{\$}\backslash{\$}n{\$}\backslash{\$}r{\$}\backslash{\$}nDie Zielgruppe dieses Buches ist somit in meinem ehemaligen T¨atigkeitsbereich{\$}\backslash{\$}r{\$}\backslash{\$}n{\$}\backslash{\$}r{\$}\backslash{\$}n? der Fahrzeug- und insbesondere in der Getriebeentwicklung ? zu suchen;{\$}\backslash{\$}r{\$}\backslash{\$}n{\$}\backslash{\$}r{\$}\backslash{\$}nes ist als Einf¨uhrungs- und Nachschlagewerk gleicherma{\{}{\ss}{\}}en konzipiert.{\$}\backslash{\$}r{\$}\backslash{\$}n{\$}\backslash{\$}r{\$}\backslash{\$}nHinzu kommen als potentielle Leser die Studierenden an den deutschsprachigen{\$}\backslash{\$}r{\$}\backslash{\$}n{\$}\backslash{\$}r{\$}\backslash{\$}ningenieurwissenschaftlichen Fakult¨aten, die sich f¨ur den Antrieb von{\$}\backslash{\$}r{\$}\backslash{\$}n{\$}\backslash{\$}r{\$}\backslash{\$}nKraftfahrzeugen interessieren. Die Ausf¨uhrungen und Auslegungsrichtlinien{\$}\backslash{\$}r{\$}\backslash{\$}n{\$}\backslash{\$}r{\$}\backslash{\$}nsind jeweils f¨ur einen Erstentwurf und dessen Dimensionierung der verschiedenen{\$}\backslash{\$}r{\$}\backslash{\$}n{\$}\backslash{\$}r{\$}\backslash{\$}nGetriebekonzepte und ihrer Komponenten umfangreich genug, f¨ur die{\$}\backslash{\$}r{\$}\backslash{\$}n{\$}\backslash{\$}r{\$}\backslash{\$}nOptimierung der Einzelteile werden viele Hinweise auf tiefergehende Quellen{\$}\backslash{\$}r{\$}\backslash{\$}n{\$}\backslash{\$}r{\$}\backslash{\$}ngegeben. Auf den Einsatz einer speziellen Software wurde ganz bewusst verzichtet,{\$}\backslash{\$}r{\$}\backslash{\$}n{\$}\backslash{\$}r{\$}\backslash{\$}nalle Auslegungsaufgaben und Beispiele sind mit dem Taschenrechner{\$}\backslash{\$}r{\$}\backslash{\$}n{\$}\backslash{\$}r{\$}\backslash{\$}noder einem einfachen Tabellenkalkulationsprogramm l¨osbar. Die ausf¨uhrlichen{\$}\backslash{\$}r{\$}\backslash{\$}n{\$}\backslash{\$}r{\$}\backslash{\$}nL¨osungen zu den enthaltenen Auslegungsfragen stelle ich gerne auf Anfrage{\$}\backslash{\$}r{\$}\backslash{\$}n{\$}\backslash{\$}r{\$}\backslash{\$}nzur Verf¨ugung.{\$}\backslash{\$}r{\$}\backslash{\$}n{\$}\backslash{\$}r{\$}\backslash{\$}nZumindest indirekt geholfen beim Entstehen haben viele ehemalige Kollegen,{\$}\backslash{\$}r{\$}\backslash{\$}n{\$}\backslash{\$}r{\$}\backslash{\$}nmit denen ich viele der hier zusammengetragenen Fakten diskutieren konnte;{\$}\backslash{\$}r{\$}\backslash{\$}n{\$}\backslash{\$}r{\$}\backslash{\$}nnamentlich genannt seien ? stellvertretend ? Georg Bednarek, Friedhelm{\$}\backslash{\$}r{\$}\backslash{\$}n{\$}\backslash{\$}r{\$}\backslash{\$}nKrake, Josef Hau und J¨org B¨onning (Alle GM Powertrain Europe) aber auch{\$}\backslash{\$}r{\$}\backslash{\$}n{\$}\backslash{\$}r{\$}\backslash{\$}nDr. Klaus Kalmbach, Dr. Peter Werth, Thomas Hackl, Ulf Polzin und Patrick{\$}\backslash{\$}r{\$}\backslash{\$}n{\$}\backslash{\$}r{\$}\backslash{\$}nVikari, alle hofer powertrain GmbH. Die letztgenannten Herren, ihre Begeisterung{\$}\backslash{\$}r{\$}\backslash{\$}n{\$}\backslash{\$}r{\$}\backslash{\$}nund ihr Wissen um die Thematik haben viele Punkte einflie{\{}{\ss}{\}}en lassen,{\$}\backslash{\$}r{\$}\backslash{\$}n{\$}\backslash{\$}r{\$}\backslash{\$}ndie hier zusammengetragen sind. Dar¨uber hinaus hat die hofer powertrain{\$}\backslash{\$}r{\$}\backslash{\$}n{\$}\backslash{\$}r{\$}\backslash{\$}nGmbH mir die Einbindung der Bilder in Farbe erm¨oglicht und stand meinen{\$}\backslash{\$}r{\$}\backslash{\$}n{\$}\backslash{\$}r{\$}\backslash{\$}nBildw¨unschen immer aufgeschlossen gegen¨uber.{\$}\backslash{\$}r{\$}\backslash{\$}n{\$}\backslash{\$}r{\$}\backslash{\$}nViele wertvolle Denkanst¨o{\{}{\ss}{\}}e zur Darstellung einzelner Fragestellungen habe{\$}\backslash{\$}r{\$}\backslash{\$}n{\$}\backslash{\$}r{\$}\backslash{\$}nich von Herrn Prof. Dr.-Ing. B. Sauer, TU Kaiserslautern erhalten; zu nennen{\$}\backslash{\$}r{\$}\backslash{\$}n{\$}\backslash{\$}r{\$}\backslash{\$}nist hier beispielsweise die explizite Auseinandersetzung mit den Wirkprinzipien{\$}\backslash{\$}r{\$}\backslash{\$}n{\$}\backslash{\$}r{\$}\backslash{\$}nmechanischer Leistungs¨ubertragung direkt in der Einleitung.{\$}\backslash{\$}r{\$}\backslash{\$}n{\$}\backslash{\$}r{\$}\backslash{\$}nWeiterhin m¨ochte ich mit bei einer Reihe von Studierenden bedanken, die im{\$}\backslash{\$}r{\$}\backslash{\$}n{\$}\backslash{\$}r{\$}\backslash{\$}nRahmen von Studien- und Diplomarbeiten Bausteine zu abgeschlossenen Themen{\$}\backslash{\$}r{\$}\backslash{\$}n{\$}\backslash{\$}r{\$}\backslash{\$}nerarbeitet und so zu diesem Buch beigetragen haben. Genannt seien hier{\$}\backslash{\$}r{\$}\backslash{\$}n{\$}\backslash{\$}r{\$}\backslash{\$}nFrau Rike Grotepass sowie die Herren Rene Johne, Hagen Plisch, Tillmann{\$}\backslash{\$}r{\$}\backslash{\$}n{\$}\backslash{\$}r{\$}\backslash{\$}nSch¨afer, Martin S¨anger, Christian Lunkenheimer, Florian Herbold, Matthias{\$}\backslash{\$}r{\$}\backslash{\$}n{\$}\backslash{\$}r{\$}\backslash{\$}nReimann und Christian Hamann. Die Herren Dr.-Ing. Andreas Laschet (Arla{\$}\backslash{\$}r{\$}\backslash{\$}n{\$}\backslash{\$}r{\$}\backslash{\$}nMaschinentechnik, K¨urten) und Dr. Jan Schlipf (GIF GmbH, Alsdorf) sowie{\$}\backslash{\$}r{\$}\backslash{\$}n{\$}\backslash{\$}r{\$}\backslash{\$}ndie Firmen GM Powertrain Europe, DaimlerChrysler, BMW, ZF Zahnradfabrik{\$}\backslash{\$}r{\$}\backslash{\$}n{\$}\backslash{\$}r{\$}\backslash{\$}nFriedrichshafen, Voith Turbo Systems, ElringKlinger, H¨orbiger Antriebstechnik,{\$}\backslash{\$}r{\$}\backslash{\$}n{\$}\backslash{\$}r{\$}\backslash{\$}nLuK, INA, Jopp, MagnaSteyr und AGCO haben mir Material zur{\$}\backslash{\$}r{\$}\backslash{\$}n{\$}\backslash{\$}r{\$}\backslash{\$}nVerf¨ugung gestellt. Ich bitte um Nachsicht, wenn ich jemanden vergessen haben{\$}\backslash{\$}r{\$}\backslash{\$}n{\$}\backslash{\$}r{\$}\backslash{\$}nsollte, der zu diesem Buch beigetragen hat.{\$}\backslash{\$}r{\$}\backslash{\$}n{\$}\backslash{\$}r{\$}\backslash{\$}nDem Springer Verlag, insbesondere Herrn Dr.-Ing. B. Gebhardt, danke ich f¨ur{\$}\backslash{\$}r{\$}\backslash{\$}n{\$}\backslash{\$}r{\$}\backslash{\$}ndie gute konstruktive Zusammenarbeit und die Unterst¨utzung bei der Wahl{\$}\backslash{\$}r{\$}\backslash{\$}n{\$}\backslash{\$}r{\$}\backslash{\$}nder Schwerpunkte dieses Buchs.{\$}\backslash{\$}r{\$}\backslash{\$}n{\$}\backslash{\$}r{\$}\backslash{\$}nEs bleibt ein riesiges Danke an meine Frau Dr. Nina Kirchner f¨ur ihre Hilfe{\$}\backslash{\$}r{\$}\backslash{\$}n{\$}\backslash{\$}r{\$}\backslash{\$}nbeim Korrekturlesen und ihre vielen Verbesserungsvorschl¨age sowie meinen{\$}\backslash{\$}r{\$}\backslash{\$}n{\$}\backslash{\$}r{\$}\backslash{\$}nKindern f¨ur ihr Verst¨andnis, wenn ich am Manuskript gearbeitet habe anstatt{\$}\backslash{\$}r{\$}\backslash{\$}n{\$}\backslash{\$}r{\$}\backslash{\$}nmit ihnen zu spielen. Mir hat es Spass gemacht, mein Wissen zum Thema Getriebe{\$}\backslash{\$}r{\$}\backslash{\$}n{\$}\backslash{\$}r{\$}\backslash{\$}nsoweit m¨oglich niederzuschreiben; ich hoffe, dass man das merkt.{\$}\backslash{\$}r{\$}\backslash{\$}n{\$}\backslash{\$}r{\$}\backslash{\$}nSaulheim bei Mainz, im Mai 2007 Eckhard Kirchner},
author = {Kirchner, Eckhard},
doi = {10.1007/978-3-540-35292-1},
isbn = {9783540352884},
journal = {Zhurnal Eksp. i Teor. Fiz.},
pages = {699},
title = {{Leistungs{\{}{\"{u}}{\}}bertragung in Fahrzeuggetrieben}},
year = {2007}
}
@article{Reaktionskinetik,
author = {Reaktionskinetik, Grundlagen Der},
title = {{3 Grundlagen der Reaktionskinetik}}
}
@article{Zienkiewicz2014e,
abstract = {This chapter is dedicated to fully describing the characteristic based split (CBS) algorithm. Both the compressible and incompressible flow problems are explained within a unified framework of the CBS algorithm. In addition to explaining various time discretization schemes within the CBS algorithm, two approaches to the split are also presented and tested. The stability properties, accuracy and many other aspects of the CBS algorithm are analysed in depth. Some examples are also provided to demonstrate the accuracy of the CBS scheme.},
author = {Zienkiewicz, O.C. and Taylor, R.L. and Nithiarasu, P.},
doi = {10.1016/B978-1-85617-635-4.00003-0},
isbn = {9781856176354},
journal = {Finite Elem. Method Fluid Dyn.},
pages = {87--125},
title = {{The Characteristic-Based Split (CBS) Algorithm: A General Procedure for Compressible and Incompressible Flow}},
url = {http://linkinghub.elsevier.com/retrieve/pii/B9781856176354000030},
year = {2014}
}
@article{Burgf,
author = {Burg, Heinz},
pages = {645--651},
title = {{B5 B5 Unf{\{}{\"{a}}{\}}lle mit Pkw B5}}
}
@article{Brecq2005,
abstract = {High frequency pressure oscillations are generated under knocking conditions within the combustion chamber of Spark Ignition engines. Although acoustic-oscillation model can give the natural frequencies of these oscillations, very few mathematical models are today available, in scientific literature, to describe the oscillation deadening effect. An analytical formulation of the deadening has been highlighted. Analytical solution has been established for future ECU implementation. Coupling this new concept and an existing high-frequency model, an achieved model of the knocking pressure high frequencies is compared to experimental data. Good behavior is obtained on a natural gas fuelled spark ignition engine.},
author = {Brecq, G. and {Le Corre}, O.},
doi = {10.4271/2005-01-1126},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2005{\_}Brecq{\_}Modeling of In-cylinder Pressure Oscillations under Knocking conditions - Intro to Pressure Envelope Curve.pdf:pdf},
isbn = {2005011126},
issn = {0148-7191},
title = {{Modeling of In-cylinder Pressure Oscillations under Knocking Conditions: Introduction to Pressure Envelope Curve}},
url = {http://papers.sae.org/2005-01-1126/},
year = {2005}
}
@inproceedings{LeFeuvre1969,
abstract = {By the use of surface thermocouples to measure instantaneous temperatures, the instantaneous heat fluxes are calculated at several positions on the cylinder head and sleeve of a direct injection diesel engine for both motored and fired operation. Existing correlations are shown to be unable to predict these data.An analysis of convective heat transfer in the engine leads to a boundary layer model which adequately correlates the data for motored operation. The extension of this motored correlation to fired operation demonstrates the need for instantaneous local gas velocity and temperature data.},
author = {LeFeuvre, T and Myers, P S and Uyehara, O A},
booktitle = {SAE Tech. Pap. 690464},
doi = {https://doi.org/10.4271/690464},
file = {:C$\backslash$:/Users/p327208/Desktop/Promotion/Literature/Motorspezifisch/Heat Transfer Combustion Chamber/1969{\_}LeFeuvre{\_}Experimental Instantaneous Heat Fluxes in a Diesel Engine and their Correlation.pdf:pdf},
publisher = {SAE International},
title = {{Experimental Instantaneous Heat Fluxes in a Diesel Engine and Their Correlation}},
year = {1969}
}
@article{Kratzsch2013a,
author = {Kratzsch, Matthias and G{\"{u}}nther, Michael},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Klopfen{\_}Ottomotor/4. Internationale Tagung Ottomotorisches Klopfen - Berlin 12{\_}2013/Knocking+in+Gasoline+Engines.pdf:pdf},
pages = {445},
title = {{Knocking in Gasoline Engines}},
year = {2013}
}
@article{Gerhard2005,
author = {Gerhard, Pahl.},
journal = {Konstr. Grundlagen erfolgreicher Produktentwicklung Methoden und Anwendung},
pages = {93--187},
title = {{3 Methoden zur Produktplanung, L{\"{o}}sungssuche und Beurteilung}},
year = {2005}
}
@article{Krank2008b,
author = {Krank, Lothar and Streit, Andreas},
doi = {10.1007/978-3-8348-9430-4},
isbn = {978-3-8348-9430-4},
journal = {Vieweg Praxiswissen},
pages = {209--266},
title = {{Infotainmentsysteme im Kraftfahrzeug}},
year = {2008}
}
@misc{Qi1999a,
author = {Qi, W and Bertram, A},
booktitle = {Int. J. Plast.},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Plasticity models/Anisotropic continuum damage modeling for single crystals at high temperatures{\_}QiAndBertram.pdf:pdf},
pages = {1197--1215},
title = {{Anisotropic continuum damage modeling for single crystals at high temperatures}},
volume = {15},
year = {1999}
}
@article{Mollenhauer2007a,
author = {Mollenhauer},
journal = {Handb. Dieselmotoren},
keywords = {ladungswechsel und aufladung},
title = {{Ladungswechsel und Aufladung}},
year = {2007}
}
@book{Riccardella1992d,
author = {Riccardella, PC and Deardorff, AF and Griesbach, TJ},
booktitle = {Adv. Fatigue Lifetime Predict. Tech.},
doi = {10.1520/STP1122-EB},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Neuer Ordner/Advances in fatigue lifetime predictive techniques Part1.pdf:pdf},
isbn = {978-0-8031-1423-4},
issn = {00660558},
keywords = {FATIGUE,MONITORING,POWER PLANTS,PRESSURE VESSELS AND PIPING,THERMAL STRESSES},
pages = {460--473},
pmid = {11439068},
title = {{Advances in Fatigue Lifetime Predictive Techniques}},
url = {https://apps.webofknowledge.com/full{\_}record.do?product=UA{\&}search{\_}mode=GeneralSearch{\&}qid=11{\&}SID=Z1UxbH6jtsqo8n9kPQr{\&}page=1{\&}doc=1},
volume = {1122},
year = {1992}
}
@article{Wissenschaftsgebiete,
author = {Wissenschaftsgebiete, Die},
journal = {Regelungstechnik},
pages = {51--60},
title = {{4 Regelung und Steuerung}}
}
@article{Modell,
author = {Modell, Diskretes and Modell, Kontinuierliches and Vorgehensweise, Von Der},
journal = {Mechanik},
pages = {1--10},
title = {{1 Einf{\"{u}}hrung}}
}
@article{Gross2011,
author = {Gross, Dietmar and Seelig, Thomas},
doi = {10.1007/978-3-642-10196-0},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Gross, Selig 2011 - Bruchmechanik/Gross, Seelig - 2011 - BruchmechanikKap10.pdf:pdf},
isbn = {978-3-642-10195-3},
title = {{Bruchmechanik}},
url = {http://link.springer.com/10.1007/978-3-642-10196-0},
year = {2011}
}
@article{Gross2011g,
author = {Gross, Dietmar and Seelig, Thomas},
doi = {10.1007/978-3-642-10196-0},
isbn = {978-3-642-10195-3},
title = {{Bruchmechanik}},
url = {http://link.springer.com/10.1007/978-3-642-10196-0},
year = {2011}
}
@article{Ausgleichsrechnung,
author = {Ausgleichsrechnung, X I Fehler- and Normalverteilung, Gausche},
journal = {Praxis (Bern. 1994).},
pages = {292--303},
title = {{XI Fehler- und Ausgleichsrechnung 1}}
}
@article{Adair1972a,
abstract = {This study first reviews, discusses, and compares existing correlations$\backslash$nfor heat transfer in reciprocating compressors and engines. Then$\backslash$nafter a discussion of the significance of obtaining accurate instantaneous$\backslash$nheat transfer data, the authors describe an experimental investigation$\backslash$nof the instantaneous heat transfer rates to the cylinder wall of$\backslash$na reciprocating refrigerating compressor. Finally, this report presents$\backslash$nan expression which correlates the time averaged data within 20{\%}.},
author = {Adair, R P and Qvale, E B and Pearson, J T},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/1972{\_}Adair{\_}Instantaneous Heat Transfer to the Cylinder Wall in Reciprocating compressors and engines.pdf:pdf},
journal = {Int. Compress. Eng. Conf.},
pages = {521--526},
title = {{Instantaneous heat transfer to cylinder wall in reciprocating compressors}},
year = {1972}
}
@article{Toleranzen,
author = {Toleranzen, Allgemeine and Projektion, Dreidimensionale and Maschinen, Elektrische},
title = {{Technische Kommunikation/Technisches Zeichnen}}
}
@article{Zienkiewicz2013a,
author = {Zienkiewicz, O.C. and Taylor, R.L. and Zhu, J.Z.},
doi = {10.1016/B978-1-85617-633-0.00014-9},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Zienkiewicz FEM - Vol 2 Solid Structural Mechanics/63212{\_}15.pdf:pdf},
isbn = {9781856176330},
issn = {00295981},
journal = {Finite Elem. Method its Basis Fundam.},
pages = {467--491},
title = {{Shells as a Special Case of Three-Dimensional Analysis}},
url = {http://linkinghub.elsevier.com/retrieve/pii/B9781856176330000149},
year = {2013}
}
@article{Zienkiewicz2014b,
abstract = {Abstract In this chapter we review the general equations for analysis of solids in which deformations remain “small” but material behavior includes effects of a nonlinear kind. We present the theory in both an indicial (or tensorial) form as well as in the matrix form commonly used in finite element developments. We also reformulate the equations of solids in a variational (Galerkin) form. The chapter also presents the notation and the methodology which we shall adopt throughout this book. The reader will note how simply the transition between forms for linear and nonlinear problems occurs. },
author = {Zienkiewicz, O.C. and Taylor, R.L. and Fox, David},
doi = {10.1016/B978-1-85617-634-7.00001-6},
isbn = {978-1-85617-634-7},
issn = {0733-9399},
journal = {Finite Elem. Method Solid Struct. Mech.},
pages = {1--20},
title = {{General Problems in Solid Mechanics and Nonlinearity}},
url = {http://linkinghub.elsevier.com/retrieve/pii/B9781856176347000016},
year = {2014}
}
@inproceedings{DentDent1977,
abstract = {Convective and radiative heat transfer measurements in a direct injection Diesel engine have been made using surface thermocouples and a pyroelectric radiation detector.Measured instantaneous local and spatially averaged convective heat fluxes agree with correlations for turbulent convection to flat surfaces, when using measured local air motion data. Two temperature zones were considered in the computation of local heat flux.Radiative heat flux measurements corroborate the findings of others, but lower flux levels are attributed to the high swirl engine used here.A proposal for computation of radiative heat flux from soot concentration shows promise.},
author = {Dent, J C and Sulaiman, S J},
booktitle = {SAE Tech. Pap.},
doi = {https://doi.org/10.4271/770407},
publisher = {SAE International},
title = {{Convective and Radiative Heat Transfer in a High Swirl Direct Injection Diesel Engine}},
year = {1977}
}
@article{Laser2006,
author = {Laser, Das Licht Der},
journal = {Gerthsen Phys.},
pages = {823--882},
title = {{15 - Laserphysik}},
year = {2006}
}
@article{Isermann1978,
author = {Isermann, Rolf},
pages = {137--168},
title = {{7 Bremsregelungen f{\"{u}}r mechatronische Bremsen}},
year = {1978}
}
@article{Rangarajan2012,
abstract = {We describe a method for discretizing planar C2-regular domains immersed in non-conforming triangulations. The method consists in constructing mappings from triangles in a background mesh to curvilinear ones that conform exactly to the immersed domain. Constructing such a map relies on a novel way of parameterizing the immersed boundary over a collection of nearby edges with its closest point projection. By interpolating the mappings to curvilinear triangles at select points, we recover isoparametric mappings for the immersed domain defined over the background mesh. Indeed, interpolating the constructed mappings just at the vertices of the background mesh yields a fast meshing algorithm that involves only perturbing a few vertices near the boundary. For the discretization of a curved domain to be robust, we have to impose restrictions on the background mesh. Conversely, these restrictions define a family of domains that can be discretized with a given background mesh. We then say that the background mesh is a universal mesh for such a family of domains. The notion of universal meshes is particularly useful in free/moving boundary problems because the same background mesh can serve as the universal mesh for the evolving domain for time intervals that are independent of the time step. Hence it facilitates a framework for finite element calculations over evolving domains while using a fixed background mesh. Furthermore, since the evolving geometry can be approximated with any desired order, numerical solutions can be computed with high-order accuracy. We demonstrate these ideas with various numerical examples.},
archivePrefix = {arXiv},
arxivId = {1201.4903},
author = {Rangarajan, Ramsharan and Lew, Adrian J},
doi = {10.1002/nme},
eprint = {1201.4903},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/2010{\_}Miehe{\_}Thermodynamically consistent phase-field models of fracture-Variational principles and multi field FE implementations.pdf:pdf},
keywords = {coupled multi-field problems,crack propagation,finite elements,fracture,gradient-type damage,incremental variational,phase-fields,principles},
number = {March},
pages = {1273--1311},
title = {{Universal Meshes: A new paradigm for computing with nonconforming triangulations}},
url = {http://arxiv.org/abs/1201.4903},
year = {2012}
}
@phdthesis{Schwiderik2013,
author = {Schwiderik, Valerij},
school = {Fakult{\"{a}}t f{\"{u}}r Technik 1 - Mechanik und Elektronik (HHN)},
title = {{Entwicklung einer Methode zur Bestimmung des Temperaturfeldes eines Verbrennungsmotors in seiner Konzeptphase}},
type = {MAster thesis},
year = {2013}
}
@article{Rothe2006,
abstract = {A general definition and an index for the assessment of different engine knock behavior have been developed. The knock onset locations have been determined by piezoresistive pressure actuators and optical fiber probes in full load engine operation mode. The thermodynamic conditions at the knock onset locations have been quantified by CFD-calculations. Therefore the local fuel concentration, mixture temperature and residual gas concentration have been considered. These calculated thermodynamic conditions were further used to calculate the necessary volume of an exothermal center for the generation of the maximal measured pressure amplitudes.},
author = {Rothe, M and Heidenreich, T and Spicher, U and Schubert, Alexander},
doi = {10.4271/2006-01-0225},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Klopfen{\_}Ottomotor/2006{\_}Rothe{\_}Knock Behavior of SI-Engines - Thermodynamic Analysis of Knock Onset Locations and Knock Intensitiespdf.pdf:pdf},
issn = {0148-7191},
title = {{Knock Behavior of SI-Engines: Thermodynamic Analysis of Knock Onset Locations and Knock Intensities}},
url = {http://papers.sae.org/2006-01-0225/},
year = {2006}
}
@article{Menter1994,
author = {Menter, F R},
doi = {https://doi.org/10.2514/3.12149},
file = {:X$\backslash$:/Proj/E/E0006/01{\_}EL{\_}Werk/Projektteam/02{\_}Antrieb/Motor{\_}TDFI/Organisation/Pr{\"{a}}sentationen/150529 Masterarbeit PeterHoelz zur AER/MasterarbeitDiverseDateien/Abgeschlossen/SST{\_}Menter.pdf:pdf},
journal = {AIAA J.},
number = {8},
pages = {1598--1605},
title = {{Two-Equation Eddy-Viscosity Turbulence Models for Engineering Applications}},
volume = {32},
year = {1994}
}
@article{Desmorat2015,
author = {Desmorat, Rodrigue and {Du Tertre}, Alban and Gaborit, Pierre},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/2 scale models papers/2015{\_}Desmorat{\_}Multiaxial Haigh Diagrams from incremental two scale damage analysis.pdf:pdf},
journal = {Aerosp. Lab J.},
number = {9},
pages = {1--15},
title = {{Multiaxial Haigh diagrams from incremental two scale damage analysis}},
volume = {en review},
year = {2015}
}
@article{Sitzbank,
author = {Sitzbank, Seitenverkleidung},
pages = {374--390},
title = {{Karosserie und Gesamtentwurf 12 Design , Aerodynamik und Karosserieauslegung}}
}
@article{Konstruktion1997,
author = {Konstruktion, Bei Der},
pages = {1--6},
title = {{1 Einf{\{}{\"{u}}{\}}hrung}},
year = {1997}
}
@article{Algebra,
author = {Algebra, I Lineare},
title = {{Anhang : Lo ¨ sungen der {\^{U}}bungsaufgaben I Lineare Algebra}}
}
@article{Foresta,
author = {Forest, Samuel},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/Folien CISM Summer School Mai2017 - Mesoscale Models/courses{\_}C1703{\_}forest{\_}Forest4-Homog.pdf:pdf},
title = {{Generalized continuum modelling of heterogeneous materials From a heterogeneous Cauchy continuum to an homogeneous equivalent micromorphic continuum}}
}
@article{Stupkiewicz2007a,
author = {Stupkiewicz, Stanis{\l}aw},
doi = {10.1007/978-3-540-49717-2_4},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Stupkievicz 2007 - Micromechanics of Contact and Interphase Layers/97165{\_}04.pdf:pdf},
isbn = {3540497161},
issn = {16137736},
journal = {Lect. Notes Appl. Comput. Mech.},
number = {30},
pages = {37--57},
title = {{Boundary layers induced by micro-inhomogeneous boundary conditions}},
volume = {2006},
year = {2007}
}
@article{Luthi2013,
abstract = {Professor Robert M. Koerner (Bob) has successfully and elegantly transitioned his research programs throughout his career. Each successive program has brought new collaborators, contacts and consumers of his developments. Past research efforts may remain unknown to those who only more recently began an association with Bob. It is interesting and insightful to develop and follow the some times convoluted path that has led to the current, well-recognized Geosynthetics Institute. In this paper, I will provide insight into what may be the missing link between Bob's research in acoustic emissions and his current program in geosythethics.},
author = {L{\"{u}}thi, Thomas},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/{\_}buecherSong/HandbookofComposites/IV/38{\_}NondestructiveEvaluationMethodsforComposites.pdf:pdf},
title = {{Non-Destructive Evaluation Methods}},
year = {2013}
}
@article{ConferenceonFatigueMechanisms:AdvancesinQuantitativeMeasurementofPhysicalDamage1983a,
author = {{Conference on Fatigue Mechanisms: Advances in Quantitative Measurement of Physical Damage}},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/1983{\_}Lankford{\_}Fatigue Mechanisms Advances in quantitative   meausrements of physical damage.pdf:pdf},
issn = {10403094},
journal = {Stp 811},
keywords = {An{\{}{\'{a}}{\}}lise quantitativa,Congresso,Dano f{\{}{\'{i}}{\}}sico,Fadiga de materiais},
pages = {496},
title = {{Fatigue mechanisms advances in quantitative measurement of physical damage {\{}{\textless}{\}}{\{}{\textless}{\}}a{\{}{\textgreater}{\}}{\{}{\textgreater}{\}} conference}},
year = {1983}
}
@article{Windes,
author = {Windes, Nachteil},
title = {{8 Windr{\{}{\"{a}}{\}}der und Propeller}}
}
@article{RajuP2011a,
abstract = {This paper presents the details of method of sample size determination to estimate the characteristic fatigue life of aluminum alloy, A356.2-T6. The characteristic fatigue life of the alloy has been estimated by assuming log normal distribution model. A step wise procedure is outlined to determine the number of specimens required at predetermined stress amplitude to estimate the fatigue life with an acceptable error at 50{\{}{\%}{\}} probability and various confidence levels, 90{\{}{\%}{\}}, 95{\{}{\%}{\}} and 99{\{}{\%}{\}}. Maximum percentage of errors has also been calculated for the above probability and confidence levels. Details of generation of S-N curve for aluminum alloy A356.2-T6 using regression analysis have been explained. From this study, the adequate sample size required for evaluating the average fatigue life of A356.2-T6 with an acceptable error at 50{\{}{\%}{\}} probability and 90{\{}{\%}{\}} confidence level using log normal distribution is established. In order to check the significance of regression equation, analysis of variance (ANOVA) is performed. Copyright 2011 Tech Science Press.},
author = {{Raju P}, R and Rajesh, S and Satyanarayana, B and Ramji, K},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Probabilistic Aspects/2011{\_}Ramamurty{\_}Statistical Analysis of Fatigue Life Data of A356.2-T6 Aluminium Alloy.pdf:pdf},
journal = {Struct. Durab. Heal. Monit.},
keywords = {aluminum alloy,fatigue life,log normal distribution,s n curve},
number = {1-2},
pages = {139--152},
title = {{Statistical analysis of fatigue life data of A356.2-T6 aluminum alloy}},
url = {http://www.scopus.com/inward/record.url?eid=2-s2.0-79957943262{\%}7B{\&}{\%}7DpartnerID=40{\%}7B{\&}{\%}7Dmd5=a5890475316795056516da22de2c7672},
volume = {7},
year = {2011}
}
@article{Torquato1997,
abstract = {The problem of determining exact expressions for the effective stiffness tensor macroscopically anisotropic, two-phase composite media of arbitrary microstructure in arbitrary space dimension d is considered. We depart from previous treatments by introducing an integral equation for the “cavity” strain field. This leads to new, exact series expansions for the effective stiffness tensor of macroscopically anisotropic, ddimensional, two-phase composite media in powers of the “elastic polarizabilities”. The nth-order tensor coefficients of these expansions are explicitly expressed as absolutely convergent integrals over products of certain tensor fields and a determinant involving n-point correlation functions that characterize the microstructure. For the special case of macroscopically isotropic media, these series expressions may be regarded as expansions that perturb about the optimal structures that realize the Hashin-Shtrikman bounds (e.g. coated-inclusion assemblages or finite-rank laminates). Similarly, for macroscopically anisotropic media, the series expressions may be regarded as expansions that perturb about optimal structures that realize Willis' bounds. For isotropic multiphase composites, we remark on the behavior of the effective moduli as the space dimension d tends to infinity.},
author = {Torquato, S.},
doi = {10.1016/S0022-5096(97)00019-7},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/Strukturmechanik MMS/Literatur/Torquato 1997.pdf:pdf},
isbn = {0022-5096},
issn = {00225096},
journal = {J. Mech. Phys. Solids},
keywords = {a,anisotropic material,b,elastic material,inhomogeneous material,microstructures},
number = {9},
pages = {1421--1448},
title = {{Effective stiffness tensor of composite media—I. Exact series expansions}},
volume = {45},
year = {1997}
}
@article{Woytowitz1999,
abstract = {Solid-particle erosion (SPE) is studied by constructing finite-element (FE) models of elastic spheres impacting normally on the surface of a kinematically hardening, elastic-plastic material. The full effects of the contact surfaces and the impact dynamics are included. An earlier phase of this study modeled multiple, coincident impacts with two-dimensional (2D) analysis, in which damage computations by strain-life, cyclic plastic work (CPW), and continuum damage mechanics (CDM) methods were shown to be roughly equivalent. Here, it is shown that a 2D model is incorrect for non-coincident impacts; a 3D FE analysis is necessary. A stochastic model of multiple impacting spheres is developed, which can describe spatial and temporal accumulation of damage. Finally, erosion rates are estimated by extrapolating the average rates of damage accumulation in the outermost layers of the target material to a value of 1.0.},
author = {Woytowitz, P. J. and Richman, R. H.},
doi = {10.1016/S0043-1648(99)00173-8},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Erosion{\_}CDM/Modeling of damage from multiple impacts by spherical particles{\_}Woytowitz.pdf:pdf},
issn = {00431648},
journal = {Wear},
keywords = {Continuum damage,Cyclic plastic work,Fatigue,Finite-element analysis,Impact damage,Solid-particle erosion,Strain-life},
pages = {120--133},
title = {{Modeling of damage from multiple impacts by spherical particles}},
volume = {233-235},
year = {1999}
}
@article{Motoren,
author = {Motoren, Tuning Von},
pages = {200--211},
title = {{5 Motorentuning}}
}
@article{Unterschied,
author = {Unterschied, Um Den},
pages = {3--4},
title = {{3 Unterschied zwischen manueller und CAD-Konstruktion}}
}
@article{Haibacha,
author = {Haibach, Erwin},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Empirical Fatigue Models + Validation/Betriebsfestigkeit{\_}ErwinHaibach/FrontMatter.pdf:pdf},
isbn = {9783540293637},
title = {{Erwin Haibach Betriebsfestigkeit}}
}
@article{Bockh2011,
abstract = {Bei erzwungener Konvektion wird der W{\"{a}}rme{\"{u}}bergang durch die Temperaturunterschiede und die Str{\"{o}}mung, die durch eine {\"{a}}u{\ss}ere Druckdifferenz aufrechterhalten wird, bestimmt. Die Druckdifferenz kann z.B. durch eine Pumpe oder einen H{\"{o}}henunterschied erzeugt werden. Erzwungene Konvektion ist die in der Technik am h{\"{a}}ufigsten vorkommende W{\"{a}}rme{\"{u}}bergangsart. In W{\"{a}}rme{\"{u}}bertragern wird zwischen zwei Fluiden, die durch eine Wand getrennt sind, W{\"{a}}rme {\"{u}}bertragen. Unsere Aufgabe wird sein, die W{\"{a}}rme{\"{u}}bergangszahlen in Abh{\"{a}}ngigkeit von den Str{\"{o}}mungsbedingungen, den Temperaturen und der Geometrie des W{\"{a}}rme{\"{u}}bertragers zu bestimmen},
author = {B{\"{o}}ckh, Peter and Wetzel, Thomas},
doi = {10.1007/978-3-642-15959-6},
isbn = {978-3-642-15958-9},
journal = {W{\"{a}}rme{\"{u}}bertragung},
pages = {121--132},
title = {{freie Konvektion}},
url = {http://www.springerlink.com/index/10.1007/978-3-642-15959-6},
volume = {0},
year = {2011}
}
@article{Gingrich2016a,
abstract = {An experimental investigation was conducted to explore the impact in-cylinder pressure oscillations have on piston heat transfer. Two fast-response surface thermocouples embedded in the piston top measured transient temperature and a commercial wireless telemetry system was used to transmit thermocouple signals from the moving piston. Measurements were made in a light-duty single-cylinder research engine operated under low temperature combustion regimes including Homogeneous Charge Compression Ignition (HCCI) and Reactivity Controlled Compression Ignition (RCCI) and Conventional Diesel (CDC). The HCCI data showed a correlated trend of higher heat transfer with increased pressure oscillation strength, while the RCCI and CDC data did not. An extensive HCCI data set was acquired. The heat transfer rate - when corrected for differences in cylinder pressure and gas temperature - was found to positively correlate with increased pressure oscillations. It is important to normalize the data before drawing conclusions as the magnitude of the effect was diminished significantly by the normalization procedure.},
author = {Gingrich, Eric and Janecek, Daniel and Ghandhi, Jaal},
doi = {10.4271/2016-01-9044},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2016{\_}Gingrich{\_}Experimental Investigation of the Impact of In-Cylinder Pressure Oscillations on Piston Heat Transfer.pdf:pdf},
issn = {1946-3944},
journal = {SAE Int. J. Engines},
number = {3},
pages = {2016--9044},
title = {{Experimental Investigation of the Impact of In-Cylinder Pressure Oscillations on Piston Heat Transfer}},
url = {http://papers.sae.org/2016-01-9044/},
volume = {9},
year = {2016}
}
@article{Rohrsystem2000,
author = {Rohrsystem, Das},
doi = {10.1007/978-3-8348-8279-0},
isbn = {9783834897831},
pages = {311--312},
title = {{18 Elemente zur Fu ¨ hrung von Fluiden (Rohrleitungen) 18.1}},
year = {2000}
}
@article{Stupkiewicz2007b,
author = {Stupkiewicz, Stanis{\l}aw},
doi = {10.1007/978-3-540-49717-2_3},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Stupkievicz 2007 - Micromechanics of Contact and Interphase Layers/97165{\_}03.pdf:pdf},
isbn = {3540497161},
issn = {16137736},
journal = {Lect. Notes Appl. Comput. Mech.},
number = {30},
pages = {17--35},
title = {{Homogeneous surface layers}},
volume = {2006},
year = {2007}
}
@article{Klein2009a,
author = {Klein, Bernd},
doi = {10.1007/978-3-8348-9965-1_18},
isbn = {978-3-8348-0701-4},
journal = {Leichtbau-Konstruktion},
pages = {215--231},
title = {{Stabilit{\{}{\"{a}}{\}}t von St{\{}{\"{a}}{\}}ben und Balken}},
year = {2009}
}
@article{Januszka2015a,
author = {Januszka, Marcin and Panfil, Wawrzyniec},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2016{\_}Lasocki{\_}ENGINE KNOCK DETECTION AND EVALUATION - A REVIEW.pdf:pdf},
number = {102},
pages = {37--48},
title = {{Proceedings of the institute of vehicles 2(102)/2015}},
volume = {2},
year = {2015}
}
@article{Algebra,
author = {Algebra, I Lineare},
title = {{Anhang : Lo ¨ sungen der {\{}{\^{U}}{\}}bungsaufgaben I Lineare Algebra}}
}
@book{Baehr_Stephan2010,
author = {Baehr, H.D and Stephan, K},
doi = {10.1007/978-3-642-10194-6},
edition = {7},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Vorlesungen/Waerme-Stoffuebertragung/2010{\_}Baehr+Stephan{\_}Waermeuebertragung{\_}KapitelWaermeuebertrager.pdf:pdf},
pages = {524--587},
publisher = {Springer-Verlag Berlin Heidelberg},
title = {{Waerme und Stoffuebertragung}},
year = {2010}
}
@misc{F1Regulation,
author = {{Federation Internationale de l'Automobile - FIA}},
title = {{2018 Formula one technical regulations}},
year = {2018}
}
@article{Schneider2016,
abstract = {{\{}{\textcopyright}{\}} 2016 Elsevier B.V.Modeling of crack propagation in materials has long been a challenge in solid-state physics and materials science. The phase-field method has now established as one of the tools for the description of crack propagation. The applied models are thermodynamically consistent and predict crack propagation in homogeneous materials under the consideration of different loading types, multiple physical fields and geometrical nonlinearities. Even dynamic loading processes are studied, including plastic effects. A multiphase-field model for crack propagation, which is indispensable to describe crack propagation on a mesoscopic length scale, is still missing. In this work, we overcome this deficiency and combine a crack propagation approach, which is based on Griffith's theory, with an established multiphase-field model for phase transformation.},
author = {Schneider, D and Schoof, E and Huang, Y and Selzer, M and Nestler, B},
doi = {10.1016/j.cma.2016.04.009},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Thermodynamik/PhasenFeld/Schneider{\_}Crack{\_}propagation{\_}multiphase{\_}systems-Dez2015.pdf:pdf},
issn = {00457825},
journal = {Comput. Methods Appl. Mech. Eng.},
keywords = {crack propagation,multiphase-field,phase-field,polycrystalline material},
title = {{Phase-field modeling of crack propagation in multiphase systems}},
url = {http://dx.doi.org/10.1016/j.cma.2016.04.009},
year = {2016}
}
@article{Reihen,
author = {Reihen, Unendliche and Vi-, Þ and Vi-, Þ},
pages = {570--639},
title = {{VI Potenzreihenentwicklungen}}
}
@article{Wallentowitz,
author = {Wallentowitz, Henning and Reif, Konrad},
doi = {10.1007/978-3-8348-8195-3},
isbn = {9783834802576},
title = {{Aus dem Programm}}
}
@article{Zusammenh,
author = {Zusammenh, Die and Entwicklung, Die},
journal = {Auslegung A Grad. J. Philos.},
pages = {117--150},
title = {{4 Einspritzsysteme und System{\"{u}}bersicht}}
}
@phdthesis{Kozuch2004_Diss,
author = {Kozuch, Peter},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Injection+Combustion+Ignitionsystems/2004{\_}Kozuch{\_}Ein ph{\"{a}}nomenologisches Modell zur kombinierten Stickoxid- und Russberechnung bei DI Dieselmotoren.pdf:pdf},
title = {{Ein ph{\"{a}}nomenologisches Modell zur kombinierten Stickoxid- und Ru{\ss}berechnung bei direkteinspritzenden Dieselmotoren Peter Ko{\v{z}}uch}},
year = {2004}
}
@article{Winkler2014b,
author = {Winkler, N.},
doi = {10.1177/1468087414544899},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2015{\_}Winkler{\_}Effect of pressure oscillations on in-cylinder heat transfer  - through LES Simulation.pdf:pdf},
isbn = {1468087414544},
issn = {1468-0874},
journal = {Int. J. Engine Res.},
keywords = {24 june 2014,6 march 2014,accepted,computational fluid dynamics,date received,heat transfer,internal combustion engines,large eddy simulation,pressure oscillations},
number = {6},
pages = {705--715},
title = {{Effect of pressure oscillations on in-cylinder heat transfer - through large eddy simulation}},
url = {http://jer.sagepub.com/lookup/doi/10.1177/1468087414544899},
volume = {16},
year = {2014}
}
@article{Tests,
author = {Tests, Chi-square and Tests, Nonparametric},
title = {12 12.2}
}
@article{Problem,
author = {Problem, Das},
title = {{Numerische Differentiation und Integration}}
}
@article{Raffinerien,
author = {Raffinerien, In Den},
journal = {Forschung},
title = {{13 Betriebsstoffe}}
}
@article{Shimada2004a,
abstract = {The effect of local lubricant viscosity on the temperature and thickness of oil film on a piston ring in a diesel engine is analyzed by using the Reynolds equation, and unsteady and two-dimensional energy equation with heat generated from viscous dissipation. The oil film viscosity for a multi-grade oil is then estimated by using the local oil film temperature and the local shear rate. Moreover, the heat transfer between ring and liner surfaces is examined. The oil film thickness calculated from this method is lesser than that of the case where the viscosity is based on the liner temperature and the mean shear rate. Maximum values of heat transfer at the ring and liner surfaces are obtained at the vicinity of crank angle where the oil film thickness is at a minimum.ER -},
author = {Shimada, Akiko and Harigaya, Yasuo and Suzuki, Michiyoshi and Takiguchi, Masaaki},
doi = {10.4271/2004-32-0024},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Heat Transfer Combustion Chamber/2004{\_}Shimada{\_}An Analysis of Oil Film Temperature - Oil Film Thickness and Heat Transfer on a piston ring of internal combustion engine.pdf:pdf},
isbn = {0791846628},
issn = {07424795},
number = {724},
title = {{An Analysis of Oil Film Temperature, Oil Film Thickness and Heat Transfer on a Piston Ring of Internal Combustion Engine: The Effect of Local Lubricant Viscosity}},
url = {http://papers.sae.org/2004-32-0024/},
year = {2004}
}
@article{Problembereiche,
author = {Problembereiche, Beide and Ziele, Beide},
title = {{Abw{\{}{\"{a}}{\}}rmeverwertung}}
}
@article{Grundlagen1939,
author = {Grundlagen, Thermodynamische},
title = {{6 Gasturbinen-Kraftwerke}},
year = {1939}
}
@article{Integration1999,
author = {Integration, Die and Aufgabe, Die and Stabilit, Elektronischen and Control, Active Body and Fahrwerke, Aktive and Beeinflussung, Die and Stabilisatoren, Aktive},
journal = {System},
title = {{16 Vernetzung von L{\"{a}}ngs-, Quer- und Vertikaldynamik-Regelung}},
year = {1999}
}
@book{Riccardella1992,
author = {Riccardella, PC and Deardorff, AF and Griesbach, TJ},
booktitle = {Adv. Fatigue Lifetime Predict. Tech.},
doi = {10.1520/STP1122-EB},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Neuer Ordner/Advances in fatigue lifetime predictive techniques Part1.pdf:pdf},
isbn = {978-0-8031-1423-4},
issn = {00660558},
keywords = {FATIGUE,MONITORING,POWER PLANTS,PRESSURE VESSELS AND PIPING,THERMAL STRESSES},
pages = {460--473},
pmid = {11439068},
title = {{Advances in Fatigue Lifetime Predictive Techniques}},
url = {https://apps.webofknowledge.com/full{\_}record.do?product=UA{\&}search{\_}mode=GeneralSearch{\&}qid=11{\&}SID=Z1UxbH6jtsqo8n9kPQr{\&}page=1{\&}doc=1},
volume = {1122},
year = {1992}
}
@article{Gross2011a,
author = {Gross, Dietmar and Seelig, Thomas},
doi = {10.1007/978-3-642-10196-0},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Gross, Selig 2011 - Bruchmechanik/Gross, Seelig - 2011 - BruchmechanikKap2.pdf:pdf},
isbn = {978-3-642-10195-3},
title = {{Bruchmechanik}},
url = {http://link.springer.com/10.1007/978-3-642-10196-0},
year = {2011}
}
@article{Allianz2003a,
author = {Allianz, Von M Pfender and Berlin, M{\"{u}}nchen},
file = {:C$\backslash$:/Users/p327208/Desktop/Promotion/Literature/Empirical Fatigue Models + Validation/Betriebsfestigkeit{\_}ErwinHaibach/Kap6 Schrifttumhinweis.pdf:pdf},
isbn = {3540440631},
number = {2},
title = {{6 Schrifttumshinweise}},
volume = {6},
year = {2003}
}
@article{Ubertragung,
author = {{\"{U}}bertragung, Die},
journal = {Frequenz},
pages = {6--13},
title = {{2 Messsignale}}
}
@article{Galindo-Nava2012,
abstract = {A new theory for describing plastic deformation in metals is presented. The approach focuses on obtaining an expression for the dislocation recovery term in terms of the energy barrier for dislocation annihilation, ?????. G???. This term is obtained from the contributions of dislocation formation and migration, the statistical entropy inherent to the annihilation process, and the chemical work due to the presence of vacancies. It is shown that at high temperatures, vacancy migration features strongly in dislocation recovery via a climb-assisted process. Employing only input parameters reported in the literature, the theory is able to reproduce experimental stress-strain relationships at temperatures ranging from cryogenic conditions to near-melting temperatures for Cu, Al, Ni and Ag at a variety of strain rates. It is demonstrated that low temperature cross-slip can operate at higher temperatures by increasing the strain rate, and that high temperature dislocation climb can feature at low temperatures by reducing the vacancy migration energy. ?? 2012 Elsevier B.V..},
author = {Galindo-Nava, E I and Rivera-D??az-del-Castillo, P E J},
doi = {10.1016/j.msea.2012.02.055},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Kriechen{\_}Spannungsrelaxation/2012{\_}Galindo-Nava+Castillo{\_}A thermostatistical theory of low and high temperature deformation in metals.pdf:pdf},
isbn = {0921-5093},
issn = {09215093},
journal = {Mater. Sci. Eng. A},
keywords = {Dislocations,Hardening,Non-ferrous alloys,Plasticity},
pages = {110--116},
publisher = {Elsevier B.V.},
title = {{A thermostatistical theory of low and high temperature deformation in metals}},
url = {http://dx.doi.org/10.1016/j.msea.2012.02.055},
volume = {543},
year = {2012}
}
@book{Kleina,
author = {Klein, Bernd},
isbn = {9783834802965},
title = {{Aus dem Programm Maschinenelemente und}}
}
@article{Wortmann2010,
author = {Wortmann, Hendrik},
doi = {10.1515/9783111376363.1},
isbn = {9783867642644},
pages = {7--9},
title = {{0 Einleitung}},
year = {2010}
}
@article{Kunzli1999,
author = {K{\"{u}}nzli, Benjamin},
isbn = {3928034804},
journal = {Soziol. Aufkl{\{}{\"{a}}{\}}rung der Erziehungswissenschaften?},
pages = {11----20 T4 ---- Anmerkungen zur Rezeption und Themenf},
title = {{2. Einleitung}},
year = {1999}
}
@article{Beispielb,
author = {Beispiel, Zum and Interpolation, Die and Computerspiel, Ein},
title = {{A Interpolation}}
}
@book{Borbely2006,
abstract = {Loss of cortical gray matter is accompanied by a commensurate increase in the sulcal and intraventricular cerebrospinal fluid volume. On diffusion-weighted magnetic resonance imaging, this would be reflected as a higher apparent diffusion coefficient in affected brain regions. On the basis of the above premise, we suggest that the apparent diffusion coefficient may be used as a surrogate marker for the assessment of regional brain volume deficits. We demonstrate this approach by voxelwise analysis of registered apparent diffusion coefficient images from a group of 15 patients with schizophrenia and 15 age-matched healthy controls. We found widespread regional apparent diffusion coefficient increases in patients. Affected areas included the bilateral insular cortex, hippocampus, temporal lobe, and occipital areas. These results largely concur with previous findings of cortical volume deficits in schizophrenia.},
author = {Borbely, Anne-marie and Kreider, Jan F and Bejan, Adrian and Cundiff, John S and Davis, Lorin R},
booktitle = {Mech. Compos. Mater.},
doi = {10.1021/ja00116a001},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Plasticity models/Elastoplasticity Theory{\_}Lubarda{\_}2002.pdf:pdf},
isbn = {9780849391392},
issn = {9780849391378},
pages = {1455--1459},
title = {{Distributed Generation : The Power Paradigm for the New Millennium Fluid Power Circuits and Controls : Fundamentals and Applications}},
url = {http://www.ncbi.nlm.nih.gov/pubmed/16110271},
volume = {23},
year = {2006}
}
@article{Forest2009b,
abstract = {A unifying thermomechanical framework is presented that reconciles several classes of gradient elastoviscoplasticity and damage models proposed in the literature during the last 40 years. It is based on the introduction of the micromorphic counterpart ϕ {\$}\chi{\$} of a selected ... {\$}\backslash{\$}n},
author = {Forest, Samuel},
doi = {10.1061/(ASCE)0733-9399(2009)135:3(117)},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/2009{\_}Forest{\_}Micromorphic Approach for Gradient Elasticity Viscoplasticity and Damage.pdf:pdf},
isbn = {0733-9399},
issn = {0733-9399},
journal = {J. Eng. Mech.},
number = {3},
pages = {117--131},
title = {{Micromorphic Approach for Gradient Elasticity, Viscoplasticity, and Damage}},
volume = {135},
year = {2009}
}
@article{CARPINTERI2001,
abstract = {Some multiaxial high-cycle fatigue criteria based on the so-called critical plane approach are reviewed. According to such an approach, the critical plane where the fatigue life assessment should be performed can be determined by maximising the amplitudes and/or values of some stress components. In the present paper, the critical plane orientation is correlated with the averaged principal stress directions deduced through the weight function method, and a new fatigue failure criterion is proposed. The results derived by applying the present criterion and the other critical plane criteria analysed are compared with experimental data related to different brittle (hard) metals under in-phase or out-of-phase sinusoidal biaxial normal and shear stress states. 0},
author = {CARPINTERI, A and SPAGNOLI, A},
doi = {10.1016/S0142-1123(00)00075-X},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Empirical Fatigue Models + Validation/2000{\_}Carpinteri{\_}Multiaxial high cycle fatigue criterion for hard metals.pdf:pdf},
isbn = {0142-1123},
issn = {01421123},
journal = {Int. J. Fatigue},
keywords = {multiaxial},
number = {2},
pages = {135--145},
title = {{Multiaxial high-cycle fatigue criterion for hard metals}},
url = {http://linkinghub.elsevier.com/retrieve/pii/S014211230000075X},
volume = {23},
year = {2001}
}
@article{Sicherungselemente,
author = {Sicherungselemente, Stiftverbindungen and Wirkung, Funktion},
pages = {274--298},
title = {{9 Bolzen-, Stiftverbindungen und Sicherungselemente 9.1}}
}
@article{Allianz2003,
author = {Allianz, Von M Pfender and Berlin, M{\"{u}}nchen},
file = {:C$\backslash$:/Users/p327208/Desktop/Promotion/Literature/Empirical Fatigue Models + Validation/Betriebsfestigkeit{\_}ErwinHaibach/Kap6 Schrifttumhinweis.pdf:pdf},
isbn = {3540440631},
number = {2},
title = {{6 Schrifttumshinweise}},
volume = {6},
year = {2003}
}
@article{Formulierung2007,
author = {Formulierung, Die and Serienfreigabe, Die and Erreichen, Zum and Konstruieren, Methodische},
journal = {Fahrzeuggetriebe},
title = {{15 Entwicklungsprozess von Fahrzeuggetrieben}},
year = {2007}
}
@article{Ermudungsfestigkeit,
author = {Erm{\"{u}}dungsfestigkeit, Nachweises Der},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Empirical Fatigue Models + Validation/Erm{\"{u}}dungsfestigkeit{\_}Radaj/Kap8{\_}Rechnerischer Nachweis der Erm{\"{u}}dungsfestigkeit.pdf:pdf},
title = {{8 Rechnerischer Nachweis der Erm{\"{u}}dungsfestigkeit}}
}
@article{Ablauf,
author = {Ablauf, F{\"{u}}r Den and Dehnung, Thermische},
journal = {System},
pages = {32--58},
title = {{3 Stoffeigenschaften}}
}
@article{Scherschneiden,
author = {Scherschneiden, Das and Schr, Der and Ausschnei-, Verfahren and Rest, Der and Schnittlinie, Die},
title = {{Spanen ; Abtragen ; thermisches Schneiden )}}
}
@article{Zavala2011,
author = {Zavala, Jos{\'{e}} Carlos and Folkerts, Charles},
doi = {10.4271/2011-01-1409},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2011{\_}Zavala{\_}Knock Detection and Estimation Based on Heat Release Startegies.pdf:pdf},
title = {{Knock Detection and Estimation Based on Heat Release Strategies}},
url = {http://papers.sae.org/2011-01-1409/},
year = {2011}
}
@article{Johnson2004,
author = {Johnson, Ws and Hillberry, Bm},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Probabilistic Aspects/2004{\_}StevenJohnson{\_}Probabilistic Aspects of Life Prediction.pdf:pdf},
journal = {Book},
title = {{Probabilistic aspects of life prediction}},
url = {http://books.google.com/books?hl=en{\%}7B{\&}{\%}7Dlr={\%}7B{\&}{\%}7Did=pDtb-CJLVbYC{\%}7B{\&}{\%}7Doi=fnd{\%}7B{\&}{\%}7Dpg=PP7{\%}7B{\&}{\%}7Ddq=Probabilistic+Aspects+of+Life+Prediction{\%}7B{\&}{\%}7Dots=fII0k-XR1K{\%}7B{\&}{\%}7Dsig=qyo{\%}7B{\_}{\%}7D6w{\%}7B{\_}{\%}7DnT7cN1tqI8pird5rUdts},
year = {2004}
}
@article{Rakopoulos2011,
author = {Mavropoulos, G C and Rakopoulos, C D and Hountalas, D T},
doi = {10.1177/0954407011402280},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Heat Transfer Combustion Chamber/2010{\_}Rakopoulos{\_}Analysis and evaluation of the thermal shock phenomena in the in-cylinder surfaces of a DI diesel engine during transient operation.pdf:pdf},
journal = {Proc. Inst. Mech. Eng. Part D J. Automob. Eng.},
keywords = {diesel engine,heat transfer,thermal shock,transient operation,unsteady},
number = {9},
pages = {1265--1289},
title = {{Analysis and evaluation of the thermal shock phenomena in the in-cylinder surfaces of a DI diesel engine during its transient operation}},
volume = {225},
year = {2011}
}
@article{Arbeitsumgebungb,
author = {Arbeitsumgebung, Die},
pages = {175--194},
title = {{7 Zeichnungsableitung aus dem 3D-Modell}}
}
@article{Loubar2005,
abstract = {This paper deals with the transient thermal signal around an engine cylinder in order to propose a new and nonintrusive method of knock detection. Numerical simulations of unsteady heat transfer through the cylinder and inside the coolant flow are carried out to account for heat flux variations due to normal and knocking combustion. The effect of rib roughened surfaces on thermal signal amplification is investigated. The geometric parameters are fixed at Pi/h=70 and w/h=1 with a Reynolds number based on hydraulic diameter of 12,000. The results reveal that square ribs give better performance in term of thermal signal amplification within the fluid. An amplification of the temperature variation up to 20 times higher is found. Finally, flow analysis shows that amplification depends on the position where the thermal signal is collected.},
author = {Loubar, Khaled and Bellettre, Jérôme and Tazerout, Mohand},
doi = {10.1115/1.1857943},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2005{\_}Loubar{\_}Unsteady Heat Transfer enhancement around an engine cylinder in order to detect knockpdf.pdf:pdf},
isbn = {0022-1481},
issn = {00221481},
journal = {J. Heat Transfer},
number = {3},
pages = {278},
title = {{Unsteady Heat Transfer Enhancement Around an Engine Cylinder in Order to Detect Knock}},
url = {http://heattransfer.asmedigitalcollection.asme.org/article.aspx?articleid=1447711},
volume = {127},
year = {2005}
}
@article{Piero2005,
author = {Piero, D E L},
number = {1967},
title = {{10 Plasticity}},
year = {2005}
}
@article{Mizuno2009b,
author = {Mizuno, Hideaki and Ashida, Koichi and Teraji, Atsushi and Ushijima, Kenshi and Takemura, Shinichi},
doi = {10.4271/2009-01-0187},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2009{\_}Mizuno{\_}Transient Analysis of the Piston Temperature with Measurement and Simulation.pdf:pdf},
journal = {SAE Int. J. Engines},
number = {1},
pages = {187--2009},
title = {{Transient Analysis of the Piston Temperature with Consideration of In-cylinder Phenomena Using Engine Measurement and Heat Transfer Simulation Coupled with Three-dimensional Combustion Simulation}},
volume = {2},
year = {2009}
}
@article{Chaboche1986a,
author = {Chaboche, J L},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/Hardening Recovery Creep/1986{\_}Chaboche{\_}Time-independent-constitutive-theories-for-cyclic-plasticity.pdf:pdf},
journal = {Int. J. Plast.},
number = {2},
pages = {149--188},
title = {{Time-independent constitutive theorems for cyclic plasticity}},
volume = {2},
year = {1986}
}
@article{Shojaefard2005,
author = {Shojaefard, M H and Noorpoor, A R and Bozchaloe, D A and Ghaffarpour, M},
doi = {https://doi.org/10.1080/10407780590959943},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Heat transfer intake+exhaust system/2005{\_}Shojaefard+Noorpoor{\_}Transient Thermal Analysis of Engine Exhaust Valve.pdf:pdf},
journal = {Numer. Heat Transf. Part A Appl.},
number = {7},
pages = {627--644},
title = {{Transient Thermal Analysis of Engine Exhaust Valve}},
volume = {48},
year = {2005}
}
@article{Potirniche2007a,
abstract = {This paper presents a polycrystalline plasticity theory including damage evolution in FCC materials. The formulation is thermodynamically-based and involves a multiplicative decomposition of the deformation gradient into its elastic, plastic and volumetric components. Plastic deformation at the grain level is assumed to occur by rate-dependent crystallographic slip. As a result of accumulated plastic strain and stress triaxiality, damage evolution leading to volumetric deformation is considered to occur within a single crystal by void nucleation, growth and coalescence. The overall stress-strain response of the polycrystalline material is obtained by Taylor averaging on the stress response of each grain. In the model, damage progression arises naturally from averaging each single crystal's damage evolution. A parametric study is performed to evaluate the amount of damage and strains at fracture on both single and polycrystals in order to understand crystal orientation effects. For validation purposes, model predictions of uniaxial stress-strain data are compared with experimental results for some aluminum alloys, and the comparison is shown to agree very well. ?? 2007 Elsevier Ltd. All rights reserved.},
author = {Potirniche, G. P. and Horstemeyer, M. F. and Ling, X. W.},
doi = {10.1016/j.mechmat.2007.04.004},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2006{\_}Potirniche{\_}An internal state variable damage model in crystal plasticity.pdf:pdf},
isbn = {0167-6636},
issn = {01676636},
journal = {Mech. Mater.},
keywords = {Crystal plasticity,Damage,Nucleation,Polycrystals,Void growth},
number = {10},
pages = {941--952},
title = {{An internal state variable damage model in crystal plasticity}},
volume = {39},
year = {2007}
}
@misc{WECRegulation,
author = {{Federation Internationale de l'Automobile - FIA}},
title = {{2018 World Endurance Championship technical regulations}},
year = {2018}
}
@article{Mesarovic2016,
abstract = {{\textcopyright} 2016 The Author(s) Published by the Royal Society. All rights reserved.Diffusional creep is characterized by growth/disappearance of lattice planes at the crystal boundaries that serve as sources/sinks of vacancies, and by diffusion of vacancies. The lattice continuum theory developed here represents a natural and intuitive framework for the analysis of diffusion in crystals and lattice growth/loss at the boundaries. The formulation includes the definition of the Lagrangian reference configuration for the newly created lattice, the transport theorem and the definition of the creep rate tensor for a polycrystal as a piecewise uniform, discontinuous field. The values associated with each crystalline grain are related to the normal diffusional flux at grain boundaries. The governing equations for Nabarro-Herring creep are derived with coupled diffusion and elasticity with compositional eigenstrain. Both, bulk diffusional dissipation and boundary dissipation accompanying vacancy nucleation and absorption, are considered, but the latter is found to be negligible. For periodic arrangements of grains, diffusion formally decouples from elasticity but at the cost of a complicated boundary condition. The equilibrium of deviatorically stressed polycrystals is impossible without inclusion of interface energies. The secondary creep rate estimates correspond to the standard Nabarro-Herring model, and the volumetric creep is small. The initial (primary) creep rate is estimated to be much larger than the secondary creep rate.},
author = {Mesarovic, Sinisa Dj},
doi = {10.1098/rspa.2016.0039},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Kriechen{\_}Spannungsrelaxation/2016{\_}Mesarovic{\_}Lattice{\_}continuum{\_}and{\_}diffusional{\_}creep.pdf:pdf},
isbn = {1471-2946},
issn = {14712946},
journal = {Proc. R. Soc. A Math. Phys. Eng. Sci.},
keywords = {materials science,mechanics},
number = {2188},
title = {{Lattice continuum and diffusional creep}},
volume = {472},
year = {2016}
}
@misc{Eshelby1951,
abstract = {The parallel between the classical theory of elasticity and the modern physical theory of the solid state is incomplete; the former has nothing analogous to the concept of the force acting on an imperfection (dislocation, foreign atom, etc.) in a stressed crystal lattice. To remedy this a general theory of the forces on singularities in a Hookean elastic continuum is developed. The singularity is taken to be any state of internal stress satisfying the equilibrium equations but not the compatibility conditions. The force on a singularity can be given as an integral over a surface enclosing it. The integral contains the elastic field quantities which would surround the singularity in an infinite medium, multiplied by the difference between these quantities and those actually present. The expression for the force is thus of essentially the same form whether the force is due to applied surface tractions, other singularities or the presence of the free surface of the body ({\{}{\{}{\}}'{\{}{\}}{\}}image force{\{}{\{}{\}}'{\{}{\}}{\}}). A region of inhomogeneity in the elastic constants modifies the stress field; if it is mobile one can define and calculate the force on it. The total force on the singularities and inhomogeneities inside a surface can be expressed in terms of the integral of a {\{}{\{}{\}}'{\{}{\}}{\}}Maxwell tensor of elasticity{\{}{\{}{\}}'{\{}{\}}{\}} taken over the surface. Possible extensions to the dynamical case are discussed.},
author = {Eshelby, J D},
booktitle = {Philos. Trans. R. Soc. A Math. Phys. Eng. Sci.},
doi = {10.1098/rsta.1951.0016},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/1951{\_}Eshelby{\_}The force oo an elastic singularity.pdf:pdf},
isbn = {00804614},
issn = {1364-503X},
number = {877},
pages = {87--112},
title = {{The Force on an Elastic Singularity}},
url = {http://rsta.royalsocietypublishing.org/cgi/doi/10.1098/rsta.1951.0016},
volume = {244},
year = {1951}
}
@article{Ermittlunga,
author = {Ermittlung, Die and Sum-, Die and Vor-, Die},
pages = {38--39},
title = {{16 Gep{\{}{\"{a}}{\}}ckraum und Volumenermittlung nach VDA ( DIN70020 )}}
}
@article{Betrachtungenk,
author = {Betrachtungen, Allgemeine},
journal = {Integr. Vlsi J.},
title = {{9 Stromfadentheorie 9.1}}
}
@article{Feuer,
author = {Feuer, Kein},
title = {{Kraftanlagen}}
}
@article{Lohe1993,
author = {Lohe, B. and Futterer, E.},
doi = {10.1002/cite.330650972},
issn = {0009-286X},
journal = {Chemie Ing. Tech.},
number = {9},
pages = {1093--1093},
title = {{70. Strukturoptimierung chemischer Anlagen auf Grundlage exergetischer Kriterien}},
url = {http://doi.wiley.com/10.1002/cite.330650972},
volume = {65},
year = {1993}
}
@article{Rostampour2015b,
abstract = {This investigation deals with the EF7 (TC) engine, a dual fuel engine equipped with a turbocharger system, consequently with a high probability of knock inception. In this study, an operating cycle of the engine was simulated using KIVA-3V code. Some modifications were carried out on the KIVA method of calculating pressure in the intake port in order to simulate turbocharger pressure correctly. Auto-ignition and knock were then simulated using the auto-ignition integral model. The modified code and the simulation were verified using three different methods; in-cylinder average pressure, gas temperature of the exhaust port, and auto-ignition timing. The simulation results using the auto-ignition integral model, as compared with the experimental data, proved to be reasonably accurate. Following this validation, the effect of the knock phenomenon on the engine heat transfer through the walls was investigated. The simulations showed that the rate of heat transfer through the walls under knocking conditions is about 2.2 times higher than that under normal conditions. However, it was also shown that the total heat transfer increases about 15{\%}.},
author = {Rostampour, Arman and Toosi, Ali Nassiri},
doi = {10.1115/1.4030517},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2015{\_}Rostampour{\_}Numerical Investigation of the effect of knock on heat transfer in a turbo si engine.pdf:pdf},
issn = {0742-4795},
journal = {J. Eng. Gas Turbines Power},
number = {12},
pages = {121502},
title = {{Numerical Investigation of the Effect of Knock on Heat Transfer in a Turbocharged Spark Ignition Engine}},
url = {http://www.scopus.com/inward/record.url?eid=2-s2.0-84930634240{\&}partnerID=tZOtx3y1},
volume = {137},
year = {2015}
}
@article{Gurson1977b,
abstract = {Widely used constitutive laws for engineering materials assume plastic incompressibility, and no effect on yield of the hydrostatic component of stress. However, void nucleation and growth (and thus bulk dilatancy) are commonly observed is some processes which are characterized by large local plastic flow, such as ductile fracture.},
author = {Gurson, A. L.},
doi = {10.1115/1.3443401},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Plasticity models/Continuum Theory of Ductile Rupture by Void Nucleation and  Growth-PartI{\_}ByGurson.pdf:pdf},
isbn = {0094-4289},
issn = {00944289},
journal = {J. Eng. Mater. Technol.},
number = {1},
pages = {2},
title = {{Continuum Theory of Ductile Rupture by Void Nucleation and Growth: Part I—Yield Criteria and Flow Rules for Porous Ductile Media}},
url = {http://materialstechnology.asmedigitalcollection.asme.org/article.aspx?articleid=1422194},
volume = {99},
year = {1977}
}
@article{Betrachtungenj,
author = {Betrachtungen, Allgemeine},
title = {{5 Grundgleichungen der Str¨ omungsmechanik 5.1}}
}
@article{Wang2014a,
author = {Wang, Cong and Shang, De Guang and Wang, Xiao Wei},
doi = {10.1007/s11665-014-1335-7},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Empirical Fatigue Models + Validation/2014{\_}Wang{\_}7075-T651 Models and validation.pdf:pdf},
issn = {15441024},
journal = {J. Mater. Eng. Perform.},
keywords = {critical plane,high-cycle fatigue,life prediction,maximum shear stress (MSS),multsiaxial fatigue},
number = {2},
pages = {816--824},
title = {{A New Multiaxial High-Cycle Fatigue Criterion Based on the Critical Plane for Ductile and Brittle Materials}},
volume = {24},
year = {2014}
}
@article{Allianz2003b,
author = {Allianz, Von M Pfender and Berlin, M{\"{u}}nchen},
isbn = {3540440631},
number = {2},
title = {{6 Schrifttumshinweise}},
volume = {6},
year = {2003}
}
@article{Rechnertechnik,
author = {Rechnertechnik, Entwicklung Der},
title = {{10 Numerische Verfahren zur Feldberechnung}}
}
@book{Zahlena,
author = {Zahlen, Reelle},
isbn = {4285714285714},
number = {x},
pages = {1--36},
title = {{1 Was man wissen sollte}}
}
@article{Zahoransky2013b,
author = {Zahoransky, Richard a. and Allelein, Hans-Josef and Schelling, Udo and Schwarz, Harald and Bollin, Elmar and Oehler, Helmut},
doi = {10.1007/978-3-8348-2279-6},
isbn = {978-3-8348-1869-0},
journal = {Energietechnik - Syst. zur Energieumwandlung},
pages = {350--359},
title = {{14 Energetische Verwertung von Biomasse}},
url = {http://www.springerlink.com/index/10.1007/978-3-8348-2279-6},
year = {2013}
}
@article{Spunk2010,
author = {Spunk, Joseph and Nuri, Aksel},
isbn = {9783642131424},
title = {{Str{\"{o}}mungslehre Einf{\"{u}}hrung in die Theorie}},
year = {2010}
}
@article{Kroner1977,
abstract = {Recently P.H. Dederichs and R. Zeller (1973) have developed a formal theory of the bounds of odd order n for the effective elastic moduli of linearly elastic, disordered materials. The bounds are established by use of statistical information given in terms of correlation functions up to order n (= 1, 3, 5,...). This theory is extended to include the bounds of even order n. It is indicated how these bounds can be made optimum under the given statistical information. The results for bounds of even and odd order are obtained in forms which resemble Neumann series, containing multiple integrals up to order (n-1). These integrals can be calculated for certain materials which are classified in terms of a gradual statistical homogeneity, isotropy and disorder. Materials which possess these properties up to the correlation functions of nth order are called overall grade n materials. The optimum bounds for overall grade 2 and grade 3 materials are given explicitly. Optimum bounds for materials which are of grade ∞ in homogeneity and isotropy (i.e. (statistically) perfectly homogeneous and isotropic) and, at the same time, disordered of grade 2 or 3 are also derived. Those for grade 2 in disorder are the Z. Hashin and S. Shtrikman's (1963) bounds. Those for grade 3 are the narrowest, explicit bounds so far derived for random elastic materials. They contain within themselves the so-called self-consistent elastic moduli. {\textcopyright} 1977.},
author = {Kr{\"{o}}ner, E.},
doi = {10.1016/0022-5096(77)90009-6},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/Strukturmechanik MMS/Literatur/Kr{\"{o}}ner 1977.pdf:pdf},
isbn = {0022-5096},
issn = {00225096},
journal = {J. Mech. Phys. Solids},
number = {2},
pages = {137--155},
title = {{Bounds for effective elastic moduli of disordered materials}},
volume = {25},
year = {1977}
}
@article{PeterSimilar2017,
author = {H{\"{o}}lz, Peter and B{\"{o}}hlke, Thomas and Kr{\"{a}}mer, Thomas},
doi = {https://doi.org/10.1007/s41104-018-0026-z},
journal = {Int. J. Automot. Engine Technol.},
pages = {1--16},
title = {{CFD-CHT calculation method using Buckingham Pi-Theorem for complex fuid-solid heat transfer problems with scattering boundary conditions}},
year = {2018}
}
@article{Druck2014,
author = {Druck, Der and Presse, Hydraulische and Schwerkraft, Der},
doi = {10.1007/978-3-642-38891-0},
isbn = {978-3-642-38890-3},
journal = {Maschinenelemente},
number = {3},
pages = {48--49},
title = {{Statik der Fl{\"{u}}ssigkeiten}},
url = {http://link.springer.com/10.1007/978-3-642-38891-0},
year = {2014}
}
@article{Anhang1995,
author = {Anhang, Der},
isbn = {0688011411},
pages = {104--111},
title = {{9 Anhang}},
year = {1995}
}
@book{Ferziger2002,
author = {Ferziger, Joel H. and Peric, Milovan},
publisher = {Springer Berlin Heidelberg},
title = {{Computational Methods for Fluid Dynamics}},
year = {2002}
}
@book{Bazant1992a,
abstract = {Elasticity, plasticity, damage mechanics and cracking are all phenomena that determine the resistance of solids to deformation and fracture. The authors of this book discuss a modern method of mathematically modeling the behavior of macroscopic volume elements. The first three chapters review physical mechanisms at the microstructural level, thermodynamics of irreversible processes, mechanics of continuous media, and the classification of the behavior of solids. The rest of the book is devoted to the modeling of different types of material behavior. In each case the authors present characteristic data for numerous materials, and discuss the physics underlying the phenomena together with methods for the numerical analysis of the resulting equations.},
author = {Ba{\v{z}}ant, Z P},
booktitle = {Can. J. Civ. Eng.},
doi = {10.1139/l92-025},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Kriechen{\_}Spannungsrelaxation/1985{\_}Jean{\_}Lemaitre+Jean-Louis+Chaboche{\_}Mechanics{\_}of{\_}Solid{\_}Materials.pdf:pdf},
isbn = {0521477581},
issn = {0315-1468},
number = {1},
pages = {197},
title = {{Mechanics of solid materials}},
url = {http://www.nrcresearchpress.com/doi/abs/10.1139/l92-025},
volume = {19},
year = {1992}
}
@article{Algebra2013,
author = {Algebra, Some Vector},
doi = {10.1016/B978-1-85617-633-0.00028-9},
isbn = {9781856176330},
pages = {655--659},
title = {{Some Vector Algebra}},
volume = {1},
year = {2013}
}
@article{Lin1989,
author = {Lin, T. H. and Lin, S. R. and Wu, X. Q.},
doi = {10.1080/01418618908221174},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/1989{\_}Lin{\_}Micromechanics of an extrusion in high-cycle fatigue.pdf:pdf},
issn = {0141-8610},
journal = {Philos. Mag. A},
number = {6},
pages = {1263--1276},
title = {{Micromechanics of an extrusion in high-cycle fatigue}},
url = {http://www.tandfonline.com/doi/abs/10.1080/01418618908221174},
volume = {59},
year = {1989}
}
@article{Darstellunga,
author = {Darstellung, Vektorielle},
title = {{XIV Vektoranalysis}}
}
@article{Guennec2013,
abstract = {Ultrasonic testing method has allowed some impressive improvements in order to better grasp fatigue properties of various metallic materials the latest 20 years. It is particularly the case in the very high cycle regime since ultrasonic fatigue tests are conducted at very high stressing frequencies. However, the question of a potential difference of fatigue strengths due to huge frequency gap between ultrasonic method (usually carried out at 20 kHz) and servo-hydraulic one (usually in the range of 1?100 Hz) is still unclear and needs to be studied for a various kind of metallic materials. The case of low carbon steels presents a singularity, as fatigue properties are significantly different between these two fatigue tests methods. It seems particularly interesting to study this kind of materials in order to get a better overview of frequency effect in metallic materials fatigue. Aim of the present work, which consists of a general survey of JIS S15C steel (0.15{\%} C) fatigue properties, is firstly to reconfirm such a frequency effect. Secondly, based on several experiments related to micro-plasticity behavior, some discussions will be held in order to explain this frequency effect in the case of low carbon steels.},
author = {Guennec, B. and Ueno, A. and Sakai, T. and Takanashi, M. and Itabashi, Y.},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Surface effects + Frequency effects/Frequency effects on high cycle fatigue of low carbon steel.PDF:PDF},
journal = {13th Int. Conf. Fract.},
keywords = {cyclic hardening,ebsd observations,frequency effect,low carbon steel,ultrasonic test},
pages = {1--10},
title = {{Effect of Loading Frequency in Fatigue Properties and Micro-Plasticity Behavior of JIS S15C Low Carbon Steel}},
year = {2013}
}
@article{Nebenaggregate,
author = {Nebenaggregate, Optimierung Der},
journal = {Stand},
title = {{12 Benzin-Direkteinspritzung im elektrischen}}
}
@article{Wei1974,
author = {Wei, K P},
pages = {19--32},
title = {{Study of in}},
volume = {6},
year = {1974}
}
@article{Ladungen,
author = {Ladungen, Die and Bild, Das and Feld, Das and Feldlinien, Die and Fl, Diese and Abschnitt, Im},
title = {{4 Elektrisches Feld}}
}
@article{Vanderbilt1989,
author = {Vanderbilt, David},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/Folien CISM Summer School Mai2017 - Mesoscale Models/courses{\_}C1703{\_}roux+{\_}lect4-elast1.pdf:pdf},
number = {8},
pages = {77--89},
title = {{Elastic Properties}},
volume = {40},
year = {1989}
}
@article{Mughrabi2010,
abstract = {In the first part, some fundamental issues that have been under discussion for a long time will be revisited, namely the effect of the cyclic slip mode on the fatigue-induced dislocation distributions, the origin and effect of cyclic slip irreversibilities and their relation to fatigue life and, finally, cyclic strain localization and fatigue crack initiation in persistent slip bands. In the second part, some topics that have recently found increasing interest will be discussed such as the cyclic deformation and fatigue behaviour of ultrafine-grained and nanostructured materials and the microstructural mechanisms that govern fatigue life of ductile and high-strength materials in the range of ultrahigh cycle fatigue. Some general conclusions will be drawn. ?? 2010 Published by Elsevier Ltd.},
author = {Mughrabi, Hael},
doi = {10.1016/j.proeng.2010.03.003},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2010{\_}Mughrabi{\_}Fatigue, an everlasting materials problem-still en vogue{\_}FatigueSlipBands-Overview.pdf:pdf},
isbn = {1877-7058},
issn = {18777058},
journal = {Procedia Eng.},
keywords = {Cyclic slip irreversibilities,Cyclic slip mode,Fatigue lives,Microstructural effects,Ultrafine-grained metals,Ultrahigh Cycle Fatigue (UHCF)},
number = {1},
pages = {3--26},
publisher = {Elsevier},
title = {{Fatigue, an everlasting materials problem - Still en vogue}},
url = {http://dx.doi.org/10.1016/j.proeng.2010.03.003},
volume = {2},
year = {2010}
}
@article{Agarwal2006b,
abstract = {Thermal loading of diesel engine pistons has increased dramatically in recent years owing to applications of various technologies to meet low emission and high power density requirements. Control of piston temperatures by cooling of these pistons has become one of the determining factors in a successful engine design. The pistons are cooled by oil jets fired at the underside from the crankcase. Any excessive piston temperature rise may lead to engine seizure because of piston warping. However, if the temperature at the underside of the piston, where the oil jet strikes the piston, is above the boiling range of the oil being used, it may contribute to the generation of mist. This mist significantly contributes to the non-tailpipe emissions in the form of unburnt hydrocarbons (UBHCs). The problem of non-tailpipe emissions has unfortunately not been looked into so seriously, as the current stress of all automobile manufacturers is to meet the tailpipe emission legislative limits.A numerical model has been developed using finite element methods for studying the oil jet cooling of pistons and has been validated experimentally on a flat plate cooled by oil jet. Using numerical modelling, the heat transfer coefficient (h) at the underside of the piston is predicted. This predicted value of heat transfer coefficient significantly helps in selecting the correct oil type, oil jet velocity, oil jet diameter, and distance of oil nozzle from the underside of the piston. It also helps to predict whether the selected grade of oil will contribute to mist generation. Isotherms of the predicted temperature profiles in a production grade piston have been plotted.},
author = {Agarwal, A K and Varghese, M B},
doi = {10.1243/14680874JER01804},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/W{\"{a}}rme-RBen Kolben/2004{\_}Varghese{\_}Numerical investigation of piston cooling using oil jet.pdf:pdf},
issn = {1468-0874},
journal = {Int. J. Engine Res.},
number = {5},
pages = {411--421},
title = {{Numerical investigations of piston cooling using oil jet in heavy duty diesel engines}},
url = {http://journals.sagepub.com/doi/10.1243/14680874JER01804},
volume = {7},
year = {2006}
}
@article{Remarks,
author = {Remarks, Introductory},
title = {{6 Reliability Analysis}}
}
@article{Gross2011i,
author = {Gross, Dietmar and Seelig, Thomas},
doi = {10.1007/978-3-642-10196-0},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Gross, Selig 2011 - Bruchmechanik/Gross, Seelig - 2011 - BruchmechanikKap3.pdf:pdf},
isbn = {978-3-642-10195-3},
title = {{Bruchmechanik}},
url = {http://link.springer.com/10.1007/978-3-642-10196-0},
year = {2011}
}
@article{Microbiol2001,
author = {Microbiol, Food and Prot, Food and Vet, Trinidad J},
isbn = {3870701854},
number = {1991},
pages = {1174--1181},
title = {{9. Literaturverzeichnis}},
volume = {60},
year = {2001}
}
@article{Fatemi1998a,
abstract = {Fatigue damage increases with applied load cycles in a cumulative manner. Cumulative fatigue damage analysis plays a key role in life prediction of components and structures subjected to field load histories. Since the introduction of damage accumulation concept by Palmgren about 70 years ago and 'linear damage rule' by Miner about 50 years ago, the treatment of cumulative fatigue damage has received increasingly more attention. As a result, many damage models have been developed. Even though early theories on cumulative fatigue damage have been reviewed by several researchers, no comprehensive report has appeared recently to review the considerable efforts made since the late 1970s. This article provides a comprehensive review of cumulative fatigue damage theories for metals and their alloys, emphasizing the approaches developed between the early 1970s to the early 1990s. These theories are grouped into six categories: linear damage rules; nonlinear damage curve and two-stage linearization approaches; life curve modification methods; approaches based on crack growth concepts; continuum damage mechanics models; and energy-based theories. {\{}{\textcopyright}{\}}},
author = {Fatemi, A and Yang, L},
doi = {10.1016/S0142-1123(97)00081-9},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/1997{\_}Fatemi{\_}Cumulative fatigue damage and life prdeiction theories-a survey of the state of the art for homogeneous materials.pdf:pdf},
isbn = {0142-1123},
issn = {01421123},
journal = {Int. J. Fatigue},
keywords = {cumulative damage rules,cumulative fatigue damage,fatigue damage accumulation,fatigue life predictions,load interac-,tion effects},
number = {1},
pages = {9--34},
title = {{Cumulative fatigue damage and life prediction theories: a survey of the state of the art for homogeneous materials}},
url = {http://linkinghub.elsevier.com/retrieve/pii/S0142112397000819},
volume = {20},
year = {1998}
}
@article{Datei,
author = {Datei, Neue},
title = {{3 Computermaus}}
}
@article{Caton1981a,
abstract = {Because of the increasing need for precise information on engine processes, this study developed and experimentally verified models for the instantaneous heat transfer in an engine exhaust port. Experimental measurements were made of the instantaneous cylinder pressure and instantaneous exhaust gas temperature for a range of engine operating conditions. The pressure measurements were used to obtain the instantaneous cylinder gas state and the temperature measurements were used to validate the heat transfer models. The exhaust port heat transfer was dominated by jet induced large-scale fluid motion as opposed to wallshear generated fluid motion. An analysis based on the jet velocity through the valve opening correctly estimated the heat transfer due to this large-scale motion. Models for the instantaneous exhaust port heat transfer provided excellent agreement with measurements as a function of engine operating conditions. A cause d'un besoin croissant d'information pr{\{}{\'{e}}{\}}cise sur le fonctionnement d'un moteur, on d{\{}{\'{e}}{\}}veloppe une {\{}{\'{e}}{\}}tude et on v{\{}{\'{e}}{\}}rifie exp{\{}{\'{e}}{\}}rimentalement des mod{\{}{\`{e}}{\}}les sur le transfert de chaleur instantan{\{}{\'{e}}{\}} {\{}{\`{a}}{\}} l'{\{}{\'{e}}{\}}chappement d'un cylindre. Des mesures de la pression instantan{\{}{\'{e}}{\}}e dans le cylindre et de la temp{\{}{\'{e}}{\}}rature instantan{\{}{\'{e}}{\}}e {\{}{\`{a}}{\}} l'{\{}{\'{e}}{\}}chappement sont effectu{\{}{\'{e}}{\}}es pour un domaine de conditions de fonctionnement d'un moteur. Les mesures de pression permettent d'atteindre l'{\{}{\'{e}}{\}}tat instantan{\{}{\'{e}}{\}} du gaz dans le cylindre et les mesures de temp{\{}{\'{e}}{\}}rature permettent de valider les mod{\{}{\`{e}}{\}}les de transfert thermique. Le transfert {\{}{\`{a}}{\}} l'{\{}{\'{e}}{\}}chappement est domin{\{}{\'{e}}{\}} par un mouvement de jet {\{}{\`{a}}{\}} large {\{}{\'{e}}{\}}chelle au contraire du mouvement de fluide {\{}{\`{a}}{\}} frottement pari{\{}{\'{e}}{\}}tal. Une analyse bas{\{}{\'{e}}{\}}e sur la vitesse du jet {\{}{\`{a}}{\}} travers l'ouverture de la soupape pr{\{}{\'{e}}{\}}dit correctement le transfert de chaleur d{\{}{\^{u}}{\}} {\{}{\`{a}}{\}} ce mouvement {\{}{\`{a}}{\}} grande {\{}{\'{e}}{\}}chelle. Des mod{\{}{\`{e}}{\}}les pour l'{\{}{\'{e}}{\}}chappement instantan{\{}{\'{e}}{\}} fournissent un accord excellent avec des mesures pour les conditions de fonctionnement du moteur. Wegen des zunehmenden Bedarfs an genauer Information {\{}{\"{u}}{\}}ber Verbrennungsmotoren-Prozesse wurden in dieser Studie Modelle f{\{}{\"{u}}{\}}r den momentanen W{\{}{\"{a}}{\}}rme{\{}{\"{u}}{\}}bergang in einer Motor-Ausla{\$}\beta{\$}-{\{}{\"{O}}{\}}ffnung entwickelt und experimentell best{\{}{\"{a}}{\}}tigt. Die Momentanwerte des Zylinderdrucks und der Abgastemperatur wurden in Versuchen f{\{}{\"{u}}{\}}r einen ausgedehnten Betriebsbereich gemessen. Druckmessungen wurden verwendet, um den momentanen Gaszustand im Zylinder zu bestimmenn und Temperaturmessungen dienten zur Best{\{}{\"{a}}{\}}tigung der W{\{}{\"{a}}{\}}rme{\{}{\"{u}}{\}}bergangs-Modelle. Der W{\{}{\"{a}}{\}}rme{\{}{\"{u}}{\}}bergang in der Ausla{\$}\beta{\$}-{\{}{\"{O}}{\}}ffnung wurde im wesentlichen durch die strahlinduzierte Makro-Bewegung des Fluides entgegen der durch Wandschubspannung erzeugten Fluidbewegung bestimmt. Eine theoretische Untersuchung, die sich auf die Strahlgeschwindigkeit durch die Ventil{\{}{\"{o}}{\}}ffnung st{\{}{\"{u}}{\}}tzt, liefert korrekt den W{\{}{\"{a}}{\}}rme{\{}{\"{u}}{\}}bergang, hervorgerufen durch diese Makro-Bewegung. Die Modelle f{\{}{\"{u}}{\}}r den momentanen W{\{}{\"{a}}{\}}rme{\{}{\"{u}}{\}}bergang in der Ausla{\$}\beta{\$}-{\{}{\"{O}}{\}}ffnung als Funktion der Arbeitsbedingungen des Motors zeigten vorz{\{}{\"{u}}{\}}gliche {\{}{\"{U}}{\}}bereinstimmung mit den Messungen. B cвязи c вce бoлee вoзpacтaющeй нeoбчoдимocтью в тoчнoй инфopмaции o пpoцeccaч, пpoиcчoдящич в двигaтeляч, пpeдлoзeны мoдeди тeплoпepeнoca в вычлoпнoм oтвepcтии двигaтeля. Измepялиcь дaвлeниe в цилиндpe и тeмпepaтypa вычлoпнoгo гaзa пpи paздичныч peзимaч paбoты двигaтeля. Дaнныe пo дaвлeнию иcпoльзoвaлиcь для oпpeдeлeния cocтoяния гaзa в цилиндpe, a пo тeмпepaтype — для пpoвepки cпpaвeдливocти пpeдлoзeнныч мoдeлeй. Teплoпepeнoc в вычлoпнoм oтвepcтии oпpeдeляeтcя кpyпнoмacштaбными пepeмeщeниями зидкocти, вoзникaющими пpи cтpyйнoм иcтeчeнии, кoтopыe cyщecтвeннo oтличaютcя oт пepeмeщeний, вызывaeмыч нaпpязeниeм cдвигa нa cтeнкe. Aнaлиз, ocнoвaный нa cкopocти иcтeчeния cтpyи чepeз oтвepcтиe клaпaнa, пoзвoляeт кoppeктнo oцeнить вeличинy тeплoвoгo пoтoкa пpи тaкич кpyпнoмacщтaбпыч пepeмeщeнияч. Moдeли тeплoпepeнoca в вычлoпнoм oтвepcтии чopoшo coглacyютcя c peзyльтaтaми измepeний пpи paзличныч peзимaч paбoты двигaтeдя.},
author = {Caton, J A and Heywood, J B},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/1981{\_}An experimental and analytical study of heat transfer in an engine exhaust port{\_}Caton.pdf:pdf},
journal = {Int. J. Heat Mass Transf.},
number = {4},
pages = {581--595},
title = {{An experimental and analytical study of heat transfer in an engine exhaust port}},
volume = {24},
year = {1981}
}
@article{Zavala2011,
author = {Zavala, Jos{\'{e}} Carlos and Folkerts, Charles},
doi = {10.4271/2011-01-1409},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2011{\_}Zavala{\_}Knock Detection and Estimation Based on Heat Release Startegies.pdf:pdf},
title = {{Knock Detection and Estimation Based on Heat Release Strategies}},
url = {http://papers.sae.org/2011-01-1409/},
year = {2011}
}
@article{Beitz2006,
abstract = {Kap 7},
author = {Beitz and Pahl},
isbn = {9783540340607},
journal = {Konstruktionslehre},
pages = {629--688},
title = {{Entwickeln von Baureihen und Bauk{\{}{\"{a}}{\}}sten - Developing size ranges and modular products}},
year = {2006}
}
@phdthesis{Grill2006Thesis,
author = {Grill, Michael},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Injection+Combustion+Ignitionsystems/2006{\_}Grill{\_}Objektorientierte Prozessrechnung{\_}Disertation.pdf:pdf},
school = {Fakult{\"{a}}t Maschinenbau der Universit{\"{a}}t Stuttgart},
title = {{Objektorientierte Prozessrechnung von Verbrennungsmotoren}},
year = {2006}
}
@article{Rinato1995,
author = {Rinato, Infrastruktur-},
pages = {619},
title = {{Teil V}},
year = {1995}
}
@article{Sharma2002a,
abstract = {This paper illustrates the micromechanics approach to cyclic creep-fatigue damage of Pb-Sn, developed by the authors with the help of a simple case study. It is demonstrated that durability predictions can be made based solely on monotonic test data. Various parametric studies of practical interest are conducted to obtain mechanistic insights into various aspects of damage in solders e.g., effect of hydrostatic stresses, grain size, ramp rate, etc.},
author = {Sharma, Pradeep and Dasgupta, Abhijit},
doi = {10.1115/1.1493203},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Kriechen{\_}Spannungsrelaxation/2002{\_}Sharma Pradeep{\_}Micro-Mechanics of Creep-Fatigue Damage in PB-SN Solder Due to Thermal Cycling PartOne.pdf:pdf},
issn = {1043-7398},
journal = {J. Electron. Packag.},
number = {3},
pages = {298--304},
title = {{Micro-Mechanics of Creep-Fatigue Damage in PB-SN Solder Due to Thermal Cycling—Part II: Mechanistic Insights and Cyclic Durability Predictions From Monotonic Data}},
url = {http://dx.doi.org/10.1115/1.1493203{\%}5Cnhttp://electronicpackaging.asmedigitalcollection.asme.org/data/Journals/JEPAE4/26206/298{\_}1.pdf},
volume = {124},
year = {2002}
}
@article{Zienkiewicz2005a,
author = {Zienkiewicz, O},
doi = {10.1016/B978-075066431-8/50204-6},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Zienkiewicz FEM - Vol 2 Solid Structural Mechanics/63212{\_}17.pdf:pdf},
isbn = {9780750664318},
pages = {517--546},
title = {{Non-linear structural problems }},
volume = {2},
year = {2005}
}
@misc{Qi1999,
author = {Qi, Weidong and Bertram, Albrecht},
booktitle = {Int. J. Plast.},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Plasticity models/Anisotropic continuum damage modeling for single crystals at high temperatures{\_}QiAndBertram.pdf:pdf},
pages = {1197--1215},
title = {{Anisotropic continuum damage modeling for single crystals at high temperatures}},
volume = {15},
year = {1999}
}
@article{Schweizer2011,
abstract = {In this paper a mechanism-based model is presented, which is able to describe the evolution of microcracks under pure low cycle fatigue (LCF) and combined LCF and high cycle fatigue (HCF) loading conditions. In order to verify the model and to calibrate the model parameters, the crack length evolution of microcracks is followed at room temperature for pure LCF and combined LCF/HCF loading in a 10{\{}{\%}{\}}-chromium steel. These studies reveal accelerated crack growth rates under LCF/HCF interaction as soon as a critical crack length is reached. The model is capable of accounting for this effect and needs only few parameters, including the threshold for fatigue crack growth, whose knowledge is crucial for the accuracy of the model. ?? 2010 Elsevier Ltd. All rights reserved.},
author = {Schweizer, C and Seifert, T and Nieweg, B and {Von Hartrott}, P and Riedel, H},
doi = {10.1016/j.ijfatigue.2010.08.008},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/2010{\_}Schweizer+Seifert{\_}Mechanisms+Modelling of fatigue crack growth under combined low and high cycle fatigue loading.pdf:pdf},
issn = {01421123},
journal = {Int. J. Fatigue},
keywords = {Crack-tip opening displacement (CTOD),Fatigue crack growth,High cycle fatigue,Low cycle fatigue,Threshold stress intensity factor},
number = {2},
pages = {194--202},
publisher = {Elsevier Ltd},
title = {{Mechanisms and modelling of fatigue crack growth under combined low and high cycle fatigue loading}},
url = {http://dx.doi.org/10.1016/j.ijfatigue.2010.08.008},
volume = {33},
year = {2011}
}
@article{Man2009a,
abstract = {Current state and historical progress in experimental and theoretical studies of surface relief appertaining to persistent slip bands (PSBs) and leading to fatigue crack initiation in cyclically deformed metals is presented as a thorough critical overview. A comprehensive inventory of microscopic techniques used for this study is tabulated chronologically with emphasis to their applicability to polycrystals. The most relevant experimental characteristics concerning surface relief evolution, namely the form of extrusions and intrusions in single- and polycrystalline materials, are surveyed. Theoretical models and computational simulations of extrusion and intrusion formation and fatigue crack initiation are critically reviewed.},
author = {Man, J and Obrtl{\'{i}}k, K and Pol{\'{a}}k, J},
doi = {10.1080/14786430902917616},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/2009{\_}Man + Polak{\_}Extrusions and intrusions in fatigued metals Part 1 State of the art and history.pdf:pdf},
isbn = {1478-6435},
issn = {1478-6435},
journal = {Philos. Mag.},
number = {16},
pages = {1295--1336},
title = {{Extrusions and intrusions in fatigued metals. Part 1. State of the art and history†}},
url = {http://www.tandfonline.com/doi/abs/10.1080/14786430902917616},
volume = {89},
year = {2009}
}
@article{Randbedingungen,
author = {Randbedingungen, Die},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Mathematik/Funktionale{\_}Konvexitaet{\_}UniKoeln.pdf:pdf},
title = {{Variationsrechnung Kapitel 4 Die zweite Variation und Konvexit ¨ at}}
}
@article{Untersuchung,
author = {Untersuchung, Die and Konstanten, Der},
pages = {34--46},
title = {{5 Messeinrichtung}}
}
@article{Programmiersprachen,
author = {Programmiersprachen, H{\"{o}}here and Vorteil, Den},
title = {{Projekte in C gel{\"{o}}st}}
}
@article{Methode,
author = {Methode, Die Finite-elemente},
title = {{8 FE-Berechnung mit Pro / MECHANICA}}
}
@article{Transformatoren,
author = {Transformatoren, {\"{U}}bersicht},
pages = {218--248},
title = {{6 Der Transformator}}
}
@inproceedings{Rakopoulos1997Inte,
abstract = {A comprehensive transient analysis simulation model is used for the calculation of diesel engine performance under variable speed and load conditions. The analysis includes a detailed description of engine subsystems under transient conditions, thus accounting for the continuously changing character of transient operation, simulating among others the fuel injection, transient mechanical friction, heat losses to the walls and governor operation.The results of engine performance, at every time step during the transient event, are used as inputs for the formulation of thermal boundary conditions, which are needed for the calculation in a parallel way of the thermal transients propagating inside the engine structure. Two-and three-dimensional finite-element analyses were implemented for the representation of the complex geometry metal components (piston, liner, cylinder head), in a way that the temperature and heat flux variations are calculated at every point of engine structure during any transient event.An extensive set of experimental measurements was conducted on a Lister LV1, four-stroke, air-cooled, direct injection, single-cylinder diesel engine in order to test the model's validity. The most important engine variables were continuously recorded, with the aid of two on-line computers through analog-to-digital converter and sub-multiplexer cards. A satisfactory degree of agreement is found between theoretical predictions and experimental measurements under all conditions tested. Presentation of temperature distributions for the cylinder head, in the form of iso-thermal areas (thermographs), provides insight into the mechanism of heat propagation inside it. The utilization of the model also reveals the most sensitive points concerning the generation of sharp temperature excursions during the engine operating transients, which lead to higher thermal loading.},
author = {Rakopoulos, C D and Hountalas, D T and Mavropoulos, G C and Giakoumis, E G},
booktitle = {SAE Tech. Pap.},
doi = {10.4271/970634},
publisher = {SAE International},
title = {{An Integrated Transient Analysis Simulation Model Applied in Thermal Loading Calculations of an Air-Cooled Diesel Engine Under Variable Speed and Load Conditions}},
year = {1997}
}
@article{Seidl1998,
author = {Seidl, Anton L},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/{\_}buecherSong/HandbookofComposites/IV/39{\_}RepairAspectsofCompositeandAdhesivelyBondedAircraftStructures.pdf:pdf},
journal = {Compos. Struct.},
title = {{Adhesively Bonded Aircraft Structures}},
year = {1998}
}
@article{Carlo,
author = {Carlo, Monte},
title = {{2 Elasticity 2.1}}
}
@article{Grundlagen1975,
author = {Grundlagen, Kerntechnische},
title = {{5 Kernkraftwerke}},
year = {1975}
}
@article{Chen2017Structure,
author = {Chen, Xiaoqiang and Yu, Xiaoli and Lu, Yiji and Huang, Rui and Liu, Zhentao and Huang, Yuqi and Paul, Anthony},
doi = {10.1016/j.applthermaleng.2017.01.037},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Thermal Coating + Water Heat Transfer + Applikation/2017{\_}Chen{\_}Study of different cooling structures on the thermal status of an ICE.pdf:pdf},
journal = {Appl. Therm. Eng.},
keywords = {different cooling structures},
pages = {419--432},
publisher = {Elsevier Ltd},
title = {{Study of different cooling structures on the thermal status of an Internal Combustion Engine}},
volume = {116},
year = {2017}
}
@book{Watson1982,
address = {London},
author = {Watson, N and Janota, M S},
isbn = {0 333 24290 4},
publisher = {MACMILLAN PRESS LTD},
title = {{Turbocharging the Internal Combustion Engine, Higher and Further Education Division}},
year = {1982}
}
@article{Torrilhon2007a,
author = {Torrilhon, Manuel},
doi = {10.1002/theDOIsuffix},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Thermodynamik/PhasenFeld/Nestler{\_}Crack{\_}propagation{\_}on{\_}mesoscopic{\_}length{\_}scale.pdf:pdf},
journal = {Pamm},
keywords = {chemo-mechanical coupling,crack propagation,multiphase-field,phase-field},
pages = {1--2},
title = {{Stability of reduced electric arc models}},
url = {http://onlinelibrary.wiley.com/doi/10.1002/pamm.200700318/abstract},
volume = {2},
year = {2007}
}
@article{Verbrennungsgase,
author = {Verbrennungsgase, Die and Gasturbinen, Mit and Abgasturbolader, Als},
title = {{4 Gasturbinen}}
}
@article{Inc.,
author = {Inc., TreeAge Software},
journal = {TreeAge Pro 2012 User's Man.},
title = {{Kapitel 18}}
}
@article{Universit2001b,
author = {Universit, Technischen},
title = {{Technische Universit{\{}{\"{a}}{\}}t M{\{}{\"{u}}{\}}nchen Institut f{\{}{\"{u}}{\}}r Werkstoffe und Verarbeitung Forschungsgruppe Prof . Schmitt-Thomas Werkstoffgerechte Auslegung und Festigkeitsnachweis f{\{}{\"{u}}{\}}r Verbrennungsmotorkolben aus Mesophasenkohlenstoff}},
year = {2001}
}
@article{Adair1972b,
abstract = {This study first reviews, discusses, and compares existing correlations$\backslash$nfor heat transfer in reciprocating compressors and engines. Then$\backslash$nafter a discussion of the significance of obtaining accurate instantaneous$\backslash$nheat transfer data, the authors describe an experimental investigation$\backslash$nof the instantaneous heat transfer rates to the cylinder wall of$\backslash$na reciprocating refrigerating compressor. Finally, this report presents$\backslash$nan expression which correlates the time averaged data within 20{\%}.},
author = {Adair, R P and Qvale, E B and Pearson, J T},
file = {:C$\backslash$:/Users/p327208/Desktop/Promotion/Literature/Motorspezifisch/Heat Transfer Combustion Chamber/1972{\_}Adair{\_}Instantaneous Heat Transfer to the Cylinder Wall in Reciprocating compressors and engines.pdf:pdf},
journal = {Int. Compress. Eng. Conf.},
pages = {521--526},
title = {{Instantaneous heat transfer to cylinder wall in reciprocating compressors}},
year = {1972}
}
@article{Manonukul2004,
abstract = {A polycrystal plasticity finite–element model has been developed for nickel–base alloy C263. That is, a representative region of the material, containing about 60 grains, has been modelled using crystal plasticity, taking account of grain morphology and crystallographic orientation. With just a single material property (in addition to standard elastic properties), namely, the critical resolved shear stress, the model is shown to be capable of predicting correctly a wide range of cyclic plasticity behaviour in face–centred cubic nickel alloy C263. A fatigue crack initiation criterion is proposed, based simply on a critical accumulated slip. When this critical slip is achieved within the microstructure, crack initiation is taken to have occurred. The model predicts the development of persistent slip bands within individual grains with a width of ca. 10 $\mu$m. The model also predicts that crack initiation can occur preferentially at grain triple points under both low– (LCF) and high–cycle fatigue (HCF). For the case of HCF, this also corresponds to a free surface. The polycrystal plasticity model combined with the fatigue crack initiation criterion are shown to predict correctly the standard Basquin and Goodman correlations in HCF, and the Coffin–Manson correlation in LCF. The model predictions are based on just two material properties: the critical resolved shear stress and the critical accumulated slip. Just one experimental test is required to determine these properties, for a given temperature, which have been obtained for nickel alloy C263. Predictions of life for nickel alloy C263 are then made over a broad range of loading conditions covering both LCF and HCF. Good agreement with experiments is achieved, despite the simplicity of the proposed ‘two–parameter' model. A simple three–dimensional form of the model has provided an estimate of the fatigue limit for HCF crack initiation in C263.},
author = {Manonukul, A. and Dunne, F. P. E.},
doi = {10.1098/rspa.2003.1258},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2003{\_}Manonukul+Dunne{\_}High- and low-cycle fatigue crack initiation using polcrystal plasticity.pdf:pdf},
isbn = {1364-5021},
issn = {1364-5021},
journal = {Proc. R. Soc. A Math. Phys. Eng. Sci.},
keywords = {crack initiation,hcf,high-cycle fatigue,lcf,low-cycle fatigue,polycrystal plasticity},
number = {2047},
pages = {1881--1903},
title = {{High- and low-cycle fatigue crack initiation using polycrystal plasticity}},
url = {http://rspa.royalsocietypublishing.org/cgi/doi/10.1098/rspa.2003.1258},
volume = {460},
year = {2004}
}
@article{Vektoren,
author = {Vektoren, Spezielle},
pages = {46--66},
title = {{II Vektorrechnung}},
volume = {0}
}
@book{Riccardella1992b,
author = {Riccardella, PC and Deardorff, AF and Griesbach, TJ},
booktitle = {Adv. Fatigue Lifetime Predict. Tech.},
doi = {10.1520/STP1122-EB},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Advances in fatigue lifetime predictive techniques - Collection of papers/Advances in fatigue lifetime predictive techniques Part2.pdf:pdf},
isbn = {978-0-8031-1423-4},
issn = {00660558},
keywords = {FATIGUE,MONITORING,POWER PLANTS,PRESSURE VESSELS AND PIPING,THERMAL STRESSES},
pages = {460--473},
pmid = {11439068},
title = {{Advances in Fatigue Lifetime Predictive Techniques}},
url = {https://apps.webofknowledge.com/full{\_}record.do?product=UA{\&}search{\_}mode=GeneralSearch{\&}qid=11{\&}SID=Z1UxbH6jtsqo8n9kPQr{\&}page=1{\&}doc=1},
volume = {1122},
year = {1992}
}
@article{Gross2011h,
author = {Gross, Dietmar and Seelig, Thomas},
doi = {10.1007/978-3-642-10196-0},
isbn = {978-3-642-10195-3},
title = {{Bruchmechanik}},
url = {http://link.springer.com/10.1007/978-3-642-10196-0},
year = {2011}
}
@article{Zienkiewicz2005b,
author = {Zienkiewicz, O C and Taylor, R L},
doi = {http://dx.doi.org/10.1016/B978-075066431-8.50203-4},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Zienkiewicz FEM - Vol 2 Solid Structural Mechanics/63212{\_}16.pdf:pdf},
isbn = {978-0-7506-6431-8},
journal = {Finite Elem. Method Solid Struct. Mech.},
pages = {498--516},
title = {{Semi-analytical finite element processes – use of orthogonal functions and ‘ finite strip ' methods}},
year = {2005}
}
@article{Stupkiewicz2007c,
author = {Stupkiewicz, Stanis{\l}aw},
doi = {10.1007/978-3-540-49717-2_5},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Stupkievicz 2007 - Micromechanics of Contact and Interphase Layers/97165{\_}05.pdf:pdf},
isbn = {3540497161},
issn = {16137736},
journal = {Lect. Notes Appl. Comput. Mech.},
number = {30},
pages = {59--73},
title = {{Micromechanics of boundary layers}},
volume = {2006},
year = {2007}
}
@article{Stoffregen2012,
author = {Stoffregen, J.},
pages = {334--351},
title = {{Motorradtechnik}},
year = {2012}
}
@article{Takeuchi1982,
abstract = {Plastic behavior of single crystals of Cu52Zn48 alloy with the CsCl structure has been examined over a temperature range between 2 K and room temperature. Both at 4.2 K and 77 K, the operative slip plane is the twinning {\{}{\{}{\}}112{\{}{\}}{\}} plane in most orientations and it is the anti-twinning {\{}{\{}{\}}112{\{}{\}}{\}} plane only in orientations with the maximum shear stress plane close to the anti-twinning {\{}{\{}{\}}112{\{}{\}}{\}} plane. Orientation dependence of the yield stress ??mssp showed a maximum near the orientation of the slip plane transition. These results agree well with those of computer simulation of superlattice screw dislocation motion [S. Takeuchi, Phil. Mag. A 41, 541 (1980)]. Temperature and strain-rate dependences of yield stress below {\{}{\~{}}{\}}130K are essentially similar to those in bcc metals. The above results together with in situ TEM observation indicate that low temperature deformation in ??-CuZn is governed by motion of screw dislocations overcoming the Peierls potential. Activation analyses revealed that the value of exponent in the Arrhenius rate equation, ??H kT, decreases rapidly below 10 K toward zero at 0 K, showing discrepancy of the classical rate theory in the very low temperature range. ?? 1982.},
author = {Takeuchi, S and Hashimoto, T and Suzuki, K and Ichihara, M},
doi = {10.1016/0001-6160(82)90232-2},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/1958{\_}Haasen{\_}Plastic deformation of nickel single crystals at low temperatures.pdf:pdf},
isbn = {1478-6435 {\{}{\%}{\}}[ July 29, 2008},
issn = {00016160},
journal = {Acta Met.},
number = {2},
pages = {513--521},
title = {{Plastic deformation of ??-CuZn single crystals at low temperatures}},
volume = {30},
year = {1982}
}
@article{Lados2006,
abstract = {Linear elastic fracture mechanics describes the fracture behavior of materials and components that respond elastically under loading. This approach is valuable and accurate for the continuum analysis of crack growth in brittle and high strength materials; however it introduces increasing inaccuracies for low-strength/high-ductility alloys (particularly low-carbon steels and light metal alloys). In the case of ductile alloys, different degrees of plastic deformation precede and accompany crack initiation and propagation, and a non-linear ductile fracture mechanics approach better characterizes the fatigue and fracture behavior under elastic-plastic conditions. To delineate plasticity effects in upper Region II and Region III of crack growth an analysis comparing linear elastic stress intensity factor ranges (??Kel) with crack tip plasticity adjusted linear elastic stress intensity factor ranges (??Kpl) is presented. To compute plasticity corrected stress intensity factor ranges (??Kpl), a new relationship for plastic zone size determination was developed taking into account effects of plane-strain and plane-stress conditions ("combo plastic zone"). In addition, for the upper part of the fatigue crack growth curve, elastic-plastic (cyclic J based) stress intensity factor (??KJ) were computed from load-displacement records and compared to plasticity corrected stress intensity factor ranges (??Kpl). A new cyclic J analysis was designed to compute elastic-plastic stress intensity factor ranges (??KJ) by determining cumulative plastic damage from load-displacement records captured in load-control (K-control) fatigue crack growth tests. The cyclic J analysis provides the true fatigue crack growth behavior of the material. A methodology to evaluate the lower and upper bound fracture toughness of the material (JIC and Jmax) directly from fatigue crack growth test data (??KFT(JIC) and ??KFT(Jmax) was developed and validated using static fracture toughness test results. The value of ??KFT(JIC) (and implicitly JIC) is determined by comparing the plasticity corrected elastic fatigue crack growth curve with the elastic-plastic fatigue crack growth curve. A most relevant finding is that plasticity adjusted linear elastic stress intensity factor ranges (??Kpl) are in remarkably good agreement with cyclic J analysis results (??KJ), and provide accurate plasticity corrections up to a ??K corresponding to JIC(i.e. ??KFT(JIC). Towards the end of the fatigue crack growth test (above ??KFT(JIC) when plasticity is accompanied by significant tearing, the cyclic J analysis provides a more accurate way to capture the true behavior of the material and determine ??KFT(Jmax). A procedure to decouple and partition plasticity and tearing effects on crack growth rates is given. Three ca st Al-Si-Mg alloys with different levels of ductility, provided by different Si contents and heat treatments (T61 and T4) are evaluated, and the effects of crack tip plasticity on fatigue crack growth are assessed. Fatigue crack growth tests were conducted at a constant stress ratio, R = 0.1, using compact tension specimens. ?? 2005 Elsevier Ltd. All rights reserved.},
author = {Lados, Diana A and Apelian, Diran},
doi = {10.1016/j.engfracmech.2005.08.010},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/2004{\_}Lados{\_}Limitations of elastic definitions in Al–Si–Mg cast alloys with enhanced plasticity{\_}LEFM vs Elastic-plastic fracture mechan.pdf:pdf},
isbn = {0013-7944},
issn = {00137944},
journal = {Eng. Fract. Mech.},
keywords = {Elastic-plastic fracture mechanics (EPFM),Linear elastic fracture mechanics (LEFM),Lower and upper bound fracture toughness,Plane-strain/plane-stress ("combo") crack tip plas,Plasticity and tearing,Plasticity corrected linear elastic fracture mecha},
number = {4},
pages = {435--455},
title = {{Limitations of elastic definitions in Al-Si-Mg cast alloys with enhanced plasticity: Linear elastic fracture mechanics versus elastic-plastic fracture mechanics}},
volume = {73},
year = {2006}
}
@article{Merker2009,
author = {Merker, G{\"{u}}nter and Schwarz, Christian},
doi = {10.1007/978-3-8348-8306-3_17},
isbn = {9783835100800},
journal = {Grundlagen der Verbrennungsmotoren},
pages = {535--580},
title = {{Simulation der Verbrennung}},
year = {2009}
}
@article{Januszka2015a,
author = {Januszka, Marcin and Panfil, Wawrzyniec},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2016{\_}Lasocki{\_}ENGINE KNOCK DETECTION AND EVALUATION - A REVIEW.pdf:pdf},
number = {102},
pages = {37--48},
title = {{Proceedings of the institute of vehicles 2(102)/2015}},
volume = {2},
year = {2015}
}
@article{Beginn,
author = {Beginn, Zu and Aufgabe, Die},
number = {L},
title = {{7 Hydrodynamische Kupplungen und Wandler}}
}
@misc{Holzapfel2000,
abstract = {Nonlinear Solid Mechanics a Continuum Approach for Engineering Gerhard A. Holzapfel Graz University of Technology, Austria With a modern, comprehensive approach directed towards computational mechanics, this book covers a unique combination of subjects at present unavailable in any other text. It includes vital information on 'variational principles' constituting the cornerstone of the finite element method. In fact this is the only method by which Nonlinear Solid Mechanics is utilized in engineering practice. The book opens with a fundamental chapter on vectors and tensors. The following chapters are based on nonlinear continuum mechanics - an inevitable prerequisite for computational mechanicians. In addition, continuum field theory (applied to a representative sample of hyperelastic materials currently used in nonlinear computations such as incompressible and compressible materials) is presented, as are transversely isotropic materials, composite materials, viscoelastic materials and hyperelastic materials with isotropic damage. Another central chapter is devoted to the thermodynamics of materials, covering both finite thermoelasticity and finite thermoviscoelasticity. Also included are: an up-to-date list of almost 300 references and a comprehensive index useful examples and exercises for the student selected topics of statistical and continuum thermodynamics. Furthermore, the principle of virtual work (in both the material and spatial descriptions) is compared with two and three-field variational principles particularly designed to capture kinematic constraints such as incompressibility. All of the features combined result in an essential text for final year undergraduates, postgraduates and researchers in mechanical, civil and aerospace engineering and applied maths and physics.},
author = {Holzapfel, G},
booktitle = {Work},
doi = {10.1023/A:1020843529530},
isbn = {0471823198},
issn = {1572-9648},
pages = {455},
title = {{Nonlinear solid mechanics: A continuum approach for engineering}},
url = {http://www.citeulike.org/group/2006/article/1044720},
volume = {First Edit},
year = {2000}
}
@article{Clements1998,
author = {Clements, Linda L.},
doi = {10.1007/978-1-4615-6389-1_11},
isbn = {978-0-412-54020-2},
pages = {202--241},
title = {{Organic Fibers}},
year = {1998}
}
@article{Worlds2016,
author = {Worlds, Small and Attachment, Preferential and Models, Voter and Distributions, Fixed Degree and Laws, Power},
isbn = {9780511546594},
pages = {5--6},
title = {{Preface 1.}},
year = {2016}
}
@article{Hauptteila,
author = {Hauptteil, Der and Technik, Rem-kl and Mikroskopie, Rem-kl and Vordergrund, Im and Mikroskopie, Kl- and Untersuchungen, Dynamische Rem-kl and Cdte, Mit and Bestandteil, Wichtiger and Versetzungen, Material},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/Crystall Plasticity Basics/Beitrag{\_}zur{\_}Versetzungsdynamik.pdf:pdf},
pages = {59--89},
title = {{Untersuchungen zur Versetzungsdynamik}}
}
@article{Rice1969,
abstract = {The fracture of ductile solids has frequently been observed to result from the large growth and coalescence of microscopic voids, a process enhanced by the superposition of hydrostatic tensile stresses on a plastic deformation field. The ductile growth of voids is treated here as a problem in continuum plasticity. First, a variational principle is established to characterize the flow field in an elastically rigid and incompressible plastic material containing an internal void or voids, and subjected to a remotely uniform stress and strain rate field. Then an approximate Rayleigh-Ritz procedure is developed and applied to the enlargement of an isolated spherical void in a nonhardening material. Growth is studied in some detail for the case of a remote tensile extension field with superposed hydrostatic stresses. The volume changing contribution to void growth is found to overwhelm the shape changing part when the mean remote normal stress is large, so that growth is essentially spherical. Further, it is found that for any remote strain rate field, the void enlargement rate is amplified over the remote strain rate by a factor rising exponentially with the ratio of mean normal stress to yield stress. Some related results are discussed, including the long cylindrical void considered by F.A. McClintock (1968, J. appl. Mech. 35, 363), and an approximate relation is given to describe growth of a spherical void in a general remote field. The results suggest a rapidly decreasing fracture ductility with increasing hydrostatic tension.},
author = {Rice, J.R. and Tracey, D.M.},
doi = {10.1016/0022-5096(69)90033-7},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Plasticity models/On the ductile enlargement of voids in triaxial stress fields {\_}RiceAndTracey.pdf:pdf},
isbn = {0022-5096},
issn = {00225096},
journal = {J. Mech. Phys. Solids},
number = {3},
pages = {201--217},
title = {{On the ductile enlargement of voids in triaxial stress fields∗}},
url = {http://linkinghub.elsevier.com/retrieve/pii/0022509669900337},
volume = {17},
year = {1969}
}
@article{Stabilitat,
author = {Stabilit{\"{a}}t, {\"{U}}bertragungsverhalten and Stabilit{\"{a}}t, Bestimmuing Der},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Vorlesungen/Messtechnik+Regelungstechnik/gmrt04.pdf:pdf},
pages = {1--20},
title = {{Stabilit{\"{a}}t im Zeitbereich}}
}
@article{Gallus,
author = {Gallus, J{\"{u}}rgen},
journal = {Elektronik},
pages = {823--834},
title = {{C9 C9 Elektronik im Kraftfahrzeug C9 Vernetzung und Bussysteme}}
}
@article{Schie??l2003,
abstract = {We investigate spatial temperature fluctuations in the unburned endgas of a spark-ignited (SI) engine. Our approach exploits the fact that the quantities (species concentrations, temperature) comprising the state of the combustion chamber gases are not independent, but often correlate sharply. Information about spatial temperature variations is obtained indirectly by observing two complementary quantities that sensitively reflect the local temperature. Spatial formaldehyde (H2CO) concentration variations in the endgas are converted to temperature fluctuations using calculated correlations between temperature and [H2CO]. Additionally, the geometrical size of inhomogeneities is deduced from LIF-images displaying the locally varying formation of temperature-sensitive intermediate species. The results indicate that temperature fluctuations exceeding 20 K are present in the nominally homogeneous endgas. The geometrical size of these fluctuations ranges from ???1 mm to ???1 cm. ?? 2003 The Combustion Institute. All rights reserved.},
author = {Schie??l, R. and Maas, U.},
doi = {10.1016/S0010-2180(02)00538-2},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Klopfen{\_}Ottomotor/2003{\_}Schiessl{\_}Analysis of endgas temperture fluctuations in an si engine by LIF.pdf:pdf},
isbn = {4907116855653},
issn = {00102180},
journal = {Combust. Flame},
keywords = {Endgas,IC engines,Laser-induced fluorescence,Temperature fluctuations},
number = {1-2},
pages = {19--27},
title = {{Analysis of endgas temperature fluctuations in an SI engine by laser-induced fluorescence}},
volume = {133},
year = {2003}
}
@article{Berger2003a,
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Berger},
doi = {10.1002/ejoc.201200111},
eprint = {arXiv:1011.1669v3},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Vortraege/Book-of-Abstracts{\_}2016-03-04{\_}GAMM.pdf:pdf},
isbn = {9781107671812},
issn = {0196-6553},
journal = {Eng. Med. Biol. Soc. 2008. EMBS 2008. 30th Annu. Int. Conf. IEEE},
pages = {2004},
pmid = {26840611},
title = {{Table of of contents}},
volume = {24},
year = {2003}
}
@article{Stiller2006,
author = {Stiller, Christoph},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Vorlesungen/Messtechnik+Regelungstechnik/gmrt01.pdf:pdf},
issn = {02731177},
journal = {Adv. Sp. Res.},
number = {12},
pages = {2820--2823},
title = {{Grundlagen der Mess- und Regelungstechnik}},
volume = {38},
year = {2006}
}
@article{Tests,
author = {Tests, Chi-square and Tests, Nonparametric},
title = {12 12.2}
}
@book{Berger2003b,
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Berger},
booktitle = {Eng. Med. Biol. Soc. 2008. EMBS 2008. 30th Annu. Int. Conf. IEEE},
doi = {10.1002/ejoc.201200111},
eprint = {arXiv:1011.1669v3},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Vortraege/Book-of-Abstracts{\_}2016-03-04{\_}GAMM.pdf:pdf},
isbn = {9781107671812},
issn = {0196-6553},
pages = {2004},
pmid = {26840611},
title = {{Table of of contents}},
volume = {24},
year = {2003}
}
@misc{Hoischen1998,
abstract = {... Book. Title, Technisches  Zeichnen : Grundlagen, Normen, Beispiele, Darstellende Geometrie. Ein Lehr, {\"{U}}bungs und Nachschlagebuch f{\"{u}}r Schule, Umschulung, Studium und Praxis. Author(s), Hoischen , Hans (ed.) ; Hesser, Wilfried (ed.). Imprint, D{\"{u}}sseldorf : Cornelsen, 2007. ... $\backslash$n},
author = {Hoischen, Hans},
isbn = {3464480070},
pages = {123, 281--283, 294--295, 305--308},
title = {{Technisches Zeichnen - Grundlagen, Normen, Beispiele - Darstellende Geometrie}},
year = {1998}
}
@article{Adair1972,
abstract = {This study first reviews, discusses, and compares existing correlations$\backslash$nfor heat transfer in reciprocating compressors and engines. Then$\backslash$nafter a discussion of the significance of obtaining accurate instantaneous$\backslash$nheat transfer data, the authors describe an experimental investigation$\backslash$nof the instantaneous heat transfer rates to the cylinder wall of$\backslash$na reciprocating refrigerating compressor. Finally, this report presents$\backslash$nan expression which correlates the time averaged data within 20{\%}.},
author = {Adair, R P and Qvale, E B and Pearson, J T},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/1972{\_}Adair{\_}Instantaneous Heat Transfer to the Cylinder Wall in Reciprocating compressors and engines.pdf:pdf},
journal = {Int. Compress. Eng. Conf.},
pages = {521--526},
title = {{Instantaneous heat transfer to cylinder wall in reciprocating compressors}},
year = {1972}
}
@phdthesis{Hoelz2015,
author = {H{\"{o}}lz, Peter},
school = {Institute of Fusion and Reactor Technology (KIT)},
title = {{Thermische Untersuchung einer Radialturbine zur Abgasenergier{\"{u}}ckgewinnung}},
type = {Master thesis},
year = {2015}
}
@article{Desmorat2007a,
abstract = {On the idea that fatigue damage is localized at the microscopic scale, a scale smaller than the mesoscopic one of the Representative Volume Element (RVE), a three-dimensional two scale damage model has been proposed for High Cycle Fatigue applications. It is extended here to anisothermal cases and then to thermo-mechanical fatigue. The modeling consists in the micromechanics analysis of a weak micro-inclusion subjected to plasticity and damage embedded in an elastic meso-element (the RVE of continuum mechanics). The consideration of plasticity coupled with damage equations at microscale, altogether with Eshelby-Kr{\{}{\"{o}}{\}}ner localization law, allows to compute the value of microscopic damage up to failure for any kind of loading, 1D or 3D, cyclic or random, isothermal or anisothermal, mechanical, thermal or thermo-mechanical. A robust numerical scheme is proposed in order to make the computations fast. A post-processor for damage and fatigue (DAMAGE{\{}{\_}{\}}2005) has been developed. It applies to complex thermo-mechanical loadings. Examples of the representation by the two scale damage model of physical phenomena related to High Cycle Fatigue are given such as the mean stress effect, the non-linear accumulation of damage. Examples of thermal and thermo-mechanical fatigue as well as complex applications on real size testing structure subjected to thermo-mechanical fatigue are detailed. {\{}{\textcopyright}{\}} 2007 Elsevier Masson SAS. All rights reserved.},
author = {Desmorat, R and Kane, A and Seyedi, M and Sermage, J P},
doi = {10.1016/j.euromechsol.2007.01.002},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/2 scale models papers/2007{\_}Desmorat+Kane+Seyedi+Sermage{\_}Two scale damage model and related numerical issues.pdf:pdf},
isbn = {09977538},
issn = {09977538},
journal = {Eur. J. Mech. A/Solids},
keywords = {Damage,Fatigue,Post-processing,Thermomechanical loading},
number = {6},
pages = {909--935},
title = {{Two scale damage model and related numerical issues for thermo-mechanical High Cycle Fatigue}},
volume = {26},
year = {2007}
}
@article{Corti2009a,
abstract = {A detailed analysis of knocking events can help improving engine performance and diagnosis strategies. The paper aim is a better understanding of the phenomena involved in knocking combustions through the combination of CFD and signals analysis tools. CFD simulations have been used in order to reproduce knock effect on the in-cylinder pressure trace. In fact, the in-cylinder pressure signal holds information about waves propagation and heat losses: for the sake of the diagnosis it is important to relate knock severity to knock indexes values. For this purpose, a CFD model has been implemented, able to predict the combustion evolution with respect to Spark Advance, from non-knocking up to heavy knocking conditions. The CFD model validation phase is crucial for a correct representation of both regular and knocking combustions: the operation has been carried out by means of an accurate statistical analysis of experimental in-cylinder pressure data. The simulation results allow relating the combustion characteristics to their effect on the in-cylinder pressure signal. It is then possible to highlight critical issues regarding typical knock detection methodologies, while disclosing novel approaches. One of the main results is the validation of knock detection strategies based on the low-frequency content of the pressure signal. These strategies can be used together with standard high-frequency based techniques in order to improve the detection robustness.},
author = {Corti, Enrico and Forte, Claudio},
doi = {10.4271/2009-24-0019},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Klopfen{\_}Ottomotor/2009{\_}Forte+Corti+Bianchi{\_}Combination on In-Cylinder Pressure Signal Analysis and CFD Simulation for Knock Detection Purposes.pdf:pdf},
issn = {1946-3944},
journal = {SAE Int. J. Engines},
number = {2},
pages = {2009--24--0019},
title = {{Combination of In-Cylinder Pressure Signal Analysis and CFD Simulation for Knock Detection Purposes}},
url = {http://papers.sae.org/2009-24-0019/},
volume = {2},
year = {2009}
}
@article{Physik2006a,
author = {Physik, Statistische},
doi = {10.1007/3-540-29381-7},
isbn = {3-540-25629-6},
issn = {09377433},
journal = {Gerthsen Phys.},
pages = {1045--1083},
title = {{19 - Statistische Physik}},
url = {http://www.springerlink.com/index/10.1007/3-540-29381-7},
volume = {18},
year = {2006}
}
@article{WoschniCsallnerFieger1979,
author = {Woschni, G. and Csallner, P. and Fieger, J.},
file = {:C$\backslash$:/Users/p327208/Desktop/Promotion/Literature/Motorspezifisch/FVV Bericht zum Thema W{\"{a}}rme{\"{u}}bergang allg+Klopfen und zu Variation Betriebsbedingungen/190{\_}Forschungsheft-280B{\_}1980-12-31.pdf:pdf},
journal = {FVV – Vorh. Nr. 190, H. Nr. 260 1. Teilabschlussbericht},
number = {190},
title = {{W{\"{a}}rme{\"{u}}bergang und Brennverlauf im Ottomotor}},
volume = {304},
year = {1979}
}
@article{Su2002b,
abstract = {Thermal fatigue presents a new challenge in cast aluminum engine design. Accurate thermomechanical stress analysis and reliable failure criterion are the keys to a successful life prediction. It is shown that the material stress and strain behavior of cast aluminum is strongly temperature and strain rate sensitive. A unified viscoplasticity constitutive relation is thus proposed to simultaneously describe the plasticity and creep of cast aluminum components deforming at high temperatures. A fatigue failure criterion based on a damage accumulation model is introduced. Damages due to mechanical fatigue, environmental impact and creep are accounted for. The material stress and strain model and thermal fatigue model are shown to be effective in accurately capturing features of thermal fatigue by simulating a component thermal fatigue test using 3D FEA with ABAQUS and comparing the results with measured data. Copyright {\textcopyright} 2002 Society of Automotive Engineers, Inc.},
author = {Su, X and Zubeck, M and Lasecki, J and Jr, C C Engler-pinto and Tang, C and Allison, J},
doi = {10.4271/2002-01-0657},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Kriechen{\_}Spannungsrelaxation/2002{\_}Su+Zubeck{\_}Thermal fatigue analysis of cast aluminium cyclinder heads.pdf:pdf},
issn = {0148-7191},
journal = {Society},
number = {724},
title = {{Thermal Fatigue Analysis of Cast Aluminum Cylinder Heads}},
year = {2002}
}
@article{Kerbwirkunga,
author = {Kerbwirkung, Bedeutung Der},
doi = {10.1007/978-3-540-71459-0},
file = {:C$\backslash$:/Users/p327208/Desktop/Promotion/Literature/Empirical Fatigue Models + Validation/Erm{\"{u}}dungsfestigkeit{\_}Radaj/Kap4{\_}Kerbwirkung.pdf:pdf},
isbn = {978-3-540-71458-3},
title = {{4 Kerbwirkung 4.1}}
}
@article{Analysis,
author = {Analysis, Finite Element and Boundary, Contact},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Stupkievicz 2007 - Micromechanics of Contact and Interphase Layers/97165{\_}06.pdf:pdf},
journal = {Analysis},
title = {{Finite Element Analysis of Contact Boundary Layers}}
}
@article{Denton,
author = {Denton, Douglas L},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/{\_}buecherSong/HandbookofComposites/V/41{\_}LandTransportationApplication.pdf:pdf},
journal = {Composites},
title = {{Land Transportation Applications}}
}
@article{Alphabet,
author = {Alphabet, Tabelle Griechisches and Z, Realteil Von and Z, Imagin{\"{a}}rteil Von},
title = {{Tabellenanhang}}
}
@article{FONTANESI_Boiling,
abstract = {Abstract The present paper proposes a numerical methodology aiming at analyzing and optimizing an internal combustion engine water cooling jacket, with particular emphasis on the assessment of the fatigue strength of the engine head. Full three-dimensional CFD and FEM analyses of the conjugate heat transfer and of the thermo-mechanical loading cycles are presented for a single bank of a currently made V6 turbocharged Diesel engine under actual operating conditions. A detailed model of the engine, consisting of both the coolant galleries and the surrounding metal components is employed in both fluid-dynamic and structural analyses to accurately mimic the influence of the cooling system layout on the thermo-mechanical behavior of the engine. In order to assess a proper CFD setup useful for the optimization of the thermal behavior of the engine, the experimentally measured temperature distribution within the engine head is compared to the CFD forecasts. Particular attention is paid to the modeling of the phase transition and of the vapor nuclei formation within the coolant galleries. Thermo-mechanical analyses are then carried out aiming at addressing the design optimization of the engine in terms of fatigue strength. Because of the wide range of thermal and mechanical loadings acting on the engine head, both high-cycle and low-cycle fatigue are considered. An energy-based multi-axial criterion specifically suited for thermal fatigue is employed in the low-cycle fatigue region (i.e. the combustion dome) while well-established multi-axial stress/strain-based criteria are adopted to investigate the high-cycle fatigue regions of the engine head (i.e. the coolant galleries). The proposed methodology shows very promising results in terms of point-wise detection of possible engine failures and proves to be an effective tool for the accurate thermo-mechanical characterization of internal combustion engines under actual life-cycle operating conditions.},
author = {Fontanesi, Stefano and Giacopini, Matteo},
doi = {https://doi.org/10.1016/j.applthermaleng.2012.12.005},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Boiling/2013{\_}Fontanesi{\_}Multiphase CFD-CHT optimization of the cooling jacket and FEM analysis of the engine head of a V6 Diesel engine.pdf:pdf},
journal = {Appl. Therm. Eng.},
number = {2},
pages = {293--303},
title = {{Multiphase CFD CHT optimization of the cooling jacket and FEM analysis of the engine head of a V6 diesel engine}},
volume = {52},
year = {2013}
}
@article{Feldhusen,
author = {Feldhusen, J{\"{o}}rg},
pages = {2--11},
title = {{1 Einleitung}}
}
@article{Hild2015c,
abstract = {{\{}{\textcopyright}{\}} Springer Science+Business Media New York 2015.This chapter is devoted to the evaluation of damage with digital image correlation (DIC). This measurement technique provides displacement fields that can be used to tune material parameters of damage models. The potential of DIC for identification purposes is illustrated hereafter for simple 1D-type geometries in the context of quasi-brittle and ductile behaviors. Beams and frames as encountered in civil engineering application can be described through damage laws. The localization of damage at single points (lumped damage mechanics) and the resulting damage law can be determined very precisely based on dedicated versions of DIC incorporating the descriptive language of beam theory. At smaller scale, plasterboards (plaster core lined with paper) constitute another example of a structure (rather than a material), which can be described as damageable. Those cases will be analyzed in details.},
author = {Hild, Fran{\c{c}}ois and Roux, St{\'{e}}phane},
doi = {10.1007/978-1-4614-5589-9},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/2015{\_}Sun+Liu{\_}Particel-Debonding modeling of metal-matrix composites.pdf:pdf},
isbn = {9781461455899},
journal = {Handb. Damage Mech. Nano to Macro Scale Mater. Struct.},
pages = {1277--1299},
title = {{Evaluating damage with digital image correlation: b. from physical to mechanical damage}},
year = {2015}
}
@article{Shojaefard2005a,
author = {Shojaefard, M H and Noorpoor, A R and Bozchaloe, D A and Ghaffarpour, M},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Heat transfer intake+exhaust system/2005{\_}Shojaefard+Noorpoor{\_}Transient Thermal Analysis of Engine Exhaust Valve.pdf:pdf},
journal = {Numer. Heat Transf. Part A Appl.},
number = {7},
pages = {627--644},
title = {{Transient Thermal Analysis of Engine Exhaust Valve}},
volume = {48},
year = {2005}
}
@article{ConferenceonFatigueMechanisms:AdvancesinQuantitativeMeasurementofPhysicalDamage1983,
author = {{Conference on Fatigue Mechanisms: Advances in Quantitative Measurement of Physical Damage}},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/1983{\_}Lankford{\_}Fatigue Mechanisms Advances in quantitative   meausrements of physical damage.pdf:pdf},
issn = {10403094},
journal = {Stp 811},
keywords = {An{\'{a}}lise quantitativa,Congresso,Dano f{\'{i}}sico,Fadiga de materiais},
pages = {496},
title = {{Fatigue mechanisms advances in quantitative measurement of physical damage {\textless}{\textless}a{\textgreater}{\textgreater} conference}},
year = {1983}
}
@article{Reifen1972,
author = {Reifen, Der Entwicklungsprozess and Reifen, Die and Beispiel, Am and Fahrzeughersteller, Jeder and Beispiel, Zum and Fahrzeuge, Mercedes-benz and Erstausr, Diese},
pages = {1--4},
title = {{1 Einleitung}},
year = {1972}
}
@article{Industrie,
author = {Industrie, Die and Bem, Viele and Gewichts-, Die and Schwerpunkt, Der and Grenzbedingungen, Als},
pages = {297--305},
title = {{13 Bauteiloptimierung}}
}
@article{Schwan1998,
author = {Schwan, F J},
journal = {Design},
title = {{Design of structure with composites 31}},
year = {1998}
}
@article{Klein2012,
author = {Klein, B},
doi = {10.1007/978-3-8348-2134-8},
isbn = {9783834821348},
pages = {89--92},
title = {{6 Wahl der Ansatzfunktionen}},
year = {2012}
}
@article{Fatemi1998,
abstract = {Fatigue damage increases with applied load cycles in a cumulative manner. Cumulative fatigue damage analysis plays a key role in life prediction of components and structures subjected to field load histories. Since the introduction of damage accumulation concept by Palmgren about 70 years ago and 'linear damage rule' by Miner about 50 years ago, the treatment of cumulative fatigue damage has received increasingly more attention. As a result, many damage models have been developed. Even though early theories on cumulative fatigue damage have been reviewed by several researchers, no comprehensive report has appeared recently to review the considerable efforts made since the late 1970s. This article provides a comprehensive review of cumulative fatigue damage theories for metals and their alloys, emphasizing the approaches developed between the early 1970s to the early 1990s. These theories are grouped into six categories: linear damage rules; nonlinear damage curve and two-stage linearization approaches; life curve modification methods; approaches based on crack growth concepts; continuum damage mechanics models; and energy-based theories. {\{}{\textcopyright}{\}}},
author = {Fatemi, A and Yang, L},
doi = {10.1016/S0142-1123(97)00081-9},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/1997{\_}Fatemi{\_}Cumulative fatigue damage and life prdeiction theories-a survey of the state of the art for homogeneous materials.pdf:pdf},
isbn = {0142-1123},
issn = {01421123},
journal = {Int. J. Fatigue},
keywords = {cumulative damage rules,cumulative fatigue damage,fatigue damage accumulation,fatigue life predictions,load interac-,tion effects},
number = {1},
pages = {9--34},
title = {{Cumulative fatigue damage and life prediction theories: a survey of the state of the art for homogeneous materials}},
url = {http://linkinghub.elsevier.com/retrieve/pii/S0142112397000819},
volume = {20},
year = {1998}
}
@article{Maere2012,
author = {Maere, Steven and Biology, Course Computational},
doi = {10.1002/wsbm.033},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Zienkiewicz FEM - Vol 2 Solid Structural Mechanics/63212{\_}18.pdf:pdf},
number = {December},
title = {{Multiscale modelling}},
year = {2012}
}
@article{Pebzy1998,
author = {Pebzy, Harry E},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/{\_}buecherSong/HandbookofComposites/IV/40{\_}ReuseandDisposal.pdf:pdf},
journal = {Perspective},
keywords = {treated waste wood, disposal, reuse, recycle, inci},
title = {{Reuse and disposal}},
year = {1998}
}
@article{Results1994,
abstract = {As a concluding comment, I should like to return to the point raised by Ayres, that it is not enough simply to tell a better version of the fourth-century history in the expectation that modern theologians will finally get it straight! This is a valid point: if we want to have Christianity's fourth-century heritage taken seriously, we need to be in dialogue with modern writers. But, if there is to be a dialogue, both sides must be allowed to speak, and so we are also responsible for expounding the historical material on its own terms. As Heidegger put it, “[O]nly when we think through what has been thought will we be of any use for what must still be thought.” Perhaps studying the figures from a distant era will open up for us possibilities we would never have dreamed of within our own modern presuppositions, so that we can recognize differences even beyond those which lie within our own horizon or tradition. If I am right in affirming that there is a different style of doing theology prior to Augustine and after him in the East than that which we find in the theological and scholarly tradition in which Ayres's book stands, then we must ask whether we need to address the question of the legitimacy of each (and ponder how one might even answer that) or whether a plurality of approaches is possible without reducing one to the other. In a way, this would be a further step toward deconstructing monolithic notions of “Orthodoxy” in recognition of genuine and legitimate diversity within early Christianity and among modern Christians. Might it be better not to speak of Nicaea and its legacy, but of the legacies of Nicaea—or better—“Christ and him crucified” (2 Cor 2:2) and the ways in which Nicaea and its interpreters affirm the true divinity of this one?},
author = {Results, Useful},
doi = {10.1007/BF02600226},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2010{\_}Jaroslav Pokluda+Pavel {\v{S}}andera{\_}Micromechanisms of fracture and fatigue{\_}Buch/Kap5{\_}FinalReflection.pdf:pdf},
isbn = {9780470434673},
issn = {08848734},
journal = {J. Gen. Intern. Med.},
number = {3 Supplement},
pages = {243--247},
title = {{Final reflections}},
volume = {9},
year = {1994}
}
@article{Prileschajew1947,
author = {Prileschajew, N and Greenlee, S O},
title = {{Epoxy Resins}},
year = {1947}
}
@article{ReviewPeter2017,
author = {H{\"{o}}lz, Peter and B{\"{o}}hlke, Thomas and Kr{\"{a}}mer, Thomas},
number = {Submitted},
title = {{Dimensional analysis and turbulent heat transfer: A reconsideration of thermal boundary conditions for internal combustion engines}}
}
@article{Bockh2006b,
abstract = {Bei erzwungener Konvektion wird der W{\"{a}}rme{\"{u}}bergang durch die Temperaturunter- schiede und die Str{\"{o}}mung, die durch eine {\"{a}}u{\ss}ere Druckdifferenz aufrechterhalten wird, bestimmt. Die Druckdifferenz kann z. B. durch eine Pumpe oder einen H{\"{o}}henunterschied erzeugt werden. Erzwungene Konvektion ist die in der Technik am h{\"{a}}u- figsten vorkommende W{\"{a}}rme{\"{u}}bergangsart. In W{\"{a}}rme{\"{u}}bertragern wird zwischen zwei Fluiden, die durch eine Wand getrennt sind, W{\"{a}}rme ausgetauscht. Unsere Aufgabe wird sein, die W{\"{a}}rme{\"{u}}bergangszahlen in Abh{\"{a}}ngigkeit von den Str{\"{o}}mungsbedingungen, den Temperaturen und der Geometrie des W{\"{a}}rme{\"{u}}bertragers zu bestimmen.},
author = {B{\"{o}}ckh, Peter},
doi = {10.1007/3-540-31433-4_3},
isbn = {978-3-540-31433-2},
journal = {W{\"{a}}rme{\"{u}}bertragung Grundlagen und Prax.},
keywords = {Engineering},
pages = {73--109},
title = {{Erzwungene Konvektion}},
url = {http://dx.doi.org/10.1007/3-540-31433-4{\_}3},
year = {2006}
}
@article{N.Chawla2007,
author = {N.Chawla, K.K. Chawla},
isbn = {9780387233062},
title = {{Metal Matrix Composites}},
year = {2007}
}
@article{Torquato1997,
abstract = {The problem of determining exact expressions for the effective stiffness tensor macroscopically anisotropic, two-phase composite media of arbitrary microstructure in arbitrary space dimension d is considered. We depart from previous treatments by introducing an integral equation for the “cavity” strain field. This leads to new, exact series expansions for the effective stiffness tensor of macroscopically anisotropic, ddimensional, two-phase composite media in powers of the “elastic polarizabilities”. The nth-order tensor coefficients of these expansions are explicitly expressed as absolutely convergent integrals over products of certain tensor fields and a determinant involving n-point correlation functions that characterize the microstructure. For the special case of macroscopically isotropic media, these series expressions may be regarded as expansions that perturb about the optimal structures that realize the Hashin-Shtrikman bounds (e.g. coated-inclusion assemblages or finite-rank laminates). Similarly, for macroscopically anisotropic media, the series expressions may be regarded as expansions that perturb about optimal structures that realize Willis' bounds. For isotropic multiphase composites, we remark on the behavior of the effective moduli as the space dimension d tends to infinity.},
author = {Torquato, S},
doi = {10.1016/S0022-5096(97)00019-7},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/Strukturmechanik MMS/Literatur/Torquato 1997.pdf:pdf},
isbn = {0022-5096},
issn = {00225096},
journal = {J. Mech. Phys. Solids},
keywords = {a,anisotropic material,b,elastic material,inhomogeneous material,microstructures},
number = {9},
pages = {1421--1448},
title = {{Effective stiffness tensor of composite media—I. Exact series expansions}},
volume = {45},
year = {1997}
}
@article{Rangarajan2012a,
abstract = {We describe a method for discretizing planar C2-regular domains immersed in non-conforming triangulations. The method consists in constructing mappings from triangles in a background mesh to curvilinear ones that conform exactly to the immersed domain. Constructing such a map relies on a novel way of parameterizing the immersed boundary over a collection of nearby edges with its closest point projection. By interpolating the mappings to curvilinear triangles at select points, we recover isoparametric mappings for the immersed domain defined over the background mesh. Indeed, interpolating the constructed mappings just at the vertices of the background mesh yields a fast meshing algorithm that involves only perturbing a few vertices near the boundary. For the discretization of a curved domain to be robust, we have to impose restrictions on the background mesh. Conversely, these restrictions define a family of domains that can be discretized with a given background mesh. We then say that the background mesh is a universal mesh for such a family of domains. The notion of universal meshes is particularly useful in free/moving boundary problems because the same background mesh can serve as the universal mesh for the evolving domain for time intervals that are independent of the time step. Hence it facilitates a framework for finite element calculations over evolving domains while using a fixed background mesh. Furthermore, since the evolving geometry can be approximated with any desired order, numerical solutions can be computed with high-order accuracy. We demonstrate these ideas with various numerical examples.},
archivePrefix = {arXiv},
arxivId = {1201.4903},
author = {Rangarajan, Ramsharan and Lew, Adrian J},
doi = {10.1002/nme},
eprint = {1201.4903},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/2010{\_}Miehe{\_}Thermodynamically consistent phase-field models of fracture-Variational principles and multi field FE implementations.pdf:pdf},
keywords = {coupled multi-field problems,crack propagation,finite elements,fracture,gradient-type damage,incremental variational,phase-fields,principles},
number = {March},
pages = {1273--1311},
title = {{Universal Meshes: A new paradigm for computing with nonconforming triangulations}},
url = {http://arxiv.org/abs/1201.4903},
year = {2012}
}
@article{Wirkprinzip,
author = {Wirkprinzip, Aufgaben},
title = {8 8.1.2}
}
@article{Kleinb,
author = {Klein, Bernd},
isbn = {9783834802965},
title = {{Aus dem Programm Maschinenelemente und}}
}
@article{Zahoransky2013c,
author = {Zahoransky, Richard a. and Allelein, Hans-Josef and Schelling, Udo and Schwarz, Harald and Bollin, Elmar and Oehler, Helmut},
doi = {10.1007/978-3-8348-2279-6},
isbn = {978-3-8348-1869-0},
journal = {Energietechnik - Syst. zur Energieumwandlung},
pages = {327--349},
title = {{13 Windenergie}},
url = {http://www.springerlink.com/index/10.1007/978-3-8348-2279-6},
year = {2013}
}
@article{Hettinger2009b,
abstract = {It is a well known fact that indicated efficiency of a SI engine at WOT is predominantly limited by knock occurrence. Therefore many investigations have been carried out to avoid knocking. Considering the further development of downsized engines knocking will also pose a greater challenge. Not only knocking but also irregular combustion in general will require further investigation in supercharged SI eingines. Premature ignition, for instance, hasn't yet been completely understood and therefore limits the low end torque of supercharged SI engines.The purpose of this paper is to introduce different analysis methods which allow to identify the knock onset and the knocking zones in the combustion chamber. In addition to established methods new techniques have been developed to account for the complex nature of pressure oscillation during knocking combustion.Experimental data was acquired on a single cylinder research engine to validate the methodology using six pressure transducers.},
author = {Hettinger, Alexander and Kulzer, Andr{\'{e}}},
doi = {10.4271/2009-01-0698},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2009{\_}Hettinger+Kulzer{\_}A new method to detect Knocking Zones.pdf:pdf},
isbn = {2009010698},
issn = {1946-3944},
journal = {SAE Int. J. Engines},
number = {1},
pages = {698--2009},
title = {{A New Method to Detect Knocking Zones}},
url = {http://papers.sae.org/2009-01-0698/},
volume = {2},
year = {2009}
}
@article{Inc.,
author = {Inc., TreeAge Software},
journal = {TreeAge Pro 2012 User's Man.},
title = {{Kapitel 18}}
}
@article{Loubar2005c,
abstract = {This paper deals with the transient thermal signal around an engine cylinder in order to propose a new and nonintrusive method of knock detection. Numerical simulations of unsteady heat transfer through the cylinder and inside the coolant flow are carried out to account for heat flux variations due to normal and knocking combustion. The effect of rib roughened surfaces on thermal signal amplification is investigated. The geometric parameters are fixed at Pi/h=70 and w/h=1 with a Reynolds number based on hydraulic diameter of 12,000. The results reveal that square ribs give better performance in term of thermal signal amplification within the fluid. An amplification of the temperature variation up to 20 times higher is found. Finally, flow analysis shows that amplification depends on the position where the thermal signal is collected.},
author = {Loubar, Khaled and Bellettre, Jérôme and Tazerout, Mohand},
doi = {10.1115/1.1857943},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2005{\_}Loubar{\_}Unsteady Heat Transfer enhancement around an engine cylinder in order to detect knockpdf.pdf:pdf},
isbn = {0022-1481},
issn = {00221481},
journal = {J. Heat Transfer},
number = {3},
pages = {278},
title = {{Unsteady Heat Transfer Enhancement Around an Engine Cylinder in Order to Detect Knock}},
url = {http://heattransfer.asmedigitalcollection.asme.org/article.aspx?articleid=1447711},
volume = {127},
year = {2005}
}
@article{Kress2004,
author = {Kress, Gerald},
journal = {Cent. Struct. Technol. ETHZ},
pages = {1--124},
title = {{Strukturanalyse mit FEM}},
url = {http://www.structures.ethz.ch/education/master/analysis/Skript/FEM{\%}7B{\_}{\%}7DD{\%}7B{\_}{\%}7DMain{\%}7B{\_}{\%}7D2009.pdf},
year = {2004}
}
@article{Kanchanomai2007a,
abstract = {Fatigue cracking due to traffic load is a major factor in road damage. Therefore, durability and lifetime prediction of roads plays a substantial role for road maintenance and cost planning. This paper reports a study of fatigue crack performance of solid asphalt and asphalt-asphalt interfaces by means of the wedge-splitting test. Instead of beams and the three- or four-point bending test, the wedge splitting method was used for the first time to observe crack growth on bituminous drilling cores. Samples of solid asphalt and samples with asphalt-interfaces were tested. One group of asphalt interfaces was untreated and the other was sandblasted before spreading the top layer during manufacturing. Due to the temperature dependency of material properties of asphalt, the tests were performed in a compact climate chamber at -10, 0 and + 10(' The challenge of determining the crack length and the crack tip were detected with an optical measurement system and picture analysis after testing. The results prove that the wedge splitting method is a highly practicable and repeatable method for crack growth testing of bituminous materials.},
author = {Kanchanomai, C and Mutoh, Y},
doi = {10.1111/j.1460-2695.2006.01088.x},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/1979{\_}Kung+Fine{\_}Fatigue crack initiation and microcrack growth in 2024-T4 and 2124-T4 Alu alloy.pdf:pdf},
issn = {8756758X},
journal = {Eng. Fract. Mech.},
keywords = {fatigue crack growth,fatigue crack initiation,lead free,low cycle fatigue},
number = {5},
pages = {443--457},
title = {{Fatigue crack initiation and growth in solder alloys}},
url = {http://doi.wiley.com/10.1111/j.1460-2695.2006.01088.x},
volume = {30},
year = {2007}
}
@article{Haghighat2018,
author = {Haghighat, Arya K and Roumi, Soheil and Madani, Navid and Bahmanpour, Davoud and Olsen, Michael G},
doi = {10.1016/j.applthermaleng.2017.08.102},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Thermal Coating + Water Heat Transfer + Applikation/2018{\_}Haghighat{\_}An intelligent cooling system and control model for improved engine thermal management.pdf:pdf},
journal = {Appl. Therm. Eng.},
keywords = {intelligent cooling system},
pages = {253--263},
publisher = {Elsevier Ltd},
title = {{An intelligent cooling system and control model for improved engine thermal management}},
volume = {128},
year = {2018}
}
@book{Riccardella1992a,
author = {Riccardella, PC and Deardorff, AF and Griesbach, TJ},
booktitle = {Adv. Fatigue Lifetime Predict. Tech.},
doi = {10.1520/STP1122-EB},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Advances in fatigue lifetime predictive techniques - Collection of papers/Advances in fatigue lifetime predictive techniques Part3.pdf:pdf},
isbn = {978-0-8031-1423-4},
issn = {00660558},
keywords = {FATIGUE,MONITORING,POWER PLANTS,PRESSURE VESSELS AND PIPING,THERMAL STRESSES},
pages = {460--473},
pmid = {11439068},
title = {{Advances in Fatigue Lifetime Predictive Techniques}},
url = {https://apps.webofknowledge.com/full{\_}record.do?product=UA{\&}search{\_}mode=GeneralSearch{\&}qid=11{\&}SID=Z1UxbH6jtsqo8n9kPQr{\&}page=1{\&}doc=1},
volume = {1122},
year = {1992}
}
@article{Erm,
author = {Erm, Unter and Beanspruchungsablauf, Der and Versagenskriterium, Als and Vorgehensweise, Diese and Vorgaben, Den and Erweiterungen, Notwendige},
file = {:C$\backslash$:/Users/p327208/Desktop/Promotion/Literature/Empirical Fatigue Models + Validation/Erm{\"{u}}dungsfestigkeit{\_}Radaj/Kap2{\_}Schwingfestigkeit.pdf:pdf},
title = {{2 Schwingfestigkeit 2.1}}
}
@book{Schade2006,
author = {Schade, Heinz and Neemann, Klaus},
isbn = {3110147416},
pages = {398},
title = {{Tensoranalysis}},
url = {http://www.amazon.de/dp/3110147416},
year = {2006}
}
@article{Tschirschwitza,
author = {Tschirschwitz, Christian},
journal = {Asphalt},
pages = {653--663},
title = {{B6 B6 Unf{\{}{\"{a}}{\}}lle mit Kleintransportern B6}}
}
@article{Festk2006,
author = {Festk, Makromolekulare},
journal = {Gerthsen Phys.},
pages = {883--967},
title = {{17 - Festk{\"{o}}rperphysik}},
year = {2006}
}
@article{Gurson1977c,
abstract = {Widely used constitutive laws for engineering materials assume plastic incompressibility, and no effect on yield of the hydrostatic component of stress. However, void nucleation and growth (and thus bulk dilatancy) are commonly observed is some processes which are characterized by large local plastic flow, such as ductile fracture.},
author = {Gurson, A. L.},
doi = {10.1115/1.3443401},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Plasticity models/Continuum Theory of Ductile Rupture by Void Nucleation and Growth-PartI{\_}ByGurson.pdf:pdf},
isbn = {0094-4289},
issn = {00944289},
journal = {J. Eng. Mater. Technol.},
number = {1},
pages = {2},
title = {{Continuum Theory of Ductile Rupture by Void Nucleation and Growth: Part I—Yield Criteria and Flow Rules for Porous Ductile Media}},
url = {http://materialstechnology.asmedigitalcollection.asme.org/article.aspx?articleid=1422194},
volume = {99},
year = {1977}
}
@article{Beanspruchungsablaufa,
author = {Beanspruchungsablauf, Der},
file = {:C$\backslash$:/Users/p327208/Desktop/Promotion/Literature/Empirical Fatigue Models + Validation/Erm{\"{u}}dungsfestigkeit{\_}Radaj/Kap5{\_}Betriebsfestigkeit.pdf:pdf},
title = {{5 Betriebsfestigkeit 5.1}}
}
@article{Rahmen,
author = {Rahmen, Im and Zeichnungsvorlagen, Bauteile and Verlauf, Im},
journal = {Pro-Engineer Prakt.},
pages = {25--30},
title = {{3 Aufgabenstellungen}}
}
@article{Sangid2011a,
abstract = {In many engineering applications, fatigue is the dominant failure mechanism governing the life of a component. Thus, many studies have focused on this phenomenon, although there is a need for a model that addresses fatigue based on the material's microstructure, specifically the energetics of the grain boundaries (GBs) and persistent slip bands (PSBs). Our approach is to model the energy of a PSB structure and use its stability with respect to dislocation motion as our failure criterion for fatigue crack initiation. The components that contribute to the energy of the PSB are identified, namely the stress field resulting from the applied external forces, dislocation pile-ups and work-hardening of the material is calculated at the continuum scale. Further, energies for dislocations creating slip in the matrix/precipitates, interacting with the GBs and nucleating/agglomerating within the PSB are computed via molecular dynamics. The results of our simulations on the stability of a PSB produce the correct fatigue crack initiation trends for the grain size, grain orientation, character of the GB, precipitate volume fraction and applied strain. From this information, we see that distinct GBs act as strong barriers to slip and increase the fatigue strength of the material. ?? 2010 Acta Materialia Inc. Published by Elsevier Ltd. All rights reserved.},
author = {Sangid, Michael D. and Maier, Hans J. and Sehitoglu, Huseyin},
doi = {10.1016/j.actamat.2010.09.036},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2010{\_}Sehitoglu{\_}A physically based fatigue model for prediction of crack initiation from persistent slip bands in polycrystals.pdf:pdf},
isbn = {1359-6454},
issn = {13596454},
journal = {Acta Mater.},
keywords = {Coincidence site lattice (CSL),Crack initiation,Fatigue,Grain boundaries,Persistent slip bands},
number = {1},
pages = {328--341},
publisher = {Acta Materialia Inc.},
title = {{A physically based fatigue model for prediction of crack initiation from persistent slip bands in polycrystals}},
url = {http://dx.doi.org/10.1016/j.actamat.2010.09.036},
volume = {59},
year = {2011}
}
@article{Tschirschwitzb,
author = {Tschirschwitz, Christian and Dre{\ss}ler, Jan},
pages = {741--754},
title = {{B12 B12 Beispiele zu Insassenverletzungen Beweissicherung und Rekonstruktion von Stra{\ss}enverkehrsunf{\"{a}}llen mit unklarer Sitzposition B12}}
}
@book{Gross2011d,
author = {Gross, Dietmar and Seelig, Thomas},
doi = {10.1007/978-3-642-10196-0},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Gross, Selig 2011 - Bruchmechanik/Gross, Seelig - 2011 - BruchmechanikKap4.pdf:pdf},
isbn = {978-3-642-10195-3},
title = {{Bruchmechanik}},
url = {http://link.springer.com/10.1007/978-3-642-10196-0},
year = {2011}
}
@article{Enomoto1985,
author = {Enomoto, Yoshiteru and Furuhama, Shoichi and Minakami, Koh},
doi = {https://doi.org/10.1299/jsme1958.28.647},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/1985{\_}Enomoto{\_}Heat Loss to Combustion Chamber Wall of 4-Stroke Gasoline Engine - Heat Loss to Piston and Cylinder.pdf:pdf},
journal = {Bull. JSME},
number = {238},
pages = {647--655},
title = {{Heat Loss to Combustion Chamber Wall of 4-Stroke Gasoline Engine: 1st Report, Heat Loss to Piston and Cylinder}},
volume = {28},
year = {1985}
}
@article{Zienkiewicz2014a,
author = {Zienkiewicz, O.C. and Taylor, R.L. and Fox, David},
doi = {10.1016/B978-1-85617-634-7.00025-9},
journal = {Finite Elem. Method Solid Struct. Mech.},
pages = {597--603},
title = {{Isoparametric Finite Element Approximations}},
url = {http://linkinghub.elsevier.com/retrieve/pii/B9781856176347000259},
year = {2014}
}
@article{Pokluda2010b,
author = {Pokluda, Jaroslav and Andera, Pavel},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2010{\_}Jaroslav Pokluda+Pavel {\v{S}}andera{\_}Micromechanisms of fracture and fatigue{\_}Buch/Kap3{\_}BrittleAndDuctileFracture.pdf:pdf},
journal = {Micromechanisms Fract. Fatigue},
pages = {69--123},
title = {{Brittle and Ductile Fracture}},
year = {2010}
}
@article{Kontinuumsmechanik2013,
author = {Kontinuumsmechanik, Grundlagen D E R},
number = {November},
pages = {1--46},
title = {{Prozesssimulation in Der Einf{\{}{\"{u}}{\}}hrung in Die Mathematischen}},
year = {2013}
}
@article{Ermittlung,
author = {Ermittlung, Die and Charakterisierung, Die and Charakterisierung, Zur},
title = {{5 Me{\{}{\ss}{\}}fehler}}
}
@article{Weidert1914,
author = {Weidert, F.},
doi = {10.1007/978-3-662-25847-7},
isbn = {978-3-662-23748-9},
pages = {1--104},
title = {{Entwicklung und Konstruktion der Unterseeboots-Sehrohre}},
url = {http://link.springer.com/10.1007/978-3-662-25847-7},
year = {1914}
}
@article{Atherosklerose2000,
author = {Atherosklerose, Die},
pages = {7--19},
title = {{1. Einleitung}},
year = {2000}
}
@inproceedings{Yang2000,
author = {Yang, L C and Hamada, A and Ohtsubo, K},
booktitle = {SAE Tech. Pap. 2000-01-0564},
doi = {https://doi.org/10.4271/2000-01-0564},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Heat transfer intake+exhaust system/2000{\_}Yang+Hamada{\_}Engine Valve Temperature Simulation System.pdf:pdf},
publisher = {SAE International},
title = {{Engine Valve Temperature Simulation System}},
year = {2000}
}
@article{Adair1972a,
abstract = {This study first reviews, discusses, and compares existing correlations{\$}\backslash{\$}nfor heat transfer in reciprocating compressors and engines. Then{\$}\backslash{\$}nafter a discussion of the significance of obtaining accurate instantaneous{\$}\backslash{\$}nheat transfer data, the authors describe an experimental investigation{\$}\backslash{\$}nof the instantaneous heat transfer rates to the cylinder wall of{\$}\backslash{\$}na reciprocating refrigerating compressor. Finally, this report presents{\$}\backslash{\$}nan expression which correlates the time averaged data within 20{\{}{\%}{\}}.},
author = {Adair, R P and Qvale, E B and Pearson, J T},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/1972{\_}Adair{\_}Instantaneous Heat Transfer to the Cylinder Wall in Reciprocating compressors and engines.pdf:pdf},
journal = {Int. Compress. Eng. Conf.},
pages = {521--526},
title = {{Instantaneous heat transfer to cylinder wall in reciprocating compressors}},
year = {1972}
}
@article{Mutzke2016,
abstract = {{\{}{\textcopyright}{\}} 2016 SAE International.Knocking combustion places a major limit on the performance and efficiency of spark ignition engines. Spontaneous ignition of the unburned air-fuel mixture ahead of the flame front leads to a rapid release of energy, which produces pressure waves that cause the engine structure to vibrate at its natural frequencies and produce an audible 'pinging' sound. In extreme cases of knock, increased temperatures and pressures in the cylinder can cause severe engine damage. Damage is thought to be caused by thermal strain effects that are directly related to the heat flux. Since it will be the maximum values that are potentially the most damaging, then the heat flux needs to be measured on a cycle-by-cycle basis. Previous work has correlated heat flux with the pressure fluctuations on an average basis, but the work here shows a correlation on a cycle-by-cycle basis. The in-cylinder pressure and surface temperature were measured using a pressure transducer and eroding-type thermocouple. These sensors were installed side-by-side at the surface of the cylinder in order to investigate the relationship between knock and heat flux on a cycle-by-cycle basis. A finite difference method was implemented to solve the one-dimensional unsteady heat conduction equation and calculate the temperature distribution away from the surface of the combustion chamber, and thus the instantaneous heat flux. The knock intensity was varied by controlling the fuel quality, compression ratio, ignition timing and air-fuel ratio. The measured heat flux was compared with pressure-based knock indices and it was found that as knock intensity increases, the correlation with peak heat flux became stronger. Results from different fuels and engine operating conditions did not collapse onto the same trend line. At higher speeds and higher compression ratios the heat flux was higher at a given level of knock intensity. The co-location of the pressure transducer and heat flux sensor meant that a correlation was found on a cycle-by-cycle basis.},
author = {Mutzke, J and Scott, B and Stone, R and Williams, J},
doi = {10.4271/2016-01-0700},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2016{\_}Mutzke{\_}The Effect of Combustion Knock on the Instantaneous Heat Flux in Spark Ignition Engines.pdf:pdf},
journal = {SAE Tech. Pap.},
title = {{The Effect of Combustion Knock on the Instantaneous Heat Flux in Spark Ignition Engines}},
volume = {2016-April},
year = {2016}
}
@article{Fertigungsverfahren,
author = {Fertigungsverfahren, Fertigungsverfahren and Folgenden, Im},
pages = {172--227},
title = {{4 Verarbeitungsmethoden}}
}
@article{Wakisaka2016,
abstract = {The reduction of the heat loss from the in-cylinder gas to the combustion chamber wall is one of the key technologies for improving the thermal efficiency of internal combustion engines. This paper describes an experimental verification of the “temperature swing” insulation concept, whereby the surface temperature of the combustion chamber wall follows that of the transient gas. First, we focus on the development of “temperature swing” insulation materials and structures with the thermo-physical properties of low thermal conductivity and low volumetric heat capacity. Heat flux measurements for the developed insulation coating show that a new insulation material formed from silica-reinforced porous anodized aluminum (SiRPA) offers both heat-rejecting properties and reliability in an internal combustion engine. Furthermore, a laser-induced phosphorescence technique was used to verify the temporal changes in the surface temperature of the developed insulation coating. This was found to quickly rise during the combustion stroke and then drop during the expansion stroke. Second, a SiRPA coating was formed over the entire surface of the diesel piston cavity, and the thermal efficiency and the heat-loss reduction were investigated for a single-cylinder direct-injection (DI) diesel engine with a bore of 86 mm and a stroke of 96 mm. An energy balance analysis showed that the SiRPA coating achieves heat loss reduction by means of heat rejection and an increase in not only the exhaust energy but also the piston work, which increases the thermal efficiency.},
author = {Wakisaka, Yoshifumi and Inayoshi, Minaji and Fukui, Kenji and Kosaka, Hidemasa and Hotta, Yoshihiro and Kawaguchi, Akio and Takada, Noriyuki},
doi = {https://doi.org/10.4271/2016-01-0661},
file = {:E$\backslash$:/UNVERS{\~{}}1/PROMOT{\~{}}3/LITERA{\~{}}1/MOTORS{\~{}}1/THERMA{\~{}}3/2016{\_}Wakisaka{\_}Reduction of Heat Loss and Improvement of Thermal Efficiency by Application of temperaturSwing insulation to direct injection diesel engines.pdf:pdf},
journal = {SAE Int. J. Engines},
month = {apr},
number = {3},
pages = {1449--1459},
title = {{Reduction of Heat Loss and Improvement of Thermal Efficiency by Application of Temperature Swing Insulation to Direct-Injection Diesel Engines}},
volume = {9},
year = {2016}
}
@article{Metzger2012,
author = {Metzger, M. and Seifert, T.},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/2012{\_}Metzger+Seifert{\_}A Mechanism-based model for LCF HCF and TMF HCF life prediction.pdf:pdf},
issn = {02323869},
journal = {Tech. Mech.},
number = {2},
pages = {435--445},
title = {{A mechanism-based model for LCF/HCF and TMF/HCF life prediction: Multiaxial formulation, finite-element implementation and application to cast iron}},
volume = {32},
year = {2012}
}
@article{Bennett2003a,
author = {Bennett, V and McDowell, D.{\~{}}L.{\~{}}},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2001{\_}Bennet{\_}Polycrystal orientation distribution effects on microslip  in high cycle fatigue.pdf:pdf},
journal = {Int. J. Fatigue},
keywords = {fatigue,microslip,orientation distribution},
pages = {27--39},
title = {{Polycrystal orientation distribution effects on microslip in high cycle fatigue}},
volume = {25},
year = {2003}
}
@article{Haibacha,
author = {Haibach, Erwin},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Empirical Fatigue Models + Validation/Betriebsfestigkeit{\_}ErwinHaibach/FrontMatter.pdf:pdf},
isbn = {9783540293637},
title = {{Erwin Haibach Betriebsfestigkeit}}
}
@article{Leidich2012,
author = {Leidich, Erhard},
doi = {10.1007/978-3-642-24301-1},
isbn = {9783642243011},
title = {{Kapitel 7 7 Achsen und Wellen}},
year = {2012}
}
@article{Basshuysen2007,
abstract = {Der Ottomotor mit Direkteinspritzung erlangt zunehmende Bedeutung. Dessen Potenzial ist bei weitem noch nicht ausgesch{\"{o}}pft. Leistungs- und Drehmomenterh{\"{o}}hung gepaart mit weiter reduziertem Kraftstoffverbrauch bei gleichzeitiger Schadstoffreduzierung geben klar die Richtung k{\"{u}}nftiger Entwicklungen vor. Als Schl{\"{u}}ssel f{\"{u}}r diese Entwicklung k{\"{o}}nnen aus heutiger Sicht neue Einspritz- und Verbrennungsverfahren gelten, die den Technologieschub bewirken. Das Buch stellt die neuesten Entwicklungen zusammen, beleuchtet und bewertet Motorkonzepte, wie z. B. Downsizing und beschreibt die Anforderungen an Werkstoffe und Betriebsstoffe. Der Ausblick am Ende des Buches beleuchtet die Frage, ob Ottomotoren in Zukunft das Niveau von Dieselmotoren erreichen werden. TS  - GBV - Gemeinsamer Bibliotheksverbund},
author = {Basshuysen, Richard},
doi = {10.1007/978-3-658-01408-7},
isbn = {9783834802026},
journal = {Verfahren, Syst. Entwicklung, Potenzial},
keywords = {Antrieb,Kraftfahrzeug},
pages = {213--248},
title = {{Ottomotor mit Direkteinspritzung}},
url = {http://dx.doi.org/10.1007/978-3-8348-0354-2},
year = {2007}
}
@article{Funktion,
author = {Funktion, Die and Wie, Beispiele and Ausdruck, Der},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Mathematik/Differentation im Komplexen{\_}Quelle TU Darmstadt.pdf:pdf},
pages = {3--9},
title = {{1 1.1 Differentiation im Komplexen}}
}
@article{Wang1985b,
author = {Wang, C S and Berry, G F},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Heat transfer intake+exhaust system/1985{\_}Wang{\_}Heat Transfer in Internal Combustion Engines.pdf:pdf},
journal = {Asme},
number = {Ic},
pages = {1--7},
title = {{Heat Transfer in Internal Combustion Engines}},
year = {1985}
}
@article{Fahrerassistenzsysteme,
author = {Fahrerassistenzsysteme, Neue and Anwendung, Zur},
pages = {407--430},
title = {{19 Fehlererkennung und -diagnose f{\"{u}}r Fahrdynamiksensoren mit querdynamischen}}
}
@article{Grandin2002,
abstract = {SI Engine knock is caused by autoignition in the unburnt part of the mixture (end-gas) ahead of the propagating flame. Autoignition of the end-gas occurs when the temperature and pressure exceeds a critical limit when comparatively slow reactions-releasing moderate amounts of heat-transform into ignition and rapid heat release.In this paper the difference in the heat released in the end-gas-by low temperature chemistry-between lean, rich, stochiometric, and stoichiometric mixtures diluted with cooled EGR was examined by measuring the temperature in the end-gas with Dual Broadband Rotational CARS. The measured temperature history was compared with an isentropic temperature calculated from the cylinder pressure trace. The experimentally obtained values for knock onset were compared with results from a two-zone thermodynamic model including detailed chemistry modeling of the end-gas reactions.},
author = {Grandin, B{\"{o}}rje and Denbratt, Ingemar and Bood, Joakim and Brackmann, Christian and Bengtsson, Per-Erik and Gogan, Adina and Mauss, Fabian and Sund{\'{e}}n, Bengt},
doi = {10.4271/2002-01-0239},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2002{\_}Grandin{\_}Heat Release in the End-Gas Prior to Knock in lean-rich-stoichiometric mixtures.pdf:pdf},
journal = {SAE Tech. Pap.},
number = {724},
title = {{Heat Release in the End-Gas Prior to Knock in Lean, Rich and Stoichiometric Mixtures With and Without EGR}},
url = {http://dx.doi.org/10.4271/2002-01-0239},
volume = {2002-01-02},
year = {2002}
}
@article{Walter2008,
author = {Walter, J{\"{u}}rgen},
isbn = {9783540667582},
title = {{Mikrocomputertechnik mit der 8051-Controller Familie}},
year = {2008}
}
@article{Verst,
author = {Verst, Elektronische},
title = {{Arker}}
}
@article{Meneghetti2016b,
abstract = {Fatigue crack initiation and propagation involve plastic strains that require some work to be done on the material. Most part of this irreversible energy is dissipated as heat and consequently the material temperature increases. The heat being an indicator of the intense plastic strains occurring at the tip of a propagating fatigue crack, the hypothesis is formed that it can be used to assess the fatigue damage accumulation rate of cracked components. Moreover, the heat energy at the crack tip is averaged according to Neuber's finite particle concept. The aim of the present paper is to present the theoretical framework and the corresponding experimental technique to evaluate the heat energy dissipated in a structural volume surrounding the crack tip. The shape and size of the structural volume have been assumed according to the literature, even though the definition of the structural volume size of the analysed material in a fatigue sense is not the scope of the present paper. The proposed experimental technique to evaluate the averaged heat energy is based on the radial temperature profiles measured around the crack tip by means of an infrared camera. The temperature fields measured within few millimetres from the crack tip have been compared successfully with existing analytical solutions.},
author = {Meneghetti, G. and Ricotta, M.},
doi = {10.1016/j.ijfatigue.2016.04.001},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2016{\_}Meneghetti{\_}Evaluating the heat energy dissipated in a small volume surrounding the tip of a fatigue crack.pdf:pdf},
issn = {01421123},
journal = {Int. J. Fatigue},
keywords = {AISI 304L,Averaging approaches,Crack propagation,Crack tip,Critical distance mechanics,Energy approaches,Fatigue assessment},
pages = {605--615},
publisher = {Elsevier Ltd},
title = {{Evaluating the heat energy dissipated in a small volume surrounding the tip of a fatigue crack}},
url = {http://dx.doi.org/10.1016/j.ijfatigue.2016.04.001},
volume = {92},
year = {2016}
}
@article{Elemente2012,
author = {Elemente, Diese and Folgenden, Im and Bild, Im and Axialkr, Element and Querkr, Ebenen and Gebrauch, Blockaddition},
doi = {10.1007/978-3-8348-2134-8},
isbn = {9783834821348},
title = {{7 Elementkatalog f{\"{u}}r elastostatische Probleme}},
year = {2012}
}
@article{Verbrennungsprozess,
author = {Verbrennungsprozess, Der},
pages = {282--299},
title = {{11 Verbrennung 11.1}}
}
@book{Shclick2013,
abstract = {In this paper, the Turing instability in reaction-diffusion models defined on complex networks is studied. Here, we focus on three types of models which generate complex networks, i.e. the Erd$\backslash$H{\{}o{\}}s-R$\backslash$'enyi, the Watts-Strogatz and the threshold network models. From analysis of the Laplacian matrices of graphs generated by these models, we reveal that the stable-unstable regions of a spatially homogeneous solution completely differ, depending on network structures. In particular, we approximately argue the existence of the stable-unstable regions in the cases of regular enhanced ring lattices which include regular circles, and networks generated by the threshold network model when the number of vertices is large enough.},
archivePrefix = {arXiv},
arxivId = {1406.6401},
author = {Shclick, Tamra and Torquato, Salvatore},
booktitle = {Phys. Rev. E - Stat. Nonlinear, Soft Matter Phys.},
doi = {10.1016/j.camwa.2013.03.019},
eprint = {1406.6401},
isbn = {4420767936},
issn = {1539-3755},
keywords = {05c82,1,2010 msc,35k57,60g05,60j60,70k50,92c15,92c40,Amplitude equation,Cortical folding,Cross diffusion,Ginzburg-Landau equation,Growing domain,Linearised stability,Morphology,Nonlinear diffusion,Pattern formation,Quintic Stuart-Landau equation,Reaction-diffusion system,Turing bifurcation,Turing system,activator,ams subject classifications,and another for inhibitor,and diffusion,approaches to the mathematical,based,clo,compartment-based models,complex network,cross-diffusion,cross-diffusion systems,deterministic models which are,diffusion models,diffusion system,epstein,growing domain,holling type-ii functional response,i,instability,introduction,le,lengyel,model,modelling of chemical reactions,non-constant positive steady state,pattern,pattern formation,reaction,reaction-diffusion,reaction-diffusion models on networks,reaction-diffusion processes,reaction-diffusion systems,self-organised spatial pattern,stationary patterns,stochastic processes,stochastic simulations,stochastic turing patterns,systems,there are two fundamental,turing instability,turing pattern,turing reaction,turing system},
number = {4},
pages = {476},
pmid = {15267983},
title = {{Interdisciplinary Applied Mathematics}},
url = {http://link.springer.com/10.1140/epjb/e2013-40570-8{\%}5Cnhttp://arxiv.org/abs/1406.6401{\%}5Cnhttp://arxiv.org/abs/1204.1475{\%}5Cnhttp://link.aps.org/doi/10.1103/PhysRevLett.91.058302{\%}5Cnhttp://arxiv.org/abs/nlin/0111059{\%}5Cnhttp://link.aps.org/doi/10.1103/PhysRe},
volume = {82},
year = {2013}
}
@article{Hartey,
author = {Hartey, Beispiel and Motorrad, B M W},
pages = {391--414},
title = {{Individualisierung 13 Zubeh{\"{o}}r , Spezialteile und technische Verfeinerung}}
}
@article{DASGUPTA2001a,
abstract = {This paper presents a micro-mechanistic approach for modeling fatigue damage initiation due to cyclic plasticity and cyclic creep in eutectic Pb-Sn solder. The issue of damage evolution is deferred to a future paper. Fatigue damage model due to cyclic plasticity is modeled with dislocation mechanics. A conceptual framework is provided to quantify the influence of temperature on fatigue damage due to cyclic plasticity. Damage mechanics due to cyclic creep is modeled with a void nucleation model based on micro-structural stress fields. Micro-structural stress states are estimated under viscoplastic phenomena like grain boundary sliding and its blocking at second phase particles, and diffusional creep relaxation. A conceptual framework is provided to quantify the creep-fatigue damage due to thermo-mechanical cycling.},
author = {DASGUPTA, A and SHARMA, P and UPADHYAYULA, K},
doi = {10.1106/NM1B-1UQH-DJCT-4YH1},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Kriechen{\_}Spannungsrelaxation/2001{\_}Dasgubta{\_}Micro-Mechanics of fatigue due to vibration and thermal cycling.pdf:pdf},
issn = {10567895},
journal = {Int. J. Damage Mech.},
number = {2},
pages = {101--132},
title = {{Micro-Mechanics of Fatigue Damage in Pb-Sn Solder Due to Vibration and Thermal Cycling}},
url = {http://techpub.metapress.com/link.asp?target=contribution{\%}7B{\&}{\%}7Did=NM1B1UQHDJCT4YH1},
volume = {10},
year = {2001}
}
@article{Gao2009,
author = {Gao, Z and Conklin, J C and Daw, C S and Chakravarthy, V K},
doi = {10.1243/14680874JER05609},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Heat transfer intake+exhaust system/2009{\_}Gao+Conklin{\_}A proposed methodology for estimating transient engine-out temperature and emissions from steady-state maps.pdf:pdf},
journal = {Int. J. Engine Res.},
keywords = {emissions,engine,methodology,steady-state maps,transient},
pages = {137--151},
title = {{A proposed methodology for estimating transient engine-out temperature and emissions from steady- state maps}},
volume = {11},
year = {2010}
}
@article{Lucasa,
author = {Lucas, Klaus},
title = {{2. Fluide Phasen}}
}
@article{Forte2014a,
abstract = {A methodology for the evaluation of the effects of twin spark ignition system on CCV (Cycle by Cycle Variability) and knocking combustions is here presented, based on both the use of Computation Fluid Dynamics (CFD) tools and experimental information. The focus of the numerical methodology is the statistical evaluation of the local air-to-fuel distribution at the spark plugs and its correlation with the variability of the initial stages of combustion. A detailed analysis of knocking events can help improving engine performance and diagnosis strategies. The use of twin spark ignition system can enhance the probability that the initial kernel could come across a zone with the correct air-to-fuel ratio, thus lowering the initial combustion instabilities. Moreover the lower distance swept from the flame fronts can considerably reduce the time for the unburnt mixture to auto-ignite, thus reducing the risk of knocking combustion. CFD simulations have been used to reproduce knock effect on the in-cylinder pressure trace. The pressure signal holds information about waves propagation and heat losses: it is crucial to relate local pressure oscillations to knock severity. For this purpose, a CFD model has been implemented, able to predict the combustion evolution with respect to Spark Advance, from non-knocking up to heavy knocking conditions. The CFD model validation phase is essential for a correct representation of both regular and knocking combustions: the operation has been carried out by means of an accurate statistical analysis of experimental in-cylinder pressure data. ?? 2013 The Authors.},
author = {Forte, Claudio and Bianchi, Gian Marco and Corti, Enrico and Fantoni, Stefano and Costa, Marco},
doi = {10.1016/j.egypro.2014.01.091},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Klopfen{\_}Ottomotor/2014{\_}Forte+Corti+Bianchi{\_}CFD Methodology for the evaluation of knock of a PFI Twin Spark Engine.pdf:pdf},
isbn = {3905120933},
issn = {18766102},
journal = {Energy Procedia},
keywords = {Cycle by Cycle Variability,High performance engine,Knock,Twin spark},
pages = {859--868},
publisher = {Elsevier B.V.},
title = {{CFD methodology for the evaluation of knock of a PFI Twin spark engine}},
url = {http://dx.doi.org/10.1016/j.egypro.2014.01.091},
volume = {45},
year = {2014}
}
@article{Leistungsangebot2007,
author = {Leistungsangebot, Leistungsbedarf},
journal = {Fahrzeuggetriebe},
title = {{3 Leistungsbedarf und Leistungsangebot}},
year = {2007}
}
@article{Ladungswechsel,
author = {Ladungswechsel, Der},
journal = {Auslegung A Grad. J. Philos.},
pages = {273--295},
title = {{5 Berechnung und Auslegung von Baugruppen}}
}
@article{Ruzzene2009,
abstract = {This article presents an overview of damage measures proposed in the area of structural health monitoring. This is an extremely active, open, and vast research field, as demonstrated by the variety of topics presented in this encyclopedia. The direction taken in this article is to present some examples of techniques that have been proposed, or that are promising tools for the estimation of location and extent of structural damage. All of the techniques considered are based on the analysis of the dynamic response of the structure under consideration. The organization of the article is based on the frequency range of analysis, which spans the low-frequency range, and correspondingly long response times, associated with the modal analysis of the structure, to frequencies associated with the propagation of guided ultrasonic waves. Hence, the methods presented belong to the classes of vibration-based and guided waves-based techniques. The damage measures discussed rely on the estimation of changes in modal parameters of the structure (natural frequencies, mode shapes, and strain energy distributions), or on features associated with the signal corresponding to the measured dynamic response. This overview is not meant to be exhaustive, but rather it provides examples of interesting solutions and approaches proposed in this area.},
author = {Ruzzene, M},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Probabilistic Aspects/A Unified Statistical Methodology for Modeling Fatigue Damage{\_}Castillo/Kap6{\_}Damage Measures.pdf:pdf},
isbn = {978-0-470-05822-0},
journal = {Encycl. Struct. Heal. Monit.},
keywords = {damage measures,guided ultrasonic waves,vibration-based technique},
number = {48},
pages = {----},
title = {{Damage measures}},
year = {2009}
}
@article{NationalPopulationCommission2009,
author = {{National Population Commission} and {Nigeria Demographic and Health Survey}},
pages = {1--3},
title = {{Appendix C}},
url = {?http://www.measuredhs.com/pubs/pdf/FR115/17AppendixC.pdf (accessed February 27?,? 2009)?},
year = {2009}
}
@article{Moscatelli2017,
author = {Moscatelli, D and Sponchioni, M},
doi = {10.1016/B978-0-08-100262-9.00012-4},
isbn = {9780081002629},
title = {12 12.1},
year = {2017}
}
@article{Band,
author = {Band, Begriff Der Ortskurve},
pages = {124--126},
title = {{5 Ortskurven}}
}
@article{Models1992,
author = {Models, Mathematical},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Anisotropic Behaviouir of Damaged Materials{\_}Skrzypek{\_}ARTICEL/Kap1{\_}Applications of Tensor Functions in Damage Mechanics of Anisotropic Materials.pdf:pdf},
keywords = {anisotropy,canonical form,constitutive equations,continuum damage,creep,creep rupture,creep rupture time,damage tensor,evolutional equa-,irreducible invariants,material,material behaviour,mechanics,monkman-grant relationship,net-stress concept,tensor,tensor function,tensor generator,tensorial interpolation,ter-,tions},
number = {January},
pages = {47--59},
title = {{Applications of Tensor Functions in Continuum Damage Mechanics}},
year = {1992}
}
@phdthesis{Hadzic1999,
author = {Hadzic, Ibrahim},
file = {:X$\backslash$:/Proj/E/E0006/01{\_}EL{\_}Werk/Projektteam/02{\_}Antrieb/Motor{\_}TDFI/Organisation/Pr{\"{a}}sentationen/150529 Masterarbeit PeterHoelz zur AER/MasterarbeitDiverseDateien/Abgeschlossen/as{\_}hadzic{\_}19990208.pdf:pdf},
school = {Technical University of Delft},
title = {{Second-moment closure modeling of transitional and unsteady turbulent flows}},
year = {1999}
}
@article{Plastification,
author = {Plastification, Ocal and Stress, H E and Series, Mechanics and Strength, Perational and Components, O F},
title = {{FEMFAT 5.2a}}
}
@article{Meister2011f,
abstract = {Die wichtigsten Verfahren zur numerischen L{\{}{\"{o}}{\}}sung von linearen Gleichungssystemen in einer umfassenden Einf{\{}{\"{u}}{\}}hrung, die zum Verst{\{}{\"{a}}{\}}ndnis nur geringe mathematische Vorkenntnisse ben{\{}{\"{o}}{\}}tigt. Behandelt werden sowohl die direkten als auch die iterativen Verfahren, wobei der Autor gro{\{}{\ss}{\}}en Wert auf eine sorgf{\{}{\"{a}}{\}}ltige Herleitung dieser Verfahren legt. Au{\{}{\ss}{\}}erdem sind sehr detaillierte Pseudocodes enthalten, mit deren Hilfe sich die jeweiligen Verfahren in einer beliebigen Programmiersprache sofort auf dem Computer realisieren lassen. Das Lehrbuch ist auch f{\{}{\"{u}}{\}}r Natur- und Ingenieurwissenschaftler geeignet, die in vielen praktischen Anwendungen mit der L{\{}{\"{o}}{\}}sung von linearen Gleichungssystemen konfrontiert sind.},
archivePrefix = {arXiv},
arxivId = {1011.1669v3},
author = {Meister, Andreas},
doi = {10.1007/978-3-8348-8100-7},
eprint = {1011.1669v3},
isbn = {978-3-8348-1550-7},
issn = {1098-6596},
journal = {Matrix},
pages = {36--68},
pmid = {25246403},
title = {{Numerik linearer Gleichungssysteme}},
url = {http://link.springer.com/10.1007/978-3-8348-8100-7},
year = {2011}
}
@article{Betrachtungena,
author = {Betrachtungen, Allgemeine},
title = {{are , eindimensionale Str ¨ omungen inkompressibler , viskoser Fluide}}
}
@inproceedings{Huegel2015,
author = {Huegel, Philipp},
booktitle = {Energieundklimaschutzbw},
title = {{Untersuchungen zum Wandw{\"{a}}rmeverlust in Ottomotoren mit Direkteinspritzung}},
year = {2015}
}
@article{Pucher2012,
abstract = {Kennfelder u.a.},
author = {Pucher, Helmut and Zinner, Karl},
doi = {10.1007/978-3-642-28990-3},
isbn = {978-3-642-28989-7},
pages = {307--363},
title = {{Aufladung von Verbrennungsmotoren}},
url = {http://link.springer.com/10.1007/978-3-642-28990-3},
year = {2012}
}
@article{Verger2002a,
abstract = {This paper presents a global approach of thermomechanical design in the automotive industry. The three steps of the method are the following: the loading definition, the modelling of the constitutive law, a failure criterion. Cracked area and lifetime prediction are described in the case of aluminium alloy cylinder heads submitted to transient thermal loadings. The main hypothesis and modelling choices are presented and results are illustrated by a series of computations on real 3D structures. {\textcopyright} 2002 Elsevier Ltd. All rights reserved.},
author = {Verger, L. and Constantinescu, A. and Charkaluk, E.},
doi = {10.1016/S1566-1369(02)80087-5},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Kriechen{\_}Spannungsrelaxation/2002{\_}Verger{\_}THERMOMECHANICAL FATIGUE DESIGN OF ALUMINIUM COMPONENTS.pdf:pdf},
issn = {15661369},
journal = {Eur. Struct. Integr. Soc.},
number = {C},
pages = {309--318},
title = {{Thermomechanical fatigue design of aluminium components}},
volume = {29},
year = {2002}
}
@article{Brij,
author = {Brij, N},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Zienkiewicz FEM - Vol 2 Solid Structural Mechanics/63212{\_}aindx.pdf:pdf},
journal = {Advances},
pages = {1--2},
title = {{Author Index *}},
volume = {115}
}
@article{Graner1982,
author = {Graner, William R.},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/{\_}buecherSong/HandbookofComposites/V/42{\_}MarineApplications.pdf:pdf},
journal = {Handb. Compos.},
pages = {699--722},
title = {{Marine Applications}},
year = {1982}
}
@article{Ince2014a,
abstract = {In this paper, two different forms of an original multiaxial fatigue damage parameter related to the maximum fatigue damage plane are proposed for performing fatigue life prediction under various loading conditions loadings. The proposed fatigue damage parameters have been applied to uniaxial and multiaxial loading conditions for geometrically different bodies. Both the damage parameters are correlated to sets of experimental data published in the literature to verify the prediction accuracy of the damage parameters. The damage parameter in the form of the GSA, when applied to the uniaxial loading, provides very good correlations with four sets of experimental mean stress fatigue data for Incoloy 901 super alloy, ASTM A723 steel, 7075-T561 aluminum alloy and 1045 HRC 55 steel. In the case of multiaxial loadings, both the GSE and GSA parameters are found to correlate well with fatigue data of 1045 steel and Inconel 718 tubular specimens under proportional and non-proportional loadings. In addition, the damage parameters show reasonably acceptable correlations with experimental fatigue data of SAE 1045 steel notched shafts subjected to proportional and non-proportional loadings. ?? 2013 Elsevier Ltd. All rights reserved.},
author = {Ince, Ayhan and Glinka, Grzegorz},
doi = {10.1016/j.ijfatigue.2013.10.007},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Empirical Fatigue Models + Validation/Energy based models/A generalized fatigue damage  parameter for multiaxial fatigue life prediction under proportional  loadings.pdf:pdf},
issn = {01421123},
journal = {Int. J. Fatigue},
keywords = {Critical plane,Fatigue damage parameter,Mean stress,Multiaxial fatigue life},
pages = {34--41},
publisher = {Elsevier Ltd},
title = {{A generalized fatigue damage parameter for multiaxial fatigue life prediction under proportional and non-proportional loadings}},
url = {http://dx.doi.org/10.1016/j.ijfatigue.2013.10.007},
volume = {62},
year = {2014}
}
@article{Grundlagen1975,
author = {Grundlagen, Kerntechnische},
title = {{5 Kernkraftwerke}},
year = {1975}
}
@book{Gross2011e,
author = {Gross, Dietmar and Seelig, Thomas},
doi = {10.1007/978-3-642-10196-0},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Gross, Selig 2011 - Bruchmechanik/Gross, Seelig - 2011 - BruchmechanikKap5.pdf:pdf},
isbn = {978-3-642-10195-3},
title = {{Bruchmechanik}},
url = {http://link.springer.com/10.1007/978-3-642-10196-0},
year = {2011}
}
@article{Agarwal2006a,
abstract = {Thermal loading of diesel engine pistons has increased dramatically in recent years owing to applications of various technologies to meet low emission and high power density requirements. Control of piston temperatures by cooling of these pistons has become one of the determining factors in a successful engine design. The pistons are cooled by oil jets fired at the underside from the crankcase. Any excessive piston temperature rise may lead to engine seizure because of piston warping. However, if the temperature at the underside of the piston, where the oil jet strikes the piston, is above the boiling range of the oil being used, it may contribute to the generation of mist. This mist significantly contributes to the non-tailpipe emissions in the form of unburnt hydrocarbons (UBHCs). The problem of non-tailpipe emissions has unfortunately not been looked into so seriously, as the current stress of all automobile manufacturers is to meet the tailpipe emission legislative limits.A numerical model has been developed using finite element methods for studying the oil jet cooling of pistons and has been validated experimentally on a flat plate cooled by oil jet. Using numerical modelling, the heat transfer coefficient (h) at the underside of the piston is predicted. This predicted value of heat transfer coefficient significantly helps in selecting the correct oil type, oil jet velocity, oil jet diameter, and distance of oil nozzle from the underside of the piston. It also helps to predict whether the selected grade of oil will contribute to mist generation. Isotherms of the predicted temperature profiles in a production grade piston have been plotted.},
author = {Agarwal, A K and Varghese, M B},
doi = {10.1243/14680874JER01804},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/W{\"{a}}rme-RBen Kolben/2004{\_}Varghese{\_}Numerical investigation of piston cooling using oil jet.pdf:pdf},
issn = {1468-0874},
journal = {Int. J. Engine Res.},
number = {5},
pages = {411--421},
title = {{Numerical investigations of piston cooling using oil jet in heavy duty diesel engines}},
url = {http://journals.sagepub.com/doi/10.1243/14680874JER01804},
volume = {7},
year = {2006}
}
@article{Gross2011c,
author = {Gross, Dietmar and Seelig, Thomas},
doi = {10.1007/978-3-642-10196-0},
isbn = {978-3-642-10195-3},
title = {{Bruchmechanik}},
url = {http://link.springer.com/10.1007/978-3-642-10196-0},
year = {2011}
}
@article{Meroth2008a,
abstract = {Der visuelle Kanal besitzt die h{\"{o}}chste Informationsdichte im Fahrzeug. Anzeigen im Fahrzeug liefern Informationen zum Betriebszustand des Fahrzeugs, warnen bei kritischen Zust{\"{a}}nden, informieren {\"{u}}ber den Zustand der Entertainmentkomponenten, geben empfangene Nachrichten wieder, unterst{\"{u}}tzen bei der Navigation (Abbiegehinweise, Karten) oder der Fahrzeugf{\"{u}}hrung (Abstand zu Hindernissen und zu Fahrbahnbegrenzungen) oder dienen der Unterhaltung (Videoentertainment). Entsprechend ihrer Funktion sind Anzeigen an verschiedenen Stellen im Fahrzeug verteilt und beruhen auf unterschiedlichen Technologien.},
author = {Meroth, Ansgar and Tolg, Boris},
isbn = {978-3-8348-9430-4},
journal = {Infotainmentsysteme im Kraftfahrzeug},
pages = {79--114},
title = {{Anzeigetechnik}},
url = {http://dx.doi.org/10.1007/978-3-8348-9430-4{\_}3},
year = {2008}
}
@article{Lenkung,
author = {Lenkung, Die and Verfahren, Beide and Im, Fahrzeuglenkung and Lan-, Kutschwagenbauer},
title = {{8 Die Lenkung}}
}
@article{Reimer2003,
abstract = {It's sometimes difficult to observe combustion in situ — inside, say, a porous material or an industrial reactor. But with the help of nuclear magnetic resonance, a new vista has opened up.},
author = {Reimer, Jeffrey},
doi = {10.1038/426508a},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Klopfen{\_}Ottomotor/2009{\_}Forte+Corti+Bianchi{\_}Combined experimental and numerical analysis of knock in SI engines.pdf:pdf},
isbn = {9789535108566},
issn = {1476-4687},
journal = {Nature},
number = {December},
pages = {508--509},
pmid = {14654825},
title = {{Internal combustion}},
volume = {426},
year = {2003}
}
@article{Gross2011e,
author = {Gross, Dietmar and Seelig, Thomas},
doi = {10.1007/978-3-642-10196-0},
isbn = {978-3-642-10195-3},
title = {{Bruchmechanik}},
url = {http://link.springer.com/10.1007/978-3-642-10196-0},
year = {2011}
}
@article{Frontlangs-allradantrieb1910,
author = {Frontl{\"{a}}ngs-allradantrieb, F L A and Heckl{\"{a}}ngs-antrieb, H L and Heckquer-antrieb, H Q},
journal = {Erkenntnis},
title = {{12 Beispiele ausgef{\{}{\"{u}}{\}}hrter Konstruktionen von Fahrzeuggetrieben}},
year = {1910}
}
@article{Kalghatgi1995a,
abstract = {Net heat release, knock characteristics and temperature were derived$\backslash$nfrom in-cylinder pressure and end-gas CARS measurements for different$\backslash$nfuels in a single-cylinder engine. The maximum net heat release rate$\backslash$nresulting from the final phase of autoignition is closely associated$\backslash$nwith knock intensity. Aromatic fuels have lower maximum heat release$\backslash$nrates and lower knock intensities than expected from their octane number$\backslash$nwhen compared to paraffinic fuels; this is observed even when there is$\backslash$nsignificant heating of the end-gas from pre-flame reactions. Leaner$\backslash$nmixtures have lower combustion rates so that pressure development is$\backslash$nslowed and hence ignition needs to be more advanced to get knock to$\backslash$noccur as frequently as in a richer mixture. However, for a given$\backslash$nfrequency of knock occurrence, there is no significant difference in$\backslash$npeak net heat release rates and hence in knock intensities for different$\backslash$nmixture strengths.},
author = {Kalghatgi, G T and Golombok, M and Snowdon, P},
doi = {10.1080/00102209508951924},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Klopfen{\_}Ottomotor/2007{\_}Kalghatgi{\_}Fuel effect on knock - heat release and CARS tempertures in SI Engine.pdf:pdf},
issn = {0010-2202},
journal = {Combust. Sci. Technol.},
number = {March},
pages = {209--228},
title = {{Fuel effects on knock, heat release and `'CARS'' temperatures in a spark ignition engine}},
volume = {111},
year = {1995}
}
@article{Bohlke2001a,
author = {B{\"{o}}hlke, Thomas and Br{\"{u}}ggemann, C},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/Strukturmechanik MMS/Literatur/Graphical Representation of the Generalized Hooke's Law{\_}SingleCrystals{\_}B{\"{o}}hlke{\_}Kommentar.pdf:pdf},
journal = {Techn,sche Mech.},
number = {2},
pages = {145--158},
title = {{Graphical Representation of the Generalized Hooke's Law}},
volume = {21},
year = {2001}
}
@article{Newman1984,
abstract = {A general crack opening stress equation is presented which may be used to correlate crack growth rate data for various materials and thicknesses, under constant amplitude loading, once the proper constraint factor has been determined. The constraint factor, alpha, is a constraint on tensile yielding; the material yields when the stress is equal to the product of alpha and sigma. Delta-K (LEFM) is plotted against rate for 2024-T3 aluminum alloy specimens 2.3 mm thick at various stress ratios. Delta-K sub eff was plotted against rate for the same data with alpha = 1.8; the rates correlate well within a factor of two.},
author = {Newman, J. C.},
doi = {10.1007/BF00020751},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/1984{\_}Newman{\_}A Crack opening stress equation for fatigue crack growth.pdf:pdf},
isbn = {0376-9429},
issn = {03769429},
journal = {Int. J. Fract.},
number = {4},
pages = {131--135},
title = {{A crack opening stress equation for fatigue crack growth}},
volume = {24},
year = {1984}
}
@article{TransientMethodPeter,
author = {H{\"{o}}lz, Peter and B{\"{o}}hlke, Thomas and Kr{\"{a}}mer, Thomas},
number = {Submitted},
title = {{Calculation method for complex fuid-solid heat transfer problems with transient and scattering boundary conditions}}
}
@article{Heck2001,
author = {Heck, Ronald M and Farrauto, Robert J},
doi = {https://doi.org/10.1016/S0926-860X(01)00818-3},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Injection+Combustion+Ignitionsystems/2001{\_}Heck+Farrauto{\_}Automobile exhaust catalysts.pdf:pdf},
journal = {Appl. Catal. A Gen.},
keywords = {catalytic converters,diesel,fuel cells,gasoline,lean-burn engines,lean-no x},
pages = {443--457},
title = {{Automobile exhaust catalysts}},
volume = {221},
year = {2001}
}
@article{Mughrabi2015,
abstract = {In this survey, the origin of fatigue crack initiation and damage evolution in different metallic materials is discussed with emphasis on the responsible microstructural mechanisms. After a historical introduction, the stages of cyclic deformation which precede the onset of fatigue damage are reviewed. Different types of cyclic slip irreversibilities in the bulk that eventually lead to the initiation of fatigue cracks are discussed. Examples of trans- and intercrystalline fatigue damage evolution in the low cycle, high cycle and ultrahigh cycle fatigue regimes in mono- and polycrystalline face-centred cubic and body-centred cubic metals and alloys and in different engineering materials are presented, and some microstructural models of fatigue crack initiation and early crack growth are discussed. The basic difficulties in defining the transition from the initiation to the growth of fatigue cracks are emphasized. In ultrahigh cycle fatigue at very low loading amplitudes, the initiation of fatigue cracks generally occupies a major fraction of fatigue life and is hence life controlling.},
author = {Mughrabi, H.},
doi = {10.1098/rsta.2014.0132},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/2015{\_}Mughrabi{\_}Microstructural mechanisms of cyclic deformatiomn fatigue crack initiaion and early crack growth.pdf:pdf},
issn = {1364-503X},
journal = {Philos. Trans. R. Soc. A Math. Phys. Eng. Sci.},
keywords = {materials science,mechanical engineering},
number = {2038},
pages = {20140132--20140132},
pmid = {25713457},
title = {{Microstructural mechanisms of cyclic deformation, fatigue crack initiation and early crack growth}},
url = {http://rsta.royalsocietypublishing.org/cgi/doi/10.1098/rsta.2014.0132},
volume = {373},
year = {2015}
}
@article{NationalPopulationCommission2009,
author = {{National Population Commission} and {Nigeria Demographic and Health Survey}},
pages = {1--3},
title = {{Appendix C}},
url = {?http://www.measuredhs.com/pubs/pdf/FR115/17AppendixC.pdf (accessed February 27?,? 2009)?},
year = {2009}
}
@article{I1986,
author = {I, Mark A Hopkins},
pages = {38--41},
title = {{Discrete Element Methods}},
year = {1986}
}
@article{DASGUPTA2001,
abstract = {This paper presents a micro-mechanistic approach for modeling fatigue damage initiation due to cyclic plasticity and cyclic creep in eutectic Pb-Sn solder. The issue of damage evolution is deferred to a future paper. Fatigue damage model due to cyclic plasticity is modeled with dislocation mechanics. A conceptual framework is provided to quantify the influence of temperature on fatigue damage due to cyclic plasticity. Damage mechanics due to cyclic creep is modeled with a void nucleation model based on micro-structural stress fields. Micro-structural stress states are estimated under viscoplastic phenomena like grain boundary sliding and its blocking at second phase particles, and diffusional creep relaxation. A conceptual framework is provided to quantify the creep-fatigue damage due to thermo-mechanical cycling.},
author = {DASGUPTA, A and SHARMA, P and UPADHYAYULA, K},
doi = {10.1106/NM1B-1UQH-DJCT-4YH1},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Kriechen{\_}Spannungsrelaxation/2001{\_}Dasgubta{\_}Micro-Mechanics of fatigue due to vibration and thermal cycling.pdf:pdf},
issn = {10567895},
journal = {Int. J. Damage Mech.},
number = {2},
pages = {101--132},
title = {{Micro-Mechanics of Fatigue Damage in Pb-Sn Solder Due to Vibration and Thermal Cycling}},
url = {http://techpub.metapress.com/link.asp?target=contribution{\%}7B{\&}{\%}7Did=NM1B1UQHDJCT4YH1},
volume = {10},
year = {2001}
}
@book{VDI-Warmeatlas2013,
abstract = {Der VDI-W{\{}{\"{a}}{\}}rmeatlas blickt im Jahr 2013, dem Erscheinungsjahr dieser 11. deutschen Auflage, auf eine 50-j{\{}{\"{a}}{\}}hrige Historie zur{\{}{\"{u}}{\}}ck. Im Jahre 1963 erschien die erste Auflage. Ziel war und ist es, Ingenieuren in einem {\{}{\"{u}}{\}}bersichtlichen und umfassenden Werk verl{\{}{\"{a}}{\}}ssliche Methoden zur Berechnung von W{\{}{\"{a}}{\}}rme{\{}{\"{u}}{\}}bertragern und w{\{}{\"{a}}{\}}rmetechnischen Apparaten an die Hand zu geben. Hierzu z{\{}{\"{a}}{\}}hlte und z{\{}{\"{a}}{\}}hlt auch die Bereitstellung von Stoffdaten. In diesen 50 Jahren ist der VDI-W{\{}{\"{a}}{\}}rmeatlas zu einem Standardwerk geworden. Nach der 10. deutschen Auflage, die im Jahr 2006 erschien, folgte 2010 die 2. englische Auflage. Der Redaktionsausschuss hatte bei diesem {\{}{\"{U}}{\}}bergang nicht nur alle Berechnungsverfahren und Stoffdaten aktualisiert, sondern auch die urspr{\{}{\"{u}}{\}}ngliche, {\{}{\"{u}}{\}}ber die Jahre gewachsene Gliederung {\{}{\"{u}}{\}}berarbeitet, um einige Themen neu ordnen und neue Themen aufnehmen zu k{\{}{\"{o}}{\}}nnen. Diese {\{}{\"{u}}{\}}berarbeitete Gliederung ist nun auch in der 11. deutschen Auflage zu finden. Zudem wurden zahlreiche Abschnitte wieder aktualisiert, so dass der VDI-W{\{}{\"{a}}{\}}rmeatlas auch weiterhin als aktuelles Standardwerk zur Auslegung von W{\{}{\"{a}}{\}}rme{\{}{\"{u}}{\}}bertragern und w{\{}{\"{a}}{\}}rmetechnischen Apparaten dienen kann. Im Namen der Mitglieder des Redaktionsausschusses danke ich allen Autoren der einzelnen Kapitel f{\{}{\"{u}}{\}}r ihr gro{\{}{\ss}{\}}es Engagement. Dem Springer-Verlag danke ich f{\{}{\"{u}}{\}}r die stets sehr gute Zusammenarbeit und die gelungene Umsetzung, insbesondere den Lekto- rinnen Frau Sigrid Cuneus und Frau Dr. Sylvia Blago.},
author = {VDI-W{\"{a}}rmeatlas},
doi = {10.1007/978-3-642-19981-3},
isbn = {978-3-642-19980-6},
pages = {1784},
title = {{VDI-W{\{}{\"{a}}{\}}rmeatlas}},
url = {http://link.springer.com/10.1007/978-3-642-19981-3},
year = {2013}
}
@article{Pahl2007,
author = {Pahl, Gerhard and Beitz†, Wolfgang and Feldhusen, J{\"{o}}rg and Grote, Karl-H.},
doi = {10.1007/b137606},
isbn = {3-540-22048-8},
journal = {Pahl/Beitz Konstr. - Grundlagen},
title = {{Methoden zur qualit{\{}{\"{a}}{\}}tssichernden Produktentwicklung}},
year = {2007}
}
@article{Lastregelung,
author = {Lastregelung, Die and Motorleistung, Die and Gemischbildungsverfahren, Das and Gemischbildung, Die},
title = {{4 Motorische Verbrennung}}
}
@article{Polak2014c,
abstract = {The role of point defects in the formation of surface relief and in the initiation of a fatigue crack in crystalline materials is analyzed. The dislocation interactions in the bands of intensive cyclic slip (persistent slip bands - PSBs) are specified and relations describing the formation and annihilation of interstitial and vacancy type defects in the channels of the ladder-like PSB are derived. The continuous formation, annihilation and primarily the migration of point defects are proposed to be responsible for the mass redistribution within PSB and between PSB and the PSB/matrix boundary. The redistribution of the matter results in local tensile and compressive stresses that are the sources of the principal irreversibility of slip within PSB. Local tensile and compressive stresses are relaxed by dislocation movement within PSB in the direction of the active Burgers vector and lead to the formation of characteristic surface relief in the form of extrusions and intrusions. The intrusions represent crack-like defects and fatigue cracks initiate in the tip of intrusions. {\{}{\textcopyright}{\}} 2013 Elsevier Ltd. All rights reserved.},
author = {Pol{\'{a}}k, Jaroslav and Man, Jiř{\'{i}}},
doi = {10.1016/j.ijfatigue.2013.10.016},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Kriechen{\_}Spannungsrelaxation/2014{\_}Polak+Man{\_}Fatigue crack initiation – The role of point defects.pdf:pdf},
isbn = {0142-1123},
issn = {01421123},
journal = {Int. J. Fatigue},
keywords = {Extrusion,Fatigue crack initiation,Intrusion,Persistent slip band (PSB),Point defects},
number = {July},
pages = {18--27},
title = {{Fatigue crack initiation - The role of point defects}},
volume = {65},
year = {2014}
}
@article{Ture1980,
author = {Ture, Nomencla},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/1980{\_}Singh{\_}Effect of prior treatement on LCF of AL alloy 2618 at 432K.pdf:pdf},
number = {January},
pages = {12--22},
title = {{Effect of ior alloy mmst oa at 423K cycle alumini l mm amr of}},
year = {1980}
}
@article{Chiodi2001b,
abstract = {Improvement of heat-transfer calculation for SI-engines in the three-dimensional simulation has been achieved and widely been tested by using a phenomenological heat-transfer model. The model is based on the local application of an improved Re-Nu-correlation (dimensional analysis) proposed by Bargende [1]. This approach takes advantage of long experience in engine heat transfer modeling in the real working process analysis. The results of numerous simulations of different engine meshes show that the proposed heat-transfer model enables to calculate the overall as well as the local heat transfer in good agreement with both real working process analyses and experimental investigations. The influence of the mesh structure has also been remarkably reduced and compared to the standard wall function approach, no additional CPU-time is required.},
author = {Chiodi, Marco and Bargende, Michael},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Heat Transfer Combustion Chamber/2001{\_}Chiodi + Bargende{\_}Improvement of engine heat transfer.pdf:pdf},
journal = {SAE Tech. Pap.},
number = {724},
title = {{Improvement of Engine Heat-Transfer Calculation in the Three-Dimensional Simulation Using a Phenomenological Heat-Transfer Model}},
year = {2001}
}
@book{Cherkaoui2009c,
author = {Cherkaoui, Mohammed and Capolungo, Laurent},
doi = {10.1007/978-0-387-46771-9},
isbn = {978-0-387-46765-8},
title = {{Atomistic and Continuum Modeling of Nanocrystalline Materials}},
url = {http://link.springer.com/10.1007/978-0-387-46771-9},
volume = {112},
year = {2009}
}
@article{Hashin1962,
abstract = {IN PREVIOUS papers (HASHIN and SHTRIKMAN 1961a, b) the authors have established some new variational principles in the linear theory of elasticity for isotropic nonhomogeneous bodies with prescribed surface displacements. These have been applied to the theory of the elastic behaviour of multiphase materials. The present work is concerned with the generalization of these principles to anisotropic and nonhomogeneous e1asticity.j and the establishn-ent of similar variational principles for a body with prescribed surface tractions. An accompanying paper deals with the application of these variational principles to the theory of the elastic behaviour of polycrystals.},
author = {Hashin, Z and Shtrikman, S},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/Strukturmechanik MMS/Literatur/HS Schranken Methodik MMS Vorlesung Details/Hashin, Shtrikman - 1962.pdf:pdf},
number = {42},
title = {{Some Principles in and}},
volume = {10},
year = {1962}
}
@article{Mathematik,
author = {Mathematik, Zentrum and Funktion, Eine},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Mathematik/Laplacetrafo{\_}Uebersicht.pdf:pdf},
pages = {1--2},
title = {{Laplace-Transformation – Definition und Rechenregeln}}
}
@article{Mechatronika,
author = {Mechatronik, Die and Feinwerktechnik, Der},
journal = {System},
pages = {183--196},
title = {{10 Feinwerktechnik}}
}
@book{Gross2011,
author = {Gross, Dietmar and Seelig, Thomas},
doi = {10.1007/978-3-642-10196-0},
isbn = {978-3-642-10195-3},
title = {{Bruchmechanik}},
url = {http://link.springer.com/10.1007/978-3-642-10196-0},
year = {2011}
}
@article{Opitz1959a,
author = {Opitz, Herwart},
doi = {10.1007/978-3-663-05002-5_6},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Empirical Fatigue Models + Validation/Betriebsfestigkeit{\_}ErwinHaibach/Backmatter.pdf:pdf},
isbn = {978-3-663-03813-9},
pages = {33--33},
title = {{Verwendete Formelzeichen}},
year = {1959}
}
@article{Corti2009,
abstract = {Specific power and efficiency of gasoline engines are influenced by factors such as compression ratio and Spark Advance (SA) regulation. These factors influence the combustion development over the crank angle: the trade-off between performance and the risk of irreversible damages is still a key element in the design of both high-performance (racing) and low-consumption engines. This paper presents a novel approach to the problem, with the objective of defining a damage-related and operating conditions-independent index. The methodology is based on the combined analysis of indicating parameters, such as Cumulated Heat Release (CHR), Indicated Mean Effective Pressure (IMEP) and 50{\%} Mass Fraction Burned (MFB50), and typical knock detection parameters, estimated by means of the in-cylinder pressure sensor signal. Knocking combustions have several consequences, therefore they can be detected in many ways. As it is well known, knock excites the combustion chamber resonant frequencies, rising high frequency components in the in-cylinder pressure signal. Additionally, knocking combustions cause a higher heat flux through the combustion chamber walls, increasing the heat losses and lowering the IMEP: this effect can be observed by evaluating IMEP or CHR, that are based on the low-frequency content of the in-cylinder signal spectrum. A knock detection index can then be based on the crossed-observation of two phenomena, one set in the low-frequencies range and the other one on the high frequencies range of the in-cylinder pressure signal. Knock-related parameters have been analyzed with a statistical approach, in order to define a detection strategy based on one single threshold value, to be used for all the engines, independently of engine speed and load: IMEP and CHR have been related to a typical high-frequency knock index, based on the Maximum Amplitude of Pressure Oscillations (MAPO) evaluated over the combustion angular window. It can be observed that, as knock intensity increases, the relationships between these parameters change. This change can be seized by evaluating the correlation coefficient between the parameters distributions and observing its trend as a function of SA (Spark Advance). The correlation coefficient is intrinsically normalized, therefore the index range is the same for every engine operating condition, and the paper shows that the threshold level, too, is constant. The same approach can be applied to determine SA corresponding to the best combustion phase, simply by evaluating the correlation coefficient for IMEP and MFB50 distributions. The methodology has been successfully applied to different engines running in different speed and load conditions.},
author = {Corti, Enrico and Forte, Claudio},
doi = {10.4271/2009-24-0019},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Klopfen{\_}Ottomotor/2009{\_}Forte+Corti{\_}Statistical Analysis of Indicating Parameters for Knock Detection Purposes.pdf:pdf},
issn = {19463936},
journal = {SAE Tech. Pap.},
number = {2009-01-0237},
title = {{Statistical Analysis of Indicating Parameters for Knock Detection Purposes}},
url = {http://papers.sae.org/2009-01-0237/},
year = {2009}
}
@article{Begr,
author = {Begr, Die and St, Die},
title = {{Umwelt und Grenzwerte}}
}
@article{Plastification,
author = {Plastification, Ocal and Stress, H E and Series, Mechanics and Strength, Perational and Components, O F},
file = {:C$\backslash$:/Users/p327208/Desktop/Promotion/Literature/Empirical Fatigue Models + Validation/FEMFAT Documents/THEORIE{\_}BASIC52{\_}E.pdf:pdf},
title = {{FEMFAT 5.2a}}
}
@article{Baaser2010,
author = {Baaser, Herbert},
title = {{FEM–Kurs - FEM-Simulationen mit ABAQUS}},
year = {2010}
}
@article{Hasan2007,
author = {Hasan, Basim O},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Boiling/Turbulence/2007{\_}Basim+Hasan{\_}Turbulent Prandtl Number and its Use in Prediction of Heat Transfer Coefficient of Liquids.pdf:pdf},
journal = {Coll. Eng. J.},
number = {1},
pages = {53--64},
title = {{Turbulent Prandtl Number and its Use in Prediction of Heat Transfer Coefficient for Liquids}},
volume = {10},
year = {2007}
}
@book{Melorose2015,
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Melorose, J and Perroy, R and Careas, S},
booktitle = {Statew. Agric. L. Use Baseline 2015},
doi = {10.1017/CBO9781107415324.004},
eprint = {arXiv:1011.1669v3},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/Crystall Plasticity Basics/Hull 2011 - Introduction to Dislocation.pdf:pdf},
isbn = {9788578110796},
issn = {1098-6596},
keywords = {icle},
pmid = {25246403},
title = {{Introduction to dislocations}},
volume = {1},
year = {2015}
}
@article{Bozza2011,
abstract = {In the present paper a combined procedure for the quasi-dimensional modelling of heat transfer, combustion and knock phenomena in a "downsized" Spark Ignition two-cylinder turbocharged engine is presented. The procedure is extended to also include the effects consequent the Cyclic Variability. Heat transfer is modelled by means of a Finite Elements model. Combustion simulation is based on a fractal description of the flame front area. Cyclic Variability (CV) is characterized through the introduction of a random variation on a number of parameters controlling the rate of heat release (air/fuel ratio, initial flame kernel duration and radius, laminar flame speed, turbulence intensity). The intensity of the random variation is specified in order to realize a Coefficient Of Variation (COV) of the Indicated Mean Effective Pressure (IMEP) similar to the one measured during an experimental campaign. Moreover, the relative importance of the various concurring effects is established on the overall COV. A kinetic scheme is then solved within the unburned gas zone, characterized by different thermodynamic conditions occurring cycle-by-cycle. In this way, an optimal choice of the "knock-limited" spark advance is effected and compared with experimental data. Finally, the CV effects on the occurrence of individual knocking cycles are assessed and discussed. {\{}{\textcopyright}{\}} 2011 Global Science Press.},
author = {Bozza, Fabio and Siano, Daniela and Costa, Michela},
doi = {10.4208/aamm.10-10s2-04},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2011{\_}Bozza{\_}heat-transfer-knock-modeling-and-cyclic-variability-in-a-downsized-spark-ignition-turbocharged-engine.pdf:pdf},
issn = {20700733},
journal = {Adv. Appl. Math. Mech.},
keywords = {Cyclic variability,Finite elements in heat transfer,Internal combustion engines modelling,Knock},
number = {3},
pages = {310--326},
title = {{Heat transfer, knock modeling and cyclic variability in a "Downsized" spark-ignition turbocharged engine}},
volume = {3},
year = {2011}
}
@article{Aerostatik2006,
author = {Aerostatik, Hydro-},
journal = {Gerthsen Phys.},
pages = {93--140},
title = {{03 - Mechanik deformierbarer K{\"{o}}rper}},
year = {2006}
}
@article{Rousselier1987b,
abstract = {Since the pioneering studies conducted by McClintock, Rice and Tracey on the growth of cavities, many studies have covered modelling of ductile fracture; a non-exhaustive list is given of these studies. In the local approach of fracture, the models are used at the tip of cracks, and in the present state, only relatively simple models can be used to solve fracture problems in a complete manner, from material characterization to the analysis of cracked structures. The paper presents two types of models based on a critical ratio of cavity growth or on continuum damage mechanics. In the framework of the local approach of fracture, their possibilities are presented with constant references to experimental validation studies. This allows conclusions to be drawn regarding the effectiveness of the methods proposed and their undeniable contribution to fracture mechanics. ?? 1987.},
author = {Rousselier, G.},
doi = {10.1016/0029-5493(87)90234-2},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Plasticity models/Ductile fracture models and their potential in local approach of fracture{\_}Rousselier.pdf:pdf},
isbn = {00295493},
issn = {00295493},
journal = {Nucl. Eng. Des.},
number = {1},
pages = {97--111},
title = {{Ductile fracture models and their potential in local approach of fracture}},
volume = {105},
year = {1987}
}
@book{Gross2011g,
author = {Gross, Dietmar and Seelig, Thomas},
doi = {10.1007/978-3-642-10196-0},
isbn = {978-3-642-10195-3},
title = {{Bruchmechanik}},
url = {http://link.springer.com/10.1007/978-3-642-10196-0},
year = {2011}
}
@article{Zienkiewicz,
abstract = {In Chapters 4, 5, and 6 the reader was shown in some detail how linear elasticity problems could be formulated and solved using very simple {\textregistered}nite element forms. In Chapter 7 this process was repeated for the quasi-harmonic equation. Although the detailed algebra was concerned with shape functions which arose from triangular and tetrahedral shapes only it should by now be obvious that other element forms could equally well be used. Indeed, once the element and the corresponding shape functions are determined, subsequent operations follow a standard, well-de{\textregistered}ned path which could be entrusted to an algebraist not familiar with the physical aspects of the problem. It will be seen later that in fact it is possible to program a computer to deal with wide classes of problems by specifying the shape functions only. The choice of these is, however, a matter to which intelligence has to be applied and in which the human factor remains paramount. In this chapter some rules for the generation of several families of one-, two-, and three-dimensional elements will be presented. In the problems of elasticity illustrated in Chapters 4, 5, and 6 the displacement variable was a vector with two or three components and the shape functions were written in matrix form. They were, however, derived for each component separately and in fact the matrix expressions in these were derived by multiplying a scalar function by an identity matrix [e.g., Eqs (4.7), (5.3), and (6.7)]. This scalar form was used directly in Chapter 7 for the quasi-harmonic equation. We shall therefore concentrate in this chapter on the scalar shape function forms, calling these simply N i . The shape functions used in the displacement formulation of elasticity problems were such that they satisfy the convergence criteria of Chapter 2: (a) the continuity of the unknown only had to occur between elements (i.e., slope continuity is not required), or, in mathematical language, C 0 continuity was needed; (b) the function has to allow any arbitrary linear form to be taken so that the constant strain (constant {\textregistered}rst derivative) criterion could be observed. The shape functions described in this chapter will require the satisfaction of these two criteria. They will thus be applicable to all the problems of the preceding chapters},
author = {Zienkiewicz, O.C.},
title = {{Standard ' anhierarchical' element shape functions: some general families of C{\_}0 continuity 8.1 Introduction}}
}
@article{Svoboda2008,
abstract = {An extremal principle is formulated for thermodynamic systems near equi- librium subjected to various external conditions. It is shown that the principle describes un- ambiguously the kinetics of the thermodynamic system and replaces classical phenomeno- logical equations. Thus the principle can be considered as an effective tool for the treatment of non-equilibrium thermodynamic systems. In two examples the principle is used for the description of Dufour and Soret effects and plasticity. 1.},
author = {Svoboda, Jiř{\'{i}} and Fischer, Franz Dieter and Vala, Jiř{\'{i}}},
doi = {10.1478/C1S0801022},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Thermodynamik/2008{\_}Svoboda+Fischer{\_}Thermodynamic extremal principle and its application to Dufour and Soret effects and Plasticity.pdf:pdf},
issn = {03650359},
journal = {AAPP Atti della Accad. Peloritana dei Pericolanti, Cl. di Sci. Fis. Mat. e Nat.},
number = {SUPPL.1},
pages = {1--11},
title = {{Thermodynamic extremal principle and its application to dufour and soret effects and plasticity}},
volume = {86},
year = {2008}
}
@article{Weng1987a,
abstract = {Based on the dislocation structures developed during plastic deformation, an anisotropic hardening law is developed to describe the latent hardening behavior of slip systems under multislip. This theory incorporates the concept of isotropic hardening, kinematic hardening, and the two-parameter representation; it automatically includes the strength differential between the forward and reversed slips and between the acute and obtuse cross slips. The self-hardening modulus of a slip system is found to be "associated" with the latent hardening law involved, and, based on some experimental evidence, two specific sets of self-hardening modulus are suggested. An important feature of this associated modulus is that the slip system with a soft latent hardening (e.g., the reversed system with a Bauschinge effect) will have an enhanced self-hardening modulus. This newly developed hardening law, together with its associated latent hardening moduli, is then applied to examine the strain-hardening behavior of a polycrystal. Although crystals with a stronger latent hardening will, in general, also lead to a stranger strain-hardening for the polycrystal, the stress-strain behavior of the polycrystal using the kinematic hardening law of single crystals is found to be not necessarily softer than that using the isotropic hardening law. Within the range of experimentally measured latent hardening ratio of slip systems, the anisotropic theory is also used to calculate the motion of yield surface of a polycrystal. The general results, employing four selected types of anisotropic hardening, all show the essential features of experimental observations by Phillips and his co-workers. The application is highlighted with a reasonably successful quantitative modeling of initial and subsequent yield surfaces of an aluminum. ?? 1987.},
author = {Weng, G. J.},
doi = {10.1016/0749-6419(87)90007-6},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/Hardening Recovery Creep/1987{\_}Weng{\_} IJP Anisotropic hardening of crystalls.pdf:pdf},
issn = {07496419},
journal = {Int. J. Plast.},
number = {4},
pages = {315--339},
title = {{Anisotropic hardening in single crystals and the plasticity of polycrystals}},
volume = {3},
year = {1987}
}
@article{Sanli2009d,
abstract = {The aim of this study is to examine numerically the effects of spark timing and load parameters on the in-cylinder heat transfer of a SI engine by using experimental engine test data. For the investigation, a four-stroke, air-cooled, single-cylinder SI engine was tested at different spark timings and loads at a single engine speed of 2000 rpm. Woschni, Hohenberg, and Han models were employed to estimate the in-cylinder heat transfer coefficient in the case of different test conditions because of being favorable models on the SI engine operations. The evaluations show that the in-cylinder heat transfer characteristics of the air-cooled SI engine strongly depend on the load while they slightly depend on the spark timing.},
author = {Sanli, A. and Sayin, C. and Gumus, M. and Kilicaslan, I. and Canakci, M.},
doi = {10.1080/10407780903244312},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2009{\_}Sanli{\_}Numerical evaluation by models of load and spark timing effects on the in-cylinder heat transfer of a si engine.pdf:pdf},
isbn = {1040-7782},
issn = {10407782},
journal = {Numer. Heat Transf. Part A Appl.},
number = {5},
pages = {444--458},
title = {{Numerical evaluation by models of load and spark timing effects on the in-cylinder heat transfer of a SI engine}},
volume = {56},
year = {2009}
}
@misc{Starccm1106,
author = {Siemens},
title = {{STAR-CCM+ User Manual, v11.06}}
}
@article{Fieberg2006,
author = {Fieberg, C and Korth{\"{a}}uer, M},
journal = {Forschungsvereinigung Verbrennungskraftmaschinen},
publisher = {FVV},
title = {{Kontaktw{\"{a}}rme{\"{u}}bergang - Vorhaben Nr. 828, Kontaktdruckabh{\"{a}}ngiger W{\"{a}}rme{\"{u}}bergang im motorischen Umfeld}},
volume = {821},
year = {2006}
}
@article{Groma2015,
abstract = {According to recent experimental and numerical investigations if the characteristic size of a specimen is in the submicron size regime several new interesting phenomena emerge during the deformation of the samples. Since in such a systems the boundaries play a crucial role, to model the plastic response of submicron sized crystals it is crucial to determine the dislocation distribution near the boundaries. In this paper a phase field type of continuum theory of the time evolution of an ensemble of parallel edge dislocations with identical Burgers vectors, corresponding to the dislocation geometry near boundaries, is presented. Since the dislocation-dislocation interaction is scale free ({\{}{\$}{\}}1/r{\{}{\$}{\}}), apart from the average dislocation spacing the theory cannot contain any length scale parameter. As shown, the continuum theory suggested is able to recover the dislocation distribution near boundaries obtained by discrete dislocation dynamics simulations.},
archivePrefix = {arXiv},
arxivId = {1404.6344},
author = {Groma, Istv??n and Vandrus, Zolt??n and Isp??novity, P??ter Dus??n},
doi = {10.1103/PhysRevLett.114.015503},
eprint = {1404.6344},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/2015{\_}Groma{\_}Scale-Free Phase Field Theory of Dislocations.pdf:pdf},
issn = {10797114},
journal = {Phys. Rev. Lett.},
number = {1},
pages = {1--5},
title = {{Scale-free phase field theory of dislocations}},
volume = {114},
year = {2015}
}
@article{Windows,
author = {Windows, Betriebssystem and Erg, Als and Microsoft, Firma and Linux, Betriebssystem and Computer, Instrumentierte},
journal = {Computer (Long. Beach. Calif).},
pages = {173--188},
title = {{11 Automatisierte Messsysteme}}
}
@article{Mittelpunkt,
author = {Mittelpunkt, Im and Motor, Der and Fahrwerk, Das and Beispiel, Am and Belastu, Hohe},
pages = {340--346},
title = {{9 Festigkeits- und Steifigkeitsuntersuchungen an Motorradfahrwerken}}
}
@article{Pan2014a,
abstract = {Knocking combustion in spark-ignition (SI) engines is a typical abnormal combustion phenomenon that severely limits engine performance and thermal efficiency. However, its mechanism has not so far been completely revealed, such as the origin of pressure oscillation with tremendous amplitude and broken mechanisms of the engine body when knock occurs. This article systematically reviews the series of physical and chemical phenomena involved in knocking combustion, including auto-ignition, gas-dynamic waves, cavity resonance, and auto-ignited flame propagation. Significant research has shown that the rapid heat release of end-gas auto-ignition and subsequent strong pressure waves play a crucial role during knocking combustion. A methodology of the interaction of flame propagation and pressure waves has been proposed to reveal knock formation in terms of positive feedback between strengthened pressure waves and auto-ignited flame propagation. Also, new suggestions on the weakness in prior research of knocking combustion have also been discussed in the present article. {\textcopyright} 2014 Copyright Taylor and Francis Group, LLC.},
author = {Pan, Jiaying and Shu, Gequn and Wei, Haiqiao},
doi = {10.1080/00102202.2013.857665},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2014{\_}Pan+Wei{\_}Interaction of Flame Propagation and Pressure Waves During Knocking Combustion in Spark-Ignition Engines.pdf:pdf},
issn = {0010-2202},
journal = {Combust. Sci. Technol.},
number = {2},
pages = {192--209},
title = {{Interaction of Flame Propagation and Pressure Waves During Knocking Combustion in Spark-Ignition Engines}},
url = {http://www.tandfonline.com/doi/abs/10.1080/00102202.2013.857665},
volume = {186},
year = {2014}
}
@article{Gerthsen2006,
author = {Gerthsen},
doi = {10.1007/3-540-29973-4_1},
isbn = {3-540-25421-8},
issn = {09377433},
journal = {Gerthsen Phys.},
pages = {1--70},
title = {{Mechanik der Massenpunkte}},
year = {2006}
}
@article{Mutzke2016,
abstract = {{\textcopyright} 2016 SAE International.Knocking combustion places a major limit on the performance and efficiency of spark ignition engines. Spontaneous ignition of the unburned air-fuel mixture ahead of the flame front leads to a rapid release of energy, which produces pressure waves that cause the engine structure to vibrate at its natural frequencies and produce an audible 'pinging' sound. In extreme cases of knock, increased temperatures and pressures in the cylinder can cause severe engine damage. Damage is thought to be caused by thermal strain effects that are directly related to the heat flux. Since it will be the maximum values that are potentially the most damaging, then the heat flux needs to be measured on a cycle-by-cycle basis. Previous work has correlated heat flux with the pressure fluctuations on an average basis, but the work here shows a correlation on a cycle-by-cycle basis. The in-cylinder pressure and surface temperature were measured using a pressure transducer and eroding-type thermocouple. These sensors were installed side-by-side at the surface of the cylinder in order to investigate the relationship between knock and heat flux on a cycle-by-cycle basis. A finite difference method was implemented to solve the one-dimensional unsteady heat conduction equation and calculate the temperature distribution away from the surface of the combustion chamber, and thus the instantaneous heat flux. The knock intensity was varied by controlling the fuel quality, compression ratio, ignition timing and air-fuel ratio. The measured heat flux was compared with pressure-based knock indices and it was found that as knock intensity increases, the correlation with peak heat flux became stronger. Results from different fuels and engine operating conditions did not collapse onto the same trend line. At higher speeds and higher compression ratios the heat flux was higher at a given level of knock intensity. The co-location of the pressure transducer and heat flux sensor meant that a correlation was found on a cycle-by-cycle basis.},
author = {Mutzke, J. and Scott, B. and Stone, R. and Williams, J.},
doi = {10.4271/2016-01-0700},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2016{\_}Mutzke{\_}The Effect of Combustion Knock on the Instantaneous Heat Flux in Spark Ignition Engines.pdf:pdf},
journal = {SAE Tech. Pap.},
title = {{The Effect of Combustion Knock on the Instantaneous Heat Flux in Spark Ignition Engines}},
volume = {2016-April},
year = {2016}
}
@article{Loud1998,
author = {Loud, Stewart N},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/{\_}buecherSong/HandbookofComposites/V/43{\_}CommercialandIndustrialApplicationsofComposites.pdf:pdf},
journal = {Rev. Lit. Arts Am.},
pages = {1--11},
title = {{Commercial and Industrial Applications of Composites}},
year = {1998}
}
@article{Faktoren,
author = {Faktoren, Alle},
title = {{Motor und Antrieb 3 Arbeitsweise , Bauformen und konstruktive Ausf{\{}{\"{u}}{\}}hrung von Motorradmotoren}}
}
@article{Darstellung,
author = {Darstellung, Vektorielle},
journal = {Differentiation},
title = {{I Vektoranalysis 1}}
}
@article{Lcmaitrc,
author = {Lcmaitrc, Cordchois},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Plasticity models/On Energy based coupled elastoplastic damage theories{\_}Ju1988.pdf:pdf},
title = {{1989-Ju{\{}{\_}{\}} On energy-based coupled elastoplastic damage theories{\{}{\_}{\}}constitutive modeling and computational aspects.pdf}}
}
@article{Kraft2000,
author = {Kraft, Kennzeichnung Der and Zerlegung, Rechnerische and Kraft, Resultierende and Kraftvektors, Betrag},
number = {1},
pages = {1--26},
title = {{Formelsammlung Technische Mechanik}},
year = {2000}
}
@article{Gr,
author = {Gr, Physikalische},
journal = {Frequenz},
pages = {55--62},
title = {{Physikalische Gr{\"{o}}{\ss}en, Definitionsgleichungen und Einheiten 2.1}}
}
@article{Metallplastizit2013b,
author = {Metallplastizit, Hrungdie and Helm, Dirk},
number = {November},
pages = {1--29},
title = {{Prozesssimulation in Der Umformtechnik}},
year = {2013}
}
@article{Reifendruck,
author = {Reifendruck, Der},
journal = {System},
number = {Xl},
pages = {1--7},
title = {{10 Reifendruck}}
}
@article{Gross2011c,
author = {Gross, Dietmar and Seelig, Thomas},
doi = {10.1007/978-3-642-10196-0},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Gross, Selig 2011 - Bruchmechanik/Gross, Seelig - 2011 - BruchmechanikKap6.pdf:pdf},
isbn = {978-3-642-10195-3},
title = {{Bruchmechanik}},
url = {http://link.springer.com/10.1007/978-3-642-10196-0},
year = {2011}
}
@article{Zienkiewicz2005c,
author = {Zienkiewicz, O},
doi = {10.1016/B978-075066431-8/50226-5},
isbn = {9780750664318},
pages = {699--700},
title = {{Integration by parts in two or three dimensions (Green}},
year = {2005}
}
@article{Anfang,
author = {Anfang, Seit and Ars, Wankstabilisierung and Drive, Namen Dynamik and Daimlerchrysler, Hause and Beschleunigungs-, Bei and Fahrsicherheit, Richtung},
isbn = {3-8348-0109-7},
journal = {Integr. Vlsi J.},
pages = {253--264},
title = {{11 Semiaktive Sto{\{}{\ss}{\}}d{\{}{\"{a}}{\}}mpfer und aktive}}
}
@article{Messtechnika,
author = {Messtechnik, Der},
pages = {1--5},
title = {{1 Messen ; Voraussetzungen und Durchf{\"{u}}hrung}}
}
@article{Hydrostatik2007,
author = {Hydrostatik, Die},
pages = {1--44},
title = {{6 Hydrostatik und Aerostatik}},
url = {papers2://publication/uuid/3EEDFA6E-E85B-4C6A-80F6-E0FF53993A84},
year = {2007}
}
@article{Mende2013,
author = {Mende},
isbn = {9192631770},
journal = {Phys. Gleichungen und Tabellen},
pages = {177--204},
title = {{Mechanik fester K{\{}{\"{o}}{\}}rper}},
year = {2013}
}
@article{Papulaa,
author = {Papula, L},
journal = {Math. f{\{}{\"{u}}{\}}r Ingenieure und Naturwissenschaftler Band 2},
title = {{IV Gew{\{}{\"{o}}{\}}hnliche Differentialgleichungen 1}}
}
@article{Gurtin1967,
author = {Gurtin, Morton E. and Williams, William O.},
doi = {10.1007/BF00285676},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Thermodynamik/An Axiomatic Foundation for Continuum Thermodynamics{\_}CommunicatedByNoll.pdf:pdf},
issn = {00039527},
journal = {Arch. Ration. Mech. Anal.},
number = {2},
pages = {83--117},
title = {{An axiomatic foundation for continuum thermodynamics}},
volume = {26},
year = {1967}
}
@article{Wallentowitz2006i,
author = {Wallentowitz, Henning and Reif, Konrad},
doi = {10.1007/978-3-8348-9121-1_3},
isbn = {978-3-528-03971-4},
journal = {Handb. Kraftfahrzeugelektronik - Grundlagen, Kompon. Syst. Anwendungen},
title = {{Fahrwerksysteme}},
url = {http://www.springerlink.com/index/10.1007/978-3-8348-9121-1{\_}3},
year = {2006}
}
@article{Betriebsfestigkeita,
author = {Betriebsfestigkeit, Problemstellung Der},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Empirical Fatigue Models + Validation/Betriebsfestigkeit{\_}ErwinHaibach/Kap1 Einf{\"{u}}hrung und Uebersicht.pdf:pdf},
pages = {1--19},
title = {{1 Einf{\"{u}}hrung und {\"{U}}bersicht}}
}
@article{Der,
author = {Der, Bei and Fe-methode, Formulierung Der},
title = {{10 Grundgleichungen der nichtlinearen}}
}
@article{Stupkiewicz2007d,
author = {Stupkiewicz, Stanis{\l}aw},
doi = {10.1007/978-3-540-49717-2_9},
isbn = {3540497161},
issn = {16137736},
journal = {Lect. Notes Appl. Comput. Mech.},
number = {30},
pages = {151--170},
title = {{Formation of stress-induced martensitic plates}},
volume = {2006},
year = {2007}
}
@article{DASGUPTA2001a,
abstract = {This paper presents a micro-mechanistic approach for modeling fatigue damage initiation due to cyclic plasticity and cyclic creep in eutectic Pb-Sn solder. The issue of damage evolution is deferred to a future paper. Fatigue damage model due to cyclic plasticity is modeled with dislocation mechanics. A conceptual framework is provided to quantify the influence of temperature on fatigue damage due to cyclic plasticity. Damage mechanics due to cyclic creep is modeled with a void nucleation model based on micro-structural stress fields. Micro-structural stress states are estimated under viscoplastic phenomena like grain boundary sliding and its blocking at second phase particles, and diffusional creep relaxation. A conceptual framework is provided to quantify the creep-fatigue damage due to thermo-mechanical cycling.},
author = {DASGUPTA, A. and SHARMA, P. and UPADHYAYULA, K.},
doi = {10.1106/NM1B-1UQH-DJCT-4YH1},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Kriechen{\_}Spannungsrelaxation/2001{\_}Dasgubta{\_}Micro-Mechanics of fatigue due to vibration and thermal cycling.pdf:pdf},
issn = {10567895},
journal = {Int. J. Damage Mech.},
number = {2},
pages = {101--132},
title = {{Micro-Mechanics of Fatigue Damage in Pb-Sn Solder Due to Vibration and Thermal Cycling}},
url = {http://techpub.metapress.com/link.asp?target=contribution{\&}id=NM1B1UQHDJCT4YH1},
volume = {10},
year = {2001}
}
@article{Lin1969a,
abstract = {The mechanics of the build-up of large local plastic strains at the free surface of a polycrystal under fatigue loading is shown. Two closely located thin slices in a most-favourably-oriented crystal located at a free surface of the polycrystal are assumed to have an initial resolved shear stress of a few psi of opposite sign. Under cyclic loading, the two thin slices slide in opposite directions, one during the forward loading and the other during the reversed loading. Based on the dependency of slip on the resolved shear stress, the increase of local plastic strain in the slices with cycles of loading is calculated by applying the analogy between plastic strain and external force. The calculated local plastic shear strain in both slices (one positive and the other negative) reaches 100 per cent at the free surface in a few hundred cycles. These large plastic shear strains clearly cause the start of an extrusion or intrusion and the nucleation of a fatigue crack.},
author = {Lin, T H and Ito, Y M},
doi = {doi: DOI: 10.1016/0022-5096(69)90006-4},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/1969{\_}Lin{\_}Mechanics of a fatigue crack nucleation mechanism.pdf:pdf},
isbn = {0022-5096},
issn = {0022-5096},
journal = {J. Mech. Phys. Solids},
pages = {511--523},
title = {{Mechanics of a Fatigue Crack Nucleation Mechanism}},
url = {http://www.sciencedirect.com/science/article/pii/0022509669900064},
volume = {17},
year = {1969}
}
@article{Mesarovic2016,
abstract = {{\{}{\textcopyright}{\}} 2016 The Author(s) Published by the Royal Society. All rights reserved.Diffusional creep is characterized by growth/disappearance of lattice planes at the crystal boundaries that serve as sources/sinks of vacancies, and by diffusion of vacancies. The lattice continuum theory developed here represents a natural and intuitive framework for the analysis of diffusion in crystals and lattice growth/loss at the boundaries. The formulation includes the definition of the Lagrangian reference configuration for the newly created lattice, the transport theorem and the definition of the creep rate tensor for a polycrystal as a piecewise uniform, discontinuous field. The values associated with each crystalline grain are related to the normal diffusional flux at grain boundaries. The governing equations for Nabarro-Herring creep are derived with coupled diffusion and elasticity with compositional eigenstrain. Both, bulk diffusional dissipation and boundary dissipation accompanying vacancy nucleation and absorption, are considered, but the latter is found to be negligible. For periodic arrangements of grains, diffusion formally decouples from elasticity but at the cost of a complicated boundary condition. The equilibrium of deviatorically stressed polycrystals is impossible without inclusion of interface energies. The secondary creep rate estimates correspond to the standard Nabarro-Herring model, and the volumetric creep is small. The initial (primary) creep rate is estimated to be much larger than the secondary creep rate.},
author = {Mesarovic, Sinisa Dj},
doi = {10.1098/rspa.2016.0039},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Kriechen{\_}Spannungsrelaxation/2016{\_}Mesarovic{\_}Lattice{\_}continuum{\_}and{\_}diffusional{\_}creep.pdf:pdf},
isbn = {1471-2946},
issn = {14712946},
journal = {Proc. R. Soc. A Math. Phys. Eng. Sci.},
keywords = {materials science,mechanics},
number = {2188},
title = {{Lattice continuum and diffusional creep}},
volume = {472},
year = {2016}
}
@article{Geimer2012,
author = {Geimer, Marcus},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Vorlesungen/Fluidtechnik/Skript Fluidtechnik.pdf:pdf},
title = {{Vorlesung Fluidtechnik}},
year = {2012}
}
@article{Funktionb,
author = {Funktion, Eine},
journal = {Integr. Vlsi J.},
title = {{Approximation von Funktionen und Daten}}
}
@article{Bozza2011,
abstract = {In the present paper a combined procedure for the quasi-dimensional modelling of heat transfer, combustion and knock phenomena in a "downsized" Spark Ignition two-cylinder turbocharged engine is presented. The procedure is extended to also include the effects consequent the Cyclic Variability. Heat transfer is modelled by means of a Finite Elements model. Combustion simulation is based on a fractal description of the flame front area. Cyclic Variability (CV) is characterized through the introduction of a random variation on a number of parameters controlling the rate of heat release (air/fuel ratio, initial flame kernel duration and radius, laminar flame speed, turbulence intensity). The intensity of the random variation is specified in order to realize a Coefficient Of Variation (COV) of the Indicated Mean Effective Pressure (IMEP) similar to the one measured during an experimental campaign. Moreover, the relative importance of the various concurring effects is established on the overall COV. A kinetic scheme is then solved within the unburned gas zone, characterized by different thermodynamic conditions occurring cycle-by-cycle. In this way, an optimal choice of the "knock-limited" spark advance is effected and compared with experimental data. Finally, the CV effects on the occurrence of individual knocking cycles are assessed and discussed. {\textcopyright} 2011 Global Science Press.},
author = {Bozza, Fabio and Siano, Daniela and Costa, Michela},
doi = {10.4208/aamm.10-10s2-04},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2011{\_}Bozza{\_}heat-transfer-knock-modeling-and-cyclic-variability-in-a-downsized-spark-ignition-turbocharged-engine.pdf:pdf},
issn = {20700733},
journal = {Adv. Appl. Math. Mech.},
keywords = {Cyclic variability,Finite elements in heat transfer,Internal combustion engines modelling,Knock},
number = {3},
pages = {310--326},
title = {{Heat transfer, knock modeling and cyclic variability in a "Downsized" spark-ignition turbocharged engine}},
volume = {3},
year = {2011}
}
@article{Triebwerks,
author = {Triebwerks, Eigenschaften},
title = {{G des Triebwerks}}
}
@article{Fs2013,
author = {Fs},
doi = {10.1007/978-1-4614-0502-3},
isbn = {2009004043},
number = {1},
pages = {0--10},
title = {{Chapter 0}},
year = {2013}
}
@article{Sandoval2003a,
abstract = {A spark-ignition engine friction model developed by Patton et al. in the late 1980s was evaluated against current engine friction data, and improved. The model, which was based on a combination of fundamental scaling laws and empirical results, includes predictions of rubbing losses from the crankshaft, reciprocating, and valvetrain components, auxiliary losses from engine accessories, and pumping losses from the intake and exhaust systems. These predictions were based on engine friction data collected between 1980 and 1988. Some of the terms are derived from lubrication theory. Other terms were derived empirically from measurements of individual friction components from engine teardown experiments. Recent engine developments (e.g., improved oils, surface finish on piston liners, valve train mechanisms) suggested that the model needed updating. So modifications were made to the piston ring tension and gas pressure loading contributions to piston assembly friction, the impact of liner roughness, and to the valvetrain mechanism friction. Lubricant viscosity scaling was added to the hydrodynamic terms in the rubbing friction component models. The improved model now gives reasonable estimates of individual friction component and total spark-ignition engine friction mean effective pressure. The inclusion of oil viscosity scaling with temperature results in cold engine friction predictions about twice the value for warmed up engines. This agrees with the limited cold engine friction data available in the literature.},
archivePrefix = {arXiv},
arxivId = {2003-01-0725},
author = {Sandoval, Daniel and Heywood, John B},
doi = {10.4271/2003-01-0725},
eprint = {2003-01-0725},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2003{\_}Sandoval{\_}An Imporved Friction Model for Spark{\_}Ign Engines.pdf:pdf},
isbn = {0148-7191},
title = {{An Improved Friction Model for Spark-Ignition Engines}},
url = {http://papers.sae.org/2003-01-0725/},
year = {2003}
}
@article{Chang2004b,
abstract = {An experimental study has been carried out to provide qualitative and quantitative insight into gas to wall heat transfer in a gasoline fueled Homogeneous Charge Compression Ignition (HCCI) engine. Fast response thermocouples are embedded in the piston top and cylinder head surface to measure instantaneous wall temperature and heat flux. Heat flux measurements obtained at multiple locations show small spatial variations, thus confirming relative uniformity of incylinder conditions in a HCCI engine operating with premixed charge. Consequently, the spatially-averaged heat flux represents well the global heat transfer from the gas to the combustion chamber walls in the premixed HCCI engine, as confirmed through the gross heat release analysis. Heat flux measurements were used for assessing several existing heat transfer correlations. One of the most popular models, the Woschni expression, was shown to be inadequate for the HCCI engine. The problem is traced back to the flame propagation term which is not appropriate for the HCCI combustion. Subsequently, a modified model is proposed which significantly improves the prediction of heat transfer in a gasoline HCCI engine and shows very good agreement over a range of conditions},
author = {Chang, Junseok and G{\"{u}}ralp, Orgun and Filipi, Zoran and Assanis, Dennis N. and Kuo, Tang-Wei and Najt, Paul and Rask, Rod},
doi = {10.4271/2004-01-2996},
file = {:C$\backslash$:/Users/p327208/Desktop/Promotion/Literature/Motorspezifisch/Heat Transfer Combustion Chamber/2004{\_}Chang{\_}New Heat Transfer Correlation for an HCCI Engine Derived from Measurements of Instantaneous Surface Heat Flux.pdf:pdf},
isbn = {0148-7191},
issn = {0148-7191},
number = {724},
title = {{New Heat Transfer Correlation for an HCCI Engine Derived from Measurements of Instantaneous Surface Heat Flux}},
url = {http://papers.sae.org/2004-01-2996/},
year = {2004}
}
@article{Borg2006,
author = {Borg, Jm and Alkidas, Ac},
doi = {10.4271/2006-01-3341},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2006{\_}Borg{\_}Characterisation of autoignition in a knocking si engine using heat release analysis.pdf:pdf},
journal = {SAE Tech. Pap.},
number = {724},
pages = {776--790},
title = {{Characterization of autoignition in a knocking SI engine using heat release analysis}},
url = {http://papers.sae.org/2006-01-3341/},
volume = {2006-01-33},
year = {2006}
}
@book{HuseyinSehitoglu2000a,
author = {{Huseyin Sehitoglu} and {Hans J. Maier}},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/2000{\_}Huseyin Sehitoglu{\_}Thermo-mechanical Fatigue Behavior of  Materials{\_}OverviewDifferentPapers.pdf:pdf},
isbn = {0803128533},
pages = {151},
title = {{Thermo-mechanical Fatigue Behavior of Materials: Third volume}},
url = {https://books.google.se/books?id=ZY84rIMG82sC{\%}7B{\&}{\%}7Dpg=PA150{\%}7B{\&}{\%}7Dlpg=PA150{\%}7B{\&}{\%}7Ddq=thermomechanical+fatigue+behavior+of+materials{\%}7B{\&}{\%}7Dsource=bl{\%}7B{\&}{\%}7Dots=93h1yoyJVR{\%}7B{\&}{\%}7Dsig=YTp4LbQdi6Kms-Ys06yBsW5LnPU{\%}7B{\&}{\%}7Dhl=sv{\%}7B{\&}{\%}7Dsa=X{\%}7B{\&}{\%}7Dved=0ahUKEwidx4jg2},
year = {2000}
}
@article{Papadopoulos1997,
abstract = {The aim of this paper is firstly, to provide a concise assessment of some commonly used high-cycle fatigue criteria and secondly, to check their predictive capabilities against synchronous sinusoidal out-of-phase bending and torsion experimental results (i.e. sinusoidal stress signals of the same frequency but with a phase difference). This bending-torsion stress system does not closely represent real load conditions undergone by a machine part. However, it is complex enough to differentiate the various fatigue criteria and to permit a first classification of the approaches examined, according to the accuracy of their predictions. A fatigue criterion recently formulated by the first of the authors is also included in this comparative study. According to this criterion the phase difference in out-of-phase bending and torsion does not affect the fatigue strength corresponding to a very high (theoretically infinite) fatigue life. It is pointed out that this theoretical finding is valid for the category of hard metals for which the ratio of the fully re-versed torsion fatigue limit over the fully reversed bending fatigue limit lies in the interval from 1√3 o approx. 0.8. Experimental results collected from the relevant literature, concerning precisely lard metals, fully support this theoretical finding.},
author = {Papadopoulos, I},
doi = {10.1016/S0142-1123(96)00064-3},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Empirical Fatigue Models + Validation/1996{\_}Papadopoulos{\_}A comparative study of multiaxial high cycle fatigue criteria for metals .pdf:pdf},
isbn = {0142-1123},
issn = {01421123},
journal = {Int. J. Fatigue},
keywords = {cycle fatigue,high,loading,metals,multiaxial fatigue,n o n -,o n a l,o r t i,p r o p},
number = {3},
pages = {219--235},
title = {{A comparative study of multiaxial high-cycle fatigue criteria for metals}},
url = {http://linkinghub.elsevier.com/retrieve/pii/S0142112396000643},
volume = {19},
year = {1997}
}
@article{Modelle,
author = {Modelle, Response Surface},
title = {{6 Optimierungsstrategien}}
}
@article{Shojaefard2005,
author = {Shojaefard, M. H. and Noorpoor, A. R. and Bozchaloe, D. A. and Ghaffarpour, M.},
doi = {https://doi.org/10.1080/10407780590959943},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Heat transfer intake+exhaust system/2005{\_}Shojaefard+Noorpoor{\_}Transient Thermal Analysis of Engine Exhaust Valve.pdf:pdf},
journal = {Numer. Heat Transf. Part A Appl.},
number = {7},
pages = {627--644},
title = {{Transient Thermal Analysis of Engine Exhaust Valve}},
volume = {48},
year = {2005}
}
@article{Stupkiewicz2007,
author = {Stupkiewicz, Stanis{\l}aw},
doi = {10.1007/978-3-540-49717-2_8},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Stupkievicz 2007 - Micromechanics of Contact and Interphase Layers/97165{\_}08.pdf:pdf},
isbn = {3540497161},
issn = {16137736},
journal = {Lect. Notes Appl. Comput. Mech.},
number = {30},
pages = {115--149},
title = {{Evolving laminates in shape memory alloys}},
volume = {2006},
year = {2007}
}
@article{Datenspeicher,
author = {Datenspeicher, Optische},
number = {Cd},
pages = {161--166},
title = {{11 Audio-Video-Technik}}
}
@article{Ganczarski2003a,
author = {Ganczarski, A},
doi = {10.1007/978-3-540-36418-4_10},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Anisotropic Behaviouir of Damaged Materials{\_}Skrzypek{\_}ARTICEL/Kap10{\_}Thermo-Damage Coupling Modelling and Applications for Creep Conditions.pdf:pdf},
isbn = {9783642055874},
issn = {16137736},
journal = {Lect. Notes Appl. Comput. Mech.},
keywords = {creep conditions,metallic materials,thermo-damage coupling},
pages = {317--349},
title = {{Thermo-Damage Coupling Modelling and Applications for Creep Conditions}},
volume = {9},
year = {2003}
}
@article{Gesamtprozessanalyse,
author = {Gesamtprozessanalyse, Als and Modellierung, Die},
pages = {385--414},
title = {{Gesamtprozessanalyse}}
}
@article{Chaboche1989a,
abstract = {The cyclic constitutive equations developed and used at ONERA and LMT-Cachan are presented in detail in terms of a hierarchy of various models. Both the time-independent and the viscoplasticity versions of the equations are discussed, as well as their ability to describe correctly most of the experimentally observed effects under monotonic or cyclic loading, constant or variable temperature, including strain hardening and time recovery effects. The reported experimental data concerns stainless steels and have been published previously. Four other theories are then presented and compared in a systematic way. They include the Ohno-Kachi time-independent plasticity theory, two unified viscoplastic models by Walker and by Krempl and Yao, the new developments of the endochronic theory by Watanabe and Atluri. All these approaches show some similarities with the first one, especially in that concerns the non.linearity of kinematic hardening, which represents the key for describing the cyclic behav- iour of metallic materials.},
author = {Chaboche, J L},
doi = {http://dx.doi.org/10.1016/0749-6419(89)90015-6},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/Hardening Recovery Creep/1989{\_}Chaboche{\_}Constitutive equations for cyclic plasticity and cyclic viscoplasticity.pdf:pdf},
isbn = {1111111111},
issn = {0749-6419},
journal = {Int. J. Plast.},
pages = {247--302},
title = {{Constitutive equations for cyclic plasticty and cyclic viscoplasticity}},
volume = {5},
year = {1989}
}
@book{Borbely2006a,
abstract = {Loss of cortical gray matter is accompanied by a commensurate increase in the sulcal and intraventricular cerebrospinal fluid volume. On diffusion-weighted magnetic resonance imaging, this would be reflected as a higher apparent diffusion coefficient in affected brain regions. On the basis of the above premise, we suggest that the apparent diffusion coefficient may be used as a surrogate marker for the assessment of regional brain volume deficits. We demonstrate this approach by voxelwise analysis of registered apparent diffusion coefficient images from a group of 15 patients with schizophrenia and 15 age-matched healthy controls. We found widespread regional apparent diffusion coefficient increases in patients. Affected areas included the bilateral insular cortex, hippocampus, temporal lobe, and occipital areas. These results largely concur with previous findings of cortical volume deficits in schizophrenia.},
author = {Borbely, Anne-marie and Kreider, Jan F and Bejan, Adrian and Cundiff, John S and Davis, Lorin R},
booktitle = {Mech. Compos. Mater.},
doi = {10.1021/ja00116a001},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Plasticity models/Elastoplasticity Theory{\_}Lubarda{\_}2002.pdf:pdf},
isbn = {9780849391392},
issn = {9780849391378},
pages = {1455--1459},
title = {{Distributed Generation : The Power Paradigm for the New Millennium Fluid Power Circuits and Controls : Fundamentals and Applications}},
url = {http://www.ncbi.nlm.nih.gov/pubmed/16110271},
volume = {23},
year = {2006}
}
@article{Aufgabeb,
author = {Aufgabe, Die and Gleichung, Navier- Stokessche and Prandtl, Ludwig and Gleichung, Navier-stokesschen and Grenzschichtgleichung, Prandtlsche and Grenzschichtgleichungen, Prandtlschen and Grenzschichttheorie, Prandtlschen},
title = {{Kapitel 12 Grenzschichttheorie}}
}
@article{Principal,
author = {Principal, A},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Zienkiewicz FEM - Vol 2 Solid Structural Mechanics/63212{\_}apdxb.pdf:pdf},
pages = {1--5},
title = {{Invariants of second-order tensors}},
volume = {13}
}
@article{Background,
author = {Background, General},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Stupkievicz 2007 - Micromechanics of Contact and Interphase Layers/97165{\_}10.pdf:pdf},
journal = {Mathematica},
pages = {1--207},
title = {{1.0 Remarks}}
}
@article{Contentsa,
author = {Contents, Chapter},
title = {{Solution of Simultaneous Linear Algebraic Equations 3.1}}
}
@article{Liu2005a,
abstract = {A new high-cycle fatigue criterion based on the critical plane approach is proposed in this paper. Unlike most of the other multiaxial fatigue criteria based on the critical plane approach, the critical plane is directly correlated with the fatigue fracture plane. The proposed criterion has a wide range of applicability from very ductile metals to extremely brittle metals. Mean stress effect is also included in this criterion. The new fatigue criterion is then extended to a fatigue life prediction model. The results of the proposed fatigue criterion and fatigue life prediction model are validated with experimental results from the literature. ?? 2005 Elsevier Ltd. All rights reserved.},
author = {Liu, Yongming and Mahadevan, Sankaran},
doi = {10.1016/j.ijfatigue.2005.01.003},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Empirical Fatigue Models + Validation/2005{\_}Mahadevan{\_}Multiaxial high-cycle fatigue criterion and life prediction for metals.pdf:pdf},
isbn = {01421123},
issn = {01421123},
journal = {Int. J. Fatigue},
keywords = {Critical plane,High-cycle fatigue,Life prediction,Metals,Multiaxial fatigue},
number = {7},
pages = {790--800},
title = {{Multiaxial high-cycle fatigue criterion and life prediction for metals}},
volume = {27},
year = {2005}
}
@article{Werdich2011,
author = {Werdich, Martin},
doi = {10.1007/978-3-8348-9951-4_6},
isbn = {978-3-8348-1433-3},
journal = {FMEA – Einf{\"{u}}hrung und Moderation},
pages = {101--108},
title = {{6 Software}},
url = {http://www.springerlink.com/index/10.1007/978-3-8348-9951-4},
year = {2011}
}
@article{Chaboche2003,
abstract = {Constitutive and damage mechanics equations of composite materials are developed and discussed in the framework of micromechanics based approaches, including some recent modeling capabilities. The approach is based on the Transformation Field Analysis (TFA) promoted by Dvorak. A correction method is proposed in order to obtain a softer overall hardening response in case of the model restriction to only two subdomains (the elastic fibre, and the elasto-plastic matrix). In order to take into account the effects of temperature and damage on the elastic properties, a Generalised Eigenstrain Method (GEM) is developed, that uses the corresponding additional strains as eigenstrains. Its validity is checked by means of finite element numerical simulations based on periodic homogenisation. The methodology is further developed for metal matrix composites in which the matrix is treated as a polycristalline aggregate and slip plasticity is written at the level of slip systems. Two imbricated scale transitions are performed, both based on TFA like rules and it is shown how the overall constitutive equations can be considered as a multi-mechanism flow rule with pseudo-slip systems. Application of the model is made for a SiC/Ti composite. The capabilities are discussed by comparison with some experimental results, including monotonic and cyclic transverse loading conditions.},
author = {Chaboche, J. L. and Carr??re, N.},
doi = {10.1007/978-3-540-36418-4_2},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Anisotropic Behaviouir of Damaged Materials{\_}Skrzypek{\_}ARTICEL/Kap2{\_}Multiscale Structural Analyses Incorporating Damage Mechanics at the Meso- or Micro-Scales.pdf:pdf},
isbn = {9783642055874},
issn = {16137736},
journal = {Lect. Notes Appl. Comput. Mech.},
keywords = {Viscoplasticity,damage mechanics,metal matrix composites,micromechanics,scale transitions},
pages = {35--74},
title = {{Multiscale Structural Analyses Incorporating Damage Mechanics at the Meso- or Micro-Scales}},
volume = {9},
year = {2003}
}
@article{Brij,
author = {Brij, N},
journal = {Advances},
pages = {1--2},
title = {{Author Index *}},
volume = {115}
}
@article{Moser,
author = {Moser, Andreas and Steffan, Hermann},
journal = {Simulation},
pages = {559--568},
title = {{A18 A18 Insassensimulation A18}}
}
@article{Controller1981,
author = {Controller, Jeder and Entwicklung, Die and Intel, Firma},
title = {{Prozessorarchitekturen im {\"{U}}berblick}},
year = {1981}
}
@article{Kalghatgi1995a,
abstract = {Net heat release, knock characteristics and temperature were derived{\$}\backslash{\$}nfrom in-cylinder pressure and end-gas CARS measurements for different{\$}\backslash{\$}nfuels in a single-cylinder engine. The maximum net heat release rate{\$}\backslash{\$}nresulting from the final phase of autoignition is closely associated{\$}\backslash{\$}nwith knock intensity. Aromatic fuels have lower maximum heat release{\$}\backslash{\$}nrates and lower knock intensities than expected from their octane number{\$}\backslash{\$}nwhen compared to paraffinic fuels; this is observed even when there is{\$}\backslash{\$}nsignificant heating of the end-gas from pre-flame reactions. Leaner{\$}\backslash{\$}nmixtures have lower combustion rates so that pressure development is{\$}\backslash{\$}nslowed and hence ignition needs to be more advanced to get knock to{\$}\backslash{\$}noccur as frequently as in a richer mixture. However, for a given{\$}\backslash{\$}nfrequency of knock occurrence, there is no significant difference in{\$}\backslash{\$}npeak net heat release rates and hence in knock intensities for different{\$}\backslash{\$}nmixture strengths.},
author = {Kalghatgi, G T and Golombok, M and Snowdon, P},
doi = {10.1080/00102209508951924},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Klopfen{\_}Ottomotor/2007{\_}Kalghatgi{\_}Fuel effect on knock - heat release and CARS tempertures in SI Engine.pdf:pdf},
issn = {0010-2202},
journal = {Combust. Sci. Technol.},
number = {March},
pages = {209--228},
title = {{Fuel effects on knock, heat release and `'CARS'' temperatures in a spark ignition engine}},
volume = {111},
year = {1995}
}
@article{Konstruktionb,
author = {Konstruktion, C Manuelle},
pages = {188--206},
title = {{27 Innenraum ( Interieur )}}
}
@article{Plewinsky,
author = {Plewinsky, B and Hennecke, M and Oppermann, W},
journal = {H{\{}{\"{u}}{\}}tte},
pages = {1--114},
title = {{C-Chemie}}
}
@article{Auflosungsgrenze,
author = {Aufl{\"{o}}sungsgrenze, Abbe and Zahl, Abbe and Mikroskoptheorie, Abbe},
journal = {H{\{}{\"{u}}{\}}tte},
pages = {1--62},
title = {{S-Sachverzeichnis}}
}
@article{Papadopoulos1997a,
abstract = {The aim of this paper is firstly, to provide a concise assessment of some commonly used high-cycle fatigue criteria and secondly, to check their predictive capabilities against synchronous sinusoidal out-of-phase bending and torsion experimental results (i.e. sinusoidal stress signals of the same frequency but with a phase difference). This bending-torsion stress system does not closely represent real load conditions undergone by a machine part. However, it is complex enough to differentiate the various fatigue criteria and to permit a first classification of the approaches examined, according to the accuracy of their predictions. A fatigue criterion recently formulated by the first of the authors is also included in this comparative study. According to this criterion the phase difference in out-of-phase bending and torsion does not affect the fatigue strength corresponding to a very high (theoretically infinite) fatigue life. It is pointed out that this theoretical finding is valid for the category of hard metals for which the ratio of the fully re-versed torsion fatigue limit over the fully reversed bending fatigue limit lies in the interval from 1√3 o approx. 0.8. Experimental results collected from the relevant literature, concerning precisely lard metals, fully support this theoretical finding.},
author = {Papadopoulos, I},
doi = {10.1016/S0142-1123(96)00064-3},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Empirical Fatigue Models + Validation/1996{\_}Papadopoulos{\_}A comparative study of multiaxial high cycle fatigue criteria for metals .pdf:pdf},
isbn = {0142-1123},
issn = {01421123},
journal = {Int. J. Fatigue},
keywords = {cycle fatigue,high,loading,metals,multiaxial fatigue,n o n -,o n a l,o r t i,p r o p},
number = {3},
pages = {219--235},
title = {{A comparative study of multiaxial high-cycle fatigue criteria for metals}},
url = {http://linkinghub.elsevier.com/retrieve/pii/S0142112396000643},
volume = {19},
year = {1997}
}
@phdthesis{DanielGhebru2013a,
author = {Ghebru, Daniel},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2009{\_}GhebruDaniel{\_}Modellierung und Analyse des instationaeren thermischen Verhaltens von VKM und Gesamtfahrzeug - Beitrag Woschni+Zapf.pdf:pdf},
isbn = {9783832534325},
keywords = {Co-Simulation,Instation{\"{a}}res Thermomanagement,Modellbildung,Thermische Gesamtfahrzeugsimulation,Thermisches Motormodell},
number = {April},
school = {Karlsruhe Institute of Technology (KIT)},
title = {{Modellierung und Analyse des instation{\"{a}}ren thermischen Verhaltens von Verbrennungsmotor und Gesamtfahrzeug}},
year = {2013}
}
@article{Kraftstoffverbrauch,
author = {Kraftstoffverbrauch, Der and Pra-, Der},
pages = {189--204},
title = {{7 Kraftstoffverbrauch}}
}
@article{Raffinerien,
author = {Raffinerien, In Den},
journal = {Forschung},
title = {{13 Betriebsstoffe}}
}
@article{Chemie1806,
author = {Chemie, Organische},
title = {{1 Einf{\{}{\"{u}}{\}}hrung}},
year = {1806}
}
@article{Borg2006a,
author = {Borg, Jm and Alkidas, Ac},
doi = {10.4271/2006-01-3341},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2006{\_}Borg{\_}Characterisation of autoignition in a knocking si engine using heat release analysis.pdf:pdf},
journal = {SAE Tech. Pap.},
number = {724},
pages = {776--790},
title = {{Characterization of autoignition in a knocking SI engine using heat release analysis}},
url = {http://papers.sae.org/2006-01-3341/},
volume = {2006-01-33},
year = {2006}
}
@article{Erstes,
author = {Erstes, Als and Beschleunigen, Ein},
title = {{Einf u ¨ hrung}}
}
@article{Band-,
author = {Band-, Die and Systeme, Moderne and Wabenstruktur, Die},
pages = {365--382},
title = {{Abgasnachbehandlungssysteme}}
}
@article{Stanley1999,
abstract = {This paper presents a simplified piston ring assembly (PRA) friction model of the piston ring pack and the piston skirt. The ring model considers both mixed and hydrodynamic lubrication; the skirt model considers hydrodynamic lubrication only. The Reynold's equation is used as a governing equation for the hydrodynamic regimes of both models. Simplified assumptions are used to include mixed lubrication in the ring model. The ring model generates unique Stribeck curves for a given ring's geometry; the skirt model generates generic relationships between the friction force and skirt geometry, piston speed, oil viscosity, and assumed boundary conditions. Inter-ring starvation effects are introduced by varying the boundary conditions, as appropriate. The models are compared to measurements made on a motored and fired single-cylinder diesel engine; the theoretical calculations provide a reasonable estimate of the measured data. .},
author = {Stanley, Richard and Taraza, Dinu and Henein, Naeim and Bryzik, Walter},
doi = {10.4271/1999-01-0974},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Mechanik+Reibung/1999{\_}Stanley{\_}A Simplified Friction Model of the Piston Ring Assembly.pdf:pdf},
isbn = {SAE 1999-01-0974},
number = {724},
title = {{A Simplified Friction Model of the Piston Ring Assembly}},
url = {http://papers.sae.org/1999-01-0974/},
year = {1999}
}
@book{Bazant1992,
abstract = {Elasticity, plasticity, damage mechanics and cracking are all phenomena that determine the resistance of solids to deformation and fracture. The authors of this book discuss a modern method of mathematically modeling the behavior of macroscopic volume elements. The first three chapters review physical mechanisms at the microstructural level, thermodynamics of irreversible processes, mechanics of continuous media, and the classification of the behavior of solids. The rest of the book is devoted to the modeling of different types of material behavior. In each case the authors present characteristic data for numerous materials, and discuss the physics underlying the phenomena together with methods for the numerical analysis of the resulting equations.},
author = {Ba{\v{z}}ant, Z. P.},
booktitle = {Can. J. Civ. Eng.},
doi = {10.1139/l92-025},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Kriechen{\_}Spannungsrelaxation/1985{\_}Jean{\_}Lemaitre+Jean-Louis+Chaboche{\_}Mechanics{\_}of{\_}Solid{\_}Materials.pdf:pdf},
isbn = {0521477581},
issn = {0315-1468},
number = {1},
pages = {197--197},
title = {{Mechanics of solid materials}},
url = {http://www.nrcresearchpress.com/doi/abs/10.1139/l92-025},
volume = {19},
year = {1992}
}
@article{Zugabe,
author = {Zugabe, Zweck Der},
pages = {102--171},
title = {{3 Additive}}
}
@article{Motork,
author = {Motork, Interne},
title = {{Motork{\"{u}}hlung}}
}
@article{Elektrotechnik2017,
author = {Elektrotechnik, Grundbegriffe Der},
isbn = {978-3-8348-0032-9},
pages = {115--160},
title = {{Grundbegriffe der Elektrotechnik 5.1}},
year = {2017}
}
@article{Entwicklung2010,
author = {Entwicklung, Zur},
journal = {System},
number = {1986},
title = {{1 Das mechatronische Kraftfahrzeug}},
year = {2010}
}
@article{Gross2011h,
author = {Gross, Dietmar and Seelig, Thomas},
doi = {10.1007/978-3-642-10196-0},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Gross, Selig 2011 - Bruchmechanik/Gross, Seelig - 2011 - BruchmechanikKap7.pdf:pdf},
isbn = {978-3-642-10195-3},
title = {{Bruchmechanik}},
url = {http://link.springer.com/10.1007/978-3-642-10196-0},
year = {2011}
}
@article{Payne2010a,
abstract = {This paper reports the results of a study of the initial stages of fatigue crack formation in the commercial aluminum alloy 7075-T651. Direct observations were made of the evolution of cracking in a notch under moderately high fatigue loads in a scanning electron microscope. The experimental conditions were designed to mimic the behavior of fastener holes in the lower wing covers of military attack aircraft, thus the loading parameters were such that local plasticity was expected. Constituent particle cracking was observed to be the sole cause of fatigue crack initiation in these experiments; particle debonding was not a factor. The iron-bearing constituent particles were the sites of nearly all of the cracks initiated by fatigue. Mg2Si particles were not effective crack initiation sites. This was attributed to the difference in the moduli of the particles: the iron-bearing particles were harder than the matrix while the Mg2Si particles were softer. A large fraction of the cracks in the constituent particles were present before any loading was applied, but a certain amount of additional constituent particle cracking was caused by the fatigue loading. A cracked constituent particle eventually gave rise to a crack in the surrounding matrix, but this process required the application of fatigue loads. No matrix cracks were observed prior to fatigue loading. Subsequent propagation of the matrix cracks also required additional fatigue cycling. These observations are being used in the development of detailed computer models of the fatigue process in 7075-T651. ?? 2009 Elsevier Ltd.},
author = {Payne, Joel and Welsh, Greg and Christ, Robert J. and Nardiello, Jerrell and Papazian, John M.},
doi = {10.1016/j.ijfatigue.2009.06.003},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/2 scale models papers/2010{\_}Papazian{\_}Observations of fatigue crack initiation in 7075-T651.pdf:pdf},
isbn = {0142-1123},
issn = {01421123},
journal = {Int. J. Fatigue},
keywords = {7075-T651,Aluminum alloy 7075,Crack initiation,Fatigue,Scanning electron microscopy},
number = {2},
pages = {247--255},
publisher = {Elsevier Ltd},
title = {{Observations of fatigue crack initiation in 7075-T651}},
url = {http://dx.doi.org/10.1016/j.ijfatigue.2009.06.003},
volume = {32},
year = {2010}
}
@article{Rechnena,
author = {Rechnen, Wissenschaftlichen},
isbn = {3-540-25005-0},
journal = {System},
title = {{2 Nichtlineare Gleichungen}},
volume = {2}
}
@book{Gross2011f,
author = {Gross, Dietmar and Seelig, Thomas},
doi = {10.1007/978-3-642-10196-0},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Gross, Selig 2011 - Bruchmechanik/Gross, Seelig - 2011 - BruchmechanikKap8.pdf:pdf},
isbn = {978-3-642-10195-3},
title = {{Bruchmechanik}},
url = {http://link.springer.com/10.1007/978-3-642-10196-0},
year = {2011}
}
@article{Numerical2003,
author = {Numerical, Advanced},
number = {4},
pages = {257--263},
title = {{Advanced Numerical Methods}},
year = {2003}
}
@article{Zienkiewicz2014e,
author = {Zienkiewicz, O.C. and Taylor, R.L. and Fox, David},
doi = {10.1016/B978-1-85617-634-7.00025-9},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Zienkiewicz FEM - Vol 2 Solid Structural Mechanics/63212{\_}apdxa.pdf:pdf},
journal = {Finite Elem. Method Solid Struct. Mech.},
pages = {597--603},
title = {{Isoparametric Finite Element Approximations}},
url = {http://linkinghub.elsevier.com/retrieve/pii/B9781856176347000259},
year = {2014}
}
@article{L,
author = {L, Bei Der},
doi = {10.1007/978-3-642-24335-6},
isbn = {9783642243356},
title = {{6 Differenzenverfahren}}
}
@article{Betrachtungenh,
author = {Betrachtungen, Allgemeine},
title = {{omungen mit W ¨ arme u ¨ bertragung}}
}
@article{Hashin1963,
abstract = {Variational principles in the linear theory of elasticity, involving the elastic polarization tensor, have been applied to the derivation of upper and lower bounds for the effective elastic moduli of quasi-isotropic and quasi-homogeneous multiphase materials of arbitrary phase geometry. When the ratios between the different phase moduli are not too large the bounds derived are close enough to provide a good estimate for the effective moduli. Comparison of theoretical and experimental results for a two-phase alloy showed good agreement.},
author = {Hashin, Zvi and Shtrikman, Shmuel},
doi = {10.1016/0022-5096(63)90060-7},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/Strukturmechanik MMS/Literatur/Hashin Shtrikman 1963.pdf:pdf},
isbn = {0022-5096},
issn = {00225096},
journal = {J. Mech. Phys. Solids},
number = {2},
pages = {127--140},
title = {{A variational approach to the theory of the elastic behaviour of multiphase materials}},
url = {http://linkinghub.elsevier.com/retrieve/pii/0022509663900607},
volume = {11},
year = {1963}
}
@article{Schwingbeanspruchung,
author = {Schwingbeanspruchung, Kennzeichnung Der},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Empirical Fatigue Models + Validation/Betriebsfestigkeit{\_}ErwinHaibach/Kap2 Experimentelle Grundlagen und Betriebsfestigkeit.pdf:pdf},
title = {{2 Experimentelle Grundlagen der Betriebsfestigkeit}}
}
@article{Umwandlung2008,
author = {Umwandlung, Die},
doi = {10.1007/978-3-642-24161-1},
isbn = {9783642241611},
title = {{8 Thermodynamik der W ¨ armekraftanlagen}},
year = {2008}
}
@article{Gurtin1967a,
author = {Gurtin, Morton E and Williams, William O},
doi = {10.1007/BF00285676},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Thermodynamik/An Axiomatic Foundation for Continuum Thermodynamics{\_}CommunicatedByNoll.pdf:pdf},
issn = {00039527},
journal = {Arch. Ration. Mech. Anal.},
number = {2},
pages = {83--117},
title = {{An axiomatic foundation for continuum thermodynamics}},
volume = {26},
year = {1967}
}
@article{Voyiajis2005,
author = {Voyiajis, G. Z.},
doi = {10.1016/j.mechmat.2004.10.003},
journal = {Handb. Mater. Model.},
pages = {1183},
title = {{Continuum damage mechanics}},
url = {http://link.aip.org/link/?JEMTA8/107/83/1},
year = {2005}
}
@article{Peters1996,
author = {Peters, S T},
journal = {Handb. Compos.},
pages = {1--20},
title = {{Introduction , Composite Basics and Road Map}},
year = {1996}
}
@article{Sanli2009,
author = {Sanli, A and Sayin, C and Gumus, M and Kilicaslan, I and Canakci, M},
doi = {https://doi.org/10.1080/10407780903244312},
journal = {Numer. Heat Transf. Part A Appl.},
number = {5},
pages = {444--458},
title = {{Numerical Evaluation by Models of Load and Spark Timing Effects on the In-Cylinder Heat Transfer of a SI Engine}},
volume = {56},
year = {2009}
}
@article{Rodi1991,
author = {Rodi, Wolfgang},
doi = {https://doi.org/10.2514/6.1991-216},
journal = {AIAA},
title = {{Experience with two-layer models combining the k-epsilon model with a one-equation model near the wall}},
volume = {91-0216},
year = {1991}
}
@article{Beispield,
author = {Beispiel, Dieses},
pages = {59--69},
title = {{6 Welle}}
}
@article{Downsizing,
author = {Downsizing, Begriffe and Prinzip, Das and Downsizing, Der Begriff},
pages = {205--211},
title = {{8 Downsizing und Downspeeding}}
}
@article{Tong2013,
abstract = {Ratchetting deformation has significant implications on material damage and fatigue life of components under service loading conditions. In this work, we explore the concept of ratchetting strain as a driving force in controlling crack growth, both time-independent and time-dependent, utilising elasto-plastic, visco-plastic and crystal-plasticity constitutive models. Characteristics of crack tip deformation were examined for both stationary and growing cracks using the finite element method. Whilst the strain range and the stress range remained largely unchanged throughout the loading cycles, distinctive strain ratchetting behaviour near the crack tip occurred in all cases, leading to progressive accumulation of tensile strain normal to the crack growth plane. It seems plausible that this tensile strain, or ratchetting strain, may be responsible for material separation leading to crack growth. The effects of material constitutive model, grain orientation and loading frequency on the development of ratchetting strain were also examined. Ratchetting strain was found to be related to accumulated plastic strain; and both were used in a crack growth criterion with which the crack growth rates of a nickel alloy were predicted. The preliminary results seem to be encouraging. ?? 2012 Elsevier Ltd. All rights reserved.},
author = {Tong, J. and Zhao, L. G. and Lin, B.},
doi = {10.1016/j.ijfatigue.2012.01.003},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/2013{\_}Tong+Zhao+Lin{\_}Ratchetting strain as a driving force for fatigue crack growth.pdf:pdf},
isbn = {01421123},
issn = {01421123},
journal = {Int. J. Fatigue},
keywords = {Constitutive model,Crack tip,Fatigue crack growth,Ratchetting},
pages = {49--57},
publisher = {Elsevier Ltd},
title = {{Ratchetting strain as a driving force for fatigue crack growth}},
url = {http://dx.doi.org/10.1016/j.ijfatigue.2012.01.003},
volume = {46},
year = {2013}
}
@article{Outline,
author = {Outline, Historical},
journal = {High Temp.},
pages = {1--12},
title = {{Material Properties for High Temperature}}
}
@article{Gross2011b,
author = {Gross, Dietmar and Seelig, Thomas},
doi = {10.1007/978-3-642-10196-0},
isbn = {978-3-642-10195-3},
title = {{Bruchmechanik}},
url = {http://link.springer.com/10.1007/978-3-642-10196-0},
year = {2011}
}
@article{Hasan2007,
author = {Hasan, Basim O},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Boiling/Turbulence/2007{\_}Basim+Hasan{\_}Turbulent Prandtl Number and its Use in Prediction of Heat Transfer Coefficient of Liquids.pdf:pdf},
journal = {Coll. Eng. J.},
number = {1},
pages = {53--64},
title = {{Turbulent Prandtl Number and its Use in Prediction of Heat Transfer Coefficient for Liquids}},
volume = {10},
year = {2007}
}
@article{Bertram2008,
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Bertram, Albrecht},
doi = {10.1007/978-3-540-69400-7},
eprint = {arXiv:1011.1669v3},
isbn = {978-3-540-69399-4},
issn = {1098-6596},
pmid = {25246403},
title = {{Elasticity and Plasticity of Large Deformations}},
url = {http://link.springer.com/10.1007/978-3-540-69400-7},
year = {2008}
}
@article{Ablauf,
author = {Ablauf, F{\"{u}}r Den and Dehnung, Thermische},
journal = {System},
pages = {32--58},
title = {{3 Stoffeigenschaften}}
}
@article{Basara2017,
author = {Basara, B and {\v{Z}}uni, Z},
doi = {10.1016/j.ijheatfluidflow.2016.06.019},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Thermal Coating + Water Heat Transfer + Applikation/2013{\_}Saric+Basara{\_}Advanced near-wall modeling for engine heat transfer.pdf:pdf},
journal = {Int. J. Heat Fluid Flow},
pages = {205--211},
title = {{International Journal of Heat and Fluid Flow Advanced near-wall modeling for engine heat transfer}},
volume = {63},
year = {2017}
}
@article{Takeuchi1982,
abstract = {Plastic behavior of single crystals of Cu52Zn48 alloy with the CsCl structure has been examined over a temperature range between 2 K and room temperature. Both at 4.2 K and 77 K, the operative slip plane is the twinning {\{}112{\}} plane in most orientations and it is the anti-twinning {\{}112{\}} plane only in orientations with the maximum shear stress plane close to the anti-twinning {\{}112{\}} plane. Orientation dependence of the yield stress ??mssp showed a maximum near the orientation of the slip plane transition. These results agree well with those of computer simulation of superlattice screw dislocation motion [S. Takeuchi, Phil. Mag. A 41, 541 (1980)]. Temperature and strain-rate dependences of yield stress below {\~{}}130K are essentially similar to those in bcc metals. The above results together with in situ TEM observation indicate that low temperature deformation in ??-CuZn is governed by motion of screw dislocations overcoming the Peierls potential. Activation analyses revealed that the value of exponent in the Arrhenius rate equation, ??H kT, decreases rapidly below 10 K toward zero at 0 K, showing discrepancy of the classical rate theory in the very low temperature range. ?? 1982.},
author = {Takeuchi, S. and Hashimoto, T. and Suzuki, K. and Ichihara, M.},
doi = {10.1016/0001-6160(82)90232-2},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/1958{\_}Haasen{\_}Plastic deformation of nickel single crystals at low temperatures.pdf:pdf},
isbn = {1478-6435 {\%}[ July 29, 2008},
issn = {00016160},
journal = {Acta Metall.},
number = {2},
pages = {513--521},
title = {{Plastic deformation of ??-CuZn single crystals at low temperatures}},
volume = {30},
year = {1982}
}
@article{Hashin1962a,
abstract = {Variational principles for anisotropic and nonhomogeneous elasticity, established by the authors in a previous paper, have been applied to the derivation of lower and upper bounds for the elastic moduli of polycrystals in terms of the moduli of the constituting crystals. The results hold for arbitrary crystal shapes. Explicit results tor cubic polycrystals showed that the present bounds are a considerable improvement of the well-known Voigt and Reuss bounds. Good agreement with experimental results has been obtained.},
author = {Hashin, Z and Shtrikman, S},
doi = {10.1016/0022-5096(62)90005-4},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/Strukturmechanik MMS/Literatur/Hashin Shtrikman 1962.pdf:pdf},
issn = {00225096},
journal = {J. Mech. Phys. Solids},
number = {4},
pages = {343--352},
title = {{A variational approach to the theory of the elastic behaviour of polycrystals}},
url = {http://linkinghub.elsevier.com/retrieve/pii/0022509662900054},
volume = {10},
year = {1962}
}
@article{Groma2016,
author = {Groma, Istv??n and Zaiser, Michael and Isp??novity, P??ter Dus??n},
doi = {10.1103/PhysRevB.93.214110},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2016{\_}Groma{\_}Dislocation patterning in a two-dimensional continuum theory of dislocations.pdf:pdf},
issn = {1550235X},
journal = {Phys. Rev. B - Condens. Matter Mater. Phys.},
number = {21},
pages = {1--10},
title = {{Dislocation patterning in a two-dimensional continuum theory of dislocations}},
volume = {93},
year = {2016}
}
@article{Auswirkung,
author = {Auswirkung, Die},
pages = {79--86},
title = {{7 Fehlertypen in Messeinrichtungen}}
}
@article{Worlds2016,
author = {Worlds, Small and Attachment, Preferential and Models, Voter and Distributions, Fixed Degree and Laws, Power},
isbn = {9780511546594},
pages = {5--6},
title = {{Preface 1.}},
year = {2016}
}
@article{Results1994b,
abstract = {As a concluding comment, I should like to return to the point raised by Ayres, that it is not enough simply to tell a better version of the fourth-century history in the expectation that modern theologians will finally get it straight! This is a valid point: if we want to have Christianity's fourth-century heritage taken seriously, we need to be in dialogue with modern writers. But, if there is to be a dialogue, both sides must be allowed to speak, and so we are also responsible for expounding the historical material on its own terms. As Heidegger put it, “[O]nly when we think through what has been thought will we be of any use for what must still be thought.” Perhaps studying the figures from a distant era will open up for us possibilities we would never have dreamed of within our own modern presuppositions, so that we can recognize differences even beyond those which lie within our own horizon or tradition. If I am right in affirming that there is a different style of doing theology prior to Augustine and after him in the East than that which we find in the theological and scholarly tradition in which Ayres's book stands, then we must ask whether we need to address the question of the legitimacy of each (and ponder how one might even answer that) or whether a plurality of approaches is possible without reducing one to the other. In a way, this would be a further step toward deconstructing monolithic notions of “Orthodoxy” in recognition of genuine and legitimate diversity within early Christianity and among modern Christians. Might it be better not to speak of Nicaea and its legacy, but of the legacies of Nicaea—or better—“Christ and him crucified” (2 Cor 2:2) and the ways in which Nicaea and its interpreters affirm the true divinity of this one?},
author = {Results, Useful},
doi = {10.1007/BF02600226},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2010{\_}Jaroslav Pokluda+Pavel {\v{S}}andera{\_}Micromechanisms of fracture and fatigue{\_}Buch/Kap5{\_}FinalReflection.pdf:pdf},
isbn = {9780470434673},
issn = {08848734},
journal = {J. Gen. Intern. Med.},
number = {3 Supplement},
pages = {243--247},
title = {{Final reflections}},
volume = {9},
year = {1994}
}
@article{Chaboche2006,
abstract = {The paper proposes a modified formalism of continuum damage mechanics in order to describe plastic compressibility in the context of ductile damage. The model uses two damage state variables, one of them playing role of porosity in micromechanics based approaches like Gurson's model. Various versions of the model are determined and compared with Gurson's model, in terms of the constitutive responses for various loading conditions, as well as for simple structural examples like a free and a clamped plate under plane strain, and an axisymmetric notched bar under tension. The classical CDM is also applied and some advantages of the proposed approach are underlined.},
author = {Chaboche, Jean Louise and Boudifa, M. and Saanouni, K.},
doi = {10.1007/s10704-005-3061-5},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Plasticity models/A CDM approach of ductile damage with plastic  compressibility {\_} By Chaboche.pdf:pdf},
isbn = {0376-9429},
issn = {03769429},
journal = {Int. J. Fract.},
keywords = {Constitutive equations,Damage mechanics,Ductile damage,Porous materials},
number = {1-4},
pages = {51--75},
title = {{A CDM approach of ductile damage with plastic compressibility}},
volume = {137},
year = {2006}
}
@article{Rechnen,
author = {Rechnen, Beim and Rechnen, Beim},
journal = {System},
title = {{A Einf u ¨ hrung in die kartesische Tensorrechnung}}
}
@article{Kochmann2009,
author = {Kochmann, D. M. and Hackl, Klaus. and Le, K. C.},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/2009{\_}Le{\_}A continuum dislocation theory for modeling dislocation microstructures in crystal plasticity.pdf:pdf},
journal = {Conf. Pap.},
keywords = {abstract,and pile up near,anisms related to the,continuum mechanics,dislocation,dislocation network,high degree on the,in order to accommodate,material moderling,mech-,microstructure,new dislocations are nucleated,plastic deformation and,plastic deformation of crystalline,plasticity,s energy,solids depends to a,the grain or,to reduce the crystal},
number = {September},
pages = {7--11},
title = {{a Continuum-Dislocation Theory for Modeling Dislocation Microstructures and Size Effects in Crystal Plastiticy}},
year = {2009}
}
@misc{Eshelby1951a,
abstract = {The parallel between the classical theory of elasticity and the modern physical theory of the solid state is incomplete; the former has nothing analogous to the concept of the force acting on an imperfection (dislocation, foreign atom, etc.) in a stressed crystal lattice. To remedy this a general theory of the forces on singularities in a Hookean elastic continuum is developed. The singularity is taken to be any state of internal stress satisfying the equilibrium equations but not the compatibility conditions. The force on a singularity can be given as an integral over a surface enclosing it. The integral contains the elastic field quantities which would surround the singularity in an infinite medium, multiplied by the difference between these quantities and those actually present. The expression for the force is thus of essentially the same form whether the force is due to applied surface tractions, other singularities or the presence of the free surface of the body ({\{}'{\}}image force{\{}'{\}}). A region of inhomogeneity in the elastic constants modifies the stress field; if it is mobile one can define and calculate the force on it. The total force on the singularities and inhomogeneities inside a surface can be expressed in terms of the integral of a {\{}'{\}}Maxwell tensor of elasticity{\{}'{\}} taken over the surface. Possible extensions to the dynamical case are discussed.},
author = {Eshelby, J. D.},
booktitle = {Philos. Trans. R. Soc. A Math. Phys. Eng. Sci.},
doi = {10.1098/rsta.1951.0016},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/1951{\_}Eshelby{\_}The force oo an elastic singularity.pdf:pdf},
isbn = {00804614},
issn = {1364-503X},
number = {877},
pages = {87--112},
title = {{The Force on an Elastic Singularity}},
url = {http://rsta.royalsocietypublishing.org/cgi/doi/10.1098/rsta.1951.0016},
volume = {244},
year = {1951}
}
@article{Wei1970a,
abstract = {Metal fatigue as an engineering problem has been well recognized. Many experiments have been carried out in recent years to assess the effects of load amplitude, mean load, load range and test frequency on the rate of fatigue-crack growth to characterize material response to different load profiles and to develop methods for estimating the service behavior of structural components. Recent studies have shown that fatigue-crack growth can be influenced strongly by the test environment; the effect being dependent on the particular material-environment involved. These results suggest that careful reassessments of the data of previous studies and of the proper direction for future fatigue research will be required. Hence, a critical review and analysis of existing fatigue-crack-growth data on high-strength aluminum and titanium alloys and high-strength steels has been made. The influences of load profile, test frequency, temperature, test environment and state-of-stress on fatigue-crack growth are discussed. Correlation with environment-enhanced crack growth under sustained loads and the associated changes in material response are examined. Possible mechanisms, synergistic effects and implications regarding methods for service-life estimation are considered. ?? 1970.},
author = {Wei, R. P.},
doi = {10.1016/0013-7944(70)90004-4},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/1970{\_}Wei{\_}Some aspects of environment-enhanced fatigue crack growth{\_}For example frequency in Al7075.pdf:pdf},
issn = {00137944},
journal = {Eng. Fract. Mech.},
number = {4},
pages = {633--651},
title = {{Some aspects of environment-enhanced fatigue-crack growth}},
volume = {1},
year = {1970}
}
@article{Haarlem1999,
author = {van Haarlem, M.P.},
doi = {10.1007/BFb0104276},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/{\_}buecherSong/HandbookofComposites/V/45{\_}ScientificApplicationsofComposites.pdf:pdf},
isbn = {978-3-540-65737-8},
journal = {Physics (College. Park. Md).},
title = {{Scientific Applications of Neural Nets}},
url = {http://www.springerlink.com/index/10.1007/BFb0104276},
volume = {522},
year = {1999}
}
@article{Xue2005,
author = {Xue, Yibin and Jordon, Brian and Horstemeyer, Stephen and Horstemeyer, Mark F},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Empirical Fatigue Models + Validation/Xue{\_}Fatigue-Experiments-Damage-Evaluation-Multiscale-Modeling-AA-7075{\_}Ansatz ueber Modellierung verschiedener Rissstadien.pdf:pdf},
isbn = {0912053909},
journal = {Proc. 2005 SEM Annu. Conf. Expo. Exp. Appl. Mech.},
pages = {1443--1450},
title = {{Fatigue Experiments , Damage Evaluation and Multiscale Modeling for AA 7075-T651}},
year = {2005}
}
@article{Bradley1996,
abstract = {Net chemical heat-release rates have been estimated experimentally, throughout the combustion, from a single-cylinder gasoline engine, running on paraffinic and aromatic fuels. These rates are compared for autoigniting and nonautoigniting cycles and, by means of a differencing procedure, the heat release rate due to autoignition found. Comparison of heat release rates in the propagating flame and in autoignition show that in knocking combustion, almost half the total energy release can occur in autoignition. Pressures were measured with transducers and gas temperatures prior to autoignition by the CARS technique. The measurements enabled volumetric autoignition heat release rates to be obtained. When plotted against the reciprocal temperature of the unburned gas just prior to autoignition, an activation temperature and Arrhenius constant were obtained for each fuel in a single global expression for the autoignition heat release rate. These constants are reexpressed in terms of the actual temperature and fuel concentration to give a more accurate kinetic representation. This is used in an analysis of the conditions necessary for the pressure wave generated at autoignition to couple with the chemical kinetics sufficiently to lead to a developing detonation. At the inception of knock, for the same temperatures and pressures, the maximum autoignition heat release rates for the paraffinic fuel are two to three times those for the aromatic fuel. Because of this, the paraffinic fuel is more prone to developing detonation than is the aromatic fuel. ?? 1996 Combustion Institute.},
author = {Bradley, D and Kalghatgi, G T and Golombok, M and Yeo, Jinku},
doi = {10.1016/S0082-0784(96)80100-7},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Klopfen{\_}Ottomotor/1996{\_}Bradley{\_}HEAT RELEASE RATES DUE TO AUTOIGNITION AND THEIR RELATIONSHIP TO KNOCK INTENSITY IN SI ENGINES.pdf:pdf},
isbn = {00820784},
issn = {00820784},
journal = {Symp. Combust.},
number = {2},
pages = {2653--2660},
title = {{Heat release rates due to autoignition, and their relationship to knock intensity in spark ignition engines}},
volume = {26},
year = {1996}
}
@article{Torsion,
author = {Torsion, Abscheren},
title = {{Sachwortverzeichnis}}
}
@article{Erw2000,
author = {Erw, Globale and Ghg, Treibhausgase},
pages = {337--346},
title = {{19 Kyoto-Protokoll 19.1}},
year = {2000}
}
@article{Begriff,
author = {Begriff, Der},
pages = {144--162},
title = {{8 Ausgleichsvorg{\"{a}}nge in linearen Netzen}}
}
@article{Mroz2003,
author = {Mr{\'{o}}z, Z. and Maciejewski, J.},
doi = {10.1007/978-3-540-36418-4_3},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Anisotropic Behaviouir of Damaged Materials{\_}Skrzypek{\_}ARTICEL/Kap3{\_}Failure Criteria and Compliance Variation of Anisotropically Damaged Materials.pdf:pdf},
isbn = {9783642055874},
issn = {16137736},
journal = {Lect. Notes Appl. Comput. Mech.},
keywords = {Failure condition,anisotropic damage,critical plane,strength variation},
pages = {75--112},
title = {{Failure Criteria and Compliance Variation of Anisotropically Damaged Materials}},
volume = {9},
year = {2003}
}
@article{Berg1998,
author = {Berg, Kenneth R},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/{\_}buecherSong/HandbookofComposites/VI/AppendixB{\_}SpecificationsandStandardsforPolymerComposites.pdf:pdf},
title = {{Typical Properties for Advanced Composites}},
year = {1998}
}
@book{Fox1918,
author = {Fox, P J},
booktitle = {Science (80-. ).},
doi = {10.1126/science.49.1254.44},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Thermodynamik/M{\"{u}}llerAndNoll{\_}Thermodynamik/Noll 1974 Mechanics and Thermodynamics{\_}SelectedPapers.pdf:pdf},
isbn = {9783642658198},
issn = {0036-8075},
number = {1240},
pages = {343--345},
pmid = {17811888},
title = {{the Foundations of Mechanics.}},
volume = {48},
year = {1918}
}
@book{Golloch2005,
address = {Berlin Heidelberg},
author = {Golloch, Rainer},
edition = {1},
isbn = {978-3-540-23883-6},
publisher = {Springer-Verlag},
title = {{Downsizing bei Verbrennungsmotoren}},
year = {2005}
}
@article{Arbeitsumgebung,
author = {Arbeitsumgebung, Die},
pages = {47--58},
title = {{4 Skizzieren 4.1}}
}
@article{Bremsvorgang,
author = {Bremsvorgang, Station{\"{a}}rer Beschleunigungs-},
title = {{6 Antrieb und Bremsung}}
}
@article{Tatigkeitsfeld,
author = {Tatigkeitsfeld, Das and Internet, Das and Software, Stromungsmechanik and Karlsru-, Universitat and Grundlagen, Die and Anwen-, Als and Anklicken, Durch and Ergebnis, Als and Absenken, Bei and Zahl, Mach-},
pages = {362--413},
title = {{Stromungsmechanik Software}}
}
@article{Lakes2006,
author = {Lakes, Roderic S},
doi = {doi:10.1201/9781420049510.ch40},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/{\_}buecherSong/HandbookofComposites/V/44{\_}CompositeBiomaterials.pdf:pdf},
isbn = {0-8493-1491-7},
journal = {Biomed. Eng. Fundam.},
number = {1},
pages = {14--1--41--14},
pmid = {1022301},
title = {{Composite Biomaterials}},
year = {2006}
}
@article{Sauzay2000,
author = {Sauzay, M and Gilormini, P},
doi = {10.1046/j.1460-2695.2000.00307.x},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2000{\_}Sauzay{\_}Surface and cyclic microplasticity{\_}SurfaceAndPlasticityInMicro.pdf:pdf},
issn = {8756758X},
journal = {Fatigue Fract. Eng. Mater. Struct.},
keywords = {crystallographic glide,fatigue,free surface,microplasticity},
number = {7},
pages = {573--579},
title = {{Surface and cyclic microplasticity}},
volume = {23},
year = {2000}
}
@article{Bertram2009,
author = {Bertram, Albrecht},
pages = {1--241},
title = {{Vorlesungsmanuskript zur Festigkeitslehre I + II}},
year = {2009}
}
@article{Spunk2010,
author = {Spunk, Joseph and Nuri, Aksel},
isbn = {9783642131424},
title = {{Str{\{}{\"{o}}{\}}mungslehre Einf{\{}{\"{u}}{\}}hrung in die Theorie}},
year = {2010}
}
@book{Warnatz2006,
author = {Warnatz, J and Maas, U and Dibble, R W},
booktitle = {New York},
edition = {4},
file = {:C$\backslash$:/Users/p327208/Desktop/Promotion/Literature/Thermodynamik/2006{\_}Maas{\_}Combustion.pdf:pdf},
isbn = {9783540259923},
publisher = {Springer Berlin Heidelberg New York},
title = {{Combustion}},
year = {2006}
}
@article{Kessler1955,
author = {Kessler, C},
journal = {Regelungstechnik},
number = {2},
pages = {40--49},
title = {{{\"{U}}ber die Vorausberechnung optimal abgestimmter Regelkreise Teil III. Die optimale Einstellung des Reglers nach dem Betragsoptimum}},
volume = {3},
year = {1955}
}
@article{Demuynck2011,
author = {Demuynck, Joachim and Paepe, Michel De and Huisseune, Henk and Sierens, Roger and Vancoillie, Jeroen and Verhelst, Sebastian},
doi = {http://dx.doi.org/10.1016/j.applthermaleng.2010.12.023},
file = {:C$\backslash$:/Users/p327208/Desktop/Promotion/Literature/Motorspezifisch/Heat Transfer Combustion Chamber/2011{\_}Demuynck{\_}Investigation of the inflence of engine settings on the heat flux in a hydrogen- and methane-fueled SI engine.pdf:pdf},
journal = {Appl. Therm. Eng.},
pages = {1220--1228},
publisher = {Elsevier Ltd},
title = {{Investigation of the in fluence of engine settings on the heat flux in a hydrogen- and methane-fueled spark ignition engine}},
volume = {31},
year = {2011}
}
@article{Nallasamy1987a,
author = {Nallasamy, M},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Boiling/Turbulence/1985{\_}Nallasamy{\_}Turbulence models and therir applications to the prediciton of internal flows - a review.pdf:pdf},
journal = {Comput. Fluids},
number = {2},
pages = {151--194},
title = {{Turbulence Models and their A lications to the Prediction of Internal Flows}},
volume = {15},
year = {1987}
}
@article{Murakami2012k,
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Murakami, Sumio},
doi = {10.1007/978-94-007-2666-6},
eprint = {arXiv:1011.1669v3},
isbn = {978-94-007-2665-9},
issn = {09250042},
number = {1995},
pages = {201--215},
pmid = {25246403},
title = {{Continuum Damage Mechanics}},
url = {http://link.springer.com/10.1007/978-94-007-2666-6},
volume = {185},
year = {2012}
}
@article{Depcik2002b,
abstract = {In this paper, the available correlations proposed in the literature for the gas-side heat transfer in the intake and exhaust system of a spark-ignition internal combustion engine were surveyed. It was noticed that theseAB - {\{}{\textless}{\}}inline-graphic xlink:href="2002-01-0372{\{}{\_}{\}}fig0001" xmlns:xlink="http://www.w3.org/1999/xlink"/{\{}{\textgreater}{\}}AB - only by empirically fitted constants. This similarity provided the impetus for the authors to explore if a universal correlation could be developed. Based on a scaling approach using microscales of turbulence, the authors have fixed the exponential factor on the Reynolds number and thus reduced the number of adjustable coefficients to just one; the latter can be determined from a least squares curve-fit of available experimental data. Using intake and exhaust side data, it was shown that the universal correlationAB - {\{}{\textless}{\}}inline-graphic xlink:href="2002-01-0372{\{}{\_}{\}}fig0002" xmlns:xlink="http://www.w3.org/1999/xlink"/{\{}{\textgreater}{\}}AB - The correlation coefficient of this proposed heat transfer model with all available experimental data is 0.845 for the intake side and 0.800 for the exhaust side.ER -},
author = {Depcik, Christopher and Assanis, Dennis},
doi = {10.4271/2002-01-0372},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2002{\_}Assanis{\_}A Universal Heat Transfer Correlation for Intake and Exhaust flows in an SI INternal Combustion Engine.pdf:pdf},
journal = {SAE Pap.},
number = {January 2016},
title = {{A Universal Heat Transfer Correlation for Intake and Exhaust Flows in an Spark-Ignition Internal Combustion Engine}},
url = {http://papers.sae.org/2002-01-0372},
volume = {2002-01-03},
year = {2002}
}
@inproceedings{Yokomori2017,
author = {Yokomori, Takeshi},
booktitle = {FVV 2017 Autumn Conf. Leipzig},
title = {{Super-Lean Burn Technology for High Thermal Efficiency SI Engines}},
year = {2017}
}
@article{Essmann1979,
abstract = {It is proposed that, during dislocation glide at low temperatures, both screw and non-screw dislocations annihilate mutually with dislocations of opposite sign approaching on closely neighbouring glide planes. The experimental evidence is summarized and possible mechanisms are discussed. Phenomenological models of dislocation accumulation during deformation, taking into account the annihilation of dislocations, are formulated. The analysis of selected examples of tensile and cyclic deformation of f. c. c. and b. c. c. metal crystals demonstrates that annihilation of edge and/or screw dislocations occurs during strain hardening and can lead to steady-state deformation. It follows that the dislocation densities introduced during deformation cannot exceed well-defined upper limits that are distinctly lower than the hypothetical upper limits estimated for the static case. The observations suggest that the critical spacings of dislocation pairs that annihilate are similar 50-500 nm for screw and similar 1. 6 nm for edge dislocations (in copper). The atomic concentration of point defects formed by the annihilation of non-screw dislocations is found to be low in most cases. However, it is concluded that, in the dislocation-rich walls of persistent slip bands in fatigued copper, a rather high concentration of point defects prevails.},
author = {Essmann, U and Mughrabi, H},
doi = {10.1080/01418617908234871},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/2006{\_}Mughrabi + Essmann{\_}Annihilation of dislocations   during tensile and cyclic deformation and limits of dislocation   densities.pdf:pdf},
isbn = {0141-8610},
issn = {0141-8610},
journal = {Philos. Mag. A},
number = {6},
pages = {731--756},
title = {{Annihilation of dislocations during tensile and cyclic deformation and limits of dislocation densities}},
url = {http://www.tandfonline.com/doi/abs/10.1080/01418617908234871},
volume = {40},
year = {1979}
}
@article{Motork,
author = {Motork, Interne},
title = {{Motork{\{}{\"{u}}{\}}hlung}}
}
@article{Winkler2014a,
author = {Winkler, N},
doi = {10.1177/1468087414544899},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2015{\_}Winkler{\_}Effect of pressure oscillations on in-cylinder heat transfer  - through LES Simulation.pdf:pdf},
isbn = {1468087414544},
issn = {1468-0874},
journal = {Int. J. Engine Res.},
keywords = {24 june 2014,6 march 2014,accepted,computational fluid dynamics,date received,heat transfer,internal combustion engines,large eddy simulation,pressure oscillations},
number = {6},
pages = {705--715},
title = {{Effect of pressure oscillations on in-cylinder heat transfer - through large eddy simulation}},
url = {http://jer.sagepub.com/lookup/doi/10.1177/1468087414544899},
volume = {16},
year = {2014}
}
@article{Gross2011j,
author = {Gross, Dietmar and Seelig, Thomas},
doi = {10.1007/978-3-642-10196-0},
isbn = {978-3-642-10195-3},
title = {{Bruchmechanik}},
url = {http://link.springer.com/10.1007/978-3-642-10196-0},
year = {2011}
}
@article{Schraubenver-,
author = {Schraubenver-, Anziehen Der},
pages = {784--802},
title = {{Sachwortverzeichnis}}
}
@article{Hettinger2009c,
abstract = {It is a well known fact that indicated efficiency of a SI engine at WOT is predominantly limited by knock occurrence. Therefore many investigations have been carried out to avoid knocking. Considering the further development of downsized engines knocking will also pose a greater challenge. Not only knocking but also irregular combustion in general will require further investigation in supercharged SI eingines. Premature ignition, for instance, hasn't yet been completely understood and therefore limits the low end torque of supercharged SI engines.The purpose of this paper is to introduce different analysis methods which allow to identify the knock onset and the knocking zones in the combustion chamber. In addition to established methods new techniques have been developed to account for the complex nature of pressure oscillation during knocking combustion.Experimental data was acquired on a single cylinder research engine to validate the methodology using six pressure transducers.},
author = {Hettinger, Alexander and Kulzer, Andr{\'{e}}},
doi = {10.4271/2009-01-0698},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2009{\_}Hettinger+Kulzer{\_}A new method to detect Knocking Zones.pdf:pdf},
isbn = {2009010698},
issn = {1946-3944},
journal = {SAE Int. J. Engines},
number = {1},
pages = {2009--01--0698},
title = {{A New Method to Detect Knocking Zones}},
url = {http://papers.sae.org/2009-01-0698/},
volume = {2},
year = {2009}
}
@article{Hansen2005b,
abstract = {The Hall-Petch relation is discussed separately for the yield stress of undeformed polycrystalline metals and the flow stress of deformed metals. The strength contributions for grain boundaries and from dislocation boundaries are given special attention. An experimental analysis supports the Hall-Petch relation for undeformed metals over a grain size range from about 20 nm to hundred of micrometres. For deformed metals the strengthening effect of low angle dislocation boundaries evolves with increasing strain in parallel with a change in their spacing. An application of the Hall-Petch relation must therefore be based on a detailed structural characterization. ?? 2005 Elsevier B.V. All rights reserved.},
author = {Hansen, Niels},
doi = {10.1016/j.msea.2005.04.061},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2005{\_}Hansen Boundary strengthening in undeformed and deformed polycrystals.pdf:pdf},
isbn = {0921-5093},
issn = {09215093},
journal = {Mater. Sci. Eng. A},
keywords = {Dislocation boundaries,Grain boundaries,Hall-Petch relation,Nanostructures},
number = {1-2},
pages = {39--45},
title = {{Boundary strengthening in undeformed and deformed polycrystals}},
volume = {409},
year = {2005}
}
@book{Bazant1992,
abstract = {Elasticity, plasticity, damage mechanics and cracking are all phenomena that determine the resistance of solids to deformation and fracture. The authors of this book discuss a modern method of mathematically modeling the behavior of macroscopic volume elements. The first three chapters review physical mechanisms at the microstructural level, thermodynamics of irreversible processes, mechanics of continuous media, and the classification of the behavior of solids. The rest of the book is devoted to the modeling of different types of material behavior. In each case the authors present characteristic data for numerous materials, and discuss the physics underlying the phenomena together with methods for the numerical analysis of the resulting equations.},
author = {Ba{\v{z}}ant, Z P},
booktitle = {Can. J. Civ. Eng.},
doi = {10.1139/l92-025},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Kriechen{\_}Spannungsrelaxation/1985{\_}Jean{\_}Lemaitre+Jean-Louis+Chaboche{\_}Mechanics{\_}of{\_}Solid{\_}Materials.pdf:pdf},
isbn = {0521477581},
issn = {0315-1468},
number = {1},
pages = {197},
title = {{Mechanics of solid materials}},
url = {http://www.nrcresearchpress.com/doi/abs/10.1139/l92-025},
volume = {19},
year = {1992}
}
@article{Brecq2005a,
abstract = {High frequency pressure oscillations are generated under knocking conditions within the combustion chamber of Spark Ignition engines. Although acoustic-oscillation model can give the natural frequencies of these oscillations, very few mathematical models are today available, in scientific literature, to describe the oscillation deadening effect. An analytical formulation of the deadening has been highlighted. Analytical solution has been established for future ECU implementation. Coupling this new concept and an existing high-frequency model, an achieved model of the knocking pressure high frequencies is compared to experimental data. Good behavior is obtained on a natural gas fuelled spark ignition engine.},
author = {Brecq, G and {Le Corre}, O},
doi = {10.4271/2005-01-1126},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2005{\_}Brecq{\_}Modeling of In-cylinder Pressure Oscillations under Knocking conditions - Intro to Pressure Envelope Curve.pdf:pdf},
isbn = {2005011126},
issn = {0148-7191},
title = {{Modeling of In-cylinder Pressure Oscillations under Knocking Conditions: Introduction to Pressure Envelope Curve}},
url = {http://papers.sae.org/2005-01-1126/},
year = {2005}
}
@article{Wang2016,
abstract = {Cracks encountered in engineering structures are typically three dimensional, and the fracture mechanism remains unclear because of the superimposed stresses induced by mixed-mode I/II/III loading. This paper introduces a general 3D mixed-mode fracture criterion based on the maximum mean principal stress (MMPS) by introducing the concept of a characteristic fracture length that is related to the material tensile strength. This criterion has clear physical significance, a systematic mathematical expression and a wide scope of applications to estimate both the in- and out-of-plane fracture angles and fracture strength. The proposed criterion is validated for all mixed-mode conditions (I/II, I/III and II/III) and is compared with several widely used criteria based on experimental results reported in previous studies. Good agreement is achieved in terms of the fracture angles and, in particular, the fracture strength between the results predicted by the new criterion and the experimental results of various brittle materials.},
author = {Wang, J. and Ren, L. and Xie, L. Z. and Xie, H. P. and Ai, T.},
doi = {10.1016/j.ijsolstr.2016.10.009},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/2016{\_}Wang{\_}Maximum mean principal stress criterion for 3D brittle fracture.pdf:pdf},
issn = {00207683},
journal = {Int. J. Solids Struct.},
keywords = {3D fracture criterion,Characteristic fracture length,Mean stress,Mixed-mode loading},
pages = {142--154},
title = {{Maximum mean principal stress criterion for three-dimensional brittle fracture}},
volume = {102-103},
year = {2016}
}
@article{Mizuno2009a,
abstract = {This study examined a method of predicting the piston temperature in reciprocating internal combustion engines with the aim of developing lightweight pistons. Since the piston temperature is strongly affected by the in-cylinder temperature distribution and turbulence, it is necessary to consider the effects of flame propagation, cooling by the intake air, temperature rise due to combustion, in-cylinder flow and the combustion chamber shape. A three-dimensional combustion simulation that can take these effects into consideration was run to calculate the heat transfer coefficient from the piston crown surface and the gas temperature. The results were used as the boundary conditions for an analysis of heat transfer from the piston, and a method was thus developed for analyzing the piston temperature. The hardness method was used to obtain the piston temperature distribution and maximum temperature during engine operation, and a comparison was made with the analytical results to examine the effects of flame propagation.},
author = {Mizuno, Hideaki and Ashida, Koichi and Teraji, Atsushi and Ushijima, Kenshi and Takemura, Shinichi},
doi = {10.4271/2009-01-0187},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/2009{\_}Mizuno{\_}Transient Analysis of the Piston Temperature with Measurement and Simulation.pdf:pdf},
isbn = {9200901018},
issn = {1946-3944},
journal = {SAE Int. J. Engines},
number = {1},
pages = {2009--01--0187},
title = {{Transient Analysis of the Piston Temperature with Consideration of In-cylinder Phenomena Using Engine Measurement and Heat Transfer Simulation Coupled with Three-dimensional Combustion Simulation}},
url = {http://papers.sae.org/2009-01-0187/},
volume = {2},
year = {2009}
}
@article{Zeit,
author = {Zeit, Zur and Gegensatz, Im and Anteil, Der and Unit, Electronic Control},
pages = {307--322},
title = {{14 Parkassistent}}
}
@article{Spa,
author = {Spa, Menschen and Systeme, Technische and Assistenz-, Derartige and Laufe, Im and Fahrer, Der and Folgenden, Im},
title = {{13 Automatisches Spurfahren auf Autobahnen}}
}
@article{Gross2011g,
author = {Gross, Dietmar and Seelig, Thomas},
doi = {10.1007/978-3-642-10196-0},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Gross, Selig 2011 - Bruchmechanik/Gross, Seelig - 2011 - BruchmechanikKap9.pdf:pdf},
isbn = {978-3-642-10195-3},
title = {{Bruchmechanik}},
url = {http://link.springer.com/10.1007/978-3-642-10196-0},
year = {2011}
}
@article{Nicoletto1989a,
author = {Nicoletto, G},
file = {:C$\backslash$:/Users/p327208/Desktop/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/1969{\_}Nicoletto{\_}Plastic zones about fatigue cracks in metlas.pdf:pdf},
keywords = {alumi-,cyclic plastic zone,effective stress intensity factor,fatigue crack growth,moir6 interferometry,monotonic plastic zone,nium alloy,overload,range,steels},
number = {2},
pages = {107--115},
title = {{P l a s t i c z o n e s a b o u t f a t i g u e c r a c k s in metals}},
volume = {2},
year = {1989}
}
@article{Brunig2015a,
author = {Br{\"{u}}nig, Michael and Gerke, Steffen and Brenner, Daniel},
doi = {10.1007/978-3-319-14660-7},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Plasticity models/Experiments and Numerical Simulations on Stress-State-Dependence of Ductile Damage Criteria{\_}Br{\"{u}}nig.pdf:pdf},
isbn = {978-3-319-14659-1},
keywords = {ductile damage},
title = {{Inelastic Behavior of Materials and Structures Under Monotonic and Cyclic Loading}},
url = {http://link.springer.com/10.1007/978-3-319-14660-7},
volume = {57},
year = {2015}
}
@article{Derb,
author = {Der, Spezielle Probleme},
title = {{7. Spezielle Probleme der Grenzschichtmesstechnik}}
}
@article{Niedziela2013,
archivePrefix = {arXiv},
arxivId = {arXiv:1011.1669v3},
author = {Niedziela, Dariusz and Latz, Arnulf and Kroll, Lothar},
doi = {10.1177/0892705711419695},
eprint = {arXiv:1011.1669v3},
isbn = {0892705711424},
issn = {21554854},
pmid = {25246403},
title = {{Composite Materials}},
year = {2013}
}
@article{Wulfinghoff2011a,
author = {Wulfinghoff, Stephan and Thomas, B},
doi = {10.1002/pamm.201110216},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Crystal Plasticity Approaches/2011{\_}Wulfinghoff{\_}Dislocation Transport in Single Crystals and Dislocation-based micromechanical hardening.pdf:pdf},
issn = {16177061},
journal = {Contin. (N. Y).},
pages = {3728},
title = {{Dislocation Transport in Single Crystals and Dislocation-based Micromechanical Hardening Models}},
volume = {87},
year = {2011}
}
@article{Meroth2008,
abstract = {Das Wort Infotainment ist ein Kunstwort, das sich aus den Begriffen Information und Unterhaltung (Entertainment) zusammensetzt. 75 Jahre nach Einf{\"{u}}hrung des ersten Autoradios hat sich Infotainment einen wertbestimmenden Rang im Automobil erobert. Sp{\"{a}}testens mit den Fahrerassistenzsystemen sind Fahrzeugfunktionen und Infotainment zu einer Einheit verschmolzen. Die Mindmap in Abbildung 1.1 zeigt einige Aspekte, die im Folgenden n{\"{a}}her erl{\"{a}}utert werden sollen.},
author = {Meroth, Ansgar and Tolg, Boris and Plappert, Christian},
isbn = {978-3-8348-9430-4},
journal = {Infotainmentsysteme im Kraftfahrzeug},
pages = {1--6},
title = {{Einf{\"{u}}hrung}},
url = {http://dx.doi.org/10.1007/978-3-8348-9430-4{\_}1},
year = {2008}
}
@article{Bastler,
author = {Bastler, F{\"{u}}r Den},
number = {Kapitel 6},
pages = {303--304},
title = {{10 Selbstbau und Tuning}}
}
@article{Fan1992,
author = {Fan, H. and Keer, L.M.},
doi = {10.1016/0013-7944(92)90059-N},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/1977{\_}Morris{\_}The early stage of fatigue crack propagation in al 2048.pdf:pdf},
issn = {00137944},
journal = {Eng. Fract. Mech.},
number = {5},
pages = {789--796},
title = {{The early stage of fatigue crack propagation}},
volume = {42},
year = {1992}
}
@article{Baehr2010,
author = {Baehr, H D and Stephan, K},
doi = {10.1007/978-3-642-10194-6},
isbn = {9783642101946},
title = {{Konvektiver W ¨ arme- und Stoff u omungen ¨ bergang . Einphasige Str ¨}},
year = {2010}
}
@article{Zahoransky2007,
author = {Zahoransky, Richard A},
isbn = {9783834804884},
pages = {337--346},
title = {{Energietechnik}},
url = {d:{\$}{\%}5C{\$}00{\%}7B{\_}{\%}7DDATA{\$}{\%}5C{\$}90{\%}5CnLiteratur{\$}{\%}5C{\$}30{\%}5CnDateien{\$}{\%}5C{\$}(Zahoransky-2007)Kyoto-Protokoll.pdf{\%}5Cnhttp://www.springerlink.com/index/10.1007/978-3-8348-9250-8},
volume = {3},
year = {2007}
}
@article{Nicoletto1989a,
author = {Nicoletto, G},
keywords = {alumi-,cyclic plastic zone,effective stress intensity factor,fatigue crack growth,moir6 interferometry,monotonic plastic zone,nium alloy,overload,range,steels},
number = {2},
pages = {107--115},
title = {{P l a s t i c z o n e s a b o u t f a t i g u e c r a c k s in metals}},
volume = {2},
year = {1989}
}
@article{Aluminium,
author = {Aluminium, Schaum- and Bild, Rechtecke},
pages = {192--214},
title = {{17 Sandwichelemente}}
}
@article{Broekaert2016I,
author = {Broekaert, Stijn and Demuynck, Joachim and Cuyper, Thomas De and Paepe, Michel De and Verhelst, Sebastian},
doi = {http://dx.doi.org/10.1016/j.energy.2016.08.065},
file = {:C$\backslash$:/Users/p327208/Desktop/Promotion/Literature/Motorspezifisch/Heat Transfer Combustion Chamber/2016{\_}Broekaert{\_}Heat transfer in premixed spark ignition engines part I - Identification of the factors inflencing heat transfer.pdf:pdf},
journal = {Energy},
pages = {380--391},
publisher = {Elsevier Ltd},
title = {{Heat transfer in premixed spark ignition engines part I : Identification of the factors influencing heat transfer}},
volume = {116},
year = {2016}
}
@book{Dresig2001,
author = {Dresig, Hans},
booktitle = {New York},
doi = {10.1007/3-540-29663-8},
isbn = {9783540260240},
pages = {459},
title = {{Schwingungen und mechanische Antriebssysteme}},
year = {2001}
}
@article{Spitsov2013,
abstract = {The paper is devoted to study specific aspects of heat transfer in the combustion chamber of compression ignited reciprocating internal combustion engines and possibility to directly measure the heat flux by means of Gradient Heat Flux Sensors (GHFS). A one – dimensional single zone model proposed by Kyung Tae Yun et al. and implemented with the aid of Matlab, was used to obtain approximate picture of heat flux behavior in the combustion chamber with relation to the crank angle. The model's numerical output was compared to the experimental results. The experiment was accomplished by A. Mityakov at four stroke diesel engine Indenor XL4D. Local heat fluxes on the surface of cylinder head were measured with fast – response, high – sensitive GHFS. The comparison of numerical data with experimental results has revealed a small deviation in obtained heat flux values throughout the cycle and different behavior of heat flux curve after Top Dead Center.},
author = {Spitsov, Oleg},
keywords = {Heat transfer,ICE,modeling},
pages = {55},
title = {{Heat transfer inside internal combustion engine: Modelling and comparison with experimental data}},
year = {2013}
}
@article{Zielsetzung2008,
author = {Zielsetzung, Einleitung and Verbrennungsmotor, Der and Generatoren, Schiffe},
pages = {1--2},
title = {{1 Einleitung und Zielsetzung}},
year = {2008}
}
@article{Wallentowitza,
author = {Wallentowitz, Henning and Reif, Konrad},
doi = {10.1007/978-3-8348-8195-3},
isbn = {9783834802576},
title = {{Aus dem Programm}}
}
@article{Papulaa,
author = {Papula, L},
journal = {Math. f{\"{u}}r Ingenieure und Naturwissenschaftler Band 2},
title = {{IV Gew{\"{o}}hnliche Differentialgleichungen 1}}
}
@article{Haarlem1999,
author = {van Haarlem, M P},
doi = {10.1007/BFb0104276},
isbn = {978-3-540-65737-8},
journal = {Phys. (College. Park. Md).},
title = {{Scientific Applications of Neural Nets}},
url = {http://www.springerlink.com/index/10.1007/BFb0104276},
volume = {522},
year = {1999}
}
@article{Industriea,
author = {Industrie, Der},
title = {{Abgasemission von Dieselmotoren}}
}
@article{LeFeuvre1969b,
abstract = {By the use of surface thermocouples to measure instantaneous temperatures, the instantaneous heat fluxes are calculated at several positions on the cylinder head and sleeve of a direct injection diesel engine for both motored and fired operation. Existing correlations are shown to be unable to predict these data.An analysis of convective heat transfer in the engine leads to a boundary layer model which adequately correlates the data for motored operation. The extension of this motored correlation to fired operation demonstrates the need for instantaneous local gas velocity and temperature data.},
author = {LeFeuvre, T and Myers, P S and Uyehara, O A},
doi = {10.4271/690464},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Heat Transfer Combustion Chamber/1969{\_}LeFeuvre{\_}Experimental Instantaneous Heat Fluxes in a Diesel Engine and their Correlation.pdf:pdf},
isbn = {690464 ST - Experimental Instantaneous Heat Fluxes in a Diesel Engine and Their Correlation},
journal = {SAE Tech. Pap.},
pages = {1717--1738},
title = {{Experimental Instantaneous Heat Fluxes in a Diesel Engine and Their Correlation}},
url = {http://dx.doi.org/10.4271/690464{\%}5Cnhttp://papers.sae.org/690464/},
volume = {690464},
year = {1969}
}
@article{Forestb,
author = {Forest, Samuel},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Homogenisierung Und Lokalisierung/Folien CISM Summer School Mai2017 - Mesoscale Models/courses{\_}C1703{\_}forest{\_}Forest1-Micromorphic.pdf:pdf},
title = {{Micromorphic media}}
}
@article{Stupkiewicz2007e,
author = {Stupkiewicz, Stanis{\l}aw},
doi = {10.1007/978-3-540-49717-2_9},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/Stupkievicz 2007 - Micromechanics of Contact and Interphase Layers/97165{\_}9.pdf:pdf},
isbn = {3540497161},
issn = {16137736},
journal = {Lect. Notes Appl. Comput. Mech.},
number = {30},
pages = {151--170},
title = {{Formation of stress-induced martensitic plates}},
volume = {2006},
year = {2007}
}
@article{Kalghatgi1995,
abstract = {Net heat release, knock characteristics and temperature were derived$\backslash$nfrom in-cylinder pressure and end-gas CARS measurements for different$\backslash$nfuels in a single-cylinder engine. The maximum net heat release rate$\backslash$nresulting from the final phase of autoignition is closely associated$\backslash$nwith knock intensity. Aromatic fuels have lower maximum heat release$\backslash$nrates and lower knock intensities than expected from their octane number$\backslash$nwhen compared to paraffinic fuels; this is observed even when there is$\backslash$nsignificant heating of the end-gas from pre-flame reactions. Leaner$\backslash$nmixtures have lower combustion rates so that pressure development is$\backslash$nslowed and hence ignition needs to be more advanced to get knock to$\backslash$noccur as frequently as in a richer mixture. However, for a given$\backslash$nfrequency of knock occurrence, there is no significant difference in$\backslash$npeak net heat release rates and hence in knock intensities for different$\backslash$nmixture strengths.},
author = {Kalghatgi, G T and Golombok, M and Snowdon, P},
doi = {10.1080/00102209508951924},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Motorspezifisch/Klopfen{\_}Ottomotor/2007{\_}Kalghatgi{\_}Fuel effect on knock - heat release and CARS tempertures in SI Engine.pdf:pdf},
issn = {0010-2202},
journal = {Combust. Sci. Technol.},
number = {March},
pages = {209--228},
title = {{Fuel effects on knock, heat release and `'CARS'' temperatures in a spark ignition engine}},
volume = {111},
year = {1995}
}
@article{Wei1974a,
author = {Wei, K P},
file = {:C$\backslash$:/Users/p327208/Desktop/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/1974{\_}Shih + Wei{\_}A study of crack closure in fatigue.pdf:pdf},
pages = {19--32},
title = {{Study of in}},
volume = {6},
year = {1974}
}
@article{Fischer2016,
author = {Fischer, Carl and Schweizer, Christoph and Seifert, Thomas},
doi = {10.1016/j.ijfatigue.2016.03.011},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Fracture Mechanics + Crack Growth + Akkumulierung von Schaedigung/2016{\_}Seifert+Schweizer{\_}A crack opening stress equation for in phase and out of phase thermomechanical fatigue loading.pdf:pdf},
issn = {01421123},
journal = {Int. J. Fatigue},
keywords = {fatigue crack closure,thermomechanical fatigue},
pages = {178--184},
publisher = {Elsevier Ltd},
title = {{A crack opening stress equation for in-phase and out-of-phase thermomechanical fatigue loading}},
url = {http://linkinghub.elsevier.com/retrieve/pii/S0142112316300160},
volume = {88},
year = {2016}
}
@article{Morris1976,
abstract = {Abstract  Fatigue crack initiation in Al 2219-T851 for fully reversed loading(R = $\sigma$/$\sigma$max =−1) parallel to the material rolling direction is found to occur at intermetallic inclusions at the specimen surface. The inclusions are not involved in crack initiation for fatigue perpendicular to the rolling direction, and for this orientation crack initiation is at grain boundaries and specimens have an increased fatigue life. Except for fatigue at low peak stress, multiple numbers of microcracks are formed and for selected failed specimens the number of cracks has been determined as a function of crack length. Such crack length distribution measurements show that there is significant retardation of microcracks by interaction with grain boundaries. Furthermore it is found that the coalescence of microcracks provides a mechanism for cracking to “jump“ grain boundaries and reduce fatigue lifetime. The effect of relative humidity on this process is to increase the observed mean crack length, and decrease the number of crack initiations apparently due to weakening of the matrix-intermetallic interface at potential initiation sites. The overall result is that no significant dependence of fatigue life on relative humidity is found.},
author = {Morris, W. L. and Buck, O. and Marcus, H. L.},
doi = {10.1007/BF02656599},
file = {:E$\backslash$:/unverschluesselt/Promotion/Literature/Micromechanic Damage/1976{\_}Morris{\_}Fatigue crack initiation and early propagation in Al 2219-T851.pdf:pdf},
isbn = {0360-2133$\backslash$r1543-1940},
issn = {03602133},
journal = {Metall. Trans. A},
number = {7},
pages = {1161--1165},
title = {{Fatigue crack initiation and early propagation in Al 2219-T851}},
volume = {7},
year = {1976}
}
@article{Mohammadi2008b,
abstract = {A computational fluid dynamics (CFD) code is applied to simulate fluid flow, heat transfer and combustion in a four-stroke single cylinder engine with pent roof combustion chamber geometry, having two inlet valves and two exhaust valves. Heat flux and heat transfer coefficient on the cylinder head, cylinder wall, piston, intake and exhaust valves are determined with respect to crank angle position. Results for a certain condition are compared for total heat transfer coefficient of the cylinder engine with available correlation proposed by experimental measurement in the literature and close agreement are observed. It was found that the local value of heat transfer coefficient varies considerably in different parts of the cylinder, but they have equivalent trend with crank angle. Based on the results, new correlations are suggested to predict maximum and minimum convective heat transfer coefficient in the combustion chamber of a SI engine. ?? 2007 Elsevier Ltd. All rights reserved.},
author = {Mohammadi, A. and Yaghoubi, M. and Rashidi, M.},
file = {:C$\backslash$:/Users/p327208/Desktop/Promotion/Literature/Motorspezifisch/Heat Transfer Combustion Chamber/2008{\_}Mohammadi{\_}Analysis of local convective heat transfer in a spark ignition engine.pdf:pdf},
journal = {Int. Commun. Heat Mass Transf.},
keywords = {Combustion chamber,Heat flux,Heat transfer coefficient,SI engine},
number = {2},
pages = {215--224},
title = {{Analysis of local convective heat transfer in a spark ignition engine}},
volume = {35},
year = {2008}
}
@article{Gesamtprozessanalyse,
author = {Gesamtprozessanalyse, Als and Modellierung, Die},
pages = {385--414},
title = {{Gesamtprozessanalyse}}
}
@article{Peters1996,
author = {Peters, S T},
file = {:C$\backslash$:/Users/p327208/Desktop/B{\"{u}}cher/booksContinuumMechanics/{\_}buecherSong/HandbookofComposites/VI/IntroductionCompositeBasicsandRoadMap.pdf:pdf},
journal = {Handb. Compos.},
pages = {1--20},
title = {{Introduction , Composite Basics and Road Map}},
year = {1996}
}
@article{Negi2015,
author = {Negi, Anjna},
doi = {10.1016/j.pedn.2008},
isbn = {0514190450},
issn = {1095-9203},
number = {2},
pages = {464--467},
pmid = {12399572},
title = {{References 1.}},
volume = {6},
year = {2015}
}
@article{Verbesserung,
author = {Verbesserung, Durch},
journal = {Stand},
pages = {261--334},
title = {{11 Einfl{\{}{\"{u}}{\}}sse der Benzin-Direkteinspritzung auf weitere Motor-Einzelsysteme}}
}
@article{Arbeitsumgebung,
author = {Arbeitsumgebung, Die},
pages = {47--58},
title = {{4 Skizzieren 4.1}}
}
@article{Ziel,
author = {Ziel, Nutzfahrzeugs Das and Ii, Dingo and Testrig, Camel-view},
journal = {Auslegung A Grad. J. Philos.},
pages = {117--136},
title = {{6 Dom{\{}{\"{a}}{\}}nen{\{}{\"{u}}{\}}bergreifende Modellbildung eines aktiv gefederten Nutzfahrzeugs ( CAMel-View TestRig )}}
}
@article{Wallentowitz,
author = {Wallentowitz, Henning and Reif, Konrad},
doi = {10.1007/978-3-8348-8195-3},
isbn = {9783834802576},
title = {{Aus dem Programm}}
}

